Higher Order Targeted Maximum Likelihood Estimation

Asymptotic efficiency of targeted maximum likelihood estimators (TMLE) of target features of the data distribution relies on a a second order remainder being asymptotically negligible. In previous work we proposed a nonparametric MLE termed Highly Adaptive Lasso (HAL) which parametrizes the relevant functional of the data distribution in terms of a multivariate real valued cadlag function that is assumed to have finite variation norm. We showed that the HAL-MLE converges in Kullback-Leibler dissimilarity at a rate n-1/3 up till logn factors. Therefore, by using HAL as initial density estimator in the TMLE, the resulting HAL-TMLE is an asymptotically efficient estimator only assuming that the relevant nuisance functions of the data density are cadlag and have finite variation norm. However, in finite samples, the second order remainder can dominate the sampling distribution so that inference based on asymptotic normality would be anti-conservative. In this article we propose a new higher order TMLE, generalizing the regular first order TMLE. We prove that it satisfies an exact linear expansion, in terms of efficient influence functions of sequentially defined higher order fluctuations of the target parameter, with a remainder that is a k+1th order remainder. As a consequence, this k-th order TMLE allows statistical inference only relying on the k+1th order remainder being negligible. We also provide a rationale for the higher order TMLE that it will be superior to the first order TMLE by (iteratively) locally minimizing the exact finite sample remainder of the first order TMLE. The second order TMLE is demonstrated for nonparametric estimation of the integrated squared density and for the treatment specific mean outcome. We also provide an initial simulation study for the second order TMLE of the treatment specific mean confirming the theoretical analysis.

==> Untitled-3.tex <==
References needed: 

from hotmle: higherordertmle_shorter.tex:


\bibliographystyle{plain}
\bibliography{higherordertmle}
}


\citealp{bkrw1997}) and estimating equations methodology (e.g., \citealp{vanderlaan2003}). More recently, targeted maximum likelihood (or minimum loss-based) estimation, hereafter referred to as TMLE (e.g., \citealp{vanderlaan2006ijb,vanderlaan2011}),  \subsection{Brief review of the relevant literature}


The building blocks of this generalization were set several decades ago, notably in the works of J. Pfanzagl \citep{pfanzagl1985}, wherein the notion of higher-order gradients was introduced and higher-order expansions of finite-dimensional parameters over arbitrary model spaces were formalized. In this work, we seek to utilize higher-order expansions to enable and guide the construction of regular and asymptotically linear estimators of statistical parameters in rich infinite-dimensional models. This is the perspective that motivated the seminal contributions of J. Robins, L. Li, E. Tchetgen \& A. van der Vaart (e.g., \citealp{robins2008imsnotes,robins2009metrika,li2011statsprobletters,vandervaart2014statscience}); these authors are the first to have provided a rigorous framework for precisely addressing this problem. The first exposition is that of \cite{robins2008imsnotes}, where the focus resides primarily on the use of higher-order gradients to derive optimal estimators in settings where regular estimation is not possible. Subsequent works are concerned with the development of a higher-order analogue of the one-step estimator introduced early on in \cite{levit1975}, \cite{ibragimov1981}, \cite{pfanzagl1982} and \cite{bickel1982annals}, for example. The general approach is thus to identify the dominating terms of an asymptotic expansion for a naive plug-in estimator and to perform, accordingly, an additive correction on this naive estimator. In \cite{robins2009metrika}, the authors carefully establish the required foundations of a second-order extension of this approach and illustrate its use in the context of two problems, namely that of estimating the square of a density function and of estimating the mean response in missing data models. In \cite{li2011statsprobletters}, the authors study in great detail the problem of inferring a treatment effect using this approach and also establish minimax rate results for certain situations in which regular inference is not possible.

An excellent review of the general higher-order extension of the one-step  estimator is provided in \cite{vandervaart2014statscience}. The one-step  estimator is simple and easy to describe. However, in finite samples, it is vulnerable to decreased performance since it does not include any safeguard ensuring that the additive correction performed on the naive plug-in estimator does not drive the estimator near and possibly beyond the natural bounds of the parameter space. Rather than performing post-hoc bias correction in the parameter space, as does the one-step procedure, the TMLE framework, which we focus on in this paper, provides guidelines for constructing an estimator of the underlying data-generating distribution, or whichever portion of it is needed to compute the parameter of interest, such that the resulting plug-in estimator enjoys regular and asymptotically linear asymptotic behavior. As such, the correction step is  performed in the model space rather than in the parameter space. The appeal of devising such an approach, even decades before its actual development, was highlighted in \cite{pfanzagl1982}. Since the resulting estimator automatically satisfies bounds on the parameter space, it never produces nonsensical output, such as a probability estimate outside the unit interval, and can outperform in finite samples asymptotically equivalent estimators that do not have a plug-in form. This issue arises when comparing first-order TMLE and one-step  estimators, but is likely of even greater importance in higher-order inference due to the increased complexity of the correction process.

As is highlighted by \cite{robins2009metrika} and discussed in this article, higher-order gradients do not exist for several statistical parameters of interest. Nonetheless, approximate higher-order gradients can be used to produce regular estimators. In practice, the notion of approximate higher-order gradients necessarily involves the selection of certain tuning parameters. This requirement is discussed in \cite{robins2009metrika} but practical guidelines are neither provided nor appear particularly easy to develop. An advantage of using TMLE in this context, as we discuss later, is that the selection of such tuning parameters can be effortlessly embedded in the framework of collaborative TMLE, hereafter referred to as C-TMLE. Thus, the practical complications associated with the need for carefully-tuned approximations in the context of inference based on higher-order expansions can be tackled readily. Furthermore, as will be discussed, the framework of TMLE also provides useful tools that aim to guarantee that the resulting higher-order estimator will not behave worse than the usual first-order TMLE.

we propose a $2$-TMLE based on an approximate second-order gradient and present a corresponding theory. This additional approximation yields a supplementary bias term for the resulting $2$-TMLE, referred to as the \emph{representation error} in \cite{robins2009metrika}, a
\citep{vanderlaan2003techreport,vandervaart2006statdecisions,vanderlaan2007sagmb,polley2011chapter} for optimal performance, and a so-called least-favorable parametric submodel 

This generality of TMLE has been utilized in several instances before (e.g., \citealp{vanderlaan2006ijb,rubin2011tmlebook,vanderlaan2011,gruber2012ijb,lendle2013techreport,vanderlaan2014ijb})

The notion of second-order scores, tangent spaces and canonical gradients have been defined and studied before (see, e.g., \citealp{pfanzagl1985,robins2009metrika,vandervaart2014statscience}). 

As has been noted in \cite{robins2009metrika}, most statistical parameters of interest are unfortunately not smooth enough as functions of the data-generating distribution to allow the required expansion for $R_2(P_n^*,P_0)$. These secon


The choice of $h$ in this problem determines the least-favorable parametric submodel used in the TMLE algorithm. Thus, the selection of $h$ can be seen as completely analogous to the selection of an estimator of the treatment or censoring mechanism, principal determinants of the first-order least-favorable submodel, in the problem of estimating a counterfactual mean when all potential confounders have been recorded or when the available data are subject to censoring. C-TMLE, as described, thoroughly discussed and implemented in \cite{vanderlaan2010ijb}, \cite{gruber2010ijb}, \cite{stitelman2010ijb}, \cite{vanderlaan2011} and \cite{gruber2012ijb}, provides a principled solution to this problem. This approach can readily be utilized here as well.

-----
general effidiency directory:
tmleefficientshort.tex: 


There are two general methods for constructing an asymptotically efficient estimator. Firstly, the one-step estimator is defined by adding to an initial plug-in estimator of the target parameter an empirical mean of an estimator of the efficient influence curve at this same initial estimator \citep{Bick93}. In the special case that the efficient influence curve can be represented as an estimating function, one can represent this methodology as an estimating equation methodology, as has been developed for censored and causal inference models in the literature \citep{mark,Robins&Rotnitzky92}.
Secondly, the TMLE defines a least favorable parametric submodel through an initial estimator of the relevant parts (nuisance parameters) of the data distribution, and updates the initial estimator with the MLE over this least favorable parametric submodel. The one-step TMLE of the target parameter is now the resulting plug-in estimator \citep{vanderLaan&Rubin06,vanderLaan08, vanderLaan&Rose11}.


A complete literature review of higher order estimation theory is
presented in \cite{carone2014}. The most relevant references for the
problem studied here are \cite{robins2009quadratic} and
\cite{robins2009semiparametric}. In particular,
\cite{robins2009quadratic} 
Following \cite{gruber2011ctmle}, l

large library of candidate estimators \citep{vanderLaan&Dudoit03,vanderVaart&Dudoit&vanderLaan06,vanderLaan&Dudoit&vanderVaart06,vanderLaan&Polley&Hubbard07,Polleyetal12}. D


In this article we  will use a  one-step CV-TMLE in order to further minimize the conditions for asymptotic efficiency \citep{Zheng&vanderLaan12,vanderLaan&Rose11}. 


accompanying technical report \citep{vanderLaan15} we present the analogue results for the one-step TMLE.
By also including a large variety of other estimators in the library of the super-learner the TMLE will also have excellent practical performance for finite samples relative to competing estimators \citep{Polleyetal12}.


\citep{vanderVaart&Wellner11} we can establish  an upper bound for this  rate  of convergence in terms of the entropy of the mod

erges in one step, and we developed a so called universal least favorable submodel that guarantees this convergence in one step \citep{vanderLaan&Gruber15}. However, we want our theory to apply to general local least favorable submodels, which can be easier to implement than a universal least favorable model. In order to deal with this challenge, we obs

If $\pl f\pl_v<\infty$, then we can, in fact, represent $f$ as follows \citep{Gill&vanderLaan&Wellner95}:
\[
f(x)=f(0) +\sum_{s\subset \{1,\ldots,d\}}\int_{(0_s,x_s]}f(du_s,o_{-s}),
\]

By Corollary 2.6.12 in van der Vaart, Wellner (1996), we ha

The proof of this lemma is a simple corollary of the  finite sample oracle inequality for cross-validation \citep{vanderLaan&Dudoit03,vanderVaart&Dudoit&vanderLaan06,vanderLaan&Dudoit&vanderVaart06}, also presented in Lemma 
\bibliography{CCbib,TMLEivan,gencens2003,gencens2003logfluct,TMLE1_TLB,TMLE_TLB,gencens2003a,gencens2003b,gencens2003c,gencens2003d,gencens2003e,Grant}

to add, n-1/3
\citep{Bibaut&vanderLaan2019}.

==> combin.tex <==
@article{vanderLaan17,
	author = {M.J. van der Laan},
	journal = {International Journal of Biostatistics},
	pages = {1106--1118},
	title = {A Generally Efficient Targeted Minimum Loss Based Estimator},
	year = {2017},
}

@techreport{Bibaut&vanderLaan19,
  author =        {A. Bibaut and M.J. van der Laan},
    institution =   {Division of Biostatistics, University of California,
                   Berkeley},
   number={},
  title =         {Fast rates for empirical risk minimization over cadlag functions with bounded sectional variation norm},
  year =          {2019},
  Optnote={ https://arxiv.org/abs/1907.0924},
  }


%- When Adaptive Group Sequential RCT meets Machine Learning W. Zheng, Antoine Chambaz and Mark van der Laan - Effect Modification by Counterfactual Baseline Modifiers: a twist to a familiar storyW. Zheng, Zhehui Luo and Mark van der Laan
%Starmans, R.J.C.M. (2011). Models, Inference and Truth; Probabilistic Reasoning in the Information Era. In Mark.J. Van der Laan & Sherri Rose (Eds.), Targeted Learning; Causal Inference for Observational and Experimental Data (Springer Series in Statistics) (pp. 1-20). Springer.

@preamble{ " \newcommand{\noop}[1]{} " } %

%Benkeser D, van der Laan M (2016). The Highly Adaptive Lasso Estimator. Accepted: Proceedings of the IEEE Conference on Data Science and Advanced Analytics.

@book{vanderLaan&Rose17,
  author =        {M.J. van der Laan and S. Rose},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  title =         {Targeted Learning in Data Science: Causal Inference for Complex Longitudinal Studies},
  year =          {2017},
}

@incollection{Caroneetal17,
	Author = {M. Carone and I. Diaz and M.J. van der Laan},
	Booktitle = {{\rm M.J. van der Laan and S. Rose, } Targeted Learning in Data Science:Causal Inference for complex longitudinal studies},
	Chapter = {26},
	pages={Tbt},
	Publisher = {Springer, New York},
	Title = {Higher order targeted loss-based estimation},
	Year = {2017}}

@article{Benkeser&vanderLaan16,
 author =        {D. Benkeser and M.J. van der Laan},
  journal =       {Proceedings of the IEEE Conference on Data Science and Advanced Analytics},
  title =         {The highly adaptive lasso estimator},
  year =          {2016},
}

@article{Benkeseretal17,
 author =        {D. Benkeser and P. Gilbert and M. van der Laan and M. Carone},
  journal =       {Biometrika},
  title =         {Nonparametric double robust inference for a counterfactual mean},
 note={To appear},
  year =          {2017},
}




@article{Starmans13,
 author =        {R.J.C.M. Starmans},
  journal =       {Stator},
  number =         {24},
  title =         {Picasso, {H}egel and the Era of Big Data (in Dutch)},
  volume =        {2},
  year =          {2013},
}

@article{Starmans&vanderLaan13,
 author =        {R.J.C.M. Starmans and M.J. van der Laan},
  journal =       {Stator},
  number =         {24},
  title =         {Inferential Statistics versus Machine Learning; a Prelude to Reconciliation (in Dutch)},
  volume =        {2},
  year =          {2013},
}



@techreport{Roseetal12,
  author =        {S. Rose and R.J.C.M. Starmans and M.J. van der Laan},
    institution =   {Division of Biostatistics, University of California,
                   Berkeley},
   number={297},
  title =         {Targeted Learning for Causality and Statistical Analysis in Medical Research},
  year =          {2011},
  Optnote={http://biostats.bepress.com/ucbbiostat/paper297},
  }



@incollection{Starmans2012,
  author =        {R.J.C.M. Starmans},
  booktitle =     {Targeted Learning: Causal Inference for Observational and Experimental Studies},
  editor =        {M.J. van der Laan and S. Rose},
  publisher =     {Springer},
  title =         {Models, Inference and Truth: Probabilistic Reasoning in the Information Era},
  pages= {1--20},
  year =          {2011},
      address =       {New York},
}







@incollection{Caroneetal12,
  author =        {M. Carone and M. Petersen and M.J. van der Laan},
  booktitle =     {Interval Censored Time To Event Data: Methods and Applications},
  editor =        {Ding-Geng (Din) Chen, Jianguo Sun, Karl E. Peace (eds)},
  publisher =     {Chapman \& Hall/CRC},
  title =         {Targeted minimum loss based estimation of a casual effect using interval censored time to event data},
  year =          {2012},
      address =       {New York},
}


@article{vanderLaan&Petersen&Zheng13,
 author =        {W. Zheng and M.L. Petersen and M.J. van der Laan},
  journal =       {Journal of Causal Inference},
  number =         {Issue 1},
  pages={83--106},
  title =         {Estimating the Effect of a Community-Based Intervention with Two Communities},
  volume =        {1},
  year =          {2013},
}

@article{Zheng&vanderLaan12a,
 author =        {W. Zheng and M.J. van der Laan},
  journal =       {International Journal of Biostatistics},
  number =         {Issue 1},
  title =         {Targeted Maximum Likelihood Estimation of Natural Direct Effects},
  volume =        {8},
  year =          {2012},
}



@techreport{Zheng&vanderLaan12b,
  author =        {W. Zheng and M.J. van der Laan},
    institution =   {Division of Biostatistics, University of California,
                   Berkeley},
   number={295},
  title =         {Causal Mediation in a Survival Setting with Time-Dependent Mediators},
  year =          {2012},
}


@article{Cotton&Heagerty11,
 author =        {C. Cotton and P. Heagerty},
  journal =       {Stat. Biosc},
  pages =         {28--44},
  title =         {A data augmentation method for estimating the causal effect of adherence to
treatment regimens targeting control of an intermediate measure},
  volume =        {3},
  year =          {2011},
}

@incollection{vanderLaan&Petersen12,
  author =        {M.J. van der Laan and M.L. Petersen},
  booktitle =     {Ensemble Machine Learning: Methods and Applications},
  editor =        {C. Zhang and Y. Ma (eds)},
  publisher =     {Springer},
  title =         {Targeted Learning},
  year =          {2012},
      address =       {New York},
}

@incollection{Zheng&vanderLaan12,
  author =        {W. Zheng and M.J. van der Laan},
  booktitle =     {Targeted Learning: Causal Inference for Observational and Experimental Studies},
  editor =        {M.J. van der Laan and S. Rose},
  publisher =     {Springer},
  title =         {Cross-validated targeted minimum loss based estimation},
  year =          {2011},
      address =       {New York},
}


@techreport{Balzer&vanderLaan13,
  author =        {L.B. Balzer and M.J. van der Laan},
    institution =   {Division of Biostatistics, University of California,
                   Berkeley},
   number={310},
  title =         {Estimating Effects on Rare Outcomes: Knowledge is Power},
  year =          {2013},
}

@techreport{vanderLaan12,
  author =        {M.J. van der Laan},
    institution =   {Division of Biostatistics, University of California,
                   Berkeley, submitted to IJB},
   number={302},
  title =         {Statistical Inference when using Data Adaptive Estimators of Nuisance Parameters},
  year =          {2012},
}

@techreport{Diaz&vanderLaan13,
  author =        {I. Diaz and M.J. van der Laan},
    institution =   {Division of Biostatistics, University of California,
                   Berkeley, submitted to JCI},
   number={306},
  title =         {Targeted Data Adaptive Estimation of the Causal Dose Response Curve},
  year =          {2013},
}


@techreport{vanderLaan&Hubbard13,
  author =        {M.J. van der Laan and A.E. Hubbard and S. Kherad},
    institution =   {Division of Biostatistics, University of California,
                   Berkeley},
   number={314},
  title =         {Statistical Inference for Data Adaptive Target Parameters},
  year =          {2013},
}



@article{Rubin&vanderLaan07,
 author =        {D. Rubin and M.J. van der Laan},
  journal =       {The International Journal of Biostatistics},
  pages =         {http://www.bepress.com/ijb/vol3/iss1/4},
  title =         {A Doubly Robust Censoring Unbiased Trans- formation},
  volume =        {Vol. 3 (1)},
  year =          {2007},
}


@article{Chakrabortietal10,
 author =        {B. Chakraborty and S.A. Murphy and V. Strecher},
  journal =       {Stat. Methods Med. Res.},
  pages =         {317--43},
  title =         {Inference for non-regular parameters in optimal dynamic
treatment regimes},
  volume =        {19},
  year =          {2010},
}

@article{Chakraborti&Murphy13,
 author =        {B. Chakraborty and S.A. Murphy},
  journal =       {Annu. Rev. Stat. Appl.},
  pages =         {1--18},
  title =         {Dynamic treatment regimens},
  volume =        {1},
  year =          {2013},
}


@article{Rubin&vanderLaan12,
  author =        {D.B. Rubin and M.J. van der Laan},
  journal =       {International Journal of Biostatistics},
  pages =         {Issue 1, Article 18},
  title =         {Statistical issues and limitations in personalized medicine research with clinical trials},
  volume =        {8},
  year =          {2012},
}
@article{Wang&vanderLaan11,
  author =        {H. Wang and M.J. van der Laan},
  journal =       {BMC Bioinformatics},
  pages =         {312},
  title =         {Dimension reduction procedure using  targeted variable  importance measurement},
  volume =        {12},
  year =          {2011},
}

@article{Westeretal12,
  author =        {C.W. Wester and O.M. Stitelman and V. De Gruttola and H. Bussmann and R.G. Marlink  and  M.J. van  der  Laan},
  journal =       {AIDS Res Hum Retroviruses},
  pages =         {781--88},
  title =         {Effect modification by sex and  baseline  CD4(+) cell count  among  adults receiving combination antiretroviral therapy in Botswana: Results  from a clinical trial},
  volume =        {28},
  year =          {2012},
}

@book{Polley&vanderLaan12,
  address =       {Available at http://cran.r-project.org/web/packages/SuperLearner/SuperLearner.pdf.
},
  author =        {E. Polley and M.J. van der Laan},
  publisher =     {R package version 2.0-6},
  title =         {Super Learner Prediction},
  year =          {2012},
}

@book{Gruber&vanderLaan12,
  address =       {Available at http://cran.r-project.org/web/packages/tmle/tmle.pdf},
  author =        {S. Gruber and M.J. van der Laan},
  publisher =     {R package version 1.2.0-1},
  title =         {Targeted Maximum Likelihood Estimation},
  year =          {2012},
}

@book{Schwabb&vanderLaan&Petersen12,
  address =       {Available at http://cran.r-project.org/web/packages/ltmle/ltmle.pdf},
  author =        {J. Schwabb and M.J. van der Laan and M.L. Petersen},
  publisher =     { },
  title =         {Longitudinal Targeted Maximum Likelihood Estimation},
  year =          {2012},
}


@article{Banks&Jang&Kwon11,
  author =        {H. Banks and T. Jang and H. Kwon},
  journal =       {Int. J. Pure Appl. Math.},
  pages =         {461--485},
  title =         {Feedback control of HIV antiviral therapy with long measurement time},
  volume =        {66},
  year =          {2011},
}

@book{Bellman57,
  address =       {Princeton, NJ},
  author =        {R. Bellman},
  edition =       {},
  publisher =     {Univ. Press},
  title =         {Dynamic Programming},
  year =          {1957},
}

@article{Benneth&Hauser12,
  author =        {C. Bennett and K. Hauser},
  journal =       {Artif. Intell. Med.},
  pages =         {9--19},
  title =         {Artificial intelligence framework for simulating clinical decision-making: a
Markov decision process approach},
  volume =        {57},
  year =          {2012},
}

%Berger R, Boos D. 1994.Pvalues maximized over a confidence set for the nuisance parameter.J. Am. Stat.Assoc.89:1012Ð16Box G, Hunter W, Hunter J. 1978.Statistics for Experimenters: An Introduction to Design, Data Analysis, andModel Building.NewYork:Wiley

@article{Cai&Tian&Wong&Wei11,
  author =        {T. Cai and L. Tian and P. Wong and L. Wei},
  journal =       {Biostatistics},
  pages =         {270--282},
  title =         {Analysis of randomized comparative clinical trial data for personalized
treatment selections},
  volume =        {12},
  year =          {2011},
}

@article{Chakraborty&Murphy&Strecher10,
  author =        {B. Chakraborty and S. Murphy and V. Strecher},
  journal =       {Stat. Methods Med. Res},
  pages =         {317--343},
  title =         {Inference for non-regular parameters in optimal dynamic
treatment regimes},
  volume =        {19},
  year =          {2010},
}


@article{Dawson&Lavori10,
  author =        {R. Dawson and P. Lavori},
  journal =       {Clin. Trials},
  pages =         {643--652},
  title =         {Sample size calculations for evaluating treatment policies in multi-stage designs},
  volume =        {7},
  year =          {2010},
}

@article{Dawson&Lavori12,
  author =        {R. Dawson and P. Lavori},
  journal =       {Biostatistics},
  pages =         {142--152},
  title =         {Efficient design and inference for multistage randomized trials of individualized
treatment policies},
  volume =        {13},
  year =          {2012},
}

@article{Ernstetal05,
  author =        {D. Ernst and P. Geurts and L. Wehenkel},
  journal =       {J. Mach. Learn. Res.},
  pages =         {503--556},
  title =         {Tree-based batch mode reinforcement learning},
  volume =        {6},
  year =          {2005},
}

@article{Gawedaetal05,
  author =        {A. Gaweda and M. Muezzinoglu and G. Aronoff and A. Jacobs and J. Zurada and M. Brier},
  journal =       {Neural Netw.},
  pages =         {826--34},
  title =         {Individualization of pharmaco-
logical anemia management using reinforcement learning},
  volume =        {18},
  year =          {2005},
}

@article{Goldberg&Kosorok12,
  author =        {Y. Goldberg and M. Kosorok},
  journal =       {Ann. Stat.},
  pages =         {529-60},
  title =         {Q-learning with censored data},
  volume =        {40},
  year =          {2012},
}

@article{Hernanetal06,
  author =        {M.A. Hernan and E. Lanoy and D. Costagliola and J.M. Robins},
  journal =       {Basic Clin. Pharmacol. Toxicol},
  pages =         {237--242},
  title =         {Comparison of dynamic treatment regimes via
inverse probability weighting},
  volume =        {98},
  year =          {2006},
}



@article{Imai&Ratkovicz13,
  author =        {K. Imai and M. Ratkovicz},
  journal =       {Ann. Appl. Stat.},
  pages =         {443-70},
  title =         {Estimating treatment effect heterogeneity in randomized program evaluation},
  volume =        {7},
  year =          {2013},
}

@article{Jones10,
  author =        {H. Jones},
  journal =       {ClinicalTrials.gov data base, updated October 19, 2012},
  pages =         {accessed July 24, 2013},
  title =         {Reinforcement-based treatment for pregnant drug abusers},
  volume =        {Natl. Inst. Health., Bethesda, MD, http://
clinicaltrials.gov/ct2/show/NCT01177982},
  year =          {2010},
}

@article{Kasari09,
  author =        {C. Kasari},
  journal =       {ClinicalTrials.gov database, updated Apr. 26, 2012},
  pages =         {accessed July 24, 2013},
  title =         {Developmental and augmented intervention for facilitating expressive language},
  volume =        {Natl. Inst. Health., Bethesda, MD, http://
clinicaltrials.gov/ct2/show/NCT01013545},
  year =          {2009},
}

@article{Kulkarnietal11,
  author =        {K. Kulkarni and A. Gosavi and S. Murray and K. Grantham},
  journal =       {J. Control Theory Appl.},
  pages =         {421--30},
  title =         {Semi-Markov adaptive critic heuristics with application
to airline revenue management},
  volume =        {9},
  year =          {2011},
}

@article{Laber&Murphy11,
  author =        {E. Laber and S. Murphy},
  journal =       {J. Am. Stat. Assoc.},
  pages =         {904--13},
  title =         {Adaptive confidence intervals for the test error in classification},
  volume =        {106},
  year =          {2011},
}

@article{Lavori&Dawson00,
  author =        {P. Lavori and R. Dawson},
  journal =       {J. R. Stat. Soc. A.},
  pages =         {29--38},
  title =         {A design for testing clinical strategies: biased adaptive within-subject randomiza-
tion},
  volume =        {163},
  year =          {2000},
}
@article{Lavori&Dawson04,
  author =        {P. Lavori and R. Dawson},
  journal =       {Clin. Trials},
  pages =         {9--20},
  title =         {Dynamic treatment regimes: practical design considerations.},
  volume =        {1},
  year =          {2004},
}

@article{Lavori&Dawson08,
  author =        {P. Lavori and R. Dawson},
  journal =       {Annu. Rev. Med.},
  pages =         {443--453},
  title =         {Adaptive treatment strategies in chronic disease},
  volume =        {59},
  year =          {2008},
}

@article{Leeb&Potscher03,
  author =        {H.P. Leeb and B. Potscher},
  journal =       {Econom. Theory},
  pages =         {100-42},
  title =         {The finite-sample distribution of post-model-selection estimators and uniform
versus nonuniform approximations.},
  volume =        {19},
  year =          {2003},
}

@article{Leietal11,
  author =        {H. Lei and I. Nahum-Shani and K. Lynch and D. Oslin and S. Murphy},
  journal =       {Annu. Rev. Clin. Psychol.},
  pages =         {21--48},
  title =         {A ÒSMARTÓ design for building individualized
treatment sequences},
  volume =        {8},
  year =          {2011},
}

@article{Li&Murphy11,
  author =        {Z. Li and S. Murphy},
  journal =       {Biometrika},
  pages =         {503--18},
  title =         {Sample size formulae for two-stage randomized trials with survival outcomes},
  volume =        {98},
  year =          {2011},
}

@article{Lizotteetal10,
  author =        {D. Lizotte and M. Bowling and S. Murphy},
  journal =       {Twenty-Seventh International Conference on Machine Learning
(ICML)},
  pages =         {695--702},
  title =         {Efficient reinforcement learning with multiple reward functions
for randomized clinical trial analysis},
  volume =        {Haifa, Israel: Omnipress},
  year =          {2010},
}

@article{Lizotteetal12,
  author =        {D. Lizotte and M. Bowling and S. Murphy},
  journal =       {J. Mach.
Learn. Res.},
  pages =         {3253--95},
  title =         {Linear fitted-Q iteration with multiple reward functions},
  volume =        {13},
  year =          {2012},
}

@article{Luncefordetal02,
  author =        {J. Lunceford and M. Davidian and A. Tsiatis},
  journal =       {Biometrics},
  pages =         {48--57},
  title =         {Estimation of survival distributions of treatment policies in
two-stage randomization designs in clinical trials},
  volume =        {58},
  year =          {2002},
}

@article{Moodieetal12,
  author =        {E. Moodie and B. Chakraborty and M. Kramer.},
  journal =       {Can. J. Stat.},
  pages =         {629--45},
  title =         {Q-learning for estimating optimal dynamic treatment rules
from observational data},
  volume =        {40},
  year =          {2012},
}

@article{Moodieetal09,
  author =        {E. Moodie and R. Platt and M. Kramer},
  journal =       {J. Am. Stat. Assoc.},
  pages =         {155--65},
  title =         {Estimating response-maximized decision rules with applications to
breastfeeding},
  volume =        {104},
  year =          {2009},
}

@article{Murphy05a,
  author =        {S. Murphy},
  journal =       {J. Mach. Learn. Res.},
  pages =         {1073--97},
  title =         {A generalization error for Q-learning},
  volume =        {6},
  year =          {2005a},
}
@article{Murphy05b,
  author =        {S. Murphy},
  journal =       {Stat. Med.},
  pages =         {1455--81},
  title =         {An experimental design for the development of adaptive treatment strategies},
  volume =        {24},
  year =          {2005b},
}
@article{Murphy&Bingham09,
  author =        {S. Murphy and D. Bingham},
  journal =       {J. Am. Stat. Assoc.},
  pages =         {391--408},
  title =         {Screening experiments for developing dynamic treatment regimes},
  volume =        {24},
  year =          {2005b},
}

@article{Murphyetal01,
  author =        {S. Murphy and M.J. van der Laan and J.M. Robins},
  journal =       {J. Am. Stat. Assoc.},
  pages =         {1410--23},
  title =         {Marginal mean models for
dynamic regimes},
  volume =        {96},
  year =          {2001},
}

@article{Nahum-Shanietal12a,
  author =        {I. Nahum-Shani and M.  Qian and D. Almiral and W.  Pelham and B.  Gnagy B, et al. },
  journal =       {Psychol. Methods},
  pages =         {457--77},
  title =         {Experimental design and primary
data analysis methods for comparing adaptive interventions},
  volume =        {17},
  year =          {2012a},
}

@article{Nahum-Shanietal12b,
  author =        {I. Nahum-Shani and M.  Qian and D. Almiral and W.  Pelham and B.  Gnagy B, et al. },
  journal =       {Psychol. Methods},
  pages =         {478--94},
  title =         {Q-learning: a data analysis method
for constructing adaptive interventions},
  volume =        {17},
  year =          {2012b},
}
@article{Nahum-Shanietal12b,
  author =        {I. Nahum-Shani and M.  Qian and D. Almiral and W.  Pelham and B.  Gnagy B, et al. },
  journal =       {Psychol. Methods},
  pages =         {478--94},
  title =         {Q-learning: a data analysis method
for constructing adaptive interventions},
  volume =        {17},
  year =          {2012b},
}


@article{Navarro-Barrientoseta11,
  author =        {J. Navarro-Barrientos and D. Rivera and L. Collins},
  journal =       {Math. Comput. Model. Dyn. Syst.},
  pages =         {183--203},
  title =         {A dynamical model for describing behavioural interventions
for weight loss and body composition change},
  volume =        {17},
  year =          {2011},
}

@article{Oettingetal11,
  author =        {A. Oetting and J. Levy and R. Weiss and S. Murphy},
  journal =       {In
Causality and Psychopathology: Finding the Determinants of Disorders and
Their Cures},
  pages =         {179--205},
  title =         { Statistical methodology for a SMART design in the development
of adaptive treatment strategies},
  volume =        {ed. PE Shrout, KM Keyes, K Ornstein, New York: Oxford Univ. Press},
  year =          {2011},
}

@article{Orellanaetal10a,
  author =        {L. Orellana and A. Rotnitzky and J.M. Robins},
  journal =       {Int. J. Biostat.},
  pages =         {6:8},
  title =         {Dynamic regime marginal structural mean models for estimation
of optimal dynamic treatment regimes, part I: main content},
  volume =        { },
  year =          {2010a},
}
@article{Orellanaetal10b,
  author =        {L. Orellana and A. Rotnitzky and J.M. Robins},
  journal =       {Int. J. Biostat.},
  pages =         {6:9},
  title =         {Dynamic regime marginal structural mean models for estimation
of optimal dynamic treatment regimes, part I: proofs and additional results},
  volume =        {  },
  year =          {2010b},
}

@article{Ormoneit&Sen02,
  author =        {D. Ormoneit and S. Sen},
  journal =       {Mach. Learn.},
  pages =         {161--78},
  title =         {Kernel-based reinforcement learning},
  volume =        {49},
  year =          {2002},
}

@article{Qian&Murphy11,
  author =        {M. Qian and S. Murphy},
  journal =       {Ann. Stat.},
  pages =         {1180--210},
  title =         {Performance guarantees for individualized treatment rules},
  volume =        {39},
  year =          {2011},
}

@article{Riveraetal07,
  author =        {D. Rivera and M. Pew and L. Collins},
  journal =       {Drug Alcohol Depend.},
  pages =         {S31--40},
  title =         {Using engineering control principles to inform the design of adaptive
interventions: a conceptual introduction},
  volume =        {88},
  year =          {2007},
}

@article{Robins04,
  author =        {J.M. Robins},
  journal =       {Proc. Seattle Symp. Biostat.},
  pages =         {189--326},
  title =         {Optimal structural nested models for optimal sequential decisions},
  volume =        {2nd, ed. D Lin, P Heagerty, New York: Springer},
  year =          {2004},
}

@article{Robinsetal08,
  author =        {J.M. Robins and L. Orellana and A. Rotnitzky},
  journal =       {Stat. Med.},
  pages =         {4678--721},
  title =         {Estimation and extrapolation of optimal treatment and testing
strategies},
  volume =        {27},
  year =          {2008},
}

@article{Rosenbergeretal07,
  author =        {E. Rosenberger and M. Davidian and H. Banks},
  journal =       {Drug Alcohol Depend.},
  pages =         {S41--51},
  title =         {Using mathematical modeling and control to develop structured
treatment interruption strategies for HIV infection},
  volume =        {88},
  year =          {2007},
}

@article{Rosthojetal06,
  author =        {S. Rosth¿j and C. Fullwood and R. Henderson and S. Stewart},
  journal =       {Stat. Med.},
  pages =         {4197--215},
  title =         {Estimation of optimal dynamic anticoagulation
regimes from observational data: a regret-based approach},
  volume ={88},
  year =          {2006},
}

@article{Shortreed&Moodie12,
  author =        {S. Shortreed and E. Moodie},
  journal =       {J.R. Stat. Soc. C.},
  pages =         {577--99},
  title =         {Estimating the optimal dynamic antipsychotic treatment regime: evidence from
the sequential-multiple assignment randomized CATIE Schizophrenia Study},
  volume ={61},
  year =          {2012},
}

@book{Sutton&Barto98,
  address =       {Cambridge, MA},
  author =        {R. Sutton and H. Sung},
  edition =       {},
  publisher =     {MIT  Press},
  title =         {Reinforcement Learning: An Introduction},
  year =          {1998},
}

@article{Thalletal00,
  author =        {P. Thall and R. Millikan and H. Sung},
  journal =       {Stat. Med.},
  pages =         {1011--128},
  title =         {Evaluating multiple treatment courses in clinical trials},
  volume ={30},
  year =          {2000},
}

@article{Thalletal02,
  author =        {P. Thall  and H. Sung and E. Estey},
  journal =       {J. Am. Stat. Assoc.},
  pages =         {29--39},
  title =         {Selecting therapeutic strategies based on efficacy and death in multicourse
clinical trials},
  volume ={39},
  year =          {2002},
}

@article{Thall&Wathen05,
  author =        {P. Thall  and J. Wathen},
  journal =       {Stat. Med.},
  pages =         {1947--64},
  title =         {Covariate-adjusted adaptive randomization in a sarcoma trial with multi-stage
treatments},
  volume ={24},
  year =          {2005},
}

@article{Thalletal07,
  author =        {P. Thall and C. Logothetis and L.C. Pagliaro and S. Wen and M.A.  Brown et al.},
  journal =       {J. Natl. Cancer Inst.},
  pages =         {1613--22},
  title =         {Adaptive therapy for androgen-
independent prostate cancer: a randomized selection trial of four regimens},
  volume ={99},
  year =          {2007},
}

%van der Laan MJ, Petersen ML. 2007a. Causal effect models for realistic individualized treatment andintention to treat rules.Int. J. Biostat.3:3van der Laan MJ, Petersen ML. 2007b. Statistical learning of origin-specific statically optimal individualizedtreatment rules.Int. J. Biostat.3:6

@article{Wagneretal01,
  author =        {E. Wagner and B. Austin and C. Davis and M. Hindmarsh and J. Schaefer and A. Bonomi},
  journal =       {Health Aff.},
  pages =         {64--78},
  title =         {Improving chronic illness care:
translating evidence into action},
  volume ={20},
  year =          {2001},
}

@article{Wahed&Tsiatis04,
  author =        {A. Wahed and A. Tsiatis},
  journal =       {Biometrics},
  pages =         {124--33},
  title =         {Optimal estimator for the survival distribution and related quantities for treatment
policies in two-stage randomized designs in clinical trials},
  volume ={60},
  year =          {2004},
}

@article{Wahed&Tsiatis06,
  author =        {A. Wahed and A. Tsiatis},
  journal =       {Biometrika},
  pages =         {163--77},
  title =         {Semiparametric efficient estimation of survival distributions in two-stage
randomisation designs in clinical trials with censored data},
  volume ={93},
  year =          {2006},
}

@article{Wangetal12,
  author =        {L. Wang and A.  Rotnitzky and X.  Lin and R.  Millikan and P. Thall},
  journal =       {J. Am. Stat. Assoc.},
  pages =         {493--508},
  title =         {Evaluation of viable dynamic treatment regimes in
a sequentially randomized trial of advanced prostate cancer},
  volume ={107},
  year =          {2012},
}

@article{Zhangetal12a,
  author =        {B. Zhang and A. Tsiatis and M. Davidian and M. Zhang and E. Laber},
  journal =       {Stat},
  pages =         {103--14},
  title =         {Estimating optimal treatment regimes from a
classification perspective},
  volume ={1},
  year =          {2012a},
}

@article{Zhangetal12b,
  author =        {B. Zhang and A. Tsiatis and M. Davidian and M. Zhang and E. Laber},
  journal =       {Biometrics},
  pages =         {1010--18},
  title =         {A robust method for estimating optimal treatment regimes},
  volume ={68},
  year =          {2012b},
}
@article{Zhaoetal12,
  author =        {Y. Zhao and D. Zeng and A. Rush and M. Kosorok},
  journal =       {J. Am. Stat. Assoc.},
  pages =         {1106--18},
  title =         {Estimating individual treatment rules using outcome weighted
learning},
  volume ={107},
  year =          {2012},
}

@article{Zhaoetal11,
  author =        {Y. Zhao and D. Zeng and A. Rush and M. Kosorok},
  journal =       {Biometrics},
  pages =         {1422--33},
  title =         {Reinforcement learning strategies for clinical trials in
nonsmall cell lung cancer},
  volume ={67},
  year =          {2011},
}




@techreport{Diaz&vanderLaan2012,
  author =        {I. Diaz and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
number={303},
  title =         {Sensitivity Analysis for Causal Inference Under Unmeasured Confounding and Measurement Error Problems},
  year =          {2012},
  note ={Submitted to IJB, also technical report http://www.bepress.com/ucbbiostat/paper303}
}
@techreport{vanderLaan2012,
  author =        {M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
number={300},
  title =         {Causal Inference for Networks},
  year =          {2012},
  note ={Submitted to JCI, also technical report http://www.bepress.com/ucbbiostat/paper300}
}

@techreport{vanderLaan&Gruber11,
  author =        {M.J. van der Laan and S. Gruber},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
number={290},
  title =         {Targeted Minimum Loss Based Estimation of an Intervention Specific Mean Outcome},
  year =          {2011},
  note ={To appear in IJB, also technical report http://www.bepress.com/ucbbiostat/paper290}
}



@incollection{Marschak53,
  address =       {New York},
  author =        {J. Marschak},
  booktitle =     {Economic measurements for policy and prediction},
  editor =        {W.~C. Hood and T.~C. Koopmans},
  publisher =     {Wiley},
  title =         {Studies in econometric method},
  year =          {1953},
}

@article{Heckman00,
  author =        {J. Heckman},
  journal =       {Q J Econ},
  pages =         {45--97},
  title =         {Causal parameters and policy analysis in economics:
                   A twentieth century retrospective.},
  volume =        {115},
  year =          {2000},
}

@article{Gruber&vanderLaan10,
  author =        {S. Gruber and M.J. van der Laan},
  journal =       {International Journal of Biostatistics},
  pages =         {article 26, www.bepress.com/ijb/vol6/iss1/26},
  title =         {A Targeted Maximum Likelihood Estimator of a Causal Effect on a Bounded Continuous Outcome},
  volume =        {6},
  year =          {2010},
}




@article{Heckman10,
  author =        {J. Heckman},
  journal =       {J Econ Lit},
  pages =         {356--398},
  title =         {Building bridges between structural and program
                   evaluation approaches to evaluating policy.},
  volume =        {48},
  year =          {2010},
}

@article{Bang&Robins05,
author={H. Bang and J.M. Robins},
 journal =       {Biometrics},
  pages =         {962--972},
  title =         {Doubly robust estimation in missing data and causal inference models},
  volume =        {61},
  year =          {2005},
}



@book{Pearson11,
  address =       {London},
  author =        {K. Pearson},
  edition =       {3rd},
  publisher =     {Black},
  title =         {Grammar of science},
  year =          {1911},
}

@article{Rubin74,
  author =        {Donald B. Rubin},
  journal =       {J Educ Psychol},
  number =        {},
  pages =         {688--701},
  title =         {Estimating causal effects of treatments in randomized
                   and nonrandomized studies.},
  volume =        {66},
  year =          {1974},
}

@article{Neyman23,
  author =        {J. Neyman},
  journal =       {Stat Sci},
  number =        {},
  pages =         {465--480},
  title =         {Sur les applications de la theorie des probabilites
                   aux experiences agricoles: Essai des principes ({In
                   Polish}). {E}nglish translation by {D.M.} {D}abrowska and
                   {T.P.} {S}peed (1990)},
  volume =        {5},
  year =          {1923},
}

@book{Pearl09,
  address =       {New York},
  author =        {J. Pearl},
  edition =       {2nd},
  publisher =     {Cambridge},
  title =         {Causality: models, reasoning, and inference},
  year =          {2009},
}

@article{Pearl95,
  author =        {J. Pearl},
  journal =       {Biometrika},
  pages =         {669--710},
  title =         {Causal diagrams for empirical research.},
  volume =        {82},
  year =          {1995},
}

@article{Robins&Greenland92,
  author =        {J.M. Robins and S. Greenland},
  journal =       {Epidemiol},
  pages =         {143--155},
  title =         {Identifiability and exchangeability for direct and
                   indirect effects},
  volume =        {3},
  year =          {1992},
}

@inproceedings{Pearl01b,
  address =       {San Francisco},
  author =        {J. Pearl},
  booktitle =     {Uncertainty in artificial intelligence, Proceedings
                   of the 17th Conference},
  publisher =     {Morgan Kaufmann},
  title =         {Direct and indirect effects.},
  year =          {2001},
}

@article{Baron&Kenny86,
  author =        {R. Baron and D. Kenny},
  journal =       {J Personal Soc Psychol},
  pages =         {1173--1182},
  title =         {The moderator-mediator variable distinction in social
                   psychological research: conceptual, strategic, and
                   statistical considerations.},
  volume =        {51},
  year =          {1986},
}

@book{MacKinnon08,
  address =       {New York},
  author =        {D. {MacKinnon}},
  publisher =     {Erlbaum},
  title =         {Introduction to statistical mediation analysis},
  year =          {2008},
}

@article{MacKinnonetal07,
  author =        {D. {MacKinnon} and C. Lockwood and C. Brown and
                   W. Wang and J. Hoffman},
  journal =       {Clin Trials},
  pages =         {499--513},
  title =         {The intermediate endpoint effect in logistic and
                   probit regression.},
  volume =        {4},
  year =          {2007},
}

@incollection{Pearl10c,
  address =       {},
  author =        {J. Pearl},
  booktitle =     {Statistical causality},
  editor =        {C. Berzuini and P. Dawid and L. Bernardinelli},
  publisher =     {},
  title =         {The mediation formula: a guide to the assessment of
                   causal pathways in nonlinear models.},
  year =          {forthcoming 2011},
}

@article{Pearl10b,
  author =        {J. Pearl},
  journal =       {Int J Biostat},
  pages =         {Article 7},
  title =         {An introduction to causal inference},
  volume =        {6},
  number={2},
  year =          {2010},
}

@article{vanderLaan&Rose10,
  author =        {M.J. van der Laan and S. Rose},
  journal =       {Amstat News},
  pages =         {38--39},
  title =         {Statistics Ready for a Revolution: next Generation of
                   Statisticians Must Build Tools for Massive Data Sets},
  volume =        {399},
  year =          {2010},
}

@techreport{vanderLaan&Dudoit03,
  author =        {M.J. van der Laan and S. Dudoit},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
number={130},
  title =         {Unified cross-validation methodology for selection
                   among estimators and a general cross-validated
                   adaptive epsilon-net estimator: finite sample oracle
                   inequalities and examples},
  year =          {2003},
}




@book{vanderLaan&Robins03,
  author =        {M.J. van der Laan and J.M. Robins},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  title =         {Unified methods for censored longitudinal data and
                   causality},
  year =          {2003},
}

@book{vanderLaan&Rose11,
  author =        {M.J. van der Laan and S. Rose},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  title =         {Targeted Learning: Causal Inference for Observational and Experimental Data},
  year =          {2011},
}

@book{Bickeletal97,
  author =        {P.J. Bickel and C.A.J. Klaassen and Y. Ritov and
                   J. Wellner},
  publisher =     {Springer},
  address={Berlin Heidelberg New York},
  title =         {Efficient and adaptive estimation for semiparametric
                   models},
  year =          {1997},
}

@article{vanderLaan&Rubin06,
  author =        {M.J. van der Laan and Daniel B. Rubin},
  journal =       {Int J Biostat},
  number =        {1},
  pages =         {Article 11},
  title =         {Targeted Maximum Likelihood Learning},
  volume =        {2},
  year =          {2006},
}

@article{Stitelman&vanderLaan11a,
  author =        {O.M. Stitelman and M.J. van der Laan},
  journal =       {Int J Biostat},
  number =        {1},
  title =         {Targeted Maximum Likelihood Estimation of Effect Modification Parameters In Survival Analysis},
  volume =        {7},
  year =          {2011},
}






@article{vanderLaan&Gruber10,
  author =        {M.J. van der Laan and S. Gruber},
  journal =       {Int J Biostat},
  number =        {1},
  title =         {Collaborative Double robust penalized targeted
                   maximum likelihood estimation},
  volume =        {6},
  year =          {2010},
}

@article{Taubes07,
  author =        {G. Taubes},
  journal =       {The New York Times},
  title =         {{Do we really know what makes us healthy?}},
  year =          {2007},
}

@article{USPrev09,
  author =        {{U.S. Preventive Services Task Force}},
  journal =       {Ann Intern Med},
  number =        {10},
  pages =         {716--726},
  title =         {{Screening for breast cancer: U.S. Preventive
                   Services Task Force recommendation statement}},
  volume =        {151},
  year =          {2009},
}

@article{Freedman&Petitti&Robins04,
  author =        {D.A. Freedman and D.B. Petitti and J.M. Robins},
  journal =       {Int J Epidemiol},
  pages =         {43--55},
  title =         {{On the efficacy of screening for breast cancer}},
  volume =        {33},
  year =          {2004},
}

@book{Rothman&Greenland98,
  address =       {Philadelphia},
  author =        {K.J. Rothman and S. Greenland},
  edition =       {2nd},
  publisher =     {Lippincott, Williams \& Wilkins},
  title =         {Modern epidemiology},
  year =          {1998},
}

@book{Jewell04,
  address =       {Boca Raton},
  author =        {N.P. Jewell},
  publisher =     {Chapman \& Hall},
  title =         {Statistics for epidemiology},
  year =          {2004},
}

@book{Freedman05,
  address =       {New York},
  author =        {D.A. Freedman},
  publisher =     {Cambridge},
  title =         {Statistical models: theory and practice},
  year =          {2005},
}

@article{Ioannidis06,
  author =        {J.P.A. Ioannidis},
  journal =       {Neonatal Intensive Care J Perinatol Neonatol},
  number =        {3},
  title =         {{Why most published research findings are false}},
  volume =        {19},
  year =          {2006},
}

@book{Freedman10,
  address =       {New York},
  author =        {D.H. Freedman},
  publisher =     {Little, Brown and Company},
  title =         {Wrong: why experts keep failing us---and how to know
                   when not to trust them},
  year =          {2010},
}

@book{Box&Draper87,
  address =       {Hoboken},
  author =        {G.E.P. Box and N.R. Draper},
  publisher =     {Wiley},
  title =         {Empirical model-building and response surfaces},
  year =          {1987},
}

@article{Robins86,
  author =        {J.M. Robins},
  journal =       {Math Mod},
  number =        {},
  pages =         {1393--1512},
  title =         {A new approach to causal inference in mortality
                   studies with sustained exposure periods--application
                   to control of the healthy worker survivor effect},
  volume =        {7},
  year =          {1986},
}

@article{Tager&Hollenberg&Satariano98,
  author =        {I. Tager and M. Hollenberg and W. Satariano},
  journal =       {Am J Epidemiol},
  pages =         {921--931},
  title =         {{Self-reported leisure-time physical activity and
                   measures of cardiorespiratory fitness in an elderly
                   population}},
  volume =        {147},
  year =          {1998},
}

@manual{RCore,
  address =       {Vienna},
  author =        {{R Development Core Team}},
  organization =  {R Foundation for Statistical Computing},
  title =         {R: a language and environment for statistical
                   computing},
  year =          {2010},
  url =           {http://www.R-project.org},
}

@article{liaw:2002,
  author =        {A. Liaw and M. Wiener},
  journal =       {R News},
  number =        {3},
  pages =         {18--22},
  title =         {Classification and Regression by randomForest},
  volume =        {2},
  year =          {2002},
  url =           {http://CRAN.R-project.org/package=randomForest},
}

@article{randomForests,
  author =        {L. Breiman},
  journal =       {Mach Learn},
  pages =         {5--32},
  title =         {Random Forests},
  volume =        {45},
  year =          {2001},
}

@manual{ipred,
  author =        {A. Peters and T. Hothorn},
  note =          {R package version 0.8-8},
  title =         {ipred: Improved Predictors},
  year =          {2009},
  url =           {http://CRAN.R-project.org/package=ipred},
}

@article{breiman96bagging,
  author =        {L. Breiman},
  journal =       {Mach Learn},
  number =        {2},
  pages =         {123--140},
  title =         {Bagging Predictors},
  volume =        {24},
  year =          {1996},
}

@incollection{gam:1992,
  author =        {T.J. Hastie},
  booktitle =     {Statistical models in {S}},
  editor =        {J.M. Chambers and T.J. Hastie},
  publisher =     {Chapman \& Hall},
  title =         {Generalized additive models},
      address =       {Boca Raton},
  year =          {1992},
}

@book{gams,
  author =        {T.J. Hastie and R.J. Tibshirani},
  publisher =     {Chapman \& Hall},
  title =         {Generalized additive models},
  year =          {1990},
    address =       {Boca Raton},
}

@manual{gbm,
  author =        {G. Ridgeway},
  note =          {R package version 1.6-3},
  title =         {gbm: generalized boosted regression models},
  year =          {2007},
}

@article{friedman:2001,
  author =        {J.H. Friedman},
  journal =       {Ann Stat},
  pages =         {1189-1232},
  title =         {Greedy Function Approximation: a Gradient Boosting
                   Machine},
  volume =        {29},
  year =          {2001},
}

@book{MASS,
  address={Berlin Heidelberg New York},
  author =        {W.N. Venables and B.D. Ripley},
  edition =       {4th},
  publisher =     {Springer},
  title =         {Modern applied statistics with S},
  year =          {2002},
}

@manual{polspline,
  author =        {C. Kooperberg},
  note =          {R package version 1.1.4},
  title =         {polspline: Polynomial spline routines},
  year =          {2009},
  url =           {http://CRAN.R-project.org/package=polspline},
}

@article{MARS,
  author =        {J.H. Friedman},
  journal =       {Ann Stat},
  number =        {1},
  pages =         {1--141},
  title =         {Multivariate Adaptive Regression Splines},
  volume =        {19},
  year =          {1991},
}

@manual{bart,
  author =        {H.A. Chipman and R.E. McCulloch},
  note =          {R package version 0.3-1},
  title =         {BayesTree: {B}ayesian methods for tree-based models},
  year =          {2009},
  url =           {http://CRAN.R-project.org/package=BayesTree},
}

@article{chipman:2009,
  author =        {H.A. Chipman and E.I. George and R.E. McCulloch},
  journal =       {Ann Appl Stat},
  title =         {{BART}: {B}ayesian Additive Regression Trees},
  volume =        {4},
  number={1},
  pages={266--298},
  year =          {2010},
}

@incollection{loess,
  author =        {W.S. Cleveland and E. Groose and W.M. Shyu},
  booktitle =     {Statistical models in {S}},
  editor =        {J.M. Chambers and T.J. Hastie},
  publisher =     {Chapman \& Hall},
  title =         {Local Regression Models},
  year =          {1992},
      address =       {Boca Raton},
}

@techreport{Polley&vanderLaan10,
  author =        {E.C. Polley and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =        {266},
  title =         {Super Learner in Prediction},
  year =          {2010},
}

@book{cook:1994,
  address =       {New York},
  author =        {D. Cook and S. Weisberg},
  publisher =     {Wiley},
  title =         {An introduction to regression graphics},
  year =          {1994},
}

@article{chu:2001,
  author =        {S. Chu},
  journal =       {J Stat Educ},
  number =        {2},
  title =         {Pricing the {C}'s of diamond stones},
  volume =        {9},
  year =          {2001},
}

@book{berndt:1991,
  address =       {New York},
  author =        {E.R. Berndt},
  publisher =     {Addison--Wesley},
  title =         {The practice of econometrics},
  year =          {1991},
}

@article{kibler:1989,
  author =        {D. Kibler and D.W. Aha and M.K. Albert},
  journal =       {Comput Intell},
  pages =         {51},
  title =         {Instance-Based Prediction of Real-Valued Attributes},
  volume =        {5},
  year =          {1989},
}

@book{rosner:1999,
  address =       {Pacific Grove},
  author =        {B. Rosner},
  edition =       {5th},
  publisher =     {Duxbury},
  title =         {Fundamentals of biostatistics},
  year =          {1999},
}

@misc{newman:1998,
  author =        {D.J. Newman and S. Hettich and C.L. Blake and
                   C.J. Merz},
  institution =   {Department of
                   Information and Computer Sciences, University of California, Irvine},
  title =         {{UCI Repository of Machine Learning Databases}},
  year =          {1998},
}

@book{afifi:1979,
  address =       {New York},
  author =        {A. Afifi and S. Azen},
  edition =       {2nd},
  publisher =     {Academic},
  title =         {Statistical analysis: a computer oriented approach},
  year =          {1979},
}

@book{cook:1998,
  address =       {New York},
  author =        {D. Cook},
  publisher =     {Wiley},
  title =         {Regression graphics: ideas for studying regression
                   through graphics},
  year =          {1998},
}

@article{liu:1999,
  author =        {Z. Liu and T. Stengos},
  journal =       {J of Appl Econom},
  pages =         {527--538},
  title =         {Nonlinearities in Cross Country Growth Regressions:
                   a Semiparametric Approach},
  volume =        {14},
  year =          {1999},
}

@article{penrose:1985,
  author =        {K. Penrose and A. Nelson and A. Fisher},
  journal =       {Med Sci Sport Exer},
  pages =         {189},
  title =         {Generalized Body Composition Prediction Equation for
                   Men Using Simple Measurement Techniques},
  volume =        {17},
  year =          {1985},
}

@book{harrell:2001,
  address={Berlin Heidelberg New York},
  author =        {Harrell, Jr., F.E.},
  publisher =     {Springer},
  title =         {Regression modeling strategies with applications to
                   linear models, logistic regression, and survival
                   analysis},
  year =          {2001},
}

@manual{arm,
  author =        {A. Gelman and Y.-S. Su and M. Yajima and J. Hill and
                   M.G. Pittau and J. Kerman and T. Zheng},
  note =          {R package version 1.3-02},
  title =         {arm: data analysis using regression and
                   multilevel/hierarchical models},
  year =          {2010},
  url =           {http://CRAN.R-project.org/package=arm},
}

@article{gelman:2009,
  author =        {A. Gelman and A. Jakulin and M.G. Pittau and
                   Y.-S. Su},
  journal =       {Ann Appl Stat},
  number =        {3},
  pages =         {1360--1383},
  title =         {A Weakly Informative Default Prior Distribution for
                   Logistic and Other Regression Models},
  volume =        {2},
  year =          {2009},
}

@article{friedman:2010,
  author =        {J.H. Friedman and T.J. Hastie and R.J. Tibshirani},
  journal =       {J Stat Softw},
  number =        {1},
  title =         {Regularization Paths for Generalized Linear Models
                   via Coordinate Descent},
  volume =        {33},
  year =          {2010},
}

@manual{glmnet,
  author =        {J.H. Friedman and T.J. Hastie and R.J. Tibshirani},
  note =          {R package version 1.1-5},
  title =         {glmnet: lasso and elastic-net regularized generalized
                   linear models},
  year =          {2010},
  url =           {http://CRAN.R-project.org/package=glmnet},
}

@manual{DSA,
  author =        {R. Neugebauer and J. Bullard},
  note =          {R package version 3.1.3},
  title =         {DSA: Data-adaptive estimation with cross-validation
                   and the D/S/A algorithm},
  year =          {2009},
  url =           {http://www.stat.berkeley.edu/~laan/Software/},
}

@article{SinisivanderLaan04,
  author =        {S.E. Sinisi and M.J. van der Laan},
  journal =       {Stat Appl Genet Mol},
  note =          {Article 18},
  number =        {1},
  title =         {{D}eletion/{S}ubstitution/{A}ddition algorithm in
                   learning with applications in genomics},
  volume =        {3},
  year =          {2004},
}

@manual{svm,
  author =        {E. Dimitriadou and K. Hornik and F. Leisch and
                   D. Meyer and A. Weingessel},
  note =          {R package version 1.5-22},
  title =         {e1071: misc functions of the Department of Statistics
                   (e1071)},
  year =          {2009},
  url =           {http://CRAN.R-project.org/package=e1071},
}

@manual{Chang:2001,
  author =        {C.-C. Chang and C.-J. Lin},
  url =           {http://www.csie.ntu.edu.tw/~cjlin/libsvm},
  title =         {{LIBSVM}: a library for support vector machines},
  year =          {2001},
}

@article{vantveer:2002,
  author =        {L.J. {van't Veer} and H. Dal and M.J. {van de Vijver} and
                   Y.D. He and A.A.M. Hart and M. Mao and H.L. Peterse and
                   K. van der Kooy and M.J. Marton and A.T. Witteveen and
                   G.J. Schreiber and R.M. Kerkhoven and C. Roberts and
                   P.S. Linsley and R. Bernards and S.H. Friend},
  journal =       {Nature},
  pages =         {530--536},
  title =         {Gene Expression Profiling Predicts Clinical Outcome
                   of Breast Cancer},
  volume =        {415},
  year =          {2002},
}

@article{vanderLaan&Polley&Hubbard07,
  author =        {M.J. van der Laan and E.C. Polley and A.E. Hubbard},
  journal =       {Stat Appl Genet Mol},
  pages =        {Article 25},
  title =         {Super Learner},
  volume =        {6},
  year =          {2007},
  number =          {1},
}

@article{Wolpert92,
  author =        {D. H. Wolpert},
  journal =       {Neural Networks},
  pages =         {241--259},
  title =         {Stacked Generalization},
  volume =        {5},
  year =          {1992},
}

@article{Breiman96d,
  author =        {L. Breiman},
  journal =       {Mach Learn},
  pages =         {49--64},
  title =         {Stacked Regressions},
  volume =        {24},
  year =          {1996},
}

@article{Leblanc96,
  author =        {M. LeBlanc and R.J. Tibshirani},
  journal =       {J Am Stat Assoc},
  pages =         {1641--1650},
  title =         {Combining estimates in regression and classification},
  volume =        {91},
  year =          {1996},
}

@article{Stone74,
  author =        {M. Stone},
  journal =       {J R Stat Soc Ser B},
  number =        {2},
  pages =         {111--147},
  title =         {Cross-validatory choice and assessment of statistical
                   predictions},
  volume =        {36},
  year =          {1974},
}

@article{Geisser75,
  author =        {S. Geisser},
  journal =       {J Am Stat Assoc},
  number =        {350},
  pages =         {320--328},
  title =         {The Predictive Sample Reuse Method with Applications},
  volume =        {70},
  year =          {1975},
}

@inproceedings{Tsybakov03,
  author =        {A.B. Tsybakov},
  booktitle =     {COLT},
  editor =        {B. Sch{\"o}lkopf and M.K. Warmuth},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  series =        {Lecture Notes in Computer Science},
  title =         {Optimal rates of aggregation},
  volume =        {2777},
  year =          {2003},
}

@inproceedings{Juditskyetal05,
  author =        {A. Juditsky and A.V. Nazin and A.B. Tsybakov and
                   N. Vayatis},
  booktitle =     {NIPS},
  title =         {Generalization Error Bounds for Aggregation by Mirror
                   Descent with Averaging},
  year =          {2005},
}

@inproceedings{Buneaetal06,
  author =        {F. Bunea and A.B. Tsybakov and M.H. Wegkamp},
  booktitle =     {COLT},
  editor =        {G. Lugosi and H.-U. Simon},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  series =        {Lecture Notes in Computer Science},
  title =         {Aggregation and sparsity via {L}1 penalized least
                   squares},
  volume =        {4005},
  year =          {2006},
}

@article{Buneaetal07,
  author =        {F. Bunea and A.B. Tsybakov and M.H. Wegkamp},
  journal =       {Ann Stat},
  number =        {4},
  pages =         {1674--1697},
  title =         {Aggregation for Gaussian Regression},
  volume =        {35},
  year =          {2007},
}

@inproceedings{Buneaetal07b,
  author =        {F. Bunea and A.B. Tsybakov and M.H. Wegkamp},
  booktitle =     {COLT},
  editor =        {N.H. Bshouty and C. Gentile},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  series =        {Lecture Notes in Computer Science},
  title =         {Sparse density estimation with {L}1 penalties},
  volume =        {4539},
  year =          {2007},
}

@inproceedings{Dalalyan&Tsybakov07,
  author =        {A.S. Dalalyan and A.B. Tsybakov},
  booktitle =     {COLT},
  editor =        {N.H. Bshouty and C. Gentile},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  series =        {Lecture Notes in Computer Science},
  title =         {Aggregation by exponential weighting and sharp oracle
                   inequalities},
  volume =        {4539},
  year =          {2007},
}

@article{Dalalyan&Tsybakov08,
  author =        {A.S. Dalalyan and A.B. Tsybakov},
  journal =       {Mach Learn},
  number =        {1--2},
  pages =         {39--61},
  title =         {Aggregation by exponential weighting, sharp
                   PAC-{B}ayesian bounds and sparsity},
  volume =        {72},
  year =          {2008},
}

@book{Lehmann86,
  author =        {E.L. Lehmann},
  edition =       {2nd},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  title =         {Testing statistical hypotheses},
  year =          {1986},
}

@book{Hastie&Tibshirani&Friedman01,
  author =        {T.J. Hastie and R.J. Tibshirani and J.H. Friedman},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  title =         {The elements of statistical learning: data mining,
                   inference, and prediction},
  year =          {2001},
}

@ inproceedings{Ruczinski&Kooperberg&LeBlanc02,
  author =        {I. Ruczinski and C. Kooperberg and M. LeBlanc},
  booktitle =       {Proceedings of the MSRI workshop on Nonlinear
                   Estimation and Classification},
  editor={D. Denison and M.
                   Hansen and C. Holmes and B. Mallick and B. Yu},
  pages =         {333--344},
  title =         {Logic Regression -- methods and software},
  year =          {2002},
}



@techreport{Birkner&Hubbard&vanderLaan05,
  author =        {M.D. Birkner and A.E. Hubbard and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =        {197},
  title =         {Data Adaptive Pathway Testing},
  year =          {2005},
}

@techreport{Chaffee&Hubbard&vanderLaan10,
  author =        {P. Chaffee and A.E. Hubbard and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =        {263},
  title =         {Permutation-based Pathway Testing using the Super
                   Learner Algorithm},
  year =          {2010},
}

@inproceedings{Polley&vanderLaan09,
  author =        {E.C. Polley and M.J. van der Laan},
  booktitle =     {Design, summarization, analysis \& interpretation
                   of clinical trials with time-to-event endpoints},
  editor =        {K.E. Peace},
  publisher =     {Chapman \& Hall},
  title =         {Predicting Optimal Treatment Assignment Based on
                   Prognostic Factors in Cancer Patients},
address =       {Boca Raton},
  year =          {2009},
}

@article{vanderLaan&Dudoit&vanderVaart06,
  author =        {M.J. van der Laan and S. Dudoit and
                   A.W. van der Vaart},
  journal =       {Stat Decis},
  number =        {3},
  pages =         {373--395},
  title =         {The Cross-Validated Adaptive Epsilon-Net Estimator},
  volume =        {24},
  year =          {2006},
}

@article{vanderVaart&Dudoit&vanderLaan06,
  author =        {A.W. van der Vaart and S. Dudoit and
                   M.J. van der Laan},
  journal =       {Stat Decis},
  number =        {3},
  pages =         {351--371},
  title =         {Oracle Inequalities for Multi-Fold Cross-Validation},
  volume =        {24},
  year =          {2006},
}

@article{vanderLaan&Dudoit&Keles04,
  author =        {M.J. van der Laan and S. Dudoit and S. Kele\c{s}},
  journal =       {Stat Appl Genet Mol},
  pages =         {Article 4},
  title =         {Asymptotic optimality of likelihood-based
                   cross-validation},
  volume =        {3},
  number={1},
  year =          {2004},
}

@article{Dudoit&vanderLaan05,
  author =        {S. Dudoit and M.J. van der Laan},
  journal =       {Stat Methodol},
  number =        {2},
  pages =         {131--154},
  title =         {Asymptotics of cross-validated risk estimation in
                   estimator selection and performance assessment},
  volume =        {2},
  year =          {2005},
}

@techreport{Keles&vanderLaan&Dudoit02,
  author =        {Kele\c{s}, S. and van der Laan, M.J. and Dudoit, S.},
  institution =       {Division of Biostatistics, University of California,
                   Berkeley},
number={124},
  title =         {Asymptotically Optimal Model Selection Method for
                   Regression on Censored Outcomes},
  year =          {2002},
}

@book{Gyorfietal02,
  address={Berlin Heidelberg New York},
  author =        {L. Gy\"{o}rfi and M. Kohler and A. Krzy\.{z}ak and
                   H. Walk},
  pages =         {100--102},
  publisher =     {Springer},
  title =         {A distribution-free theory of nonparametric
                   regression},
  year =          {2002},
}

@article{Stone77,
  author =        {M. Stone},
  journal =       {Biometrika},
  number =        {1},
  pages =         {29--35},
  title =         {Asymptotics for and against cross-validation},
  volume =        {64},
  year =          {1977},
}

@book{Breimanetal84,
  author =        {L. Breiman and J.H. Friedman and R. Olshen and
                   C.J. Stone},
  publisher =     {Chapman \& Hall},
  title =         {Classification and regression trees},
  year =          {1984},
    address =       {Boca Raton},
}

@article{Breiman&Spector92,
  author =        {L. Breiman and P. Spector},
  journal =       {Int Stat Rev},
  pages =         {291--319},
  title =         {Submodel Selection and Evaluation in Regression. {T}he
                   {$X$} Random Case},
  volume =        {60},
  year =          {1992},
}

@book{Efron&Tibshirani93,
  author =        {B. Efron and R. J. Tibshirani},
  publisher =     {Chapman \& Hall},
  title =         {An Introduction to the bootstrap},
  year =          {1993},
      address =       {Boca Raton},
}

@article{Breiman96,
  author =        {L. Breiman},
  journal =       {Ann Stat},
  number =        {6},
  pages =         {2350--2383},
  title =         {Heuristics of instability and stabilization in model
                   selection},
  volume =        {24},
  year =          {1996},
}

@techreport{Breiman96c,
  author =        {L. Breiman},
  institution =   {Department of Statistics, University of California, Berkeley},
  type={Technical {R}eport},
  title =         {Out-of-bag estimation},
  year =          {1996},
}

@book{Ripley96,
  address =       {New York},
  author =        {B.D. Ripley},
  publisher =     {Cambridge},
  title =         {Pattern recognition and neural networks},
  year =          {1996},
}

@article{Breiman98,
  author =        {L. Breiman},
  journal =       {Ann Stat},
  pages =         {801--824},
  title =         {Arcing classifiers},
  volume =        {26},
  year =          {1998},
}

@article{Ambroise&McLachlan02,
  author =        {C. Ambroise and G.J. McLachlan},
  journal =       {Proc Natl Acad Sci},
  number =        {10},
  pages =         {6562--6566},
  title =         {Selection bias in gene extraction on the basis of
                   microarray gene-expression data},
  volume =        {99},
  year =          {2002},
}

@article{Pavlic&vanderLaan03,
  author =        {M. Pavlic and M.J. van der Laan},
  journal =       {Comput Stat Data An},
  pages =         {413--428},
  title =         {Fitting of mixtures with unspecified number of
                   components using cross validation distance estimate},
  volume =        {41},
  year =          {2003},
}

@inproceedings{Akaike73,
  author =        {H. Akaike},
  booktitle =     {Second International Symposium on Information Theory},
  editor =        {B.N. Petrov and F. Csaki},
  organization =  {Academiai Kiado},
  address={Budapest},
  title =         {Information theory and an extension of the maximum
                   likelihood principle},
  year =          {1973},
}

@article{Bozdogan00,
  author =        {H. Bozdogan},
  journal =       {J Math Psychol},
  pages =         {62--91},
  title =         {Akaike's information criterion and recent
                   developments in information complexity},
  volume =        {44},
  year =          {2000},
}

@article{Schwartz78,
  author =        {G. Schwartz},
  journal =       {Ann Stat},
  pages =         {461--464},
  title =         {Estimating the Dimension of a Model},
  volume =        {6},
  year =          {1978},
}

@article{Rissanen78,
  author =        {J. Rissanen},
  journal =       {Automatica},
  pages =         {465--471},
  title =         {Modelling by shortest data description},
  volume =        {14},
  year =          {1978},
}

@incollection{Bozdogan93,
  author =        {H. Bozdogan},
    address={Berlin Heidelberg New York},
  booktitle =     {Information and classification},
  editor =        {O. Opitz and B. Lausen and R. Klar},
  publisher =     {Springer},
  title =         {Choosing the number of component clusters in the
                   mixture model using a new informational complexity
                   criterion of the inverse Fisher information matrix},
  year =          {1993},
}

@article{Snowden&Rose&Mortimer11,
  author =        {J.M. Snowden and S. Rose and K.M. Mortimer},
  journal =       {Am J Epidemiol},
  number =        {00},
  pages =         {000--000},
  title =         {Implementation of G-Computation on a Simulated
                   Data set: demonstration of a Causal Inference
                   Technique},
  volume =        {173},
  year =          {2011},
}

@article{Rose&Snowden&Mortimer11,
author={S. Rose and J.M. Snowden and K.M. Mortimer},
title={Rose et al. Respond to ``{G}-Computation and Standardization in Epidemiology''},
journal={Am J Epidemiol},
volume={173},
number={00},
pages={000--000},
year={2011},
}

@incollection{Robins99b,
  author =        {Robins, J.M.},
  booktitle =     {Statistical models in epidemiology: the environment
                   and clinical trials},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  title =         {Marginal structural models versus structural nested
                   models as tools for causal inference},
  year =          {1999},
}

@article{Hernan&Brumback&Robins00,
  author =        {Hernan, M.A. and Brumback, B. and Robins, J.M.},
  journal =       {Epidemiol},
  number =        {5},
  pages =         {561--570},
  title =         {Marginal structural models to estimate the causal
                   effect of zidovudine on the survival of
                   {HIV}-positive men},
  volume =        {11},
  year =          {2000},
}

@article{Robins&Rotnitzky&vanderLaan00,
  author =        {J.M. Robins and A. Rotnitzky and M.J. van der Laan},
  journal =       {J Am Stat Assoc},
  pages =         {431--435},
  title =         {Comment on ``{O}n profile likelihood"},
  volume =        {450},
  year =          {2000},
}

@inproceedings{Robins00,
  author =        {J.M. Robins},
  booktitle =     {Proceedings of the American Statistical Association},
  editor =        {},
  organization =  {},
  pages =         {},
  title =         {Robust estimation in sequentially ignorable missing
                   data and causal inference models},
  year =          {2000},
}

@article{Robins&Rotnitzky01,
  author =        {J.M. Robins and A. Rotnitzky},
  journal =       {Stat Sinica},
  number =        {4},
  pages =         {920--936},
  title =         {Comment on the {B}ickel and {K}won article,
                   ``{I}nference for semiparametric models: some
                   questions and an answer''},
  volume =        {11},
  year =          {2001},
}

@incollection{Robins&Rotnitzky92,
  author =        {J.M. Robins and A. Rotnitzky},
  booktitle =     {AIDS epidemiology},
  publisher =     {Birkh\"{a}user},
      address={Basel},
  title =         {Recovery of information and adjustment for dependent
                   censoring using surrogate markers},
                   pages={297--331},
  year =          {1992},
}

@article{Robins&Hernan&Brumback00,
  author =        {Robins, J.M. and Hernan, M.A. and Brumback, B.},
  journal =       {Epidemiol},
  number =        {5},
  pages =         {550--560},
  title =         {Marginal structural models and causal inference in
                   epidemiology},
  volume =        {11},
  year =          {2000},
}

@article{Mortimeretal05,
  author =        {K.M. Mortimer and R. Neugebauer and M.J. van der Laan and
                   I.B. Tager},
  journal =       {Am J Epidemiol},
  number =        {4},
  pages =         {382--388},
  title =         {An Application of Model-Fitting Procedures for
                   Marginal Structural Models},
  volume =        {162},
  year =          {2005},
}

@article{Cole&Hernan08,
  author =        {S.R. Cole and M.A. Hernan},
  journal =       {Am J Epidemiol},
  pages =         {656--664},
  title =         {Constructing Inverse Probability Weights for Marginal
                   Structural Models},
  volume =        {168},
  year =          {2008},
}

@article{Bembom&vanderLaan07,
  author =        {O. Bembom and M.J. van der Laan},
  journal =       {Electron J Stat},
volume={1},
pages={574--596},
  title =         {A practical illustration of the importance of
                   realistic individualized treatment rules in causal
                   inference},
  year =          {2007},
}

@article{vanderLaan08,
  author =        {M.J. van der Laan},
  journal =       {Int J Biostat},
  volume={4},
  number={1},
pages={Article 17},
  title =         {Estimation based on case-control designs with known
                   prevalance probability},
  year =          {2008},
}

@article{Rose&vanderLaan08,
  author =        {S. Rose and M.J. van der Laan},
  journal =       {Int J Biostat},
  volume={4},
  number={1},
pages={Article 19},
  title =         {Simple optimal weighting of cases and controls in
                   case-control studies},
  year =          {2008},
}

@article{Rose&vanderLaan09,
  author =        {S. Rose and M.J. van der Laan},
  journal =       {Int J Biostat},
    volume={5},
  number={1},
pages={Article 1},
  title =         {Why match? {I}nvestigating matched case-control study
                   designs with causal effect estimation},
  year =          {2009},
}

@inproceedings{Moore&vanderLaan09,
  author =        {K.L. Moore and M.J. van der Laan},
  booktitle =     {Design, summarization, analysis \& interpretation
                   of clinical trials with time-to-event endpoints},
  editor =        {Karl E. Peace},
        address =       {Boca Raton},
  publisher =     {Chapman \& Hall},
  title =         {Application of Time-to-Event Methods in the
                   Assessment of Safety in Clinical Trials},
  year =          {2009},
}

@article{Moore&vanderLaan092,
  author =        {Moore, K.L. and van der Laan, M.J.},
  journal =       {Stat Med},
  number =        {1},
  pages =         {39--64},
  title =         {Covariate Adjustment in Randomized Trials with Binary
                   Outcomes: targeted Maximum Likelihood Estimation},
  volume =        {28},
  year =          {2009},
}

@article{Moore&vanderLaan093,
  author =        {Moore, K.L. and van der Laan, M.J.},
  journal =       {J Biopharm Stat},
  number =        {6},
  pages =         {1099--1131},
  title =         {Increasing Power in Randomized Trials with Right
                   Censored Outcomes Through Covariate Adjustment},
  volume =        {19},
  year =          {2009},
}

@article{Bembometal09b,
  author =        {O. Bembom and M.L. Petersen and S.-Y. Rhee and
                   W.J. Fessel and S.E. Sinisi and R.W. Shafer and
                   M.J. van der Laan},
  journal =       {Stat Med},
  pages =         {152--72},
  title =         {Biomarker discovery using targeted maximum likelihood
                   estimation: application to the treatment of
                   antiretroviral resistant {HIV} infection},
  volume =        {28},
  year =          {2009},
}

@article{Rosenblumetal09,
  author =        {M. Rosenblum and S.G. Deeks and M.J. van der Laan and
                   D.R. Bangsberg},
  journal =       {PLoS ONE},
  title =         {The Risk of Virologic Failure Decreases with Duration
                   of {HIV} Suppression, at Greater than 50\% Adherence to
                   Antiretroviral Therapy},
  volume =        {4(9): e7196.doi:10.1371/journal.pone.0007196},
  year =          {2009},
}

@article{Gruber&vanderLaan10a,
  author =        {S. Gruber and M.J. van der Laan},
  journal =       {Int J Biostat},
  number =        {1},
  title =         {An application of collaborative targeted maximum
                   likelihood estimation in causal inference and
                   genomics},
  volume =        {6},
  year =          {2010},
}

@article{Rosenblum&vanderLaan10,
  author =        {M. Rosenblum and M.J. van der Laan},
  journal =       {Int J Biostat},
    volume={6},
  number={2},
pages={Article 19},
  title =         {Targeted maximum likelihood estimation of the
                   parameter of a marginal structural model},
  year =          {2010},
}

@book{Dudoit&vanderLaan08,
address={Berlin Heidelberg New York},
  author =        {S. Dudoit and M.J. van der Laan},
  publisher =     {Springer},
  title =         {Resampling based multiple testing with applications
                   to genomics},
  year =          {2008},
}

@article{Robins94,
  author =        {J.M. Robins},
  journal =       {Commun Stat},
  number =        {},
  pages =         {2379--2412},
  title =         {Correcting for noncompliance in randomized trials
                   using structural nested mean models},
  volume =        {23},
  year =          {1994},
}

@article{Robins&Rotnitzky&Zhao95,
  author =        {J.M. Robins and A. Rotnitzky and L.P. Zhao},
  journal =       {J Am Stat Assoc},
  pages =         {106--121},
  title =         {Analysis of semiparametric regression models for
                   repeated outcomes in the presence of missing data.},
  volume =        {90},
  year =          {1995},
}

@article{Scharfstein&Rotnitzky&Robins99,
  author =        {D.O. Scharfstein and A. Rotnitzky and J.M. Robins},
  journal =       {J Am Stat Assoc},
  pages =         {1096-1120 (1121-1146)},
  title =         {Adjusting for Nonignorable Drop-out Using
                   Semiparametric Nonresponse Models, (with Discussion
                   and Rejoinder)},
  volume =        {94},
  year =          {1999},
}

@article{Leon&Tsiatis&Davidian03,
  author =        {S. Leon and A.A. Tsiatis and M. Davidian},
  journal =       {Biometrics},
  pages =         {1046--1055},
  title =         {Semiparametric estimation of treatment effect in a
                   pretest-posttest study},
  volume =        {59},
  year =          {2003},
}

@article{Tan06,
  author =        {Z. Tan},
  journal =       {J Am Stat Assoc},
  pages =         {1619-1637},
  title =         {A distributional approach for causal inference using
                   propensity scores},
  volume =        {101},
  year =          {2006},
}

@book{Tsiatis062,
  address={Berlin Heidelberg New York},
  author =        {A.A. Tsiatis},
  publisher =     {Springer},
  title =         {Semiparametric theory and missing data},
  year =          {2006},
}

@article{Zhang&Tsiatis&Davidian08,
  author =        {M. Zhang and A.A. Tsiatis and M. Davidian},
  journal =       {Biometrics},
  number =        {3},
  pages =         {707--715},
  title =         {Improving efficiency of inferences in randomized
                   clinical trials using auxiliary covariates},
  volume =        {64},
  year =          {2008},
}

@article{Rubin&vanderLaan08,
  author =        {Daniel B. Rubin and M.J. van der Laan},
  journal =       {Int J Biostat},
  title =         {Empirical efficiency maximization: improved locally
                   efficient covariate adjustment in randomized
                   experiments and survival analysis},
  volume =        {4},
  number={1},
  pages={Article 5},
  year =          {2008},
}

@article{Freedman08,
  author =        {D.A. Freedman},
  journal =       {Adv Appl Math},
  pages =         {180--193},
  title =         {On regression adjustments to experimental data},
  volume =        {40},
  year =          {2008},
}

@article{Freedman082,
  author =        {D.A. Freedman},
  journal =       {Ann Appl Stat},
  pages =         {176--96},
  title =         {On regression adjustments to experiments with several
                   treatments},
  volume =        {2},
  year =          {2008},
}

@article{Rosenblum&vanderLaan09,
  author =        {M. Rosenblum and M.J. van der Laan},
  journal =       {Biometrics},
  number =        {3},
  pages =         {937--945},
  title =         {Using Regression Models to Analyze Randomized Trials:
                   asymptotically Valid Hypothesis Tests Despite
                   Incorrectly Specified Models},
  volume =        {65},
  year =          {2009},
}

@book{Hampeletal86,
  author =        {Hampel, F.R. and Ronchetti, E.M. and Rousseeuw, P.J. and
                   Stahel, W.A.},
  address =       {New York},
  publisher =     {Wiley},
  title =         {{Robust statistics: the approach based on influence
                   functions}},
  year =          {1986},
}

@book{vanderVaart98,
  author =        {A.W. van der Vaart},
  publisher =     {Cambridge},
  title =         {Asymptotic statistics},
    address =       {New York},
  year =          {1998},
}

@book{vanderVaart&Wellner96,
  author =        {A.W. van der Vaart and J.A. Wellner},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  title =         {Weak convergence and empirical processes},
  year =          {1996},
}

@article{Rosenbaum&Rubin83,
  author =        {P.R. Rosenbaum and Donald B. Rubin},
  journal =       {Biometrika},
  pages =         {41--55},
  title =         {The central role of the propensity score in
                   observational studies for causal effects},
  volume =        {70},
  year =          {1983},
}

@article{Stitelman&vanderLaan10,
  author =        {O.M. Stitelman and M.J. van der Laan},
Journal={Int J Biostat},
volume={6},
number={1},
pages={Article 21},
  title =         {Collaborative Targeted Maximum Likelihood for
                   Time-to-Event Data},
  year =          {2010},
}


@article{Wedderburn74,
  author =        {R.W.M. Wedderburn},
  journal =       {Biometrika},
  pages =         {439--447},
  title =         {Quasi-likelihood functions, generalized linear
                   models, and the Gauss-Newton method},
  volume =        {61},
  number={3},
  year =          {1974},
}

@article{McCullagh83,
  author =        {P. Mc{C}ullagh},
  journal =       {Ann Stat},
  pages =         {59--67},
  title =         {Quasi-likelihood functions},
  volume =        {11},
  year =          {1983},
}

@article{vanderLaan&Petersen08,
  author =        {M.J. van der Laan and M.L. Petersen},
  journal =       {Int J Biostat},
  number =        {1},
  title =         {Direct effect models},
  volume =        {4},
  pages={Article 23},
  year =          {2008},
}

@techreport{vanderLaan10c,
  author =        {M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =        {268},
  title =         {Estimation of Causal Effects of Community-Based
                   Interventions},
  year =          {2010},
}

@article{Heckman&Ichimura&Todd97,
  author =        {J. Heckman and H. Ichimura and R. Todd},
  journal =       {Rev of Econ Stud},
  pages =         {605--654},
  title =         {Matching as an Econometric Evaluation Estimator:
                   evidence from Evaluating a Job Training Programme},
  volume =        {64},
  year =          {1997},
}

@techreport{Sekhon06,
  author =        {J.S. Sekhon},
  institution =   {University of California,
                   Berkeley},
  type={Technical {R}eport},
  title =         {Alternative balance metrics for bias reduction in
                   matching methods for causal inference},
  year =          {2006},
}

@article{Hansen08,
  author =        {B.B. Hansen},
  journal =       {Biometrika},
  pages =         {481--8},
  title =         {The prognostic analogue of the propensity score},
  volume =        {95},
  year =          {2008},
}

@book{Haignere02,
  address =       {Washington, DC},
  author =        {Haignere, L.},
  edition =       {2nd},
  publisher =     {American Association of University Professors},
  title =         {Paychecks: a guide to conducting salary-equity
                   studies for higher education faculty},
  year =          {2002},
}

@article{Holland88,
  author =        {P.W. Holland},
  journal =       {Stat Sci},
  number =        {2},
  pages =         {186--188.},
  title =         {Comment: Causal Mechanism or Causal Effect: which Is
                   Best for Statistical Science?},
  volume =        {3},
  year =          {1988},
}

@article{Robins98,
  author =        {J.M. Robins},
  journal =       {1997 Proceedings of the American Statistical
                   Association. Section on {B}ayesian Statistical Science},
  pages =         {1--10},
  title =         {Marginal Structural Models},
  year =          {1998},
}

@article{Mossetal04,
  author =        {A.R. Moss and J.A. Hahn and S. Perry and
                   E.D. Charlebois and D. Guzman and R.A. Clark and
                   D.R. Bangsberg},
  journal =       {Clin Infect Dis},
  number =        {8},
  pages =         {1190--1198},
  title =         {Adherence to highly active antiretroviral therapy in
                   the homeless population in {S}an {F}rancisco: a
                   prospective study},
  volume =        {39},
  year =          {2004},
}

@article{Bangsbergetal01,
  author =        {D.R. Bangsberg and F. Hecht and E.D. Charlebois and
                   M. Chesney and A.R. Moss},
  journal =       {AIDS Behav},
  pages =         {275--281},
  title =         {Comparing Objectives Measures of Adherence to HIV
                   Antiretroviral Therapy: electronic Medication
                   Monitors and Unannounced Pill Counts.},
  volume =        {5},
  year =          {2001},
}

@article{Neugebauer&vanderLaan07,
  author =        {R. Neugebauer and M. J. van der Laan},
  journal =       {J Stat Plan Infer},
  number =        {2},
  pages =         {419--434},
  title =         {Nonparametric causal effects based on marginal
                   structural models},
  volume =        {137},
  year =          {2007},
}

@article{Efron87,
  author =        {B. Efron},
  journal =       {J Am Stat Assoc},
  number =        {397},
  pages =         {171--185},
  title =         {Better Bootstrap Confidence Intervals},
  volume =        {82},
  year =          {1987},
}

@article{Kirschetal08,
  author =        {I. Kirsch and B.J. Deacon and T.B. Huedo-Medina and
                   A. Scoboria and T.J. Moore and B.T. Johnson},
  journal =       {PLoS Med},
  number =        {2},
  pages =         {e45. doi:10.1371/journal.pmed.0050045},
  title =         {Initial Severity and Antidepressant Benefits: a
                   Meta-Analysis of Data Submitted to the {Food and Drug
                   Administration}},
  volume =        {5},
  year =          {2008},
}

@article{Baselga01,
  author =        {J. Baselga},
  journal =       {Oncology},
  pages =         {14--21},
  title =         {Herceptin alone or in combination with chemotherapy
                   in the treatment of {HER2}-positive metastatic breast
                   cancer: pivotal trials},
  volume =        {61(S2)},
  year =          {2001},
}

@techreport{Wangetal06,
  author =        {Y. Wang and M.L. Petersen and D.R. Bangsberg and
                   M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =        {211},
  title =         {Diagnosing Bias in the Inverse Probability of
                   Treatment Weighted Estimator Resulting from Violation
                   of Experimental Treatment Assignment.},
  year =          {2006},
}

@article{Robins87,
  author =        {Robins, J.M.},
  journal =       {Comput Math Appl},
  number =        {9--12},
  pages =         {923--945},
  title =         {Addendum to: ``{A} new approach to causal inference
                   in mortality studies with a sustained exposure
                   period---application to control of the healthy worker
                   survivor effect''},
  volume =        {14},
  year =          {1987},
}

@article{Robins872,
  author =        {J.M. Robins},
  journal =       {J Chron Dis (40, Supplement)},
  pages =         {139s--161s},
  title =         {A graphical approach to the identification and
                   estimation of causal parameters in mortality studies
                   with sustained exposure periods},
  volume =        {2},
  year =          {1987},
}

@article{Rosenblum&vanderLaan09b,
  author =        {M. Rosenblum and M.J. van der Laan},
  journal =       {Int J Biostat},
  pages =         {Article 4},
  title =         {Confidence Intervals for the Population Mean Tailored
                   to Small Sample Sizes, with Applications to Survey
                   Sampling},
  volume =        {1},
  year =          {2009},
}

@article{Neugebauer&vanderLaan05,
  author =        {Neugebauer, R. and van der Laan, M.J.},
  journal =       {J Stat Plan Infer},
  number =        {1-2},
  pages =         {405--26},
  title =         {Why prefer double robust estimates},
  volume =        {129},
  year =          {2005},
}

@techreport{Mooreetal09,
  author =        {K.L. Moore and R.S. Neugebauer and M.J. van der Laan and
                   I.B. Tager},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =        {255},
  title =         {Causal Inference in Epidemiological Studies with
                   Strong Confounding},
  year =          {2009},
}

@article{Kish92,
  author =        {L. Kish},
  journal =       {J Off Stat},
  number =        {},
  pages =         {183--200},
  title =         {Weighting for unequal $P_i$},
  volume =        {8},
  year =          {1992},
}

@techreport{Bembom&vanderLaan08,
  author =        {O. Bembom and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =        {230},
  title =         {Data-adaptive selection of the truncation level for
                   Inverse-Probability-of-Treatment-Weighted estimators},
  year =          {2008},
}

@article{Freedman&Berk08,
  author =        {D.A. Freedman and R.A. Berk},
  journal =       {Eval Rev},
  pages =         {392--409},
  title =         {Weighting Regressions by Propensity Scores},
  volume =        {3},
  year =          {2008},
}

@article{Petersenetal10,
  author =        {M.L. Petersen and K.E. Porter and S. Gruber and
                   Y. Wang and M.J. van der Laan},
journal = {Stat Meth Med Res},
  title =         {Diagnosing and responding to violations in the
                   positivity assumption},
     volume =        {published online 28 Oct (doi:
                   10.1177/0962280210386207)},
  year =          {2010},
}

@article{Johnsonetal09,
  author =        {V.A. Johnson and F. Brun-Vezinet and B. Clotet and
                   H.F. Gunthard and D.R. Kuritzkes and D. Pillay and
                   J.M. Schapiro and D.D. Richman},
  journal =       {Top HIV Med},
  number =        {5},
  pages =         {138--45},
  title =         {Update of the drug resistance mutations in {HIV}-1:
                   {D}ecember 2009.},
  volume =        {17},
  year =          {2009},
}

@techreport{Bembometal08b,
  author =        {O. Bembom and W.J. Fessel and R.W. Shafer and
                   M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  type =          {231},
  title =         {Data-adaptive Selection Of The Adjustment Set In
                   Variable Importance Estimation},
  year =          {2008},
}

@techreport{Crumpetal06,
  author =        {R.K. Crump and V.J. Hotz and G.W. Imbens and
                   O.A. Mitnik},
  institution =   {National Bureau of Economic Research},
  number =        {330},
  title =         {Moving the goalposts: addressing limited overlap in
                   the estimation of average treatment effects by
                   changing the estimand},
  year =          {2006},
}

@article{LaLonde86,
  author =        {R.J. LaLonde},
  journal =       {Am Econ Rev},
  pages =         {604--620},
  title =         {Evaluating the Econometric Evaluations of Training
                   Programs with Experimental Data},
  volume =        {76},
  year =          {1986},
}

@article{Dehejia&Wahba99,
  author =        {R. Dehejia and S. Wahba},
  journal =       {J Am Stat Assoc},
  pages =         {1053--1062},
  title =         {Causal Effects in Nonexperimental Studies:
                   reevaluating the Evaluation of Training Programs},
  volume =        {94},
  year =          {1999},
}

@article{vanderLaan&Petersen07,
  author =        {M.J. van der Laan and M.L. Petersen},
  journal =       {Int J Biostat},
  number =        {1},
  pages =         {Article 3},
  title =         {Causal Effect Models for Realistic Individualized
                   Treatment and Intention to Treat Rules},
  volume =        {3},
  year =          {2007},
}

@article{Robins&Orellana&Rotnitzky08,
  author =        {J.M. Robins and L. Orellana and A. Rotnitzky},
  journal =       {Stat Med},
  pages =         {4678--4721},
  title =         {Estimation and extrapolation of optimal treatment and
                   testing strategies},
  volume =        {27},
  year =          {2008},
}

@article{Cochran57,
  author =        {W.G. Cochran},
  journal =       {Biometrics},
  number =        {},
  pages =         {261--281},
  title =         {Analysis of Covariance: its Nature and Uses.},
  volume =        {13},
  year =          {1957},
}

@techreport{Moore&vanderLaan07,
  author =        {K.L. Moore and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  month =         {April},
  number =          {215},
  title =         {Covariate adjustment in randomized trials with binary
                   outcomes},
  year =          {2007},
}

@article{Rosenblum&vanderLaan102,
  author =        {M. Rosenblum and M.J. van der Laan},
  journal =       {Int J Biostat},
  number =        {1},
  pages =         {Article 13},
  title =         {Simple, Efficient Estimators of Treatment Effects in
                   Randomized Trials Using Generalized Linear Models to
                   Leverage Baseline Variables},
  volume =        {6},
  year =          {2010},
}

@article{Freedman083,
  author =        {D.A. Freedman},
  journal =       {Stat Sci},
  pages =         {237--249},
  title =         {Randomization does not justify logistic regression},
  volume =        {23},
  year =          {2008},
}

@article{Yang&Tsiatis01,
  author =        {L. Yang and A.A. Tsiatis},
  journal =       {Am Stat},
  pages =         {29--38},
  title =         {Efficiency study for a treatment effect in a
                   pretest-posttest trial},
  volume =        {56},
  year =          {2001},
}

@book{McCullagh&Nelder89,
  address =       {Boca Raton},
  author =        {P. McCullagh and J.A. Nelder},
  edition =       {2nd},
  publisher =     {Chapman \& Hall},
  title =         {Generalized linear models},
  year =          {1989},
}

@incollection{Gail86,
  address =       {New York},
 author =        {M.H. Gail},
  booktitle =     {Modern Statistical Methods in Chronic Disease
                   Epidemiology},
  editor =        {S.~H. Moolvankar and R.~L.
                   Prentice},
  publisher =     {Wiley},
  title =         {Adjusting for covariates that have the same
                   distribution in exposed and unexposed cohorts},
  year =          {1986},
}

@article{Tsiatisetal08,
  author =        {A.A. Tsiatis and M. Davidian and M. Zhang and X. Lu},
  journal =       {Stat Med},
  pages =         {4658--4677},
  title =         {Covariate adjustment for two-sample treatment
                   comparisons in randomized clinical trials: a
                   principled yet flexible approach},
  volume =        {27},
  year =          {2008},
}

@article{Kochetal98,
  author =        {G.G. Koch and C.M. Tangen and J.W. Jung and
                   I.A. Amara},
  journal =       {Stat Med},
  pages =         {1863--1892},
  title =         {Issues for covariance analysis of dichotomous and
                   ordered categorical data from randomized clinical
                   trials and nonparametric strategies for addressing
                   them},
  volume =        {17},
  year =          {1998},
}

@article{Pococketal02,
  author =        {S.J. Pocock and S.E. Assmann and L.E. Enos and
                   L.E. Kasten},
  journal =       {Stat Med},
  pages =         {2917--2930},
  title =         {Subgroup analysis, covariate adjustment, and baseline
                   comparisons in clinical trial reporting: current
                   practice and problems.},
  volume =        {21},
  year =          {2002},
}

@article{Anderson72,
  author =        {J.A. Anderson},
  journal =       {Biometrika},
  pages =         {19--35},
  title =         {Separate sample logistic discrimination},
  volume =        {59},
  year =          {1972},
}

@article{Robins99,
  author =        {J.M. Robins},
  journal =       {Stat Sci},
  number =        {3},
  pages =         {281--293},
  title =         {[{C}hoice as an Alternative to Control in Observational
                   Studies]: Comment},
  volume =        {14},
  year =          {1999},
}

@article{Manssonetal07,
  author =        {R. Mansson and M.M. Joffe and W. Sun and S. Hennessy},
  journal =       {Am J Epidemiol},
  number =        {3},
  pages =         {332-339},
  title =         {On the Estimation and Use of Propensity Scores in
                   Case-Control and Case-Cohort Studies.},
  volume =        {166},
  year =          {2007},
}

@article{Prentice&Pyke79,
  author =        {R.L. Prentice and R. Pyke},
  journal =       {Biometrika},
  pages =         {403--411},
  title =         {Logistic disease incidence models and case-control
                   studies},
  volume =        {66},
  year =          {1979},
}

@book{Breslow&Day80,
  address =       {Lyon},
  author =        {N.E. Breslow and N.E. Day},
  publisher =     {International Agency for Research on Cancer},
  title =         {Statistical methods in cancer research: {V}olume 1 --
                   {T}he analysis of case-control studies},
  year =          {1980},
}

@article{Breslow96,
  author =        {N.E. Breslow},
  journal =       {J Am Stat Soc},
  pages =         {14--28},
  title =         {Statistics in Epidemiology: the Case-Control Study},
  volume =        {91},
  year =          {1996},
}

@article{Greenland81,
  author =        {S. Greenland},
  journal =       {J Chron Dis},
  pages =         {445--453},
  title =         {Multivariate Estimation of Exposure-Specific
                   Incidence from Case-Control Studies.},
  volume =        {34},
  year =          {1981},
}

@incollection{Holland&Rubin88,
  address =       {Cambridge, MA},
  author =        {P.W. Holland and Donald B. Rubin},
  booktitle =     {Matched sampling for causal effects.},
  editor =        {Donald B. Rubin},
  publisher =     {Cambridge},
  title =         {Causal inference in retrospective studies},
  year =          {1988},
}

@article{Greenland04,
  author =        {S. Greenland},
  journal =       {Am J Epidemiol},
  number =        {4},
  pages =         {301--305},
  title =         {Model-based Estimation of Relative Risks and Other
                   Epidemiologic Measures in Studies of Common Outcomes
                   and in Case-Control Studies.},
  volume =        {160},
  year =          {2004},
}

@article{Newman06,
  author =        {S. Newman},
  journal =       {Epid Persp Innov},
  pages =         {2},
  title =         {Causal analysis of case-control data},
  volume =        {3},
  year =          {2006},
}

@article{Cornfield51,
  author =        {J. Cornfield},
  journal =       {J Nat Cancer Inst},
  pages =         {1269--1275},
  title =         {A method of estimating comparative rates from
                   clinical data. Applications to cancer of the lung,
                   breast, and cervix.},
  volume =        {11},
  year =          {1951},
}

@inproceedings{Cornfield56,
  author =        {J. Cornfield},
    address =       {Berkeley},
  booktitle =     {Proceedings of the 3rd Berkeley symposium, {V}ol
                   IV},
  editor =        {J. Neyman},
  publisher =     {University of California Press},
  title =         {A statistical problem arising from retrospective
                   studies},
  year =          {1956},
}

@article{Prentice&Breslow78,
  author =        {R.L. Prentice and N.E. Breslow},
  journal =       {Biometrika},
  number =        {1},
  pages =         {153--158},
  title =         {Retrospective studies and failure time models.},
  volume =        {65},
  year =          {1978},
}

@article{Moriseetal96,
  author =        {A.P. Morise and G.A. Diamon and R. Detrano and
                   M. Bobbio and Erdogan Gunel},
  journal =       {Med Decis Making},
  pages =         {133--142},
  title =         {The Effect of Disease-prevalence Adjustments on the
                   Accuracy of a Logistic Prediction Model.},
  volume =        {16},
  year =          {1996},
}

@article{Wacholder96,
  author =        {S. Wacholder},
  journal =       {Epidemiol},
  number =        {2},
  pages =         {144--150},
  title =         {The Case-Control Study as Data Missing by Design:
                   estimating Risk Differences.},
  volume =        {7},
  year =          {1996},
}

@article{Rose&vanderLaan11,
  author =        {S. Rose and M.J. van der Laan},
  journal =       {Int J Biostat},
  number =        {17},
  title =         {A Targeted Maximum Likelihood Estimator for Two-Stage
                   Designs},
  volume =        {7},
  year =          {2011},
}

@article{Freedman50,
  author =        {R. Freedman},
  journal =       {Am J of Soc},
  number =        {5},
  pages =         {485--487},
  title =         {Incomplete Matching in Ex Post Facto Studies},
  volume =        {55},
  year =          {1950},
}

@article{Cochran65,
  author =        {W.G. Cochran},
  journal =       {J R Stat Soc Ser A Gen},
  number =        {2},
  pages =         {234--266},
  title =         {The Planning of Observational Studies of Human
                   Populations},
  volume =        {128},
  year =          {1965},
}

@article{Billewicz65,
  author =        {W.Z. Billewicz},
  journal =       {Biometrics},
  number =        {3},
  pages =         {623--644},
  title =         {The Efficiency of Matched Samples: an Empirical
                   Investigation},
  volume =        {21},
  year =          {1965},
}

@article{McKinlay77,
  author =        {S.M. McKinlay},
  journal =       {Biometrics},
  number =        {4},
  pages =         {725--735},
  title =         {Pair-Matching -- A reappraisal of a Popular
                   Technique},
  volume =        {33},
  year =          {1977},
}

@article{Kupperetal81,
  author =        {L.L. Kupper and J.M. Karon and D.G. Kleinbaum and
                   H. Morgenstern and D.K. Lewis},
  journal =       {Biometrics},
  pages =         {271--291},
  title =         {Matching in Epidemiologic Studies: validity and
                   Efficiency Considerations},
  volume =        {37},
  year =          {1981},
}

@article{Costanza95,
  author =        {M.C. Costanza},
  journal =       {Prev Med},
  pages =         {425--433},
  title =         {Matching},
  volume =        {24},
  year =          {1995},
}

@book{Schlesselman82,
  address =       {Oxford},
  author =        {J.J. Schlesselman},
  publisher =     {Oxford},
  title =         {Case-control studies: design, conduct, analysis},
  year =          {1982},
}

@article{Vandenbroukeetal07,
  author =        {J.P. Vandenbrouke and E. von Elm and D.G. Altman and
                   P.C. Gotzsche and C.D. Mulrow and S.J. Pocock and
                   C. Poole and J.J. Schlesselman and
                   M. Egger for the STROBE Initiative},
  journal =       {PLoS Med},
  number =        {10},
  pages =         {1628--1654},
  title =         {Strengthening the Reporting of Observational
                   Studies in Epidemiology ({STROBE}): explanation
                   and Elaboration.},
  volume =        {4},
  year =          {2007},
}

@article{Cochran53,
  author =        {W.G. Cochran},
  journal =       {Am J Public Health},
  pages =         {684--691},
  title =         {Matching in Analytical Studies},
  volume =        {43},
  year =          {1953},
}

@article{Breslowetal78,
  author =        {N.E. Breslow and N.E. Day and K.T. Halvorsen and
                   R.L. Prentice and C. Sabal},
  journal =       {Am J Epidemiol},
  number =        {4},
  pages =         {299--307},
  title =         {Estimation of Multiple Relative Risk Functions in
                   Matched Case-Control Studies},
  volume =        {108},
  year =          {1978},
}

@article{Holford&White&Kelsey78,
  author =        {T.R. Holford and C. White and J.L. Kelsey},
  journal =       {Am J Epidemiol},
  number =        {3},
  pages =         {245--255},
  title =         {Multivariate Analysis for Matched Case-Control
                   Studies},
  volume =        {107},
  year =          {1978},
}

@article{Kannel&McGee&Gordon76,
  author =        {W.B. Kannel and D. McGee and T. Gordon},
  journal =       {Am J Cardiol},
  pages =         {46--51},
  title =         {A general cardiovascular risk profile: the {F}ramingham
                   Study},
  volume =        {38},
  year =          {1976},
}

@article{Andersonetal91,
  author =        {K.M. Anderson and P.W.F. Wilson and P.M. Odell and
                   W.B. Kannel},
  journal =       {Circulation},
  pages =         {356--362},
  title =         {An updated coronary risk profile. A statement for
                   health professionals.},
  volume =        {83},
  year =          {1991},
}

@article{Ramsayetal95,
  author =        {L.E. Ramsay and I.U. Haq and P.R. Jackson and
                   W.W. Yeo},
  journal =       {Lancet},
  number =        {8988},
  pages =         {1467--1471},
  title =         {Sheffield risk and treatment table for cholesterol
                   lowering for primary prevention of coronary heart
                   disease.},
  volume =        {346},
  year =          {1995},
}

@article{Ramsayetal96,
  author =        {L.E. Ramsay and I.U. Haq and P.R. Jackson and
                   W.W. Yeo},
  journal =       {Lancet},
  number =        {9036},
  pages =         {1251},
  title =         {The {S}heffield table for primary prevention of
                   coronary heart disease: corrected.},
  volume =        {348},
  year =          {1996},
}

@article{Wilsonetal98,
  author =        {P.W.F. Wilson and R.B. D'Agostino and D. Levy and
                   A.M. Belanger and H. Silbershatz and W.B. Kannel},
  journal =       {Circulation},
  pages =         {1837--1847},
  title =         {Prediction of coronary heart disease using risk
                   factor categories},
  volume =        {97},
  year =          {1998},
}

@article{Jackson00,
  author =        {R. Jackson},
  journal =       {Br Med J},
  number =        {7236},
  pages =         {709--710},
  title =         {Updated New Zealand cardiovascular disease
                   risk-benefit prediction guide.},
  volume =        {320},
  year =          {2000},
}

@article{Gailetal89,
  author =        {M.H. Gail and L.A. Brinton and D.P. Byar and
                   D.K. Corle and S.B. Green and C. Schairer and
                   J.J. Mulvihill},
  journal =       {J Natl Cancer Inst},
  number =        {24},
  pages =         {1879--1886},
  title =         {Projecting individualized probabilities of developing
                   breast cancer for white females who are being
                   examined annually.},
  volume =        {81},
  year =          {1989},
}

@article{Costantinoetal99,
  author =        {J.P. Costantino and M.H. Gail and D. Pee and
                   S. Anderson and C.K. Redmond and J. Benichou and
                   H.S. Wieand},
  journal =       {J Natl Cancer Inst},
  number =        {18},
  pages =         {1541--1548},
  title =         {Validation studies for models projecting the risk of
                   invasive and total breast cancer incidence.},
  volume =        {91},
  year =          {1999},
}

@article{Tyrer&Duffy&Cuzick04,
  author =        {J. Tyrer and S.W. Duffy and J. Cuzick},
  journal =       {Stat Med},
  number =        {7},
  pages =         {1111--1130},
  title =         {A breast cancer prediction model incorporating
                   familial and personal risk factors},
  volume =        {23},
  year =          {2004},
}

@article{Barlowetal06,
  author =        {W.E. Barlow and E. White and R. Ballard-Barbash and
                   P.M. Vacek and L. Titus-Ernstoff and P.A. Carney and
                   J.A. Tice and D.S. Buist and B.M. Geller and
                   R. Rosenberg and B.C. Yankaskas and K. Kerlikowske},
  journal =       {J Natl Cancer Inst},
  number =        {17},
  pages =         {1204--1214},
  title =         {Prospective breats cancer risk prediction model for
                   women undergoing screening mammography.},
  volume =        {98},
  year =          {2006},
}

@article{Loprinzietal94,
  author =        {C.L. Loprinzi and J.A. Laurie and H.S. Wieand and
                   J.E. Krook and P.J. Novotny and J.W. Kugler and
                   J. Bartel and M. Law and M. Bateman and N.E. Klatt},
  journal =       {J Clin Oncol},
  number =        {3},
  pages =         {601--607},
  title =         {Prospective Evaluation of Prognostic Variables from
                   Patient-Completed Questionnaires, {N}orth {C}entral
                   {C}ancer {T}reatment {G}roup},
  volume =        {12},
  year =          {1994},
}

@manual{Therneau&Lumley09,
  author =        {T. Therneau and T. Lumley},
  note =          {R package version 2.35-8},
  title =         {survival: survival analysis, including penalised
                   likelihood},
  year =          {2009},
  url =           {http://CRAN.R-project.org/package=survival},
}

@article{Tibshirani97,
  author =        {R.J. Tibshirani},
  journal =       {Stat Med},
  pages =         {385--395},
  title =         {The Lasso Method for Variable Selection in the {C}ox
                   Model},
  volume =        {16},
  year =          {1997},
}

@article{Zhang&Lu07,
  author =        {H.H. Zhang and W. Lu},
  journal =       {Biometrika},
  number =        {3},
  pages =         {691--703},
  title =         {Adaptive Lasso for {C}ox's Proportional Hazards Model},
  volume =        {94},
  year =          {2007},
}

@article{Kooperberg&Stone&Truong95,
  author =        {C. Kooperberg and C.J. Stone and Y.K. Truong},
  journal =       {J Am Stat Assoc},
  number =        {429},
  pages =         {78--94},
  title =         {Hazard Regression},
  volume =        {90},
  year =          {1995},
}

@article{Leblanc&Crowley92,
  author =        {M. LeBlanc and J. Crowley},
  journal =       {Biometrics},
  number =        {},
  pages =         {411--425},
  title =         {Relative Risk trees for censored data},
  volume =        {48},
  year =          {1992},
}

@article{Segal88,
  author =        {M.R. Segal},
  journal =       {Biometrics},
  pages =         {35--47},
  title =         {Regression trees for censored data},
  volume =        {44},
  year =          {1988},
}

@article{Hothornetal06,
  author =        {T. Hothorn and P. Buhlmann and S. Dudoit and
                   A.M. Molinaro and M.J. van der Laan},
  journal =       {Biostatistics},
  pages =         {355--373},
  title =         {Survival Ensembles},
  volume =        {7},
  year =          {2006},
}

@article{Ishwaranetal08,
  author =        {H. Ishwaran and U.B. Kogalur and E.H. Blackstone and
                   M.S. Lauer},
  journal =       {Ann Appl Stat},
  number =        {3},
  pages =         {841--860},
  title =         {Random Survival Forests},
  volume =        {2},
  year =          {2008},
}

@article{vanHouwelingenetal06,
  author =        {H.C. van Houwelingen and T. Bruinsma and A.A.M. Hart and
                   L.J. {van't Veer} and L.F.A. Wessels},
  journal =       {Stat Med},
  pages =         {3201--3216},
  title =         {Cross-validated {C}ox Regression on Microarray Gene
                   Expression Data},
  volume =        {25},
  year =          {2006},
}

@techreport{vanderLaan&Rubin07,
  author =        {M.J. van der Laan and Daniel B. Rubin},
    institution =   {Division of Biostatistics, University of California,
                   Berkeley},
   number={226},
  title =         {A note on targeted maximum likelihood and right-censored data},
  year =          {2007},
}

@inproceedings{Robins93,
  author =        {J.M. Robins},
  booktitle =     {Proceedings of the Biopharmaceutical Section},
  organization =  {American Statistical Association},
  title =         {Information recovery and bias adjustment in
                   proportional hazards regression analysis of
                   randomized trials using surrogate markers},
  year =          {1993},
}

@incollection{Hubbard&vanderLaan&Robins99,
  address={Berlin Heidelberg New York},
  author =        {A.E. Hubbard and M.J. van der Laan and J.M. Robins},
  booktitle =     {Statistical models in epidemiology: the environment
                   and clinical trials},
  editor =        {E. Halloran, D. Berry},
   publisher =     {Springer},
  title =         {Nonparametric locally efficient estimation of the
                   treatment specific survival distributions with right
                   censored data and covariates in observational
                   studies},
  year =          {1999},
}

@article{Hernandez&Eijkemans&Steyerberg06,
  author =        {Hern\'{a}ndez, A.V. and Eijkemans, M.J. and
                   Steyerberg, E.W.},
  journal =       {Ann Epidemiol},
  number =        {1},
  pages =         {41--48},
  title =         {Randomized controlled trials With time-to-event
                   outcomes: how much does prespecified covariate
                   adjustment increase power?},
  volume =        {16},
  year =          {2006},
}

@article{Lu&Tsiatis08,
  author =        {Lu, X. and Tsiatis, A.A},
  journal =       {Biometrika},
  number =        {3},
  pages =         {679--694},
  title =         {Improving the efficiency of the log-rank test using
                   auxiliary covariates},
  volume =        {95},
  year =          {2008},
}

@article{Tangen&Koch99,
  author =        {Tangen, C.M. and Koch, G.G.},
  journal =       {J Biopharm Stat},
  number =        {2},
  pages =         {307--338},
  title =         {On-parametric analysis of covariance for hypothesis
                   testing with logrank and {W}ilcoxon scores and
                   survival-rate estimation in a randomized clinical
                   trial},
  volume =        {9},
  year =          {1999},
}

@article{Jiangetal08,
  author =        {Jiang, H. and Symanowski, J. and Paul, S. and Qu, Y. and
                   Zagar, A. and Hong, S.},
  journal =       {Stat Med},
  number =        {28},
  pages =         {5850--5860},
  title =         {The type {I} error and power of nonparametric logrank
                   and {W}ilcoxon tests with adjustment for covariates -- A
                   simulation study},
  volume =        {27},
  year =          {2008},
}

@article{Akazawa&Nakamura&Palesch97,
  author =        {Akazawa, K. and Nakamura, T. and Palesch, Y.},
  journal =       {Stat Med},
  number =        {5},
  pages =         {583--597},
  title =         {Power of logrank test and {C}ox regression model in
                   clinical trials with heterogenous samples},
  volume =        {16},
  year =          {1997},
}

@article{Westeretal10,
  author =        {C.W. Wester and A.M. Thomas and H. Bussmann and
                   S. Moyo and J.M. Gaolathe and V. Novitsky and
                   M. Essex and V. De Gruttola and R.G. Marlink},
  journal =       {AIDS},
  pages =         {S27--S36},
  title =         {Nonnucleoside reverse transcriptase inhibitor
                   outcomes among combination antiretroviral
                   therapy-treated adults in {B}otswana},
  volume =        {24},
  year =          {2010},
}

@book{Andersenetal93,
  author =        {P.K. Andersen and O. Borgan and R.D. Gill and
                   N. Keiding},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  title =         {Statistical models based on counting processes},
  year =          {1993},
}

@techreport{Rudser&LeBlanc&Emerson08,
  author =        {K. Rudser and M. LeBlanc and S.S. Emerson},
  institution={Department of Biostatistics, University of Washington},
  title =         {Estimation for Arbitrary Functionals of Survival},
  number =        {335},
  year =          {2008},
}

@article{vanderLaan10,
  author =        {van der Laan, M.J.},
  journal =       {Int J Biostat},
  pages =          {Article 2},
  number =        {2},
  title =         {Targeted maximum likelihood based causal inference:
                   Part {I}},
  volume =        {6},
  year =          {2010},
}

@article{vanderLaan10b,
  author =        {van der Laan, M.J.},
  journal =       {Int J Biostat},
  pages =          {Article 3},
  number =        {2},
  title =         {Targeted maximum likelihood based causal inference:
                   Part {II}},
  volume =        {6},
  year =          {2010},
}

@article{Sekhon08,
  author =        {J.S. Sekhon},
  journal =       {J Stat Softw},
  title =         {Multivariate and Propensity Score Matching Software
                   with Automated Balance Optimization: the Matching
                   package for {R}},
  year =          {2008},
}

@article{Holland&Reitman77,
  address =       {New York},
  author =        {J.H. Holland and J.S. Reitman},
  journal =       {SIGART Bull},
  pages =         {49--49},
  title =         {Cognitive systems based on adaptive algorithms},
  volume =        {63},
  year =          {1977},
}

@article{Koul&Susarla&vanRyzin81,
  author =        {H. Koul and V. Susarla and J. van Ryzin},
  journal =       {Ann Stat},
  pages =         {1276--88},
  title =         {Regression analysis with randomly right censored
                   data},
  volume =        {9},
  year =          {1981},
}

@article{Keiding&Hols&Green89,
  author =        {N. Keiding and C. Hols and A. Green},
  journal =       {Am J Epidemiol},
  pages =         {588--600},
  title =         {Retrospective estimation of diabetes incidence from
                   information in a current prevalent population and
                   historical mortality},
  volume =        {130},
  year =          {1989},
}

@article{Robins&Rotnitzky&Zhao94,
  author =        {J.M. Robins and A. Rotnitzky and L.P. Zhao},
  journal =       {J Am Stat Assoc},
  month =         {September},
  number =        {427},
  pages =         {846--66},
  title =         {Estimation of regression coefficients when some
                   regressors are not always observed},
  volume =        {89},
  year =          {1994},
}

@article{Robins&Rotnitzky95,
  author =        {Robins, J.M. and A. Rotnitzky},
  journal =       {J Am Stat Assoc},
  pages =         {122--129},
  title =         {Semiparametric Efficiency in Multivariate Regression
                   Models with Missing Data},
  volume =        {90},
  year =          {1995},
}

@article{Kang&Schafer07,
  author =        {J. Kang and J.L. Schafer},
  journal =       {Stat Sci},
  pages =         {523--39},
  title =         {Demystifying Double Robustness: a Comparison of
                   Alternative Strategies for Estimating a Population
                   Mean from Incomplete Data (with discussion)},
  volume =        {22},
  year =          {2007},
}

@article{Robins&Wang00,
  author =        {J.M. Robins and N. Wang},
  journal =       {Biometrika},
  pages =         {113--124},
  title =         {Inference for imputation estimators},
  volume =        {87},
  year =          {2000},
}

@techreport{Bhattacharya&Vogt07,
  author =        {Bhattacharya, J. and Vogt, W.},
  institution =          {National Bureau of
                   Economic Research},
  number={343},
  title =         {Do Instrumental Variables Belong in Propensity
                   Scores?},
  year =          {2007},
}

@techreport{Wooldridge09,
  author =        {Wooldridge, J.},
  institution={Michigan State University},
  type={Technical {R}eport},
  title =         {Should Instrumental Variables be Used as Matching
                   Variables?},
  year =          {2009},
}

@article{Pearl10,
  author =        {Pearl, J.},
  journal =       {Proceedings of Uncertainty in Artificial Intelligence},
  title =         {On a Class of Bias-Amplifying Variables that Endanger
                   Effect Estimates},
  year =          {2010},
}

@article{Holland86,
  author =        {Holland, P.W.},
  journal =       {J Am Stat Assoc},
  number =        {396},
  pages =         {945--960},
  title =         {Statistics and Causal Inference},
  volume =        {81},
  year =          {1986},
}

@book{Rubin06,
  address =       {Cambridge, MA},
  author =        {Donald B. Rubin},
  publisher =     {Cambridge},
  title =         {Matched sampling for causal effects.},
  year =          {2006},
}

@book{Rosenbaum02,
  address={Berlin Heidelberg New York},
  author =        {Rosenbaum, P.R.},
  edition =       {2nd},
  publisher =     {Springer},
  title =         {Observational studies},
  year =          {2002},
}

@article{Rubin97,
  author =        {Rubin, Donald B.},
  journal =       {Ann of Intern Med},
  number =        {8S},
  pages =         {757--763},
  title =         {Estimating causal effects from large data sets using
                   propensity scores},
  volume =        {127},
  year =          {1997},
}

@article{Christakis&Iwashyna03,
  author =        {Christakis, N.A. and Iwashyna, T.I.},
  journal =       {Soc Sci Med},
  number =        {3},
  pages =         {465--475},
  title =         {The Health Impact of Health Care on Families: a
                   matched cohort study of hospice use by decedents and
                   mortality outcomes in surviving, widowed spouses},
  volume =        {57},
  year =          {2003},
}

@article{Dehejia&Wahba02,
  author =        {R. Dehejia and S. Wahba},
  journal =       {Rev Econ Stat},
  number =        {1},
  pages =         {151--161},
  title =         {Propensity Score Matching Methods for Nonexperimental
                   Causal Studies},
  volume =        {84},
  year =          {2002},
}

@article{Galiani&Gertler&Schargrodsky05,
  author =        {Galiani, S. and P. Gertler and E. Schargrodsky},
  journal =       {J Polit Econ},
  number =        {1},
  pages =         {83--120},
  title =         {Water for Life: the Impact of the Privatization of
                   Water Services on Child Mortality},
  volume =        {113},
  year =          {2005},
}

@article{Abadie&Imbens06,
  author =        {Abadie, A. and G.W. Imbens},
  journal =       {Econometrica},
  pages =         {235--267},
  title =         {Large Sample Properties of Matching Estimators for
                   Average Treatment Effects},
  volume =        {74},
  year =          {2006},
}

@article{Herron&Wand07,
  author =        {Herron, M.C. and J. Wand},
  journal =       {Elect Stud},
  number =        {2},
  pages =         {247--261},
  title =         {Assessing Partisan Bias in Voting Technology: the
                   Case of the 2004 {N}ew {H}ampshire Recount},
  volume =        {26},
  year =          {2007},
}

@article{Imai05,
  author =        {K. Imai},
  journal =       {Am Polit Sci Rev},
  number =        {2},
  pages =         {283--300},
  title =         {Do Get-Out-The-Vote Calls Reduce Turnout? The
                   Importance of Statistical Methods for Field
                   Experiments},
  volume =        {99},
  year =          {2005},
}

@incollection{Sekhon08b,
  address =       {New York},
  author =        {Sekhon, J.S.},
  booktitle =     {The Oxford handbook of political methodology},
  editor =        {J.M. Box-Steffensmeier and H.E. Brady and
                   D. Collier},
  publisher =     {Oxford},
  title =         {The {N}eyman-{R}ubin Model of Causal Inference and
                   Estimation via Matching Methods},
  year =          {2008},
}

@article{Morgan&Harding06,
  author =        {Morgan, S.L. and D.J. Harding},
  journal =       {Sociol Meth Res},
  number =        {1},
  pages =         {3--60},
  title =         {Matching Estimators of Causal Effects: prospects and
                   Pitfalls in Theory and Practice},
  volume =        {35},
  year =          {2006},
}

@article{Diprete&Engelhardt04,
  author =        {Diprete, T.A. and H. Engelhardt},
  journal =       {Sociol Meth Res},
  number =        {4},
  pages =         {501--528},
  title =         {Estimating Causal Effects With Matching Methods in
                   the Presence and Absence of Bias Cancellation},
  volume =        {32},
  year =          {2004},
}

@article{Winship&Morgan99,
  author =        {Winship, C. and S.L. Morgan},
  journal =       {Annu Rev Sociol},
  pages =         {659--707},
  title =         {The estimation of causal effects from observational
                   data},
  volume =        {25},
  year =          {1999},
}

@article{Smith97,
  author =        {Smith, H.L.},
  journal =       {Sociol Meth},
  pages =         {305--353},
  title =         {Matching with Multiple Controls to Estimate Treatment
                   Effects in Observational Studies},
  volume =        {27},
  year =          {1997},
}

@article{Rubin02,
  author =        {Rubin, Donald B.},
  journal =       {Health Serv Outcome Res Meth},
  number =        {1},
  pages =         {169--188},
  title =         {Using Propensity Scores to Help Design Observational
                   Studies: application to the Tobacco Litigation},
  volume =        {2},
  year =          {2002},
}

@incollection{Brady08,
  address =       {New York},
  author =        {Brady, H.},
  booktitle =     {The Oxford handbook of political methodology},
  editor =        {J.M. Box-Steffensmeier and H.E. Brady and
                   D. Collier},
  publisher =     {Oxford},
  title =         {Causation and explanation in social science},
  year =          {2008},
}

@article{Freedman06,
  author =        {Freedman, D.A.},
  journal =       {Eval Rev},
  pages =         {691--713},
  title =         {Statistical Models for Causation: what Inferential
                   leverage Do They Provide?},
  volume =        {30},
  year =          {2006},
}

@article{Rubin90,
  author =        {Rubin, Donald B.},
  journal =       {Stat Sci},
  number =        {4},
  pages =         {472--480},
  title =         {Comment: {N}eyman (1923) and Causal Inference in
                   Experiments and Observational Studies},
  volume =        {5},
  year =          {1990},
}

@article{Speed90,
  author =        {T.P. Speed},
  journal =       {Stat Sci},
  number =        {4},
  pages =         {463--464},
  title =         {Introductory Remarks on {N}eyman (1923)},
  volume =        {5},
  year =          {1990},
}

@book{Cox58,
  address =       {New York},
  author =        {Cox, D.R.},
  publisher =     {Wiley},
  title =         {Planning of experiments},
  year =          {1958},
}

@article{Rubin78,
  author =        {Donald B. Rubin},
  journal =       {Ann Stat},
  number =        {},
  pages =         {34--58},
  title =         {Bayesian Inference for causal effects: the role of
                   randomization},
  volume =        {6},
  year =          {1978},
}

@incollection{Rubin75,
  address =       {Alexandria},
  author =        {Rubin, Donald B.},
  booktitle =     {The proceedings of the Social Statistics Section of
                   the American Statistical Association},
  publisher =     {American Statistical Association},
  title =         {Bayesian Inference for Causality: the Importance of
                   Randomization},
  year =          {1975},
}

@article{Rubin08,
  author =        {Rubin, Donald B.},
  journal =       {Ann of Appl Stat},
  number =        {3},
  pages =         {808--840},
  title =         {For Objective Causal Inference, Design Trumps
                   Analysis},
  volume =        {2},
  year =          {2008},
}

@article{Sekhon10,
  author =        {Sekhon, J.S.},
  journal =       {Annu Rev of Polit Sci},
  pages =         {487--508},
  title =         {Opiates for the Matches: matching Methods for Causal
                   Inference},
  volume =        {12},
  year =          {2010},
}

@article{Rubin76,
  author =        {Rubin, Donald B.},
  journal =       {Biometrics},
  number =        {1},
  pages =         {121--132},
  title =         {Multivariate Matching Methods That are Equal Percent
                   Bias Reducing, {II}: maximums on Bias Reduction for
                   Fixed Sample Sizes},
  volume =        {32},
  year =          {1976},
}

@article{Cochran&Rubin73,
  author =        {Cochran, W.G. and Donald B. Rubin},
  journal =       {Sankhya Ser A},
  pages =         {417--446},
  title =         {Controlling Bias in Observational Studies: a Review},
  volume =        {35},
  year =          {1973},
}

@book{Cochran83,
  address =       {New York},
  author =        {Cochran, W.G.},
  note =          {Edited posthumously by L.E. Moses and F. Mosteller},
  publisher =     {Wiley},
  title =         {Planning and analysis of observational studies},
  year =          {1983},
}

@article{Robinsetal07,
  author =        {J.M. Robins and M. Sued and Q. Lei-Gomez and
                   A. Rotnitzky},
  journal =       {Stat Sci},
  pages =         {544--559},
  title =         {Comment: {P}erformance of Double-Robust Estimators When
                   ``Inverse Probability'' Weights Are Highly Variable},
  volume =        {22},
  year =          {2007},
}

@article{Cortes&Vapnik95,
  author =        {C. Cortes and V. Vapnik},
  journal =       {Mach Learn},
  month =         {December},
  pages =         {273--297},
  title =         {Support-vector networks},
  volume =        {20},
  year =          {1995},
}

@techreport{Friedman94,
  author =        {J.H. Friedman},
  institution =   {Department of Statistics, Stanford University},
  type={Technical {R}eport},
  title =         {Flexible metric nearest neighbor classification},
  year =          {1994},
}

@techreport{FDA06,
  author =        {{Food and Drug Administration}},
  institution =   {U.S. Department of Health and Human Services, Food
                   and Drug Administration},
  type={Technical {R}eport},
  title =         {Critical Path Opportunities List},
  year =          {2006},
}

@article{Efronetal04,
  author =        {B. Efron and T. Hastie and I. Johnstone and
                   R. Tibshirani},
  journal =       {Ann Stat (with discussion)},
  number =        {2},
  pages =         {407--499},
  title =         {Least Angle Regression},
  volume =        {32},
  year =          {2004},
}

@techreport{Breiman99,
  author =        {L. Breiman},
  institution =   {Department of Statistics, University of California, Berkeley},
  number =        {567},
  title =         {Random forests - random features},
  year =          {1999},
}

@manual{Breiman01b,
  author =        {L. Breiman},
  title =         {Notes on setting up, using, and understanding random
                   forests V3.0},
  year =          {2001},
}

@article{Golubetal99,
  author =        {T.R. Golub and D.K. Slonim and P. Tamayo and C. Huard and
                   M. Gaasenbeek and J.P. Mesirov and H. Coller and
                   M.L. Loh and J.R. Downing and M.A. Caligiuri and
                   C.D. Bloomfield and E.S. Lander},
  journal =       {Science},
  pages =         {531--537},
  title =         {Molecular classification of cancer: class discovery
                   and class prediction by gene expression monitoring},
  volume =        {286},
  year =          {1999},
}

@article{vanderLaan06a,
  author =        {M.J. van der Laan},
  journal =       {Int J Biostat},
  number =        {1},
  pages =         {Article 2},
  title =         {Statistical Inference for Variable Importance},
  volume =        {2},
  year =          {2006},
}

@article{Robins&Mark&Newey92,
  author =        {J.M. Robins and S.D. Mark and W.K. Newey},
  journal =       {Biometrics},
  number =        {479--495},
  title =         {Estimating exposure effects by modelling the
                   expectation of exposure conditional on confounders},
  volume =        {48},
  year =          {1992},
}

@techreport{Yu&VanderLaan03,
  author =        {Z. Yu and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number={136},
  title =         {Measuring treatment effects using semiparametric
                   models},
  year =          {2003},
}

@techreport{Tuglus&vanderLaan08,
  author =        {C. Tuglus and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
number={233},
  title =         {Targeted Methods for Biomarker Discovery, the Search
                   for a Standard},
  year =          {2008},
}

@book{Hastie&Tibshirani90,
  address =       {London},
  author =        {T.J. Hastie and R.J. Tibshirani},
  publisher =     {Chapman \& Hall},
  title =         {Generalized additive models},
  year =          {1990},
}

@misc{Efron&Hastie07,
  author =        {B. Efron and T. Hastie},
  howpublished =  {R package},
  title =         {lars},
  year =          {2007},
}

@article{Benjamini&Hochberg95,
  author =        {Y. Benjamini and Y. Hochberg},
  journal =       {J R Stat Soc Ser B},
  pages =         {289--300},
  title =         {Controlling the false discovery rate: a practical and
                   powerful approach to multiple testing},
  volume =        {57},
  year =          {1995},
}

@misc{Ge&Dudoit02,
  author =        {Y. Ge and S. Dudoit},
  howpublished =  {R package},
  title =         {Multiple Testing Procedures, multtest},
  year =          {2002},
  url =           {www.bioconductor.org},
}

@article{Tibshirani96,
  author =        {R. Tibshirani},
  journal =       {J R Stat Soc Ser B},
  number =        {1},
  pages =         {267--288},
  title =         {Regression shrinkage and selection via the lasso.},
  volume =        {58},
  year =          {1996},
}

@article{Tuglus&vanderLaan09,
  author =        {C. Tuglus and M.J. van der Laan},
  journal =       {Stat Appl Genet Mol},
  number =        {1},
  pages =         {Article 12},
  title =         {Modified {FDR} Controlling Procedure for Multi-Stage
                   Analyses},
  volume =        {8},
  year =          {2009},
}

@article{Dudoit&Fridlyand&Speed02,
  author =        {S. Dudoit and J. Fridlyand and T. P. Speed},
  journal =       {J Am Stat Assoc},
  number =        {457},
  pages =         {77--87},
  title =         {Comparison of Discrimination Methods for the
                   Classification of Tumors Using Gene Expression Data},
  volume =        {97},
  year =          {2002},
}

@article{Kos&Lah98,
  author =        {J. Kos and T.T. Lah},
  journal =       {Oncol Rep},
  number =        {6},
  pages =         {1349--61},
  title =         {Cysteine proteinases and their endogenous inhibitors:
                   target proteins for prognosis, diagnosis and therapy
                   in cancer (review)},
  volume =        {5},
  year =          {1998},
}

@article{Vitaleetal01,
  author =        {C. Vitale and C. Romagnani and A. Puccetti and
                   D. Olive and R. Costello and L. Chiossone and
                   A. Pitto and A. Bacigalupo and L. Moretta and
                   M.C. Mingari},
  journal =       {Proc Natl Acad Sci},
  pages =         {5764--5769},
  title =         {Surface expression and function of p75/{AIRM}-1 or {CD}33
                   in acute myeloid leukemias: engagement of {CD}33
                   induces apoptosis of leukemic cells},
  volume =        {98},
  year =          {2001},
}

@article{Clappieretal07,
  author =        {E. Clappier and W. Cuccuini and A. Kalota and
                   A. Crinquette and J.M. Cayuela and W.A. Dik and
                   A.W. Langerak and B. Montpellier and B. Nadel and
                   P. Walrafen and O. Delattre and A. Aurias and
                   T. Leblanc and H. Dombret and A.M. Gewirtz and
                   A. Baruchel and F. Sigaux and J. Soulier},
  journal =       {Blood},
  number =        {4},
  pages =         {1251--61},
  title =         {The {C-MYB} locus is involved in chromosomal
                   translocation and genomic duplications in human
                   T-cell acute leukemia ({T-ALL}), the translocation
                   defining a new {T-ALL} subtype in very young children},
  volume =        {110},
  year =          {2007},
}

@article{Lane&Ley03,
  author =        {A.A. Lane and T.J. Ley},
  journal =       {Cell},
  number =        {305-318},
  title =         {Neutrophil elastase cleaves {PML-RAR}-alpha and is
                   important for the development of acute promyelocytic
                   leukemia in mice},
  volume =        {115},
  year =          {2003},
}

@article{Hunger96,
  author =        {S.P. Hunger},
  journal =       {Blood},
  pages =         {1211--1224},
  title =         {Chromosomal translocations involving the {E2A} gene in
                   acute lymphoblastic leukemia: clinical features and
                   molecular pathogenesis.},
  volume =        {87},
  year =          {1996},
}

@article{Nebraletal05,
  author =        {K. Nebral and H.H. Schmidt and O.A. Haas and
                   S. Strehl},
  journal =       {Clin Cancer Res},
  number =        {18},
  pages =         {6489--6494},
  title =         {{NUP}98 Is Fused to Topoisomerase {(DNA)} {II}{beta} 180
                   {kDa} {(TOP2B)} in a Patient with Acute Myeloid Leukemia
                   with a New {t(3;11)(p24;p15)}},
  volume =        {11},
  year =          {2005},
}

@article{Kaufmannetal98b,
  author =        {S.H. Kaufmann and S.D. Gore and C.B. Miller and
                   R.J. Jones and L.A. Zwelling and E. Schneider and
                   P.J. Burke and J.E. Karp},
  journal =       {Leukemia Lymphoma},
  month =         {Apr},
  number =        {3-4},
  pages =         {217--237},
  title =         {Topoisomerase {II} and the response to antileukemic
                   therapy},
  volume =        {29},
  year =          {1998},
}

@article{Kozaretal04,
  author =        {K. Kozar and M.A. Ciemerych and V.I. Rebel and
                   H. Shigematsu and A. Zagozdzon and E. Sicinska and
                   Y. Geng and Q. Yu and S. Bhattacharya and
                   R.T. Bronson and K. Akashi and P. Sicinski},
  journal =       {Cell},
  pages =         {477--491},
  title =         {Mouse development and cell proliferation in the
                   absence of {D}-cyclins},
  volume =        {118},
  year =          {2004},
}

@article{MartinSuberoetal07,
  author =        {J.I. Martin-Subero and R. Ibbotson and W. Klapper and
                   L. Michaux and E. Callet-Bauchu and F. Berger and
                   M.J. Calasanz and C. De Wolf-Peeters and M.J. Dyer and
                   P. Felman and A. Gardiner and R.D. Gascoyne and
                   S. Gesk and L. Harder and D.E. Horsman and M. Kneba and
                   R. Kuppers and A. Majid and N. Parry-Jones and
                   M. Ritgen and M. Salido and F. Sole and G. Thiel and
                   H.H. Wacker and D. Oscier and I. Wlodarska and
                   R. Siebert},
  journal =       {Leukemia},
  number =        {7},
  pages =         {1532--1544},
  title =         {A comprehensive genetic and histopathologic analysis
                   identifies two subgroups of {B}-cell malignancies
                   carrying a t(14;19)(q32;q13) or variant
                   {BCL3}-translocation},
  volume =        {21},
  year =          {2007},
}

@article{Palomeroetal06,
  author =        {T. Palomero and D.T. Odom and J. O'Neil and
                   A.A. Ferrando and A. Margolin and D.S. Neuberg and
                   S.S. Winter and R.S. Larson and W. Li and X.S. Liu and
                   R.A. Young and A.T. Look},
  journal =       {Blood},
  number =        {3},
  pages =         {986--992},
  title =         {Transcriptional regulatory networks downstream of
                   {TAL1/SCL} in {T}-cell acute lymphoblastic leukemia},
  volume =        {108},
  year =          {2006},
}

@article{Wongetal07,
  author =        {H.P. Wong and L. Yu and E.K. Lam and E.K. Tai and
                   W.K. Wu and C.H. Cho},
  journal =       {Toxicol Appl Pharm},
  number =        {3},
  pages =         {261--267},
  title =         {Nicotine promotes cell proliferation via
                   alpha7-nicotinic acetylcholine receptor and
                   catecholamine-synthesizing enzymes-mediated pathway
                   in human colon adenocarcinoma {HT}-29 cells.},
  volume =        {221},
  year =          {2007},
}

@article{Ramaswamyetal03,
  author =        {S. Ramaswamy and K.N. Ross and E.S. Lander and
                   T.R. Golub},
  journal =       {Nat Genet},
  pages =         {49--54},
  title =         {A molecular signature of metastasis in primary solid
                   tumors},
  volume =        {33},
  year =          {2003},
}

@article{Purietal01,
  author =        {R. Puri and A. Tousson and L. Chen and S.S. Kakar},
  journal =       {Cancer Lett},
  pages =         {131--139},
  title =         {Molecular cloning of pituitary tumor transforming
                   gene 1 from ovarian tumors and its expression in
                   tumors},
  volume =        {163},
  year =          {2001},
}

@article{Fujiietal06,
  author =        {T. Fujii and S. Nomoto and K. Koshikawa and Y.Yatabe and
                   O. Teshigawara and T. Mori and S. Inoue and S. Takeda and
                   A. Nakao},
  journal =       {Hepatology},
  pages =         {1267--1275},
  title =         {Overexpression of pituitary tumor transforming gene 1
                   in {HCC} is associated with angiogenesis and poor
                   prognosis},
  volume =        {43},
  year =          {2006},
}

@article{Zhuetal06,
  author =        {X. Zhu and Z. Mao and Y. Na and Y. Guo and X. Wang and
                   D. Xin},
  journal =       {Anticancer Res},
  pages =         {1253--1259},
  title =         {Significance of pituitary tumor transforming gene 1
                   ({PTTG1}) in prostate cancer},
  volume =        {26},
  year =          {2006},
}

@article{Kaufmannetal98a,
  author =        {S.H. Kaufmann and J.E. Karp and P.A. Svingen and
                   S. Krajewski and P.J. Burke and S.D. Gore and
                   J.C. Reed},
  journal =       {Blood},
  number =        {3},
  pages =         {991--1000},
  title =         {Elevated expression of the apoptotic regulator {Mcl}-1
                   at the time of leukemic relapse},
  volume =        {91},
  year =          {1998},
}

@article{Frumanetal99,
  author =        {D.A. Fruman and S.B. Snapper and C.M. Yballe and
                   L. Davidson and J.Y. Yu and F.W. Alt and
                   L.C. Cantley},
  journal =       {Science},
  pages =         {393--397},
  title =         {Impaired {B} cell development and proliferation in
                   absence of phosphoinositide 3-kinase p85-alpha},
  volume =        {283},
  year =          {1999},
}

@article{Tombes&Krystal97,
  author =        {R.M. Tombes and G.W. Krystal},
  journal =       {Biochim Biophys Acta},
  pages =         {281--292},
  title =         {Identification of novel human tumor cell-specific
                   {CaMK-II} variants},
  volume =        {1355},
  year =          {1997},
}

@article{Senturkeretal97,
  author =        {S. Senturker and B. Karahalil and M. Inal and
                   H. Yilmaz and H. Muslumanoglu and G. Gedikoglu and
                   M. Dizdaroglu},
  journal =       {FEBS Letters},
  number =        {3},
  pages =         {286--290},
  title =         {Oxidative {DNA} base damage and antioxidant enzyme
                   levels in childhood acute lymphoblastic leukemia},
  volume =        {416},
  year =          {1997},
}

@article{Komuroetal05,
  author =        {I. Komuro and T. Yasuda and A. Iwamoto and
                   K.S. Akagawa},
  journal =       {J Biol Chem},
  number =        {50},
  pages =         {41137--45},
  title =         {Catalase plays a critical role in the {CSF}-independent
                   survival of human macrophages via regulation of the
                   expression of {BCL}-2 family},
  volume =        {280},
  year =          {2005},
}

@article{Balciunaiteetal05,
  author =        {E. Balciunaite and A. Spektor and N.H. Lents and
                   H. Cam and H. Te Riele and A. Scime and M.A. Rudnicki and
                   R. Young and B.D. Dynlacht},
  journal =       {Mol Cell Biol},
  number =        {18},
  pages =         {8166--78},
  title =         {Pocket protein complexes are recruited to distinct
                   targets in quiescent and proliferating cells},
  volume =        {25},
  year =          {2005},
}

@article{Leoneetal01,
  author =        {G. Leone and R. Sears and E. Huang and R. Rempel and
                   F. Nuckolls and C.H. Park and P. Giangrande and L. Wu and
                   H.I. Saavedra and S.J. Field and M.A. Thompson and
                   H. Yang and Y. Fujiwara and M.E. Greenberg and
                   S. Orkin and C. Smith and J.R. Nevins},
  journal =       {Mol Cell},
  pages =         {105--113},
  title =         {Myc requires distinct {E2F} activities to induce {S}
                   phase and apoptosis},
  volume =        {8},
  year =          {2001},
}

@article{Sax23,
  author =        {Sax, K.},
  journal =       {Genetics},
  title =         {The association of size difference with seed-coat
                   pattern and pigmentation in \textit{Phaseolus
                   vulgaris}},
  year =          {1923},
}

@article{Thoday60,
  author =        {Thoday, J.M.},
  journal =       {Nature},
  title =         {Location of polygenes},
  year =          {1960},
}

@article{Lander&Botstein89,
  author =        {Lander, E.S. and Botstein, D.},
  journal =       {Genetics},
  title =         {Mapping {M}endelian factors underlying quantitative
                   traits using {RFLP} linkage maps},
  year =          {1989},
}

@article{Haley&Knott92,
  author =        {Haley, C.S. and Knott, S.A.},
  journal =       {Heredity},
  title =         {A simple regression method for mapping quantitative
                   trait loci in line crosses using flanking markers},
  year =          {1992},
}

@article{Jansen93,
  author =        {Jansen, R.C.},
  journal =       {Genetics},
  title =         {Interval mapping of multiple quantitative trait loci},
  year =          {1993},
}

@article{Zeng94,
  author =        {Zeng, Z.B.},
  journal =       {Genetics},
  title =         {Precision mapping of quantitative trait loci},
  year =          {1994},
}

@article{Kao&Zeng&Teasdale99,
  author =        {Kao, C.H. and Zeng, Z.B. and Teasdale, R.D.},
  journal =       {Genetics},
  title =         {Multiple interval mapping for quantitative trait
                   loci},
  year =          {1999},
}

@article{Satagopanetal96,
  author =        {Satagopan, J.M. and B.S. Yandell and M.A. Newton and
                   T.C. Osborn},
  journal =       {Genetics},
  title =         {A {B}ayesian approach to detect quantitative trait loci
                   using {M}arkov chain {M}onte {C}arlo},
  year =          {1996},
}

@article{Heath97,
  author =        {Heath, S.C.},
  journal =       {Am J Hum Genet},
  title =         {Markov chain {M}onte {C}arlo segregation and linkage
                   analysis of oligogenic models},
  year =          {1997},
}

@article{Sillanpaa&Arjas98,
  author =        {Sillanpaa, M.J. and Arjas, E.},
  journal =       {Genetics},
  title =         {Bayesian mapping of multiple quantitative trait loci
                   from incomplete inbred line cross data},
  year =          {1998},
}

@article{Leeetal08,
  author =        {Lee, S.S.F. and L. Sun and R. Kustra and S.B. Bull},
  journal =       {Bioinformatics},
  title =         {{EM}-random forest and new measures of variable
                   importance for multi-locus quantitative trait linkage
                   analysis},
  year =          {2008},
}

@article{Wang&Rose&vanderLaan10,
  author =        {H. Wang and S. Rose and M.J. van der Laan},
  journal =       {Stat Prob Lett},
  title =         {Finding quantitative Trait Loci Genes with
                   Collaborative Targeted Maximum Likelihood Learning},
  volume =        {published online 11 Nov (doi:
                   10.1016/j.spl.2010.11.001)},
  year =          {2010},
}

@techreport{Wang&Rose&vanderLaan11,
  author =        {H. Wang and S. Rose and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  type =          {Technical {R}eport},
  title =         {Targeted Methods for Finding Quantitative Trait Loci},
  year =          {2011},
}

@manual{Basten&Weir&Zeng01,
  author =        {C.J. Basten and B.S. Weir and Z.B. Zeng},
  title =         {QTL Cartographer},
  year =          {2001},
  url =           {http://statgen.ncsu.edu/qtlcart/},
}

@article{Masindeetal01,
  author =        {Masinde, G.L. and X. Li and W. Gu and H. Davidson and
                   S. Mohan and D.J. Baylink},
  journal =       {Genome Res},
  title =         {Identification of wound healing/regeneration
                   quantitative trait loci ({QTL}) at multiple time points
                   that explain seventy percent of variance in ({MRL/MpJ
                   and SJL/J}) mice {F2} population},
  year =          {2001},
}

@article{Boyartchuk01,
  author =        {Boyartchuk, V.L. and K.W. Broman and R.E. Mosher and
                   S.E.F. D'Orazio and M.N. Starnbach and W.F. Dietrich},
  journal =       {Nat Genet},
  title =         {Multigenic control of Listeria monocytogenes
                   susceptibility in mice},
  year =          {2001},
}

@article{Broman03,
  author =        {Broman, K.W.},
  journal =       {Genetics},
  title =         {Mapping quantitative trait loci in the case of a
                   spike in the phenotype distribution},
  year =          {2003},
}

@article{Jin&Fine&Yandell07,
  author =        {Jin, C. and J.P. Fine and B.S. Yandell},
  journal =       {J Am Stat Assoc},
  title =         {A unified semiparametric framework for quantitative
                   trait loci analysis, with application to spike
                   phenotypes},
  year =          {2007},
}

@article{Petersenetal08,
  author =        {M.L. Petersen and M.J. van der Laan and S. Napravnik and
                   J.J. Eron and R.D. Moore and S.G. Deeks},
  journal =       {AIDS},
  number =        {16},
  pages =         {2097--106},
  title =         {Long-term consequences of the delay between virologic
                   failure of highly active antiretroviral therapy and
                   regimen modification},
  volume =        {22},
  year =          {2008},
}

@article{Rodgeretal09,
  author =        {A.J. Rodger and Z. Fox and J.D. Lundgren and
                   J.L. Kuller and C. Boesecke and D. Gey and
                   A. Skoutelis and M.B. Goetz and A.N. Phillips and
                     {INSIGHT Strategies for Management of Antiretroviral
  Therapy (SMART) Study Group}},
  journal =       {J Infect Dis},
  number =        {6},
  pages =         {973--83},
  title =         {Activation and coagulation biomarkers are independent
                   predictors of the development of opportunistic
                   disease in patients with {HIV} infection.},
  volume =        {200},
  year =          {2009},
}

@article{Hammeretal08,
  author =        {S.M. Hammer and J.J. Eron and P. Reiss and
                   R.T. Schooley and M.A. Thompson and S. Walmsley and
                   P. Cahn and M.A. Fischl and J.M. Gatell and
                   M.S. Hirsch and D.M. Jacobsen and J.S.G. Montaner and
                   D.D. Richman and P.G. Yeni and P.A. Volberding},
  journal =       {J Am Med Asoc},
  number =        {5},
  pages =         {555--70},
  title =         {Antiretroviral treatment of adult {HIV} infection:
                   2008 recommendations of the {I}nternational {AIDS}
                   {S}ociety-{USA} panel},
  volume =        {300},
  year =          {2008},
}

@article{Stringeretal06,
  author =        {J.S. Stringer and I. Zulu and J. Levy and
                   E.M. Stringer and A. Mwango and B.H. Chi and
                   V. Mtonga and S. Reid and R.A. Cantrell and
                   M. Bulterys and M.S. Saag and R.G. Marlink and
                   A. Mwinga and T.V. Ellerbrock and M. Sinkala},
  journal =       {J Am Med Asoc},
  number =        {7},
  pages =         {782--93},
  title =         {Rapid scale-up of antiretroviral therapy at primary
                   care sites in {Z}ambia: feasibility and early outcomes},
  volume =        {296},
  year =          {2006},
}

@misc{WHO06,
  author =        {{{W}orld {H}ealth {O}rganization}},
  title =         {Antiretroviral therapy for {HIV} infection in adults
                   and adoloescents: recommendations for a public health
                   approach},
  year =          {2006},
}

@article{Reynoldsetal09,
  author =        {S.J. Reynolds and G. Nakigozi and K. Newell and
                   A. Ndyanabo and R. Galiwongo and I. Boaz and
                   T.C. Quinn and R. Gray and M. Wawer and D. Serwadda},
  journal =       {{AIDS}},
  number =        {6},
  pages =         {697--700},
  title =         {Failure of immunologic criteria to appropriately
                   identify antiretroviral treatment failure in {U}ganda},
  volume =        {23},
  year =          {2009},
}

@article{Petersenetal07,
  author =        {M.L Petersen and S.G. Deeks and J.N. Martin and
                   M.J. van der Laan},
  journal =       {Am J Epidemiol},
  number =        {9},
  pages =         {985--993},
  title =         {History-Adjusted Marginal Structural Models to
                   Estimate Time-Varying Effect Modification},
  volume =        {166},
  year =          {2007},
}

@article{Robins&Hernan&Rotnitzky07,
  author =        {J.M. Robins and M.A. Hernan and A. Rotnitzky},
  journal =       {Am J Epidemiol},
  number =        {9},
  pages =         {994--1002},
  title =         {Effect Modification by Time-varying Covariates},
  volume =        {166},
  year =          {2007},
}

@article{vanderLaan&Petersen&Joffe07,
  author =        {M.J. van der Laan and M.L. Petersen and M.M. Joffe},
  journal =       {Am J Epidemiol},
  number =        {9},
  pages =         {1003--1004},
  title =         {Response to Invited Commentary: {P}etersen et. al.
                   Respond to ``{E}ffect Modification by Time-varying
                   Covariates''},
  volume =        {166},
  year =          {2007},
}

@article{vanderLaan&Petersen07b,
  author =        {M.J. van der Laan and M.L. Petersen},
  journal =       {Int J Biostat},
  number =        {1},
  pages =         {Article 6},
  title =         {Statistical Learning of Origin-Specific Statically
                   Optimal Individualized Treatment Rules.},
  volume =        {3},
  year =          {2007},
}

@article{Petersen&Deeks&vanderLaan07,
  author =        {M.L. Petersen and S.G. Deeks and M.J. van der Laan},
  journal =       {Stat Med},
  number =        {25},
  pages =         {4578--601},
  title =         {Individualized Treatment Rules: generating Candidate
                   Clinical Trials.},
  volume =        {26},
  year =          {2007},
}

@article{vanderLaan&Petersen&Joffe05,
  author =        {M.J. van der Laan and M.L. Petersen and M.M. Joffe},
  journal =       {Int J Biostat},
  number =        {1},
  pages =         {10--20},
  title =         {History-Adjusted Marginal Structural Models and
                   Statically-Optimal Dynamic Treatment Regimens},
  volume =        {1},
  year =          {2005},
}

@article{Hernanetal06,
  author =        {M.A. Hernan and E. Lanoy and D. Costagliola and
                   J.M. Robins},
  journal =       {Basic Clin Pharmacol},
  pages =         {237--242},
  title =         {Comparison of dynamic treatment regimes via inverse
                   probability weighting.},
  volume =        {98},
  year =          {2006},
}

@techreport{vanderLaan08b,
  author =        {M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =          {232},
  title =         {The construction and analysis of adaptive group
                   sequential designs},
  year =          {2008},
}

@article{Boivinetal07,
  author =        {Boivin, J. and Bunting, L. and Collins, J.A. and
                   Nygren, K.G.},
  journal =       {Hum Reproduct},
  pages =        {1506--1512},
  title =         {International estimates of infertility prevalence and
                   treatment-seeking: potential need and demand for
                   infertility medical care},
  volume =        {22},
  year =          {2007},
}

@article{Adamsonetal06,
  author =        {Adamson, G.D. and de {M}ouzon, J. and Lancaster, P. and
                   Nygren, K.-G. and Sullivan, E. and
                   Zegers-Hochschild, F.},
  journal =       {Fertil Steril},
  pages =        {1586--1622},
  title =         {World collaborative report on in vitro fertilization,
                   2000},
  volume =        {85},
  year =          {2006},
}

@article{Soullieretal08,
  author =        {Soullier, N. and Bouyer, J. and Pouly J-L. and
                   Guibert, J. and de la {R}ochebrochard},
  journal =       {Hum Reproduct},
  pages =         {187--192},
  title =         {Estimating the success of an in vitro fertilization
                   programme using multiple imputation},
  volume =        {23},
  year =          {2008},
}

@article{delaRochebrochardetal08,
  author =        {de la {R}ochebrochard, E. and Soullier, N. and
                   Peikrishvili, R. and Guibert, J. and Bouyer, J.},
  journal =       {Int J Gynecol Obstet},
  pages =         {74--75},
  title =         {High in vitro fertilization discontinuation rate in
                   {F}rance},
  volume =        {103},
  year =          {2008},
}

@article{delaRochebrochardetal09,
  author =        {de la {R}ochebrochard, E. and Quelen, C. and
                   Peikrishvili, R. and Guibert, J. and Bouyer, J.},
  journal =       {Fertil Steril},
  pages =         {149--156},
  title =         {Long-term outcome of parenthood project during in
                   vitro fertilization and after discontinuation of
                   unscuccessful in vitro fertilization},
  volume =        {92},
  year =          {2009},
}

@book{Schafer97,
  address =       {London},
  author =        {Schafer, J.L.},
  publisher =     {Chapman \& Hall},
  title =         {Analysis of incomplete multivariate data},
  year =          {1997},
}

@book{Little&Rubin02,
  address =       {Hoboken},
  author =        {Little, R.J.A. and Rubin, Donald B.},
  edition =       {2nd},
  publisher =     {Wiley},
  title =         {Statistical analysis with missing data},
  year =          {2002},
}

@techreport{Yu&vanderLaan02,
  author =        {Z. Yu and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number={122},
  title =         {Construction of counterfactuals and the
                   G-computation formula},
  year =          {2002},
}

@article{Gill&Robins01,
  author =        {Gill, R.D. and Robins, J.M.},
  journal =       {Ann Stat},
  number =        {6},
  pages =         {1785--1811},
  title =         {Causal inference in complex longitudinal studies:
                   continuous case},
  volume =        {29},
  year =          {2001},
}

@techreport{DHHS04,
  author =        {{Department of Health and Human Services}},
  institution =   {Panel on Clinical Practices for Treatment of {HIV}
                   Infection},
type={Technical {R}eport},
  title =         {Guidelines for the use of antiretroviral agents in
                   {HIV}-1 infected adults and adolescents},
  year =          {2004},
}

@article{CDC92,
  author =        {{Centers for Disease Control and Prevention}},
  journal =       {Morbid Mortal W Rep},
  pages =         {1--19},
  title =         {{1993 revised classification system for {HIV} infection
                   and expanded surveillance case definition for AIDS
                   among adolescents and adults}},
  volume =        {41},
  year =          {1992},
}

@incollection{Selbyetal05,
  author =        {J.V. Selby and D.H. Smith and E.S. Johnson and
                   M.A. Raebel and G.D. Friedman and B.H. McFarland},
  booktitle =     {Pharmacoepidemiology},
  editor =        {B.L. Strom},
  publisher =     {Wiley},
  title =         {Kaiser {P}ermanente Medical Care Program},
  year =          {2005},
}

@techreport{Neugebauer&Silverberg&vanderLaan10,
  author =        {R. Neugebauer and M.J. Silverberg and
                   M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  type =          {272},
  title =         {Observational Study and Individualized Antiretroviral
                   Therapy Initiation Rules for Reducing Cancer
                   Incidence in {HIV}-Infected Patients},
  year =          {2010},
}




@techreport{Stitelmanetal11,
  author =        {O.M. Stitelman and V. De Gruttola and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  type =          {Technical {R}eport 281, http://www.bepress.com/ucbbiostat/paper281},
  title =         {A General Implementation of TMLE for Longitudinal Data Applied to Causal Inference in Survival Analysis},
  year =          {2011},
}
@techreport{Stitelman&vanderLaan11,
  author =        {O.M. Stitelman and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  type =          {Technical {R}eport},
  title =         {Targeted Maximum Likelihood Estimation of
                   Time-To-Event Parameters With Time-Dependent
                   Covariates},
  year =          {2011},
}

@article{Thalletal07,
  author =        {P.F. Thall and C. Logothetis and L.C. Pagliaro and
                   S. Wen and M.A. Brown and D. Williams and
                   R.E. Millikan},
  journal =       {J Natl Cancer Inst},
  pages =         {1613--22},
  title =         {Adaptive Therapy for Androgen-Independent Prostate
                   Cancer: a randomized Selection Trial of Four
                   Regimens},
  volume =        {99},
  year =          {2007},
}

@article{Bembom&vanderLaan07a,
  author =        {O. Bembom and M.J. van der Laan},
  journal =       {J Natl Cancer Inst},
  pages =         {1577--1582},
  title =         {Comment: Statistical Methods for analyzing sequentially
                   randomized trials},
  volume =        {99(21)},
  year =          {2007},
}

@techreport{Zheng&vanderLaan10,
  author =        {W. Zheng and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =          {273},
  title =         {Asymptotic Theory for Cross-validated Targeted
                   Maximum Likelihood Estimation},
  year =          {2010},
}

@techreport{Zheng&vanderLaan11,
  author =        {W. Zheng and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =          {288},
  title =         {Targeted Maximum Likelihood Estimation of Natural Direct Effect},
  year =          {2011},
}

@book{Robert07,
  address={Berlin Heidelberg New York},
  author =        {Robert, P.C.},
  publisher =     {Springer},
  title =         {{T}he {B}ayesian choice: from
                   decision-thoeretic foundations to
                   computational implementation},
  year =          {2007},
}

@book{Lindley80,
  address =       {Cambridge, MA},
  author =        {Lindley, D.V.},
  publisher =     {Cambridge},
  title =         {{I}ntroduction to probability and statistics from
                   a {B}ayesian point of view, {P}art 2},
  year =          {1980},
}

@article{Golub06,
  author =        {Golub, H.L.},
  journal =       {Stat Med},
  pages =         {3231--3235},
  title =         {The need for more efficient trial designs},
  volume =        {25},
  year =          {2006},
}

@article{Emerson06,
  author =        {Emerson, S.S.},
  journal =       {Stat Med},
  pages =         {3270--3296},
  title =         {Issues in the use of adaptive clinical trial designs},
  volume =        {25},
  year =          {2006},
}

@book{Hu&Rosenberger06,
address = {New York},
  author =        {F. Hu and W.F. Rosenberger},
  publisher =     {Wiley},
  title =         {The theory of response adaptive randomization in
                   clinical trials},
  year =          {2006},
}

@book{Jennison&Turnbull00,
  address =       {Boca Raton},
  author =        {Jennison, C. and Turnbull, B.W.},
  editor =        {},
  publisher =     {Chapman \& Hall},
  title =         {Group sequential methods with applications to
                   clinical trials},
  year =          {2000},
}

@article{Rosenberger96,
  author =        {W.F. Rosenberger},
  journal =       {Stat Sci},
  number =        {},
  pages =         {137--149},
  title =         {New directions in adaptive designs},
  volume =        {11},
  year =          {1996},
}

@techreport{Chambaz&vanderLaan10,
  author =        {Chambaz, A. and van der Laan, M.J.},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
   number={258},
  title =         {Targeting the optimal design in randomized clinical
                   trials with binary outcomes and no covariate},
  year =          {2010},
}

@article{Rosenberger&Vidyashankar&Agarwal01,
  author =        {Rosenberger, W.F. and Vidyashankar, A.N. and
                   Agarwal, D.K.},
  journal =       {J Biopharm Stat},
  number =        {227--236},
  title =         {Covariate-adjusted response-adaptive designs for
                   binary response},
  volume =        {11},
  year =          {2001},
}

@article{Bandyopadhyay&Biswas01,
  author =        {Bandyopadhyay, U. and Biswas, A.},
  journal =       {Biometrika},
  number =        {2},
  pages =         {409--419},
  title =         {Adaptive designs for normal responses with prognostic
                   factors},
  volume =        {88},
  year =          {2001},
}

@article{Atkinson&Biswas05,
  author =        {Atkinson, A.C. and Biswas, A.},
  journal =       {Stat Med},
  number =        {16},
  pages =         {2477--2492},
  title =         {Adaptive biased-coin designs for skewing the
                   allocation proportion in clinical trials with normal
                   responses},
  volume =        {24},
  year =          {2005},
}

@article{Zhangetal07,
  author =        {Zhang, L.-X. and Hu, F.-F. and Cheung, S.H. and
                   Chan, W.S.},
  journal =       {Ann Stat},
  number =        {3},
  pages =         {1166--1182},
  title =         {Asymptotic properties of covariate-adjusted
                   response-adaptive designs},
  volume =        {35},
  year =          {2007},
}

@article{Zhang&Hu09,
  author =        {Zhang, L.-X. and Hu, F.-F.},
  journal =       {Appl Math J Chinese Univ Ser B},
  number =        {1},
  pages =         {1--13},
  title =         {A new family of covariate-adjusted response adaptive
                   designs and their properties},
  volume =        {24},
  year =          {2009},
}

@article{Shao&Yu&Zhong10,
  author =        {Shao, J. and Yu, X. and Bob Zhong, B.},
  journal =       {Biometrika},
  title =         {A theory for testing hypotheses under
                   covariate-adaptive randomization},
  year =          {2010},
}

@article{Gill89,
  author =        {Gill, R.D.},
  journal =       {Scand J Stat},
  title =         {Non- and semiparametric maximum likelihood estimators
                   and the Von {M}ises method (Part 1)},
 number={16},
 pages={97--128},
  year =          {1989},
}

@article{Tan08,
  author =        {Z. Tan},
  journal =       {Int J Biostat},
  pages =         {Article 10},
  title =         {Comment: {I}mproved Local Efficiency and Double
                   Robustness},
  volume =        {4},
  number={1},
  year =          {2008},
}

@techreport{Gruber&vanderLaan11,
  author =        {S. Gruber and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =        {275},
  type =          {Technical Report},
  title =         {{tmle}: an {R} Package for Targeted Maximum Likelihood
                   Estimation},
  year =          {2011},
}

@proceedings{DBLP:conf/colt/2003,
  booktitle =     {COLT},
  editor =        {B. Sch{\"o}lkopf and M.K. Warmuth},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  series =        {Lecture Notes in Computer Science},
  title =         {Computational Learning Theory and Kernel Machines,
                   16th Annual Conference on Computational Learning
                   Theory and 7th Kernel Workshop, COLT/Kernel 2003,
                   Washington, DC, USA, August 24-27, 2003, Proceedings},
  volume =        {2777},
  year =          {2003},
}

@proceedings{DBLP:conf/nips/2005,
  booktitle =     {NIPS},
  title =         {Advances in Neural Information Processing Systems 18
                   [Neural Information Processing Systems, NIPS 2005,
                   December 5-8, 2005, Vancouver, British Columbia,
                   Canada]},
  year =          {2005},
}

@proceedings{DBLP:conf/colt/2006,
  booktitle =     {COLT},
  editor =        {G. Lugosi and H.-U. Simon},
  publisher =     {Springer},
  series =        {Lecture Notes in Computer Science},
    address={Berlin Heidelberg New York},
  title =         {Learning Theory, 19th Annual Conference on Learning
                   Theory, COLT 2006, Pittsburgh, PA, USA, June 22-25,
                   2006, Proceedings},
  volume =        {4005},
  year =          {2006},
}

%% This BibTeX bibliography file was created using BibDesk.
%% http://bibdesk.sourceforge.net/


%% Created for Ivan Diaz at 2011-09-14 16:32:22 -0700


%% Saved with string encoding Unicode (UTF-8)

@article{Rubin76,
  title={Inference and missing data},
  author={Rubin, D.B.},
  journal={Biometrika},
  volume={63},
  number={3},
  pages={581--592},
  year={1976},
  publisher={Biometrika Trust}
}
    @article{Hernan2009,
     title = {Invited commentary: causal diagrams and measurement bias},
     author = {Hern\'an, M. A. and Cole, S. R.},
     journal = {American Journal of Epidemiology},
     volume = {170},
     number = {8},
     pages = {pp. 963-954},
     year = {2009},
    }

    @article{Scharfstein2002,
     title = {Estimation of the Failure Time Distribution in the Presence of Informative Censoring},
     author = {Scharfstein, D. O. and Robins, J. M.},
     journal = {Biometrika},
     volume = {89},
     number = {3},
     pages = {pp. 617-634},
     year = {2002},
     publisher = {Biometrika Trust},
     copyright = {Copyright © 2002 Biometrika Trust},
    }

@article{Rotnitzky2001,
author = {A. Rotnitzky and D. Scharfstein and Su, S. Ting-Li and J. Robins},
title = {Methods for Conducting Sensitivity Analysis of Trials with Potentially Nonignorable Competing Causes of Censoring},
journal = {Biometrics},
volume = {57},
number = {1},
publisher = {Blackwell Publishing Ltd},
issn = {1541-0420},
pages = {103--113},
keywords = {Attrition, Augmented inverse probability of censoring weighted estimation, Curse of dimensionality, Longitudinal data, Noncompliance, Pattern-mixture models, Selection bias, Selection models},
year = {2001},
}
@ARTICLE{Scharfstein1999,
    author = {D. O. Scharfstein and A. Rotnitzky and J. M. Robins},
    title = {Adjusting for Nonignorable Drop-out Using Semiparametric Non-response Models (with discussion)},
    journal = {Journal of the American Statistical Association},
    year = {1999},
    volume = {94},
    pages = {1096--1146}
}

@incollection{Robins1999,
  title={Sensitivity Analysis for Selection Bias and Unmeasured Confounding in Missing Data and Causal Inference Models},
  booktitle={Statistical Models in Epidemiology, the Environment and Clinical Trials},
  author={Robins, J. M. and Rotnitzky, A. and Scharfstein, D. O.},
  series={IMA Volumes in Mathematics and Its Applications},
  year={1999},
  publisher={Springer}
}


@article{Rotnitsky1998,
author = {Rotnitzky, Andrea and Robins, James M. and Scharfstein, Daniel O.},
title = {Semiparametric Regression for Repeated Outcomes with Nonignorable Nonresponse},
journal = {Journal of the American Statistical Association},
volume = {93},
number = {444},
pages = {1321-1339},
year = {1998},
}

@incollection {vanderLaan&Petersen2012,
   author = {van der Laan, Mark J. and Petersen, Maya L.},
   affiliation = {Division of Biostatistics, School of Public Health, University of California, Berkeley, CA, USA},
   title = {Targeted Learning},
   booktitle = {Ensemble Machine Learning},
   editor = {Zhang, Cha and Ma, Yunqian},
   publisher = {Springer US},
   isbn = {978-1-4419-9326-7},
   keyword = {Engineering},
   pages = {117-156},
   year = {2012}
}
@inproceedings{Didelezetal2006,
	Author = {Vanessa Didelez and A. Philip Dawid and Sara Geneletti},
	Bibsource = {DBLP, http://dblp.uni-trier.de},
	Booktitle = {UAI},
	Crossref = {DBLP:conf/uai/2006},
	Date-Added = {2012-04-19 19:44:15 -0700},
	Date-Modified = {2012-04-19 19:48:48 -0700},
	Title = {Direct and Indirect Effects of Sequential Treatments},
	Year = {2006},
	Bdsk-Url-1 = {http://uai.sis.pitt.edu/displayArticleDetails.jsp?mmnu=1&smnu=2&article_id=1276&proceeding_id=22}}


@incollection{korb04,
	Affiliation = {School of Computer Science and Software Engineering, Monash University, Clayton, Victoria 3800, Australia},
	Author = {Korb, Kevin. and Hope, Lucas. and Nicholson, Ann. and Axnick, Karl.},
	Booktitle = {PRICAI 2004: Trends in Artificial Intelligence},
	Date-Added = {2012-04-19 19:07:55 -0700},
	Date-Modified = {2012-04-19 19:07:56 -0700},
	Editor = {Zhang, Chengqi and W. Guesgen, Hans and Yeap, Wai-Kiang},
	Pages = {322-331},
	Publisher = {Springer Berlin / Heidelberg},
	Series = {Lecture Notes in Computer Science},
	Title = {Varieties of Causal Intervention},
	Volume = {3157},
	Year = {2004}}

@article{DawidDidelez2010,
	Author = {A. Philip Dawid and Vanessa Didelez},
	Bibsource = {DBLP, http://dblp.uni-trier.de},
	Date-Added = {2012-04-19 19:34:46 -0700},
	Date-Modified = {2012-04-19 19:38:44 -0700},
	Journal = {CoRR},
	Title = {Identifying the consequences of dynamic treatment strategies: A decision-theoretic overview},
	Volume = {abs/1010.3425},
	Year = {2010},
	Bdsk-Url-1 = {http://arxiv.org/abs/1010.3425}}

@techreport{Diaz12a,
title={Assessing the Causal Effect of Policies: An
Approach Based on Stochastic Interventions},
author={D\'iaz, Iv\'an and van der Laan, Mark},
year={2012},
journal={U.C. Berkeley Division of Biostatistics Working Paper Series}
}

@ARTICLE{Diaz11,
title = {Super Learner Based Conditional Density Estimation with Application to Marginal Structural Models},
author = {D\'iaz, Iv\'an and van der Laan, Mark},
year = {2011},
journal = {The International Journal of Biostatistics},
volume = {7},
number = {1},
pages = {38},
keywords = {Statistical Theory and Methods; causal inference; conditional density; cross validation; efficient estimation; marginal structural models; oracle selector},
}

@article {Diaz12,
author = {Iv\'an D\'iaz and van der Laan, Mark},
title = {Population Intervention Causal Effects Based on Stochastic Interventions},
journal = {Biometrics},
volume = {68},
number = {2},
publisher = {Blackwell Publishing Inc},
issn = {1541-0420},
url = {http://dx.doi.org/10.1111/j.1541-0420.2011.01685.x},
doi = {10.1111/j.1541-0420.2011.01685.x},
pages = {541--549},
keywords = {Causal effect, Counterfactual outcome, Double robustness, Stochastic intervention, Targeted maximum likelihood estimation},
year = {2012},
}
@incollection {Zheng11,
   author = {Zheng, Wenjing and van der Laan, Mark J.},
   affiliation = {Division of Biostatistics, University of California, Berkeley, 101 Haviland Hall, #7358, Berkeley, CA 94720, USA},
   title = {Cross-Validated Targeted Minimum-Loss-Based Estimation},
   booktitle = {Targeted Learning},
   series = {Springer Series in Statistics},
   editor = {Bickel, P. and Diggle, P. and Fienberg, S. and Krickeberg, K. and Olkin, I. and Wermuth, N. and Zeger, S.},
   publisher = {Springer New York},
   isbn = {978-1-4419-9782-1},
   keyword = {Mathematics and Statistics},
   pages = {459-474},
   year = 2011
}

@string{jasa = {Journal of the American Statistical Association}}

@string{jc = {Journal of Classification}}

@string{jrssb = {Journal of the Royal Statistical Society, Series B}}

@string{jspi = {Journal of Statistical Planning and Inference}}

@string{pnas = {Proc. Natl. Acad. Sci.}}

@article{Rubin1974,
    abstract = {Randomization should be employed whenever possible but the use of carefully controlled nonrandomized data to estimate causal effects is a reasonable and necessary procedure in many cases. ({Author/BJG})},
    author = {Rubin, Donald B.},
    citeulike-article-id = {4632390},
    citeulike-linkout-0 = {http://www.eric.ed.gov/ERICWebPortal/detail?accno=EJ118470},
    day = {0},
    journal = {Journal of Educational Psychology},
    keywords = {causality\_detection},
    month = {},
    posted-at = {2009-05-25 17:19:51},
    priority = {2},
    title = {Estimating Causal Effects of Treatments in Randomized and Nonrandomized Studies},
    url = {http://www.eric.ed.gov/ERICWebPortal/detail?accno=EJ118470},
    year = {1974}
}

@article{Mannetal2010,
	Author = {Mann, Jennifer K. AND Balmes, John R. AND Bruckner, Tim A. AND Mortimer, Kathleen M. AND Margolis, Helene G. AND Pratt, Boriana AND Hammond, S. Katharine AND Lurmann, Frederick W. AND Tager, Ira B.},
	Date-Added = {2011-09-14 16:32:02 -0700},
	Date-Modified = {2011-09-14 16:32:19 -0700},
	Doi = {10.1289/ehp.0901292},
	Journal = {Environ Health Perspect},
	Month = {06},
	Number = {10},
	Publisher = {National Institute of Environmental Health Sciences},
	Title = {Short-Term Effects of Air Pollution on Wheeze in Asthmatic Children in Fresno, California},
	Url = {http://dx.doi.org/10.1289%2Fehp.0901292},
	Volume = {118},
	Year = {2010},
	Bdsk-Url-1 = {http://dx.doi.org/10.1289/ehp.0901292}}

@incollection{korb04,
	Affiliation = {School of Computer Science and Software Engineering, Monash University, Clayton, Victoria 3800, Australia},
	Author = {Korb, Kevin. and Hope, Lucas. and Nicholson, Ann. and Axnick, Karl.},
	Booktitle = {PRICAI 2004: Trends in Artificial Intelligence},
	Editor = {Zhang, Chengqi and W. Guesgen, Hans and Yeap, Wai-Kiang},
	Pages = {322-331},
	Publisher = {Springer Berlin / Heidelberg},
	Series = {Lecture Notes in Computer Science},
	Title = {Varieties of Causal Intervention},
	Volume = {3157},
	Year = {2004}}

@article{Petersen10,
	Author = {Petersen, Maya L and Porter, Kristin E. and Gruber, Susan. and Wang, Yue. and van der Laan, Mark J.},
	Issn = {1477-0334},
	Journal = {Stat Methods Med Res},
	Pubmedid = {21030422},
	Title = {Diagnosing and responding to violations in the positivity assumption.},
	Url = {http://www.biomedsearch.com/nih/Diagnosing-responding-to-violations-in/21030422.html},
	Year = {2010},
	Bdsk-Url-1 = {http://www.biomedsearch.com/nih/Diagnosing-responding-to-violations-in/21030422.html}}

@article{Stitelmanetal10,
	Author = {Stitelman, Ori M and Hubbard, Alan E and Jewell, Nicholas P.},
	Publisher = {The Berkeley Electronic Press},
	Title = {The Impact Of Coarsening The Explanatory Variable Of Interest In Making Causal Inferences: Implicit Assumptions Behind Dichotomizing Variables},
	Url = {http://www.bepress.com/ucbbiostat/paper264},
	Year = {2010},
	Bdsk-Url-1 = {http://www.bepress.com/ucbbiostat/paper264}}

@article{Taubman01122009,
	Author = {Taubman, Sarah L and Robins, James M and Mittleman, Murray A and Hern{\'a}n, Miguel A},
	Doi = {10.1093/ije/dyp192},
	Eprint = {http://ije.oxfordjournals.org/content/38/6/1599.full.pdf+html},
	Journal = {International Journal of Epidemiology},
	Number = {6},
	Pages = {1599-1611},
	Title = {Intervening on risk factors for coronary heart disease: an application of the parametric g-formula},
	Url = {http://ije.oxfordjournals.org/content/38/6/1599.abstract},
	Volume = {38},
	Year = {2009},
	Bdsk-Url-1 = {http://ije.oxfordjournals.org/content/38/6/1599.abstract},
	Bdsk-Url-2 = {http://dx.doi.org/10.1093/ije/dyp192}}

@article{Laurenetal10,
	Author = {Cain, Lauren E and Robins, James M and Lanoy, Emilie and Logan, Roger and Costagliola, Dominique and Hern\'an, Miguel A.},
	Journal = {The International Journal of Biostatistics},
	Title = {When to Start Treatment? A Systematic Approach to the Comparison of Dynamic Regimes Using Observational Data},
	Url = {http://www.bepress.com/ijb/vol6/iss2/18},
	Volume = {6},
	Year = {2010},
	Bdsk-Url-1 = {http://www.bepress.com/ijb/vol6/iss2/18}}

@article{Eberhardt&Scheines06,
	Author = {F. Eberhardt and R. Scheines},
	Journal = {Department of Philosophy. Paper 415},
	Title = {Interventions and Causal Inference},
	Url = {http://repository.cmu.edu/philosophy/415},
	Year = {2006},
	Bdsk-Url-1 = {http://repository.cmu.edu/philosophy/415}}

@article{Orellana&Rotnitzky&Robins10,
	Author = {L. Orellana and A. Rotnitzky and J.M. Robins},
	Journal = {The International Journal of Biostatistics},
	Pages = {523-39},
	Title = {Dynamic Regime Marginal Structural Mean Models for Estimation of Optimal Dynamic Treatment Regimes, Part I: Main Content},
	Volume = {6},
	Year = {2010}}

@article{Kang&Shafer07,
	Author = {J. Kang and J. Schafer},
	Journal = {Statistical Science},
	Pages = {523-39},
	Title = {Demystifying Double Robustness: A Comparison of Alternative Strategies for Estimating a Population Mean from Incomplete Data (with discussion)},
	Volume = {22},
	Year = {2007}}

@article{Ridgeway&McCaffrey07,
	Author = {G. Ridgeway and D. McCaffrey},
	Journal = {Statistical Science},
	Pages = {540-43},
	Title = {Comment: Demystifying Double Robustness: A Comparison of Alternative Strategies for Estimating a Population Mean from Incomplete Data (with discussion)},
	Volume = {22},
	Year = {2007}}

@article{Robinsetal07,
	Author = {J. M. Robins and M. Sued and Q. Lei-Gomez and A. Rotnitzky},
	Journal = {Statistical Science},
	Pages = {544-559},
	Title = {Comment: Performance of Double-Robust Estimators When ``Inverse Probability'' Weights Are Highly Variable},
	Volume = {22},
	Year = {2007}}

@article{Tan07,
	Author = {Z. Tan},
	Journal = {Statistical Science},
	Pages = {560-568},
	Title = {Comment: Understanding OR, PS and DR},
	Volume = {22},
	Year = {2007}}
@article {Diaz&vanderLaan1101,
author = {Diaz, Ivan and van der Laan, Mark},
title = {Population Intervention Causal Effects Based on Stochastic Interventions},
journal = {Biometrics},
publisher = {Blackwell Publishing Inc},
issn = {1541-0420},
url = {http://dx.doi.org/10.1111/j.1541-0420.2011.01685.x},
doi = {10.1111/j.1541-0420.2011.01685.x},
pages = {In press.},
keywords = {Causal effect, Counterfactual outcome, Double robustness, Stochastic intervention, Targeted maximum likelihood estimation},
year = {2011},
}


@article{Tsiatis&Davidian07,
	Author = {A. Tsiatis and M. Davidian},
	Journal = {Statistical Science},
	Pages = {569-73},
	Title = {Comment: Demystifying Double Robustness: A Comparison of Alternative Strategies for Estimating a Population Mean from Incomplete Data (with discussion)},
	Volume = {22},
	Year = {2007}}

@article{Kang&Shafer07b,
	Author = {J. Kang and J. Schafer},
	Journal = {Statistical Science},
	Pages = {574-80},
	Title = {Rejoinder: Demystifying Double Robustness: A Comparison of Alternative Strategies for Estimating a Population Mean from Incomplete Data},
	Volume = {22},
	Year = {2007}}

@article{Murphy05,
	Author = {S. Murphy},
	Journal = {Statistics in Medicine},
	Pages = {1455�1481},
	Title = {An experimental design for the development of adaptive treatment strategies},
	Volume = {24},
	Year = {2005}}

@book{Zhang&Ma12,
  title={Ensemble Machine Learning: Methods and Applications},
  author={Zhang, C. and Ma, Y.},
  isbn={9781441993250},
  url={http://books.google.com/books?id=CjAs4stLXhAC},
  year={2012},
  publisher={Springer}
}

@article{Lavori&Dawson00,
	Author = {P. Lavori and R. Dawson},
	Journal = {Journal of the Royal Statistical Society, Series A},
	Pages = {29�38},
	Title = {A design for testing clinical strategies: biased adaptive within-subject randomization},
	Volume = {163},
	Year = {2000}}

@article{Lavori&Dawson04,
	Author = {P. Lavori and R. Dawson},
	Journal = {Clinical trials},
	Pages = {9�20},
	Title = {Dynamic treatment regimes: practical design considerations},
	Volume = {1},
	Year = {2004}}

@article{Thall&Millikan&Sung00,
	Author = {P. Thall and R. Millikan and H.-G. Sung},
	Journal = {Statistics in Medicine},
	Pages = {1011�1028},
	Title = {Evaluating multiple treatment courses in clinical trials},
	Volume = {19},
	Year = {2000}}

@article{Rush&Trivedi&Fava03,
	Author = {A.J. Rush and M. Trivedi and M. Fava},
	Journal = {IV. American Journal of Psychiatry},
	Pages = {237},
	Title = {Depression},
	Volume = {160(2)},
	Year = {2003}}

@article{Schneideretal06,
	Author = {Schneider, L. and Tariot.P.N. and Dagerman, K. and Davis, S. and Hsiao, J. and Ismail, S. and Lebowitz, B. and Lyketsos, C. and Ryan J. and Stroup T. and Sultzer D. and Weintraub, D. and Lieberman, J.},
	Journal = {New England Journal of Medicine},
	Pages = {1525�1538},
	Title = {Effectiveness of atypical antipsychotic drugs in patients with Alzheimer�s disease},
	Volume = {355(15)},
	Year = {2006}}

@article{Swartzetal07,
	Author = {Swartz, M. and Perkins, D. and Stroup, T. and Davis, S. and Capuano, G. and Rosenheck, R. and Reimherr, F. and McGee, M. and Keefe, R. and McEvoy, J. and Hsiao, J. and Lieberman, J.},
	Journal = {American Journal of Psychiatry},
	Pages = {428�436},
	Title = {Effects of antipsychotic medications on psychosocial functioning in patients with chronic shizophrenia: Findings from the nimh catie study},
	Volume = {164},
	Year = {2007}}

@article{Rubin&vanderLaan08,
	Author = {D.B. Rubin and M.J. van der Laan},
	Journal = {The International Journal of Biostatistics},
	Location = {http://www.bepress.com/ijb/vol4/iss1/5},
	Title = {Empirical Efficiency Maximization: Improved Locally Efficient Covariate Adjustment in Randomized Experiments and Survival Analysis},
	Volume = {Vol. 4, Iss. 1, Article 5},
	Year = {2008}}

@article{vanderLaan&Rose&Gruber09,
	Author = {M.J. van der Laan and S. Rose and S. Gruber},
	Journal = {Technical report, working paper series http://www.bepress.com/ucbbiostat/paper254/},
	Title = {Readings on Targeted Maximum Likelihood Estimation},
	Year = {September, 2009}}

@article{Bembometal09,
	Author = {O. Bembom and M.J. van der Laan and T. Haight and I.B. Tager},
	Journal = {Epidemiology},
	Title = {Lifetime and current leisure time physical activity and all-cause mortality in an elderly cohort},
	Year = {2009}}

@article{Bembom&vanderLaan07a,
	Author = {O. Bembom and M.J. van der Laan},
	Journal = {Journal of the National Cancer Institute},
	Pages = {1577-1582},
	Title = {Statistical Methods for analyzing sequentially randomized trials, commentary on JNCI article Adaptive therapy for androgen independent prostate cancer: A Randomized selection trial including four regimens, by Peter F. Thall, C. Logothetis, C. Pagliaro, S. Wen, M.A. Brown, D. Williams, R. Millikan (2007).},
	Volume = {99(21)},
	Year = {2007}}

@article{Rosenblumetal09,
	Author = {M. Rosenblum and S.G. Deeks and M.J. van der Laan and D.R. Bangsberg},
	Journal = {PLoS ONE},
	Title = {The Risk of Virologic Failure Decreases with Duration of HIV Suppression, at Greater than 50\% Adherence to Antiretroviral Therapy},
	Volume = {4(9): e7196.doi:10.1371/journal.pone.0007196},
	Year = {2009}}

@article{Robins&Orallana&Rotnitzky08,
	Author = {J. M. Robins and L. Orallana and A. Rotnitzky},
	Journal = {Statistics in Medicine},
	Pages = {4678-4721},
	Title = {Estimaton and extrapolation of optimal treatment and testing strategies},
	Volume = {27(23)},
	Year = {2008}}

@article{Bembom&vanderLaan07,
	Author = {O. Bembom and M.J. van der Laan},
	Journal = {Electronic Journal of Statistics},
	Title = {A practical illustration of the importance of realistic individualized treatment rules in causal inference},
	Year = {2007}}

@article{Bembometal08,
	Author = {O. Bembom and M.L. Petersen and S.-Y. Rhee and W. J. Fessel and S.E. Sinisi and R.W. Shafer and M.J. van der Laan},
	Journal = {Statistics in Medicine},
	Pages = {http://www3.interscience.wiley.com/journal/121422393/abstract},
	Title = {Biomarker discovery using targeted maximum likelihood estimation: Application to the treatment of antiretroviral resistant HIV infection},
	Year = {2008}}

@article{Tuglus&vanderLaan08,
	Author = {C. Tuglus and M.J. van der Laan},
	Journal = {UC Berkeley Working Paper Series},
	Pages = {http://www.bepress.com/ucbbiostat/paper233/.},
	Title = {Targeted Methods for Biomarker Discovery, the Search for a Standard},
	Year = {2008}}

@article{vanderLaan08,
	Author = {M.J. van der Laan},
	Journal = {The International Journal of Biostatistics},
	Pages = {http://www.bepress.com/ijb/vol4/iss1/17/},
	Title = {Estimation Based on Case-Control Designs with Known Prevalance Probability},
	Year = {2008}}

@article{Rose&vanderLaan08,
	Author = {S. Rose and M.J. van der Laan},
	Journal = {The International Journal of Biostatistics},
	Pages = {http://www.bepress.com/ijb/vol4/iss1/19/.},
	Title = {Simple Optimal Weighting of Cases and Controls in Case-Control Studies},
	Year = {2008}}

@article{Rose&vanderLaan09,
	Author = {S. Rose and M.J. van der Laan},
	Journal = {The International Journal of Biostatistics},
	Pages = {http://www.bepress.com/ijb/vol5/iss1/1/.},
	Title = {Why Match? [Investigating Matched Case-Control Study Designs with Causal Effect Estimation},
	Year = {2009}}

@inproceedings{Moore&vanderLaan09,
	Author = {K.L. Moore and M.J. van der Laan},
	Booktitle = {in Design, Summarization, Analysis \& Interpretation of Clinical Trials with Time-to-Event Endpoints},
	Editor = {Karl E. Peace},
	Publisher = {Chapman and Hall},
	Title = {Application of Time-to-Event Methods in the Assessment of Safety in Clinical Trials},
	Year = {2009}}

@inproceedings{Polley&vanderLaan09,
	Author = {E.C. Polley and M.J. van der Laan},
	Booktitle = {in Design, Summarization, Analysis \& Interpretation of Clinical Trials with Time-to-Event Endpoints},
	Editor = {Karl E. Peace},
	Publisher = {Chapman and Hall},
	Title = {Predicting Optimal Treatment Assignment Based on Prognostic Factors in Cancer Patients},
	Year = {2009}}

@article{vanderVaart&Dudoit&vanderLaan06,
	Author = {A.W. van der Vaart and S. Dudoit and M.J. van der Laan},
	Journal = {Statistics and Decisions},
	Number = {3},
	Pages = {351--371},
	Title = {Oracle Inequalities for Multi-Fold Cross-Validation},
	Volume = {24},
	Year = {2006}}

@article{vanderLaan&Dudoit&vanderVaart06,
	Author = {M.J. van der Laan and S. Dudoit and A.W. van der Vaart},
	Journal = {Statistics and Decisions},
	Number = {3},
	Pages = {373--395},
	Title = {The Cross-Validated Adaptive Epsilon-Net Estimator},
	Volume = {24},
	Year = {2006}}

@article{Rosenbaum&Rubin83,
	Author = {P.R. Rosenbaum and D.B. Rubin},
	Journal = {Biometrika},
	Pages = {41-55},
	Title = {The Central Role of the Propensity Score in Observational Studies for Causal Effects},
	Volume = {70},
	Year = {1983}}

@article{vanderLaan&Polley&Hubbard07,
	Author = {M.J. van der Laan and E. Polley and A. Hubbard},
	Issn = {1},
	Journal = {Statistical Applications in Genetics and Molecular Biology},
	Location = {http://www.bepress.con/sagmb/vol6/iss1/art25},
	Number = {25},
	Title = {Super Learner},
	Volume = {6},
	Year = {2007}}

@article{Sekhon08,
	Author = {J.S. Sekhon},
	Journal = {Journal of Statistical Sotware, Forthcoming},
	Location = {http://ssrn.com/paper=1009044},
	Publisher = {SSRN},
	Title = {Multivariate and Propensity Score Matching Software with Automated Balance Optimization: The Matching package for {R}},
	Year = {2008}}

@article{Zheng&vanderLaan10,
	Author = {Wenjing Zheng and Mark J. van der Laan},
	Journal = {Division of Biostatistics Working Paper Series},
	Location = {http://works.bepress.com/wenjing_zheng/1/},
	Publisher = {U.C. Berkeley},
	Title = {Asymptotic Theory for Cross-validated Targeted Maximum Likelihood Estimation},
	Year = {2010}}

@article{Bembometal08,
	Author = {O. Bembom and J.W. Fessel and R.W. Shafer and M.J. van der Laan},
	Institution = {DigitalCommons@Florida Atlantic University [http://digitalcommons.fau.edu/cgi/oai2.cgi] (United States)},
	Keywords = {General Biostatistics},
	Location = {http://www.scientificcommons.org/36721107},
	Publisher = {The Berkeley Electronic Press},
	Title = {Data-adaptive Selection Of The Adjustment Set In Variable Importance Estimation},
	Url = {http://www.bepress.com/ucbbiostat/paper231},
	Year = {2008},
	Bdsk-Url-1 = {http://www.bepress.com/ucbbiostat/paper231}}

@article{Holland&Reitman77,
	Address = {New York, NY, USA},
	Author = {J.H. Holland and J.S. Reitman},
	Doi = {http://doi.acm.org/10.1145/1045343.1045373},
	Issn = {0163-5719},
	Journal = {SIGART Bull.},
	Pages = {49--49},
	Publisher = {ACM},
	Title = {Cognitive systems based on adaptive algorithms},
	Volume = {63},
	Year = {1977},
	Bdsk-Url-1 = {http://doi.acm.org/10.1145/1045343.1045373}}

@book{Rubin06,
	Address = {Cambridge, MA},
	Author = {D.B. Rubin},
	Publisher = {Cambridge University Press},
	Title = {Matched Sampling for Causal Effects.},
	Year = {2006}}

@incollection{Mansk1&McFadden81,
	Address = {Cambridge, MA},
	Author = {C.F. Manski and D. McFadden},
	Booktitle = {Structural Analysis of Discrete Data with Econometric Applications},
	Editor = {C.F. Manski and D. McFadden},
	Publisher = {The MIT Press},
	Title = {Alternative estimators and sample designs for discrete choice analysis},
	Year = {1981}}

@article{Manski&Lerman77,
	Author = {C.F. Manski and S.R. Lerman},
	Journal = {Econometrica},
	Number = {8},
	Pages = {1977-1988},
	Title = {The Estimation of Choice Probabilities from Choice Based Samples},
	Volume = {45},
	Year = {1977}}

@article{Cosslett81,
	Author = {S.R. Cosslett},
	Journal = {Econometrica},
	Number = {5},
	Pages = {1289-1316},
	Title = {Maximum Likelihood Estimator for Choice-Based Samples},
	Volume = {49},
	Year = {1981}}

@article{Cornfield51,
	Author = {J. Cornfield},
	Journal = {J Nat Cancer Inst},
	Pages = {1269-1275},
	Title = {A method of estimating comparative rates from clinical data. Applications to cancer of the lung, breast, and cervix.},
	Volume = {11},
	Year = {1951}}

@inproceedings{Cornfield56,
	Author = {J. Cornfield},
	Booktitle = {Proceedings of the Third Berkeley Symposium, Volume IV},
	Editor = {J. Neyman},
	Pages = {133-148},
	Publisher = {University of California Press},
	Title = {A statistical problem arising from retrospective studies},
	Year = {1956}}

@article{Benichou&Wacholder94,
	Author = {J. Benichou and S. Wacholder},
	Journal = {Statistics in Medicine},
	Pages = {651-661},
	Title = {A comparison of three approaches to estimate exposure-specific incidence rates from population-based case-control data.},
	Volume = {13},
	Year = {1994}}

@article{Breslow&Robins&Wellner00,
	Author = {N.E. Breslow and J.M. Robins and J.A. Wellner},
	Journal = {Bernoulli},
	Pages = {447--455},
	Title = {On the semi-parametric efficiency of logistic regression under case-control sampling},
	Volume = {6(3)},
	Year = {2000}}

@article{Mansonetal07,
	Author = {R. Mansson, M.M. Joffe, W. Sun, S. Hennessy},
	Journal = {Am J Epidemiol},
	Number = {3},
	Pages = {332-339},
	Title = {On the Estimation and Use of Propensity Scores in Case-Control and Case-Cohort Studies.},
	Volume = {166},
	Year = {2007}}

@article{Anderson79,
	Author = {J.A. Anderson},
	Journal = {Biometrika},
	Pages = {19--35},
	Title = {Separate sample logistic discrimination},
	Volume = {59},
	Year = {1972}}

@article{Prentice&Pyke79,
	Author = {R.L. Prentice and R. Pyke},
	Journal = {Biometrika},
	Pages = {403--411},
	Title = {Logistic disease incidence models and case-control studies},
	Volume = {66},
	Year = {1979}}

@article{Breslow96,
	Author = {N.E. Breslow},
	Journal = {J Am Stat Soc},
	Pages = {14--28},
	Title = {Statistics in Epidemiology: the Case-Control Study},
	Volume = {91},
	Year = {1996}}

@book{Breslow&Day80,
	Address = {Lyon},
	Author = {N.E. Breslow and N.E. Day},
	Publisher = {International Agency for Research on Cancer},
	Title = {Statistical Methods in Cancer Research: Volume 1 -- The analysis of case-control studies},
	Year = {1980}}

@article{Holford&White&Kelsey78,
	Author = {T.R. Holford and C. White and J.L. Kelsey},
	Journal = {Am J Epid},
	Number = {3},
	Pages = {245--255},
	Title = {Multivariate Analysis for Matched Case-Control Studies},
	Volume = {107},
	Year = {1978}}

@article{Breslowetal78,
	Author = {N.E. Breslow and N.E. Day and K.T. Halvorsen and R.L. Prentice and C. Sabal},
	Journal = {Am J Epid},
	Number = {4},
	Pages = {299--307},
	Title = {Estimation of Multiple Relative Risk Functions in Matched Case-Control Studies},
	Volume = {108},
	Year = {1978}}

@book{Schlesselman82,
	Address = {Oxford},
	Author = {J.J. Schlesselman},
	Publisher = {Oxford University Press},
	Title = {Case-Control Studies: Design, Conduct, Analysis},
	Year = {1982}}

@book{Collett91,
	Address = {London},
	Author = {D. Collett},
	Publisher = {Chapman and Hall},
	Title = {Modeling Binary Data},
	Year = {1991}}

@book{Jewell04,
	Address = {Boca Raton},
	Author = {N.P. Jewell},
	Publisher = {Chapman and Hall/CRC},
	Title = {Statistics for Epidemiology},
	Year = {2004}}

@book{Hosmer&Lemeshow00,
	Address = {New York},
	Author = {D.W. Hosmer and S. Lemeshow},
	Edition = {2nd},
	Publisher = {John Wiley and Sons},
	Title = {Applied Logistic Regression},
	Year = {2000}}

@article{Robins99,
	Author = {J.M. Robins},
	Journal = {Statistical Science},
	Number = {3},
	Pages = {281--293},
	Title = {[Choice as an Alternative to Control in Observational Studies]: Comment},
	Volume = {14},
	Year = {1999}}

@article{Newman06,
	Author = {S. Newman},
	Journal = {Epid Persp Innov},
	Pages = {2},
	Title = {Causal Analysis of Case-Control Data},
	Url = {http://www.epi-perspectives.com/content/3/1/2},
	Volume = {3},
	Year = {2006},
	Bdsk-Url-1 = {http://www.epi-perspectives.com/content/3/1/2}}

@article{Zelen&Parker86,
	Author = {M. Zelen and R.A. Parker},
	Journal = {Stat Med},
	Number = {3},
	Pages = {261--269},
	Title = {Case-Control Studies and Bayesian Inference},
	Volume = {5},
	Year = {1986}}

@article{Sinhetal04,
	Author = {S. SInha and B. Mukherjee and M Ghosh},
	Journal = {Biometrics},
	Pages = {41--49},
	Title = {Bayesian Semiparametric Modeling for Matched Case-Control Studies with Multiple Disease States},
	Volume = {60},
	Year = {2004}}

@article{Ritchieetal01,
	Author = {M.D. Ritchie and L.W. Hahn and N. Roodi and L.R. Bailey and W.D. Dupont and F.F. Parl and J.H. Moore},
	Journal = {Am J Hum Genet},
	Number = {1},
	Pages = {138--47},
	Title = {Multifactor-dimensionality reduction reveals high-order interactions among estrogen-metabolism genes in sporadic breast cancer.},
	Volume = {69},
	Year = {2001}}

@article{Mei&Cuccaro&Martin07,
	Author = {H. Mei and M.L. Cuccaro and E.R. Martin},
	Journal = {Am J Hum Genet},
	Number = {6},
	Pages = {1251-61},
	Title = {Multifactor dimensionality reduction-phenomics: a novel method to capture genetic heterogeneity with use of phenotypic variables.},
	Volume = {81},
	Year = {2007}}

@article{Bangsberg&Moss&Deeks04,
	Abstract = {Public health debates about providing HIV antiretroviral therapy to impoverished populations have centred on the relationship between adherence and risk of drug resistance. Recent data indicate that each antiretroviral therapeutic class has a unique adherence-resistance relationship. Resistance to single protease inhibitor therapy occurs most frequently at moderate to high levels of adherence, resistance to non-nucleoside reverse transcriptase inhibitor therapy occurs at low to moderate levels of adherence, and resistance to ritonavir-boosted protease inhibitor therapy is most likely to occur at middle ranges of adherence. These dynamic relationships should be considered in balancing the individual and public health benefits of therapy.},
	Author = {D.R. Bangsberg and A.R. Moss and S.G. Deeks},
	Journal = {J Antimicrob Chemother},
	Keywords = {Anti-HIV Agents/*therapeutic use Developing Countries *Drug Resistance, Viral Humans *Patient Compliance Public Health Research Support, Non-U.S. Gov't Research Support, U.S. Gov't, P.H.S.},
	Note = {0305-7453 (Print) Journal Article Review},
	Number = {5},
	Pages = {696-9},
	Title = {Paradoxes of adherence and drug resistance to {HIV} antiretroviral therapy},
	Volume = {53},
	Year = {2004}}

@article{Scharfstein&Tsiatis&Robins97,
	Author = {D.O. Scharfstein and A.A. Tsiatis and J.M. Robins},
	Journal = {Journal of the American Statistical Association},
	Number = {440},
	Pages = {1342--1350},
	Title = {Semiparametric efficiency and its implications on the design and analysis of group-sequential studies},
	Volume = {92},
	Year = {1997}}

@article{Bembometal07,
	Author = {O. Bembom and M. Petersen and SY Rhee and W.J. Fessel and S.E. Sinisi and R.W. Shafer and M.J. van der Laan},
	Journal = {U.C. Berkeley Division of Biostatistics Working Paper Series},
	Optmonth = {August},
	Optnote = {http://www.bepress.com/ucbbiostat/paper221},
	Title = {Biomarker Discovery Using Targeted Maximum Likelihood Estimation: Application to the Treatment of Antiretroviral Resistant {HIV} Infection},
	Volume = {221},
	Year = {2007}}

@article{vanderLaan&Gruber09,
	Author = {M.J. van der Laan and S. Gruber},
	Journal = {The International Journal of Biostatistics},
	Title = {Collaborative Double robust penalized targeted maximum likelihood estimation},
	Year = {2009}}

@article{vanderLaan&Rubin06,
	Author = {M.J. van der Laan and D. Rubin},
	Journal = {The International Journal of Biostatistics},
	Number = {1},
	Optnote = {http://www.bepress.com/ijb/vol2/iss1/11},
	Title = {Targeted Maximum Likelihood Learning},
	Volume = {2},
	Year = {2006}}

@article{Scharfstein&Tsiatis98,
	Author = {D.O. Scharfstein and A.A. Tsiatis},
	Journal = {Statistics in Medicine},
	Pages = {75--87},
	Title = {The use of simulation and bootstrap in information based group sequential studies},
	Volume = {17},
	Year = {1998}}

@article{Pampallona&Tsiatis&Kim01,
	Author = {S. Pampallona and A.A. Tsiatis and K. Kim},
	Journal = {Drug Informational Journal},
	Pages = {1113-1121},
	Title = {Interim monitoring of group sequential trials using spending functions for the type I and type II error probabilities},
	Volume = {35},
	Year = {2001}}

@article{Tsiatis&Mehta03,
	Author = {A.A. Tsiatis and C. Mehta},
	Journal = {Biometrika},
	Pages = {367-378},
	Title = {On the inefficiency of the adaptive design for monitoring clinical trials},
	Volume = {90},
	Year = {2003}}

@book{tsiatis2006,
	Author = {Tsiatis, A.A.},
	Isbn = {9780387324487},
	Lccn = {2006921164},
	Publisher = {Springer},
	Series = {Springer series in statistics},
	Title = {Semiparametric theory and missing data},
	Url = {http://books.google.com/books?id=xqZFi2EMB40C},
	Year = {2006},
	Bdsk-Url-1 = {http://books.google.com/books?id=xqZFi2EMB40C}}

@article{Banerjee&Tsiatis06,
	Author = {A. Banerjee and A.A. Tsiatis},
	Journal = {Statistics in Medicine},
	Optnote = {In press},
	Title = {Adaptive two-stage designs in phase II clinical trials},
	Year = {2006}}

@article{Tsiatis06,
	Author = {A.A. Tsiatis},
	Journal = {Statistics in Medicine},
	Optnote = {In press},
	Title = {Information based monitoring of clinical trials},
	Year = {2006}}

@article{Lokhnygina&Tsiatis06,
	Author = {Y. Lokhnygina and A.A. Tsiatis},
	Journal = {Journal of Statistical Planning and Inference},
	Optnote = {In press},
	Title = {Optimal two-stage group sequential designs},
	Year = {2006}}

@article{Bauer&Kohne94,
	Author = {P. Bauer and Kohne},
	Journal = {Biometrics},
	Pages = {1029--1041},
	Title = {Evaluation of experiments with adaptive interim analysis},
	Year = {1994}}

@article{Cui&Hung&Wang99,
	Author = {L. Cui and H.M.J. Hung and S-J Wang},
	Journal = {Biometrics},
	Pages = {853--857},
	Title = {Modification of sample size in group sequential trials},
	Year = {1999}}

@article{Jennison&Turnbull03,
	Author = {C. Jennison and B.W. Turnbull},
	Journal = {Statistics in Medicine},
	Pages = {971--993},
	Title = {Mid course sample size modification in clinical trials based on hte observed treatment effect},
	Year = {2003}}

@article{Koyama&Sampson&Gleser04,
	Author = {T. Koyama and A.R. Sampson and L.J. Gleser},
	Journal = {Journal of the Americal Statistical Association},
	Title = {A calculus for design of two stage adaptive procedures},
	Year = {2004}}

@article{Lan&Trost97,
	Author = {K.K.G Lan and D.C. Trost},
	Journal = {Proceedings Biopharm Section},
	Pages = {48-51},
	Title = {Estimation of parameters and sample size re-estimation},
	Year = {1997}}

@article{Lietal02,
	Author = {G. Li and W.J. Shih and T. Xie and J. Lu},
	Journal = {Biostatistics},
	Pages = {277--287},
	Title = {A sample size adjustment procedure for clinical trials based on conditional power},
	Year = {2002}}

@article{Mehta&Tsiatis01,
	Author = {C.R. Mehta and A.A. Tsiatis},
	Journal = {Drug Informational Journal},
	Pages = {1095--1112},
	Title = {Flexible sample size considerations using information based interim monitoring},
	Volume = {35},
	Year = {2001}}

@article{Mulle&Shafer01,
	Author = {H.H. Mulle and H. Shafer},
	Journal = {Biometrics},
	Pages = {886--891},
	Title = {Adaptive group sequential designs for clinical trials: combining the advantages of adaptive and classical group sequential approaches},
	Volume = {57},
	Year = {2001}}

@article{Proschan&Hunsberger95,
	Author = {M.A. Proschan and S.A. Hunsberger},
	Journal = {Biometrics},
	Pages = {1315--1324},
	Title = {Designed extension studies based on conditional power},
	Volume = {51},
	Year = {1995}}

@article{Shen&Fisher99,
	Author = {Y. Shen and L.D. Fisher},
	Journal = {Biometrics},
	Pages = {190--197},
	Title = {Statistical Inference for self-designing clinical trials with a one-sided hypothesis},
	Volume = {55},
	Year = {1999}}

@article{Wittes&Brittain90,
	Author = {J. Wittes and E. Brittain},
	Journal = {Statistics in Medicine},
	Pages = {65--72},
	Title = {The role of internal pilot studies in increasing efficiency of clinical trials},
	Volume = {9},
	Year = {1999}}

@article{Shen&Cheng06,
	Author = {Y. Shen and Y. Cheng},
	Journal = {Biostatistics},
	Optnote = {In Press},
	Title = {Adaptive design: Estimation and Inference with censored data in a semiparametric model},
	Year = {2006}}

@book{Spiegelalter&Abrams&Myles04,
	Author = {D.J. Spiegelalter and K.R. Abrams and J.P. Myles},
	Publisher = {Wiley, Chichester},
	Title = {Bayesian approaches to clinical trials and health care evaluation},
	Year = {2004}}

@book{Berry&Stangl96,
	Author = {D.A. Berry and D.K. Stangl},
	Publisher = {Marcel Dekker, New York},
	Title = {Bayesian biostatistics},
	Year = {1996}}

@article{Berry06,
	Author = {D.A. Berry},
	Journal = {Nature Reviews, Drug Discovery},
	Title = {Bayesian clinical trials},
	Volume = {5},
	Year = {2006}}

@book{Hu&Rosenberger06,
	Author = {F. Hu and W.F. Rosenberger},
	Publisher = {New York Wiley},
	Title = {The theory of response adaptive randomization in clinical trials},
	Year = {2006}}

@book{Dudoit&vanderLaan08,
	Author = {S. Dudoit and M.J. van der Laan},
	Publisher = {Springer Series of Statistics, New York},
	Title = {Resampling based multiple testing with applications to genomics},
	Year = {2008}}

@book{Sen&Singer93,
	Author = {P.K. Sen and J.M. Singer},
	Publisher = {Chapman \& Hall, New York},
	Title = {Large Sample Methods in Statistics: An Introduction with Applications},
	Year = {1993}}

@article{Bai&Hu&Rosenberger02,
	Author = {Z.D. Bai and F. Hu and W.F. Rosenberger},
	Journal = {Annals of Statistics},
	Number = {1},
	Pages = {122--139},
	Title = {Asymptotic properties of adaptive designs for clinical trials with delayed response},
	Volume = {30},
	Year = {2002}}

@article{Andersen&Faries&Tamura94,
	Author = {J. Andersen and D. Faries and R. Tamura},
	Journal = {Communication in Statistical Theory},
	Pages = {309--323},
	Title = {A randomized play-the-winner design for multiarm clinical trials},
	Volume = {23},
	Year = {1994}}

@book{Flournoy&Rosenberger95,
	Author = {N. Flournoy and W.F. Rosenberger},
	Publisher = {Hayward, Institute of Mathematical Statistics},
	Title = {Adaptive Designs},
	Year = {1995}}

@article{Hu&Rosenberger00,
	Author = {F. Hu and W.F. Rosenberger},
	Journal = {Statistics in Medicine},
	Pages = {2067--2075},
	Title = {Analysis of time trends in adaptive designs withi appliation to a neurophysiology experiment},
	Volume = {19},
	Year = {2000}}

@article{Rosenberger96,
	Author = {W.F. Rosenberger},
	Journal = {Statistical Science},
	Pages = {137--149},
	Title = {New directions in adaptive designs},
	Volume = {11},
	Year = {1996}}

@article{Rosenberger&Flournoy&Durham97,
	Author = {W.F. Rosenberger and N. Flournoy and S.D. Durham},
	Journal = {Journal of Statistical Planning and Inference},
	Pages = {69--76},
	Title = {Asymptotic normality of maximum likelihood estimators from multiparameter response driven designs},
	Year = {1997}}

@article{Rosenberger&Grill97,
	Author = {W.F. Rosenberger and S.E. Grill},
	Journal = {Statistics in Medicine},
	Pages = {2245--2260},
	Title = {A sequential design for psychophysical experiments: An application to estimating timing of sensory events},
	Volume = {16},
	Year = {1997}}

@article{Rosenberger&Sriram97,
	Author = {W.F. Rosenberger and T.N. Shiram},
	Journal = {Journal of Statistical Planning and Inference},
	Pages = {309--319},
	Title = {Estimation for an adaptive allocation design},
	Volume = {59},
	Year = {1997}}

@article{Tamuraetal94,
	Author = {R.N. Tamura and D.E. Faries and J.S. Andersen and J.H. Heiligenstein},
	Journal = {Journal of the American Statistical Association},
	Pages = {768--776},
	Title = {A case study of an adaptive clinical trial in the treatment of out-patients with depressive disorder},
	Volume = {89},
	Year = {1994}}

@article{Wei&Durham78,
	Author = {L.J. Wei and S. Durham},
	Journal = {Journal of the American Statistical Association},
	Pages = {840--843},
	Title = {The randomize play-the-winner rule in medical trials},
	Volume = {73},
	Year = {1978}}

@article{Weietal90,
	Author = {L.J. Wei and R.T. Smythe and D.Y. Lin and T.S. Park},
	Journal = {Journal of the American Statistical Association},
	Pages = {156--162},
	Title = {Statistical Inference with data-dependent treatment allocation rules},
	Volume = {85},
	Year = {1990}}

@article{Zelen69,
	Author = {M. Zelen},
	Journal = {Journal of the American Statistical Association},
	Pages = {131--146},
	Title = {Play the winner rule and the controlled clinical trial},
	Volume = {64},
	Year = {1969}}

@article{Cheng&Shen05,
	Author = {Y. Cheng and Y. Shen},
	Journal = {Biometrika},
	Number = {3},
	Pages = {633--646},
	Title = {Bayesian adaptive designs for clinical trials},
	Volume = {92},
	Year = {2005}}

@article{Wei79,
	Author = {L.J. Wei},
	Journal = {Annals of Statistics},
	Pages = {291--296},
	Title = {The generalized Polya's urn design for sequential medical trials},
	Volume = {7},
	Year = {1979}}

@article{Benito&Lopez&Soriano03,
	Author = {Benito, J. M. and Lopez, M. and Soriano, V.},
	Journal = {J Infect Dis},
	Keywords = {ADP-ribosyl Cyclase/metabolism Anti-HIV Agents/therapeutic use Antigens, CD/metabolism CD4-Positive T-Lymphocytes/*immunology CD8-Positive T-Lymphocytes/immunology HIV Infections/drug therapy/*immunology/virology HIV-1/*physiology Human *Viral Load Virus Replication},
	Note = {0022-1899 Comment Letter},
	Number = {5},
	Pages = {794-5; author reply 795-6},
	Title = {Virus load and cytolitic responses in human immunodeficiency virus infection: what is cause and what is effect},
	Volume = {188},
	Year = {2003}}

@article{DEttorreetal02,
	Abstract = {OBJECTIVE: To study virologic and immunologic factors associated with discordant treatment response in HIV-infected patients receiving highly active antiretroviral therapy (HAART). DESIGN: Study participants included a total of 27 patients: (a) 10 discordant patients (mean CD4+ cell count, 396.1 x 10 cells/l; mean HIV-RNA, 5.4 log copies/ml); (b) seven responder patients (mean CD4+ cell count, 997.5 x 10 cells/l); and (c) 10 failing patients (mean CD4+ cell count 66.5 x 10 cells/l; mean HIV-RNA, 5.4 log copies/ml).(10) (10)METHODS: The HIV-1 isolation rate and biological phenotype, drug resistance genotypic mutations of HIV-1 strains, recall and HIV-1-specific antigen lymphocyte proliferation (LP), and interleukin (IL)-15 production were studied. RESULTS: Virus isolation was obtained in 30% of discordant patients, and in 100% of failing patients. A higher replication constant was reported in discordant patients. No difference in the number of drug resistance mutations and biological phenotypes of HIV-1 was found in discordant patients with respect to failing patients. Discordant patients developed positive LP responses to and HIV-1 p24. LP in response to, HIV-1 p24 and gp160 was positive in responder patients. No significant LP was found in failing patients. Increased levels of IL-15 after stimulation with lipopolysaccaride (LPS) and were found in both discordant patients and responder patients. Conversely, a strong reduction of IL-15 levels was observed in failing patients. CONCLUSION: The present results suggest that decreased virus isolation rate, restoration of both lymphocyte proliferation and IL-15 production are factors involved in the discordant antiretroviral therapy response of HIV-infected patients.},
	Author = {D'Ettorre, G. and Forcina, G. and Andreotti, M. and Sarmati, L. and Palmisano, L. and Galluzzo, C. M. and Nicastri, E. and Mastroianni, C. M. and Vullo, V. and Vella, S. and Andreoni, M.},
	Journal = {Aids},
	Keywords = {Adult Anti-HIV Agents/*therapeutic use Antiretroviral Therapy, Highly Active CD4 Lymphocyte Count CD8-Positive T-Lymphocytes/drug effects/immunology Candida albicans Drug Resistance, Viral Female HIV Infections/complications/*drug therapy/immunology/virology HIV-1/drug effects/genetics/*immunology/isolation & purification Human Interleukin-15/*blood Male Middle Aged Mutation Viral Load Virus Replication/drug effects},
	Note = {0269-9370 Journal Article},
	Number = {14},
	Pages = {1877-85},
	Title = {Discordant response to antiretroviral therapy: {HIV} isolation, genotypic mutations, T-cell proliferation and cytokine production},
	Volume = {16},
	Year = {2002}}

@article{Davenportetal02,
	Abstract = {Early infection with HIV-1 is dominated by CCR5-tropic (R5, non-syncytium-inducing) viruses. The evolution of CXCR4-tropic (X4, syncytium-inducing) viruses occurs later in the infection and is associated with rapid disease progression. Here, we propose that the tropism of X4 viruses for naive CD4+ T cells is disadvantageous in early infection owing to the low division rate of these cells. In healthy individuals, the division rate of memory cells is nearly ten times higher than that of naive cells and thus the memory-cell tropism of R5 viruses could account for their dominance early in infection. As the division rate of naive T cells increases with CD4+ depletion, X4 viruses come to dominate in late disease.},
	Author = {Davenport, M. P. and Zaunders, J. J. and Hazenberg, M. D. and Schuitemaker, H. and van Rij, R. P.},
	Journal = {Trends Microbiol},
	Keywords = {CD4-Positive T-Lymphocytes/*virology HIV Infections/*immunology/metabolism HIV-1/*pathogenicity Human Immunologic Memory Macrophages/*virology Models, Biological Receptors, CCR5/metabolism Receptors, CXCR4/metabolism Tropism},
	Note = {0966-842x Journal Article},
	Number = {6},
	Pages = {275-8},
	Title = {Cell turnover and cell tropism in HIV-1 infection},
	Volume = {10},
	Year = {2002}}

@article{Deeksetal00,
	Abstract = {The relationship between plasma human immunodeficiency virus (HIV) RNA levels and peripheral CD4+ T cell counts was examined in 380 HIV-infected adults receiving long-term protease inhibitor therapy. Patients experiencing virologic failure (persistent HIV RNA >500 copies RNA/mL) generally had CD4+ T cell counts that remained greater than pretherapy baseline levels, at least through 96 weeks of follow-up. The CD4+ T cell response was directly and independently related to degree of viral suppression below the pretreatment baseline. For any given HIV RNA level measured 12 weeks after virologic failure, subsequent CD4+ T cell decline was slower in patients receiving a protease inhibitor-based regimen than in a historical control group of untreated patients. These observations suggest that transient or partial declines in plasma HIV RNA levels can have sustained effects on CD4+ T cell levels.},
	Author = {Deeks, S. G. and Barbour, J. D. and Martin, J. N. and Swanson, M. S. and Grant, R. M.},
	Journal = {J Infect Dis},
	Keywords = {Adult *CD4 Lymphocyte Count Female HIV Infections/*drug therapy/immunology/virology HIV Protease Inhibitors/*therapeutic use Human Male RNA, Viral/*blood Support, Non-U.S. Gov't Support, U.S. Gov't, P.H.S.},
	Note = {0022-1899 Journal Article},
	Number = {3},
	Pages = {946-53},
	Title = {Sustained CD4+ T cell response after virologic failure of protease inhibitor-based regimens in patients with human immunodeficiency virus infection},
	Volume = {181},
	Year = {2000}}

@article{Deeksetal01,
	Abstract = {BACKGROUND: In many patients with human immunodeficiency virus (HIV) infection, therapy with potent antiretroviral drugs does not result in complete suppression of HIV replication. The effect of cessation of therapy in these patients is unknown. METHODS: Sixteen patients who had a plasma HIV RNA level of more than 2500 copies per milliliter during combination antiretroviral-drug therapy were randomly assigned, in a 2:1 ratio, to discontinue or continue therapy. Plasma HIV RNA levels, CD4 cell counts, and drug susceptibility were measured weekly. Viral replicative capacity was measured at base line and at week 12. RESULTS: Discontinuation of therapy for 12 weeks was associated with a median decrease in the CD4 cell count of 128 cells per cubic millimeter and an increase in the plasma HIV RNA level of 0.84 log copies per milliliter. Virus from all patients with detectable resistance at entry became susceptible to HIV-protease inhibitors within 16 weeks after the discontinuation of therapy. Drug susceptibility began to increase a median of six weeks after the discontinuation of therapy and was temporally associated with increases in plasma HIV RNA levels and decreases in CD4 cell counts. Viral replicative capacity, measured by means of a recombinant-virus assay, was low at entry into the study and increased after therapy was discontinued. Despite the loss of detectable resistance in plasma, resistant virus was cultured from peripheral-blood mononuclear cells in five of nine patients who could be evaluated. Plasma HIV RNA levels, CD4 cell counts, and drug susceptibility remained stable in the patients who continued therapy. CONCLUSIONS: Despite the presence of reduced drug susceptibility, antiretroviral-drug therapy can provide immunologic and virologic benefit. This benefit reflects continued antiviral-drug activity and the maintenance of a viral population with a reduced replicative capacity.},
	Author = {Deeks, S. G. and Wrin, T. and Liegler, T. and Hoh, R. and Hayden, M. and Barbour, J. D. and Hellmann, N. S. and Petropoulos, C. J. and McCune, J. M. and Hellerstein, M. K. and Grant, R. M.},
	Journal = {N Engl J Med},
	Keywords = {Adult Anti-HIV Agents/pharmacology/*therapeutic use CD4 Lymphocyte Count Drug Resistance, Microbial Drug Therapy, Combination HIV Infections/*drug therapy/immunology/virology HIV Protease Inhibitors/pharmacology/*therapeutic use HIV-1/*drug effects/genetics/isolation & purification Human Male Middle Aged Proportional Hazards Models Prospective Studies RNA, Viral/blood Support, Non-U.S. Gov't Support, U.S. Gov't, P.H.S. Viremia/drug therapy},
	Note = {0028-4793 Clinical Trial Journal Article Randomized Controlled Trial},
	Number = {7},
	Pages = {472-80},
	Title = {Virologic and immunologic consequences of discontinuing combination antiretroviral-drug therapy in HIV-infected patients with detectable viremia},
	Volume = {344},
	Year = {2001}}

@article{Deeks01,
	Abstract = {Although understanding of nonnucleoside reverse transcriptase inhibitor (NNRTI) resistance is less clearly established than that of other classes of antiretroviral drugs, certain facts have been established. The treatment-associated genetic mutation profiles of the available NNRTIs have been mapped, and resistance has been found to develop rapidly after initiation of NNRTI therapy. Despite the chemical diversity of the NNRTIs, cross-resistance among agents of this class is nearly universal. Although the viral replicative capacity (``fitness") of NNRTI-induced viral variants has not been extensively studied, available data suggest that NNRTI-selected mutations confer little damage to viral fitness, and thus a single point mutation produces a strain that is both resistant and fit. Furthermore, with continued therapy, viral evolution persists, creating species with greater numbers of mutations and higher level phenotypic resistance. Taken together, these facts suggest that continued use of NNRTIs after emergence of resistance will produce variants of complex mutational patterns that limit future treatment options, and, therefore, strong consideration should be given to discontinuing NNRTIs after virologic failure is confirmed. This article describes the scientific literature establishing the efficacy and limitations of NNRTI therapy and attempts to define a role for this class of drug in the long-term treatment of HIV-1 disease.},
	Author = {Deeks, S. G.},
	Journal = {J Acquir Immune Defic Syndr},
	Keywords = {Anti-HIV Agents/*pharmacology/therapeutic use Clinical Trials Delavirdine/pharmacology/therapeutic use *Drug Resistance, Microbial Drug Therapy, Combination HIV Infections/drug therapy/transmission HIV-1/*drug effects/genetics/metabolism HIV-1 Reverse Transcriptase/chemistry/genetics Human Nevirapine/pharmacology/therapeutic use Oxazines/pharmacology/therapeutic use Phylogeny Point Mutation/drug effects Protein Conformation Reverse Transcriptase Inhibitors/*pharmacology/therapeutic use Virus Replication/drug effects},
	Note = {1525-4135 Journal Article Review Review, Tutorial},
	Pages = {S25-33},
	Title = {International perspectives on antiretroviral resistance. Nonnucleoside reverse transcriptase inhibitor resistance},
	Volume = {26 Suppl 1},
	Year = {2001}}

@article{Deeksetal02,
	Abstract = {BACKGROUND: Sustained elevations in CD4 cell counts commonly occur despite incomplete viral suppression with protease inhibitor-based antiretroviral therapy. OBJECTIVES: To determine the incidence and risk factors associated with return of CD4 cell count to pre-therapy levels in patients experiencing virologic failure of protease inhibitor therapy. DESIGN: This is a clinic-based cohort study of HIV-infected adults who failed to maintain durable viral suppression on a protease inhibitor-based regimen. MAIN OUTCOME MEASURES: Virologic failure was defined as persistent plasma HIV RNA level > 500 copies/ml. Immunologic failure was defined as return of CD4 cell count to pre-therapy levels. RESULTS: A total of 291 patients experienced virologic failure on a protease inhibitor-based regimen and had a treatment-mediated CD4 cell increase above pre-therapy levels at the time of virologic failure. If patient data were censored at the time a successful salvage regimen was initiated, then the median time to immunologic failure after the onset of virologic failure was 3 years. If patient data were also censored at the time therapy was discontinued, then 36.8% of the cohort experienced immunologic failure after 3 years of continuous virologic failure. The change in viral load from a pre-treatment baseline, and not the absolute level of viremia achieved, was a strong and independent predictor of immunologic failure. Discontinuing therapy was associated with immunologic failure independent of viral load changes. CONCLUSION: Reduction in T CD4+ cell numbers may eventually occur during prolonged virologic failure of a protease inhibitor-based regimen and is predicted by the degree of virologic suppression below a pre-therapy 'set-point'.},
	Author = {Deeks, S. G. and Barbour, J. D. and Grant, R. M. and Martin, J. N.},
	Journal = {Aids},
	Keywords = {Adult Antiretroviral Therapy, Highly Active CD4 Lymphocyte Count CD4-Positive T-Lymphocytes/cytology/*drug effects Disease Progression HIV Infections/blood/*drug therapy/immunology/virology HIV Protease Inhibitors/*therapeutic use HIV-1/*drug effects/genetics Human Indinavir/therapeutic use Nelfinavir/therapeutic use RNA, Viral/blood Ritonavir/therapeutic use Saquinavir/therapeutic use Support, Non-U.S. Gov't Support, U.S. Gov't, P.H.S. Time Factors Treatment Failure Viremia/blood/*drug therapy/immunology/virology},
	Note = {0269-9370 Journal Article},
	Number = {2},
	Pages = {201-7},
	Title = {Duration and predictors of CD4 T-cell gains in patients who continue combination therapy despite detectable plasma viremia},
	Volume = {16},
	Year = {2002}}

@article{Deeks03,
	Abstract = {Drug-resistant HIV-1 is a cause of growing clinical and public-health concern. In many patients, combination antiretroviral therapy fails to achieve complete viral suppression (virological failure). Continuing viral replication during therapy leads to the accumulation of drug-resistance mutations, resulting in increased viral load and a greater risk of disease progression. Patients with drug-resistant HIV-1 infection have three therapeutic options: a change to a salvage regimen with the aim of fully suppressing viral replication; interruption of therapy; or continuation of a partially effective regimen. The first strategy is preferred for most patients failing their first or perhaps their second regimen. However, the best approach remains unclear for patients who have failed multiple treatment regimens and who have limited options for complete viral suppression. The management of such patients requires a careful understanding of the pathogenesis of drug-resistant HIV-1, the clinical consequences of virological failure, the potential benefits and limitations of diagnostic assays, and the likelihood that agents in development will be effective.},
	Author = {Deeks, S. G.},
	Journal = {Lancet},
	Keywords = {Anti-HIV Agents/*immunology/*therapeutic use Antiretroviral Therapy, Highly Active/methods Drug Resistance, Viral/genetics/immunology Drug Therapy, Combination HIV Infections/*drug therapy/immunology/virology HIV Protease Inhibitors/immunology/therapeutic use *HIV-1/drug effects/genetics/immunology Human Randomized Controlled Trials Ritonavir/immunology/therapeutic use Support, Non-U.S. Gov't Support, U.S. Gov't, P.H.S. Treatment Outcome Viral Load/statistics & numerical data Virus Replication/drug effects/immunology},
	Note = {1474-547x Journal Article Review Review, Academic},
	Number = {9400},
	Pages = {2002-11},
	Title = {Treatment of antiretroviral-drug-resistant HIV-1 infection},
	Volume = {362},
	Year = {2003}}

@incollection{robins&Li2008,
address = "Beachwood, Ohio, USA",
author = "Robins, James and Li, Lingling and Tchetgen, Eric and van der Vaart, Aad",
booktitle = "Probability and Statistics: Essays in Honor of David A. Freedman",
doi = "10.1214/193940307000000527",
editor = "Nolan, Deborah and Speed, Terry",
pages = "335--421",
publisher = "Institute of Mathematical Statistics",
series = "Collections",
title = "Higher order influence functions and minimax estimation of nonlinear functionals",
url = "http://dx.doi.org/10.1214/193940307000000527",
volume = "Volume 2",
year = "2008"
}


@article{Deeks&Walker04,
	Abstract = {A potent antigen-specific T cell response to HIV infection can contribute to the control of viral replication and is therefore beneficial to the host. However, HIV-mediated increases in generalized T cell activation also appear to accelerate both viral replication and CD4+ T cell depletion. A new study in the JCI attempts to experimentally distinguish the beneficial versus harmful aspects of this immune response.},
	Author = {Deeks, S. G. and Walker, B. D.},
	Journal = {J Clin Invest},
	Note = {0021-9738 Comment Journal Article},
	Number = {6},
	Pages = {808-10},
	Title = {The immune response to AIDS virus infection: good, bad, or both?},
	Volume = {113},
	Year = {2004}}

@techreport{DHHS04,
	Author = {DHHS},
	Institution = {Panel on Clinical Practices for Treatment of HIV Infection, Department of Health and Human Services},
	Month = {March 23},
	Title = {Guidelines for the use of antiretroviral agents in HIV-1 infected adults and adolescents},
	Year = {2004}}

@article{Faureetal00,
	Abstract = {Human immunodeficiency virus (HIV) enters cells in vitro via CD4 and a coreceptor. Which of 15 known coreceptors are important in vivo is poorly defined but may be inferred from disease-modifying mutations, as for CCR5. Here two single nucleotide polymorphisms are described in Caucasians in CX3CR1, an HIV coreceptor and leukocyte chemotactic/adhesion receptor for the chemokine fractalkine. HIV-infected patients homozygous for CX3CR1-I249 M280, a variant haplotype affecting two amino acids (isoleucine-249 and methionine-280), progressed to AIDS more rapidly than those with other haplotypes. Functional CX3CR1 analysis showed that fractalkine binding is reduced among patients homozygous for this particular haplotype. Thus, CX3CR1-I249 M280 is a recessive genetic risk factor in HIV/AIDS.},
	Author = {Faure, S. and Meyer, L. and Costagliola, D. and Vaneensberghe, C. and Genin, E. and Autran, B. and Delfraissy, J. F. and McDermott, D. H. and Murphy, P. M. and Debre, P. and Theodorou, I. and Combadiere, C.},
	Journal = {Science},
	Keywords = {Acquired Immunodeficiency Syndrome/genetics/*physiopathology/virology Case-Control Studies *Chemokines, CX3C Chemokines, CXC/metabolism Chromosomes, Human, Pair 3 Cohort Studies Disease Progression European Continental Ancestry Group/genetics Genotype HIV/physiology HIV Infections/genetics/*physiopathology/virology Haplotypes Homozygote Human Leukocytes, Mononuclear/metabolism Linkage Disequilibrium Membrane Proteins/metabolism Mutation Polymorphism, Restriction Fragment Length *Polymorphism, Single Nucleotide Polymorphism, Single-Stranded Conformational Receptors, Cytokine/*genetics/*physiology Receptors, HIV/*genetics/*physiology Support, Non-U.S. Gov't Survival Analysis Variation (Genetics)},
	Note = {0036-8075 Comment Journal Article},
	Number = {5461},
	Pages = {2274-7},
	Title = {Rapid progression to AIDS in HIV+ individuals with a structural variant of the chemokine receptor CX3CR1},
	Volume = {287},
	Year = {2000}}

@article{Gaoetal01,
	Abstract = {BACKGROUND: From studies of genetic polymorphisms and the rate of progression from human immunodeficiency virus type 1 (HIV-1) infection to the acquired immunodeficiency syndrome (AIDS), it appears that the strongest susceptibility is conferred by the major-histocompatibility-complex (MHC) class I type HLA-B*35,Cw*04 allele. However, cytotoxic T-lymphocyte responses have been observed against HIV-1 epitopes presented by HLA-B*3501, the most common HLA-B*35 subtype. We examined subtypes of HLA-B*35 in five cohorts and analyzed the relation of structural differences between HLA-B*35 subtypes to the risk of progression to AIDS. METHODS: Genotyping of HLA class I loci was performed for 850 patients who seroconverted and had known dates of HIV-1 infection. Survival analyses with respect to the rate of progression to AIDS were performed to identify the effects of closely related HLA-B*35 subtypes with different peptide-binding specificities. RESULTS: HLA-B*35 subtypes were divided into two groups according to peptide-binding specificity: the HLA-B*35-PY group, which consists primarily of HLA-B*3501 and binds epitopes with proline in position 2 and tyrosine in position 9; and the more broadly reactive HLA-B*35-Px group, which also binds epitopes with proline in position 2 but can bind several different amino acids (not including tyrosine) in position 9. The influence of HLA-B*35 in accelerating progression to AIDS was completely attributable to HLA-B*35-Px alleles, some of which differ from HLA-B*35-PY alleles by only one amino acid residue. CONCLUSIONS: This analysis shows that, in patients with HIV-1 infection, a single amino acid change in HLA molecules has a substantial effect on the rate of progression to AIDS. The different consequences of HLA-B*35-PY and HLA-B*35-Px in terms of disease progression highlight the importance of the epitope specificities of closely related class I molecules in the immune defense against HIV-1.},
	Author = {Gao, X. and Nelson, G. W. and Karacki, P. and Martin, M. P. and Phair, J. and Kaslow, R. and Goedert, J. J. and Buchbinder, S. and Hoots, K. and Vlahov, D. and O'Brien, S. J. and Carrington, M.},
	Journal = {N Engl J Med},
	Keywords = {Acquired Immunodeficiency Syndrome/*genetics African Continental Ancestry Group/genetics Alleles Amino Acid Sequence Binding Sites/genetics Disease Progression Disease-Free Survival European Continental Ancestry Group/genetics *Genes, MHC Class I Genotype HIV Infections/ethnology/*genetics/immunology HLA-B35 Antigen/chemistry/*genetics HLA-C Antigens Human Peptides/metabolism Proportional Hazards Models Receptors, Peptide/chemistry/genetics/metabolism Support, U.S. Gov't, P.H.S.},
	Note = {0028-4793 Journal Article Multicenter Study},
	Number = {22},
	Pages = {1668-75},
	Title = {Effect of a single amino acid change in MHC class I molecules on the rate of progression to AIDS},
	Volume = {344},
	Year = {2001}}

@article{Grabaretal00,
	Abstract = {BACKGROUND: The prognostic value of discordant immunologic (CD4 cell increase) and virologic (plasma HIV RNA level decrease) responses to antiretroviral treatment is not known. OBJECTIVE: To study the relation between clinical outcome of HIV-infected patients receiving highly active antiretroviral therapy (HAART) and early immunologic and virologic responses to such therapy. DESIGN: Prospective cohort study. SETTING: 68 hospitals in France. PATIENTS: 2236 protease inhibitor-naive patients. INTERVENTION: Initiation of HAART with one protease inhibitor and two nucleoside analogues between July 1996 and March 1997. MEASUREMENTS: Immunologic and virologic response at 6 months. Multivariate Cox models were used to assess the relation between these responses and progression to a new AIDS-defining event or death. RESULTS: On the basis of 6-month immunologic and virologic responses, patients were classified into four groups: complete response (47.5%), complete nonresponse (16.2%), immunologic response only (19.0%), and virologic response only (17.3%). After month 6 and within a median of 18 months, 69 patients died and 123 experienced a new AIDS-defining event. After adjustment, complete nonresponders and those with only a virologic response had significantly higher risks for clinical progression at 6 months (relative risk, 3.38 [95% CI, 2.28 to 5.02] and 1.98 [CI, 1.26 to 3.10], respectively) than complete responders. The difference between complete responders and those with only an immunologic response at 6 months was weaker and nonsignificant (relative risk, 1.55 [CI, 0.96 to 2.50]). CONCLUSIONS: Immunologic response after 6 months of HAART indicates a favorable clinical outcome in HIV-infected patients regardless of virologic response. This suggests that both immunologic and virologic markers should be used in clinical practice to evaluate treatment response.},
	Author = {Grabar, S. and Le Moing, V. and Goujard, C. and Leport, C. and Kazatchkine, M. D. and Costagliola, D. and Weiss, L.},
	Journal = {Ann Intern Med},
	Keywords = {Adult CD4 Lymphocyte Count Disease Progression Drug Therapy, Combination Female HIV Infections/*drug therapy/immunology/virology HIV Protease Inhibitors/*therapeutic use *HIV-1/genetics Human Male Multivariate Analysis Proportional Hazards Models Prospective Studies RNA, Viral/blood Reverse Transcriptase Inhibitors/*therapeutic use Support, Non-U.S. Gov't Treatment Outcome Viral Load},
	Note = {0003-4819 Journal Article Multicenter Study},
	Number = {6},
	Pages = {401-10},
	Title = {Clinical outcome of patients with HIV-1 infection according to immunologic and virologic response after 6 months of highly active antiretroviral therapy},
	Volume = {133},
	Year = {2000}}

@article{Gruebetal00,
	Abstract = {BACKGROUND: Hepatitis C virus (HCV) infection is highly prevalent among HIV-1-infected individuals, but its contribution to the morbidity and mortality of coinfected patients who receive potent antiretroviral therapy is controversial. We used data from the ongoing Swiss HIV Cohort Study to analyse clinical progression of HIV-1, and the virological and immunological response to potent antiretroviral therapy in HIV-1-infected patients with or without concurrent HCV infection. METHODS: We analysed prospective data on survival, clinical disease progression, suppression of HIV-1 replication, CD4-cell recovery, and frequency of changes in antiretroviral therapy according to HCV status in 3111 patients starting potent antiretroviral therapy. RESULTS: 1157 patients (37.2%) were coinfected with HCV, 1015 of whom (87.7%) had a history of intravenous drug use. In multivariate Cox's regression, the probability of progression to a new AIDS-defining clinical event or to death was independently associated with HCV seropositivity (hazard ratio 1.7 [95% CI 1.26-2.30]), and with active intravenous drug use (1.38 [1.02-1.88]). Virological response to antiretroviral therapy and the probability of treatment change were not associated with HCV serostatus. In contrast, HCV seropositivity was associated with a smaller CD4-cell recovery (hazard ratio for a CD4-cell count increase of at least 50 cells/microL=0.79 [0.72-0.87]). INTERPRETATION: HCV and active intravenous drug use could be important factors in the morbidity and mortality among HIV-1-infected patients, possibly through impaired CD4-cell recovery in HCV seropositive patients receiving potent antiretroviral therapy. These findings are relevant for decisions about optimum timing for HCV treatment in the setting of HIV infection.},
	Author = {Greub, G. and Ledergerber, B. and Battegay, M. and Grob, P. and Perrin, L. and Furrer, H. and Burgisser, P. and Erb, P. and Boggian, K. and Piffaretti, J. C. and Hirschel, B. and Janin, P. and Francioli, P. and Flepp, M. and Telenti, A.},
	Journal = {Lancet},
	Keywords = {AIDS-Related Opportunistic Infections/*drug therapy Adolescent Adult Anti-HIV Agents/*therapeutic use CD4 Lymphocyte Count Cohort Studies Disease Progression Female Hepatitis C/complications/*drug therapy Human Male Middle Aged Prospective Studies Support, Non-U.S. Gov't Survival Analysis Switzerland Viral Load Viremia/etiology},
	Note = {0140-6736 Clinical Trial Journal Article},
	Number = {9244},
	Pages = {1800-5},
	Title = {Clinical progression, survival, and immune recovery during antiretroviral therapy in patients with HIV-1 and hepatitis C virus coinfection: the Swiss HIV Cohort Study},
	Volume = {356},
	Year = {2000}}

@article{Katzensteinetal96,
	Abstract = {BACKGROUND: We studied measures of human immunodeficiency virus (HIV) replication, the viral phenotype, and immune function (CD4 cell counts) and the relation of changes in these indicators to clinical outcomes in a subgroup of patients in a controlled trial of early antiretroviral treatment for HIV, the AIDS Clinical Trials Group Study 175. METHODS: The 391 subjects, each of whom entered the study with a single screening CD4 cell count of 200 to 500 per cubic millimeter, were randomly assigned to receive zidovudine alone, didanosine alone, zidovudine plus didanosine, or zidovudine plus zalcitabine. Plasma concentrations of HIV RNA were assessed in 366 subjects, and viral isolates from 332 subjects were assayed for the presence of the syncytium-inducing phenotype. RESULTS: After eight weeks, the mean (+/-SE) decrease from base line in the concentration of HIV RNA, expressed as the change in the base 10 log of the number of copies per milliliter, was 0.26+/-0.06 for patients treated with zidovudine alone, 0.65+/-0.07 for didanosine alone, 0.93+/-0.10 for zidovudine plus didanosine, and 0.89+/-0.06 for zidovudine plus zalcitabine (P<0.001 for each of the pairwise comparisons with zidovudine alone). Multivariate proportional-hazards models showed that higher base-line concentrations of plasma HIV RNA, less suppression of plasma HIV RNA by treatment, and the presence of the syncytium-inducing phenotype were significantly associated with an increased risk of progression to the acquired immunodeficiency syndrome and death. After adjustment for these measures of viral replication and for the viral phenotype, CD4 cell counts were not significant predictors of clinical outcome. CONCLUSIONS: Both the risk of the progression of HIV disease and the efficacy of antiretroviral therapy are strongly associated with the plasma level of HIV RNA and with the viral phenotype. The changes in the plasma concentration of HIV RNA predict the changes in CD4 cell counts and survival after treatment with reverse-transcriptase inhibitors.},
	Author = {Katzenstein, D. A. and Hammer, S. M. and Hughes, M. D. and Gundacker, H. and Jackson, J. B. and Fiscus, S. and Rasheed, S. and Elbeik, T. and Reichman, R. and Japour, A. and Merigan, T. C. and Hirsch, M. S.},
	Journal = {N Engl J Med},
	Keywords = {Adult Antiviral Agents/*therapeutic use CD4 Lymphocyte Count Didanosine/*therapeutic use Disease Progression Drug Therapy, Combination Female HIV/*genetics/isolation & purification/physiology HIV Infections/drug therapy/immunology/*virology Human Male Middle Aged Multivariate Analysis Phenotype Proportional Hazards Models RNA, Viral/*blood Support, U.S. Gov't, P.H.S. Treatment Outcome Virus Replication/drug effects Zidovudine/*therapeutic use},
	Note = {0028-4793 Clinical Trial Journal Article Multicenter Study Randomized Controlled Trial},
	Number = {15},
	Pages = {1091-8},
	Title = {The relation of virologic and immunologic markers to clinical outcomes after nucleoside therapy in HIV-infected adults with 200 to 500 CD4 cells per cubic millimeter. AIDS Clinical Trials Group Study 175 Virology Study Team},
	Volume = {335},
	Year = {1996}}

@article{Kaufmannetal98,
	Author = {Kaufmann, D. and Pantaleo, G. and Sudre, P. and Telenti, A.},
	Journal = {Lancet},
	Keywords = {Anti-HIV Agents/*therapeutic use CD4 Lymphocyte Count HIV Infections/drug therapy/*immunology Human Protease Inhibitors/*therapeutic use Support, Non-U.S. Gov't Viremia/drug therapy/*immunology},
	Note = {0140-6736 Letter},
	Number = {9104},
	Pages = {723-4},
	Title = {CD4-cell count in HIV-1-infected individuals remaining viraemic with highly active antiretroviral therapy (HAART). Swiss HIV Cohort Study},
	Volume = {351},
	Year = {1998}}

@article{Kaufmannetal03,
	Abstract = {BACKGROUND: Highly active antiretroviral therapy (HAART) for human immunodeficiency virus (HIV)-1 infection allows recovery of CD4 T lymphocytes. Few studies have explored the long-term T-lymphocyte responses to HAART. METHODS: Plasma HIV-1 RNA levels and CD4 and CD8 T-lymphocyte counts were longitudinally analyzed over 4 years in 2235 participants of the Swiss HIV Cohort, commencing HAART between 1996 and 1997. The CD4 T-lymphocyte count increase, the percentage of individuals with a CD4 T-lymphocyte count of 500/microL or greater and less than 200/microL, and the determinants of CD4 T-lymphocyte recovery were evaluated in individuals treated with continuous (CONT; n = 985) and discontinuous (DISCONT; n = 1250) HAART. RESULTS: At 4 years, 69.5% of subjects (CONT, 84.5%; DISCONT, 53.6%; P<.001) showed HIV-1 RNA levels below 400 copies/mL, while the median CD4 T-lymphocyte count increased from 190/microL to 423/microL (CONT, 486/microL; DISCONT, 343/microL; P<.001). Of the 2235 participants, 38.8% (CONT, 47.7%; DISCONT, 29.4%; P<.001) reached a CD4 T-lymphocyte count of 500/microL or greater, but in 15.6%, CD4 T-lymphocyte count remained below 200/microL (CONT, 5.9%; DISCONT, 25.9%; P<.001). Larger increases in CD4 T-lymphocyte count were associated with higher baseline HIV-1 RNA, a larger percentage of undetectable HIV-1 RNA levels, lower baseline CD8 T-lymphocyte count, and younger age. Individuals reaching a CD4 T-lymphocyte count of 500/microL or greater at 4 years were characterized by higher nadir and baseline CD4 T-lymphocyte counts and a more sustained reduction of HIV-1 RNA levels. CONCLUSIONS: At 4 years, only 39% of individuals treated with HAART reached a CD4 T-lymphocyte count of 500/microL or greater, and 16% with CD4 T-lymphocyte counts less than 200/microL remained susceptible to opportunistic infections. Treatment interruptions, a poor virologic response, and older age were the major factors negatively affecting the recovery of CD4 T lymphocytes.},
	Author = {Kaufmann, G. R. and Perrin, L. and Pantaleo, G. and Opravil, M. and Furrer, H. and Telenti, A. and Hirschel, B. and Ledergerber, B. and Vernazza, P. and Bernasconi, E. and Rickenbach, M. and Egger, M. and Battegay, M.},
	Journal = {Arch Intern Med},
	Keywords = {Adult *Antiretroviral Therapy, Highly Active *CD4 Lymphocyte Count CD8-Positive T-Lymphocytes Female HIV Infections/*drug therapy/*immunology *Hiv-1 Human Lymphocyte Count Male Middle Aged Prospective Studies RNA, Viral/*analysis Support, Non-U.S. Gov't Viral Load},
	Note = {0003-9926 Journal Article},
	Number = {18},
	Pages = {2187-95},
	Title = {CD4 T-lymphocyte recovery in individuals with advanced HIV-1 infection receiving potent antiretroviral therapy for 4 years: the Swiss HIV Cohort Study},
	Volume = {163},
	Year = {2003}}

@article{MartinezPicadoetal99,
	Abstract = {The relative replicative fitness of human immunodeficiency virus type 1 (HIV-1) mutants selected by different protease inhibitors (PIs) in vivo was determined. Each mutant was compared to wild type (WT), NL4-3, in the absence of drugs by several methods, including clonal genotyping of cultures infected with two competing viral variants, kinetics of viral antigen production, and viral infectivity/virion particle ratios. A nelfinavir-selected protease D30N substitution substantially decreased replicative capacity relative to WT, while a saquinavir-selected L90M substitution moderately decreased fitness. The D30N mutant virus was also outcompeted by the L90M mutant in the absence of drugs. A major natural polymorphism of the HIV-1 protease, L63P, compensated well for the impairment of fitness caused by L90M but only slightly improved the fitness of D30N. Multiply substituted indinavir-selected mutants M46I/L63P/V82T/I84V and L10R/M46I/L63P/V82T/I84V were just as fit as WT. These results indicate that the mutations which are usually initially selected by nelfinavir and saquinavir, D30N and L90M, respectively, impair fitness. However, additional mutations may improve the replicative capacity of these and other drug-resistant mutants. Hypotheses based on the greater fitness impairment of the nelfinavir-selected D30N mutant are suggested to explain observations that prolonged responses to delayed salvage regimens, including alternate PIs, may be relatively common after nelfinavir failure.},
	Author = {Martinez-Picado, J. and Savara, A. V. and Sutton, L. and D'Aquila, R. T.},
	Journal = {J Virol},
	Keywords = {Adaptation, Biological Amino Acid Substitution Animals Anti-HIV Agents/*pharmacology Cells, Cultured Drug Resistance, Microbial HIV Protease Inhibitors/*pharmacology HIV-1/*drug effects/genetics/physiology Human Mice Mutagenesis, Site-Directed Nelfinavir/*pharmacology Saquinavir/*pharmacology Support, Non-U.S. Gov't Support, U.S. Gov't, P.H.S. Tumor Cells, Cultured Virus Replication/*drug effects},
	Note = {0022-538x Journal Article},
	Number = {5},
	Pages = {3744-52},
	Title = {Replicative fitness of protease inhibitor-resistant mutants of human immunodeficiency virus type 1},
	Volume = {73},
	Year = {1999}}

@article{Mellorsetal96,
	Abstract = {The relation between viremia and clinical outcome in individuals infected with human immunodeficiency virus-type 1 (HIV-1) has important implications for therapeutic research and clinical care. HIV-1 RNA in plasma was quantified with a branched-DNA signal amplification assay as a measure of viral load in a cohort of 180 seropositive men studied for more than 10 years. The risk of acquired immunodeficiency syndrome (AIDS) and death in study subjects, including those with normal numbers of CD4+ T cells, was directly related to plasma viral load at study entry. Plasma viral load was a better predictor of progression to AIDS and death than was the number of CD4+ T cells.},
	Author = {Mellors, J. W. and Rinaldo, C. R., Jr. and Gupta, P. and White, R. M. and Todd, J. A. and Kingsley, L. A.},
	Journal = {Science},
	Keywords = {Acquired Immunodeficiency Syndrome/*virology Antiviral Agents/therapeutic use Biological Markers/blood CD4 Lymphocyte Count CD4-Positive T-Lymphocytes/virology Cohort Studies Disease Progression Follow-Up Studies HIV Infections/drug therapy/mortality/*virology HIV-1/genetics/*physiology Human Male Prognosis Proportional Hazards Models RNA, Viral/*blood Support, Non-U.S. Gov't Support, U.S. Gov't, Non-P.H.S. Support, U.S. Gov't, P.H.S. Survival Rate Time Factors Viremia/*virology Virus Replication},
	Note = {0036-8075 Comment Journal Article},
	Number = {5265},
	Pages = {1167-70},
	Title = {Prognosis in HIV-1 infection predicted by the quantity of virus in plasma},
	Volume = {272},
	Year = {1996}}

@article{Milleretal00,
	Abstract = {OBJECTIVE: To compare the rate of disease progression according to viral load and CD4 cell count in patients receiving or not receiving highly active antiretroviral therapy (HAART), defined as protease inhibitor-containing regimens. DESIGN: An observational study, with prospectively collected data. METHODS: All patients attending the HIV Outpatient clinic as of 1 January 1995 (n = 2083) were included. Follow-up was until the first AIDS-defining event or death. Associations between viral load or CD4 cell count and disease progression were assessed using a person-years approach. Event rates were compared using Poisson regression analysis; a multivariate model was used to assess the independent effects of CD4, viral load and treatment group on event rates and to consider interactions between these variables. RESULTS: The event rates increased with lower CD4 cell count and higher viral load for both treatment groups and were generally lower in the HAART group. In a multivariate analysis, lower CD4 cell counts and higher viral loads remained significantly associated with disease progression, irrespective of treatment group. However, the event rate was significantly lower for the HAART group compared with the control group (relative rate 0.53, P < 0.001). CONCLUSIONS: HAART-treated patients with high viral loads and CD4 cell counts experienced reduced disease progression compared with individuals with the same CD4 cell count and viral load not receiving HAART. Consequently, the short-term prognosis associated with viral load levels and CD4 cell counts may differ in patients on HAART. Whether this effect will be observed with non-protease-inhibitor-containing HAART is not known at this time.},
	Author = {Miller, V. and Sabin, C. A. and Phillips, A. N. and Rottmann, C. and Rabenau, H. and Weidmann, E. and Rickerts, V. and Findhammer, S. and Helm, E. B. and Staszewski, S.},
	Journal = {Aids},
	Keywords = {Adolescent Adult Aged Antiretroviral Therapy, Highly Active CD4 Lymphocyte Count Disease Progression HIV Infections/*drug therapy/pathology/virology HIV Protease Inhibitors/*therapeutic use *HIV-1/isolation & purification Human Middle Aged Prospective Studies RNA, Viral/analysis Regression Analysis Support, Non-U.S. Gov't Viral Load},
	Note = {0269-9370 Clinical Trial Journal Article},
	Number = {14},
	Pages = {2129-36},
	Title = {The impact of protease inhibitor-containing highly active antiretroviral therapy on progression of HIV disease and its relationship to CD4 and viral load},
	Volume = {14},
	Year = {2000}}

@article{Pikettyetal98,
	Abstract = {OBJECTIVES: To determine the clinical, virological and immunological outcome in a cohort of unselected patients receiving triple combination therapy for more than 1 year. METHODS: Prospective follow-up of a cohort of 162 unselected, protease inhibitor-naive, antiretroviral-experienced patients with advanced HIV disease, treated with indinavir combined with two nucleoside analogues. RESULTS: The mean CD4 cell count and plasma HIV RNA level in the study group at baseline were 69+/-5 x 10(6)/l and 4.75+/-0.07 log10 copies/ml, respectively. Five per cent of patients died prematurely or were lost to follow-up. Fifty-seven per cent of patients responded to therapy, as assessed by a sustained increase in CD4 cell counts above 50 x 10(6)/l and a decrease in plasma HIV RNA greater than 1 log10 copies/ml, throughout 12.1 months of follow-up. Seventeen per cent of patients were immunological and virological non-responders. Twenty-one per cent of patients exhibited discrepant virological and immunological responses to treatment, of whom one-half failed to exhibit significant increases in CD4 cells despite a virological response to therapy and one-half exhibited increased CD4 cell counts in the absence of significant decrease in plasma viral load. The incidence of AIDS-defining events in the latter group of patients was similar to that of responder patients, whereas their incidence was higher in patients who failed to exhibit a virological and immunological response and those who failed to increase CD4 cells despite a significant decrease in viral load. CONCLUSION: Our observations of discrepant immunological and virological responses to treatment raise the issue of the significance of persistent elevated levels of plasma HIV RNA and of the relevance of measurements of plasma viral load for assessing the efficacy of antiretroviral therapy in patients whose CD4 cell counts increase despite the absence of significant decrease in plasma HIV viral load.},
	Author = {Piketty, C. and Castiel, P. and Belec, L. and Batisse, D. and Si Mohamed, A. and Gilquin, J. and Gonzalez-Canali, G. and Jayle, D. and Karmochkine, M. and Weiss, L. and Aboulker, J. P. and Kazatchkine, M. D.},
	Journal = {Aids},
	Keywords = {Adult Aged Anti-HIV Agents/*therapeutic use Cohort Studies Drug Therapy, Combination Female Follow-Up Studies HIV Infections/*drug therapy/immunology/physiopathology/virology HIV Protease Inhibitors/*therapeutic use Human Indinavir/*therapeutic use Lamivudine/*therapeutic use Male Middle Aged Prospective Studies Reverse Transcriptase Inhibitors/*therapeutic use Stavudine/*therapeutic use Support, Non-U.S. Gov't Treatment Outcome Zidovudine/*therapeutic use},
	Note = {0269-9370 Journal Article},
	Number = {7},
	Pages = {745-50},
	Title = {Discrepant responses to triple combination antiretroviral therapy in advanced HIV disease},
	Volume = {12},
	Year = {1998}}

@article{Pikettyetal01,
	Abstract = {Within a prospective cohort of 150 human immunodeficiency virus (HIV)-infected patients who began first-line protease inhibitor therapy in 1996, the outcome of 42 patients with discrepant virologic and immunologic responses to antiretroviral treatment at 12 months was analyzed at 30 months of treatment. The incidence of AIDS-defining events and deaths (14%) in the group of patients with immunologic responses in the absence of a virologic response was higher than that in full-responder patients (2%); yet, the incidence in this group was lower than that in patients with no immunologic response, despite a virologic response (21%), and was lower than that in patients without an immunologic or virologic response (67%; P<.0001, log-rank test). Differences in outcome were significant (relative risk, 6.9; 95% confidence interval, 1.9-39.3) when factors for progression were compared with those of responder patients. The results support the relevance of the CD4 cell marker over plasma HIV load for predicting clinical outcome in patients who do not achieve full immunologic and virologic responses.},
	Author = {Piketty, C. and Weiss, L. and Thomas, F. and Mohamed, A. S. and Belec, L. and Kazatchkine, M. D.},
	Journal = {J Infect Dis},
	Keywords = {Adult Aged Antiretroviral Therapy, Highly Active CD4 Lymphocyte Count Cohort Studies Disease Progression Female HIV Infections/*drug therapy/immunology/virology HIV Protease Inhibitors/*therapeutic use Human Incidence Longitudinal Studies Male Middle Aged Mortality Prospective Studies RNA, Viral/blood Time Factors Treatment Outcome Viral Load},
	Note = {0022-1899 Journal Article},
	Number = {9},
	Pages = {1328-35},
	Title = {Long-term clinical outcome of human immunodeficiency virus-infected patients with discordant immunologic and virologic responses to a protease inhibitor-containing regimen},
	Volume = {183},
	Year = {2001}}

@article{Pilonetal02,
	Abstract = {Inhibition of human immunodeficiency virus type 1 reverse transcriptase (RT) by both nucleoside and nonnucleoside RT inhibitors profoundly inhibits virus replication. Nucleoside RT inhibitors are known to be toxic, but there is little information regarding the toxicities of nonnucleoside RT inhibitors (NNRTI). We demonstrate that efavirenz (an NNRTI) induces caspase- and mitochondrion-dependent apoptosis of Jurkat T cells and human peripheral blood mononuclear cells. The clinical relevance of these observations is not yet clear.},
	Author = {Pilon, A. A. and Lum, J. J. and Sanchez-Dardon, J. and Phenix, B. N. and Douglas, R. and Badley, A. D.},
	Journal = {Antimicrob Agents Chemother},
	Keywords = {Annexin V/diagnostic use Apoptosis/*drug effects Caspases/physiology Enzyme Inhibitors/diagnostic use Fluorescein-5-isothiocyanate Fluorescent Dyes HIV-1 Reverse Transcriptase/*antagonists & inhibitors Human Jurkat Cells Membrane Potentials/drug effects Mitochondria/drug effects/physiology Oxazines/*pharmacology Reverse Transcriptase Inhibitors/*pharmacology Support, Non-U.S. Gov't},
	Note = {0066-4804 Journal Article},
	Number = {8},
	Pages = {2687-91},
	Title = {Induction of apoptosis by a nonnucleoside human immunodeficiency virus type 1 reverse transcriptase inhibitor},
	Volume = {46},
	Year = {2002}}

@article{Priceetal03,
	Abstract = {Many individuals chronically infected with human immunodeficiency virus type 1 (HIV-1) experience a recrudescence of plasma virus during continuous combination antiretroviral therapy (ART) due either to the emergence of drug-resistant viruses or to poor compliance. In most cases, virologic failure on ART is associated with a coincident decline in CD4(+) T lymphocyte levels. However, a proportion of discordant individuals retain a stable or even increasing CD4(+) T lymphocyte count despite virological failure. In order to address the nature of these different outcomes, we evaluated virologic and immunologic variables in a prospective, single-blinded, nonrandomized cohort of 53 subjects with chronic HIV-1 infection who had been treated with continuous ART and monitored intensively over a period of 19 months. In all individuals with detectable viremia on ART, multiple drug resistance mutations with similar impacts on viral growth kinetics were detected in the pol gene of circulating plasma virus. Further, C2V3 env gene analysis demonstrated sequences indicative of CCR5 coreceptor usage in the majority of those with detectable plasma viremia. In contrast to this homogeneous virologic pattern, comprehensive screening with a range of antigens derived from HIV-1 revealed substantial immunologic differences. Discordant subjects with stable CD4(+) T lymphocyte counts in the presence of recrudescent virus demonstrated potent virus-specific CD4(+) and CD8(+) T lymphocyte responses. In contrast, subjects with virologic failure associated with declining CD4(+) T lymphocyte counts had substantially weaker HIV-specific CD4(+) T lymphocyte responses and exhibited a trend towards weaker HIV-specific CD8(+) T lymphocyte responses. Importantly the CD4(+) response was sustained over periods as long as 11 months, confirming the stability of the phenomenon. These correlative data lead to the testable hypothesis that the consequences of viral recrudescence during continuous ART are modulated by the HIV-specific cellular immune response.},
	Author = {Price, D. A. and Scullard, G. and Oxenius, A. and Braganza, R. and Beddows, S. A. and Kazmi, S. and Clarke, J. R. and Johnson, G. E. and Weber, J. N. and Phillips, R. E.},
	Journal = {J Virol},
	Keywords = {Adult Amino Acid Sequence Anti-HIV Agents/pharmacology/*therapeutic use CD4-Positive T-Lymphocytes/*immunology CD8-Positive T-Lymphocytes/*immunology Chronic Disease Drug Resistance, Viral/genetics Drug Therapy, Combination HIV Envelope Protein gp120/chemistry/genetics HIV Infections/*drug therapy/immunology/physiopathology HIV-1/*drug effects/genetics/physiology Human Lymphocyte Count Middle Aged Molecular Sequence Data Mutation Peptide Fragments/chemistry/genetics Prospective Studies RNA, Viral/blood Single-Blind Method Support, Non-U.S. Gov't *Treatment Failure Viral Load},
	Note = {0022-538x Clinical Trial Journal Article},
	Number = {10},
	Pages = {6041-9},
	Title = {Discordant outcomes following failure of antiretroviral therapy are associated with substantial differences in human immunodeficiency virus-specific cellular immunity},
	Volume = {77},
	Year = {2003}}

@article{Quinonesetal00,
	Abstract = {This study was designed to examine the impact of human immunodeficiency virus type 1 (HIV-1) fitness on disease progression through the use of a dual competition/heteroduplex tracking assay (HTA). Despite numerous studies on the impact of HIV-1 diversity and HIV-specific immune response on disease progression, we still do not have a firm understanding of the long-term pathogenesis of this virus. Strong and early CD8-positive cytotoxic T-cell and CD4-positive T-helper cell responses directed toward HIV-infected cells appear to curb HIV pathogenesis. However, the rate at which the virus infects the CD4(+) T-cell population and possibly destroys the HIV-specific immune response may also alter the rate of disease progression. For HIV-1 fitness studies, we established conditions for dual HIV-1 infections of peripheral blood mononuclear cells (PBMC) and a sensitive HTA to measure relative virus production. A pairwise comparison was then performed to estimate the relative fitness of various non-syncytium-inducing/CCR5-tropic (NSI/R5) and syncytium-inducing/CXCR4-tropic (SI/X4) HIV-1 isolates. Four HIV-1 strains (two NSI/R5 and two SI/X4) with moderate ex vivo fitness were then selected as controls and competed against primary HIV-1 isolates from an HIV-infected Belgian cohort. HIV-1 isolates from long-term survivors (LTS) were outcompeted by control strains and were significantly less fit than HIV-1 isolates from patients with accelerated progression to AIDS (PRO). In addition, NSI/R5 HIV-1 isolates from PRO overgrew control SI/X4 strains, suggesting that not all SI/X4 HIV-1 isolates replicate more efficiently than all NSI/R5 isolates. Finally, there were strong, independent correlations between viral load and the total relative fitness values of HIV-1 isolates from PRO (r = 0.84, P = 0.033) and LTS (r = 0.86, P = 0.028). Separation of the PRO and LTS plots suggest that HIV-1 fitness together with viral load may be a strong predictor for the rate of disease progression.},
	Author = {Quinones-Mateu, M. E. and Ball, S. C. and Marozsan, A. J. and Torre, V. S. and Albright, J. L. and Vanham, G. and van Der Groen, G. and Colebunders, R. L. and Arts, E. J.},
	Journal = {J Virol},
	Keywords = {*Biological Assay HIV Infections/*physiopathology/*virology *HIV-1/physiology Human Predictive Value of Tests Prognosis Support, Non-U.S. Gov't Support, U.S. Gov't, P.H.S.},
	Note = {0022-538x Journal Article},
	Number = {19},
	Pages = {9222-33},
	Title = {A dual infection/competition assay shows a correlation between ex vivo human immunodeficiency virus type 1 fitness and disease progression},
	Volume = {74},
	Year = {2000}}

@article{Racinanetal02,
	Abstract = {OBJECTIVE: To study whether hepatitis C virus (HCV) co-infection or the severe elevation of transaminases is associated with survival after the initiation of antiretroviral combination therapy. DESIGN: Prospective hospital-based cohort (Aquitaine Cohort). METHODS: HIV-infected adults started on an antiretroviral combination before 30 June 1999. HCV infection was defined as antibody detection or positive HCV RNA. Severe elevation of transaminases was defined as a value of aspartate or alanine aminotransferase (AST, ALT) above five times the upper limit of normal values. Survival was studied using a Cox model, including at least baseline HCV status and transaminases as a time-dependent covariate. RESULTS: Overall, 995 patients were analysed, including 576 HCV-positive individuals (58%). At baseline, HCV-positive patients were younger, more often injecting drug users and women, and had more frequently elevated transaminases. A shorter survival was associated with AIDS stage [hazard ratio (HR) versus non-AIDS 1.67; 95% confidence interval (CI) 1.03; 2.68], lower CD4 cell count (HR for 50 cells/mm3 lower 1.33; CI 1.17; 1.51), lower haemoglobin (HR for 1 g/dl lower 1.20; CI 1.07; 1.35), lower platelet count (HR for 10 000 cells/mm3 lower 1.04; CI 1.01; 1.07), and AST during follow-up (HR for > or = 200 IU/l 2.30; CI 1.32; 4.03). HCV co-infection (HR 1.20; CI 0.75; 1.92) was not statistically associated with survival. CONCLUSION: The occurrence of a severe elevation of transaminases was associated with poorer survival, although HCV was not. If liver toxicity may be treatment induced, plasma drug concentrations could guide dosage adjustments of antiretroviral treatments currently prescribed to optimize their use.},
	Author = {Rancinan, C. and Neau, D. and Saves, M. and Lawson-Ayayi, S. and Bonnet, F. and Mercie, P. and Dupon, M. and Couzigou, P. and Dabis, F. and Chene, G.},
	Journal = {Aids},
	Keywords = {Acquired Immunodeficiency Syndrome/complications Age Factors Anti-HIV Agents/*therapeutic use Antiretroviral Therapy, Highly Active Cohort Studies Comparative Study Disease Progression Female Follow-Up Studies HIV Infections/blood/*complications/*drug therapy Hepatitis C/blood/*complications Human Male Proportional Hazards Models Substance Abuse, Intravenous Support, Non-U.S. Gov't Survival Analysis Transaminases/blood},
	Note = {0269-9370 Journal Article},
	Number = {10},
	Pages = {1357-62},
	Title = {Is hepatitis C virus co-infection associated with survival in HIV-infected patients treated by combination antiretroviral therapy?},
	Volume = {16},
	Year = {2002}}

@article{Rogeretal99,
	Abstract = {HAART may increase CD4+ T cell counts despite a persistently detectable HIV load. The impact of HAART on apoptosis, which may play a role in the disease process in HIV-infected patients, has not been extensively studied. We performed a study to compare the level of spontaneous T cell apoptosis and anti-retroviral treatments in a cohort of HIV-1-infected patients. Data were obtained from a computerized medical record. Quantification of apoptotic cells was by cytofluorometric technique. From November 1995 to December 1997 we studied T cell apoptosis in 112 HIV-infected patients. Forty patients were classified A, 36 B and 36 C. Thirty patients were naive and 82 received an anti-retroviral treatment, 49 including a protease inhibitor (PI). The median plasma viraemia determined in 63 patients was 3.6 (range 1.3-5.6) log10. The median apoptotic cell count was 22% (range 2-73%) and 12% (range 2-60%) for CD4+ and CD8+ T cells, respectively. We did not observe any correlation between the HIV viraemia and the level of apoptosis of T cell subsets. Patients with HAART showed a lower percentage of apoptotic CD4+ T cells only: 16% (range 2-61%) versus 25% (range 5-73%) for patients receiving two nucleoside analogues (P = 0.02). This effect was significant in stage A patients and remained observable during the whole course of HIV disease. In conclusion, HAART, without any relation to plasma viraemia, is able to reduce apoptosis of CD4+ T cells.},
	Author = {Roger, P. M. and Breittmayer, J. P. and Arlotto, C. and Pugliese, P. and Pradier, C. and Bernard-Pomier, G. and Dellamonica, P. and Bernard, A.},
	Journal = {Clin Exp Immunol},
	Keywords = {Adult Aged Anti-HIV Agents/*therapeutic use *Apoptosis CD4-Positive T-Lymphocytes/cytology/*drug effects CD8-Positive T-Lymphocytes/drug effects Didanosine/therapeutic use Drug Therapy, Combination Female HIV Infections/*drug therapy/immunology/pathology HIV Protease Inhibitors/therapeutic use Human Lamivudine/therapeutic use Male Middle Aged Multivariate Analysis Retrospective Studies Stavudine/therapeutic use Viral Load Zalcitabine/therapeutic use Zidovudine/therapeutic use},
	Note = {0009-9104 Journal Article},
	Number = {3},
	Pages = {412-6},
	Title = {Highly active anti-retroviral therapy (HAART) is associated with a lower level of CD4+ T cell apoptosis in HIV-infected patients},
	Volume = {118},
	Year = {1999}}

@article{Stoddaretalt01,
	Abstract = {Many HIV-1-infected patients treated with protease inhibitors (PI) develop PI-resistant HIV-1 variants and rebounds in viremia, but their CD4+ T-cell counts often do not fall. We hypothesized that in these patients, T-cell counts remain elevated because PI-resistant virus spares intrathymic T-cell production. To test this, we studied recombinant HIV-1 clones containing wild-type or PI-resistant protease domains, as well as uncloned isolates from patients, in activated peripheral blood mononuclear cells, human thymic organ cultures and human thymus implants in SCID-hu Thy/Liv mice. In most cases, wild-type and PI-resistant HIV-1 isolates replicated to similar degrees in peripheral blood mononuclear cells. However, the replication of PI-resistant but not wild-type HIV-1 isolates was highly impaired in thymocytes. In addition, patients who had PI-resistant HIV-1 had abundant thymus tissue as assessed by computed tomography. We propose that the inability of PI-resistant HIV-1 to replicate efficiently in thymus contributes to the preservation of CD4+ T-cell counts in patients showing virologic rebound on PI therapy.},
	Author = {Stoddart, C. A. and Liegler, T. J. and Mammano, F. and Linquist-Stepps, V. D. and Hayden, M. S. and Deeks, S. G. and Grant, R. M. and Clavel, F. and McCune, J. M.},
	Journal = {Nat Med},
	Keywords = {Adult Animals CD4 Lymphocyte Count Drug Resistance, Microbial Fetal Tissue Transplantation Flow Cytometry HIV Core Protein p24/metabolism HIV Infections/immunology/pathology/*virology HIV Protease/genetics/*metabolism HIV Protease Inhibitors/*pharmacology HIV-1/*drug effects/enzymology/genetics/*physiology Human Mice Mice, SCID Middle Aged Organ Culture Recombination, Genetic Support, Non-U.S. Gov't Support, U.S. Gov't, P.H.S. T-Lymphocytes/*physiology/virology Thymus Gland/pathology/physiopathology/transplantation/*virology Viral Load *Virus Replication},
	Note = {1078-8956 Journal Article},
	Number = {6},
	Pages = {712-8},
	Title = {Impaired replication of protease inhibitor-resistant HIV-1 in human thymus},
	Volume = {7},
	Year = {2001}}

@article{Sufkaetal03,
	Abstract = {Mechanisms that underly discordant CD4+ cell/virus load (VL) responses in patients who receive highly active antiretroviral therapy (HAART) were studied in 30 human immunodeficiency virus (HIV)-positive patients, in 3 groups. Discordant responders maintained CD4+ cell levels >200/mm(3) with stable or increasing trend, despite sustained VLs of 500-5000 copies/mL, for >2 years. Treatment-success patients had CD4+ cell counts >200/mm(3) with stable or increasing trend and VLs <50 copies/mL, for >2 years. Treatment-failure patients initially responded to HAART, followed by decreasing CD4+ cell counts and increasing VLs. Interferon-gamma production to gag and noncytolytic CD8+ cell suppressive activity were greater in discordant responders. Cellular activation was greatest in patients with treatment failure. All discordant responders had non-syncytium-inducing (CCR5-tropic) viruses. Viruses from discordant responders and from patients with treatment failure had extensive resistance mutations; discordant responders had significantly lower viral replication capacities. These findings suggest that discordant responses may be related to enhanced HIV-directed immune responses, diminished cellular activation, decreased viral replication capacity, and preservation of non-syncytium-inducing virus strains.},
	Author = {Sufka, S. A. and Ferrari, G. and Gryszowka, V. E. and Wrin, T. and Fiscus, S. A. and Tomaras, G. D. and Staats, H. F. and Patel, D. D. and Sempowski, G. D. and Hellmann, N. S. and Weinhold, K. J. and Hicks, C. B.},
	Journal = {J Infect Dis},
	Keywords = {Adult *Antiretroviral Therapy, Highly Active *CD4 Lymphocyte Count Female HIV/*drug effects HIV Infections/*drug therapy/*immunology/virology HIV Protease Inhibitors/*pharmacology/therapeutic use Human Male Middle Aged Support, Non-U.S. Gov't Support, U.S. Gov't, P.H.S. Time Factors Treatment Failure *Viral Load Virus Replication/drug effects},
	Note = {0022-1899 Clinical Trial Journal Article},
	Number = {7},
	Pages = {1027-37},
	Title = {Prolonged CD4+ cell/virus load discordance during treatment with protease inhibitor-based highly active antiretroviral therapy: immune response and viral control},
	Volume = {187},
	Year = {2003}}

@article{Tebaldietal03,
	Abstract = {To ascertain the impact of hepatitis C virus (HCV) infection on human immunodeficiency virus (HIV) disease progression and associated death in the era of highly active antiretroviral therapy (HAART), we examined mortality rates, the presence of other diseases, and antiretroviral use in an observational cohort of 823 HIV-infected patients with and without HCV coinfection during the period of January 1996 through June 2001. Analyses were used to compare patient characteristics, comorbid conditions, and survival durations in HIV-infected and HIV-HCV-coinfected patients. HIV-HCV-coinfected persons did not have a statistically greater rate of acquired immunodeficiency syndrome or of renal or cardiovascular disease, but they did have more cases of cirrhosis and transaminase elevations. There were proportionately more deaths in the HIV-HCV-coinfected group. Age, baseline CD4+ cell count, and duration of HAART were significantly associated with survival, but HCV infection was not. HAART use was a strong predictor of increased duration of survival, suggesting that treatment is more important to survival than is HCV coinfection status.},
	Author = {Tedaldi, E. M. and Baker, R. K. and Moorman, A. C. and Alzola, C. F. and Furhrer, J. and McCabe, R. E. and Wood, K. C. and Holmberg, S. D.},
	Journal = {Clin Infect Dis},
	Keywords = {Anti-HIV Agents/therapeutic use *Antiretroviral Therapy, Highly Active *Hiv HIV Infections/*complications/drug therapy/epidemiology/mortality *Hepacivirus Hepatitis C/*complications/epidemiology/mortality Human Morbidity Mortality Support, U.S. Gov't, P.H.S.},
	Note = {1537-6591 Journal Article},
	Number = {3},
	Pages = {363-7},
	Title = {Influence of coinfection with hepatitis C virus on morbidity and mortality due to human immunodeficiency virus infection in the era of highly active antiretroviral therapy},
	Volume = {36},
	Year = {2003}}

@article{Wang&Bembom&vanderLaan06,
	Author = {Y. Wang and O. Bembom and M.J. van der Laan},
	Journal = {Journal of Statistical Planning and Inference},
	Optnote = {also http://www.bepress.com/ucbbiostat/paper159},
	Title = {Data adaptive estimation of the treatment specific mean},
	Year = {2006}}

@article{Sinisi&vanderLaan04,
	Author = {S. Sinisi and M.J. van der Laan},
	Journal = {Journal of Statistical Methods in Molecular Biology},
	Number = {1},
	Optnote = {http://www.bepress.com/sagmb/vol3/iss1/art18},
	Title = {The deletion/substitution/addition algorithm in loss function based estimation: Applications in Genomics},
	Volume = {3},
	Year = {2004}}

@techreport{Petersenetal05,
	Author = {M. L. Petersen and S.G. Deeks and J. N. Martin and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Month = {December},
	Optnote = {http://www.bepress.com/ucbbiostat/paper199},
	Title = {History-Adjusted Marginal Structural Models: Time-Varying Effect Modification and Dynamic Treatment Regimens},
	Type = {Technical Report 199},
	Year = {2005}}

@techreport{vanderLaan&Rubin05,
	Author = {M.J. van der Laan and D. Rubin},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper180},
	Title = {Estimating Function Based Cross-Validation and Learning},
	Type = {Technical Report 180},
	Year = {2005}}

@article{vanderLaan&Petersen07,
	Author = {M.J. van der Laan and M.L. Petersen},
	Journal = {International Journal of Biostatistics},
	Number = {1},
	Optnote = {http://www.bepress.com/ijb/vol3/iss1/art3},
	Title = {Causal Effect Models for Realistic Individualized Treatment and Intention to Treat Rules},
	Volume = {3},
	Year = {2007}}

@techreport{vanderLaan06,
	Author = {M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper203},
	Title = {Causal Effect Models for Intention to Treat and Realistic Individualized Treatment Rules},
	Type = {Technical Report 203},
	Year = {2006}}

@techreport{vanderLaan08b,
	Author = {M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Month = {March},
	Optnote = {http://www.bepress.com/ucbbiostat/paper232},
	Title = {The construction and analysis of adaptive group sequential designs},
	Type = {Technical Report 232},
	Year = {2008}}

@techreport{Moore&vanderLaan07,
	Author = {K.L. Moore and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Month = {April},
	Optnote = {http://www.bepress.com/ucbbiostat/paper215},
	Title = {Covariate adjustment in randomized trials with binary outcomes},
	Type = {Technical Report 215},
	Year = {2007}}

@techreport{vanderLaan&Petersen05,
	Author = {M.J. van der Laan and M.L. Petersen},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper187},
	Title = {Direct Effect Models},
	Type = {Technical Report 187},
	Year = {2005}}

@techreport{Petersen&vanderLaan06,
	Author = {M.L. Petersen and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Title = {Individualized Treatment Rules and Clinical Trials},
	Type = {Technical Report},
	Year = {2006}}

@article{vanderLaan&Petersen&Joffe05,
	Author = {M.J. van der Laan and M.L. Petersen and M.M. Joffe},
	Journal = {The International Journal of Biostatistics},
	Number = {1},
	Optnote = {http://www.bepress.com/ijb/vol1/iss1/4},
	Pages = {10-20},
	Title = {History-Adjusted Marginal Structural Models and Statically-Optimal Dynamic Treatment Regimens},
	Volume = {1},
	Year = {2005}}

@article{vanderLaan06a,
	Author = {M.J. van der Laan},
	Journal = {International Journal of Biostatistics},
	Number = {1},
	Optnote = {http://www.bepress.com/ijb/vol2/iss1/art2},
	Title = {Statistical Inference for Variable Importance},
	Volume = {2},
	Year = {2006}}

@article{vanderLaan&Birkner&Hubbard05,
	Author = {M.J. van der Laan and M.D. Birkner and A.E. Hubbard},
	Journal = {Journal of Statistical Applications in Genetics and Molecular Biology},
	Number = {1},
	Optnote = {http://www.bepress.com/sagmb/vol4/iss1/art29},
	Title = {Empirical Bayes and resampling based multiple testing procedure controlling tail probability of the proportion of false positives},
	Volume = {4},
	Year = {2005}}

@article{vanderLaan&Dudoit&Pollard04b,
	Author = {M.J. van der Laan and S. Dudoit and K.S. Pollard},
	Journal = {Journal of Statistical Applications in Genetics and Molecular Biology},
	Number = {1},
	Optnote = {http://www.bepress.com/sagmb/vol3/iss1/art15},
	Title = {Augmentation procedures for control of the generalized family-wise error rate and tail probabilities for the proportion of false positives},
	Volume = {3},
	Year = {2004}}

@article{vanderLaan&Dudoit&Pollard04,
	Author = {S. Dudoit and M.J. van der Laan and K.S. Pollard},
	Journal = {Journal of Statistical Applications in Genetics and Molecular Biology},
	Number = {1},
	Optnote = {http://www.bepress.com/sagmb/vol3/iss1/art14},
	Title = {Multiple testing. Part II. Step-down procedures for control of the family-wise error rate},
	Volume = {3},
	Year = {2004}}

@article{Dudoit&vanderLaan&Pollard04,
	Author = {S. Dudoit and M.J. van der Laan and K.S. Pollard},
	Journal = {Journal of Statistical Applications in Genetics and Molecular Biology},
	Number = {1},
	Optnote = {http://www.bepress.com/sagmb/vol3/iss1/art13},
	Title = {Multiple testing. Part I. Single-step procedures for control of general Type I error rates},
	Volume = {3},
	Year = {2004}}

@article{Birkner&Sinisi&vanderLaan05,
	Author = {M.D. Birkner and S.E. Sinisi and M.J. van der Laan},
	Journal = {Journal of Statistical Applications in Genetics and Molecular Biology},
	Number = {1},
	Optnote = {http://www.bepress.com/sagmb/vol4/iss1/art8},
	Title = {Multiple Testing and Data Adaptive Regression: An Application to {HIV}-1 Sequence Data},
	Volume = {4},
	Year = {2005}}

@techreport{vanderLaan&Hubbard06,
	Author = {M.J. van der Laan and A.E. Hubbard},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper198},
	Title = {Quantile-Function Based Null Distribution in Resampling Based Multiple Testing},
	Type = {Technical Report},
	Year = {2006}}

@techreport{Molinaro&vanderLaan04,
	Author = {A. Molinaro and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper162},
	Title = {Deletion/Substitution/Addition Algorithm for Partitioning the Covariate Space in Prediction},
	Type = {Technical Report},
	Year = {2004}}

@techreport{Birkner&vanderLaan05,
	Author = {M.D. Birkner and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Title = {Application of a Variable Importance Measure Method to {HIV}-1 Sequence Data},
	Type = {Technical Report},
	Year = {2005}}

@article{Neugebauer2007419,
	Author = {Romain Neugebauer and Mark van der Laan},
	Doi = {DOI: 10.1016/j.jspi.2005.12.008},
	Issn = {0378-3758},
	Journal = {Journal of Statistical Planning and Inference},
	Number = {2},
	Pages = {419 - 434},
	Title = {Nonparametric causal effects based on marginal structural models},
	Url = {http://www.sciencedirect.com/science/article/pii/S0378375806000334},
	Volume = {137},
	Year = {2007},
	Bdsk-Url-1 = {http://www.sciencedirect.com/science/article/pii/S0378375806000334},
	Bdsk-Url-2 = {http://dx.doi.org/10.1016/j.jspi.2005.12.008}}

@techreport{Neugebauer&vanderLaan05b,
	Author = {R. Neugebauer and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {134},
	Optnote = {http://www.bepress.com/ucbbiostat/paper134, to appear in {JSPI}},
	Title = {Locally Efficient Estimation of Nonparametric Causal Effects on Mean Outcomes in Longitudinal Studies},
	Type = {Technical Report},
	Year = {2005}}

@techreport{Wang&Petersen&vanderLaan06,
	Author = {Y. Wang and M. Petersen and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Title = {A statistical method for diagnosing ETA bias in IPTW estimators},
	Type = {Technical Report},
	Year = {2006}}

@techreport{vanderLaan&Dudoit&vanderVaart,
	Author = {M.J. van der Laan and S. Dudoit and A.W. van der Vaart},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Month = {February},
	Optnote = {http://www.bepress.com/ucbbiostat/paper142},
	Title = {The Cross-Validated Adaptive Epsilon-Net Estimator},
	Type = {Technical Report 142},
	Year = {2004}}

@techreport{vanderLaan&Dudoit03,
	Author = {M.J. van der Laan and S. Dudoit},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Month = {November},
	Optnote = {http://www.bepress.com/ucbbiostat/paper130},
	Title = {Unified cross-validation methodology for selection among estimators and a general cross-validated adaptive epsilon-net estimator: Finite sample oracle inequalities and examples},
	Type = {Technical Report},
	Year = {2003}}

@techreport{Petersen&vanderLaan05,
	Author = {M. Petersen and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Title = {Estimation of direct and indirect causal effects in Epidemiology},
	Type = {Technical Report},
	Year = {2005}}

@techreport{vanderLaan&Petersen04,
	Author = {M.J. van der Laan and M. Petersen},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Month = {August},
	Title = {Estimation of direct and indirect causal effects in longitudinal studies},
	Type = {Technical Report 155},
	Year = {2004}}

@techreport{vanderLaan&Hubbard&Jewell04,
	Author = {M.J. van der Laan and A.E. Hubbard and N.P. Jewell},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Month = {September},
	Optnote = {http://www.bepress.com/ucbbiostat/paper157},
	Title = {Estimation of Treatment Effects in Randomized Trials with Noncompliance and a Dichotomous Outcome},
	Type = {Technical Report 157},
	Year = {2004}}

@techreport{Bein&Hubbard&vanderLaan05,
	Author = {E. Bein and A.E. Hubbard and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Title = {Estimating Function Based Cross-Validation in Estimation of the Causal Effect in Randomized Trials},
	Type = {Technical Report},
	Year = {2005}}

@techreport{Molinaroetal05,
	Author = {A.M. Molinaro and M.J. van der Laan and D.H. Moore and K. Kerlikowske},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Note = {http://www.bepress.com/ucbbiostat/paper149},
	Title = {Survival point estimate prediction in matched and non-matched case-control subsample designed studies},
	Year = {2005}}

@techreport{Dudoitetal04,
	Author = {S. Dudoit and M.J. van der Laan and S. Kele\c{s} and A. M. Molinaro and S. E. Sinisi and S.L. Teng},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Note = {to appear in \emph{SIGKDD} Explorations on Microarray Data Mining},
	Title = {Loss-Based Estimation with Cross-Validation: Applications to Microarray Data Analysis and Motif Finding.},
	Year = {2004}}

@book{Friedman&Furberg&Demets98,
	Author = {L.M.Friedman and C.D. Furberg and D.L. DeMets},
	Publisher = {Springer-Verlag New York},
	Title = {Fundamentals of Clinical Trials},
	Year = {1998}}

@book{Andersenetal93,
	Author = {P.K. Andersen and O. Borgan and R.D. Gill and N. Keiding},
	Publisher = {Springer-Verlag New York},
	Title = {Statistical Models Based on Counting Processes},
	Year = {1993}}

@article{Wittes&Brittain90,
	Author = {J. Wittes and E. Brittain},
	Journal = {Statistics in Medicine},
	Pages = {65--72},
	Title = {The role of internal pilot studies in increasing efficiency of clinical trials},
	Volume = {9},
	Year = {1999}}

@incollection{Robins03,
	Author = {J.M. Robins},
	Booktitle = {Highly Structured Stochastic Systems},
	Editor = {P. Green, N. Hjort, and S. Richardson},
	Pages = {70--81},
	Publisher = {Oxford University Press, Oxford},
	Title = {Semantics of causal DAG models and the identification of direct and indirect effects},
	Year = {2003}}

@techreport{Pearl01,
	Author = {J. Pearl},
	Institution = {University of California, Los Angeles, Department of Computer Science},
	Title = {Cognitive systems Laboratory},
	Year = {2001}}

@book{Pearl00,
	Author = {J. Pearl},
	Publisher = {Cambridge University Press, Cambridge},
	Title = {Causality: Models, Reasoning, and Inference},
	Year = {2000}}

@article{Robins&Greenland92,
	Author = {J.M. Robins and S. Greenland},
	Journal = {Epidemiology},
	Number = {0},
	Pages = {143--155},
	Title = {Identifiability and exchangeability for direct and indirect effects},
	Volume = {3},
	Year = {1992}}

@article{vanderLaan95,
	Author = {M.J. van der Laan},
	Journal = {Bernoulli},
	Number = {4},
	Pages = {335--341},
	Title = {Identity for NPMLE in missing data and biased sampling models},
	Volume = {1},
	Year = {1995}}

@article{vanderLaan98,
	Author = {M.J. van der Laan},
	Journal = {Lifetime Data Models},
	Number = {0},
	Pages = {83--102},
	Title = {Identity for NPMLE in Censored Data Models},
	Volume = {4},
	Year = {1998}}

@article{Klaassen86,
	Author = {C.A.J. Klaassen},
	Journal = {Annals of Statistics},
	Pages = {1548--1562},
	Title = {Consistent estimation of the influence function of locally asymptotically linear estimators},
	Volume = {15},
	Year = {1987}}

@article{Robins&Rotnitzky04,
	Author = {J.M. Robins and A. Rotnitzky},
	Journal = {Biometrika},
	Number = {0},
	Optnote = {To Appear},
	Pages = {0},
	Title = {Estimation of Treatment Effects in Randomized Trials with Noncompliance and a Dichotomous Outcome using Structural Nested Mean Models},
	Volume = {0},
	Year = {2004}}

@article{vanderVaart91,
	Author = {A.W. van der Vaart},
	Journal = {Annals of Statistics},
	Pages = {178--204},
	Title = {On differentiable functionals},
	Volume = {19},
	Year = {1991}}

@article{Rubin78,
	Author = {D.B. Rubin},
	Journal = {Annals of Statistics},
	Pages = {34--58},
	Title = {Bayesian Inference for causal effects: the role of randomization},
	Volume = {6},
	Year = {1978}}

@article{Neyman23,
	Author = {Neyman, J.},
	Journal = {Statistical Science},
	Optnote = {Translation of 1923 article},
	Pages = {465--480},
	Title = {On the application of probability theory to agricultural experiments},
	Volume = {5},
	Year = {1990}}

@article{Robins86,
	Author = {J.M. Robins},
	Journal = {Mathematical Modelling},
	Pages = {1393--1512},
	Title = {A new approach to causal inference in mortality studies with sustained exposure periods - Application to control of the healthy worker survivor effect},
	Volume = {7},
	Year = {1986}}

@article{Robins94,
	Author = {J.M. Robins},
	Journal = {Communications in Statistics},
	Pages = {2379--2412},
	Title = {Correcting for non-compliance in randomized trials using structural nested mean models},
	Volume = {23},
	Year = {1994}}

@article{Vansteelandt&Goetghebeur03,
	Author = {S. Vansteelandt and E. Goetghebeur},
	Journal = {Journal of the Royal Statistical Society, Series B},
	Optnote = {In print},
	Title = {Causal inference with generalized structural mean models},
	Volume = {23},
	Year = {2003}}

@incollection{Robins97a,
	Address = {Chichester, UK},
	Author = {Robins, J.M.},
	Booktitle = {The Encyclopedia of Biostatistics},
	Editor = {Armitage, P. and Colton, T. and Andersen, P.K. and Keiding, N.},
	Publisher = {John Wiley and Sons},
	Title = {Structural Nested Failure Time Models},
	Year = {1997}}

@article{Hernan&Brumback&Robins,
	Author = {Hernan, M. A. and Brumback, B. and Robins, J. M.},
	Journal = {Epidemiology},
	Number = {5},
	Pages = {561--570},
	Title = {Marginal structural models to estimate the causal effect of zidovudine on the survival of {HIV}-positive men},
	Volume = {11},
	Year = {2000}}

@article{Robins87,
	Author = {Robins, J.M.},
	Coden = {CMAPDK},
	Fjournal = {Computers \& Mathematics with Applications. An International Journal},
	Issn = {0097-4943},
	Journal = {Comput. Math. Appl.},
	Number = {9-12},
	Pages = {923--945},
	Title = {Addendum to: ``{A} new approach to causal inference in mortality studies with a sustained exposure period---application to control of the healthy worker survivor effect'' [{M}ath.\ {M}odelling {\bf 7} (1986), no.\ 9-12, 1393--1512; {M}{R} 87m:92078]},
	Volume = {14},
	Year = {1987}}

@article{Robins&Hernan&Brumback00,
	Author = {Robins, J. M. and Hernan, M. A. and Brumback, B.},
	Journal = {Epidemiology},
	Number = {5},
	Pages = {550--560},
	Title = {Marginal structural models and causal inference in epidemiology},
	Volume = {11},
	Year = {2000}}

@article{Bryan&Yu&vanderLaan03,
	Author = {Bryan, J. and Yu, Z. and van der Laan, M.J.},
	Journal = {Biostatistics},
	Number = {3},
	Pages = {361--380},
	Title = {Analysis of Longitudinal Marginal Structural Models},
	Volume = {5},
	Year = {2003}}

@techreport{Yu&vanderLaan03b,
	Author = {Yu, Z. and van der Laan, M.J.},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper132},
	Optnumber = {132},
	Title = {Double Robust Estimation in Longitudinal Marginal Structural Models},
	Year = {2003}}

@article{Neugebauer&vanderLaan05,
	Author = {Neugebauer, R. and van der Laan, M.J.},
	Journal = {Journal of Statistical Planning and Inference},
	Number = {1-2},
	Pages = {405--26},
	Title = {Why prefer double robust estimates},
	Volume = {129},
	Year = {2005}}

@article{Murphy03,
	Author = {Murphy, S.A.},
	Journal = {Journal of the Royal Statistical Society: Series B},
	Number = {2},
	Pages = {331-66},
	Title = {Optimal dynamic treatment regimes},
	Volume = {65},
	Year = {2003}}

@article{Robins03a,
	Author = {Robins, J.M.},
	Journal = {Journal of the Royal Statistical Society: Series B},
	Number = {2},
	Pages = {355--66},
	Title = {Discussion of ``Optimal dynamic treatment regimes" by Susan A. Murphy},
	Volume = {65},
	Year = {2003}}

@article{Murphy&vanderLaan&Robins01,
	Author = {S.A. Murphy and M.J. van der Laan and J.M. Robins},
	Journal = {Journal of the American Statistical Association},
	Pages = {1410--1424},
	Title = {Marginal mean models for dynamic treatment regimens},
	Volume = {96},
	Year = {2001}}

@incollection{Robins98,
	Address = {New York},
	Author = {Robins, J.M.},
	Booktitle = {Statistical models in epidemiology, the environment, and clinical trials (Minneapolis, MN, 1997)},
	Mrclass = {62N01 (62G08 62P10)},
	Mrnumber = {2001a:62124},
	Pages = {95--133},
	Publisher = {Springer},
	Title = {Marginal structural models versus structural nested models as tools for causal inference},
	Year = {2000}}

@incollection{Robins97,
	Author = {J.M. Robins},
	Booktitle = {Latent Variable Modeling and Applications to Causality},
	Editor = {M. Berkane, Editor},
	Optseries = {Lecture Notes in Statistics},
	Optvolume = {120},
	Pages = {69--117},
	Publisher = {Springer Verlag, New York},
	Title = {Causal Inference from Complex Longitudinal Data},
	Year = {1997}}

@incollection{Robins89,
	Address = {Washington D.C.},
	Author = {J.M. Robins},
	Booktitle = {Health Service Methodology: A Focus on AIDS},
	Editor = {L. Sechrest and H. Freeman and A. Mulley},
	Optseries = {Lecture Notes in Statistics},
	Pages = {113--159},
	Publisher = {U.S. Public Health Service, National Center for Health SErvices Research},
	Title = {The analysis of randomized and non-randomized AIDS treatment trials using a new approach in causal inference in longitudinal studies},
	Year = {1989}}

@techreport{Abadie00,
	Author = {A. Abadie},
	Institution = {NBER Technical Working Paper},
	Optnumber = {260},
	Title = {Semiparametric estimation of instrumental variables models for causal effects},
	Year = {2000}}

@article{Abadie03,
	Author = {A. Abadie},
	Journal = {Journal of Econometrics},
	Pages = {231-263},
	Title = {Semiparametric instrumental variable estimation of treatment response models},
	Volume = {113},
	Year = {2003}}

@article{Abadie03,
	Author = {A. Abadie},
	Journal = {Journal of Econometrics},
	Pages = {231-263},
	Title = {Semiparametric instrumental variable estimation of treatment response models},
	Volume = {113},
	Year = {2003}}

@techreport{Wang&Vanderlaan04,
	Author = {Y. Wang and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper159},
	Optnumber = {159},
	Title = {Data adaptive estimation of the treatment specific mean},
	Year = {2004}}

@techreport{Yu&Vanderlaan02,
	Author = {Z. Yu and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper122},
	Optnumber = {122},
	Title = {Construction of counterfactuals and the {G}-computation formula},
	Year = {2002}}

@techreport{Yu&Vanderlaan03,
	Author = {Z. Yu and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper136},
	Optnumber = {136},
	Title = {Measuring treatment effects using semiparametric models},
	Year = {2003}}

@article{Angristetal&Imbens&Rubin96,
	Author = {J. Angrist and G. Imbens and D.B. Rubin},
	Journal = {Journal of the American Statistical Association},
	Pages = {444-555},
	Title = {Identification of causal effects using instrumental variables},
	Volume = {91},
	Year = {1996}}

@article{Robins&Rotnitzky01A,
	Author = {J.M Robins and A. Rotnitzky},
	Journal = {Statistica Sinica},
	Pages = {920-935},
	Title = {Comment on {I}nference for semiparametric models: some questions and an answer, by {B}ickel, {P}.{J}. and {K}won, {J}.},
	Volume = {11},
	Year = {2001}}

@article{Angrist01,
	Author = {J. Angrist},
	Journal = {Journal of Business and Economics Statistics},
	Pages = {1--16},
	Title = {Estimation of limited dependent variable models with dummy endogenous regressors: simple strategies for empirical practice},
	Volume = {19},
	Year = {2001}}

@article{Chamberlain87,
	Author = {G. Chamberlain},
	Journal = {Journal of Econometrics},
	Pages = {305--334},
	Title = {Asymptotic efficiency in estimation with conditional moment restrictions},
	Volume = {34},
	Year = {1987}}

@article{Hiranoetal00,
	Author = {K. Hirano and G. Imbens and D.B. Rubin and X-H. Zhou},
	Journal = {Biostatistics},
	Pages = {69--88},
	Title = {Assessing the effects of influenza vaccine in an encouragement design},
	Volume = {1},
	Year = {2000}}

@article{Neyman23,
	Author = {J. Neyman},
	Journal = {Statistical Science},
	Pages = {463--472},
	Title = {Sur les applications de la thar des probabilites aux experiences Agaricales: Essay des principle (1923). Excerpts reprinted (1990) in English (D. Dabrowska and T. Speed), Trans.},
	Volume = {5},
	Year = {1990}}

@inproceedings{Robins05,
	Author = {J.M. Robins},
	Booktitle = {Proceedings of the 2nd Seattle symposium in biostatistics},
	Editor = {Lin, D.Y, Heagerty P.J},
	Optpublisher = {Springer Verlag Lecture Notes in Statistics},
	Pages = {189--326},
	Title = {Optimal structural nested models for optimal sequential decisions},
	Volume = {179},
	Year = {2005}}

@techreport{Robins05b,
	Author = {J.M. Robins},
	Institution = {Department of Biostatistics, Havard University},
	Title = {Optimal structural nested models for optimal sequential decisions},
	Year = {2005}}

@inproceedings{Akaike73,
	Author = {H. Akaike},
	Booktitle = {Second International Symposium on Information Theory},
	Editor = {B.N. Petrov and F. Csaki},
	Organization = {Budapest: Academiai Kiado},
	Pages = {267-281},
	Title = {Information theory and an extension of the maximum likelihood principle},
	Year = {1973}}

@article{Balke&Pearl97,
	Author = {A. Balke and J. Pearl},
	Journal = {Journal of the American Statistical Association},
	Pages = {1172--1176},
	Title = {Bound on treatment effects from studies with imperfect compliance},
	Volume = {92},
	Year = {1997}}

@inproceedings{Balke&Pearl94,
	Author = {A. Balke and J. Pearl},
	Booktitle = {In Proceedings of the 12th National Conference on Artificial Intelligence},
	Optaddress = {Menlo Park, CA},
	Optpublisher = {MIT Press},
	Pages = {230--237},
	Title = {Counterfactual probabilities: Computational methods, bounds, and applications},
	Volume = {I},
	Year = {1994}}

@article{Ambroise&McLachlan02,
	Author = {C. Ambroise and G. J. McLachlan},
	Journal = PNAS,
	Number = {10},
	Pages = {6562--6566},
	Title = {Selection bias in gene extraction on the basis of microarray gene-expression data},
	Volume = {99},
	Year = {2002}}

@incollection{Arabie&Hubert96,
	Address = {River Edge, NJ},
	Author = {P. Arabie and L. J. Hubert},
	Booktitle = {Clustering and Classification},
	Editor = {P. Arabie and L. J. Hubert and G. De Soete},
	Pages = {5--63},
	Publisher = {World Scientific Publishing Co.},
	Title = {An overview of combinatorial data analysis},
	Year = {1996}}

@article{Schwartz78,
	Author = {G. Schwartz},
	Journal = {Annals of Statistics},
	Pages = {461-464},
	Title = {Estimating the Dimension of a Model},
	Volume = {6},
	Year = {1978}}

@article{Barnard35,
	Author = {M. Barnard},
	Journal = {Annals of Eugenics},
	Pages = {352--371},
	Title = {The secular variations of skull characters in four series of Egyptian skulls},
	Volume = {6},
	Year = {1935}}

@inproceedings{BenHur&Elisseeff&Guyon02,
	Author = {A. Ben-Hur and A. Elisseeff and I. Guyon},
	Booktitle = {Pacific Symposium on Biocomputing},
	Pages = {6--17},
	Title = {A stability based method for discovering structure in clustered data},
	Volume = {7},
	Year = {2002}}

@article{Benjamini&Hochberg95,
	Author = {Y. Benjamini and Y. Hochberg},
	Journal = {J. R. Statist. Soc. B},
	Pages = {289--300},
	Title = {Controlling the false discovery rate: a practical and powerful approach to multiple testing},
	Volume = {57},
	Year = {1995}}

@article{Benjamini&Yekutieli01,
	Author = {Y. Benjamini and D. Yekutieli},
	Journal = {Annals of Statistics},
	Number = {4},
	Pages = {1165--1188},
	Title = {The control of the false discovery rate in multiple testing under dependency},
	Volume = {29},
	Year = {2001}}

@article{Beran88,
	Author = {R. Beran},
	Journal = JASA,
	Pages = {679--686},
	Title = {Balanced simultaneous confidence sets},
	Volume = {83},
	Year = {1988}}

@article{Bock85,
	Author = {H-H Bock},
	Journal = {Journal of Classification},
	Pages = {77--108},
	Title = {On some significance tests in cluster analysis},
	Volume = {2},
	Year = {1985}}

@incollection{Bock96,
	Address = {River Edge, NJ},
	Author = {H-H Bock},
	Booktitle = {Clustering and Classification},
	Editor = {P. Arabie and L. J. Hubert and G. De Soete},
	Pages = {377--453},
	Publisher = {World Scientific Publishing Co.},
	Title = {Probability models and hypotheses testing in partitioning cluster analysis},
	Year = {1996}}

@article{Boldricketal02,
	Author = {J. C. Boldrick and A. A. Alizadeh and M. Diehn and S. Dudoit and C. L. Liu and C. E. Belcher and D. Botstein and L. M. Staudt and P. O. Brown and D. A. Relman},
	Journal = PNAS,
	Number = {2},
	Pages = {972--977},
	Title = {Stereotyped and specific gene expression programs in human innate immue responses to bacteria},
	Volume = {99},
	Year = {2002}}

@article{Bozdogan00,
	Author = {H. Bozdogan},
	Journal = {Journal of Mathematical Psychology},
	Pages = {62-91},
	Title = {Akaike's information criterion and recent developments in information complexity},
	Volume = {44},
	Year = {2000}}

@incollection{Bozdogan93,
	Author = {H. Bozdogan},
	Booktitle = {Information and Classification},
	Editor = {O. Opitz and B. Lausen and R. Klar},
	Publisher = {Heidelberg: Springer Verlag},
	Title = {Choosing the number of component clusters in the mixture model using a new informational complexity criterion of the inverse Fisher information matrix},
	Year = {1993}}

@article{Braver,
	Author = {S. L. Braver},
	Journal = {Educational and Psychological Measurement},
	Pages = {283--301},
	Title = {On splitting the tails unequally: a new perspective on one-versus two-tailed tests},
	Volume = {35},
	Year = {1975}}

@article{Breckenridge89,
	Author = {J. Breckenridge},
	Journal = {Multivariate Behavioral Research},
	Pages = {147--161},
	Title = {Replicating cluster analysis: Method, consistency and validity},
	Volume = {24},
	Year = {1989}}

@article{Breiman&Spector92,
	Author = {L. Breiman and P. Spector},
	Journal = {International Statistical Review},
	Pages = {291--319},
	Title = {Submodel Selection and Evaluation in Regression. The $X$ Random Case},
	Volume = {60},
	Year = {1992}}

@article{Breiman01,
	Author = {L. Breiman},
	Journal = {Statistical Science},
	Number = {3},
	Pages = {199--215},
	Title = {Statistical modeling: the two cultures},
	Volume = {16},
	Year = {2001}}

@article{Breiman96,
	Author = {L. Breiman},
	Journal = {Annals of Statistics},
	Number = {6},
	Pages = {2350--2383},
	Title = {Heuristics of instability and stabilization in model selection},
	Volume = {24},
	Year = {1996}}

@article{Breiman98,
	Author = {L. Breiman},
	Journal = {Annals of Statistics},
	Pages = {801-824},
	Title = {Arcing classifiers},
	Volume = {26},
	Year = {1998}}

@article{Breiman96b,
	Author = {L. Breiman},
	Journal = {Machine Learning},
	Pages = {123-140},
	Title = {Bagging predictors},
	Volume = {24},
	Year = {1996}}

@techreport{Breiman98b,
	Author = {L. Breiman},
	Institution = {Department of Statistics, U.C. Berkeley},
	Month = {March},
	Number = {513},
	Title = {Using Convex pseudo-data to increase prediction accuracy},
	Year = {1998}}

@article{Breiman92,
	Author = {L. Breiman},
	Journal = JASA,
	Number = {419},
	Pages = {738--754},
	Title = {The Little Bootstrap and Other Methods for Dimensionality Selection in Regression: $X$-Fixed Prediction Error},
	Volume = {87},
	Year = {1992}}

@techreport{Breiman96c,
	Author = {L. Breiman},
	Institution = {Department of Statistics, U.C. Berkeley},
	Title = {Out-of-bag estimation},
	Year = {1996}}

@techreport{Breiman99,
	Author = {L. Breiman},
	Institution = {Department of Statistics, U.C. Berkeley},
	Number = {567},
	Title = {Random forests - random features},
	Year = {1999}}

@book{Breimanetal84,
	Author = {L. Breiman and J. H. Friedman and R. Olshen and C. J. Stone},
	Publisher = {Wadsworth International Group},
	Series = {The Wadsworth statistics/probability series},
	Title = {Classification and regression trees},
	Year = {1984}}

@book{Hastie&Tibshirani&Friedman02,
	Author = {T. Hastie and R. Tibshirani and J. Friedman},
	Publisher = {Springer},
	Series = {Springer Series in Statistics},
	Title = {The Elements of Statistical Learning},
	Year = {2002}}

@article{Broman01,
	Author = {K. W. Broman},
	Journal = {Lab Animal},
	Number = {7},
	Pages = {44--52},
	Title = {Review of statistical methods for QTL mapping in experimental crosses},
	Volume = {30},
	Year = {2001}}

@phdthesis{Broman97,
	Author = {K. W. Broman},
	School = {Department of Statistics, U.C. Berkeley},
	Title = {Identifying quantitative trait loci in experimental crosses},
	Type = {Ph.{D}. thesis},
	Year = {1997}}

@article{Brown&Koplowitz79,
	Author = {T. A. Brown and J. Koplowitz},
	Journal = {IEEE Transactions on Information Theory},
	Number = {5},
	Pages = {617--619},
	Title = {The weighted nearest neighbor rule for class dependent sample sizes},
	Volume = {25},
	Year = {1979}}

@article{Buhlmann&Yu,
	Author = {P. Buhlmann and B. Yu},
	Journal = {Annals of Statistics},
	Title = {Explaining Bagging.},
	Year = {(Accepted)}}

@article{Burges98,
	Author = {C. J. C. Burges},
	Journal = {Data Mining and Knowledge Discovery},
	Month = {December},
	Pages = {121--167},
	Title = {A tutorial on support vector machines for pattern recognition},
	Volume = {2},
	Year = {1998}}

@article{Burman89,
	Author = {P. Burman},
	Journal = {Biometrika},
	Pages = {503-514},
	Title = {A comparative study of ordinary cross-validation, $v$-fold cross-validati on and the repeated learning testing methods},
	Volume = {76},
	Year = {1989}}

@techreport{Buttrey&Karo02,
	Author = {S. E. Buttrey and C. Karo},
	Institution = {Naval Postgraduate School, Monterey, CA},
	Title = {Using k--neareset neighbor classification in the leaves of a tree},
	Year = {2002}}

@article{Calinski&Harabasz74l,
	Author = {R. Calinski and J. Harabasz},
	Journal = {Communications in Statistics},
	Pages = {1--27},
	Title = {A dendrite method for cluster analysis},
	Volume = {3},
	Year = {1974}}

@article{Callowetal00,
	Author = {M. J. Callow and S. Dudoit and E. L. Gong and T. P. Speed and E. M. Rubin},
	Journal = {Genome Research},
	Number = {12},
	Pages = {2022--2029},
	Title = {Microarray expression profiling identifies genes with altered expression in {HDL} deficient mice},
	Volume = {10},
	Year = {2000}}

@book{Chambers98,
	Author = {J. M. Chambers},
	Publisher = {Springer-Verlag New York},
	Title = {Programming with Data: A Guide to the S Language},
	Year = {1998}}

@book{Diggleetal02,
	Author = {Peter J. Diggle and P. Heagerty and K-Y Liang and S.L. Zeger},
	Publisher = {Oxford University Press},
	Title = {Analysis of Longitudinal Data},
	Year = {2002 (Second Edition)}}

@techreport{Chang&Lin01,
	Author = {C.-C. Chang and C.-J. Lin},
	Note = {\\ {\tt http://www.csie.ntu.edu.tw/~cjlin/papers/libsvm2.ps.gz}},
	Title = {LIBSVM: a Library for Support Vector Machines (Version 2.31)},
	Year = {2001}}

@article{Changetal02,
	Author = {H. Y. Chang and J. T. Chi and S. Dudoit and C. Bondre and M. van de Rijn and D. Botstein D and P. O. Brown},
	Journal = PNAS,
	Number = {20},
	Pages = {12877--12882},
	Title = {Diversity, topographic differentiation, and positional memory in human fibroblasts},
	Volume = {99},
	Year = {2002}}

@article{Chenetal02,
	Author = {X. Chen and S. T. Cheung and S. So and S. T. Fan and C. Barry and J. Higgins and K.-M. Lai and J. Ji and S. Dudoit and I. O. L. Ng and M. van de Rijn and D. Botstein and P. O. Brown},
	Journal = {Molecular Biology of the Cell},
	Number = {6},
	Pages = {1929--1939},
	Title = {Gene expression patterns in human liver cancers},
	Volume = {13},
	Year = {2002}}

@article{Cleveland&Devlin88,
	Author = {W. S. Cleveland and S. J. Devlin},
	Journal = JASA,
	Pages = {596--610},
	Title = {Locally-Weighted Regression: An Approach to Regression Analysis by Local Fitting},
	Volume = {83},
	Year = {1988}}

@article{Cleveland79,
	Author = {W. S. Cleveland},
	Journal = JASA,
	Number = {368},
	Pages = {829--836},
	Title = {Robust locally weighted regression and smoothing scatterplots},
	Volume = {74},
	Year = {1979}}

@article{Correa&Wolfson99,
	Author = {J. A. Correa and D. B. Wolfson},
	Journal = {Journal of Statistical Computation and Simulation},
	Pages = {209--219},
	Title = {Length-bias: some characterizations and applications},
	Tnumber = {3},
	Volume = {64},
	Year = {1999}}

@article{Correa&Dudoit&Goldstein02,
	Author = {J. A. Correa and S. Dudoit and D. R. Goldstein},
	Note = {(Submitted)},
	Optjournal = {Statistics in Medicine},
	Title = {Multiple testing in the survival analysis of microarray data},
	Year = {2002}}

@article{Cortes&Vapnik95,
	Author = {C. Cortes and V. Vapnik},
	Journal = {Machine Learning},
	Month = {December},
	Pages = {273-297},
	Title = {Support-vector networks},
	Volume = {20},
	Year = {1995}}

@inproceedings{Davies&Bouldin79,
	Author = {D. Davies and D. Bouldin},
	Booktitle = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
	Optnumber = {PAMI-1},
	Pages = {224--227},
	Title = {A cluster separation measure},
	Volume = {1},
	Year = {1979}}

@article{Davis&Anderson89,
	Author = {R. B. Davis and J. R. Anderson},
	Journal = {Statistics in Medicine},
	Pages = {947-961},
	Title = {Exponential survival trees},
	Volume = {8},
	Year = {1989}}

@incollection{Day96,
	Address = {River Edge, NJ},
	Author = {W. H. E. Day},
	Booktitle = {Clustering and Classification},
	Editor = {P. Arabie and L. J. Hubert and G. De Soete},
	Pages = {199--233},
	Publisher = {World Scientific Publishing Co.},
	Title = {Complexity theory: {A}n introduction for practitioners of classification},
	Year = {1996}}

@article{Dettling&Buhlmann02,
	Author = {M. Dettling and P. B\"{u}hlmann},
	Title = {How to Use Boosting for Tumor Classification with Gene Expression Data},
	Year = {2002}}

@article{Dudoit&Fridlyand02,
	Author = {S. Dudoit and J. Fridlyand},
	Optjournal = {Bioinformatics},
	Title = {Bagging to improve the accuracy of a clustering procedure},
	Year = {2002}}

@incollection{Dudoit&Fridlyand02b,
	Author = {S. Dudoit and J. Fridlyand},
	Booktitle = {Statistical Analysis of Gene Expression Microarray Data},
	Editor = {T. P. Speed},
	Note = {(To appear)},
	Publisher = {Chapman \& Hall/CRC},
	Title = {Classification in microarray experiments},
	Year = {2002}}

@article{Dudoit&Fridlyand02c,
	Author = {S. Dudoit and J. Fridlyand},
	Journal = {Genome Biology},
	Number = {7},
	Pages = {0036.1--0036.21},
	Title = {A prediction-based resampling method to estimate the number of clusters in a dataset},
	Volume = {3},
	Year = {2002}}

@techreport{Dudoit&Fridlyand01,
	Author = {S. Dudoit and J. Fridlyand},
	Institution = {Department of Statistics, Uiversity of California, Berkeley},
	Number = {600},
	Title = {Applications of resampling methods to estimate the number of clusters and to improve the accuracy of a clustering method},
	Url = {stat-www.berkeley.edu/users/sandrine/publications.html},
	Year = {2001},
	Bdsk-Url-1 = {stat-www.berkeley.edu/users/sandrine/publications.html}}

@article{Dudoit&vanderLaan05,
	Author = {S. Dudoit and M.J. van der Laan},
	Journal = {Statistical Methodology},
	Number = {2},
	Optnote = {www.bepress.com/ucbbiostat/paper126},
	Pages = {131--154},
	Title = {Asymptotics of cross-validated risk estimation in estimator selection and performance assessment},
	Volume = {2},
	Year = {2005}}

@article{Dudoit&Speed99,
	Author = {S. Dudoit and T. P. Speed},
	Journal = {Annals of Statistics},
	Number = {3},
	Pages = {943--986},
	Title = {A score test for linkage using identity by descent data from sibships},
	Volume = {27},
	Year = {1999}}

@article{Dudoit&Speed00,
	Author = {S. Dudoit and T. P. Speed},
	Journal = {Biostatistics},
	Number = {1},
	Pages = {1--26},
	Title = {A score test for the linkage analysis of qualitative and quantitative traits based on identity by descent data on sib-pairs},
	Volume = {1},
	Year = {2000}}

@incollection{Dudoit&Speed99b,
	Address = {New York},
	Author = {S. Dudoit and T. P. Speed},
	Booktitle = {Statistics in Genetics},
	Editor = {M. E. Halloran and S. Geisser},
	Pages = {181--221},
	Publisher = {Springer-Verlag},
	Series = {IMA Volumes in Mathematics and its Applications},
	Title = {Triangle constraints for sib-pair identity by descent probabilities under a general multilocus model for disease susceptibility},
	Volume = {112},
	Year = {1999}}

@incollection{Dudoit&Yang03,
	Author = {S. Dudoit and Y. H. Yang},
	Booktitle = {The Analysis of Gene Expression Data: Methods and Software},
	Editor = {G. Parmigiani and E. S. Garrett and R. A. Irizarry and S. L. Zeger},
	Publisher = {Springer, New York},
	Title = {Bioconductor {R} packages for exploratory analysis and normalization of c{DNA} microarray data},
	Year = {2003}}

@article{Dudoit&Fridlyand&Speed02,
	Author = {S. Dudoit and J. Fridlyand and T. P. Speed},
	Journal = JASA,
	Number = {457},
	Pages = {77--87},
	Title = {Comparison of Discrimination Methods for the Classification of Tumors Using Gene Expression Data},
	Volume = {97},
	Year = {2002}}

@article{Dudoitetal02,
	Author = {S. Dudoit and Y. H. Yang and M. J. Callow and T. P. Speed},
	Journal = {Statistica Sinica},
	Number = {1},
	Pages = {111--139},
	Title = {Statistical methods for identifying differentially expressed genes in replicated c{DNA} microarray experiments},
	Volume = {12},
	Year = {2002}}

@techreport{Dudoit&Shaffer&Boldrick02,
	Author = {S. Dudoit and J. P. Shaffer and J. C. Boldrick},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {110},
	Title = {Multiple hypothesis testing in microarray experiments},
	Url = {www.bepress.com/ucbbiostat/paper110/},
	Year = {2002},
	Bdsk-Url-1 = {www.bepress.com/ucbbiostat/paper110/}}

@article{Duffy&Quiroz91,
	Author = {D. E. Duffy and A. J. Quiroz},
	Journal = {Journal of Classification},
	Pages = {65--91},
	Title = {A permutation-based algorithm for block clustering},
	Volume = {8},
	Year = {1991}}

@article{Dunn58,
	Author = {O. J. Dunn},
	Journal = {Annals of Mathematical Statistics},
	Pages = {1095-111},
	Title = {Estimation of the means of dependent variables},
	Volume = {29},
	Year = {1958}}

@book{Efron&Tibshirani93,
	Author = {B. Efron and R. J. Tibshirani},
	Publisher = {Chapman \& Hall/CRC},
	Title = {An Introduction to the Bootstrap},
	Year = {1993}}

@article{EfronetalJASA01,
	Author = {B. Efron and R. Tibshirani and J. D. Storey and V. Tusher},
	Journal = JASA,
	Pages = {1151--1160},
	Title = {Empirical Bayes analysis of a microarray experiment},
	Volume = {96},
	Year = {2001}}

@techreport{Efron&Storey&Tibshirani01,
	Author = {B. Efron and J. D. Storey and R. Tibshirani},
	Institution = {Department of Statistics, Stanford University},
	Number = {2001-218},
	Title = {Microarrays, empirical Bayes methods, and false discovery rates},
	Year = {2001}}

@article{Finner99,
	Author = {H. Finner},
	Journal = {Annals of Statistics},
	Pages = {274--289},
	Title = {Stepwise multiple test procedures and control of directional errors},
	Volume = {27},
	Year = {1999}}

@article{Fisher36,
	Author = {R. A. Fisher},
	Journal = {Annals of Eugenics},
	Pages = {179-188},
	Title = {The use of multiple measurements in taxonomic problems},
	Volume = {7},
	Year = {1936}}

@article{Fisher26,
	Author = {R. A. Fisher},
	Journal = {J. Min. Agric. Gr. Br},
	Pages = {505--513},
	Title = {The arrangement of field experiments},
	Volume = {33},
	Year = {1926}}

@techreport{Fix&Hodges51,
	Author = {E. Fix and J. Hodges},
	Institution = {Randolph Field, Texas: USAF School of Aviation Medicine},
	Title = {Discriminatory analysis, nonparametric discrimination: consistency properties},
	Year = {1951}}

@article{Fowlkes&Mallows83,
	Author = {E. B. Fowlkes and C. L. Mallows},
	Journal = JASA,
	Optnumber = {383},
	Pages = {553--584},
	Title = {A method for comparing two hierarchical clusterings},
	Volume = {78},
	Year = {1983}}

@article{Fowlkes&Gnanadesikan&Kettenring88,
	Author = {E. B. Fowlkes and R. Gnanadesikan and J. R. Kettenring},
	Journal = JC,
	Pages = {205--228},
	Title = {Variable selection in clustering},
	Volume = {5},
	Year = {1988}}

@techreport{Fraley&Raftery98,
	Author = {C. Fraley and A. Raftery},
	Institution = {Department of Statistics, University of Washington},
	Note = {\url{http://www.stat.washington.edu/www/research/reports/1990s/#1998}},
	Number = {329},
	Title = {How many clusters? Which clustering method? -- answers via model-based cluster analysis},
	Year = {1998}}

@article{Freund&Schapire97,
	Author = {Y. Freund and R. E. Schapire},
	Journal = {Journal of Computer and System Sciences},
	Pages = {119--139},
	Title = {A decision-theoretic generalization of on-line learning and an application to boosting},
	Volume = {55},
	Year = {1997}}

@phdthesis{Fridlyand01,
	Author = {J. Fridlyand},
	School = {Department of Statistics, U.C. Berkeley},
	Title = {Resampling methods for variable selection and classification: applications to genomics},
	Type = {Ph.{D}. thesis},
	Year = {2001}}

@techreport{Friedman94,
	Author = {J. H. Friedman},
	Institution = {Department of Statistics, Stanford University},
	Title = {Flexible metric nearest neighbor clasification},
	Year = {1994}}

@techreport{Friedman96a,
	Author = {J. H. Friedman},
	Institution = {Department of Statistics, Stanford University},
	Title = {On bias, variance, 0/1-loss, and the curse--of--dimensionality},
	Year = {1996}}

@techreport{Friedman96b,
	Author = {J. H. Friedman},
	Institution = {Department of Statistics, Stanford University},
	Title = {Another approach to polychotomous classification},
	Year = {1996}}

@article{Friedman&Hastie&Tibshirani00,
	Author = {J. Friedman and T. Hastie and R. Tibshirani},
	Journal = {Annals of Statistics},
	Note = {(with discussion)},
	Pages = {337--404},
	Title = {Additive logistic regression: a statistical view of boosting},
	Volume = {28},
	Year = {2000}}

@book{Hastie&Tibshirani90,
	Address = {London},
	Author = {T. J. Hastie and R.J. Tibshirani},
	Publisher = {Chapman and Hall},
	Title = {Generalized Additive Models},
	Year = {1990}}

@article{Gabriel71,
	Author = {K. R. Gabriel},
	Journal = {Biometrika},
	Pages = {453--467},
	Title = {The biplot graphic display of matrices with application to principal component analysis},
	Volume = {58},
	Year = {1971}}

@incollection{Gabriel75,
	Author = {K. R. Gabriel},
	Booktitle = {Multivariate Statistical Methods: Among-groups covariation; Within-group covariation},
	Pages = {61--80},
	Title = {A comparison of some methods of simultaneous inference in {MANOVA}},
	Year = {1975}}

@inproceedings{Gabriel&Pun79,
	Author = {K. R. Gabriel and F. C. Pun},
	Booktitle = {Sixth Conference on Probability and Statistics in Atmospheric Science},
	Organization = {American Meterological Society},
	Pages = {248--253},
	Title = {Binary prediction of weather events with several predictors},
	Year = {1979}}

@unpublished{Ge&Dudoit02,
	Author = {Y. Ge and S. Dudoit},
	Note = {(In preparation)},
	Title = {Fast algorithm for resampling-based $p$-value adjustment in multiple testing},
	Year = {2002}}

@article{Geisser75,
	Author = {S. Geisser},
	Journal = {Journal of the American Statistical Association},
	Pages = {320-328},
	Title = {The predictive sample reuse method with applications},
	Volume = {70},
	Year = {1975}}

@techreport{Genovese&Wasserman01,
	Author = {C. Genovese and L. Wasserman},
	Institution = {Department of Statistics, Carnegie Mellon},
	Number = {737},
	Title = {Operating Characteristics and Extensions of the FDR Procedure},
	Year = {2001}}

@article{Gnanadesikan&Kettenring95,
	Author = {R. Gnanadesikan and J. R. Kettenring},
	Journal = JC,
	Pages = {113--136},
	Title = {Weighting and selection of variables for cluster analysis},
	Volume = {12},
	Year = {1995}}

@article{Goldstein&Dudoit&Speed00,
	Author = {D. R. Goldstein and S. Dudoit and T. P. Speed},
	Journal = {Genetic Epidemiology},
	Number = {Suppl. 1},
	Pages = {S85--S91},
	Title = {Power of a score test for quantitative trait linkage analysis of relative pairs.},
	Volume = {19},
	Year = {2000}}

@article{Goldstein&Dudoit&Sped01,
	Author = {D. R. Goldstein and S. Dudoit and T. P. Speed},
	Journal = {Genetic Epidemiology},
	Number = {4},
	Pages = {415--431},
	Title = {Power and robustness of a score test for linkage analysis of quantitative traits using identity by descent data on sib pairs},
	Volume = {20},
	Year = {2001}}

@article{Gordon&Olshen85,
	Author = {L. Gordon and R.A. Olshen},
	Journal = {Cancer Treatment Reports},
	Pages = {10065-1069},
	Title = {Tree-structured survival analysis},
	Volume = {69},
	Year = {1985}}

@incollection{Gordon96,
	Address = {River Edge, NJ},
	Author = {A. D. Gordon},
	Booktitle = {Clustering and Classification},
	Editor = {P. Arabie and L. J. Hubert and G. De Soete},
	Pages = {65--121},
	Publisher = {World Scientific Publishing Co.},
	Title = {Hierarchical classification},
	Year = {1996}}

@book{Gower&Hand96,
	Author = {J. C. Gower and D. J. Hand},
	Edition = {1st},
	Number = {54},
	Publisher = {Chapman \& Hall},
	Series = {Monographs on statistics and applied probability},
	Title = {Biplots},
	Year = {1996}}

@book{Gyorfietal02,
	Address = {New York},
	Author = {L. Gy\"{o}rfi and M. Kohler and A. Krzy\.{z}ak and H. Walk},
	Pages = {100-102},
	Publisher = {Springer-Verlag},
	Title = {A Distribution-Free Theory of Nanparametric Regression},
	Year = {2002}}

@book{Gyorfietal02b,
	Author = {L. Gy\"orfi and M. Kohler and A. Krzy\'{z}ak and H. Walk},
	Publisher = {Springer-Verlag, New York},
	Title = {A distribution-free theory of nonparametric regression},
	Year = {2002}}

@book{Hastie&Tibshirani&Friedman01,
	Author = {T. Hastie and R. Tibshirani and J. H. Friedman},
	Publisher = {Springer Verlag},
	Title = {The Elements of Statistical Learning : Data Mining, Inference, and Prediction},
	Year = {2001}}

@article{Hansen&Yu01,
	Author = {M. H. Hansen and B. Yu},
	Journal = {Journal of the American Statistical Association},
	Pages = {746-774},
	Title = {Model selection and the principle of minimum description length},
	Volume = {96},
	Year = {2001}}

@article{Hardle&Marron85a,
	Author = {W. H{\"a}rdle and J. S. Marron},
	Journal = {Biometrika},
	Pages = {481--484},
	Title = {Asymptotic nonequivalence of some bandwidth selectors in nonparametric regression},
	Volume = {72},
	Year = {1985}}

@article{Hardle&Marron85b,
	Author = {W. H{\"a}rdle and J. S. Marron},
	Journal = {Annals of Statistics},
	Pages = {1465-1481},
	Title = {Optimal bandwidth selection in nonparametric regression function estimation},
	Volume = {13},
	Year = {1985}}

@book{Hardle93,
	Author = {W. H{\"a}rdle},
	Publisher = {Cambridge University Press},
	Title = {Applied Nonparametric Regression},
	Year = {1993}}

@article{Hartigan72,
	Author = {J. A. Hartigan},
	Journal = {Journal of the American Statistical Association},
	Pages = {123--129},
	Title = {Direct clustering of a data matrix},
	Volume = {67},
	Year = {1972}}

@book{Hartigan75,
	Author = {J. A. Hartigan},
	Publisher = {Wiley},
	Title = {Clustering Algorithms},
	Year = {1975}}

@article{Hartigan78,
	Author = {J. Hartigan},
	Journal = {Annals of Statistics},
	Pages = {117--131},
	Title = {Asymptotic distributions for clustering criteria},
	Volume = {6},
	Year = {1978}}

@article{Hartigan85,
	Author = {J. A. Hartigan},
	Journal = JC,
	Pages = {63--76},
	Title = {Statistical theory in clustering},
	Volume = {2},
	Year = {1985}}

@article{Hastie&Tibshirani96a,
	Author = {T. Hastie and R. Tibshirani},
	Journal = {IEEE Pattern Recognition and Machine Intelligence},
	Pages = {607--616},
	Title = {Discriminant adaptive nearest-nieghbor classification},
	Volume = {18},
	Year = {1996}}

@techreport{Hastie&Tibshirani96b,
	Author = {T. Hastie and R. Tibshirani},
	Institution = {Department of Statistics, Stanford University},
	Title = {Classification by pairwise coupling},
	Year = {1996}}

@article{Hastie&Tibshirani90,
	Author = {T.J. Hastie and R.J. Tibshirani},
	Journal = {Biometrics},
	Number = {4},
	Pages = {1005-1016},
	Title = {Exploring the nature of covariate effects in the proportional hazar ds model},
	Volume = {46},
	Year = {1990}}

@book{Hochberg&Tamhane87,
	Author = {Y. Hochberg and A. C. Tamhane},
	Publisher = {Wiley--Interscience},
	Series = {Probability and Mathematical Statistics},
	Title = {Multiple Comparison Procedures},
	Year = {1987}}

@article{Hochberg88,
	Author = {Y. Hochberg},
	Journal = {Biometrika},
	Pages = {800--802},
	Title = {A sharper Bonferroni procedure for multiple tests of significance},
	Volume = {75},
	Year = {1988}}

@article{Holm79,
	Author = {S. Holm},
	Journal = {Scand. J. Statist.},
	Pages = {65--70},
	Title = {A simple sequentially rejective multiple test procedure},
	Volume = {6},
	Year = {1979}}

@article{Hommel&Bernhard99,
	Author = {G. Hommel and G. Bernhard},
	Journal = {Journal of Statistical Planning and Inference},
	Pages = {119--128},
	Title = {Bonferroni procedures for logically related hypotheses},
	Volume = {82},
	Year = {1999}}

@article{Hommel88,
	Author = {G. Hommel},
	Journal = {Biometrika},
	Pages = {383--386},
	Title = {A stagewise rejective multiple test procedure based on a modified Bonferroni test},
	Volume = {75},
	Year = {1988}}

@article{Hubert&Arabie85,
	Author = {L. Hubert and P. Arabie},
	Journal = JC,
	Pages = {193--218},
	Title = {Comparing partitions},
	Volume = {2},
	Year = {1985}}

@book{Jain&Dubes88,
	Address = {Englewood Cliffs, N. J.},
	Author = {A. K. Jain and R. C. Dubes},
	Publisher = {Prentice-Hall},
	Title = {Algorithms for Clustering Data},
	Year = {1988}}

@article{Jogdeo77,
	Author = {K. Jogdeo},
	Journal = {Annals of Statistics},
	Pages = {495--504},
	Title = {Association and probability inequalities},
	Volume = {5},
	Year = {1977}}

@book{Kaufman&Rousseeuw90,
	Author = {L. Kaufman and P. J. Rousseeuw},
	Publisher = {Wiley, New York.},
	Title = {Finding Groups in Data: An Introduction to Cluster Analysis},
	Year = {1990}}

@article{Keles&vanderLaan&Dudoit03,
	Author = {Kele\c{s}, S. and van der Laan, M. and Dudoit, S.},
	Journal = {Technical Report, Division of Biostatistics, UC Berkeley},
	Title = {Asymptotically Optimal Model Selection Method for Regression on Censored Outcomes},
	Year = {2002}}

@article{Kohonen90,
	Author = {T. Kohonen},
	Journal = {Proc. IEEE},
	Number = {9},
	Pages = {1464--1480},
	Title = {The self-organizing map},
	Volume = {78},
	Year = {1990}}

@book{Kohonen95,
	Address = {Berlin, Heidelberg},
	Author = {T. Kohonen},
	Editor = {T. S. Huang and T. Kohonen and M. R. Schroeder},
	Publisher = {Springer},
	Series = {Springer Series in Information Sciences},
	Title = {Self-Organizing Maps},
	Volume = {30},
	Year = {1995}}

@article{Kooperberg&Stone&Truong95,
	Author = {C. Kooperberg and C.J. Stone and Y. K. Truong},
	Journal = {Journal of the American Statistical Association},
	Number = {429},
	Pages = {78-94},
	Title = {Hazard Regression},
	Volume = {90},
	Year = {1995}}

@article{Koutsoukosetal94,
	Author = {A. D. Koutsoukos and L. V. Rubinstein and D. Faraggi and R.M. Simon and S. Kalyandrug and J. N. Weinstein and K.W. Kohn and K.D. Paull},
	Journal = {Statistics in Medicine},
	Pages = {719--730},
	Title = {Discrimination techniques applied to the {NCI} in vitro anti-tumor drug screen: predicting biochemical mechanism of action},
	Volume = {13},
	Year = {1994}}

@article{Krishnaiah&Reising85,
	Author = {P. R. Krishnaiah and J. M. Reising},
	Journal = {Encyclopedia of Statistical Sciences},
	Number = {6},
	Pages = {88--95},
	Title = {Multivariate multiple comparisons},
	Volume = {9},
	Year = {1985}}

@article{Krzanowski&Lai85,
	Author = {W. Krzanowski and Y. Lai},
	Journal = {Biometrics},
	Pages = {23--34},
	Title = {A criterion for determining the number of groups in a dataset using sum of squares clustering},
	Volume = {44},
	Year = {1985}}

@article{Laan&Bryan01,
	Author = {M. J. van der Laan and J. Bryan},
	Journal = {Biostatistics},
	Number = {4},
	Pages = {445--461},
	Title = {Gene expression analysis with the parametric bootstrap},
	Volume = {2},
	Year = {2001}}

@article{Pollard&vanderLaan04,
	Author = {K. S. Pollard and M.J. van der Laan},
	Journal = JSPI,
	Optpages = {85--101},
	Optvolume = {125},
	Title = {Choice of Null Distribution in Resampling Based Multiple Testing},
	Year = {2004}}

@article{vanderLaan&Pollard02,
	Author = {M. J. van der Laan and K. S. Pollard},
	Journal = JSPI,
	Note = {(To appear)},
	Title = {Hybrid clustering of gene expression data with visualization and the bootstrap},
	Year = {2002}}

@article{Leblanc&Crowley92,
	Author = {M. Leblanc and J. Crowley},
	Journal = {Biometrics},
	Pages = {411-425},
	Title = {Relative Risk trees for censored data},
	Volume = {48},
	Year = {1992}}

@inproceedings{Leisch02,
	Author = {F. Leisch},
	Booktitle = {Compstat 2002 --- Proceedings in Computational Statistics},
	Editor = {Wolfgang H{\"a}rdle and Bernd R{\"o}nz},
	Note = {ISBN 3-7908-1517-9},
	Publisher = {Physika Verlag, Heidelberg, Germany},
	Title = {Sweave: Dynamic Generation of Statistical Reports Using Literate Data Analysis},
	Tpages = {575--580},
	Url = {http://www.ci.tuwien.ac.at/~leisch/Sweave},
	Year = {2002},
	Bdsk-Url-1 = {http://www.ci.tuwien.ac.at/~leisch/Sweave}}

@techreport{Leisch02Tb,
	Author = {F. Leisch},
	Institution = {SFB Adaptive Information Systems and Modelling in Economics and Management Science, Vienna University of Economics and Business Administration},
	Month = {March},
	Number = {69},
	Title = {Dynamic generation of statistical reports using literate data analysis},
	Year = {2002}}

@techreport{Leisch99,
	Author = {F. Leisch},
	Institution = {SFB Adaptive Information Systems and Modelling in Economics and Management Science, Vienna University of Economics and Business Administration},
	Month = {August},
	Note = {\url{http://www.ci.tuwien.ac.at/~leisch/papers/fl-techrep.html}},
	Title = {Bagged clustering},
	Year = {1999}}

@article{Lim&Low&Shih00,
	Author = {T-S Lim and W-Y Loh and Y-S Shih},
	Journal = {Machine Learning},
	Pages = {203--229},
	Title = {A comparison of prediction accuracy, complexity, and training time of thiry-three old and new classification algorithms},
	Volume = {40},
	Year = {2000}}

@book{Mardia&Kent&Bibby79,
	Address = {San Diego},
	Author = {K. V. Mardia and J. T. Kent and J. M. Bibby},
	Publisher = {Academic Press, Inc.},
	Title = {Multivariate Analysis},
	Year = {1979}}

@unpublished{Mayo&Spanos02,
	Author = {D. C. Mayo and A. Spanos},
	Title = {A severe-testing interpretation of {N}eyman-{P}earson methods. Unpublished manuscript},
	Year = {2002}}

@book{McCullagh&Nelder89,
	Author = {P. McCullagh and J. A. Nelder},
	Edition = {2nd},
	Number = {37},
	Publisher = {Chapman \& Hall},
	Series = {Monographs on Statistics and Applied Probability},
	Title = {Generalized Linear Models},
	Year = {1989}}

@book{McLachlan92,
	Address = {New York},
	Author = {G. J. McLachlan},
	Publisher = {Wiley},
	Title = {Discriminant analysis and statistical pattern recognition},
	Year = {1992}}

@article{McLachlan&Bean&Peel01,
	Author = {G. J. McLachlan and R. Bean and D. Peel},
	Journal = {Bioinformatics},
	Pages = {413--422},
	Title = {A mixture model-based approach to the clustering of microarray expression data.},
	Volume = {18},
	Year = {2002}}

@book{Miller90,
	Author = {A. J. Miller},
	Publisher = {Chapman and Hall},
	Title = {Subset Selection in Regression},
	Year = {1990}}

@article{Milligan&Cooper85,
	Author = {G. W. Milligan and M. C. Cooper},
	Journal = {Psychometrika},
	Pages = {159--179},
	Title = {An examination of procedures for determining the number of clusters in a data set},
	Volume = {50},
	Year = {1985}}

@article{Milligan&Cooper86,
	Author = {G. W. Milligan and M. C. Cooper},
	Journal = {Multivariate Behavioral Research},
	Pages = {441--458},
	Title = {A study of the comparability of external criteria for hierarchical cluster analysis},
	Volume = {21},
	Year = {1986}}

@article{Milligan&Cooper87,
	Author = {G. W. Milligan and M. C. Cooper},
	Journal = {Applied Psychological Measurement},
	Optmonth = {December},
	Optnumber = {4},
	Pages = {329--354},
	Title = {Methodology review: {C}lustering methods},
	Volume = {11},
	Year = {1987}}

@article{Milligan89,
	Author = {G. W. Milligan},
	Journal = {Multivariate Behavioral Research},
	Pages = {163--176},
	Title = {A study of the beta-flexible clustering method},
	Volume = {24(2)},
	Year = {1989}}

@incollection{Milligan96,
	Address = {River Edge, NJ},
	Author = {G. W. Milligan},
	Booktitle = {Clustering and Classification},
	Editor = {P. Arabie and L. J. Hubert and G. De Soete},
	Pages = {341--375},
	Publisher = {World Scientific Publishing Co.},
	Title = {Clustering validation: {R}esults and implications for applied analyses},
	Year = {1996}}

@article{Morey&Blashfield&Skinnerl83,
	Author = {L. C. Morey, R. K. Blashfield and H. A. Skinner},
	Journal = {Multivariate Behavioral Research},
	Pages = {309--329},
	Title = {A comparison of cluster analysis techniques within a sequential validation framework},
	Volume = {18},
	Year = {1983}}

@book{Morrison90,
	Author = {D. F. Morrison},
	Edition = {3rd},
	Publisher = {McGraw-Hill, NY},
	Title = {Multivariate Statistical Methods},
	Year = {1990}}

@incollection{Murtagh96,
	Address = {River Edge, NJ},
	Author = {F. Murtagh},
	Booktitle = {Clustering and Classification},
	Editor = {P. Arabie and L. J. Hubert and G. De Soete},
	Pages = {235--269},
	Publisher = {World Scientific Publishing Co.},
	Title = {Neural networks for clustering},
	Year = {1996}}

@article{PanelDACC89,
	Author = {{Panel on Discriminant Analysis, Classification, and Clustering}},
	Journal = {Statistical Science},
	Pages = {34--69},
	Title = {Discriminant analysis and clustering},
	Volume = {4},
	Year = {1989}}

@techreport{Pavlic&vanderLaan89,
	Author = {M. Pavlic and M. J. van der Laan},
	Institution = {Division of Biostatistics, U.C. Berkeley},
	Month = {February},
	Number = {89},
	Title = {Fitting of mixtures with unspecified number of components using cross-validation distance estimate},
	Year = {2001}}

@article{Pavlic&vanderLaan02,
	Author = {M. Pavlic and M. J. van der Laan},
	Issue = {3-4},
	Journal = {Computational Statistics and Data Analysis},
	Pages = {413-428},
	Title = {Fitting of mixtures with unspecified number of components using cross validation distance estimate},
	Volume = {41},
	Year = {2003}}

@techreport{Pollard&vanderLaan02,
	Author = {K. S. Pollard and M. J. van der Laan},
	Institution = {Division of Biostatistics, U.C. Berkeley},
	Month = {April},
	Number = {107},
	Title = {A Method to Identify Significant Clusters in Gene Expression Data},
	Year = {2002}}

@techreport{Pollard&vanderLaan02b,
	Author = {K. S. Pollard and M. J. van der Laan},
	Institution = {Division of Biostatistics, U.C. Berkeley},
	Number = {121},
	Title = {Resampling-based methods for identification of significant subsets of genes in expression data},
	Year = {2002}}

@article{Ramsey78,
	Author = {P. H. Ramsey},
	Journal = JASA,
	Pages = {479--485},
	Title = {Power differences between pairwise multiple comparisons},
	Volume = {73},
	Year = {1978}}

@manual{Breiman01b,
	Author = {L. Breiman},
	Title = {Notes on setting up, using, and understanding random forests V3.0},
	Year = {2001}}

@article{Rand71,
	Author = {W. M. Rand},
	Journal = {Journal of the American Statistical Association},
	Optnumber = {336},
	Pages = {846--850},
	Title = {Objective criteria for the evaluation of clustering methods},
	Volume = {66},
	Year = {1971}}

@unpublished{Reiner&Yekutieli&Benjaminil01,
	Author = {A. Reiner and D. Yekutieli and Y. Benjamini},
	Title = {Using resampling-based {FDR} controlling multiple test procedures for analyzing microarray gene expression data},
	Year = {2001}}

@book{Ripley96,
	Address = {Cambridge, New York},
	Author = {B. D. Ripley},
	Publisher = {Cambridge University Press},
	Title = {Pattern recognition and neural networks},
	Year = {1996}}

@article{Rissanen78,
	Author = {J. Rissanen},
	Journal = {Automatica},
	Pages = {465-471},
	Title = {Modelling by shortest data description},
	Volume = {14},
	Year = {1978}}

@article{Rnews:Dudoit&Yang&Bolstad02,
	Author = {S. Dudoit and Y. H. Yang and B. Bolstad},
	Journal = {R News},
	Month = {March},
	Number = 1,
	Pages = {24--32},
	Title = {Using {R} for the Analysis of {DNA} Microarray Data},
	Url = {CRAN.R-project.org/doc/Rnews/},
	Volume = 2,
	Year = 2002,
	Bdsk-Url-1 = {CRAN.R-project.org/doc/Rnews/}}

@article{Robins&Botnitzky00,
	Author = {J. M. Robins and A. Rotnitzky},
	Journal = {Statistica Sinica},
	Number = {4},
	Pages = {920-936},
	Title = {Comment on the {B}ickel and {K}won article, ``{I}nference for semiparametric models: {S}ome questions and an answer''},
	Volume = {11},
	Year = {2001}}

@inproceedings{Robins00,
	Author = {J.M. Robins},
	Booktitle = {Proceedings of the American Statistical Association},
	Title = {Robust estimation in sequentially ignorable missing data and causal inference models},
	Year = {2000}}

@article{Robins&Rotnitzky&vanderLaan00,
	Author = {J. M. Robins and A. Rotnitzky and M.J. van der Laan},
	Journal = {Journal of the American Statistical Association -- Theory and Methods},
	Pages = {431-435},
	Title = {Comment on ``{O}n {P}rofile {L}ikelihood" by {S}.{A}. {M}urphy and {A}.{W}. van der {V}aart},
	Volume = {450},
	Year = {2000}}

@article{Birge83,
	Author = {L. Birg{\'e}},
	Journal = {Verw. Gebiete},
	Pages = {181--238},
	Title = {Approximation dans les espaces m{/'e}triques et th{\'e}orie de l'estimation},
	Volume = {65},
	Year = {1983}}

@article{lecam73,
	Author = {L.M. le Cam},
	Journal = {Annals of Statistics},
	Pages = {38--53},
	Title = {Convergence of estimates under dimensionality restrictions},
	Volume = {22},
	Year = {1973}}

@article{Rom90,
	Author = {D. M. Rom},
	Journal = {Biometrika},
	Pages = {663-665},
	Title = {A sequentially rejective test procedure based on a modified {Bonferroni} inequality},
	Volume = {77},
	Year = {1990}}

@techreport{Rosenblatt57,
	Author = {F. Rosenblatt},
	Institution = {Cornell Aeronautical Laboratory},
	Number = {86-460-1},
	Title = {The perceptron -- a perceiving and recognizing automation},
	Year = {1957}}

@article{Ruczinskietal&Kooperberg&LeBlanc01,
	Author = {I. Ruczinski and C. Kooperberg and M. LeBlanc},
	Note = {Submitted, \url{http://biosun01.biostat.jhsph.edu/~iruczins/html/publications.html}},
	Title = {Logic regression},
	Year = {2001}}

@article{Saltstone&Stange96,
	Author = {R. Saltstone and K. Stange},
	Journal = {Journal of Classification},
	Pages = {169--172},
	Title = {A computer program to calculate Hubert and Arabie's adjusted Rand index},
	Volume = {13},
	Year = {1996}}

@techreport{vanderVaart03,
	Author = {A.W. van der Vaart},
	Institution = {Department of Mathematics, Free University, Amsterdam},
	Optannote = {Unpublished manuscript},
	Title = {Notes on Cross-validation},
	Year = {2003}}

@techreport{Sarle83,
	Author = {W. Sarle},
	Institution = {SAS Institute, Inc.},
	Note = {\url{http://www.sas.com/service/library/onlinedoc/trindex.html}},
	Number = {A-108},
	Title = {Cubic clustering criterion},
	Year = {1983}}

@techreport{Sarle&Kuo93,
	Author = {W. Sarle and A. Kuo},
	Institution = {SAS Institute, Inc.},
	Number = {P-256},
	Title = {The MODECLUS Procedures},
	Year = {1993}}

@article{Schapireetal98,
	Author = {R. E. Schapire and Y. Freund and P. Bartlett and W. S. Lee},
	Journal = {Annals of Statistics},
	Pages = {1651--1686},
	Title = {Boosting the margin: a new explanation for the effectiveness of voting methods},
	Volume = {26},
	Year = {1998}}

@book{Scheffe59,
	Author = {H. Scheff\'{e}},
	Publisher = {John Wiley \& Sons},
	Title = {The analysis of variance},
	Year = {1959}}

@article{Scheibler&Schneider85,
	Author = {D. Scheibler and W. Schneider},
	Journal = {Multivariate Behavioral Research},
	Pages = {283--304},
	Title = {Monte Carlo tests of the accuracy of cluster analysis algorithms: A comparison of hierarchical and nonhierarchical methods},
	Volume = {20},
	Year = {1985}}

@inproceedings{Schuster&Gregory81,
	Author = {E. F. Schuster and C. G. Gregory},
	Booktitle = {Computer Science and Statistics: Proceedings of the 13th Symposium on the interface},
	Editor = {Eddy, W.F.},
	Pages = {295-298},
	Title = {On the non-consistency of maximum likelihood nonparametric density estimators},
	Year = {1981}}

@article{Scott&Factor81,
	Author = {D. W. Scott and L. E. Factor},
	Journal = {Journal of the American Statistical Association},
	Pages = {9-15},
	Title = {Monte Carlo study of three data-based nonparametric density estimators},
	Volume = {76},
	Year = {1981}}

@article{Seeger68,
	Author = {P. Seeger},
	Journal = {Technometrics},
	Number = {3},
	Pages = {586--593},
	Title = {A note on a method for the analysis of significances en masse},
	Volume = {10},
	Year = {1968}}

@article{Segal88,
	Author = {M. R. Segal},
	Journal = {Biometrics},
	Pages = {35--47},
	Title = {Regression trees for censored data},
	Volume = {44},
	Year = {1988}}

@article{Shaffer02,
	Author = {J. P. Shaffer},
	Journal = {Psychological Methods},
	Pages = {356--369},
	Title = {Multiplicity, directional ({T}ype {III}) errors, and the null hypothesis},
	Volume = {7},
	Year = {2002}}

@article{Shaffer86,
	Author = {J. P. Shaffer},
	Journal = JASA,
	Pages = {826--831},
	Title = {Modified sequentially rejective multiple test procedures},
	Volume = {81},
	Year = {1986}}

@article{Shaffer95,
	Author = {J. P. Shaffer},
	Journal = {Annu. Rev. Psychol.},
	Pages = {561--584},
	Title = {Multiple hypothesis testing},
	Volume = {46},
	Year = {1995}}

@article{Shao93,
	Author = {Shao, J.},
	Journal = {Journal of the American Statistical Association},
	Pages = {486-494},
	Title = {Linear Model Selection by Cross-Validation},
	Volume = {88},
	Year = {1993}}

@article{Sidak67,
	Author = {Z. \v{S}id\'{a}k},
	Journal = JASA,
	Pages = {626-633},
	Title = {Rectangular confidence regions for the means of multivariate normal distributions},
	Volume = {62},
	Year = {1967}}

@article{Silverman96,
	Author = {B. W. Silverman},
	Journal = {Annals of Statistics},
	Pages = {1--24},
	Title = {Smoothed functional principal components analysis by choice of norm},
	Volume = {24},
	Year = {1996}}

@article{Silverman84,
	Author = {B. W. Silverman},
	Journal = JASA,
	Number = {387},
	Pages = {584--589},
	Title = {A fast and efficient cross-validation method for smoothing parameter choice in spline regression},
	Volume = {79},
	Year = {1984}}

@book{Silverman86,
	Author = {B. W. Silverman},
	Publisher = {Chapman \& Hall},
	Title = {Density Estimation for Statistics and Data analysis},
	Year = {1986}}

@article{vanderLaan&Dudoit&Keles04,
	Author = {M.J. van der Laan and S. Dudoit and S. Keles},
	Journal = {Statistical Applications in Genetics and Molecular Biology},
	Optnote = {http://www.bepress.com/sagmb/vol3/iss1/art4},
	Optnumber = {1},
	Title = {Asymptotic optimality of likelihood-based cross-validation},
	Volume = {3},
	Year = {2004}}

@article{Simes86,
	Author = {R. J. Simes},
	Journal = {Biometrika},
	Pages = {751--754},
	Title = {An improved Bonferroni procedure for multiple tests of significance},
	Volume = {73},
	Year = {1986}}

@article{Smyth00,
	Author = {P. Smyth},
	Journal = {Statistics and Computing},
	Pages = {63-72},
	Title = {Model selection of probabilistic clustering using cross-validated likelihood},
	Volume = {10},
	Year = {2000}}

@article{Soric89,
	Author = {B. Sori\'{c}},
	Journal = JASA,
	Number = {406},
	Pages = {608--610},
	Title = {Statistical ``discoveries" and effect-size estimation},
	Volume = {84},
	Year = {1989}}

@article{Stone74,
	Author = {M. Stone},
	Journal = {Journal of the Royal Statistical Society, Series B},
	Pages = {111-147},
	Title = {Cross-validatory choice and assessment of statistical predictions},
	Volume = {36},
	Year = {1974}}

@article{Stone84,
	Author = {C. J. Stone},
	Journal = {Annals of Statistics},
	Number = {4},
	Pages = {1285--1297},
	Title = {An asymptotically optimal window selection rule for kernel density estimates},
	Volume = {12},
	Year = {1984}}

@article{Stone74,
	Author = {M. Stone},
	Journal = JRSSB,
	Number = {2},
	Pages = {111--147},
	Title = {Cross-validatory choice and assessment of statistics predictions},
	Volume = {36},
	Year = {1974}}

@article{Stone77,
	Author = {M. Stone},
	Journal = {Biometrika},
	Number = {1},
	Pages = {29--35},
	Title = {Asymptotics for and against cross-validation},
	Volume = {64},
	Year = {1977}}

@techreport{Storey&Tibshirani01,
	Author = {J. D. Storey and R. Tibshirani},
	Institution = {Department of Statistics, Stanford University},
	Number = {2001-28},
	Title = {Estimating false discovery rates under dependence, with applications to DNA microarrays},
	Year = {2001}}

@article{Storey02,
	Author = {J. D. Storey},
	Journal = JRSSB,
	Pages = {479--498},
	Title = {A direct approach to false discovery rates},
	Volume = {64},
	Year = {2002}}

@techreport{Storey01,
	Author = {J. D. Storey},
	Institution = {Department of Statistics, Stanford University},
	Number = {2001-12},
	Title = {The positive False Discovery Rate: A Bayesian interpretation and the q-value},
	Year = {2001}}

@book{Lehmann86,
	Author = {E. L. Lehmann},
	Edition = {2nd},
	Publisher = {Springer-Verlag, New York},
	Title = {Testing Statistical Hypotheses},
	Year = {1986}}

@article{Tibshiranietal02a,
	Author = {R. Tibshirani and T. Hastie and B. Narasimhan and. G. Chu},
	Journal = PNAS,
	Note = {In press},
	Title = {Diagnosis of multiple cancer types by shrunken centroids of gene expression},
	Year = {2002}}

@article{Troendle95,
	Author = {J. F. Troendle},
	Journal = JASA,
	Pages = {370--378},
	Title = {A stepwise resampling method of multiple hypothesis testing},
	Volume = {90},
	Year = {1995}}

@article{Troendle96,
	Author = {J. F. Troendle},
	Journal = {Biometrics},
	Pages = {846--859},
	Title = {A permutational step-up method of testing multiple outcomes},
	Volume = {52},
	Year = {1996}}

@book{vanderVaart&Wellner96,
	Author = {A. W. van der Vaart and J. A. Wellner},
	Pages = {102},
	Publisher = {Springer-Verlag New York},
	Title = {Weak {C}onvergence and {E}mprical {P}rocesses},
	Year = {1996}}

@book{vanderVaart98,
	Author = {A. W. van der Vaart},
	Pages = {62},
	Publisher = {Cambridge University Press},
	Title = {Asymptotic Statistics},
	Year = {1998}}

@book{Vapnik00,
	Address = {New York},
	Author = {V. N. Vapnik},
	Edition = {2nd},
	Publisher = {Springer},
	Series = {Statistics for engineering and information science},
	Title = {The nature of statistical learning theory},
	Year = {2000}}

@article{Vapnik79,
	Author = {V. Vapnik},
	Journal = {Nauka, Moskow},
	Title = {Estimation of dependences based on empirical data (in Russian)},
	Year = {1979}}

@book{Vapnik98,
	Address = {New York},
	Author = {V. Vapnik},
	Edition = {1st},
	Publisher = {Wiley},
	Title = {Statistical Learning Theory},
	Year = {1998}}

@book{Venables&Ripley99,
	Author = {W. N. Venables and B. D. Ripley},
	Edition = {3rd},
	Publisher = {Springer},
	Title = {Modern applied statistics with S-PLUS},
	Year = {1999}}

@book{Westfall&Young93,
	Author = {P. H. Westfall and S. S. Young},
	Publisher = {John Wiley \& Sons},
	Title = {Resampling-based multiple testing: {E}xamples and methods for $p$-value adjustment},
	Year = {1993}}

@incollection{Westfalletal&Zaykin&Young01,
	Author = {P. H. Westfall and D. V. Zaykin and S. S. Young},
	Booktitle = {Biostatistical Methods},
	Editor = {S. Looney},
	Pages = {143--168},
	Publisher = {Humana Press, Toloway, NJ},
	Series = {Methods in Molecular Biology},
	Title = {Multiple tests for genetic effects in association studies},
	Volume = {184},
	Year = {2001}}

@article{Westonetal2000,
	Author = {J. Weston and S. Mukherjee and O. Chappelle and M. Pontil and T. Poggio and V. Vapnik},
	Journal = {Advances in Neural Processing Systems},
	Pages = {668--674},
	Title = {Feature Selection for {SVM}s},
	Volume = {13},
	Year = {2001}}

@article{Wright92,
	Author = {S. P. Wright},
	Journal = {Biometrics},
	Number = {4},
	Pages = {1005--1013},
	Title = {Adjusted P-values for simultaneous inference},
	Volume = {48},
	Year = {1992}}

@article{Yangetal02,
	Author = {Y. H. Yang and M. J. Buckley and S. Dudoit and T. P. Speed},
	Journal = {Journal of Computational and Graphical Statistics},
	Number = {1},
	Pages = {108--136},
	Title = {Comparison of methods for image analysis on c{DNA} microarray data},
	Volume = {11},
	Year = {2002}}

@article{Yangetal02b,
	Author = {Y. H. Yang and S. Dudoit and P. Luu and D. M. Lin and V. Peng and J. Ngai and T. P. Speed},
	Journal = {Nucleic Acids Research},
	Number = {4},
	Pages = {e15},
	Title = {Normalization for c{DNA} microarray data: {A} robust composite method addressing single and multiple slide systematic variation},
	Volume = {30},
	Year = {2002}}

@inproceedings{Yangetal01,
	Address = {San Jose, CA},
	Author = {Y. H. Yang and S. Dudoit and P. Luu and T. P. Speed},
	Booktitle = {Microarrays: Optical Technologies and Informatics},
	Editor = {Michael L. Bittner and Yidong Chen and Andreas N. Dorsel and Edward R. Dougherty},
	Month = {May},
	Optorganization = {SPIE},
	Pages = {141--152},
	Publisher = {SPIE-International Society for Optical Engineering},
	Series = {Proceedings of SPIE},
	Title = {Normalization for c{DNA} microarray data},
	Volume = {4266},
	Year = {2001}}

@article{Yekutieli&Benjamini99,
	Author = {D. Yekutieli and Y. Benjamini},
	Journal = JSPI,
	Pages = {171--196},
	Title = {Resampling-based false discovery rate controlling multiple test procedures for correlated test statistics},
	Volume = {82},
	Year = {1999}}

@incollection{Youden69,
	Author = {W. J. Youden},
	Booktitle = {Precision measurement and calibration: Statistical concepts and procedures},
	Editor = {H. H. Ku},
	Month = {February},
	Pages = {146--151},
	Publisher = {National Bureau of Standards, United States Department of Commerce},
	Series = {Special Publication 300},
	Title = {Measurement agreement comparisons},
	Type = {NBS Miscelaneous Publication 248, Proceedings of the 1962 Standards Laboratory Conference},
	Volume = {1},
	Year = {1969}}

@article{Zhang93,
	Author = {Zhang, P.},
	Journal = {Annals of Statistics},
	Pages = {299-313},
	Title = {Model selection via multifold cross-validation},
	Volume = {21},
	Year = {1993}}

@article{Zhang&Carey&Gentleman02,
	Author = {J. Zhang and V. Carey and R. Gentleman},
	Journal = {Bioinformatics},
	Note = {(In press)},
	Title = {An extensible application for assembling annotation for genomic data},
	Url = {http://www.R-project.org/},
	Year = {2002},
	Bdsk-Url-1 = {http://www.R-project.org/}}

@book{Bickeletal97,
	Author = {P.J. Bickel and C.A.J. Klaassen and Y. Ritov and J. Wellner},
	Publisher = {Springer-Verlag},
	Title = {Efficient and Adaptive Estimation for Semiparametric Models},
	Year = {1997}}

@article{Bozdogan00,
	Author = {H. Bozdogan},
	Journal = {Journal of Mathematical Psychology},
	Pages = {62-91},
	Title = {Akaike's information criterion and recent developments in information complexity},
	Volume = {44},
	Year = {2000}}

@book{Breimanetal84,
	Address = {Monterey},
	Author = {L. Breiman and J. H. Friedman and R. A. Olshen and C. J. Stone},
	Publisher = {Wadsworth \& Brooks/Cole},
	Title = {Classification and Regression Trees},
	Year = {1984}}

@book{vanderlaan&Robins03,
	Author = {M.J. van der Laan and J.M. Robins},
	Publisher = {Springer, New York},
	Title = {Unified methods for censored longitudinal data and causality},
	Year = {2003}}

@manual{effsize,
	Author = {{National Reading Panel}},
	Organization = {National Institute of Child Health and Human Development, National Institutes of Health},
	Title = {Teaching Children to Read},
	Year = {1999}}

@techreport{Tibshirani&Walther&Hastie00,
	Author = {R. Tibshirani and G. Walther and T. Hastie.},
	Institution = {Department of Biostatistics, Stanford University},
	Month = {March},
	Note = {\url{http://www-stat.stanford.edu/~tibs/research.html}},
	Title = {Estimating the number of clusters in a dataset via the gap statistic},
	Year = {2000}}

@inproceedings{Gill&vanderLaan&Robins97,
	Address = {New York},
	Author = {R.D. Gill and M.J. van der Laan and J.M. Robins},
	Booktitle = {Proceedings of the First Seattle Symposium in Biostatistics},
	Editor = {D.Y. Lin and T.R. Fleming},
	Pages = {255-94},
	Publisher = {Springer Verlag},
	Title = {Coarsening at random: characterizations, conjectures and counter-examples},
	Year = {1997}}

@article{Gill&Robins01,
	Author = {Gill, R. and Robins, J.M.},
	Fjournal = {The Annals of Statistics},
	Journal = {Ann. Stat.},
	Number = {6},
	Title = {Causal inference in complex longitudinal studies: continuous case},
	Volume = {29},
	Year = {2001}}

@article{Jacobsen&Keiding95,
	Author = {M. Jacobsen and N. Keiding},
	Journal = {Annals of Statistics},
	Pages = {774-86},
	Title = {Coarsening at random in general sample spaces and random censoring in continuous time},
	Volume = {23},
	Year = {1995}}

@misc{Dudoit&Yang02,
	Author = {S. Dudoit and Y. H. Yang},
	Howpublished = {{\tt R} packages},
	Title = {Normalization and diagnostic plots for cDNA microarray data, {\tt marrayClasses}, {\tt marrayInput}, {\tt marrayNorm}, {\tt marrayPlots}},
	Url = {www.bioconductor.org},
	Year = {2002},
	Bdsk-Url-1 = {www.bioconductor.org}}

@techreport{Fraley&Raftery98,
	Author = {C. Fraley and A. E. Raftery},
	Institution = {Department of Statistics, University of Washington},
	Month = {November},
	Number = {342},
	Title = {MCLUST: Software for Model-Based Cluster Analysis},
	Year = {1998}}

@misc{Ge&Dudoit02,
	Author = {Y. Ge and S. Dudoit},
	Howpublished = {{\tt R} package},
	Title = {Multiple Testing Procedures, {\tt multtest}},
	Url = {www.bioconductor.org},
	Year = {2002},
	Bdsk-Url-1 = {www.bioconductor.org}}

@inproceedings{Robins93,
	Author = {J.M. Robins},
	Booktitle = {Proceeding of the Biopharmaceutical section},
	Organization = {American Statistical Association},
	Pages = {24-33},
	Title = {Information recovery and bias adjustment in proportional hazards regression analysis of randomized trials using surrogate markers},
	Year = {1993}}

@incollection{Robins&Rotnitzky92,
	Author = {J.M. Robins and A. Rotnitzky},
	Booktitle = {AIDS Epidemiology},
	Publisher = {Bikh\"{a}user},
	Series = {Methodological issues},
	Title = {Recovery of information and adjustment for dependent censoring using surrogate markers},
	Year = {1992}}

@article{Robins&Rotnitzky&Zhao94,
	Author = {J.M. Robins and A. Rotnitzky and L.P. Zhao},
	Journal = {Journal of the American Statistical Association},
	Month = {September},
	Number = {427},
	Pages = {846-866},
	Title = {Estimation of regression coefficients when some regressors are not always observed},
	Volume = {89},
	Year = {1994}}

@article{Heitjan&Rubin91,
	Author = {D.F. Heitjan and D.B. Rubin},
	Journal = {Annals of statistics},
	Month = {December},
	Number = {4},
	Pages = {2244-2253},
	Title = {Ignorability and coarse data},
	Volume = {19},
	Year = {1991}}

@misc{Dudoit&Yang&Bolstad01,
	Author = {S. Dudoit and Y. H. Yang and B. M. Bolstad},
	Howpublished = {{\tt R} package},
	Note = {Contributions from Natalie Thorne, Ingrid L\"{o}nnstedt, and Jessica Mar},
	Title = {Statistical {M}icroarray {A}nalysis, {\tt sma}},
	Url = {cran.r-project.org/src/contrib/PACKAGES.html\#sma},
	Year = {2001},
	Bdsk-Url-1 = {cran.r-project.org/src/contrib/PACKAGES.html%5C#sma}}

@phdthesis{Dudoit99,
	Author = {S. Dudoit},
	School = {Department of Statistics, University of California, Berkeley},
	Title = {Linkage analysis of complex human traits using identity by descent data},
	Type = {Ph.D. thesis},
	Year = {1999}}

@book{vanderVaart&Wellner96,
	Author = {A. van der Vaart and J. Wellner},
	Publisher = {Springer-Verlag, New York},
	Title = {Weak Convergence and Empirical Processes},
	Year = {1996}}

@book{Robert07,
	Address = {New York},
	Author = {Robert, P. C.},
	Publisher = {Springer},
	Title = {{T}he {B}ayesian {C}hoice: {F}rom {D}ecision-{T}hoeretic {F}oundations to {C}omputational {I}mplementation},
	Year = {2007}}

@book{Lindley80,
	Address = {Cambridge},
	Author = {Lindley, D. V.},
	Publisher = {Cambridge University Press},
	Title = {{I}ntroduction to {P}robability and {S}tatistics from a {B}ayesian {P}oint of {V}iew, Part 2},
	Year = {1965}}

@article{Tager&Hollenberg&Satariano98,
	Author = {I.B. Tager and M. Hollenberg and W. Satariano},
	Publisher = {American Journal of Epidemiology},
	Title = {Self-reported leisure-time physical activity and measures of cardiorespiratory fitness in an elderly population},
	Year = {1998}}

@techreport{Hubbard&vanderLaan05,
	Author = {A.E. Hubbard and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper191},
	Title = {Population Intervention Models in Causal Inference},
	Type = {Technical Report 191},
	Year = {2005}}

@manual{Ghalanos&Theussl10,
	Author = {A. Ghalanos and S. Theussl},
	Title = {Rsolnp: General Non-linear Optimization Using Augmented Lagrange Multiplier Method. R package},
	Year = {2010}}

@phdthesis{Ye87,
	Author = {Yinyu Ye},
	School = {Department of EES, Stanford University},
	Title = {Interior Algorithms for Linear, Quadratic, and Linearly Constrained Non-Linear Programming},
	Year = {1987}}

@book{vanderLaan&Rose11,
	Address = {New York},
	Author = {M.J. van der Laan and S. Rose},
	Publisher = {Springer},
	Title = {Targeted Learning: Causal Inference for Observational and Experimental Data},
	Year = {2011}}

@book{Kullback59,
	Author = {S. Kullback},
	year = {1959},
	Title = {Information Theory and Statistics},
	Publisher = {John Wiley \& Sons}
	Address = {New York}
}

@incollection {vandervaart02,
   author = {van der Vaart, Aad},
   title = {Semiparameric Statistics},
   booktitle = {Lectures on Probability Theory and Statistics},
   series = {Lecture Notes in Mathematics},
   publisher = {Springer Berlin / Heidelberg},
   keyword = {Mathematics and Statistics},
   pages = {331-457},
   volume = {1781},
   note = {},
   year = {2002}
}

%A. Donner and N. Klar. Design and Analysis of Cluster Randomization Trials in Health Research. Arnold, London, 2000.
%R.J. Hayes and L.H. Moulton. Cluster randomised trials. Chapman & Hall/CRC, Boca Raton, 2009.
%MJ Campbell, A. Donner, and N. Klar. Developments in cluster randomized trials and Statistics in Medicine. Statistics in Medicine, 26(1):2Ð19, 2007. doi: 10.1002/sim.2731.

@article{Robins&Ritov97,
title={Towards a curse of dimensionality appropriate asymptotic theory for semi parametric models},
author={J.M. Robins and Y. Ritov},
year={1997},
journal={Statistics in Medicine},
volume={16},
pages={285--319},
}

@article{vanderLaan&Gruber15,
title={One-step targeted minimum loss-based estimation based on universal least favorable one-dimensional submodels},
author={M.J. van der Laan and S. Gruber},
year={2015},
journal={to appear in International Journal of Biostatistics},
volume={},
pages={},
}


@article{Neuhaus71,
title={On weak convergence of stochastic processes with multidimensional time parameter},
author={G. Neuhaus},
year={1971},
journal={Annals of Statistics},
volume={42},
pages={1285--1295},
}


@article{vanderVaart&Wellner11,
title={A local maximal inequality under uniform entropy},
author={A.W. van der Vaart and J.A. Wellner},
year={2011},
journal={Electronic Journal of Statistics},
volume={5},
pages={192--203},
note={ISSN: 1935-7524, DOI: 10.1214/11-EJS605},
}


@article{Porteretal11,
title={The relative performance of targeted maximum likelihood estimators},
author={K.E. Porter and S. Gruber and M. J. van der Laan and J. S. Sekhon},
year= {2011},
journal={Int J Biostat.},
volume={Jan 1, 2011; 7(1): Article 31.},
note={Published online Aug 17, 2011. doi:  10.2202/1557-4679.1308. Also available at: U.C. Berkeley Division of Biostatistics Working Paper Series. Working Paper 279, http://www.bepress.com/ucbbiostat/paper279},
}

@incollection{Sekhonetal12,
	Address = {New York Dordrecht Heidelberg London},
	Author = {J.S. Sekhon and S. Gruber and K.E. Porter and M.J. van der Laan},
	Booktitle = {Targeted Learning: Causal Inference for Observational and Experimental Data},
	Date-Added = {2012-08-24 11:01:37 -0700},
	Date-Modified = {2012-08-24 11:02:54 -0700},
	Editor = {van der Laan, M.J. and Rose, S.},
	Keywords = {Chpt3},
	Publisher = {Springer},
	Title = {Propensity score-based estimators and C-TMLE},
	Year = {2012}}


@incollection{Robinsetal08,
year={2008},
isbn={DOI:
10.1214/1939403070000005, arXiv:0805.3040v1},
booktitle={Essays in Honor of David A. Freedman
},
series={IMS, Collections Probability and Statistics},
title={Higher order influence functions and minimax estimation of non-linear functionals},
publisher={Springer New York},
author={J.M. Robins and L. Li and E. Tchetgen and A.W. van der Vaart},
pages={335-421},
language={English}
}

@techreport{vanderLaan15,
  author =        {M.J. van der Laan},
  institution =   {UC Berkeley},
number={300},
  title =         {A generally efficient targeted minimum loss-based estimator },
  year =          {2015},
  note ={http://biostats.bepress.com/ucbbiostat/paper343, 2015}
}

@techreport{vanderLaan12network,
  author =        {M.J. van der Laan},
  institution =   {UC Berkeley},
number={300},
  title =         {Causal Inference for Networks},
  year =          {2012},
  note ={http://biostats.bepress.com/ucbbiostat/paper300,to appear in Journal of Causal Inference}
}

@techreport{vanderLaanetal13,
  author =        {M.J. van der Laan and A.E. Hubbard and S. Kherad},
  institution =   {UC Berkeley},
number={314},
  title =         {Statistical Inference for Data Adaptive Target Parameters},
  year =          {June 2013},
  note ={http://biostats.bepress.com/ucbbiostat/paper314, Revised for Biometrics}
}

@techreport{vanderLaan13,
  author =        {M.J. van der Laan},
  institution =   {UC Berkeley},
number={317},
  title =         {Targeted Learning of an Optimal Dynamic Treatment and Statistical Inference for its Mean Outcome},
  year =          {2013},
  note ={http://biostats.bepress.com/ucbbiostat/paper317, to appear in Journal of Causal Inference}
}



@techreport{Balzer@vanderLaan13,
  author =        {L. Balzer and M.J. van der Laan},
  institution =   {UC Berkeley},
number={310},
  title =         {Estimating effects on rare outcomes: Knowledge is Power},
  year =          {2013},
  note ={Revised for Biometrics}
}


@article{Schnitzeretal13,
title = {Targeted minimum loss based estimator that outperforms a given estimator},
author = {M. Schnitzer,   E. Moodie, M.J. van der Laan, R. Platt, M. Klei3},
year = {2013},
journal = {to appear in Biometrics
},
volume = {},
number = {},
pages = {http://biostats.bepress.com/ucbbiostat/paper304},
}

@article{Rotnitzkyetal12,
title = {Improved double-robust estimation in missing data and causal inference models},
author = {A. Rotnitzky and Q. Lei and M. Sued and J. M. Robins},
year = {2012},
journal = {Biometrika},
volume = {99},
number = {2},
pages = {439--456, doi:  10.1093/biomet/ass013},
}

@article{Gruber&vanderLaan12,
title = {Targeted minimum loss based estimator that outperforms a given estimator},
author = {S. Gruber and M.J. van der Laan},
year = {2012},
journal = {The International Journal of Biostatistics},
volume = {8},
number = {1},
pages = {Article 11, doi: 10.1515/1557-4679.1332},
}

@techreport{Sapp&vanderLaan13,
  author =        {S. Sapp and M.J. van der Laan and K. Page},
  institution =   {UC Berkeley},
number={307},
  title =         {Targeted Estimation of Variable Importance Measures with Interval-Censored Outcomes},
  year =          {2013},
  note ={Submitted to IJB}
}


@techreport{Neugebaueretal13,
  author =        {R. Neugebauer and J.A. Schmittdiel and M.J. van der Laan},
  institution =   {The Agency for Healthcare Research and Quality},
number={No. HHSA29020050016I},
  title =         {Targeted Learning in real-world comparative effectiveness research with time-varying interventions},
  year =          {2013},
  note ={http://diabetestranslation.org/en/news_publications/Reports}
}


@article{Diaz11,
title = {Super Learner Based Conditional Density Estimation with Application to Marginal Structural Models},
author = {D\'iaz, Iv\'an and van der Laan, Mark},
year = {2011},
journal = {The International Journal of Biostatistics},
volume = {7},
number = {1},
pages = {38},
}

@article {Diaz12,
author = {Iv\'an D\'iaz and van der Laan, Mark},
title = {Population Intervention Causal Effects Based on Stochastic Interventions},
journal = {Biometrics},
volume = {68},
number = {2},
publisher = {Blackwell Publishing Inc},
issn = {1541-0420},
pages = {541--549},
keywords = {Causal effect, Counterfactual outcome, Double robustness, Stochastic intervention, Targeted maximum likelihood estimation},
year = {2012},
}

@article{Diaz13a,
title={Sensitivity Analysis for Causal Inference Under Unmeasured Confounding and Measurement Error Problems},
author={D{\'\i}az, Iv{\'a}n and van der Laan, Mark J},
year= {{2013}, In press},
journal={International Journal of Biostatistics}
}

@article{Diaz13b,
title={Assessing the Causal Effect of Policies: An Example Using Stochastic Interventions},
author={D{\'\i}az, Iv{\'a}n and van der Laan, Mark J},
year= {{2013}, In press},
journal={International Journal of Biostatistics}
}

@incollection{Starmans11,
year={2011},
isbn={978-1-4419-9781-4},
booktitle={Targeted Learning},
series={Springer Series in Statistics},
title={Models, Inference, and Truth},
publisher={Springer New York},
author={R. Starmans},
pages={1-20},
language={English}
}
@incollection{Diaz11a,
year={2011},
isbn={978-1-4419-9781-4},
booktitle={Targeted Learning},
series={Springer Series in Statistics},
title={Targeted Bayesian Learning},
publisher={Springer New York},
author={Iv\'an D\'iaz and Hubbard, Alan E. and van der Laan, Mark J.},
pages={475--493},
language={English}
}



@article{Diaz13c,
title={Targeted Data Adaptive Estimation of the Causal Dose Response Curve},
author={D{\'\i}az, I. and van der Laan, M. J.},
year= {2013},
journal={Journal of Causal Inference},
Volume={1 (2)},
pages={171--192}
}

@article{ndeu,
  title={Identification and efficient estimation of the natural direct effect among the untreated},
  author={Lendle, Samuel D and Subbaraman, Meenakshi S and van der Laan, Mark J},
  journal={Biometrics},
  pages={1--8},
  year={2013},
  publisher={Wiley Online Library}
}

@article{tmle_safety,
  title={Targeted maximum likelihood estimation in safety analysis},
  author={Lendle, Samuel D and Fireman, Bruce and van der Laan, Mark J},
  journal={Journal of clinical epidemiology},
  volume={66},
  number={8},
  pages={S91--S98},
  year={2013},
  publisher={Elsevier}
}

@article{subbaraman2013cravings,
  title={Cravings as a mediator and moderator of drinking outcomes in the COMBINE study},
  author={Subbaraman, Meenakshi Sabina and Lendle, Samuel and Laan, Mark and Kaskutas, Lee Ann and Ahern, Jennifer},
  journal={Addiction},
  year={2013},
  publisher={Wiley Online Library}
}

@article{bsatmle,
  title={Balancing Score Adjusted Targeted Minimum Loss-based Estimation},
  author={Lendle, Samuel D and Fireman, Bruce and van der Laan, Mark J},
  year={2013},
  publisher={bepress}
}
@article{brooks2013,
author = "Jordan Brooks and Mark J {van der Laan} and Daniel E Singer and Alan S Go",
institution = "Division of Biostatistics, University of California",
title = "Targeted Minimum Loss-Based Estimation of Causal Effects in Right-Censored Survival Data with Time-Dependent Covariates: Warfarin, Stroke, and Death in Atrial Fibrillation",
journal = {Journal of Causal Inference},
year = {2013},
volume = {1},
issue	 = {2},
page = {235-254},
doi = {10.1515/jci-2013-0001}
}

@article{brooks2012,
author = "Jordan Brooks and Mark J {van der Laan} and Alan S Go",
institution = "Division of Biostatistics, University of California",
title = "Targeted Maximum Likelihood Estimation for Prediction Calibration",
journal = {International Journal of Biostatistics},
year = "2012"
volume = {8},
issue	 = {1},
article = {30},
doi = {10.1515/1557-4679.1385}
}@techreport{Chambazetal13,
  author =        {A. Chambaz and N. Pierre and M.J. van der Laan},
  institution =   {UC Berkeley},
number={292},
  title =         {Estimation of a Non-Parametric Variable Importance Measure of a Continuous Exposure},
  year =          {2013},
  note ={to appear in Electronic Journal of Applied Statistics}
}




@techreport{Aronow&Samii13,
  author =        {P.M. Aronow and C. Samii},
  institution =   {Yale University and New York University},
number={},
  title =         {Estimating average causal effects under general interference},
  year =          {2013},
  note ={Unpublished manuscript}
}



@book{Carringtonetal05,
  address =       {},
  author =        {P.J. Carrington and J. Scott and S. Wasserman},
  edition =       {},
  publisher =     {Cambridge University Press},
  title =         {Models and Methods in Social Network Analysis (Structural Analysis in the Social Sciences)},
  year =          {2005},
}



@article{Bakshyetal12,
	Author = {E. Bakshy and D. Eckles and R. Yan and I. Rosenn},
	Journal = {EC 2012: Proceedings of the ACM Conference on Electronic Commerce},
	Month = {},
	Volume={ACM. http://arxiv.org/abs/1206.4327},
	Title = {Social influence in social advertising: Evidence from field experiments},
	Year = {2012}
}

@article{Airoldietal13,
	Author = {E. M. Airoldi and P. Toulis and E. Kao and D.B. Rubin},
	Journal = {Proceedings of the 30 th International Conference on Ma-
chine Learning, Atlanta, Georgia, USA, 2013},
	Month = {},
	Volume={JMLR: W\&CP volume 28},
	Title = {Estimation of causal peer influence effects},
	Year = {2013}
}


@article{Gruber&vanderLaan12a,
	Author = {S. Gruber and M.J. van der Laan},
	Journal = {Statistical Methods in Medical Research},
	Month = {February},
	Title = {Consistent causal effect estimation under dual misspecification and implications for confounder selection procedure},
	Year = {2012}
}
@article{vanderLaan&Balzer&Petersen13,
	Author = {M.J. van der Laan and L.B. Balzer and M.L. Petersen},
	Journal = {Journal of Statistical Research},
	Month = {},
	Pages={113-156},
	Volume={46(2)},
	Title = {Adaptive Matching in Randomized Trials and Observational Studies},
	Year = {2013}
}


@incollection{vanderLaan&Petersen12,
	Author = {M.J. van der Laan and M.L. Petersen},
	Booktitle = {Ensemble Machine Learning},
	Chapter = {pages 117--156, ISBN 978-1-4419-9326-7},
	Publisher = {Springer, New York},
	Title = {Targeted Learning},
	Year = {2012}}


@incollection{Zheng&vanderLaan11,
	Author = {W. Zheng and M.J. van der Laan},
	Booktitle = {{\rm M.J. van der Laan and S. Rose, } Targeted Learning:Causal Inference for Observational and Experimental Data},
	Chapter = {21},
	pages={459-474},
	Publisher = {Springer, New York},
	Title = {Cross-validated Targeted Minimum Loss Based Estimation},
	Year = {2011}}

@incollection{Wang&Rose&vanderLaan11,
	Author = {H. Wang and S. Rose and M.J. van der Laan},
	Booktitle = {{\rm M.J. van der Laan and S. Rose, } Targeted Learning:Causal Inference for Observational and Experimental Data},
	Chapter = {23},
	Publisher = {Springer, New York},
	Title = {Finding Quantitative Trait Loci Genes},
	Year = {2011}}

	@incollection{Tuglus&vanderLaan11,
	Author = {C. Tuglus and M.J. van der Laan},
	Booktitle = {{\rm M.J. van der Laan and S. Rose, } Targeted Learning:Causal Inference for Observational and Experimental Data},
	Chapter = {22},
	Publisher = {Springer, New York},
	Title = {Targeted Methods for Biomarker Discoveries},
	Year = {2011}}

@incollection{Polley&Rose&vanderLaan11,
	Author = {E.C. Polley and S. Rose and M.J. van der Laan},
	Booktitle = {{\rm M.J. van der Laan and S. Rose, } Targeted Learning:Causal Inference for Observational and Experimental Data},
	Chapter = {3},
	Publisher = {Springer, New York},
	Title = {Super Learning},
	Year = {2011}}

@book{vanderLaan96b,
  address =       {Amsterdam},
  author =        {M.J. van der Laan},
  edition =       {CWI tract 114},
  publisher =     {Centre of Computer Science and Mathematics},
  title =         {Efficient and Inefficient Estimation in Semiparametric Models},
  year =          {1996},
}
@book{Donner&Klar00,
  address =       {London},
  author =        {A. Donner and N. Klar},
  edition =       {},
  publisher =     {Arnold},
  title =         {Design and Analysis of Cluster Randomization Trials in Health Research},
  year =          {2000},
}

@book{Hayes&Moulton09,
  address =       {Boca Raton},
  author =        {R.J. Hayes and L.H. Moulton},
  edition =       {},
  publisher =     {Chapman \& Hall/CRC},
  title =         {Cluster Randomized Trials},
  year =          {2009},
}
@book{vanderLaan&Rose12,
  address =       {New York},
  author =        {M.J. van der Laan and S. Rose},
  edition =       {},
  publisher =     {Springer},
  title =         {Targeted Learning: Causal Inference for Observational and Experimental Data},
  year =          {2012},
}
@book{Murray98,
  address =       {Oxford},
  author =        {D.M. Murray},
  edition =       {},
  publisher =     {Oxford University Press},
  title =         {Design and Analysis of Community Randomized Trials},
  year =          {1998},
}
 @article{Campbelletal07,
  author =        {M.J. Campbell and A. Donner and N. Klar},
  journal =       {Statistics in Medicine},
  pages =         {2--19, doi: 10.1002/sim.2731},
  title =         {Developments in cluster randomized trials and statistics in medicine},
  volume =        {26},
  year =          {2007},
}
 @article{Klar&Donner97,
  author =        {N. Klar and A. Donner},
  journal =       {Statistics in Medicine},
  pages =         {1753--1764},
  title =         {The merits of matching in community intervention trials: a cautionary tale},
  volume =        {16(15)},
  year =          {1997},
}


 @article{Raudenbush&Martinez&Spybrook07,
  author =        {S.W. Raudenbush and A. Martinez and J. Spybrook},
  journal =       {Educational Evaluation and Policy Analysis},
  pages =         {5--29},
  title =         {Developments in cluster randomized trials and statistics in medicine},
  volume =        {29},
  year =          {2007},
}

@article{Freedman&Green&Byar90,
  author =        {L.S. Freedman and S.B. Green and D.P. Byar},
  journal =       {Statistics in Medicine},
  pages =         {943--952},
  title =         {Assessing the gain in efficiency due to matching in a community intervention study},
  volume =        {9},
  year =          {1990},
}
@article{Gill&vanderLaan&Wellner95,
  author =        {R.D. Gill and M.J. van der Laan and J.A. Wellner},
  journal =       {Annales de l'Institut Henri Poincar{\'e}},
  pages =         {545--597},
  title =         {Inefficient estimators of the bivariate survival function for three models},
  volume =        {31},
  year =          {1995},
}
@article{Freedmanetal97,
  author =        {L. Freedman and M. Gail and S. Green and D. Corle},
  journal =       {Controlled clinical trials},
  pages =         {131--139, doi:10.1016/S0197-2456(96)00115-8},
  title =         {The efficiency of the matched-pairs design of the community intervention trial for smoking cessation (COMMIT)},
  volume =        {18(2)},
  year =          {1997},
}

@article{Toftageretal11,
  author =        {M. Toftager and L.B. Christiansen and P.L. Kristensen and J. Troelsen},
  journal =       {BMC Public Health},
  pages =         {711--777},
  title =         {SPACE for physical activity-a multicomponent intervention study: study design and baseline findings from a cluster randomized controlled trial},
  volume =        {10},
  year =          {2011},
}

@article{Koetheetal10,
  author =        {J.R. Koethe and A.O. Westfall and D.K. Luhanga and G.M. Clark and J.D. Goldman and P.L Mulenga and R.A. Cantrell and B.H. Chi and I. Zulu and M.S. Saag and J. S. Stringer},
  journal =       {PlLoS One},
  pages =         {5(3):e9680},
  title =         {A cluster randomized trial of routine HIV-1 viral load monitoring in Zambia},
  volume =        {5},
  year =          {2010},
}

@article{Watsonetal04,
  author =        {L. Watson and R. Small and S. Brown and W. Dawson and J. Lumley},
  journal =       {Journal of Controlled Clinical Trials},
  pages =         {235--250},
  title =         {Mounting a community-randomized trial: sample size, matching, selection, and randomization issues in PRISM},
  volume =        {3},
  year =          {2004},
}

@article{Gailetal92,
  author =        {M.H. Gail and D.P. Byar and T.F. Pechacek and D.K. Corle},
  journal =       {Controlled clinical trials},
  pages =         {6-21},
  title =         {Aspects of statistical design for the community intervention trial for smoking cessation},
  volume =        {13},
  year =          {1992},
}

@article{Commit91,
  author =        {COMMIT Research Group},
  journal =       {Journal of National Cancer Institute},
  pages =         {1620-1628},
  title =         {Summary of design and intervention},
  volume =        {83(22)},
  year =          {1991},
}

 @article{Imai&King&Nall09,
  author =        {Kosuke Imai and G. King and C. Nall},
  journal =       {Statistical Science},
  pages =         {29--53},
  title =         {The essential role of pair matching in cluster randomized experiments with applicationto the Mexican Universal Health Insurance Evaluation},
  volume =        {24 (1)},
  year =          {2009},
}


@article{Imai08,
  author =        {K. Imai},
  journal =       {Statistics in Medicine},
  pages =         {4857--4873},
  title =         {Variance identification and efficiency analysis in randomized experiments under the matched-pair design},
  volume =        {27(24)},
  year =          {2008},
}



@techreport{vanderLaan&Gruber11,
  author =        {M.J. van der Laan and S. Gruber},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
number={290},
  title =         {Targeted Minimum Loss Based Estimation of an Intervention Specific Mean Outcome},
  year =          {2011},
  note ={To appear  in IJB, also technical report http://www.bepress.com/ucbbiostat/paper290 }
}

@techreport{vanderLaan08,
  author =        {M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
number={232},
  title =         {The construction and analysis of adaptive group sequential designs},
  year =          {2008},
  note ={http://www.bepress.com/ucbbiostat/paper234 }
}


@techreport{Balzer&Petersen&vanderLaan12,
  author =        {L.B. Balzer and M.L. Petersen and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
number={294},
  title =         {Why match in individually and cluster randomized trials},
  year =          {2012},
  note ={To appear  in Statistics in Medicine, also technical report http://www.bepress.com/ucbbiostat/paper294}
}



@incollection{Marschak53,
  address =       {New York},
  author =        {J. Marschak},
  booktitle =     {Economic measurements for policy and prediction},
  editor =        {W.~C. Hood and T.~C. Koopmans},
  publisher =     {Wiley},
  title =         {Studies in econometric method},
  year =          {1953},
}

@article{Heckman00,
  author =        {J. Heckman},
  journal =       {Q J Econ},
  pages =         {45--97},
  title =         {Causal parameters and policy analysis in economics:
                   A twentieth century retrospective.},
  volume =        {115},
  year =          {2000},
}

@article{Gruber&vanderLaan10,
  author =        {S. Gruber and M.J. van der Laan},
  journal =       {International Journal of Biostatistics},
  pages =         {article 26, www.bepress.com/ijb/vol6/iss1/26},
  title =         {A Targeted Maximum Likelihood Estimator of a Causal Effect on a Bounded Continuous Outcome},
  volume =        {6},
  year =          {2010},
}




@article{Heckman10,
  author =        {J. Heckman},
  journal =       {J Econ Lit},
  pages =         {356--398},
  title =         {Building bridges between structural and program
                   evaluation approaches to evaluating policy.},
  volume =        {48},
  year =          {2010},
}

@article{Bang&Robins05,
author={H. Bang and J.M. Robins},
 journal =       {Biometrics},
  pages =         {962--972},
  title =         {Doubly robust estimation in missing data and causal inference models},
  volume =        {61},
  year =          {2005},
}



@book{Pearson11,
  address =       {London},
  author =        {K. Pearson},
  edition =       {3rd},
  publisher =     {Black},
  title =         {Grammar of science},
  year =          {1911},
}

@article{Rubin74,
  author =        {Donald B. Rubin},
  journal =       {J Educ Psychol},
  number =        {},
  pages =         {688--701},
  title =         {Estimating causal effects of treatments in randomized
                   and nonrandomized studies.},
  volume =        {66},
  year =          {1974},
}

@article{Neyman23,
  author =        {J. Neyman},
  journal =       {Stat Sci},
  number =        {},
  pages =         {465--480},
  title =         {Sur les applications de la theorie des probabilites
                   aux experiences agricoles: Essai des principes ({In
                   Polish}). {E}nglish translation by {D.M.} {D}abrowska and
                   {T.P.} {S}peed (1990)},
  volume =        {5},
  year =          {1923},
}

@book{Pearl09,
  address =       {New York},
  author =        {J. Pearl},
  edition =       {2nd},
  publisher =     {Cambridge},
  title =         {Causality: models, reasoning, and inference},
  year =          {2009},
}

@article{Pearl95,
  author =        {J. Pearl},
  journal =       {Biometrika},
  pages =         {669--710},
  title =         {Causal diagrams for empirical research.},
  volume =        {82},
  year =          {1995},
}

@article{Robins&Greenland92,
  author =        {J.M. Robins and S. Greenland},
  journal =       {Epidemiol},
  pages =         {143--155},
  title =         {Identifiability and exchangeability for direct and
                   indirect effects},
  volume =        {3},
  year =          {1992},
}

@inproceedings{Pearl01b,
  address =       {San Francisco},
  author =        {J. Pearl},
  booktitle =     {Uncertainty in artificial intelligence, Proceedings
                   of the 17th Conference},
  publisher =     {Morgan Kaufmann},
  title =         {Direct and indirect effects.},
  year =          {2001},
}

@article{Baron&Kenny86,
  author =        {R. Baron and D. Kenny},
  journal =       {J Personal Soc Psychol},
  pages =         {1173--1182},
  title =         {The moderator-mediator variable distinction in social
                   psychological research: conceptual, strategic, and
                   statistical considerations.},
  volume =        {51},
  year =          {1986},
}

@book{MacKinnon08,
  address =       {New York},
  author =        {D. {MacKinnon}},
  publisher =     {Erlbaum},
  title =         {Introduction to statistical mediation analysis},
  year =          {2008},
}

@article{MacKinnonetal07,
  author =        {D. {MacKinnon} and C. Lockwood and C. Brown and
                   W. Wang and J. Hoffman},
  journal =       {Clin Trials},
  pages =         {499--513},
  title =         {The intermediate endpoint effect in logistic and
                   probit regression.},
  volume =        {4},
  year =          {2007},
}

@incollection{Pearl10c,
  address =       {},
  author =        {J. Pearl},
  booktitle =     {Statistical causality},
  editor =        {C. Berzuini and P. Dawid and L. Bernardinelli},
  publisher =     {},
  title =         {The mediation formula: a guide to the assessment of
                   causal pathways in nonlinear models.},
  year =          {forthcoming 2011},
}

@article{Pearl10b,
  author =        {J. Pearl},
  journal =       {Int J Biostat},
  pages =         {Article 7},
  title =         {An introduction to causal inference},
  volume =        {6},
  number={2},
  year =          {2010},
}

@article{vanderLaan&Rose10,
  author =        {M.J. van der Laan and S. Rose},
  journal =       {Amstat News},
  pages =         {38--39},
  title =         {Statistics Ready for a Revolution: next Generation of
                   Statisticians Must Build Tools for Massive Data Sets},
  volume =        {399},
  year =          {2010},
}

@techreport{vanderLaan&Dudoit03,
  author =        {M.J. van der Laan and S. Dudoit},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
number={130},
  title =         {Unified cross-validation methodology for selection
                   among estimators and a general cross-validated
                   adaptive epsilon-net estimator: finite sample oracle
                   inequalities and examples},
  year =          {2003},
}




@book{vanderLaan&Robins03,
  author =        {M.J. van der Laan and J.M. Robins},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  title =         {Unified methods for censored longitudinal data and
                   causality},
  year =          {2003},
}

@book{vanderLaan&Rose11,
  author =        {M.J. van der Laan and S. Rose},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  title =         {Targeted Learning: Causal Inference for Observational and Experimental Data},
  year =          {2011},
}
@book{Bickeletal97,
  author =        {P.J. Bickel and C.A.J. Klaassen and Y. Ritov and
                   J. Wellner},
  publisher =     {Springer},
  address={Berlin Heidelberg New York},
  title =         {Efficient and adaptive estimation for semiparametric
                   models},
  year =          {1997},
}

@article{vanderLaan&Rubin06,
  author =        {M.J. van der Laan and Daniel B. Rubin},
  journal =       {Int J Biostat},
  number =        {1},
  pages =         {Article 11},
  title =         {Targeted Maximum Likelihood Learning},
  volume =        {2},
  year =          {2006},
}

@article{Stitelman&vanderLaan11a,
  author =        {O.M. Stitelman and M.J. van der Laan},
  journal =       {Int J Biostat},
  number =        {1},
  title =         {Targeted Maximum Likelihood Estimation of Effect Modification Parameters In Survival Analysis},
  volume =        {7},
  year =          {2011},
}






@article{vanderLaan&Gruber10,
  author =        {M.J. van der Laan and S. Gruber},
  journal =       {Int J Biostat},
  number =        {1},
  title =         {Collaborative Double robust penalized targeted
                   maximum likelihood estimation},
  volume =        {6},
  year =          {2010},
}

@article{Taubes07,
  author =        {G. Taubes},
  journal =       {The New York Times},
  title =         {{Do we really know what makes us healthy?}},
  year =          {2007},
}

@article{USPrev09,
  author =        {{U.S. Preventive Services Task Force}},
  journal =       {Ann Intern Med},
  number =        {10},
  pages =         {716--726},
  title =         {{Screening for breast cancer: U.S. Preventive
                   Services Task Force recommendation statement}},
  volume =        {151},
  year =          {2009},
}

@article{Freedman&Petitti&Robins04,
  author =        {D.A. Freedman and D.B. Petitti and J.M. Robins},
  journal =       {Int J Epidemiol},
  pages =         {43--55},
  title =         {{On the efficacy of screening for breast cancer}},
  volume =        {33},
  year =          {2004},
}

@book{Rothman&Greenland98,
  address =       {Philadelphia},
  author =        {K.J. Rothman and S. Greenland},
  edition =       {2nd},
  publisher =     {Lippincott, Williams \& Wilkins},
  title =         {Modern epidemiology},
  year =          {1998},
}

@book{Jewell04,
  address =       {Boca Raton},
  author =        {N.P. Jewell},
  publisher =     {Chapman \& Hall},
  title =         {Statistics for epidemiology},
  year =          {2004},
}

@book{Freedman05,
  address =       {New York},
  author =        {D.A. Freedman},
  publisher =     {Cambridge},
  title =         {Statistical models: theory and practice},
  year =          {2005},
}

@article{Ioannidis06,
  author =        {J.P.A. Ioannidis},
  journal =       {Neonatal Intensive Care J Perinatol Neonatol},
  number =        {3},
  title =         {{Why most published research findings are false}},
  volume =        {19},
  year =          {2006},
}

@book{Freedman10,
  address =       {New York},
  author =        {D.H. Freedman},
  publisher =     {Little, Brown and Company},
  title =         {Wrong: why experts keep failing us---and how to know
                   when not to trust them},
  year =          {2010},
}

@book{Box&Draper87,
  address =       {Hoboken},
  author =        {G.E.P. Box and N.R. Draper},
  publisher =     {Wiley},
  title =         {Empirical model-building and response surfaces},
  year =          {1987},
}

@article{Robins86,
  author =        {J.M. Robins},
  journal =       {Math Mod},
  number =        {},
  pages =         {1393--1512},
  title =         {A new approach to causal inference in mortality
                   studies with sustained exposure periods--application
                   to control of the healthy worker survivor effect},
  volume =        {7},
  year =          {1986},
}

@article{Tager&Hollenberg&Satariano98,
  author =        {I. Tager and M. Hollenberg and W. Satariano},
  journal =       {Am J Epidemiol},
  pages =         {921--931},
  title =         {{Self-reported leisure-time physical activity and
                   measures of cardiorespiratory fitness in an elderly
                   population}},
  volume =        {147},
  year =          {1998},
}

@manual{RCore,
  address =       {Vienna},
  author =        {{R Development Core Team}},
  organization =  {R Foundation for Statistical Computing},
  title =         {R: a language and environment for statistical
                   computing},
  year =          {2010},
  url =           {http://www.R-project.org},
}

@article{liaw:2002,
  author =        {A. Liaw and M. Wiener},
  journal =       {R News},
  number =        {3},
  pages =         {18--22},
  title =         {Classification and Regression by randomForest},
  volume =        {2},
  year =          {2002},
  url =           {http://CRAN.R-project.org/package=randomForest},
}

@article{randomForests,
  author =        {L. Breiman},
  journal =       {Mach Learn},
  pages =         {5--32},
  title =         {Random Forests},
  volume =        {45},
  year =          {2001},
}

@manual{ipred,
  author =        {A. Peters and T. Hothorn},
  note =          {R package version 0.8-8},
  title =         {ipred: Improved Predictors},
  year =          {2009},
  url =           {http://CRAN.R-project.org/package=ipred},
}

@article{breiman96bagging,
  author =        {L. Breiman},
  journal =       {Mach Learn},
  number =        {2},
  pages =         {123--140},
  title =         {Bagging Predictors},
  volume =        {24},
  year =          {1996},
}

@incollection{gam:1992,
  author =        {T.J. Hastie},
  booktitle =     {Statistical models in {S}},
  editor =        {J.M. Chambers and T.J. Hastie},
  publisher =     {Chapman \& Hall},
  title =         {Generalized additive models},
      address =       {Boca Raton},
  year =          {1992},
}

@book{gams,
  author =        {T.J. Hastie and R.J. Tibshirani},
  publisher =     {Chapman \& Hall},
  title =         {Generalized additive models},
  year =          {1990},
    address =       {Boca Raton},
}

@manual{gbm,
  author =        {G. Ridgeway},
  note =          {R package version 1.6-3},
  title =         {gbm: generalized boosted regression models},
  year =          {2007},
}

@article{friedman:2001,
  author =        {J.H. Friedman},
  journal =       {Ann Stat},
  pages =         {1189-1232},
  title =         {Greedy Function Approximation: a Gradient Boosting
                   Machine},
  volume =        {29},
  year =          {2001},
}

@book{MASS,
  address={Berlin Heidelberg New York},
  author =        {W.N. Venables and B.D. Ripley},
  edition =       {4th},
  publisher =     {Springer},
  title =         {Modern applied statistics with S},
  year =          {2002},
}

@manual{polspline,
  author =        {C. Kooperberg},
  note =          {R package version 1.1.4},
  title =         {polspline: Polynomial spline routines},
  year =          {2009},
  url =           {http://CRAN.R-project.org/package=polspline},
}

@article{MARS,
  author =        {J.H. Friedman},
  journal =       {Ann Stat},
  number =        {1},
  pages =         {1--141},
  title =         {Multivariate Adaptive Regression Splines},
  volume =        {19},
  year =          {1991},
}

@manual{bart,
  author =        {H.A. Chipman and R.E. McCulloch},
  note =          {R package version 0.3-1},
  title =         {BayesTree: {B}ayesian methods for tree-based models},
  year =          {2009},
  url =           {http://CRAN.R-project.org/package=BayesTree},
}

@article{chipman:2009,
  author =        {H.A. Chipman and E.I. George and R.E. McCulloch},
  journal =       {Ann Appl Stat},
  title =         {{BART}: {B}ayesian Additive Regression Trees},
  volume =        {4},
  number={1},
  pages={266--298},
  year =          {2010},
}

@incollection{loess,
  author =        {W.S. Cleveland and E. Groose and W.M. Shyu},
  booktitle =     {Statistical models in {S}},
  editor =        {J.M. Chambers and T.J. Hastie},
  publisher =     {Chapman \& Hall},
  title =         {Local Regression Models},
  year =          {1992},
      address =       {Boca Raton},
}

@techreport{Polley&vanderLaan10,
  author =        {E.C. Polley and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =        {266},
  title =         {Super Learner in Prediction},
  year =          {2010},
}

@book{cook:1994,
  address =       {New York},
  author =        {D. Cook and S. Weisberg},
  publisher =     {Wiley},
  title =         {An introduction to regression graphics},
  year =          {1994},
}

@article{chu:2001,
  author =        {S. Chu},
  journal =       {J Stat Educ},
  number =        {2},
  title =         {Pricing the {C}'s of diamond stones},
  volume =        {9},
  year =          {2001},
}

@book{berndt:1991,
  address =       {New York},
  author =        {E.R. Berndt},
  publisher =     {Addison--Wesley},
  title =         {The practice of econometrics},
  year =          {1991},
}

@article{kibler:1989,
  author =        {D. Kibler and D.W. Aha and M.K. Albert},
  journal =       {Comput Intell},
  pages =         {51},
  title =         {Instance-Based Prediction of Real-Valued Attributes},
  volume =        {5},
  year =          {1989},
}

@book{rosner:1999,
  address =       {Pacific Grove},
  author =        {B. Rosner},
  edition =       {5th},
  publisher =     {Duxbury},
  title =         {Fundamentals of biostatistics},
  year =          {1999},
}

@misc{newman:1998,
  author =        {D.J. Newman and S. Hettich and C.L. Blake and
                   C.J. Merz},
  institution =   {Department of
                   Information and Computer Sciences, University of California, Irvine},
  title =         {{UCI Repository of Machine Learning Databases}},
  year =          {1998},
}

@book{afifi:1979,
  address =       {New York},
  author =        {A. Afifi and S. Azen},
  edition =       {2nd},
  publisher =     {Academic},
  title =         {Statistical analysis: a computer oriented approach},
  year =          {1979},
}

@book{cook:1998,
  address =       {New York},
  author =        {D. Cook},
  publisher =     {Wiley},
  title =         {Regression graphics: ideas for studying regression
                   through graphics},
  year =          {1998},
}

@article{liu:1999,
  author =        {Z. Liu and T. Stengos},
  journal =       {J of Appl Econom},
  pages =         {527--538},
  title =         {Nonlinearities in Cross Country Growth Regressions:
                   a Semiparametric Approach},
  volume =        {14},
  year =          {1999},
}

@article{penrose:1985,
  author =        {K. Penrose and A. Nelson and A. Fisher},
  journal =       {Med Sci Sport Exer},
  pages =         {189},
  title =         {Generalized Body Composition Prediction Equation for
                   Men Using Simple Measurement Techniques},
  volume =        {17},
  year =          {1985},
}

@book{harrell:2001,
  address={Berlin Heidelberg New York},
  author =        {Harrell, Jr., F.E.},
  publisher =     {Springer},
  title =         {Regression modeling strategies with applications to
                   linear models, logistic regression, and survival
                   analysis},
  year =          {2001},
}

@manual{arm,
  author =        {A. Gelman and Y.-S. Su and M. Yajima and J. Hill and
                   M.G. Pittau and J. Kerman and T. Zheng},
  note =          {R package version 1.3-02},
  title =         {arm: data analysis using regression and
                   multilevel/hierarchical models},
  year =          {2010},
  url =           {http://CRAN.R-project.org/package=arm},
}

@article{gelman:2009,
  author =        {A. Gelman and A. Jakulin and M.G. Pittau and
                   Y.-S. Su},
  journal =       {Ann Appl Stat},
  number =        {3},
  pages =         {1360--1383},
  title =         {A Weakly Informative Default Prior Distribution for
                   Logistic and Other Regression Models},
  volume =        {2},
  year =          {2009},
}

@article{friedman:2010,
  author =        {J.H. Friedman and T.J. Hastie and R.J. Tibshirani},
  journal =       {J Stat Softw},
  number =        {1},
  title =         {Regularization Paths for Generalized Linear Models
                   via Coordinate Descent},
  volume =        {33},
  year =          {2010},
}

@manual{glmnet,
  author =        {J.H. Friedman and T.J. Hastie and R.J. Tibshirani},
  note =          {R package version 1.1-5},
  title =         {glmnet: lasso and elastic-net regularized generalized
                   linear models},
  year =          {2010},
  url =           {http://CRAN.R-project.org/package=glmnet},
}

@manual{DSA,
  author =        {R. Neugebauer and J. Bullard},
  note =          {R package version 3.1.3},
  title =         {DSA: Data-adaptive estimation with cross-validation
                   and the D/S/A algorithm},
  year =          {2009},
  url =           {http://www.stat.berkeley.edu/~laan/Software/},
}

@article{SinisivanderLaan04,
  author =        {S.E. Sinisi and M.J. van der Laan},
  journal =       {Stat Appl Genet Mol},
  note =          {Article 18},
  number =        {1},
  title =         {{D}eletion/{S}ubstitution/{A}ddition algorithm in
                   learning with applications in genomics},
  volume =        {3},
  year =          {2004},
}

@manual{svm,
  author =        {E. Dimitriadou and K. Hornik and F. Leisch and
                   D. Meyer and A. Weingessel},
  note =          {R package version 1.5-22},
  title =         {e1071: misc functions of the Department of Statistics
                   (e1071)},
  year =          {2009},
  url =           {http://CRAN.R-project.org/package=e1071},
}

@manual{Chang:2001,
  author =        {C.-C. Chang and C.-J. Lin},
  url =           {http://www.csie.ntu.edu.tw/~cjlin/libsvm},
  title =         {{LIBSVM}: a library for support vector machines},
  year =          {2001},
}

@article{vantveer:2002,
  author =        {L.J. {van't Veer} and H. Dal and M.J. {van de Vijver} and
                   Y.D. He and A.A.M. Hart and M. Mao and H.L. Peterse and
                   K. van der Kooy and M.J. Marton and A.T. Witteveen and
                   G.J. Schreiber and R.M. Kerkhoven and C. Roberts and
                   P.S. Linsley and R. Bernards and S.H. Friend},
  journal =       {Nature},
  pages =         {530--536},
  title =         {Gene Expression Profiling Predicts Clinical Outcome
                   of Breast Cancer},
  volume =        {415},
  year =          {2002},
}

@article{vanderLaan&Polley&Hubbard07,
  author =        {M.J. van der Laan and E.C. Polley and A.E. Hubbard},
  journal =       {Stat Appl Genet Mol},
  pages =        {Article 25},
  title =         {Super Learner},
  volume =        {6},
  year =          {2007},
  number =          {1},
}

@article{Wolpert92,
  author =        {D. H. Wolpert},
  journal =       {Neural Networks},
  pages =         {241--259},
  title =         {Stacked Generalization},
  volume =        {5},
  year =          {1992},
}

@article{Breiman96d,
  author =        {L. Breiman},
  journal =       {Mach Learn},
  pages =         {49--64},
  title =         {Stacked Regressions},
  volume =        {24},
  year =          {1996},
}

@article{Leblanc96,
  author =        {M. LeBlanc and R.J. Tibshirani},
  journal =       {J Am Stat Assoc},
  pages =         {1641--1650},
  title =         {Combining estimates in regression and classification},
  volume =        {91},
  year =          {1996},
}

@article{Stone74,
  author =        {M. Stone},
  journal =       {J R Stat Soc Ser B},
  number =        {2},
  pages =         {111--147},
  title =         {Cross-validatory choice and assessment of statistical
                   predictions},
  volume =        {36},
  year =          {1974},
}

@article{Geisser75,
  author =        {S. Geisser},
  journal =       {J Am Stat Assoc},
  number =        {350},
  pages =         {320--328},
  title =         {The Predictive Sample Reuse Method with Applications},
  volume =        {70},
  year =          {1975},
}

@inproceedings{Tsybakov03,
  author =        {A.B. Tsybakov},
  booktitle =     {COLT},
  editor =        {B. Sch{\"o}lkopf and M.K. Warmuth},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  series =        {Lecture Notes in Computer Science},
  title =         {Optimal rates of aggregation},
  volume =        {2777},
  year =          {2003},
}

@inproceedings{Juditskyetal05,
  author =        {A. Juditsky and A.V. Nazin and A.B. Tsybakov and
                   N. Vayatis},
  booktitle =     {NIPS},
  title =         {Generalization Error Bounds for Aggregation by Mirror
                   Descent with Averaging},
  year =          {2005},
}

@inproceedings{Buneaetal06,
  author =        {F. Bunea and A.B. Tsybakov and M.H. Wegkamp},
  booktitle =     {COLT},
  editor =        {G. Lugosi and H.-U. Simon},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  series =        {Lecture Notes in Computer Science},
  title =         {Aggregation and sparsity via {L}1 penalized least
                   squares},
  volume =        {4005},
  year =          {2006},
}

@article{Buneaetal07,
  author =        {F. Bunea and A.B. Tsybakov and M.H. Wegkamp},
  journal =       {Ann Stat},
  number =        {4},
  pages =         {1674--1697},
  title =         {Aggregation for Gaussian Regression},
  volume =        {35},
  year =          {2007},
}

@inproceedings{Buneaetal07b,
  author =        {F. Bunea and A.B. Tsybakov and M.H. Wegkamp},
  booktitle =     {COLT},
  editor =        {N.H. Bshouty and C. Gentile},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  series =        {Lecture Notes in Computer Science},
  title =         {Sparse density estimation with {L}1 penalties},
  volume =        {4539},
  year =          {2007},
}

@inproceedings{Dalalyan&Tsybakov07,
  author =        {A.S. Dalalyan and A.B. Tsybakov},
  booktitle =     {COLT},
  editor =        {N.H. Bshouty and C. Gentile},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  series =        {Lecture Notes in Computer Science},
  title =         {Aggregation by exponential weighting and sharp oracle
                   inequalities},
  volume =        {4539},
  year =          {2007},
}

@article{Dalalyan&Tsybakov08,
  author =        {A.S. Dalalyan and A.B. Tsybakov},
  journal =       {Mach Learn},
  number =        {1--2},
  pages =         {39--61},
  title =         {Aggregation by exponential weighting, sharp
                   PAC-{B}ayesian bounds and sparsity},
  volume =        {72},
  year =          {2008},
}

@book{Lehmann86,
  author =        {E.L. Lehmann},
  edition =       {2nd},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  title =         {Testing statistical hypotheses},
  year =          {1986},
}

@book{Hastie&Tibshirani&Friedman01,
  author =        {T.J. Hastie and R.J. Tibshirani and J.H. Friedman},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  title =         {The elements of statistical learning: data mining,
                   inference, and prediction},
  year =          {2001},
}

@ inproceedings{Ruczinski&Kooperberg&LeBlanc02,
  author =        {I. Ruczinski and C. Kooperberg and M. LeBlanc},
  booktitle =       {Proceedings of the MSRI workshop on Nonlinear
                   Estimation and Classification},
  editor={D. Denison and M.
                   Hansen and C. Holmes and B. Mallick and B. Yu},
  pages =         {333--344},
  title =         {Logic Regression -- methods and software},
  year =          {2002},
}



@techreport{Birkner&Hubbard&vanderLaan05,
  author =        {M.D. Birkner and A.E. Hubbard and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =        {197},
  title =         {Data Adaptive Pathway Testing},
  year =          {2005},
}

@techreport{Chaffee&Hubbard&vanderLaan10,
  author =        {P. Chaffee and A.E. Hubbard and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =        {263},
  title =         {Permutation-based Pathway Testing using the Super
                   Learner Algorithm},
  year =          {2010},
}
@incollection{Polleyetal12,
	Address = {New York Dordrecht Heidelberg London},
	Author = {E.C. Polley and Sherri Rose and M.J. van der Laan},
	Booktitle = {Targeted Learning: Causal Inference for Observational and Experimental Data},
	Date-Added = {2012-08-24 11:01:37 -0700},
	Date-Modified = {2012-08-24 11:02:54 -0700},
	Editor = {van der Laan, M.J. and Rose, S.},
	Keywords = {Chpt3},
	Publisher = {Springer},
	Title = {Super Learning},
	Year = {2012}}

	@inproceedings{Polley&vanderLaan09,
  author =        {E.C. Polley and M.J. van der Laan},
  booktitle =     {Design, summarization, analysis \& interpretation
                   of clinical trials with time-to-event endpoints},
  editor =        {K.E. Peace},
  publisher =     {Chapman \& Hall},
  title =         {Predicting Optimal Treatment Assignment Based on
                   Prognostic Factors in Cancer Patients},
address =       {Boca Raton},
  year =          {2009},
}

@article{vanderLaan&Dudoit&vanderVaart06,
  author =        {M.J. van der Laan and S. Dudoit and
                   A.W. van der Vaart},
  journal =       {Stat Decis},
  number =        {3},
  pages =         {373--395},
  title =         {The Cross-Validated Adaptive Epsilon-Net Estimator},
  volume =        {24},
  year =          {2006},
}

@article{vanderVaart&Dudoit&vanderLaan06,
  author =        {A.W. van der Vaart and S. Dudoit and
                   M.J. van der Laan},
  journal =       {Stat Decis},
  number =        {3},
  pages =         {351--371},
  title =         {Oracle Inequalities for Multi-Fold Cross-Validation},
  volume =        {24},
  year =          {2006},
}

@article{vanderLaan&Dudoit&Keles04,
  author =        {M.J. van der Laan and S. Dudoit and S. Kele\c{s}},
  journal =       {Stat Appl Genet Mol},
  pages =         {Article 4},
  title =         {Asymptotic optimality of likelihood-based
                   cross-validation},
  volume =        {3},
  number={1},
  year =          {2004},
}

@article{Dudoit&vanderLaan05,
  author =        {S. Dudoit and M.J. van der Laan},
  journal =       {Stat Methodol},
  number =        {2},
  pages =         {131--154},
  title =         {Asymptotics of cross-validated risk estimation in
                   estimator selection and performance assessment},
  volume =        {2},
  year =          {2005},
}

@techreport{Keles&vanderLaan&Dudoit02,
  author =        {Kele\c{s}, S. and van der Laan, M.J. and Dudoit, S.},
  institution =       {Division of Biostatistics, University of California,
                   Berkeley},
number={124},
  title =         {Asymptotically Optimal Model Selection Method for
                   Regression on Censored Outcomes},
  year =          {2002},
}

@book{Gyorfietal02,
  address={Berlin Heidelberg New York},
  author =        {L. Gy\"{o}rfi and M. Kohler and A. Krzy\.{z}ak and
                   H. Walk},
  pages =         {100--102},
  publisher =     {Springer},
  title =         {A distribution-free theory of nonparametric
                   regression},
  year =          {2002},
}

@article{Stone77,
  author =        {M. Stone},
  journal =       {Biometrika},
  number =        {1},
  pages =         {29--35},
  title =         {Asymptotics for and against cross-validation},
  volume =        {64},
  year =          {1977},
}

@book{Breimanetal84,
  author =        {L. Breiman and J.H. Friedman and R. Olshen and
                   C.J. Stone},
  publisher =     {Chapman \& Hall},
  title =         {Classification and regression trees},
  year =          {1984},
    address =       {Boca Raton},
}

@article{Breiman&Spector92,
  author =        {L. Breiman and P. Spector},
  journal =       {Int Stat Rev},
  pages =         {291--319},
  title =         {Submodel Selection and Evaluation in Regression. {T}he
                   {$X$} Random Case},
  volume =        {60},
  year =          {1992},
}

@book{Efron&Tibshirani93,
  author =        {B. Efron and R. J. Tibshirani},
  publisher =     {Chapman \& Hall},
  title =         {An Introduction to the bootstrap},
  year =          {1993},
      address =       {Boca Raton},
}

@article{Breiman96,
  author =        {L. Breiman},
  journal =       {Ann Stat},
  number =        {6},
  pages =         {2350--2383},
  title =         {Heuristics of instability and stabilization in model
                   selection},
  volume =        {24},
  year =          {1996},
}

@techreport{Breiman96c,
  author =        {L. Breiman},
  institution =   {Department of Statistics, University of California, Berkeley},
  type={Technical {R}eport},
  title =         {Out-of-bag estimation},
  year =          {1996},
}

@book{Ripley96,
  address =       {New York},
  author =        {B.D. Ripley},
  publisher =     {Cambridge},
  title =         {Pattern recognition and neural networks},
  year =          {1996},
}

@article{Breiman98,
  author =        {L. Breiman},
  journal =       {Ann Stat},
  pages =         {801--824},
  title =         {Arcing classifiers},
  volume =        {26},
  year =          {1998},
}

@article{Ambroise&McLachlan02,
  author =        {C. Ambroise and G.J. McLachlan},
  journal =       {Proc Natl Acad Sci},
  number =        {10},
  pages =         {6562--6566},
  title =         {Selection bias in gene extraction on the basis of
                   microarray gene-expression data},
  volume =        {99},
  year =          {2002},
}

@article{Pavlic&vanderLaan03,
  author =        {M. Pavlic and M.J. van der Laan},
  journal =       {Comput Stat Data An},
  pages =         {413--428},
  title =         {Fitting of mixtures with unspecified number of
                   components using cross validation distance estimate},
  volume =        {41},
  year =          {2003},
}

@inproceedings{Akaike73,
  author =        {H. Akaike},
  booktitle =     {Second International Symposium on Information Theory},
  editor =        {B.N. Petrov and F. Csaki},
  organization =  {Academiai Kiado},
  address={Budapest},
  title =         {Information theory and an extension of the maximum
                   likelihood principle},
  year =          {1973},
}

@article{Bozdogan00,
  author =        {H. Bozdogan},
  journal =       {J Math Psychol},
  pages =         {62--91},
  title =         {Akaike's information criterion and recent
                   developments in information complexity},
  volume =        {44},
  year =          {2000},
}

@article{Schwartz78,
  author =        {G. Schwartz},
  journal =       {Ann Stat},
  pages =         {461--464},
  title =         {Estimating the Dimension of a Model},
  volume =        {6},
  year =          {1978},
}

@article{Rissanen78,
  author =        {J. Rissanen},
  journal =       {Automatica},
  pages =         {465--471},
  title =         {Modelling by shortest data description},
  volume =        {14},
  year =          {1978},
}

@incollection{Bozdogan93,
  author =        {H. Bozdogan},
    address={Berlin Heidelberg New York},
  booktitle =     {Information and classification},
  editor =        {O. Opitz and B. Lausen and R. Klar},
  publisher =     {Springer},
  title =         {Choosing the number of component clusters in the
                   mixture model using a new informational complexity
                   criterion of the inverse Fisher information matrix},
  year =          {1993},
}

@article{Snowden&Rose&Mortimer11,
  author =        {J.M. Snowden and S. Rose and K.M. Mortimer},
  journal =       {Am J Epidemiol},
  number =        {00},
  pages =         {000--000},
  title =         {Implementation of G-Computation on a Simulated
                   Data set: demonstration of a Causal Inference
                   Technique},
  volume =        {173},
  year =          {2011},
}

@article{Rose&Snowden&Mortimer11,
author={S. Rose and J.M. Snowden and K.M. Mortimer},
title={Rose et al. Respond to ``{G}-Computation and Standardization in Epidemiology''},
journal={Am J Epidemiol},
volume={173},
number={00},
pages={000--000},
year={2011},
}

@incollection{Robins99b,
  author =        {Robins, J.M.},
  booktitle =     {Statistical models in epidemiology: the environment
                   and clinical trials},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  title =         {Marginal structural models versus structural nested
                   models as tools for causal inference},
  year =          {1999},
}

@article{Hernan&Brumback&Robins00,
  author =        {Hernan, M.A. and Brumback, B. and Robins, J.M.},
  journal =       {Epidemiol},
  number =        {5},
  pages =         {561--570},
  title =         {Marginal structural models to estimate the causal
                   effect of zidovudine on the survival of
                   {HIV}-positive men},
  volume =        {11},
  year =          {2000},
}

@article{Robins&Rotnitzky&vanderLaan00,
  author =        {J.M. Robins and A. Rotnitzky and M.J. van der Laan},
  journal =       {J Am Stat Assoc},
  pages =         {431--435},
  title =         {Comment on ``{O}n profile likelihood"},
  volume =        {450},
  year =          {2000},
}

@inproceedings{Robins00,
  author =        {J.M. Robins},
  booktitle =     {Proceedings of the American Statistical Association},
  editor =        {},
  organization =  {},
  pages =         {},
  title =         {Robust estimation in sequentially ignorable missing
                   data and causal inference models},
  year =          {2000},
}

@article{Robins&Rotnitzky01,
  author =        {J.M. Robins and A. Rotnitzky},
  journal =       {Stat Sinica},
  number =        {4},
  pages =         {920--936},
  title =         {Comment on the {B}ickel and {K}won article,
                   ``{I}nference for semiparametric models: some
                   questions and an answer''},
  volume =        {11},
  year =          {2001},
}

@article{Dawid&Didelez10,
  author =        {P. Dawid and V. Didelez},
  journal =       {Statist. Surv.},
  number =        {},
  pages =         {184--231},
  title =         {Identifying the consequences of dynamic treatment strategies: A decision-theoretic overview},
  volume =        {4},
  year =          {2010},
}



@incollection{Robins&Rotnitzky92,
  author =        {J.M. Robins and A. Rotnitzky},
  booktitle =     {AIDS epidemiology},
  editor ={Jewell N., Dietz K., Farewell V.},
  pages={296--231},
  publisher =     {Birkh\"{a}user},
      address={Basel},
  title =         {Recovery of information and adjustment for dependent
                   censoring using surrogate markers},
  year =          {1992},
}

@article{Robins&Hernan&Brumback00,
  author =        {Robins, J.M. and Hernan, M.A. and Brumback, B.},
  journal =       {Epidemiol},
  number =        {5},
  pages =         {550--560},
  title =         {Marginal structural models and causal inference in
                   epidemiology},
  volume =        {11},
  year =          {2000},
}

@article{Mortimeretal05,
  author =        {K.M. Mortimer and R. Neugebauer and M.J. van der Laan and
                   I.B. Tager},
  journal =       {Am J Epidemiol},
  number =        {4},
  pages =         {382--388},
  title =         {An Application of Model-Fitting Procedures for
                   Marginal Structural Models},
  volume =        {162},
  year =          {2005},
}

@article{Cole&Hernan08,
  author =        {S.R. Cole and M.A. Hernan},
  journal =       {Am J Epidemiol},
  pages =         {656--664},
  title =         {Constructing Inverse Probability Weights for Marginal
                   Structural Models},
  volume =        {168},
  year =          {2008},
}

@article{Bembom&vanderLaan07,
  author =        {O. Bembom and M.J. van der Laan},
  journal =       {Electron J Stat},
volume={1},
pages={574--596},
  title =         {A practical illustration of the importance of
                   realistic individualized treatment rules in causal
                   inference},
  year =          {2007},
}

@article{vanderLaan08,
  author =        {M.J. van der Laan},
  journal =       {Int J Biostat},
  volume={4},
  number={1},
pages={Article 17},
  title =         {Estimation based on case-control designs with known
                   prevalance probability},
  year =          {2008},
}

@article{Rose&vanderLaan08,
  author =        {S. Rose and M.J. van der Laan},
  journal =       {Int J Biostat},
  volume={4},
  number={1},
pages={Article 19},
  title =         {Simple optimal weighting of cases and controls in
                   case-control studies},
  year =          {2008},
}

@article{Rose&vanderLaan09,
  author =        {S. Rose and M.J. van der Laan},
  journal =       {Int J Biostat},
    volume={5},
  number={1},
pages={Article 1},
  title =         {Why match? {I}nvestigating matched case-control study
                   designs with causal effect estimation},
  year =          {2009},
}

@inproceedings{Moore&vanderLaan09,
  author =        {K.L. Moore and M.J. van der Laan},
  booktitle =     {Design, summarization, analysis \& interpretation
                   of clinical trials with time-to-event endpoints},
  editor =        {Karl E. Peace},
        address =       {Boca Raton},
  publisher =     {Chapman \& Hall},
  title =         {Application of Time-to-Event Methods in the
                   Assessment of Safety in Clinical Trials},
  year =          {2009},
}

@article{Moore&vanderLaan092,
  author =        {Moore, K.L. and van der Laan, M.J.},
  journal =       {Stat Med},
  number =        {1},
  pages =         {39--64},
  title =         {Covariate Adjustment in Randomized Trials with Binary
                   Outcomes: targeted Maximum Likelihood Estimation},
  volume =        {28},
  year =          {2009},
}

@article{Moore&vanderLaan093,
  author =        {Moore, K.L. and van der Laan, M.J.},
  journal =       {J Biopharm Stat},
  number =        {6},
  pages =         {1099--1131},
  title =         {Increasing Power in Randomized Trials with Right
                   Censored Outcomes Through Covariate Adjustment},
  volume =        {19},
  year =          {2009},
}

@article{Bembometal09b,
  author =        {O. Bembom and M.L. Petersen and S.-Y. Rhee and
                   W.J. Fessel and S.E. Sinisi and R.W. Shafer and
                   M.J. van der Laan},
  journal =       {Stat Med},
  pages =         {152--72},
  title =         {Biomarker discovery using targeted maximum likelihood
                   estimation: application to the treatment of
                   antiretroviral resistant {HIV} infection},
  volume =        {28},
  year =          {2009},
}

@article{Rosenblumetal09,
  author =        {M. Rosenblum and S.G. Deeks and M.J. van der Laan and
                   D.R. Bangsberg},
  journal =       {PLoS ONE},
  title =         {The Risk of Virologic Failure Decreases with Duration
                   of {HIV} Suppression, at Greater than 50\% Adherence to
                   Antiretroviral Therapy},
  volume =        {4(9): e7196.doi:10.1371/journal.pone.0007196},
  year =          {2009},
}

@article{Gruber&vanderLaan10a,
  author =        {S. Gruber and M.J. van der Laan},
  journal =       {Int J Biostat},
  number =        {1},
  title =         {An application of collaborative targeted maximum
                   likelihood estimation in causal inference and
                   genomics},
  volume =        {6},
  year =          {2010},
}

@article{Rosenblum&vanderLaan10,
  author =        {M. Rosenblum and M.J. van der Laan},
  journal =       {Int J Biostat},
    volume={6},
  number={2},
pages={Article 19},
  title =         {Targeted maximum likelihood estimation of the
                   parameter of a marginal structural model},
  year =          {2010},
}

@book{Dudoit&vanderLaan08,
address={Berlin Heidelberg New York},
  author =        {S. Dudoit and M.J. van der Laan},
  publisher =     {Springer},
  title =         {Resampling based multiple testing with applications
                   to genomics},
  year =          {2008},
}

@article{Robins94,
  author =        {J.M. Robins},
  journal =       {Commun Stat},
  number =        {},
  pages =         {2379--2412},
  title =         {Correcting for noncompliance in randomized trials
                   using structural nested mean models},
  volume =        {23},
  year =          {1994},
}

@article{Robins&Rotnitzky&Zhao95,
  author =        {J.M. Robins and A. Rotnitzky and L.P. Zhao},
  journal =       {J Am Stat Assoc},
  pages =         {106--121},
  title =         {Analysis of semiparametric regression models for
                   repeated outcomes in the presence of missing data.},
  volume =        {90},
  year =          {1995},
}

@article{Scharfstein&Rotnitzky&Robins99,
  author =        {D.O. Scharfstein and A. Rotnitzky and J.M. Robins},
  journal =       {J Am Stat Assoc},
  pages =         {1096-1120 (1121-1146)},
  title =         {Adjusting for Nonignorable Drop-out Using
                   Semiparametric Nonresponse Models, (with Discussion
                   and Rejoinder)},
  volume =        {94},
  year =          {1999},
}

@article{Leon&Tsiatis&Davidian03,
  author =        {S. Leon and A.A. Tsiatis and M. Davidian},
  journal =       {Biometrics},
  pages =         {1046--1055},
  title =         {Semiparametric estimation of treatment effect in a
                   pretest-posttest study},
  volume =        {59},
  year =          {2003},
}

@article{Tan06,
  author =        {Z. Tan},
  journal =       {J Am Stat Assoc},
  pages =         {1619-1637},
  title =         {A distributional approach for causal inference using
                   propensity scores},
  volume =        {101},
  year =          {2006},
}

@book{Tsiatis062,
  address={Berlin Heidelberg New York},
  author =        {A.A. Tsiatis},
  publisher =     {Springer},
  title =         {Semiparametric theory and missing data},
  year =          {2006},
}

@article{Zhang&Tsiatis&Davidian08,
  author =        {M. Zhang and A.A. Tsiatis and M. Davidian},
  journal =       {Biometrics},
  number =        {3},
  pages =         {707--715},
  title =         {Improving efficiency of inferences in randomized
                   clinical trials using auxiliary covariates},
  volume =        {64},
  year =          {2008},
}

@article{Rubin&vanderLaan08,
  author =        {Daniel B. Rubin and M.J. van der Laan},
  journal =       {Int J Biostat},
  title =         {Empirical efficiency maximization: improved locally
                   efficient covariate adjustment in randomized
                   experiments and survival analysis},
  volume =        {4},
  number={1},
  pages={Article 5},
  year =          {2008},
}

@article{Freedman08,
  author =        {D.A. Freedman},
  journal =       {Adv Appl Math},
  pages =         {180--193},
  title =         {On regression adjustments to experimental data},
  volume =        {40},
  year =          {2008},
}

@article{Freedman082,
  author =        {D.A. Freedman},
  journal =       {Ann Appl Stat},
  pages =         {176--96},
  title =         {On regression adjustments to experiments with several
                   treatments},
  volume =        {2},
  year =          {2008},
}

@article{Rosenblum&vanderLaan09,
  author =        {M. Rosenblum and M.J. van der Laan},
  journal =       {Biometrics},
  number =        {3},
  pages =         {937--945},
  title =         {Using Regression Models to Analyze Randomized Trials:
                   asymptotically Valid Hypothesis Tests Despite
                   Incorrectly Specified Models},
  volume =        {65},
  year =          {2009},
}

@book{Hampeletal86,
  author =        {Hampel, F.R. and Ronchetti, E.M. and Rousseeuw, P.J. and
                   Stahel, W.A.},
  address =       {New York},
  publisher =     {Wiley},
  title =         {{Robust statistics: the approach based on influence
                   functions}},
  year =          {1986},
}

@book{vanderVaart98,
  author =        {A.W. van der Vaart},
  publisher =     {Cambridge},
  title =         {Asymptotic statistics},
    address =       {New York},
  year =          {1998},
}

@book{vanderVaart&Wellner96,
  author =        {A.W. van der Vaart and J.A. Wellner},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  title =         {Weak convergence and empirical processes},
  year =          {1996},
}

@article{Rosenbaum&Rubin83,
  author =        {P.R. Rosenbaum and Donald B. Rubin},
  journal =       {Biometrika},
  pages =         {41--55},
  title =         {The central role of the propensity score in
                   observational studies for causal effects},
  volume =        {70},
  year =          {1983},
}

@article{Stitelman&vanderLaan10,
  author =        {O.M. Stitelman and M.J. van der Laan},
Journal={Int J Biostat},
volume={6},
number={1},
pages={Article 21},
  title =         {Collaborative Targeted Maximum Likelihood for
                   Time-to-Event Data},
  year =          {2010},
}


@article{Wedderburn74,
  author =        {R.W.M. Wedderburn},
  journal =       {Biometrika},
  pages =         {439--447},
  title =         {Quasi-likelihood functions, generalized linear
                   models, and the Gauss-Newton method},
  volume =        {61},
  number={3},
  year =          {1974},
}

@article{McCullagh83,
  author =        {P. Mc{C}ullagh},
  journal =       {Ann Stat},
  pages =         {59--67},
  title =         {Quasi-likelihood functions},
  volume =        {11},
  year =          {1983},
}

@article{vanderLaan&Petersen08,
  author =        {M.J. van der Laan and M.L. Petersen},
  journal =       {Int J Biostat},
  number =        {1},
  title =         {Direct effect models},
  volume =        {4},
  pages={Article 23},
  year =          {2008},
}

@techreport{vanderLaan10c,
  author =        {M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =        {268},
  title =         {Estimation of Causal Effects of Community-Based
                   Interventions},
  year =          {2010},
}

@article{Heckman&Ichimura&Todd97,
  author =        {J. Heckman and H. Ichimura and R. Todd},
  journal =       {Rev of Econ Stud},
  pages =         {605--654},
  title =         {Matching as an Econometric Evaluation Estimator:
                   evidence from Evaluating a Job Training Programme},
  volume =        {64},
  year =          {1997},
}

@techreport{Sekhon06,
  author =        {J.S. Sekhon},
  institution =   {University of California,
                   Berkeley},
  type={Technical {R}eport},
  title =         {Alternative balance metrics for bias reduction in
                   matching methods for causal inference},
  year =          {2006},
}

@article{Hansen08,
  author =        {B.B. Hansen},
  journal =       {Biometrika},
  pages =         {481--8},
  title =         {The prognostic analogue of the propensity score},
  volume =        {95},
  year =          {2008},
}

@book{Haignere02,
  address =       {Washington, DC},
  author =        {Haignere, L.},
  edition =       {2nd},
  publisher =     {American Association of University Professors},
  title =         {Paychecks: a guide to conducting salary-equity
                   studies for higher education faculty},
  year =          {2002},
}

@article{Holland88,
  author =        {P.W. Holland},
  journal =       {Stat Sci},
  number =        {2},
  pages =         {186--188.},
  title =         {Comment: Causal Mechanism or Causal Effect: which Is
                   Best for Statistical Science?},
  volume =        {3},
  year =          {1988},
}

@article{Robins98,
  author =        {J.M. Robins},
  journal =       {1997 Proceedings of the American Statistical
                   Association. Section on {B}ayesian Statistical Science},
  pages =         {1--10},
  title =         {Marginal Structural Models},
  year =          {1998},
}

@article{Mossetal04,
  author =        {A.R. Moss and J.A. Hahn and S. Perry and
                   E.D. Charlebois and D. Guzman and R.A. Clark and
                   D.R. Bangsberg},
  journal =       {Clin Infect Dis},
  number =        {8},
  pages =         {1190--1198},
  title =         {Adherence to highly active antiretroviral therapy in
                   the homeless population in {S}an {F}rancisco: a
                   prospective study},
  volume =        {39},
  year =          {2004},
}

@article{Bangsbergetal01,
  author =        {D.R. Bangsberg and F. Hecht and E.D. Charlebois and
                   M. Chesney and A.R. Moss},
  journal =       {AIDS Behav},
  pages =         {275--281},
  title =         {Comparing Objectives Measures of Adherence to HIV
                   Antiretroviral Therapy: electronic Medication
                   Monitors and Unannounced Pill Counts.},
  volume =        {5},
  year =          {2001},
}

@article{Neugebauer&vanderLaan07,
  author =        {R. Neugebauer and M. J. van der Laan},
  journal =       {J Stat Plan Infer},
  number =        {2},
  pages =         {419--434},
  title =         {Nonparametric causal effects based on marginal
                   structural models},
  volume =        {137},
  year =          {2007},
}

@article{Efron87,
  author =        {B. Efron},
  journal =       {J Am Stat Assoc},
  number =        {397},
  pages =         {171--185},
  title =         {Better Bootstrap Confidence Intervals},
  volume =        {82},
  year =          {1987},
}

@article{Kirschetal08,
  author =        {I. Kirsch and B.J. Deacon and T.B. Huedo-Medina and
                   A. Scoboria and T.J. Moore and B.T. Johnson},
  journal =       {PLoS Med},
  number =        {2},
  pages =         {e45. doi:10.1371/journal.pmed.0050045},
  title =         {Initial Severity and Antidepressant Benefits: a
                   Meta-Analysis of Data Submitted to the {Food and Drug
                   Administration}},
  volume =        {5},
  year =          {2008},
}

@article{Baselga01,
  author =        {J. Baselga},
  journal =       {Oncology},
  pages =         {14--21},
  title =         {Herceptin alone or in combination with chemotherapy
                   in the treatment of {HER2}-positive metastatic breast
                   cancer: pivotal trials},
  volume =        {61(S2)},
  year =          {2001},
}

@techreport{Wangetal06,
  author =        {Y. Wang and M.L. Petersen and D.R. Bangsberg and
                   M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =        {211},
  title =         {Diagnosing Bias in the Inverse Probability of
                   Treatment Weighted Estimator Resulting from Violation
                   of Experimental Treatment Assignment.},
  year =          {2006},
}

@article{Robins87,
  author =        {Robins, J.M.},
  journal =       {Comput Math Appl},
  number =        {9--12},
  pages =         {923--945},
  title =         {Addendum to: ``{A} new approach to causal inference
                   in mortality studies with a sustained exposure
                   period---application to control of the healthy worker
                   survivor effect''},
  volume =        {14},
  year =          {1987},
}



@article{Robins872,
  author =        {J.M. Robins},
  journal =       {J Chron Dis (40, Supplement)},
  pages =         {139s--161s},
  title =         {A graphical approach to the identification and
                   estimation of causal parameters in mortality studies
                   with sustained exposure periods},
  volume =        {2},
  year =          {1987},
}

@article{Rosenblum&vanderLaan09b,
  author =        {M. Rosenblum and M.J. van der Laan},
  journal =       {Int J Biostat},
  pages =         {Article 4},
  title =         {Confidence Intervals for the Population Mean Tailored
                   to Small Sample Sizes, with Applications to Survey
                   Sampling},
  volume =        {1},
  year =          {2009},
}

@article{Neugebauer&vanderLaan05,
  author =        {Neugebauer, R. and van der Laan, M.J.},
  journal =       {J Stat Plan Infer},
  number =        {1-2},
  pages =         {405--26},
  title =         {Why prefer double robust estimates},
  volume =        {129},
  year =          {2005},
}

@techreport{Mooreetal09,
  author =        {K.L. Moore and R.S. Neugebauer and M.J. van der Laan and
                   I.B. Tager},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =        {255},
  title =         {Causal Inference in Epidemiological Studies with
                   Strong Confounding},
  year =          {2009},
}

@article{Kish92,
  author =        {L. Kish},
  journal =       {J Off Stat},
  number =        {},
  pages =         {183--200},
  title =         {Weighting for unequal $P_i$},
  volume =        {8},
  year =          {1992},
}

@techreport{Bembom&vanderLaan08,
  author =        {O. Bembom and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =        {230},
  title =         {Data-adaptive selection of the truncation level for
                   Inverse-Probability-of-Treatment-Weighted estimators},
  year =          {2008},
}

@article{Freedman&Berk08,
  author =        {D.A. Freedman and R.A. Berk},
  journal =       {Eval Rev},
  pages =         {392--409},
  title =         {Weighting Regressions by Propensity Scores},
  volume =        {3},
  year =          {2008},
}

@article{Petersenetal10,
  author =        {M.L. Petersen and K.E. Porter and S. Gruber and
                   Y. Wang and M.J. van der Laan},
journal = {Stat Meth Med Res},
  title =         {Diagnosing and responding to violations in the
                   positivity assumption},
     volume =        {published online 28 Oct (doi:
                   10.1177/0962280210386207)},
  year =          {2010},
}

@article{Johnsonetal09,
  author =        {V.A. Johnson and F. Brun-Vezinet and B. Clotet and
                   H.F. Gunthard and D.R. Kuritzkes and D. Pillay and
                   J.M. Schapiro and D.D. Richman},
  journal =       {Top HIV Med},
  number =        {5},
  pages =         {138--45},
  title =         {Update of the drug resistance mutations in {HIV}-1:
                   {D}ecember 2009.},
  volume =        {17},
  year =          {2009},
}

@techreport{Bembometal08b,
  author =        {O. Bembom and W.J. Fessel and R.W. Shafer and
                   M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  type =          {231},
  title =         {Data-adaptive Selection Of The Adjustment Set In
                   Variable Importance Estimation},
  year =          {2008},
}

@techreport{Crumpetal06,
  author =        {R.K. Crump and V.J. Hotz and G.W. Imbens and
                   O.A. Mitnik},
  institution =   {National Bureau of Economic Research},
  number =        {330},
  title =         {Moving the goalposts: addressing limited overlap in
                   the estimation of average treatment effects by
                   changing the estimand},
  year =          {2006},
}

@article{LaLonde86,
  author =        {R.J. LaLonde},
  journal =       {Am Econ Rev},
  pages =         {604--620},
  title =         {Evaluating the Econometric Evaluations of Training
                   Programs with Experimental Data},
  volume =        {76},
  year =          {1986},
}

@article{Dehejia&Wahba99,
  author =        {R. Dehejia and S. Wahba},
  journal =       {J Am Stat Assoc},
  pages =         {1053--1062},
  title =         {Causal Effects in Nonexperimental Studies:
                   reevaluating the Evaluation of Training Programs},
  volume =        {94},
  year =          {1999},
}

@article{vanderLaan&Petersen07,
  author =        {M.J. van der Laan and M.L. Petersen},
  journal =       {Int J Biostat},
  number =        {1},
  pages =         {Article 3},
  title =         {Causal Effect Models for Realistic Individualized
                   Treatment and Intention to Treat Rules},
  volume =        {3},
  year =          {2007},
}

@article{Robins&Orellana&Rotnitzky08,
  author =        {J.M. Robins and L. Orellana and A. Rotnitzky},
  journal =       {Stat Med},
  pages =         {4678--4721},
  title =         {Estimation and extrapolation of optimal treatment and
                   testing strategies},
  volume =        {27},
  year =          {2008},
}

@article{Cochran57,
  author =        {W.G. Cochran},
  journal =       {Biometrics},
  number =        {},
  pages =         {261--281},
  title =         {Analysis of Covariance: its Nature and Uses.},
  volume =        {13},
  year =          {1957},
}

@techreport{Moore&vanderLaan07,
  author =        {K.L. Moore and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  month =         {April},
  number =          {215},
  title =         {Covariate adjustment in randomized trials with binary
                   outcomes},
  year =          {2007},
}

@article{Rosenblum&vanderLaan102,
  author =        {M. Rosenblum and M.J. van der Laan},
  journal =       {Int J Biostat},
  number =        {1},
  pages =         {Article 13},
  title =         {Simple, Efficient Estimators of Treatment Effects in
                   Randomized Trials Using Generalized Linear Models to
                   Leverage Baseline Variables},
  volume =        {6},
  year =          {2010},
}

@article{Freedman083,
  author =        {D.A. Freedman},
  journal =       {Stat Sci},
  pages =         {237--249},
  title =         {Randomization does not justify logistic regression},
  volume =        {23},
  year =          {2008},
}

@article{Yang&Tsiatis01,
  author =        {L. Yang and A.A. Tsiatis},
  journal =       {Am Stat},
  pages =         {29--38},
  title =         {Efficiency study for a treatment effect in a
                   pretest-posttest trial},
  volume =        {56},
  year =          {2001},
}

@book{McCullagh&Nelder89,
  address =       {Boca Raton},
  author =        {P. McCullagh and J.A. Nelder},
  edition =       {2nd},
  publisher =     {Chapman \& Hall},
  title =         {Generalized linear models},
  year =          {1989},
}

@incollection{Gail86,
  address =       {New York},
 author =        {M.H. Gail},
  booktitle =     {Modern Statistical Methods in Chronic Disease
                   Epidemiology},
  editor =        {S.~H. Moolvankar and R.~L.
                   Prentice},
  publisher =     {Wiley},
  title =         {Adjusting for covariates that have the same
                   distribution in exposed and unexposed cohorts},
  year =          {1986},
}

@article{Tsiatisetal08,
  author =        {A.A. Tsiatis and M. Davidian and M. Zhang and X. Lu},
  journal =       {Stat Med},
  pages =         {4658--4677},
  title =         {Covariate adjustment for two-sample treatment
                   comparisons in randomized clinical trials: a
                   principled yet flexible approach},
  volume =        {27},
  year =          {2008},
}

@article{Kochetal98,
  author =        {G.G. Koch and C.M. Tangen and J.W. Jung and
                   I.A. Amara},
  journal =       {Stat Med},
  pages =         {1863--1892},
  title =         {Issues for covariance analysis of dichotomous and
                   ordered categorical data from randomized clinical
                   trials and nonparametric strategies for addressing
                   them},
  volume =        {17},
  year =          {1998},
}

@article{Pococketal02,
  author =        {S.J. Pocock and S.E. Assmann and L.E. Enos and
                   L.E. Kasten},
  journal =       {Stat Med},
  pages =         {2917--2930},
  title =         {Subgroup analysis, covariate adjustment, and baseline
                   comparisons in clinical trial reporting: current
                   practice and problems.},
  volume =        {21},
  year =          {2002},
}

@article{Anderson72,
  author =        {J.A. Anderson},
  journal =       {Biometrika},
  pages =         {19--35},
  title =         {Separate sample logistic discrimination},
  volume =        {59},
  year =          {1972},
}

@article{Robins99,
  author =        {J.M. Robins},
  journal =       {Stat Sci},
  number =        {3},
  pages =         {281--293},
  title =         {[{C}hoice as an Alternative to Control in Observational
                   Studies]: Comment},
  volume =        {14},
  year =          {1999},
}

@article{Manssonetal07,
  author =        {R. Mansson and M.M. Joffe and W. Sun and S. Hennessy},
  journal =       {Am J Epidemiol},
  number =        {3},
  pages =         {332-339},
  title =         {On the Estimation and Use of Propensity Scores in
                   Case-Control and Case-Cohort Studies.},
  volume =        {166},
  year =          {2007},
}

@article{Prentice&Pyke79,
  author =        {R.L. Prentice and R. Pyke},
  journal =       {Biometrika},
  pages =         {403--411},
  title =         {Logistic disease incidence models and case-control
                   studies},
  volume =        {66},
  year =          {1979},
}

@book{Breslow&Day80,
  address =       {Lyon},
  author =        {N.E. Breslow and N.E. Day},
  publisher =     {International Agency for Research on Cancer},
  title =         {Statistical methods in cancer research: {V}olume 1 --
                   {T}he analysis of case-control studies},
  year =          {1980},
}

@article{Breslow96,
  author =        {N.E. Breslow},
  journal =       {J Am Stat Soc},
  pages =         {14--28},
  title =         {Statistics in Epidemiology: the Case-Control Study},
  volume =        {91},
  year =          {1996},
}

@article{Greenland81,
  author =        {S. Greenland},
  journal =       {J Chron Dis},
  pages =         {445--453},
  title =         {Multivariate Estimation of Exposure-Specific
                   Incidence from Case-Control Studies.},
  volume =        {34},
  year =          {1981},
}

@incollection{Holland&Rubin88,
  address =       {Cambridge, MA},
  author =        {P.W. Holland and Donald B. Rubin},
  booktitle =     {Matched sampling for causal effects.},
  editor =        {Donald B. Rubin},
  publisher =     {Cambridge},
  title =         {Causal inference in retrospective studies},
  year =          {1988},
}

@article{Greenland04,
  author =        {S. Greenland},
  journal =       {Am J Epidemiol},
  number =        {4},
  pages =         {301--305},
  title =         {Model-based Estimation of Relative Risks and Other
                   Epidemiologic Measures in Studies of Common Outcomes
                   and in Case-Control Studies.},
  volume =        {160},
  year =          {2004},
}

@article{Newman06,
  author =        {S. Newman},
  journal =       {Epid Persp Innov},
  pages =         {2},
  title =         {Causal analysis of case-control data},
  volume =        {3},
  year =          {2006},
}

@article{Cornfield51,
  author =        {J. Cornfield},
  journal =       {J Nat Cancer Inst},
  pages =         {1269--1275},
  title =         {A method of estimating comparative rates from
                   clinical data. Applications to cancer of the lung,
                   breast, and cervix.},
  volume =        {11},
  year =          {1951},
}

@inproceedings{Cornfield56,
  author =        {J. Cornfield},
    address =       {Berkeley},
  booktitle =     {Proceedings of the 3rd Berkeley symposium, {V}ol
                   IV},
  editor =        {J. Neyman},
  publisher =     {University of California Press},
  title =         {A statistical problem arising from retrospective
                   studies},
  year =          {1956},
}

@article{Prentice&Breslow78,
  author =        {R.L. Prentice and N.E. Breslow},
  journal =       {Biometrika},
  number =        {1},
  pages =         {153--158},
  title =         {Retrospective studies and failure time models.},
  volume =        {65},
  year =          {1978},
}

@article{Moriseetal96,
  author =        {A.P. Morise and G.A. Diamon and R. Detrano and
                   M. Bobbio and Erdogan Gunel},
  journal =       {Med Decis Making},
  pages =         {133--142},
  title =         {The Effect of Disease-prevalence Adjustments on the
                   Accuracy of a Logistic Prediction Model.},
  volume =        {16},
  year =          {1996},
}

@article{Wacholder96,
  author =        {S. Wacholder},
  journal =       {Epidemiol},
  number =        {2},
  pages =         {144--150},
  title =         {The Case-Control Study as Data Missing by Design:
                   estimating Risk Differences.},
  volume =        {7},
  year =          {1996},
}

@article{Rose&vanderLaan11,
  author =        {S. Rose and M.J. van der Laan},
  journal =       {Int J Biostat},
  number =        {17},
  title =         {A Targeted Maximum Likelihood Estimator for Two-Stage
                   Designs},
  volume =        {7},
  year =          {2011},
}

@article{Freedman50,
  author =        {R. Freedman},
  journal =       {Am J of Soc},
  number =        {5},
  pages =         {485--487},
  title =         {Incomplete Matching in Ex Post Facto Studies},
  volume =        {55},
  year =          {1950},
}

@article{Cochran65,
  author =        {W.G. Cochran},
  journal =       {J R Stat Soc Ser A Gen},
  number =        {2},
  pages =         {234--266},
  title =         {The Planning of Observational Studies of Human
                   Populations},
  volume =        {128},
  year =          {1965},
}

@article{Billewicz65,
  author =        {W.Z. Billewicz},
  journal =       {Biometrics},
  number =        {3},
  pages =         {623--644},
  title =         {The Efficiency of Matched Samples: an Empirical
                   Investigation},
  volume =        {21},
  year =          {1965},
}

@article{McKinlay77,
  author =        {S.M. McKinlay},
  journal =       {Biometrics},
  number =        {4},
  pages =         {725--735},
  title =         {Pair-Matching -- A reappraisal of a Popular
                   Technique},
  volume =        {33},
  year =          {1977},
}

@article{Kupperetal81,
  author =        {L.L. Kupper and J.M. Karon and D.G. Kleinbaum and
                   H. Morgenstern and D.K. Lewis},
  journal =       {Biometrics},
  pages =         {271--291},
  title =         {Matching in Epidemiologic Studies: validity and
                   Efficiency Considerations},
  volume =        {37},
  year =          {1981},
}

@article{Costanza95,
  author =        {M.C. Costanza},
  journal =       {Prev Med},
  pages =         {425--433},
  title =         {Matching},
  volume =        {24},
  year =          {1995},
}

@book{Schlesselman82,
  address =       {Oxford},
  author =        {J.J. Schlesselman},
  publisher =     {Oxford},
  title =         {Case-control studies: design, conduct, analysis},
  year =          {1982},
}

@article{Vandenbroukeetal07,
  author =        {J.P. Vandenbrouke and E. von Elm and D.G. Altman and
                   P.C. Gotzsche and C.D. Mulrow and S.J. Pocock and
                   C. Poole and J.J. Schlesselman and
                   M. Egger for the STROBE Initiative},
  journal =       {PLoS Med},
  number =        {10},
  pages =         {1628--1654},
  title =         {Strengthening the Reporting of Observational
                   Studies in Epidemiology ({STROBE}): explanation
                   and Elaboration.},
  volume =        {4},
  year =          {2007},
}

@article{Cochran53,
  author =        {W.G. Cochran},
  journal =       {Am J Public Health},
  pages =         {684--691},
  title =         {Matching in Analytical Studies},
  volume =        {43},
  year =          {1953},
}

@article{Breslowetal78,
  author =        {N.E. Breslow and N.E. Day and K.T. Halvorsen and
                   R.L. Prentice and C. Sabal},
  journal =       {Am J Epidemiol},
  number =        {4},
  pages =         {299--307},
  title =         {Estimation of Multiple Relative Risk Functions in
                   Matched Case-Control Studies},
  volume =        {108},
  year =          {1978},
}

@article{Holford&White&Kelsey78,
  author =        {T.R. Holford and C. White and J.L. Kelsey},
  journal =       {Am J Epidemiol},
  number =        {3},
  pages =         {245--255},
  title =         {Multivariate Analysis for Matched Case-Control
                   Studies},
  volume =        {107},
  year =          {1978},
}

@article{Kannel&McGee&Gordon76,
  author =        {W.B. Kannel and D. McGee and T. Gordon},
  journal =       {Am J Cardiol},
  pages =         {46--51},
  title =         {A general cardiovascular risk profile: the {F}ramingham
                   Study},
  volume =        {38},
  year =          {1976},
}

@article{Andersonetal91,
  author =        {K.M. Anderson and P.W.F. Wilson and P.M. Odell and
                   W.B. Kannel},
  journal =       {Circulation},
  pages =         {356--362},
  title =         {An updated coronary risk profile. A statement for
                   health professionals.},
  volume =        {83},
  year =          {1991},
}

@article{Ramsayetal95,
  author =        {L.E. Ramsay and I.U. Haq and P.R. Jackson and
                   W.W. Yeo},
  journal =       {Lancet},
  number =        {8988},
  pages =         {1467--1471},
  title =         {Sheffield risk and treatment table for cholesterol
                   lowering for primary prevention of coronary heart
                   disease.},
  volume =        {346},
  year =          {1995},
}

@article{Ramsayetal96,
  author =        {L.E. Ramsay and I.U. Haq and P.R. Jackson and
                   W.W. Yeo},
  journal =       {Lancet},
  number =        {9036},
  pages =         {1251},
  title =         {The {S}heffield table for primary prevention of
                   coronary heart disease: corrected.},
  volume =        {348},
  year =          {1996},
}

@article{Wilsonetal98,
  author =        {P.W.F. Wilson and R.B. D'Agostino and D. Levy and
                   A.M. Belanger and H. Silbershatz and W.B. Kannel},
  journal =       {Circulation},
  pages =         {1837--1847},
  title =         {Prediction of coronary heart disease using risk
                   factor categories},
  volume =        {97},
  year =          {1998},
}

@article{Jackson00,
  author =        {R. Jackson},
  journal =       {Br Med J},
  number =        {7236},
  pages =         {709--710},
  title =         {Updated New Zealand cardiovascular disease
                   risk-benefit prediction guide.},
  volume =        {320},
  year =          {2000},
}

@article{Gailetal89,
  author =        {M.H. Gail and L.A. Brinton and D.P. Byar and
                   D.K. Corle and S.B. Green and C. Schairer and
                   J.J. Mulvihill},
  journal =       {J Natl Cancer Inst},
  number =        {24},
  pages =         {1879--1886},
  title =         {Projecting individualized probabilities of developing
                   breast cancer for white females who are being
                   examined annually.},
  volume =        {81},
  year =          {1989},
}

@article{Costantinoetal99,
  author =        {J.P. Costantino and M.H. Gail and D. Pee and
                   S. Anderson and C.K. Redmond and J. Benichou and
                   H.S. Wieand},
  journal =       {J Natl Cancer Inst},
  number =        {18},
  pages =         {1541--1548},
  title =         {Validation studies for models projecting the risk of
                   invasive and total breast cancer incidence.},
  volume =        {91},
  year =          {1999},
}

@article{Tyrer&Duffy&Cuzick04,
  author =        {J. Tyrer and S.W. Duffy and J. Cuzick},
  journal =       {Stat Med},
  number =        {7},
  pages =         {1111--1130},
  title =         {A breast cancer prediction model incorporating
                   familial and personal risk factors},
  volume =        {23},
  year =          {2004},
}

@article{Barlowetal06,
  author =        {W.E. Barlow and E. White and R. Ballard-Barbash and
                   P.M. Vacek and L. Titus-Ernstoff and P.A. Carney and
                   J.A. Tice and D.S. Buist and B.M. Geller and
                   R. Rosenberg and B.C. Yankaskas and K. Kerlikowske},
  journal =       {J Natl Cancer Inst},
  number =        {17},
  pages =         {1204--1214},
  title =         {Prospective breats cancer risk prediction model for
                   women undergoing screening mammography.},
  volume =        {98},
  year =          {2006},
}

@article{Loprinzietal94,
  author =        {C.L. Loprinzi and J.A. Laurie and H.S. Wieand and
                   J.E. Krook and P.J. Novotny and J.W. Kugler and
                   J. Bartel and M. Law and M. Bateman and N.E. Klatt},
  journal =       {J Clin Oncol},
  number =        {3},
  pages =         {601--607},
  title =         {Prospective Evaluation of Prognostic Variables from
                   Patient-Completed Questionnaires, {N}orth {C}entral
                   {C}ancer {T}reatment {G}roup},
  volume =        {12},
  year =          {1994},
}

@manual{Therneau&Lumley09,
  author =        {T. Therneau and T. Lumley},
  note =          {R package version 2.35-8},
  title =         {survival: survival analysis, including penalised
                   likelihood},
  year =          {2009},
  url =           {http://CRAN.R-project.org/package=survival},
}

@article{Tibshirani97,
  author =        {R.J. Tibshirani},
  journal =       {Stat Med},
  pages =         {385--395},
  title =         {The Lasso Method for Variable Selection in the {C}ox
                   Model},
  volume =        {16},
  year =          {1997},
}

@article{Zhang&Lu07,
  author =        {H.H. Zhang and W. Lu},
  journal =       {Biometrika},
  number =        {3},
  pages =         {691--703},
  title =         {Adaptive Lasso for {C}ox's Proportional Hazards Model},
  volume =        {94},
  year =          {2007},
}

@article{Kooperberg&Stone&Truong95,
  author =        {C. Kooperberg and C.J. Stone and Y.K. Truong},
  journal =       {J Am Stat Assoc},
  number =        {429},
  pages =         {78--94},
  title =         {Hazard Regression},
  volume =        {90},
  year =          {1995},
}

@article{Leblanc&Crowley92,
  author =        {M. LeBlanc and J. Crowley},
  journal =       {Biometrics},
  number =        {},
  pages =         {411--425},
  title =         {Relative Risk trees for censored data},
  volume =        {48},
  year =          {1992},
}

@article{Segal88,
  author =        {M.R. Segal},
  journal =       {Biometrics},
  pages =         {35--47},
  title =         {Regression trees for censored data},
  volume =        {44},
  year =          {1988},
}

@article{Hothornetal06,
  author =        {T. Hothorn and P. Buhlmann and S. Dudoit and
                   A.M. Molinaro and M.J. van der Laan},
  journal =       {Biostatistics},
  pages =         {355--373},
  title =         {Survival Ensembles},
  volume =        {7},
  year =          {2006},
}

@article{Ishwaranetal08,
  author =        {H. Ishwaran and U.B. Kogalur and E.H. Blackstone and
                   M.S. Lauer},
  journal =       {Ann Appl Stat},
  number =        {3},
  pages =         {841--860},
  title =         {Random Survival Forests},
  volume =        {2},
  year =          {2008},
}

@article{vanHouwelingenetal06,
  author =        {H.C. van Houwelingen and T. Bruinsma and A.A.M. Hart and
                   L.J. {van't Veer} and L.F.A. Wessels},
  journal =       {Stat Med},
  pages =         {3201--3216},
  title =         {Cross-validated {C}ox Regression on Microarray Gene
                   Expression Data},
  volume =        {25},
  year =          {2006},
}

@techreport{vanderLaan&Rubin07,
  author =        {M.J. van der Laan and Daniel B. Rubin},
    institution =   {Division of Biostatistics, University of California,
                   Berkeley},
   number={226},
  title =         {A note on targeted maximum likelihood and right-censored data},
  year =          {2007},
}

@inproceedings{Robins93,
  author =        {J.M. Robins},
  booktitle =     {Proceedings of the Biopharmaceutical Section},
  organization =  {American Statistical Association},
  title =         {Information recovery and bias adjustment in
                   proportional hazards regression analysis of
                   randomized trials using surrogate markers},
  year =          {1993},
}

@incollection{Hubbard&vanderLaan&Robins99,
  address={Berlin Heidelberg New York},
  author =        {A.E. Hubbard and M.J. van der Laan and J.M. Robins},
  booktitle =     {Statistical models in epidemiology: the environment
                   and clinical trials},
  editor =        {E. Halloran, D. Berry},
   publisher =     {Springer},
  title =         {Nonparametric locally efficient estimation of the
                   treatment specific survival distributions with right
                   censored data and covariates in observational
                   studies},
  year =          {1999},
}

@article{Hernandez&Eijkemans&Steyerberg06,
  author =        {Hern\'{a}ndez, A.V. and Eijkemans, M.J. and
                   Steyerberg, E.W.},
  journal =       {Ann Epidemiol},
  number =        {1},
  pages =         {41--48},
  title =         {Randomized controlled trials With time-to-event
                   outcomes: how much does prespecified covariate
                   adjustment increase power?},
  volume =        {16},
  year =          {2006},
}

@article{Lu&Tsiatis08,
  author =        {Lu, X. and Tsiatis, A.A},
  journal =       {Biometrika},
  number =        {3},
  pages =         {679--694},
  title =         {Improving the efficiency of the log-rank test using
                   auxiliary covariates},
  volume =        {95},
  year =          {2008},
}

@article{Tangen&Koch99,
  author =        {Tangen, C.M. and Koch, G.G.},
  journal =       {J Biopharm Stat},
  number =        {2},
  pages =         {307--338},
  title =         {On-parametric analysis of covariance for hypothesis
                   testing with logrank and {W}ilcoxon scores and
                   survival-rate estimation in a randomized clinical
                   trial},
  volume =        {9},
  year =          {1999},
}

@article{Jiangetal08,
  author =        {Jiang, H. and Symanowski, J. and Paul, S. and Qu, Y. and
                   Zagar, A. and Hong, S.},
  journal =       {Stat Med},
  number =        {28},
  pages =         {5850--5860},
  title =         {The type {I} error and power of nonparametric logrank
                   and {W}ilcoxon tests with adjustment for covariates -- A
                   simulation study},
  volume =        {27},
  year =          {2008},
}

@article{Akazawa&Nakamura&Palesch97,
  author =        {Akazawa, K. and Nakamura, T. and Palesch, Y.},
  journal =       {Stat Med},
  number =        {5},
  pages =         {583--597},
  title =         {Power of logrank test and {C}ox regression model in
                   clinical trials with heterogenous samples},
  volume =        {16},
  year =          {1997},
}

@article{Westeretal10,
  author =        {C.W. Wester and A.M. Thomas and H. Bussmann and
                   S. Moyo and J.M. Gaolathe and V. Novitsky and
                   M. Essex and V. De Gruttola and R.G. Marlink},
  journal =       {AIDS},
  pages =         {S27--S36},
  title =         {Nonnucleoside reverse transcriptase inhibitor
                   outcomes among combination antiretroviral
                   therapy-treated adults in {B}otswana},
  volume =        {24},
  year =          {2010},
}

@book{Andersenetal93,
  author =        {P.K. Andersen and O. Borgan and R.D. Gill and
                   N. Keiding},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  title =         {Statistical models based on counting processes},
  year =          {1993},
}

@techreport{Rudser&LeBlanc&Emerson08,
  author =        {K. Rudser and M. LeBlanc and S.S. Emerson},
  institution={Department of Biostatistics, University of Washington},
  title =         {Estimation for Arbitrary Functionals of Survival},
  number =        {335},
  year =          {2008},
}

@article{vanderLaan10,
  author =        {van der Laan, M.J.},
  journal =       {Int J Biostat},
  pages =          {Article 2},
  number =        {2},
  title =         {Targeted maximum likelihood based causal inference:
                   Part {I}},
  volume =        {6},
  year =          {2010},
}

@article{vanderLaan10b,
  author =        {van der Laan, M.J.},
  journal =       {Int J Biostat},
  pages =          {Article 3},
  number =        {2},
  title =         {Targeted maximum likelihood based causal inference:
                   Part {II}},
  volume =        {6},
  year =          {2010},
}

@article{Sekhon08,
  author =        {J.S. Sekhon},
  journal =       {J Stat Softw},
  title =         {Multivariate and Propensity Score Matching Software
                   with Automated Balance Optimization: the Matching
                   package for {R}},
  year =          {2008},
}

@article{Holland&Reitman77,
  address =       {New York},
  author =        {J.H. Holland and J.S. Reitman},
  journal =       {SIGART Bull},
  pages =         {49--49},
  title =         {Cognitive systems based on adaptive algorithms},
  volume =        {63},
  year =          {1977},
}

@article{Koul&Susarla&vanRyzin81,
  author =        {H. Koul and V. Susarla and J. van Ryzin},
  journal =       {Ann Stat},
  pages =         {1276--88},
  title =         {Regression analysis with randomly right censored
                   data},
  volume =        {9},
  year =          {1981},
}

@article{Keiding&Hols&Green89,
  author =        {N. Keiding and C. Hols and A. Green},
  journal =       {Am J Epidemiol},
  pages =         {588--600},
  title =         {Retrospective estimation of diabetes incidence from
                   information in a current prevalent population and
                   historical mortality},
  volume =        {130},
  year =          {1989},
}

@article{Robins&Rotnitzky&Zhao94,
  author =        {J.M. Robins and A. Rotnitzky and L.P. Zhao},
  journal =       {J Am Stat Assoc},
  month =         {September},
  number =        {427},
  pages =         {846--66},
  title =         {Estimation of regression coefficients when some
                   regressors are not always observed},
  volume =        {89},
  year =          {1994},
}

@article{Robins&Rotnitzky95,
  author =        {Robins, J.M. and A. Rotnitzky},
  journal =       {J Am Stat Assoc},
  pages =         {122--129},
  title =         {Semiparametric Efficiency in Multivariate Regression
                   Models with Missing Data},
  volume =        {90},
  year =          {1995},
}

@article{Kang&Schafer07,
  author =        {J. Kang and J.L. Schafer},
  journal =       {Stat Sci},
  pages =         {523--39},
  title =         {Demystifying Double Robustness: a Comparison of
                   Alternative Strategies for Estimating a Population
                   Mean from Incomplete Data (with discussion)},
  volume =        {22},
  year =          {2007},
}

@article{Robins&Wang00,
  author =        {J.M. Robins and N. Wang},
  journal =       {Biometrika},
  pages =         {113--124},
  title =         {Inference for imputation estimators},
  volume =        {87},
  year =          {2000},
}

@techreport{Bhattacharya&Vogt07,
  author =        {Bhattacharya, J. and Vogt, W.},
  institution =          {National Bureau of
                   Economic Research},
  number={343},
  title =         {Do Instrumental Variables Belong in Propensity
                   Scores?},
  year =          {2007},
}

@techreport{Wooldridge09,
  author =        {Wooldridge, J.},
  institution={Michigan State University},
  type={Technical {R}eport},
  title =         {Should Instrumental Variables be Used as Matching
                   Variables?},
  year =          {2009},
}

@article{Pearl10,
  author =        {Pearl, J.},
  journal =       {Proceedings of Uncertainty in Artificial Intelligence},
  title =         {On a Class of Bias-Amplifying Variables that Endanger
                   Effect Estimates},
  year =          {2010},
}

@article{Holland86,
  author =        {Holland, P.W.},
  journal =       {J Am Stat Assoc},
  number =        {396},
  pages =         {945--960},
  title =         {Statistics and Causal Inference},
  volume =        {81},
  year =          {1986},
}

@book{Rubin06,
  address =       {Cambridge, MA},
  author =        {Donald B. Rubin},
  publisher =     {Cambridge},
  title =         {Matched sampling for causal effects.},
  year =          {2006},
}

@book{Rosenbaum02,
  address={Berlin Heidelberg New York},
  author =        {Rosenbaum, P.R.},
  edition =       {2nd},
  publisher =     {Springer},
  title =         {Observational studies},
  year =          {2002},
}

@article{Rubin97,
  author =        {Rubin, Donald B.},
  journal =       {Ann of Intern Med},
  number =        {8S},
  pages =         {757--763},
  title =         {Estimating causal effects from large data sets using
                   propensity scores},
  volume =        {127},
  year =          {1997},
}

@article{Christakis&Iwashyna03,
  author =        {Christakis, N.A. and Iwashyna, T.I.},
  journal =       {Soc Sci Med},
  number =        {3},
  pages =         {465--475},
  title =         {The Health Impact of Health Care on Families: a
                   matched cohort study of hospice use by decedents and
                   mortality outcomes in surviving, widowed spouses},
  volume =        {57},
  year =          {2003},
}

@article{Dehejia&Wahba02,
  author =        {R. Dehejia and S. Wahba},
  journal =       {Rev Econ Stat},
  number =        {1},
  pages =         {151--161},
  title =         {Propensity Score Matching Methods for Nonexperimental
                   Causal Studies},
  volume =        {84},
  year =          {2002},
}

@article{Galiani&Gertler&Schargrodsky05,
  author =        {Galiani, S. and P. Gertler and E. Schargrodsky},
  journal =       {J Polit Econ},
  number =        {1},
  pages =         {83--120},
  title =         {Water for Life: the Impact of the Privatization of
                   Water Services on Child Mortality},
  volume =        {113},
  year =          {2005},
}

@article{Abadie&Imbens06,
  author =        {Abadie, A. and G.W. Imbens},
  journal =       {Econometrica},
  pages =         {235--267},
  title =         {Large Sample Properties of Matching Estimators for
                   Average Treatment Effects},
  volume =        {74},
  year =          {2006},
}

@article{Herron&Wand07,
  author =        {Herron, M.C. and J. Wand},
  journal =       {Elect Stud},
  number =        {2},
  pages =         {247--261},
  title =         {Assessing Partisan Bias in Voting Technology: the
                   Case of the 2004 {N}ew {H}ampshire Recount},
  volume =        {26},
  year =          {2007},
}

@article{Imai05,
  author =        {K. Imai},
  journal =       {Am Polit Sci Rev},
  number =        {2},
  pages =         {283--300},
  title =         {Do Get-Out-The-Vote Calls Reduce Turnout? The
                   Importance of Statistical Methods for Field
                   Experiments},
  volume =        {99},
  year =          {2005},
}

@incollection{Sekhon08b,
  address =       {New York},
  author =        {Sekhon, J.S.},
  booktitle =     {The Oxford handbook of political methodology},
  editor =        {J.M. Box-Steffensmeier and H.E. Brady and
                   D. Collier},
  publisher =     {Oxford},
  title =         {The {N}eyman-{R}ubin Model of Causal Inference and
                   Estimation via Matching Methods},
  year =          {2008},
}

@article{Morgan&Harding06,
  author =        {Morgan, S.L. and D.J. Harding},
  journal =       {Sociol Meth Res},
  number =        {1},
  pages =         {3--60},
  title =         {Matching Estimators of Causal Effects: prospects and
                   Pitfalls in Theory and Practice},
  volume =        {35},
  year =          {2006},
}

@article{Diprete&Engelhardt04,
  author =        {Diprete, T.A. and H. Engelhardt},
  journal =       {Sociol Meth Res},
  number =        {4},
  pages =         {501--528},
  title =         {Estimating Causal Effects With Matching Methods in
                   the Presence and Absence of Bias Cancellation},
  volume =        {32},
  year =          {2004},
}

@article{Winship&Morgan99,
  author =        {Winship, C. and S.L. Morgan},
  journal =       {Annu Rev Sociol},
  pages =         {659--707},
  title =         {The estimation of causal effects from observational
                   data},
  volume =        {25},
  year =          {1999},
}

@article{Smith97,
  author =        {Smith, H.L.},
  journal =       {Sociol Meth},
  pages =         {305--353},
  title =         {Matching with Multiple Controls to Estimate Treatment
                   Effects in Observational Studies},
  volume =        {27},
  year =          {1997},
}

@article{Rubin02,
  author =        {Rubin, Donald B.},
  journal =       {Health Serv Outcome Res Meth},
  number =        {1},
  pages =         {169--188},
  title =         {Using Propensity Scores to Help Design Observational
                   Studies: application to the Tobacco Litigation},
  volume =        {2},
  year =          {2002},
}

@incollection{Brady08,
  address =       {New York},
  author =        {Brady, H.},
  booktitle =     {The Oxford handbook of political methodology},
  editor =        {J.M. Box-Steffensmeier and H.E. Brady and
                   D. Collier},
  publisher =     {Oxford},
  title =         {Causation and explanation in social science},
  year =          {2008},
}

@article{Freedman06,
  author =        {Freedman, D.A.},
  journal =       {Eval Rev},
  pages =         {691--713},
  title =         {Statistical Models for Causation: what Inferential
                   leverage Do They Provide?},
  volume =        {30},
  year =          {2006},
}

@article{Rubin90,
  author =        {Rubin, Donald B.},
  journal =       {Stat Sci},
  number =        {4},
  pages =         {472--480},
  title =         {Comment: {N}eyman (1923) and Causal Inference in
                   Experiments and Observational Studies},
  volume =        {5},
  year =          {1990},
}

@article{Speed90,
  author =        {T.P. Speed},
  journal =       {Stat Sci},
  number =        {4},
  pages =         {463--464},
  title =         {Introductory Remarks on {N}eyman (1923)},
  volume =        {5},
  year =          {1990},
}

@book{Cox58,
  address =       {New York},
  author =        {Cox, D.R.},
  publisher =     {Wiley},
  title =         {Planning of experiments},
  year =          {1958},
}

@article{Rubin78,
  author =        {Donald B. Rubin},
  journal =       {Ann Stat},
  number =        {},
  pages =         {34--58},
  title =         {Bayesian Inference for causal effects: the role of
                   randomization},
  volume =        {6},
  year =          {1978},
}

@incollection{Rubin75,
  address =       {Alexandria},
  author =        {Rubin, Donald B.},
  booktitle =     {The proceedings of the Social Statistics Section of
                   the American Statistical Association},
  publisher =     {American Statistical Association},
  title =         {Bayesian Inference for Causality: the Importance of
                   Randomization},
  year =          {1975},
}

@article{Rubin08,
  author =        {Rubin, Donald B.},
  journal =       {Ann of Appl Stat},
  number =        {3},
  pages =         {808--840},
  title =         {For Objective Causal Inference, Design Trumps
                   Analysis},
  volume =        {2},
  year =          {2008},
}

@article{Sekhon10,
  author =        {Sekhon, J.S.},
  journal =       {Annu Rev of Polit Sci},
  pages =         {487--508},
  title =         {Opiates for the Matches: matching Methods for Causal
                   Inference},
  volume =        {12},
  year =          {2010},
}

@article{Rubin76,
  author =        {Rubin, Donald B.},
  journal =       {Biometrics},
  number =        {1},
  pages =         {121--132},
  title =         {Multivariate Matching Methods That are Equal Percent
                   Bias Reducing, {II}: maximums on Bias Reduction for
                   Fixed Sample Sizes},
  volume =        {32},
  year =          {1976},
}

@article{Cochran&Rubin73,
  author =        {Cochran, W.G. and Donald B. Rubin},
  journal =       {Sankhya Ser A},
  pages =         {417--446},
  title =         {Controlling Bias in Observational Studies: a Review},
  volume =        {35},
  year =          {1973},
}

@book{Cochran83,
  address =       {New York},
  author =        {Cochran, W.G.},
  note =          {Edited posthumously by L.E. Moses and F. Mosteller},
  publisher =     {Wiley},
  title =         {Planning and analysis of observational studies},
  year =          {1983},
}

@article{Robinsetal07,
  author =        {J.M. Robins and M. Sued and Q. Lei-Gomez and
                   A. Rotnitzky},
  journal =       {Stat Sci},
  pages =         {544--559},
  title =         {Comment: {P}erformance of Double-Robust Estimators When
                   ``Inverse Probability'' Weights Are Highly Variable},
  volume =        {22},
  year =          {2007},
}

@article{Cortes&Vapnik95,
  author =        {C. Cortes and V. Vapnik},
  journal =       {Mach Learn},
  month =         {December},
  pages =         {273--297},
  title =         {Support-vector networks},
  volume =        {20},
  year =          {1995},
}

@techreport{Friedman94,
  author =        {J.H. Friedman},
  institution =   {Department of Statistics, Stanford University},
  type={Technical {R}eport},
  title =         {Flexible metric nearest neighbor classification},
  year =          {1994},
}

@techreport{FDA06,
  author =        {{Food and Drug Administration}},
  institution =   {U.S. Department of Health and Human Services, Food
                   and Drug Administration},
  type={Technical {R}eport},
  title =         {Critical Path Opportunities List},
  year =          {2006},
}

@article{Efronetal04,
  author =        {B. Efron and T. Hastie and I. Johnstone and
                   R. Tibshirani},
  journal =       {Ann Stat (with discussion)},
  number =        {2},
  pages =         {407--499},
  title =         {Least Angle Regression},
  volume =        {32},
  year =          {2004},
}

@techreport{Breiman99,
  author =        {L. Breiman},
  institution =   {Department of Statistics, University of California, Berkeley},
  number =        {567},
  title =         {Random forests - random features},
  year =          {1999},
}

@manual{Breiman01b,
  author =        {L. Breiman},
  title =         {Notes on setting up, using, and understanding random
                   forests V3.0},
  year =          {2001},
}

@article{Golubetal99,
  author =        {T.R. Golub and D.K. Slonim and P. Tamayo and C. Huard and
                   M. Gaasenbeek and J.P. Mesirov and H. Coller and
                   M.L. Loh and J.R. Downing and M.A. Caligiuri and
                   C.D. Bloomfield and E.S. Lander},
  journal =       {Science},
  pages =         {531--537},
  title =         {Molecular classification of cancer: class discovery
                   and class prediction by gene expression monitoring},
  volume =        {286},
  year =          {1999},
}

@article{vanderLaan06a,
  author =        {M.J. van der Laan},
  journal =       {Int J Biostat},
  number =        {1},
  pages =         {Article 2},
  title =         {Statistical Inference for Variable Importance},
  volume =        {2},
  year =          {2006},
}

@article{Robins&Mark&Newey92,
  author =        {J.M. Robins and S.D. Mark and W.K. Newey},
  journal =       {Biometrics},
  number =        {479--495},
  title =         {Estimating exposure effects by modelling the
                   expectation of exposure conditional on confounders},
  volume =        {48},
  year =          {1992},
}

@techreport{Yu&VanderLaan03,
  author =        {Z. Yu and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number={136},
  title =         {Measuring treatment effects using semiparametric
                   models},
  year =          {2003},
}

@techreport{Tuglus&vanderLaan08,
  author =        {C. Tuglus and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
number={233},
  title =         {Targeted Methods for Biomarker Discovery, the Search
                   for a Standard},
  year =          {2008},
}

@book{Hastie&Tibshirani90,
  address =       {London},
  author =        {T.J. Hastie and R.J. Tibshirani},
  publisher =     {Chapman \& Hall},
  title =         {Generalized additive models},
  year =          {1990},
}

@misc{Efron&Hastie07,
  author =        {B. Efron and T. Hastie},
  howpublished =  {R package},
  title =         {lars},
  year =          {2007},
}

@article{Benjamini&Hochberg95,
  author =        {Y. Benjamini and Y. Hochberg},
  journal =       {J R Stat Soc Ser B},
  pages =         {289--300},
  title =         {Controlling the false discovery rate: a practical and
                   powerful approach to multiple testing},
  volume =        {57},
  year =          {1995},
}

@misc{Ge&Dudoit02,
  author =        {Y. Ge and S. Dudoit},
  howpublished =  {R package},
  title =         {Multiple Testing Procedures, multtest},
  year =          {2002},
  url =           {www.bioconductor.org},
}

@article{Tibshirani96,
  author =        {R. Tibshirani},
  journal =       {J R Stat Soc Ser B},
  number =        {1},
  pages =         {267--288},
  title =         {Regression shrinkage and selection via the lasso.},
  volume =        {58},
  year =          {1996},
}

@article{Tuglus&vanderLaan09,
  author =        {C. Tuglus and M.J. van der Laan},
  journal =       {Stat Appl Genet Mol},
  number =        {1},
  pages =         {Article 12},
  title =         {Modified {FDR} Controlling Procedure for Multi-Stage
                   Analyses},
  volume =        {8},
  year =          {2009},
}

@article{Dudoit&Fridlyand&Speed02,
  author =        {S. Dudoit and J. Fridlyand and T. P. Speed},
  journal =       {J Am Stat Assoc},
  number =        {457},
  pages =         {77--87},
  title =         {Comparison of Discrimination Methods for the
                   Classification of Tumors Using Gene Expression Data},
  volume =        {97},
  year =          {2002},
}

@article{Kos&Lah98,
  author =        {J. Kos and T.T. Lah},
  journal =       {Oncol Rep},
  number =        {6},
  pages =         {1349--61},
  title =         {Cysteine proteinases and their endogenous inhibitors:
                   target proteins for prognosis, diagnosis and therapy
                   in cancer (review)},
  volume =        {5},
  year =          {1998},
}

@article{Vitaleetal01,
  author =        {C. Vitale and C. Romagnani and A. Puccetti and
                   D. Olive and R. Costello and L. Chiossone and
                   A. Pitto and A. Bacigalupo and L. Moretta and
                   M.C. Mingari},
  journal =       {Proc Natl Acad Sci},
  pages =         {5764--5769},
  title =         {Surface expression and function of p75/{AIRM}-1 or {CD}33
                   in acute myeloid leukemias: engagement of {CD}33
                   induces apoptosis of leukemic cells},
  volume =        {98},
  year =          {2001},
}

@article{Clappieretal07,
  author =        {E. Clappier and W. Cuccuini and A. Kalota and
                   A. Crinquette and J.M. Cayuela and W.A. Dik and
                   A.W. Langerak and B. Montpellier and B. Nadel and
                   P. Walrafen and O. Delattre and A. Aurias and
                   T. Leblanc and H. Dombret and A.M. Gewirtz and
                   A. Baruchel and F. Sigaux and J. Soulier},
  journal =       {Blood},
  number =        {4},
  pages =         {1251--61},
  title =         {The {C-MYB} locus is involved in chromosomal
                   translocation and genomic duplications in human
                   T-cell acute leukemia ({T-ALL}), the translocation
                   defining a new {T-ALL} subtype in very young children},
  volume =        {110},
  year =          {2007},
}

@article{Lane&Ley03,
  author =        {A.A. Lane and T.J. Ley},
  journal =       {Cell},
  number =        {305-318},
  title =         {Neutrophil elastase cleaves {PML-RAR}-alpha and is
                   important for the development of acute promyelocytic
                   leukemia in mice},
  volume =        {115},
  year =          {2003},
}

@article{Hunger96,
  author =        {S.P. Hunger},
  journal =       {Blood},
  pages =         {1211--1224},
  title =         {Chromosomal translocations involving the {E2A} gene in
                   acute lymphoblastic leukemia: clinical features and
                   molecular pathogenesis.},
  volume =        {87},
  year =          {1996},
}

@article{Nebraletal05,
  author =        {K. Nebral and H.H. Schmidt and O.A. Haas and
                   S. Strehl},
  journal =       {Clin Cancer Res},
  number =        {18},
  pages =         {6489--6494},
  title =         {{NUP}98 Is Fused to Topoisomerase {(DNA)} {II}{beta} 180
                   {kDa} {(TOP2B)} in a Patient with Acute Myeloid Leukemia
                   with a New {t(3;11)(p24;p15)}},
  volume =        {11},
  year =          {2005},
}

@article{Kaufmannetal98b,
  author =        {S.H. Kaufmann and S.D. Gore and C.B. Miller and
                   R.J. Jones and L.A. Zwelling and E. Schneider and
                   P.J. Burke and J.E. Karp},
  journal =       {Leukemia Lymphoma},
  month =         {Apr},
  number =        {3-4},
  pages =         {217--237},
  title =         {Topoisomerase {II} and the response to antileukemic
                   therapy},
  volume =        {29},
  year =          {1998},
}

@article{Kozaretal04,
  author =        {K. Kozar and M.A. Ciemerych and V.I. Rebel and
                   H. Shigematsu and A. Zagozdzon and E. Sicinska and
                   Y. Geng and Q. Yu and S. Bhattacharya and
                   R.T. Bronson and K. Akashi and P. Sicinski},
  journal =       {Cell},
  pages =         {477--491},
  title =         {Mouse development and cell proliferation in the
                   absence of {D}-cyclins},
  volume =        {118},
  year =          {2004},
}

@article{MartinSuberoetal07,
  author =        {J.I. Martin-Subero and R. Ibbotson and W. Klapper and
                   L. Michaux and E. Callet-Bauchu and F. Berger and
                   M.J. Calasanz and C. De Wolf-Peeters and M.J. Dyer and
                   P. Felman and A. Gardiner and R.D. Gascoyne and
                   S. Gesk and L. Harder and D.E. Horsman and M. Kneba and
                   R. Kuppers and A. Majid and N. Parry-Jones and
                   M. Ritgen and M. Salido and F. Sole and G. Thiel and
                   H.H. Wacker and D. Oscier and I. Wlodarska and
                   R. Siebert},
  journal =       {Leukemia},
  number =        {7},
  pages =         {1532--1544},
  title =         {A comprehensive genetic and histopathologic analysis
                   identifies two subgroups of {B}-cell malignancies
                   carrying a t(14;19)(q32;q13) or variant
                   {BCL3}-translocation},
  volume =        {21},
  year =          {2007},
}

@article{Palomeroetal06,
  author =        {T. Palomero and D.T. Odom and J. O'Neil and
                   A.A. Ferrando and A. Margolin and D.S. Neuberg and
                   S.S. Winter and R.S. Larson and W. Li and X.S. Liu and
                   R.A. Young and A.T. Look},
  journal =       {Blood},
  number =        {3},
  pages =         {986--992},
  title =         {Transcriptional regulatory networks downstream of
                   {TAL1/SCL} in {T}-cell acute lymphoblastic leukemia},
  volume =        {108},
  year =          {2006},
}

@article{Wongetal07,
  author =        {H.P. Wong and L. Yu and E.K. Lam and E.K. Tai and
                   W.K. Wu and C.H. Cho},
  journal =       {Toxicol Appl Pharm},
  number =        {3},
  pages =         {261--267},
  title =         {Nicotine promotes cell proliferation via
                   alpha7-nicotinic acetylcholine receptor and
                   catecholamine-synthesizing enzymes-mediated pathway
                   in human colon adenocarcinoma {HT}-29 cells.},
  volume =        {221},
  year =          {2007},
}

@article{Ramaswamyetal03,
  author =        {S. Ramaswamy and K.N. Ross and E.S. Lander and
                   T.R. Golub},
  journal =       {Nat Genet},
  pages =         {49--54},
  title =         {A molecular signature of metastasis in primary solid
                   tumors},
  volume =        {33},
  year =          {2003},
}

@article{Purietal01,
  author =        {R. Puri and A. Tousson and L. Chen and S.S. Kakar},
  journal =       {Cancer Lett},
  pages =         {131--139},
  title =         {Molecular cloning of pituitary tumor transforming
                   gene 1 from ovarian tumors and its expression in
                   tumors},
  volume =        {163},
  year =          {2001},
}

@article{Fujiietal06,
  author =        {T. Fujii and S. Nomoto and K. Koshikawa and Y.Yatabe and
                   O. Teshigawara and T. Mori and S. Inoue and S. Takeda and
                   A. Nakao},
  journal =       {Hepatology},
  pages =         {1267--1275},
  title =         {Overexpression of pituitary tumor transforming gene 1
                   in {HCC} is associated with angiogenesis and poor
                   prognosis},
  volume =        {43},
  year =          {2006},
}

@article{Zhuetal06,
  author =        {X. Zhu and Z. Mao and Y. Na and Y. Guo and X. Wang and
                   D. Xin},
  journal =       {Anticancer Res},
  pages =         {1253--1259},
  title =         {Significance of pituitary tumor transforming gene 1
                   ({PTTG1}) in prostate cancer},
  volume =        {26},
  year =          {2006},
}

@article{Kaufmannetal98a,
  author =        {S.H. Kaufmann and J.E. Karp and P.A. Svingen and
                   S. Krajewski and P.J. Burke and S.D. Gore and
                   J.C. Reed},
  journal =       {Blood},
  number =        {3},
  pages =         {991--1000},
  title =         {Elevated expression of the apoptotic regulator {Mcl}-1
                   at the time of leukemic relapse},
  volume =        {91},
  year =          {1998},
}

@article{Frumanetal99,
  author =        {D.A. Fruman and S.B. Snapper and C.M. Yballe and
                   L. Davidson and J.Y. Yu and F.W. Alt and
                   L.C. Cantley},
  journal =       {Science},
  pages =         {393--397},
  title =         {Impaired {B} cell development and proliferation in
                   absence of phosphoinositide 3-kinase p85-alpha},
  volume =        {283},
  year =          {1999},
}

@article{Tombes&Krystal97,
  author =        {R.M. Tombes and G.W. Krystal},
  journal =       {Biochim Biophys Acta},
  pages =         {281--292},
  title =         {Identification of novel human tumor cell-specific
                   {CaMK-II} variants},
  volume =        {1355},
  year =          {1997},
}

@article{Senturkeretal97,
  author =        {S. Senturker and B. Karahalil and M. Inal and
                   H. Yilmaz and H. Muslumanoglu and G. Gedikoglu and
                   M. Dizdaroglu},
  journal =       {FEBS Letters},
  number =        {3},
  pages =         {286--290},
  title =         {Oxidative {DNA} base damage and antioxidant enzyme
                   levels in childhood acute lymphoblastic leukemia},
  volume =        {416},
  year =          {1997},
}

@article{Komuroetal05,
  author =        {I. Komuro and T. Yasuda and A. Iwamoto and
                   K.S. Akagawa},
  journal =       {J Biol Chem},
  number =        {50},
  pages =         {41137--45},
  title =         {Catalase plays a critical role in the {CSF}-independent
                   survival of human macrophages via regulation of the
                   expression of {BCL}-2 family},
  volume =        {280},
  year =          {2005},
}

@article{Balciunaiteetal05,
  author =        {E. Balciunaite and A. Spektor and N.H. Lents and
                   H. Cam and H. Te Riele and A. Scime and M.A. Rudnicki and
                   R. Young and B.D. Dynlacht},
  journal =       {Mol Cell Biol},
  number =        {18},
  pages =         {8166--78},
  title =         {Pocket protein complexes are recruited to distinct
                   targets in quiescent and proliferating cells},
  volume =        {25},
  year =          {2005},
}

@article{Leoneetal01,
  author =        {G. Leone and R. Sears and E. Huang and R. Rempel and
                   F. Nuckolls and C.H. Park and P. Giangrande and L. Wu and
                   H.I. Saavedra and S.J. Field and M.A. Thompson and
                   H. Yang and Y. Fujiwara and M.E. Greenberg and
                   S. Orkin and C. Smith and J.R. Nevins},
  journal =       {Mol Cell},
  pages =         {105--113},
  title =         {Myc requires distinct {E2F} activities to induce {S}
                   phase and apoptosis},
  volume =        {8},
  year =          {2001},
}

@article{Sax23,
  author =        {Sax, K.},
  journal =       {Genetics},
  title =         {The association of size difference with seed-coat
                   pattern and pigmentation in \textit{Phaseolus
                   vulgaris}},
  year =          {1923},
}

@article{Thoday60,
  author =        {Thoday, J.M.},
  journal =       {Nature},
  title =         {Location of polygenes},
  year =          {1960},
}

@article{Lander&Botstein89,
  author =        {Lander, E.S. and Botstein, D.},
  journal =       {Genetics},
  title =         {Mapping {M}endelian factors underlying quantitative
                   traits using {RFLP} linkage maps},
  year =          {1989},
}

@article{Haley&Knott92,
  author =        {Haley, C.S. and Knott, S.A.},
  journal =       {Heredity},
  title =         {A simple regression method for mapping quantitative
                   trait loci in line crosses using flanking markers},
  year =          {1992},
}

@article{Jansen93,
  author =        {Jansen, R.C.},
  journal =       {Genetics},
  title =         {Interval mapping of multiple quantitative trait loci},
  year =          {1993},
}

@article{Zeng94,
  author =        {Zeng, Z.B.},
  journal =       {Genetics},
  title =         {Precision mapping of quantitative trait loci},
  year =          {1994},
}

@article{Kao&Zeng&Teasdale99,
  author =        {Kao, C.H. and Zeng, Z.B. and Teasdale, R.D.},
  journal =       {Genetics},
  title =         {Multiple interval mapping for quantitative trait
                   loci},
  year =          {1999},
}

@article{Satagopanetal96,
  author =        {Satagopan, J.M. and B.S. Yandell and M.A. Newton and
                   T.C. Osborn},
  journal =       {Genetics},
  title =         {A {B}ayesian approach to detect quantitative trait loci
                   using {M}arkov chain {M}onte {C}arlo},
  year =          {1996},
}

@article{Heath97,
  author =        {Heath, S.C.},
  journal =       {Am J Hum Genet},
  title =         {Markov chain {M}onte {C}arlo segregation and linkage
                   analysis of oligogenic models},
  year =          {1997},
}

@article{Sillanpaa&Arjas98,
  author =        {Sillanpaa, M.J. and Arjas, E.},
  journal =       {Genetics},
  title =         {Bayesian mapping of multiple quantitative trait loci
                   from incomplete inbred line cross data},
  year =          {1998},
}

@article{Leeetal08,
  author =        {Lee, S.S.F. and L. Sun and R. Kustra and S.B. Bull},
  journal =       {Bioinformatics},
  title =         {{EM}-random forest and new measures of variable
                   importance for multi-locus quantitative trait linkage
                   analysis},
  year =          {2008},
}

@article{Wang&Rose&vanderLaan10,
  author =        {H. Wang and S. Rose and M.J. van der Laan},
  journal =       {Stat Prob Lett},
  title =         {Finding quantitative Trait Loci Genes with
                   Collaborative Targeted Maximum Likelihood Learning},
  volume =        {published online 11 Nov (doi:
                   10.1016/j.spl.2010.11.001)},
  year =          {2010},
}

@techreport{Wang&Rose&vanderLaan11,
  author =        {H. Wang and S. Rose and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  type =          {Technical {R}eport},
  title =         {Targeted Methods for Finding Quantitative Trait Loci},
  year =          {2011},
}

@manual{Basten&Weir&Zeng01,
  author =        {C.J. Basten and B.S. Weir and Z.B. Zeng},
  title =         {QTL Cartographer},
  year =          {2001},
  url =           {http://statgen.ncsu.edu/qtlcart/},
}

@article{Masindeetal01,
  author =        {Masinde, G.L. and X. Li and W. Gu and H. Davidson and
                   S. Mohan and D.J. Baylink},
  journal =       {Genome Res},
  title =         {Identification of wound healing/regeneration
                   quantitative trait loci ({QTL}) at multiple time points
                   that explain seventy percent of variance in ({MRL/MpJ
                   and SJL/J}) mice {F2} population},
  year =          {2001},
}

@article{Boyartchuk01,
  author =        {Boyartchuk, V.L. and K.W. Broman and R.E. Mosher and
                   S.E.F. D'Orazio and M.N. Starnbach and W.F. Dietrich},
  journal =       {Nat Genet},
  title =         {Multigenic control of Listeria monocytogenes
                   susceptibility in mice},
  year =          {2001},
}

@article{Broman03,
  author =        {Broman, K.W.},
  journal =       {Genetics},
  title =         {Mapping quantitative trait loci in the case of a
                   spike in the phenotype distribution},
  year =          {2003},
}

@article{Jin&Fine&Yandell07,
  author =        {Jin, C. and J.P. Fine and B.S. Yandell},
  journal =       {J Am Stat Assoc},
  title =         {A unified semiparametric framework for quantitative
                   trait loci analysis, with application to spike
                   phenotypes},
  year =          {2007},
}

@article{Petersenetal08,
  author =        {M.L. Petersen and M.J. van der Laan and S. Napravnik and
                   J.J. Eron and R.D. Moore and S.G. Deeks},
  journal =       {AIDS},
  number =        {16},
  pages =         {2097--106},
  title =         {Long-term consequences of the delay between virologic
                   failure of highly active antiretroviral therapy and
                   regimen modification},
  volume =        {22},
  year =          {2008},
}

@article{Rodgeretal09,
  author =        {A.J. Rodger and Z. Fox and J.D. Lundgren and
                   J.L. Kuller and C. Boesecke and D. Gey and
                   A. Skoutelis and M.B. Goetz and A.N. Phillips and
                     {INSIGHT Strategies for Management of Antiretroviral
  Therapy (SMART) Study Group}},
  journal =       {J Infect Dis},
  number =        {6},
  pages =         {973--83},
  title =         {Activation and coagulation biomarkers are independent
                   predictors of the development of opportunistic
                   disease in patients with {HIV} infection.},
  volume =        {200},
  year =          {2009},
}

@article{Hammeretal08,
  author =        {S.M. Hammer and J.J. Eron and P. Reiss and
                   R.T. Schooley and M.A. Thompson and S. Walmsley and
                   P. Cahn and M.A. Fischl and J.M. Gatell and
                   M.S. Hirsch and D.M. Jacobsen and J.S.G. Montaner and
                   D.D. Richman and P.G. Yeni and P.A. Volberding},
  journal =       {J Am Med Asoc},
  number =        {5},
  pages =         {555--70},
  title =         {Antiretroviral treatment of adult {HIV} infection:
                   2008 recommendations of the {I}nternational {AIDS}
                   {S}ociety-{USA} panel},
  volume =        {300},
  year =          {2008},
}

@article{Stringeretal06,
  author =        {J.S. Stringer and I. Zulu and J. Levy and
                   E.M. Stringer and A. Mwango and B.H. Chi and
                   V. Mtonga and S. Reid and R.A. Cantrell and
                   M. Bulterys and M.S. Saag and R.G. Marlink and
                   A. Mwinga and T.V. Ellerbrock and M. Sinkala},
  journal =       {J Am Med Asoc},
  number =        {7},
  pages =         {782--93},
  title =         {Rapid scale-up of antiretroviral therapy at primary
                   care sites in {Z}ambia: feasibility and early outcomes},
  volume =        {296},
  year =          {2006},
}

@misc{WHO06,
  author =        {{{W}orld {H}ealth {O}rganization}},
  title =         {Antiretroviral therapy for {HIV} infection in adults
                   and adoloescents: recommendations for a public health
                   approach},
  year =          {2006},
}

@article{Reynoldsetal09,
  author =        {S.J. Reynolds and G. Nakigozi and K. Newell and
                   A. Ndyanabo and R. Galiwongo and I. Boaz and
                   T.C. Quinn and R. Gray and M. Wawer and D. Serwadda},
  journal =       {{AIDS}},
  number =        {6},
  pages =         {697--700},
  title =         {Failure of immunologic criteria to appropriately
                   identify antiretroviral treatment failure in {U}ganda},
  volume =        {23},
  year =          {2009},
}

@article{Petersenetal07,
  author =        {M.L Petersen and S.G. Deeks and J.N. Martin and
                   M.J. van der Laan},
  journal =       {Am J Epidemiol},
  number =        {9},
  pages =         {985--993},
  title =         {History-Adjusted Marginal Structural Models to
                   Estimate Time-Varying Effect Modification},
  volume =        {166},
  year =          {2007},
}

@article{Robins&Hernan&Rotnitzky07,
  author =        {J.M. Robins and M.A. Hernan and A. Rotnitzky},
  journal =       {Am J Epidemiol},
  number =        {9},
  pages =         {994--1002},
  title =         {Effect Modification by Time-varying Covariates},
  volume =        {166},
  year =          {2007},
}

@article{vanderLaan&Petersen&Joffe07,
  author =        {M.J. van der Laan and M.L. Petersen and M.M. Joffe},
  journal =       {Am J Epidemiol},
  number =        {9},
  pages =         {1003--1004},
  title =         {Response to Invited Commentary: {P}etersen et. al.
                   Respond to ``{E}ffect Modification by Time-varying
                   Covariates''},
  volume =        {166},
  year =          {2007},
}

@article{vanderLaan&Petersen07b,
  author =        {M.J. van der Laan and M.L. Petersen},
  journal =       {Int J Biostat},
  number =        {1},
  pages =         {Article 6},
  title =         {Statistical Learning of Origin-Specific Statically
                   Optimal Individualized Treatment Rules.},
  volume =        {3},
  year =          {2007},
}

@article{Petersen&Deeks&vanderLaan07,
  author =        {M.L. Petersen and S.G. Deeks and M.J. van der Laan},
  journal =       {Stat Med},
  number =        {25},
  pages =         {4578--601},
  title =         {Individualized Treatment Rules: generating Candidate
                   Clinical Trials.},
  volume =        {26},
  year =          {2007},
}

@article{vanderLaan&Petersen&Joffe05,
  author =        {M.J. van der Laan and M.L. Petersen and M.M. Joffe},
  journal =       {Int J Biostat},
  number =        {1},
  pages =         {10--20},
  title =         {History-Adjusted Marginal Structural Models and
                   Statically-Optimal Dynamic Treatment Regimens},
  volume =        {1},
  year =          {2005},
}

@article{Hernanetal06,
  author =        {M.A. Hernan and E. Lanoy and D. Costagliola and
                   J.M. Robins},
  journal =       {Basic Clin Pharmacol},
  pages =         {237--242},
  title =         {Comparison of dynamic treatment regimes via inverse
                   probability weighting.},
  volume =        {98},
  year =          {2006},
}

@techreport{vanderLaan08b,
  author =        {M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =          {232},
  title =         {The construction and analysis of adaptive group
                   sequential designs},
  year =          {2008},
}

@article{Boivinetal07,
  author =        {Boivin, J. and Bunting, L. and Collins, J.A. and
                   Nygren, K.G.},
  journal =       {Hum Reproduct},
  pages =        {1506--1512},
  title =         {International estimates of infertility prevalence and
                   treatment-seeking: potential need and demand for
                   infertility medical care},
  volume =        {22},
  year =          {2007},
}

@article{Adamsonetal06,
  author =        {Adamson, G.D. and de {M}ouzon, J. and Lancaster, P. and
                   Nygren, K.-G. and Sullivan, E. and
                   Zegers-Hochschild, F.},
  journal =       {Fertil Steril},
  pages =        {1586--1622},
  title =         {World collaborative report on in vitro fertilization,
                   2000},
  volume =        {85},
  year =          {2006},
}

@article{Soullieretal08,
  author =        {Soullier, N. and Bouyer, J. and Pouly J-L. and
                   Guibert, J. and de la {R}ochebrochard},
  journal =       {Hum Reproduct},
  pages =         {187--192},
  title =         {Estimating the success of an in vitro fertilization
                   programme using multiple imputation},
  volume =        {23},
  year =          {2008},
}

@article{delaRochebrochardetal08,
  author =        {de la {R}ochebrochard, E. and Soullier, N. and
                   Peikrishvili, R. and Guibert, J. and Bouyer, J.},
  journal =       {Int J Gynecol Obstet},
  pages =         {74--75},
  title =         {High in vitro fertilization discontinuation rate in
                   {F}rance},
  volume =        {103},
  year =          {2008},
}

@article{delaRochebrochardetal09,
  author =        {de la {R}ochebrochard, E. and Quelen, C. and
                   Peikrishvili, R. and Guibert, J. and Bouyer, J.},
  journal =       {Fertil Steril},
  pages =         {149--156},
  title =         {Long-term outcome of parenthood project during in
                   vitro fertilization and after discontinuation of
                   unscuccessful in vitro fertilization},
  volume =        {92},
  year =          {2009},
}

@book{Schafer97,
  address =       {London},
  author =        {Schafer, J.L.},
  publisher =     {Chapman \& Hall},
  title =         {Analysis of incomplete multivariate data},
  year =          {1997},
}

@book{Little&Rubin02,
  address =       {Hoboken},
  author =        {Little, R.J.A. and Rubin, Donald B.},
  edition =       {2nd},
  publisher =     {Wiley},
  title =         {Statistical analysis with missing data},
  year =          {2002},
}

@techreport{Yu&vanderLaan02,
  author =        {Z. Yu and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number={122},
  title =         {Construction of counterfactuals and the
                   G-computation formula},
  year =          {2002},
}

@article{Gill&Robins01,
  author =        {Gill, R.D. and Robins, J.M.},
  journal =       {Ann Stat},
  number =        {6},
  pages =         {1785--1811},
  title =         {Causal inference in complex longitudinal studies:
                   continuous case},
  volume =        {29},
  year =          {2001},
}

@techreport{DHHS04,
  author =        {{Department of Health and Human Services}},
  institution =   {Panel on Clinical Practices for Treatment of {HIV}
                   Infection},
type={Technical {R}eport},
  title =         {Guidelines for the use of antiretroviral agents in
                   {HIV}-1 infected adults and adolescents},
  year =          {2004},
}

@article{CDC92,
  author =        {{Centers for Disease Control and Prevention}},
  journal =       {Morbid Mortal W Rep},
  pages =         {1--19},
  title =         {{1993 revised classification system for {HIV} infection
                   and expanded surveillance case definition for AIDS
                   among adolescents and adults}},
  volume =        {41},
  year =          {1992},
}

@incollection{Selbyetal05,
  author =        {J.V. Selby and D.H. Smith and E.S. Johnson and
                   M.A. Raebel and G.D. Friedman and B.H. McFarland},
  booktitle =     {Pharmacoepidemiology},
  editor =        {B.L. Strom},
  publisher =     {Wiley},
  title =         {Kaiser {P}ermanente Medical Care Program},
  year =          {2005},
}

@techreport{Neugebauer&Silverberg&vanderLaan10,
  author =        {R. Neugebauer and M.J. Silverberg and
                   M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  type =          {272},
  title =         {Observational Study and Individualized Antiretroviral
                   Therapy Initiation Rules for Reducing Cancer
                   Incidence in {HIV}-Infected Patients},
  year =          {2010},
}




@techreport{Stitelmanetal11,
  author =        {O.M. Stitelman and V. De Gruttola and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  type =          {Technical {R}eport 281, http://www.bepress.com/ucbbiostat/paper281},
  title =         {A General Implementation of TMLE for Longitudinal Data Applied to Causal Inference in Survival Analysis},
  year =          {2011},
}
@techreport{Stitelman&vanderLaan11,
  author =        {O.M. Stitelman and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  type =          {Technical {R}eport},
  title =         {Targeted Maximum Likelihood Estimation of
                   Time-To-Event Parameters With Time-Dependent
                   Covariates},
  year =          {2011},
}

@article{Thalletal07,
  author =        {P.F. Thall and C. Logothetis and L.C. Pagliaro and
                   S. Wen and M.A. Brown and D. Williams and
                   R.E. Millikan},
  journal =       {J Natl Cancer Inst},
  pages =         {1613--22},
  title =         {Adaptive Therapy for Androgen-Independent Prostate
                   Cancer: a randomized Selection Trial of Four
                   Regimens},
  volume =        {99},
  year =          {2007},
}

@article{Bembom&vanderLaan07a,
  author =        {O. Bembom and M.J. van der Laan},
  journal =       {J Natl Cancer Inst},
  pages =         {1577--1582},
  title =         {Comment: Statistical Methods for analyzing sequentially
                   randomized trials},
  volume =        {99(21)},
  year =          {2007},
}

@techreport{Zheng&vanderLaan10,
  author =        {W. Zheng and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =          {273},
  title =         {Asymptotic Theory for Cross-validated Targeted
                   Maximum Likelihood Estimation},
  year =          {2010},
}

@techreport{Zheng&vanderLaan11,
  author =        {W. Zheng and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =          {288},
  title =         {Targeted Maximum Likelihood Estimation of Natural Direct Effect},
  year =          {2011},
}

@book{Robert07,
  address={Berlin Heidelberg New York},
  author =        {Robert, P.C.},
  publisher =     {Springer},
  title =         {{T}he {B}ayesian choice: from
                   decision-thoeretic foundations to
                   computational implementation},
  year =          {2007},
}

@book{Lindley80,
  address =       {Cambridge, MA},
  author =        {Lindley, D.V.},
  publisher =     {Cambridge},
  title =         {{I}ntroduction to probability and statistics from
                   a {B}ayesian point of view, {P}art 2},
  year =          {1980},
}

@article{Golub06,
  author =        {Golub, H.L.},
  journal =       {Stat Med},
  pages =         {3231--3235},
  title =         {The need for more efficient trial designs},
  volume =        {25},
  year =          {2006},
}

@article{Emerson06,
  author =        {Emerson, S.S.},
  journal =       {Stat Med},
  pages =         {3270--3296},
  title =         {Issues in the use of adaptive clinical trial designs},
  volume =        {25},
  year =          {2006},
}

@book{Hu&Rosenberger06,
address = {New York},
  author =        {F. Hu and W.F. Rosenberger},
  publisher =     {Wiley},
  title =         {The theory of response adaptive randomization in
                   clinical trials},
  year =          {2006},
}

@book{Jennison&Turnbull00,
  address =       {Boca Raton},
  author =        {Jennison, C. and Turnbull, B.W.},
  editor =        {},
  publisher =     {Chapman \& Hall},
  title =         {Group sequential methods with applications to
                   clinical trials},
  year =          {2000},
}

@article{Rosenberger96,
  author =        {W.F. Rosenberger},
  journal =       {Stat Sci},
  number =        {},
  pages =         {137--149},
  title =         {New directions in adaptive designs},
  volume =        {11},
  year =          {1996},
}

@techreport{Chambaz&vanderLaan10,
  author =        {Chambaz, A. and van der Laan, M.J.},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
   number={258},
  title =         {Targeting the optimal design in randomized clinical
                   trials with binary outcomes and no covariate},
  year =          {2010},
}

@article{Rosenberger&Vidyashankar&Agarwal01,
  author =        {Rosenberger, W.F. and Vidyashankar, A.N. and
                   Agarwal, D.K.},
  journal =       {J Biopharm Stat},
  number =        {227--236},
  title =         {Covariate-adjusted response-adaptive designs for
                   binary response},
  volume =        {11},
  year =          {2001},
}

@article{Bandyopadhyay&Biswas01,
  author =        {Bandyopadhyay, U. and Biswas, A.},
  journal =       {Biometrika},
  number =        {2},
  pages =         {409--419},
  title =         {Adaptive designs for normal responses with prognostic
                   factors},
  volume =        {88},
  year =          {2001},
}

@article{Atkinson&Biswas05,
  author =        {Atkinson, A.C. and Biswas, A.},
  journal =       {Stat Med},
  number =        {16},
  pages =         {2477--2492},
  title =         {Adaptive biased-coin designs for skewing the
                   allocation proportion in clinical trials with normal
                   responses},
  volume =        {24},
  year =          {2005},
}

@article{Zhangetal07,
  author =        {Zhang, L.-X. and Hu, F.-F. and Cheung, S.H. and
                   Chan, W.S.},
  journal =       {Ann Stat},
  number =        {3},
  pages =         {1166--1182},
  title =         {Asymptotic properties of covariate-adjusted
                   response-adaptive designs},
  volume =        {35},
  year =          {2007},
}

@article{Zhang&Hu09,
  author =        {Zhang, L.-X. and Hu, F.-F.},
  journal =       {Appl Math J Chinese Univ Ser B},
  number =        {1},
  pages =         {1--13},
  title =         {A new family of covariate-adjusted response adaptive
                   designs and their properties},
  volume =        {24},
  year =          {2009},
}

@article{Shao&Yu&Zhong10,
  author =        {Shao, J. and Yu, X. and Bob Zhong, B.},
  journal =       {Biometrika},
  title =         {A theory for testing hypotheses under
                   covariate-adaptive randomization},
  year =          {2010},
}

@article{Gill89,
  author =        {Gill, R.D.},
  journal =       {Scand J Stat},
  title =         {Non- and semiparametric maximum likelihood estimators
                   and the Von {M}ises method (Part 1)},
  year =          {1989},
}

@article{Tan08,
  author =        {Z. Tan},
  journal =       {Int J Biostat},
  pages =         {Article 10},
  title =         {Comment: {I}mproved Local Efficiency and Double
                   Robustness},
  volume =        {4},
  number={1},
  year =          {2008},
}

@techreport{Gruber&vanderLaan11,
  author =        {S. Gruber and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =        {275},
  type =          {Technical Report},
  title =         {{tmle}: an {R} Package for Targeted Maximum Likelihood
                   Estimation},
  year =          {2011},
}

@proceedings{DBLP:conf/colt/2003,
  booktitle =     {COLT},
  editor =        {B. Sch{\"o}lkopf and M.K. Warmuth},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  series =        {Lecture Notes in Computer Science},
  title =         {Computational Learning Theory and Kernel Machines,
                   16th Annual Conference on Computational Learning
                   Theory and 7th Kernel Workshop, COLT/Kernel 2003,
                   Washington, DC, USA, August 24-27, 2003, Proceedings},
  volume =        {2777},
  year =          {2003},
}

@proceedings{DBLP:conf/nips/2005,
  booktitle =     {NIPS},
  title =         {Advances in Neural Information Processing Systems 18
                   [Neural Information Processing Systems, NIPS 2005,
                   December 5-8, 2005, Vancouver, British Columbia,
                   Canada]},
  year =          {2005},
}

@proceedings{DBLP:conf/colt/2006,
  booktitle =     {COLT},
  editor =        {G. Lugosi and H.-U. Simon},
  publisher =     {Springer},
  series =        {Lecture Notes in Computer Science},
    address={Berlin Heidelberg New York},
  title =         {Learning Theory, 19th Annual Conference on Learning
                   Theory, COLT 2006, Pittsburgh, PA, USA, June 22-25,
                   2006, Proceedings},
  volume =        {4005},
  year =          {2006},
}



@ARTICLE{Diaz11,
title = {Super Learner Based Conditional Density Estimation with Application to Marginal Structural Models},
author = {D\'iaz, Iv\'an and van der Laan, Mark},
year = {2011},
journal = {The International Journal of Biostatistics},
volume = {7},
number = {1},
pages = {38},
}

@article {Diaz12,
author = {Iv\'an D\'iaz and van der Laan, Mark},
title = {Population Intervention Causal Effects Based on Stochastic Interventions},
journal = {Biometrics},
volume = {68},
number = {2},
publisher = {Blackwell Publishing Inc},
issn = {1541-0420},
pages = {541--549},
keywords = {Causal effect, Counterfactual outcome, Double robustness, Stochastic intervention, Targeted maximum likelihood estimation},
year = {2012},
}

@article{Diaz13,
title={Sensitivity Analysis for Causal Inference Under Unmeasured Confounding and Measurement Error Problems},
author={D{\'\i}az, Iv{\'a}n and van der Laan, Mark J},
year= {\noop{2013}In press},
journal={International Journal of Biostatistics}
}

@article{Diaz13,
title={Assessing the Causal Effect of Policies: An Example Using Stochastic Interventions},
author={D{\'\i}az, Iv{\'a}n and van der Laan, Mark J},
year= {\noop{2013}In press},
journal={International Journal of Biostatistics}
}


@incollection{Diaz11a,
year={2011},
isbn={978-1-4419-9781-4},
booktitle={Targeted Learning},
series={Springer Series in Statistics},
title={Targeted Bayesian Learning},
publisher={Springer New York},
author={Iv\'an D\'iaz and Hubbard, Alan E. and van der Laan, Mark J.},
pages={475-493},
language={English}
}

@article{Diaz13,
title={Targeted Data Adaptive Estimation of the Causal Dose Response Curve},
author={D{\'\i}az, Iv{\'a}n and van der Laan, Mark J},
year= {\noop{2013}In press},
journal={Journal of Causal Inference},
}


@ARTICLE{Diaz11,
title = {Super Learner Based Conditional Density Estimation with Application to Marginal Structural Models},
author = {D\'iaz, Iv\'an and van der Laan, Mark},
year = {2011},
journal = {The International Journal of Biostatistics},
volume = {7},
number = {1},
pages = {38},
}

@article {Diaz12,
author = {Iv\'an D\'iaz and van der Laan, Mark},
title = {Population Intervention Causal Effects Based on Stochastic Interventions},
journal = {Biometrics},
volume = {68},
number = {2},
publisher = {Blackwell Publishing Inc},
issn = {1541-0420},
pages = {541--549},
keywords = {Causal effect, Counterfactual outcome, Double robustness, Stochastic intervention, Targeted maximum likelihood estimation},
year = {2012},
}

@article{Diaz13,
title={Sensitivity Analysis for Causal Inference Under Unmeasured Confounding and Measurement Error Problems},
author={D{\'\i}az, Iv{\'a}n and van der Laan, Mark J},
year= {\noop{2013}In press},
journal={International Journal of Biostatistics}
}

@article{Diaz13,
title={Assessing the Causal Effect of Policies: An Example Using Stochastic Interventions},
author={D{\'\i}az, Iv{\'a}n and van der Laan, Mark J},
year= {\noop{2013}In press},
journal={International Journal of Biostatistics}
}


@incollection{Diaz11a,
year={2011},
isbn={978-1-4419-9781-4},
booktitle={Targeted Learning},
series={Springer Series in Statistics},
title={Targeted Bayesian Learning},
publisher={Springer New York},
author={Iv\'an D\'iaz and Hubbard, Alan E. and van der Laan, Mark J.},
pages={475-493},
language={English}
}

@article{Diaz13,
title={Targeted Data Adaptive Estimation of the Causal Dose Response Curve},
author={D{\'\i}az, Iv{\'a}n and van der Laan, Mark J},
year= {\noop{2013}In press},
journal={Journal of Causal Inference},
}


@ARTICLE{Diaz11,
title = {Super Learner Based Conditional Density Estimation with Application to Marginal Structural Models},
author = {D\'iaz, Iv\'an and van der Laan, Mark},
year = {2011},
journal = {The International Journal of Biostatistics},
volume = {7},
number = {1},
pages = {38},
}

@article {Diaz12,
author = {Iv\'an D\'iaz and van der Laan, Mark},
title = {Population Intervention Causal Effects Based on Stochastic Interventions},
journal = {Biometrics},
volume = {68},
number = {2},
publisher = {Blackwell Publishing Inc},
issn = {1541-0420},
pages = {541--549},
keywords = {Causal effect, Counterfactual outcome, Double robustness, Stochastic intervention, Targeted maximum likelihood estimation},
year = {2012},
}

@article{Diaz13,
title={Sensitivity Analysis for Causal Inference Under Unmeasured Confounding and Measurement Error Problems},
author={D{\'\i}az, Iv{\'a}n and van der Laan, Mark J},
year= {\noop{2013}In press},
journal={International Journal of Biostatistics}
}

@article{Diaz13,
title={Assessing the Causal Effect of Policies: An Example Using Stochastic Interventions},
author={D{\'\i}az, Iv{\'a}n and van der Laan, Mark J},
year= {\noop{2013}In press},
journal={International Journal of Biostatistics}
}


@incollection{Diaz11a,
year={2011},
isbn={978-1-4419-9781-4},
booktitle={Targeted Learning},
series={Springer Series in Statistics},
title={Targeted Bayesian Learning},
publisher={Springer New York},
author={Iv\'an D\'iaz and Hubbard, Alan E. and van der Laan, Mark J.},
pages={475-493},
language={English}
}

@article{Diaz13,
title={Targeted Data Adaptive Estimation of the Causal Dose Response Curve},
author={D{\'\i}az, I. and van der Laan, M. J.},
year= {2013},
journal={Journal of Causal Inference},
volume={1},
number={2},
pages={171--192},
}



@ARTICLE{Diaz11,
title = {Super Learner Based Conditional Density Estimation with Application to Marginal Structural Models},
author = {D\'iaz, Iv\'an and van der Laan, Mark},
year = {2011},
journal = {The International Journal of Biostatistics},
volume = {7},
number = {1},
pages = {38},
}

@article {Diaz12,
author = {Iv\'an D\'iaz and van der Laan, Mark},
title = {Population Intervention Causal Effects Based on Stochastic Interventions},
journal = {Biometrics},
volume = {68},
number = {2},
publisher = {Blackwell Publishing Inc},
issn = {1541-0420},
pages = {541--549},
keywords = {Causal effect, Counterfactual outcome, Double robustness, Stochastic intervention, Targeted maximum likelihood estimation},
year = {2012},
}

@article{Diaz13,
title={Sensitivity Analysis for Causal Inference Under Unmeasured Confounding and Measurement Error Problems},
author={D{\'\i}az, Iv{\'a}n and van der Laan, Mark J},
year= {\noop{2013}In press},
journal={International Journal of Biostatistics}
}

@article{Diaz13,
title={Assessing the Causal Effect of Policies: An Example Using Stochastic Interventions},
author={D{\'\i}az, Iv{\'a}n and van der Laan, Mark J},
year= {\noop{2013}In press},
journal={International Journal of Biostatistics}
}


@incollection{Diaz11a,
year={2011},
isbn={978-1-4419-9781-4},
booktitle={Targeted Learning},
series={Springer Series in Statistics},
title={Targeted Bayesian Learning},
publisher={Springer New York},
author={Iv\'an D\'iaz and Hubbard, Alan E. and van der Laan, Mark J.},
pages={475-493},
language={English}
}

@article{Diaz13,
title={Targeted Data Adaptive Estimation of the Causal Dose Response Curve},
author={D{\'\i}az, Iv{\'a}n and van der Laan, Mark J},
year= {\noop{2013}In press},
journal={Journal of Causal Inference},
}
%% This BibTeX bibliography file was created using BibDesk.
%% http://bibdesk.sourceforge.net/


%% Created for Laura Balzer at 2012-08-26 21:21:41 -0700


%% Saved with string encoding Unicode (UTF-8)

@article{Chambaz&vanderLaan11a,
Title={Targeting The Optimal Design In Randomized Clinical Trials With Binary Outcomes And No Covariate, Theoretical Study},	Author = {A. Chambaz and M.J. van der Laan},
	Journal = {Int J Biostat},
	Note = {Working paper 258, www.bepress.com/ucbbiostat},
	Number = {1},
	Pages = {1-32},
	Volume = {7},
	Year = {2011}}

	@article{Chambaz&vanderLaan11b,
Title={Targeting The Optimal Design In Randomized Clinical Trials With Binary Outcomes And No Covariate, Simulation Study},	Author = {A. Chambaz and M.J. van der Laan},
	Journal = {Int J Biostat},
	Note = {Working paper 258,www.bepress.com/ucbbiostat},
	Number = {1},
	Pages = {33-},
	Volume = {7},
	Year = {2011}}


@article{Dawid&Didelez10,
Title={Identifying the consequences of dynamic treatment strategies: A decision theoretic overview},
Author = {A. Dawid and V. Didelez},
	Journal = {Statistics Surveys},
	Note = {},
	Number = {4},
	Pages = {184--231},
	Volume = {},
	Year = {2010}}

@inproceedings{Polley2009,
	Address = {Boca Raton},
	Author = {E.C. Polley and M.J. van der Laan},
	Booktitle = {Design and Analysis Clinical Trials with Time-to-Event Endpoints},
	Date-Added = {2012-08-26 20:23:48 -0700},
	Date-Modified = {2012-08-26 20:25:05 -0700},
	Editor = {Karl E. Peace},
	Keywords = {App},
	Publisher = {Chapman \& Hall/CRC},
	Title = {Selecting Optimal Treatments Based on Predictive Factors},
	Year = {2009}}

@article{Arnold2009,
	Author = {B. Arnold and B. Arana and D. M\"{a}usezahl and A. Hubbard and J.M. Colford},
	Date-Added = {2012-08-26 20:07:08 -0700},
	Date-Modified = {2012-08-26 20:08:37 -0700},
	Journal = {Int J Biostat},
	Note = {PMCID: PMC2786251},
	Number = {6},
	Pages = {1651-1661},
	Title = {Evaluation of a pre-existing, 3-year household water treatment and handwashing intervention in rural Guatemala},
	Volume = {38},
	Year = {2009}}

@article{Odden2011,
	Author = {M.C. Odden and I.B. Tager and M.J. van der Laan and J.A Delaney and C.A. Peralta and R. Katz and M.J. Sarnak and B.M. Psaty and M.G. Shlipak},
	Date-Added = {2012-08-26 20:00:36 -0700},
	Date-Modified = {2012-08-26 20:02:31 -0700},
	Journal = {Int J Biostat},
	Keywords = {App},
	Note = {PMCID: PMC3204667},
	Number = {1},
	Pages = {Article 34},
	Title = {Antihypertensive medication use and change in kidney function in elderly adults: a marginal structural model analysis},
	Volume = {7},
	Year = {2011}}

@unpublished{Josh2012,
	Author = {M. Petersen and J. Schwab and M. van der Laan},
	Date-Added = {2012-08-26 16:32:16 -0700},
	Date-Modified = {2012-08-26 21:08:43 -0700},
	Note = {Unpublished, Division of Biostatistics, University of California, Berkeley},
	Title = {Estimating the impact of clinic-based interventions},
	Year = {2012}}

@book{Bickel1993,
	Address = {Baltimore},
	Author = {Bickel, P.J. and Klaassen, C.A.J. and Ritov, Y. and Wellner, J.A.},
	Date-Added = {2012-08-26 15:53:44 -0700},
	Date-Modified = {2012-08-26 15:55:11 -0700},
	Keywords = {book},
	Publisher = {Johns Hopkins University Press},
	Title = {{Efficient and Adaptive Estimation for Semiparametric Models}},
	Year = {1993}}

@article{Rosenblum2011,
	Author = {M. Rosenblum and M.J. van der Laan},
	Date-Added = {2012-08-26 01:25:31 -0700},
	Date-Modified = {2012-08-26 01:30:42 -0700},
	Journal = {Biometrika},
	Number = {4},
	Pages = {845--860},
	Title = {Optimizing randomized trial designs to distinguish which subpopulations benefit from treatment},
	Volume = {98},
	Year = {2011}}

@unpublished{Geeven2012,
	Author = {G. Geeven and M.J. van der Laan and M.C.M. de Gunst},
	Date-Added = {2012-08-26 01:09:47 -0700},
	Date-Modified = {2012-08-26 21:05:35 -0700},
	Keywords = {unpub},
	Note = {Unpublished, Division of Biostatistics, University of California, Berkeley},
	Title = {Comparison of targeted maximum likelihood and shrinkage estimators of parameters in gene networks},
	Year = {2012}}

@unpublished{Brooks2012,
	Author = {J. Brooks and M.J. van der Laan},
	Date-Added = {2012-08-26 01:08:46 -0700},
	Date-Modified = {2012-08-26 21:05:29 -0700},
	Note = {Unpublished, Division of Biostatistics, University of California, Berkeley},
	Title = {Targeted Maximum Likelihood Estimation for Prediction Calibration},
	Year = {2012}}

@article{Tuglus2011,
	Author = {C. Tuglus and M.J. van der Laan},
	Date-Added = {2012-08-26 00:51:25 -0700},
	Date-Modified = {2012-08-26 00:52:39 -0700},
	Journal = {Stat Appl Genet Mol Biol},
	Keywords = {App},
	Note = {PMCID: PMC3122882},
	Number = {1},
	Pages = {Article 2},
	Title = {Repeated measures semiparametric regression using targeted maximum likelihood methodology with application to transcription factor activity discovery},
	Volume = {10},
	Year = {2011}}

@article{Wang2011,
	Author = {H. Wang and M.J. van der Laan},
	Date-Added = {2012-08-26 00:41:51 -0700},
	Date-Modified = {2012-08-26 00:42:47 -0700},
	Journal = {BMC Bioinformatics},
	Keywords = {App},
	Note = {PMCID: PMC3166941},
	Number = {312},
	Title = {Dimension Reduction Procedure Using Targeted Variable Importance Measurement},
	Volume = {12},
	Year = {2011}}

@article{Moore2011,
	Author = {K.L. Moore and R. Neugebauer and T. Valappil and M.J. van der Laan},
	Date-Added = {2012-08-26 00:17:52 -0700},
	Date-Modified = {2012-08-26 00:19:34 -0700},
	Journal = {Stat Med},
	Note = {PMID: 21751231},
	Number = {19},
	Pages = {2389--2408},
	Title = {Robust extraction of covariate information to improve estimation efficiency in randomized trials},
	Volume = {30},
	Year = {2011}}

@article{Chaffee2012,
	Author = {P.H. Chaffee and M.J. van der Laan},
	Date-Added = {2012-08-25 23:46:42 -0700},
	Date-Modified = {2012-08-25 23:47:53 -0700},
	Journal = {Int J Biostat},
	Keywords = {Simulation},
	Note = {PMID: 22740582},
	Number = {1},
	Pages = {Article 14},
	Title = {Targeted maximum likelihood estimation for dynamic treatment regimes in sequentially randomized controlled trials},
	Volume = {8},
	Year = {2012}}

@article{Atkinson2010,
	Author = {R.W. Atkinson and G.W. Fuller and H.R. Anderson and R.M. Harrison and B. Armstrong},
	Date-Added = {2012-08-25 22:10:07 -0700},
	Date-Modified = {2012-08-25 22:11:33 -0700},
	Journal = {Epidemiology},
	Keywords = {Aim3},
	Note = {PMID: 20502338},
	Number = {4},
	Pages = {501-511},
	Title = {Urban ambient particle metrics and health:a time-series analysis},
	Volume = {21},
	Year = {2010}}

@article{Catalano2006,
	Author = {R. Catalano and T. Bruckner and A.R. Marks and B. Eskenazi},
	Date-Added = {2012-08-25 22:03:01 -0700},
	Date-Modified = {2012-08-25 22:04:09 -0700},
	Journal = {Hum Reprod},
	Keywords = {Aim3},
	Note = {PMID: 16936298},
	Number = {12},
	Pages = {3127-3131},
	Title = {Exogenous shocks to the human sex ratio: the case of {S}eptember 11, 2001 in {N}ew {Y}ork {C}ity},
	Volume = {21},
	Year = {2006}}

@article{Eskenazi2007,
	Author = {B. Eskenazi and A.R. Marks and R. Catalano and T. Bruckner and P.G. Toniolo},
	Date-Added = {2012-08-25 21:57:52 -0700},
	Date-Modified = {2012-08-25 21:59:23 -0700},
	Journal = {Hum Reprod},
	Keywords = {Aim3},
	Number = {11},
	Pages = {3013-3020},
	Title = {Low birthweight in {N}ew {Y}ork {C}ity and upstate {N}ew {Y}ork following the events of {S}eptember 11th},
	Volume = {22},
	Year = {2007}}

@article{Diaz&vanderLaan12,
	Author = {I. Diaz and M.J. van der Laan},
	Date-Added = {},
	Date-Modified = {},
	Journal = {Biometrics, to appear},
	Keywords = {},
	Number = {},
	Pages = {},
	Title = {Population intervention causal effects based on stochastic interventions},
	Volume = {},
	Year = {2012}}

@article{Imbens2007,
	Author = {G.W. Imbens and T. Lemieux},
	Date-Added = {2012-08-25 21:48:32 -0700},
	Date-Modified = {2012-08-25 21:55:33 -0700},
	Journal = {J Econom},
	Keywords = {Aim3},
	Number = {2},
	Pages = {615--635},
	Title = {Regression discontinuity designs: {A} guide to practice},
	Volume = {142},
	Year = {2008}}

@article{Imbens2009,
	Author = {G.W. Imbens and J.M. Wooldridge},
	Date-Added = {2012-08-25 20:46:14 -0700},
	Date-Modified = {2012-08-25 20:46:57 -0700},
	Journal = {J Econ Lit},
	Keywords = {Aim3},
	Number = {1},
	Pages = {5-86},
	Title = {Recent Developments in the Econometrics of Program Evaluation},
	Volume = {47},
	Year = {2009}}

@article{Sobel2006,
	Author = {M.E. Sobel},
	Date-Added = {2012-08-25 17:38:58 -0700},
	Date-Modified = {2012-08-26 20:36:23 -0700},
	Journal = {J Am Stat Assoc Asoc},
	Keywords = {Aim2},
	Number = {476},
	Pages = {1398--1407},
	Title = {What Do Randomized Studies of Housing Mobility Demonstrate?: {C}ausal inference in the face of interference},
	Volume = {101},
	Year = {2006}}

@article{Hong2006,
	Author = {G. Hong and S.W. Raudenbush},
	Date-Added = {2012-08-25 17:31:23 -0700},
	Date-Modified = {2012-08-25 17:49:36 -0700},
	Journal = {J Am Stat Assoc},
	Keywords = {Aim2},
	Number = {475},
	Pages = {901--910},
	Title = {Evaluating Kindergarten Retention Policy: {A} Case Study of Causal Inference for Multilevel Observational Data},
	Volume = {101},
	Year = {2006}}

@article{Halloran&Struchiner95,
	Author = {M.E. Halloran and C.J. Struchiner},
	Date-Added = {2012-08-25 17:27:15 -0700},
	Date-Modified = {2012-08-25 17:28:57 -0700},
	Journal = {Epidemiology},
	Keywords = {Aim2},
	Note = {PMID: 7742400},
	Number = {2},
	Pages = {142-151},
	Title = {Causal inference in infectious diseases},
	Volume = {6},
	Year = {1995}}

@article{Hudgens&Halloran08,
	Author = {M.G. Hudgens and M.E. Halloran},
	Date-Added = {2012-08-25 15:30:45 -0700},
	Date-Modified = {2012-08-25 15:32:14 -0700},
	Journal = {J Am Stat Assoc},
	Keywords = {Aim2},
	Note = {PMCID: PMC2600548},
	Number = {482},
	Pages = {832--842},
	Title = {Toward {C}ausal {I}nference {W}ith {I}nterference},
	Volume = {103},
	Year = {2008},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAZgAAAAAAZgAAgAADE1hY2ludG9zaCBIRAAAAAAAAAAAAAAAAAAAAMobz/1IKwAABsaXyhAyMDA4X0h1ZGdlbnMucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAHSNyEzF6XmgAAAAAAAAAAAAEAAgAACSAAAAAAAAAAAAAAAAAAAAAKTGl0ZXJhdHVyZQAQAAgAAMocMm0AAAARAAgAAMxe+goAAAABABAGxpfKAAxX9QAMUlIAAAAeAAIAPE1hY2ludG9zaCBIRDpVc2VyczpsYXVyYTpEZXNrdG9wOkxpdGVyYXR1cmU6MjAwOF9IdWRnZW5zLnBkZgAOACIAEAAyADAAMAA4AF8ASAB1AGQAZwBlAG4AcwAuAHAAZABmAA8AGgAMAE0AYQBjAGkAbgB0AG8AcwBoACAASABEABIAL1VzZXJzL2xhdXJhL0Rlc2t0b3AvTGl0ZXJhdHVyZS8yMDA4X0h1ZGdlbnMucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAeLi4vTGl0ZXJhdHVyZS8yMDA4X0h1ZGdlbnMucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAjwCPgJDAkwCVwJbAmkCcAJ5ApoCnwKiAq8CtAAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAALG}}

@article{Tchetgen&vanderWeele12,
	Author = {E.J. {Tchetgen Tchetgen} and T.J. VanderWeele},
	Date-Added = {2012-08-25 15:28:32 -0700},
	Date-Modified = {2012-08-25 17:48:19 -0700},
	Journal = {Stat Meth Med Res},
	Keywords = {Aim2},
	Note = {PMID: 21068053},
	Number = {1},
	Pages = {55-75},
	Title = {On causal inference in the presence of interference},
	Volume = {21},
	Year = {2012}}

@article{vanderWeeleetal12,
	Author = {T.J. VanderWeele and J.P. Vandenbrouke and E.J. {Tchetgen Tchetgen} and J.M. Robins},
	Date-Added = {2012-08-25 13:41:16 -0700},
	Date-Modified = {2012-08-25 17:52:19 -0700},
	Journal = {Epidemiology},
	Keywords = {Aim2},
	Note = {PMID: 22317812},
	Number = {3},
	Pages = {285--292},
	Title = {A mapping between interactions and interference: implications for vaccine trials},
	Volume = {23},
	Year = {2012},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAagAAAAAAagAAgAADE1hY2ludG9zaCBIRAAAAAAAAAAAAAAAAAAAAMobz/1IKwAABsaXyhQyMDEyX1ZhbmRlcldlZWxlLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAHSPAnzF6GJQAAAAAAAAAAAAEAAgAACSAAAAAAAAAAAAAAAAAAAAAKTGl0ZXJhdHVyZQAQAAgAAMocMm0AAAARAAgAAMxe6JUAAAABABAGxpfKAAxX9QAMUlIAAAAeAAIAQE1hY2ludG9zaCBIRDpVc2VyczpsYXVyYTpEZXNrdG9wOkxpdGVyYXR1cmU6MjAxMl9WYW5kZXJXZWVsZS5wZGYADgAqABQAMgAwADEAMgBfAFYAYQBuAGQAZQByAFcAZQBlAGwAZQAuAHAAZABmAA8AGgAMAE0AYQBjAGkAbgB0AG8AcwBoACAASABEABIAM1VzZXJzL2xhdXJhL0Rlc2t0b3AvTGl0ZXJhdHVyZS8yMDEyX1ZhbmRlcldlZWxlLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QIi4uL0xpdGVyYXR1cmUvMjAxMl9WYW5kZXJXZWVsZS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACTAJOAlMCXAJnAmsCeQKAAokCrgKzArYCwwLIAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAto=}}

@book{Fitzmaurice2004,
	Address = {Hoboken},
	Author = {G.M. Fitzmaurice and N.M. Laird and J.H. Ware},
	Date-Added = {2012-08-25 13:17:30 -0700},
	Date-Modified = {2012-08-25 13:20:50 -0700},
	Keywords = {book},
	Publisher = {John Wiley \& Sons},
	Title = {Applied {L}ongitudinal {A}nalysis},
	Year = {2004}}

@booklet{UNAIDS,
	Address = {Johannesburg, Republic of South Africa},
	Author = {{UNAIDS RST-ESA}},
	Date-Added = {2012-08-24 17:33:29 -0700},
	Date-Modified = {2012-08-24 17:42:29 -0700},
	Keywords = {HIV},
	Note = {Avaliable at \url{http://www.unaidsrstesa.org/media-corner/factsheets/high-level-meeting-aids-implication-estern-and-southern-africa}},
	Title = {High level meeting on {AIDS}: {I}mplication for {E}aster and {S}outhern {A}frica},
	Year = {2012},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAX4AAAAAAX4AAgAADE1hY2ludG9zaCBIRAAAAAAAAAAAAAAAAAAAAMobz/1IKwAABq+JbwpVTkFJRFMucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAHRmOizF1rYQAAAAAAAAAAAAEAAgAACSAAAAAAAAAAAAAAAAAAAAAJR3JhbnQyMDEyAAAQAAgAAMocMm0AAAARAAgAAMxdzdEAAAABABAGr4lvAAxX9QAMUlIAAAAeAAIANU1hY2ludG9zaCBIRDpVc2VyczpsYXVyYTpEZXNrdG9wOkdyYW50MjAxMjpVTkFJRFMucGRmAAAOABYACgBVAE4AQQBJAEQAUwAuAHAAZABmAA8AGgAMAE0AYQBjAGkAbgB0AG8AcwBoACAASABEABIAKFVzZXJzL2xhdXJhL0Rlc2t0b3AvR3JhbnQyMDEyL1VOQUlEUy5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdFpVTkFJRFMucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAiICJAIpAjICPQJBAk8CVgJfAmoCbwJyAn8ChAAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKW}}

@conference{Zheng2011community,
	Address = {Ann Habor, MI},
	Author = {W. Zheng and M.J. van der Laan and M.L. Petersen},
	Booktitle = {Atlantic Causal Inference Conference},
	Date-Added = {2012-08-24 14:08:26 -0700},
	Date-Modified = {2012-08-24 14:11:36 -0700},
	Keywords = {Community},
	Title = {Causal inference for community based studies with few communities},
	Year = {2011}}

@conference{Balzer2012wnar,
	Address = {Fort Collins, CO},
	Author = {L. Balzer and M. Petersen and J. Schwab and M. van der Laan},
	Booktitle = {WNAR},
	Date-Added = {2012-08-24 11:58:45 -0700},
	Date-Modified = {2012-08-24 12:04:14 -0700},
	Keywords = {community},
	Title = {Estimating the impact of community-level interventions: {T}he {SEARCH} {T}rial and {HIV} {P}revention in {S}ub-{S}aharan {A}frica},
	Year = {2012}}

@incollection{Chpt24,
	Address = {New York Dordrecht Heidelberg London},
	Author = {M.L. Petersen and M.J. van der Laan},
	Booktitle = {Targeted Learning: Causal Inference for Observational and Experimental Data},
	Date-Added = {2012-08-24 11:01:37 -0700},
	Date-Modified = {2012-08-24 11:02:54 -0700},
	Editor = {van der Laan, M.J. and Rose, S.},
	Keywords = {Chpt4},
	Publisher = {Springer},
	Title = {Case {S}tudy: {L}ongitudinal {HIV} {C}ohort {D}ata},
	Year = {2011}}

@incollection{vanderLaan2012sl,
	Address = {New York Dordrecht Heidelberg London},
	Author = {M.J. van der Laan and M.L. Petersen},
	Booktitle = {{Ensemble Machine Learning}},
	Date-Added = {2012-08-24 10:43:01 -0700},
	Date-Modified = {2012-08-24 10:50:07 -0700},
	Editor = {C. Zhang and Y. Ma},
	Keywords = {Superlearner},
	Publisher = {Springer},
	Title = {Targeted {L}earning},
	Year = {2012}}

@incollection{Chpt6,
	Address = {New York Dordrecht Heidelberg London},
	Author = {S. Rose and M.J. van der Laan},
	Booktitle = {Targeted Learning: Causal Inference for Observational and Experimental Data},
	Date-Added = {2012-08-24 10:19:20 -0700},
	Date-Modified = {2012-08-24 10:20:25 -0700},
	Editor = {van der Laan, M.J. and Rose, S.},
	Keywords = {Chpt6},
	Publisher = {Springer},
	Title = {Why {TMLE}?},
	Year = {2011}}

@techreport{Pearl2010transport,
	Author = {J. Pearl and E. Bareinboim},
	Date-Added = {2012-08-24 09:47:13 -0700},
	Date-Modified = {2012-08-24 09:48:55 -0700},
	Institution = {Computer Science Department, University of California, Los Angeles},
	Keywords = {Other},
	Number = {R-372},
	Title = {Transportability across studies: {A} formal approach},
	Url = {ftp://www.mmss.cs.ucla.edu/pub/stat_ser/r372.pdf},
	Year = {2012},
	Bdsk-Url-1 = {ftp://www.mmss.cs.ucla.edu/pub/stat_ser/r372.pdf}}

@article{VanderWeele2009,
	Author = {T.J. VanderWeele},
	Date-Added = {2012-08-23 18:19:15 -0700},
	Date-Modified = {2012-08-23 18:20:15 -0700},
	Journal = {Epidemiology},
	Keywords = {Aim2},
	Note = {PMID: 19234398},
	Number = {1},
	Pages = {18-26},
	Title = {Marginal structural models for the estimation of direct and indirect effects},
	Volume = {20},
	Year = {2009}}

@article{Petersen2006b,
	Author = {M.L. Petersen and S.E. Sinisi and M.J. van der Laan},
	Date-Added = {2012-08-23 18:16:52 -0700},
	Date-Modified = {2012-08-23 18:18:16 -0700},
	Journal = {Epidemiology},
	Keywords = {Aim2},
	Note = {PMID: 16617276},
	Number = {3},
	Pages = {276--284},
	Title = {Estimation of direct causal effects},
	Volume = {17},
	Year = {2006}}

@article{Cain2010,
	Author = {L.E. Cain and J.M. Robins and E. Lanoy and R. Logan and D. Costagliola and M.A. Hern\'{a}n},
	Date-Added = {2012-08-23 18:13:50 -0700},
	Date-Modified = {2012-08-26 21:02:08 -0700},
	Journal = {Int J Biostat},
	Keywords = {Aim1},
	Note = {PMCID: PMC3406513},
	Number = {2},
	Pages = {Article 18},
	Title = {When to start treatment? {A} systematic approach to the comparison of dynamic regimes using observational data},
	Volume = {6},
	Year = {2010}}

@article{Hernan2009b,
	Author = {M.A. Hern\'{a}n and J.M. Robins},
	Date-Added = {2012-08-23 18:07:50 -0700},
	Date-Modified = {2012-08-23 18:09:24 -0700},
	Journal = {N Engl J Med},
	Keywords = {Aim1},
	Note = {PMID: 19701984},
	Number = {8},
	Pages = {823--824},
	Title = {{Comment on: Early versus deferred antiretroviral therapy for HIV on survival}},
	Volume = {361},
	Year = {2009}}

@article{Kitahata2009,
	Date-Added = {2012-08-23 18:04:16 -0700},
	Date-Modified = {2012-08-23 18:05:43 -0700},
	Journal = {N Engl J Med},
	Keywords = {Aim1},
	Note = {PMCID: PMC2854555},
	Number = {18},
	Pages = {1815--1826},
	Title = {{Effect of early versus deferred antiretroviral therapy for HIV on survival}},
	Volume = {360},
	Year = {2009}}

@article{Bodnar2004,
	Author = {L.M. Bodnar and M. Davidian and A.M. Siega-Riz and A.A. Tsiatis},
	Date-Added = {2012-08-23 18:00:22 -0700},
	Date-Modified = {2012-08-23 18:00:22 -0700},
	Journal = {Am J Epidemiol},
	Keywords = {Aim1},
	Note = {PMID: 15128604},
	Number = {10},
	Pages = {926--934},
	Title = {{Marginal Structural Models for Analyzing Causal Effects of Time-dependent Treatments: An Application in Perinatal Epidemiology}},
	Volume = {159},
	Year = {2004}}

@article{Hernan2009,
	Author = {M.A. Hern\'{a}n and S.R. Cole},
	Date-Added = {2012-08-23 17:31:04 -0700},
	Date-Modified = {2012-08-23 17:32:34 -0700},
	Journal = {Am J Epidemiol},
	Keywords = {Roadmap},
	Note = {PMCID: PMC2765368},
	Number = {8},
	Pages = {959--962 with discussion 963-963},
	Title = {{Invited Commentary: Causal diagrams and measurement bias}},
	Volume = {170},
	Year = {2009}}

@incollection{Robins2009,
	Address = {Boca Raton, FL},
	Author = {J.M. Robins and M.A. Hern\'{a}n},
	Booktitle = {{Longitudinal Data Analysis}},
	Chapter = {23},
	Date-Added = {2012-08-23 17:26:46 -0700},
	Date-Modified = {2012-08-23 17:43:10 -0700},
	Editor = {G. Fitzmaurice and M. Davidian and G. Verbeke and G. Molenberghs},
	Keywords = {Aim2},
	Publisher = {Chapman \& Hall/CRC},
	Title = {{Estimation of the causal effects of time-varying exposures}},
	Year = {2009}}

@article{Hernan2006b,
	Author = {M.A. Hern\'{a}n and J.M. Robins},
	Date-Added = {2012-08-23 17:07:52 -0700},
	Date-Modified = {2012-08-23 17:09:25 -0700},
	Journal = {J Epidemiol Community Health},
	Keywords = {Aim2},
	Note = {PMCID: PMC2652882},
	Number = {7},
	Pages = {578--586},
	Title = {Estimating causal effects from epidemiological data},
	Volume = {60},
	Year = {2006}}

@article{Munoz2011,
	Annote = {DOI: 10.2202/1557-4679.1356},
	Author = {I. D\'{i}az Munoz and M.J. van der Laan},
	Date-Added = {2012-08-23 16:58:00 -0700},
	Date-Modified = {2012-08-26 21:03:47 -0700},
	Journal = {Int J Biostat},
	Keywords = {Superlearner},
	Note = {PMID: 22718677},
	Pages = {Article 38},
	Title = {Super learner based conditional density estimation with application to marginal structural models},
	Volume = {7},
	Year = {2011}}

@article{Houssaini2012,
	Author = {A. Houssa\"{i}ni and L. Assoumou and A.G. Marcelin and J.M. Calvez and P. Flandre},
	Date-Added = {2012-08-23 16:54:44 -0700},
	Date-Modified = {2012-08-23 16:57:15 -0700},
	Journal = {AIDS Res Treat},
	Keywords = {Superlearner},
	Note = {PMCID: PMC3324131},
	Number = {Article ID 478467},
	Pages = {Epub},
	Title = {{Investigation of Super Learner Methodology on HIV-1 Small Sample: Application on Jaguar Trial Data}},
	Volume = {2012},
	Year = {2012}}

@article{Sinisi2007,
	Annote = {. doi:  10.2202/1544-6115.1240},
	Author = {S.E. Sinisi and E.C. Polley and M.L. Petersen and M.J. van der Laan},
	Date-Added = {2012-08-23 14:06:15 -0700},
	Date-Modified = {2012-08-23 16:51:18 -0700},
	Journal = {Stat Appl Genet Mol},
	Keywords = {Superlearner},
	Note = {PMCID: PMC2473869},
	Number = {Article 7},
	Pages = {Epub},
	Read = {0},
	Title = {{Super learning: an application to the prediction of HIV-1 drug resistance}},
	Volume = {6},
	Year = {2007}}

@article{Petersen2006,
	Author = {M.L. Petersen and Y. Wang and M.J. van der Laan and D.R. Bangsberg},
	Date-Added = {2012-08-23 13:56:04 -0700},
	Date-Modified = {2012-08-23 14:04:00 -0700},
	Journal = {J Acquir Immune Defic Syndr},
	Keywords = {Aim1},
	Note = {PMID: 17133209},
	Number = {Suppl 1},
	Pages = {S96--S103},
	Title = {{Assessing the effectiveness of antiretroviral adherence interventions. Using marginal structural models to replicate the findings of randomized controlled trials}},
	Volume = {43},
	Year = {2006}}

@article{Hernan2004,
	Author = {M.A. Hern\'{a}n and S. Hern\'{a}ndez-D\'{i}az and J.M. Robins},
	Date-Added = {2012-08-23 10:56:44 -0700},
	Date-Modified = {2012-08-23 10:58:39 -0700},
	Journal = {Epidemiology},
	Keywords = {Roadmap},
	Note = {PMID: 15308962},
	Number = {5},
	Pages = {615--625},
	Title = {A structural approach to selection bias},
	Volume = {15},
	Year = {2004}}

@article{Robins1999,
	Author = {J.M. Robins},
	Date-Added = {2012-08-23 10:53:51 -0700},
	Date-Modified = {2012-08-23 10:55:18 -0700},
	Journal = {Synthese},
	Keywords = {Roadmap + MSM},
	Number = {1-2},
	Pages = {151-179},
	Title = {{Association, Causation, and Marginal Structural Models}},
	Volume = {121},
	Year = {1999}}

@article{Greenland1999,
	Author = {S. Greenland and J. Pearl and J.M. Robins},
	Date-Added = {2012-08-23 10:33:03 -0700},
	Date-Modified = {2012-08-23 10:34:19 -0700},
	Journal = {Epidemiology},
	Keywords = {Roadmap},
	Note = {PMID: 9888278},
	Number = {1},
	Pages = {37--48},
	Title = {Causal diagrams for empirical research.},
	Volume = {10},
	Year = {1999}}

@article{Pearl2009b,
	Author = {J. Pearl},
	Date-Added = {2012-08-23 10:29:27 -0700},
	Date-Modified = {2012-08-26 20:45:51 -0700},
	Journal = {Statist Surv},
	Keywords = {Roadmap},
	Pages = {96--146},
	Title = {{Causal inference in statistics: An overview}},
	Volume = {3},
	Year = {2009},
	Bdsk-Url-1 = {http://www.i-journals.org/ss/viewarticle.php?id=57}}

@incollection{GreenlandPearl2007,
	Address = {Thousand Oaks},
	Author = {S. Greenland and J. Pearl},
	Booktitle = {Encyclopedia of Epidemiology},
	Date-Added = {2012-08-23 10:11:07 -0700},
	Date-Modified = {2012-08-26 20:45:23 -0700},
	Editor = {S. Boslaugh},
	Keywords = {Roadmap},
	Pages = {149--156},
	Publisher = {SAGE Publications},
	Title = {Causal Diagrams},
	Volume = {1},
	Year = {2007}}

@incollection{Pearl2012,
	Address = {New York},
	Annote = {Technical report available at ftp://pike.cs.ucla.edu/pub/stat_ser/r370.pdf},
	Author = {J. Pearl},
	Booktitle = {Handbook of Structural Equation Modeling},
	Chapter = {5},
	Date-Added = {2012-08-23 09:41:04 -0700},
	Date-Modified = {2012-08-26 20:46:32 -0700},
	Editor = {R. Hoyle},
	Institution = {Computer Science Department, University of California, Los Angeles},
	Keywords = {Roadmap},
	Pages = {68--91},
	Publisher = {Guilford Press},
	Title = {The Causal Foundations of Structural Equation Modeling},
	Volume = {R-370},
	Year = {2012}}

@article{Lighthouse2012,
	Annote = {http://www.ncbi.nlm.nih.gov/pubmed/22808948},
	Author = {C. Feldacker and H. Tweya and O. Keiser and R. Weigel and M. Kalulu and L. Fenner and M. Egger and E. Manda and J.B. Mwafilaso and C. Kamba and S. Phiri},
	Date-Added = {2012-08-22 22:26:03 -0700},
	Date-Modified = {2012-08-22 22:29:06 -0700},
	Journal = {Trop Med Int Health},
	Keywords = {HIV},
	Note = {PMID: 22808948},
	Title = {{Characteristics of adults and children diagnosed with tuberculosis in Lilongwe, Malawi: findings from an integrated HIV/TB clinic}},
	Volume = {Epub ahead of print},
	Year = {2012}}

@conference{LREC2010,
	Address = {Presentation \# THAE0305, Vienna, Austria},
	Author = {K. Wools-Kaloustian and R. Kosgei and S. Kimaiyo and P. Braitstein and E. Sang and B. Musick and C. Yiannoutsos and A. Siika},
	Booktitle = {{XVIII International AIDS Conference}},
	Date-Added = {2012-08-22 22:21:13 -0700},
	Date-Modified = {2012-08-26 20:35:11 -0700},
	Keywords = {HIV},
	Title = {{Low risk express care: A nurse-centered model for the management of stable patients on combination antiretroviral therapy (cART)}},
	Year = {2010}}

@article{Young2011,
	Author = {J.G. Young and L.E. Cain and J.M. Robins and E.J. O'Reilly and M.A. Hern\'{a}n},
	Date-Added = {2012-08-22 22:11:06 -0700},
	Date-Modified = {2012-08-26 20:34:12 -0700},
	Journal = {Stat Biosci},
	Keywords = {Aim1},
	Pages = {119-143},
	Title = {Comparative Effectiveness of Dynamic Treatment Regimes: An Application of the Parametric G-Formula},
	Volume = {3},
	Year = {2011}}

@article{Taubman2009,
	Author = {S.L. Taubman and J.M. Robins and M.A. Mittleman and M.A. Hern\'{a}n},
	Date-Added = {2012-08-22 21:46:33 -0700},
	Date-Modified = {2012-08-22 22:09:34 -0700},
	Journal = {Int J Epidemiol},
	Keywords = {Aim1},
	Note = {PMCID: PMC2786249},
	Number = {6},
	Pages = {1599--1611},
	Title = {Intervening on risk factors for coronary heart disease: an application of the parametric g-formula},
	Volume = {38},
	Year = {2009}}

@article{Cain2011,
	Author = {{HIV-CAUSAL Collaboration} and L.E. Cain and R. Logan and J.M. Robins and J.A. Sterne and C. Sabin and L. Bansi and A. Justice and J. Goulet and A. van Sighem and F. de Wolf and H.C. Bucher and V. von Wyl and A. Esteve and J. Casabona and J. del Amo and S. Moreno and R. Seng and L. Meyer and S. Perez-Hoyos and R. Muga and S. Lodi and E. Lanoy and D. Costagliola and M.A. Hern\'{a}n},
	Date-Added = {2012-08-22 21:36:52 -0700},
	Date-Modified = {2012-08-22 21:43:12 -0700},
	Journal = {Ann Intern Med},
	Keywords = {Aim1},
	Note = {PMID: 21502648},
	Number = {8},
	Pages = {509-515},
	Title = {{When to initiate combined antiretroviral therapy to reduce mortality and AIDS-defining illness in HIV-infected persons in developed countries: an observational study}},
	Volume = {154},
	Year = {2011}}

@article{DART2010,
	Author = {{DART Trial Team}},
	Date-Added = {2012-08-22 21:23:22 -0700},
	Date-Modified = {2012-08-22 21:24:46 -0700},
	Journal = {Lancet},
	Keywords = {HIV},
	Note = {PMCID: PMC280572},
	Number = {9709},
	Pages = {123-131},
	Title = {{Routine versus clinically driven laboratory monitoring of HIV antiretroviral therapy in Africa (DART): a randomised non-inferiority trial}},
	Volume = {375},
	Year = {2010}}

@conference{Saag2012,
	Address = {Paper \#87, Seattle, WA},
	Author = {M. Saag and A. Westfall and D. Luhanga and P. Mulenga and B. Chi and L. Mulenga and R. Cantrell and A. Mwango and J. Koethe and J. Stringer},
	Booktitle = {CROI},
	Date-Added = {2012-08-22 21:18:33 -0700},
	Date-Modified = {2012-08-26 20:32:56 -0700},
	Keywords = {HIV},
	Title = {A Cluster Randomized Trial of Routine vs Discretionary Viral Load Monitoring among Adults Starting {ART}: {Z}ambia.},
	Year = {2012}}

@article{Cohen2011,
	Author = {M.S. Cohen and Y.Q. Chen and M. McCauley and T. Gamble and M.C. Hosseinipour and N. Kumarasamy and J.G. Hakim and J. Kumwenda and B. Grinsztejn and J.H. Pilotto and S.V. Godbole and S. Mehendale and S. Chariyalertsak and B.R. Santos and K.H. Mayer and I.F. Hoffman and S.H. Eshleman and E. Piwowar-Manning and L. Wang and J. Makhema and L.A. Mills and G. de Bruyn and I. Sanne and J. Eron and J. Gallant and D. Havlir and S. Swindells and H. Ribaudo and V. Elharrar and D. Burns and T.E. Taha and K. Nielsen-Saines and D. Celentano and M. Essex and T.R. Fleming},
	Date-Added = {2012-08-22 11:31:09 -0700},
	Date-Modified = {2012-08-22 21:04:10 -0700},
	Journal = {N Engl J Med},
	Keywords = {HIV},
	Note = {PMCID: PMC3200068},
	Number = {6},
	Pages = {493-505},
	Title = {{Prevention of HIV-1 infection with early antiretroviral therapy}},
	Volume = {365},
	Year = {2011}}

@article{Green2008,
	Author = {L.W. Green},
	Date-Added = {2012-08-22 11:23:38 -0700},
	Date-Modified = {2012-08-22 11:25:49 -0700},
	Journal = {Fam Pract},
	Keywords = {HIV},
	Note = {PMID: 18794201},
	Number = {Suppl1},
	Pages = {i20-i24},
	Title = {{Making research relevant: if it is an evidence-based practice, where's the practice-based evidence?}},
	Volume = {25},
	Year = {2006}}

@article{Jamshidian2011,
	Author = {F. Jamshidian and A.E. Hubbard and N.P. Jewell},
	Date-Added = {2012-08-22 09:29:55 -0700},
	Date-Modified = {2012-08-26 21:04:37 -0700},
	Journal = {Stat Meth Med Res},
	Keywords = {Application},
	Note = {PMID: 21908418},
	Title = {Accounting for perception, placebo and unmasking effects in estimating treatment effects in randomised clinical trials},
	Year = {2011},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAagAAAAAAagAAgAADE1hY2ludG9zaCBIRAAAAAAAAAAAAAAAAAAAAMobz/1IKwAABsaXyhQyMDExXyBKYW1zaGlkaWFuLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAHPD5UzFpW1AAAAAAAAAAAAAEAAgAACSAAAAAAAAAAAAAAAAAAAAAKTGl0ZXJhdHVyZQAQAAgAAMocMm0AAAARAAgAAMxauUQAAAABABAGxpfKAAxX9QAMUlIAAAAeAAIAQE1hY2ludG9zaCBIRDpVc2VyczpsYXVyYTpEZXNrdG9wOkxpdGVyYXR1cmU6MjAxMV8gSmFtc2hpZGlhbi5wZGYADgAqABQAMgAwADEAMQBfACAASgBhAG0AcwBoAGkAZABpAGEAbgAuAHAAZABmAA8AGgAMAE0AYQBjAGkAbgB0AG8AcwBoACAASABEABIAM1VzZXJzL2xhdXJhL0Rlc2t0b3AvTGl0ZXJhdHVyZS8yMDExXyBKYW1zaGlkaWFuLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QIi4uL0xpdGVyYXR1cmUvMjAxMV8gSmFtc2hpZGlhbi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACTAJOAlMCXAJnAmsCeQKAAokCrgKzArYCwwLIAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAto=}}

@article{Gruber2012,
	Author = {S. Gruber and M.J. van der Laan},
	Date-Added = {2012-08-22 09:24:55 -0700},
	Date-Modified = {2012-08-24 13:51:01 -0700},
	Journal = {Int J Biostat},
	Keywords = {TMLE},
	Note = {PMID: 22628356},
	Number = {1},
	Pages = {Article 11},
	Title = {Targeted minimum loss based estimator that outperforms a given estimator},
	Volume = {8},
	Year = {2012}}

@incollection{HubbardJewellvanderLaan11,
	Address = {New York Dordrecht Heidelberg London},
	Author = {A.E. Hubbard and N.P. Jewell and M.J. van der Laan},
	Booktitle = {Targeted Learning: Causal Inference for Observational and Experimental Data},
	Date-Added = {2012-08-22 09:17:35 -0700},
	Date-Modified = {2012-08-22 09:20:29 -0700},
	Editor = {van der Laan, M.J. and Rose, S.},
	Keywords = {Chpt8},
	Publisher = {Springer},
	Title = {{Direct Effects and Effect Among the Treated}},
	Year = {2011}}

@incollection{MunozHubbardVdL11,
	Address = {New York Dordrecht Heidelberg London},
	Author = {I.D. Mu\~{n}oz and M. van der Laan},
	Booktitle = {Targeted Learning: Causal Inference for Observational and Experimental Data},
	Date-Added = {2012-08-22 09:14:07 -0700},
	Date-Modified = {2012-08-22 09:15:41 -0700},
	Editor = {van der Laan, M.J. and Rose, S.},
	Keywords = {Chpt28},
	Publisher = {Springer},
	Title = {{Targeted Bayesian Learning}},
	Year = {2011}}

@article{Hubbard2010,
	Author = {A.E. Hubbard and J. Ahern and N.L. Fleischer and M. van der Laan and S.A. Lippman and N. Jewell and T. Bruckner and W.A. Satariano},
	Date-Added = {2012-08-22 08:50:55 -0700},
	Date-Modified = {2012-08-24 10:10:42 -0700},
	Journal = {Epidemiology},
	Keywords = {Community},
	Note = {PMID: 20220526},
	Number = {4},
	Pages = {467-474},
	Title = {To {GEE} or Not to {GEE} Comparing Population Average and Mixed Models for Estimating the Associations Between Neighborhood Risk Factors and Health},
	Volume = {21},
	Year = {2010}}

@article{Oakes2004,
	Author = {J.M. Oakes},
	Date-Added = {2012-08-22 08:48:00 -0700},
	Date-Modified = {2012-08-22 08:49:35 -0700},
	Journal = {Soc Sci Med},
	Keywords = {Community},
	Note = {PMID: 15020009},
	Number = {10},
	Pages = {1929-1952},
	Title = {The (mis)estimation of neighborhood effects: causal inference for a practicable social epidemiology (with discussion)},
	Volume = {58},
	Year = {2004}}

@article{LiangZeger86,
	Author = {K.Y. Liang and S.L. Zeger},
	Date-Added = {2012-08-22 08:41:06 -0700},
	Date-Modified = {2012-08-22 08:46:50 -0700},
	Journal = {Biometrika},
	Keywords = {Community},
	Number = {1},
	Pages = {13-22},
	Title = {{Longitudinal Data Analysis Using Generalized Linear Models}},
	Url = {http://www.jstor.org/stable/2336267},
	Volume = {73},
	Year = {1986},
	Bdsk-Url-1 = {http://www.jstor.org/stable/2336267}}

@article{LairdWare82,
	Author = {N.M. Laird and J.H. Ware},
	Date-Added = {2012-08-22 08:37:25 -0700},
	Date-Modified = {2012-08-22 08:47:14 -0700},
	Journal = {Biometrics},
	Keywords = {Community},
	Note = {PMID: 7168798},
	Number = {4},
	Pages = {963--974},
	Title = {Random-effects models for longitudinal data},
	Volume = {38},
	Year = {1982}}

@article{ZegerLiangAlbert88,
	Author = {S.L. Zeger and K.Y. Liang and P.S. Albert},
	Date-Added = {2012-08-22 08:35:18 -0700},
	Date-Modified = {2012-08-22 08:46:59 -0700},
	Journal = {Biometrics},
	Keywords = {Community},
	Note = {PMID: 3233245},
	Number = {4},
	Pages = {1049-1060},
	Title = {Models for longitudinal data: a generalized estimating equation approach},
	Volume = {44},
	Year = {1988}}

@article{Wester2012,
	Author = {C.W. Wester and O.M. Stitelman and V. De Gruttola and H. Bussmann and R.G. Marlink and M.J. van der Laan},
	Date-Added = {2012-08-22 08:27:34 -0700},
	Date-Modified = {2012-08-26 21:00:48 -0700},
	Journal = {AIDS Res Hum Retroviruses},
	Keywords = {Application},
	Note = {PMID: 22309114},
	Number = {9},
	Pages = {781-788},
	Title = {Effect Modification by Sex and Baseline {CD4}(+) Cell Count Among Adults Receiving Combination Antiretroviral Therapy in {B}otswana: Results from a Clinical Trial},
	Volume = {28},
	Year = {2012}}

@manual{tmlePackage,
	Author = {S. Gruber and M. van der Laan},
	Date-Added = {2012-08-22 07:17:24 -0700},
	Date-Modified = {2012-08-26 21:18:22 -0700},
	Keywords = {R tmle},
	Note = {R package version 1.2.0-1, Available at \url{http://cran.r-project.org/web/packages/tmle/tmle.pdf}},
	Title = {{Targeted Maximum Likelihood Estimation}},
	Year = {2012}}

@manual{SuperLearnerPackage,
	Author = {E. Polley and M. van der Laan},
	Date-Added = {2012-08-22 07:14:31 -0700},
	Date-Modified = {2012-08-26 21:16:59 -0700},
	Keywords = {Superlearner},
	Note = {R package version 2.0-6, Available at \url{http://cran.r-project.org/web/packages/SuperLearner/SuperLearner.pdf}},
	Title = {{Super Learner Prediction}},
	Year = {2012},
	Bdsk-Url-1 = {http://cran.r-project.org/web/packages/SuperLearner/SuperLearner.pdf}}

@techreport{vanderLaan&Petersen12b,
	Author = {M.J. van der Laan, L. Balzer and M.L. Petersen},
	Date-Added = {2012-08-21 19:16:35 -0700},
	Date-Modified = {2012-08-26 21:15:43 -0700},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Keywords = {Allocation},
	Note = {Available at \url{http://biostats.bepress.com/ucbbiostat/paper296/}},
	Number = {296},
	Title = {Randomized Trials and Observational Studies in which Treatment Allocation Depends on the Baseline Characteristics of all Sampled Units},
	Year = {2012}}

@article{Munoz2012,
	Author = {I. D\'{i}az Munoz and M. van der Laan},
	Date-Added = {2012-08-21 19:12:50 -0700},
	Date-Modified = {2012-08-26 20:59:07 -0700},
	Journal = {Biometrics},
	Keywords = {Stochastic},
	Note = {PMID: 21977966},
	Number = {2},
	Pages = {541-549},
	Title = {Population Intervention Causal Effects Based on Stochastic Interventions},
	Volume = {68},
	Year = {2012}}

@inproceedings{Didelezetal06,
	Address = {Cambridge, MA},
	Author = {V. Didelez and A.P. Dawid and S. Geneletti},
	Booktitle = {{Proceedings of the 22nd Annual Conference on Uncertainty in Artificial Intelligence}},
	Date-Added = {2012-08-21 19:09:44 -0700},
	Date-Modified = {2012-08-26 21:14:54 -0700},
	Keywords = {Stochastic},
	Pages = {138--146},
	Title = {{Direct and Indirect Effects of Sequential Treatments}},
	Year = {2006}}

@techreport{Zheng&vanderLaan12,
	Author = {W. Zheng and M.J. van der Laan},
	Date-Added = {2012-08-21 19:05:33 -0700},
	Date-Modified = {2012-08-26 21:11:53 -0700},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Keywords = {NDE-long},
	Note = {Available at \url{http://biostats.bepress.com/ucbbiostat/paper295/}},
	Number = {295},
	Title = {Causal Mediation in a Survival Setting with Time-Dependent Mediators},
	Year = {2012}}

@article{Zheng2012,
	Author = {W. Zheng and M.J. van der Laan},
	Date-Added = {2012-08-21 19:02:52 -0700},
	Date-Modified = {2012-08-26 01:05:10 -0700},
	Journal = {Int J Biostat},
	Keywords = {NDE},
	Note = {PMID: 22499725},
	Number = {1},
	Pages = {1--40},
	Title = {Targeted maximum likelihood estimation for natural direct effects},
	Volume = {8},
	Year = {2012}}

@article{Schnitzer2012,
	Author = {M.E. Schnitzer and E.E. Moodie and R.W. Platt},
	Date-Added = {2012-08-21 18:59:59 -0700},
	Date-Modified = {2012-08-26 21:01:32 -0700},
	Journal = {Biostatistics},
	Keywords = {tmle},
	Note = {PMID: 22797173},
	Title = {Targeted maximum likelihood estimation for marginal time-dependent treatment effects under density misspecification},
	Year = {2012}}

@article{vanderLaan&Gruber12,
	Author = {M.J. van der Laan and S. Gruber},
	Date-Added = {2012-08-21 18:54:29 -0700},
	Date-Modified = {2012-08-24 11:33:54 -0700},
	Journal = {Int J Biostat},
	Keywords = {TMLE},
	Note = {PMID: 22611591},
	Number = {1},
	Title = {Targeted minimum loss based estimation of causal effects of multiple time point interventions},
	Volume = {8},
	Year = {2012},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAawAAAAAAawAAgAADE1hY2ludG9zaCBIRAAAAAAAAAAAAAAAAAAAAMobz/1IKwAABsaXyhUyMDEyX3ZkTFRvd2VyVE1MRS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAHO3ATzFpBoQAAAAAAAAAAAAEAAgAACSAAAAAAAAAAAAAAAAAAAAAKTGl0ZXJhdHVyZQAQAAgAAMocMm0AAAARAAgAAMxapBEAAAABABAGxpfKAAxX9QAMUlIAAAAeAAIAQU1hY2ludG9zaCBIRDpVc2VyczpsYXVyYTpEZXNrdG9wOkxpdGVyYXR1cmU6MjAxMl92ZExUb3dlclRNTEUucGRmAAAOACwAFQAyADAAMQAyAF8AdgBkAEwAVABvAHcAZQByAFQATQBMAEUALgBwAGQAZgAPABoADABNAGEAYwBpAG4AdABvAHMAaAAgAEgARAASADRVc2Vycy9sYXVyYS9EZXNrdG9wL0xpdGVyYXR1cmUvMjAxMl92ZExUb3dlclRNTEUucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfECMuLi9MaXRlcmF0dXJlLzIwMTJfdmRMVG93ZXJUTUxFLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAJQAlICVwJgAmsCbwJ9AoQCjQKzArgCuwLIAs0AAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAC3w==}}

@article{Porter2011,
	Author = {K.E. Porter and S. Gruber and M.J. van der Laan and J.S. Sekhon},
	Date-Added = {2012-08-21 18:45:58 -0700},
	Date-Modified = {2012-08-24 10:56:49 -0700},
	Journal = {Int J Biostat},
	Keywords = {TMLE},
	Note = {PMCID: PMC3173607},
	Number = {1},
	Pages = {Article 31},
	Title = {The relative performance of targeted maximum likelihood estimators},
	Volume = {7},
	Year = {2011},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAZQAAAAAAZQAAgAADE1hY2ludG9zaCBIRAAAAAAAAAAAAAAAAAAAAMobz/1IKwAABsaXyg8yMDEwX1BvcnRlci5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAHOgUYzFmHbQAAAAAAAAAAAAEAAgAACSAAAAAAAAAAAAAAAAAAAAAKTGl0ZXJhdHVyZQAQAAgAAMocMm0AAAARAAgAAMxZ6d0AAAABABAGxpfKAAxX9QAMUlIAAAAeAAIAO01hY2ludG9zaCBIRDpVc2VyczpsYXVyYTpEZXNrdG9wOkxpdGVyYXR1cmU6MjAxMF9Qb3J0ZXIucGRmAAAOACAADwAyADAAMQAwAF8AUABvAHIAdABlAHIALgBwAGQAZgAPABoADABNAGEAYwBpAG4AdABvAHMAaAAgAEgARAASAC5Vc2Vycy9sYXVyYS9EZXNrdG9wL0xpdGVyYXR1cmUvMjAxMF9Qb3J0ZXIucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi9MaXRlcmF0dXJlLzIwMTBfUG9ydGVyLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAI4AjoCPwJIAlMCVwJlAmwCdQKVApoCnQKqAq8AAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACwQ==}}

@article{Gruber2012ctmle,
	Author = {S. Gruber and M.J. van der Laan},
	Date-Added = {2012-08-21 18:30:43 -0700},
	Date-Modified = {2012-08-24 11:27:09 -0700},
	Journal = {Stat Meth Med Res},
	Keywords = {TMLE},
	Note = {PMID: 22368176},
	Title = {Consistent causal effect estimation under dual misspecification and implications for confounder selection procedures},
	Year = {2012}}

@article{Moore2012,
	Author = {K.L. Moore and R. Neugebauer and M.J. van der Laan and I.B. Tager},
	Date-Added = {2012-08-21 18:06:06 -0700},
	Date-Modified = {2012-08-22 22:16:22 -0700},
	Journal = {Stat Med},
	Keywords = {Aim1},
	Note = {PMID: 22362629},
	Number = {13},
	Pages = {1380--1404},
	Title = {Causal inference in epidemiological studies with strong confounding},
	Volume = {31},
	Year = {2012}}

@incollection{GruberVanderLaan2011,
	Address = {New York Dordrecht Heidelberg London},
	Author = {S. Gruber and M.J. van der Laan},
	Booktitle = {Targeted Learning: Causal Inference for Observational and Experimental Data},
	Date-Added = {2012-08-21 17:57:04 -0700},
	Date-Modified = {2012-08-22 07:57:20 -0700},
	Editor = {van der Laan, M.J. and Rose, S.},
	Keywords = {Chpt19},
	Publisher = {Springer},
	Title = {{C-TMLE of an Additive Point Treatment Effect}},
	Year = {2011}}

@article{Moodie2011,
	Author = {E.E. Moodie and D.A. Stephens},
	Date-Added = {2012-08-21 17:46:11 -0700},
	Date-Modified = {2012-08-23 17:34:11 -0700},
	Journal = {Int J Public Health},
	Keywords = {Aim1},
	Note = {PMID: 20931349},
	Number = {1},
	Pages = {117-119},
	Title = {{Marginal Structural Models: unbiased estimation for longitudinal studies}},
	Volume = {56},
	Year = {2011}}

@unpublished{Balzer2012,
	Author = {L.B. Balzer and M.L. Petersen and M.J. van der Laan},
	Date-Added = {2012-08-21 17:40:53 -0700},
	Date-Modified = {2012-08-26 21:05:25 -0700},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Keywords = {Superlearner},
	Note = {Unpublished, Division of Biostatistics, University of California, Berkeley},
	Title = {Adaptive estimation with few independent units},
	Year = {2012}}

@incollection{Rosenblum11,
	Address = {New York Dordrecht Heidelberg London},
	Author = {M. Rosenblum},
	Booktitle = {Targeted Learning: Causal Inference for Observational and Experimental Data},
	Date-Added = {2012-08-21 17:37:05 -0700},
	Date-Modified = {2012-08-22 08:12:21 -0700},
	Editor = {van der Laan, M.J. and Rose, S.},
	Keywords = {Chpt9},
	Publisher = {Springer},
	Title = {{Marginal Structural Models}},
	Year = {2011}}

@incollection{Chpt10,
	Address = {New York Dordrecht Heidelberg London},
	Author = {M.L. Petersen and K.E. Porter and S. Gruber and Y. Wang and M.J. van der Laan},
	Booktitle = {Targeted Learning: Causal Inference for Observational and Experimental Data},
	Date-Added = {2012-08-21 17:34:18 -0700},
	Date-Modified = {2012-08-24 11:19:47 -0700},
	Editor = {van der Laan, M.J. and Rose, S.},
	Keywords = {Chpt10},
	Publisher = {Springer},
	Title = {Positivity},
	Year = {2011}}

@incollection{Chpt3,
	Address = {New York Dordrecht Heidelberg London},
	Author = {E.C. Polley and S. Rose and M.J. van der Laan},
	Booktitle = {Targeted Learning: Causal Inference for Observational and Experimental Data},
	Date-Added = {2012-08-21 17:32:12 -0700},
	Date-Modified = {2012-08-24 12:09:45 -0700},
	Editor = {van der Laan, M.J. and Rose, S.},
	Keywords = {Chpt3},
	Publisher = {Springer},
	Title = {{Super Learner}},
	Year = {2011}}

@unpublished{Petersen&vanderLaan12,
	Author = {M.L. Petersen and M.J. van der Laan},
	Date-Added = {2012-08-21 17:22:48 -0700},
	Date-Modified = {2012-08-26 20:39:05 -0700},
	Keywords = {Roadmap},
	Note = {Unpublished, Division of Biostatistics, University of California, Berkeley},
	Title = {A General Roadmap for the Estimation of Causal Effects},
	Year = {2012}}

@article{Gsponer2012,
	Author = {T. Gsponer and M. Petersen and M. Egger and S. Phiri and M.H. Maathuis and P. Musondad and H. Tweya and K. Peter and B.H. Chi and O. Keiser and {IeDEA Southern Africa}},
	Date-Added = {2012-08-21 17:15:06 -0700},
	Date-Modified = {2012-08-24 11:58:18 -0700},
	Journal = {{AIDS}},
	Keywords = {HIV},
	Note = {PMID: 22089376},
	Number = {1},
	Pages = {57--65},
	Title = {{The causal effect of switching to second-line ART in programmes without access to routine viral load monitoring}},
	Volume = {36},
	Year = {2012}}

@book{Hernan&Robins13,
	Author = {M.A. Hern\'{a}n and J.M. Robins},
	Date-Added = {2012-08-21 17:06:54 -0700},
	Date-Modified = {2012-08-26 20:30:31 -0700},
	Keywords = {Book},
	Note = {Unpublished},
	Publisher = {Chapman \& Hall/CRC},
	Title = {{Causal Inference}},
	Year = {2012}}

@article{Petersen2012,
	Author = {M.L. Petersen and K.E. Porter and S. Gruber and Y. Wang and M.J. van der Laan},
	Date-Added = {2012-08-21 16:51:22 -0700},
	Date-Modified = {2012-08-22 22:15:34 -0700},
	Journal = {Stat Meth Med Res},
	Keywords = {Aim1},
	Note = {PMID: 21030422},
	Number = {1},
	Pages = {31--54},
	Title = {Diagnosing and responding to violations in the positivity assumption},
	Volume = {21},
	Year = {2012}}

@book{Donner&Klar00,
	Address = {London},
	Author = {A. Donner and N. Klar},
	Date-Modified = {2012-08-22 08:06:45 -0700},
	Keywords = {Community},
	Publisher = {Arnold},
	Title = {Design and Analysis of Cluster Randomization Trials in Health Research},
	Year = {2000}}

@book{Hayes2009,
	Address = {Boca Raton},
	Author = {R.J. Hayes and L.H. Moulton},
	Date-Modified = {2012-08-25 22:52:13 -0700},
	Publisher = {Chapman \& Hall/CRC},
	Title = {Cluster Randomized Trials},
	Year = {2009}}

@book{vanderLaanRose2011,
	Address = {New York Dordrecht Heidelberg London},
	Author = {M.J. van der Laan and S. Rose},
	Date-Modified = {2012-08-22 21:07:34 -0700},
	Keywords = {Book},
	Publisher = {Springer},
	Title = {{Targeted Learning: Causal Inference for Observational and Experimental Data}},
	Year = {2011}}

@book{Murray98,
	Address = {Oxford},
	Author = {D.M. Murray},
	Date-Modified = {2012-08-22 08:09:26 -0700},
	Keywords = {Community},
	Publisher = {Oxford University Press},
	Title = {Design and Analysis of Community Randomized Trials},
	Year = {1998}}

@article{Campbell&Donner&Klar07,
	Author = {M.J. Campbell and A. Donner and N. Klar},
	Journal = {Statistics in Medicine},
	Pages = {2--19, doi: 10.1002/sim.2731},
	Title = {Developments in cluster randomized trials and statistics in medicine},
	Volume = {26},
	Year = {2007}}

@article{Klar&Donner97,
	Author = {N. Klar and A. Donner},
	Date-Modified = {2012-08-22 08:08:30 -0700},
	Journal = {Statistics in Medicine},
	Keywords = {Community},
	Pages = {1753--1764},
	Title = {The merits of matching in community intervention trials: a cautionary tale},
	Volume = {16(15)},
	Year = {1997}}

@article{Raudenbush&Martinez&Spybrook07,
	Author = {S.W. Raudenbush and A. Martinez and J. Spybrook},
	Journal = {Educational Evaluation and Policy Analysis},
	Pages = {5--29},
	Title = {Developments in cluster randomized trials and statistics in medicine},
	Volume = {29},
	Year = {2007}}

@article{Freedman&Green&Byar90,
	Author = {L.S. Freedman and S.B. Green and D.P. Byar},
	Journal = {Statistics in Medicine},
	Pages = {943--952},
	Title = {Assessing the gain in efficiency due to matching in a community intervention study},
	Volume = {9},
	Year = {1990}}

@article{Freedmanetal97,
	Author = {L. Freedman and M. Gail and S. Green and D. Corle},
	Journal = {Controlled clinical trials},
	Pages = {131--139, doi:10.1016/S0197-2456(96)00115-8},
	Title = {The efficiency of the matched-pairs design of the community intervention trial for smoking cessation (COMMIT)},
	Volume = {18(2)},
	Year = {1997}}

@article{Toftageretal11,
	Author = {M. Toftager and L.B. Christiansen and P.L. Kristensen and J. Troelsen},
	Journal = {BMC Public Health},
	Pages = {711--777},
	Title = {SPACE for physical activity-a multicomponent intervention study: study design and baseline findings from a cluster randomized controlled trial},
	Volume = {10},
	Year = {2011}}

@article{Koetheetal10,
	Author = {J.R. Koethe and A.O. Westfall and D.K. Luhanga and G.M. Clark and J.D. Goldman and P.L Mulenga and R.A. Cantrell and B.H. Chi and I. Zulu and M.S. Saag and J. S. Stringer},
	Journal = {PlLoS One},
	Pages = {5(3):e9680},
	Title = {A cluster randomized trial of routine HIV-1 viral load monitoring in Zambia},
	Volume = {5},
	Year = {2010}}

@article{Watsonetal04,
	Author = {L. Watson and R. Small and S. Brown and W. Dawson and J. Lumley},
	Journal = {Journal of Controlled Clinical Trials},
	Pages = {235--250},
	Title = {Mounting a community-randomized trial: sample size, matching, selection, and randomization issues in PRISM},
	Volume = {3},
	Year = {2004}}

@article{Gailetal92,
	Author = {M.H. Gail and D.P. Byar and T.F. Pechacek and D.K. Corle},
	Journal = {Controlled clinical trials},
	Pages = {6-21},
	Title = {Aspects of statistical design for the community intervention trial for smoking cessation},
	Volume = {13},
	Year = {1992}}

@article{Commit91,
	Author = {COMMIT Research Group},
	Journal = {Journal of National Cancer Institute},
	Pages = {1620-1628},
	Title = {Summary of design and intervention},
	Volume = {83(22)},
	Year = {1991}}

@article{Imai&King&Nall09,
	Author = {Kosuke Imai and G. King and C. Nall},
	Journal = {Statistical Science},
	Pages = {29--53},
	Title = {The essential role of pair matching in cluster randomized experiments with applicationto the Mexican Universal Health Insurance Evaluation},
	Volume = {24 (1)},
	Year = {2009}}

@article{Imai08,
	Author = {K. Imai},
	Journal = {Statistics in Medicine},
	Pages = {4857--4873},
	Title = {Variance identification and efficiency analysis in randomized experiments under the matched-pair design},
	Volume = {27(24)},
	Year = {2008}}

@techreport{vanderLaan2011,
	Author = {M.J. van der Laan and S. Gruber},
	Date-Modified = {2012-08-26 20:48:45 -0700},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Keywords = {TMLE},
	Note = {Available at \url{http://www.bepress.com/ucbbiostat/paper290}; To appear in Int J. Biostat},
	Number = {290},
	Title = {Targeted Minimum Loss Based Estimation of an Intervention Specific Mean Outcome},
	Year = {2011}}

@techreport{vanderLaan08,
	Author = {M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Note = {http://www.bepress.com/ucbbiostat/paper234},
	Number = {232},
	Title = {The construction and analysis of adaptive group sequential designs},
	Year = {2008}}

@techreport{Balzer&Petersen&vanderLaan12,
	Author = {L.B. Balzer and M.L. Petersen and M.J. van der Laan},
	Date-Modified = {2012-08-21 17:14:20 -0700},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Note = {Under Review at Statistics in Medicine; Technical report available at http://www.bepress.com/ucbbiostat/paper294},
	Number = {294},
	Title = {{Why Match in Individually and Cluster Randomized Trials?}},
	Year = {2012}}

@incollection{Marschak53,
	Address = {New York},
	Author = {J. Marschak},
	Booktitle = {Economic measurements for policy and prediction},
	Editor = {W.~C. Hood and T.~C. Koopmans},
	Publisher = {Wiley},
	Title = {Studies in econometric method},
	Year = {1953}}

@article{Heckman00,
	Author = {J. Heckman},
	Journal = {Q J Econ},
	Pages = {45--97},
	Title = {Causal parameters and policy analysis in economics: A twentieth century retrospective.},
	Volume = {115},
	Year = {2000}}

@article{Gruber2010,
	Author = {S. Gruber and M.J. van der Laan},
	Date-Modified = {2012-08-26 00:48:08 -0700},
	Journal = {Int J BiostatBiostatistics},
	Keywords = {App},
	Note = {PMCID: PMC3126669},
	Number = {1},
	Pages = {Article 26},
	Title = {A Targeted Maximum Likelihood Estimator of a Causal Effect on a Bounded Continuous Outcome},
	Volume = {6},
	Year = {2010}}

@article{Heckman10,
	Author = {J. Heckman},
	Journal = {J Econ Lit},
	Pages = {356--398},
	Title = {Building bridges between structural and program evaluation approaches to evaluating policy.},
	Volume = {48},
	Year = {2010}}

@article{Bang&Robins05,
	Author = {H. Bang and J.M. Robins},
	Journal = {Biometrics},
	Pages = {962--972},
	Title = {Doubly robust estimation in missing data and causal inference models},
	Volume = {61},
	Year = {2005}}

@book{Pearson11,
	Address = {London},
	Author = {K. Pearson},
	Edition = {3rd},
	Publisher = {Black},
	Title = {Grammar of science},
	Year = {1911}}

@article{Rubin74,
	Author = {Donald B. Rubin},
	Journal = {J Educ Psychol},
	Pages = {688--701},
	Title = {Estimating causal effects of treatments in randomized and nonrandomized studies.},
	Volume = {66},
	Year = {1974}}

@article{Neyman23,
	Author = {J. Neyman},
	Journal = {Stat Sci},
	Pages = {465--480},
	Title = {Sur les applications de la theorie des probabilites aux experiences agricoles: Essai des principes ({In Polish}). {E}nglish translation by {D.M.} {D}abrowska and {T.P.} {S}peed (1990)},
	Volume = {5},
	Year = {1923}}

@book{Pearl2009,
	Address = {New York},
	Author = {J. Pearl},
	Date-Modified = {2012-08-22 21:06:39 -0700},
	Edition = {2nd},
	Keywords = {Book},
	Publisher = {Cambridge University Press},
	Title = {{Causality: Models, Reasoning and Inference}},
	Year = {2009}}

@article{Pearl95,
	Author = {J. Pearl},
	Journal = {Biometrika},
	Pages = {669--710},
	Title = {Causal diagrams for empirical research.},
	Volume = {82},
	Year = {1995}}

@article{RobinsGreenland1992,
	Author = {J.M. Robins and S. Greenland},
	Date-Modified = {2012-08-26 16:42:09 -0700},
	Journal = {Epidemiol},
	Keywords = {DE},
	Note = {PMID: 1576220},
	Pages = {143--155},
	Title = {Identifiability and exchangeability for direct and indirect effects},
	Volume = {3},
	Year = {1992}}

@inproceedings{Pearl2001,
	Address = {San Francisco},
	Author = {J. Pearl},
	Booktitle = {Proceedings of the Seventeenth Conference on Uncertainty in artificial intelligence},
	Date-Modified = {2012-08-26 20:43:51 -0700},
	Pages = {411--420},
	Publisher = {Morgan Kaufmann},
	Title = {Direct and indirect effects},
	Year = {2001}}

@article{Baron&Kenny86,
	Author = {R. Baron and D. Kenny},
	Journal = {J Personal Soc Psychol},
	Pages = {1173--1182},
	Title = {The moderator-mediator variable distinction in social psychological research: conceptual, strategic, and statistical considerations.},
	Volume = {51},
	Year = {1986}}

@book{MacKinnon08,
	Address = {New York},
	Author = {D. {MacKinnon}},
	Publisher = {Erlbaum},
	Title = {Introduction to statistical mediation analysis},
	Year = {2008}}

@article{MacKinnonetal07,
	Author = {D. {MacKinnon} and C. Lockwood and C. Brown and W. Wang and J. Hoffman},
	Journal = {Clin Trials},
	Pages = {499--513},
	Title = {The intermediate endpoint effect in logistic and probit regression.},
	Volume = {4},
	Year = {2007}}

@incollection{Pearl10c,
	Author = {J. Pearl},
	Booktitle = {Statistical causality},
	Editor = {C. Berzuini and P. Dawid and L. Bernardinelli},
	Title = {The mediation formula: a guide to the assessment of causal pathways in nonlinear models.},
	Year = {forthcoming 2011}}

@article{Pearl2010,
	Author = {J. Pearl},
	Date-Modified = {2012-08-26 20:46:05 -0700},
	Journal = {Int J Biostat},
	Keywords = {Roadmap},
	Note = {PMCID: PMC2836213},
	Number = {2},
	Pages = {Article 7},
	Title = {An Introduction to Causal Inference},
	Volume = {6},
	Year = {2010}}

@article{vanderLaan&Rose10,
	Author = {M.J. van der Laan and S. Rose},
	Journal = {Amstat News},
	Pages = {38--39},
	Title = {Statistics Ready for a Revolution: next Generation of Statisticians Must Build Tools for Massive Data Sets},
	Volume = {399},
	Year = {2010}}

@techreport{vanderLaan2003,
	Author = {M.J. van der Laan and S. Dudoit},
	Date-Modified = {2012-08-26 20:51:01 -0700},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Keywords = {Superlearner},
	Note = {Available at \url{http://biostats.bepress.com/ucbbiostat/paper130}},
	Number = {130},
	Title = {Unified Cross-Validation Methodology For Selection Among Estimators and a General Cross-Validated Adaptive Epsilon-Net Estimator: Finite Sample Oracle Inequalities and Examples},
	Year = {2003}}

@book{vanderLaanRobins2003,
	Address = {New York Berlin Heidelberg},
	Author = {M.J. van der Laan and J.M. Robins},
	Date-Modified = {2012-08-22 21:07:29 -0700},
	Keywords = {Book},
	Publisher = {Springer-Verlag},
	Title = {{Unified Methods for Censored Longitudinal Data and Causality}},
	Year = {2003}}

@book{Bickel1997,
	Address = {Berlin Heidelberg New York},
	Author = {P.J. Bickel and C.A.J. Klaassen and Y. Ritov and J. Wellner},
	Date-Modified = {2012-08-26 15:51:23 -0700},
	Publisher = {Springer},
	Title = {Efficient and adaptive estimation for semiparametric models},
	Year = {1997}}

@article{vanderLaan2006,
	Author = {M.J. van der Laan and Daniel B. Rubin},
	Date-Modified = {2012-08-26 20:31:54 -0700},
	Journal = {Int J Biostat},
	Keywords = {TMLE},
	Number = {1},
	Pages = {Article 11},
	Title = {Targeted Maximum Likelihood Learning},
	Volume = {2},
	Year = {2006}}

@article{Stitelman2011b,
	Author = {O.M. Stitelman and M.J. van der Laan},
	Date-Modified = {2012-08-26 00:54:24 -0700},
	Journal = {Int J Biostat},
	Keywords = {App},
	Note = {PMCID: PMC3083138},
	Number = {1},
	Pages = {19},
	Read = {1},
	Title = {Targeted Maximum Likelihood Estimation of Effect Modification Parameters In Survival Analysis},
	Volume = {7},
	Year = {2011}}

@article{vanderLaan2010ctmle,
	Author = {M.J. van der Laan and S. Gruber},
	Date-Modified = {2012-08-24 11:26:51 -0700},
	Journal = {Int J Biostat},
	Keywords = {TMLE},
	Note = {PMCID: PMC2898626},
	Number = {1},
	Title = {Collaborative double robust penalized targeted maximum likelihood estimation},
	Volume = {6},
	Year = {2010}}

@article{Taubes07,
	Author = {G. Taubes},
	Journal = {The New York Times},
	Title = {{Do we really know what makes us healthy?}},
	Year = {2007}}

@article{USPrev09,
	Author = {{U.S. Preventive Services Task Force}},
	Journal = {Ann Intern Med},
	Number = {10},
	Pages = {716--726},
	Title = {{Screening for breast cancer: U.S. Preventive Services Task Force recommendation statement}},
	Volume = {151},
	Year = {2009}}

@article{Freedman&Petitti&Robins04,
	Author = {D.A. Freedman and D.B. Petitti and J.M. Robins},
	Journal = {Int J Epidemiol},
	Pages = {43--55},
	Title = {{On the efficacy of screening for breast cancer}},
	Volume = {33},
	Year = {2004}}

@book{Rothman&Greenland98,
	Address = {Philadelphia},
	Author = {K.J. Rothman and S. Greenland},
	Edition = {2nd},
	Publisher = {Lippincott, Williams \& Wilkins},
	Title = {Modern epidemiology},
	Year = {1998}}

@book{Jewell04,
	Address = {Boca Raton},
	Author = {N.P. Jewell},
	Publisher = {Chapman \& Hall},
	Title = {Statistics for epidemiology},
	Year = {2004}}

@book{Freedman05,
	Address = {New York},
	Author = {D.A. Freedman},
	Publisher = {Cambridge},
	Title = {Statistical models: theory and practice},
	Year = {2005}}

@article{Ioannidis06,
	Author = {J.P.A. Ioannidis},
	Journal = {Neonatal Intensive Care J Perinatol Neonatol},
	Number = {3},
	Title = {{Why most published research findings are false}},
	Volume = {19},
	Year = {2006}}

@book{Freedman10,
	Address = {New York},
	Author = {D.H. Freedman},
	Publisher = {Little, Brown and Company},
	Title = {Wrong: why experts keep failing us---and how to know when not to trust them},
	Year = {2010}}

@book{Box&Draper87,
	Address = {Hoboken},
	Author = {G.E.P. Box and N.R. Draper},
	Publisher = {Wiley},
	Title = {Empirical model-building and response surfaces},
	Year = {1987}}

@article{Robins1986,
	Author = {J.M. Robins},
	Date-Modified = {2012-08-26 14:52:27 -0700},
	Journal = {Math Mod},
	Pages = {1393--1512},
	Title = {A new approach to causal inference in mortality studies with sustained exposure periods--application to control of the healthy worker survivor effect},
	Volume = {7},
	Year = {1986}}

@article{Tager&Hollenberg&Satariano98,
	Author = {I. Tager and M. Hollenberg and W. Satariano},
	Journal = {Am J Epidemiol},
	Pages = {921--931},
	Title = {{Self-reported leisure-time physical activity and measures of cardiorespiratory fitness in an elderly population}},
	Volume = {147},
	Year = {1998}}

@manual{RCore,
	Address = {Vienna},
	Author = {{R Development Core Team}},
	Date-Modified = {2012-08-22 08:11:48 -0700},
	Keywords = {R},
	Organization = {R Foundation for Statistical Computing},
	Title = {R: a language and environment for statistical computing},
	Url = {http://www.R-project.org},
	Year = {2010},
	Bdsk-Url-1 = {http://www.R-project.org}}

@article{liaw:2002,
	Author = {A. Liaw and M. Wiener},
	Journal = {R News},
	Number = {3},
	Pages = {18--22},
	Title = {Classification and Regression by randomForest},
	Url = {http://CRAN.R-project.org/package=randomForest},
	Volume = {2},
	Year = {2002},
	Bdsk-Url-1 = {http://CRAN.R-project.org/package=randomForest}}

@article{randomForests,
	Author = {L. Breiman},
	Journal = {Mach Learn},
	Pages = {5--32},
	Title = {Random Forests},
	Volume = {45},
	Year = {2001}}

@manual{ipred,
	Author = {A. Peters and T. Hothorn},
	Note = {R package version 0.8-8},
	Title = {ipred: Improved Predictors},
	Url = {http://CRAN.R-project.org/package=ipred},
	Year = {2009},
	Bdsk-Url-1 = {http://CRAN.R-project.org/package=ipred}}

@article{breiman96bagging,
	Author = {L. Breiman},
	Journal = {Mach Learn},
	Number = {2},
	Pages = {123--140},
	Title = {Bagging Predictors},
	Volume = {24},
	Year = {1996}}

@incollection{gam:1992,
	Address = {Boca Raton},
	Author = {T.J. Hastie},
	Booktitle = {Statistical models in {S}},
	Editor = {J.M. Chambers and T.J. Hastie},
	Publisher = {Chapman \& Hall},
	Title = {Generalized additive models},
	Year = {1992}}

@book{gams,
	Address = {Boca Raton},
	Author = {T.J. Hastie and R.J. Tibshirani},
	Publisher = {Chapman \& Hall},
	Title = {Generalized additive models},
	Year = {1990}}

@manual{gbm,
	Author = {G. Ridgeway},
	Note = {R package version 1.6-3},
	Title = {gbm: generalized boosted regression models},
	Year = {2007}}

@article{friedman:2001,
	Author = {J.H. Friedman},
	Journal = {Ann Stat},
	Pages = {1189-1232},
	Title = {Greedy Function Approximation: a Gradient Boosting Machine},
	Volume = {29},
	Year = {2001}}

@book{MASS,
	Address = {Berlin Heidelberg New York},
	Author = {W.N. Venables and B.D. Ripley},
	Edition = {4th},
	Publisher = {Springer},
	Title = {Modern applied statistics with S},
	Year = {2002}}

@manual{polspline,
	Author = {C. Kooperberg},
	Note = {R package version 1.1.4},
	Title = {polspline: Polynomial spline routines},
	Url = {http://CRAN.R-project.org/package=polspline},
	Year = {2009},
	Bdsk-Url-1 = {http://CRAN.R-project.org/package=polspline}}

@article{MARS,
	Author = {J.H. Friedman},
	Journal = {Ann Stat},
	Number = {1},
	Pages = {1--141},
	Title = {Multivariate Adaptive Regression Splines},
	Volume = {19},
	Year = {1991}}

@manual{bart,
	Author = {H.A. Chipman and R.E. McCulloch},
	Note = {R package version 0.3-1},
	Title = {BayesTree: {B}ayesian methods for tree-based models},
	Url = {http://CRAN.R-project.org/package=BayesTree},
	Year = {2009},
	Bdsk-Url-1 = {http://CRAN.R-project.org/package=BayesTree}}

@article{chipman:2009,
	Author = {H.A. Chipman and E.I. George and R.E. McCulloch},
	Journal = {Ann Appl Stat},
	Number = {1},
	Pages = {266--298},
	Title = {{BART}: {B}ayesian Additive Regression Trees},
	Volume = {4},
	Year = {2010}}

@incollection{loess,
	Address = {Boca Raton},
	Author = {W.S. Cleveland and E. Groose and W.M. Shyu},
	Booktitle = {Statistical models in {S}},
	Editor = {J.M. Chambers and T.J. Hastie},
	Publisher = {Chapman \& Hall},
	Title = {Local Regression Models},
	Year = {1992}}

@techreport{Polley2010,
	Author = {E.C. Polley and M.J. van der Laan},
	Date-Modified = {2012-08-26 21:10:49 -0700},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Keywords = {Superlearner},
	Note = {Available at \url{http://www.bepress.com/ucbbiostat/paper266/}},
	Number = {266},
	Title = {Super Learner in Prediction},
	Year = {2010}}

@book{cook:1994,
	Address = {New York},
	Author = {D. Cook and S. Weisberg},
	Publisher = {Wiley},
	Title = {An introduction to regression graphics},
	Year = {1994}}

@article{chu:2001,
	Author = {S. Chu},
	Journal = {J Stat Educ},
	Number = {2},
	Title = {Pricing the {C}'s of diamond stones},
	Volume = {9},
	Year = {2001}}

@book{berndt:1991,
	Address = {New York},
	Author = {E.R. Berndt},
	Publisher = {Addison--Wesley},
	Title = {The practice of econometrics},
	Year = {1991}}

@article{kibler:1989,
	Author = {D. Kibler and D.W. Aha and M.K. Albert},
	Journal = {Comput Intell},
	Pages = {51},
	Title = {Instance-Based Prediction of Real-Valued Attributes},
	Volume = {5},
	Year = {1989}}

@book{rosner:1999,
	Address = {Pacific Grove},
	Author = {B. Rosner},
	Edition = {5th},
	Publisher = {Duxbury},
	Title = {Fundamentals of biostatistics},
	Year = {1999}}

@misc{newman:1998,
	Author = {D.J. Newman and S. Hettich and C.L. Blake and C.J. Merz},
	Institution = {Department of Information and Computer Sciences, University of California, Irvine},
	Title = {{UCI Repository of Machine Learning Databases}},
	Year = {1998}}

@book{afifi:1979,
	Address = {New York},
	Author = {A. Afifi and S. Azen},
	Edition = {2nd},
	Publisher = {Academic},
	Title = {Statistical analysis: a computer oriented approach},
	Year = {1979}}

@book{cook:1998,
	Address = {New York},
	Author = {D. Cook},
	Publisher = {Wiley},
	Title = {Regression graphics: ideas for studying regression through graphics},
	Year = {1998}}

@article{liu:1999,
	Author = {Z. Liu and T. Stengos},
	Journal = {J of Appl Econom},
	Pages = {527--538},
	Title = {Nonlinearities in Cross Country Growth Regressions: a Semiparametric Approach},
	Volume = {14},
	Year = {1999}}

@article{penrose:1985,
	Author = {K. Penrose and A. Nelson and A. Fisher},
	Journal = {Med Sci Sport Exer},
	Pages = {189},
	Title = {Generalized Body Composition Prediction Equation for Men Using Simple Measurement Techniques},
	Volume = {17},
	Year = {1985}}

@book{harrell:2001,
	Address = {Berlin Heidelberg New York},
	Author = {Harrell, Jr., F.E.},
	Publisher = {Springer},
	Title = {Regression modeling strategies with applications to linear models, logistic regression, and survival analysis},
	Year = {2001}}

@manual{arm,
	Author = {A. Gelman and Y.-S. Su and M. Yajima and J. Hill and M.G. Pittau and J. Kerman and T. Zheng},
	Note = {R package version 1.3-02},
	Title = {arm: data analysis using regression and multilevel/hierarchical models},
	Url = {http://CRAN.R-project.org/package=arm},
	Year = {2010},
	Bdsk-Url-1 = {http://CRAN.R-project.org/package=arm}}

@article{gelman:2009,
	Author = {A. Gelman and A. Jakulin and M.G. Pittau and Y.-S. Su},
	Journal = {Ann Appl Stat},
	Number = {3},
	Pages = {1360--1383},
	Title = {A Weakly Informative Default Prior Distribution for Logistic and Other Regression Models},
	Volume = {2},
	Year = {2009}}

@article{friedman:2010,
	Author = {J.H. Friedman and T.J. Hastie and R.J. Tibshirani},
	Journal = {J Stat Softw},
	Number = {1},
	Title = {Regularization Paths for Generalized Linear Models via Coordinate Descent},
	Volume = {33},
	Year = {2010}}

@manual{glmnet,
	Author = {J.H. Friedman and T.J. Hastie and R.J. Tibshirani},
	Note = {R package version 1.1-5},
	Title = {glmnet: lasso and elastic-net regularized generalized linear models},
	Url = {http://CRAN.R-project.org/package=glmnet},
	Year = {2010},
	Bdsk-Url-1 = {http://CRAN.R-project.org/package=glmnet}}

@manual{DSA,
	Author = {R. Neugebauer and J. Bullard},
	Note = {R package version 3.1.3},
	Title = {DSA: Data-adaptive estimation with cross-validation and the D/S/A algorithm},
	Url = {http://www.stat.berkeley.edu/~laan/Software/},
	Year = {2009},
	Bdsk-Url-1 = {http://www.stat.berkeley.edu/~laan/Software/}}

@article{SinisivanderLaan04,
	Author = {S.E. Sinisi and M.J. van der Laan},
	Journal = {Stat Appl Genet Mol},
	Note = {Article 18},
	Number = {1},
	Title = {{D}eletion/{S}ubstitution/{A}ddition algorithm in learning with applications in genomics},
	Volume = {3},
	Year = {2004}}

@manual{svm,
	Author = {E. Dimitriadou and K. Hornik and F. Leisch and D. Meyer and A. Weingessel},
	Note = {R package version 1.5-22},
	Title = {e1071: misc functions of the Department of Statistics (e1071)},
	Url = {http://CRAN.R-project.org/package=e1071},
	Year = {2009},
	Bdsk-Url-1 = {http://CRAN.R-project.org/package=e1071}}

@manual{Chang:2001,
	Author = {C.-C. Chang and C.-J. Lin},
	Title = {{LIBSVM}: a library for support vector machines},
	Url = {http://www.csie.ntu.edu.tw/~cjlin/libsvm},
	Year = {2001},
	Bdsk-Url-1 = {http://www.csie.ntu.edu.tw/~cjlin/libsvm}}

@article{vantveer:2002,
	Author = {L.J. {van't Veer} and H. Dal and M.J. {van de Vijver} and Y.D. He and A.A.M. Hart and M. Mao and H.L. Peterse and K. van der Kooy and M.J. Marton and A.T. Witteveen and G.J. Schreiber and R.M. Kerkhoven and C. Roberts and P.S. Linsley and R. Bernards and S.H. Friend},
	Journal = {Nature},
	Pages = {530--536},
	Title = {Gene Expression Profiling Predicts Clinical Outcome of Breast Cancer},
	Volume = {415},
	Year = {2002}}

@article{vanderLaan2007,
	Author = {M.J. van der Laan and E.C. Polley and A.E. Hubbard},
	Date-Modified = {2012-08-23 17:06:55 -0700},
	Journal = {Stat Appl Genet Mol},
	Keywords = {Superlearner},
	Note = {PMID: 17910531},
	Number = {1},
	Pages = {Article 25},
	Title = {Super Learner},
	Volume = {6},
	Year = {2007}}

@article{Wolpert92,
	Author = {D. H. Wolpert},
	Journal = {Neural Networks},
	Pages = {241--259},
	Title = {Stacked Generalization},
	Volume = {5},
	Year = {1992}}

@article{Breiman96d,
	Author = {L. Breiman},
	Journal = {Mach Learn},
	Pages = {49--64},
	Title = {Stacked Regressions},
	Volume = {24},
	Year = {1996}}

@article{Leblanc96,
	Author = {M. LeBlanc and R.J. Tibshirani},
	Journal = {J Am Stat Assoc},
	Pages = {1641--1650},
	Title = {Combining estimates in regression and classification},
	Volume = {91},
	Year = {1996}}

@article{Stone74,
	Author = {M. Stone},
	Journal = {J R Stat Soc Ser B},
	Number = {2},
	Pages = {111--147},
	Title = {Cross-validatory choice and assessment of statistical predictions},
	Volume = {36},
	Year = {1974}}

@article{Geisser75,
	Author = {S. Geisser},
	Journal = {J Am Stat Assoc},
	Number = {350},
	Pages = {320--328},
	Title = {The Predictive Sample Reuse Method with Applications},
	Volume = {70},
	Year = {1975}}

@inproceedings{Tsybakov03,
	Address = {Berlin Heidelberg New York},
	Author = {A.B. Tsybakov},
	Booktitle = {COLT},
	Editor = {B. Sch{\"o}lkopf and M.K. Warmuth},
	Publisher = {Springer},
	Series = {Lecture Notes in Computer Science},
	Title = {Optimal rates of aggregation},
	Volume = {2777},
	Year = {2003}}

@inproceedings{Juditskyetal05,
	Author = {A. Juditsky and A.V. Nazin and A.B. Tsybakov and N. Vayatis},
	Booktitle = {NIPS},
	Title = {Generalization Error Bounds for Aggregation by Mirror Descent with Averaging},
	Year = {2005}}

@inproceedings{Buneaetal06,
	Address = {Berlin Heidelberg New York},
	Author = {F. Bunea and A.B. Tsybakov and M.H. Wegkamp},
	Booktitle = {COLT},
	Editor = {G. Lugosi and H.-U. Simon},
	Publisher = {Springer},
	Series = {Lecture Notes in Computer Science},
	Title = {Aggregation and sparsity via {L}1 penalized least squares},
	Volume = {4005},
	Year = {2006}}

@article{Buneaetal07,
	Author = {F. Bunea and A.B. Tsybakov and M.H. Wegkamp},
	Journal = {Ann Stat},
	Number = {4},
	Pages = {1674--1697},
	Title = {Aggregation for Gaussian Regression},
	Volume = {35},
	Year = {2007}}

@inproceedings{Buneaetal07b,
	Address = {Berlin Heidelberg New York},
	Author = {F. Bunea and A.B. Tsybakov and M.H. Wegkamp},
	Booktitle = {COLT},
	Editor = {N.H. Bshouty and C. Gentile},
	Publisher = {Springer},
	Series = {Lecture Notes in Computer Science},
	Title = {Sparse density estimation with {L}1 penalties},
	Volume = {4539},
	Year = {2007}}

@inproceedings{Dalalyan&Tsybakov07,
	Address = {Berlin Heidelberg New York},
	Author = {A.S. Dalalyan and A.B. Tsybakov},
	Booktitle = {COLT},
	Editor = {N.H. Bshouty and C. Gentile},
	Publisher = {Springer},
	Series = {Lecture Notes in Computer Science},
	Title = {Aggregation by exponential weighting and sharp oracle inequalities},
	Volume = {4539},
	Year = {2007}}

@article{Dalalyan&Tsybakov08,
	Author = {A.S. Dalalyan and A.B. Tsybakov},
	Journal = {Mach Learn},
	Number = {1--2},
	Pages = {39--61},
	Title = {Aggregation by exponential weighting, sharp PAC-{B}ayesian bounds and sparsity},
	Volume = {72},
	Year = {2008}}

@book{Lehmann86,
	Address = {Berlin Heidelberg New York},
	Author = {E.L. Lehmann},
	Edition = {2nd},
	Publisher = {Springer},
	Title = {Testing statistical hypotheses},
	Year = {1986}}

@book{Hastie&Tibshirani&Friedman01,
	Address = {Berlin Heidelberg New York},
	Author = {T.J. Hastie and R.J. Tibshirani and J.H. Friedman},
	Date-Modified = {2012-08-23 17:04:42 -0700},
	Publisher = {Springer},
	Title = {{The Elements of Statistical Learning: Data Mining, Inference, and Prediction}},
	Year = {2001}}

@inproceedings{Ruczinski&Kooperberg&LeBlanc02,
	Author = {I. Ruczinski and C. Kooperberg and M. LeBlanc},
	Booktitle = {Proceedings of the MSRI workshop on Nonlinear Estimation and Classification},
	Editor = {D. Denison and M. Hansen and C. Holmes and B. Mallick and B. Yu},
	Pages = {333--344},
	Title = {Logic Regression -- methods and software},
	Year = {2002}}

@techreport{Birkner&Hubbard&vanderLaan05,
	Author = {M.D. Birkner and A.E. Hubbard and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {197},
	Title = {Data Adaptive Pathway Testing},
	Year = {2005}}

@techreport{Chaffee&Hubbard&vanderLaan10,
	Author = {P. Chaffee and A.E. Hubbard and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {263},
	Title = {Permutation-based Pathway Testing using the Super Learner Algorithm},
	Year = {2010}}

@inproceedings{Polley&vanderLaan09,
	Address = {Boca Raton},
	Author = {E.C. Polley and M.J. van der Laan},
	Booktitle = {Design, summarization, analysis \& interpretation of clinical trials with time-to-event endpoints},
	Editor = {K.E. Peace},
	Publisher = {Chapman \& Hall},
	Title = {Predicting Optimal Treatment Assignment Based on Prognostic Factors in Cancer Patients},
	Year = {2009}}

@article{vanderLaan&Dudoit&vanderVaart06,
	Author = {M.J. van der Laan and S. Dudoit and A.W. van der Vaart},
	Journal = {Stat Decis},
	Number = {3},
	Pages = {373--395},
	Title = {The Cross-Validated Adaptive Epsilon-Net Estimator},
	Volume = {24},
	Year = {2006}}

@article{vanderVaart&Dudoit&vanderLaan06,
	Author = {A.W. van der Vaart and S. Dudoit and M.J. van der Laan},
	Journal = {Stat Decis},
	Number = {3},
	Pages = {351--371},
	Title = {Oracle Inequalities for Multi-Fold Cross-Validation},
	Volume = {24},
	Year = {2006}}

@article{vanderLaan&Dudoit&Keles04,
	Author = {M.J. van der Laan and S. Dudoit and S. Kele\c{s}},
	Journal = {Stat Appl Genet Mol},
	Number = {1},
	Pages = {Article 4},
	Title = {Asymptotic optimality of likelihood-based cross-validation},
	Volume = {3},
	Year = {2004}}

@article{Dudoit&vanderLaan05,
	Author = {S. Dudoit and M.J. van der Laan},
	Journal = {Stat Methodol},
	Number = {2},
	Pages = {131--154},
	Title = {Asymptotics of cross-validated risk estimation in estimator selection and performance assessment},
	Volume = {2},
	Year = {2005}}

@techreport{Keles&vanderLaan&Dudoit02,
	Author = {Kele\c{s}, S. and van der Laan, M.J. and Dudoit, S.},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {124},
	Title = {Asymptotically Optimal Model Selection Method for Regression on Censored Outcomes},
	Year = {2002}}

@book{Gyorfietal02,
	Address = {Berlin Heidelberg New York},
	Author = {L. Gy\"{o}rfi and M. Kohler and A. Krzy\.{z}ak and H. Walk},
	Pages = {100--102},
	Publisher = {Springer},
	Title = {A distribution-free theory of nonparametric regression},
	Year = {2002}}

@article{Stone77,
	Author = {M. Stone},
	Journal = {Biometrika},
	Number = {1},
	Pages = {29--35},
	Title = {Asymptotics for and against cross-validation},
	Volume = {64},
	Year = {1977}}

@book{Breimanetal84,
	Address = {Boca Raton},
	Author = {L. Breiman and J.H. Friedman and R. Olshen and C.J. Stone},
	Publisher = {Chapman \& Hall},
	Title = {Classification and regression trees},
	Year = {1984}}

@article{Breiman&Spector92,
	Author = {L. Breiman and P. Spector},
	Journal = {Int Stat Rev},
	Pages = {291--319},
	Title = {Submodel Selection and Evaluation in Regression. {T}he {$X$} Random Case},
	Volume = {60},
	Year = {1992}}

@book{Efron&Tibshirani93,
	Address = {Boca Raton},
	Author = {B. Efron and R. J. Tibshirani},
	Publisher = {Chapman \& Hall},
	Title = {An Introduction to the bootstrap},
	Year = {1993}}

@article{Breiman96,
	Author = {L. Breiman},
	Journal = {Ann Stat},
	Number = {6},
	Pages = {2350--2383},
	Title = {Heuristics of instability and stabilization in model selection},
	Volume = {24},
	Year = {1996}}

@techreport{Breiman96c,
	Author = {L. Breiman},
	Institution = {Department of Statistics, University of California, Berkeley},
	Title = {Out-of-bag estimation},
	Type = {Technical {R}eport},
	Year = {1996}}

@book{Ripley96,
	Address = {New York},
	Author = {B.D. Ripley},
	Publisher = {Cambridge},
	Title = {Pattern recognition and neural networks},
	Year = {1996}}

@article{Breiman98,
	Author = {L. Breiman},
	Journal = {Ann Stat},
	Pages = {801--824},
	Title = {Arcing classifiers},
	Volume = {26},
	Year = {1998}}

@article{Ambroise&McLachlan02,
	Author = {C. Ambroise and G.J. McLachlan},
	Journal = {Proc Natl Acad Sci},
	Number = {10},
	Pages = {6562--6566},
	Title = {Selection bias in gene extraction on the basis of microarray gene-expression data},
	Volume = {99},
	Year = {2002}}

@article{Pavlic&vanderLaan03,
	Author = {M. Pavlic and M.J. van der Laan},
	Journal = {Comput Stat Data An},
	Pages = {413--428},
	Title = {Fitting of mixtures with unspecified number of components using cross validation distance estimate},
	Volume = {41},
	Year = {2003}}

@inproceedings{Akaike73,
	Address = {Budapest},
	Author = {H. Akaike},
	Booktitle = {Second International Symposium on Information Theory},
	Editor = {B.N. Petrov and F. Csaki},
	Organization = {Academiai Kiado},
	Title = {Information theory and an extension of the maximum likelihood principle},
	Year = {1973}}

@article{Bozdogan00,
	Author = {H. Bozdogan},
	Journal = {J Math Psychol},
	Pages = {62--91},
	Title = {Akaike's information criterion and recent developments in information complexity},
	Volume = {44},
	Year = {2000}}

@article{Schwartz78,
	Author = {G. Schwartz},
	Journal = {Ann Stat},
	Pages = {461--464},
	Title = {Estimating the Dimension of a Model},
	Volume = {6},
	Year = {1978}}

@article{Rissanen78,
	Author = {J. Rissanen},
	Journal = {Automatica},
	Pages = {465--471},
	Title = {Modelling by shortest data description},
	Volume = {14},
	Year = {1978}}

@incollection{Bozdogan93,
	Address = {Berlin Heidelberg New York},
	Author = {H. Bozdogan},
	Booktitle = {Information and classification},
	Editor = {O. Opitz and B. Lausen and R. Klar},
	Publisher = {Springer},
	Title = {Choosing the number of component clusters in the mixture model using a new informational complexity criterion of the inverse Fisher information matrix},
	Year = {1993}}

@article{Snowden&Rose&Mortimer11,
	Author = {J.M. Snowden and S. Rose and K.M. Mortimer},
	Journal = {Am J Epidemiol},
	Number = {00},
	Pages = {000--000},
	Title = {Implementation of G-Computation on a Simulated Data set: demonstration of a Causal Inference Technique},
	Volume = {173},
	Year = {2011}}

@article{Rose&Snowden&Mortimer11,
	Author = {S. Rose and J.M. Snowden and K.M. Mortimer},
	Journal = {Am J Epidemiol},
	Number = {00},
	Pages = {000--000},
	Title = {Rose et al. Respond to ``{G}-Computation and Standardization in Epidemiology''},
	Volume = {173},
	Year = {2011}}

@incollection{Robins99b,
	Address = {Berlin Heidelberg New York},
	Author = {Robins, J.M.},
	Booktitle = {Statistical models in epidemiology: the environment and clinical trials},
	Publisher = {Springer},
	Title = {Marginal structural models versus structural nested models as tools for causal inference},
	Year = {1999}}

@article{Hernan2000,
	Author = {M.A. Hern\'{a}n and B. Brumback and J.M. Robins},
	Date-Modified = {2012-08-23 11:06:09 -0700},
	Journal = {Epidemiol},
	Keywords = {Roadmap + MSM},
	Note = {PMID: 10955409},
	Number = {5},
	Pages = {561--570},
	Title = {Marginal structural models to estimate the causal effect of zidovudine on the survival of {HIV}-positive men},
	Volume = {11},
	Year = {2000}}

@article{Robins&Rotnitzky&vanderLaan00,
	Author = {J.M. Robins and A. Rotnitzky and M.J. van der Laan},
	Journal = {J Am Stat Assoc},
	Pages = {431--435},
	Title = {Comment on ``{O}n profile likelihood"},
	Volume = {450},
	Year = {2000}}

@inproceedings{Robins2000b,
	Address = {Alexandria, VA},
	Author = {J.M. Robins},
	Booktitle = {1999 Proceedings of the American Statistical Association},
	Date-Modified = {2012-08-26 20:55:09 -0700},
	Pages = {6-10},
	Publisher = {American Statistical Association},
	Title = {Robust estimation in sequentially ignorable missing data and causal inference models},
	Year = {2000}}

@article{Robins&Rotnitzky01,
	Author = {J.M. Robins and A. Rotnitzky},
	Journal = {Stat Sinica},
	Number = {4},
	Pages = {920--936},
	Title = {Comment on the {B}ickel and {K}won article, ``{I}nference for semiparametric models: some questions and an answer''},
	Volume = {11},
	Year = {2001}}

@incollection{Robins&Rotnitzky92,
	Address = {Basel},
	Author = {J.M. Robins and A. Rotnitzky},
	Booktitle = {AIDS epidemiology},
	Publisher = {Birkh\"{a}user},
	Title = {Recovery of information and adjustment for dependent censoring using surrogate markers},
	Year = {1992}}

@article{Robins2000,
	Author = {J.M. Robins and M.A. Hern\'{a}n and B. Brumback},
	Date-Modified = {2012-08-23 10:26:28 -0700},
	Journal = {Epidemiology},
	Keywords = {Roadmap},
	Note = {PMID: 10955408},
	Number = {5},
	Pages = {550--560},
	Title = {Marginal structural models and causal inference in epidemiology},
	Volume = {11},
	Year = {2000}}

@article{Mortimeretal05,
	Author = {K.M. Mortimer and R. Neugebauer and M.J. van der Laan and I.B. Tager},
	Journal = {Am J Epidemiol},
	Number = {4},
	Pages = {382--388},
	Title = {An Application of Model-Fitting Procedures for Marginal Structural Models},
	Volume = {162},
	Year = {2005}}

@article{Cole2008,
	Annote = {http://www.ncbi.nlm.nih.gov/pmc/articles/PMC2732954/},
	Author = {S.R. Cole and M.A. Hern\'{a}n},
	Date-Modified = {2012-08-26 20:34:41 -0700},
	Journal = {Am J Epidemiol},
	Keywords = {Aim1},
	Note = {PMCID: PMC2732954},
	Number = {6},
	Pages = {656--664},
	Title = {Constructing Inverse Probability Weights for Marginal Structural Models},
	Volume = {168},
	Year = {2008}}

@article{Bembom2007,
	Author = {O. Bembom and M.J. van der Laan},
	Date-Modified = {2012-08-23 18:03:30 -0700},
	Journal = {Electron J Stat},
	Keywords = {Aim1},
	Note = {PMCID: PMC2600532},
	Pages = {574--596},
	Title = {A practical illustration of the importance of realistic individualized treatment rules in causal inference},
	Volume = {1},
	Year = {2007}}

@article{vanderLaan2008casecontrol,
	Author = {M.J. van der Laan},
	Date-Modified = {2012-08-24 09:45:10 -0700},
	Journal = {Int J Biostat},
	Keywords = {Application},
	Note = {PMID: 22462152},
	Number = {1},
	Pages = {Article 17},
	Title = {Estimation based on case-control designs with known prevalance probability},
	Volume = {4},
	Year = {2008}}

@article{Rose2008,
	Author = {S. Rose and M.J. van der Laan},
	Date-Modified = {2012-08-24 09:43:57 -0700},
	Journal = {Int J Biostat},
	Keywords = {Application},
	Note = {PMCID: PMC2835459},
	Number = {1},
	Pages = {Article 19},
	Title = {Simple optimal weighting of cases and controls in case-control studies},
	Volume = {4},
	Year = {2008}}

@article{Rose2009,
	Author = {S. Rose and M.J. van der Laan},
	Date-Modified = {2012-08-24 09:43:07 -0700},
	Journal = {Int J Biostat},
	Keywords = {Application},
	Note = {PMCID: PMC2827892},
	Number = {1},
	Pages = {Article 1},
	Title = {Why match? {I}nvestigating matched case-control study designs with causal effect estimation},
	Volume = {5},
	Year = {2009}}

@inproceedings{Moore2009c,
	Address = {Boca Raton},
	Author = {K.L. Moore and M.J. van der Laan},
	Booktitle = {Design and Analysis Clinical Trials with Time-to-Event Endpoints},
	Date-Modified = {2012-08-26 20:23:23 -0700},
	Editor = {Karl E. Peace},
	Keywords = {App},
	Publisher = {Chapman \& Hall/CRC},
	Title = {Application of Time-to-Event Methods in the Assessment of Safety in Clinical Trials},
	Year = {2009}}

@article{Moore2009,
	Author = {Moore, K.L. and van der Laan, M.J.},
	Date-Modified = {2012-08-26 00:15:23 -0700},
	Journal = {Stat Med},
	Keywords = {Application},
	Note = {PMCID: PMC2857590},
	Number = {1},
	Pages = {39--64},
	Title = {Covariate Adjustment in Randomized Trials with Binary Outcomes: {T}argeted Maximum Likelihood Estimation},
	Volume = {28},
	Year = {2009}}

@article{Moore2009b,
	Author = {Moore, K.L. and van der Laan, M.J.},
	Date-Modified = {2012-08-26 00:22:36 -0700},
	Journal = {J Biopharm Stat},
	Keywords = {Application},
	Note = {PMID: 20183467},
	Number = {6},
	Pages = {1099--1131},
	Title = {Increasing Power in Randomized Trials with Right Censored Outcomes Through Covariate Adjustment},
	Volume = {19},
	Year = {2009}}

@article{Bembom2009,
	Author = {O. Bembom and M.L. Petersen and S.-Y. Rhee and W.J. Fessel and S.E. Sinisi and R.W. Shafer and M.J. van der Laan},
	Date-Modified = {2012-08-24 10:55:57 -0700},
	Journal = {Stat Med},
	Keywords = {Application},
	Note = {PMID: 18825650},
	Number = {1},
	Pages = {152--721},
	Title = {Biomarker discovery using targeted maximum likelihood estimation: application to the treatment of antiretroviral resistant {HIV} infection},
	Volume = {28},
	Year = {2009}}

@article{Rosenblum2009,
	Author = {M. Rosenblum and S.G. Deeks and M.J. van der Laan and D.R. Bangsberg},
	Date-Modified = {2012-08-26 00:27:48 -0700},
	Journal = {PLoS ONE},
	Keywords = {Application},
	Note = {PMCID: PMC2747009},
	Number = {9},
	Pages = {e7196},
	Title = {The Risk of Virologic Failure Decreases with Duration of {HIV} Suppression, at Greater than 50\% Adherence to Antiretroviral Therapy},
	Volume = {4},
	Year = {2009}}

@article{Gruber2010ctmle,
	Author = {S. Gruber and M.J. van der Laan},
	Date-Modified = {2012-08-24 11:27:25 -0700},
	Journal = {Int J Biostat},
	Keywords = {TMLE},
	Note = {PMCID: PMC3126668},
	Number = {1},
	Title = {An application of collaborative targeted maximum likelihood estimation in causal inference and genomics},
	Volume = {6},
	Year = {2010},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAZQAAAAAAZQAAgAADE1hY2ludG9zaCBIRAAAAAAAAAAAAAAAAAAAAMobz/1IKwAABsaXyg8yMDEwX0dydWJlci5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAHROAxzF0WKwAAAAAAAAAAAAEAAgAACSAAAAAAAAAAAAAAAAAAAAAKTGl0ZXJhdHVyZQAQAAgAAMocMm0AAAARAAgAAMxdeJsAAAABABAGxpfKAAxX9QAMUlIAAAAeAAIAO01hY2ludG9zaCBIRDpVc2VyczpsYXVyYTpEZXNrdG9wOkxpdGVyYXR1cmU6MjAxMF9HcnViZXIucGRmAAAOACAADwAyADAAMQAwAF8ARwByAHUAYgBlAHIALgBwAGQAZgAPABoADABNAGEAYwBpAG4AdABvAHMAaAAgAEgARAASAC5Vc2Vycy9sYXVyYS9EZXNrdG9wL0xpdGVyYXR1cmUvMjAxMF9HcnViZXIucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi9MaXRlcmF0dXJlLzIwMTBfR3J1YmVyLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAI4AjoCPwJIAlMCVwJlAmwCdQKVApoCnQKqAq8AAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACwQ==}}

@article{Rosenblum2010,
	Author = {M. Rosenblum and M.J. van der Laan},
	Date-Modified = {2012-08-23 17:02:41 -0700},
	Journal = {Int J Biostat},
	Keywords = {MSM},
	Note = {PMCID: PMC3126671},
	Number = {2},
	Pages = {Article 19},
	Title = {Targeted maximum likelihood estimation of the parameter of a marginal structural model},
	Volume = {6},
	Year = {2010}}

@book{Dudoit&vanderLaan08,
	Address = {Berlin Heidelberg New York},
	Author = {S. Dudoit and M.J. van der Laan},
	Publisher = {Springer},
	Title = {Resampling based multiple testing with applications to genomics},
	Year = {2008}}

@article{Robins94,
	Author = {J.M. Robins},
	Journal = {Commun Stat},
	Pages = {2379--2412},
	Title = {Correcting for noncompliance in randomized trials using structural nested mean models},
	Volume = {23},
	Year = {1994}}

@article{Robins&Rotnitzky&Zhao95,
	Author = {J.M. Robins and A. Rotnitzky and L.P. Zhao},
	Journal = {J Am Stat Assoc},
	Pages = {106--121},
	Title = {Analysis of semiparametric regression models for repeated outcomes in the presence of missing data.},
	Volume = {90},
	Year = {1995}}

@article{Scharfstein&Rotnitzky&Robins99,
	Author = {D.O. Scharfstein and A. Rotnitzky and J.M. Robins},
	Journal = {J Am Stat Assoc},
	Pages = {1096-1120 (1121-1146)},
	Title = {Adjusting for Nonignorable Drop-out Using Semiparametric Nonresponse Models, (with Discussion and Rejoinder)},
	Volume = {94},
	Year = {1999}}

@article{Leon&Tsiatis&Davidian03,
	Author = {S. Leon and A.A. Tsiatis and M. Davidian},
	Journal = {Biometrics},
	Pages = {1046--1055},
	Title = {Semiparametric estimation of treatment effect in a pretest-posttest study},
	Volume = {59},
	Year = {2003}}

@article{Tan06,
	Author = {Z. Tan},
	Journal = {J Am Stat Assoc},
	Pages = {1619-1637},
	Title = {A distributional approach for causal inference using propensity scores},
	Volume = {101},
	Year = {2006}}

@book{Tsiatis2006,
	Address = {Berlin Heidelberg New York},
	Author = {A.A. Tsiatis},
	Date-Modified = {2012-08-22 21:08:28 -0700},
	Keywords = {Book},
	Publisher = {Springer},
	Title = {{Semiparametric Theory and Missing Data}},
	Year = {2006}}

@article{Zhang&Tsiatis&Davidian08,
	Author = {M. Zhang and A.A. Tsiatis and M. Davidian},
	Journal = {Biometrics},
	Number = {3},
	Pages = {707--715},
	Title = {Improving efficiency of inferences in randomized clinical trials using auxiliary covariates},
	Volume = {64},
	Year = {2008}}

@article{Rubin&vanderLaan08,
	Author = {Daniel B. Rubin and M.J. van der Laan},
	Journal = {Int J Biostat},
	Number = {1},
	Pages = {Article 5},
	Title = {Empirical efficiency maximization: improved locally efficient covariate adjustment in randomized experiments and survival analysis},
	Volume = {4},
	Year = {2008}}

@article{Freedman08,
	Author = {D.A. Freedman},
	Journal = {Adv Appl Math},
	Pages = {180--193},
	Title = {On regression adjustments to experimental data},
	Volume = {40},
	Year = {2008}}

@article{Freedman082,
	Author = {D.A. Freedman},
	Journal = {Ann Appl Stat},
	Pages = {176--96},
	Title = {On regression adjustments to experiments with several treatments},
	Volume = {2},
	Year = {2008}}

@article{Rosenblum2009b,
	Author = {M. Rosenblum and M.J. van der Laan},
	Date-Modified = {2012-08-26 01:20:38 -0700},
	Journal = {Biometrics},
	Keywords = {App},
	Note = {PMCID: PMC2748134},
	Number = {3},
	Pages = {937--945},
	Title = {Using Regression Models to Analyze Randomized Trials: asymptotically Valid Hypothesis Tests Despite Incorrectly Specified Models},
	Volume = {65},
	Year = {2009}}

@book{Hampeletal86,
	Address = {New York},
	Author = {Hampel, F.R. and Ronchetti, E.M. and Rousseeuw, P.J. and Stahel, W.A.},
	Publisher = {Wiley},
	Title = {{Robust statistics: the approach based on influence functions}},
	Year = {1986}}

@book{vanderVaart98,
	Address = {New York},
	Author = {A.W. van der Vaart},
	Publisher = {Cambridge},
	Title = {Asymptotic statistics},
	Year = {1998}}

@book{vanderVaartWellner1996,
	Address = {Berlin Heidelberg New York},
	Author = {A.W. van der Vaart and J.A. Wellner},
	Date-Modified = {2012-08-24 12:13:06 -0700},
	Publisher = {Springer},
	Title = {Weak convergence and empirical processes},
	Year = {1996}}

@article{Rosenbaum&Rubin83,
	Author = {P.R. Rosenbaum and Donald B. Rubin},
	Journal = {Biometrika},
	Pages = {41--55},
	Title = {The central role of the propensity score in observational studies for causal effects},
	Volume = {70},
	Year = {1983}}

@article{Stitelman2010ctmle,
	Author = {O.M. Stitelman and M.J. van der Laan},
	Date-Modified = {2012-08-24 11:27:04 -0700},
	Journal = {Int J Biostat},
	Keywords = {TMLE},
	Note = {PMID: 21969976},
	Number = {1},
	Pages = {Article 21},
	Title = {Collaborative targeted maximum likelihood for time to event data},
	Volume = {6},
	Year = {2010}}

@article{Wedderburn74,
	Author = {R.W.M. Wedderburn},
	Journal = {Biometrika},
	Number = {3},
	Pages = {439--447},
	Title = {Quasi-likelihood functions, generalized linear models, and the Gauss-Newton method},
	Volume = {61},
	Year = {1974}}

@article{McCullagh83,
	Author = {P. Mc{C}ullagh},
	Journal = {Ann Stat},
	Pages = {59--67},
	Title = {Quasi-likelihood functions},
	Volume = {11},
	Year = {1983}}

@article{vanderLaan2008de,
	Author = {M.J. van der Laan and M.L. Petersen},
	Date-Modified = {2012-08-24 13:46:46 -0700},
	Journal = {Int J Biostat},
	Keywords = {NDE},
	Note = {PMID: 22462121},
	Number = {1},
	Pages = {Article 23},
	Title = {Direct effect models},
	Volume = {4},
	Year = {2008}}

@techreport{vanderLaan2010community,
	Author = {M.J. van der Laan},
	Date-Modified = {2012-08-26 21:16:04 -0700},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Keywords = {Community},
	Note = {Available at \url{http://biostats.bepress.com/ucbbiostat/paper268/}},
	Number = {268},
	Title = {Estimation of Causal Effects of Community-Based Interventions},
	Year = {2010}}

@article{Heckman&Ichimura&Todd97,
	Author = {J. Heckman and H. Ichimura and R. Todd},
	Journal = {Rev of Econ Stud},
	Pages = {605--654},
	Title = {Matching as an Econometric Evaluation Estimator: evidence from Evaluating a Job Training Programme},
	Volume = {64},
	Year = {1997}}

@techreport{Sekhon06,
	Author = {J.S. Sekhon},
	Institution = {University of California, Berkeley},
	Title = {Alternative balance metrics for bias reduction in matching methods for causal inference},
	Type = {Technical {R}eport},
	Year = {2006}}

@article{Hansen08,
	Author = {B.B. Hansen},
	Journal = {Biometrika},
	Pages = {481--8},
	Title = {The prognostic analogue of the propensity score},
	Volume = {95},
	Year = {2008}}

@book{Haignere02,
	Address = {Washington, DC},
	Author = {Haignere, L.},
	Edition = {2nd},
	Publisher = {American Association of University Professors},
	Title = {Paychecks: a guide to conducting salary-equity studies for higher education faculty},
	Year = {2002}}

@article{Holland88,
	Author = {P.W. Holland},
	Journal = {Stat Sci},
	Number = {2},
	Pages = {186--188.},
	Title = {Comment: Causal Mechanism or Causal Effect: which Is Best for Statistical Science?},
	Volume = {3},
	Year = {1988}}

@article{Robins98,
	Author = {J.M. Robins},
	Journal = {1997 Proceedings of the American Statistical Association. Section on {B}ayesian Statistical Science},
	Pages = {1--10},
	Title = {Marginal Structural Models},
	Year = {1998}}

@article{Mossetal04,
	Author = {A.R. Moss and J.A. Hahn and S. Perry and E.D. Charlebois and D. Guzman and R.A. Clark and D.R. Bangsberg},
	Journal = {Clin Infect Dis},
	Number = {8},
	Pages = {1190--1198},
	Title = {Adherence to highly active antiretroviral therapy in the homeless population in {S}an {F}rancisco: a prospective study},
	Volume = {39},
	Year = {2004}}

@article{Bangsbergetal01,
	Author = {D.R. Bangsberg and F. Hecht and E.D. Charlebois and M. Chesney and A.R. Moss},
	Journal = {AIDS Behav},
	Pages = {275--281},
	Title = {Comparing Objectives Measures of Adherence to HIV Antiretroviral Therapy: electronic Medication Monitors and Unannounced Pill Counts.},
	Volume = {5},
	Year = {2001}}

@article{Neugebauer2007,
	Author = {R. Neugebauer and M. J. van der Laan},
	Date-Modified = {2012-08-26 20:45:08 -0700},
	Journal = {J Stat Plan Infer},
	Keywords = {Roadmap + MSM},
	Number = {2},
	Pages = {419--434},
	Title = {Nonparametric causal effects based on marginal structural models},
	Volume = {137},
	Year = {2007},
	Bdsk-Url-1 = {http://www.sciencedirect.com/science/article/pii/S0378375806000334}}

@article{Efron87,
	Author = {B. Efron},
	Journal = {J Am Stat Assoc},
	Number = {397},
	Pages = {171--185},
	Title = {Better Bootstrap Confidence Intervals},
	Volume = {82},
	Year = {1987}}

@article{Kirschetal08,
	Author = {I. Kirsch and B.J. Deacon and T.B. Huedo-Medina and A. Scoboria and T.J. Moore and B.T. Johnson},
	Journal = {PLoS Med},
	Number = {2},
	Pages = {e45. doi:10.1371/journal.pmed.0050045},
	Title = {Initial Severity and Antidepressant Benefits: a Meta-Analysis of Data Submitted to the {Food and Drug Administration}},
	Volume = {5},
	Year = {2008}}

@article{Baselga01,
	Author = {J. Baselga},
	Journal = {Oncology},
	Pages = {14--21},
	Title = {Herceptin alone or in combination with chemotherapy in the treatment of {HER2}-positive metastatic breast cancer: pivotal trials},
	Volume = {61(S2)},
	Year = {2001}}

@techreport{Wangetal06,
	Author = {Y. Wang and M.L. Petersen and D.R. Bangsberg and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {211},
	Title = {Diagnosing Bias in the Inverse Probability of Treatment Weighted Estimator Resulting from Violation of Experimental Treatment Assignment.},
	Year = {2006}}

@article{Robins87,
	Author = {Robins, J.M.},
	Journal = {Comput Math Appl},
	Number = {9--12},
	Pages = {923--945},
	Title = {Addendum to: ``{A} new approach to causal inference in mortality studies with a sustained exposure period---application to control of the healthy worker survivor effect''},
	Volume = {14},
	Year = {1987}}

@article{Robins872,
	Author = {J.M. Robins},
	Journal = {J Chron Dis (40, Supplement)},
	Pages = {139s--161s},
	Title = {A graphical approach to the identification and estimation of causal parameters in mortality studies with sustained exposure periods},
	Volume = {2},
	Year = {1987}}

@article{Rosenblum&vanderLaan09b,
	Author = {M. Rosenblum and M.J. van der Laan},
	Journal = {Int J Biostat},
	Pages = {Article 4},
	Title = {Confidence Intervals for the Population Mean Tailored to Small Sample Sizes, with Applications to Survey Sampling},
	Volume = {1},
	Year = {2009}}

@article{Neugebauer2005,
	Author = {Neugebauer, R. and van der Laan, M.J.},
	Date-Modified = {2012-08-26 21:21:41 -0700},
	Journal = {J Stat Plan Infer},
	Number = {1-2},
	Pages = {405--26},
	Title = {Why prefer double robust estimates in causal inference?},
	Volume = {129},
	Year = {2005}}

@techreport{Mooreetal09,
	Author = {K.L. Moore and R.S. Neugebauer and M.J. van der Laan and I.B. Tager},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {255},
	Title = {Causal Inference in Epidemiological Studies with Strong Confounding},
	Year = {2009}}

@article{Kish92,
	Author = {L. Kish},
	Journal = {J Off Stat},
	Pages = {183--200},
	Title = {Weighting for unequal $P_i$},
	Volume = {8},
	Year = {1992}}

@techreport{Bembom2008,
	Author = {O. Bembom and M.J. van der Laan},
	Date-Modified = {2012-08-26 21:02:51 -0700},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Keywords = {Aim1},
	Note = {Available at \url{http://biostats.bepress.com/ucbbiostat/paper230}},
	Number = {230},
	Title = {Data-adaptive selection of the truncation level for Inverse-Probability-of-Treatment-Weighted estimators},
	Year = {2008},
	Bdsk-Url-1 = {http://biostats.bepress.com/ucbbiostat/paper230}}

@article{Freedman&Berk08,
	Author = {D.A. Freedman and R.A. Berk},
	Journal = {Eval Rev},
	Pages = {392--409},
	Title = {Weighting Regressions by Propensity Scores},
	Volume = {3},
	Year = {2008}}

@article{Petersenetal10,
	Author = {M.L. Petersen and K.E. Porter and S. Gruber and Y. Wang and M.J. van der Laan},
	Journal = {Stat Meth Med Res},
	Title = {Diagnosing and responding to violations in the positivity assumption},
	Volume = {published online 28 Oct (doi: 10.1177/0962280210386207)},
	Year = {2010}}

@article{Johnsonetal09,
	Author = {V.A. Johnson and F. Brun-Vezinet and B. Clotet and H.F. Gunthard and D.R. Kuritzkes and D. Pillay and J.M. Schapiro and D.D. Richman},
	Journal = {Top HIV Med},
	Number = {5},
	Pages = {138--45},
	Title = {Update of the drug resistance mutations in {HIV}-1: {D}ecember 2009.},
	Volume = {17},
	Year = {2009}}

@techreport{Bembometal08b,
	Author = {O. Bembom and W.J. Fessel and R.W. Shafer and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Title = {Data-adaptive Selection Of The Adjustment Set In Variable Importance Estimation},
	Type = {231},
	Year = {2008}}

@techreport{Crumpetal06,
	Author = {R.K. Crump and V.J. Hotz and G.W. Imbens and O.A. Mitnik},
	Institution = {National Bureau of Economic Research},
	Number = {330},
	Title = {Moving the goalposts: addressing limited overlap in the estimation of average treatment effects by changing the estimand},
	Year = {2006}}

@article{LaLonde86,
	Author = {R.J. LaLonde},
	Journal = {Am Econ Rev},
	Pages = {604--620},
	Title = {Evaluating the Econometric Evaluations of Training Programs with Experimental Data},
	Volume = {76},
	Year = {1986}}

@article{Dehejia&Wahba99,
	Author = {R. Dehejia and S. Wahba},
	Journal = {J Am Stat Assoc},
	Pages = {1053--1062},
	Title = {Causal Effects in Nonexperimental Studies: reevaluating the Evaluation of Training Programs},
	Volume = {94},
	Year = {1999}}

@article{vanderLaan2007indvtxt,
	Author = {M.J. van der Laan and M.L. Petersen},
	Date-Modified = {2012-08-26 20:33:40 -0700},
	Journal = {Int J Biostat},
	Keywords = {Aim1},
	Note = {PMCID: PMC2613338},
	Number = {1},
	Pages = {Article 3},
	Title = {Causal Effect Models for Realistic Individualized Treatment and Intention to Treat Rules},
	Volume = {3},
	Year = {2007}}

@article{Robins2008,
	Author = {J.M. Robins and L. Orellana and A. Rotnitzky},
	Date-Modified = {2012-08-22 21:31:41 -0700},
	Journal = {Stat Med},
	Keywords = {Aim1},
	Note = {PMID: 18646286},
	Number = {23},
	Pages = {4678--4721},
	Title = {Estimation and extrapolation of optimal treatment and testing strategies},
	Volume = {27},
	Year = {2008}}

@article{Cochran57,
	Author = {W.G. Cochran},
	Journal = {Biometrics},
	Pages = {261--281},
	Title = {Analysis of Covariance: its Nature and Uses.},
	Volume = {13},
	Year = {1957}}

@techreport{Moore&vanderLaan07,
	Author = {K.L. Moore and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Month = {April},
	Number = {215},
	Title = {Covariate adjustment in randomized trials with binary outcomes},
	Year = {2007}}

@article{Rosenblum2010b,
	Author = {M. Rosenblum and M.J. van der Laan},
	Date-Modified = {2012-08-26 00:37:20 -0700},
	Journal = {Int J Biostat},
	Keywords = {Application},
	Note = {PMCID: PMC2898625},
	Number = {1},
	Pages = {Article 13},
	Title = {Simple, Efficient Estimators of Treatment Effects in Randomized Trials Using Generalized Linear Models to Leverage Baseline Variables},
	Volume = {6},
	Year = {2010}}

@article{Freedman083,
	Author = {D.A. Freedman},
	Journal = {Stat Sci},
	Pages = {237--249},
	Title = {Randomization does not justify logistic regression},
	Volume = {23},
	Year = {2008}}

@article{Yang&Tsiatis01,
	Author = {L. Yang and A.A. Tsiatis},
	Journal = {Am Stat},
	Pages = {29--38},
	Title = {Efficiency study for a treatment effect in a pretest-posttest trial},
	Volume = {56},
	Year = {2001}}

@book{McCullagh&Nelder89,
	Address = {Boca Raton},
	Author = {P. McCullagh and J.A. Nelder},
	Edition = {2nd},
	Publisher = {Chapman \& Hall},
	Title = {Generalized linear models},
	Year = {1989}}

@incollection{Gail86,
	Address = {New York},
	Author = {M.H. Gail},
	Booktitle = {Modern Statistical Methods in Chronic Disease Epidemiology},
	Editor = {S.~H. Moolvankar and R.~L. Prentice},
	Publisher = {Wiley},
	Title = {Adjusting for covariates that have the same distribution in exposed and unexposed cohorts},
	Year = {1986}}

@article{Tsiatisetal08,
	Author = {A.A. Tsiatis and M. Davidian and M. Zhang and X. Lu},
	Journal = {Stat Med},
	Pages = {4658--4677},
	Title = {Covariate adjustment for two-sample treatment comparisons in randomized clinical trials: a principled yet flexible approach},
	Volume = {27},
	Year = {2008}}

@article{Kochetal98,
	Author = {G.G. Koch and C.M. Tangen and J.W. Jung and I.A. Amara},
	Journal = {Stat Med},
	Pages = {1863--1892},
	Title = {Issues for covariance analysis of dichotomous and ordered categorical data from randomized clinical trials and nonparametric strategies for addressing them},
	Volume = {17},
	Year = {1998}}

@article{Pococketal02,
	Author = {S.J. Pocock and S.E. Assmann and L.E. Enos and L.E. Kasten},
	Journal = {Stat Med},
	Pages = {2917--2930},
	Title = {Subgroup analysis, covariate adjustment, and baseline comparisons in clinical trial reporting: current practice and problems.},
	Volume = {21},
	Year = {2002}}

@article{Anderson72,
	Author = {J.A. Anderson},
	Journal = {Biometrika},
	Pages = {19--35},
	Title = {Separate sample logistic discrimination},
	Volume = {59},
	Year = {1972}}

@article{Robins99,
	Author = {J.M. Robins},
	Journal = {Stat Sci},
	Number = {3},
	Pages = {281--293},
	Title = {[{C}hoice as an Alternative to Control in Observational Studies]: Comment},
	Volume = {14},
	Year = {1999}}

@article{Manssonetal07,
	Author = {R. Mansson and M.M. Joffe and W. Sun and S. Hennessy},
	Journal = {Am J Epidemiol},
	Number = {3},
	Pages = {332-339},
	Title = {On the Estimation and Use of Propensity Scores in Case-Control and Case-Cohort Studies.},
	Volume = {166},
	Year = {2007}}

@article{Prentice&Pyke79,
	Author = {R.L. Prentice and R. Pyke},
	Journal = {Biometrika},
	Pages = {403--411},
	Title = {Logistic disease incidence models and case-control studies},
	Volume = {66},
	Year = {1979}}

@book{Breslow&Day80,
	Address = {Lyon},
	Author = {N.E. Breslow and N.E. Day},
	Publisher = {International Agency for Research on Cancer},
	Title = {Statistical methods in cancer research: {V}olume 1 -- {T}he analysis of case-control studies},
	Year = {1980}}

@article{Breslow96,
	Author = {N.E. Breslow},
	Journal = {J Am Stat Soc},
	Pages = {14--28},
	Title = {Statistics in Epidemiology: the Case-Control Study},
	Volume = {91},
	Year = {1996}}

@article{Greenland81,
	Author = {S. Greenland},
	Journal = {J Chron Dis},
	Pages = {445--453},
	Title = {Multivariate Estimation of Exposure-Specific Incidence from Case-Control Studies.},
	Volume = {34},
	Year = {1981}}

@incollection{Holland&Rubin88,
	Address = {Cambridge, MA},
	Author = {P.W. Holland and Donald B. Rubin},
	Booktitle = {Matched sampling for causal effects.},
	Editor = {Donald B. Rubin},
	Publisher = {Cambridge},
	Title = {Causal inference in retrospective studies},
	Year = {1988}}

@article{Greenland04,
	Author = {S. Greenland},
	Journal = {Am J Epidemiol},
	Number = {4},
	Pages = {301--305},
	Title = {Model-based Estimation of Relative Risks and Other Epidemiologic Measures in Studies of Common Outcomes and in Case-Control Studies.},
	Volume = {160},
	Year = {2004}}

@article{Newman06,
	Author = {S. Newman},
	Journal = {Epid Persp Innov},
	Pages = {2},
	Title = {Causal analysis of case-control data},
	Volume = {3},
	Year = {2006}}

@article{Cornfield51,
	Author = {J. Cornfield},
	Journal = {J Nat Cancer Inst},
	Pages = {1269--1275},
	Title = {A method of estimating comparative rates from clinical data. Applications to cancer of the lung, breast, and cervix.},
	Volume = {11},
	Year = {1951}}

@inproceedings{Cornfield56,
	Address = {Berkeley},
	Author = {J. Cornfield},
	Booktitle = {Proceedings of the 3rd Berkeley symposium, {V}ol IV},
	Editor = {J. Neyman},
	Publisher = {University of California Press},
	Title = {A statistical problem arising from retrospective studies},
	Year = {1956}}

@article{Prentice&Breslow78,
	Author = {R.L. Prentice and N.E. Breslow},
	Journal = {Biometrika},
	Number = {1},
	Pages = {153--158},
	Title = {Retrospective studies and failure time models.},
	Volume = {65},
	Year = {1978}}

@article{Moriseetal96,
	Author = {A.P. Morise and G.A. Diamon and R. Detrano and M. Bobbio and Erdogan Gunel},
	Journal = {Med Decis Making},
	Pages = {133--142},
	Title = {The Effect of Disease-prevalence Adjustments on the Accuracy of a Logistic Prediction Model.},
	Volume = {16},
	Year = {1996}}

@article{Wacholder96,
	Author = {S. Wacholder},
	Journal = {Epidemiol},
	Number = {2},
	Pages = {144--150},
	Title = {The Case-Control Study as Data Missing by Design: estimating Risk Differences.},
	Volume = {7},
	Year = {1996}}

@article{Rose2011,
	Author = {S. Rose and M.J. van der Laan},
	Date-Modified = {2012-08-26 00:49:30 -0700},
	Journal = {Int J Biostat},
	Keywords = {App},
	Note = {PMCID: PMC3083136},
	Number = {17},
	Title = {A Targeted Maximum Likelihood Estimator for Two-Stage Designs},
	Volume = {7},
	Year = {2011}}

@article{Freedman50,
	Author = {R. Freedman},
	Journal = {Am J of Soc},
	Number = {5},
	Pages = {485--487},
	Title = {Incomplete Matching in Ex Post Facto Studies},
	Volume = {55},
	Year = {1950}}

@article{Cochran65,
	Author = {W.G. Cochran},
	Journal = {J R Stat Soc Ser A Gen},
	Number = {2},
	Pages = {234--266},
	Title = {The Planning of Observational Studies of Human Populations},
	Volume = {128},
	Year = {1965}}

@article{Billewicz65,
	Author = {W.Z. Billewicz},
	Journal = {Biometrics},
	Number = {3},
	Pages = {623--644},
	Title = {The Efficiency of Matched Samples: an Empirical Investigation},
	Volume = {21},
	Year = {1965}}

@article{McKinlay77,
	Author = {S.M. McKinlay},
	Journal = {Biometrics},
	Number = {4},
	Pages = {725--735},
	Title = {Pair-Matching -- A reappraisal of a Popular Technique},
	Volume = {33},
	Year = {1977}}

@article{Kupperetal81,
	Author = {L.L. Kupper and J.M. Karon and D.G. Kleinbaum and H. Morgenstern and D.K. Lewis},
	Journal = {Biometrics},
	Pages = {271--291},
	Title = {Matching in Epidemiologic Studies: validity and Efficiency Considerations},
	Volume = {37},
	Year = {1981}}

@article{Costanza95,
	Author = {M.C. Costanza},
	Journal = {Prev Med},
	Pages = {425--433},
	Title = {Matching},
	Volume = {24},
	Year = {1995}}

@book{Schlesselman82,
	Address = {Oxford},
	Author = {J.J. Schlesselman},
	Publisher = {Oxford},
	Title = {Case-control studies: design, conduct, analysis},
	Year = {1982}}

@article{Vandenbroukeetal07,
	Author = {J.P. Vandenbrouke and E. von Elm and D.G. Altman and P.C. Gotzsche and C.D. Mulrow and S.J. Pocock and C. Poole and J.J. Schlesselman and M. Egger for the STROBE Initiative},
	Journal = {PLoS Med},
	Number = {10},
	Pages = {1628--1654},
	Title = {Strengthening the Reporting of Observational Studies in Epidemiology ({STROBE}): explanation and Elaboration.},
	Volume = {4},
	Year = {2007}}

@article{Cochran53,
	Author = {W.G. Cochran},
	Journal = {Am J Public Health},
	Pages = {684--691},
	Title = {Matching in Analytical Studies},
	Volume = {43},
	Year = {1953}}

@article{Breslowetal78,
	Author = {N.E. Breslow and N.E. Day and K.T. Halvorsen and R.L. Prentice and C. Sabal},
	Journal = {Am J Epidemiol},
	Number = {4},
	Pages = {299--307},
	Title = {Estimation of Multiple Relative Risk Functions in Matched Case-Control Studies},
	Volume = {108},
	Year = {1978}}

@article{Holford&White&Kelsey78,
	Author = {T.R. Holford and C. White and J.L. Kelsey},
	Journal = {Am J Epidemiol},
	Number = {3},
	Pages = {245--255},
	Title = {Multivariate Analysis for Matched Case-Control Studies},
	Volume = {107},
	Year = {1978}}

@article{Kannel&McGee&Gordon76,
	Author = {W.B. Kannel and D. McGee and T. Gordon},
	Journal = {Am J Cardiol},
	Pages = {46--51},
	Title = {A general cardiovascular risk profile: the {F}ramingham Study},
	Volume = {38},
	Year = {1976}}

@article{Andersonetal91,
	Author = {K.M. Anderson and P.W.F. Wilson and P.M. Odell and W.B. Kannel},
	Journal = {Circulation},
	Pages = {356--362},
	Title = {An updated coronary risk profile. A statement for health professionals.},
	Volume = {83},
	Year = {1991}}

@article{Ramsayetal95,
	Author = {L.E. Ramsay and I.U. Haq and P.R. Jackson and W.W. Yeo},
	Journal = {Lancet},
	Number = {8988},
	Pages = {1467--1471},
	Title = {Sheffield risk and treatment table for cholesterol lowering for primary prevention of coronary heart disease.},
	Volume = {346},
	Year = {1995}}

@article{Ramsayetal96,
	Author = {L.E. Ramsay and I.U. Haq and P.R. Jackson and W.W. Yeo},
	Journal = {Lancet},
	Number = {9036},
	Pages = {1251},
	Title = {The {S}heffield table for primary prevention of coronary heart disease: corrected.},
	Volume = {348},
	Year = {1996}}

@article{Wilsonetal98,
	Author = {P.W.F. Wilson and R.B. D'Agostino and D. Levy and A.M. Belanger and H. Silbershatz and W.B. Kannel},
	Journal = {Circulation},
	Pages = {1837--1847},
	Title = {Prediction of coronary heart disease using risk factor categories},
	Volume = {97},
	Year = {1998}}

@article{Jackson00,
	Author = {R. Jackson},
	Journal = {Br Med J},
	Number = {7236},
	Pages = {709--710},
	Title = {Updated New Zealand cardiovascular disease risk-benefit prediction guide.},
	Volume = {320},
	Year = {2000}}

@article{Gailetal89,
	Author = {M.H. Gail and L.A. Brinton and D.P. Byar and D.K. Corle and S.B. Green and C. Schairer and J.J. Mulvihill},
	Journal = {J Natl Cancer Inst},
	Number = {24},
	Pages = {1879--1886},
	Title = {Projecting individualized probabilities of developing breast cancer for white females who are being examined annually.},
	Volume = {81},
	Year = {1989}}

@article{Costantinoetal99,
	Author = {J.P. Costantino and M.H. Gail and D. Pee and S. Anderson and C.K. Redmond and J. Benichou and H.S. Wieand},
	Journal = {J Natl Cancer Inst},
	Number = {18},
	Pages = {1541--1548},
	Title = {Validation studies for models projecting the risk of invasive and total breast cancer incidence.},
	Volume = {91},
	Year = {1999}}

@article{Tyrer&Duffy&Cuzick04,
	Author = {J. Tyrer and S.W. Duffy and J. Cuzick},
	Journal = {Stat Med},
	Number = {7},
	Pages = {1111--1130},
	Title = {A breast cancer prediction model incorporating familial and personal risk factors},
	Volume = {23},
	Year = {2004}}

@article{Barlowetal06,
	Author = {W.E. Barlow and E. White and R. Ballard-Barbash and P.M. Vacek and L. Titus-Ernstoff and P.A. Carney and J.A. Tice and D.S. Buist and B.M. Geller and R. Rosenberg and B.C. Yankaskas and K. Kerlikowske},
	Journal = {J Natl Cancer Inst},
	Number = {17},
	Pages = {1204--1214},
	Title = {Prospective breats cancer risk prediction model for women undergoing screening mammography.},
	Volume = {98},
	Year = {2006}}

@article{Loprinzietal94,
	Author = {C.L. Loprinzi and J.A. Laurie and H.S. Wieand and J.E. Krook and P.J. Novotny and J.W. Kugler and J. Bartel and M. Law and M. Bateman and N.E. Klatt},
	Journal = {J Clin Oncol},
	Number = {3},
	Pages = {601--607},
	Title = {Prospective Evaluation of Prognostic Variables from Patient-Completed Questionnaires, {N}orth {C}entral {C}ancer {T}reatment {G}roup},
	Volume = {12},
	Year = {1994}}

@manual{Therneau&Lumley09,
	Author = {T. Therneau and T. Lumley},
	Note = {R package version 2.35-8},
	Title = {survival: survival analysis, including penalised likelihood},
	Url = {http://CRAN.R-project.org/package=survival},
	Year = {2009},
	Bdsk-Url-1 = {http://CRAN.R-project.org/package=survival}}

@article{Tibshirani97,
	Author = {R.J. Tibshirani},
	Journal = {Stat Med},
	Pages = {385--395},
	Title = {The Lasso Method for Variable Selection in the {C}ox Model},
	Volume = {16},
	Year = {1997}}

@article{Zhang&Lu07,
	Author = {H.H. Zhang and W. Lu},
	Journal = {Biometrika},
	Number = {3},
	Pages = {691--703},
	Title = {Adaptive Lasso for {C}ox's Proportional Hazards Model},
	Volume = {94},
	Year = {2007}}

@article{Kooperberg&Stone&Truong95,
	Author = {C. Kooperberg and C.J. Stone and Y.K. Truong},
	Journal = {J Am Stat Assoc},
	Number = {429},
	Pages = {78--94},
	Title = {Hazard Regression},
	Volume = {90},
	Year = {1995}}

@article{Leblanc&Crowley92,
	Author = {M. LeBlanc and J. Crowley},
	Journal = {Biometrics},
	Pages = {411--425},
	Title = {Relative Risk trees for censored data},
	Volume = {48},
	Year = {1992}}

@article{Segal88,
	Author = {M.R. Segal},
	Journal = {Biometrics},
	Pages = {35--47},
	Title = {Regression trees for censored data},
	Volume = {44},
	Year = {1988}}

@article{Hothornetal06,
	Author = {T. Hothorn and P. Buhlmann and S. Dudoit and A.M. Molinaro and M.J. van der Laan},
	Journal = {Biostatistics},
	Pages = {355--373},
	Title = {Survival Ensembles},
	Volume = {7},
	Year = {2006}}

@article{Ishwaranetal08,
	Author = {H. Ishwaran and U.B. Kogalur and E.H. Blackstone and M.S. Lauer},
	Journal = {Ann Appl Stat},
	Number = {3},
	Pages = {841--860},
	Title = {Random Survival Forests},
	Volume = {2},
	Year = {2008}}

@article{vanHouwelingenetal06,
	Author = {H.C. van Houwelingen and T. Bruinsma and A.A.M. Hart and L.J. {van't Veer} and L.F.A. Wessels},
	Journal = {Stat Med},
	Pages = {3201--3216},
	Title = {Cross-validated {C}ox Regression on Microarray Gene Expression Data},
	Volume = {25},
	Year = {2006}}

@techreport{vanderLaan&Rubin07,
	Author = {M.J. van der Laan and Daniel B. Rubin},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {226},
	Title = {A note on targeted maximum likelihood and right-censored data},
	Year = {2007}}

@inproceedings{Robins93,
	Author = {J.M. Robins},
	Booktitle = {Proceedings of the Biopharmaceutical Section},
	Organization = {American Statistical Association},
	Title = {Information recovery and bias adjustment in proportional hazards regression analysis of randomized trials using surrogate markers},
	Year = {1993}}

@incollection{Hubbard&vanderLaan&Robins99,
	Address = {Berlin Heidelberg New York},
	Author = {A.E. Hubbard and M.J. van der Laan and J.M. Robins},
	Booktitle = {Statistical models in epidemiology: the environment and clinical trials},
	Editor = {E. Halloran, D. Berry},
	Publisher = {Springer},
	Title = {Nonparametric locally efficient estimation of the treatment specific survival distributions with right censored data and covariates in observational studies},
	Year = {1999}}

@article{Hernandez&Eijkemans&Steyerberg06,
	Author = {Hern\'{a}ndez, A.V. and Eijkemans, M.J. and Steyerberg, E.W.},
	Journal = {Ann Epidemiol},
	Number = {1},
	Pages = {41--48},
	Title = {Randomized controlled trials With time-to-event outcomes: how much does prespecified covariate adjustment increase power?},
	Volume = {16},
	Year = {2006}}

@article{Lu&Tsiatis08,
	Author = {Lu, X. and Tsiatis, A.A},
	Journal = {Biometrika},
	Number = {3},
	Pages = {679--694},
	Title = {Improving the efficiency of the log-rank test using auxiliary covariates},
	Volume = {95},
	Year = {2008}}

@article{Tangen&Koch99,
	Author = {Tangen, C.M. and Koch, G.G.},
	Journal = {J Biopharm Stat},
	Number = {2},
	Pages = {307--338},
	Title = {On-parametric analysis of covariance for hypothesis testing with logrank and {W}ilcoxon scores and survival-rate estimation in a randomized clinical trial},
	Volume = {9},
	Year = {1999}}

@article{Jiangetal08,
	Author = {Jiang, H. and Symanowski, J. and Paul, S. and Qu, Y. and Zagar, A. and Hong, S.},
	Journal = {Stat Med},
	Number = {28},
	Pages = {5850--5860},
	Title = {The type {I} error and power of nonparametric logrank and {W}ilcoxon tests with adjustment for covariates -- A simulation study},
	Volume = {27},
	Year = {2008}}

@article{Akazawa&Nakamura&Palesch97,
	Author = {Akazawa, K. and Nakamura, T. and Palesch, Y.},
	Journal = {Stat Med},
	Number = {5},
	Pages = {583--597},
	Title = {Power of logrank test and {C}ox regression model in clinical trials with heterogenous samples},
	Volume = {16},
	Year = {1997}}

@article{Westeretal10,
	Author = {C.W. Wester and A.M. Thomas and H. Bussmann and S. Moyo and J.M. Gaolathe and V. Novitsky and M. Essex and V. De Gruttola and R.G. Marlink},
	Journal = {AIDS},
	Pages = {S27--S36},
	Title = {Nonnucleoside reverse transcriptase inhibitor outcomes among combination antiretroviral therapy-treated adults in {B}otswana},
	Volume = {24},
	Year = {2010}}

@book{Andersenetal93,
	Address = {Berlin Heidelberg New York},
	Author = {P.K. Andersen and O. Borgan and R.D. Gill and N. Keiding},
	Publisher = {Springer},
	Title = {Statistical models based on counting processes},
	Year = {1993}}

@techreport{Rudser&LeBlanc&Emerson08,
	Author = {K. Rudser and M. LeBlanc and S.S. Emerson},
	Institution = {Department of Biostatistics, University of Washington},
	Number = {335},
	Title = {Estimation for Arbitrary Functionals of Survival},
	Year = {2008}}

@article{vanderLaan10,
	Author = {van der Laan, M.J.},
	Date-Modified = {2012-08-24 10:54:39 -0700},
	Journal = {Int J Biostat},
	Keywords = {tmle},
	Note = {PMID: 21969992},
	Number = {2},
	Pages = {Article 2},
	Title = {Targeted maximum likelihood based causal inference: Part {I}},
	Volume = {6},
	Year = {2010}}

@article{vanderLaan10b,
	Author = {van der Laan, M.J.},
	Date-Modified = {2012-08-24 10:54:44 -0700},
	Journal = {Int J Biostat},
	Keywords = {tmle},
	Note = {PMCID: PMC3126672},
	Number = {2},
	Pages = {Article 3},
	Title = {Targeted maximum likelihood based causal inference: Part {II}},
	Volume = {6},
	Year = {2010}}

@article{Sekhon08,
	Author = {J.S. Sekhon},
	Journal = {J Stat Softw},
	Title = {Multivariate and Propensity Score Matching Software with Automated Balance Optimization: the Matching package for {R}},
	Year = {2008}}

@article{Holland&Reitman77,
	Address = {New York},
	Author = {J.H. Holland and J.S. Reitman},
	Journal = {SIGART Bull},
	Pages = {49--49},
	Title = {Cognitive systems based on adaptive algorithms},
	Volume = {63},
	Year = {1977}}

@article{Koul&Susarla&vanRyzin81,
	Author = {H. Koul and V. Susarla and J. van Ryzin},
	Journal = {Ann Stat},
	Pages = {1276--88},
	Title = {Regression analysis with randomly right censored data},
	Volume = {9},
	Year = {1981}}

@article{Keiding&Hols&Green89,
	Author = {N. Keiding and C. Hols and A. Green},
	Journal = {Am J Epidemiol},
	Pages = {588--600},
	Title = {Retrospective estimation of diabetes incidence from information in a current prevalent population and historical mortality},
	Volume = {130},
	Year = {1989}}

@article{Robins&Rotnitzky&Zhao94,
	Author = {J.M. Robins and A. Rotnitzky and L.P. Zhao},
	Journal = {J Am Stat Assoc},
	Month = {September},
	Number = {427},
	Pages = {846--66},
	Title = {Estimation of regression coefficients when some regressors are not always observed},
	Volume = {89},
	Year = {1994}}

@article{Robins&Rotnitzky95,
	Author = {Robins, J.M. and A. Rotnitzky},
	Journal = {J Am Stat Assoc},
	Pages = {122--129},
	Title = {Semiparametric Efficiency in Multivariate Regression Models with Missing Data},
	Volume = {90},
	Year = {1995}}

@article{Kang&Schafer07,
	Author = {J. Kang and J.L. Schafer},
	Journal = {Stat Sci},
	Pages = {523--39},
	Title = {Demystifying Double Robustness: a Comparison of Alternative Strategies for Estimating a Population Mean from Incomplete Data (with discussion)},
	Volume = {22},
	Year = {2007}}

@article{Robins&Wang00,
	Author = {J.M. Robins and N. Wang},
	Journal = {Biometrika},
	Pages = {113--124},
	Title = {Inference for imputation estimators},
	Volume = {87},
	Year = {2000}}

@techreport{Bhattacharya&Vogt07,
	Author = {Bhattacharya, J. and Vogt, W.},
	Institution = {National Bureau of Economic Research},
	Number = {343},
	Title = {Do Instrumental Variables Belong in Propensity Scores?},
	Year = {2007}}

@techreport{Wooldridge09,
	Author = {Wooldridge, J.},
	Institution = {Michigan State University},
	Title = {Should Instrumental Variables be Used as Matching Variables?},
	Type = {Technical {R}eport},
	Year = {2009}}

@article{Pearl10,
	Author = {Pearl, J.},
	Journal = {Proceedings of Uncertainty in Artificial Intelligence},
	Title = {On a Class of Bias-Amplifying Variables that Endanger Effect Estimates},
	Year = {2010}}

@article{Holland86,
	Author = {Holland, P.W.},
	Journal = {J Am Stat Assoc},
	Number = {396},
	Pages = {945--960},
	Title = {Statistics and Causal Inference},
	Volume = {81},
	Year = {1986}}

@book{Rubin06,
	Address = {Cambridge, MA},
	Author = {Donald B. Rubin},
	Publisher = {Cambridge},
	Title = {Matched sampling for causal effects.},
	Year = {2006}}

@book{Rosenbaum02,
	Address = {Berlin Heidelberg New York},
	Author = {Rosenbaum, P.R.},
	Edition = {2nd},
	Publisher = {Springer},
	Title = {Observational studies},
	Year = {2002}}

@article{Rubin97,
	Author = {Rubin, Donald B.},
	Journal = {Ann of Intern Med},
	Number = {8S},
	Pages = {757--763},
	Title = {Estimating causal effects from large data sets using propensity scores},
	Volume = {127},
	Year = {1997}}

@article{Christakis&Iwashyna03,
	Author = {Christakis, N.A. and Iwashyna, T.I.},
	Journal = {Soc Sci Med},
	Number = {3},
	Pages = {465--475},
	Title = {The Health Impact of Health Care on Families: a matched cohort study of hospice use by decedents and mortality outcomes in surviving, widowed spouses},
	Volume = {57},
	Year = {2003}}

@article{Dehejia&Wahba02,
	Author = {R. Dehejia and S. Wahba},
	Journal = {Rev Econ Stat},
	Number = {1},
	Pages = {151--161},
	Title = {Propensity Score Matching Methods for Nonexperimental Causal Studies},
	Volume = {84},
	Year = {2002}}

@article{Galiani&Gertler&Schargrodsky05,
	Author = {Galiani, S. and P. Gertler and E. Schargrodsky},
	Journal = {J Polit Econ},
	Number = {1},
	Pages = {83--120},
	Title = {Water for Life: the Impact of the Privatization of Water Services on Child Mortality},
	Volume = {113},
	Year = {2005}}

@article{Abadie&Imbens06,
	Author = {Abadie, A. and G.W. Imbens},
	Journal = {Econometrica},
	Pages = {235--267},
	Title = {Large Sample Properties of Matching Estimators for Average Treatment Effects},
	Volume = {74},
	Year = {2006}}

@article{Herron&Wand07,
	Author = {Herron, M.C. and J. Wand},
	Journal = {Elect Stud},
	Number = {2},
	Pages = {247--261},
	Title = {Assessing Partisan Bias in Voting Technology: the Case of the 2004 {N}ew {H}ampshire Recount},
	Volume = {26},
	Year = {2007}}

@article{Imai05,
	Author = {K. Imai},
	Journal = {Am Polit Sci Rev},
	Number = {2},
	Pages = {283--300},
	Title = {Do Get-Out-The-Vote Calls Reduce Turnout? The Importance of Statistical Methods for Field Experiments},
	Volume = {99},
	Year = {2005}}

@incollection{Sekhon08b,
	Address = {New York},
	Author = {Sekhon, J.S.},
	Booktitle = {The Oxford handbook of political methodology},
	Editor = {J.M. Box-Steffensmeier and H.E. Brady and D. Collier},
	Publisher = {Oxford},
	Title = {The {N}eyman-{R}ubin Model of Causal Inference and Estimation via Matching Methods},
	Year = {2008}}

@article{Morgan&Harding06,
	Author = {Morgan, S.L. and D.J. Harding},
	Journal = {Sociol Meth Res},
	Number = {1},
	Pages = {3--60},
	Title = {Matching Estimators of Causal Effects: prospects and Pitfalls in Theory and Practice},
	Volume = {35},
	Year = {2006}}

@article{Diprete&Engelhardt04,
	Author = {Diprete, T.A. and H. Engelhardt},
	Journal = {Sociol Meth Res},
	Number = {4},
	Pages = {501--528},
	Title = {Estimating Causal Effects With Matching Methods in the Presence and Absence of Bias Cancellation},
	Volume = {32},
	Year = {2004}}

@article{Winship&Morgan99,
	Author = {Winship, C. and S.L. Morgan},
	Journal = {Annu Rev Sociol},
	Pages = {659--707},
	Title = {The estimation of causal effects from observational data},
	Volume = {25},
	Year = {1999}}

@article{Smith97,
	Author = {Smith, H.L.},
	Journal = {Sociol Meth},
	Pages = {305--353},
	Title = {Matching with Multiple Controls to Estimate Treatment Effects in Observational Studies},
	Volume = {27},
	Year = {1997}}

@article{Rubin02,
	Author = {Rubin, Donald B.},
	Journal = {Health Serv Outcome Res Meth},
	Number = {1},
	Pages = {169--188},
	Title = {Using Propensity Scores to Help Design Observational Studies: application to the Tobacco Litigation},
	Volume = {2},
	Year = {2002}}

@incollection{Brady08,
	Address = {New York},
	Author = {Brady, H.},
	Booktitle = {The Oxford handbook of political methodology},
	Editor = {J.M. Box-Steffensmeier and H.E. Brady and D. Collier},
	Publisher = {Oxford},
	Title = {Causation and explanation in social science},
	Year = {2008}}

@article{Freedman06,
	Author = {Freedman, D.A.},
	Journal = {Eval Rev},
	Pages = {691--713},
	Title = {Statistical Models for Causation: what Inferential leverage Do They Provide?},
	Volume = {30},
	Year = {2006}}

@article{Rubin90,
	Author = {Rubin, Donald B.},
	Journal = {Stat Sci},
	Number = {4},
	Pages = {472--480},
	Title = {Comment: {N}eyman (1923) and Causal Inference in Experiments and Observational Studies},
	Volume = {5},
	Year = {1990}}

@article{Speed90,
	Author = {T.P. Speed},
	Journal = {Stat Sci},
	Number = {4},
	Pages = {463--464},
	Title = {Introductory Remarks on {N}eyman (1923)},
	Volume = {5},
	Year = {1990}}

@book{Cox58,
	Address = {New York},
	Author = {Cox, D.R.},
	Publisher = {Wiley},
	Title = {Planning of experiments},
	Year = {1958}}

@article{Rubin78,
	Author = {Donald B. Rubin},
	Journal = {Ann Stat},
	Pages = {34--58},
	Title = {Bayesian Inference for causal effects: the role of randomization},
	Volume = {6},
	Year = {1978}}

@incollection{Rubin75,
	Address = {Alexandria},
	Author = {Rubin, Donald B.},
	Booktitle = {The proceedings of the Social Statistics Section of the American Statistical Association},
	Publisher = {American Statistical Association},
	Title = {Bayesian Inference for Causality: the Importance of Randomization},
	Year = {1975}}

@article{Rubin08,
	Author = {Rubin, Donald B.},
	Journal = {Ann of Appl Stat},
	Number = {3},
	Pages = {808--840},
	Title = {For Objective Causal Inference, Design Trumps Analysis},
	Volume = {2},
	Year = {2008}}

@article{Sekhon10,
	Author = {Sekhon, J.S.},
	Journal = {Annu Rev of Polit Sci},
	Pages = {487--508},
	Title = {Opiates for the Matches: matching Methods for Causal Inference},
	Volume = {12},
	Year = {2010}}

@article{Rubin76,
	Author = {Rubin, Donald B.},
	Journal = {Biometrics},
	Number = {1},
	Pages = {121--132},
	Title = {Multivariate Matching Methods That are Equal Percent Bias Reducing, {II}: maximums on Bias Reduction for Fixed Sample Sizes},
	Volume = {32},
	Year = {1976}}

@article{Cochran&Rubin73,
	Author = {Cochran, W.G. and Donald B. Rubin},
	Journal = {Sankhya Ser A},
	Pages = {417--446},
	Title = {Controlling Bias in Observational Studies: a Review},
	Volume = {35},
	Year = {1973}}

@book{Cochran83,
	Address = {New York},
	Author = {Cochran, W.G.},
	Note = {Edited posthumously by L.E. Moses and F. Mosteller},
	Publisher = {Wiley},
	Title = {Planning and analysis of observational studies},
	Year = {1983}}

@article{Robinsetal07,
	Author = {J.M. Robins and M. Sued and Q. Lei-Gomez and A. Rotnitzky},
	Journal = {Stat Sci},
	Pages = {544--559},
	Title = {Comment: {P}erformance of Double-Robust Estimators When ``Inverse Probability'' Weights Are Highly Variable},
	Volume = {22},
	Year = {2007}}

@article{Cortes&Vapnik95,
	Author = {C. Cortes and V. Vapnik},
	Journal = {Mach Learn},
	Month = {December},
	Pages = {273--297},
	Title = {Support-vector networks},
	Volume = {20},
	Year = {1995}}

@techreport{Friedman94,
	Author = {J.H. Friedman},
	Institution = {Department of Statistics, Stanford University},
	Title = {Flexible metric nearest neighbor classification},
	Type = {Technical {R}eport},
	Year = {1994}}

@techreport{FDA06,
	Author = {{Food and Drug Administration}},
	Institution = {U.S. Department of Health and Human Services, Food and Drug Administration},
	Title = {Critical Path Opportunities List},
	Type = {Technical {R}eport},
	Year = {2006}}

@article{Efronetal04,
	Author = {B. Efron and T. Hastie and I. Johnstone and R. Tibshirani},
	Journal = {Ann Stat (with discussion)},
	Number = {2},
	Pages = {407--499},
	Title = {Least Angle Regression},
	Volume = {32},
	Year = {2004}}

@techreport{Breiman99,
	Author = {L. Breiman},
	Institution = {Department of Statistics, University of California, Berkeley},
	Number = {567},
	Title = {Random forests - random features},
	Year = {1999}}

@manual{Breiman01b,
	Author = {L. Breiman},
	Title = {Notes on setting up, using, and understanding random forests V3.0},
	Year = {2001}}

@article{Golubetal99,
	Author = {T.R. Golub and D.K. Slonim and P. Tamayo and C. Huard and M. Gaasenbeek and J.P. Mesirov and H. Coller and M.L. Loh and J.R. Downing and M.A. Caligiuri and C.D. Bloomfield and E.S. Lander},
	Journal = {Science},
	Pages = {531--537},
	Title = {Molecular classification of cancer: class discovery and class prediction by gene expression monitoring},
	Volume = {286},
	Year = {1999}}

@article{vanderLaan06a,
	Author = {M.J. van der Laan},
	Journal = {Int J Biostat},
	Number = {1},
	Pages = {Article 2},
	Title = {Statistical Inference for Variable Importance},
	Volume = {2},
	Year = {2006}}

@article{Robins&Mark&Newey92,
	Author = {J.M. Robins and S.D. Mark and W.K. Newey},
	Journal = {Biometrics},
	Number = {479--495},
	Title = {Estimating exposure effects by modelling the expectation of exposure conditional on confounders},
	Volume = {48},
	Year = {1992}}

@techreport{Yu&VanderLaan03,
	Author = {Z. Yu and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {136},
	Title = {Measuring treatment effects using semiparametric models},
	Year = {2003}}

@techreport{Tuglus&vanderLaan08,
	Author = {C. Tuglus and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {233},
	Title = {Targeted Methods for Biomarker Discovery, the Search for a Standard},
	Year = {2008}}

@book{Hastie&Tibshirani90,
	Address = {London},
	Author = {T.J. Hastie and R.J. Tibshirani},
	Publisher = {Chapman \& Hall},
	Title = {Generalized additive models},
	Year = {1990}}

@misc{Efron&Hastie07,
	Author = {B. Efron and T. Hastie},
	Howpublished = {R package},
	Title = {lars},
	Year = {2007}}

@article{Benjamini&Hochberg95,
	Author = {Y. Benjamini and Y. Hochberg},
	Journal = {J R Stat Soc Ser B},
	Pages = {289--300},
	Title = {Controlling the false discovery rate: a practical and powerful approach to multiple testing},
	Volume = {57},
	Year = {1995}}

@misc{Ge&Dudoit02,
	Author = {Y. Ge and S. Dudoit},
	Howpublished = {R package},
	Title = {Multiple Testing Procedures, multtest},
	Url = {www.bioconductor.org},
	Year = {2002},
	Bdsk-Url-1 = {www.bioconductor.org}}

@article{Tibshirani96,
	Author = {R. Tibshirani},
	Journal = {J R Stat Soc Ser B},
	Number = {1},
	Pages = {267--288},
	Title = {Regression shrinkage and selection via the lasso.},
	Volume = {58},
	Year = {1996}}

@article{Tuglus&vanderLaan09,
	Author = {C. Tuglus and M.J. van der Laan},
	Journal = {Stat Appl Genet Mol},
	Number = {1},
	Pages = {Article 12},
	Title = {Modified {FDR} Controlling Procedure for Multi-Stage Analyses},
	Volume = {8},
	Year = {2009}}

@article{Dudoit&Fridlyand&Speed02,
	Author = {S. Dudoit and J. Fridlyand and T. P. Speed},
	Journal = {J Am Stat Assoc},
	Number = {457},
	Pages = {77--87},
	Title = {Comparison of Discrimination Methods for the Classification of Tumors Using Gene Expression Data},
	Volume = {97},
	Year = {2002}}

@article{Kos&Lah98,
	Author = {J. Kos and T.T. Lah},
	Journal = {Oncol Rep},
	Number = {6},
	Pages = {1349--61},
	Title = {Cysteine proteinases and their endogenous inhibitors: target proteins for prognosis, diagnosis and therapy in cancer (review)},
	Volume = {5},
	Year = {1998}}

@article{Vitaleetal01,
	Author = {C. Vitale and C. Romagnani and A. Puccetti and D. Olive and R. Costello and L. Chiossone and A. Pitto and A. Bacigalupo and L. Moretta and M.C. Mingari},
	Journal = {Proc Natl Acad Sci},
	Pages = {5764--5769},
	Title = {Surface expression and function of p75/{AIRM}-1 or {CD}33 in acute myeloid leukemias: engagement of {CD}33 induces apoptosis of leukemic cells},
	Volume = {98},
	Year = {2001}}

@article{Clappieretal07,
	Author = {E. Clappier and W. Cuccuini and A. Kalota and A. Crinquette and J.M. Cayuela and W.A. Dik and A.W. Langerak and B. Montpellier and B. Nadel and P. Walrafen and O. Delattre and A. Aurias and T. Leblanc and H. Dombret and A.M. Gewirtz and A. Baruchel and F. Sigaux and J. Soulier},
	Journal = {Blood},
	Number = {4},
	Pages = {1251--61},
	Title = {The {C-MYB} locus is involved in chromosomal translocation and genomic duplications in human T-cell acute leukemia ({T-ALL}), the translocation defining a new {T-ALL} subtype in very young children},
	Volume = {110},
	Year = {2007}}

@article{Lane&Ley03,
	Author = {A.A. Lane and T.J. Ley},
	Journal = {Cell},
	Number = {305-318},
	Title = {Neutrophil elastase cleaves {PML-RAR}-alpha and is important for the development of acute promyelocytic leukemia in mice},
	Volume = {115},
	Year = {2003}}

@article{Hunger96,
	Author = {S.P. Hunger},
	Journal = {Blood},
	Pages = {1211--1224},
	Title = {Chromosomal translocations involving the {E2A} gene in acute lymphoblastic leukemia: clinical features and molecular pathogenesis.},
	Volume = {87},
	Year = {1996}}

@article{Nebraletal05,
	Author = {K. Nebral and H.H. Schmidt and O.A. Haas and S. Strehl},
	Journal = {Clin Cancer Res},
	Number = {18},
	Pages = {6489--6494},
	Title = {{NUP}98 Is Fused to Topoisomerase {(DNA)} {II}{beta} 180 {kDa} {(TOP2B)} in a Patient with Acute Myeloid Leukemia with a New {t(3;11)(p24;p15)}},
	Volume = {11},
	Year = {2005}}

@article{Kaufmannetal98b,
	Author = {S.H. Kaufmann and S.D. Gore and C.B. Miller and R.J. Jones and L.A. Zwelling and E. Schneider and P.J. Burke and J.E. Karp},
	Journal = {Leukemia Lymphoma},
	Month = {Apr},
	Number = {3-4},
	Pages = {217--237},
	Title = {Topoisomerase {II} and the response to antileukemic therapy},
	Volume = {29},
	Year = {1998}}

@article{Kozaretal04,
	Author = {K. Kozar and M.A. Ciemerych and V.I. Rebel and H. Shigematsu and A. Zagozdzon and E. Sicinska and Y. Geng and Q. Yu and S. Bhattacharya and R.T. Bronson and K. Akashi and P. Sicinski},
	Journal = {Cell},
	Pages = {477--491},
	Title = {Mouse development and cell proliferation in the absence of {D}-cyclins},
	Volume = {118},
	Year = {2004}}

@article{MartinSuberoetal07,
	Author = {J.I. Martin-Subero and R. Ibbotson and W. Klapper and L. Michaux and E. Callet-Bauchu and F. Berger and M.J. Calasanz and C. De Wolf-Peeters and M.J. Dyer and P. Felman and A. Gardiner and R.D. Gascoyne and S. Gesk and L. Harder and D.E. Horsman and M. Kneba and R. Kuppers and A. Majid and N. Parry-Jones and M. Ritgen and M. Salido and F. Sole and G. Thiel and H.H. Wacker and D. Oscier and I. Wlodarska and R. Siebert},
	Journal = {Leukemia},
	Number = {7},
	Pages = {1532--1544},
	Title = {A comprehensive genetic and histopathologic analysis identifies two subgroups of {B}-cell malignancies carrying a t(14;19)(q32;q13) or variant {BCL3}-translocation},
	Volume = {21},
	Year = {2007}}

@article{Palomeroetal06,
	Author = {T. Palomero and D.T. Odom and J. O'Neil and A.A. Ferrando and A. Margolin and D.S. Neuberg and S.S. Winter and R.S. Larson and W. Li and X.S. Liu and R.A. Young and A.T. Look},
	Journal = {Blood},
	Number = {3},
	Pages = {986--992},
	Title = {Transcriptional regulatory networks downstream of {TAL1/SCL} in {T}-cell acute lymphoblastic leukemia},
	Volume = {108},
	Year = {2006}}

@article{Wongetal07,
	Author = {H.P. Wong and L. Yu and E.K. Lam and E.K. Tai and W.K. Wu and C.H. Cho},
	Journal = {Toxicol Appl Pharm},
	Number = {3},
	Pages = {261--267},
	Title = {Nicotine promotes cell proliferation via alpha7-nicotinic acetylcholine receptor and catecholamine-synthesizing enzymes-mediated pathway in human colon adenocarcinoma {HT}-29 cells.},
	Volume = {221},
	Year = {2007}}

@article{Ramaswamyetal03,
	Author = {S. Ramaswamy and K.N. Ross and E.S. Lander and T.R. Golub},
	Journal = {Nat Genet},
	Pages = {49--54},
	Title = {A molecular signature of metastasis in primary solid tumors},
	Volume = {33},
	Year = {2003}}

@article{Purietal01,
	Author = {R. Puri and A. Tousson and L. Chen and S.S. Kakar},
	Journal = {Cancer Lett},
	Pages = {131--139},
	Title = {Molecular cloning of pituitary tumor transforming gene 1 from ovarian tumors and its expression in tumors},
	Volume = {163},
	Year = {2001}}

@article{Fujiietal06,
	Author = {T. Fujii and S. Nomoto and K. Koshikawa and Y.Yatabe and O. Teshigawara and T. Mori and S. Inoue and S. Takeda and A. Nakao},
	Journal = {Hepatology},
	Pages = {1267--1275},
	Title = {Overexpression of pituitary tumor transforming gene 1 in {HCC} is associated with angiogenesis and poor prognosis},
	Volume = {43},
	Year = {2006}}

@article{Zhuetal06,
	Author = {X. Zhu and Z. Mao and Y. Na and Y. Guo and X. Wang and D. Xin},
	Journal = {Anticancer Res},
	Pages = {1253--1259},
	Title = {Significance of pituitary tumor transforming gene 1 ({PTTG1}) in prostate cancer},
	Volume = {26},
	Year = {2006}}

@article{Kaufmannetal98a,
	Author = {S.H. Kaufmann and J.E. Karp and P.A. Svingen and S. Krajewski and P.J. Burke and S.D. Gore and J.C. Reed},
	Journal = {Blood},
	Number = {3},
	Pages = {991--1000},
	Title = {Elevated expression of the apoptotic regulator {Mcl}-1 at the time of leukemic relapse},
	Volume = {91},
	Year = {1998}}

@article{Frumanetal99,
	Author = {D.A. Fruman and S.B. Snapper and C.M. Yballe and L. Davidson and J.Y. Yu and F.W. Alt and L.C. Cantley},
	Journal = {Science},
	Pages = {393--397},
	Title = {Impaired {B} cell development and proliferation in absence of phosphoinositide 3-kinase p85-alpha},
	Volume = {283},
	Year = {1999}}

@article{Tombes&Krystal97,
	Author = {R.M. Tombes and G.W. Krystal},
	Journal = {Biochim Biophys Acta},
	Pages = {281--292},
	Title = {Identification of novel human tumor cell-specific {CaMK-II} variants},
	Volume = {1355},
	Year = {1997}}

@article{Senturkeretal97,
	Author = {S. Senturker and B. Karahalil and M. Inal and H. Yilmaz and H. Muslumanoglu and G. Gedikoglu and M. Dizdaroglu},
	Journal = {FEBS Letters},
	Number = {3},
	Pages = {286--290},
	Title = {Oxidative {DNA} base damage and antioxidant enzyme levels in childhood acute lymphoblastic leukemia},
	Volume = {416},
	Year = {1997}}

@article{Komuroetal05,
	Author = {I. Komuro and T. Yasuda and A. Iwamoto and K.S. Akagawa},
	Journal = {J Biol Chem},
	Number = {50},
	Pages = {41137--45},
	Title = {Catalase plays a critical role in the {CSF}-independent survival of human macrophages via regulation of the expression of {BCL}-2 family},
	Volume = {280},
	Year = {2005}}

@article{Balciunaiteetal05,
	Author = {E. Balciunaite and A. Spektor and N.H. Lents and H. Cam and H. Te Riele and A. Scime and M.A. Rudnicki and R. Young and B.D. Dynlacht},
	Journal = {Mol Cell Biol},
	Number = {18},
	Pages = {8166--78},
	Title = {Pocket protein complexes are recruited to distinct targets in quiescent and proliferating cells},
	Volume = {25},
	Year = {2005}}

@article{Leoneetal01,
	Author = {G. Leone and R. Sears and E. Huang and R. Rempel and F. Nuckolls and C.H. Park and P. Giangrande and L. Wu and H.I. Saavedra and S.J. Field and M.A. Thompson and H. Yang and Y. Fujiwara and M.E. Greenberg and S. Orkin and C. Smith and J.R. Nevins},
	Journal = {Mol Cell},
	Pages = {105--113},
	Title = {Myc requires distinct {E2F} activities to induce {S} phase and apoptosis},
	Volume = {8},
	Year = {2001}}

@article{Sax23,
	Author = {Sax, K.},
	Journal = {Genetics},
	Title = {The association of size difference with seed-coat pattern and pigmentation in \textit{Phaseolus vulgaris}},
	Year = {1923}}

@article{Thoday60,
	Author = {Thoday, J.M.},
	Journal = {Nature},
	Title = {Location of polygenes},
	Year = {1960}}

@article{Lander&Botstein89,
	Author = {Lander, E.S. and Botstein, D.},
	Journal = {Genetics},
	Title = {Mapping {M}endelian factors underlying quantitative traits using {RFLP} linkage maps},
	Year = {1989}}

@article{Haley&Knott92,
	Author = {Haley, C.S. and Knott, S.A.},
	Journal = {Heredity},
	Title = {A simple regression method for mapping quantitative trait loci in line crosses using flanking markers},
	Year = {1992}}

@article{Jansen93,
	Author = {Jansen, R.C.},
	Journal = {Genetics},
	Title = {Interval mapping of multiple quantitative trait loci},
	Year = {1993}}

@article{Zeng94,
	Author = {Zeng, Z.B.},
	Journal = {Genetics},
	Title = {Precision mapping of quantitative trait loci},
	Year = {1994}}

@article{Kao&Zeng&Teasdale99,
	Author = {Kao, C.H. and Zeng, Z.B. and Teasdale, R.D.},
	Journal = {Genetics},
	Title = {Multiple interval mapping for quantitative trait loci},
	Year = {1999}}

@article{Satagopanetal96,
	Author = {Satagopan, J.M. and B.S. Yandell and M.A. Newton and T.C. Osborn},
	Journal = {Genetics},
	Title = {A {B}ayesian approach to detect quantitative trait loci using {M}arkov chain {M}onte {C}arlo},
	Year = {1996}}

@article{Heath97,
	Author = {Heath, S.C.},
	Journal = {Am J Hum Genet},
	Title = {Markov chain {M}onte {C}arlo segregation and linkage analysis of oligogenic models},
	Year = {1997}}

@article{Sillanpaa&Arjas98,
	Author = {Sillanpaa, M.J. and Arjas, E.},
	Journal = {Genetics},
	Title = {Bayesian mapping of multiple quantitative trait loci from incomplete inbred line cross data},
	Year = {1998}}

@article{Leeetal08,
	Author = {Lee, S.S.F. and L. Sun and R. Kustra and S.B. Bull},
	Journal = {Bioinformatics},
	Title = {{EM}-random forest and new measures of variable importance for multi-locus quantitative trait linkage analysis},
	Year = {2008}}

@article{Wang2011ctmle,
	Author = {H. Wang and S. Rose and M.J. van der Laan},
	Date-Modified = {2012-08-26 00:45:19 -0700},
	Journal = {Stat Prob Lett},
	Keywords = {App},
	Note = {PMCID: PMC3090625},
	Number = {7},
	Pages = {792--796},
	Title = {{F}inding {Q}uantitative {T}rait {L}oci {G}enes with {C}ollaborative {T}argeted {M}aximum {L}ikelihood {L}earning},
	Volume = {81},
	Year = {2011}}

@techreport{Wang&Rose&vanderLaan11,
	Author = {H. Wang and S. Rose and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Title = {Targeted Methods for Finding Quantitative Trait Loci},
	Type = {Technical {R}eport},
	Year = {2011}}

@manual{Basten&Weir&Zeng01,
	Author = {C.J. Basten and B.S. Weir and Z.B. Zeng},
	Title = {QTL Cartographer},
	Url = {http://statgen.ncsu.edu/qtlcart/},
	Year = {2001},
	Bdsk-Url-1 = {http://statgen.ncsu.edu/qtlcart/}}

@article{Masindeetal01,
	Author = {Masinde, G.L. and X. Li and W. Gu and H. Davidson and S. Mohan and D.J. Baylink},
	Journal = {Genome Res},
	Title = {Identification of wound healing/regeneration quantitative trait loci ({QTL}) at multiple time points that explain seventy percent of variance in ({MRL/MpJ and SJL/J}) mice {F2} population},
	Year = {2001}}

@article{Boyartchuk01,
	Author = {Boyartchuk, V.L. and K.W. Broman and R.E. Mosher and S.E.F. D'Orazio and M.N. Starnbach and W.F. Dietrich},
	Journal = {Nat Genet},
	Title = {Multigenic control of Listeria monocytogenes susceptibility in mice},
	Year = {2001}}

@article{Broman03,
	Author = {Broman, K.W.},
	Journal = {Genetics},
	Title = {Mapping quantitative trait loci in the case of a spike in the phenotype distribution},
	Year = {2003}}

@article{Jin&Fine&Yandell07,
	Author = {Jin, C. and J.P. Fine and B.S. Yandell},
	Journal = {J Am Stat Assoc},
	Title = {A unified semiparametric framework for quantitative trait loci analysis, with application to spike phenotypes},
	Year = {2007}}

@article{Petersenetal08,
	Author = {M.L. Petersen and M.J. van der Laan and S. Napravnik and J.J. Eron and R.D. Moore and S.G. Deeks},
	Journal = {AIDS},
	Number = {16},
	Pages = {2097--106},
	Title = {Long-term consequences of the delay between virologic failure of highly active antiretroviral therapy and regimen modification},
	Volume = {22},
	Year = {2008}}

@article{Rodgeretal09,
	Author = {A.J. Rodger and Z. Fox and J.D. Lundgren and J.L. Kuller and C. Boesecke and D. Gey and A. Skoutelis and M.B. Goetz and A.N. Phillips and {INSIGHT Strategies for Management of Antiretroviral Therapy (SMART) Study Group}},
	Journal = {J Infect Dis},
	Number = {6},
	Pages = {973--83},
	Title = {Activation and coagulation biomarkers are independent predictors of the development of opportunistic disease in patients with {HIV} infection.},
	Volume = {200},
	Year = {2009}}

@article{Hammeretal08,
	Author = {S.M. Hammer and J.J. Eron and P. Reiss and R.T. Schooley and M.A. Thompson and S. Walmsley and P. Cahn and M.A. Fischl and J.M. Gatell and M.S. Hirsch and D.M. Jacobsen and J.S.G. Montaner and D.D. Richman and P.G. Yeni and P.A. Volberding},
	Journal = {J Am Med Asoc},
	Number = {5},
	Pages = {555--70},
	Title = {Antiretroviral treatment of adult {HIV} infection: 2008 recommendations of the {I}nternational {AIDS} {S}ociety-{USA} panel},
	Volume = {300},
	Year = {2008}}

@article{Stringeretal06,
	Author = {J.S. Stringer and I. Zulu and J. Levy and E.M. Stringer and A. Mwango and B.H. Chi and V. Mtonga and S. Reid and R.A. Cantrell and M. Bulterys and M.S. Saag and R.G. Marlink and A. Mwinga and T.V. Ellerbrock and M. Sinkala},
	Journal = {J Am Med Asoc},
	Number = {7},
	Pages = {782--93},
	Title = {Rapid scale-up of antiretroviral therapy at primary care sites in {Z}ambia: feasibility and early outcomes},
	Volume = {296},
	Year = {2006}}

@misc{WHO06,
	Author = {{{W}orld {H}ealth {O}rganization}},
	Title = {Antiretroviral therapy for {HIV} infection in adults and adoloescents: recommendations for a public health approach},
	Year = {2006}}

@article{Reynoldsetal09,
	Author = {S.J. Reynolds and G. Nakigozi and K. Newell and A. Ndyanabo and R. Galiwongo and I. Boaz and T.C. Quinn and R. Gray and M. Wawer and D. Serwadda},
	Journal = {{AIDS}},
	Number = {6},
	Pages = {697--700},
	Title = {Failure of immunologic criteria to appropriately identify antiretroviral treatment failure in {U}ganda},
	Volume = {23},
	Year = {2009}}

@article{Petersen2007,
	Author = {M.L Petersen and S.G. Deeks and J.N. Martin and M.J. van der Laan},
	Date-Modified = {2012-08-25 23:33:55 -0700},
	Journal = {Am J Epidemiol},
	Keywords = {Aim1},
	Note = {PMCID: PMC2561999},
	Number = {9},
	Pages = {985--993},
	Title = {History-adjusted Marginal Structural Models for Estimating Time-varying Effect Modification},
	Volume = {166},
	Year = {2007}}

@article{Robins&Hernan&Rotnitzky07,
	Author = {J.M. Robins and M.A. Hernan and A. Rotnitzky},
	Journal = {Am J Epidemiol},
	Number = {9},
	Pages = {994--1002},
	Title = {Effect Modification by Time-varying Covariates},
	Volume = {166},
	Year = {2007}}

@article{vanderLaan&Petersen&Joffe07,
	Author = {M.J. van der Laan and M.L. Petersen and M.M. Joffe},
	Journal = {Am J Epidemiol},
	Number = {9},
	Pages = {1003--1004},
	Title = {Response to Invited Commentary: {P}etersen et. al. Respond to ``{E}ffect Modification by Time-varying Covariates''},
	Volume = {166},
	Year = {2007}}

@article{vanderLaan&Petersen07b,
	Author = {M.J. van der Laan and M.L. Petersen},
	Journal = {Int J Biostat},
	Number = {1},
	Pages = {Article 6},
	Title = {Statistical Learning of Origin-Specific Statically Optimal Individualized Treatment Rules.},
	Volume = {3},
	Year = {2007}}

@article{Petersen&Deeks&vanderLaan07,
	Author = {M.L. Petersen and S.G. Deeks and M.J. van der Laan},
	Date-Modified = {2012-08-20 22:22:11 -0700},
	Journal = {Stat Med},
	Note = {PubMed Central PMCID: PMC2442037},
	Number = {25},
	Pages = {4578--601},
	Title = {{Individualized treatment rules: Generating candidate clinical trials}},
	Volume = {26},
	Year = {2007}}

@article{vanderLaan2005,
	Author = {M.J. van der Laan and M.L. Petersen and M.M. Joffe},
	Date-Modified = {2012-08-24 09:41:11 -0700},
	Journal = {Int J Biostat},
	Keywords = {Aim1},
	Number = {1},
	Pages = {10--20},
	Title = {{History-Adjusted Marginal Structural Models and Statically-Optimal Dynamic Treatment Regimens}},
	Volume = {1},
	Year = {2005}}

@article{Hernan2006,
	Author = {M.A. Hern\'{a}n and E. Lanoy and D. Costagliola and J.M. Robins},
	Date-Modified = {2012-08-23 18:01:19 -0700},
	Journal = {Basic Clin Pharmacol Toxicol},
	Keywords = {Aim1},
	Note = {PMID: 16611197},
	Number = {3},
	Pages = {237--242},
	Title = {Comparison of dynamic treatment regimes via inverse probability weighting},
	Volume = {98},
	Year = {2006}}

@techreport{vanderLaan08b,
	Author = {M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {232},
	Title = {The construction and analysis of adaptive group sequential designs},
	Year = {2008}}

@article{Boivinetal07,
	Author = {Boivin, J. and Bunting, L. and Collins, J.A. and Nygren, K.G.},
	Journal = {Hum Reproduct},
	Pages = {1506--1512},
	Title = {International estimates of infertility prevalence and treatment-seeking: potential need and demand for infertility medical care},
	Volume = {22},
	Year = {2007}}

@article{Adamsonetal06,
	Author = {Adamson, G.D. and de {M}ouzon, J. and Lancaster, P. and Nygren, K.-G. and Sullivan, E. and Zegers-Hochschild, F.},
	Journal = {Fertil Steril},
	Pages = {1586--1622},
	Title = {World collaborative report on in vitro fertilization, 2000},
	Volume = {85},
	Year = {2006}}

@article{Soullieretal08,
	Author = {Soullier, N. and Bouyer, J. and Pouly J-L. and Guibert, J. and de la {R}ochebrochard},
	Journal = {Hum Reproduct},
	Pages = {187--192},
	Title = {Estimating the success of an in vitro fertilization programme using multiple imputation},
	Volume = {23},
	Year = {2008}}

@article{delaRochebrochardetal08,
	Author = {de la {R}ochebrochard, E. and Soullier, N. and Peikrishvili, R. and Guibert, J. and Bouyer, J.},
	Journal = {Int J Gynecol Obstet},
	Pages = {74--75},
	Title = {High in vitro fertilization discontinuation rate in {F}rance},
	Volume = {103},
	Year = {2008}}

@article{delaRochebrochardetal09,
	Author = {de la {R}ochebrochard, E. and Quelen, C. and Peikrishvili, R. and Guibert, J. and Bouyer, J.},
	Journal = {Fertil Steril},
	Pages = {149--156},
	Title = {Long-term outcome of parenthood project during in vitro fertilization and after discontinuation of unscuccessful in vitro fertilization},
	Volume = {92},
	Year = {2009}}

@book{Schafer97,
	Address = {London},
	Author = {Schafer, J.L.},
	Publisher = {Chapman \& Hall},
	Title = {Analysis of incomplete multivariate data},
	Year = {1997}}

@book{Little&Rubin02,
	Address = {Hoboken},
	Author = {Little, R.J.A. and Rubin, Donald B.},
	Edition = {2nd},
	Publisher = {Wiley},
	Title = {Statistical analysis with missing data},
	Year = {2002}}

@techreport{Yu&vanderLaan02,
	Author = {Z. Yu and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {122},
	Title = {Construction of counterfactuals and the G-computation formula},
	Year = {2002}}

@article{Gill&Robins01,
	Author = {Gill, R.D. and Robins, J.M.},
	Journal = {Ann Stat},
	Number = {6},
	Pages = {1785--1811},
	Title = {Causal inference in complex longitudinal studies: continuous case},
	Volume = {29},
	Year = {2001}}

@techreport{DHHS04,
	Author = {{Department of Health and Human Services}},
	Institution = {Panel on Clinical Practices for Treatment of {HIV} Infection},
	Title = {Guidelines for the use of antiretroviral agents in {HIV}-1 infected adults and adolescents},
	Type = {Technical {R}eport},
	Year = {2004}}

@article{CDC92,
	Author = {{Centers for Disease Control and Prevention}},
	Journal = {Morbid Mortal W Rep},
	Pages = {1--19},
	Title = {{1993 revised classification system for {HIV} infection and expanded surveillance case definition for AIDS among adolescents and adults}},
	Volume = {41},
	Year = {1992}}

@incollection{Selbyetal05,
	Author = {J.V. Selby and D.H. Smith and E.S. Johnson and M.A. Raebel and G.D. Friedman and B.H. McFarland},
	Booktitle = {Pharmacoepidemiology},
	Editor = {B.L. Strom},
	Publisher = {Wiley},
	Title = {Kaiser {P}ermanente Medical Care Program},
	Year = {2005}}

@techreport{Neugebauer&Silverberg&vanderLaan10,
	Author = {R. Neugebauer and M.J. Silverberg and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Title = {Observational Study and Individualized Antiretroviral Therapy Initiation Rules for Reducing Cancer Incidence in {HIV}-Infected Patients},
	Type = {272},
	Year = {2010}}

@techreport{Stitelman2011,
	Author = {O.M. Stitelman and V. De Gruttola and M.J. van der Laan},
	Date-Modified = {2012-08-26 20:56:50 -0700},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Keywords = {tmle},
	Note = {Available at \url{http://www.bepress.com/ucbbiostat/paper281}; To appear in Int J. Biostat},
	Number = {281},
	Title = {A General Implementation of TMLE for Longitudinal Data Applied to Causal Inference in Survival Analysis},
	Year = {2011}}

@techreport{Stitelman2011a,
	Author = {O.M. Stitelman and M.J. van der Laan},
	Date-Modified = {2012-08-24 11:37:04 -0700},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Title = {Targeted Maximum Likelihood Estimation of Time-To-Event Parameters With Time-Dependent Covariates},
	Type = {Technical {R}eport},
	Year = {2011}}

@article{Thalletal07,
	Author = {P.F. Thall and C. Logothetis and L.C. Pagliaro and S. Wen and M.A. Brown and D. Williams and R.E. Millikan},
	Journal = {J Natl Cancer Inst},
	Pages = {1613--22},
	Title = {Adaptive Therapy for Androgen-Independent Prostate Cancer: a randomized Selection Trial of Four Regimens},
	Volume = {99},
	Year = {2007}}

@article{Bembom&vanderLaan07a,
	Author = {O. Bembom and M.J. van der Laan},
	Journal = {J Natl Cancer Inst},
	Pages = {1577--1582},
	Title = {Comment: Statistical Methods for analyzing sequentially randomized trials},
	Volume = {99(21)},
	Year = {2007}}

@techreport{Zheng&vanderLaan10,
	Author = {W. Zheng and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {273},
	Title = {Asymptotic Theory for Cross-validated Targeted Maximum Likelihood Estimation},
	Year = {2010}}

@techreport{Zheng&vanderLaan11,
	Author = {W. Zheng and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {288},
	Title = {Targeted Maximum Likelihood Estimation of Natural Direct Effect},
	Year = {2011}}

@book{Robert07,
	Address = {Berlin Heidelberg New York},
	Author = {Robert, P.C.},
	Publisher = {Springer},
	Title = {{T}he {B}ayesian choice: from decision-thoeretic foundations to computational implementation},
	Year = {2007}}

@book{Lindley80,
	Address = {Cambridge, MA},
	Author = {Lindley, D.V.},
	Publisher = {Cambridge},
	Title = {{I}ntroduction to probability and statistics from a {B}ayesian point of view, {P}art 2},
	Year = {1980}}

@article{Golub06,
	Author = {Golub, H.L.},
	Journal = {Stat Med},
	Pages = {3231--3235},
	Title = {The need for more efficient trial designs},
	Volume = {25},
	Year = {2006}}

@article{Emerson06,
	Author = {Emerson, S.S.},
	Journal = {Stat Med},
	Pages = {3270--3296},
	Title = {Issues in the use of adaptive clinical trial designs},
	Volume = {25},
	Year = {2006}}

@book{Hu&Rosenberger06,
	Address = {New York},
	Author = {F. Hu and W.F. Rosenberger},
	Publisher = {Wiley},
	Title = {The theory of response adaptive randomization in clinical trials},
	Year = {2006}}

@book{Jennison&Turnbull00,
	Address = {Boca Raton},
	Author = {Jennison, C. and Turnbull, B.W.},
	Publisher = {Chapman \& Hall},
	Title = {Group sequential methods with applications to clinical trials},
	Year = {2000}}

@article{Rosenberger96,
	Author = {W.F. Rosenberger},
	Journal = {Stat Sci},
	Pages = {137--149},
	Title = {New directions in adaptive designs},
	Volume = {11},
	Year = {1996}}

@techreport{Chambaz10,
	Author = {Chambaz, A. and van der Laan, M.J.},
	Date-Modified = {2012-08-26 20:55:57 -0700},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Keywords = {App},
	Note = {Available at \url{http://biostats.bepress.com/ucbbiostat/paper258/}},
	Number = {258},
	Title = {Targeting the optimal design in randomized clinical trials with binary outcomes and no covariate},
	Year = {2010}}

@article{Rosenberger&Vidyashankar&Agarwal01,
	Author = {Rosenberger, W.F. and Vidyashankar, A.N. and Agarwal, D.K.},
	Journal = {J Biopharm Stat},
	Number = {227--236},
	Title = {Covariate-adjusted response-adaptive designs for binary response},
	Volume = {11},
	Year = {2001}}

@article{Bandyopadhyay&Biswas01,
	Author = {Bandyopadhyay, U. and Biswas, A.},
	Journal = {Biometrika},
	Number = {2},
	Pages = {409--419},
	Title = {Adaptive designs for normal responses with prognostic factors},
	Volume = {88},
	Year = {2001}}

@article{Atkinson&Biswas05,
	Author = {Atkinson, A.C. and Biswas, A.},
	Journal = {Stat Med},
	Number = {16},
	Pages = {2477--2492},
	Title = {Adaptive biased-coin designs for skewing the allocation proportion in clinical trials with normal responses},
	Volume = {24},
	Year = {2005}}

@article{Zhangetal07,
	Author = {Zhang, L.-X. and Hu, F.-F. and Cheung, S.H. and Chan, W.S.},
	Journal = {Ann Stat},
	Number = {3},
	Pages = {1166--1182},
	Title = {Asymptotic properties of covariate-adjusted response-adaptive designs},
	Volume = {35},
	Year = {2007}}

@article{Zhang&Hu09,
	Author = {Zhang, L.-X. and Hu, F.-F.},
	Journal = {Appl Math J Chinese Univ Ser B},
	Number = {1},
	Pages = {1--13},
	Title = {A new family of covariate-adjusted response adaptive designs and their properties},
	Volume = {24},
	Year = {2009}}

@article{Shao&Yu&Zhong10,
	Author = {Shao, J. and Yu, X. and Bob Zhong, B.},
	Journal = {Biometrika},
	Title = {A theory for testing hypotheses under covariate-adaptive randomization},
	Year = {2010}}

@article{Gill89,
	Author = {Gill, R.D.},
	Journal = {Scand J Stat},
	Title = {Non- and semiparametric maximum likelihood estimators and the Von Mises method (Part 1)},
	Year = {1989}}

@article{Tan08,
	Author = {Z. Tan},
	Journal = {Int J Biostat},
	Number = {1},
	Pages = {Article 10},
	Title = {Comment: {I}mproved Local Efficiency and Double Robustness},
	Volume = {4},
	Year = {2008}}

@techreport{tmlePackageb,
	Author = {S. Gruber and M.J. van der Laan},
	Date-Modified = {2012-08-26 21:19:43 -0700},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Keywords = {tmle},
	Note = {Available at \url{http://biostats.bepress.com/ucbbiostat/paper275/}},
	Number = {275},
	Title = {{tmle}: an {R} Package for Targeted Maximum Likelihood Estimation},
	Year = {2011}}

@proceedings{DBLP:conf/colt/2003,
	Address = {Berlin Heidelberg New York},
	Booktitle = {COLT},
	Editor = {B. Sch{\"o}lkopf and M.K. Warmuth},
	Publisher = {Springer},
	Series = {Lecture Notes in Computer Science},
	Title = {Computational Learning Theory and Kernel Machines, 16th Annual Conference on Computational Learning Theory and 7th Kernel Workshop, COLT/Kernel 2003, Washington, DC, USA, August 24-27, 2003, Proceedings},
	Volume = {2777},
	Year = {2003}}

@proceedings{DBLP:conf/nips/2005,
	Booktitle = {NIPS},
	Title = {Advances in Neural Information Processing Systems 18 [Neural Information Processing Systems, NIPS 2005, December 5-8, 2005, Vancouver, British Columbia, Canada]},
	Year = {2005}}

@proceedings{DBLP:conf/colt/2006,
	Address = {Berlin Heidelberg New York},
	Booktitle = {COLT},
	Editor = {G. Lugosi and H.-U. Simon},
	Publisher = {Springer},
	Series = {Lecture Notes in Computer Science},
	Title = {Learning Theory, 19th Annual Conference on Learning Theory, COLT 2006, Pittsburgh, PA, USA, June 22-25, 2006, Proceedings},
	Volume = {4005},
	Year = {2006}}

%% This BibTeX bibliography file was created using BibDesk.
%% http://bibdesk.sourceforge.net/


%% Created for Susan Gruber at 2012-01-03 21:41:54 -0500


%% Saved with string encoding Unicode (UTF-8)


@string{jasa = {Journal of the American Statistical Association}}

@string{jc = {Journal of Classification}}

@string{jrssb = {Journal of the Royal Statistical Society, Series B}}

@string{jspi = {Journal of Statistical Planning and Inference}}

@string{pnas = {Proc. Natl. Acad. Sci.}}

@article{Xiao&Abrahamowicz&Moodie10,
	Author = {Y. Xiao, M. Abrahamowicz, E.E.M. Moodie},
	Journal = {The International Journal of Biostatistics},
	Title = {Accuracy of Conventional and Marginal Structural Cox Model Estimators: A Simulation Study},
	Volume = {6},
	Issue = {2},
	Article={13},
	Year = {2010}
}

@article{Moore&vanderLaan092,
  author =        {Moore, K.L. and van der Laan, M.J.},
  journal =       {Stat Med},
  number =        {1},
  pages =         {39--64},
  title =         {Covariate Adjustment in Randomized Trials with Binary
                   Outcomes: targeted Maximum Likelihood Estimation},
  volume =        {28},
  year =          {2009},
}

@article{Gruber&vanderLaanTygacil,
  author = {S. Gruber and M.J. van der Laan},
  journal = {Biometrics},
  title = {An Application of Targeted Maximum Likelihood Estimation to the Meta-Analysis of Safety Data},
  Year = {2012 (in press)}
  }

@article{Hahn04,
	Author = {J. Hahn},
	Date-Added = {2012-01-03 21:40:45 -0500},
	Date-Modified = {2012-01-03 21:41:54 -0500},
	Journal = {Rev Econ Stat},
	Pages = {73-76},
	Title = {Functional restriction and efficiency in causal inference},
	Volume = {86},
	Year = {2004}}

@techreport{DiazHubbard&vanderLaan10,
	Author = {I. Diaz Munoz and A. E. Hubbard and M. J. van der Laan},
	Date-Added = {2011-12-29 11:12:37 -0500},
	Date-Modified = {2011-12-29 11:13:20 -0500},
	Institution = {UC Berkeley Division of Biostatistics Working Paper Series},
	Month = {October},
	Number = {270},
	Title = {Targeted Bayesian Learning},
	Type = {Working Paper},
	Year = {2010}}

@article{Abadie&Imbens11,
	Author = {A. Abadie and G.W. Imbens},
	Journal = {Journal of Business and Economic Statistics},
	Number = {1},
	Pages = {1-11},
	Title = {Bias-Corrected Matching Estimators for Average Treatment Effects},
	Volume = {29},
	Year = {2011}}

@article{Hernan10,
	Author = {The HIV-CAUSAL Collaboration},
	Date = {2010///},
	Date-Added = {2011-12-11 13:32:38 -0500},
	Date-Modified = {2011-12-11 13:33:01 -0500},
	Id = {00002030-201001020-00017},
	Isbn = {0269-9370},
	Journal = {AIDS},
	Number = {1},
	Title = {The effect of combined antiretroviral therapy on the overall mortality of {HIV}-infected individuals},
	Ty = {JOUR},
	Volume = {24},
	Year = {2010}}

@article{Newey90,
	Author = {W. K. Newey},
	Issue = {2},
	Journal = {Journal of Applied Econometrics},
	Pages = {99-135},
	Title = {Semiparametric Efficiency Bounds},
	Volume = {5},
	Year = {1990}}

@article{Robins&Mark&Newey92,
	Author = {J.M. Robins, S.D. Mark, W.K. Newey},
	Journal = {Biometrics},
	Volume = {48},
	pages = {479-95},
	Month = {June},
	Year = {1992},
	Title = {Estimating Exposure Effects by Modelling the Expectation of Exposure Conditional on Confounders}}

@article{Porteretal11,
	Author = {K.E. Porter and S. Gruber and M.J. van der Laan and J. S. Sekhon},
	Date-Added = {2011-12-08 18:06:10 -0500},
	Date-Modified = {2011-12-08 18:08:07 -0500},
	Journal = {The International Journal of Biostatistics},
	Number = {31},
	Issue = {1},
	Pages = {1-34},
	Title = {The Relative Performance of Targeted Maximum Likelihood Estimators},
	Volume = {7},
	Year = {2011}}

@article{Petersenetal10,
	Author = {M.L. Petersen and K.E. Porter and S. Gruber and Y. Wang and M.J. van der Laan},
	Date-Added = {2011-12-08 18:04:58 -0500},
	Date-Modified = {2011-12-08 18:04:58 -0500},
	Journal = {Stat Meth Med Res},
	Title = {Diagnosing and responding to violations in the positivity assumption},
	Volume = {published online 28 Oct (doi: 10.1177/0962280210386207)},
	Year = {2010}}

@techreport{Polley&vanderLaan10,
	Author = {E. C. Polley and M. J. van der Laan},
	Date-Added = {2011-07-11 21:14:27 -0700},
	Date-Modified = {2011-07-11 21:16:20 -0700},
	Institution = {U.C. Berkeley Division of Biostatistics Working Paper Series},
	Number = {200},
	Title = {Super Learner in Prediction},
	Year = {2010}}

@article{Breiman01c,
	Author = {L. Breiman},
	Date-Added = {2011-07-11 21:01:09 -0700},
	Date-Modified = {2011-07-11 21:02:03 -0700},
	Journal = {Machine Learning},
	Number = {1},
	Pages = {5-32},
	Title = {Random Forests},
	Volume = {45},
	Year = {2001}}

@techreport{Gruber&vanderLaan10c,
	Author = {S. Gruber and M.J. van der Laan},
	Date-Added = {2011-04-03 23:22:01 -0700},
	Date-Modified = {2011-04-03 23:22:01 -0700},
	Institution = {UC Berkeley},
	Number = {265},
	Title = {A Targeted Maximum Likelihood Estimator of a Causal Effect on a Bounded Continuous Outcome},
	Year = {2010}}

@book{Pearl00,
	Author = {J. Pearl},
	Date-Added = {2011-04-03 23:19:36 -0700},
	Date-Modified = {2011-04-03 23:19:36 -0700},
	Publisher = {Cambridge University Press, Cambridge},
	Title = {Causality: Models, Reasoning, and Inference},
	Year = {2000}}

@article{Imai&vanDyk04,
	Author = {K. Imai and D.A. van Dyk},
	Journal={Journal of the American Statistical Association},
	Volume={99},
	pages={854-66},
	year={2004},
	title={Causal inference with general treatment regimes: generalizing the propensity score}}


@article{Rotnitzkyetal12,
	Author = {A. Rotnitzky and Q. Lei and M. Sued and J. Robins},
	Journal={Biometrika},
	Volume = {99},
	Issue = {2},
	pages = {439-56},
	Title = {Improved Double-Robust Estimation in missing data and causal inference models},
	Year = {2012}}


@misc{Rotnitzkyetal11,
	Author = {A. Rotnitzky and Q. Lei and M. Sued and J. Robins},
	Date-Added = {2011-04-02 21:41:14 -0700},
	Date-Modified = {2011-04-03 23:25:42 -0700},
	Howpublished = {ENAR 2011 Spring Meeting},
	Month = {March},
	Title = {Enhanced Double-Robust Locally- Efficient Estimation in Regression Models for Longitudinal Studies},
	Year = {2011}}

@article{Rotnitzky&Li&Li10,
	Author = {A. Rotnitzky and L. Li and X. Li},
	Date-Added = {2011-03-14 17:15:47 -0700},
	Date-Modified = {2011-03-15 10:47:49 -0700},
	Journal = {Biometrika},
	Number = {4},
	Pages = {997-1001},
	Title = {A note on overadjustment in inverse probability weighted estimation},
	Type = {article},
	Volume = {97},
	Year = {2010}}

@manual{trustPKG,
	Author = {C. J. Geyer},
	Date-Added = {2011-03-07 21:04:15 -0800},
	Date-Modified = {2011-03-07 21:04:15 -0800},
	Note = {R package version 0.1-2},
	Title = {trust: Trust Region Optimization},
	Url = {http://CRAN.R-project.org/package=trust},
	Year = {2009},
	Bdsk-Url-1 = {http://CRAN.R-project.org/package=trust}}

@manual{alabamaPKG,
	Author = {R. Varadhan},
	Date-Added = {2011-03-07 21:04:06 -0800},
	Date-Modified = {2011-03-07 21:04:06 -0800},
	Note = {R package version 2010.10-1},
	Title = {alabama: Constrained nonlinear optimization},
	Url = {http://CRAN.R-project.org/package=alabama},
	Year = {2010},
	Bdsk-Url-1 = {http://CRAN.R-project.org/package=alabama}}

@article{Bembometal09b,
	Author = {O. Bembom and M.L. Petersen and S.-Y. Rhee and W. J. Fessel and S.E. Sinisi and R.W. Shafer and M.J. van der Laan},
	Date-Added = {2011-02-28 15:57:47 -0800},
	Date-Modified = {2011-02-28 15:57:47 -0800},
	Issue = {1},
	Journal = {Statistics in Medicine},
	Pages = {152-72},
	Title = {Biomarker discovery using targeted maximum likelihood estimation: Application to the treatment of antiretroviral resistant {HIV} infection},
	Volume = {28},
	Year = {2009}}

@article{Holland77,
	Address = {New York, NY, USA},
	Author = {J.H. Holland and J.S. Reitman},
	Date-Added = {2011-02-28 15:57:47 -0800},
	Date-Modified = {2011-02-28 15:57:47 -0800},
	Doi = {http://doi.acm.org/10.1145/1045343.1045373},
	Issn = {0163-5719},
	Journal = {SIGART Bull.},
	Pages = {49--49},
	Publisher = {ACM},
	Title = {Cognitive systems based on adaptive algorithms},
	Volume = {63},
	Year = {1977},
	Bdsk-Url-1 = {http://doi.acm.org/10.1145/1045343.1045373}}

@article{Abadie&Imbens06,
	Author = {A. Abadie and G.W. Imbens},
	Date-Added = {2011-02-28 15:57:47 -0800},
	Date-Modified = {2011-02-28 15:57:47 -0800},
	Issue = {1},
	Journal = {Econometrica},
	Pages = {235-67},
	Title = {Large Sample Properties of Matching Estimators for Average Treatment Effects},
	Volume = {74},
	Year = {2006}}

@article{hernan&brumback&robins03,
	Author = {Hernan, M. A. and Brumback, B. and Robins, J. M.},
	Date-Added = {2011-02-28 15:57:47 -0800},
	Date-Modified = {2011-02-28 15:57:47 -0800},
	Journal = {Epidemiology},
	Number = {5},
	Pages = {561--570},
	Title = {Marginal structural models to estimate the causal effect of zidovudine on the survival of {HIV}-positive men},
	Volume = {11},
	Year = {2000}}

@techreport{Bembom&Fessel&Shafer&vanderLaan08,
	Author = {O. Bembom and J.W. Fessel and R.W. Shafer and M.J. van der Laan},
	Date-Added = {2011-02-28 15:57:47 -0800},
	Date-Modified = {2011-02-28 15:57:47 -0800},
	Institution = {DigitalCommons@Florida Atlantic University [http://digitalcommons.fau.edu/cgi/oai2.cgi] (United States)},
	Keywords = {General Biostatistics},
	Location = {http://www.scientificcommons.org/36721107},
	Publisher = {The Berkeley Electronic Press},
	Title = {Data-adaptive Selection Of The Adjustment Set In Variable Importance Estimation},
	Url = {http://www.bepress.com/ucbbiostat/paper231},
	Year = {2008},
	Bdsk-Url-1 = {http://www.bepress.com/ucbbiostat/paper231}}

@article{vanderLaan&Gruber09,
	Author = {M.J. van der Laan and S. Gruber},
	Date-Added = {2011-02-22 20:50:28 -0800},
	Date-Modified = {2011-02-22 20:50:28 -0800},
	Journal = {The International Journal of Biostatistics},
	Title = {Collaborative Double robust penalized targeted maximum likelihood estimation},
	Year = {2009}}

@manual{HmiscPKG,
	Author = {F.E. {Harrell Jr}},
	Date-Added = {2011-02-22 20:48:50 -0800},
	Date-Modified = {2011-02-22 20:48:50 -0800},
	Note = {R package version 3.8-3},
	Title = {Hmisc: Harrell Miscellaneous},
	Url = {http://CRAN.R-project.org/package=Hmisc},
	Year = {2010},
	Bdsk-Url-1 = {http://CRAN.R-project.org/package=Hmisc}}

@article{Freedman&Berk08,
	Author = {D.A. Freedman and R.A. Berk},
	Date-Added = {2011-02-22 20:47:43 -0800},
	Date-Modified = {2011-03-13 16:18:51 -0700},
	Issue = {4},
	Journal = {Evaluation Review},
	Pages = {392-409},
	Title = {Weighting Regressions by Propensity Scores},
	Volume = {32},
	Year = {2008}}

@article{Shpitser08,
	Author = {I. Shpitser and J. Pearl},
	Journal = {Journal of Machine Learning Research},
	Pages = {1941-79},
	Title = {Complete Identification Methods for the Causal Hierarchy},
	Volume = {9},
	Year = {2008}}

@article{Tan08,
	Author = {Z. Tan},
	Date-Added = {2011-02-22 20:42:13 -0800},
	Date-Modified = {2011-02-22 20:42:13 -0800},
	Issue = {2},
	Journal = {Biometrika},
	Pages = {1-22},
	Title = {Bounded, efficient, and doubly robust estimation with inverse weighting},
	Volume = {94},
	Year = {2008}}

@article{McCullagh83,
	Author = {P. Mc{C}ullagh},
	Date-Added = {2011-02-22 20:42:13 -0800},
	Date-Modified = {2011-02-22 20:42:13 -0800},
	Issue = {1},
	Journal = {The Annals of Statistics},
	Pages = {59-67},
	Title = {Quasi-likelihood functions},
	Volume = {11},
	Year = {1983}}

@article{Dehejia&Wahba02,
	Author = {R.H. Dehejia and S. Wahba},
	Date-Added = {2011-02-22 20:42:13 -0800},
	Date-Modified = {2011-02-22 20:42:13 -0800},
	Journal = {The Review of Economics and Statistics},
	Pages = {151-61},
	Title = {Propensity Score Matching Methods for Nonexperimental Causal Studies},
	Volume = {84},
	Year = {2002}}

@article{Stukeletal07,
	Author = {T.A. Stukel and E.S. Fisher and D.E. Wennberg and D.A.Alter and D.J.Gottlieb and M.J. Vermeulen},
	Date-Added = {2011-02-22 20:42:13 -0800},
	Date-Modified = {2011-02-22 20:42:13 -0800},
	Journal = {JAMA},
	Pages = {278-85},
	Title = {Analysis of Observational Studies in the Presence of Treatment Selection Bias: Effects of Invasive Cardiac Management on {AMI} Survival Using Propensity Score and Instrumental Variable Methods},
	Volume = {297},
	Year = {2007}}

@book{mark,
	Author = {M.J. van der Laan and J.M. Robins},
	Date-Added = {2011-02-22 20:42:13 -0800},
	Date-Modified = {2011-02-22 20:42:13 -0800},
	Publisher = {Springer, New York},
	Title = {Unified methods for censored longitudinal data and causality},
	Year = {2003}}

@book{vanderLaan&Rose11,
	Author = {M.J. van der Laan and S. Rose},
	Publisher = {Springer, New York},
	Title = {Targeted Learning: Prediction and Causal Inference for Observational and Experimental Data},
	Year = {2011}}

@incollection{KS_vanderLaan&Rose11,
	Author = {J.S. Sekhon and S. Gruber and K. Porter and M.J. van der Laan},
	Booktitle = {{\rm M.J. van der Laan and S. Rose, } Targeted Learning: Prediction and Causal Inference for Observational and Experimental Data},
	Chapter = {21},
	Publisher = {Springer, New York},
	Title = {Propensity-Score-Based Estimators and {C-TMLE}},
	Year = {2011}}


	@incollection{RosenblumTMLEChapter,
	Author = {M. Rosenblum},
	Booktitle = {{\rm M.J. van der Laan and S. Rose, } Targeted Learning: Prediction and Causal Inference for Observational and Experimental Data},
	Chapter = {9},
	Publisher = {Springer, New York},
	Title = {Marginal Structural Models},
	Year = {2011}}

	@incollection{GruberCTMLEChapter,
	Author = {S. Gruber and M.J. van der Laan},
	Booktitle = {{\rm M.J. van der Laan and S. Rose, } C-TMLE of an Additive Point Treatment Effect},
	Chapter = {19},
	Publisher = {Springer, New York},
	Title = {Marginal Structural Models},
	Year = {2011}}


	@incollection{AntoineTMLEChapter,
	Author = {A. Chambaz},
	Booktitle = {{\rm M.J. van der Laan and S. Rose, } Targeted Learning: Prediction and Causal Inference for Observational and Experimental Data},
	Chapter = {29},
	Publisher = {Springer, New York},
	Title = {TMLE in Adaptive Group Sequential Covariate-Adjusted RCTs},
	Year = {2011}}





@article{Stitelman&vanderLaan10,
	Author = {O.M. Stitelman and M.J. van der Laan},
	Date-Added = {2011-02-22 20:35:37 -0800},
	Date-Modified = {2011-12-08 18:09:52 -0500},
	Journal = {The International Journal of Biostatistics},
	Number = {1},
	Title = {Collaborative Targeted Maximum Likelihood for Time to Event Data},
	Volume = {6},
	Year = {2010}}

@article{Breslow74,
	Author = {Breslow, N.},
	Date-Added = {2010-06-28 13:31:45 -0700},
	Date-Modified = {2010-06-28 13:33:19 -0700},
	Journal = {Biometrics},
	Month = {March},
	Number = {1},
	Pages = {89-99},
	Title = {Covariance Analysis of Censored Survival Data},
	Volume = {30},
	Year = {1974}}

@article{Effronetal02,
	Author = {Efron, B. and Hastie H. and Johnstone and Tibshirani},
	Date-Added = {2010-05-27 13:34:30 -0700},
	Date-Modified = {2010-05-27 13:36:40 -0700},
	Journal = {The Annals of Statistics},
	Title = {Least Angle Regression (with discussion)},
	Year = {2003}}

@manual{RDCT10,
	Address = {Vienna, Austria},
	Author = {R Development Core Team},
	Date-Added = {2010-05-27 13:15:41 -0700},
	Date-Modified = {2010-05-27 13:18:22 -0700},
	Organization = {R Foundation for Statistical Computing},
	Title = {{R}: A Language and Environment for Statistical Computing},
	Url = {http://www.R-project.org},
	Year = {2010},
	Bdsk-Url-1 = {http://www.R-project.org}}


@manual{RDCT12,
	Address = {Vienna, Austria},
	Author = {{R Development Core Team}},
	Date-Added = {2010-05-27 13:15:41 -0700},
	Date-Modified = {2010-05-27 13:18:22 -0700},
	Organization = {{R} Foundation for Statistical Computing},
	Title = {{R}: A Language and Environment for Statistical Computing},
	Url = {http://www.R-project.org},
	Year = {2012},
	Bdsk-Url-1 = {http://www.R-project.org}}

  @Manual{RDCT11,
    title = {R: A Language and Environment for Statistical Computing},
    author = {{R Development Core Team}},
    organization = {R Foundation for Statistical Computing},
    address = {Vienna, Austria},
    year = {2011},
    note = {{ISBN} 3-900051-07-0},
    url = {http://www.R-project.org/},
  }

@manual{bartPKG,
	Author = {Hugh Chipman and Robert McCulloch},
	Note = {{R} package version~0.3-1.1},
	Title = {{BayesTree}: Bayesian Methods for Tree Based Models},
	Url = {http://CRAN.R-project.org/package=BayesTree},
	Year = {2010},
	Bdsk-Url-1 = {http://CRAN.R-project.org/package=BayesTree}}

@manual{SLPKG,
	Author = {E.C. Polley},
	Note = {{R}~package version~1.1-17},
	Title = {{SuperLearner}: {S}uper {L}earner Prediction},
	Url = {http://www.stat.berkeley.edu/~ecpolley/SL/},
	Year = {2010},
	Bdsk-Url-1 = {http://www.stat.berkeley.edu/~ecpolley/SL/}}

@manual{caretPKG,
	Author = {M. Kuhn and J. Wing and S. Weston and A. Williams and C. Keefer and A. Engelhardt},
	Note = {{R} package version~4.72},
	Title = {{caret}: Classification and Regression Training},
	Url = {http://CRAN.R-project.org/package=caret},
	Year = {2010},
	Bdsk-Url-1 = {http://CRAN.R-project.org/package=caret}}

@manual{TMLEPKG,
	Author = {S. Gruber},
	Note = {{R}~package version~1.2.0},
	Title = {{tmle}: Targeted Maximum Likelihood Estimation},
	Url = {http://CRAN.R-project.org/package=tmle},
	Year = {2012},
	Bdsk-Url-1 = {http://CRAN.R-project.org/package=tmle}}

@manual{CTMLEPKG,
	Author = {S. Gruber},
	Note = {{R}~software version~0.5},
	Title = {Collaborative Targeted Maximum Likelihood Estimation},
	Url = {http://www.stat.berkeley.edu/~laan/Software/},
	Year = {2010},
	Bdsk-Url-1 = {http://www.stat.berkeley.edu/~laan/Software/}}

@article{SL_jss,
	Author = {E.C. Polley and M.J. van der Laan},
	Note = {submitted...},
	Title = {Super Learner},
	Year = {2011}}

@manual{ipredPKG,
	Author = {A. Peters and T. Hothorn},
	Note = {{R} package version~0.8-8},
	Title = {{ipred}: Improved Predictors},
	Url = {http://CRAN.R-project.org/package=ipred},
	Year = {2009},
	Bdsk-Url-1 = {http://CRAN.R-project.org/package=ipred}}

@manual{dsaPKG,
	Author = {R. Neugebauer and J. Bullard},
	Note = {{R} package version~3.1.4},
	Title = {{DSA}: Deletion/Substitution/Addition Algorithm},
	Url = {http://www.stat.berkeley.edu/~laan/Software/},
	Year = {2010},
	Bdsk-Url-1 = {http://www.stat.berkeley.edu/~laan/Software/}}

@manual{earthPKG,
	Author = {S. Milborrow},
	Note = {{R} package version~2.4-0},
	Title = {{earth}: Multivariate Adaptive Regression Spline Models},
	Url = {http://CRAN.R-project.org/package=earth},
	Year = {2009},
	Bdsk-Url-1 = {http://CRAN.R-project.org/package=earth}}

@book{nnetPKG,
	Address = {New York},
	Author = {W. N. Venables and B. D. Ripley},
	Edition = {4th},
	Note = {ISBN 0-387-95457-0},
	Publisher = {Springer},
	Title = {Modern Applied Statistics with S},
	Url = {http://www.stats.ox.ac.uk/pub/MASS4},
	Year = {2002},
	Bdsk-Url-1 = {http://www.stats.ox.ac.uk/pub/MASS4}}

@manual{e1071PKG,
	Author = {E. Dimitriadou and K. Hornik and F. Leisch and D. Meyer and and A. Weingessel},
	Note = {{R} package version~1.5-24},
	Title = {{e1071}: Misc Functions of the Department of Statistics (e1071), TU Wien},
	Url = {http://CRAN.R-project.org/package=e1071},
	Year = {2010},
	Bdsk-Url-1 = {http://CRAN.R-project.org/package=e1071}}

@manual{gamPKG,
	Author = {T.J. Hastie},
	Note = {{R} package version~1.01},
	Title = {{gam}: Generalized Additive Models},
	Url = {http://CRAN.R-project.org/package=gam},
	Year = {2009},
	Bdsk-Url-1 = {http://CRAN.R-project.org/package=gam}}

@article{Zhang&Yu98,
	Author = {Zhang, J and Yu, KF},
	Date-Added = {2010-05-26 14:58:38 -0700},
	Date-Modified = {2010-05-26 15:00:17 -0700},
	Journal = {JAMA},
	Pages = {1690-1},
	Title = {What's relative risk? A method of correcting the odds ratio in cohort studies of common outcomes},
	Volume = {280},
	Year = {1998}}

@article{Zocchettietal97,
	Author = {Zocchetti, C and Consonni, D and Bertazzi, P A},
	Date-Added = {2010-05-26 14:54:07 -0700},
	Date-Modified = {2010-05-26 14:57:40 -0700},
	Journal = {International Journal of Epidemiology},
	Pages = {220-223},
	Title = {Relationship between prevalence rate ratios and odds ratios in cross-sectional studies},
	Volume = {26},
	Year = {1997}}

@article{Greenland03,
	Author = {Greenland, S},
	Date-Added = {2010-05-26 14:39:43 -0700},
	Date-Modified = {2010-05-26 14:41:15 -0700},
	Journal = {Am J Epidemiol},
	Number = {4},
	Pages = {301-305},
	Title = {Model-based Estimation of Relative Risks and Other Epidemiologic Measures in Studies of Common Outcomes and in Case-Control Studies},
	Volume = {160},
	Year = {2003}}

@article{Hogueetal83,
	Author = {Hogue, C.J.R. and Gaylor, DW and Schulz, KF},
	Date-Added = {2010-05-26 14:32:50 -0700},
	Date-Modified = {2010-05-26 14:34:43 -0700},
	Journal = {Am J Epidemiol},
	Number = {3},
	Pages = {396-407},
	Title = {Estimators of Relative Risk for Case-Control Studies},
	Volume = {118},
	Year = {1983}}

@article{Carteretal05,
	Author = {Carter, RE and Lipsitz, SR and Tilley, BC},
	Date-Added = {2010-05-26 13:07:18 -0700},
	Date-Modified = {2010-05-26 13:08:31 -0700},
	Title = {Quasi-likelihood estimation for relative risk regression models}}

@article{McNuttetal01,
	Author = {McNutt, Louise-Anne and hu, Chuntao and Xue, Xiaonana and Hafner, Paul},
	Date-Added = {2010-05-26 12:38:16 -0700},
	Date-Modified = {2010-05-26 12:40:01 -0700},
	Journal = {Am J Epidemiol},
	Number = {10},
	Pages = {940-943},
	Title = {Estimating the Relative Risk in Cohort Studies and Clinical Trials of Common Outcomes},
	Volume = {157},
	Year = {2003}}

@article{Zou04,
	Author = {Zou, G.},
	Date-Added = {2010-05-26 11:56:32 -0700},
	Date-Modified = {2010-05-26 11:57:29 -0700},
	Journal = {Am J Epidemiol},
	Pages = {702-6},
	Title = {A modified Poisson regresion approach to prospective studies with binary data},
	Volume = {159},
	Year = {2004}}

@article{Zocchettietal95,
	Author = {Zocchett, C and Consonni, Dario and Bertazzi, Pier Alberto},
	Date-Added = {2010-05-26 11:50:39 -0700},
	Date-Modified = {2010-05-26 11:52:18 -0700},
	Journal = {Int J Epidemiol},
	Pages = {1064-1105},
	Title = {RE: Estimation of prevalence rate ratios from cross-sectional data (letter)},
	Volume = {24},
	Year = {1995}}

@article{Skovetal98,
	Author = {Skov, T and Deddens, J.A. and Petersen, M.R.},
	Date-Added = {2010-05-26 11:47:20 -0700},
	Date-Modified = {2010-05-26 11:50:06 -0700},
	Journal = {Int J Epidemiol},
	Pages = {91-95},
	Title = {Prevalence proportion ratios: estimation and hypothesis testing},
	Volume = {27},
	Year = {1998}}

@proceedings{Deddensetal08,
	Address = {Cary, NC},
	Author = {Deddens, J.A. and Petersen, M.R. and Lei, X.},
	Date-Added = {2010-05-24 14:27:56 -0700},
	Date-Modified = {2010-05-24 14:31:49 -0700},
	Number = {270-28},
	Organization = {SAS Institute},
	Publisher = {Proceedings of the 28th Annual SAS Users Group International Conference, March 30-April 2, 2003},
	Title = {Estimation of prevalence ratios when PROC GENMOD does not converge},
	Year = {2003}}

@article{Lee&Chia98,
	Author = {Lee, J and Chia, KS},
	Date-Added = {2010-05-24 14:06:12 -0700},
	Date-Modified = {2010-05-24 14:07:51 -0700},
	Journal = {Br J Ind Med},
	Pages = {861-2},
	Title = {Estimation of prevalence rate ratios for cross-sectional data: an example in occupational epidemiology},
	Volume = {50},
	Year = {1993}}

@article{Lee94,
	Author = {Lee, J.},
	Date-Added = {2010-05-24 14:04:58 -0700},
	Date-Modified = {2010-05-24 14:09:36 -0700},
	Journal = {Int J Epidemiol},
	Pages = {201-3},
	Title = {Odds ratio or relative risk for cross-sectional data?},
	Volume = {23},
	Year = {1994}}

@article{Wacholder86,
	Author = {Wacholder, S},
	Date-Added = {2010-05-24 13:59:47 -0700},
	Date-Modified = {2010-05-24 14:01:31 -0700},
	Journal = {Am J Epidemiol},
	Pages = {174-84},
	Title = {Binomial regression in {GLIM}, estimating risk ratios and risk differences.},
	Volume = {123},
	Year = {1986}}

@techreport{Lumleyetal06,
	Author = {Lumley, Thomas and Kronmal, Richard and Ma, Shuangge},
	Date-Added = {2010-05-24 13:27:04 -0700},
	Date-Modified = {2010-05-24 13:29:21 -0700},
	Institution = {University of Washington},
	Number = {293},
	Title = {Relative Risk Regresssion in Medical Research: Models, Contrasts, Estimators, and Algorithms},
	Year = {2006}}

@article{Barros&Hirakata03,
	Author = {Barros, Alu{\'\i}sio J D and Hirakata, V{\^a}nia N},
	Date-Added = {2010-05-24 13:25:16 -0700},
	Date-Modified = {2010-05-24 13:25:16 -0700},
	Doi = {10.1186/1471-2288-3-21},
	Journal = {BMC Med Res Methodol},
	Journal-Full = {BMC medical research methodology},
	Mesh = {Cross-Sectional Studies; Empirical Research; Humans; Linear Models; Logistic Models; Models, Statistical; Odds Ratio; Poisson Distribution; Prevalence; Proportional Hazards Models},
	Month = {Oct},
	Pages = {21},
	Pmc = {PMC521200},
	Pmid = {14567763},
	Pst = {epublish},
	Title = {Alternatives for logistic regression in cross-sectional studies: an empirical comparison of models that directly estimate the prevalence ratio},
	Volume = {3},
	Year = {2003},
	Bdsk-Url-1 = {http://dx.doi.org/10.1186/1471-2288-3-21}}

@article{Neutra&Drolette78,
	Author = {Neutra, R R and Drolette, M E},
	Date-Added = {2009-10-05 15:02:58 -0700},
	Date-Modified = {2009-10-05 15:02:58 -0700},
	Journal = {Am J Epidemiol},
	Journal-Full = {American journal of epidemiology},
	Mesh = {Biometry; Communicable Diseases; Environmental Exposure; Humans; Methods; Models, Theoretical; Probability Theory; Retrospective Studies},
	Month = {Sep},
	Number = {3},
	Pages = {214-22},
	Pmid = {707490},
	Title = {Estimating exposure-specific disease rates from case-control studies using Bayes' theorem},
	Volume = {108},
	Year = {1978}}

@article{Miettinen76,
	Author = {Miettinen, Olli S},
	Date-Added = {2009-10-05 13:42:11 -0700},
	Date-Modified = {2009-10-05 13:43:23 -0700},
	Journal = {American Journal of Epidemiology},
	Pages = {226-35.},
	Title = {Estimability and estimation in case-referent studies},
	Volume = {103},
	Year = {1976}}

@book{Checkowayetaletal04,
	Author = {Harvey Checkoway and Neil Pearce and David Kriebel},
	Date-Added = {2009-10-05 14:34:34 -0700},
	Date-Modified = {2009-10-05 14:36:29 -0700},
	Publisher = {Oxford University Press},
	Title = {Research Methods in Occupational Epidemiology},
	Year = {2004}}

@article{Kang&Schafer07,
	Author = {J. Kang and J. Schafer},
	Journal = {Statistical Science},
	Pages = {523-39},
	Title = {Demystifying Double Robustness: A Comparison of Alternative Strategies for Estimating a Population Mean from Incomplete Data (with discussion)},
	Volume = {22},
	Year = {2007}}

@article{Robinsetal07,
	Author = {J. M. Robins and M. Sued and Q. Lei-Gomez and A. Rotnitzky},
	Journal = {Statistical Science},
	Pages = {544-559},
	Title = {Comment: Performance of Double-Robust Estimators When ``Inverse Probability'' Weights Are Highly Variable},
	Volume = {22},
	Year = {2007}}

@article{Tan07,
	Author = {Z. Tan},
	Journal = {Statistical Science},
	Pages = {560-568},
	Title = {Comment: Understanding {OR}, {PS} and {DR}},
	Volume = {22},
	Year = {2007}}

@article{Neugebauer&vanderLaan05,
	Author = {R. Neugebauer and M.J. van der Laan},
	Journal = {Journal of Statistical Planning and Inference},
	Pages = {405--426},
	Title = {Why prefer double robust estimators in causal inference?},
	Volume = {129, Issues 1-2},
	Year = {2005}}

@article{vanderLaan&Petersen07,
	Author = {M.J. van der Laan and M.L. Petersen},
	Journal = {The International Journal of Biostatistics},
	Title = {Causal Effect Models for Realistic Individualized Treatment and Intention to Treat Rules},
	Volume = {3, Issue 1, Article 3},
	Year = {2007}}

@article{Tsiatis&Davidian07,
	Author = {A. Tsiatis and M. Davidian},
	Journal = {Statistical Science},
	Pages = {569-73},
	Title = {Comment: Demystifying Double Robustness: A Comparison of Alternative Strategies for Estimating a Population Mean from Incomplete Data (with discussion)},
	Volume = {22},
	Year = {2007}}

@article{Kang&Shafer07b,
	Author = {J. Kang and J. Schafer},
	Journal = {Statistical Science},
	Pages = {574-80},
	Title = {Rejoinder: Demystifying Double Robustness: A Comparison of Alternative Strategies for Estimating a Population Mean from Incomplete Data},
	Volume = {22},
	Year = {2007}}

@article{Schafer99,
	Author = {J.L. Schafer},
	Issue = {1},
	Journal = {Stat Methods Med Res},
	Month = {March},
	Pages = {3-15},
	Title = {Multiple imputation: a primer},
	Volume = {8},
	Year = {1999}}

@article{Pearl10a,
	Author = {J. Pearl},
	Journal = {The International Journal of Biostatistics},
	Number = {2},
	Title = {An Introduction to Causal Inference},
	Volume = {6},
	Year = {2010}}

@article{Hampel74,
	Author = {F.R. Hampel},
	Journal = {Journal of the American Statistical Association},
	Number = {346},
	Pages = {383-93},
	Title = {The Influence Curve and Its Role in Robust Estimation},
	Volume = {69},
	Year = {1974}}

@article{Murphy05,
	Author = {S. Murphy},
	Journal = {Statistics in Medicine},
	Title = {An experimental design for the development of adaptive treatment strategies},
	Volume = {24},
	Year = {2005}}

@article{Lavori&Dawson00,
	Author = {P. Lavori and R. Dawson},
	Journal = {Journal of the Royal Statistical Society, Series A},
	Title = {A design for testing clinical strategies: biased adaptive within-subject randomization},
	Volume = {163},
	Year = {2000}}

@article{Lavori&Dawson04,
	Author = {P. Lavori and R. Dawson},
	Journal = {Clinical trials},
	Title = {Dynamic treatment regimes: practical design considerations},
	Volume = {1},
	Year = {2004}}

@article{Thall&Millikan&Sung00,
	Author = {P. Thall and R. Millikan and H.-G. Sung},
	Journal = {Statistics in Medicine},
	Title = {Evaluating multiple treatment courses in clinical trials},
	Volume = {19},
	Year = {2000}}

@article{Rush&Trivedi&Fava03,
	Author = {A.J. Rush and M. Trivedi and M. Fava},
	Journal = {IV. American Journal of Psychiatry},
	Pages = {237},
	Title = {Depression},
	Volume = {160(2)},
	Year = {2003}}

@article{Schneideretal06,
	Author = {Schneider, L. and Tariot.P.N. and Dagerman, K. and Davis, S. and Hsiao, J. and Ismail, S. and Lebowitz, B. and Lyketsos, C. and Ryan J. and Stroup T. and Sultzer D. and Weintraub, D. and Lieberman, J.},
	Journal = {New England Journal of Medicine},
	Volume = {355(15)},
	Year = {2006}}

@article{Swartzetal07,
	Author = {Swartz, M. and Perkins, D. and Stroup, T. and Davis, S. and Capuano, G. and Rosenheck, R. and Reimherr, F. and McGee, M. and Keefe, R. and McEvoy, J. and Hsiao, J. and Lieberman, J.},
	Journal = {American Journal of Psychiatry},
	Title = {Effects of antipsychotic medications on psychosocial functioning in patients with chronic shizophrenia: Findings from the nimh catie study},
	Volume = {164},
	Year = {2007}}

@article{Rubin&vanderLaan08,
	Author = {D.B. Rubin and M.J. van der Laan},
	Journal = {The International Journal of Biostatistics},
	Location = {http://www.bepress.com/ijb/vol4/iss1/5},
	Title = {Empirical Efficiency Maximization: Improved Locally Efficient Covariate Adjustment in Randomized Experiments and Survival Analysis},
	Volume = {Vol. 4, Iss. 1, Article 5},
	Year = {2008}}

@article{vanderLaan&Rubin07,
	Author = {M.J. van der Laan and D.B. Rubin},
	Journal = {Technical report, working paper series http://www.bepress.com/ucbbiostat/paper226},
	Title = {A Note on Targeted Maximum Likelihood and Right Censored Data},
	Year = {2007}}

@article{vanderLaan&Rose&Gruber09,
	Author = {M.J. van der Laan and S. Rose and S. Gruber},
	Journal = {U.C. Berkeley Division of Biostatistics Working Paper Series, Paper 254},
	Title = {Readings in Targeted Maximum Likelihood Estimation},
	Year = {2009}}

@article{Bembometal09,
	Author = {O. Bembom and M.J. van der Laan and T. Haight and I.B. Tager},
	Journal = {Epidemiology},
	Title = {Lifetime and current leisure time physical activity and all-cause mortality in an elderly cohort},
	Year = {2009}}

@article{Bembom&vanderLaan07a,
	Author = {O. Bembom and M.J. van der Laan},
	Journal = {Journal of the National Cancer Institute},
	Pages = {1577-1582},
	Title = {Statistical Methods for analyzing sequentially randomized trials, commentary on JNCI article Adaptive therapy for androgen independent prostate cancer: A Randomized selection trial including four regimens, by Peter F. Thall, C. Logothetis, C. Pagliaro, S. Wen, M.A. Brown, D. Williams, R. Millikan (2007).},
	Volume = {99(21)},
	Year = {2007}}

@article{Rosenblumetal09,
	Author = {M. Rosenblum and S.G. Deeks and M.J. van der Laan and D.R. Bangsberg},
	Journal = {PLoS ONE},
	Title = {The Risk of Virologic Failure Decreases with Duration of HIV Suppression, at Greater than 50\% Adherence to Antiretroviral Therapy},
	Volume = {4(9): e7196.doi:10.1371/journal.pone.0007196},
	Year = {2009}}

@article{Robins&Orallana&Rotnitzky08,
	Author = {J. M. Robins and L. Orallana and A. Rotnitzky},
	Journal = {Statistics in Medicine},
	Pages = {4678-4721},
	Title = {Estimaton and extrapolation of optimal treatment and testing strategies},
	Volume = {27(23)},
	Year = {2008}}

@article{Bembom&vanderLaan07,
	Author = {O. Bembom and M.J. van der Laan},
	Journal = {Electronic Journal of Statistics},
	Pages = {http://www.i-journals.org/ejs/viewarticle.php?id=105&layout=abstract},
	Title = {A practical illustration of the importance of realistic individualized treatment rules in causal inference},
	Year = {2007}}

@article{Bembometal08,
	Author = {O. Bembom and M.L. Petersen and S.-Y. Rhee and W. J. Fessel and S.E. Sinisi and R.W. Shafer and M.J. van der Laan},
	Journal = {Statistics in Medicine},
	Pages = {http://www3.interscience.wiley.com/journal/121422393/abstract},
	Title = {Biomarker discovery using targeted maximum likelihood estimation: Application to the treatment of antiretroviral resistant HIV infection},
	Year = {2008}}

@article{Tuglus&vanderLaan08,
	Author = {C. Tuglus and M.J. van der Laan},
	Journal = {UC Berkeley Working Paper Series},
	Pages = {http://www.bepress.com/ucbbiostat/paper233/.},
	Title = {Targeted Methods for Biomarker Discovery, the Search for a Standard},
	Year = {2008}}

@article{vanderLaan08,
	Author = {M.J. van der Laan},
	Journal = {The International Journal of Biostatistics},
	Pages = {http://www.bepress.com/ijb/vol4/iss1/17/},
	Title = {Estimation Based on Case-Control Designs with Known Prevalance Probability},
	Year = {2008}}

@article{Rose&vanderLaan08,
	Author = {S. Rose and M.J. van der Laan},
	Journal = {The International Journal of Biostatistics},
	Pages = {http://www.bepress.com/ijb/vol4/iss1/19/.},
	Title = {Simple Optimal Weighting of Cases and Controls in Case-Control Studies},
	Year = {2008}}

@article{Rose&vanderLaan09,
	Author = {S. Rose and M.J. van der Laan},
	Journal = {The International Journal of Biostatistics},
	Pages = {http://www.bepress.com/ijb/vol5/iss1/1/.},
	Title = {Why Match? [Investigating Matched Case-Control Study Designs with Causal Effect Estimation},
	Year = {2009}}

@inproceedings{Moore&vanderLaan09,
	Author = {K.L. Moore and M.J. van der Laan},
	Booktitle = {in Design, Summarization, Analysis \& Interpretation of Clinical Trials with Time-to-Event Endpoints},
	Editor = {Karl E. Peace},
	Publisher = {Chapman and Hall},
	Title = {Application of Time-to-Event Methods in the Assessment of Safety in Clinical Trials},
	Year = {2009}}

@inproceedings{Polley&vanderLaan09,
	Author = {E.C. Polley and M.J. van der Laan},
	Booktitle = {in Design, Summarization, Analysis \& Interpretation of Clinical Trials with Time-to-Event Endpoints},
	Editor = {Karl E. Peace},
	Publisher = {Chapman and Hall},
	Title = {Predicting Optimal Treatment Assignment Based on Prognostic Factors in Cancer Patients},
	Year = {2009}}

@article{vanderVaart&Dudoit&vanderLaan06,
	Author = {A.W. van der Vaart and S. Dudoit and M.J. van der Laan},
	Journal = {Statistics and Decisions},
	Number = {3},
	Pages = {351--371},
	Title = {Oracle Inequalities for Multi-Fold Cross-Validation},
	Volume = {24},
	Year = {2006}}

@article{vanderLaan&Dudoit&vanderVaart06,
	Author = {M.J. van der Laan and S. Dudoit and A.W. van der Vaart},
	Journal = {Statistics and Decisions},
	Number = {3},
	Pages = {373--395},
	Title = {The Cross-Validated Adaptive Epsilon-Net Estimator},
	Volume = {24},
	Year = {2006}}

@article{Rosenbaum&Rubin83,
	Author = {P.R. Rosenbaum and D.B. Rubin},
	Journal = {Biometrika},
	Pages = {41-55},
	Title = {The Central Role of the Propensity Score in Observational Studies for Causal Effects},
	Volume = {70},
	Year = {1983}}

@article{vanderLaan&Polley&Hubbard07,
	Author = {M.J. van der Laan and E. Polley and A. Hubbard},
	Issn = {1},
	Journal = {Statistical Applications in Genetics and Molecular Biology},
	Location = {http://www.bepress.con/sagmb/vol6/iss1/art25},
	Number = {25},
	Title = {{S}uper {L}earner},
	Volume = {6},
	Year = {2007}}

@article{Sekhon08,
	Author = {J.S. Sekhon},
	Journal = {Journal of Statistical Sotware, Forthcoming},
	Location = {http://ssrn.com/paper=1009044},
	Publisher = {SSRN},
	Title = {Multivariate and Propensity Score Matching Software with Automated Balance Optimization: The Matching package for {R}},
	Year = {2008}}

@article{Bembometal08b,
	Author = {O. Bembom and J.W. Fessel and R.W. Shafer and M.J. van der Laan},
	Institution = {DigitalCommons\@Florida Atlantic University [http://digitalcommons.fau.edu/cgi/oai2.cgi] (United States)},
	Keywords = {General Biostatistics},
	Location = {http://www.scientificcommons.org/36721107},
	Publisher = {The Berkeley Electronic Press},
	Title = {Data-adaptive Selection Of The Adjustment Set In Variable Importance Estimation},
	Url = {http://www.bepress.com/ucbbiostat/paper231},
	Year = {2008},
	Bdsk-Url-1 = {http://www.bepress.com/ucbbiostat/paper231}}

@article{Holland&Reitman77,
	Address = {New York, NY, USA},
	Author = {J.H. Holland and J.S. Reitman},
	Doi = {http://doi.acm.org/10.1145/1045343.1045373},
	Issn = {0163-5719},
	Journal = {SIGART Bull.},
	Pages = {49--49},
	Publisher = {ACM},
	Title = {Cognitive systems based on adaptive algorithms},
	Volume = {63},
	Year = {1977},
	Bdsk-Url-1 = {http://doi.acm.org/10.1145/1045343.1045373}}

@book{Rubin06,
	Address = {Cambridge, MA},
	Author = {D.B. Rubin},
	Publisher = {Cambridge University Press},
	Title = {Matched Sampling for Causal Effects.},
	Year = {2006}}

@incollection{Mansk1&McFadden81,
	Address = {Cambridge, MA},
	Author = {C.F. Manski and D. McFadden},
	Booktitle = {Structural Analysis of Discrete Data with Econometric Applications},
	Editor = {C.F. Manski and D. McFadden},
	Publisher = {The MIT Press},
	Title = {Alternative estimators and sample designs for discrete choice analysis},
	Year = {1981}}

@article{Manski&Lerman77,
	Author = {C.F. Manski and S.R. Lerman},
	Journal = {Econometrica},
	Number = {8},
	Pages = {1977-1988},
	Title = {The Estimation of Choice Probabilities from Choice Based Samples},
	Volume = {45},
	Year = {1977}}

@article{Cosslett81,
	Author = {S.R. Cosslett},
	Journal = {Econometrica},
	Number = {5},
	Pages = {1289-1316},
	Title = {Maximum Likelihood Estimator for Choice-Based Samples},
	Volume = {49},
	Year = {1981}}

@article{Cornfield51,
	Author = {J. Cornfield},
	Journal = {J Nat Cancer Inst},
	Pages = {1269-1275},
	Title = {A method of estimating comparative rates from clinical data. Applications to cancer of the lung, breast, and cervix.},
	Volume = {11},
	Year = {1951}}

@inproceedings{Cornfield56,
	Author = {J. Cornfield},
	Booktitle = {Proceedings of the Third Berkeley Symposium, Volume IV},
	Editor = {J. Neyman},
	Pages = {133-148},
	Publisher = {University of California Press},
	Title = {A statistical problem arising from retrospective studies},
	Year = {1956}}

@article{Benichou&Wacholder94,
	Author = {J. Benichou and S. Wacholder},
	Journal = {Statistics in Medicine},
	Pages = {651-661},
	Title = {A comparison of three approaches to estimate exposure-specific incidence rates from population-based case-control data.},
	Volume = {13},
	Year = {1994}}

@article{Breslow&Robins&Wellner00,
	Author = {N.E. Breslow and J.M. Robins and J.A. Wellner},
	Journal = {Bernoulli},
	Pages = {447--455},
	Title = {On the semi-parametric efficiency of logistic regression under case-control sampling},
	Volume = {6(3)},
	Year = {2000}}

@article{Mansonetal07,
	Author = {R. Mansson, M.M. Joffe, W. Sun, S. Hennessy},
	Journal = {Am J Epidemiol},
	Number = {3},
	Pages = {332-339},
	Title = {On the Estimation and Use of Propensity Scores in Case-Control and Case-Cohort Studies.},
	Volume = {166},
	Year = {2007}}

@article{Anderson79,
	Author = {J.A. Anderson},
	Journal = {Biometrika},
	Pages = {19--35},
	Title = {Separate sample logistic discrimination},
	Volume = {59},
	Year = {1972}}

@article{Prentice&Pyke79,
	Author = {R.L. Prentice and R. Pyke},
	Journal = {Biometrika},
	Pages = {403--411},
	Title = {Logistic disease incidence models and case-control studies},
	Volume = {66},
	Year = {1979}}

@article{Breslow96,
	Author = {N.E. Breslow},
	Journal = {J Am Stat Soc},
	Pages = {14--28},
	Title = {Statistics in Epidemiology: the Case-Control Study},
	Volume = {91},
	Year = {1996}}

@book{Breslow&Day80,
	Address = {Lyon},
	Author = {N.E. Breslow and N.E. Day},
	Publisher = {International Agency for Research on Cancer},
	Title = {Statistical Methods in Cancer Research: Volume 1 -- The analysis of case-control studies},
	Year = {1980}}

@article{Holford&White&Kelsey78,
	Author = {T.R. Holford and C. White and J.L. Kelsey},
	Journal = {Am J Epid},
	Number = {3},
	Pages = {245--255},
	Title = {Multivariate Analysis for Matched Case-Control Studies},
	Volume = {107},
	Year = {1978}}

@article{Breslowetal78,
	Author = {N.E. Breslow and N.E. Day and K.T. Halvorsen and R.L. Prentice and C. Sabal},
	Journal = {Am J Epid},
	Number = {4},
	Pages = {299--307},
	Title = {Estimation of Multiple Relative Risk Functions in Matched Case-Control Studies},
	Volume = {108},
	Year = {1978}}

@book{Schlesselman82,
	Address = {Oxford},
	Author = {J.J. Schlesselman},
	Publisher = {Oxford University Press},
	Title = {Case-Control Studies: Design, Conduct, Analysis},
	Year = {1982}}

@book{Collett91,
	Address = {London},
	Author = {D. Collett},
	Publisher = {Chapman and Hall},
	Title = {Modeling Binary Data},
	Year = {1991}}

@book{Jewell04,
	Address = {Boca Raton},
	Author = {N.P. Jewell},
	Publisher = {Chapman and Hall/CRC},
	Title = {Statistics for Epidemiology},
	Year = {2004}}

@book{Hosmer&Lemeshow00,
	Address = {New York},
	Author = {D.W. Hosmer and S. Lemeshow},
	Edition = {2nd},
	Publisher = {John Wiley and Sons},
	Title = {Applied Logistic Regression},
	Year = {2000}}

@article{Robins99,
	Author = {J.M. Robins},
	Journal = {Statistical Science},
	Number = {3},
	Pages = {281--293},
	Title = {[Choice as an Alternative to Control in Observational Studies]: Comment},
	Volume = {14},
	Year = {1999}}

@article{Newman06,
	Author = {S. Newman},
	Journal = {Epid Persp Innov},
	Pages = {2},
	Title = {Causal Analysis of Case-Control Data},
	Url = {http://www.epi-perspectives.com/content/3/1/2},
	Volume = {3},
	Year = {2006},
	Bdsk-Url-1 = {http://www.epi-perspectives.com/content/3/1/2}}

@article{Zelen&Parker86,
	Author = {M. Zelen and R.A. Parker},
	Journal = {Stat Med},
	Number = {3},
	Pages = {261--269},
	Title = {Case-Control Studies and Bayesian Inference},
	Volume = {5},
	Year = {1986}}

@article{Sinhetal04,
	Author = {S. SInha and B. Mukherjee and M Ghosh},
	Journal = {Biometrics},
	Pages = {41--49},
	Title = {Bayesian Semiparametric Modeling for Matched Case-Control Studies with Multiple Disease States},
	Volume = {60},
	Year = {2004}}

@article{Ritchieetal01,
	Author = {M.D. Ritchie and L.W. Hahn and N. Roodi and L.R. Bailey and W.D. Dupont and F.F. Parl and J.H. Moore},
	Journal = {Am J Hum Genet},
	Number = {1},
	Pages = {138--47},
	Title = {Multifactor-dimensionality reduction reveals high-order interactions among estrogen-metabolism genes in sporadic breast cancer.},
	Volume = {69},
	Year = {2001}}

@article{Mei&Cuccaro&Martin07,
	Author = {H. Mei and M.L. Cuccaro and E.R. Martin},
	Journal = {Am J Hum Genet},
	Number = {6},
	Pages = {1251-61},
	Title = {Multifactor dimensionality reduction-phenomics: a novel method to capture genetic heterogeneity with use of phenotypic variables.},
	Volume = {81},
	Year = {2007}}

@article{Bangsberg&Moss&Deeks04,
	Abstract = {Public health debates about providing HIV antiretroviral therapy to impoverished populations have centred on the relationship between adherence and risk of drug resistance. Recent data indicate that each antiretroviral therapeutic class has a unique adherence-resistance relationship. Resistance to single protease inhibitor therapy occurs most frequently at moderate to high levels of adherence, resistance to non-nucleoside reverse transcriptase inhibitor therapy occurs at low to moderate levels of adherence, and resistance to ritonavir-boosted protease inhibitor therapy is most likely to occur at middle ranges of adherence. These dynamic relationships should be considered in balancing the individual and public health benefits of therapy.},
	Author = {D.R. Bangsberg and A.R. Moss and S.G. Deeks},
	Journal = {J Antimicrob Chemother},
	Keywords = {Anti-HIV Agents/*therapeutic use Developing Countries *Drug Resistance, Viral Humans *Patient Compliance Public Health Research Support, Non-U.S. Gov't Research Support, U.S. Gov't, P.H.S.},
	Note = {0305-7453 (Print) Journal Article Review},
	Number = {5},
	Pages = {696-9},
	Title = {Paradoxes of adherence and drug resistance to {HIV} antiretroviral therapy},
	Volume = {53},
	Year = {2004}}

@article{Scharfstein&Tsiatis&Robins97,
	Author = {D.O. Scharfstein and A.A. Tsiatis and J.M. Robins},
	Journal = {Journal of the American Statistical Association},
	Number = {440},
	Pages = {1342--1350},
	Title = {Semiparametric efficiency and its implications on the design and analysis of group-sequential studies},
	Volume = {92},
	Year = {1997}}

@article{Bembometal07,
	Author = {O. Bembom and M. Petersen and SY Rhee and W.J. Fessel and S.E. Sinisi and R.W. Shafer 	 and M.J. van der Laan},
	Journal = {U.C. Berkeley Division of Biostatistics Working Paper Series},
	Optmonth = {August},
	Optnote = {http://www.bepress.com/ucbbiostat/paper221},
	Title = {Biomarker Discovery Using Targeted Maximum Likelihood Estimation: Application to the Treatment of Antiretroviral Resistant {HIV} Infection},
	Volume = {221},
	Year = {2007}}


@article{vanderLaan&Gruber12,
	Author = {M.J. van der Laan and S. Gruber},
	Journal = {The International Journal of Biostatistics},
	Title = {Targeted Minimum Loss Based Estimation of an Intervention Specific Mean},
	Volume = {in press},
	Year = {2012}}

@article{vanderLaan&Gruber12a,
	Author = {M.J. van der Laan and S. Gruber},
	Journal = {The International Journal of Biostatistics},
	Title = {Targeted Minimum Loss Based Estimation of Causal Effects of Multiple Time Point Interventions},
	Volume = {8},
	Year = {2012}}

@article{Gruber&vanderLaan12b,
	Author = {S. Gruber and M.J. van der Laan},
	Journal = {The International Journal of Biostatistics},
	Title = {Targeted Minimum Loss Based Estimation of a Causal Effect on an Outcome with Known Conditional Bounds},
	Volume = {8},
	Year = {2012}}

@techreport{Polley&vanderLaan10,
	Author = {E.C. Polley and M.J. van der Laan},
	Title = {Super Learner in Prediction},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper266},
	Year = {2010}}




@techreport{Stitelman&DeGruttola&vanderLaan11,
	Author = {O. M. Stitelman and  V. De Gruttola and M. J. van der Laan},
	Title = {A General Implementation of TMLE for Longitudinal Data Applied to Causal Inference in Survival Analysis},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper281},
	Month = {April},
	Year = {2011}
}




@techreport{tmleTR12,
	Author = {S. Gruber and M.J. van der Laan },
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper275},
	Title = {tmle: An {R} Package for Targeted Maximum Likelihood Estimation},
	Type = {Technical Report 275},
	Year = {revised: 2012}}

@techreport{vanderLaan&Gruber11TR,
	Author = {M.J. van der Laan and S. Gruber},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper290},
	Title = {Targeted Maximum Loss Based Estimation of an Intervention Specific Mean},
	Type = {Technical Report 290},
	Year = {2011}}

@article{vanderLaan&Gruber10,
	Author = {M.J. van der Laan and S. Gruber},
	Journal = {The International Journal of Biostatistics},
	Month = {January},
	Number = {1},
	Title = {Collaborative Double Robust Penalized Targeted Maximum Likelihood Estimation},
	Volume = {6},
	Year = {2010}}

@article{vanderLaan&Rubin06,
	Author = {M.J. van der Laan and D. Rubin},
	Journal = {The International Journal of Biostatistics},
	Number = {1},
	Optnote = {http://www.bepress.com/ijb/vol2/iss1/11},
	Title = {Targeted Maximum Likelihood Learning},
	Volume = {2},
	Year = {2006}}

@techreport{vanderLaan&Rubin06TR,
	Author = {M.J. van der Laan and D. Rubin},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper199},
	Title = {Targeted Maximum Likelihood Learning},
	Type = {Technical Report 213},
	Year = {2006}}

@article{Scharfstein&Tsiatis98,
	Author = {D.O. Scharfstein and A.A. Tsiatis},
	Journal = {Statistics in Medicine},
	Pages = {75--87},
	Title = {The use of simulation and bootstrap in information based group sequential studies},
	Volume = {17},
	Year = {1998}}

@article{Pampallona&Tsiatis&Kim01,
	Author = {S. Pampallona and A.A. Tsiatis and K. Kim},
	Journal = {Drug Informational Journal},
	Pages = {1113-1121},
	Title = {Interim monitoring of group sequential trials using spending functions for the type I and type II error probabilities},
	Volume = {35},
	Year = {2001}}

@article{Tsiatis&Mehta03,
	Author = {A.A. Tsiatis and C. Mehta},
	Journal = {Biometrika},
	Pages = {367-378},
	Title = {On the inefficiency of the adaptive design for monitoring clinical trials},
	Volume = {90},
	Year = {2003}}

@article{Banerjee&Tsiatis06,
	Author = {A. Banerjee and A.A. Tsiatis},
	Journal = {Statistics in Medicine},
	Optnote = {In press},
	Title = {Adaptive two-stage designs in phase II clinical trials},
	Year = {2006}}

@article{Tsiatis06,
	Author = {A.A. Tsiatis},
	Journal = {Statistics in Medicine},
	Optnote = {In press},
	Title = {Information based monitoring of clinical trials},
	Year = {2006}}

@article{Lokhnygina&Tsiatis06,
	Author = {Y. Lokhnygina and A.A. Tsiatis},
	Journal = {Journal of Statistical Planning and Inference},
	Optnote = {In press},
	Title = {Optimal two-stage group sequential designs},
	Year = {2006}}

@article{Bauer&Kohne94,
	Author = {P. Bauer and Kohne},
	Journal = {Biometrics},
	Pages = {1029--1041},
	Title = {Evaluation of experiments with adaptive interim analysis},
	Year = {1994}}

@article{Cui&Hung&Wang99,
	Author = {L. Cui and H.M.J. Hung and S-J Wang},
	Journal = {Biometrics},
	Pages = {853--857},
	Title = {Modification of sample size in group sequential trials},
	Year = {1999}}

@article{Jennison&Turnbull03,
	Author = {C. Jennison and B.W. Turnbull},
	Journal = {Statistics in Medicine},
	Pages = {971--993},
	Title = {Mid course sample size modification in clinical trials based on hte observed treatment effect},
	Year = {2003}}

@article{Koyama&Sampson&Gleser04,
	Author = {T. Koyama and A.R. Sampson and L.J. Gleser},
	Journal = {Journal of the Americal Statistical Association},
	Title = {A calculus for design of two stage adaptive procedures},
	Year = {2004}}

@article{Lan&Trost97,
	Author = {K.K.G Lan and D.C. Trost},
	Journal = {Proceedings Biopharm Section},
	Pages = {48-51},
	Title = {Estimation of parameters and sample size re-estimation},
	Year = {1997}}

@article{Lietal02,
	Author = {G. Li and W.J. Shih and T. Xie and J. Lu},
	Journal = {Biostatistics},
	Pages = {277--287},
	Title = {A sample size adjustment procedure for clinical trials based on conditional power},
	Year = {2002}}

@article{Mehta&Tsiatis01,
	Author = {C.R. Mehta and A.A. Tsiatis},
	Journal = {Drug Informational Journal},
	Pages = {1095--1112},
	Title = {Flexible sample size considerations using information based interim monitoring},
	Volume = {35},
	Year = {2001}}

@article{Mulle&Shafer01,
	Author = {H.H. Mulle and H. Shafer},
	Journal = {Biometrics},
	Pages = {886--891},
	Title = {Adaptive group sequential designs for clinical trials: combining the advantages of adaptive and classical group sequential approaches},
	Volume = {57},
	Year = {2001}}

@article{Proschan&Hunsberger95,
	Author = {M.A. Proschan and S.A. Hunsberger},
	Journal = {Biometrics},
	Pages = {1315--1324},
	Title = {Designed extension studies based on conditional power},
	Volume = {51},
	Year = {1995}}

@article{Shen&Fisher99,
	Author = {Y. Shen and L.D. Fisher},
	Journal = {Biometrics},
	Pages = {190--197},
	Title = {Statistical Inference for self-designing clinical trials with a one-sided hypothesis},
	Volume = {55},
	Year = {1999}}

@article{Wittes&Brittain90,
	Author = {J. Wittes and E. Brittain},
	Journal = {Statistics in Medicine},
	Pages = {65--72},
	Title = {The role of internal pilot studies in increasing efficiency of clinical trials},
	Volume = {9},
	Year = {1999}}

@article{Shen&Cheng06,
	Author = {Y. Shen and Y. Cheng},
	Journal = {Biostatistics},
	Optnote = {In Press},
	Title = {Adaptive design: Estimation and Inference with censored data in a semiparametric model},
	Year = {2006}}

@book{Spiegelalter&Abrams&Myles04,
	Author = {D.J. Spiegelalter and K.R. Abrams and J.P. Myles},
	Publisher = {Wiley, Chichester},
	Title = {Bayesian approaches to clinical trials and health care evaluation},
	Year = {2004}}

@book{Berry&Stangl96,
	Author = {D.A. Berry and D.K. Stangl},
	Publisher = {Marcel Dekker, New York},
	Title = {Bayesian biostatistics},
	Year = {1996}}

@article{Berry06,
	Author = {D.A. Berry},
	Journal = {Nature Reviews, Drug Discovery},
	Title = {Bayesian clinical trials},
	Volume = {5},
	Year = {2006}}

@book{Hu&Rosenberger06,
	Author = {F. Hu and W.F. Rosenberger},
	Publisher = {New York Wiley},
	Title = {The theory of response adaptive randomization in clinical trials},
	Year = {2006}}

@book{Dudoit&vanderLaan08,
	Author = {S. Dudoit and M.J. van der Laan},
	Publisher = {Springer Series of Statistics, New York},
	Title = {Resampling based multiple testing with applications to genomics},
	Year = {2008}}

@book{Sen&Singer93,
	Author = {P.K. Sen and J.M. Singer},
	Publisher = {Chapman \& Hall, New York},
	Title = {Large Sample Methods in Statistics: An Introduction with Applications},
	Year = {1993}}

@article{Bai&Hu&Rosenberger02,
	Author = {Z.D. Bai and F. Hu and W.F. Rosenberger},
	Journal = {The Annals of Statistics},
	Number = {1},
	Pages = {122--139},
	Title = {Asymptotic properties of adaptive designs for clinical trials with delayed response},
	Volume = {30},
	Year = {2002}}

@article{Andersen&Faries&Tamura94,
	Author = {J. Andersen and D. Faries and R. Tamura},
	Journal = {Communication in Statistical Theory},
	Pages = {309--323},
	Title = {A randomized play-the-winner design for multiarm clinical trials},
	Volume = {23},
	Year = {1994}}

@book{Flournoy&Rosenberger95,
	Author = {N. Flournoy and W.F. Rosenberger},
	Publisher = {Hayward, Institute of Mathematical Statistics},
	Title = {Adaptive Designs},
	Year = {1995}}

@article{Hu&Rosenberger00,
	Author = {F. Hu and W.F. Rosenberger},
	Journal = {Statistics in Medicine},
	Pages = {2067--2075},
	Title = {Analysis of time trends in adaptive designs withi appliation to a neurophysiology experiment},
	Volume = {19},
	Year = {2000}}

@article{Rosenberger96,
	Author = {W.F. Rosenberger},
	Journal = {Statistical Science},
	Pages = {137--149},
	Title = {New directions in adaptive designs},
	Volume = {11},
	Year = {1996}}

@article{Rosenberger&Flournoy&Durham97,
	Author = {W.F. Rosenberger and N. Flournoy and S.D. Durham},
	Journal = {Journal of Statistical Planning and Inference},
	Pages = {69--76},
	Title = {Asymptotic normality of maximum likelihood estimators from multiparameter response driven designs},
	Year = {1997}}

@article{Rosenberger&Grill97,
	Author = {W.F. Rosenberger and S.E. Grill},
	Journal = {Statistics in Medicine},
	Pages = {2245--2260},
	Title = {A sequential design for psychophysical experiments: An application to estimating timing of sensory events},
	Volume = {16},
	Year = {1997}}

@article{Rosenberger&Sriram97,
	Author = {W.F. Rosenberger and T.N. Shiram},
	Journal = {Journal of Statistical Planning and Inference},
	Pages = {309--319},
	Title = {Estimation for an adaptive allocation design},
	Volume = {59},
	Year = {1997}}

@article{Tamuraetal94,
	Author = {R.N. Tamura and D.E. Faries and J.S. Andersen and J.H. Heiligenstein},
	Journal = {Journal of the American Statistical Association},
	Pages = {768--776},
	Title = {A case study of an adaptive clinical trial in the treatment of out-patients with depressive disorder},
	Volume = {89},
	Year = {1994}}

@article{Wei&Durham78,
	Author = {L.J. Wei and S. Durham},
	Journal = {Journal of the American Statistical Association},
	Pages = {840--843},
	Title = {The randomize play-the-winner rule in medical trials},
	Volume = {73},
	Year = {1978}}

@article{Weietal90,
	Author = {L.J. Wei and R.T. Smythe and D.Y. Lin and T.S. Park},
	Journal = {Journal of the American Statistical Association},
	Pages = {156--162},
	Title = {Statistical Inference with data-dependent treatment allocation rules},
	Volume = {85},
	Year = {1990}}

@article{Zelen69,
	Author = {M. Zelen},
	Journal = {Journal of the American Statistical Association},
	Pages = {131--146},
	Title = {Play the winner rule and the controlled clinical trial},
	Volume = {64},
	Year = {1969}}

@article{Cheng&Shen05,
	Author = {Y. Cheng and Y. Shen},
	Journal = {Biometrika},
	Number = {3},
	Pages = {633--646},
	Title = {Bayesian adaptive designs for clinical trials},
	Volume = {92},
	Year = {2005}}

@article{Wei79,
	Author = {L.J. Wei},
	Journal = {The Annals of Statistics},
	Pages = {291--296},
	Title = {The generalized Polya's urn design for sequential medical trials},
	Volume = {7},
	Year = {1979}}

@article{Benito&Lopez&Soriano03,
	Author = {Benito, J. M. and Lopez, M. and Soriano, V.},
	Journal = {J Infect Dis},
	Keywords = {ADP-ribosyl Cyclase/metabolism Anti-HIV Agents/therapeutic use Antigens, CD/metabolism CD4-Positive T-Lymphocytes/*immunology CD8-Positive T-Lymphocytes/immunology HIV Infections/drug therapy/*immunology/virology HIV-1/*physiology Human *Viral Load Virus Replication},
	Note = {0022-1899 Comment Letter},
	Number = {5},
	Pages = {794-5; author reply 795-6},
	Title = {Virus load and cytolitic responses in human immunodeficiency virus infection: what is cause and what is effect},
	Volume = {188},
	Year = {2003}}

@article{DEttorreetal02,
	Abstract = {OBJECTIVE: To study virologic and immunologic factors associated with discordant treatment response in HIV-infected patients receiving highly active antiretroviral therapy (HAART). DESIGN: Study participants included a total of 27 patients: (a) 10 discordant patients (mean CD4+ cell count, 396.1 x 10 cells/l; mean HIV-RNA, 5.4 log copies/ml); (b) seven responder patients (mean CD4+ cell count, 997.5 x 10 cells/l); and (c) 10 failing patients (mean CD4+ cell count 66.5 x 10 cells/l; mean HIV-RNA, 5.4 log copies/ml).(10) (10)METHODS: The HIV-1 isolation rate and biological phenotype, drug resistance genotypic mutations of HIV-1 strains, recall and HIV-1-specific antigen lymphocyte proliferation (LP), and interleukin (IL)-15 production were studied. RESULTS: Virus isolation was obtained in 30% of discordant patients, and in 100% of failing patients. A higher replication constant was reported in discordant patients. No difference in the number of drug resistance mutations and biological phenotypes of HIV-1 was found in discordant patients with respect to failing patients. Discordant patients developed positive LP responses to and HIV-1 p24. LP in response to, HIV-1 p24 and gp160 was positive in responder patients. No significant LP was found in failing patients. Increased levels of IL-15 after stimulation with lipopolysaccaride (LPS) and were found in both discordant patients and responder patients. Conversely, a strong reduction of IL-15 levels was observed in failing patients. CONCLUSION: The present results suggest that decreased virus isolation rate, restoration of both lymphocyte proliferation and IL-15 production are factors involved in the discordant antiretroviral therapy response of HIV-infected patients.},
	Author = {D'Ettorre, G. and Forcina, G. and Andreotti, M. and Sarmati, L. and Palmisano, L. and Galluzzo, C. M. and Nicastri, E. and Mastroianni, C. M. and Vullo, V. and Vella, S. and Andreoni, M.},
	Journal = {Aids},
	Keywords = {Adult Anti-HIV Agents/*therapeutic use Antiretroviral Therapy, Highly Active CD4 Lymphocyte Count CD8-Positive T-Lymphocytes/drug effects/immunology Candida albicans Drug Resistance, Viral Female HIV Infections/complications/*drug therapy/immunology/virology HIV-1/drug effects/genetics/*immunology/isolation & purification Human Interleukin-15/*blood Male Middle Aged Mutation Viral Load Virus Replication/drug effects},
	Note = {0269-9370 Journal Article},
	Number = {14},
	Pages = {1877-85},
	Title = {Discordant response to antiretroviral therapy: {HIV} isolation, genotypic mutations, T-cell proliferation and cytokine production},
	Volume = {16},
	Year = {2002}}

@article{Davenportetal02,
	Abstract = {Early infection with HIV-1 is dominated by CCR5-tropic (R5, non-syncytium-inducing) viruses. The evolution of CXCR4-tropic (X4, syncytium-inducing) viruses occurs later in the infection and is associated with rapid disease progression. Here, we propose that the tropism of X4 viruses for naive CD4+ T cells is disadvantageous in early infection owing to the low division rate of these cells. In healthy individuals, the division rate of memory cells is nearly ten times higher than that of naive cells and thus the memory-cell tropism of R5 viruses could account for their dominance early in infection. As the division rate of naive T cells increases with CD4+ depletion, X4 viruses come to dominate in late disease.},
	Author = {Davenport, M. P. and Zaunders, J. J. and Hazenberg, M. D. and Schuitemaker, H. and van Rij, R. P.},
	Journal = {Trends Microbiol},
	Keywords = {CD4-Positive T-Lymphocytes/*virology HIV Infections/*immunology/metabolism HIV-1/*pathogenicity Human Immunologic Memory Macrophages/*virology Models, Biological Receptors, CCR5/metabolism Receptors, CXCR4/metabolism Tropism},
	Note = {0966-842x Journal Article},
	Number = {6},
	Pages = {275-8},
	Title = {Cell turnover and cell tropism in HIV-1 infection},
	Volume = {10},
	Year = {2002}}

@article{Deeksetal00,
	Abstract = {The relationship between plasma human immunodeficiency virus (HIV) RNA levels and peripheral CD4+ T cell counts was examined in 380 HIV-infected adults receiving long-term protease inhibitor therapy. Patients experiencing virologic failure (persistent HIV RNA >500 copies RNA/mL) generally had CD4+ T cell counts that remained greater than pretherapy baseline levels, at least through 96 weeks of follow-up. The CD4+ T cell response was directly and independently related to degree of viral suppression below the pretreatment baseline. For any given HIV RNA level measured 12 weeks after virologic failure, subsequent CD4+ T cell decline was slower in patients receiving a protease inhibitor-based regimen than in a historical control group of untreated patients. These observations suggest that transient or partial declines in plasma HIV RNA levels can have sustained effects on CD4+ T cell levels.},
	Author = {Deeks, S. G. and Barbour, J. D. and Martin, J. N. and Swanson, M. S. and Grant, R. M.},
	Journal = {J Infect Dis},
	Keywords = {Adult *CD4 Lymphocyte Count Female HIV Infections/*drug therapy/immunology/virology HIV Protease Inhibitors/*therapeutic use Human Male RNA, Viral/*blood Support, Non-U.S. Gov't Support, U.S. Gov't, P.H.S.},
	Note = {0022-1899 Journal Article},
	Number = {3},
	Pages = {946-53},
	Title = {Sustained CD4+ T cell response after virologic failure of protease inhibitor-based regimens in patients with human immunodeficiency virus infection},
	Volume = {181},
	Year = {2000}}

@article{Deeksetal01,
	Abstract = {BACKGROUND: In many patients with human immunodeficiency virus (HIV) infection, therapy with potent antiretroviral drugs does not result in complete suppression of HIV replication. The effect of cessation of therapy in these patients is unknown. METHODS: Sixteen patients who had a plasma HIV RNA level of more than 2500 copies per milliliter during combination antiretroviral-drug therapy were randomly assigned, in a 2:1 ratio, to discontinue or continue therapy. Plasma HIV RNA levels, CD4 cell counts, and drug susceptibility were measured weekly. Viral replicative capacity was measured at base line and at week 12. RESULTS: Discontinuation of therapy for 12 weeks was associated with a median decrease in the CD4 cell count of 128 cells per cubic millimeter and an increase in the plasma HIV RNA level of 0.84 log copies per milliliter. Virus from all patients with detectable resistance at entry became susceptible to HIV-protease inhibitors within 16 weeks after the discontinuation of therapy. Drug susceptibility began to increase a median of six weeks after the discontinuation of therapy and was temporally associated with increases in plasma HIV RNA levels and decreases in CD4 cell counts. Viral replicative capacity, measured by means of a recombinant-virus assay, was low at entry into the study and increased after therapy was discontinued. Despite the loss of detectable resistance in plasma, resistant virus was cultured from peripheral-blood mononuclear cells in five of nine patients who could be evaluated. Plasma HIV RNA levels, CD4 cell counts, and drug susceptibility remained stable in the patients who continued therapy. CONCLUSIONS: Despite the presence of reduced drug susceptibility, antiretroviral-drug therapy can provide immunologic and virologic benefit. This benefit reflects continued antiviral-drug activity and the maintenance of a viral population with a reduced replicative capacity.},
	Author = {Deeks, S. G. and Wrin, T. and Liegler, T. and Hoh, R. and Hayden, M. and Barbour, J. D. and Hellmann, N. S. and Petropoulos, C. J. and McCune, J. M. and Hellerstein, M. K. and Grant, R. M.},
	Journal = {N Engl J Med},
	Keywords = {Adult Anti-HIV Agents/pharmacology/*therapeutic use CD4 Lymphocyte Count Drug Resistance, Microbial Drug Therapy, Combination HIV Infections/*drug therapy/immunology/virology HIV Protease Inhibitors/pharmacology/*therapeutic use HIV-1/*drug effects/genetics/isolation & purification Human Male Middle Aged Proportional Hazards Models Prospective Studies RNA, Viral/blood Support, Non-U.S. Gov't Support, U.S. Gov't, P.H.S. Viremia/drug therapy},
	Note = {0028-4793 Clinical Trial Journal Article Randomized Controlled Trial},
	Number = {7},
	Pages = {472-80},
	Title = {Virologic and immunologic consequences of discontinuing combination antiretroviral-drug therapy in HIV-infected patients with detectable viremia},
	Volume = {344},
	Year = {2001}}

@article{Deeks01,
	Abstract = {Although understanding of nonnucleoside reverse transcriptase inhibitor (NNRTI) resistance is less clearly established than that of other classes of antiretroviral drugs, certain facts have been established. The treatment-associated genetic mutation profiles of the available NNRTIs have been mapped, and resistance has been found to develop rapidly after initiation of NNRTI therapy. Despite the chemical diversity of the NNRTIs, cross-resistance among agents of this class is nearly universal. Although the viral replicative capacity (``fitness") of NNRTI-induced viral variants has not been extensively studied, available data suggest that NNRTI-selected mutations confer little damage to viral fitness, and thus a single point mutation produces a strain that is both resistant and fit. Furthermore, with continued therapy, viral evolution persists, creating species with greater numbers of mutations and higher level phenotypic resistance. Taken together, these facts suggest that continued use of NNRTIs after emergence of resistance will produce variants of complex mutational patterns that limit future treatment options, and, therefore, strong consideration should be given to discontinuing NNRTIs after virologic failure is confirmed. This article describes the scientific literature establishing the efficacy and limitations of NNRTI therapy and attempts to define a role for this class of drug in the long-term treatment of HIV-1 disease.},
	Author = {Deeks, S. G.},
	Journal = {J Acquir Immune Defic Syndr},
	Keywords = {Anti-HIV Agents/*pharmacology/therapeutic use Clinical Trials Delavirdine/pharmacology/therapeutic use *Drug Resistance, Microbial Drug Therapy, Combination HIV Infections/drug therapy/transmission HIV-1/*drug effects/genetics/metabolism HIV-1 Reverse Transcriptase/chemistry/genetics Human Nevirapine/pharmacology/therapeutic use Oxazines/pharmacology/therapeutic use Phylogeny Point Mutation/drug effects Protein Conformation Reverse Transcriptase Inhibitors/*pharmacology/therapeutic use Virus Replication/drug effects},
	Note = {1525-4135 Journal Article Review Review, Tutorial},
	Pages = {S25-33},
	Title = {International perspectives on antiretroviral resistance. Nonnucleoside reverse transcriptase inhibitor resistance},
	Volume = {26 Suppl 1},
	Year = {2001}}

@article{Deeksetal02,
	Abstract = {BACKGROUND: Sustained elevations in CD4 cell counts commonly occur despite incomplete viral suppression with protease inhibitor-based antiretroviral therapy. OBJECTIVES: To determine the incidence and risk factors associated with return of CD4 cell count to pre-therapy levels in patients experiencing virologic failure of protease inhibitor therapy. DESIGN: This is a clinic-based cohort study of HIV-infected adults who failed to maintain durable viral suppression on a protease inhibitor-based regimen. MAIN OUTCOME MEASURES: Virologic failure was defined as persistent plasma HIV RNA level > 500 copies/ml. Immunologic failure was defined as return of CD4 cell count to pre-therapy levels. RESULTS: A total of 291 patients experienced virologic failure on a protease inhibitor-based regimen and had a treatment-mediated CD4 cell increase above pre-therapy levels at the time of virologic failure. If patient data were censored at the time a successful salvage regimen was initiated, then the median time to immunologic failure after the onset of virologic failure was 3 years. If patient data were also censored at the time therapy was discontinued, then 36.8% of the cohort experienced immunologic failure after 3 years of continuous virologic failure. The change in viral load from a pre-treatment baseline, and not the absolute level of viremia achieved, was a strong and independent predictor of immunologic failure. Discontinuing therapy was associated with immunologic failure independent of viral load changes. CONCLUSION: Reduction in T CD4+ cell numbers may eventually occur during prolonged virologic failure of a protease inhibitor-based regimen and is predicted by the degree of virologic suppression below a pre-therapy 'set-point'.},
	Author = {Deeks, S. G. and Barbour, J. D. and Grant, R. M. and Martin, J. N.},
	Journal = {Aids},
	Keywords = {Adult Antiretroviral Therapy, Highly Active CD4 Lymphocyte Count CD4-Positive T-Lymphocytes/cytology/*drug effects Disease Progression HIV Infections/blood/*drug therapy/immunology/virology HIV Protease Inhibitors/*therapeutic use HIV-1/*drug effects/genetics Human Indinavir/therapeutic use Nelfinavir/therapeutic use RNA, Viral/blood Ritonavir/therapeutic use Saquinavir/therapeutic use Support, Non-U.S. Gov't Support, U.S. Gov't, P.H.S. Time Factors Treatment Failure Viremia/blood/*drug therapy/immunology/virology},
	Note = {0269-9370 Journal Article},
	Number = {2},
	Pages = {201-7},
	Title = {Duration and predictors of CD4 T-cell gains in patients who continue combination therapy despite detectable plasma viremia},
	Volume = {16},
	Year = {2002}}

@article{Deeks03,
	Abstract = {Drug-resistant HIV-1 is a cause of growing clinical and public-health concern. In many patients, combination antiretroviral therapy fails to achieve complete viral suppression (virological failure). Continuing viral replication during therapy leads to the accumulation of drug-resistance mutations, resulting in increased viral load and a greater risk of disease progression. Patients with drug-resistant HIV-1 infection have three therapeutic options: a change to a salvage regimen with the aim of fully suppressing viral replication; interruption of therapy; or continuation of a partially effective regimen. The first strategy is preferred for most patients failing their first or perhaps their second regimen. However, the best approach remains unclear for patients who have failed multiple treatment regimens and who have limited options for complete viral suppression. The management of such patients requires a careful understanding of the pathogenesis of drug-resistant HIV-1, the clinical consequences of virological failure, the potential benefits and limitations of diagnostic assays, and the likelihood that agents in development will be effective.},
	Author = {Deeks, S. G.},
	Journal = {Lancet},
	Keywords = {Anti-HIV Agents/*immunology/*therapeutic use Antiretroviral Therapy, Highly Active/methods Drug Resistance, Viral/genetics/immunology Drug Therapy, Combination HIV Infections/*drug therapy/immunology/virology HIV Protease Inhibitors/immunology/therapeutic use *HIV-1/drug effects/genetics/immunology Human Randomized Controlled Trials Ritonavir/immunology/therapeutic use Support, Non-U.S. Gov't Support, U.S. Gov't, P.H.S. Treatment Outcome Viral Load/statistics & numerical data Virus Replication/drug effects/immunology},
	Note = {1474-547x Journal Article Review Review, Academic},
	Number = {9400},
	Pages = {2002-11},
	Title = {Treatment of antiretroviral-drug-resistant HIV-1 infection},
	Volume = {362},
	Year = {2003}}

@article{Deeks&Walker04,
	Abstract = {A potent antigen-specific T cell response to HIV infection can contribute to the control of viral replication and is therefore beneficial to the host. However, HIV-mediated increases in generalized T cell activation also appear to accelerate both viral replication and CD4+ T cell depletion. A new study in the JCI attempts to experimentally distinguish the beneficial versus harmful aspects of this immune response.},
	Author = {Deeks, S. G. and Walker, B. D.},
	Journal = {J Clin Invest},
	Note = {0021-9738 Comment Journal Article},
	Number = {6},
	Pages = {808-10},
	Title = {The immune response to AIDS virus infection: good, bad, or both?},
	Volume = {113},
	Year = {2004}}

@techreport{DHHS04,
	Author = {DHHS},
	Institution = {Panel on Clinical Practices for Treatment of HIV Infection, Department of Health and Human Services},
	Month = {March 23},
	Title = {Guidelines for the use of antiretroviral agents in HIV-1 infected adults and adolescents},
	Year = {2004}}

@article{Faureetal00,
	Abstract = {Human immunodeficiency virus (HIV) enters cells in vitro via CD4 and a coreceptor. Which of 15 known coreceptors are important in vivo is poorly defined but may be inferred from disease-modifying mutations, as for CCR5. Here two single nucleotide polymorphisms are described in Caucasians in CX3CR1, an HIV coreceptor and leukocyte chemotactic/adhesion receptor for the chemokine fractalkine. HIV-infected patients homozygous for CX3CR1-I249 M280, a variant haplotype affecting two amino acids (isoleucine-249 and methionine-280), progressed to AIDS more rapidly than those with other haplotypes. Functional CX3CR1 analysis showed that fractalkine binding is reduced among patients homozygous for this particular haplotype. Thus, CX3CR1-I249 M280 is a recessive genetic risk factor in HIV/AIDS.},
	Author = {Faure, S. and Meyer, L. and Costagliola, D. and Vaneensberghe, C. and Genin, E. and Autran, B. and Delfraissy, J. F. and McDermott, D. H. and Murphy, P. M. and Debre, P. and Theodorou, I. and Combadiere, C.},
	Journal = {Science},
	Keywords = {Acquired Immunodeficiency Syndrome/genetics/*physiopathology/virology Case-Control Studies *Chemokines, CX3C Chemokines, CXC/metabolism Chromosomes, Human, Pair 3 Cohort Studies Disease Progression European Continental Ancestry Group/genetics Genotype HIV/physiology HIV Infections/genetics/*physiopathology/virology Haplotypes Homozygote Human Leukocytes, Mononuclear/metabolism Linkage Disequilibrium Membrane Proteins/metabolism Mutation Polymorphism, Restriction Fragment Length *Polymorphism, Single Nucleotide Polymorphism, Single-Stranded Conformational Receptors, Cytokine/*genetics/*physiology Receptors, HIV/*genetics/*physiology Support, Non-U.S. Gov't Survival Analysis Variation (Genetics)},
	Note = {0036-8075 Comment Journal Article},
	Number = {5461},
	Pages = {2274-7},
	Title = {Rapid progression to AIDS in HIV+ individuals with a structural variant of the chemokine receptor CX3CR1},
	Volume = {287},
	Year = {2000}}

@article{Gaoetal01,
	Abstract = {BACKGROUND: From studies of genetic polymorphisms and the rate of progression from human immunodeficiency virus type 1 (HIV-1) infection to the acquired immunodeficiency syndrome (AIDS), it appears that the strongest susceptibility is conferred by the major-histocompatibility-complex (MHC) class I type HLA-B*35,Cw*04 allele. However, cytotoxic T-lymphocyte responses have been observed against HIV-1 epitopes presented by HLA-B*3501, the most common HLA-B*35 subtype. We examined subtypes of HLA-B*35 in five cohorts and analyzed the relation of structural differences between HLA-B*35 subtypes to the risk of progression to AIDS. METHODS: Genotyping of HLA class I loci was performed for 850 patients who seroconverted and had known dates of HIV-1 infection. Survival analyses with respect to the rate of progression to AIDS were performed to identify the effects of closely related HLA-B*35 subtypes with different peptide-binding specificities. RESULTS: HLA-B*35 subtypes were divided into two groups according to peptide-binding specificity: the HLA-B*35-PY group, which consists primarily of HLA-B*3501 and binds epitopes with proline in position 2 and tyrosine in position 9; and the more broadly reactive HLA-B*35-Px group, which also binds epitopes with proline in position 2 but can bind several different amino acids (not including tyrosine) in position 9. The influence of HLA-B*35 in accelerating progression to AIDS was completely attributable to HLA-B*35-Px alleles, some of which differ from HLA-B*35-PY alleles by only one amino acid residue. CONCLUSIONS: This analysis shows that, in patients with HIV-1 infection, a single amino acid change in HLA molecules has a substantial effect on the rate of progression to AIDS. The different consequences of HLA-B*35-PY and HLA-B*35-Px in terms of disease progression highlight the importance of the epitope specificities of closely related class I molecules in the immune defense against HIV-1.},
	Author = {Gao, X. and Nelson, G. W. and Karacki, P. and Martin, M. P. and Phair, J. and Kaslow, R. and Goedert, J. J. and Buchbinder, S. and Hoots, K. and Vlahov, D. and O'Brien, S. J. and Carrington, M.},
	Journal = {N Engl J Med},
	Keywords = {Acquired Immunodeficiency Syndrome/*genetics African Continental Ancestry Group/genetics Alleles Amino Acid Sequence Binding Sites/genetics Disease Progression Disease-Free Survival European Continental Ancestry Group/genetics *Genes, MHC Class I Genotype HIV Infections/ethnology/*genetics/immunology HLA-B35 Antigen/chemistry/*genetics HLA-C Antigens Human Peptides/metabolism Proportional Hazards Models Receptors, Peptide/chemistry/genetics/metabolism Support, U.S. Gov't, P.H.S.},
	Note = {0028-4793 Journal Article Multicenter Study},
	Number = {22},
	Pages = {1668-75},
	Title = {Effect of a single amino acid change in MHC class I molecules on the rate of progression to AIDS},
	Volume = {344},
	Year = {2001}}

@article{Grabaretal00,
	Abstract = {BACKGROUND: The prognostic value of discordant immunologic (CD4 cell increase) and virologic (plasma HIV RNA level decrease) responses to antiretroviral treatment is not known. OBJECTIVE: To study the relation between clinical outcome of HIV-infected patients receiving highly active antiretroviral therapy (HAART) and early immunologic and virologic responses to such therapy. DESIGN: Prospective cohort study. SETTING: 68 hospitals in France. PATIENTS: 2236 protease inhibitor-naive patients. INTERVENTION: Initiation of HAART with one protease inhibitor and two nucleoside analogues between July 1996 and March 1997. MEASUREMENTS: Immunologic and virologic response at 6 months. Multivariate Cox models were used to assess the relation between these responses and progression to a new AIDS-defining event or death. RESULTS: On the basis of 6-month immunologic and virologic responses, patients were classified into four groups: complete response (47.5%), complete nonresponse (16.2%), immunologic response only (19.0%), and virologic response only (17.3%). After month 6 and within a median of 18 months, 69 patients died and 123 experienced a new AIDS-defining event. After adjustment, complete nonresponders and those with only a virologic response had significantly higher risks for clinical progression at 6 months (relative risk, 3.38 [95% CI, 2.28 to 5.02] and 1.98 [CI, 1.26 to 3.10], respectively) than complete responders. The difference between complete responders and those with only an immunologic response at 6 months was weaker and nonsignificant (relative risk, 1.55 [CI, 0.96 to 2.50]). CONCLUSIONS: Immunologic response after 6 months of HAART indicates a favorable clinical outcome in HIV-infected patients regardless of virologic response. This suggests that both immunologic and virologic markers should be used in clinical practice to evaluate treatment response.},
	Author = {Grabar, S. and Le Moing, V. and Goujard, C. and Leport, C. and Kazatchkine, M. D. and Costagliola, D. and Weiss, L.},
	Journal = {Ann Intern Med},
	Keywords = {Adult CD4 Lymphocyte Count Disease Progression Drug Therapy, Combination Female HIV Infections/*drug therapy/immunology/virology HIV Protease Inhibitors/*therapeutic use *HIV-1/genetics Human Male Multivariate Analysis Proportional Hazards Models Prospective Studies RNA, Viral/blood Reverse Transcriptase Inhibitors/*therapeutic use Support, Non-U.S. Gov't Treatment Outcome Viral Load},
	Note = {0003-4819 Journal Article Multicenter Study},
	Number = {6},
	Pages = {401-10},
	Title = {Clinical outcome of patients with HIV-1 infection according to immunologic and virologic response after 6 months of highly active antiretroviral therapy},
	Volume = {133},
	Year = {2000}}

@article{Gruebetal00,
	Abstract = {BACKGROUND: Hepatitis C virus (HCV) infection is highly prevalent among HIV-1-infected individuals, but its contribution to the morbidity and mortality of coinfected patients who receive potent antiretroviral therapy is controversial. We used data from the ongoing Swiss HIV Cohort Study to analyse clinical progression of HIV-1, and the virological and immunological response to potent antiretroviral therapy in HIV-1-infected patients with or without concurrent HCV infection. METHODS: We analysed prospective data on survival, clinical disease progression, suppression of HIV-1 replication, CD4-cell recovery, and frequency of changes in antiretroviral therapy according to HCV status in 3111 patients starting potent antiretroviral therapy. RESULTS: 1157 patients (37.2%) were coinfected with HCV, 1015 of whom (87.7%) had a history of intravenous drug use. In multivariate Cox's regression, the probability of progression to a new AIDS-defining clinical event or to death was independently associated with HCV seropositivity (hazard ratio 1.7 [95% CI 1.26-2.30]), and with active intravenous drug use (1.38 [1.02-1.88]). Virological response to antiretroviral therapy and the probability of treatment change were not associated with HCV serostatus. In contrast, HCV seropositivity was associated with a smaller CD4-cell recovery (hazard ratio for a CD4-cell count increase of at least 50 cells/microL=0.79 [0.72-0.87]). INTERPRETATION: HCV and active intravenous drug use could be important factors in the morbidity and mortality among HIV-1-infected patients, possibly through impaired CD4-cell recovery in HCV seropositive patients receiving potent antiretroviral therapy. These findings are relevant for decisions about optimum timing for HCV treatment in the setting of HIV infection.},
	Author = {Greub, G. and Ledergerber, B. and Battegay, M. and Grob, P. and Perrin, L. and Furrer, H. and Burgisser, P. and Erb, P. and Boggian, K. and Piffaretti, J. C. and Hirschel, B. and Janin, P. and Francioli, P. and Flepp, M. and Telenti, A.},
	Journal = {Lancet},
	Keywords = {AIDS-Related Opportunistic Infections/*drug therapy Adolescent Adult Anti-HIV Agents/*therapeutic use CD4 Lymphocyte Count Cohort Studies Disease Progression Female Hepatitis C/complications/*drug therapy Human Male Middle Aged Prospective Studies Support, Non-U.S. Gov't Survival Analysis Switzerland Viral Load Viremia/etiology},
	Note = {0140-6736 Clinical Trial Journal Article},
	Number = {9244},
	Pages = {1800-5},
	Title = {Clinical progression, survival, and immune recovery during antiretroviral therapy in patients with HIV-1 and hepatitis C virus coinfection: the Swiss HIV Cohort Study},
	Volume = {356},
	Year = {2000}}

@article{Katzensteinetal96,
	Abstract = {BACKGROUND: We studied measures of human immunodeficiency virus (HIV) replication, the viral phenotype, and immune function (CD4 cell counts) and the relation of changes in these indicators to clinical outcomes in a subgroup of patients in a controlled trial of early antiretroviral treatment for HIV, the AIDS Clinical Trials Group Study 175. METHODS: The 391 subjects, each of whom entered the study with a single screening CD4 cell count of 200 to 500 per cubic millimeter, were randomly assigned to receive zidovudine alone, didanosine alone, zidovudine plus didanosine, or zidovudine plus zalcitabine. Plasma concentrations of HIV RNA were assessed in 366 subjects, and viral isolates from 332 subjects were assayed for the presence of the syncytium-inducing phenotype. RESULTS: After eight weeks, the mean (+/-SE) decrease from base line in the concentration of HIV RNA, expressed as the change in the base 10 log of the number of copies per milliliter, was 0.26+/-0.06 for patients treated with zidovudine alone, 0.65+/-0.07 for didanosine alone, 0.93+/-0.10 for zidovudine plus didanosine, and 0.89+/-0.06 for zidovudine plus zalcitabine (P<0.001 for each of the pairwise comparisons with zidovudine alone). Multivariate proportional-hazards models showed that higher base-line concentrations of plasma HIV RNA, less suppression of plasma HIV RNA by treatment, and the presence of the syncytium-inducing phenotype were significantly associated with an increased risk of progression to the acquired immunodeficiency syndrome and death. After adjustment for these measures of viral replication and for the viral phenotype, CD4 cell counts were not significant predictors of clinical outcome. CONCLUSIONS: Both the risk of the progression of HIV disease and the efficacy of antiretroviral therapy are strongly associated with the plasma level of HIV RNA and with the viral phenotype. The changes in the plasma concentration of HIV RNA predict the changes in CD4 cell counts and survival after treatment with reverse-transcriptase inhibitors.},
	Author = {Katzenstein, D. A. and Hammer, S. M. and Hughes, M. D. and Gundacker, H. and Jackson, J. B. and Fiscus, S. and Rasheed, S. and Elbeik, T. and Reichman, R. and Japour, A. and Merigan, T. C. and Hirsch, M. S.},
	Journal = {N Engl J Med},
	Keywords = {Adult Antiviral Agents/*therapeutic use CD4 Lymphocyte Count Didanosine/*therapeutic use Disease Progression Drug Therapy, Combination Female HIV/*genetics/isolation & purification/physiology HIV Infections/drug therapy/immunology/*virology Human Male Middle Aged Multivariate Analysis Phenotype Proportional Hazards Models RNA, Viral/*blood Support, U.S. Gov't, P.H.S. Treatment Outcome Virus Replication/drug effects Zidovudine/*therapeutic use},
	Note = {0028-4793 Clinical Trial Journal Article Multicenter Study Randomized Controlled Trial},
	Number = {15},
	Pages = {1091-8},
	Title = {The relation of virologic and immunologic markers to clinical outcomes after nucleoside therapy in HIV-infected adults with 200 to 500 CD4 cells per cubic millimeter. AIDS Clinical Trials Group Study 175 Virology Study Team},
	Volume = {335},
	Year = {1996}}

@article{Kaufmannetal98,
	Author = {Kaufmann, D. and Pantaleo, G. and Sudre, P. and Telenti, A.},
	Journal = {Lancet},
	Keywords = {Anti-HIV Agents/*therapeutic use CD4 Lymphocyte Count HIV Infections/drug therapy/*immunology Human Protease Inhibitors/*therapeutic use Support, Non-U.S. Gov't Viremia/drug therapy/*immunology},
	Note = {0140-6736 Letter},
	Number = {9104},
	Pages = {723-4},
	Title = {CD4-cell count in HIV-1-infected individuals remaining viraemic with highly active antiretroviral therapy (HAART). Swiss HIV Cohort Study},
	Volume = {351},
	Year = {1998}}

@article{Kaufmannetal03,
	Abstract = {BACKGROUND: Highly active antiretroviral therapy (HAART) for human immunodeficiency virus (HIV)-1 infection allows recovery of CD4 T lymphocytes. Few studies have explored the long-term T-lymphocyte responses to HAART. METHODS: Plasma HIV-1 RNA levels and CD4 and CD8 T-lymphocyte counts were longitudinally analyzed over 4 years in 2235 participants of the Swiss HIV Cohort, commencing HAART between 1996 and 1997. The CD4 T-lymphocyte count increase, the percentage of individuals with a CD4 T-lymphocyte count of 500/microL or greater and less than 200/microL, and the determinants of CD4 T-lymphocyte recovery were evaluated in individuals treated with continuous (CONT; n = 985) and discontinuous (DISCONT; n = 1250) HAART. RESULTS: At 4 years, 69.5% of subjects (CONT, 84.5%; DISCONT, 53.6%; P<.001) showed HIV-1 RNA levels below 400 copies/mL, while the median CD4 T-lymphocyte count increased from 190/microL to 423/microL (CONT, 486/microL; DISCONT, 343/microL; P<.001). Of the 2235 participants, 38.8% (CONT, 47.7%; DISCONT, 29.4%; P<.001) reached a CD4 T-lymphocyte count of 500/microL or greater, but in 15.6%, CD4 T-lymphocyte count remained below 200/microL (CONT, 5.9%; DISCONT, 25.9%; P<.001). Larger increases in CD4 T-lymphocyte count were associated with higher baseline HIV-1 RNA, a larger percentage of undetectable HIV-1 RNA levels, lower baseline CD8 T-lymphocyte count, and younger age. Individuals reaching a CD4 T-lymphocyte count of 500/microL or greater at 4 years were characterized by higher nadir and baseline CD4 T-lymphocyte counts and a more sustained reduction of HIV-1 RNA levels. CONCLUSIONS: At 4 years, only 39% of individuals treated with HAART reached a CD4 T-lymphocyte count of 500/microL or greater, and 16% with CD4 T-lymphocyte counts less than 200/microL remained susceptible to opportunistic infections. Treatment interruptions, a poor virologic response, and older age were the major factors negatively affecting the recovery of CD4 T lymphocytes.},
	Author = {Kaufmann, G. R. and Perrin, L. and Pantaleo, G. and Opravil, M. and Furrer, H. and Telenti, A. and Hirschel, B. and Ledergerber, B. and Vernazza, P. and Bernasconi, E. and Rickenbach, M. and Egger, M. and Battegay, M.},
	Journal = {Arch Intern Med},
	Keywords = {Adult *Antiretroviral Therapy, Highly Active *CD4 Lymphocyte Count CD8-Positive T-Lymphocytes Female HIV Infections/*drug therapy/*immunology *Hiv-1 Human Lymphocyte Count Male Middle Aged Prospective Studies RNA, Viral/*analysis Support, Non-U.S. Gov't Viral Load},
	Note = {0003-9926 Journal Article},
	Number = {18},
	Pages = {2187-95},
	Title = {CD4 T-lymphocyte recovery in individuals with advanced HIV-1 infection receiving potent antiretroviral therapy for 4 years: the Swiss HIV Cohort Study},
	Volume = {163},
	Year = {2003}}

@article{MartinezPicadoetal99,
	Abstract = {The relative replicative fitness of human immunodeficiency virus type 1 (HIV-1) mutants selected by different protease inhibitors (PIs) in vivo was determined. Each mutant was compared to wild type (WT), NL4-3, in the absence of drugs by several methods, including clonal genotyping of cultures infected with two competing viral variants, kinetics of viral antigen production, and viral infectivity/virion particle ratios. A nelfinavir-selected protease D30N substitution substantially decreased replicative capacity relative to WT, while a saquinavir-selected L90M substitution moderately decreased fitness. The D30N mutant virus was also outcompeted by the L90M mutant in the absence of drugs. A major natural polymorphism of the HIV-1 protease, L63P, compensated well for the impairment of fitness caused by L90M but only slightly improved the fitness of D30N. Multiply substituted indinavir-selected mutants M46I/L63P/V82T/I84V and L10R/M46I/L63P/V82T/I84V were just as fit as WT. These results indicate that the mutations which are usually initially selected by nelfinavir and saquinavir, D30N and L90M, respectively, impair fitness. However, additional mutations may improve the replicative capacity of these and other drug-resistant mutants. Hypotheses based on the greater fitness impairment of the nelfinavir-selected D30N mutant are suggested to explain observations that prolonged responses to delayed salvage regimens, including alternate PIs, may be relatively common after nelfinavir failure.},
	Author = {Martinez-Picado, J. and Savara, A. V. and Sutton, L. and D'Aquila, R. T.},
	Journal = {J Virol},
	Keywords = {Adaptation, Biological Amino Acid Substitution Animals Anti-HIV Agents/*pharmacology Cells, Cultured Drug Resistance, Microbial HIV Protease Inhibitors/*pharmacology HIV-1/*drug effects/genetics/physiology Human Mice Mutagenesis, Site-Directed Nelfinavir/*pharmacology Saquinavir/*pharmacology Support, Non-U.S. Gov't Support, U.S. Gov't, P.H.S. Tumor Cells, Cultured Virus Replication/*drug effects},
	Note = {0022-538x Journal Article},
	Number = {5},
	Pages = {3744-52},
	Title = {Replicative fitness of protease inhibitor-resistant mutants of human immunodeficiency virus type 1},
	Volume = {73},
	Year = {1999}}

@article{Mellorsetal96,
	Abstract = {The relation between viremia and clinical outcome in individuals infected with human immunodeficiency virus-type 1 (HIV-1) has important implications for therapeutic research and clinical care. HIV-1 RNA in plasma was quantified with a branched-DNA signal amplification assay as a measure of viral load in a cohort of 180 seropositive men studied for more than 10 years. The risk of acquired immunodeficiency syndrome (AIDS) and death in study subjects, including those with normal numbers of CD4+ T cells, was directly related to plasma viral load at study entry. Plasma viral load was a better predictor of progression to AIDS and death than was the number of CD4+ T cells.},
	Author = {Mellors, J. W. and Rinaldo, C. R., Jr. and Gupta, P. and White, R. M. and Todd, J. A. and Kingsley, L. A.},
	Journal = {Science},
	Keywords = {Acquired Immunodeficiency Syndrome/*virology Antiviral Agents/therapeutic use Biological Markers/blood CD4 Lymphocyte Count CD4-Positive T-Lymphocytes/virology Cohort Studies Disease Progression Follow-Up Studies HIV Infections/drug therapy/mortality/*virology HIV-1/genetics/*physiology Human Male Prognosis Proportional Hazards Models RNA, Viral/*blood Support, Non-U.S. Gov't Support, U.S. Gov't, Non-P.H.S. Support, U.S. Gov't, P.H.S. Survival Rate Time Factors Viremia/*virology Virus Replication},
	Note = {0036-8075 Comment Journal Article},
	Number = {5265},
	Pages = {1167-70},
	Title = {Prognosis in HIV-1 infection predicted by the quantity of virus in plasma},
	Volume = {272},
	Year = {1996}}

@article{Milleretal00,
	Abstract = {OBJECTIVE: To compare the rate of disease progression according to viral load and CD4 cell count in patients receiving or not receiving highly active antiretroviral therapy (HAART), defined as protease inhibitor-containing regimens. DESIGN: An observational study, with prospectively collected data. METHODS: All patients attending the HIV Outpatient clinic as of 1 January 1995 (n = 2083) were included. Follow-up was until the first AIDS-defining event or death. Associations between viral load or CD4 cell count and disease progression were assessed using a person-years approach. Event rates were compared using Poisson regression analysis; a multivariate model was used to assess the independent effects of CD4, viral load and treatment group on event rates and to consider interactions between these variables. RESULTS: The event rates increased with lower CD4 cell count and higher viral load for both treatment groups and were generally lower in the HAART group. In a multivariate analysis, lower CD4 cell counts and higher viral loads remained significantly associated with disease progression, irrespective of treatment group. However, the event rate was significantly lower for the HAART group compared with the control group (relative rate 0.53, P < 0.001). CONCLUSIONS: HAART-treated patients with high viral loads and CD4 cell counts experienced reduced disease progression compared with individuals with the same CD4 cell count and viral load not receiving HAART. Consequently, the short-term prognosis associated with viral load levels and CD4 cell counts may differ in patients on HAART. Whether this effect will be observed with non-protease-inhibitor-containing HAART is not known at this time.},
	Author = {Miller, V. and Sabin, C. A. and Phillips, A. N. and Rottmann, C. and Rabenau, H. and Weidmann, E. and Rickerts, V. and Findhammer, S. and Helm, E. B. and Staszewski, S.},
	Journal = {Aids},
	Keywords = {Adolescent Adult Aged Antiretroviral Therapy, Highly Active CD4 Lymphocyte Count Disease Progression HIV Infections/*drug therapy/pathology/virology HIV Protease Inhibitors/*therapeutic use *HIV-1/isolation & purification Human Middle Aged Prospective Studies RNA, Viral/analysis Regression Analysis Support, Non-U.S. Gov't Viral Load},
	Note = {0269-9370 Clinical Trial Journal Article},
	Number = {14},
	Pages = {2129-36},
	Title = {The impact of protease inhibitor-containing highly active antiretroviral therapy on progression of HIV disease and its relationship to CD4 and viral load},
	Volume = {14},
	Year = {2000}}

@article{Pikettyetal98,
	Abstract = {OBJECTIVES: To determine the clinical, virological and immunological outcome in a cohort of unselected patients receiving triple combination therapy for more than 1 year. METHODS: Prospective follow-up of a cohort of 162 unselected, protease inhibitor-naive, antiretroviral-experienced patients with advanced HIV disease, treated with indinavir combined with two nucleoside analogues. RESULTS: The mean CD4 cell count and plasma HIV RNA level in the study group at baseline were 69+/-5 x 10(6)/l and 4.75+/-0.07 log10 copies/ml, respectively. Five per cent of patients died prematurely or were lost to follow-up. Fifty-seven per cent of patients responded to therapy, as assessed by a sustained increase in CD4 cell counts above 50 x 10(6)/l and a decrease in plasma HIV RNA greater than 1 log10 copies/ml, throughout 12.1 months of follow-up. Seventeen per cent of patients were immunological and virological non-responders. Twenty-one per cent of patients exhibited discrepant virological and immunological responses to treatment, of whom one-half failed to exhibit significant increases in CD4 cells despite a virological response to therapy and one-half exhibited increased CD4 cell counts in the absence of significant decrease in plasma viral load. The incidence of AIDS-defining events in the latter group of patients was similar to that of responder patients, whereas their incidence was higher in patients who failed to exhibit a virological and immunological response and those who failed to increase CD4 cells despite a significant decrease in viral load. CONCLUSION: Our observations of discrepant immunological and virological responses to treatment raise the issue of the significance of persistent elevated levels of plasma HIV RNA and of the relevance of measurements of plasma viral load for assessing the efficacy of antiretroviral therapy in patients whose CD4 cell counts increase despite the absence of significant decrease in plasma HIV viral load.},
	Author = {Piketty, C. and Castiel, P. and Belec, L. and Batisse, D. and Si Mohamed, A. and Gilquin, J. and Gonzalez-Canali, G. and Jayle, D. and Karmochkine, M. and Weiss, L. and Aboulker, J. P. and Kazatchkine, M. D.},
	Journal = {Aids},
	Keywords = {Adult Aged Anti-HIV Agents/*therapeutic use Cohort Studies Drug Therapy, Combination Female Follow-Up Studies HIV Infections/*drug therapy/immunology/physiopathology/virology HIV Protease Inhibitors/*therapeutic use Human Indinavir/*therapeutic use Lamivudine/*therapeutic use Male Middle Aged Prospective Studies Reverse Transcriptase Inhibitors/*therapeutic use Stavudine/*therapeutic use Support, Non-U.S. Gov't Treatment Outcome Zidovudine/*therapeutic use},
	Note = {0269-9370 Journal Article},
	Number = {7},
	Pages = {745-50},
	Title = {Discrepant responses to triple combination antiretroviral therapy in advanced HIV disease},
	Volume = {12},
	Year = {1998}}

@article{Pikettyetal01,
	Abstract = {Within a prospective cohort of 150 human immunodeficiency virus (HIV)-infected patients who began first-line protease inhibitor therapy in 1996, the outcome of 42 patients with discrepant virologic and immunologic responses to antiretroviral treatment at 12 months was analyzed at 30 months of treatment. The incidence of AIDS-defining events and deaths (14%) in the group of patients with immunologic responses in the absence of a virologic response was higher than that in full-responder patients (2%); yet, the incidence in this group was lower than that in patients with no immunologic response, despite a virologic response (21%), and was lower than that in patients without an immunologic or virologic response (67%; P<.0001, log-rank test). Differences in outcome were significant (relative risk, 6.9; 95% confidence interval, 1.9-39.3) when factors for progression were compared with those of responder patients. The results support the relevance of the CD4 cell marker over plasma HIV load for predicting clinical outcome in patients who do not achieve full immunologic and virologic responses.},
	Author = {Piketty, C. and Weiss, L. and Thomas, F. and Mohamed, A. S. and Belec, L. and Kazatchkine, M. D.},
	Journal = {J Infect Dis},
	Keywords = {Adult Aged Antiretroviral Therapy, Highly Active CD4 Lymphocyte Count Cohort Studies Disease Progression Female HIV Infections/*drug therapy/immunology/virology HIV Protease Inhibitors/*therapeutic use Human Incidence Longitudinal Studies Male Middle Aged Mortality Prospective Studies RNA, Viral/blood Time Factors Treatment Outcome Viral Load},
	Note = {0022-1899 Journal Article},
	Number = {9},
	Pages = {1328-35},
	Title = {Long-term clinical outcome of human immunodeficiency virus-infected patients with discordant immunologic and virologic responses to a protease inhibitor-containing regimen},
	Volume = {183},
	Year = {2001}}

@article{Pilonetal02,
	Abstract = {Inhibition of human immunodeficiency virus type 1 reverse transcriptase (RT) by both nucleoside and nonnucleoside RT inhibitors profoundly inhibits virus replication. Nucleoside RT inhibitors are known to be toxic, but there is little information regarding the toxicities of nonnucleoside RT inhibitors (NNRTI). We demonstrate that efavirenz (an NNRTI) induces caspase- and mitochondrion-dependent apoptosis of Jurkat T cells and human peripheral blood mononuclear cells. The clinical relevance of these observations is not yet clear.},
	Author = {Pilon, A. A. and Lum, J. J. and Sanchez-Dardon, J. and Phenix, B. N. and Douglas, R. and Badley, A. D.},
	Journal = {Antimicrob Agents Chemother},
	Keywords = {Annexin V/diagnostic use Apoptosis/*drug effects Caspases/physiology Enzyme Inhibitors/diagnostic use Fluorescein-5-isothiocyanate Fluorescent Dyes HIV-1 Reverse Transcriptase/*antagonists & inhibitors Human Jurkat Cells Membrane Potentials/drug effects Mitochondria/drug effects/physiology Oxazines/*pharmacology Reverse Transcriptase Inhibitors/*pharmacology Support, Non-U.S. Gov't},
	Note = {0066-4804 Journal Article},
	Number = {8},
	Pages = {2687-91},
	Title = {Induction of apoptosis by a nonnucleoside human immunodeficiency virus type 1 reverse transcriptase inhibitor},
	Volume = {46},
	Year = {2002}}

@article{Priceetal03,
	Abstract = {Many individuals chronically infected with human immunodeficiency virus type 1 (HIV-1) experience a recrudescence of plasma virus during continuous combination antiretroviral therapy (ART) due either to the emergence of drug-resistant viruses or to poor compliance. In most cases, virologic failure on ART is associated with a coincident decline in CD4(+) T lymphocyte levels. However, a proportion of discordant individuals retain a stable or even increasing CD4(+) T lymphocyte count despite virological failure. In order to address the nature of these different outcomes, we evaluated virologic and immunologic variables in a prospective, single-blinded, nonrandomized cohort of 53 subjects with chronic HIV-1 infection who had been treated with continuous ART and monitored intensively over a period of 19 months. In all individuals with detectable viremia on ART, multiple drug resistance mutations with similar impacts on viral growth kinetics were detected in the pol gene of circulating plasma virus. Further, C2V3 env gene analysis demonstrated sequences indicative of CCR5 coreceptor usage in the majority of those with detectable plasma viremia. In contrast to this homogeneous virologic pattern, comprehensive screening with a range of antigens derived from HIV-1 revealed substantial immunologic differences. Discordant subjects with stable CD4(+) T lymphocyte counts in the presence of recrudescent virus demonstrated potent virus-specific CD4(+) and CD8(+) T lymphocyte responses. In contrast, subjects with virologic failure associated with declining CD4(+) T lymphocyte counts had substantially weaker HIV-specific CD4(+) T lymphocyte responses and exhibited a trend towards weaker HIV-specific CD8(+) T lymphocyte responses. Importantly the CD4(+) response was sustained over periods as long as 11 months, confirming the stability of the phenomenon. These correlative data lead to the testable hypothesis that the consequences of viral recrudescence during continuous ART are modulated by the HIV-specific cellular immune response.},
	Author = {Price, D. A. and Scullard, G. and Oxenius, A. and Braganza, R. and Beddows, S. A. and Kazmi, S. and Clarke, J. R. and Johnson, G. E. and Weber, J. N. and Phillips, R. E.},
	Journal = {J Virol},
	Keywords = {Adult Amino Acid Sequence Anti-HIV Agents/pharmacology/*therapeutic use CD4-Positive T-Lymphocytes/*immunology CD8-Positive T-Lymphocytes/*immunology Chronic Disease Drug Resistance, Viral/genetics Drug Therapy, Combination HIV Envelope Protein gp120/chemistry/genetics HIV Infections/*drug therapy/immunology/physiopathology HIV-1/*drug effects/genetics/physiology Human Lymphocyte Count Middle Aged Molecular Sequence Data Mutation Peptide Fragments/chemistry/genetics Prospective Studies RNA, Viral/blood Single-Blind Method Support, Non-U.S. Gov't *Treatment Failure Viral Load},
	Note = {0022-538x Clinical Trial Journal Article},
	Number = {10},
	Pages = {6041-9},
	Title = {Discordant outcomes following failure of antiretroviral therapy are associated with substantial differences in human immunodeficiency virus-specific cellular immunity},
	Volume = {77},
	Year = {2003}}

@article{Quinonesetal00,
	Abstract = {This study was designed to examine the impact of human immunodeficiency virus type 1 (HIV-1) fitness on disease progression through the use of a dual competition/heteroduplex tracking assay (HTA). Despite numerous studies on the impact of HIV-1 diversity and HIV-specific immune response on disease progression, we still do not have a firm understanding of the long-term pathogenesis of this virus. Strong and early CD8-positive cytotoxic T-cell and CD4-positive T-helper cell responses directed toward HIV-infected cells appear to curb HIV pathogenesis. However, the rate at which the virus infects the CD4(+) T-cell population and possibly destroys the HIV-specific immune response may also alter the rate of disease progression. For HIV-1 fitness studies, we established conditions for dual HIV-1 infections of peripheral blood mononuclear cells (PBMC) and a sensitive HTA to measure relative virus production. A pairwise comparison was then performed to estimate the relative fitness of various non-syncytium-inducing/CCR5-tropic (NSI/R5) and syncytium-inducing/CXCR4-tropic (SI/X4) HIV-1 isolates. Four HIV-1 strains (two NSI/R5 and two SI/X4) with moderate ex vivo fitness were then selected as controls and competed against primary HIV-1 isolates from an HIV-infected Belgian cohort. HIV-1 isolates from long-term survivors (LTS) were outcompeted by control strains and were significantly less fit than HIV-1 isolates from patients with accelerated progression to AIDS (PRO). In addition, NSI/R5 HIV-1 isolates from PRO overgrew control SI/X4 strains, suggesting that not all SI/X4 HIV-1 isolates replicate more efficiently than all NSI/R5 isolates. Finally, there were strong, independent correlations between viral load and the total relative fitness values of HIV-1 isolates from PRO (r = 0.84, P = 0.033) and LTS (r = 0.86, P = 0.028). Separation of the PRO and LTS plots suggest that HIV-1 fitness together with viral load may be a strong predictor for the rate of disease progression.},
	Author = {Quinones-Mateu, M. E. and Ball, S. C. and Marozsan, A. J. and Torre, V. S. and Albright, J. L. and Vanham, G. and van Der Groen, G. and Colebunders, R. L. and Arts, E. J.},
	Journal = {J Virol},
	Keywords = {*Biological Assay HIV Infections/*physiopathology/*virology *HIV-1/physiology Human Predictive Value of Tests Prognosis Support, Non-U.S. Gov't Support, U.S. Gov't, P.H.S.},
	Note = {0022-538x Journal Article},
	Number = {19},
	Pages = {9222-33},
	Title = {A dual infection/competition assay shows a correlation between ex vivo human immunodeficiency virus type 1 fitness and disease progression},
	Volume = {74},
	Year = {2000}}

@article{Racinanetal02,
	Abstract = {OBJECTIVE: To study whether hepatitis C virus (HCV) co-infection or the severe elevation of transaminases is associated with survival after the initiation of antiretroviral combination therapy. DESIGN: Prospective hospital-based cohort (Aquitaine Cohort). METHODS: HIV-infected adults started on an antiretroviral combination before 30 June 1999. HCV infection was defined as antibody detection or positive HCV RNA. Severe elevation of transaminases was defined as a value of aspartate or alanine aminotransferase (AST, ALT) above five times the upper limit of normal values. Survival was studied using a Cox model, including at least baseline HCV status and transaminases as a time-dependent covariate. RESULTS: Overall, 995 patients were analysed, including 576 HCV-positive individuals (58%). At baseline, HCV-positive patients were younger, more often injecting drug users and women, and had more frequently elevated transaminases. A shorter survival was associated with AIDS stage [hazard ratio (HR) versus non-AIDS 1.67; 95% confidence interval (CI) 1.03; 2.68], lower CD4 cell count (HR for 50 cells/mm3 lower 1.33; CI 1.17; 1.51), lower haemoglobin (HR for 1 g/dl lower 1.20; CI 1.07; 1.35), lower platelet count (HR for 10 000 cells/mm3 lower 1.04; CI 1.01; 1.07), and AST during follow-up (HR for > or = 200 IU/l 2.30; CI 1.32; 4.03). HCV co-infection (HR 1.20; CI 0.75; 1.92) was not statistically associated with survival. CONCLUSION: The occurrence of a severe elevation of transaminases was associated with poorer survival, although HCV was not. If liver toxicity may be treatment induced, plasma drug concentrations could guide dosage adjustments of antiretroviral treatments currently prescribed to optimize their use.},
	Author = {Rancinan, C. and Neau, D. and Saves, M. and Lawson-Ayayi, S. and Bonnet, F. and Mercie, P. and Dupon, M. and Couzigou, P. and Dabis, F. and Chene, G.},
	Journal = {Aids},
	Keywords = {Acquired Immunodeficiency Syndrome/complications Age Factors Anti-HIV Agents/*therapeutic use Antiretroviral Therapy, Highly Active Cohort Studies Comparative Study Disease Progression Female Follow-Up Studies HIV Infections/blood/*complications/*drug therapy Hepatitis C/blood/*complications Human Male Proportional Hazards Models Substance Abuse, Intravenous Support, Non-U.S. Gov't Survival Analysis Transaminases/blood},
	Note = {0269-9370 Journal Article},
	Number = {10},
	Pages = {1357-62},
	Title = {Is hepatitis C virus co-infection associated with survival in HIV-infected patients treated by combination antiretroviral therapy?},
	Volume = {16},
	Year = {2002}}

@article{Rogeretal99,
	Abstract = {HAART may increase CD4+ T cell counts despite a persistently detectable HIV load. The impact of HAART on apoptosis, which may play a role in the disease process in HIV-infected patients, has not been extensively studied. We performed a study to compare the level of spontaneous T cell apoptosis and anti-retroviral treatments in a cohort of HIV-1-infected patients. Data were obtained from a computerized medical record. Quantification of apoptotic cells was by cytofluorometric technique. From November 1995 to December 1997 we studied T cell apoptosis in 112 HIV-infected patients. Forty patients were classified A, 36 B and 36 C. Thirty patients were naive and 82 received an anti-retroviral treatment, 49 including a protease inhibitor (PI). The median plasma viraemia determined in 63 patients was 3.6 (range 1.3-5.6) log10. The median apoptotic cell count was 22% (range 2-73%) and 12% (range 2-60%) for CD4+ and CD8+ T cells, respectively. We did not observe any correlation between the HIV viraemia and the level of apoptosis of T cell subsets. Patients with HAART showed a lower percentage of apoptotic CD4+ T cells only: 16% (range 2-61%) versus 25% (range 5-73%) for patients receiving two nucleoside analogues (P = 0.02). This effect was significant in stage A patients and remained observable during the whole course of HIV disease. In conclusion, HAART, without any relation to plasma viraemia, is able to reduce apoptosis of CD4+ T cells.},
	Author = {Roger, P. M. and Breittmayer, J. P. and Arlotto, C. and Pugliese, P. and Pradier, C. and Bernard-Pomier, G. and Dellamonica, P. and Bernard, A.},
	Journal = {Clin Exp Immunol},
	Keywords = {Adult Aged Anti-HIV Agents/*therapeutic use *Apoptosis CD4-Positive T-Lymphocytes/cytology/*drug effects CD8-Positive T-Lymphocytes/drug effects Didanosine/therapeutic use Drug Therapy, Combination Female HIV Infections/*drug therapy/immunology/pathology HIV Protease Inhibitors/therapeutic use Human Lamivudine/therapeutic use Male Middle Aged Multivariate Analysis Retrospective Studies Stavudine/therapeutic use Viral Load Zalcitabine/therapeutic use Zidovudine/therapeutic use},
	Note = {0009-9104 Journal Article},
	Number = {3},
	Pages = {412-6},
	Title = {Highly active anti-retroviral therapy (HAART) is associated with a lower level of CD4+ T cell apoptosis in HIV-infected patients},
	Volume = {118},
	Year = {1999}}

@article{Stoddaretalt01,
	Abstract = {Many HIV-1-infected patients treated with protease inhibitors (PI) develop PI-resistant HIV-1 variants and rebounds in viremia, but their CD4+ T-cell counts often do not fall. We hypothesized that in these patients, T-cell counts remain elevated because PI-resistant virus spares intrathymic T-cell production. To test this, we studied recombinant HIV-1 clones containing wild-type or PI-resistant protease domains, as well as uncloned isolates from patients, in activated peripheral blood mononuclear cells, human thymic organ cultures and human thymus implants in SCID-hu Thy/Liv mice. In most cases, wild-type and PI-resistant HIV-1 isolates replicated to similar degrees in peripheral blood mononuclear cells. However, the replication of PI-resistant but not wild-type HIV-1 isolates was highly impaired in thymocytes. In addition, patients who had PI-resistant HIV-1 had abundant thymus tissue as assessed by computed tomography. We propose that the inability of PI-resistant HIV-1 to replicate efficiently in thymus contributes to the preservation of CD4+ T-cell counts in patients showing virologic rebound on PI therapy.},
	Author = {Stoddart, C. A. and Liegler, T. J. and Mammano, F. and Linquist-Stepps, V. D. and Hayden, M. S. and Deeks, S. G. and Grant, R. M. and Clavel, F. and McCune, J. M.},
	Journal = {Nat Med},
	Keywords = {Adult Animals CD4 Lymphocyte Count Drug Resistance, Microbial Fetal Tissue Transplantation Flow Cytometry HIV Core Protein p24/metabolism HIV Infections/immunology/pathology/*virology HIV Protease/genetics/*metabolism HIV Protease Inhibitors/*pharmacology HIV-1/*drug effects/enzymology/genetics/*physiology Human Mice Mice, SCID Middle Aged Organ Culture Recombination, Genetic Support, Non-U.S. Gov't Support, U.S. Gov't, P.H.S. T-Lymphocytes/*physiology/virology Thymus Gland/pathology/physiopathology/transplantation/*virology Viral Load *Virus Replication},
	Note = {1078-8956 Journal Article},
	Number = {6},
	Pages = {712-8},
	Title = {Impaired replication of protease inhibitor-resistant HIV-1 in human thymus},
	Volume = {7},
	Year = {2001}}

@article{Sufkaetal03,
	Abstract = {Mechanisms that underly discordant CD4+ cell/virus load (VL) responses in patients who receive highly active antiretroviral therapy (HAART) were studied in 30 human immunodeficiency virus (HIV)-positive patients, in 3 groups. Discordant responders maintained CD4+ cell levels >200/mm(3) with stable or increasing trend, despite sustained VLs of 500-5000 copies/mL, for >2 years. Treatment-success patients had CD4+ cell counts >200/mm(3) with stable or increasing trend and VLs <50 copies/mL, for >2 years. Treatment-failure patients initially responded to HAART, followed by decreasing CD4+ cell counts and increasing VLs. Interferon-gamma production to gag and noncytolytic CD8+ cell suppressive activity were greater in discordant responders. Cellular activation was greatest in patients with treatment failure. All discordant responders had non-syncytium-inducing (CCR5-tropic) viruses. Viruses from discordant responders and from patients with treatment failure had extensive resistance mutations; discordant responders had significantly lower viral replication capacities. These findings suggest that discordant responses may be related to enhanced HIV-directed immune responses, diminished cellular activation, decreased viral replication capacity, and preservation of non-syncytium-inducing virus strains.},
	Author = {Sufka, S. A. and Ferrari, G. and Gryszowka, V. E. and Wrin, T. and Fiscus, S. A. and Tomaras, G. D. and Staats, H. F. and Patel, D. D. and Sempowski, G. D. and Hellmann, N. S. and Weinhold, K. J. and Hicks, C. B.},
	Journal = {J Infect Dis},
	Keywords = {Adult *Antiretroviral Therapy, Highly Active *CD4 Lymphocyte Count Female HIV/*drug effects HIV Infections/*drug therapy/*immunology/virology HIV Protease Inhibitors/*pharmacology/therapeutic use Human Male Middle Aged Support, Non-U.S. Gov't Support, U.S. Gov't, P.H.S. Time Factors Treatment Failure *Viral Load Virus Replication/drug effects},
	Note = {0022-1899 Clinical Trial Journal Article},
	Number = {7},
	Pages = {1027-37},
	Title = {Prolonged CD4+ cell/virus load discordance during treatment with protease inhibitor-based highly active antiretroviral therapy: immune response and viral control},
	Volume = {187},
	Year = {2003}}

@article{Tebaldietal03,
	Abstract = {To ascertain the impact of hepatitis C virus (HCV) infection on human immunodeficiency virus (HIV) disease progression and associated death in the era of highly active antiretroviral therapy (HAART), we examined mortality rates, the presence of other diseases, and antiretroviral use in an observational cohort of 823 HIV-infected patients with and without HCV coinfection during the period of January 1996 through June 2001. Analyses were used to compare patient characteristics, comorbid conditions, and survival durations in HIV-infected and HIV-HCV-coinfected patients. HIV-HCV-coinfected persons did not have a statistically greater rate of acquired immunodeficiency syndrome or of renal or cardiovascular disease, but they did have more cases of cirrhosis and transaminase elevations. There were proportionately more deaths in the HIV-HCV-coinfected group. Age, baseline CD4+ cell count, and duration of HAART were significantly associated with survival, but HCV infection was not. HAART use was a strong predictor of increased duration of survival, suggesting that treatment is more important to survival than is HCV coinfection status.},
	Author = {Tedaldi, E. M. and Baker, R. K. and Moorman, A. C. and Alzola, C. F. and Furhrer, J. and McCabe, R. E. and Wood, K. C. and Holmberg, S. D.},
	Journal = {Clin Infect Dis},
	Keywords = {Anti-HIV Agents/therapeutic use *Antiretroviral Therapy, Highly Active *Hiv HIV Infections/*complications/drug therapy/epidemiology/mortality *Hepacivirus Hepatitis C/*complications/epidemiology/mortality Human Morbidity Mortality Support, U.S. Gov't, P.H.S.},
	Note = {1537-6591 Journal Article},
	Number = {3},
	Pages = {363-7},
	Title = {Influence of coinfection with hepatitis C virus on morbidity and mortality due to human immunodeficiency virus infection in the era of highly active antiretroviral therapy},
	Volume = {36},
	Year = {2003}}

@article{Wang&Bembom&vanderLaan06,
	Author = {Y. Wang and O. Bembom and M.J. van der Laan},
	Journal = {Journal of Statistical Planning and Inference},
	Optnote = {also http://www.bepress.com/ucbbiostat/paper159},
	Title = {Data adaptive estimation of the treatment specific mean},
	Year = {2006}}

@article{Sinisi&vanderLaan04,
	Author = {S. Sinisi and M.J. van der Laan},
	Journal = {Journal of Statistical Methods in Molecular Biology},
	Optnote = {http://www.bepress.com/sagmb/vol3/iss1/art18},
	Title = {The {D}eletion/{S}ubstitution/{A}ddition Algorithm in Loss Function Based Estimation: Applications in Genomics},
	Volume = {3},
	Year = {2004}}

@techreport{Petersenetal05,
	Author = {M. L. Petersen and S.G. Deeks and J. N. Martin and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Month = {December},
	Optnote = {http://www.bepress.com/ucbbiostat/paper199},
	Title = {History-Adjusted Marginal Structural Models: Time-Varying Effect Modification and Dynamic Treatment Regimens},
	Type = {Technical Report 199},
	Year = {2005}}

@techreport{vanderLaan&Rubin05,
	Author = {M.J. van der Laan and D. Rubin},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper180},
	Title = {Estimating Function Based Cross-Validation and Learning},
	Type = {Technical Report 180},
	Year = {2005}}

@article{Chambaz&Rousseau08,
	Author = {A. Chambaz and J. Rousseau},
	Issue = {2},
	Journal = {The Annals of Statistics},
	Pages = {938-62},
	Title = {Bounds for Bayesian order identification with application to mixtures},
	Volume = {36},
	Year = {2008}}

@techreport{Gruber&vanderLaan09,
	Author = {S. Gruber and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper252},
	Title = {Targeted Maximum Likelihood Estimation: A Gentle Introduction},
	Type = {Technical Report 252},
	Year = {2009}}

@techreport{vanderLaan06,
	Author = {M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper203},
	Title = {Causal Effect Models for Intention to Treat and Realistic Individualized Treatment Rules},
	Type = {Technical Report 203},
	Year = {2006}}

@techreport{vanderLaan08b,
	Author = {M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Month = {March},
	Optnote = {http://www.bepress.com/ucbbiostat/paper232},
	Title = {The construction and analysis of adaptive group sequential designs},
	Type = {Technical Report 232},
	Year = {2008}}

@techreport{Moore&vanderLaan07,
	Author = {K.L. Moore and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Month = {April},
	Optnote = {http://www.bepress.com/ucbbiostat/paper215},
	Title = {Covariate adjustment in randomized trials with binary outcomes},
	Type = {Technical Report 215},
	Year = {2007}}

@techreport{vanderLaan&Petersen05,
	Author = {M.J. van der Laan and M.L. Petersen},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper187},
	Title = {Direct Effect Models},
	Type = {Technical Report 187},
	Year = {2005}}

@techreport{Petersen&vanderLaan06,
	Author = {M.L. Petersen and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Title = {Individualized Treatment Rules and Clinical Trials},
	Type = {Technical Report},
	Year = {2006}}

@article{vanderLaan&Petersen&Joffe05,
	Author = {M.J. van der Laan and M.L. Petersen and M.M. Joffe},
	Journal = {The International Journal of Biostatistics},
	Number = {1},
	Optnote = {http://www.bepress.com/ijb/vol1/iss1/4},
	Pages = {10-20},
	Title = {History-Adjusted Marginal Structural Models and Statically-Optimal Dynamic Treatment Regimens},
	Volume = {1},
	Year = {2005}}

@article{vanderLaan06a,
	Author = {M.J. van der Laan},
	Journal = {International Journal of Biostatistics},
	Number = {1},
	Optnote = {http://www.bepress.com/ijb/vol2/iss1/art2},
	Title = {Statistical Inference for Variable Importance},
	Volume = {2},
	Year = {2006}}

@article{vanderLaan&Birkner&Hubbard05,
	Author = {M.J. van der Laan and M.D. Birkner and A.E. Hubbard},
	Journal = {Journal of Statistical Applications in Genetics and Molecular Biology},
	Number = {1},
	Optnote = {http://www.bepress.com/sagmb/vol4/iss1/art29},
	Title = {Empirical Bayes and resampling based multiple testing procedure controlling tail probability of the proportion of false positives},
	Volume = {4},
	Year = {2005}}

@article{vanderLaan&Dudoit&Pollard04b,
	Author = {M.J. van der Laan and S. Dudoit and K.S. Pollard},
	Journal = {Journal of Statistical Applications in Genetics and Molecular Biology},
	Number = {1},
	Optnote = {http://www.bepress.com/sagmb/vol3/iss1/art15},
	Title = {Augmentation procedures for control of the generalized family-wise error rate and tail probabilities for the proportion of false positives},
	Volume = {3},
	Year = {2004}}

@article{vanderLaan&Dudoit&Pollard04,
	Author = {S. Dudoit and M.J. van der Laan and K.S. Pollard},
	Journal = {Journal of Statistical Applications in Genetics and Molecular Biology},
	Number = {1},
	Optnote = {http://www.bepress.com/sagmb/vol3/iss1/art14},
	Title = {Multiple testing. Part II. Step-down procedures for control of the family-wise error rate},
	Volume = {3},
	Year = {2004}}

@article{Dudoit&vanderLaan&Pollard04,
	Author = {S. Dudoit and M.J. van der Laan and K.S. Pollard},
	Journal = {Journal of Statistical Applications in Genetics and Molecular Biology},
	Number = {1},
	Optnote = {http://www.bepress.com/sagmb/vol3/iss1/art13},
	Title = {Multiple testing. Part I. Single-step procedures for control of general Type I error rates},
	Volume = {3},
	Year = {2004}}

@article{Birkner&Sinisi&vanderLaan05,
	Author = {M.D. Birkner and S.E. Sinisi and M.J. van der Laan},
	Journal = {Journal of Statistical Applications in Genetics and Molecular Biology},
	Number = {1},
	Optnote = {http://www.bepress.com/sagmb/vol4/iss1/art8},
	Title = {Multiple Testing and Data Adaptive Regression: An Application to {HIV}-1 Sequence Data},
	Volume = {4},
	Year = {2005}}

@techreport{vanderLaan&Hubbard06,
	Author = {M.J. van der Laan and A.E. Hubbard},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper198},
	Title = {Quantile-Function Based Null Distribution in Resampling Based Multiple Testing},
	Type = {Technical Report},
	Year = {2006}}

@techreport{Molinaro&vanderLaan04,
	Author = {A. Molinaro and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper162},
	Title = {Deletion/Substitution/Addition Algorithm for Partitioning the Covariate Space in Prediction},
	Type = {Technical Report},
	Year = {2004}}

@techreport{Birkner&vanderLaan05,
	Author = {M.D. Birkner and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Title = {Application of a Variable Importance Measure Method to {HIV}-1 Sequence Data},
	Type = {Technical Report},
	Year = {2005}}

@techreport{Neugebauer&vanderLaan05b,
	Author = {R. Neugebauer and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {134},
	Optnote = {http://www.bepress.com/ucbbiostat/paper134, to appear in {JSPI}},
	Title = {Locally Efficient Estimation of Nonparametric Causal Effects on Mean Outcomes in Longitudinal Studies},
	Type = {Technical Report},
	Year = {2005}}

@techreport{Wang&Petersen&vanderLaan06,
	Author = {Y. Wang and M. Petersen and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Title = {A statistical method for diagnosing {ETA} bias in {IPTW} estimators},
	Type = {Technical Report},
	Year = {2006}}

@techreport{vanderLaan&Dudoit&vanderVaart,
	Author = {M.J. van der Laan and S. Dudoit and A.W. van der Vaart},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Month = {February},
	Optnote = {http://www.bepress.com/ucbbiostat/paper142},
	Title = {The Cross-Validated Adaptive Epsilon-Net Estimator},
	Type = {Technical Report 142},
	Year = {2004}}

@techreport{vanderLaan&Dudoit03,
	Author = {M.J. van der Laan and S. Dudoit},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Month = {November},
	Optnote = {http://www.bepress.com/ucbbiostat/paper130},
	Title = {Unified cross-validation methodology for selection among estimators and a general cross-validated adaptive epsilon-net estimator: Finite sample oracle inequalities and examples},
	Type = {Technical Report},
	Year = {2003}}

@techreport{Petersen&vanderLaan05,
	Author = {M. Petersen and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Title = {Estimation of direct and indirect causal effects in Epidemiology},
	Type = {Technical Report},
	Year = {2005}}

@techreport{vanderLaan&Petersen04,
	Author = {M.J. van der Laan and M. Petersen},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Month = {August},
	Title = {Estimation of direct and indirect causal effects in longitudinal studies},
	Type = {Technical Report 155},
	Year = {2004}}

@techreport{vanderLaan&Hubbard&Jewell04,
	Author = {M.J. van der Laan and A.E. Hubbard and N.P. Jewell},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Month = {September},
	Optnote = {http://www.bepress.com/ucbbiostat/paper157},
	Title = {Estimation of Treatment Effects in Randomized Trials with Noncompliance and a Dichotomous Outcome},
	Type = {Technical Report 157},
	Year = {2004}}

@techreport{Bein&Hubbard&vanderLaan05,
	Author = {E. Bein and A.E. Hubbard and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Title = {Estimating Function Based Cross-Validation in Estimation of the Causal Effect in Randomized Trials},
	Type = {Technical Report},
	Year = {2005}}

@techreport{Molinaroetal05,
	Author = {A.M. Molinaro and M.J. van der Laan and D.H. Moore and K. Kerlikowske},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Note = {http://www.bepress.com/ucbbiostat/paper149},
	Title = {Survival point estimate prediction in matched and non-matched case-control subsample designed studies},
	Year = {2005}}

@techreport{Dudoitetal04,
	Author = {S. Dudoit and M.J. van der Laan and S. Kele\c{s} and A. M. Molinaro and S. E. Sinisi and S.L. Teng},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Note = {to appear in \emph{SIGKDD} Explorations on Microarray Data Mining},
	Title = {Loss-Based Estimation with Cross-Validation: Applications to Microarray Data Analysis and Motif Finding.},
	Year = {2004}}

@book{Friedman&Furberg&Demets98,
	Author = {L.M.Friedman and C.D. Furberg and D.L. DeMets},
	Publisher = {Springer-Verlag New York},
	Title = {Fundamentals of Clinical Trials},
	Year = {1998}}

@book{Andersenetal93,
	Author = {P.K. Andersen and O. Borgan and R.D. Gill and N. Keiding},
	Publisher = {Springer-Verlag New York},
	Title = {Statistical Models Based on Counting Processes},
	Year = {1993}}

@incollection{Robins03,
	Author = {J.M. Robins},
	Booktitle = {Highly Structured Stochastic Systems},
	Editor = {P. Green, N. Hjort, and S. Richardson},
	Pages = {70--81},
	Publisher = {Oxford University Press, Oxford},
	Title = {Semantics of causal DAG models and the identification of direct and indirect effects},
	Year = {2003}}

@techreport{Pearl01,
	Author = {J. Pearl},
	Institution = {University of California, Los Angeles, Department of Computer Science},
	Title = {Cognitive systems Laboratory},
	Year = {2001}}

@techreport{Pearl10b,
	Author = {J. Pearl},
	Institution = {University of California, Los Angeles, Department of Computer Science},
	Month = {August},
	Number = {R-370},
	Title = {The Causal Foundations of Structural Equation Modeling},
	Year = {2010}}

@book{Pearl09,
	Author = {J. Pearl},
	Date-Modified = {2011-04-03 23:20:08 -0700},
	Edition = {2nd},
	Publisher = {Cambridge University Press, Cambridge},
	Title = {Causality: Models, Reasoning, and Inference},
	Year = {2000}}

@article{Robins&Greenland92,
	Author = {J.M. Robins and S. Greenland},
	Journal = {Epidemiology},
	Number = {0},
	Pages = {143--155},
	Title = {Identifiability and exchangeability for direct and indirect effects},
	Volume = {3},
	Year = {1992}}

@article{vanderLaan95,
	Author = {M.J. van der Laan},
	Journal = {Bernoulli},
	Number = {4},
	Pages = {335--341},
	Title = {Identity for NPMLE in missing data and biased sampling models},
	Volume = {1},
	Year = {1995}}

@article{vanderLaan98,
	Author = {M.J. van der Laan},
	Journal = {Lifetime Data Models},
	Number = {0},
	Pages = {83--102},
	Title = {Identity for NPMLE in Censored Data Models},
	Volume = {4},
	Year = {1998}}

@article{Klaassen86,
	Author = {C.A.J. Klaassen},
	Journal = {The Annals of Statistics},
	Pages = {1548--1562},
	Title = {Consistent estimation of the influence function of locally asymptotically linear estimators},
	Volume = {15},
	Year = {1987}}

@article{Robins&Rotnitzky04,
	Author = {J.M. Robins and A. Rotnitzky},
	Journal = {Biometrika},
	Number = {0},
	Optnote = {To Appear},
	Pages = {0},
	Title = {Estimation of Treatment Effects in Randomized Trials with Noncompliance and a Dichotomous Outcome using Structural Nested Mean Models},
	Volume = {0},
	Year = {2004}}

@article{vanderVaart91,
	Author = {A.W. van der Vaart},
	Journal = {The Annals of Statistics},
	Pages = {178--204},
	Title = {On differentiable functionals},
	Volume = {19},
	Year = {1991}}

@article{Rubin78,
	Author = {D.B. Rubin},
	Journal = {The Annals of Statistics},
	Pages = {34--58},
	Title = {Bayesian Inference for causal effects: the role of randomization},
	Volume = {6},
	Year = {1978}}

@article{Neyman23,
	Author = {Neyman, J.},
	Journal = {Statistical Science},
	Optnote = {Translation of 1923 article},
	Pages = {465--480},
	Title = {On the application of probability theory to agricultural experiments},
	Volume = {5},
	Year = {1990}}

@article{Robins86,
	Author = {J.M. Robins},
	Journal = {Mathematical Modelling},
	Pages = {1393--1512},
	Title = {A New Approach to Causal Inference in Mortality Studies with Sustained Exposure Periods - Application to Control of the Healthy Worker Survivor Effect},
	Volume = {7},
	Year = {1986}}

@article{Robins94,
	Author = {J.M. Robins},
	Journal = {Communications in Statistics},
	Pages = {2379--2412},
	Title = {Correcting for non-compliance in randomized trials using structural nested mean models},
	Volume = {23},
	Year = {1994}}


@inproceedings{Robins00c,
	Author = {J.M. Robins},
	Booktitle = {Proceedings of the American Statistical Association: Section on Bayesian Statistical Science},
	Pages = {6-10},
	Title = {Robust Estimation in Sequentially Ignorable Missing Data and Causal Inference Models},
	Year = {2000}}

@article{Stuart10,
	Author = {B.K. Lee and J. Lessler and E.A. Stuart},
	Issue = {3},
	Journal = {Statistics in Medicine},
	Pages = {337-46},
	Title = {Improved propensity score weighting using machine learning},
	Volume = {29},
	Year = {2009}}

@article{Leeetal10,
	Author = {B.K. Lee and J. Lessler and E.A. Stuart},
	Issue = {3},
	Journal = {Statistics in Medicine},
	Pages = {337-46},
	Volume = {29},
	Year = {2009}}


@article{Schneeweiss09,
	Author = {S. Schneeweiss and J.A. Rassen and R. J. Glynn and J. Avorn and H. Mogun and M. A. Brookhart},
	Journal = {Epidemiology},
	Title = {High-dimensional propensity score adjustment in studies of treatment effects using health care claims data},
	Volume = {20(4)},
	pages={512--522},
	Optnote={doi:  10.1097/EDE.0b013e3181a663cc},	Year = {2009}}

@article{Brookhart11,
	Author = {D. Westreich and S.R. Cole and M.J. Funk and M.A. Brookhart and T Sturmer},
	Journal = {Pharmacoepidemiology and Drug Safety},
	Pages = {317-20},
	Title = {The role of the c-statistic in variable selection for propensity scores},
	Volume = {20},
	Year = 2011}

@article{Westreichetal11,
	Author = {D. Westreich and S.R. Cole and M.J. Funk and M.A. Brookhart and T Sturmer},
	Journal = {Pharmacoepidemiology and Drug Safety},
	Pages = {317-20},
	Title = {The role of the c-statistic in variable selection for propensity scores},
	Volume = {20},
	Year = 2011}


@article{Vansteelandt10,
	Author = {S. Vansteelandt and M. Bekaert and G. Claeskens},
	Journal = {Statistical Methods in Medical Research},
	Title = {On model selection and model misspecification in causal inference},
	Volume={21(1)},
	pages={7--30},
	Optnote={doi: 10.1177/0962280210387717},	Year = {2010}}

@article{Vansteelandt&Goetghebeur03,
	Author = {S. Vansteelandt and E. Goetghebeur},
	Journal = {Journal of the Royal Statistical Society, Series B},
	Optnote = {In print},
	Title = {Causal inference with generalized structural mean models},
	Volume = {23},
	Year = {2003}}

@incollection{Robins97a,
	Address = {Chichester, UK},
	Author = {Robins, J.M.},
	Booktitle = {The Encyclopedia of Biostatistics},
	Editor = {Armitage, P. and Colton, T. and Andersen, P.K. and Keiding, N.},
	Publisher = {John Wiley and Sons},
	Title = {Structural Nested Failure Time Models},
	Year = {1997}}



@article{RobinsMSM97,
	Author = {Robins, J. M.},
	Title = {Marginal structural models},
	Journal = {1997 Proceedings of the American Statistical Association Section on Bayesian Statistical Science},
	Pages = {1-10},
	Year = {1997}
}

@article{Hernan&Brumback&Robins,
	Author = {Hernan, M. A. and Brumback, B. and Robins, J. M.},
	Journal = {Epidemiology},
	Number = {5},
	Pages = {561--570},
	Title = {Marginal Structural Models to Estimate the Causal Effect of Zidovudine on the Survival of {HIV}-Positive Men},
	Volume = {11},
	Year = {2000}}

@article{Robins87,
	Author = {Robins, J.M.},
	Coden = {CMAPDK},
	Fjournal = {Computers \& Mathematics with Applications. An International Journal},
	Issn = {0097-4943},
	Journal = {Comput. Math. Appl.},
	Number = {9-12},
	Pages = {923--945},
	Title = {Addendum to: ``{A} new approach to causal inference in mortality studies with a sustained exposure period---application to control of the healthy worker survivor effect'' [{M}ath.\ {M}odelling {\bf 7} (1986), no.\ 9-12, 1393--1512; {M}{R} 87m:92078]},
	Volume = {14},
	Year = {1987}}

@article{Robins&Hernan&Brumback00,
	Author = {Robins, J. M. and Hernan, M. A. and Brumback, B.},
	Journal = {Epidemiology},
	Number = {5},
	Pages = {550--560},
	Title = {Marginal Structural Models and Causal Inference in Epidemiology},
	Volume = {11},
	Year = {2000}}

@article{Bryan&Yu&vanderLaan03,
	Author = {Bryan, J. and Yu, Z. and van der Laan, M.J.},
	Journal = {Biostatistics},
	Number = {3},
	Pages = {361--380},
	Title = {Analysis of Longitudinal Marginal Structural Models},
	Volume = {5},
	Year = {2003}}

@techreport{Yu&vanderLaan03b,
	Author = {Yu, Z. and van der Laan, M.J.},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper132},
	Optnumber = {132},
	Title = {Double Robust Estimation in Longitudinal Marginal Structural Models},
	Year = {2003}}

@article{Murphy03,
	Author = {Murphy, S.A.},
	Journal = {Journal of the Royal Statistical Society: Series B},
	Number = {2},
	Pages = {331-66},
	Title = {Optimal dynamic treatment regimes},
	Volume = {65},
	Year = {2003}}

@article{Robins03a,
	Author = {Robins, J.M.},
	Journal = {Journal of the Royal Statistical Society: Series B},
	Number = {2},
	Pages = {355--66},
	Title = {Discussion of ``Optimal dynamic treatment regimes" by Susan A. Murphy},
	Volume = {65},
	Year = {2003}}

@article{Murphy&vanderLaan&Robins01,
	Author = {S.A. Murphy and M.J. van der Laan and J.M. Robins},
	Journal = {Journal of the American Statistical Association},
	Pages = {1410--1424},
	Title = {Marginal mean models for dynamic treatment regimens},
	Volume = {96},
	Year = {2001}}



@incollection{Robins98,
	Address = {New York},
	Author = {Robins, J.M.},
	Booktitle = {Statistical Models in Epidemiology, the Environment, and Clinical Trials (Minneapolis, MN, 1997)},
	Mrclass = {62N01 (62G08 62P10)},
	Mrnumber = {2001a:62124},
	Pages = {95-133},
	Publisher = {Springer-Verlag},
	Title = {Marginal Structural Models versus Structural Nested Models as Tools for Causal Inference},
	Year = {2000}}

@incollection{Robins97,
	Author = {J.M. Robins},
	Booktitle = {Latent Variable Modeling and Applications to Causality},
	Editor = {M. Berkane, Editor},
	Optseries = {Lecture Notes in Statistics},
	Optvolume = {120},
	Pages = {69--117},
	Publisher = {Springer-Verlag, New York},
	Title = {Causal Inference from Complex Longitudinal Data},
	Year = {1997}}

@incollection{Robins89,
	Address = {Washington D.C.},
	Author = {J.M. Robins},
	Booktitle = {Health Service Methodology: A Focus on AIDS},
	Editor = {L. Sechrest and H. Freeman and A. Mulley},
	Optseries = {Lecture Notes in Statistics},
	Pages = {113--159},
	Publisher = {U.S. Public Health Service, National Center for Health SErvices Research},
	Title = {The analysis of randomized and non-randomized AIDS treatment trials using a new approach in causal inference in longitudinal studies},
	Year = {1989}}

@techreport{Abadie00,
	Author = {A. Abadie},
	Institution = {NBER Technical Working Paper},
	Optnumber = {260},
	Title = {Semiparametric estimation of instrumental variables models for causal effects},
	Year = {2000}}

@article{Abadie03,
	Author = {A. Abadie},
	Journal = {Journal of Econometrics},
	Pages = {231-263},
	Title = {Semiparametric instrumental variable estimation of treatment response models},
	Volume = {113},
	Year = {2003}}

@techreport{Wang&Vanderlaan04,
	Author = {Y. Wang and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper159},
	Optnumber = {159},
	Title = {Data adaptive estimation of the treatment specific mean},
	Year = {2004}}

@techreport{Yu&Vanderlaan02,
	Author = {Z. Yu and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper122},
	Optnumber = {122},
	Title = {Construction of counterfactuals and the {G}-computation formula},
	Year = {2002}}

@techreport{Yu&Vanderlaan03,
	Author = {Z. Yu and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper136},
	Optnumber = {136},
	Title = {Measuring treatment effects using semiparametric models},
	Year = {2003}}

@article{Angristetal&Imbens&Rubin96,
	Author = {J. Angrist and G. Imbens and D.B. Rubin},
	Journal = {Journal of the American Statistical Association},
	Pages = {444-555},
	Title = {Identification of causal effects using instrumental variables},
	Volume = {91},
	Year = {1996}}

@article{Robins&Rotnitzky01A,
	Author = {J.M Robins and A. Rotnitzky},
	Journal = {Statistica Sinica},
	Pages = {920-935},
	Title = {Comment on {I}nference for Semiparametric Models: Some Questions and an Answer, by {B}ickel, {P}.{J}. and {K}won, {J}.},
	Volume = {11},
	Year = {2001}}

@article{Rubin96,
	Author = {D.B. Rubin},
	Journal = {Journal of the American Statistical Association},
	Month = {June},
	Number = {434},
	Pages = {473-89},
	Title = {Multiple Imputation After 18+ Years},
	Volume = {91},
	Year = {1996}}

@article{Angrist01,
	Author = {J. Angrist},
	Journal = {Journal of Business and Economics Statistics},
	Pages = {1--16},
	Title = {Estimation of limited dependent variable models with dummy endogenous regressors: simple strategies for empirical practice},
	Volume = {19},
	Year = {2001}}

@article{Chamberlain87,
	Author = {G. Chamberlain},
	Journal = {Journal of Econometrics},
	Pages = {305--334},
	Title = {Asymptotic efficiency in estimation with conditional moment restrictions},
	Volume = {34},
	Year = {1987}}

@article{Hiranoetal00,
	Author = {K. Hirano and G. Imbens and D.B. Rubin and X-H. Zhou},
	Journal = {Biostatistics},
	Pages = {69--88},
	Title = {Assessing the effects of influenza vaccine in an encouragement design},
	Volume = {1},
	Year = {2000}}

@inproceedings{Robins05,
	Author = {J.M. Robins},
	Booktitle = {Proceedings of the 2nd Seattle symposium in biostatistics},
	Editor = {Lin, D.Y, Heagerty P.J},
	Optpublisher = {Springer-Verlag Lecture Notes in Statistics},
	Pages = {189--326},
	Title = {Optimal structural nested models for optimal sequential decisions},
	Volume = {179},
	Year = {2005}}

@techreport{Robins05b,
	Author = {J.M. Robins},
	Institution = {Department of Biostatistics, Havard University},
	Title = {Optimal structural nested models for optimal sequential decisions},
	Year = {2005}}

@inproceedings{Akaike73,
	Author = {H. Akaike},
	Booktitle = {Second International Symposium on Information Theory},
	Editor = {B.N. Petrov and F. Csaki},
	Organization = {Budapest: Academiai Kiado},
	Pages = {267-281},
	Title = {Information theory and an extension of the maximum likelihood principle},
	Year = {1973}}

@article{Balke&Pearl97,
	Author = {A. Balke and J. Pearl},
	Journal = {Journal of the American Statistical Association},
	Pages = {1172--1176},
	Title = {Bound on treatment effects from studies with imperfect compliance},
	Volume = {92},
	Year = {1997}}

@inproceedings{Balke&Pearl94,
	Author = {A. Balke and J. Pearl},
	Booktitle = {In Proceedings of the 12th National Conference on Artificial Intelligence},
	Optaddress = {Menlo Park, CA},
	Optpublisher = {MIT Press},
	Pages = {230--237},
	Title = {Counterfactual probabilities: Computational methods, bounds, and applications},
	Volume = {I},
	Year = {1994}}

@article{Ambroise&McLachlan02,
	Author = {C. Ambroise and G. J. McLachlan},
	Journal = PNAS,
	Number = {10},
	Pages = {6562--6566},
	Title = {Selection bias in gene extraction on the basis of microarray gene-expression data},
	Volume = {99},
	Year = {2002}}

@incollection{Arabie&Hubert96,
	Address = {River Edge, NJ},
	Author = {P. Arabie and L. J. Hubert},
	Booktitle = {Clustering and Classification},
	Editor = {P. Arabie and L. J. Hubert and G. De Soete},
	Pages = {5--63},
	Publisher = {World Scientific Publishing Co.},
	Title = {An overview of combinatorial data analysis},
	Year = {1996}}

@article{Schwartz78,
	Author = {G. Schwartz},
	Journal = {The Annals of Statistics},
	Pages = {461-464},
	Title = {Estimating the Dimension of a Model},
	Volume = {6},
	Year = {1978}}

@article{Barnard35,
	Author = {M. Barnard},
	Journal = {Annals of Eugenics},
	Pages = {352--371},
	Title = {The secular variations of skull characters in four series of Egyptian skulls},
	Volume = {6},
	Year = {1935}}

@inproceedings{BenHur&Elisseeff&Guyon02,
	Author = {A. Ben-Hur and A. Elisseeff and I. Guyon},
	Booktitle = {Pacific Symposium on Biocomputing},
	Pages = {6--17},
	Title = {A stability based method for discovering structure in clustered data},
	Volume = {7},
	Year = {2002}}

@article{Benjamini&Hochberg95,
	Author = {Y. Benjamini and Y. Hochberg},
	Journal = {J. R. Statist. Soc. B},
	Pages = {289--300},
	Title = {Controlling the false discovery rate: a practical and powerful approach to multiple testing},
	Volume = {57},
	Year = {1995}}

@article{Benjamini&Yekutieli01,
	Author = {Y. Benjamini and D. Yekutieli},
	Journal = {The Annals of Statistics},
	Number = {4},
	Pages = {1165--1188},
	Title = {The control of the false discovery rate in multiple testing under dependency},
	Volume = {29},
	Year = {2001}}

@article{Beran88,
	Author = {R. Beran},
	Journal = JASA,
	Pages = {679--686},
	Title = {Balanced simultaneous confidence sets},
	Volume = {83},
	Year = {1988}}

@article{Bock85,
	Author = {H-H Bock},
	Journal = {Journal of Classification},
	Pages = {77--108},
	Title = {On some significance tests in cluster analysis},
	Volume = {2},
	Year = {1985}}

@incollection{Bock96,
	Address = {River Edge, NJ},
	Author = {H-H Bock},
	Booktitle = {Clustering and Classification},
	Editor = {P. Arabie and L. J. Hubert and G. De Soete},
	Pages = {377--453},
	Publisher = {World Scientific Publishing Co.},
	Title = {Probability models and hypotheses testing in partitioning cluster analysis},
	Year = {1996}}

@article{Boldricketal02,
	Author = {J. C. Boldrick and A. A. Alizadeh and M. Diehn and S. Dudoit and C. L. Liu and C. E. Belcher and D. Botstein and L. M. Staudt and P. O. Brown and D. A. Relman},
	Journal = PNAS,
	Number = {2},
	Pages = {972--977},
	Title = {Stereotyped and specific gene expression programs in human innate immue responses to bacteria},
	Volume = {99},
	Year = {2002}}

@article{Bozdogan00,
	Author = {H. Bozdogan},
	Journal = {Journal of Mathematical Psychology},
	Pages = {62-91},
	Title = {Akaike's information criterion and recent developments in information complexity},
	Volume = {44},
	Year = {2000}}

@incollection{Bozdogan93,
	Author = {H. Bozdogan},
	Booktitle = {Information and Classification},
	Editor = {O. Opitz and B. Lausen and R. Klar},
	Publisher = {Heidelberg: Springer-Verlag},
	Title = {Choosing the number of component clusters in the mixture model using a new informational complexity criterion of the inverse Fisher information matrix},
	Year = {1993}}

@article{Braver,
	Author = {S. L. Braver},
	Journal = {Educational and Psychological Measurement},
	Pages = {283--301},
	Title = {On splitting the tails unequally: a new perspective on one-versus two-tailed tests},
	Volume = {35},
	Year = {1975}}

@article{Breckenridge89,
	Author = {J. Breckenridge},
	Journal = {Multivariate Behavioral Research},
	Pages = {147--161},
	Title = {Replicating cluster analysis: Method, consistency and validity},
	Volume = {24},
	Year = {1989}}

@article{Breiman&Spector92,
	Author = {L. Breiman and P. Spector},
	Journal = {International Statistical Review},
	Pages = {291--319},
	Title = {Submodel Selection and Evaluation in Regression. The $X$ Random Case},
	Volume = {60},
	Year = {1992}}

@article{Breiman01,
	Author = {L. Breiman},
	Journal = {Statistical Science},
	Number = {3},
	Pages = {199--215},
	Title = {Statistical modeling: the two cultures},
	Volume = {16},
	Year = {2001}}

@article{Breiman96,
	Author = {L. Breiman},
	Journal = {The Annals of Statistics},
	Number = {6},
	Pages = {2350--2383},
	Title = {Heuristics of instability and stabilization in model selection},
	Volume = {24},
	Year = {1996}}

@article{Breiman98,
	Author = {L. Breiman},
	Journal = {The Annals of Statistics},
	Pages = {801-824},
	Title = {Arcing classifiers},
	Volume = {26},
	Year = {1998}}

@article{Breiman96b,
	Author = {L. Breiman},
	Journal = {Machine Learning},
	Pages = {123-140},
	Title = {Bagging predictors},
	Volume = {24},
	Year = {1996}}

@techreport{Breiman98b,
	Author = {L. Breiman},
	Institution = {Department of Statistics, U.C. Berkeley},
	Month = {March},
	Number = {513},
	Title = {Using Convex pseudo-data to increase prediction accuracy},
	Year = {1998}}

@article{Breiman92,
	Author = {L. Breiman},
	Journal = JASA,
	Number = {419},
	Pages = {738--754},
	Title = {The Little Bootstrap and Other Methods for Dimensionality Selection in Regression: $X$-Fixed Prediction Error},
	Volume = {87},
	Year = {1992}}

@techreport{Breiman96c,
	Author = {L. Breiman},
	Institution = {Department of Statistics, U.C. Berkeley},
	Title = {Out-of-bag estimation},
	Year = {1996}}

@techreport{Breiman99,
	Author = {L. Breiman},
	Institution = {Department of Statistics, U.C. Berkeley},
	Number = {567},
	Title = {Random forests - random features},
	Year = {1999}}

@book{Little&Rubin87,
	Author = { R.J.A. Little and D. B. Rubin},
	Publisher = {Wiley},
	Series = {Wiley Series in Probability and Mathematical Statistics},
	Title = {Statistical Analysis With Missing Data},
	Year = {1987}}

@book{Breimanetal84,
	Author = {L. Breiman and J. H. Friedman and R. Olshen and C. J. Stone},
	Publisher = {Wadsworth International Group},
	Series = {The Wadsworth statistics/probability series},
	Title = {Classification and regression trees},
	Year = {1984}}

@book{Hastie&Tibshirani&Friedman02,
	Author = {T. Hastie and R. Tibshirani and J. Friedman},
	Publisher = {Springer},
	Series = {Springer Series in Statistics},
	Title = {The Elements of Statistical Learning},
	Year = {2002}}

@article{Broman01,
	Author = {K. W. Broman},
	Journal = {Lab Animal},
	Number = {7},
	Pages = {44--52},
	Title = {Review of statistical methods for QTL mapping in experimental crosses},
	Volume = {30},
	Year = {2001}}

@phdthesis{Broman97,
	Author = {K. W. Broman},
	School = {Department of Statistics, U.C. Berkeley},
	Title = {Identifying quantitative trait loci in experimental crosses},
	Type = {Ph.{D}. thesis},
	Year = {1997}}

@article{Brown&Koplowitz79,
	Author = {T. A. Brown and J. Koplowitz},
	Journal = {IEEE Transactions on Information Theory},
	Number = {5},
	Pages = {617--619},
	Title = {The weighted nearest neighbor rule for class dependent sample sizes},
	Volume = {25},
	Year = {1979}}

@article{Buhlmann&Yu,
	Author = {P. Buhlmann and B. Yu},
	Journal = {The Annals of Statistics},
	Title = {Explaining Bagging.},
	Year = {(Accepted)}}

@article{Burges98,
	Author = {C. J. C. Burges},
	Journal = {Data Mining and Knowledge Discovery},
	Month = {December},
	Pages = {121--167},
	Title = {A tutorial on support vector machines for pattern recognition},
	Volume = {2},
	Year = {1998}}

@article{Burman89,
	Author = {P. Burman},
	Journal = {Biometrika},
	Pages = {503-514},
	Title = {A comparative study of ordinary cross-validation, $v$-fold cross-validati on and the repeated learning testing methods},
	Volume = {76},
	Year = {1989}}

@techreport{Buttrey&Karo02,
	Author = {S. E. Buttrey and C. Karo},
	Institution = {Naval Postgraduate School, Monterey, CA},
	Title = {Using k--neareset neighbor classification in the leaves of a tree},
	Year = {2002}}

@article{Calinski&Harabasz74l,
	Author = {R. Calinski and J. Harabasz},
	Journal = {Communications in Statistics},
	Pages = {1--27},
	Title = {A dendrite method for cluster analysis},
	Volume = {3},
	Year = {1974}}

@article{Callowetal00,
	Author = {M. J. Callow and S. Dudoit and E. L. Gong and T. P. Speed and E. M. Rubin},
	Journal = {Genome Research},
	Number = {12},
	Pages = {2022--2029},
	Title = {Microarray expression profiling identifies genes with altered expression in {HDL} deficient mice},
	Volume = {10},
	Year = {2000}}

@book{Chambers98,
	Author = {J. M. Chambers},
	Publisher = {Springer-Verlag New York},
	Title = {Programming with Data: A Guide to the S Language},
	Year = {1998}}

@book{Diggleetal02,
	Author = {Peter J. Diggle and P. Heagerty and K-Y Liang and S.L. Zeger},
	Publisher = {Oxford University Press},
	Title = {Analysis of Longitudinal Data},
	Year = {2002 (Second Edition)}}

@techreport{Chang&Lin01,
	Author = {C.-C. Chang and C.-J. Lin},
	Note = {\\ {\tt http://www.csie.ntu.edu.tw/~cjlin/papers/libsvm2.ps.gz}},
	Title = {{LIBSVM}: a Library for Support Vector Machines (Version 2.31)},
	Year = {2001}}

@article{Changetal02,
	Author = {H. Y. Chang and J. T. Chi and S. Dudoit and C. Bondre and M. van de Rijn and D. Botstein D and P. O. Brown},
	Journal = PNAS,
	Number = {20},
	Pages = {12877--12882},
	Title = {Diversity, topographic differentiation, and positional memory in human fibroblasts},
	Volume = {99},
	Year = {2002}}

@article{Chenetal02,
	Author = {X. Chen and S. T. Cheung and S. So and S. T. Fan and C. Barry and J. Higgins and K.-M. Lai and J. Ji and S. Dudoit and I. O. L. Ng and M. van de Rijn and D. Botstein and P. O. Brown},
	Journal = {Molecular Biology of the Cell},
	Number = {6},
	Pages = {1929--1939},
	Title = {Gene expression patterns in human liver cancers},
	Volume = {13},
	Year = {2002}}

@incollection{Cleveland&Grosse&Shyu92,
	Author = {W. S. Cleveland, E. Grosse and W. M. Shyu},
	Booktitle = {Statistical Models in S},
	Chapter = {6},
	Editor = {J. M. Chambers and T. J. Hastie},
	Publisher = {Wadsworth \& Brooks/Cole},
	Title = {Local regression models},
	Year = 1992}

@article{Cleveland&Devlin88,
	Author = {W. S. Cleveland and S. J. Devlin},
	Journal = JASA,
	Pages = {596--610},
	Title = {Locally-Weighted Regression: An Approach to Regression Analysis by Local Fitting},
	Volume = {83},
	Year = {1988}}

@article{Cleveland79,
	Author = {W. S. Cleveland},
	Journal = JASA,
	Number = {368},
	Pages = {829--836},
	Title = {Robust locally weighted regression and smoothing scatterplots},
	Volume = {74},
	Year = {1979}}

@article{Correa&Wolfson99,
	Author = {J. A. Correa and D. B. Wolfson},
	Journal = {Journal of Statistical Computation and Simulation},
	Pages = {209--219},
	Title = {Length-bias: some characterizations and applications},
	Tnumber = {3},
	Volume = {64},
	Year = {1999}}

@article{Correa&Dudoit&Goldstein02,
	Author = {J. A. Correa and S. Dudoit and D. R. Goldstein},
	Note = {(Submitted)},
	Optjournal = {Statistics in Medicine},
	Title = {Multiple testing in the survival analysis of microarray data},
	Year = {2002}}

@article{Cortes&Vapnik95,
	Author = {C. Cortes and V. Vapnik},
	Journal = {Machine Learning},
	Month = {December},
	Pages = {273-297},
	Title = {Support-vector networks},
	Volume = {20},
	Year = {1995}}

@inproceedings{Davies&Bouldin79,
	Author = {D. Davies and D. Bouldin},
	Booktitle = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
	Optnumber = {PAMI-1},
	Pages = {224--227},
	Title = {A cluster separation measure},
	Volume = {1},
	Year = {1979}}

@article{Davis&Anderson89,
	Author = {R. B. Davis and J. R. Anderson},
	Journal = {Statistics in Medicine},
	Pages = {947-961},
	Title = {Exponential survival trees},
	Volume = {8},
	Year = {1989}}

@incollection{Day96,
	Address = {River Edge, NJ},
	Author = {W. H. E. Day},
	Booktitle = {Clustering and Classification},
	Editor = {P. Arabie and L. J. Hubert and G. De Soete},
	Pages = {199--233},
	Publisher = {World Scientific Publishing Co.},
	Title = {Complexity theory: {A}n introduction for practitioners of classification},
	Year = {1996}}

@article{Dettling&Buhlmann02,
	Author = {M. Dettling and P. B\"{u}hlmann},
	Title = {How to Use Boosting for Tumor Classification with Gene Expression Data},
	Year = {2002}}

@article{Dudoit&Fridlyand02,
	Author = {S. Dudoit and J. Fridlyand},
	Optjournal = {Bioinformatics},
	Title = {Bagging to improve the accuracy of a clustering procedure},
	Year = {2002}}

@incollection{Dudoit&Fridlyand02b,
	Author = {S. Dudoit and J. Fridlyand},
	Booktitle = {Statistical Analysis of Gene Expression Microarray Data},
	Editor = {T. P. Speed},
	Note = {(To appear)},
	Publisher = {Chapman \& Hall/CRC},
	Title = {Classification in microarray experiments},
	Year = {2002}}

@article{Dudoit&Fridlyand02c,
	Author = {S. Dudoit and J. Fridlyand},
	Journal = {Genome Biology},
	Number = {7},
	Pages = {0036.1--0036.21},
	Title = {A prediction-based resampling method to estimate the number of clusters in a dataset},
	Volume = {3},
	Year = {2002}}

@techreport{Dudoit&Fridlyand01,
	Author = {S. Dudoit and J. Fridlyand},
	Institution = {Department of Statistics, Uiversity of California, Berkeley},
	Number = {600},
	Title = {Applications of resampling methods to estimate the number of clusters and to improve the accuracy of a clustering method},
	Url = {stat-www.berkeley.edu/users/sandrine/publications.html},
	Year = {2001},
	Bdsk-Url-1 = {stat-www.berkeley.edu/users/sandrine/publications.html}}

@article{Dudoit&vanderLaan05,
	Author = {S. Dudoit and M.J. van der Laan},
	Journal = {Statistical Methodology},
	Number = {2},
	Optnote = {www.bepress.com/ucbbiostat/paper126},
	Pages = {131--154},
	Title = {Asymptotics of cross-validated risk estimation in estimator selection and performance assessment},
	Volume = {2},
	Year = {2005}}

@article{Dudoit&Speed99,
	Author = {S. Dudoit and T. P. Speed},
	Journal = {The Annals of Statistics},
	Number = {3},
	Pages = {943--986},
	Title = {A score test for linkage using identity by descent data from sibships},
	Volume = {27},
	Year = {1999}}

@article{Dudoit&Speed00,
	Author = {S. Dudoit and T. P. Speed},
	Journal = {Biostatistics},
	Number = {1},
	Pages = {1--26},
	Title = {A score test for the linkage analysis of qualitative and quantitative traits based on identity by descent data on sib-pairs},
	Volume = {1},
	Year = {2000}}

@incollection{Dudoit&Speed99b,
	Address = {New York},
	Author = {S. Dudoit and T. P. Speed},
	Booktitle = {Statistics in Genetics},
	Editor = {M. E. Halloran and S. Geisser},
	Pages = {181--221},
	Publisher = {Springer-Verlag},
	Series = {IMA Volumes in Mathematics and its Applications},
	Title = {Triangle constraints for sib-pair identity by descent probabilities under a general multilocus model for disease susceptibility},
	Volume = {112},
	Year = {1999}}

@incollection{Dudoit&Yang03,
	Author = {S. Dudoit and Y. H. Yang},
	Booktitle = {The Analysis of Gene Expression Data: Methods and Software},
	Editor = {G. Parmigiani and E. S. Garrett and R. A. Irizarry and S. L. Zeger},
	Publisher = {Springer-Verlag, New York},
	Title = {Bioconductor {R} packages for exploratory analysis and normalization of c{DNA} microarray data},
	Year = {2003}}

@article{Dudoit&Fridlyand&Speed02,
	Author = {S. Dudoit and J. Fridlyand and T. P. Speed},
	Journal = JASA,
	Number = {457},
	Pages = {77--87},
	Title = {Comparison of Discrimination Methods for the Classification of Tumors Using Gene Expression Data},
	Volume = {97},
	Year = {2002}}

@article{Dudoitetal02,
	Author = {S. Dudoit and Y. H. Yang and M. J. Callow and T. P. Speed},
	Journal = {Statistica Sinica},
	Number = {1},
	Pages = {111--139},
	Title = {Statistical methods for identifying differentially expressed genes in replicated c{DNA} microarray experiments},
	Volume = {12},
	Year = {2002}}

@techreport{Dudoit&Shaffer&Boldrick02,
	Author = {S. Dudoit and J. P. Shaffer and J. C. Boldrick},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {110},
	Title = {Multiple hypothesis testing in microarray experiments},
	Url = {www.bepress.com/ucbbiostat/paper110/},
	Year = {2002},
	Bdsk-Url-1 = {www.bepress.com/ucbbiostat/paper110/}}

@article{Duffy&Quiroz91,
	Author = {D. E. Duffy and A. J. Quiroz},
	Journal = {Journal of Classification},
	Pages = {65--91},
	Title = {A permutation-based algorithm for block clustering},
	Volume = {8},
	Year = {1991}}

@article{Dunn58,
	Author = {O. J. Dunn},
	Journal = {Annals of Mathematical Statistics},
	Pages = {1095-111},
	Title = {Estimation of the means of dependent variables},
	Volume = {29},
	Year = {1958}}

@book{Efron&Tibshirani93,
	Author = {B. Efron and R. J. Tibshirani},
	Publisher = {Chapman \& Hall/CRC},
	Title = {An Introduction to the Bootstrap},
	Year = {1993}}

@article{EfronetalJASA01,
	Author = {B. Efron and R. Tibshirani and J. D. Storey and V. Tusher},
	Journal = JASA,
	Pages = {1151--1160},
	Title = {Empirical Bayes analysis of a microarray experiment},
	Volume = {96},
	Year = {2001}}

@techreport{Efron&Storey&Tibshirani01,
	Author = {B. Efron and J. D. Storey and R. Tibshirani},
	Institution = {Department of Statistics, Stanford University},
	Number = {2001-218},
	Title = {Microarrays, empirical Bayes methods, and false discovery rates},
	Year = {2001}}

@article{Finner99,
	Author = {H. Finner},
	Journal = {The Annals of Statistics},
	Pages = {274--289},
	Title = {Stepwise multiple test procedures and control of directional errors},
	Volume = {27},
	Year = {1999}}

@article{Fisher36,
	Author = {R. A. Fisher},
	Journal = {Annals of Eugenics},
	Pages = {179-188},
	Title = {The use of multiple measurements in taxonomic problems},
	Volume = {7},
	Year = {1936}}

@article{Fisher26,
	Author = {R. A. Fisher},
	Journal = {J. Min. Agric. Gr. Br},
	Pages = {505--513},
	Title = {The arrangement of field experiments},
	Volume = {33},
	Year = {1926}}

@techreport{Fix&Hodges51,
	Author = {E. Fix and J. Hodges},
	Institution = {Randolph Field, Texas: USAF School of Aviation Medicine},
	Title = {Discriminatory analysis, nonparametric discrimination: consistency properties},
	Year = {1951}}

@article{Fowlkes&Mallows83,
	Author = {E. B. Fowlkes and C. L. Mallows},
	Journal = JASA,
	Optnumber = {383},
	Pages = {553--584},
	Title = {A method for comparing two hierarchical clusterings},
	Volume = {78},
	Year = {1983}}

@article{Fowlkes&Gnanadesikan&Kettenring88,
	Author = {E. B. Fowlkes and R. Gnanadesikan and J. R. Kettenring},
	Journal = JC,
	Pages = {205--228},
	Title = {Variable selection in clustering},
	Volume = {5},
	Year = {1988}}

@techreport{Fraley&Raftery98,
	Author = {C. Fraley and A. Raftery},
	Institution = {Department of Statistics, University of Washington},
	Note = {\url{http://www.stat.washington.edu/www/research/reports/1990s/#1998}},
	Number = {329},
	Title = {How many clusters? Which clustering method? -- answers via model-based cluster analysis},
	Year = {1998}}

@article{Freund&Schapire97,
	Author = {Y. Freund and R. E. Schapire},
	Journal = {Journal of Computer and System Sciences},
	Pages = {119--139},
	Title = {A decision-theoretic generalization of on-line learning and an application to boosting},
	Volume = {55},
	Year = {1997}}

@phdthesis{Fridlyand01,
	Author = {J. Fridlyand},
	School = {Department of Statistics, U.C. Berkeley},
	Title = {Resampling methods for variable selection and classification: applications to genomics},
	Type = {Ph.{D}. thesis},
	Year = {2001}}

@article{Friedman91,
	Abstract = {A new method is presented for flexible regression modeling of high dimensional data. The model takes the form of an expansion in product spline basis functions, where the number of basis functions as well as the parameters associated with each one (product degree and knot locations) are automatically determined by the data. This procedure is motivated by the recursive partitioning approach to regression and shares its attractive properties. Unlike recursive partitioning, however, this method produces continuous models with continuous derivatives. It has more power and flexibility to model relationships that are nearly additive or involve interactions in at most a few variables. In addition, the model can be represented in a form that separately identifies the additive contributions and those associated with the different multivariable interactions.},
	Author = {Friedman, Jerome H.},
	Copyright = {Copyright � 1991 Institute of Mathematical Statistics},
	Issn = {00905364},
	Journal = {The Annals of Statistics},
	Jstor_Formatteddate = {Mar., 1991},
	Language = {English},
	Number = {1},
	Pages = {pp. 1-67},
	Publisher = {Institute of Mathematical Statistics},
	Title = {Multivariate Adaptive Regression Splines},
	Url = {http://www.jstor.org/stable/2241837},
	Volume = {19},
	Year = {1991},
	Bdsk-Url-1 = {http://www.jstor.org/stable/2241837}}

@techreport{Friedman93,
	Author = {J. H. Friedman},
	Institution = {Department of Statistics, Stanford University},
	Title = {Fast {MARS}},
	Year = {1993}}

@techreport{Friedman94,
	Author = {J. H. Friedman},
	Institution = {Department of Statistics, Stanford University},
	Title = {Flexible metric nearest neighbor classification},
	Year = {1994}}

@techreport{Friedman96a,
	Author = {J. H. Friedman},
	Institution = {Department of Statistics, Stanford University},
	Title = {On bias, variance, 0/1-loss, and the curse--of--dimensionality},
	Year = {1996}}

@techreport{Friedman96b,
	Author = {J. H. Friedman},
	Institution = {Department of Statistics, Stanford University},
	Title = {Another approach to polychotomous classification},
	Year = {1996}}

@article{Friedman&Hastie&Tibshirani00,
	Author = {J. Friedman and T. Hastie and R. Tibshirani},
	Journal = {The Annals of Statistics},
	Note = {(with discussion)},
	Pages = {337--404},
	Title = {Additive logistic regression: a statistical view of boosting},
	Volume = {28},
	Year = {2000}}

@book{Hastie&Tibshirani90,
	Address = {London},
	Author = {T. J. Hastie and R.J. Tibshirani},
	Publisher = {Chapman and Hall},
	Title = {Generalized Additive Models},
	Year = {1990}}

@article{Gabriel71,
	Author = {K. R. Gabriel},
	Journal = {Biometrika},
	Pages = {453--467},
	Title = {The biplot graphic display of matrices with application to principal component analysis},
	Volume = {58},
	Year = {1971}}

@incollection{Gabriel75,
	Author = {K. R. Gabriel},
	Booktitle = {Multivariate Statistical Methods: Among-groups covariation; Within-group covariation},
	Pages = {61--80},
	Title = {A comparison of some methods of simultaneous inference in {MANOVA}},
	Year = {1975}}

@inproceedings{Gabriel&Pun79,
	Author = {K. R. Gabriel and F. C. Pun},
	Booktitle = {Sixth Conference on Probability and Statistics in Atmospheric Science},
	Organization = {American Meterological Society},
	Pages = {248--253},
	Title = {Binary prediction of weather events with several predictors},
	Year = {1979}}

@unpublished{Ge&Dudoit02,
	Author = {Y. Ge and S. Dudoit},
	Note = {(In preparation)},
	Title = {Fast algorithm for resampling-based $p$-value adjustment in multiple testing},
	Year = {2002}}

@article{Geisser75,
	Author = {S. Geisser},
	Journal = {Journal of the American Statistical Association},
	Pages = {320-328},
	Title = {The predictive sample reuse method with applications},
	Volume = {70},
	Year = {1975}}

@techreport{Genovese&Wasserman01,
	Author = {C. Genovese and L. Wasserman},
	Institution = {Department of Statistics, Carnegie Mellon},
	Number = {737},
	Title = {Operating Characteristics and Extensions of the FDR Procedure},
	Year = {2001}}

@article{Gnanadesikan&Kettenring95,
	Author = {R. Gnanadesikan and J. R. Kettenring},
	Journal = JC,
	Pages = {113--136},
	Title = {Weighting and selection of variables for cluster analysis},
	Volume = {12},
	Year = {1995}}

@article{Goldstein&Dudoit&Speed00,
	Author = {D. R. Goldstein and S. Dudoit and T. P. Speed},
	Journal = {Genetic Epidemiology},
	Number = {Suppl. 1},
	Pages = {S85--S91},
	Title = {Power of a score test for quantitative trait linkage analysis of relative pairs.},
	Volume = {19},
	Year = {2000}}

@article{Goldstein&Dudoit&Sped01,
	Author = {D. R. Goldstein and S. Dudoit and T. P. Speed},
	Journal = {Genetic Epidemiology},
	Number = {4},
	Pages = {415--431},
	Title = {Power and robustness of a score test for linkage analysis of quantitative traits using identity by descent data on sib pairs},
	Volume = {20},
	Year = {2001}}

@article{Gordon&Olshen85,
	Author = {L. Gordon and R.A. Olshen},
	Journal = {Cancer Treatment Reports},
	Pages = {10065-1069},
	Title = {Tree-structured survival analysis},
	Volume = {69},
	Year = {1985}}

@incollection{Gordon96,
	Address = {River Edge, NJ},
	Author = {A. D. Gordon},
	Booktitle = {Clustering and Classification},
	Editor = {P. Arabie and L. J. Hubert and G. De Soete},
	Pages = {65--121},
	Publisher = {World Scientific Publishing Co.},
	Title = {Hierarchical classification},
	Year = {1996}}

@book{Gower&Hand96,
	Author = {J. C. Gower and D. J. Hand},
	Edition = {1st},
	Number = {54},
	Publisher = {Chapman \& Hall},
	Series = {Monographs on statistics and applied probability},
	Title = {Biplots},
	Year = {1996}}

@book{Gyorfietal02,
	Address = {New York},
	Author = {L. Gy\"{o}rfi and M. Kohler and A. Krzy\.{z}ak and H. Walk},
	Pages = {100-102},
	Publisher = {Springer-Verlag},
	Title = {A Distribution-Free Theory of Nanparametric Regression},
	Year = {2002}}

@book{Gyorfietal02b,
	Author = {L. Gy\"orfi and M. Kohler and A. Krzy\'{z}ak and H. Walk},
	Publisher = {Springer-Verlag, New York},
	Title = {A distribution-free theory of nonparametric regression},
	Year = {2002}}

@book{Hastie&Tibshirani&Friedman01,
	Author = {T. Hastie and R. Tibshirani and J. H. Friedman},
	Publisher = {Springer-Verlag},
	Title = {The Elements of Statistical Learning : Data Mining, Inference, and Prediction},
	Year = {2001}}

@article{Hansen&Yu01,
	Author = {M. H. Hansen and B. Yu},
	Journal = {Journal of the American Statistical Association},
	Pages = {746-774},
	Title = {Model selection and the principle of minimum description length},
	Volume = {96},
	Year = {2001}}

@article{Hardle&Marron85a,
	Author = {W. H{\"a}rdle and J. S. Marron},
	Journal = {Biometrika},
	Pages = {481--484},
	Title = {Asymptotic nonequivalence of some bandwidth selectors in nonparametric regression},
	Volume = {72},
	Year = {1985}}

@article{Hardle&Marron85b,
	Author = {W. H{\"a}rdle and J. S. Marron},
	Journal = {The Annals of Statistics},
	Pages = {1465-1481},
	Title = {Optimal bandwidth selection in nonparametric regression function estimation},
	Volume = {13},
	Year = {1985}}

@book{Hardle93,
	Author = {W. H{\"a}rdle},
	Publisher = {Cambridge University Press},
	Title = {Applied Nonparametric Regression},
	Year = {1993}}

@article{Hartigan72,
	Author = {J. A. Hartigan},
	Journal = {Journal of the American Statistical Association},
	Pages = {123--129},
	Title = {Direct clustering of a data matrix},
	Volume = {67},
	Year = {1972}}

@book{Hartigan75,
	Author = {J. A. Hartigan},
	Publisher = {Wiley},
	Title = {Clustering Algorithms},
	Year = {1975}}

@article{Hartigan78,
	Author = {J. Hartigan},
	Journal = {The Annals of Statistics},
	Pages = {117--131},
	Title = {Asymptotic distributions for clustering criteria},
	Volume = {6},
	Year = {1978}}

@article{Hartigan85,
	Author = {J. A. Hartigan},
	Journal = JC,
	Pages = {63--76},
	Title = {Statistical theory in clustering},
	Volume = {2},
	Year = {1985}}

@incollection{Hastie&Pregibon92,
	Author = {T.J. Hastie and D. Pregibon},
	Booktitle = {Statistical Models in S},
	Chapter = {6},
	Editor = {J. M. Chambers and T. J. Hastie},
	Publisher = {Wadsworth \& Brooks/Cole},
	Title = {Generalized linear models},
	Year = {1992}}

@article{Hastie&Tibshirani96a,
	Author = {T. Hastie and R. Tibshirani},
	Journal = {IEEE Pattern Recognition and Machine Intelligence},
	Pages = {607--616},
	Title = {Discriminant adaptive nearest-nieghbor classification},
	Volume = {18},
	Year = {1996}}

@techreport{Hastie&Tibshirani96b,
	Author = {T. Hastie and R. Tibshirani},
	Institution = {Department of Statistics, Stanford University},
	Title = {Classification by pairwise coupling},
	Year = {1996}}

@article{Hastie&Tibshirani90b,
	Author = {T.J. Hastie and R.J. Tibshirani},
	Date-Modified = {2011-02-22 20:11:53 -0800},
	Journal = {Biometrics},
	Number = {4},
	Pages = {1005-1016},
	Title = {Exploring the nature of covariate effects in the proportional hazar ds model},
	Volume = {46},
	Year = {1990}}

@e{Hochberg&Tamhane87,
	Author = {Y. Hochberg and A. C. Tamhane},
	Publisher = {Wiley--Interscience},
	Series = {Probability and Mathematical Statistics},
	Title = {Multiple Comparison Procedures},
	Year = {1987}}

@article{Hochberg88,
	Author = {Y. Hochberg},
	Journal = {Biometrika},
	Pages = {800--802},
	Title = {A sharper Bonferroni procedure for multiple tests of significance},
	Volume = {75},
	Year = {1988}}

@article{Holm79,
	Author = {S. Holm},
	Journal = {Scand. J. Statist.},
	Pages = {65--70},
	Title = {A simple sequentially rejective multiple test procedure},
	Volume = {6},
	Year = {1979}}

@article{Hommel&Bernhard99,
	Author = {G. Hommel and G. Bernhard},
	Journal = {Journal of Statistical Planning and Inference},
	Pages = {119--128},
	Title = {Bonferroni procedures for logically related hypotheses},
	Volume = {82},
	Year = {1999}}

@article{Hommel88,
	Author = {G. Hommel},
	Journal = {Biometrika},
	Pages = {383--386},
	Title = {A stagewise rejective multiple test procedure based on a modified Bonferroni test},
	Volume = {75},
	Year = {1988}}

@article{Hubert&Arabie85,
	Author = {L. Hubert and P. Arabie},
	Journal = JC,
	Pages = {193--218},
	Title = {Comparing partitions},
	Volume = {2},
	Year = {1985}}

@book{Jain&Dubes88,
	Address = {Englewood Cliffs, N. J.},
	Author = {A. K. Jain and R. C. Dubes},
	Publisher = {Prentice-Hall},
	Title = {Algorithms for Clustering Data},
	Year = {1988}}

@article{Jogdeo77,
	Author = {K. Jogdeo},
	Journal = {The Annals of Statistics},
	Pages = {495--504},
	Title = {Association and probability inequalities},
	Volume = {5},
	Year = {1977}}

@book{Kaufman&Rousseeuw90,
	Author = {L. Kaufman and P. J. Rousseeuw},
	Publisher = {Wiley, New York.},
	Title = {Finding Groups in Data: An Introduction to Cluster Analysis},
	Year = {1990}}

@article{Keles&vanderLaan&Dudoit03,
	Author = {Kele\c{s}, S. and van der Laan, M. and Dudoit, S.},
	Journal = {Technical Report, Division of Biostatistics, UC Berkeley},
	Title = {Asymptotically Optimal Model Selection Method for Regression on Censored Outcomes},
	Year = {2002}}

@article{Kohonen90,
	Author = {T. Kohonen},
	Journal = {Proc. IEEE},
	Number = {9},
	Pages = {1464--1480},
	Title = {The self-organizing map},
	Volume = {78},
	Year = {1990}}

@book{Kohonen95,
	Address = {Berlin, Heidelberg},
	Author = {T. Kohonen},
	Editor = {T. S. Huang and T. Kohonen and M. R. Schroeder},
	Publisher = {Springer-Verlag},
	Series = {Springer Series in Information Sciences},
	Title = {Self-Organizing Maps},
	Volume = {30},
	Year = {1995}}

@article{Kooperberg&Stone&Truong95,
	Author = {C. Kooperberg and C.J. Stone and Y. K. Truong},
	Journal = {Journal of the American Statistical Association},
	Number = {429},
	Pages = {78-94},
	Title = {Hazard Regression},
	Volume = {90},
	Year = {1995}}

@article{Koutsoukosetal94,
	Author = {A. D. Koutsoukos and L. V. Rubinstein and D. Faraggi and R.M. Simon and S. Kalyandrug and J. N. Weinstein and K.W. Kohn and K.D. Paull},
	Journal = {Statistics in Medicine},
	Pages = {719--730},
	Title = {Discrimination techniques applied to the {NCI} in vitro anti-tumor drug screen: predicting biochemical mechanism of action},
	Volume = {13},
	Year = {1994}}

@article{Krishnaiah&Reising85,
	Author = {P. R. Krishnaiah and J. M. Reising},
	Journal = {Encyclopedia of Statistical Sciences},
	Number = {6},
	Pages = {88--95},
	Title = {Multivariate multiple comparisons},
	Volume = {9},
	Year = {1985}}

@article{Krzanowski&Lai85,
	Author = {W. Krzanowski and Y. Lai},
	Journal = {Biometrics},
	Pages = {23--34},
	Title = {A criterion for determining the number of groups in a dataset using sum of squares clustering},
	Volume = {44},
	Year = {1985}}

@article{Laan&Bryan01,
	Author = {M. J. van der Laan and J. Bryan},
	Journal = {Biostatistics},
	Number = {4},
	Pages = {445--461},
	Title = {Gene expression analysis with the parametric bootstrap},
	Volume = {2},
	Year = {2001}}

@article{Pollard&vanderLaan04,
	Author = {K. S. Pollard and M.J. van der Laan},
	Journal = JSPI,
	Optpages = {85--101},
	Optvolume = {125},
	Title = {Choice of Null Distribution in Resampling Based Multiple Testing},
	Year = {2004}}

@article{vanderLaan&Pollard02,
	Author = {M. J. van der Laan and K. S. Pollard},
	Journal = JSPI,
	Note = {(To appear)},
	Title = {Hybrid clustering of gene expression data with visualization and the bootstrap},
	Year = {2002}}

@article{Leblanc&Crowley92,
	Author = {M. Leblanc and J. Crowley},
	Journal = {Biometrics},
	Pages = {411-425},
	Title = {Relative Risk trees for censored data},
	Volume = {48},
	Year = {1992}}

@inproceedings{Leisch02,
	Author = {F. Leisch},
	Booktitle = {Compstat 2002 --- Proceedings in Computational Statistics},
	Editor = {Wolfgang H{\"a}rdle and Bernd R{\"o}nz},
	Note = {ISBN 3-7908-1517-9},
	Publisher = {Physika Verlag, Heidelberg, Germany},
	Title = {Sweave: Dynamic Generation of Statistical Reports Using Literate Data Analysis},
	Tpages = {575--580},
	Url = {http://www.ci.tuwien.ac.at/~leisch/Sweave},
	Year = {2002},
	Bdsk-Url-1 = {http://www.ci.tuwien.ac.at/~leisch/Sweave}}

@techreport{Leisch02Tb,
	Author = {F. Leisch},
	Institution = {SFB Adaptive Information Systems and Modelling in Economics and Management Science, Vienna University of Economics and Business Administration},
	Month = {March},
	Number = {69},
	Title = {Dynamic generation of statistical reports using literate data analysis},
	Year = {2002}}

@techreport{Leisch99,
	Author = {F. Leisch},
	Institution = {SFB Adaptive Information Systems and Modelling in Economics and Management Science, Vienna University of Economics and Business Administration},
	Month = {August},
	Note = {\url{http://www.ci.tuwien.ac.at/~leisch/papers/fl-techrep.html}},
	Title = {Bagged clustering},
	Year = {1999}}

@article{Lim&Low&Shih00,
	Author = {T-S Lim and W-Y Loh and Y-S Shih},
	Journal = {Machine Learning},
	Pages = {203--229},
	Title = {A comparison of prediction accuracy, complexity, and training time of thiry-three old and new classification algorithms},
	Volume = {40},
	Year = {2000}}

@book{Mardia&Kent&Bibby79,
	Address = {San Diego},
	Author = {K. V. Mardia and J. T. Kent and J. M. Bibby},
	Publisher = {Academic Press, Inc.},
	Title = {Multivariate Analysis},
	Year = {1979}}

@unpublished{Mayo&Spanos02,
	Author = {D. C. Mayo and A. Spanos},
	Title = {A severe-testing interpretation of {N}eyman-{P}earson methods. Unpublished manuscript},
	Year = {2002}}

@book{McCullagh&Nelder89,
	Author = {P. McCullagh and J. A. Nelder},
	Edition = {2nd},
	Number = {37},
	Publisher = {Chapman \& Hall},
	Series = {Monographs on Statistics and Applied Probability},
	Title = {Generalized Linear Models},
	Year = {1989}}

@book{McLachlan92,
	Address = {New York},
	Author = {G. J. McLachlan},
	Publisher = {Wiley},
	Title = {Discriminant analysis and statistical pattern recognition},
	Year = {1992}}

@article{McLachlan&Bean&Peel01,
	Author = {G. J. McLachlan and R. Bean and D. Peel},
	Journal = {Bioinformatics},
	Pages = {413--422},
	Title = {A mixture model-based approach to the clustering of microarray expression data.},
	Volume = {18},
	Year = {2002}}

@book{Miller90,
	Author = {A. J. Miller},
	Publisher = {Chapman and Hall},
	Title = {Subset Selection in Regression},
	Year = {1990}}

@article{Milligan&Cooper85,
	Author = {G. W. Milligan and M. C. Cooper},
	Journal = {Psychometrika},
	Pages = {159--179},
	Title = {An examination of procedures for determining the number of clusters in a data set},
	Volume = {50},
	Year = {1985}}

@article{Milligan&Cooper86,
	Author = {G. W. Milligan and M. C. Cooper},
	Journal = {Multivariate Behavioral Research},
	Pages = {441--458},
	Title = {A study of the comparability of external criteria for hierarchical cluster analysis},
	Volume = {21},
	Year = {1986}}

@article{Milligan&Cooper87,
	Author = {G. W. Milligan and M. C. Cooper},
	Journal = {Applied Psychological Measurement},
	Optmonth = {December},
	Optnumber = {4},
	Pages = {329--354},
	Title = {Methodology review: {C}lustering methods},
	Volume = {11},
	Year = {1987}}

@article{Milligan89,
	Author = {G. W. Milligan},
	Journal = {Multivariate Behavioral Research},
	Pages = {163--176},
	Title = {A study of the beta-flexible clustering method},
	Volume = {24(2)},
	Year = {1989}}

@incollection{Milligan96,
	Address = {River Edge, NJ},
	Author = {G. W. Milligan},
	Booktitle = {Clustering and Classification},
	Editor = {P. Arabie and L. J. Hubert and G. De Soete},
	Pages = {341--375},
	Publisher = {World Scientific Publishing Co.},
	Title = {Clustering validation: {R}esults and implications for applied analyses},
	Year = {1996}}

@article{Morey&Blashfield&Skinnerl83,
	Author = {L. C. Morey, R. K. Blashfield and H. A. Skinner},
	Journal = {Multivariate Behavioral Research},
	Pages = {309--329},
	Title = {A comparison of cluster analysis techniques within a sequential validation framework},
	Volume = {18},
	Year = {1983}}

@book{Morrison90,
	Author = {D. F. Morrison},
	Edition = {3rd},
	Publisher = {McGraw-Hill, NY},
	Title = {Multivariate Statistical Methods},
	Year = {1990}}

@incollection{Murtagh96,
	Address = {River Edge, NJ},
	Author = {F. Murtagh},
	Booktitle = {Clustering and Classification},
	Editor = {P. Arabie and L. J. Hubert and G. De Soete},
	Pages = {235--269},
	Publisher = {World Scientific Publishing Co.},
	Title = {Neural networks for clustering},
	Year = {1996}}

@article{PanelDACC89,
	Author = {{Panel on Discriminant Analysis, Classification, and Clustering}},
	Journal = {Statistical Science},
	Pages = {34--69},
	Title = {Discriminant analysis and clustering},
	Volume = {4},
	Year = {1989}}

@techreport{Pavlic&vanderLaan89,
	Author = {M. Pavlic and M. J. van der Laan},
	Institution = {Division of Biostatistics, U.C. Berkeley},
	Month = {February},
	Number = {89},
	Title = {Fitting of mixtures with unspecified number of components using cross-validation distance estimate},
	Year = {2001}}

@article{Pavlic&vanderLaan02,
	Author = {M. Pavlic and M. J. van der Laan},
	Issue = {3-4},
	Journal = {Computational Statistics and Data Analysis},
	Pages = {413-428},
	Title = {Fitting of mixtures with unspecified number of components using cross validation distance estimate},
	Volume = {41},
	Year = {2003}}

@techreport{Pollard&vanderLaan02,
	Author = {K. S. Pollard and M. J. van der Laan},
	Institution = {Division of Biostatistics, U.C. Berkeley},
	Month = {April},
	Number = {107},
	Title = {A Method to Identify Significant Clusters in Gene Expression Data},
	Year = {2002}}

@techreport{Pollard&vanderLaan02b,
	Author = {K. S. Pollard and M. J. van der Laan},
	Institution = {Division of Biostatistics, U.C. Berkeley},
	Number = {121},
	Title = {Resampling-based methods for identification of significant subsets of genes in expression data},
	Year = {2002}}

@article{Ramsey78,
	Author = {P. H. Ramsey},
	Journal = JASA,
	Pages = {479--485},
	Title = {Power differences between pairwise multiple comparisons},
	Volume = {73},
	Year = {1978}}

@manual{Breiman01b,
	Author = {L. Breiman},
	Title = {Notes on setting up, using, and understanding random forests V3.0},
	Year = {2001}}

@article{Rand71,
	Author = {W. M. Rand},
	Journal = {Journal of the American Statistical Association},
	Optnumber = {336},
	Pages = {846--850},
	Title = {Objective criteria for the evaluation of clustering methods},
	Volume = {66},
	Year = {1971}}

@unpublished{Reiner&Yekutieli&Benjaminil01,
	Author = {A. Reiner and D. Yekutieli and Y. Benjamini},
	Title = {Using resampling-based {FDR} controlling multiple test procedures for analyzing microarray gene expression data},
	Year = {2001}}

@book{Ripley96,
	Address = {Cambridge, New York},
	Author = {B. D. Ripley},
	Publisher = {Cambridge University Press},
	Title = {Pattern recognition and neural networks},
	Year = {1996}}

@book{Rosner99,
	Address = {Pacific Grove, CA},
	Author = {B. Rosner},
	Publisher = {Duxbury Press},
	Title = {Fundamentals of Biostatistics, 5th Ed.},
	Year = {1999}}

@misc{FEVdata,
	Author = {B. Rosner},
	Note = {Submitted by M.J. Kahn, Wheaton College, Norton, MA},
	Optnote = {accessed 12/20/2010},
	Title = {FEV dataset},
	Year = {1999}}

@article{Kahn05,
	Author = {M. Kahn},
	Journal = {The Journal of Statistical Education},
	Number = {2},
	Title = {An Exhalent Problem for Teaching Statistics},
	Volume = {13},
	Year = {2005}}

@article{Rissanen78,
	Author = {J. Rissanen},
	Journal = {Automatica},
	Pages = {465-471},
	Title = {Modelling by shortest data description},
	Volume = {14},
	Year = {1978}}

@article{Rnews:Dudoit&Yang&Bolstad02,
	Author = {S. Dudoit and Y. H. Yang and B. Bolstad},
	Journal = {R News},
	Month = {March},
	Number = 1,
	Pages = {24--32},
	Title = {Using {R} for the Analysis of {DNA} Microarray Data},
	Url = {CRAN.R-project.org/doc/Rnews/},
	Volume = 2,
	Year = 2002,
	Bdsk-Url-1 = {CRAN.R-project.org/doc/Rnews/}}

@article{Robins&Rotnitzky00,
	Author = {J. M. Robins and A. Rotnitzky},
	Journal = {Statistica Sinica},
	Number = {4},
	Pages = {920-936},
	Title = {Comment on the {B}ickel and {K}won article, `{I}nference for Semiparametric Models: {S}ome Questions and an Answer'},
	Volume = {11},
	Year = {2001}}

@inproceedings{Robins00,
	Author = {J.M. Robins},
	Booktitle = {Proceedings of the American Statistical Association},
	Title = {Robust estimation in sequentially ignorable missing data and causal inference models},
	Year = {2000}}

@article{Robins00a,
	Author = {J. M. Robins and A. Rotnitzky},
	Journal = {Statistica Sinica},
	Number = {4},
	Pages = {920-936},
	Title = {Comment on the {B}ickel and {K}won article, `{I}nference for Semiparametric Models: {S}ome Questions and an Answer'},
	Volume = {11},
	Year = {2001}}

@article{Rubin74,
	Author = {D.B. Rubin},
	Journal = {Journal of Educational Psychology},
	Pages = {688-701},
	Title = {Estimating Causal Effects of Treatments in Randomized and Nonrandomized Studies},
	Volume = {64},
	Year = {1974}}

@article{Robins00b,
	Author = {J. M. Robins and A. Rotnitzky and M.J. van der Laan},
	Journal = {Journal of the American Statistical Association -- Theory and Methods},
	Pages = {431-435},
	Title = {Comment on ``{O}n {P}rofile {L}ikelihood" by {S}.{A}. {M}urphy and {A}.{W}. van der {V}aart},
	Volume = {450},
	Year = {2000}}

@article{hernan_brumback_robins,
	Author = {Hernan, M. A. and Brumback, B. and Robins, J. M.},
	Journal = {Epidemiology},
	Number = {5},
	Pages = {561--570},
	Title = {Marginal Structural Models to Estimate the Causal Effect of Zidovudine on the Survival of {HIV}-Positive Men},
	Volume = {11},
	Year = {2000}}

@article{Robins&Rotnitzky&vanderLaan00,
	Author = {J. M. Robins and A. Rotnitzky and M.J. van der Laan},
	Journal = {Journal of the American Statistical Association -- Theory and Methods},
	Pages = {431-435},
	Title = {Comment on ``{O}n {P}rofile {L}ikelihood" by {S}.{A}. {M}urphy and {A}.{W}. van der {V}aart},
	Volume = {450},
	Year = {2000}}

@article{Birge83,
	Author = {L. Birg{\'e}},
	Journal = {Verw. Gebiete},
	Pages = {181--238},
	Title = {Approximation dans les espaces m{/'e}triques et th{\'e}orie de l'estimation},
	Volume = {65},
	Year = {1983}}

@article{lecam73,
	Author = {L.M. le Cam},
	Journal = {The Annals of Statistics},
	Pages = {38--53},
	Title = {Convergence of estimates under dimensionality restrictions},
	Volume = {22},
	Year = {1973}}

@article{Rom90,
	Author = {D. M. Rom},
	Journal = {Biometrika},
	Pages = {663-665},
	Title = {A sequentially rejective test procedure based on a modified {Bonferroni} inequality},
	Volume = {77},
	Year = {1990}}

@techreport{Rosenblatt57,
	Author = {F. Rosenblatt},
	Institution = {Cornell Aeronautical Laboratory},
	Number = {86-460-1},
	Title = {The perceptron -- a perceiving and recognizing automation},
	Year = {1957}}

@article{Ruczinskietal&Kooperberg&LeBlanc01,
	Author = {I. Ruczinski and C. Kooperberg and M. LeBlanc},
	Note = {Submitted, \url{http://biosun01.biostat.jhsph.edu/~iruczins/html/publications.html}},
	Title = {Logic regression},
	Year = {2001}}

@article{Saltstone&Stange96,
	Author = {R. Saltstone and K. Stange},
	Journal = {Journal of Classification},
	Pages = {169--172},
	Title = {A computer program to calculate Hubert and Arabie's adjusted Rand index},
	Volume = {13},
	Year = {1996}}

@techreport{vanderVaart03,
	Author = {A.W. van der Vaart},
	Institution = {Department of Mathematics, Free University, Amsterdam},
	Optannote = {Unpublished manuscript},
	Title = {Notes on Cross-validation},
	Year = {2003}}

@techreport{Sarle83,
	Author = {W. Sarle},
	Institution = {SAS Institute, Inc.},
	Note = {\url{http://www.sas.com/service/library/onlinedoc/trindex.html}},
	Number = {A-108},
	Title = {Cubic clustering criterion},
	Year = {1983}}

@techreport{Sarle&Kuo93,
	Author = {W. Sarle and A. Kuo},
	Institution = {SAS Institute, Inc.},
	Number = {P-256},
	Title = {The MODECLUS Procedures},
	Year = {1993}}

@article{Schapireetal98,
	Author = {R. E. Schapire and Y. Freund and P. Bartlett and W. S. Lee},
	Journal = {The Annals of Statistics},
	Pages = {1651--1686},
	Title = {Boosting the margin: a new explanation for the effectiveness of voting methods},
	Volume = {26},
	Year = {1998}}

@book{Scheffe59,
	Author = {H. Scheff\'{e}},
	Publisher = {John Wiley \& Sons},
	Title = {The analysis of variance},
	Year = {1959}}

@article{Scheibler&Schneider85,
	Author = {D. Scheibler and W. Schneider},
	Journal = {Multivariate Behavioral Research},
	Pages = {283--304},
	Title = {Monte Carlo tests of the accuracy of cluster analysis algorithms: A comparison of hierarchical and nonhierarchical methods},
	Volume = {20},
	Year = {1985}}

@inproceedings{Schuster&Gregory81,
	Author = {E. F. Schuster and C. G. Gregory},
	Booktitle = {Computer Science and Statistics: Proceedings of the 13th Symposium on the interface},
	Editor = {Eddy, W.F.},
	Pages = {295-298},
	Title = {On the non-consistency of maximum likelihood nonparametric density estimators},
	Year = {1981}}

@article{Scott&Factor81,
	Author = {D. W. Scott and L. E. Factor},
	Journal = {Journal of the American Statistical Association},
	Pages = {9-15},
	Title = {Monte Carlo study of three data-based nonparametric density estimators},
	Volume = {76},
	Year = {1981}}

@article{Seeger68,
	Author = {P. Seeger},
	Journal = {Technometrics},
	Number = {3},
	Pages = {586--593},
	Title = {A note on a method for the analysis of significances en masse},
	Volume = {10},
	Year = {1968}}

@article{Segal88,
	Author = {M. R. Segal},
	Journal = {Biometrics},
	Pages = {35--47},
	Title = {Regression trees for censored data},
	Volume = {44},
	Year = {1988}}

@article{Shaffer02,
	Author = {J. P. Shaffer},
	Journal = {Psychological Methods},
	Pages = {356--369},
	Title = {Multiplicity, directional ({T}ype {III}) errors, and the null hypothesis},
	Volume = {7},
	Year = {2002}}

@article{Shaffer86,
	Author = {J. P. Shaffer},
	Journal = JASA,
	Pages = {826--831},
	Title = {Modified sequentially rejective multiple test procedures},
	Volume = {81},
	Year = {1986}}

@article{Shaffer95,
	Author = {J. P. Shaffer},
	Journal = {Annu. Rev. Psychol.},
	Pages = {561--584},
	Title = {Multiple hypothesis testing},
	Volume = {46},
	Year = {1995}}

@article{Shao93,
	Author = {Shao, J.},
	Journal = {Journal of the American Statistical Association},
	Pages = {486-494},
	Title = {Linear Model Selection by Cross-Validation},
	Volume = {88},
	Year = {1993}}

@article{Sidak67,
	Author = {Z. \v{S}id\'{a}k},
	Journal = JASA,
	Pages = {626-633},
	Title = {Rectangular confidence regions for the means of multivariate normal distributions},
	Volume = {62},
	Year = {1967}}

@article{Silverman96,
	Author = {B. W. Silverman},
	Journal = {The Annals of Statistics},
	Pages = {1--24},
	Title = {Smoothed functional principal components analysis by choice of norm},
	Volume = {24},
	Year = {1996}}

@article{Silverman84,
	Author = {B. W. Silverman},
	Journal = JASA,
	Number = {387},
	Pages = {584--589},
	Title = {A fast and efficient cross-validation method for smoothing parameter choice in spline regression},
	Volume = {79},
	Year = {1984}}

@book{Silverman86,
	Author = {B. W. Silverman},
	Publisher = {Chapman \& Hall},
	Title = {Density Estimation for Statistics and Data analysis},
	Year = {1986}}

@article{vanderLaan&Dudoit&Keles04,
	Author = {M.J. van der Laan and S. Dudoit and S. Keles},
	Journal = {Statistical Applications in Genetics and Molecular Biology},
	Optnote = {http://www.bepress.com/sagmb/vol3/iss1/art4},
	Optnumber = {1},
	Title = {Asymptotic optimality of likelihood-based cross-validation},
	Volume = {3},
	Year = {2004}}

@article{Simes86,
	Author = {R. J. Simes},
	Journal = {Biometrika},
	Pages = {751--754},
	Title = {An improved Bonferroni procedure for multiple tests of significance},
	Volume = {73},
	Year = {1986}}

@article{Smyth00,
	Author = {P. Smyth},
	Journal = {Statistics and Computing},
	Pages = {63-72},
	Title = {Model selection of probabilistic clustering using cross-validated likelihood},
	Volume = {10},
	Year = {2000}}

@article{Soric89,
	Author = {B. Sori\'{c}},
	Journal = JASA,
	Number = {406},
	Pages = {608--610},
	Title = {Statistical ``discoveries" and effect-size estimation},
	Volume = {84},
	Year = {1989}}

@article{Stone84,
	Author = {C. J. Stone},
	Journal = {The Annals of Statistics},
	Number = {4},
	Pages = {1285--1297},
	Title = {An asymptotically optimal window selection rule for kernel density estimates},
	Volume = {12},
	Year = {1984}}

@article{Stone74,
	Author = {M. Stone},
	Journal = JRSSB,
	Number = {2},
	Pages = {111--147},
	Title = {Cross-validatory choice and assessment of statistics predictions},
	Volume = {36},
	Year = {1974}}

@article{Stone77,
	Author = {M. Stone},
	Journal = {Biometrika},
	Number = {1},
	Pages = {29--35},
	Title = {Asymptotics for and against cross-validation},
	Volume = {64},
	Year = {1977}}

@techreport{Storey&Tibshirani01,
	Author = {J. D. Storey and R. Tibshirani},
	Institution = {Department of Statistics, Stanford University},
	Number = {2001-28},
	Title = {Estimating false discovery rates under dependence, with applications to DNA microarrays},
	Year = {2001}}

@article{Storey02,
	Author = {J. D. Storey},
	Journal = JRSSB,
	Pages = {479--498},
	Title = {A direct approach to false discovery rates},
	Volume = {64},
	Year = {2002}}

@techreport{Storey01,
	Author = {J. D. Storey},
	Institution = {Department of Statistics, Stanford University},
	Number = {2001-12},
	Title = {The positive False Discovery Rate: A Bayesian interpretation and the q-value},
	Year = {2001}}

@book{Lehmann86,
	Author = {E. L. Lehmann},
	Edition = {2nd},
	Publisher = {Springer-Verlag, New York},
	Title = {Testing Statistical Hypotheses},
	Year = {1986}}

@article{Tibshiranietal02a,
	Author = {R. Tibshirani and T. Hastie and B. Narasimhan and. G. Chu},
	Journal = PNAS,
	Note = {In press},
	Title = {Diagnosis of multiple cancer types by shrunken centroids of gene expression},
	Year = {2002}}

@article{Troendle95,
	Author = {J. F. Troendle},
	Journal = JASA,
	Pages = {370--378},
	Title = {A stepwise resampling method of multiple hypothesis testing},
	Volume = {90},
	Year = {1995}}

@article{Troendle96,
	Author = {J. F. Troendle},
	Journal = {Biometrics},
	Pages = {846--859},
	Title = {A permutational step-up method of testing multiple outcomes},
	Volume = {52},
	Year = {1996}}

@book{vanderVaart&Wellner96,
	Author = {A. W. van der Vaart and J. A. Wellner},
	Pages = {102},
	Publisher = {Springer-Verlag New York},
	Title = {Weak {C}onvergence and {E}mprical {P}rocesses},
	Year = {1996}}

@book{vanderVaart98,
	Author = {A. W. van der Vaart},
	Pages = {62},
	Publisher = {Cambridge University Press},
	Title = {Asymptotic Statistics},
	Year = {1998}}

@book{Vapnik00,
	Address = {New York},
	Author = {V. N. Vapnik},
	Edition = {2nd},
	Publisher = {Springer-Verlag},
	Series = {Statistics for engineering and information science},
	Title = {The nature of statistical learning theory},
	Year = {2000}}

@article{Vapnik79,
	Author = {V. Vapnik},
	Journal = {Nauka, Moskow},
	Title = {Estimation of dependences based on empirical data (in Russian)},
	Year = {1979}}

@book{Vapnik98,
	Address = {New York},
	Author = {V. Vapnik},
	Edition = {1st},
	Publisher = {Wiley},
	Title = {Statistical Learning Theory},
	Year = {1998}}

@book{Venables&Ripley99,
	Author = {W. N. Venables and B. D. Ripley},
	Edition = {3rd},
	Publisher = {Springer-Verlag},
	Title = {Modern applied statistics with S-PLUS},
	Year = {1999}}

@book{Venables&Ripley02,
	Address = {New York},
	Author = {W. N. Venables and B. D. Ripley},
	Edition = {4th},
	Publisher = {Springer-Verlag},
	Title = {Modern Applied Statistics with S},
	Year = {2002}}

@book{Westfall&Young93,
	Author = {P. H. Westfall and S. S. Young},
	Publisher = {John Wiley \& Sons},
	Title = {Resampling-based multiple testing: {E}xamples and methods for $p$-value adjustment},
	Year = {1993}}

@incollection{Westfalletal&Zaykin&Young01,
	Author = {P. H. Westfall and D. V. Zaykin and S. S. Young},
	Booktitle = {Biostatistical Methods},
	Editor = {S. Looney},
	Pages = {143--168},
	Publisher = {Humana Press, Toloway, NJ},
	Series = {Methods in Molecular Biology},
	Title = {Multiple tests for genetic effects in association studies},
	Volume = {184},
	Year = {2001}}

@article{Westonetal2000,
	Author = {J. Weston and S. Mukherjee and O. Chappelle and M. Pontil and T. Poggio and V. Vapnik},
	Journal = {Advances in Neural Processing Systems},
	Pages = {668--674},
	Title = {Feature Selection for {SVM}s},
	Volume = {13},
	Year = {2001}}

@article{Wright92,
	Author = {S. P. Wright},
	Journal = {Biometrics},
	Number = {4},
	Pages = {1005--1013},
	Title = {Adjusted P-values for simultaneous inference},
	Volume = {48},
	Year = {1992}}

@article{Yangetal02,
	Author = {Y. H. Yang and M. J. Buckley and S. Dudoit and T. P. Speed},
	Journal = {Journal of Computational and Graphical Statistics},
	Number = {1},
	Pages = {108--136},
	Title = {Comparison of methods for image analysis on c{DNA} microarray data},
	Volume = {11},
	Year = {2002}}

@article{Yangetal02b,
	Author = {Y. H. Yang and S. Dudoit and P. Luu and D. M. Lin and V. Peng and J. Ngai and T. P. Speed},
	Journal = {Nucleic Acids Research},
	Number = {4},
	Pages = {e15},
	Title = {Normalization for c{DNA} microarray data: {A} robust composite method addressing single and multiple slide systematic variation},
	Volume = {30},
	Year = {2002}}

@inproceedings{Yangetal01,
	Address = {San Jose, CA},
	Author = {Y. H. Yang and S. Dudoit and P. Luu and T. P. Speed},
	Booktitle = {Microarrays: Optical Technologies and Informatics},
	Editor = {Michael L. Bittner and Yidong Chen and Andreas N. Dorsel and Edward R. Dougherty},
	Month = {May},
	Optorganization = {SPIE},
	Pages = {141--152},
	Publisher = {SPIE-International Society for Optical Engineering},
	Series = {Proceedings of SPIE},
	Title = {Normalization for c{DNA} microarray data},
	Volume = {4266},
	Year = {2001}}

@article{Yekutieli&Benjamini99,
	Author = {D. Yekutieli and Y. Benjamini},
	Journal = JSPI,
	Pages = {171--196},
	Title = {Resampling-based false discovery rate controlling multiple test procedures for correlated test statistics},
	Volume = {82},
	Year = {1999}}

@incollection{Youden69,
	Author = {W. J. Youden},
	Booktitle = {Precision measurement and calibration: Statistical concepts and procedures},
	Editor = {H. H. Ku},
	Month = {February},
	Pages = {146--151},
	Publisher = {National Bureau of Standards, United States Department of Commerce},
	Series = {Special Publication 300},
	Title = {Measurement agreement comparisons},
	Type = {NBS Miscelaneous Publication 248, Proceedings of the 1962 Standards Laboratory Conference},
	Volume = {1},
	Year = {1969}}

@article{Zhang93,
	Author = {Zhang, P.},
	Journal = {The Annals of Statistics},
	Pages = {299-313},
	Title = {Model selection via multifold cross-validation},
	Volume = {21},
	Year = {1993}}

@article{Zhang&Carey&Gentleman02,
	Author = {J. Zhang and V. Carey and R. Gentleman},
	Journal = {Bioinformatics},
	Note = {(In press)},
	Title = {An extensible application for assembling annotation for genomic data},
	Url = {http://www.R-project.org/},
	Year = {2002},
	Bdsk-Url-1 = {http://www.R-project.org/}}

@article{Gradyetal09,
	Author = {D. Grady and J. Macer and M. Kristof and H. Shen and M. Tagliaferri and J. Creasman},
	Issue = {5},
	Journal = {Menopause},
	Pages = {932-6},
	Title = {Is a shorter hot flash diary just as good as a 7-day diary?},
	Volume = {16},
	Year = {2009}}

@book{Bickeletal97,
	Author = {P.J. Bickel and C.A.J. Klaassen and Y. Ritov and J. Wellner},
	Publisher = {Springer-Verlag},
	Title = {Efficient and Adaptive Estimation for Semiparametric Models},
	Year = {1997}}

@book{vanderLaan&Robins03,
	Author = {M.J. van der Laan and J.M. Robins},
	Publisher = {Springer-Verlag, New York},
	Title = {Unified Methods for Censored Longitudinal Data and Causality},
	Year = {2003}}

@manual{effsize,
	Author = {{National Reading Panel}},
	Organization = {National Institute of Child Health and Human Development, National Institutes of Health},
	Title = {Teaching Children to Read},
	Year = {1999}}

@techreport{Tibshirani&Walther&Hastie00,
	Author = {R. Tibshirani and G. Walther and T. Hastie.},
	Institution = {Department of Biostatistics, Stanford University},
	Month = {March},
	Note = {\url{http://www-stat.stanford.edu/~tibs/research.html}},
	Title = {Estimating the number of clusters in a dataset via the gap statistic},
	Year = {2000}}

@inproceedings{Gill&vanderLaan&Robins97,
	Address = {New York},
	Author = {R.D. Gill and M.J. van der Laan and J.M. Robins},
	Booktitle = {Proceedings of the First Seattle Symposium in Biostatistics},
	Editor = {D.Y. Lin and T.R. Fleming},
	Pages = {255-94},
	Publisher = {Springer-Verlag},
	Title = {Coarsening At Random: Characterizations, Conjectures and Counter-Examples},
	Year = {1997}}

@article{Gill&Robins01,
	Author = {Gill, R. and Robins, J.M.},
	Fjournal = {The Annals of Statistics},
	Journal = {Ann. Stat.},
	Number = {6},
	Title = {Causal inference in complex longitudinal studies: continuous case},
	Volume = {29},
	Year = {2001}}

@article{Jacobsen&Keiding95,
	Author = {M. Jacobsen and N. Keiding},
	Journal = {The Annals of Statistics},
	Pages = {774-86},
	Title = {Coarsening at Random in General Sample Spaces and Random Censoring in Continuous Time},
	Volume = {23},
	Year = {1995}}

@misc{Dudoit&Yang02,
	Author = {S. Dudoit and Y. H. Yang},
	Howpublished = {{\tt R} packages},
	Title = {Normalization and diagnostic plots for cDNA microarray data, {\tt marrayClasses}, {\tt marrayInput}, {\tt marrayNorm}, {\tt marrayPlots}},
	Url = {www.bioconductor.org},
	Year = {2002},
	Bdsk-Url-1 = {www.bioconductor.org}}

@techreport{Fraley&Raftery98b,
	Author = {C. Fraley and A. E. Raftery},
	Date-Modified = {2011-02-22 20:11:02 -0800},
	Institution = {Department of Statistics, University of Washington},
	Month = {November},
	Number = {342},
	Title = {MCLUST: Software for Model-Based Cluster Analysis},
	Year = {1998}}

@misc{Ge&Dudoit02b,
	Author = {Y. Ge and S. Dudoit},
	Date-Modified = {2011-02-22 20:11:23 -0800},
	Howpublished = {{\tt R} package},
	Title = {Multiple Testing Procedures, {\tt multtest}},
	Url = {www.bioconductor.org},
	Year = {2002},
	Bdsk-Url-1 = {www.bioconductor.org}}

@article{Robins&Rotnitzky95,
	Author = {J.M. Robins and A. Rotnitzky},
	Journal = {Journal of the American Statistical Association},
	Month = {March},
	Number = {429},
	Pages = {122-9},
	Title = {Semiparametric Efficiency in Multivariate Regression Models with Missing Data},
	Volume = {90},
	Year = {1995}}


@inproceedings{Robins93,
	Author = {J.M. Robins},
	Booktitle = {Proceeding of the Biopharmaceutical section},
	Organization = {American Statistical Association},
	Pages = {24-33},
	Title = {Information recovery and bias adjustment in proportional hazards regression analysis of randomized trials using surrogate markers},
	Year = {1993}}

@incollection{Robins&Rotnitzky92,
	Author = {J.M. Robins and A. Rotnitzky},
	Booktitle = {AIDS Epidemiology},
	Publisher = {Bikh\"{a}user},
	Series = {Methodological issues},
	Title = {Recovery of information and adjustment for dependent censoring using surrogate markers},
	Year = {1992}}

@article{Robins&Rotnitzky&Zhao94,
	Author = {J.M. Robins and A. Rotnitzky and L.P. Zhao},
	Journal = {Journal of the American Statistical Association},
	Month = {September},
	Number = {427},
	Pages = {846-66},
	Title = {Estimation of regression coefficients when some regressors are not always observed},
	Volume = {89},
	Year = {1994}}

@article{Hubbard&vanderLaan08,
	Author = {A.E. Hubbard and M.J. van der Laan},
	Journal = {Biometrika},
	Number = {1},
	Pages = {35-47},
	Title = {Population intervention models in causal inference},
	Volume = {95},
	Year = {2008}}

@article{Heitjan&Rubin91,
	Author = {D.F. Heitjan and D.B. Rubin},
	Journal = {The Annals of Statistics},
	Month = {December},
	Number = {4},
	Pages = {2244-2253},
	Title = {Ignorability and Coarse Data},
	Volume = {19},
	Year = {1991}}

@misc{Dudoit&Yang&Bolstad01,
	Author = {S. Dudoit and Y. H. Yang and B. M. Bolstad},
	Howpublished = {{\tt R} package},
	Note = {Contributions from Natalie Thorne, Ingrid L\"{o}nnstedt, and Jessica Mar},
	Title = {Statistical {M}icroarray {A}nalysis, {\tt sma}},
	Url = {cran.r-project.org/src/contrib/PACKAGES.html\#sma},
	Year = {2001},
	Bdsk-Url-1 = {cran.r-project.org/src/contrib/PACKAGES.html%5C#sma}}

@phdthesis{Dudoit99,
	Author = {S. Dudoit},
	School = {Department of Statistics, University of California, Berkeley},
	Title = {Linkage analysis of complex human traits using identity by descent data},
	Type = {Ph.D. thesis},
	Year = {1999}}

@article{Rosenblum&vanderLaan10,
	Author = {M. Rosenblum and M.J. van der Laan},
	Journal = {The International Journal of Biostatistics},
	Number = {19},
	Title = {Targeted Maximum Likelihood Estimation of the Parameter of a Marginal Structural Model},
	Volume = {6},
	Year = {2010}}

@article{Gruber&vanderLaan10a,
	Author = {S. Gruber and M.J. van der Laan},
	Issue = {26},
	Journal = {The International Journal of Biostatistics},
	Number = {1},
	Title = {A Targeted Maximum Likelihood Estimator of a Causal Effect on a Bounded Continuous Outcome},
	Volume = {6},
	Year = {2010}}

@article{Gruber&vanderLaan10b,
	Author = {S. Gruber and M.J. van der Laan},
	Issue = {18},
	Journal = {The International Journal of Biostatistics},
	Number = {1},
	Title = {An Application of Collaborative Targeted Maximum Likelihood Estimation in Causal Inference and Genomics},
	Volume = {6},
	Year = {2010}}

@unpublished{bhattacharya.vogt.zbias,
	Author = {Bhattacharya, J. and Vogt, W},
	Note = {NBER Technical Working Paper 343, National Bureau of Economic Research, MA.},
	Title = {Do Instrumental Variables Belong in Propensity Scores?},
	Year = {2007}}

@unpublished{wooldridge.zbias,
	Author = {Wooldridge, J.},
	Note = {Tech.\ Rep.\ Michigan State University, MI.},
	Title = {Should Instrumental Variables be Used as Matching Variables?},
	Year = {2009}}

@article{pearl.zbias,
	Author = {Pearl, Judea},
	Journal = {Proceedings of UAI},
	Note = {forthcoming},
	Title = {On a Class of Bias-Amplifying Variables that Endanger Effect Estimates},
	Year = {2010}}

@unpublished{Bhattacharya&Vogt07,
	Author = {Bhattacharya, J. and Vogt, W},
	Note = {NBER Technical Working Paper 343, National Bureau of Economic Research, MA.},
	Title = {Do Instrumental Variables Belong in Propensity Scores?},
	Year = {2007}}

@unpublished{Wooldridge09,
	Author = {Wooldridge, J.},
	Note = {Tech.\ Rep.\ Michigan State University, MI.},
	Title = {Should Instrumental Variables be Used as Matching Variables?},
	Year = {2009}}

@article{Bang&Robins05,
	Author = {Bang, H. and J. M. Robins},
	Journal = {Biometrics},
	Pages = {962-72},
	Title = {Doubly Robust Estimation in Missing Data and Causal Inference Models},
	Volume = {61},
	Year = {2005}}

@article{Pearl10,
	Author = {Pearl, J.},
	Journal = {Proceedings of UAI},
	Note = {forthcoming},
	Title = {On a Class of Bias-Amplifying Variables that Endanger Effect Estimates},
	Year = {{2010}}}

@article{Scharfstein&Rotnitzky&Robins99,
	Author = {Scharfstein, D.O. and Rotnitzky, A. and Robins, J.M.},
	Journal = {Journal of the American Statistical Association},
	Number = {448},
	Pages = {1096-1120 (1121-1146)},
	Title = {Adjusting for Non-Ignorable Drop-out Using Semiparametric Nonresponse Models, (with Discussion and Rejoinder)},
	Volume = {94},
	Year = {{1999}}}

@article{Scharfstein99,
	Author = {Scharfstein, D.O. and Rotnitzky, A. and Robins, J.M.},
	Journal = {Journal of the American Statistical Association},
	Number = {448},
	Pages = {1096-1120 (1121-1146)},
	Title = {Adjusting for Non-Ignorable Drop-out Using Semiparametric Nonresponse Models, (with Discussion and Rejoinder)},
	Volume = {94},
	Year = {{1999}}}

@article{Robins1999,
	Author = {Robins, J.M.},
	Journal = {Statistics in Medicine},
	Number = {21},
	Pages = {1663-1680},
	Title = {Commentary on Using Inverse Weighting and Predictive Inference to Estimate the Effecs of Time-Varying Treatments on the Discrete-time Hazard},
	Year = {{1999}}}

@techreport{Wang06,
	Author = {Y. Wang and M. Petersen and D. Bangsberg and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {211},
	Optnote = {http://www.bepress.com/ucbbiostat/paper211},
	Opturl = {www.bepress.com/ucbbiostat/paper211/},
	Title = {Diagnosing Bias in the Inverse Probability of Treatment Weighted Estimator Resulting from Violation of Experimental Treatment Assignment.},
	Year = {2006}}

@techreport{Moore09,
	Author = {K.L. Moore and R.S. Neugebauer and M.J. van der Laan and I.B. Tager},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {255},
	Optmonth = {Oct},
	Title = {Causal Inference in Epidemiological Studies with Strong Confounding},
	Url = {www.bepress.com/ucbbiostat/paper255/},
	Year = {2009},
	Bdsk-Url-1 = {www.bepress.com/ucbbiostat/paper255/}}

@article{Cole&Hernan08,
	Author = {S.R. Cole and M.A. Hernan},
	Journal = {American Journal of Epidemiology},
	Pages = {656-664},
	Title = {Constructing Inverse Probability Weights for Marginal Structural Models},
	Volume = {168},
	Year = {2008}}

@article{Kish92,
	Author = {L. Kish},
	Journal = {Journal of Official Statistics},
	Pages = {183--200},
	Title = {Weighting for unequal {P}$_i$},
	Volume = {8},
	Year = {1992}}

@techreport{Bembom.trunc,
	Author = {O. Bembom and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {230},
	Title = {Data-adaptive selection of the truncation level for Inverse-Probability-of-Treatment-Weighted estimators},
	Url = {www.bepress.com/ucbbiostat/paper230/},
	Year = {2008},
	Bdsk-Url-1 = {www.bepress.com/ucbbiostat/paper230/}}

@article{Ridgeway&McCaffrey07,
	Author = {G. Ridgeway and D.F. McCaffrey},
	Journal = {Statistical Science},
	Pages = {540-443},
	Title = {Comment: Demystifying Double Robustness: A Comparison of Alternative Strategies for Estimating a Population Mean from Incomplete Data},
	Volume = {22:4},
	Year = {2007}}

@article{Robinsetal1994b,
	Author = {J.M. Robins, A. Rotnitzky and L.P. Zhao},
	Journal = {J. Am. Statist. Assoc.},
	Pages = {846-66},
	Title = {Estimation of Regression Coefficients When Some Regressors are Not Always Observed},
	Volume = {89},
	Year = {1994}}

@article{Tan10,
	Author = {Z. Tan},
	Date-Modified = {2011-03-07 21:06:22 -0800},
	Journal = {Biometrika},
	Pages = {661-682},
	Title = {Bounded, efficient and doubly robust estimation with inverse weighting},
	Volume = {97,3},
	Year = {2010}}

@article{Tan06,
	Author = {Z. Tan},
	Date-Modified = {2011-03-07 21:06:16 -0800},
	Journal = {J. Am. Statist. Assoc.},
	Pages = {1619-37},
	Title = {A distributional approach for causal inference using propensity scores},
	Volume = {101},
	Year = {2006}}

@article{Cao&Tsiatis&Davidian09,
	Author = {W. Cao and A.A. Tsiatis and M. Davidian},
	Date-Modified = {2011-03-07 21:06:41 -0800},
	Journal = {Biometrika},
	Pages = {723-734},
	Title = {Improving efficiency and robustness of the doubly robust estimator for a population mean with incomplete data},
	Volume = {96,3},
	Year = {2009}}

@misc{Gruber&vanderLaanWNAR11,
	Author = {S. Gruber and M.J. van der Laan},
	Date-Added = {2011-12-08},
	Date-Modified = {2011-12-08},
	Howpublished = {WNAR 2011 Spring Meeting},
	Month = {June},
	Title = {Collaborative Targeted Maximum Likelihood Estimation},
	Year = {2011}}

@misc{Rotnitzky11,
	Author = {A. Rotnitzky},
	Date-Added = {2011-04-02 21:38:04 -0700},
	Date-Modified = {2011-04-02 21:41:08 -0700},
	Howpublished = {ENAR 2011 Spring Meeting},
	Month = {March},
	Title = {Enhanced Double-Robust Locally- Efficient Estimation in Regression Models for Longitudinal Studies},
	Year = {2011}}

@article{Gruber&vanderLaan12Outperforms,
	Author = {S. Gruber and M.J. van der Laan},
	Date-Modified = {2011-12-13 12:08:39 -0500},
	Journal = {The International Journal of Biostatistics},
	Volume = {8},
	Issue = {1},
	Title = {Targeted minimum loss based estimator that outperforms a given estimator},
	Year = {2012}}

@article{Wedderburn74,
	Author = {R.W.M. Wedderburn},
	Date-Modified = {2011-03-07 21:46:06 -0800},
	Issue = {3},
	Journal = {Biometrika},
	Title = {Quasi-likelihood functions, generalized linear models, and the {G}auss-{N}ewton method},
	Volume = {61},
	Year = {1974}}

@article{Robins&Wang2000,
	Author = {J.M. Robins and N. Wang},
	Journal = {Biometrika},
	Pages = {113-124},
	Title = {Inference for imputation estimators},
	Volume = {87},
	Year = {2000}}

@article{Petersen&Schwab&vanderLaan13,
  title={Targeted maximum likelihood estimation of dynamic and static marginal Structural Working Models},
  author={M. Petersen and J. Schwab and S. Gruber and N. Blaser and M. Schomaker and M.J. van der Laan},
  journal={Journal of Causal Inference},
  volume={2},
  Issue={2},
  pages={147--185},
  year={2013}
  note={DOI: https://doi.org/10.1515/jci-2013-0007},
  }









@article{Sobel06,
  title={What Do Randomized Studies of Housing Mobility Demonstrate? Causal Inference in the Face of Interference},
  author={M. Sobel},
  journal={Journal of the American Statistical Association},
  volume={101},
  pages={1398--1407},
  year={2006}
  }

@techreport{vanderLaan&Gruber11TR,
	Author = {M.J. van der Laan and S. Gruber},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper290},
	Title = {Targeted Maximum Loss Based Estimation of an Intervention Specific Mean},
	Type = {Technical Report 290},
	Year = {2011}}
@article{Raudenbush&Bryk86,
  author = {S.W. Raudenbush and A.S. Bryk},
  title= {A hierarchical model
for studying school effects. Sociology of Education},
  journal = {Sociology of Education},
  volume = {59},
  issue = {},
  pages = {1--17},
  year = {1986}
}

@techreport{vanderLaan08,
	Author = {Mark J. van der Laan},
	Date-Added = {2008-03},
	Institution = {University of California, Berkeley},
	Number = {232, www.bepress.com/ucbbiostat/paper232},
	Title = {The Construction and Analysis of Adaptive Group Sequential Designs},
	Year = {2008}}

@book{Raudenbush&Bryk02,
author={S.W. Raudenbush and A.S. Bryk},
title={Hierarchical linear models: Application and data analysis methods},
publisher={Newbury
Park: Sage.},
year={2002}
}



@book{vanderLaan96,
author={M.J. van der Laan},
title={Efficient and Inefficient Estimation in Semiparametric Models},
publisher={Center for Mathematics and Computer Science, CWI-tract 114},
year={1996}
}

@article{Raudenbush&Liu00,
author={ S.W. Raudenbush and X. Liu},
titlte={Statistical power and
optimal design for multisite randomized trials},
journal={Psychological
Methods},
volume={5},
pages={199Ð213},
year={2000}
}


 @article{Raudenbush&Sampson99a,
 author={S.W. Raudenbush and  R.J. Sampson},
  title={Assessing direct
and indirect effects in multilevel designs with latent
variables},
  journal={Sociological Methods \& Research},
  volume={28},
  pages={123Ð153},
  year={1999}
   }

  @inCollection{Raudenbush&Sampson99b,
 author={S.W. Raudenbush and  R.J. Sampson},
title={Ecometrics: Toward a science of assessing ecological settings, with
application to the systematic social observation of neighbor-
hoods. In M. P. Becker (Ed.)},
 booktitle={Sociological methodology},
OPTvolume={29},
 pages={1Ð41},
 publisher={Boston, MA: Blackwell},
 year={1999}
 }

 @article{Raudenbush&Whillms95,
 author={S.W. Raudenbush and J.D. Whillms},
 title={The estimation of
school effects},
 journal={Journal of Educational and Behavioral
Statistics},
 volume={20},
 pages={307Ð335},
 year={1995}
 }

@article{Coleman58,
author={J.S. Coleman},
title={Relational analysis: The study of social
organizations with survey methods},
journal={Human Organization},
volume={17},
pages={28Ð36},
year={1958}
}

@article{Colemanetal66,
author={J.S.
Coleman and E.Q. Campbell and C.J. Hobson and J. McPartland and
A.M. Mood and F.D. Weinfeld and R.L. York},
title={Equality of educational opportunity. Washington, DC:
Government Printing OfÞce},
journal={Journal of the Royal Statistical Society, Series A},
volume={156},
pages={9Ð38},
year={1966}
}


@article{Aitkin&Longford86,
author={M. Aitkin and N. Longford},
title={Statistical modeling issues
in school effectiveness studies},
journal={Journal of the Royal
Statistical Society, Series A},
volume={149},
pages={1Ð43},
year={1986}
}

@book{Rubin06,
author={D.B. Rubin},
title={Matched Sampling for Causal Effects.},
publisher={Cambridge University Press},
address={Cambridge, MA},
year={2006},
}

@book{Goldstein95,
author={H. Goldstein},
title={Multilevel statistical models},
publisher={London:
Edward Arnold},
year={1995}
}

@article{McMichael99,
author={A.J. McMichael},
title={Prisoners of the proximate: Loosening
the constraints on epidemiology in an age of change},
journal={American Journal of Epidemiology},
volume={149},
pages={887Ð897},
year={1999}
}

@article{Susser99,
author={M. Susser},
title={Should the epidemiologist be a social
scientist or a molecular biologist?},
journal={International Journal of
Epidemiology},
volume={28},
pages={1019Ð1022},
year={1999}
}

@article{Berkmanetal00,
author={L.F. Berkman and T. Glass and I. Brissette and T.E. Seeman},
title={From social integration to health: Durkheim
in the new millennium},
journal={Social Science \& Medicine},
volume={51},
pages={843Ð857},
year={2000}
}

@article{Krieger01,
author={N. Krieger},
title={Theories for social epidemiology in the 21st
century: An ecosocial perspective},
journal={International Journal of
Epidemiology},
volume={30},
pages={668Ð677},
year={2001}
}

@book{Parsons51,
author={T. Parsons},
title={The social system},
publisher={New York: Free Press},
year={1951}
}

@book{Starr82,
author={P. Starr},
title={The social transformation of American medicine},
publisher={New York: Basic Books},
year={1982}
}

@article{Rose85,
author={G. Rose},
title={Sick individuals and sick populations},
journal={International Journal of Epidemiology},
volume={14},
pages={32Ð38},
year={1985}
}

@article{Clarketal91,
author={J. Clark and D.A. Potter and J.B. McKinlay},
title={Bringing
social structure back into clinical decision making},
journal={Social
Science \& Medicine},
volume={32},
pages={853Ð866},
year={1991}
}

@article{Barr95,
author={D.A. Barr},
title={The effects of organizational structure on
primary care outcomes under managed care},
journal={Annals of
Internal Medicine},
volume={122},
pages={353Ð359},
year={1995}
}


@article{McKinlay96,
author={J.B. McKinlay},
title={Some contributions from the social
system to gender inequalities in heart disease},
journal={Journal of
Health and Social Behavior},
volume={37},
pages={1Ð26},
year={1996}
}



@article{Feldmanetal97,
author={H.A. Feldman and J. B. McKinlay and D.A. Potter and K.M. Freund and
R.B. Burns and M.A. Moskowitz and L.E. Kasten},
title={Nonmedical inßuences on medical decision making: An
experimental technique using videotapes, factorial
design, and survey sampling},
journal={Health Services Research},
volume={32},
pages={343Ð366},
year={1997}
}

@article{Hook01,
author={E.B. Hook},
title={(Letter to Editor) RE: Neighborhood social
environment and risk of death: Multilevel evidence from the
Alameda County Study},
journal={American Journal of Epidemiology},
volume={151},
pages={1132Ð1133},
year={2001}
}

@article{Draper95,
author={D. Draper},
title={Inference and hierarchical modeling in the
social sciences},
journal={Journal of Educational and Behavioral
Statistics},
volume={20},
pages={115Ð147},
year={1995}
}

@article{Lindley&Smith72,
author={D. Lindley and A. Smith},
title={Bayes estimation for linear
models},
journal={Journal of the Royal Statistical Society, Series B},
volume={34},
pages={1Ð41},
year={1972}
}


@article{Dempsteretal77,
author={A.P. Dempster and N.M. Laird and D.B. Rubin},
title={Maximum
likelihood from incomplete data via the EM algorithm},
journal={Journal of the Royal Statistical Society, Series B},
volume={39},
pages={1Ð8},
year={1977}
}

@article{Laird&Ware82,
author={
N.M. Laird and J.H. Ware},
title={Random-effects models for
longitudinal data},
journal={Biometrics},
volume={38},
pages={963Ð974},
year={1982}
}


@inCollection{Masonetal84,
author={W.M. Mason and G.Y. Wong and B. Entwisle},
title={Contextual
analysis through the multilevel Linear Model. In S.
Leinhardt (Ed.)},
booktitle={Sociological methodology: 1983Ð1984},
publisher={San
Francisco: Jossey-Bass},
year={1984}
}




@book{Goldstein87,
author={H. Goldstein},
title={Multilevel statistical models in educational
and social research},
publisher={London: Edward Arnold},
year={1987}
}



@book{Bryk&Raudenbush92,
author={A.S. Bryk and S.W. Raudenbush},
title= {Hierarchical linear
models},
publisher={Newbury Park: Sage},
year={1992}
}


@book{Verbeke&Molenbergs97,
author={G. Verbeke and G. Molenbergs},
title={Linear mixed models in practice: A SAS oriented approach},
publisher={New York: Springer},
year={1997}
}



@article{Singer98,
author={J.D. Singer},
title={Using SAS proc mixed to Þt multilevel
models, hierarchical models, and individual growth models},
journal={Journal of Educational and Behavioral Statistics},
volume={24},
pages={323Ð355},
year={1998}
}


@article{Kreftetal94,
author={I.G.G. Kreft and J. de Leeuw and R. van der Leeden},
title={Review of Þve multilevel analysis programs: BMDP-5,
GENMOD, HLM, ML3, VARCL. },
journal={American Statistician},
volume={48},
pages={324Ð335},
year={1994}
}

@inCollection{Deleeuw&Kreft01,
author={J. De Leeuw and I.G.G. Kreft},
title={Software for multilevel
analysis},
booktitle={In H. Goldstein (Ed.), Multilevel modelling of
health statistics},
pages={187Ð204},
publisher={New York: Wiley},
year={2001}
}


@book{Susser73,
author={M. Susser},
title={Causal thinking in health sciences: Concepts
and strategies of epidemiology},
publisher={New York: Oxford},
year={1973}
}

@inCollection{Freedman91,
author={D. Freedman},
title={Statistical models and shoe leather (with
discussion). In P. V. Marsden (Ed.)},
booktitle={Sociological methodol-
ogy},
OPTvol={21},
publisher={San Francisco: Jossey-Banks},
year={1991}
}

@article{Freedman97,
author={D. Freedman},
title={From association to causation via
regression (with comments). In S. P. Turner (Ed.)},
booktitle={Causality in crisis? Statistical methods and the search for causal
knowledge in the social sciences},
OPTpages={113Ð182},
publisher={Notre Dame,
IN: Notre Dame University Press},
year={1997}
}


@article{Greenland90,
author={S. Greenland},
title={Randomization, statistics, and causal
inference},
journal={Epidemiology},
volume={1},
pages={421Ð429},
year={1990}
}


@article{Greenland96,
author={S. Greenland},
title={Basic methods for sensitivity analysis of
biases},
journal={International Journal of Epidemiology},
volume={25},
pages={1107Ð1116},
year={1996}
}

@article{Greenland00,
author={S. Greenland},
title={Principles of multilevel modelling},
journal={International Journal of Epidemiology},
volume={29},
pages={158Ð167},
year={2000}
}

@article{Greenland01,
author={S. Greenland},
title={Ecologic versus individual-level sources of
bias in ecologic estimates of contextual health effects},
journal={International Journal of Epidemiology},
volume={30},
pages={1343Ð1350},
year={2001}
}

@article{Greenland02,
author={S. Greenland},
title={A review of multilevel theory for
ecological analyses},
journal={Statistics in Medicine},
volume={21},
pages={389Ð395},
year={2002}
}

@article{Greenland&Morgenstern01,
author={S. Greenland and H. Morgenstern},
title={Confounding in
health research},
journal={Annual Review of Public Health},
volume={22},
pages={189Ð212},
year={2001}
}

@article{Greenlandetal99,
author={S. Greenland and J. Pearl and J.M. Robins},
title= {Causal
diagrams for epidemiologic research},
journal={Epidemiology},
volume={10},
pages={37Ð48},
year={1999}
}


@article{Manski93,
author={C.F. Manski},
title={IdentiÞcation of endogenous social
effects: The reßection problem},
journal={Review of Economic Studies},
volume={60},
pages={531Ð542},
year={1993}
}


@inCollection{Manski93b,
author={C.F. Manski},
title={IdentiÞcation problems in the social
sciences. In P. V. Marsden (Ed.)},
booktitle={Sociological methodology},
publisher={San Francisco: Jossey-Banks},
year={1993}
}


@article{Halloran&Struchiner95,
author={M.E. Halloran and C.J. Struchiner},
title={Causal inference in
infectious diseases},
journal={Epidemiology},
volume={6},
pages={142Ð151},
year={1995}
}

@article{Morgenstern95,
author={H. Morgenstern},
title={Ecologic studies in epidemiology:
Concepts, principles, and methods},
journal={Annual Review of Public
Health},
volume={16},
pages={61Ð81},
year={1995}
}

@inCollection{Sobel95,
author={M.E.Sobel},
title={Causal inference in the social and
behavioral sciences},
booktitle={In M. E. Sobel (Ed.), Handbook of
statistical modeling for the social and behavioral sciences},
pages={1Ð38},
publisher={New York: Plenum.},
year={1995}
}


@article{Kaufman&Cooper99,
author={J.S. Kaufman and R.S. Cooper},
title={Seeking causal
explanations in social epidemiology},
journal={American Journal of
Epidemiology},
volume={150},
pages={113Ð120},
year={1995}
}

@article{Kaufman&Poole00,
author={J.S. Kaufman and C. Poole},
title={Looking back on causal
thinking in the health sciences},
journal={Annual Review of Public
Health},
volume={21},
pages={101Ð119},
year={2000}
}

@article{Kaufman&Kaufman01,
author={J. S. Kaufman and S. Kaufman},
title={Assessment of
structured socioeconomic effects on health},
journal={Epidemiology},
volume={12},
pages={157Ð167},
year={2001}
}

@article{Robins01,
author={J.M. Robins},
title={Data, design, and background knowledge
in etiologic inference},
journal={Epidemiology},
volume={12},
pages={313Ð320},
year={2001}
}


@article{Maldonado&Greenland02,
author={G. Maldonado and S. Greenland},
title={Estimating causal effects},
journal={International Journal of Epidemiology},
volume={31},
pages={422Ð438},
year={2002}
}

@book{Campbell&Stanley63,
author={D.T. Campbell and J.C. Stanley},
title={Experimental and
quasi-experimental designs for research},
publisher={Hopewell, NJ:
Houghton Mifßin},
year={1963}
}

@article{Cochran65,
author={W.G. Cochran},
title={The planning of observational studies
of human populations},
journal={Journal of the Royal Statistical
Society, Series A},
volume={128},
pages={243Ð265},
year={1965}
}

@article{McKinlay75,
author={S.M. McKinlay},
title={The design and analysis of the
observational studyÑa review},
journal={Journal of the American
Statistical Association},
volume={70},
pages={503Ð523},
year={1975}
}

@article{Heckman79,
author={J.J. Heckman},
title={Sample selection bias as a speciÞcation
error},
journal={Econometrica},
volume={47},
pages={153Ð162},
year={1979}
}


@article{Leamer83,
author={E. Leamer},
title={LetÕs take the con out of econometrics},
journal={American Economic Review},
volume={73},
pages={32Ð43},
year={1983}
}

@inCollection{Smith90,
author={H.L. Smith},
title={SpeciÞcation problems in experimental and
nonexperimental social research},
booktitle={In C. C. Clogg (Ed.), Sociological methodology},
volume={20},
publisher={Oxford: Basil},
year={1990}
}

@article{Rubin91,
author={D.B. Rubin},
title={Practical implications of modes of
statistical inference for causal effects and the critical role
of the assignment mechanism},
journal={Biometrics},
volume={47},
pages={1213Ð1234},
year={1991}
}

@inCollection{Clogg&Haritou97,
author={C.C. Clogg and A. Haritou},
title={The regression method for causal inference and a dilemma confronting this method},
booktitle={In S. P. Turner (Ed.), Causality in crisis? Statistical methods
and the search for causal knowledge in the social sciences},
pages={83Ð112},
publisher={Notre Dame, IN: Notre Dame University Press},
year={1997}
}

@article{Copas&Li97,
author={J.B. Copas and H.G. Li},
title={Inference for non-random
samples (with discussion)},
journal={Journal of the Royal Statistical
Society, Series B},
volume={59},
pages={55Ð95},
year={1997}
}

@inCollection{Freedman97,
author={D. Freedman},
title={From association to causation via
regression (with comments)},
booktitle={In S. P. Turner (Ed.), Causality
in crisis? Statistical methods and the search for causal
knowledge in the social sciences},
pages={113Ð182},
publisher={Notre Dame,
IN: Notre Dame University Press},
year={1997}
}

@article{Winship&Morgan99,
author={C. Winship and S.L.  Morgan},
title={The estimation of causal
effects from observational data},
journal={Annual Review of Sociology},
volume={25},
pages={659Ð707},
year={1999}
}

@book{Pearl00,
author={J. Pearl},
title={Causality: Models, reasoning, and inference},
publisher={ New York: Cambridge University Press},
year={2000}
}

@book{Rosenbaum02,
author={P.R. Rosenbaum},
title={Observational studies},
publisher={New York:
Springer},
year={2002}
}


@article{Charltonetal85,
author={J.R. Charlton and M.F. DÕSouza and M. Tooley and R. Silver},
title={A community trial strategy for evaluating treatment
for symptomatic conditions},
journal={Statistics in Medicine},
volume={4},
pages={11Ð21},
year={1985}
}

@article{Meyeretal91,
author={L. Meyer and N. Job-Spira and J. Bouyer and E. Bouvet and A. Spira},
title={Prevention of sexually transmitted diseases: A
randomised community trial},
journal={Journal of Epidemiology and
Community Health},
volume={45},
pages={152Ð158},
year={1991}
}


@article{Shipleyetal95,
author={R.H. Shipley and T.D. Hartwell and W.D. Austin and A.C. Clayton and L.C. Stanley },
title={Community stop-smoking contests
in the COMMIT trial: Relationship of participation to
costs},
journal={Community intervention trials. Preventive Medicine},
volume={ 24},
pages={286Ð292},
year={1995}
}

@article{Holderetal97,
author={H.D. Holder and R.F. Saltz and A.J. Treno and J.W. Grube and R.B. Voas},
title={Evaluation design for a community prevention
trial. An environmental approach to reduce alcohol-
involved trauma},
journal={Evaluation Review},
volume={21},
pages={140Ð165},
year={1997}
}

@article{Feldmanetal98,
author={H.A. Feldman and M.A. Proschan and D.M. Murray and D.C. Goff and M.
Stylianou and E. Dulberg and P.G. McGovern and W. Chan and N.C.
Mann and V. Bittner},
title={Statistical design of
REACT (Rapid Early Action for Coronary Treatment), a
multisite community trial with continual data collection},
journal={Controlled Clinicial Trials},
volume={19},
pages={391Ð403},
year={1998}
}

@article{LeFortetal98,
author={S.M. LeFort and K. Gray-Donald and K.M. Rowat and M.E. Jeans},
title={Randomized controlled trial of a community-based
psychoeducation program for the self-management of
chronic pain},
journal={Pain},
volume={74},
pages={297Ð306},
year={1998}
}


@article{Perskyetal99,
author={V. Persky and L. Coover and E. Hernandez and A. Contreras and J. Slezak and J. Piorkowski and L. Curtis and M. Turyk and V. Ramakrishnan and  P. Scheff},
title={Chicago community-based asthma
intervention trial: Feasibility of delivering peer education in
an inner-city population},
journal={Chest},
volume={116},
pages={216SÐ223S},
year={1999}
}

@article{Biglanetal00,
author={A. Biglan and K. Smolkowski and T. Duncan and C. Black},
title={A randomised controlled trial of a community
intervention to prevent adolescent tobacco use},
journal={Tobacco
Control},
volume={9},
pages={24Ð32},
year={2000}
}


@article{Luepkeretal00,
author={R.V. Luepker and J.M. Raczynski and S. Osganian and R.J Goldberg and
Jr. J.R.  Finnegan and J.R. Hedges and Jr. D.C. Goff and M.S.
Eisenberg and J.G. Zapka and H.A. Feldman and D.R. Labarthe and P.G. McGovern and C.E. Cornell and M.A. Proschan and D.G. Simons-Morton},
title={Effect of a community
intervention on patient delay and emergency medical service
use in acute coronary heart disease: The rapid early action
for coronary treatment (REACT) trial},
journal={JAMA},
volume={284},
pages={60Ð67},
year={2000}
}


@Article{Oakes04,
  author = {J.M. Oakes},
  title= {The (mis)estimation of neigborhood effects: causal inference for a practicable social epidemiology },
  journal = {Social Science and Medicine},
  volume = {58},
  issue = {},
  pages = {1929--1952},
  year = {2004}
}

@Article{Abadie&Imbens06,
  author = {A. Abadie and G.W. Imbens},
  title= {Large Sample Properties of Matching Estimators for Average Treatment Effects},
  journal = {Econometrica},
  volume = {74},
  issue = {1},
  pages = {235-67},
  year = {2006}
}

@Article{Greenland&Morgenstern90,
  author = {S. Greenland and H. Morgenstern},
  title= {Matching and Efficiency in Cohort Studies},
  journal = {American Journal of Epidemiology},
  volume = {131},
  issue = {1},
  pages = {151-159},
  year = {1990}
}

@Article{Costanza95,
  author = {M. Costanza},
  title= {Theoretical Epidemiology, Matching},
  journal = {Preventive Medicine},
  volume = {24},
  issue = {},
  pages = {425-433},
  year = {1995}
}

@Article{Joffe&Rosenbaum99,
  author = {M.M. Joffe and P.R. Rosenbaum},
  title= {Invited Commentary: Propensity Scores},
  journal = {American Journal of Epidemiology},
  volume = {150},
  issue = {4},
  pages = {327-333},
  year = {1999}
}


@article{Neugebauer&vanderLaan07,
author={R. Neugebauer, M. J. van der Laan},
title={ Nonparametric Causal E?ects based on
marginal structural models},
journal={Journal of Statistical Planning and Inference},
year={2007},
volume={137},
pages={419Ð434},
}




@article{Murphy05,
author={S. Murphy},
title={An experimental design for the development of adaptive treatment strategies},
journal={Statistics in Medicine},
year={2005},
volume={24},
pages={1455Ð1481},
}

@article{Lavori&Dawson00,
author={P. Lavori and R. Dawson},
title={A design for testing clinical strategies: biased adaptive within-subject
randomization},
journal={Journal of the Royal Statistical Society, Series A},
volume={163},
pages={29Ð38},
year={2000},
}

@article{Lavori&Dawson04,
author={P. Lavori  and R. Dawson},
title={Dynamic treatment regimes: practical design considerations},
journal={Clinical trials},
volume={1},
pages={9Ð20},
year={2004},
}

@article{Thalletal00,
author={P. Thall and R. Millikan and H.-G. Sung},
title={Evaluating multiple treatment courses in clinical trials},
journal={Statistics in Medicine},
volume={19},
pages={1011Ð1028},
year={2000},
}

@article{Rushetal03,
author={A.J. Rush and M. Trivedi and M. Fava},
title={Depression},
journal={IV. American Journal of Psychiatry},
volume={160(2)},
pages={237},
year={2003},
}

@article{Schneideretal06,
author={Schneider, L. and Tariot.P.N. and Dagerman, K. and Davis, S. and Hsiao, J. and Ismail, S. and Lebowitz, B. and Lyketsos, C. and Ryan
J. and Stroup T. and Sultzer D. and Weintraub, D. and Lieberman, J.},
title= {E?ectiveness of atypical antipsychotic
drugs in patients with AlzheimerÕs disease},
journal={New England Journal of Medicine},
volume={355(15)},
pages={1525Ð1538},
year={2006},
}

@article{Swartzetal07,
author={Swartz, M. and Perkins, D. and Stroup, T. and Davis, S. and Capuano, G. and Rosenheck, R. and Reimherr, F. and McGee, M. and Keefe,
R. and McEvoy, J. and Hsiao, J. and Lieberman, J.},
title={Effects of antipsychotic medications on psychosocial
functioning in patients with chronic shizophrenia: Findings from the nimh catie study},
year={2007},
journal={American Journal
of Psychiatry},
volume={164},
pages={428Ð436},
}

@article{Rubin&vanderLaan08,
author={D.B. Rubin and M.J. van der Laan},
title={Empirical Efficiency Maximization: Improved Locally Efficient Covariate Adjustment in Randomized Experiments and Survival Analysis},
year={2008},
journal={The International Journal of Biostatistics},
volume={Vol. 4, Iss. 1, Article 5},
location={http://www.bepress.com/ijb/vol4/iss1/5},
}


@article{vanderLaan&Rose&Gruber09,
author={M.J. van der Laan and S. Rose and S. Gruber},
title={Readings on Targeted Maximum Likelihood Estimation},
year={September, 2009},
journal={Technical report, working paper series http://www.bepress.com/ucbbiostat/paper254/},
}

@article{Bembometal09,
author={O. Bembom and M.J. van der Laan and T. Haight and I.B. Tager},
title={Lifetime and
current leisure time physical activity and all-cause mortality in an elderly cohort},
year={2009},
journal={Epidemiology},
volume={},
pages={},
}

@article{Bembom&vanderLaan07a,
author={Oliver Bembom and Mark van der Laan},
title={Statistical Methods for analyzing sequentially randomized trials, commentary on JNCI article Adaptive therapy for androgen independent prostate cancer: A Randomized selection trial including four regimens, by Peter F. Thall, C. Logothetis, C. Pagliaro, S. Wen, M.A. Brown, D. Williams, R. Millikan (2007). },
journal={Journal of the National Cancer Institute},
year={2007},
volume={99(21)},
pages={1577-1582},
 }

@article{Rosenblumetal09,
author={M. Rosenblum and S.G. Deeks and M.J. van der Laan and D.R. Bangsberg},
title={The Risk
of Virologic Failure Decreases with Duration of HIV Suppression, at Greater
than 50\% Adherence to Antiretroviral Therapy},
year={2009},
journal={PLoS ONE},
volume={4(9): e7196.doi:10.1371/journal.pone.0007196},
}



@article{Robinsetal08,
author={J. Robins and L. Orallana and A. Rotnitzky},
title={Estimaton and extrapolation of optimal treatment and  testing strategies},
journal={Statistics in Medicine},
year={2008},
volume={27(23)},
pages={ 4678-4721},
}


@article{Bembom&vanderLaan07,
author= {O. Bembom and M.J. van der Laan},
title={A practical illustration of the importance of realistic individualized treatment rules in causal inference},
journal={Electronic Journal of Statistics},
year={2007},
pages={http://www.i-journals.org/ejs/viewarticle.php?id=105&layout=abstract},
}

@article{Bembometal08,
author={O. Bembom and M.L. Petersen and S.-Y. Rhee and W. J. Fessel and S.E. Sinisi and R.W. Shafer and M.J. van der Laan},
title ={Biomarker discovery using targeted maximum likelihood estimation: Application to the treatment of antiretroviral resistant HIV infection},
journal={Statistics in Medicine},
year={2008},
pages={http://www3.interscience.wiley.com/journal/121422393/abstract},
}

@article{Cassel76,
author={J. Cassel},
title={The contribution of the social environment to host resistance},
journal={American Journal of Epidemiology},
volume={104},
pages={107--123},
year={1976}
}

@article{Tuglus&vanderLaan08,
author={C. Tuglus and M.J. van der Laan},
title={Targeted Methods for Biomarker Discovery, the Search for a Standard},
journal={UC Berkeley Working Paper Series},
year={2008},
pages={http://www.bepress.com/ucbbiostat/paper233/.},
}

@article{vanderLaan08,
author={M.J. van der Laan},
title={Estimation Based on Case-Control Designs with Known Prevalance Probability},
journal={The International Journal of Biostatistics},
year={2008},
volume={http://www.bepress.com/ijb/vol4/iss1/17/},
}

@article{Rose&vanderLaan08,
author={S. Rose and M.J. van der Laan},
title={Simple Optimal Weighting of Cases and Controls in Case-Control Studies},
journal={The International Journal of Biostatistics},
year={2008},
pages={http://www.bepress.com/ijb/vol4/iss1/19/.},
}

@article{Rose&vanderLaan09,
author={S. Rose and M.J. van der Laan},
title={Why Match? Investigating Matched Case-Control Study Designs with Causal Effect Estimation},
journal={The International Journal of Biostatistics},
year={2009},
pages={http://www.bepress.com/ijb/vol5/iss1/1/.},
}


@inproceedings{Moore&vanderLaan09,
author={K.L. Moore and M.J. van der Laan},
title={Application of Time-to-Event Methods in the Assessment of Safety in Clinical Trials},
booktitle={in Design, Summarization, Analysis \& Interpretation of Clinical Trials with Time-to-Event Endpoints},
year={2009},
editor={Karl E. Peace},
publisher={Chapman and Hall},
}

@inproceedings{Polley&vanderLaan09,
author={E.C. Polley and M.J. van der Laan},
title={Predicting Optimal Treatment Assignment Based on Prognostic Factors in Cancer Patients},
booktitle={in Design, Summarization, Analysis \& Interpretation of Clinical Trials with Time-to-Event Endpoints},
year={2009},
editor={Karl E. Peace},
publisher={Chapman and Hall},
}


@article{vanderVaart&Dudoit&vanderLaan06,
  author =       {A.W. van der Vaart and S. Dudoit and M.J. van der Laan},
  title =        {Oracle Inequalities for Multi-Fold Cross-Validation},
   journal = {Statistics and Decisions},
   volume={24},
 number={3},
 year={2006},
 pages={351--371},
}

@article{vanderLaan&Dudoit&vanderVaart06,
  author =       {M.J. van der Laan and S. Dudoit and A.W. van der Vaart},
  title =        {The Cross-Validated Adaptive Epsilon-Net Estimator},
   journal = {Statistics and Decisions},
   volume={24},
 number={3},
 year={2006},
 pages={373--395},
}

 @article{Rosenbaum&Rubin83,
 author={P.R. Rosenbaum and D.B. Rubin},
 title={The Central Role of the Propensity Score in Observational Studies for Causal Effects},
 journal={Biometrika},
 volume={70},
 year={1983},
 pages={41-55}
 }

@article{vanderLaan&Polley&Hubbard07,
 author = {M.J. van der Laan and E. Polley and A. Hubbard},
 title = {Super Learner},
 journal = {Statistical Applications in Genetics and Molecular Biology},
 volume = {6},
 number ={25},
 year = {2007},
 issn = {1},
 location={http://www.bepress.con/sagmb/vol6/iss1/art25},
 }

 @article{Sekhon08,
 author={J.S. Sekhon},
 title= {Multivariate and Propensity Score Matching
 Software with Automated Balance Optimization: The Matching package for {R}},
 journal = {Journal of Statistical Sotware, Forthcoming},
 publisher={SSRN},
location = {http://ssrn.com/paper=1009044},
year={2008}
}

@article{Bembom&Fessel&Shafer&vanderLaan08,
	location = {http://www.scientificcommons.org/36721107},
	title = {Data-adaptive Selection Of The Adjustment Set In Variable Importance Estimation},
	author = {O. Bembom and J.W. Fessel and R.W. Shafer  and M.J. van der Laan},
	year = {2008},
	keywords = {General Biostatistics},
	publisher = {The Berkeley Electronic Press},
	url = {http://www.bepress.com/ucbbiostat/paper231},
	institution = {DigitalCommons@Florida Atlantic University [http://digitalcommons.fau.edu/cgi/oai2.cgi] (United States)},
}

@article{Holland77,
 author = {J.H. Holland and J.S. Reitman},
 title = {Cognitive systems based on adaptive algorithms},
 journal = {SIGART Bull.},
 volume = {63},
 year = {1977},
 issn = {0163-5719},
 pages = {49--49},
 doi = {http://doi.acm.org/10.1145/1045343.1045373},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

@book{Rubin06,
author={D.B. Rubin},
title={Matched Sampling for Causal Effects.},
publisher={Cambridge University Press},
address={Cambridge, MA},
year={2006},
}

@incollection{Mans81,
author={C.F. Manski and D. McFadden},
title={Alternative estimators and sample designs for discrete choice analysis},
booktitle={Structural Analysis of Discrete Data with Econometric Applications},
publisher={The MIT Press},
address={Cambridge, MA},
year={1981},
editor={C.F. Manski and D. McFadden},
}

@article{Mans77,
author={C.F. Manski and S.R. Lerman},
title={The Estimation of Choice Probabilities from Choice Based Samples},
journal={Econometrica},
volume={45},
number={8},
pages={1977-1988},
year={1977},
}

@article{Coss81,
author={S.R. Cosslett},
title={Maximum Likelihood Estimator for Choice-Based Samples},
journal={Econometrica},
volume={49},
number={5},
pages={1289-1316},
year={1981},
}


@article{Corn51,
author={J. Cornfield},
title={A method of estimating comparative rates from clinical data.  Applications to cancer of the lung, breast, and cervix.},
journal={J Nat Cancer Inst},
volume={11},
pages={1269-1275},
year={1951},
}

@inproceedings{Corn56,
author={J. Cornfield},
title={A statistical problem arising from retrospective studies},
booktitle={Proceedings of the Third Berkeley Symposium, Volume IV},
year={1956},
editor={J. Neyman},
pages={133-148},
publisher={University of California Press},
}

@article{Beni94,
author={J. Benichou and S. Wacholder},
title={A comparison of three approaches to estimate exposure-specific incidence rates from population-based case-control data.},
journal={Statistics in Medicine},
volume={13},
pages={651-661},
year={1994},
}
@article{Breslow&Robins&Wellner00,
author={N.E. Breslow and J.M. Robins and J.A. Wellner},
title={On the semi-parametric efficiency of logistic regression under case-control sampling},
journal={Bernoulli},
volume={6(3)},
pages={447--455},
year={2000},
}
@article{Mansonetal07,
author = {R. Mansson, M.M. Joffe, W. Sun, S. Hennessy},
title = {On the Estimation and Use of Propensity Scores in Case-Control and Case-Cohort Studies.},
journal = {Am J Epidemiol},
volume = {166},
number = {3},
pages = {332-339},
year = {2007},
}

@article{And79,
author={J.A. Anderson},
title={Separate sample logistic discrimination},
journal={Biometrika},
volume={59},
pages={19--35},
year={1972},
}

@article{Prentice&Pike79,
author={R.L. Prentice and R. Pyke},
title={Logistic disease incidence models and case-control studies},
journal={Biometrika},
volume={66},
pages={403--411},
year={1979},
}

@article{Breslow96,
author={N.E. Breslow},
title={Statistics in Epidemiology: the Case-Control Study},
journal={J Am Stat Soc},
volume={91},
pages={14--28},
year={1996},
}

@book{Breslow&Day80,
author={N.E. Breslow and N.E. Day},
title={Statistical Methods in Cancer Research:  Volume 1 -- The analysis of case-control studies},
publisher={International Agency for Research on Cancer},
address={Lyon},
year={1980},
}

@article{Holfordetal78,
author={T.R. Holford and C. White and J.L. Kelsey},
title={Multivariate Analysis for Matched Case-Control Studies},
journal={Am J Epid},
volume={107},
number={3},
pages={245--255},
year={1978},
}

@article{Breslowetal78,
author={N.E. Breslow and N.E. Day and K.T. Halvorsen and R.L. Prentice and C. Sabal},
title={Estimation of Multiple Relative Risk Functions in Matched Case-Control Studies},
journal={Am J Epid},
volume={108},
number={4},
pages={299--307},
year={1978},
}

@book{Schlesselman82,
author={J.J. Schlesselman},
title={Case-Control Studies:  Design, Conduct, Analysis},
publisher={Oxford University Press},
address={Oxford},
year={1982},
}

@book{Collett91,
author={D. Collett},
title={Modeling Binary Data},
publisher={Chapman and Hall},
address={London},
year={1991},
}

@book{Jewell04,
author={N.P. Jewell},
title={Statistics for Epidemiology},
publisher={Chapman and Hall/CRC},
address={Boca Raton},
year={2004},
}

@book{Hosmer&Lemeshow00,
author={D.W. Hosmer and S. Lemeshow},
title={Applied Logistic Regression},
edition={2nd},
publisher={John Wiley and Sons},
address={New York},
year={2000},
}

@article{Robins99,
author={J.M. Robins},
title={[Choice as an Alternative to Control in Observational Studies]:  Comment},
journal={Statistical Science},
volume={14},
number={3},
pages={281--293},
year={1999},
}

@article{Newman06,
author={S. Newman},
title={Causal Analysis of Case-Control Data},
journal={Epid Persp Innov},
volume={3},
pages={2},
url={http://www.epi-perspectives.com/content/3/1/2},
year={2006},
}

@article{Zele86,
author={M. Zelen and R.A. Parker},
title={Case-Control Studies and Bayesian Inference},
journal={Stat Med},
volume={5},
number={3},
pages={261--269},
year={1986},
}

@article{Sinh04,
author={S. SInha and B. Mukherjee and M Ghosh},
title={Bayesian Semiparametric Modeling for Matched Case-Control Studies with Multiple Disease States},
journal={Biometrics},
volume={60},
pages={41--49},
year={2004},
}

@article{Ritc01,
author = {M.D. Ritchie and L.W. Hahn and N. Roodi and L.R. Bailey and W.D. Dupont and F.F. Parl and J.H. Moore},
title = {Multifactor-dimensionality reduction reveals high-order interactions among estrogen-metabolism genes in sporadic breast cancer.},
journal = {Am J Hum Genet},
volume = {69},
number = {1},
pages = {138--47},
year = {2001},
}

@article{Mei07,
author = {H. Mei and M.L. Cuccaro and E.R. Martin},
title = {Multifactor dimensionality reduction-phenomics: a novel method to capture genetic heterogeneity with use of phenotypic variables.},
journal = {Am J Hum Genet},
volume = {81},
number = {6},
pages = {1251-61},
year = {2007},
}




@article{
Bangsberg04,
   Author = {D.R. Bangsberg and A.R. Moss and S.G. Deeks},
   Title = {Paradoxes of adherence and drug resistance to {HIV} antiretroviral therapy},
   Journal = {J Antimicrob Chemother},
   Volume = {53},
   Number = {5},
   Pages = {696-9},
   Note = {0305-7453 (Print)
Journal Article
Review},
   Abstract = {Public health debates about providing HIV antiretroviral therapy to impoverished populations have centred on the relationship between adherence and risk of drug resistance. Recent data indicate that each antiretroviral therapeutic class has a unique adherence-resistance relationship. Resistance to single protease inhibitor therapy occurs most frequently at moderate to high levels of adherence, resistance to non-nucleoside reverse transcriptase inhibitor therapy occurs at low to moderate levels of adherence, and resistance to ritonavir-boosted protease inhibitor therapy is most likely to occur at middle ranges of adherence. These dynamic relationships should be considered in balancing the individual and public health benefits of therapy.},
 Keywords = {Anti-HIV Agents/*therapeutic use
Developing Countries
*Drug Resistance, Viral
Humans
*Patient Compliance
Public Health
Research Support, Non-U.S. Gov't
Research Support, U.S. Gov't, P.H.S.},
   Year = {2004} }


@Article{Scharfstein&Tsiatis&Robins97,
  author =   {D.O. Scharfstein and A.A. Tsiatis and J.M. Robins},
  title =    {Semiparametric efficiency and its implications on the design and analysis of group-sequential studies},
journal =      {Journal of the American Statistical Association},
  year =     {1997},
  OPTkey =   {},
  volume =   {92},
  number =   {440},
  pages =    {1342--1350},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Bembom&Petersen07,
   author={O. Bembom and M. Petersen and SY Rhee and W.J. Fessel and S.E. Sinisi and R.W. Shafer 	     and M.J. van der Laan},
   title={Biomarker Discovery Using Targeted Maximum Likelihood Estimation: Application to the  Treatment of Antiretroviral Resistant {HIV} Infection},
   journal= {U.C. Berkeley Division of Biostatistics Working Paper Series},
   year={2007},
  volume={221},
   OPTmonth={August},
  OPTnote={http://www.bepress.com/ucbbiostat/paper221}
}

@Article{vanderLaan&Gruber09,
  author=  {M.J. van der Laan and S. Gruber},
  title={Collaborative Double robust penalized targeted maximum likelihood estimation},
  journal={The International Journal of Biostatistics},
  year={2010},
  volume={},
 }
@Article{Gruber&vanderLaan09,
  author=  {S. Gruber and M.J. van der Laan},
  title={An application of collaborative targeted maximum likelihood estimation in causal inference and genomics},
  journal={The International Journal of Biostatistics},
  year={2010},
  volume={},
 }
@Article{vanderLaan&Rubin06,
  author =   {M.J. van der Laan and D. Rubin},
  title =    {Targeted Maximum Likelihood Learning},
journal =      {The International Journal of Biostatistics},
  year =     {2006},
  OPTkey =   {},
  volume =   {2},
  number =   {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/ijb/vol2/iss1/11},
  OPTannote =    {}
}


@Article{Scharfstein&Tsiatis98,
  author =   {D.O. Scharfstein and A.A. Tsiatis},
  title =    {The use of simulation and bootstrap in information based group sequential studies},
journal =      {Statistics in Medicine},
  year =     {1998},
  OPTkey =   {},
  volume =   {17},
  number =   {},
  pages =    {75--87},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Pampallona&Tsiatis&Kim01,
  author =   {S. Pampallona and A.A. Tsiatis and K. Kim},
  title =    {Interim monitoring of group sequential trials using spending functions for the type I and type II error probabilities},
journal =      {Drug Informational Journal},
  year =     {2001},
  OPTkey =   {},
  volume =   {35},
  number =   {},
  pages =    {1113-1121},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Tsiatis&Mehta03,
  author =   {A.A. Tsiatis and C. Mehta},
  title =    {On the inefficiency of the adaptive design for monitoring clinical trials},
journal =      {Biometrika},
  year =     {2003},
  OPTkey =   {},
  volume =   {90},
  number =   {},
  pages =    {367-378},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Banerjee&Tsiatis06,
  author =   {A. Banerjee and A.A. Tsiatis},
  title =    {Adaptive two-stage designs in phase II clinical trials},
journal =      {Statistics in Medicine},
  year =     {2006},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {In press},
  OPTannote =    {}
}
@Article{Tsiatis06,
  author =   {A.A. Tsiatis},
  title =    {Information based monitoring of clinical trials},
journal =      {Statistics in Medicine},
  year =     {2006},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {In press},
  OPTannote =    {}
}

@Article{Lokhnygina&Tsiatis06,
  author =   {Y. Lokhnygina and A.A. Tsiatis},
  title =    {Optimal two-stage group sequential designs},
journal =      {Journal of Statistical Planning and Inference},
  year =     {2006},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {},
  OPTnote =      {In press},
  OPTannote =    {}
}

  @Article{Bauer&Kohne94,
  author =   {P. Bauer and Kohne},
  title =    {Evaluation of experiments with adaptive interim analysis},
journal =      {Biometrics},
  year =     {1994},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {1029--1041},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Cui&Hung&Wang99,
  author =   {L. Cui and H.M.J. Wang and S-J Wang},
  title =    {Modification of sample size in group sequential trials},
journal =      {Biometrics},
  year =     {1999},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {853--857},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Jennison&Turnbull03,
  author =   {C. Jennison and B.W. Turnbull},
  title =    {Mid course sample size modification in clinical trials based on hte observed treatment effect},
journal =      {Statistics in Medicine},
  year =     {2003},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {971--993},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Koyama&Sampson&Gleser04,
  author =   {T. Koyama and A.R. Sampson and L.J. Gleser},
  title =    {A calculus for design of two stage adaptive procedures},
journal =      {Journal of the Americal Statistical Association},
  year =     {2004},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Lan&Trost97,
  author =   {K.K.G Lan and D.C. Trost},
  title =    {Estimation of parameters and sample size re-estimation},
journal =      {Proceedings Biopharm Section},
  year =     {1997},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {48-51},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Li&Shih&Xie&Lu02,
  author =   {G. Li and W.J. Shih and T. Xie and J. Lu},
  title =    {A sample size adjustment procedure for clinical trials based on conditional power},
journal =      {Biostatistics},
  year =     {2002},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {277--287},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Mehta&Tsiatis01,
  author =   {C.R. Mehta and A.A. Tsiatis},
  title =    {Flexible sample size considerations using information based interim monitoring},
journal =      {Drug Informational Journal},
  year =     {2001},
  OPTkey =   {},
  volume =   {35},
  number =   {},
  pages =    {1095--1112},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Mulle&Shafer01,
  author =   {H.H. Mulle and H. Shafer},
  title =    {Adaptive group sequential designs for clinical trials: combining the advantages of adaptive and classical group sequential approaches},
journal =      {Biometrics},
  year =     {2001},
  OPTkey =   {},
  volume =   {57},
  number =   {},
  pages =    {886--891},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Proschan&Hunsberger95,
  author =   {M.A. Proschan and S.A. Hunsberger},
  title =    {Designed extension studies based on conditional power},
journal =      {Biometrics},
  year =     {1995},
  OPTkey =   {},
  volume =   {51},
  number =   {},
  pages =    {1315--1324},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Shen&Fisher99,
  author =   {Y. Shen and L.D. Fisher},
  title =    {Statistical Inference for self-designing clinical trials with a one-sided hypothesis},
journal =      {Biometrics},
  year =     {1999},
  OPTkey =   {},
  volume =   {55},
  number =   {},
  pages =    {190--197},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Wittes&Brittain90,
  author =   {J. Wittes and E. Brittain},
  title =    {The role of internal pilot studies in increasing efficiency of clinical trials},
journal =      {Statistics in Medicine},
  year =     {1999},
  OPTkey =   {},
  volume =   {9},
  number =   {},
  pages =    {65--72},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Shen&Cheng06,
  author =   {Y. Shen and Y. Cheng},
  title =    {Adaptive design: Estimation and Inference with censored data in a semiparametric model},
journal =      {Biostatistics},
  year =     {2006},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {In Press},
  OPTannote =    {}
}

%next reference for adaptive allocation of treatments

@Book{Spiegelalteretal04,
  author =       {D.J. Spiegelalter and K.R. Abrams and J.P. Myles},
  title =        {Bayesian approaches to clinical trials and health care evaluation},
  publisher =    {Wiley, Chichester},
  year =         {2004}
}
@Book{Berry&Stangl96,
  author =       {D.A. Berry and D.K. Stangl},
  title =        {Bayesian biostatistics},
  publisher =    {Marcel Dekker, New York},
  year =         {1996}
}


@Article{Berry06,
  author =   {D.A. Berry},
  title =    {Bayesian clinical trials},
journal =      {Nature Reviews, Drug Discovery},
  year =     {2006},
  OPTkey =   {},
  volume =   {5},
  number =   {},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

%D. A. Berry, Bayesian clinical trials, Nature Reviews, Drug
%Recovery, vol 5, january 2006.


@Book{Hu&Rosenberger06,
  author =       {F. Hu and W.F. Rosenberger},
  title =        {The theory of response adaptive randomization in clinical trials},
  publisher =    {New York Wiley},
  year =         {2006}
}

@Book{Dudoit&vanderLaan08,
  author =       {S. Dudoit and M.J. van der Laan},
  title =        {Resampling based multiple testing with applications to genomics},
  publisher =    {Springer Series of Statistics, New York},
  year =         {2008}
}

@Book{Sen&Singer93,
  author =       {P.K. Sen and J.M. Singer},
  title =        {Large Sample Methods in Statistics: An Introduction with Applications},
  publisher =    {Chapman \& Hall, New York},
  year =         {1993}
}


@Article{Bai&Hu&Rosenberger02,
  author =   {Z.D. Bai and F. Hu and W.F. Rosenberger},
  title =    {Asymptotic properties of adaptive designs for clinical trials with delayed response},
journal =      {Annals of Statistics},
  year =     {2002},
  OPTkey =   {},
  volume =   {30},
  number =   {1},
  pages =    {122--139},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Andersen&Faries&Tamura94,
  author =   {J. Andersen and D. Faries and R. Tamura},
  title =    {A randomized play-the-winner design for multiarm clinical trials},
journal =      {Communication in Statistical Theory},
  year =     {1994},
  OPTkey =   {},
  volume =   {23},
  number =   {},
  pages =    {309--323},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Flournoy&Rosenberger95,
  author =       {N. Flournoy and W.F. Rosenberger},
  title =        {Adaptive Designs},
  publisher =    {Hayward, Institute of Mathematical Statistics},
  year =         {1995}
}

@Article{Hu&Rosenberger00,
  author =   {F. Hu and W.F. Rosenberger},
  title =    {Analysis of time trends in adaptive designs withi appliation to a neurophysiology experiment},
journal =      {Statistics in Medicine},
  year =     {2000},
  OPTkey =   {},
  volume =   {19},
  number =   {},
  pages =    {2067--2075},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Rosenberger96,
  author =   {W.F. Rosenberger},
  title =    {New directions in adaptive designs},
journal =      {Statistical Science},
  year =     {1996},
  OPTkey =   {},
  volume =   {11},
  number =   {},
  pages =    {137--149},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Rosenberger&Flournoy&Durham97,
  author =   {W.F. Rosenberger and N. Flournoy and S.D. Durham},
  title =    {Asymptotic normality of maximum likelihood estimators
  from multiparameter response driven designs},
journal =      {Journal of Statistical Planning and Inference},
  year =     {1997},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {69--76},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Rosenberger&Grill97,
  author =   {W.F. Rosenberger and S.E. Grill},
  title =    {A sequential design for psychophysical experiments: An application to estimating timing of sensory events},
journal =      {Statistics in Medicine},
  year =     {1997},
  OPTkey =   {},
  volume =   {16},
  number =   {},
  pages =    {2245--2260},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Rosenberger&Sriram97,
  author =   {W.F. Rosenberger and T.N. Shiram},
  title =    {Estimation for an adaptive allocation design},
journal =      {Journal of Statistical Planning and Inference},
  year =     {1997},
  OPTkey =   {},
  volume =   {59},
  number =   {},
  pages =    {309--319},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Tamura&Faries&Andersen&Heiligenstein94,
  author =   {R.N. Tamura and D.E. Faries and J.S. Andersen and J.H. Heiligenstein},
  title =    {A case study of an adaptive clinical trial in the treatment of out-patients with depressive disorder},
journal =      {Journal of the American Statistical Association},
  year =     {1994},
  OPTkey =   {},
  volume =   {89},
  number =   {},
  pages =    {768--776},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Wei&Durham78,
  author =   {L.J. Wei and S. Durham},
  title =    {The randomize play-the-winner rule in medical trials},
journal =      {Journal of the American Statistical Association},
  year =     {1978},
  OPTkey =   {},
  volume =   {73},
  number =   {},
  pages =    {840--843},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Wei&Smythe&Lin&Park90,
  author =   {L.J. Wei and R.T. Smythe and D.Y. Lin and T.S. Park},
  title =    {Statistical Inference with data-dependent treatment allocation rules},
journal =      {Journal of the American Statistical Association},
  year =     {1990},
  OPTkey =   {},
  volume =   {85},
  number =   {},
  pages =    {156--162},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Zelen69,
  author =   {M. Zelen},
  title =    {Play the winner rule and the controlled clinical trial},
journal =      {Journal of the American Statistical Association},
  year =     {1969},
  OPTkey =   {},
  volume =   {64},
  number =   {},
  pages =    {131--146},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Cheng&Shen05,
  author =   {Y. Cheng and Y. Shen},
  title =    {Bayesian adaptive designs for clinical trials},
journal =      {Biometrika},
  year =     {2005},
  OPTkey =   {},
  volume =   {92},
  number =   {3},
  pages =    {633--646},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Wei79,
  author =   {L.J. Wei},
  title =    {The generalized Polya's urn design for sequential medical trials},
journal =      {Annals of Statistics},
  year =     {1979},
  OPTkey =   {},
  volume =   {7},
  number =   {},
  pages =    {291--296},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}








@article{
Benito03,
   Author = {Benito, J. M. and Lopez, M. and Soriano, V.},
   Title = {Virus load and cytolitic responses in human immunodeficiency virus infection: what is cause and what is effect},
   Journal = {J Infect Dis},
   Volume = {188},
   Number = {5},
   Pages = {794-5; author reply 795-6},
   Note = {0022-1899
Comment
Letter},
 Keywords = {ADP-ribosyl Cyclase/metabolism
Anti-HIV Agents/therapeutic use
Antigens, CD/metabolism
CD4-Positive T-Lymphocytes/*immunology
CD8-Positive T-Lymphocytes/immunology
HIV Infections/drug therapy/*immunology/virology
HIV-1/*physiology
Human
*Viral Load
Virus Replication},
   Year = {2003} }



@article{
DEttorre02,
   Author = {D'Ettorre, G. and Forcina, G. and Andreotti, M. and Sarmati, L. and Palmisano, L. and Galluzzo, C. M. and Nicastri, E. and Mastroianni, C. M. and Vullo, V. and Vella, S. and Andreoni, M.},
   Title = {Discordant response to antiretroviral therapy: {HIV} isolation, genotypic mutations, T-cell proliferation and cytokine production},
   Journal = {Aids},
   Volume = {16},
   Number = {14},
   Pages = {1877-85},
   Note = {0269-9370
Journal Article},
   Abstract = {OBJECTIVE: To study virologic and immunologic factors associated with discordant treatment response in HIV-infected patients receiving highly active antiretroviral therapy (HAART). DESIGN: Study participants included a total of 27 patients: (a) 10 discordant patients (mean CD4+ cell count, 396.1 x 10 cells/l; mean HIV-RNA, 5.4 log copies/ml); (b) seven responder patients (mean CD4+ cell count, 997.5 x 10 cells/l); and (c) 10 failing patients (mean CD4+ cell count 66.5 x 10 cells/l; mean HIV-RNA, 5.4 log copies/ml).(10) (10)METHODS: The HIV-1 isolation rate and biological phenotype, drug resistance genotypic mutations of HIV-1 strains, recall and HIV-1-specific antigen lymphocyte proliferation (LP), and interleukin (IL)-15 production were studied. RESULTS: Virus isolation was obtained in 30% of discordant patients, and in 100% of failing patients. A higher replication constant was reported in discordant patients. No difference in the number of drug resistance mutations and biological phenotypes of HIV-1 was found in discordant patients with respect to failing patients. Discordant patients developed positive LP responses to and HIV-1 p24. LP in response to, HIV-1 p24 and gp160 was positive in responder patients. No significant LP was found in failing patients. Increased levels of IL-15 after stimulation with lipopolysaccaride (LPS) and were found in both discordant patients and responder patients. Conversely, a strong reduction of IL-15 levels was observed in failing patients. CONCLUSION: The present results suggest that decreased virus isolation rate, restoration of both lymphocyte proliferation and IL-15 production are factors involved in the discordant antiretroviral therapy response of HIV-infected patients.},
 Keywords = {Adult
Anti-HIV Agents/*therapeutic use
Antiretroviral Therapy, Highly Active
CD4 Lymphocyte Count
CD8-Positive T-Lymphocytes/drug effects/immunology
Candida albicans
Drug Resistance, Viral
Female
HIV Infections/complications/*drug therapy/immunology/virology
HIV-1/drug effects/genetics/*immunology/isolation & purification
Human
Interleukin-15/*blood
Male
Middle Aged
Mutation
Viral Load
Virus Replication/drug effects},
   Year = {2002} }



@article{
Davenport02,
   Author = {Davenport, M. P. and Zaunders, J. J. and Hazenberg, M. D. and Schuitemaker, H. and van Rij, R. P.},
   Title = {Cell turnover and cell tropism in HIV-1 infection},
   Journal = {Trends Microbiol},
   Volume = {10},
   Number = {6},
   Pages = {275-8},
   Note = {0966-842x
Journal Article},
   Abstract = {Early infection with HIV-1 is dominated by CCR5-tropic (R5, non-syncytium-inducing) viruses. The evolution of CXCR4-tropic (X4, syncytium-inducing) viruses occurs later in the infection and is associated with rapid disease progression. Here, we propose that the tropism of X4 viruses for naive CD4+ T cells is disadvantageous in early infection owing to the low division rate of these cells. In healthy individuals, the division rate of memory cells is nearly ten times higher than that of naive cells and thus the memory-cell tropism of R5 viruses could account for their dominance early in infection. As the division rate of naive T cells increases with CD4+ depletion, X4 viruses come to dominate in late disease.},
 Keywords = {CD4-Positive T-Lymphocytes/*virology
HIV Infections/*immunology/metabolism
HIV-1/*pathogenicity
Human
Immunologic Memory
Macrophages/*virology
Models, Biological
Receptors, CCR5/metabolism
Receptors, CXCR4/metabolism
Tropism},
   Year = {2002} }



@article{
Deeks00,
   Author = {Deeks, S. G. and Barbour, J. D. and Martin, J. N. and Swanson, M. S. and Grant, R. M.},
   Title = {Sustained CD4+ T cell response after virologic failure of protease inhibitor-based regimens in patients with human immunodeficiency virus infection},
   Journal = {J Infect Dis},
   Volume = {181},
   Number = {3},
   Pages = {946-53},
   Note = {0022-1899
Journal Article},
   Abstract = {The relationship between plasma human immunodeficiency virus (HIV) RNA levels and peripheral CD4+ T cell counts was examined in 380 HIV-infected adults receiving long-term protease inhibitor therapy. Patients experiencing virologic failure (persistent HIV RNA >500 copies RNA/mL) generally had CD4+ T cell counts that remained greater than pretherapy baseline levels, at least through 96 weeks of follow-up. The CD4+ T cell response was directly and independently related to degree of viral suppression below the pretreatment baseline. For any given HIV RNA level measured 12 weeks after virologic failure, subsequent CD4+ T cell decline was slower in patients receiving a protease inhibitor-based regimen than in a historical control group of untreated patients. These observations suggest that transient or partial declines in plasma HIV RNA levels can have sustained effects on CD4+ T cell levels.},
 Keywords = {Adult
*CD4 Lymphocyte Count
Female
HIV Infections/*drug therapy/immunology/virology
HIV Protease Inhibitors/*therapeutic use
Human
Male
RNA, Viral/*blood
Support, Non-U.S. Gov't
Support, U.S. Gov't, P.H.S.},
   Year = {2000} }



@article{
Deeks01,
   Author = {Deeks, S. G. and Wrin, T. and Liegler, T. and Hoh, R. and Hayden, M. and Barbour, J. D. and Hellmann, N. S. and Petropoulos, C. J. and McCune, J. M. and Hellerstein, M. K. and Grant, R. M.},
   Title = {Virologic and immunologic consequences of discontinuing combination antiretroviral-drug therapy in HIV-infected patients with detectable viremia},
   Journal = {N Engl J Med},
   Volume = {344},
   Number = {7},
   Pages = {472-80},
   Note = {0028-4793
Clinical Trial
Journal Article
Randomized Controlled Trial},
   Abstract = {BACKGROUND: In many patients with human immunodeficiency virus (HIV) infection, therapy with potent antiretroviral drugs does not result in complete suppression of HIV replication. The effect of cessation of therapy in these patients is unknown. METHODS: Sixteen patients who had a plasma HIV RNA level of more than 2500 copies per milliliter during combination antiretroviral-drug therapy were randomly assigned, in a 2:1 ratio, to discontinue or continue therapy. Plasma HIV RNA levels, CD4 cell counts, and drug susceptibility were measured weekly. Viral replicative capacity was measured at base line and at week 12. RESULTS: Discontinuation of therapy for 12 weeks was associated with a median decrease in the CD4 cell count of 128 cells per cubic millimeter and an increase in the plasma HIV RNA level of 0.84 log copies per milliliter. Virus from all patients with detectable resistance at entry became susceptible to HIV-protease inhibitors within 16 weeks after the discontinuation of therapy. Drug susceptibility began to increase a median of six weeks after the discontinuation of therapy and was temporally associated with increases in plasma HIV RNA levels and decreases in CD4 cell counts. Viral replicative capacity, measured by means of a recombinant-virus assay, was low at entry into the study and increased after therapy was discontinued. Despite the loss of detectable resistance in plasma, resistant virus was cultured from peripheral-blood mononuclear cells in five of nine patients who could be evaluated. Plasma HIV RNA levels, CD4 cell counts, and drug susceptibility remained stable in the patients who continued therapy. CONCLUSIONS: Despite the presence of reduced drug susceptibility, antiretroviral-drug therapy can provide immunologic and virologic benefit. This benefit reflects continued antiviral-drug activity and the maintenance of a viral population with a reduced replicative capacity.},
 Keywords = {Adult
Anti-HIV Agents/pharmacology/*therapeutic use
CD4 Lymphocyte Count
Drug Resistance, Microbial
Drug Therapy, Combination
HIV Infections/*drug therapy/immunology/virology
HIV Protease Inhibitors/pharmacology/*therapeutic use
HIV-1/*drug effects/genetics/isolation & purification
Human
Male
Middle Aged
Proportional Hazards Models
Prospective Studies
RNA, Viral/blood
Support, Non-U.S. Gov't
Support, U.S. Gov't, P.H.S.
Viremia/drug therapy},
   Year = {2001} }



@article{
Deeks01b,
   Author = {Deeks, S. G.},
   Title = {International perspectives on antiretroviral resistance. Nonnucleoside reverse transcriptase inhibitor resistance},
   Journal = {J Acquir Immune Defic Syndr},
   Volume = {26 Suppl 1},
   Pages = {S25-33},
   Note = {1525-4135
Journal Article
Review
Review, Tutorial},
   Abstract = {Although understanding of nonnucleoside reverse transcriptase inhibitor (NNRTI) resistance is less clearly established than that of other classes of antiretroviral drugs, certain facts have been established. The treatment-associated genetic mutation profiles of the available NNRTIs have been mapped, and resistance has been found to develop rapidly after initiation of NNRTI therapy. Despite the chemical diversity of the NNRTIs, cross-resistance among agents of this class is nearly universal. Although the viral replicative capacity (``fitness") of NNRTI-induced viral variants has not been extensively studied, available data suggest that NNRTI-selected mutations confer little damage to viral fitness, and thus a single point mutation produces a strain that is both resistant and fit. Furthermore, with continued therapy, viral evolution persists, creating species with greater numbers of mutations and higher level phenotypic resistance. Taken together, these facts suggest that continued use of NNRTIs after emergence of resistance will produce variants of complex mutational patterns that limit future treatment options, and, therefore, strong consideration should be given to discontinuing NNRTIs after virologic failure is confirmed. This article describes the scientific literature establishing the efficacy and limitations of NNRTI therapy and attempts to define a role for this class of drug in the long-term treatment of HIV-1 disease.},
 Keywords = {Anti-HIV Agents/*pharmacology/therapeutic use
Clinical Trials
Delavirdine/pharmacology/therapeutic use
*Drug Resistance, Microbial
Drug Therapy, Combination
HIV Infections/drug therapy/transmission
HIV-1/*drug effects/genetics/metabolism
HIV-1 Reverse Transcriptase/chemistry/genetics
Human
Nevirapine/pharmacology/therapeutic use
Oxazines/pharmacology/therapeutic use
Phylogeny
Point Mutation/drug effects
Protein Conformation
Reverse Transcriptase Inhibitors/*pharmacology/therapeutic use
Virus Replication/drug effects},
   Year = {2001} }



@article{
Deeks02,
   Author = {Deeks, S. G. and Barbour, J. D. and Grant, R. M. and Martin, J. N.},
   Title = {Duration and predictors of CD4 T-cell gains in patients who continue combination therapy despite detectable plasma viremia},
   Journal = {Aids},
   Volume = {16},
   Number = {2},
   Pages = {201-7},
   Note = {0269-9370
Journal Article},
   Abstract = {BACKGROUND: Sustained elevations in CD4 cell counts commonly occur despite incomplete viral suppression with protease inhibitor-based antiretroviral therapy. OBJECTIVES: To determine the incidence and risk factors associated with return of CD4 cell count to pre-therapy levels in patients experiencing virologic failure of protease inhibitor therapy. DESIGN: This is a clinic-based cohort study of HIV-infected adults who failed to maintain durable viral suppression on a protease inhibitor-based regimen. MAIN OUTCOME MEASURES: Virologic failure was defined as persistent plasma HIV RNA level > 500 copies/ml. Immunologic failure was defined as return of CD4 cell count to pre-therapy levels. RESULTS: A total of 291 patients experienced virologic failure on a protease inhibitor-based regimen and had a treatment-mediated CD4 cell increase above pre-therapy levels at the time of virologic failure. If patient data were censored at the time a successful salvage regimen was initiated, then the median time to immunologic failure after the onset of virologic failure was 3 years. If patient data were also censored at the time therapy was discontinued, then 36.8% of the cohort experienced immunologic failure after 3 years of continuous virologic failure. The change in viral load from a pre-treatment baseline, and not the absolute level of viremia achieved, was a strong and independent predictor of immunologic failure. Discontinuing therapy was associated with immunologic failure independent of viral load changes. CONCLUSION: Reduction in T CD4+ cell numbers may eventually occur during prolonged virologic failure of a protease inhibitor-based regimen and is predicted by the degree of virologic suppression below a pre-therapy 'set-point'.},
 Keywords = {Adult
Antiretroviral Therapy, Highly Active
CD4 Lymphocyte Count
CD4-Positive T-Lymphocytes/cytology/*drug effects
Disease Progression
HIV Infections/blood/*drug therapy/immunology/virology
HIV Protease Inhibitors/*therapeutic use
HIV-1/*drug effects/genetics
Human
Indinavir/therapeutic use
Nelfinavir/therapeutic use
RNA, Viral/blood
Ritonavir/therapeutic use
Saquinavir/therapeutic use
Support, Non-U.S. Gov't
Support, U.S. Gov't, P.H.S.
Time Factors
Treatment Failure
Viremia/blood/*drug therapy/immunology/virology},
   Year = {2002} }



@article{
Deeks03,
   Author = {Deeks, S. G.},
   Title = {Treatment of antiretroviral-drug-resistant HIV-1 infection},
   Journal = {Lancet},
   Volume = {362},
   Number = {9400},
   Pages = {2002-11},
   Note = {1474-547x
Journal Article
Review
Review, Academic},
   Abstract = {Drug-resistant HIV-1 is a cause of growing clinical and public-health concern. In many patients, combination antiretroviral therapy fails to achieve complete viral suppression (virological failure). Continuing viral replication during therapy leads to the accumulation of drug-resistance mutations, resulting in increased viral load and a greater risk of disease progression. Patients with drug-resistant HIV-1 infection have three therapeutic options: a change to a salvage regimen with the aim of fully suppressing viral replication; interruption of therapy; or continuation of a partially effective regimen. The first strategy is preferred for most patients failing their first or perhaps their second regimen. However, the best approach remains unclear for patients who have failed multiple treatment regimens and who have limited options for complete viral suppression. The management of such patients requires a careful understanding of the pathogenesis of drug-resistant HIV-1, the clinical consequences of virological failure, the potential benefits and limitations of diagnostic assays, and the likelihood that agents in development will be effective.},
 Keywords = {Anti-HIV Agents/*immunology/*therapeutic use
Antiretroviral Therapy, Highly Active/methods
Drug Resistance, Viral/genetics/immunology
Drug Therapy, Combination
HIV Infections/*drug therapy/immunology/virology
HIV Protease Inhibitors/immunology/therapeutic use
*HIV-1/drug effects/genetics/immunology
Human
Randomized Controlled Trials
Ritonavir/immunology/therapeutic use
Support, Non-U.S. Gov't
Support, U.S. Gov't, P.H.S.
Treatment Outcome
Viral Load/statistics & numerical data
Virus Replication/drug effects/immunology},
   Year = {2003} }



@article{Deeks04,
   Author = {Deeks, S. G. and Walker, B. D.},
   Title = {The immune response to AIDS virus infection: good, bad, or both?},
   Journal = {J Clin Invest},
   Volume = {113},
   Number = {6},
   Pages = {808-10},
   Note = {0021-9738
Comment
Journal Article},
   Abstract = {A potent antigen-specific T cell response to HIV infection can contribute to the control of viral replication and is therefore beneficial to the host. However, HIV-mediated increases in generalized T cell activation also appear to accelerate both viral replication and CD4+ T cell depletion. A new study in the JCI attempts to experimentally distinguish the beneficial versus harmful aspects of this immune response.},
 Year = {2004} }

@techreport{
DHHS04,
   Author = {DHHS},
   Title = {Guidelines for the use of antiretroviral agents in HIV-1 infected adults and adolescents},
   Institution = {Panel on Clinical Practices for Treatment of HIV Infection, Department of Health and Human Services},
   Month= {March 23},
 Year = {2004} }



@article{
Faure00,
   Author = {Faure, S. and Meyer, L. and Costagliola, D. and Vaneensberghe, C. and Genin, E. and Autran, B. and Delfraissy, J. F. and McDermott, D. H. and Murphy, P. M. and Debre, P. and Theodorou, I. and Combadiere, C.},
   Title = {Rapid progression to AIDS in HIV+ individuals with a structural variant of the chemokine receptor CX3CR1},
   Journal = {Science},
   Volume = {287},
   Number = {5461},
   Pages = {2274-7},
   Note = {0036-8075
Comment
Journal Article},
   Abstract = {Human immunodeficiency virus (HIV) enters cells in vitro via CD4 and a coreceptor. Which of 15 known coreceptors are important in vivo is poorly defined but may be inferred from disease-modifying mutations, as for CCR5. Here two single nucleotide polymorphisms are described in Caucasians in CX3CR1, an HIV coreceptor and leukocyte chemotactic/adhesion receptor for the chemokine fractalkine. HIV-infected patients homozygous for CX3CR1-I249 M280, a variant haplotype affecting two amino acids (isoleucine-249 and methionine-280), progressed to AIDS more rapidly than those with other haplotypes. Functional CX3CR1 analysis showed that fractalkine binding is reduced among patients homozygous for this particular haplotype. Thus, CX3CR1-I249 M280 is a recessive genetic risk factor in HIV/AIDS.},
 Keywords = {Acquired Immunodeficiency Syndrome/genetics/*physiopathology/virology
Case-Control Studies
*Chemokines, CX3C
Chemokines, CXC/metabolism
Chromosomes, Human, Pair 3
Cohort Studies
Disease Progression
European Continental Ancestry Group/genetics
Genotype
HIV/physiology
HIV Infections/genetics/*physiopathology/virology
Haplotypes
Homozygote
Human
Leukocytes, Mononuclear/metabolism
Linkage Disequilibrium
Membrane Proteins/metabolism
Mutation
Polymorphism, Restriction Fragment Length
*Polymorphism, Single Nucleotide
Polymorphism, Single-Stranded Conformational
Receptors, Cytokine/*genetics/*physiology
Receptors, HIV/*genetics/*physiology
Support, Non-U.S. Gov't
Survival Analysis
Variation (Genetics)},
   Year = {2000} }



@article{
Gao01,
   Author = {Gao, X. and Nelson, G. W. and Karacki, P. and Martin, M. P. and Phair, J. and Kaslow, R. and Goedert, J. J. and Buchbinder, S. and Hoots, K. and Vlahov, D. and O'Brien, S. J. and Carrington, M.},
   Title = {Effect of a single amino acid change in MHC class I molecules on the rate of progression to AIDS},
   Journal = {N Engl J Med},
   Volume = {344},
   Number = {22},
   Pages = {1668-75},
   Note = {0028-4793
Journal Article
Multicenter Study},
   Abstract = {BACKGROUND: From studies of genetic polymorphisms and the rate of progression from human immunodeficiency virus type 1 (HIV-1) infection to the acquired immunodeficiency syndrome (AIDS), it appears that the strongest susceptibility is conferred by the major-histocompatibility-complex (MHC) class I type HLA-B*35,Cw*04 allele. However, cytotoxic T-lymphocyte responses have been observed against HIV-1 epitopes presented by HLA-B*3501, the most common HLA-B*35 subtype. We examined subtypes of HLA-B*35 in five cohorts and analyzed the relation of structural differences between HLA-B*35 subtypes to the risk of progression to AIDS. METHODS: Genotyping of HLA class I loci was performed for 850 patients who seroconverted and had known dates of HIV-1 infection. Survival analyses with respect to the rate of progression to AIDS were performed to identify the effects of closely related HLA-B*35 subtypes with different peptide-binding specificities. RESULTS: HLA-B*35 subtypes were divided into two groups according to peptide-binding specificity: the HLA-B*35-PY group, which consists primarily of HLA-B*3501 and binds epitopes with proline in position 2 and tyrosine in position 9; and the more broadly reactive HLA-B*35-Px group, which also binds epitopes with proline in position 2 but can bind several different amino acids (not including tyrosine) in position 9. The influence of HLA-B*35 in accelerating progression to AIDS was completely attributable to HLA-B*35-Px alleles, some of which differ from HLA-B*35-PY alleles by only one amino acid residue. CONCLUSIONS: This analysis shows that, in patients with HIV-1 infection, a single amino acid change in HLA molecules has a substantial effect on the rate of progression to AIDS. The different consequences of HLA-B*35-PY and HLA-B*35-Px in terms of disease progression highlight the importance of the epitope specificities of closely related class I molecules in the immune defense against HIV-1.},
 Keywords = {Acquired Immunodeficiency Syndrome/*genetics
African Continental Ancestry Group/genetics
Alleles
Amino Acid Sequence
Binding Sites/genetics
Disease Progression
Disease-Free Survival
European Continental Ancestry Group/genetics
*Genes, MHC Class I
Genotype
HIV Infections/ethnology/*genetics/immunology
HLA-B35 Antigen/chemistry/*genetics
HLA-C Antigens
Human
Peptides/metabolism
Proportional Hazards Models
Receptors, Peptide/chemistry/genetics/metabolism
Support, U.S. Gov't, P.H.S.},
   Year = {2001} }



@article{
Grabar00,
   Author = {Grabar, S. and Le Moing, V. and Goujard, C. and Leport, C. and Kazatchkine, M. D. and Costagliola, D. and Weiss, L.},
   Title = {Clinical outcome of patients with HIV-1 infection according to immunologic and virologic response after 6 months of highly active antiretroviral therapy},
   Journal = {Ann Intern Med},
   Volume = {133},
   Number = {6},
   Pages = {401-10},
   Note = {0003-4819
Journal Article
Multicenter Study},
   Abstract = {BACKGROUND: The prognostic value of discordant immunologic (CD4 cell increase) and virologic (plasma HIV RNA level decrease) responses to antiretroviral treatment is not known. OBJECTIVE: To study the relation between clinical outcome of HIV-infected patients receiving highly active antiretroviral therapy (HAART) and early immunologic and virologic responses to such therapy. DESIGN: Prospective cohort study. SETTING: 68 hospitals in France. PATIENTS: 2236 protease inhibitor-naive patients. INTERVENTION: Initiation of HAART with one protease inhibitor and two nucleoside analogues between July 1996 and March 1997. MEASUREMENTS: Immunologic and virologic response at 6 months. Multivariate Cox models were used to assess the relation between these responses and progression to a new AIDS-defining event or death. RESULTS: On the basis of 6-month immunologic and virologic responses, patients were classified into four groups: complete response (47.5%), complete nonresponse (16.2%), immunologic response only (19.0%), and virologic response only (17.3%). After month 6 and within a median of 18 months, 69 patients died and 123 experienced a new AIDS-defining event. After adjustment, complete nonresponders and those with only a virologic response had significantly higher risks for clinical progression at 6 months (relative risk, 3.38 [95% CI, 2.28 to 5.02] and 1.98 [CI, 1.26 to 3.10], respectively) than complete responders. The difference between complete responders and those with only an immunologic response at 6 months was weaker and nonsignificant (relative risk, 1.55 [CI, 0.96 to 2.50]). CONCLUSIONS: Immunologic response after 6 months of HAART indicates a favorable clinical outcome in HIV-infected patients regardless of virologic response. This suggests that both immunologic and virologic markers should be used in clinical practice to evaluate treatment response.},
 Keywords = {Adult
CD4 Lymphocyte Count
Disease Progression
Drug Therapy, Combination
Female
HIV Infections/*drug therapy/immunology/virology
HIV Protease Inhibitors/*therapeutic use
*HIV-1/genetics
Human
Male
Multivariate Analysis
Proportional Hazards Models
Prospective Studies
RNA, Viral/blood
Reverse Transcriptase Inhibitors/*therapeutic use
Support, Non-U.S. Gov't
Treatment Outcome
Viral Load},
   Year = {2000} }



@article{
Grueb00,
   Author = {Greub, G. and Ledergerber, B. and Battegay, M. and Grob, P. and Perrin, L. and Furrer, H. and Burgisser, P. and Erb, P. and Boggian, K. and Piffaretti, J. C. and Hirschel, B. and Janin, P. and Francioli, P. and Flepp, M. and Telenti, A.},
   Title = {Clinical progression, survival, and immune recovery during antiretroviral therapy in patients with HIV-1 and hepatitis C virus coinfection: the Swiss HIV Cohort Study},
   Journal = {Lancet},
   Volume = {356},
   Number = {9244},
   Pages = {1800-5},
   Note = {0140-6736
Clinical Trial
Journal Article},
   Abstract = {BACKGROUND: Hepatitis C virus (HCV) infection is highly prevalent among HIV-1-infected individuals, but its contribution to the morbidity and mortality of coinfected patients who receive potent antiretroviral therapy is controversial. We used data from the ongoing Swiss HIV Cohort Study to analyse clinical progression of HIV-1, and the virological and immunological response to potent antiretroviral therapy in HIV-1-infected patients with or without concurrent HCV infection. METHODS: We analysed prospective data on survival, clinical disease progression, suppression of HIV-1 replication, CD4-cell recovery, and frequency of changes in antiretroviral therapy according to HCV status in 3111 patients starting potent antiretroviral therapy. RESULTS: 1157 patients (37.2%) were coinfected with HCV, 1015 of whom (87.7%) had a history of intravenous drug use. In multivariate Cox's regression, the probability of progression to a new AIDS-defining clinical event or to death was independently associated with HCV seropositivity (hazard ratio 1.7 [95% CI 1.26-2.30]), and with active intravenous drug use (1.38 [1.02-1.88]). Virological response to antiretroviral therapy and the probability of treatment change were not associated with HCV serostatus. In contrast, HCV seropositivity was associated with a smaller CD4-cell recovery (hazard ratio for a CD4-cell count increase of at least 50 cells/microL=0.79 [0.72-0.87]). INTERPRETATION: HCV and active intravenous drug use could be important factors in the morbidity and mortality among HIV-1-infected patients, possibly through impaired CD4-cell recovery in HCV seropositive patients receiving potent antiretroviral therapy. These findings are relevant for decisions about optimum timing for HCV treatment in the setting of HIV infection.},
 Keywords = {AIDS-Related Opportunistic Infections/*drug therapy
Adolescent
Adult
Anti-HIV Agents/*therapeutic use
CD4 Lymphocyte Count
Cohort Studies
Disease Progression
Female
Hepatitis C/complications/*drug therapy
Human
Male
Middle Aged
Prospective Studies
Support, Non-U.S. Gov't
Survival Analysis
Switzerland
Viral Load
Viremia/etiology},
   Year = {2000} }



@article{
Katzenstein96,
   Author = {Katzenstein, D. A. and Hammer, S. M. and Hughes, M. D. and Gundacker, H. and Jackson, J. B. and Fiscus, S. and Rasheed, S. and Elbeik, T. and Reichman, R. and Japour, A. and Merigan, T. C. and Hirsch, M. S.},
   Title = {The relation of virologic and immunologic markers to clinical outcomes after nucleoside therapy in HIV-infected adults with 200 to 500 CD4 cells per cubic millimeter. AIDS Clinical Trials Group Study 175 Virology Study Team},
   Journal = {N Engl J Med},
   Volume = {335},
   Number = {15},
   Pages = {1091-8},
   Note = {0028-4793
Clinical Trial
Journal Article
Multicenter Study
Randomized Controlled Trial},
   Abstract = {BACKGROUND: We studied measures of human immunodeficiency virus (HIV) replication, the viral phenotype, and immune function (CD4 cell counts) and the relation of changes in these indicators to clinical outcomes in a subgroup of patients in a controlled trial of early antiretroviral treatment for HIV, the AIDS Clinical Trials Group Study 175. METHODS: The 391 subjects, each of whom entered the study with a single screening CD4 cell count of 200 to 500 per cubic millimeter, were randomly assigned to receive zidovudine alone, didanosine alone, zidovudine plus didanosine, or zidovudine plus zalcitabine. Plasma concentrations of HIV RNA were assessed in 366 subjects, and viral isolates from 332 subjects were assayed for the presence of the syncytium-inducing phenotype. RESULTS: After eight weeks, the mean (+/-SE) decrease from base line in the concentration of HIV RNA, expressed as the change in the base 10 log of the number of copies per milliliter, was 0.26+/-0.06 for patients treated with zidovudine alone, 0.65+/-0.07 for didanosine alone, 0.93+/-0.10 for zidovudine plus didanosine, and 0.89+/-0.06 for zidovudine plus zalcitabine (P<0.001 for each of the pairwise comparisons with zidovudine alone). Multivariate proportional-hazards models showed that higher base-line concentrations of plasma HIV RNA, less suppression of plasma HIV RNA by treatment, and the presence of the syncytium-inducing phenotype were significantly associated with an increased risk of progression to the acquired immunodeficiency syndrome and death. After adjustment for these measures of viral replication and for the viral phenotype, CD4 cell counts were not significant predictors of clinical outcome. CONCLUSIONS: Both the risk of the progression of HIV disease and the efficacy of antiretroviral therapy are strongly associated with the plasma level of HIV RNA and with the viral phenotype. The changes in the plasma concentration of HIV RNA predict the changes in CD4 cell counts and survival after treatment with reverse-transcriptase inhibitors.},
 Keywords = {Adult
Antiviral Agents/*therapeutic use
CD4 Lymphocyte Count
Didanosine/*therapeutic use
Disease Progression
Drug Therapy, Combination
Female
HIV/*genetics/isolation & purification/physiology
HIV Infections/drug therapy/immunology/*virology
Human
Male
Middle Aged
Multivariate Analysis
Phenotype
Proportional Hazards Models
RNA, Viral/*blood
Support, U.S. Gov't, P.H.S.
Treatment Outcome
Virus Replication/drug effects
Zidovudine/*therapeutic use},
   Year = {1996} }



@article{
Kaufmann98,
   Author = {Kaufmann, D. and Pantaleo, G. and Sudre, P. and Telenti, A.},
   Title = {CD4-cell count in HIV-1-infected individuals remaining viraemic with highly active antiretroviral therapy (HAART). Swiss HIV Cohort Study},
   Journal = {Lancet},
   Volume = {351},
   Number = {9104},
   Pages = {723-4},
   Note = {0140-6736
Letter},
 Keywords = {Anti-HIV Agents/*therapeutic use
CD4 Lymphocyte Count
HIV Infections/drug therapy/*immunology
Human
Protease Inhibitors/*therapeutic use
Support, Non-U.S. Gov't
Viremia/drug therapy/*immunology},
   Year = {1998} }



@article{
Kaufmann03,
   Author = {Kaufmann, G. R. and Perrin, L. and Pantaleo, G. and Opravil, M. and Furrer, H. and Telenti, A. and Hirschel, B. and Ledergerber, B. and Vernazza, P. and Bernasconi, E. and Rickenbach, M. and Egger, M. and Battegay, M.},
   Title = {CD4 T-lymphocyte recovery in individuals with advanced HIV-1 infection receiving potent antiretroviral therapy for 4 years: the Swiss HIV Cohort Study},
   Journal = {Arch Intern Med},
   Volume = {163},
   Number = {18},
   Pages = {2187-95},
   Note = {0003-9926
Journal Article},
   Abstract = {BACKGROUND: Highly active antiretroviral therapy (HAART) for human immunodeficiency virus (HIV)-1 infection allows recovery of CD4 T lymphocytes. Few studies have explored the long-term T-lymphocyte responses to HAART. METHODS: Plasma HIV-1 RNA levels and CD4 and CD8 T-lymphocyte counts were longitudinally analyzed over 4 years in 2235 participants of the Swiss HIV Cohort, commencing HAART between 1996 and 1997. The CD4 T-lymphocyte count increase, the percentage of individuals with a CD4 T-lymphocyte count of 500/microL or greater and less than 200/microL, and the determinants of CD4 T-lymphocyte recovery were evaluated in individuals treated with continuous (CONT; n = 985) and discontinuous (DISCONT; n = 1250) HAART. RESULTS: At 4 years, 69.5% of subjects (CONT, 84.5%; DISCONT, 53.6%; P<.001) showed HIV-1 RNA levels below 400 copies/mL, while the median CD4 T-lymphocyte count increased from 190/microL to 423/microL (CONT, 486/microL; DISCONT, 343/microL; P<.001). Of the 2235 participants, 38.8% (CONT, 47.7%; DISCONT, 29.4%; P<.001) reached a CD4 T-lymphocyte count of 500/microL or greater, but in 15.6%, CD4 T-lymphocyte count remained below 200/microL (CONT, 5.9%; DISCONT, 25.9%; P<.001). Larger increases in CD4 T-lymphocyte count were associated with higher baseline HIV-1 RNA, a larger percentage of undetectable HIV-1 RNA levels, lower baseline CD8 T-lymphocyte count, and younger age. Individuals reaching a CD4 T-lymphocyte count of 500/microL or greater at 4 years were characterized by higher nadir and baseline CD4 T-lymphocyte counts and a more sustained reduction of HIV-1 RNA levels. CONCLUSIONS: At 4 years, only 39% of individuals treated with HAART reached a CD4 T-lymphocyte count of 500/microL or greater, and 16% with CD4 T-lymphocyte counts less than 200/microL remained susceptible to opportunistic infections. Treatment interruptions, a poor virologic response, and older age were the major factors negatively affecting the recovery of CD4 T lymphocytes.},
 Keywords = {Adult
*Antiretroviral Therapy, Highly Active
*CD4 Lymphocyte Count
CD8-Positive T-Lymphocytes
Female
HIV Infections/*drug therapy/*immunology
*Hiv-1
Human
Lymphocyte Count
Male
Middle Aged
Prospective Studies
RNA, Viral/*analysis
Support, Non-U.S. Gov't
Viral Load},
   Year = {2003} }



@article{
MartinezPicado99,
   Author = {Martinez-Picado, J. and Savara, A. V. and Sutton, L. and D'Aquila, R. T.},
   Title = {Replicative fitness of protease inhibitor-resistant mutants of human immunodeficiency virus type 1},
   Journal = {J Virol},
   Volume = {73},
   Number = {5},
   Pages = {3744-52},
   Note = {0022-538x
Journal Article},
   Abstract = {The relative replicative fitness of human immunodeficiency virus type 1 (HIV-1) mutants selected by different protease inhibitors (PIs) in vivo was determined. Each mutant was compared to wild type (WT), NL4-3, in the absence of drugs by several methods, including clonal genotyping of cultures infected with two competing viral variants, kinetics of viral antigen production, and viral infectivity/virion particle ratios. A nelfinavir-selected protease D30N substitution substantially decreased replicative capacity relative to WT, while a saquinavir-selected L90M substitution moderately decreased fitness. The D30N mutant virus was also outcompeted by the L90M mutant in the absence of drugs. A major natural polymorphism of the HIV-1 protease, L63P, compensated well for the impairment of fitness caused by L90M but only slightly improved the fitness of D30N. Multiply substituted indinavir-selected mutants M46I/L63P/V82T/I84V and L10R/M46I/L63P/V82T/I84V were just as fit as WT. These results indicate that the mutations which are usually initially selected by nelfinavir and saquinavir, D30N and L90M, respectively, impair fitness. However, additional mutations may improve the replicative capacity of these and other drug-resistant mutants. Hypotheses based on the greater fitness impairment of the nelfinavir-selected D30N mutant are suggested to explain observations that prolonged responses to delayed salvage regimens, including alternate PIs, may be relatively common after nelfinavir failure.},
 Keywords = {Adaptation, Biological
Amino Acid Substitution
Animals
Anti-HIV Agents/*pharmacology
Cells, Cultured
Drug Resistance, Microbial
HIV Protease Inhibitors/*pharmacology
HIV-1/*drug effects/genetics/physiology
Human
Mice
Mutagenesis, Site-Directed
Nelfinavir/*pharmacology
Saquinavir/*pharmacology
Support, Non-U.S. Gov't
Support, U.S. Gov't, P.H.S.
Tumor Cells, Cultured
Virus Replication/*drug effects},
   Year = {1999} }



@article{
Mellors96,
   Author = {Mellors, J. W. and Rinaldo, C. R., Jr. and Gupta, P. and White, R. M. and Todd, J. A. and Kingsley, L. A.},
   Title = {Prognosis in HIV-1 infection predicted by the quantity of virus in plasma},
   Journal = {Science},
   Volume = {272},
   Number = {5265},
   Pages = {1167-70},
   Note = {0036-8075
Comment
Journal Article},
   Abstract = {The relation between viremia and clinical outcome in individuals infected with human immunodeficiency virus-type 1 (HIV-1) has important implications for therapeutic research and clinical care. HIV-1 RNA in plasma was quantified with a branched-DNA signal amplification assay as a measure of viral load in a cohort of 180 seropositive men studied for more than 10 years. The risk of acquired immunodeficiency syndrome (AIDS) and death in study subjects, including those with normal numbers of CD4+ T cells, was directly related to plasma viral load at study entry. Plasma viral load was a better predictor of progression to AIDS and death than was the number of CD4+ T cells.},
 Keywords = {Acquired Immunodeficiency Syndrome/*virology
Antiviral Agents/therapeutic use
Biological Markers/blood
CD4 Lymphocyte Count
CD4-Positive T-Lymphocytes/virology
Cohort Studies
Disease Progression
Follow-Up Studies
HIV Infections/drug therapy/mortality/*virology
HIV-1/genetics/*physiology
Human
Male
Prognosis
Proportional Hazards Models
RNA, Viral/*blood
Support, Non-U.S. Gov't
Support, U.S. Gov't, Non-P.H.S.
Support, U.S. Gov't, P.H.S.
Survival Rate
Time Factors
Viremia/*virology
Virus Replication},
   Year = {1996} }



@article{
Miller00,
   Author = {Miller, V. and Sabin, C. A. and Phillips, A. N. and Rottmann, C. and Rabenau, H. and Weidmann, E. and Rickerts, V. and Findhammer, S. and Helm, E. B. and Staszewski, S.},
   Title = {The impact of protease inhibitor-containing highly active antiretroviral therapy on progression of HIV disease and its relationship to CD4 and viral load},
   Journal = {Aids},
   Volume = {14},
   Number = {14},
   Pages = {2129-36},
   Note = {0269-9370
Clinical Trial
Journal Article},
   Abstract = {OBJECTIVE: To compare the rate of disease progression according to viral load and CD4 cell count in patients receiving or not receiving highly active antiretroviral therapy (HAART), defined as protease inhibitor-containing regimens. DESIGN: An observational study, with prospectively collected data. METHODS: All patients attending the HIV Outpatient clinic as of 1 January 1995 (n = 2083) were included. Follow-up was until the first AIDS-defining event or death. Associations between viral load or CD4 cell count and disease progression were assessed using a person-years approach. Event rates were compared using Poisson regression analysis; a multivariate model was used to assess the independent effects of CD4, viral load and treatment group on event rates and to consider interactions between these variables. RESULTS: The event rates increased with lower CD4 cell count and higher viral load for both treatment groups and were generally lower in the HAART group. In a multivariate analysis, lower CD4 cell counts and higher viral loads remained significantly associated with disease progression, irrespective of treatment group. However, the event rate was significantly lower for the HAART group compared with the control group (relative rate 0.53, P < 0.001). CONCLUSIONS: HAART-treated patients with high viral loads and CD4 cell counts experienced reduced disease progression compared with individuals with the same CD4 cell count and viral load not receiving HAART. Consequently, the short-term prognosis associated with viral load levels and CD4 cell counts may differ in patients on HAART. Whether this effect will be observed with non-protease-inhibitor-containing HAART is not known at this time.},
 Keywords = {Adolescent
Adult
Aged
Antiretroviral Therapy, Highly Active
CD4 Lymphocyte Count
Disease Progression
HIV Infections/*drug therapy/pathology/virology
HIV Protease Inhibitors/*therapeutic use
*HIV-1/isolation & purification
Human
Middle Aged
Prospective Studies
RNA, Viral/analysis
Regression Analysis
Support, Non-U.S. Gov't
Viral Load},
   Year = {2000} }



@article{
Piketty98,
   Author = {Piketty, C. and Castiel, P. and Belec, L. and Batisse, D. and Si Mohamed, A. and Gilquin, J. and Gonzalez-Canali, G. and Jayle, D. and Karmochkine, M. and Weiss, L. and Aboulker, J. P. and Kazatchkine, M. D.},
   Title = {Discrepant responses to triple combination antiretroviral therapy in advanced HIV disease},
   Journal = {Aids},
   Volume = {12},
   Number = {7},
   Pages = {745-50},
   Note = {0269-9370
Journal Article},
   Abstract = {OBJECTIVES: To determine the clinical, virological and immunological outcome in a cohort of unselected patients receiving triple combination therapy for more than 1 year. METHODS: Prospective follow-up of a cohort of 162 unselected, protease inhibitor-naive, antiretroviral-experienced patients with advanced HIV disease, treated with indinavir combined with two nucleoside analogues. RESULTS: The mean CD4 cell count and plasma HIV RNA level in the study group at baseline were 69+/-5 x 10(6)/l and 4.75+/-0.07 log10 copies/ml, respectively. Five per cent of patients died prematurely or were lost to follow-up. Fifty-seven per cent of patients responded to therapy, as assessed by a sustained increase in CD4 cell counts above 50 x 10(6)/l and a decrease in plasma HIV RNA greater than 1 log10 copies/ml, throughout 12.1 months of follow-up. Seventeen per cent of patients were immunological and virological non-responders. Twenty-one per cent of patients exhibited discrepant virological and immunological responses to treatment, of whom one-half failed to exhibit significant increases in CD4 cells despite a virological response to therapy and one-half exhibited increased CD4 cell counts in the absence of significant decrease in plasma viral load. The incidence of AIDS-defining events in the latter group of patients was similar to that of responder patients, whereas their incidence was higher in patients who failed to exhibit a virological and immunological response and those who failed to increase CD4 cells despite a significant decrease in viral load. CONCLUSION: Our observations of discrepant immunological and virological responses to treatment raise the issue of the significance of persistent elevated levels of plasma HIV RNA and of the relevance of measurements of plasma viral load for assessing the efficacy of antiretroviral therapy in patients whose CD4 cell counts increase despite the absence of significant decrease in plasma HIV viral load.},
 Keywords = {Adult
Aged
Anti-HIV Agents/*therapeutic use
Cohort Studies
Drug Therapy, Combination
Female
Follow-Up Studies
HIV Infections/*drug therapy/immunology/physiopathology/virology
HIV Protease Inhibitors/*therapeutic use
Human
Indinavir/*therapeutic use
Lamivudine/*therapeutic use
Male
Middle Aged
Prospective Studies
Reverse Transcriptase Inhibitors/*therapeutic use
Stavudine/*therapeutic use
Support, Non-U.S. Gov't
Treatment Outcome
Zidovudine/*therapeutic use},
   Year = {1998} }



@article{
Piketty01,
   Author = {Piketty, C. and Weiss, L. and Thomas, F. and Mohamed, A. S. and Belec, L. and Kazatchkine, M. D.},
   Title = {Long-term clinical outcome of human immunodeficiency virus-infected patients with discordant immunologic and virologic responses to a protease inhibitor-containing regimen},
   Journal = {J Infect Dis},
   Volume = {183},
   Number = {9},
   Pages = {1328-35},
   Note = {0022-1899
Journal Article},
   Abstract = {Within a prospective cohort of 150 human immunodeficiency virus (HIV)-infected patients who began first-line protease inhibitor therapy in 1996, the outcome of 42 patients with discrepant virologic and immunologic responses to antiretroviral treatment at 12 months was analyzed at 30 months of treatment. The incidence of AIDS-defining events and deaths (14%) in the group of patients with immunologic responses in the absence of a virologic response was higher than that in full-responder patients (2%); yet, the incidence in this group was lower than that in patients with no immunologic response, despite a virologic response (21%), and was lower than that in patients without an immunologic or virologic response (67%; P<.0001, log-rank test). Differences in outcome were significant (relative risk, 6.9; 95% confidence interval, 1.9-39.3) when factors for progression were compared with those of responder patients. The results support the relevance of the CD4 cell marker over plasma HIV load for predicting clinical outcome in patients who do not achieve full immunologic and virologic responses.},
 Keywords = {Adult
Aged
Antiretroviral Therapy, Highly Active
CD4 Lymphocyte Count
Cohort Studies
Disease Progression
Female
HIV Infections/*drug therapy/immunology/virology
HIV Protease Inhibitors/*therapeutic use
Human
Incidence
Longitudinal Studies
Male
Middle Aged
Mortality
Prospective Studies
RNA, Viral/blood
Time Factors
Treatment Outcome
Viral Load},
   Year = {2001} }



@article{
Pilon02,
   Author = {Pilon, A. A. and Lum, J. J. and Sanchez-Dardon, J. and Phenix, B. N. and Douglas, R. and Badley, A. D.},
   Title = {Induction of apoptosis by a nonnucleoside human immunodeficiency virus type 1 reverse transcriptase inhibitor},
   Journal = {Antimicrob Agents Chemother},
   Volume = {46},
   Number = {8},
   Pages = {2687-91},
   Note = {0066-4804
Journal Article},
   Abstract = {Inhibition of human immunodeficiency virus type 1 reverse transcriptase (RT) by both nucleoside and nonnucleoside RT inhibitors profoundly inhibits virus replication. Nucleoside RT inhibitors are known to be toxic, but there is little information regarding the toxicities of nonnucleoside RT inhibitors (NNRTI). We demonstrate that efavirenz (an NNRTI) induces caspase- and mitochondrion-dependent apoptosis of Jurkat T cells and human peripheral blood mononuclear cells. The clinical relevance of these observations is not yet clear.},
 Keywords = {Annexin V/diagnostic use
Apoptosis/*drug effects
Caspases/physiology
Enzyme Inhibitors/diagnostic use
Fluorescein-5-isothiocyanate
Fluorescent Dyes
HIV-1 Reverse Transcriptase/*antagonists & inhibitors
Human
Jurkat Cells
Membrane Potentials/drug effects
Mitochondria/drug effects/physiology
Oxazines/*pharmacology
Reverse Transcriptase Inhibitors/*pharmacology
Support, Non-U.S. Gov't},
   Year = {2002} }



@article{
Price03,
   Author = {Price, D. A. and Scullard, G. and Oxenius, A. and Braganza, R. and Beddows, S. A. and Kazmi, S. and Clarke, J. R. and Johnson, G. E. and Weber, J. N. and Phillips, R. E.},
   Title = {Discordant outcomes following failure of antiretroviral therapy are associated with substantial differences in human immunodeficiency virus-specific cellular immunity},
   Journal = {J Virol},
   Volume = {77},
   Number = {10},
   Pages = {6041-9},
   Note = {0022-538x
Clinical Trial
Journal Article},
   Abstract = {Many individuals chronically infected with human immunodeficiency virus type 1 (HIV-1) experience a recrudescence of plasma virus during continuous combination antiretroviral therapy (ART) due either to the emergence of drug-resistant viruses or to poor compliance. In most cases, virologic failure on ART is associated with a coincident decline in CD4(+) T lymphocyte levels. However, a proportion of discordant individuals retain a stable or even increasing CD4(+) T lymphocyte count despite virological failure. In order to address the nature of these different outcomes, we evaluated virologic and immunologic variables in a prospective, single-blinded, nonrandomized cohort of 53 subjects with chronic HIV-1 infection who had been treated with continuous ART and monitored intensively over a period of 19 months. In all individuals with detectable viremia on ART, multiple drug resistance mutations with similar impacts on viral growth kinetics were detected in the pol gene of circulating plasma virus. Further, C2V3 env gene analysis demonstrated sequences indicative of CCR5 coreceptor usage in the majority of those with detectable plasma viremia. In contrast to this homogeneous virologic pattern, comprehensive screening with a range of antigens derived from HIV-1 revealed substantial immunologic differences. Discordant subjects with stable CD4(+) T lymphocyte counts in the presence of recrudescent virus demonstrated potent virus-specific CD4(+) and CD8(+) T lymphocyte responses. In contrast, subjects with virologic failure associated with declining CD4(+) T lymphocyte counts had substantially weaker HIV-specific CD4(+) T lymphocyte responses and exhibited a trend towards weaker HIV-specific CD8(+) T lymphocyte responses. Importantly the CD4(+) response was sustained over periods as long as 11 months, confirming the stability of the phenomenon. These correlative data lead to the testable hypothesis that the consequences of viral recrudescence during continuous ART are modulated by the HIV-specific cellular immune response.},
 Keywords = {Adult
Amino Acid Sequence
Anti-HIV Agents/pharmacology/*therapeutic use
CD4-Positive T-Lymphocytes/*immunology
CD8-Positive T-Lymphocytes/*immunology
Chronic Disease
Drug Resistance, Viral/genetics
Drug Therapy, Combination
HIV Envelope Protein gp120/chemistry/genetics
HIV Infections/*drug therapy/immunology/physiopathology
HIV-1/*drug effects/genetics/physiology
Human
Lymphocyte Count
Middle Aged
Molecular Sequence Data
Mutation
Peptide Fragments/chemistry/genetics
Prospective Studies
RNA, Viral/blood
Single-Blind Method
Support, Non-U.S. Gov't
*Treatment Failure
Viral Load},
   Year = {2003} }



@article{
Quinones00,
   Author = {Quinones-Mateu, M. E. and Ball, S. C. and Marozsan, A. J. and Torre, V. S. and Albright, J. L. and Vanham, G. and van Der Groen, G. and Colebunders, R. L. and Arts, E. J.},
   Title = {A dual infection/competition assay shows a correlation between ex vivo human immunodeficiency virus type 1 fitness and disease progression},
   Journal = {J Virol},
   Volume = {74},
   Number = {19},
   Pages = {9222-33},
   Note = {0022-538x
Journal Article},
   Abstract = {This study was designed to examine the impact of human immunodeficiency virus type 1 (HIV-1) fitness on disease progression through the use of a dual competition/heteroduplex tracking assay (HTA). Despite numerous studies on the impact of HIV-1 diversity and HIV-specific immune response on disease progression, we still do not have a firm understanding of the long-term pathogenesis of this virus. Strong and early CD8-positive cytotoxic T-cell and CD4-positive T-helper cell responses directed toward HIV-infected cells appear to curb HIV pathogenesis. However, the rate at which the virus infects the CD4(+) T-cell population and possibly destroys the HIV-specific immune response may also alter the rate of disease progression. For HIV-1 fitness studies, we established conditions for dual HIV-1 infections of peripheral blood mononuclear cells (PBMC) and a sensitive HTA to measure relative virus production. A pairwise comparison was then performed to estimate the relative fitness of various non-syncytium-inducing/CCR5-tropic (NSI/R5) and syncytium-inducing/CXCR4-tropic (SI/X4) HIV-1 isolates. Four HIV-1 strains (two NSI/R5 and two SI/X4) with moderate ex vivo fitness were then selected as controls and competed against primary HIV-1 isolates from an HIV-infected Belgian cohort. HIV-1 isolates from long-term survivors (LTS) were outcompeted by control strains and were significantly less fit than HIV-1 isolates from patients with accelerated progression to AIDS (PRO). In addition, NSI/R5 HIV-1 isolates from PRO overgrew control SI/X4 strains, suggesting that not all SI/X4 HIV-1 isolates replicate more efficiently than all NSI/R5 isolates. Finally, there were strong, independent correlations between viral load and the total relative fitness values of HIV-1 isolates from PRO (r = 0.84, P = 0.033) and LTS (r = 0.86, P = 0.028). Separation of the PRO and LTS plots suggest that HIV-1 fitness together with viral load may be a strong predictor for the rate of disease progression.},
 Keywords = {*Biological Assay
HIV Infections/*physiopathology/*virology
*HIV-1/physiology
Human
Predictive Value of Tests
Prognosis
Support, Non-U.S. Gov't
Support, U.S. Gov't, P.H.S.},
   Year = {2000} }



@article{
Racinan02,
   Author = {Rancinan, C. and Neau, D. and Saves, M. and Lawson-Ayayi, S. and Bonnet, F. and Mercie, P. and Dupon, M. and Couzigou, P. and Dabis, F. and Chene, G.},
   Title = {Is hepatitis C virus co-infection associated with survival in HIV-infected patients treated by combination antiretroviral therapy?},
   Journal = {Aids},
   Volume = {16},
   Number = {10},
   Pages = {1357-62},
   Note = {0269-9370
Journal Article},
   Abstract = {OBJECTIVE: To study whether hepatitis C virus (HCV) co-infection or the severe elevation of transaminases is associated with survival after the initiation of antiretroviral combination therapy. DESIGN: Prospective hospital-based cohort (Aquitaine Cohort). METHODS: HIV-infected adults started on an antiretroviral combination before 30 June 1999. HCV infection was defined as antibody detection or positive HCV RNA. Severe elevation of transaminases was defined as a value of aspartate or alanine aminotransferase (AST, ALT) above five times the upper limit of normal values. Survival was studied using a Cox model, including at least baseline HCV status and transaminases as a time-dependent covariate. RESULTS: Overall, 995 patients were analysed, including 576 HCV-positive individuals (58%). At baseline, HCV-positive patients were younger, more often injecting drug users and women, and had more frequently elevated transaminases. A shorter survival was associated with AIDS stage [hazard ratio (HR) versus non-AIDS 1.67; 95% confidence interval (CI) 1.03; 2.68], lower CD4 cell count (HR for 50 cells/mm3 lower 1.33; CI 1.17; 1.51), lower haemoglobin (HR for 1 g/dl lower 1.20; CI 1.07; 1.35), lower platelet count (HR for 10 000 cells/mm3 lower 1.04; CI 1.01; 1.07), and AST during follow-up (HR for > or = 200 IU/l 2.30; CI 1.32; 4.03). HCV co-infection (HR 1.20; CI 0.75; 1.92) was not statistically associated with survival. CONCLUSION: The occurrence of a severe elevation of transaminases was associated with poorer survival, although HCV was not. If liver toxicity may be treatment induced, plasma drug concentrations could guide dosage adjustments of antiretroviral treatments currently prescribed to optimize their use.},
 Keywords = {Acquired Immunodeficiency Syndrome/complications
Age Factors
Anti-HIV Agents/*therapeutic use
Antiretroviral Therapy, Highly Active
Cohort Studies
Comparative Study
Disease Progression
Female
Follow-Up Studies
HIV Infections/blood/*complications/*drug therapy
Hepatitis C/blood/*complications
Human
Male
Proportional Hazards Models
Substance Abuse, Intravenous
Support, Non-U.S. Gov't
Survival Analysis
Transaminases/blood},
   Year = {2002} }



@article{
Roger99,
   Author = {Roger, P. M. and Breittmayer, J. P. and Arlotto, C. and Pugliese, P. and Pradier, C. and Bernard-Pomier, G. and Dellamonica, P. and Bernard, A.},
   Title = {Highly active anti-retroviral therapy (HAART) is associated with a lower level of CD4+ T cell apoptosis in HIV-infected patients},
   Journal = {Clin Exp Immunol},
   Volume = {118},
   Number = {3},
   Pages = {412-6},
   Note = {0009-9104
Journal Article},
   Abstract = {HAART may increase CD4+ T cell counts despite a persistently detectable HIV load. The impact of HAART on apoptosis, which may play a role in the disease process in HIV-infected patients, has not been extensively studied. We performed a study to compare the level of spontaneous T cell apoptosis and anti-retroviral treatments in a cohort of HIV-1-infected patients. Data were obtained from a computerized medical record. Quantification of apoptotic cells was by cytofluorometric technique. From November 1995 to December 1997 we studied T cell apoptosis in 112 HIV-infected patients. Forty patients were classified A, 36 B and 36 C. Thirty patients were naive and 82 received an anti-retroviral treatment, 49 including a protease inhibitor (PI). The median plasma viraemia determined in 63 patients was 3.6 (range 1.3-5.6) log10. The median apoptotic cell count was 22% (range 2-73%) and 12% (range 2-60%) for CD4+ and CD8+ T cells, respectively. We did not observe any correlation between the HIV viraemia and the level of apoptosis of T cell subsets. Patients with HAART showed a lower percentage of apoptotic CD4+ T cells only: 16% (range 2-61%) versus 25% (range 5-73%) for patients receiving two nucleoside analogues (P = 0.02). This effect was significant in stage A patients and remained observable during the whole course of HIV disease. In conclusion, HAART, without any relation to plasma viraemia, is able to reduce apoptosis of CD4+ T cells.},
 Keywords = {Adult
Aged
Anti-HIV Agents/*therapeutic use
*Apoptosis
CD4-Positive T-Lymphocytes/cytology/*drug effects
CD8-Positive T-Lymphocytes/drug effects
Didanosine/therapeutic use
Drug Therapy, Combination
Female
HIV Infections/*drug therapy/immunology/pathology
HIV Protease Inhibitors/therapeutic use
Human
Lamivudine/therapeutic use
Male
Middle Aged
Multivariate Analysis
Retrospective Studies
Stavudine/therapeutic use
Viral Load
Zalcitabine/therapeutic use
Zidovudine/therapeutic use},
   Year = {1999} }



@article{
Stoddart01,
   Author = {Stoddart, C. A. and Liegler, T. J. and Mammano, F. and Linquist-Stepps, V. D. and Hayden, M. S. and Deeks, S. G. and Grant, R. M. and Clavel, F. and McCune, J. M.},
   Title = {Impaired replication of protease inhibitor-resistant HIV-1 in human thymus},
   Journal = {Nat Med},
   Volume = {7},
   Number = {6},
   Pages = {712-8},
   Note = {1078-8956
Journal Article},
   Abstract = {Many HIV-1-infected patients treated with protease inhibitors (PI) develop PI-resistant HIV-1 variants and rebounds in viremia, but their CD4+ T-cell counts often do not fall. We hypothesized that in these patients, T-cell counts remain elevated because PI-resistant virus spares intrathymic T-cell production. To test this, we studied recombinant HIV-1 clones containing wild-type or PI-resistant protease domains, as well as uncloned isolates from patients, in activated peripheral blood mononuclear cells, human thymic organ cultures and human thymus implants in SCID-hu Thy/Liv mice. In most cases, wild-type and PI-resistant HIV-1 isolates replicated to similar degrees in peripheral blood mononuclear cells. However, the replication of PI-resistant but not wild-type HIV-1 isolates was highly impaired in thymocytes. In addition, patients who had PI-resistant HIV-1 had abundant thymus tissue as assessed by computed tomography. We propose that the inability of PI-resistant HIV-1 to replicate efficiently in thymus contributes to the preservation of CD4+ T-cell counts in patients showing virologic rebound on PI therapy.},
 Keywords = {Adult
Animals
CD4 Lymphocyte Count
Drug Resistance, Microbial
Fetal Tissue Transplantation
Flow Cytometry
HIV Core Protein p24/metabolism
HIV Infections/immunology/pathology/*virology
HIV Protease/genetics/*metabolism
HIV Protease Inhibitors/*pharmacology
HIV-1/*drug effects/enzymology/genetics/*physiology
Human
Mice
Mice, SCID
Middle Aged
Organ Culture
Recombination, Genetic
Support, Non-U.S. Gov't
Support, U.S. Gov't, P.H.S.
T-Lymphocytes/*physiology/virology
Thymus Gland/pathology/physiopathology/transplantation/*virology
Viral Load
*Virus Replication},
   Year = {2001} }



@article{
Sufka03,
   Author = {Sufka, S. A. and Ferrari, G. and Gryszowka, V. E. and Wrin, T. and Fiscus, S. A. and Tomaras, G. D. and Staats, H. F. and Patel, D. D. and Sempowski, G. D. and Hellmann, N. S. and Weinhold, K. J. and Hicks, C. B.},
   Title = {Prolonged CD4+ cell/virus load discordance during treatment with protease inhibitor-based highly active antiretroviral therapy: immune response and viral control},
   Journal = {J Infect Dis},
   Volume = {187},
   Number = {7},
   Pages = {1027-37},
   Note = {0022-1899
Clinical Trial
Journal Article},
   Abstract = {Mechanisms that underly discordant CD4+ cell/virus load (VL) responses in patients who receive highly active antiretroviral therapy (HAART) were studied in 30 human immunodeficiency virus (HIV)-positive patients, in 3 groups. Discordant responders maintained CD4+ cell levels >200/mm(3) with stable or increasing trend, despite sustained VLs of 500-5000 copies/mL, for >2 years. Treatment-success patients had CD4+ cell counts >200/mm(3) with stable or increasing trend and VLs <50 copies/mL, for >2 years. Treatment-failure patients initially responded to HAART, followed by decreasing CD4+ cell counts and increasing VLs. Interferon-gamma production to gag and noncytolytic CD8+ cell suppressive activity were greater in discordant responders. Cellular activation was greatest in patients with treatment failure. All discordant responders had non-syncytium-inducing (CCR5-tropic) viruses. Viruses from discordant responders and from patients with treatment failure had extensive resistance mutations; discordant responders had significantly lower viral replication capacities. These findings suggest that discordant responses may be related to enhanced HIV-directed immune responses, diminished cellular activation, decreased viral replication capacity, and preservation of non-syncytium-inducing virus strains.},
 Keywords = {Adult
*Antiretroviral Therapy, Highly Active
*CD4 Lymphocyte Count
Female
HIV/*drug effects
HIV Infections/*drug therapy/*immunology/virology
HIV Protease Inhibitors/*pharmacology/therapeutic use
Human
Male
Middle Aged
Support, Non-U.S. Gov't
Support, U.S. Gov't, P.H.S.
Time Factors
Treatment Failure
*Viral Load
Virus Replication/drug effects},
   Year = {2003} }



@article{
Tebaldi03,
   Author = {Tedaldi, E. M. and Baker, R. K. and Moorman, A. C. and Alzola, C. F. and Furhrer, J. and McCabe, R. E. and Wood, K. C. and Holmberg, S. D.},
   Title = {Influence of coinfection with hepatitis C virus on morbidity and mortality due to human immunodeficiency virus infection in the era of highly active antiretroviral therapy},
   Journal = {Clin Infect Dis},
   Volume = {36},
   Number = {3},
   Pages = {363-7},
   Note = {1537-6591
Journal Article},
   Abstract = {To ascertain the impact of hepatitis C virus (HCV) infection on human immunodeficiency virus (HIV) disease progression and associated death in the era of highly active antiretroviral therapy (HAART), we examined mortality rates, the presence of other diseases, and antiretroviral use in an observational cohort of 823 HIV-infected patients with and without HCV coinfection during the period of January 1996 through June 2001. Analyses were used to compare patient characteristics, comorbid conditions, and survival durations in HIV-infected and HIV-HCV-coinfected patients. HIV-HCV-coinfected persons did not have a statistically greater rate of acquired immunodeficiency syndrome or of renal or cardiovascular disease, but they did have more cases of cirrhosis and transaminase elevations. There were proportionately more deaths in the HIV-HCV-coinfected group. Age, baseline CD4+ cell count, and duration of HAART were significantly associated with survival, but HCV infection was not. HAART use was a strong predictor of increased duration of survival, suggesting that treatment is more important to survival than is HCV coinfection status.},
 Keywords = {Anti-HIV Agents/therapeutic use
*Antiretroviral Therapy, Highly Active
*Hiv
HIV Infections/*complications/drug therapy/epidemiology/mortality
*Hepacivirus
Hepatitis C/*complications/epidemiology/mortality
Human
Morbidity
Mortality
Support, U.S. Gov't, P.H.S.},
   Year = {2003} }




@string{JASA= {Journal of the American Statistical Association}}
@string{JC = {Journal of Classification}}
@string{JSPI = {Journal of Statistical Planning and Inference}}
@string{JRSSB = {Journal of the Royal Statistical Society, Series B}}
@string{PNAS = {Proc. Natl. Acad. Sci.}}

@Article{Wang&Bembom&vanderLaan06,
  author =   {Y. Wang and O. Bembom and M.J. van der Laan},
  title =    {Data adaptive estimation of the treatment specific mean},
  journal =      {Journal of Statistical Planning and Inference},
  year =     {2006},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {also http://www.bepress.com/ucbbiostat/paper159},
  OPTannote =    {}
}
@Article{Sinisi&vanderLaan04,
  author =   {S. Sinisi and M.J. van der Laan},
  title =    {The deletion/substitution/addition algorithm in loss function based estimation:
Applications in Genomics},
  journal =      {Journal of Statistical Methods in Molecular Biology},
  year =     {2004},
  OPTkey =   {},
  volume =   {3},
  number =   {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/sagmb/vol3/iss1/art18},
  OPTannote =    {}
}



@TECHREPORT{Petersen&Deeks&Martin&vanderLaan05,
  author =       {Maya L. Petersen and Steven G. Deeks and Jeffrey N. Martin and Mark J. van der Laan},
  title =        {History-Adjusted Marginal Structural Models: Time-Varying Effect Modification
  and Dynamic Treatment Regimens},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2005},
  type =         {Technical Report 199},
OPTnote =      {http://www.bepress.com/ucbbiostat/paper199},
  month =        {December},
}

@TECHREPORT{vanderLaan&Rubin05,
  author =       {M.J. van der Laan and D. Rubin},
  title =        {Estimating Function Based Cross-Validation and Learning},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2005},
  type =         {Technical Report 180},
OPTnote =      {http://www.bepress.com/ucbbiostat/paper180},
  month =        {},
}

@Article{vanderLaan&Petersen07,
  author =   {M.J. van der Laan and M.L. Petersen},
  title =    {Causal Effect Models for Realistic Individualized Treatment and Intention to Treat Rules},
  journal =      {International Journal of Biostatistics},
  year =     {2007},
  OPTkey =   {},
  volume =   {3},
  number =   {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/ijb/vol3/iss1/art3},
  OPTannote =    {}
}


@TECHREPORT{vanderLaan06,
  author =       {M.J. van der Laan},
  title =        {Causal Effect Models for Intention to Treat and Realistic Individualized
  Treatment Rules},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2006},
  type =         {Technical Report 203},
OPTnote =      {http://www.bepress.com/ucbbiostat/paper203},
  month =        {},
}
@TECHREPORT{vanderLaan08b,
  author =       {M.J. van der Laan},
  title =        {The construction and analysis of adaptive group sequential designs},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2008},
  type =         {Technical Report 232},
OPTnote =      {http://www.bepress.com/ucbbiostat/paper232},
  month =        {March},
}
@TECHREPORT{Moore&vanderLaan07,
  author =       {K.L. Moore and M.J. van der Laan},
  title =        {Covariate adjustment in randomized trials with binary outcomes},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2007},
  type =         {Technical Report 215},
OPTnote =      {http://www.bepress.com/ucbbiostat/paper215},
  month =        {April},
}

@TECHREPORT{vanderLaan&Petersen05,
  author =       {M.J. van der Laan and M.L. Petersen},
  title =        {Direct Effect Models},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2005},
  type =         {Technical Report 187},
OPTnote =      {http://www.bepress.com/ucbbiostat/paper187},
  month =        {},
}
@TECHREPORT{Petersen&vanderLaan06,
  author =       {M.L. Petersen and M.J. van der Laan},
  title =        {Individualized Treatment Rules and Clinical Trials},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2006},
  type =         {Technical Report},
OPTnote =      {},
  month =        {},
}

@Article{vanderLaan&Petersen&Joffe05,
  author =   {M.J. van der Laan and M.L. Petersen and M.M. Joffe},
  title =    {History-Adjusted Marginal Structural Models and Statically-Optimal Dynamic Treatment Regimens},
  journal =      {The International Journal of Biostatistics},
  year =     {2005},
  OPTkey =   {},
  volume =   {1},
  number =   {1},
  pages =    {10-20},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/ijb/vol1/iss1/4},
  OPTannote =    {}
}

@Article{vanderLaan06a,
  author =   {M.J. van der Laan},
  title =    {Statistical Inference for Variable Importance},
  journal =      {International Journal of Biostatistics},
  year =     {2006},
  OPTkey =   {},
  volume =   {2},
  number =   {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/ijb/vol2/iss1/art2},
  OPTannote =    {}
}

@Article{vanderLaan&Birkner&Hubbard05,
  author =   {M.J. van der Laan and M.D. Birkner and A.E. Hubbard},
  title =    {Empirical Bayes and resampling based multiple testing procedure controlling tail probability of the proportion of false positives},
  journal =      {Journal of Statistical Applications in Genetics and Molecular Biology},
  year =     {2005},
  OPTkey =   {},
  volume =   {4},
  number =   {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/sagmb/vol4/iss1/art29},
  OPTannote =    {}
}



@Article{vanderLaan&Dudoit&Pollard04b,
  author =   {M.J. van der Laan and S. Dudoit and K.S. Pollard},
  title =    {Augmentation procedures for control of the generalized family-wise
  error rate and tail probabilities for the proportion of false positives},
journal =      {Journal of Statistical Applications in Genetics and Molecular Biology},
  year =     {2004},
  OPTkey =   {},
  volume =   {3},
  number =   {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/sagmb/vol3/iss1/art15},
  OPTannote =    {}
}
@Article{vanderLaan&Dudoit&Pollard04,
  author =   {S. Dudoit and M.J. van der Laan and K.S. Pollard},
  title =    {Multiple testing. Part II.
  Step-down procedures for control of the family-wise error rate
  },
journal =      {Journal of Statistical Applications in Genetics and Molecular Biology},
  year =     {2004},
  OPTkey =   {},
  volume =   {3},
  number =   {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/sagmb/vol3/iss1/art14},
  OPTannote =    {}
}

@Article{Dudoit&vanderLaan&Pollard04,
  author =   {S. Dudoit and M.J. van der Laan and K.S. Pollard},
  title =    {Multiple testing. Part I. Single-step procedures for control of general Type I error rates},
journal =      {Journal of Statistical Applications in Genetics and Molecular Biology},
  year =     {2004},
  OPTkey =   {},
  volume =   {3},
  number =   {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/sagmb/vol3/iss1/art13},
  OPTannote =    {}
}


@Article{Birkner&Sinisi&vanderLaan05,
  author =   {M.D. Birkner and S.E. Sinisi and M.J. van der Laan},
  title =    {Multiple Testing and Data Adaptive Regression: An Application
  to {HIV}-1 Sequence Data},
  journal =      {Journal of Statistical Applications in Genetics and Molecular Biology},
  year =     {2005},
  OPTkey =   {},
  volume =   {4},
  number =   {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/sagmb/vol4/iss1/art8},
  OPTannote =    {}
}

@TECHREPORT{vanderLaan&Hubbard06,
  author =       {M.J. van der Laan and A.E. Hubbard},
  title =        {Quantile-Function Based Null Distribution in Resampling Based Multiple Testing},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2006},
  type =         {Technical Report},
OPTnote =      {http://www.bepress.com/ucbbiostat/paper198},
  month =        {},
}
@TECHREPORT{Molinaro&vanderLaan04,
  author =       {A. Molinaro and M.J. van der Laan},
  title =        {Deletion/Substitution/Addition Algorithm for Partitioning the Covariate Space in Prediction},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2004},
  type =         {Technical Report},
OPTnote =      {http://www.bepress.com/ucbbiostat/paper162},
  month =        {},
}
@TECHREPORT{Birkner&vanderLaan05,
  author =       {M.D. Birkner and M.J. van der Laan},
  title =        {Application of a Variable Importance Measure Method to {HIV}-1 Sequence Data},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2005},
  type =         {Technical Report},
  month =        {},
}



@TECHREPORT{Neugebauer&vanderLaan05b,
  author =       {R. Neugebauer and M.J. van der Laan},
  title =        {Locally Efficient Estimation of Nonparametric
                    Causal Effects on Mean Outcomes in Longitudinal Studies},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2005},
  number =       {134},
  type =         {Technical Report},
OPTnote =    {http://www.bepress.com/ucbbiostat/paper134, to appear in {JSPI}},
  month =        {},
}
@TECHREPORT{Wang&Petersen&vanderLaan06,
  author =       {Y. Wang and M. Petersen and M.J. van der Laan},
  title =        {A statistical method for diagnosing ETA bias in IPTW estimators},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2006},
  number =       {},
  type =         {Technical Report},
OPTnote =    {},
  month =        {},
}

@TECHREPORT{Moore&vanderLaan07,
  author =       {K.L. Moore and M.J. van der Laan},
  title =        {Covariate adjustment in randomized trials with binary outcomes},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2007},
  type =         {Technical Report 215},
OPTnote =    {http://www.bepress.com/ucbbiostat/paper215},
  month =        {April},
}

@TECHREPORT{vanderLaan&Dudoit&vanderVaart,
  author =       {M.J. van der Laan and S. Dudoit and A.W. van der Vaart},
  title =        {The Cross-Validated Adaptive Epsilon-Net Estimator},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2004},
  type =         {Technical Report 142},
OPTnote =    {http://www.bepress.com/ucbbiostat/paper142},
  month =        {February},
}

@TECHREPORT{vanderLaan&DudoitTechRep130,
  author =       {M.J. van der Laan and S. Dudoit},
  title =        {Unified cross-validation methodology for selection among estimators
  and a general cross-validated adaptive epsilon-net estimator: Finite sample oracle
  inequalities and examples},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2003},
  type =         {Technical Report},
OPTnote =    {http://www.bepress.com/ucbbiostat/paper130},
  month =        {November},
}

@TECHREPORT{Petersen&vanderLaan05,
  author =       {M. Petersen and M.J. van der Laan},
  title =        {Estimation of direct and indirect causal effects in
Epidemiology},
  institution =  {Division of Biostatistics, University of California,
Berkeley},
  year =         {2005},
  type =         {Technical Report},
  month =        {},
}

@TECHREPORT{Petersen&Deeks&Martin&vanderLaan05,
  author =       {M.L. Petersen and S.G. Deeks and J.N. Martin and M.J. van der Laan},
  title =        {History-Adjusted Marginal Structural Models: Time-Varying Effect Modification and Dynamic Treatment Regimens},
  institution =  {Division of Biostatistics, University of California,
Berkeley},
  year =         {2005},
  type =         {Technical Report 199},
OPTnote =      {http://www.bepress.com/ucbbiostat/paper199},
  month =        {},
}

@TECHREPORT{vanderLaan&Petersen04,
  author =       {M.J. van der Laan and M. Petersen},
  title =        {Estimation of direct and indirect causal effects in longitudinal studies},
  institution =  {Division of Biostatistics, University of California,
Berkeley},
  year =         {2004},
  type =         {Technical Report 155},
  month =        {August},
}

@TECHREPORT{vanderLaan&Hubbard&Jewell04,
 author =       {M.J. van der Laan and A.E. Hubbard and N.P. Jewell},
  title =        {Estimation of Treatment Effects in Randomized Trials with Noncompliance and a Dichotomous Outcome},
  institution =  {Division of Biostatistics, University of California,
Berkeley},
  year =         {2004},
  type =         {Technical Report 157},
  OPTnote =      {http://www.bepress.com/ucbbiostat/paper157},
month =        {September},
}
@TECHREPORT{Bein&Hubbard&vanderLaan05,
 author =       {E. Bein and A.E. Hubbard and M.J. van der Laan},
  title =        {Estimating Function Based Cross-Validation in
Estimation of the Causal Effect in Randomized Trials},
  institution =  {Division of Biostatistics, University of California,
Berkeley},
  year =         {2005},
  type =         {Technical Report},
}





@TECHREPORT{vanderLaan&DudoitTechRep130,
  author =       {M.J. van der Laan and S. Dudoit},
  title =        {Unified cross-validation methodology for
selection among estimators and a general cross-validated adaptive
epsilon net estimator: Finite sample oracle inequalities and
examples},
  institution =  {Division of Biostatistics, University of California,
Berkeley},
  year =         {2003},
  type =         {Technical Report 130},
  month =        {Nov.},
}


@TECHREPORT{Molinaroetal05,
  author =       {A.M. Molinaro and M.J. van der Laan and D.H. Moore and K. Kerlikowske},
  title =        {Survival point estimate prediction in matched and non-matched case-control subsample designed studies},
  institution =  {Division of Biostatistics, University of California,
Berkeley},
  year =         {2005},
  note =         {http://www.bepress.com/ucbbiostat/paper149},
}


@TECHREPORT{DudoitetalSIGKDD04,
  author =       {S. Dudoit and M.J. van der Laan and S. Kele\c{s} and A.
M. Molinaro and S. E. Sinisi
and S.L. Teng},
  title =        {Loss-Based Estimation with Cross-Validation:
Applications to Microarray Data
Analysis and Motif Finding.},
  institution =  {Division of Biostatistics, University of California,
Berkeley},
  year =         {2004},
  note =         {to appear in \emph{SIGKDD} Explorations on Microarray Data Mining},
}

@Book{Friedman&Furberg&Demets98,
  author =       {L.M.Friedman and C.D. Furberg and D.L. DeMets},
  title =        {Fundamentals of Clinical Trials},
  publisher =    {Springer-Verlag New York},
  year =         {1998}
}

@Book{ABGK,
  author =       {P.K. Andersen and O. Borgan and R.D. Gill and N. Keiding},
  title =        {Statistical Models Based on Counting Processes},
  publisher =    {Springer-Verlag New York},
  year =         {1993}
}
@Article{Wittes&Brittain90,
  author =   {J. Wittes and E. Brittain},
  title =    {The role of internal pilot studies in increasing efficiency of clinical trials},
journal =      {Statistics in Medicine},
  year =     {1999},
  OPTkey =   {},
  volume =   {9},
  number =   {},
  pages =    {65--72},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

%references for direct and indirect effects:
@InCollection{Robins03,
  author =   {J.M. Robins},
  title =    {Semantics of causal DAG models and the identification of direct and
indirect effects},
  booktitle =    {Highly Structured Stochastic Systems},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher = {Oxford University Press, Oxford},
  year =     {2003},
  editor =   {P. Green, N. Hjort, and S. Richardson},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {70--81},
  OPTnote =      {},
  OPTannote =    {}
}

@InCollection{Hubbard&vanderLaan&Robins99,
  author =   {A. Hubbard and M.J. van der Laan and J.M. Robins},
  title =    {Nonparametric locally ecient
estimation of the treatment specic survival distribution with right censored data
and covariates in observational studies},
  booktitle =    {Statistical Models in Epidemiology, The Environment and Clinical Trials},
  publisher = {Springer Verlag},
  year =     {1999},
editor={M.E. Halloran and D. Berry},
volume={116},
pages={135--178},
  series =   {IMA Volumes in Mathematics and its Applications, Ed. M.E. Halloran and D. Berry}
}

@TechReport{Pearl01,
  author =   {J. Pearl},
  title =    {Cognitive systems Laboratory},
  institution =  {University of California, Los Angeles, Department of Computer Science},
  year =     {2001},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Pearl00,
  author =   {J. Pearl},
  title =    {Causality: Models, Reasoning, and Inference},
  publisher =    {Cambridge University Press, Cambridge},
  year =     {2000},
  OPTkey =   {},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  series =   {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Robins&Greenland92,
  author =   {J.M. Robins and S. Greenland},
  title =    {Identifiability and exchangeability for direct and indirect
effects},
  journal =      {Epidemiology},
  year =     {1992},
  OPTkey =   {},
  volume =   {3},
  number =   {0},
  pages =    {143--155},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{vanderLaan95,
  author =   {M.J. van der Laan},
  title =    {Identity for NPMLE in missing data and biased sampling models},
  journal =      {Bernoulli},
  year =     {1995},
  OPTkey =   {},
  volume =   {1},
  number =   {4},
  pages =    {335--341},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{vanderLaan98,
  author =   {M.J. van der Laan},
  title =    {Identity for NPMLE in Censored Data Models},
  journal =      {Lifetime Data Models},
  year =     {1998},
  OPTkey =   {},
  volume =   {4},
  number =   {0},
  pages =    {83--102},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Klaassen86,
  author =   {C.A.J. Klaassen},
  title =    {Consistent estimation of the influence function of locally asymptotically linear estimators},
  journal =      {Annals of Statistics},
  year =     {1987},
  OPTkey =   {},
  volume =   {15},
  number =   {},
  pages =    {1548--1562},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}





%the next references are for instrumental variable article
@Article{Robins&Rotnitzky04,
  author =   {J.M. Robins and A. Rotnitzky},
  title =    {Estimation of Treatment Effects in Randomized Trials
with Noncompliance and a Dichotomous Outcome using Structural Nested
Mean Models},
  journal =      {Biometrika},
  year =     {2004},
  OPTkey =   {},
  volume =   {0},
  number =   {0},
  pages =    {0},
  OPTmonth =     {},
  OPTnote =      {To Appear},
  OPTannote =    {}
}

@Article{Vandervaart91,
  author =   {A.W. van der Vaart},
  title =    {On differentiable functionals},
  journal =      {Annals of Statistics},
  year =     {1991},
  OPTkey =   {},
  volume =   {19},
  number =   {},
  pages =    {178--204},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}




@Article{Rubin78,
  author =   {D.B. Rubin},
  title =    {Bayesian Inference for causal effects: the role of randomization},
  journal =      {Annals of Statistics},
  year =     {1978},
  OPTkey =   {},
  volume =   {6},
  number =   {},
  pages =    {34--58},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Neyman23,
  author =   {Neyman, J.},
  title =    {On the application of probability theory to agricultural
experiments},
  journal =      {Statistical Science},
  year =     {1990},
  OPTkey =   {},
  volume =   {5},
  number =   {},
  pages =    {465--480},
  OPTmonth =     {},
  OPTnote =      {Translation of 1923 article},
  OPTannote =    {}
}
@Article{Robins86,
  author =   {J.M. Robins},
  title =    {A new approach to causal inference in mortality studies with sustained exposure periods - Application to control of the healthy worker survivor effect},
  journal =      {Mathematical Modelling},
  year =     {1986},
  OPTkey =   {},
  volume =   {7},
  number =   {},
  pages =    {1393--1512},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}





@Article{Robins94,
  author =   {J.M. Robins},
  title =    {Correcting for non-compliance in randomized trials
using structural nested mean models},
  journal =      {Communications in Statistics},
  year =     {1994},
  OPTkey =   {},
  volume =   {23},
  number =   {},
  pages =    {2379--2412},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Vansteelandt03,
  author =   {S. Vansteelandt and E. Goetghebeur},
  title =    {Causal inference with generalized structural  mean
models},
  journal =      {Journal of the Royal Statistical Society, Series B},
  year =     {2003},
  OPTkey =   {},
  volume =   {23},
  number =   {},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {In print},
  OPTannote =    {}
}

@incollection {Robins97a,
   AUTHOR = {Robins, J.M.},
    TITLE = {Structural Nested Failure Time Models},
BOOKTITLE = {The Encyclopedia of Biostatistics},
PUBLISHER = {John Wiley and Sons},
  ADDRESS = {Chichester, UK},
     YEAR = {1997},
   EDITOR = {Armitage, P. and Colton, T. and Andersen, P.K. and Keiding, N.}
}
@article {hernan_brumback_robins,
   AUTHOR = {Hernan, M. A. and Brumback, B. and Robins, J. M.},
    TITLE = {Marginal structural models to estimate the causal effect of zidovudine on the survival of {HIV}-positive men},
  JOURNAL = {Epidemiology},
   VOLUME = {11},
   NUMBER = {5},
     YEAR = {2000},
    PAGES = {561--570}
}
@article {Robins87,
   AUTHOR = {Robins, J.M.},
    TITLE = {Addendum to: ``{A} new approach to causal inference in
             mortality studies with a sustained exposure
             period---application to control of the healthy worker survivor
             effect'' [{M}ath.\ {M}odelling {\bf 7} (1986), no.\ 9-12,
             1393--1512; {M}{R} 87m:92078]},
  JOURNAL = {Comput. Math. Appl.},
 FJOURNAL = {Computers \& Mathematics with Applications. An International
             Journal},
   VOLUME = {14},
     YEAR = {1987},
   NUMBER = {9-12},
    PAGES = {923--945},
     ISSN = {0097-4943},
    CODEN = {CMAPDK},
}

@article {robins_hernan_brumback,
   AUTHOR = {Robins, J. M. and Hernan, M. A. and Brumback, B.},
    TITLE = {Marginal structural models and causal inference in epidemiology},
  JOURNAL = {Epidemiology},
   VOLUME = {11},
   NUMBER = {5},
     YEAR = {2000},
    PAGES = {550--560}
}





@article {Bryan&Yu&vanderLaan03,
   AUTHOR = {Bryan, J. and Yu, Z. and van der Laan, M.J.},
    TITLE = {Analysis of Longitudinal Marginal Structural Models},
  JOURNAL = {Biostatistics},
   VOLUME = {5},
   NUMBER = {3},
     YEAR = {2003},
    PAGES = {361--380}
}

@TechReport{Yu&vanderLaan03,
  author =   {Yu, Z. and van der Laan, M.J.},
  title =    {Double Robust Estimation in Longitudinal Marginal Structural
                    Models},
  institution =  {Division of Biostatistics, University of California,
Berkeley},
  year =     {2003},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {132},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/ucbbiostat/paper132},
  OPTannote =    {}
}

@Article{Neugebauer&vanderLaan05,
  author =   {Neugebauer, R. and van der Laan, M.J.},
  title =    {Why prefer double robust estimates},
  journal =      {Journal of Statistical Planning and Inference},
  year =     {2005},
  OPTkey =   {},
  volume =   {129},
  number =   {1-2},
  pages =    {405--426},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@article {Murphy03,
   AUTHOR = {Murphy, S.A.},
    TITLE = {Optimal dynamic treatment regimes},
  JOURNAL = {Journal of the Royal Statistical Society: Series B},
   VOLUME = {65},
   NUMBER = {2},
     YEAR = {2003},
    PAGES = {?}
}
@article {Robins03a,
   AUTHOR = {Robins, J.M.},
    TITLE = {Discussion of ''{O}ptimal dynamic treatment regimes" by {S}usan {A}. {M}urphy},
  JOURNAL = {Journal of the Royal Statistical Society: Series B},
   VOLUME = {65},
   NUMBER = {2},
     YEAR = {2003},
    PAGES = {355--366}
}

@article {Murphy&vanderLaan&Robins01,
   AUTHOR = {S.A. Murphy and M.J. van der Laan and J.M. Robins},
    TITLE = {Marginal mean models for dynamic treatment regimens},
  JOURNAL = {Journal of the American Statistical Association},
   VOLUME = {96},
   NUMBER = {},
     YEAR = {2001},
    PAGES = {1410--1424}
}
@incollection {Robins98,
    AUTHOR = {Robins, J.M.},
     TITLE = {Marginal structural models versus structural nested models as
              tools for causal inference},
 BOOKTITLE = {Statistical models in epidemiology, the environment, and
              clinical trials (Minneapolis, MN, 1997)},
     PAGES = {95--133},
 PUBLISHER = {Springer},
   ADDRESS = {New York},
      YEAR = {2000},
   MRCLASS = {62N01 (62G08 62P10)},
  MRNUMBER = {2001a:62124},
}
%Robins, J.M. (2003). Discussion of "Optimal dynamic treatment regimes". by Susan A. Murphy.
  %Journal of the Royal Statistical Society: Series B, 65(2):355-366.
@InCollection{Robins97,
  author =   {J.M. Robins},
  title =    {Causal Inference from Complex Longitudinal Data},
  booktitle =    {Latent Variable Modeling and Applications to Causality},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher = {Springer Verlag, New York},
  year =     {1997},
  editor =   {M. Berkane, Editor},
  OPTvolume =    {120},
  OPTnumber =    {},
  OPTseries =    {Lecture Notes in Statistics},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {69--117},
  OPTnote =      {},
  OPTannote =    {}
}

@InCollection{Robins89,
  author =   {J.M. Robins},
  title =    {The analysis of randomized and non-randomized AIDS
treatment trials using a new approach in causal inference in longitudinal studies},
  booktitle =    {Health Service Methodology: A Focus on AIDS},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher = {U.S. Public Health Service, National Center for Health SErvices Research},
  year =     {1989},
  editor =   {L. Sechrest and H. Freeman and A. Mulley},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {Lecture Notes in Statistics},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {Washington D.C.},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {113--159},
  OPTnote =      {},
  OPTannote =    {}
}



@TechReport{Abadie00,
  author =   {A. Abadie},
  title =    {Semiparametric estimation of instrumental variables models for causal effects},
  institution =  {NBER Technical Working Paper},
  year =     {2000},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {260},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Abadie03,
  author =   {A. Abadie},
  title =    {Semiparametric instrumental variable estimation of treatment response models},
  journal =      {Journal of Econometrics},
  year =     {2003},
  OPTkey =   {},
  volume =   {113},
  number =   {},
  pages =    {231-263},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Abadie03,
  author =   {A. Abadie},
  title =    {Semiparametric instrumental variable estimation of treatment response models},
  journal =      {Journal of Econometrics},
  year =     {2003},
  OPTkey =   {},
  volume =   {113},
  number =   {},
  pages =    {231-263},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@TechReport{Wang&Vanderlaan04,
  author =   {Y. Wang and M.J. van der Laan},
  title =    {Data adaptive estimation of the treatment specific mean},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =     {2004},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {159},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/ucbbiostat/paper159},
  OPTannote =    {}
}
@TechReport{Yu&vanderLaan02,
  author =   {Z. Yu and M.J. van der Laan},
  title =    {Construction of counterfactuals and the {G}-computation formula},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =     {2002},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {122},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/ucbbiostat/paper122},
  OPTannote =    {}
}
@TechReport{Yu&Vanderlaan03,
  author =   {Z. Yu and M.J. van der Laan},
  title =    {Measuring treatment effects using semiparametric models},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =     {2003},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {136},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/ucbbiostat/paper136},
  OPTannote =    {}
}

@Article{Angristetal96,
  author =   {J. Angrist and G. Imbens and D.B. Rubin},
  title =    {Identification of causal effects using instrumental variables},
  journal =      {Journal of the American Statistical Association},
  year =     {1996},
  OPTkey =   {},
  volume =   {91},
  number =   {},
  pages =    {444-555},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Robins&Rotnitzky01A,
  author =   {J.M Robins and A. Rotnitzky},
  title =    {Comment on {I}nference for semiparametric models: some questions
  and an answer, by {B}ickel, {P}.{J}. and {K}won, {J}.},
  journal =      {Statistica Sinica},
  year =     {2001},
  OPTkey =   {},
  volume =   {11},
  number =   {},
  pages =    {920-935},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Angrist01,
  author =   {J. Angrist},
  title =    {Estimation of limited dependent variable models with dummy endogenous regressors: simple strategies for empirical practice},
  journal =      {Journal of Business and Economics Statistics},
  year =     {2001},
  OPTkey =   {},
  volume =   {19},
  number =   {},
  pages =    {1--16},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Chamberlain87,
  author =   {G. Chamberlain},
  title =    {Asymptotic efficiency in estimation with conditional moment
restrictions},
  journal =      {Journal of Econometrics},
  year =     {1987},
  OPTkey =   {},
  volume =   {34},
  number =   {},
  pages =    {305--334},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Hiranoetal00,
  author =   {K. Hirano and G. Imbens and D.B. Rubin and X-H. Zhou},
  title =    {Assessing the effects of influenza vaccine in an encouragement design},
  journal =      {Biostatistics},
  year =     {2000},
  OPTkey =   {},
  volume =   {1},
  number =   {},
  pages =    {69--88},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Neyman23,
  author =   {J. Neyman},
  title =    {Sur les applications de la thar des probabilites aux
experiences Agaricales: Essay des principle (1923). Excerpts reprinted (1990) in
English (D. Dabrowska and T. Speed), Trans.},
  journal =      {Statistical Science},
  year =     {1990},
  OPTkey =   {},
  volume =   {5},
  number =   {},
  pages =    {463--472},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



optimal structural nested models for optimal
sequential decisions Proceedings of the 2nd seattle symposium in
biostatistics eds. Lin DY, Heagerty PJ  Springer Verlag Lecture Notes in
Statisitics No. 179  pages 189-326

@InProceedings{Robins05,
  author =   {J.M. Robins},
  title =    {Optimal structural nested models for optimal sequential decisions},
  booktitle =    {Proceedings of the 2nd Seattle symposium in
biostatistics},
  pages =    {189--326},
  year =     {2005},
  editor =   {Lin, D.Y, Heagerty P.J},
  volume =   {179},
  organization = {},
OPTpublisher = {Springer Verlag Lecture Notes in Statistics}
}


@TechReport{Robins05tech,
  author =   {J.M. Robins},
  title =    {Optimal structural nested models for optimal sequential decisions},
  institution =  {Department of Biostatistics, Havard University},
  year =     {2005},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}





@InProceedings{AIC,
  author =   {H. Akaike},
  title =    {Information theory and an extension of the maximum likelihood principle},
  booktitle =    {Second International Symposium on Information Theory},
  pages =    {267-281},
  year =     {1973},
  editor =   {B.N. Petrov and F. Csaki},
  organization = {Budapest: Academiai Kiado}
}


@Article{Balke&Pearl97,
  author =   {A. Balke and J. Pearl},
  title =    {Bound on treatment effects from studies with imperfect compliance},
  journal =      {Journal of the American Statistical Association},
  year =     {1997},
  OPTkey =   {},
  volume =   {92},
  number =   {},
  pages =    {1172--1176},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{Balke&Pearl94,
author =     {A. Balke and J. Pearl},
  title =    {Counterfactual probabilities: Computational methods, bounds, and applications},
  booktitle =    {In Proceedings of the 12th National Conference on Artificial Intelligence},
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {230--237},
  year =     {1994},
  OPTeditor =    {},
  volume =   {I},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {Menlo Park, CA},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {MIT Press},
  OPTnote =      {},
  OPTannote =    {}
}






@Article{Ambroise&McLachlan02,
  author =   {C. Ambroise and G. J. McLachlan},
  title =    {Selection bias in gene extraction on the basis of microarray gene-expression data},
  journal =      PNAS,
  year =     {2002},
  OPTkey =   {},
  volume =   {99},
  number =   {10},
  pages =    {6562--6566},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@InCollection{Arabie&Hubert96,
  author =   {P. Arabie and L. J. Hubert},
  title =    {An overview of combinatorial data analysis},
  booktitle =    {Clustering and Classification},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher = {World Scientific Publishing Co.},
  year =     {1996},
  editor =   {P. Arabie and L. J. Hubert and G. De Soete},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {River Edge, NJ},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {5--63},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{BIC,
  author =   {G. Schwartz},
  title =    {Estimating the Dimension of a Model},
  journal =      {Annals of Statistics},
  year =     {1978},
  volume =   {6},
  pages =    {461-464}
}


@Article{Barnard,
  author =   {M. Barnard},
  title =    {The secular variations of skull characters in four series of Egyptian skulls},
  journal =      {Annals of Eugenics},
  year =     {1935},
  OPTkey =   {},
  volume =   {6},
  OPTnumber =    {},
  pages =    {352--371},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@InProceedings{BenHuretal02,
  author =   {A. Ben-Hur and A. Elisseeff and I. Guyon},
  title =    {A stability based method for discovering structure in clustered data},
  booktitle =    {Pacific Symposium on Biocomputing},
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {6--17},
  year =     {2002},
  OPTeditor =    {},
  volume =   {7},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Benjamini&Hochberg95,
  author =   {Y. Benjamini and Y. Hochberg},
  title =    {Controlling the false discovery rate: a practical and powerful approach to multiple testing},
  journal =      {J. R. Statist. Soc. B},
  year =     {1995},
  OPTkey =   {},
  volume =   {57},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {289--300},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Benjamini&Yekutieli01,
  author =   {Y. Benjamini and D. Yekutieli},
  title =    {The control of the false discovery rate in multiple testing under
   dependency},
  journal =      {Annals of Statistics},
  year =     {2001},
  OPTkey =   {},
  volume =   {29},
  number =   {4},
  pages =    {1165--1188},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Beran88,
  author =   {R. Beran},
  title =    {Balanced simultaneous confidence sets},
  journal =      JASA,
  year =     {1988},
  OPTkey =   {},
  volume =   {83},
  OPTnumber =    {},
  pages =    {679--686},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Bock85,
  author =   {H-H Bock},
  title =    {On some significance tests in cluster analysis},
  journal =      {Journal of Classification},
  year =     {1985},
  OPTkey =   {},
  volume =   {2},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {77--108},
  OPTnote =      {},
  OPTannote =    {}
}



@InCollection{Bock96,
  author =   {H-H Bock},
  title =    {Probability models and hypotheses testing in partitioning cluster analysis},
  booktitle =    {Clustering and Classification},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher = {World Scientific Publishing Co.},
  year =     {1996},
  editor =   {P. Arabie and L. J. Hubert and G. De Soete},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {River Edge, NJ},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {377--453},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Boldricketal02,
  author =   {J. C. Boldrick and A. A. Alizadeh and M. Diehn and S. Dudoit and C. L. Liu and C. E. Belcher and D. Botstein and L. M. Staudt and P. O. Brown
and D. A. Relman},
  title =    {Stereotyped and specific gene expression programs in human innate immue responses to bacteria},
  journal =      PNAS,
  year =     {2002},
  OPTkey =   {},
  volume =   {99},
  number =   {2},
  pages =    {972--977},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Bozdogan00,
  author =   {H. Bozdogan},
  title =    {Akaike's information criterion and recent developments in information complexity},
  journal =      {Journal of Mathematical Psychology},
  year =     {2000},
  volume =   {44},
  pages =    {62-91}
}




@InCollection{Bozdogan93,
  author =   {H. Bozdogan},
  title =    {Choosing the number of component clusters in the mixture model  using a new informational complexity criterion of the inverse Fisher information matrix},
  booktitle =    {Information and Classification},
  publisher = {Heidelberg: Springer Verlag},
  editor = {O. Opitz and B. Lausen and R. Klar},
  year =     {1993},
  series =   {}
}

@Article{Braver,
  author =   {S. L. Braver},
  title =    {On splitting the tails unequally: a new perspective on one-versus two-tailed tests},
  journal =      {Educational and Psychological Measurement},
  year =     {1975},
  OPTkey =   {},
  volume =   {35},
  OPTnumber =    {},
  pages =    {283--301},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Breckenridge89,
  author =   {J. Breckenridge},
  title =    {Replicating cluster analysis: Method, consistency and validity},
  journal =      {Multivariate Behavioral Research},
  year =     {1989},
  OPTkey =   {},
  volume =   {24},
  OPTnumber =    {},
  pages =    {147--161},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Breiman&Spector92,
  author =   {L. Breiman and P. Spector},
  title =    {Submodel Selection and Evaluation in Regression. The
  $X$ Random Case},
  journal =      {International Statistical Review},
  year =     {1992},
  OPTkey =   {},
  volume =   {60},
  OPTnumber =    {},
  pages =    {291--319},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Breiman01,
  author =   {L. Breiman},
  title =    {Statistical modeling: the two cultures},
  journal =      {Statistical Science},
  year =     {2001},
  OPTkey =   {},
  volume =   {16},
  number =   {3},
  pages =    {199--215},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{BreimanAnnals96,
  author =   {L. Breiman},
  title =    {Heuristics of instability and stabilization in model selection},
  journal =      {Annals of Statistics},
  year =     {1996},
  OPTkey =   {},
  volume =   {24},
  number =   {6},
  pages =    {2350--2383},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{BreimanArcing,
  author =   {L. Breiman},
  title =    {Arcing classifiers},
  journal =      {Annals of Statistics},
  year =     {1998},
  OPTkey =   {},
  volume =   {26},
  OPTnumber =    {},
  pages =    {801-824},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{BreimanBagging,
  author =   {L. Breiman},
  title =    {Bagging predictors},
  journal =      {Machine Learning},
  year =     {1996},
  OPTkey =   {},
  volume =   {24},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {123-140},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{BreimanCPD,
  author =   {L. Breiman},
  title =    {Using Convex pseudo-data to increase prediction accuracy},
  institution =  {Department of Statistics, U.C. Berkeley},
  year =     {1998},
  OPTkey =   {},
  OPTtype =      {},
  number =   {513},
  OPTaddress =   {},
  month =    {March},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{BreimanJASA92,
  author =   {L. Breiman},
  title =    {The Little Bootstrap and Other Methods for
  Dimensionality Selection in Regression: $X$-Fixed Prediction Error},
  journal =      JASA,
  year =     {1992},
  OPTkey =   {},
  volume =   {87},
  number =   {419},
  pages =    {738--754},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@TechReport{BreimanOB,
  author =   {L. Breiman},
  title =    {Out-of-bag estimation},
  institution =  {Department of Statistics, U.C. Berkeley},
  year =     {1996},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@TechReport{BreimanRanForests,
  author =   {L. Breiman},
  title =    {Random forests - random features},
  institution =  {Department of Statistics, U.C. Berkeley},
  year =     {1999},
  OPTkey =   {},
  OPTtype =      {},
  number =   {567},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Breimanetal84,
  author =   {L. Breiman and J. H. Friedman and R. Olshen and C. J. Stone},
  title =    {Classification and regression trees},
  publisher =    {Wadsworth International Group},
  year =     {1984},
  OPTkey =   {},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  series =   {The Wadsworth statistics/probability series},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Book{Hastieetal02,
  author =   {T. Hastie and R. Tibshirani and J. Friedman},
  title =    {The Elements of Statistical Learning},
  publisher =    {Springer},
  year =     {2002},
  OPTkey =   {},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  series =   {Springer Series in Statistics},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Broman01,
  author =   {K. W. Broman},
  title =    {Review of statistical methods for QTL mapping in experimental crosses},
  journal =      {Lab Animal},
  year =     {2001},
  OPTkey =   {},
  volume =   {30},
  number =   {7},
  pages =    {44--52},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@PhdThesis{Broman97,
  author =   {K. W. Broman},
  title =    {Identifying quantitative trait loci in experimental crosses},
  school =   {Department of Statistics, U.C. Berkeley},
  year =     {1997},
  OPTkey =   {},
  type =     {Ph.{D}. thesis},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Brown&Koplowitz79,
  author =   {T. A. Brown and J. Koplowitz},
  title =    {The weighted nearest neighbor rule for class dependent sample sizes},
  journal =      {IEEE Transactions on Information Theory},
  year =     {1979},
  OPTkey =   {},
  volume =   {25},
  number =   {5},
  pages =    {617--619},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Buhlmann&Yu,
  author =   {P. Buhlmann and B. Yu},
  title =    {Explaining Bagging.},
  journal =      {Annals of Statistics},
  year =     {(Accepted)},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTpages =     {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Burgessvm98,
  author =   {C. J. C. Burges},
  title =    {A tutorial on support vector machines for pattern recognition},
  journal =      {Data Mining and Knowledge Discovery},
  year =     {1998},
  OPTkey =   {},
  volume =   {2},
  number =   {},
  pages =    {121--167},
  month =    {December},
  OPTnote =      {},
  OPTannote =    {}
}



@article{Burman89,
AUTHOR={P. Burman},
TITLE={A comparative study of ordinary cross-validation, $v$-fold cross-validati
on and the repeated learning testing methods},
JOURNAL={Biometrika},
VOLUME={76},
YEAR={1989},
PAGES={503-514}
}





@TechReport{Buttrey&Karo02,
  author =   {S. E. Buttrey and C. Karo},
  title =    {Using k--neareset neighbor classification in the leaves of a tree},
  institution =  {Naval Postgraduate School, Monterey, CA},
  year =     {2002},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Calinskietal,
  author =   {R. Calinski and J. Harabasz},
  title =    {A dendrite method for cluster analysis},
  journal =      {Communications in Statistics},
  year =     {1974},
  OPTkey =   {},
  volume =   {3},
  OPTnumber =    {},
  pages =    {1--27},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Callowetal00,
  author =   {M. J. Callow and S. Dudoit and E. L. Gong and T. P. Speed and E. M. Rubin},
  title =    {Microarray expression profiling identifies genes with altered expression in {HDL} deficient mice},
  journal =      {Genome Research},
  year =     {2000},
  OPTkey =   {},
  volume =   {10},
  number =   {12},
  OPTmonth =     {},
  pages =    {2022--2029},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Chambers98,
   author = {J. M. Chambers},
   title = {Programming with Data: A Guide to the S Language},
   publisher = {Springer-Verlag New York},
   year = {1998}
}
@Book{Diggleetal2002,
   author = {Peter J. Diggle and P. Heagerty and K-Y Liang and S.L. Zeger},
   title = {Analysis of Longitudinal Data},
   publisher = {Oxford University Press},
   year = {2002 (Second Edition)}
}

@TechReport{ChangLin2001,
  author =       {C.-C. Chang and C.-J. Lin},
  title =        {LIBSVM: a Library for Support Vector Machines (Version 2.31)},
  institution =  {},
  year =         {2001},
  OPTkey =       {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  note =         {\\ {\tt http://www.csie.ntu.edu.tw/~cjlin/papers/libsvm2.ps.gz}},
  OPTannote =    {}
}



@Article{Changetal02,
  author =   {H. Y. Chang and J. T. Chi and S. Dudoit and C. Bondre and M. van de Rijn and D. Botstein D and P. O. Brown},
  title =    {Diversity, topographic differentiation, and positional memory in human fibroblasts},
  journal =      PNAS,
  year =     {2002},
  OPTkey =   {},
  volume =   {99},
  number =   {20},
  pages =    {12877--12882},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Chenetal02,
  author =   {X. Chen and S. T. Cheung and S. So and S. T. Fan and C. Barry and J. Higgins and K.-M. Lai and J. Ji and S. Dudoit and I. O. L. Ng and M. van de Rijn and D. Botstein and P. O. Brown },
  title =    {Gene expression patterns in human liver cancers},
  journal =      {Molecular Biology of the Cell},
  year =     {2002},
  OPTkey =   {},
  volume =   {13},
  number =   {6},
  pages =    {1929--1939},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Cleveland&Devlin88,
  author =   {W. S. Cleveland and S. J. Devlin},
  title =    {Locally-Weighted Regression: An Approach to Regression Analysis by Local Fitting},
  journal =      JASA,
  year =     {1988},
  OPTkey =   {},
  volume =   {83},
  OPTnumber =    {},
  pages =    {596--610},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Cleveland79,
  author =   {W. S. Cleveland},
  title =    {Robust locally weighted regression and smoothing scatterplots},
  journal =      JASA,
  year =     {1979},
  OPTkey =   {},
  volume =   {74},
  number =   {368},
  pages =    {829--836},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Correa&Wolfson99,
  author =   {J. A. Correa and D. B. Wolfson},
  title =    {Length-bias: some characterizations and applications},
  journal =      {Journal of Statistical Computation and Simulation},
  year =     {1999},
  OPTkey =   {},
  volume =   {64},
  Tnumber =      {3},
  pages =    {209--219},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Correaetal02,
  author =   {J. A. Correa and S. Dudoit and D. R. Goldstein},
  title =    {Multiple testing in the survival analysis of microarray data},
  OPTjournal =   {Statistics in Medicine},
  year =     {2002},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTpages =     {},
  OPTmonth =     {},
  note =     {(Submitted)},
  OPTannote =    {}
}


@Article{CortesVapnik95,
  author =   {C. Cortes and V. Vapnik},
  title =    {Support-vector networks},
  journal =      {Machine Learning},
  year =     {1995},
  OPTkey =   {},
  volume =   {20},
  number =   {},
  pages =    {273-297},
  month =    {December},
  OPTnote =      {},
  OPTannote =    {}
}

@InProceedings{Davies&Bouldin,
  author =   {D. Davies and D. Bouldin},
  title =    {A cluster separation measure},
  booktitle =    {IEEE Transactions on Pattern Analysis and Machine Intelligence},
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {224--227},
  year =     {1979},
  OPTeditor =    {},
  volume =   {1},
  OPTnumber =    {PAMI-1},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@article {Davis89,
AUTHOR ={R. B. Davis  and J. R. Anderson},
TITLE ={Exponential survival trees},
JOURNAL = {Statistics in Medicine},
VOLUME = {8},
YEAR ={1989},
NUMBER={},
PAGES = {947-961},
ISSN = {},
CODEN = {},
}




@InCollection{Day96,
  author =   {W. H. E. Day},
  title =    {Complexity theory: {A}n introduction for practitioners of classification},
  booktitle =    {Clustering and Classification},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher = {World Scientific Publishing Co.},
  year =     {1996},
  editor =   {P. Arabie and L. J. Hubert and G. De Soete},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {River Edge, NJ},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {199--233},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Dettling&Buhlmann02,
  author =   {M. Dettling and P. B\"{u}lmann},
  title =    {How to Use Boosting for Tumor Classification with Gene Expression Data},
  journal =      {},
  year =     {2002},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTpages =     {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Dudoit&Fridlyand02II,
  author =   {S. Dudoit and J. Fridlyand},
  title =    {Bagging to improve the accuracy of a clustering procedure},
  OPTjournal =   {Bioinformatics},
  year =     {2002},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTpages =     {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
  }



@InCollection{Dudoit&FridlyandCRC02,
  author =   {S. Dudoit and J. Fridlyand},
  title =    {Classification in microarray experiments},
  booktitle =    {Statistical Analysis of Gene Expression Microarray Data},
  OPTcrossref =  {},
  OPTkey =   {},
  OPTpages =     {},
  publisher =    {Chapman \& Hall/CRC},
  year =     {2002},
  editor =   {T. P. Speed},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTtype =      {},
  OPTchapter =   {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  note =     {(To appear)},
  OPTannote =    {}
}

@Article{Dudoit&FridlyandGenBio02,
  author =   {S. Dudoit and J. Fridlyand},
  title =    {A prediction-based resampling method to estimate the number of clusters in a dataset},
  journal =      {Genome Biology},
  year =     {2002},
  OPTkey =   {},
  volume =   {3},
  number =   {7},
  pages =    {0036.1--0036.21},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@TechReport{Dudoit&FridlyandTechRep600,
  author =   {S. Dudoit and J. Fridlyand},
  title =    {Applications of resampling methods to estimate the number of clusters and to improve the accuracy of a clustering method},
  institution =  {Department of Statistics, Uiversity of California, Berkeley},
  year =     {2001},
  OPTkey =   {},
  OPTtype =      {},
  number =   {600},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {},
  url={stat-www.berkeley.edu/users/sandrine/publications.html},
}

S. Dudoit, M.J. van der Laan (2005),
 Asymptotics of cross-validated
risk estimation in estimator selection and performance assessment.
{\em Statistical Methodology 2}, 2, 131--54.

@Article{Dudoit&vanderLaan05,
  author =   {S. Dudoit and M.J. van der Laan},
  title =    {Asymptotics of cross-validated risk estimation in estimator selection and performance assessment},
  journal =      {Statistical Methodology},
  year =     {2005},
  OPTkey =   {},
  volume =   {2},
  number =   {2},
  OPTmonth =     {},
  pages =    {131--154},
  OPTnote =      {www.bepress.com/ucbbiostat/paper126},
  OPTannote =    {}
}
@Article{Dudoit&SpeedAnnals99,
  author =   {S. Dudoit and T. P. Speed},
  title =    {A score test for linkage using identity by descent data from sibships},
  journal =      {Annals of Statistics},
  year =     {1999},
  OPTkey =   {},
  volume =   {27},
  number =   {3},
  OPTmonth =     {},
  pages =    {943--986},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Dudoit&SpeedBios00,
  author =   {S. Dudoit and T. P. Speed},
  title =    {A score test for the linkage analysis of qualitative and quantitative traits based on identity by descent data on sib-pairs},
  journal =      {Biostatistics},
  year =     {2000},
  OPTkey =   {},
  volume =   {1},
  number =   {1},
  pages =    {1--26},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}




@InCollection{Dudoit&SpeedIMA99,
  author =   {S. Dudoit and T. P. Speed},
  title =    {Triangle constraints for sib-pair identity by descent probabilities under a general multilocus model for disease susceptibility},
  booktitle =    {Statistics in Genetics},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher =    {Springer-Verlag},
  year =     {1999},
  editor =   {M. E. Halloran and S. Geisser},
  volume =   {112},
  OPTnumber =    {},
  series =   {IMA Volumes in Mathematics and its Applications},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {New York},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {181--221},
  OPTnote =      {},
  OPTannote =    {}
}

@InCollection{Dudoit&YangSpringer03,
  author =   {S. Dudoit and Y. H. Yang},
  title =    {Bioconductor {R} packages for exploratory analysis and normalization of c{DNA} microarray data},
  booktitle =    {The Analysis of Gene Expression Data: Methods and Software},
  OPTcrossref =  {},
  OPTkey =   {},
  OPTpages =     {},
  publisher =    {Springer, New York},
  year =     {2003},
  editor =   {G. Parmigiani and E. S. Garrett and R. A. Irizarry and S. L. Zeger},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTtype =      {},
  OPTchapter =   {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{DudoitetalJASA02,
  author =       {S. Dudoit and J. Fridlyand and T. P. Speed},
  title =        {Comparison of Discrimination Methods for the Classification of
 Tumors Using Gene Expression Data},
  journal =      JASA,
  year =         {2002},
  OPTkey =       {},
  volume =    {97},
  number =    {457},
  pages =     {77--87},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{DudoitetalSinica02,
  author =   {S. Dudoit and Y. H. Yang and M. J. Callow and T. P. Speed},
  title =    {Statistical methods for identifying differentially expressed genes in replicated c{DNA} microarray experiments},
  journal =      {Statistica Sinica},
  year =     {2002},
  OPTkey =   {},
  volume =   {12},
  number =   {1},
  pages =    {111--139},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{DudoitetalTechRep110,
  author =   {S. Dudoit and J. P. Shaffer and J. C. Boldrick},
  title =    {Multiple hypothesis testing in microarray experiments},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =     {2002},
  OPTkey =   {},
  OPTtype =      {},
  number =   {110},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {},
  url={www.bepress.com/ucbbiostat/paper110/}

}


@Article{Duffy&Quiroz,
  author =   {D. E. Duffy and A. J. Quiroz},
  title =    {A permutation-based algorithm for block clustering},
  journal =      {Journal of Classification},
  year =     {1991},
  OPTkey =   {},
  volume =   {8},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {65--91},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Dunn58,
  author =   {O. J. Dunn},
  title =    {Estimation of the means of dependent variables},
  journal =      {Annals of Mathematical Statistics},
  year =     {1958},
  OPTkey =   {},
  volume =   {29},
  OPTnumber =    {},
  pages =    {1095-111},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Book{Efron&Tibs93,
  author =   {B. Efron and R. J. Tibshirani},
  ALTeditor =    {},
  title =    {An Introduction to the Bootstrap},
  publisher =    {Chapman \& Hall/CRC},
  year =     {1993},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{EfronetalJASA01,
  author =   {B. Efron and R. Tibshirani and J. D. Storey and V. Tusher},
  title =    {Empirical Bayes analysis of a microarray
experiment},
  journal =      JASA,
  year =     {2001},
  OPTkey =   {},
  volume =   {96},
  OPTnumber =    {},
  pages =    {1151--1160},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@TechReport{EfronetalTechRep01,
  author =   {B. Efron and J. D. Storey and R. Tibshirani},
  title =    {Microarrays, empirical Bayes methods, and false discovery
rates},
  institution =  {Department of Statistics, Stanford University},
  year =     {2001},
  OPTkey =   {},
  OPTtype =      {},
  number =   {2001-218},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Finner99,
  author =   {H. Finner},
  title =    {Stepwise multiple test procedures and control of directional errors},
  journal =      {Annals of Statistics},
  year =     {1999},
  OPTkey =   {},
  volume =   {27},
  OPTnumber =    {},
  pages =    {274--289},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Fisher,
  author =   {R. A. Fisher},
  title =    {The use of multiple measurements in taxonomic problems},
  journal =      {Annals of Eugenics},
  year =     {1936},
  OPTkey =   {},
  volume =   {7},
  OPTnumber =    {},
  pages =    {179-188},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Fisher26,
  author =   {R. A. Fisher},
  title =    {The arrangement of field experiments},
  journal =      {J. Min. Agric. Gr. Br},
  year =     {1926},
  OPTkey =   {},
  volume =   {33},
  OPTnumber =    {},
  pages =    {505--513},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{Fix&Hodges,
  author =   {E. Fix and J. Hodges},
  title =    {Discriminatory analysis, nonparametric discrimination: consistency properties},
  institution =  {Randolph Field, Texas: USAF School of Aviation Medicine},
  year =     {1951},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Fowlkes&Mallows83,
  author =   {E. B. Fowlkes and C. L. Mallows},
  title =    {A method for comparing two hierarchical clusterings},
  journal =      JASA,
  year =     {1983},
  OPTkey =   {},
  volume =   {78},
  OPTnumber =    {383},
  OPTmonth =     {},
  pages =    {553--584},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Fowlkesetal88,
  author =   {E. B. Fowlkes and R. Gnanadesikan and J. R. Kettenring},
  title =    {Variable selection in clustering},
  journal =      JC,
  year =     {1988},
  OPTkey =   {},
  volume =   {5},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {205--228},
  OPTnote =      {},
  OPTannote =    {}
}

@TechReport{Fraley&Raftery98,
  author =   {C. Fraley and A. Raftery},
  title =    {How many clusters? Which clustering method? -- answers via model-based cluster analysis},
  institution =  {Department of Statistics, University of Washington},
  year =     {1998},
  OPTkey =   {},
  OPTtype =      {},
  number =   {329},
  OPTaddress =   {},
  OPTmonth =     {},
  note =     {\url{http://www.stat.washington.edu/www/research/reports/1990s/#1998}},
  OPTannote =    {}
}




@Article{Freund&Schapire97,
  author =   {Y. Freund and R. E. Schapire},
  title =    {A decision-theoretic generalization of on-line learning and an application to boosting},
  journal =      {Journal of Computer and System Sciences},
  year =     {1997},
  OPTkey =   {},
  volume =   {55},
  OPTnumber =    {},
  pages =    {119--139},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@PhdThesis{Fridlyand,
  author =   {J. Fridlyand},
  title =    {Resampling methods for variable selection and classification: applications to genomics},
  school =   {Department of Statistics, U.C. Berkeley},
  year =     {2001},
  OPTkey =   {},
  type =     {Ph.{D}. thesis},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{Friedman94 ,
  author =   {J. H. Friedman},
  title =    {Flexible metric nearest neighbor clasification},
  institution =  {Department of Statistics, Stanford University},
  year =     {1994},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@TechReport{Friedman96a,
  author =   {J. H. Friedman},
  title =    {On bias, variance, 0/1-loss, and the curse--of--dimensionality },
  institution =  {Department of Statistics, Stanford University},
  year =     {1996},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{Friedman96b,
  author =   {J. H. Friedman},
  title =    {Another approach to polychotomous classification},
  institution =  {Department of Statistics, Stanford University},
  year =     {1996},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Friedmanetal00,
  author =   {J. Friedman and T. Hastie and R. Tibshirani},
  title =    {Additive logistic regression: a statistical view of boosting},
  journal =      {Annals of Statistics},
  year =     {2000},
  OPTkey =   {},
  volume =   {28},
  OPTnumber =    {},
  pages =    {337--404},
  OPTmonth =     {},
  note =     {(with discussion)},
  OPTannote =    {}
}

@book {GAM,
   AUTHOR = {T. J. Hastie and R.J. Tibshirani},
    TITLE = {Generalized Additive Models},
PUBLISHER = {Chapman and Hall},
  ADDRESS = {London},
     YEAR = {1990},
    PAGES = {},
     ISBN = {},
}



@Article{Gabriel,
  author =   {K. R. Gabriel},
  title =    {The biplot graphic display of matrices with application to principal component analysis},
  journal =      {Biometrika},
  year =     {1971},
  OPTkey =   {},
  volume =   {58},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {453--467},
  OPTnote =      {},
  OPTannote =    {}
}

@InCollection{Gabriel75,
  author =   {K. R. Gabriel},
  title =    {A comparison of some methods of simultaneous inference in {MANOVA}},
  booktitle =    {Multivariate Statistical Methods: Among-groups covariation; Within-group covariation},
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {61--80},
  OPTpublisher = {},
  year =     {1975},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTtype =      {},
  OPTchapter =   {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@InProceedings{GabrielPun,
  author =       {K. R. Gabriel and F. C. Pun},
  title =        {Binary prediction of weather events with several predictors},
  booktitle =    {Sixth Conference on Probability and Statistics in Atmospheric Science},
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {248--253},
  year =     {1979},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  organization = {American Meterological Society},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}


@Unpublished{Ge&Dudoit,
  author =   {Y. Ge and S. Dudoit},
  title =    {Fast algorithm for resampling-based $p$-value adjustment in multiple testing},
  note =     {(In preparation)},
  OPTkey =   {},
  OPTmonth =     {},
  year =     {2002},
  OPTannote =    {}
}

@Article{Geisser75,
  author =   {S. Geisser},
  title =    {The predictive sample reuse method with applications},
  journal =      {Journal of the American Statistical Association},
  year =     {1975},
  volume =   {70},
  pages =    {320-328}
}

@TechReport{Genovese&Wasserman01,
  author =   {C. Genovese and L. Wasserman},
  title =    {Operating Characteristics and Extensions of the FDR Procedure},
  institution =  {Department of Statistics, Carnegie Mellon},
  year =     {2001},
  OPTkey =   {},
  OPTtype =      {},
  number =   {737},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Gnanadesikan&Kettering95,
  author =   {R. Gnanadesikan and J. R. Kettenring},
  title =    {Weighting and selection of variables for cluster analysis},
  journal =      JC,
  year =     {1995},
  OPTkey =   {},
  volume =   {12},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {113--136},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{GoldsteinetalGenEpi00,
  author =   {D. R. Goldstein and S. Dudoit and T. P. Speed},
  title =    {Power of a score test for quantitative trait linkage analysis of relative pairs.},
  journal =      {Genetic Epidemiology},
  year =     {2000},
  OPTkey =   {},
  volume =   {19},
  number =   {Suppl. 1},
  pages =    {S85--S91},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{GoldsteinetalGenEpi01,
  author =   {D. R. Goldstein and S. Dudoit and T. P. Speed},
  title =    {Power and robustness of a score  test for linkage analysis of quantitative traits using identity by descent data on sib pairs},
  journal =      {Genetic Epidemiology},
  year =     {2001},
  OPTkey =   {},
  volume =   {20},
  number =   {4},
  pages =    {415--431},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@article {Gordon85,
AUTHOR ={L. Gordon and R.A. Olshen},
TITLE ={Tree-structured survival analysis},
JOURNAL = {Cancer Treatment Reports},
VOLUME = {69},
YEAR ={1985},
NUMBER={},
PAGES = {10065-1069},
ISSN = {},
CODEN = {},
}



@InCollection{Gordon96,
  author =   {A. D. Gordon},
  title =    {Hierarchical classification},
  booktitle =    {Clustering and Classification},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher = {World Scientific Publishing Co.},
  year =     {1996},
  editor =   {P. Arabie and L. J. Hubert and G. De Soete},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {River Edge, NJ},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {65--121},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Gower&Hand,
  author = {J. C. Gower and D. J. Hand},
  title =    {Biplots},
  publisher =    {Chapman \& Hall},
  year =     {1996},
  OPTkey =   {},
  OPTeditor =    {},
  OPTvolume =    {},
  number =   {54},
  series =   {Monographs on statistics and applied probability},
  OPTaddress =   {},
  edition =      {1st},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@book {Gyorfi02,
   AUTHOR = {L. Gy\"{o}rfi and M. Kohler and A. Krzy\.{z}ak  and H. Walk},
    TITLE = {A Distribution-Free Theory of Nanparametric Regression},
PUBLISHER = {Springer-Verlag},
  ADDRESS = {New York},
     YEAR = {2002},
    PAGES = {100-102},
     ISBN = {}
}




@Book{Gyorfietal02,
  author =   {L. Gy\"orfi and M. Kohler and A. Krzy\'{z}ak and H. Walk},
  ALTeditor =    {},
  title =    {A distribution-free theory of nonparametric regression},
  publisher =    {Springer-Verlag, New York},
  year =     {2002},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Book{HTF01,
  author =   {T. Hastie and R. Tibshirani and J. H. Friedman},
  ALTeditor =    {},
  title =    {The Elements of Statistical Learning : Data Mining, Inference, and Prediction },
  publisher =    {Springer Verlag},
  year =     {2001},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Hansen01,
  author =   {M. H. Hansen  and B. Yu},
  title =    {Model selection and the principle of minimum description length},
  journal =      {Journal of the American Statistical Association},
  year =     {2001},
  volume =   {96},
  pages =    {746-774}
}

@Article{Hardle85a,
  author =   {W. H{\"a}rdle and J. S. Marron},
  title =    {Asymptotic nonequivalence of some bandwidth selectors in nonparametric regression},
  journal =      {Biometrika},
  year =     {1985},
  volume =   {72},
  pages =    {481--484}
}




@Article{Hardle85b,
  author =   {W. H{\"a}rdle and J. S. Marron},
  title =    {Optimal bandwidth selection in nonparametric regression function estimation},
  journal =      {Annals of Statistics},
  year =     {1985},
  volume =   {13},
  pages =    {1465-1481}
}

@Book{Hardle93,
  author =       {W. H{\"a}rdle},
  title =        {Applied Nonparametric Regression},
  publisher =    {Cambridge University Press},
  pages = {},
  year =         {1993}
}

@Article{Hartigan72,
  author =   {J. A. Hartigan},
  title =    {Direct clustering of a data matrix},
  journal =      {Journal of the American Statistical Association},
  year =     {1972},
  OPTkey =   {},
  volume =   {67},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {123--129},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Hartigan75,
  author =   {J. A. Hartigan},
  title =    {Clustering Algorithms},
  publisher =    {Wiley},
  year =     {1975},
  OPTkey =   {},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Hartigan78,
  author =   {J. Hartigan},
  title =    {Asymptotic distributions for clustering criteria},
  journal =      {Annals of Statistics},
  year =     {1978},
  OPTkey =   {},
  volume =   {6},
  OPTnumber =    {},
  pages =    {117--131},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Hartigan85,
  author =   {J. A. Hartigan},
  title =   {Statistical theory in clustering} ,
  journal =      JC,
  year =     {1985},
  OPTkey =   {},
  volume =   {2},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {63--76},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Hastie&Tibshirani96a,
  author =   {T. Hastie and R. Tibshirani},
  title =    {Discriminant adaptive nearest-nieghbor classification},
  journal =      {IEEE Pattern Recognition and Machine Intelligence},
  year =     {1996},
  OPTkey =   {},
  volume =   {18},
  OPTnumber =    {},
  pages =    {607--616},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{Hastie&Tibshirani96b,
  author =   {T. Hastie and R. Tibshirani},
  title =    {Classification by pairwise coupling},
  institution =  {Department of Statistics, Stanford University},
  year =     {1996},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@article {Hastie90,
   AUTHOR = {T.J. Hastie and  R.J. Tibshirani},
    TITLE = {Exploring the nature of covariate effects in the proportional hazar
ds model},
  JOURNAL = {Biometrics},
   VOLUME = {46},
     YEAR = {1990},
   NUMBER = {4},
    PAGES = {1005-1016},
     ISSN = {},
    CODEN = {},
}


@Book{Hochberg&Tamhane,
  author =   {Y. Hochberg and A. C. Tamhane},
  ALTeditor =    {},
  title =    {Multiple Comparison Procedures},
  publisher =    {Wiley--Interscience},
  year =     {1987},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  series =   {Probability and Mathematical Statistics},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Hochberg88,
  author =   {Y. Hochberg},
  title =    {A sharper Bonferroni procedure for multiple tests of significance},
  journal =      {Biometrika},
  year =     {1988},
  OPTkey =   {},
  volume =   {75},
  OPTnumber =    {},
  pages =    {800--802},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Holm79,
  author =   {S. Holm},
  title =    {A simple sequentially rejective multiple test procedure},
  journal =      {Scand. J. Statist.},
  year =     {1979},
  OPTkey =   {},
  volume =   {6},
  OPTnumber =    {},
  pages =    {65--70},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Hommel&Bernhard99,
  author =   {G. Hommel and G. Bernhard},
  title =    {Bonferroni procedures for logically related hypotheses},
  journal =      {Journal of Statistical Planning and Inference},
  year =     {1999},
  OPTkey =   {},
  volume =   {82},
  OPTnumber =    {},
  pages =    {119--128},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Hommel88,
  author =   {G. Hommel},
  title =    {A stagewise rejective multiple test procedure based on a modified Bonferroni test},
  journal =      {Biometrika},
  year =     {1988},
  OPTkey =   {},
  volume =   {75},
  OPTnumber =    {},
  pages =    {383--386},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Hubert&Arabie85,
  author =   {L. Hubert and P. Arabie},
  title =    {Comparing partitions},
  journal =      JC,
  year =     {1985},
  OPTkey =   {},
  volume =   {2},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {193--218},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Jain&DubesBook,
  author =   {A. K. Jain and R. C. Dubes},
  editor =   {},
  title =    {Algorithms for Clustering Data},
  publisher =    {Prentice-Hall},
  year =     {1988},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {Englewood Cliffs, N. J.},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Jogdeo77,
  author =   {K. Jogdeo},
  title =    {Association and probability inequalities},
  journal =      {Annals of Statistics},
  year =     {1977},
  OPTkey =   {},
  volume =   {5},
  OPTnumber =    {},
  pages =    {495--504},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Kaufman&Rousseeuw90,
  author =   {L. Kaufman and P. J. Rousseeuw},
  ALTeditor =    {},
  title =    {Finding Groups in Data: An Introduction to Cluster Analysis},
  publisher =    {Wiley, New York.},
  year =     {1990},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@article {Keles03,
AUTHOR ={Kele\c{s}, S. and van der Laan, M. and Dudoit,  S.},
TITLE ={Asymptotically Optimal  Model Selection Method for Regression on Censored Outcomes },
JOURNAL = {Technical Report, Division of Biostatistics, UC Berkeley},
VOLUME = {},
YEAR ={2002},
PAGES = {},
ISSN = {},
CODEN = {},
}



@Article{Kohonen90,
  author =   {T. Kohonen},
  title =    {The self-organizing map},
  journal =      {Proc. IEEE},
  year =     {1990},
  OPTkey =   {},
  volume =   {78},
  number =   {9},
  OPTmonth =     {},
  pages =    {1464--1480},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Kohonen95,
  author =   {T. Kohonen},
  title =    {Self-Organizing Maps},
  publisher =    {Springer},
  year =     {1995},
  OPTkey =   {},
  editor =   {T. S. Huang and T. Kohonen and M. R. Schroeder},
  volume =   {30},
  OPTnumber =    {},
  series =   {Springer Series in Information Sciences},
  address =      {Berlin, Heidelberg},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@article {Kooperberg95,
AUTHOR ={C. Kooperberg and C.J.  Stone and Y. K.  Truong},
TITLE ={Hazard Regression},
JOURNAL = {Journal of the American Statistical Association},
VOLUME = {90},
YEAR ={1995},
NUMBER={429},
PAGES = {78-94},
ISSN = {},
CODEN = {},
}



@Article{Koutsoukosetal,
  author =   {A. D. Koutsoukos and L. V. Rubinstein and D. Faraggi and R.M. Simon and S. Kalyandrug and J. N. Weinstein and K.W. Kohn and K.D. Paull},
  title =    {Discrimination techniques applied to the {NCI} in vitro anti-tumor drug screen: predicting biochemical mechanism of action},
  journal =      {Statistics in Medicine},
  year =     {1994},
  OPTkey =   {},
  volume =   {13},
  OPTnumber =    {},
  pages =    {719--730},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Krishnaiah&Reising85,
  author =   {P. R. Krishnaiah and J. M. Reising},
  title =    {Multivariate multiple comparisons},
  journal =      {Encyclopedia of Statistical Sciences},
  year =     {1985},
  OPTkey =   {},
  volume =   {9},
  number =   {6},
  pages =    {88--95},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Krzanowski&Lai,
  author =   {W. Krzanowski and Y. Lai },
  title =    {A criterion for determining the number of groups in a dataset using sum of squares clustering},
  journal =      {Biometrics},
  year =     {1985},
  OPTkey =   {},
  volume =   {44},
  OPTnumber =    {},
  pages =    {23--34},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Laan&Bryan01,
  author =   {M. J. van der Laan and J. Bryan},
  title =    {Gene expression analysis with the parametric bootstrap},
  journal =      {Biostatistics},
  year =     {2001},
  OPTkey =   {},
  volume =   {2},
  number =   {4},
  pages =    {445--461},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Pollard&vanderLaan04,
  author =   {K. S. Pollard and M.J. van der Laan},
  title =    {Choice of Null Distribution in Resampling Based Multiple Testing},
  journal =      JSPI,
  year =     {2004},
  OPTkey =   {},
  OPTvolume =    {125},
  OPTnumber =    {},
  OPTpages =     {85--101},
  OPTmonth =     {},
  note =     {},
  OPTannote =    {}
}


@Article{Laan&PollardJSPI02,
  author =   {M. J. van der Laan and K. S. Pollard},
  title =    {Hybrid clustering of gene expression data with visualization and the bootstrap},
  journal =      JSPI,
  year =     {2002},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTpages =     {},
  OPTmonth =     {},
  note =     {(To appear)},
  OPTannote =    {}
}


@article {Leblanc92,
AUTHOR ={M. Leblanc and J. Crowley},
TITLE ={Relative Risk trees for censored data},
JOURNAL = {Biometrics},
VOLUME = {48},
YEAR ={1992},
NUMBER={},
PAGES = {411-425},
ISSN = {},
CODEN = {},
}





@InProceedings{Leisch02,
  author =   {F. Leisch},
  title =    {Sweave: Dynamic Generation of Statistical Reports Using
                  Literate Data Analysis},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle = {Compstat 2002 --- Proceedings in Computational
                  Statistics},
  Tpages =   {575--580},
  year =     {2002},
  editor =   {Wolfgang H{\"a}rdle and Bernd R{\"o}nz},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  publisher = {Physika Verlag, Heidelberg, Germany},
  note =     {ISBN 3-7908-1517-9},
  OPTannote =    {},
  url =      {http://www.ci.tuwien.ac.at/~leisch/Sweave}
}

@TechReport{Leisch02TR,
  author =   {F. Leisch},
  title =    {Dynamic generation of statistical reports using literate data analysis},
  institution =  {SFB Adaptive Information Systems and Modelling in Economics and Management
Science, Vienna University of Economics and Business Administration},
  year =     {2002},
  OPTkey =   {},
  OPTtype =      {},
  number =   {69},
  OPTaddress =   {},
  month =    {March},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{Leisch99,
  author =   {F. Leisch},
  title =    {Bagged clustering},
  institution =  {SFB Adaptive Information Systems and Modelling in Economics and Management Science, Vienna University of Economics and Business Administration},
  year =     {1999},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  month =    {August},
  note =     {\url{http://www.ci.tuwien.ac.at/~leisch/papers/fl-techrep.html}},
  OPTannote =    {}
}

@Article{Limetal00,
  author =   {T-S Lim and W-Y Loh and Y-S Shih},
  title =    {A comparison of prediction accuracy, complexity, and training time of thiry-three old and new classification algorithms},
  journal =      {Machine Learning},
  year =     {2000},
  OPTkey =   {},
  volume =   {40},
  OPTnumber =    {},
  pages =    {203--229},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Book{Mardiaetal,
  author =   {K. V. Mardia and J. T. Kent and J. M. Bibby},
  title =    {Multivariate Analysis},
  publisher =    {Academic Press, Inc.},
  year =     {1979},
  OPTkey =   {},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {San Diego},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Unpublished{Mayo&Spanos02,
  author =       {D. C. Mayo and A. Spanos},
  title =        {A severe-testing interpretation of {N}eyman-{P}earson methods.  Unpublished manuscript},
  OPTnote =         {},
  OPTkey =       {},
  OPTmonth =     {},
  year =         {2002},
  OPTannote =    {}
}


@Book{McCullagh&Nelder89,
  author =   {P. McCullagh and J. A. Nelder},
  ALTeditor =    {},
  title =    {Generalized Linear Models},
  publisher =    {Chapman \& Hall},
  year =     {1989},
  OPTkey =   {},
  OPTvolume =    {},
  number =   {37},
  series =   {Monographs on Statistics and Applied Probability},
  OPTaddress =   {},
  edition =      {2nd},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Book{McLachlan,
  author =   {G. J. McLachlan},
  OPTeditor =    {},
  title =    {Discriminant analysis and statistical pattern recognition},
  publisher =    {Wiley},
  year =     {1992},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {New York},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{McLachlanetal01,
  author =   {G. J. McLachlan and R. Bean and D. Peel},
  title =    {A mixture model-based approach to the clustering of microarray expression data.},
  journal =      {Bioinformatics},
  year =     {2002},
  OPTkey =   {},
  volume =   {18},
  OPTnumber =    {},
  pages =    {413--422},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{MillerSubsets,
  author =   {A. J. Miller},
  OPTeditor =    {},
  title =    {Subset Selection in Regression},
  publisher =    {Chapman and Hall},
  year =     {1990},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Milligan&Cooper85,
  author =   {G. W. Milligan and M. C. Cooper},
  title =    {An examination of procedures for determining the number of clusters in a data set},
  journal =      {Psychometrika},
  year =     {1985},
  OPTkey =   {},
  volume =   {50},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {159--179},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Milligan&Cooper86,
  author =   {G. W. Milligan and M. C. Cooper},
  title =    {A study of the comparability of external criteria for hierarchical cluster analysis},
  journal =      {Multivariate Behavioral Research},
  year =     {1986},
  OPTkey =   {},
  volume =   {21},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {441--458},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Milligan&Cooper87,
  author =   {G. W. Milligan and M. C. Cooper},
  title =    {Methodology review: {C}lustering methods},
  journal =      {Applied Psychological Measurement},
  year =     {1987},
  OPTkey =   {},
  volume =   {11},
  OPTnumber =    {4},
  OPTmonth =     {December},
  pages =    {329--354},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Milligan89,
  author =   {G. W. Milligan},
  title =    {A study of the beta-flexible clustering method},
  journal =      {Multivariate Behavioral Research},
  year =     {1989},
  OPTkey =   {},
  volume =   {24(2)},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {163--176},
  OPTnote =      {},
  OPTannote =    {}
}


@InCollection{Milligan96,
  author =   {G. W. Milligan},
  title =    {Clustering validation: {R}esults and implications for applied analyses},
  booktitle =    {Clustering and Classification},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher = {World Scientific Publishing Co.},
  year =     {1996},
  editor =   {P. Arabie and L. J. Hubert and G. De Soete},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {River Edge, NJ},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {341--375},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Moreyetal83,
  author =   {L. C. Morey, R. K. Blashfield and H. A. Skinner},
  title =    {A comparison of cluster analysis techniques within a sequential validation framework},
  journal =      {Multivariate Behavioral Research},
  year =     {1983},
  OPTkey =   {},
  volume =   {18},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {309--329},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Morrison90,
  author =   {D. F. Morrison},
  ALTeditor =    {},
  title =    {Multivariate Statistical Methods},
  publisher =    {McGraw-Hill, NY},
  year =     {1990},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  edition =      {3rd},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@InCollection{Murtagh96,
  author =   {F. Murtagh},
  title =    {Neural networks for clustering},
  booktitle =    {Clustering and Classification},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher = {World Scientific Publishing Co.},
  year =     {1996},
  editor =   {P. Arabie and L. J. Hubert and G. De Soete},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {River Edge, NJ},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {235--269},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{PanelDACC,
  author =   {{Panel on Discriminant Analysis, Classification, and Clustering}},
  title =    {Discriminant analysis and clustering},
  journal =      {Statistical Science},
  year =     {1989},
  OPTkey =   {},
  volume =   {4},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {34--69},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{Pavlic&vanderLaanTechRep89,
  author =   {M. Pavlic and M. J. van der Laan},
  title =    {Fitting of mixtures with unspecified number of components using cross-validation distance estimate},
  institution =  {Division of Biostatistics, U.C. Berkeley},
  year =     {2001},
  OPTkey =   {},
  OPTtype =      {},
  number =   {89},
  OPTaddress =   {},
  month =    {February},
  OPTnote =      {},
  OPTannote =    {}
}

@article{Pavlic02,
author  = {M. Pavlic and M. J. van der Laan},
title   = {Fitting of mixtures with unspecified number of components using
cross validation distance estimate},
journal = {Computational Statistics and Data Analysis},
volume  = {41},
issue   = {3-4},
pages   = {413-428},
year    = {2003}
}



@TechReport{Pollard&LaanTechRep107,
  author =   {K. S. Pollard and M. J. van der Laan},
  title =    {A Method to Identify Significant Clusters in Gene Expression Data},
  institution =  {Division of Biostatistics, U.C. Berkeley},
  year =     {2002},
  OPTkey =   {},
  OPTtype =      {},
  number =   {107},
  OPTaddress =   {},
  month =    {April},
  OPTnote =      {},
  OPTannote =    {}
}

@TechReport{Pollard&LaanTechRep121,
  author =   {K. S. Pollard and M. J. van der Laan},
  title =    {Resampling-based methods for identification of significant subsets of genes in expression data},
  institution =  {Division of Biostatistics, U.C. Berkeley},
  year =     {2002},
  OPTkey =   {},
  OPTtype =      {},
  number =   {121},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Ramsey78,
  author =   {P. H. Ramsey},
  title =    {Power differences between pairwise multiple comparisons},
  journal =      JASA,
  year =     {1978},
  OPTkey =   {},
  volume =   {73},
  OPTnumber =    {},
  pages =    {479--485},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Manual{RanForests,
  title =    {Notes on setting up, using, and understanding random forests V3.0},
  OPTkey =   {},
  author =   {L. Breiman},
  OPTorganization = {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  year =     {2001},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Rand,
  author =   {W. M. Rand},
  title =    {Objective criteria for the evaluation of clustering methods},
  journal =      {Journal of the American Statistical Association},
  year =     {1971},
  OPTkey =   {},
  volume =   {66},
  OPTnumber =    {336},
  OPTmonth =     {},
  pages =    {846--850},
  OPTnote =      {},
  OPTannote =    {}
}

@Unpublished{Reineretal01,
  author =   {A. Reiner and D. Yekutieli and Y. Benjamini},
  title =    {Using resampling-based {FDR} controlling multiple test procedures for analyzing microarray gene expression data},
  OPTnote =      {},
  OPTkey =   {},
  OPTmonth =     {},
  year =     {2001},
  OPTannote =    {}
}


@Book{Ripley96,
  author =   {B. D. Ripley},
  title =    {Pattern recognition and neural networks},
  publisher =    {Cambridge University Press},
  year =     {1996},
  OPTkey =   {},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {Cambridge, New York},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}




%very first reference to use trees in survival analysis
@Article{Rissanen78,
  author =   {J. Rissanen},
  title =    {Modelling by shortest data description},
  journal =      {Automatica},
  year =     {1978},
  volume =   {14},
  pages =    {465-471}
}

@Article{Rnews:Dudoit+Yang+Bolstad:2002,
  author       = {S. Dudoit and Y. H.  Yang and B. Bolstad},
  title        = {Using {R} for the Analysis of {DNA} Microarray Data},
  journal      = {R News},
  year         = 2002,
  volume       = 2,
  number       = 1,
  pages        = {24--32},
  month        = {March},
  url          = {CRAN.R-project.org/doc/Rnews/}
}

@article {Robins00a,
AUTHOR ={J. M. Robins and A.  Rotnitzky},
TITLE ={Comment on the {B}ickel and {K}won article, ``{I}nference for semiparametric models: {S}ome questions and an answer''},
JOURNAL = {Statistica Sinica},
VOLUME = {11},
NUMBER={4},
YEAR ={2001},
PAGES = {920-936},
ISSN = {},
CODEN = {}
}


@InProceedings{Robins00c,
  author =   {J.M. Robins},
  title =    {Robust estimation in sequentially ignorable
missing data and causal inference models},
  booktitle =    {Proceedings of the American
Statistical Association},
  pages =    {},
  year =     {2000},
  editor =   {},
  organization = {}
}


@article {Robins00b,
AUTHOR ={J. M. Robins and A.  Rotnitzky and M.J. van der Laan},
TITLE ={Comment on ``{O}n {P}rofile {L}ikelihood" by {S}.{A}. {M}urphy and
{A}.{W}. van der {V}aart},
JOURNAL = {Journal of the American Statistical Association -- Theory and
Methods
},
VOLUME = {450},
YEAR ={2000},
PAGES = {431-435},
ISSN = {},
CODEN = {}
}



@Article{Birge83,
  author =   {L. Birg{\'e}},
  title =    {Approximation dans les espaces m{/'e}triques et th{\'e}orie
  de l'estimation},
  journal =      {Verw. Gebiete},
  year =     {1983},
  OPTkey =   {},
  volume =   {65},
  number =   {},
  OPTmonth =     {},
  pages =    {181--238},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{lecam73,
  author =   {L.M. le Cam},
  title =    {Convergence of estimates under dimensionality restrictions},
  journal =      {Annals of Statistics},
  year =     {1973},
  OPTkey =   {},
  volume =   {22},
  number =   {},
  OPTmonth =     {},
  pages =    {38--53},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Rom90,
  author =   {D. M. Rom},
  title =    {A sequentially rejective test procedure based on a modified {Bonferroni} inequality},
  journal =      {Biometrika},
  year =     {1990},
  OPTkey =   {},
  volume =   {77},
  OPTnumber =    {},
  pages =    {663-665},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{Rosenblatt57,
  author =       {F. Rosenblatt},
  title =        {The perceptron -- a perceiving and recognizing automation},
  institution =  {Cornell Aeronautical Laboratory },
  year =         {1957},
  OPTkey =       {},
  OPTtype =      {},
  number =       {86-460-1},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Ruczinskietal,
  author =   {I. Ruczinski and C. Kooperberg and M. LeBlanc},
  title =    {Logic regression},
  journal =      {},
  year =     {2001},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTpages =     {},
  OPTmonth =     {},
  note =     {Submitted, \url{http://biosun01.biostat.jhsph.edu/~iruczins/html/publications.html}},
  OPTannote =    {}
}

@Article{Saltstone&Stange,
  author =   {R. Saltstone and K. Stange},
  title =    {A computer program to calculate Hubert and Arabie's adjusted Rand index},
  journal =      {Journal of Classification},
  year =     {1996},
  OPTkey =   {},
  volume =   {13},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {169--172},
  OPTnote =      {},
  OPTannote =    {}
}
@TechReport{vanderVaart03,
  author =   {A.W. van der Vaart},
  title =    {Notes on Cross-validation},
  institution =  {Department of Mathematics, Free University, Amsterdam},
  year =     {2003},
  OPTkey =   {},
  OPTtype =      {},
  number =   {},
  OPTaddress =   {},
  OPTmonth =     {},
  note =     {},
  OPTannote =    {Unpublished manuscript}
}

@TechReport{Sarle,
  author =   {W. Sarle},
  title =    {Cubic clustering criterion},
  institution =  {SAS Institute, Inc.},
  year =     {1983},
  OPTkey =   {},
  OPTtype =      {},
  number =   {A-108},
  OPTaddress =   {},
  OPTmonth =     {},
  note =     {\url{http://www.sas.com/service/library/onlinedoc/trindex.html}},
  OPTannote =    {}
}

@TechReport{Sarle&Kuo,
  author =   {W. Sarle and A. Kuo},
  title =    {The MODECLUS Procedures},
  institution =  {SAS Institute, Inc.},
  year =     {1993},
  OPTkey =   {},
  OPTtype =      {},
  number =   {P-256},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Schapireetal,
  author =   {R. E. Schapire and Y. Freund and P. Bartlett and W. S. Lee},
  title =    {Boosting the margin: a new explanation for the effectiveness of voting methods},
  journal =      {Annals of Statistics},
  year =     {1998},
  OPTkey =   {},
  volume =   {26},
  OPTnumber =    {},
  pages =    {1651--1686},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Book{Scheffe,
  author =   {H. Scheff\'{e}},
  ALTeditor =    {},
  title =    {The analysis of variance},
  publisher =    {John Wiley \& Sons},
  year =     {1959},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Scheibler&Schneider,
  author =   {D. Scheibler and W. Schneider},
  title =    {Monte Carlo tests of the accuracy of cluster analysis algorithms: A comparison of hierarchical and nonhierarchical methods},
  journal =      {Multivariate Behavioral Research},
  year =     {},
  OPTkey =   {},
  volume =   {20},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {283--304},
  OPTnote =      {},
  OPTannote =    {}
}


@InProceedings{Schuster81,
  author =   {E. F. Schuster and C. G. Gregory},
  title =    {On the non-consistency of maximum likelihood nonparametric density estimators},
  booktitle =    {Computer Science and Statistics: Proceedings of the 13th Symposium on the interface},
  pages =    {295-298},
  year =     {1981},
  editor =   {Eddy, W.F.},
  organization = {}
}


@Article{Scott81,
  author =   {D. W. Scott and L. E. Factor},
  title =    {Monte Carlo study of three data-based nonparametric density estimators},
  journal =      {Journal of the American Statistical Association},
  year =     {1981},
  volume =   {76},
  pages =    {9-15}
}

@Article{Seeger68,
  author =   {P. Seeger},
  title =    {A note on a method for the analysis of significances en masse},
  journal =      {Technometrics},
  year =     {1968},
  OPTkey =   {},
  volume =   {10},
  number =   {3},
  pages =    {586--593},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Segal88,
  author =   {M. R. Segal},
  title =    {Regression trees for censored data},
  journal =      {Biometrics},
  year =     {1988},
  OPTkey =   {},
  volume =   {44},
  OPTnumber =    {},
  pages =    {35--47},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}





@string{JASA= {Journal of the American Statistical Association}}
@string{JC = {Journal of Classification}}
@string{JSPI = {Journal of Statistical Planning and Inference}}
@string{JRSSB = {Journal of the Royal Statistical Society, Series B}}
@string{PNAS = {Proc. Natl. Acad. Sci.}}

@Article{Shaffer02,
  author =   {J. P. Shaffer},
  title =    {Multiplicity, directional ({T}ype {III}) errors, and
the null hypothesis},
  journal =      {Psychological Methods},
  year =     {2002},
  OPTkey =   {},
  volume =   {7},
  OPTnumber =    {},
  pages =    {356--369},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Shaffer86,
  author =   {J. P. Shaffer},
  title =    {Modified sequentially rejective multiple test procedures},
  journal =      JASA,
  year =     {1986},
  OPTkey =   {},
  volume =   {81},
  OPTnumber =    {},
  pages =    {826--831},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Shaffer95,
  author =   {J. P. Shaffer},
  title =    {Multiple hypothesis testing},
  journal =      {Annu. Rev. Psychol.},
  year =     {1995},
  OPTkey =   {},
  volume =   {46},
  OPTnumber =    {},
  pages =    {561--584},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@article{Shao93,
AUTHOR={Shao, J.},
TITLE={Linear Model Selection by Cross-Validation},
JOURNAL={Journal of the American Statistical Association},
VOLUME={88},
YEAR={1993},
PAGES={486-494}
}




@Article{Sidak67,
  author =   {Z. \v{S}id\'{a}k},
  title =    {Rectangular confidence regions for the means of multivariate normal distributions},
  journal =      JASA,
  year =     {1967},
  OPTkey =   {},
  volume =   {62},
  OPTnumber =    {},
  pages =    {626-633},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Silverman,
  author =   {B. W. Silverman},
  title =    {Smoothed functional principal components analysis by choice of norm},
  journal =      {Annals of Statistics},
  year =     {1996},
  OPTkey =   {},
  volume =   {24},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {1--24},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Silverman84,
  author =   {B. W. Silverman},
  title =    {A fast and efficient cross-validation method for smoothing parameter choice in spline regression},
  journal =      JASA,
  year =     {1984},
  OPTkey =   {},
  volume =   {79},
  number =   {387},
  pages =    {584--589},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}




@Book{Silverman86,
  author =       {B. W. Silverman},
  title =        {Density Estimation for Statistics and Data analysis},
  publisher =    {Chapman \& Hall},
  pages = {},
  year =         {1986}
}

@Article{vanderLaan&Dudoit&Keles04,
  author =   {M.J. van der Laan and S. Dudoit and S. Keles},
  title =    {Asymptotic optimality of likelihood-based cross-validation},
  journal =      {Statistical Applications in Genetics and Molecular Biology},
  year =     {2004},
  OPTkey =   {},
  volume =   {3},
  OPTnumber =    {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/sagmb/vol3/iss1/art4},
  OPTannote =    {}
}
@Article{Simes86,
  author =   {R. J. Simes},
  title =    {An improved Bonferroni procedure for multiple tests of significance},
  journal =      {Biometrika},
  year =     {1986},
  OPTkey =   {},
  volume =   {73},
  OPTnumber =    {},
  pages =    {751--754},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Smyth00,
  author =   {P. Smyth},
  title =    {Model selection of probabilistic clustering using cross-validated likelihood},
  journal =      {Statistics and Computing},
  year =     {2000},
  volume =   {10},
  pages =    {63-72}
}




@Article{Soric89,
  author =   {B. Sori\'{c}},
  title =    {Statistical ``discoveries" and effect-size estimation},
  journal =      JASA,
  year =     {1989},
  OPTkey =   {},
  volume =   {84},
  number =   {406},
  pages =    {608--610},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Stone74,
  author =   {M. Stone},
  title =    {Cross-validatory choice and  assessment of statistical predictions},
  journal =      {Journal of the Royal Statistical Society, Series B},
  year =     {1974},
  volume =   {36},
  pages =    {111-147}
}

@Article{Stone84,
  author =   {C. J. Stone},
  title =    {An asymptotically optimal window selection rule for kernel density estimates},
  journal =      {The Annals of Statistics},
  year =     {1984},
  volume =   {12},
  pages =    {1285-1297}
}

@Article{StoneC84,
  author =   {C. J. Stone},
  title =    {An asymptotically optimal window selection rule for kernel density estimates},
  journal =      {Annals of Statistics},
  year =     {1984},
  OPTkey =   {},
  volume =   {12},
  number =   {4},
  pages =    {1285--1297},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{StoneM74,
  author =   {M. Stone},
  title =    {Cross-validatory choice and assessment of statistics predictions},
  journal =      JRSSB,
  year =     {1974},
  OPTkey =   {},
  volume =   {36},
  number =   {2},
  pages =    {111--147},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}






@Article{StoneM77,
  author =   {M. Stone},
  title =    {Asymptotics for and against cross-validation},
  journal =      {Biometrika},
  year =     {1977},
  OPTkey =   {},
  volume =   {64},
  number =   {1},
  pages =    {29--35},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@TechReport{Storey&TibshiraniTechRep01,
  author =   {J. D. Storey and R. Tibshirani},
  title =    {Estimating false discovery rates under dependence, with applications
to DNA microarrays},
  institution =  {Department of Statistics, Stanford University},
  year =     {2001},
  OPTkey =   {},
  OPTtype =      {},
  number =   {2001-28},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{StoreyJRSSB02,
  author =   {J. D. Storey},
  title =    {A direct approach to false discovery rates},
  journal =      JRSSB,
  year =     {2002},
  OPTkey =   {},
  volume =   {64},
  OPTnumber =    {},
  pages =    {479--498},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{StoreyTechRep01,
  author =   {J. D. Storey},
  title =    {The positive False Discovery Rate: A Bayesian interpretation and the q-value},
  institution =  {Department of Statistics, Stanford University},
  year =     {2001},
  OPTkey =   {},
  OPTtype =      {},
  number =   {2001-12},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{TSH,
  author =   {E. L. Lehmann},
  ALTeditor =    {},
  title =    {Testing Statistical Hypotheses},
  publisher =    {Springer-Verlag, New York},
  year =     {1986},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  edition =      {2nd},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Tibshiranietal02a,
  author =   {R. Tibshirani and T. Hastie and B. Narasimhan and. G. Chu},
  title =    {Diagnosis of multiple cancer types by shrunken centroids of gene expression},
  journal =      PNAS,
  year =     {2002},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTpages =     {},
  OPTmonth =     {},
  note =     {In press},
  OPTannote =    {}
}


@Article{Troendle95,
  author =   {J. F. Troendle},
  title =    {A stepwise resampling method of multiple hypothesis testing},
  journal =      JASA,
  year =     {1995},
  OPTkey =   {},
  volume =   {90},
  OPTnumber =    {},
  pages =    {370--378},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Troendle96,
  author =   {J. F. Troendle},
  title =    {A permutational step-up method of testing multiple outcomes},
  journal =      {Biometrics},
  year =     {1996},
  OPTkey =   {},
  volume =   {52},
  OPTnumber =    {},
  pages =    {846--859},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{VR,
 author = { W. N. Venables and B. D. Ripley },
 title = {Modern Applied Statistics with S--PLUS},
 publisher = {Springer},
 year = {1999}
}


@Book{Vaart96,
  author =       {A. W. van der Vaart  and J. A. Wellner},
  title =        {Weak {C}onvergence and {E}mprical {P}rocesses},
  publisher =    {Springer-Verlag New York},
  pages = {102},
  year =         {1996}
}





@Book{Vaart98,
  author =       {A. W. van der Vaart},
  title =        {Asymptotic Statistics},
  publisher =    {Cambridge University Press},
  pages = {62},
  year =         {1998}
}


@Book{Vapnik,
  author =   {V. N. Vapnik},
  OPTeditor =    {},
  title =    {The nature of statistical learning theory},
  publisher =    {Springer},
  year =     {2000},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  series =   {Statistics for engineering and information science},
  address =      {New York},
  edition =      {2nd},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Vapnik79,
  author =   {V. Vapnik},
  title =    {Estimation of dependences based on empirical data (in Russian)},
  journal =      {Nauka, Moskow},
  year =     {1979},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Book{Vapnik98,
  author =       {V. Vapnik},
  title =        {Statistical Learning Theory},
  publisher =    {Wiley},
  year =         {1998},
  OPTkey =       {},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {New York},
  edition =      {1st},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Book{Venables&Ripley99,
  author =   {W. N. Venables and B. D. Ripley},
  title =    {Modern applied statistics with S-PLUS},
  publisher =    {Springer},
  year =     {1999},
  OPTkey =   {},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  edition =      {3rd},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Westfall&Young93,
  author =   {P. H. Westfall and S. S. Young},
  OPTeditor =    {},
  title =    {Resampling-based multiple testing: {E}xamples and methods for $p$-value adjustment},
  publisher =    {John Wiley \& Sons},
  year =     {1993},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{,
  author =       {},
  title =        {},
  publisher =    {},
  pages = {},
  year =         {}
}


@InCollection{Westfalletal01,
  author =   {P. H. Westfall and D. V. Zaykin and S. S. Young},
  title =    {Multiple tests for genetic effects in association studies},
  booktitle =    {Biostatistical Methods},
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {143--168},
  publisher = {Humana Press, Toloway, NJ},
  year =     {2001},
  editor =   {S. Looney},
  volume =   {184},
  OPTnumber =    {},
  series =   {Methods in Molecular Biology},
  OPTtype =      {},
  OPTchapter =   {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Westonetal2000,
  author =   {J. Weston and S. Mukherjee and  O. Chappelle and  M. Pontil and  T. Poggio and V. Vapnik},
  title =    {Feature Selection for {SVM}s},
  journal =      {Advances in Neural Processing Systems},
  year =     {2001},
  OPTkey =   {},
  volume =   {13},
  number =   {},
  pages =    {668--674},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Wright92,
  author =   {S. P. Wright},
  title =    {Adjusted P-values for simultaneous inference},
  journal =      {Biometrics},
  year =     {1992},
  OPTkey =   {},
  volume =   {48},
  number =   {4},
  pages =    {1005--1013},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{YangetalJCGS02,
  author =   {Y. H. Yang and M. J. Buckley and S. Dudoit and T. P. Speed},
  title =    {Comparison of methods for image analysis on c{DNA} microarray data},
  journal =      {Journal of Computational and Graphical Statistics},
  year =     {2002},
  OPTkey =   {},
  volume =   {11},
  number =   {1},
  pages =    {108--136},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{YangetalNAR02,
  author =   {Y. H. Yang and S. Dudoit and P. Luu and D. M. Lin and V. Peng and J. Ngai and T. P. Speed},
  title =    {Normalization for c{DNA} microarray data: {A} robust composite method addressing single and multiple slide systematic variation},
  journal =      {Nucleic Acids Research},
  year =     {2002},
  OPTkey =   {},
  volume =   {30},
  number =   {4},
  pages =    {e15},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@InProceedings{YangetalSPIE01,
  author =   {Y. H. Yang and S. Dudoit and P. Luu and T. P. Speed},
  title =    {Normalization for c{DNA} microarray data},
  booktitle =    {Microarrays: Optical Technologies and Informatics},
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {141--152},
  year =     {2001},
  editor =   {Michael L. Bittner and Yidong Chen and Andreas N. Dorsel and Edward R. Dougherty},
  volume =   {4266},
  OPTnumber =    {},
  series =   {Proceedings of SPIE},
  address =      {San Jose, CA},
  month =    {May},
  OPTorganization = {SPIE},
  publisher = {SPIE-International Society for Optical Engineering},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Yekutieli&Benjamini99,
  author =   {D. Yekutieli and Y. Benjamini},
  title =    {Resampling-based false discovery rate controlling multiple test procedures for correlated test statistics},
  journal =      JSPI,
  year =     {1999},
  OPTkey =   {},
  volume =   {82},
  OPTnumber =    {},
  pages =    {171--196},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@InCollection{Youden69,
  author =   {W. J. Youden},
  title =    {Measurement agreement comparisons},
  booktitle =    {Precision measurement and calibration: Statistical concepts and procedures},
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {146--151},
  publisher = {National Bureau of Standards, United States Department of Commerce},
  year =     {1969},
  editor =   {H. H. Ku},
  volume =   {1},
  OPTnumber =    {},
  series =   {Special Publication 300},
  type =     {NBS Miscelaneous Publication 248, Proceedings of the 1962 Standards Laboratory Conference},
  OPTchapter =   {},
  OPTaddress =   {},
  OPTedition =   {},
  month =    {February},
  OPTnote =      {},
  OPTannote =    {}
}




@article{Zhang93,
AUTHOR={Zhang, P.},
TITLE={Model selection via multifold cross-validation},
JOURNAL={Annals of Statistics},
VOLUME={21},
YEAR={1993},
PAGES={299-313}
}

@Article{ZhangetalBioinf02,
  author =   {J. Zhang and V. Carey and R. Gentleman},
  title =    {An extensible application for assembling annotation for
genomic data},
  journal =      {Bioinformatics},
  year =     {2002},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {},
  OPTmonth =     {},
  note =     {(In press)},
  OPTannote =    {},
  url = {http://www.R-project.org/}
}



@Book{vanderVaart98,
  author =   {A.W. van der Vaart},
  title =    {Asymptotic Statistics},
  publisher =    {Cambridge University Press},
  year =     {1998}
}




@Book{BKRW,
  author =   {P.J. Bickel and C.A.J. Klaassen and Y. Ritov and J. Wellner},
  title =    {Efficient and Adaptive Estimation for Semiparametric Models},
  publisher =    {Springer-Verlag},
  year =     {1997}
}




@Article{bozdoganaic,
  author =   {H. Bozdogan},
  title =    {Akaike's information criterion and recent developments in information complexity},
  journal =      {Journal of Mathematical Psychology},
  year =     {2000},
  volume =   {44},
  pages =    {62-91}
}



@book {cart,
   AUTHOR = {L. Breiman and J. H. Friedman and R. A. Olshen and C. J. Stone},
    TITLE = {Classification and Regression Trees},
PUBLISHER = {Wadsworth \& Brooks/Cole},
  ADDRESS = {Monterey},
     YEAR = {1984},
    PAGES = {},
     ISBN = {}
}

@book {mark,
 author = {M.J. van der Laan and J.M. Robins},
  title = {Unified methods for censored longitudinal  data and causality},
  publisher = {Springer, New York},
  year =     {2003}
}


@Manual{effsize,
  title =    {Teaching Children to Read},
  OPTkey =   {},
  author =   {{National Reading Panel}},
  organization = {National Institute of Child Health and Human Development, National Institutes of Health},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  year =     {1999},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{gapstats,
  author =   {R. Tibshirani and  G. Walther and T. Hastie.},
  title =    {Estimating the number of clusters in a dataset via the gap statistic},
  institution =  {Department of Biostatistics, Stanford University},
  year =     {2000},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  month =    {March},
  note =     {\url{http://www-stat.stanford.edu/~tibs/research.html}},
  OPTannote =    {}
}




@InProceedings{gillcar,
  author =   {R.D. Gill and M.J. van der Laan and J.M. Robins},
  title =    {Coarsening at random: characterizations, conjectures and counter-examples},
  booktitle =    {Proceedings of the First Seattle Symposium in Biostatistics},
  pages =    {255-94},
  year =     {1997},
  editor =   {D.Y. Lin and T.R. Fleming},
  address =      {New York},
  publisher = {Springer Verlag}
}
@article{Gill&Robins01,
   AUTHOR = {Gill, R. and Robins, J.M.},
    TITLE = {Causal inference in complex longitudinal studies: continuous case},
  JOURNAL = {Ann. Stat.},
 FJOURNAL = {The Annals of Statistics},
   VOLUME = {29},
     YEAR = {2001},
   NUMBER = {6},
    PAGES = {},
     ISSN = {},
    CODEN = {},
  MRCLASS = {},
 MRNUMBER = {},
}


%uses exponential mode at each node
@Article{jacobsen,
  author =   {M. Jacobsen and N. Keiding},
  title =    {Coarsening at random in general sample spaces and random censoring in continuous time},
  journal =      {Annals of Statistics},
  year =     {1995},
  volume =   {23},
  pages =    {774-86}
}

%very first reference to use trees in survival analysis










@Misc{marray,
  OPTkey =   {},
  author =   {S. Dudoit and Y. H. Yang},
  title =    {Normalization and diagnostic plots for cDNA microarray data, {\tt marrayClasses}, {\tt marrayInput}, {\tt marrayNorm}, {\tt marrayPlots}},
  howpublished = {{\tt R} packages},
  OPTmonth =     {},
  year =     {2002},
  OPTnote =      {},
  OPTannote =    {},
  url =          {www.bioconductor.org},
}

@TechReport{mclust98,
  author =   {C. Fraley and A. E. Raftery},
  title =    {MCLUST: Software for Model-Based Cluster Analysis},
  institution =  {Department of Statistics, University of Washington},
  year =     {1998},
  OPTkey =   {},
  OPTtype =      {},
  number =   {342},
  OPTaddress =   {},
  month =    {November},
  OPTnote =      {},
  OPTannote =    {}
}


@Misc{multtest,
  OPTkey =   {},
  author =   {Y. Ge and S. Dudoit},
  title =    {Multiple Testing Procedures, {\tt multtest}},
  howpublished = {{\tt R} package},
  OPTmonth =     {},
  year =     {2002},
  OPTnote =      {},
  OPTannote =    {},
  url =          {www.bioconductor.org},
}

@InProceedings{robins93,
  author =   {J.M. Robins},
  title =    {Information recovery and bias adjustment in proportional hazards regression analysis of randomized trials using surrogate markers},
  booktitle =    {Proceeding of the Biopharmaceutical section},
  pages =    {24-33},
  year =     {1993},
  organization = {American Statistical Association}
}

@InCollection{robrot,
  author =   {J.M. Robins and A. Rotnitzky},
  title =    {Recovery of information and adjustment for dependent censoring using surrogate markers},
  booktitle =    {AIDS Epidemiology},
  publisher = {Bikh\"{a}user},
  year =     {1992},
  series =   {Methodological issues}
}


@Article{robzhao,
  author =   {J.M. Robins and A. Rotnitzky and L.P. Zhao},
  title =    {Estimation of regression coefficients when some regressors are not always observed},
  journal =      {Journal of the American Statistical Association},
  year =     {1994},
  volume =   {89},
  number =   {427},
  pages =    {846-866},
  month =    {September}
}







@Article{Heitjan&Rubin91,
  author =   {D.F. Heitjan and D.B. Rubin},
  title =    {Ignorability and coarse data},
  journal =      {Annals of statistics},
  year =     {1991},
  volume =   {19},
  number =   {4},
  pages =    {2244-2253},
  month =    {December}
}

@Misc{sma,
  OPTkey =   {},
  author =   {S. Dudoit and Y. H. Yang and B. M. Bolstad},
  title =    {Statistical {M}icroarray {A}nalysis, {\tt sma}},
  howpublished = {{\tt R} package},
  OPTmonth =     {},
  year =     {2001},
  note =     {Contributions from Natalie Thorne, Ingrid L\"{o}nnstedt, and Jessica Mar},
  OPTannote =    {},
  url =          {cran.r-project.org/src/contrib/PACKAGES.html\#sma}
}

@PhdThesis{thesis,
  author =   {S. Dudoit},
  title =    {Linkage analysis of complex human traits using identity by descent data},
  school =   {Department of Statistics, University of California, Berkeley},
  year =     {1999},
  OPTkey =   {},
  OPTaddress =   {},
  type =     {Ph.D. thesis},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{vanderVaart&Wellner96,
  author =   {A. van der Vaart and J. Wellner},
  ALTeditor =    {},
  title =    {Weak Convergence and Empirical Processes},
  publisher =    {Springer-Verlag, New York},
  year =     {1996},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@article{Raudenbush&Bryk86,
  author = {S.W. Raudenbush and A.S. Bryk},
  title= {A hierarchical model
for studying school effects. Sociology of Education},
  journal = {Sociology of Education},
  volume = {59},
  issue = {},
  pages = {1--17},
  year = {1986}
}

@techreport{vanderLaan08,
	Author = {Mark J. van der Laan},
	Date-Added = {2008-03},
	Institution = {University of California, Berkeley},
	Number = {232, www.bepress.com/ucbbiostat/paper232},
	Title = {The Construction and Analysis of Adaptive Group Sequential Designs},
	Year = {2008}}

@book{Raudenbush&Bryk02,
author={S.W. Raudenbush and A.S. Bryk},
title={Hierarchical linear models: Application and data analysis methods},
publisher={Newbury
Park: Sage.},
year={2002}
}


@article{Raudenbush&Liu00,
author={ S.W. Raudenbush and X. Liu},
titlte={Statistical power and
optimal design for multisite randomized trials},
journal={Psychological
Methods},
volume={5},
pages={199Ð213},
year={2000}
}


 @article{Raudenbush&Sampson99a,
 author={S.W. Raudenbush and  R.J. Sampson},
  title={Assessing direct
and indirect effects in multilevel designs with latent
variables},
  journal={Sociological Methods \& Research},
  volume={28},
  pages={123Ð153},
  year={1999}
   }

  @inCollection{Raudenbush&Sampson99b,
 author={S.W. Raudenbush and  R.J. Sampson},
title={Ecometrics: Toward a science of assessing ecological settings, with
application to the systematic social observation of neighbor-
hoods. In M. P. Becker (Ed.)},
 booktitle={Sociological methodology},
OPTvolume={29},
 pages={1Ð41},
 publisher={Boston, MA: Blackwell},
 year={1999}
 }

 @article{Raudenbush&Whillms95,
 author={S.W. Raudenbush and J.D. Whillms},
 title={The estimation of
school effects},
 journal={Journal of Educational and Behavioral
Statistics},
 volume={20},
 pages={307Ð335},
 year={1995}
 }

@article{Coleman58,
author={J.S. Coleman},
title={Relational analysis: The study of social
organizations with survey methods},
journal={Human Organization},
volume={17},
pages={28Ð36},
year={1958}
}

@article{Colemanetal66,
author={J.S.
Coleman and E.Q. Campbell and C.J. Hobson and J. McPartland and
A.M. Mood and F.D. Weinfeld and R.L. York},
title={Equality of educational opportunity. Washington, DC:
Government Printing OfÞce},
journal={Journal of the Royal Statistical Society, Series A},
volume={156},
pages={9Ð38},
year={1966}
}


@article{Aitkin&Longford86,
author={M. Aitkin and N. Longford},
title={Statistical modeling issues
in school effectiveness studies},
journal={Journal of the Royal
Statistical Society, Series A},
volume={149},
pages={1Ð43},
year={1986}
}

@book{Rubin06,
author={D.B. Rubin},
title={Matched Sampling for Causal Effects.},
publisher={Cambridge University Press},
address={Cambridge, MA},
year={2006},
}

@book{Goldstein95,
author={H. Goldstein},
title={Multilevel statistical models},
publisher={London:
Edward Arnold},
year={1995}
}

@article{McMichael99,
author={A.J. McMichael},
title={Prisoners of the proximate: Loosening
the constraints on epidemiology in an age of change},
journal={American Journal of Epidemiology},
volume={149},
pages={887Ð897},
year={1999}
}

@article{Susser99,
author={M. Susser},
title={Should the epidemiologist be a social
scientist or a molecular biologist?},
journal={International Journal of
Epidemiology},
volume={28},
pages={1019Ð1022},
year={1999}
}

@article{Berkmanetal00,
author={L.F. Berkman and T. Glass and I. Brissette and T.E. Seeman},
title={From social integration to health: Durkheim
in the new millennium},
journal={Social Science \& Medicine},
volume={51},
pages={843Ð857},
year={2000}
}

@article{Krieger01,
author={N. Krieger},
title={Theories for social epidemiology in the 21st
century: An ecosocial perspective},
journal={International Journal of
Epidemiology},
volume={30},
pages={668Ð677},
year={2001}
}

@book{Parsons51,
author={T. Parsons},
title={The social system},
publisher={New York: Free Press},
year={1951}
}

@book{Starr82,
author={P. Starr},
title={The social transformation of American medicine},
publisher={New York: Basic Books},
year={1982}
}

@article{Rose85,
author={G. Rose},
title={Sick individuals and sick populations},
journal={International Journal of Epidemiology},
volume={14},
pages={32Ð38},
year={1985}
}

@article{Clarketal91,
author={J. Clark and D.A. Potter and J.B. McKinlay},
title={Bringing
social structure back into clinical decision making},
journal={Social
Science \& Medicine},
volume={32},
pages={853Ð866},
year={1991}
}

@article{Barr95,
author={D.A. Barr},
title={The effects of organizational structure on
primary care outcomes under managed care},
journal={Annals of
Internal Medicine},
volume={122},
pages={353Ð359},
year={1995}
}


@article{McKinlay96,
author={J.B. McKinlay},
title={Some contributions from the social
system to gender inequalities in heart disease},
journal={Journal of
Health and Social Behavior},
volume={37},
pages={1Ð26},
year={1996}
}



@article{Feldmanetal97,
author={H.A. Feldman and J. B. McKinlay and D.A. Potter and K.M. Freund and
R.B. Burns and M.A. Moskowitz and L.E. Kasten},
title={Nonmedical inßuences on medical decision making: An
experimental technique using videotapes, factorial
design, and survey sampling},
journal={Health Services Research},
volume={32},
pages={343Ð366},
year={1997}
}

@article{Hook01,
author={E.B. Hook},
title={(Letter to Editor) RE: Neighborhood social
environment and risk of death: Multilevel evidence from the
Alameda County Study},
journal={American Journal of Epidemiology},
volume={151},
pages={1132Ð1133},
year={2001}
}

@article{Draper95,
author={D. Draper},
title={Inference and hierarchical modeling in the
social sciences},
journal={Journal of Educational and Behavioral
Statistics},
volume={20},
pages={115Ð147},
year={1995}
}

@article{Lindley&Smith72,
author={D. Lindley and A. Smith},
title={Bayes estimation for linear
models},
journal={Journal of the Royal Statistical Society, Series B},
volume={34},
pages={1Ð41},
year={1972}
}


@article{Dempsteretal77,
author={A.P. Dempster and N.M. Laird and D.B. Rubin},
title={Maximum
likelihood from incomplete data via the EM algorithm},
journal={Journal of the Royal Statistical Society, Series B},
volume={39},
pages={1Ð8},
year={1977}
}

@article{Laird&Ware82,
author={
N.M. Laird and J.H. Ware},
title={Random-effects models for
longitudinal data},
journal={Biometrics},
volume={38},
pages={963Ð974},
year={1982}
}


@inCollection{Masonetal84,
author={W.M. Mason and G.Y. Wong and B. Entwisle},
title={Contextual
analysis through the multilevel Linear Model. In S.
Leinhardt (Ed.)},
booktitle={Sociological methodology: 1983Ð1984},
publisher={San
Francisco: Jossey-Bass},
year={1984}
}




@book{Goldstein87,
author={H. Goldstein},
title={Multilevel statistical models in educational
and social research},
publisher={London: Edward Arnold},
year={1987}
}



@book{Bryk&Raudenbush92,
author={A.S. Bryk and S.W. Raudenbush},
title= {Hierarchical linear
models},
publisher={Newbury Park: Sage},
year={1992}
}


@book{Verbeke&Molenbergs97,
author={G. Verbeke and G. Molenbergs},
title={Linear mixed models in practice: A SAS oriented approach},
publisher={New York: Springer},
year={1997}
}



@article{Singer98,
author={J.D. Singer},
title={Using SAS proc mixed to Þt multilevel
models, hierarchical models, and individual growth models},
journal={Journal of Educational and Behavioral Statistics},
volume={24},
pages={323Ð355},
year={1998}
}


@article{Kreftetal94,
author={I.G.G. Kreft and J. de Leeuw and R. van der Leeden},
title={Review of Þve multilevel analysis programs: BMDP-5,
GENMOD, HLM, ML3, VARCL. },
journal={American Statistician},
volume={48},
pages={324Ð335},
year={1994}
}

@inCollection{Deleeuw&Kreft01,
author={J. De Leeuw and I.G.G. Kreft},
title={Software for multilevel
analysis},
booktitle={In H. Goldstein (Ed.), Multilevel modelling of
health statistics},
pages={187Ð204},
publisher={New York: Wiley},
year={2001}
}


@book{Susser73,
author={M. Susser},
title={Causal thinking in health sciences: Concepts
and strategies of epidemiology},
publisher={New York: Oxford},
year={1973}
}

@inCollection{Freedman91,
author={D. Freedman},
title={Statistical models and shoe leather (with
discussion). In P. V. Marsden (Ed.)},
booktitle={Sociological methodol-
ogy},
OPTvol={21},
publisher={San Francisco: Jossey-Banks},
year={1991}
}

@article{Freedman97,
author={D. Freedman},
title={From association to causation via
regression (with comments). In S. P. Turner (Ed.)},
booktitle={Causality in crisis? Statistical methods and the search for causal
knowledge in the social sciences},
OPTpages={113Ð182},
publisher={Notre Dame,
IN: Notre Dame University Press},
year={1997}
}


@article{Greenland90,
author={S. Greenland},
title={Randomization, statistics, and causal
inference},
journal={Epidemiology},
volume={1},
pages={421Ð429},
year={1990}
}


@article{Greenland96,
author={S. Greenland},
title={Basic methods for sensitivity analysis of
biases},
journal={International Journal of Epidemiology},
volume={25},
pages={1107Ð1116},
year={1996}
}

@article{Greenland00,
author={S. Greenland},
title={Principles of multilevel modelling},
journal={International Journal of Epidemiology},
volume={29},
pages={158Ð167},
year={2000}
}

@article{Greenland01,
author={S. Greenland},
title={Ecologic versus individual-level sources of
bias in ecologic estimates of contextual health effects},
journal={International Journal of Epidemiology},
volume={30},
pages={1343Ð1350},
year={2001}
}

@article{Greenland02,
author={S. Greenland},
title={A review of multilevel theory for
ecological analyses},
journal={Statistics in Medicine},
volume={21},
pages={389Ð395},
year={2002}
}

@article{Greenland&Morgenstern01,
author={S. Greenland and H. Morgenstern},
title={Confounding in
health research},
journal={Annual Review of Public Health},
volume={22},
pages={189Ð212},
year={2001}
}

@article{Greenlandetal99,
author={S. Greenland and J. Pearl and J.M. Robins},
title= {Causal
diagrams for epidemiologic research},
journal={Epidemiology},
volume={10},
pages={37Ð48},
year={1999}
}


@article{Manski93,
author={C.F. Manski},
title={IdentiÞcation of endogenous social
effects: The reßection problem},
journal={Review of Economic Studies},
volume={60},
pages={531Ð542},
year={1993}
}


@inCollection{Manski93b,
author={C.F. Manski},
title={IdentiÞcation problems in the social
sciences. In P. V. Marsden (Ed.)},
booktitle={Sociological methodology},
publisher={San Francisco: Jossey-Banks},
year={1993}
}


@article{Halloran&Struchiner95,
author={M.E. Halloran and C.J. Struchiner},
title={Causal inference in
infectious diseases},
journal={Epidemiology},
volume={6},
pages={142Ð151},
year={1995}
}

@article{Morgenstern95,
author={H. Morgenstern},
title={Ecologic studies in epidemiology:
Concepts, principles, and methods},
journal={Annual Review of Public
Health},
volume={16},
pages={61Ð81},
year={1995}
}

@inCollection{Sobel95,
author={M.E.Sobel},
title={Causal inference in the social and
behavioral sciences},
booktitle={In M. E. Sobel (Ed.), Handbook of
statistical modeling for the social and behavioral sciences},
pages={1Ð38},
publisher={New York: Plenum.},
year={1995}
}


@article{Kaufman&Cooper99,
author={J.S. Kaufman and R.S. Cooper},
title={Seeking causal
explanations in social epidemiology},
journal={American Journal of
Epidemiology},
volume={150},
pages={113Ð120},
year={1995}
}

@article{Kaufman&Poole00,
author={J.S. Kaufman and C. Poole},
title={Looking back on causal
thinking in the health sciences},
journal={Annual Review of Public
Health},
volume={21},
pages={101Ð119},
year={2000}
}

@article{Kaufman&Kaufman01,
author={J. S. Kaufman and S. Kaufman},
title={Assessment of
structured socioeconomic effects on health},
journal={Epidemiology},
volume={12},
pages={157Ð167},
year={2001}
}

@article{Robins01,
author={J.M. Robins},
title={Data, design, and background knowledge
in etiologic inference},
journal={Epidemiology},
volume={12},
pages={313Ð320},
year={2001}
}


@article{Maldonado&Greenland02,
author={G. Maldonado and S. Greenland},
title={Estimating causal effects},
journal={International Journal of Epidemiology},
volume={31},
pages={422Ð438},
year={2002}
}

@book{Campbell&Stanley63,
author={D.T. Campbell and J.C. Stanley},
title={Experimental and
quasi-experimental designs for research},
publisher={Hopewell, NJ:
Houghton Mifßin},
year={1963}
}

@article{Cochran65,
author={W.G. Cochran},
title={The planning of observational studies
of human populations},
journal={Journal of the Royal Statistical
Society, Series A},
volume={128},
pages={243Ð265},
year={1965}
}

@article{McKinlay75,
author={S.M. McKinlay},
title={The design and analysis of the
observational studyÑa review},
journal={Journal of the American
Statistical Association},
volume={70},
pages={503Ð523},
year={1975}
}

@article{Heckman79,
author={J.J. Heckman},
title={Sample selection bias as a speciÞcation
error},
journal={Econometrica},
volume={47},
pages={153Ð162},
year={1979}
}


@article{Leamer83,
author={E. Leamer},
title={LetÕs take the con out of econometrics},
journal={American Economic Review},
volume={73},
pages={32Ð43},
year={1983}
}

@inCollection{Smith90,
author={H.L. Smith},
title={SpeciÞcation problems in experimental and
nonexperimental social research},
booktitle={In C. C. Clogg (Ed.), Sociological methodology},
volume={20},
publisher={Oxford: Basil},
year={1990}
}

@article{Rubin91,
author={D.B. Rubin},
title={Practical implications of modes of
statistical inference for causal effects and the critical role
of the assignment mechanism},
journal={Biometrics},
volume={47},
pages={1213Ð1234},
year={1991}
}

@inCollection{Clogg&Haritou97,
author={C.C. Clogg and A. Haritou},
title={The regression method for causal inference and a dilemma confronting this method},
booktitle={In S. P. Turner (Ed.), Causality in crisis? Statistical methods
and the search for causal knowledge in the social sciences},
pages={83Ð112},
publisher={Notre Dame, IN: Notre Dame University Press},
year={1997}
}

@article{Copas&Li97,
author={J.B. Copas and H.G. Li},
title={Inference for non-random
samples (with discussion)},
journal={Journal of the Royal Statistical
Society, Series B},
volume={59},
pages={55Ð95},
year={1997}
}

@inCollection{Freedman97,
author={D. Freedman},
title={From association to causation via
regression (with comments)},
booktitle={In S. P. Turner (Ed.), Causality
in crisis? Statistical methods and the search for causal
knowledge in the social sciences},
pages={113Ð182},
publisher={Notre Dame,
IN: Notre Dame University Press},
year={1997}
}

@article{Winship&Morgan99,
author={C. Winship and S.L.  Morgan},
title={The estimation of causal
effects from observational data},
journal={Annual Review of Sociology},
volume={25},
pages={659Ð707},
year={1999}
}

@book{Pearl00,
author={J. Pearl},
title={Causality: Models, reasoning, and inference},
publisher={ New York: Cambridge University Press},
year={2000}
}

@book{Rosenbaum02,
author={P.R. Rosenbaum},
title={Observational studies},
publisher={New York:
Springer},
year={2002}
}


@article{Charltonetal85,
author={J.R. Charlton and M.F. DÕSouza and M. Tooley and R. Silver},
title={A community trial strategy for evaluating treatment
for symptomatic conditions},
journal={Statistics in Medicine},
volume={4},
pages={11Ð21},
year={1985}
}

@article{Meyeretal91,
author={L. Meyer and N. Job-Spira and J. Bouyer and E. Bouvet and A. Spira},
title={Prevention of sexually transmitted diseases: A
randomised community trial},
journal={Journal of Epidemiology and
Community Health},
volume={45},
pages={152Ð158},
year={1991}
}


@article{Shipleyetal95,
author={R.H. Shipley and T.D. Hartwell and W.D. Austin and A.C. Clayton and L.C. Stanley },
title={Community stop-smoking contests
in the COMMIT trial: Relationship of participation to
costs},
journal={Community intervention trials. Preventive Medicine},
volume={ 24},
pages={286Ð292},
year={1995}
}

@article{Holderetal97,
author={H.D. Holder and R.F. Saltz and A.J. Treno and J.W. Grube and R.B. Voas},
title={Evaluation design for a community prevention
trial. An environmental approach to reduce alcohol-
involved trauma},
journal={Evaluation Review},
volume={21},
pages={140Ð165},
year={1997}
}

@article{Feldmanetal98,
author={H.A. Feldman and M.A. Proschan and D.M. Murray and D.C. Goff and M.
Stylianou and E. Dulberg and P.G. McGovern and W. Chan and N.C.
Mann and V. Bittner},
title={Statistical design of
REACT (Rapid Early Action for Coronary Treatment), a
multisite community trial with continual data collection},
journal={Controlled Clinicial Trials},
volume={19},
pages={391Ð403},
year={1998}
}

@article{LeFortetal98,
author={S.M. LeFort and K. Gray-Donald and K.M. Rowat and M.E. Jeans},
title={Randomized controlled trial of a community-based
psychoeducation program for the self-management of
chronic pain},
journal={Pain},
volume={74},
pages={297Ð306},
year={1998}
}


@article{Perskyetal99,
author={V. Persky and L. Coover and E. Hernandez and A. Contreras and J. Slezak and J. Piorkowski and L. Curtis and M. Turyk and V. Ramakrishnan and  P. Scheff},
title={Chicago community-based asthma
intervention trial: Feasibility of delivering peer education in
an inner-city population},
journal={Chest},
volume={116},
pages={216SÐ223S},
year={1999}
}

@article{Biglanetal00,
author={A. Biglan and K. Smolkowski and T. Duncan and C. Black},
title={A randomised controlled trial of a community
intervention to prevent adolescent tobacco use},
journal={Tobacco
Control},
volume={9},
pages={24Ð32},
year={2000}
}


@article{Luepkeretal00,
author={R.V. Luepker and J.M. Raczynski and S. Osganian and R.J Goldberg and
Jr. J.R.  Finnegan and J.R. Hedges and Jr. D.C. Goff and M.S.
Eisenberg and J.G. Zapka and H.A. Feldman and D.R. Labarthe and P.G. McGovern and C.E. Cornell and M.A. Proschan and D.G. Simons-Morton},
title={Effect of a community
intervention on patient delay and emergency medical service
use in acute coronary heart disease: The rapid early action
for coronary treatment (REACT) trial},
journal={JAMA},
volume={284},
pages={60Ð67},
year={2000}
}


@Article{Oakes04,
  author = {J.M. Oakes},
  title= {The (mis)estimation of neigborhood effects: causal inference for a practicable social epidemiology },
  journal = {Social Science and Medicine},
  volume = {58},
  issue = {},
  pages = {1929--1952},
  year = {2004}
}

@Article{Abadie&Imbens06,
  author = {A. Abadie and G.W. Imbens},
  title= {Large Sample Properties of Matching Estimators for Average Treatment Effects},
  journal = {Econometrica},
  volume = {74},
  issue = {1},
  pages = {235-67},
  year = {2006}
}

@Article{Greenland&Morgenstern90,
  author = {S. Greenland and H. Morgenstern},
  title= {Matching and Efficiency in Cohort Studies},
  journal = {American Journal of Epidemiology},
  volume = {131},
  issue = {1},
  pages = {151-159},
  year = {1990}
}

@Article{Costanza95,
  author = {M. Costanza},
  title= {Theoretical Epidemiology, Matching},
  journal = {Preventive Medicine},
  volume = {24},
  issue = {},
  pages = {425-433},
  year = {1995}
}

@Article{Joffe&Rosenbaum99,
  author = {M.M. Joffe and P.R. Rosenbaum},
  title= {Invited Commentary: Propensity Scores},
  journal = {American Journal of Epidemiology},
  volume = {150},
  issue = {4},
  pages = {327-333},
  year = {1999}
}


@article{Neugebauer&vanderLaan07,
author={R. Neugebauer, M. J. van der Laan},
title={ Nonparametric Causal E?ects based on
marginal structural models},
journal={Journal of Statistical Planning and Inference},
year={2007},
volume={137},
pages={419Ð434},
}




@article{Murphy05,
author={S. Murphy},
title={An experimental design for the development of adaptive treatment strategies},
journal={Statistics in Medicine},
year={2005},
volume={24},
pages={1455Ð1481},
}

@article{Lavori&Dawson00,
author={P. Lavori and R. Dawson},
title={A design for testing clinical strategies: biased adaptive within-subject
randomization},
journal={Journal of the Royal Statistical Society, Series A},
volume={163},
pages={29Ð38},
year={2000},
}

@article{Lavori&Dawson04,
author={P. Lavori  and R. Dawson},
title={Dynamic treatment regimes: practical design considerations},
journal={Clinical trials},
volume={1},
pages={9Ð20},
year={2004},
}

@article{Thalletal00,
author={P. Thall and R. Millikan and H.-G. Sung},
title={Evaluating multiple treatment courses in clinical trials},
journal={Statistics in Medicine},
volume={19},
pages={1011Ð1028},
year={2000},
}

@article{Rushetal03,
author={A.J. Rush and M. Trivedi and M. Fava},
title={Depression},
journal={IV. American Journal of Psychiatry},
volume={160(2)},
pages={237},
year={2003},
}

@article{Schneideretal06,
author={Schneider, L. and Tariot.P.N. and Dagerman, K. and Davis, S. and Hsiao, J. and Ismail, S. and Lebowitz, B. and Lyketsos, C. and Ryan
J. and Stroup T. and Sultzer D. and Weintraub, D. and Lieberman, J.},
title= {E?ectiveness of atypical antipsychotic
drugs in patients with AlzheimerÕs disease},
journal={New England Journal of Medicine},
volume={355(15)},
pages={1525Ð1538},
year={2006},
}

@article{Swartzetal07,
author={Swartz, M. and Perkins, D. and Stroup, T. and Davis, S. and Capuano, G. and Rosenheck, R. and Reimherr, F. and McGee, M. and Keefe,
R. and McEvoy, J. and Hsiao, J. and Lieberman, J.},
title={Effects of antipsychotic medications on psychosocial
functioning in patients with chronic shizophrenia: Findings from the nimh catie study},
year={2007},
journal={American Journal
of Psychiatry},
volume={164},
pages={428Ð436},
}

@article{Rubin&vanderLaan08,
author={D.B. Rubin and M.J. van der Laan},
title={Empirical Efficiency Maximization: Improved Locally Efficient Covariate Adjustment in Randomized Experiments and Survival Analysis},
year={2008},
journal={The International Journal of Biostatistics},
volume={Vol. 4, Iss. 1, Article 5},
location={http://www.bepress.com/ijb/vol4/iss1/5},
}


@article{vanderLaan&Rose&Gruber09,
author={M.J. van der Laan and S. Rose and S. Gruber},
title={Readings on Targeted Maximum Likelihood Estimation},
year={September, 2009},
journal={Technical report, working paper series http://www.bepress.com/ucbbiostat/paper254/},
}

@article{Bembometal09,
author={O. Bembom and M.J. van der Laan and T. Haight and I.B. Tager},
title={Lifetime and
current leisure time physical activity and all-cause mortality in an elderly cohort},
year={2009},
journal={Epidemiology},
volume={},
pages={},
}

@article{Bembom&vanderLaan07a,
author={Oliver Bembom and Mark van der Laan},
title={Statistical Methods for analyzing sequentially randomized trials, commentary on JNCI article Adaptive therapy for androgen independent prostate cancer: A Randomized selection trial including four regimens, by Peter F. Thall, C. Logothetis, C. Pagliaro, S. Wen, M.A. Brown, D. Williams, R. Millikan (2007). },
journal={Journal of the National Cancer Institute},
year={2007},
volume={99(21)},
pages={1577-1582},
 }

@article{Rosenblumetal09,
author={M. Rosenblum and S.G. Deeks and M.J. van der Laan and D.R. Bangsberg},
title={The Risk
of Virologic Failure Decreases with Duration of HIV Suppression, at Greater
than 50\% Adherence to Antiretroviral Therapy},
year={2009},
journal={PLoS ONE},
volume={4(9): e7196.doi:10.1371/journal.pone.0007196},
}



@article{Robinsetal08,
author={J. Robins and L. Orallana and A. Rotnitzky},
title={Estimaton and extrapolation of optimal treatment and  testing strategies},
journal={Statistics in Medicine},
year={2008},
volume={27(23)},
pages={ 4678-4721},
}


@article{Bembom&vanderLaan07,
author= {O. Bembom and M.J. van der Laan},
title={A practical illustration of the importance of realistic individualized treatment rules in causal inference},
journal={Electronic Journal of Statistics},
year={2007},
pages={http://www.i-journals.org/ejs/viewarticle.php?id=105&layout=abstract},
}

@article{Bembometal08,
author={O. Bembom and M.L. Petersen and S.-Y. Rhee and W. J. Fessel and S.E. Sinisi and R.W. Shafer and M.J. van der Laan},
title ={Biomarker discovery using targeted maximum likelihood estimation: Application to the treatment of antiretroviral resistant HIV infection},
journal={Statistics in Medicine},
year={2008},
pages={http://www3.interscience.wiley.com/journal/121422393/abstract},
}

@article{Cassel76,
author={J. Cassel},
title={The contribution of the social environment to host resistance},
journal={American Journal of Epidemiology},
volume={104},
pages={107--123},
year={1976}
}

@article{Tuglus&vanderLaan08,
author={C. Tuglus and M.J. van der Laan},
title={Targeted Methods for Biomarker Discovery, the Search for a Standard},
journal={UC Berkeley Working Paper Series},
year={2008},
pages={http://www.bepress.com/ucbbiostat/paper233/.},
}

@article{vanderLaan08,
author={M.J. van der Laan},
title={Estimation Based on Case-Control Designs with Known Prevalance Probability},
journal={The International Journal of Biostatistics},
year={2008},
pages={http://www.bepress.com/ijb/vol4/iss1/17/},
}

@article{Rose&vanderLaan08,
author={S. Rose and M.J. van der Laan},
title={Simple Optimal Weighting of Cases and Controls in Case-Control Studies},
journal={The International Journal of Biostatistics},
year={2008},
pages={http://www.bepress.com/ijb/vol4/iss1/19/.},
}

@article{Rose&vanderLaan09,
author={S. Rose and M.J. van der Laan},
title={Why Match? Investigating Matched Case-Control Study Designs with Causal Effect Estimation},
journal={The International Journal of Biostatistics},
year={2009},
pages={http://www.bepress.com/ijb/vol5/iss1/1/.},
}


@inproceedings{Moore&vanderLaan09,
author={K.L. Moore and M.J. van der Laan},
title={Application of Time-to-Event Methods in the Assessment of Safety in Clinical Trials},
booktitle={in Design, Summarization, Analysis \& Interpretation of Clinical Trials with Time-to-Event Endpoints},
year={2009},
editor={Karl E. Peace},
publisher={Chapman and Hall},
}

@inproceedings{Polley&vanderLaan09,
author={E.C. Polley and M.J. van der Laan},
title={Predicting Optimal Treatment Assignment Based on Prognostic Factors in Cancer Patients},
booktitle={in Design, Summarization, Analysis \& Interpretation of Clinical Trials with Time-to-Event Endpoints},
year={2009},
editor={Karl E. Peace},
publisher={Chapman and Hall},
}


@article{vanderVaart&Dudoit&vanderLaan06,
  author =       {A.W. van der Vaart and S. Dudoit and M.J. van der Laan},
  title =        {Oracle Inequalities for Multi-Fold Cross-Validation},
   journal = {Statistics and Decisions},
   volume={24},
 number={3},
 year={2006},
 pages={351--371},
}

@article{vanderLaan&Dudoit&vanderVaart06,
  author =       {M.J. van der Laan and S. Dudoit and A.W. van der Vaart},
  title =        {The Cross-Validated Adaptive Epsilon-Net Estimator},
   journal = {Statistics and Decisions},
   volume={24},
 number={3},
 year={2006},
 pages={373--395},
}

 @article{Rosenbaum&Rubin83,
 author={P.R. Rosenbaum and D.B. Rubin},
 title={The Central Role of the Propensity Score in Observational Studies for Causal Effects},
 journal={Biometrika},
 volume={70},
 year={1983},
 pages={41-55}
 }

@article{vanderLaan&Polley&Hubbard07,
 author = {M.J. van der Laan and E. Polley and A. Hubbard},
 title = {Super Learner},
 journal = {Statistical Applications in Genetics and Molecular Biology},
 volume = {6},
 number ={25},
 year = {2007},
 issn = {1},
 location={http://www.bepress.con/sagmb/vol6/iss1/art25},
 }

 @article{Sekhon08,
 author={J.S. Sekhon},
 title= {Multivariate and Propensity Score Matching
 Software with Automated Balance Optimization: The Matching package for {R}},
 journal = {Journal of Statistical Sotware, Forthcoming},
 publisher={SSRN},
location = {http://ssrn.com/paper=1009044},
year={2008}
}

@article{Bembom&Fessel&Shafer&vanderLaan08,
	location = {http://www.scientificcommons.org/36721107},
	title = {Data-adaptive Selection Of The Adjustment Set In Variable Importance Estimation},
	author = {O. Bembom and J.W. Fessel and R.W. Shafer  and M.J. van der Laan},
	year = {2008},
	keywords = {General Biostatistics},
	publisher = {The Berkeley Electronic Press},
	url = {http://www.bepress.com/ucbbiostat/paper231},
	institution = {DigitalCommons@Florida Atlantic University [http://digitalcommons.fau.edu/cgi/oai2.cgi] (United States)},
}

@article{Holland77,
 author = {J.H. Holland and J.S. Reitman},
 title = {Cognitive systems based on adaptive algorithms},
 journal = {SIGART Bull.},
 volume = {63},
 year = {1977},
 issn = {0163-5719},
 pages = {49--49},
 doi = {http://doi.acm.org/10.1145/1045343.1045373},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

@book{Rubin06,
author={D.B. Rubin},
title={Matched Sampling for Causal Effects.},
publisher={Cambridge University Press},
address={Cambridge, MA},
year={2006},
}

@incollection{Mans81,
author={C.F. Manski and D. McFadden},
title={Alternative estimators and sample designs for discrete choice analysis},
booktitle={Structural Analysis of Discrete Data with Econometric Applications},
publisher={The MIT Press},
address={Cambridge, MA},
year={1981},
editor={C.F. Manski and D. McFadden},
}

@article{Mans77,
author={C.F. Manski and S.R. Lerman},
title={The Estimation of Choice Probabilities from Choice Based Samples},
journal={Econometrica},
volume={45},
number={8},
pages={1977-1988},
year={1977},
}

@article{Coss81,
author={S.R. Cosslett},
title={Maximum Likelihood Estimator for Choice-Based Samples},
journal={Econometrica},
volume={49},
number={5},
pages={1289-1316},
year={1981},
}


@article{Corn51,
author={J. Cornfield},
title={A method of estimating comparative rates from clinical data.  Applications to cancer of the lung, breast, and cervix.},
journal={J Nat Cancer Inst},
volume={11},
pages={1269-1275},
year={1951},
}

@inproceedings{Corn56,
author={J. Cornfield},
title={A statistical problem arising from retrospective studies},
booktitle={Proceedings of the Third Berkeley Symposium, Volume IV},
year={1956},
editor={J. Neyman},
pages={133-148},
publisher={University of California Press},
}

@article{Beni94,
author={J. Benichou and S. Wacholder},
title={A comparison of three approaches to estimate exposure-specific incidence rates from population-based case-control data.},
journal={Statistics in Medicine},
volume={13},
pages={651-661},
year={1994},
}
@article{Breslow&Robins&Wellner00,
author={N.E. Breslow and J.M. Robins and J.A. Wellner},
title={On the semi-parametric efficiency of logistic regression under case-control sampling},
journal={Bernoulli},
volume={6(3)},
pages={447--455},
year={2000},
}
@article{Mansonetal07,
author = {R. Mansson, M.M. Joffe, W. Sun, S. Hennessy},
title = {On the Estimation and Use of Propensity Scores in Case-Control and Case-Cohort Studies.},
journal = {Am J Epidemiol},
volume = {166},
number = {3},
pages = {332-339},
year = {2007},
}

@article{And79,
author={J.A. Anderson},
title={Separate sample logistic discrimination},
journal={Biometrika},
volume={59},
pages={19--35},
year={1972},
}

@article{Prentice&Pike79,
author={R.L. Prentice and R. Pyke},
title={Logistic disease incidence models and case-control studies},
journal={Biometrika},
volume={66},
pages={403--411},
year={1979},
}

@article{Breslow96,
author={N.E. Breslow},
title={Statistics in Epidemiology: the Case-Control Study},
journal={J Am Stat Soc},
volume={91},
pages={14--28},
year={1996},
}

@book{Breslow&Day80,
author={N.E. Breslow and N.E. Day},
title={Statistical Methods in Cancer Research:  Volume 1 -- The analysis of case-control studies},
publisher={International Agency for Research on Cancer},
address={Lyon},
year={1980},
}

@article{Holfordetal78,
author={T.R. Holford and C. White and J.L. Kelsey},
title={Multivariate Analysis for Matched Case-Control Studies},
journal={Am J Epid},
volume={107},
number={3},
pages={245--255},
year={1978},
}

@article{Breslowetal78,
author={N.E. Breslow and N.E. Day and K.T. Halvorsen and R.L. Prentice and C. Sabal},
title={Estimation of Multiple Relative Risk Functions in Matched Case-Control Studies},
journal={Am J Epid},
volume={108},
number={4},
pages={299--307},
year={1978},
}

@book{Schlesselman82,
author={J.J. Schlesselman},
title={Case-Control Studies:  Design, Conduct, Analysis},
publisher={Oxford University Press},
address={Oxford},
year={1982},
}

@book{Collett91,
author={D. Collett},
title={Modeling Binary Data},
publisher={Chapman and Hall},
address={London},
year={1991},
}

@book{Jewell04,
author={N.P. Jewell},
title={Statistics for Epidemiology},
publisher={Chapman and Hall/CRC},
address={Boca Raton},
year={2004},
}

@book{Hosmer&Lemeshow00,
author={D.W. Hosmer and S. Lemeshow},
title={Applied Logistic Regression},
edition={2nd},
publisher={John Wiley and Sons},
address={New York},
year={2000},
}

@article{Robins99,
author={J.M. Robins},
title={[Choice as an Alternative to Control in Observational Studies]:  Comment},
journal={Statistical Science},
volume={14},
number={3},
pages={281--293},
year={1999},
}

@article{Newman06,
author={S. Newman},
title={Causal Analysis of Case-Control Data},
journal={Epid Persp Innov},
volume={3},
pages={2},
url={http://www.epi-perspectives.com/content/3/1/2},
year={2006},
}

@article{Zele86,
author={M. Zelen and R.A. Parker},
title={Case-Control Studies and Bayesian Inference},
journal={Stat Med},
volume={5},
number={3},
pages={261--269},
year={1986},
}

@article{Sinh04,
author={S. SInha and B. Mukherjee and M Ghosh},
title={Bayesian Semiparametric Modeling for Matched Case-Control Studies with Multiple Disease States},
journal={Biometrics},
volume={60},
pages={41--49},
year={2004},
}

@article{Ritc01,
author = {M.D. Ritchie and L.W. Hahn and N. Roodi and L.R. Bailey and W.D. Dupont and F.F. Parl and J.H. Moore},
title = {Multifactor-dimensionality reduction reveals high-order interactions among estrogen-metabolism genes in sporadic breast cancer.},
journal = {Am J Hum Genet},
volume = {69},
number = {1},
pages = {138--47},
year = {2001},
}

@article{Mei07,
author = {H. Mei and M.L. Cuccaro and E.R. Martin},
title = {Multifactor dimensionality reduction-phenomics: a novel method to capture genetic heterogeneity with use of phenotypic variables.},
journal = {Am J Hum Genet},
volume = {81},
number = {6},
pages = {1251-61},
year = {2007},
}




@article{
Bangsberg04,
   Author = {D.R. Bangsberg and A.R. Moss and S.G. Deeks},
   Title = {Paradoxes of adherence and drug resistance to {HIV} antiretroviral therapy},
   Journal = {J Antimicrob Chemother},
   Volume = {53},
   Number = {5},
   Pages = {696-9},
   Note = {0305-7453 (Print)
Journal Article
Review},
   Abstract = {Public health debates about providing HIV antiretroviral therapy to impoverished populations have centred on the relationship between adherence and risk of drug resistance. Recent data indicate that each antiretroviral therapeutic class has a unique adherence-resistance relationship. Resistance to single protease inhibitor therapy occurs most frequently at moderate to high levels of adherence, resistance to non-nucleoside reverse transcriptase inhibitor therapy occurs at low to moderate levels of adherence, and resistance to ritonavir-boosted protease inhibitor therapy is most likely to occur at middle ranges of adherence. These dynamic relationships should be considered in balancing the individual and public health benefits of therapy.},
 Keywords = {Anti-HIV Agents/*therapeutic use
Developing Countries
*Drug Resistance, Viral
Humans
*Patient Compliance
Public Health
Research Support, Non-U.S. Gov't
Research Support, U.S. Gov't, P.H.S.},
   Year = {2004} }


@Article{Scharfstein&Tsiatis&Robins97,
  author =   {D.O. Scharfstein and A.A. Tsiatis and J.M. Robins},
  title =    {Semiparametric efficiency and its implications on the design and analysis of group-sequential studies},
journal =      {Journal of the American Statistical Association},
  year =     {1997},
  OPTkey =   {},
  volume =   {92},
  number =   {440},
  pages =    {1342--1350},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Bembom&Petersen07,
   author={O. Bembom and M. Petersen and SY Rhee and W.J. Fessel and S.E. Sinisi and R.W. Shafer 	     and M.J. van der Laan},
   title={Biomarker Discovery Using Targeted Maximum Likelihood Estimation: Application to the  Treatment of Antiretroviral Resistant {HIV} Infection},
   journal= {U.C. Berkeley Division of Biostatistics Working Paper Series},
   year={2007},
  volume={221},
   OPTmonth={August},
  OPTnote={http://www.bepress.com/ucbbiostat/paper221}
}

@Article{vanderLaan&Gruber09,
  author=  {M.J. van der Laan and S. Gruber},
  title={Collaborative Double robust penalized targeted maximum likelihood estimation},
  journal={The International Journal of Biostatistics},
  year={2010},
  volume={},
 }
@Article{Gruber&vanderLaan09,
  author=  {S. Gruber and M.J. van der Laan},
  title={An application of collaborative targeted maximum likelihood estimation in causal inference and genomics},
  journal={The International Journal of Biostatistics},
  year={2010},
  volume={},
 }
@Article{vanderLaan&Rubin06,
  author =   {M.J. van der Laan and D. Rubin},
  title =    {Targeted Maximum Likelihood Learning},
journal =      {The International Journal of Biostatistics},
  year =     {2006},
  OPTkey =   {},
  volume =   {2},
  number =   {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/ijb/vol2/iss1/11},
  OPTannote =    {}
}


@Article{Scharfstein&Tsiatis98,
  author =   {D.O. Scharfstein and A.A. Tsiatis},
  title =    {The use of simulation and bootstrap in information based group sequential studies},
journal =      {Statistics in Medicine},
  year =     {1998},
  OPTkey =   {},
  volume =   {17},
  number =   {},
  pages =    {75--87},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Pampallona&Tsiatis&Kim01,
  author =   {S. Pampallona and A.A. Tsiatis and K. Kim},
  title =    {Interim monitoring of group sequential trials using spending functions for the type I and type II error probabilities},
journal =      {Drug Informational Journal},
  year =     {2001},
  OPTkey =   {},
  volume =   {35},
  number =   {},
  pages =    {1113-1121},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Tsiatis&Mehta03,
  author =   {A.A. Tsiatis and C. Mehta},
  title =    {On the inefficiency of the adaptive design for monitoring clinical trials},
journal =      {Biometrika},
  year =     {2003},
  OPTkey =   {},
  volume =   {90},
  number =   {},
  pages =    {367-378},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Banerjee&Tsiatis06,
  author =   {A. Banerjee and A.A. Tsiatis},
  title =    {Adaptive two-stage designs in phase II clinical trials},
journal =      {Statistics in Medicine},
  year =     {2006},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {In press},
  OPTannote =    {}
}
@Article{Tsiatis06,
  author =   {A.A. Tsiatis},
  title =    {Information based monitoring of clinical trials},
journal =      {Statistics in Medicine},
  year =     {2006},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {In press},
  OPTannote =    {}
}

@Article{Lokhnygina&Tsiatis06,
  author =   {Y. Lokhnygina and A.A. Tsiatis},
  title =    {Optimal two-stage group sequential designs},
journal =      {Journal of Statistical Planning and Inference},
  year =     {2006},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {},
  OPTnote =      {In press},
  OPTannote =    {}
}

  @Article{Bauer&Kohne94,
  author =   {P. Bauer and Kohne},
  title =    {Evaluation of experiments with adaptive interim analysis},
journal =      {Biometrics},
  year =     {1994},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {1029--1041},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Cui&Hung&Wang99,
  author =   {L. Cui and H.M.J. Wang and S-J Wang},
  title =    {Modification of sample size in group sequential trials},
journal =      {Biometrics},
  year =     {1999},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {853--857},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Jennison&Turnbull03,
  author =   {C. Jennison and B.W. Turnbull},
  title =    {Mid course sample size modification in clinical trials based on hte observed treatment effect},
journal =      {Statistics in Medicine},
  year =     {2003},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {971--993},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Koyama&Sampson&Gleser04,
  author =   {T. Koyama and A.R. Sampson and L.J. Gleser},
  title =    {A calculus for design of two stage adaptive procedures},
journal =      {Journal of the Americal Statistical Association},
  year =     {2004},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Lan&Trost97,
  author =   {K.K.G Lan and D.C. Trost},
  title =    {Estimation of parameters and sample size re-estimation},
journal =      {Proceedings Biopharm Section},
  year =     {1997},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {48-51},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Li&Shih&Xie&Lu02,
  author =   {G. Li and W.J. Shih and T. Xie and J. Lu},
  title =    {A sample size adjustment procedure for clinical trials based on conditional power},
journal =      {Biostatistics},
  year =     {2002},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {277--287},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Mehta&Tsiatis01,
  author =   {C.R. Mehta and A.A. Tsiatis},
  title =    {Flexible sample size considerations using information based interim monitoring},
journal =      {Drug Informational Journal},
  year =     {2001},
  OPTkey =   {},
  volume =   {35},
  number =   {},
  pages =    {1095--1112},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Mulle&Shafer01,
  author =   {H.H. Mulle and H. Shafer},
  title =    {Adaptive group sequential designs for clinical trials: combining the advantages of adaptive and classical group sequential approaches},
journal =      {Biometrics},
  year =     {2001},
  OPTkey =   {},
  volume =   {57},
  number =   {},
  pages =    {886--891},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Proschan&Hunsberger95,
  author =   {M.A. Proschan and S.A. Hunsberger},
  title =    {Designed extension studies based on conditional power},
journal =      {Biometrics},
  year =     {1995},
  OPTkey =   {},
  volume =   {51},
  number =   {},
  pages =    {1315--1324},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Shen&Fisher99,
  author =   {Y. Shen and L.D. Fisher},
  title =    {Statistical Inference for self-designing clinical trials with a one-sided hypothesis},
journal =      {Biometrics},
  year =     {1999},
  OPTkey =   {},
  volume =   {55},
  number =   {},
  pages =    {190--197},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Wittes&Brittain90,
  author =   {J. Wittes and E. Brittain},
  title =    {The role of internal pilot studies in increasing efficiency of clinical trials},
journal =      {Statistics in Medicine},
  year =     {1999},
  OPTkey =   {},
  volume =   {9},
  number =   {},
  pages =    {65--72},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Shen&Cheng06,
  author =   {Y. Shen and Y. Cheng},
  title =    {Adaptive design: Estimation and Inference with censored data in a semiparametric model},
journal =      {Biostatistics},
  year =     {2006},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {In Press},
  OPTannote =    {}
}

%next reference for adaptive allocation of treatments

@Book{Spiegelalteretal04,
  author =       {D.J. Spiegelalter and K.R. Abrams and J.P. Myles},
  title =        {Bayesian approaches to clinical trials and health care evaluation},
  publisher =    {Wiley, Chichester},
  year =         {2004}
}
@Book{Berry&Stangl96,
  author =       {D.A. Berry and D.K. Stangl},
  title =        {Bayesian biostatistics},
  publisher =    {Marcel Dekker, New York},
  year =         {1996}
}


@Article{Berry06,
  author =   {D.A. Berry},
  title =    {Bayesian clinical trials},
journal =      {Nature Reviews, Drug Discovery},
  year =     {2006},
  OPTkey =   {},
  volume =   {5},
  number =   {},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

%D. A. Berry, Bayesian clinical trials, Nature Reviews, Drug
%Recovery, vol 5, january 2006.


@Book{Hu&Rosenberger06,
  author =       {F. Hu and W.F. Rosenberger},
  title =        {The theory of response adaptive randomization in clinical trials},
  publisher =    {New York Wiley},
  year =         {2006}
}

@Book{Dudoit&vanderLaan08,
  author =       {S. Dudoit and M.J. van der Laan},
  title =        {Resampling based multiple testing with applications to genomics},
  publisher =    {Springer Series of Statistics, New York},
  year =         {2008}
}

@Book{Sen&Singer93,
  author =       {P.K. Sen and J.M. Singer},
  title =        {Large Sample Methods in Statistics: An Introduction with Applications},
  publisher =    {Chapman \& Hall, New York},
  year =         {1993}
}


@Article{Bai&Hu&Rosenberger02,
  author =   {Z.D. Bai and F. Hu and W.F. Rosenberger},
  title =    {Asymptotic properties of adaptive designs for clinical trials with delayed response},
journal =      {Annals of Statistics},
  year =     {2002},
  OPTkey =   {},
  volume =   {30},
  number =   {1},
  pages =    {122--139},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Andersen&Faries&Tamura94,
  author =   {J. Andersen and D. Faries and R. Tamura},
  title =    {A randomized play-the-winner design for multiarm clinical trials},
journal =      {Communication in Statistical Theory},
  year =     {1994},
  OPTkey =   {},
  volume =   {23},
  number =   {},
  pages =    {309--323},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Flournoy&Rosenberger95,
  author =       {N. Flournoy and W.F. Rosenberger},
  title =        {Adaptive Designs},
  publisher =    {Hayward, Institute of Mathematical Statistics},
  year =         {1995}
}

@Article{Hu&Rosenberger00,
  author =   {F. Hu and W.F. Rosenberger},
  title =    {Analysis of time trends in adaptive designs withi appliation to a neurophysiology experiment},
journal =      {Statistics in Medicine},
  year =     {2000},
  OPTkey =   {},
  volume =   {19},
  number =   {},
  pages =    {2067--2075},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Rosenberger96,
  author =   {W.F. Rosenberger},
  title =    {New directions in adaptive designs},
journal =      {Statistical Science},
  year =     {1996},
  OPTkey =   {},
  volume =   {11},
  number =   {},
  pages =    {137--149},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Rosenberger&Flournoy&Durham97,
  author =   {W.F. Rosenberger and N. Flournoy and S.D. Durham},
  title =    {Asymptotic normality of maximum likelihood estimators
  from multiparameter response driven designs},
journal =      {Journal of Statistical Planning and Inference},
  year =     {1997},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {69--76},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Rosenberger&Grill97,
  author =   {W.F. Rosenberger and S.E. Grill},
  title =    {A sequential design for psychophysical experiments: An application to estimating timing of sensory events},
journal =      {Statistics in Medicine},
  year =     {1997},
  OPTkey =   {},
  volume =   {16},
  number =   {},
  pages =    {2245--2260},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Rosenberger&Sriram97,
  author =   {W.F. Rosenberger and T.N. Shiram},
  title =    {Estimation for an adaptive allocation design},
journal =      {Journal of Statistical Planning and Inference},
  year =     {1997},
  OPTkey =   {},
  volume =   {59},
  number =   {},
  pages =    {309--319},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Tamura&Faries&Andersen&Heiligenstein94,
  author =   {R.N. Tamura and D.E. Faries and J.S. Andersen and J.H. Heiligenstein},
  title =    {A case study of an adaptive clinical trial in the treatment of out-patients with depressive disorder},
journal =      {Journal of the American Statistical Association},
  year =     {1994},
  OPTkey =   {},
  volume =   {89},
  number =   {},
  pages =    {768--776},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Wei&Durham78,
  author =   {L.J. Wei and S. Durham},
  title =    {The randomize play-the-winner rule in medical trials},
journal =      {Journal of the American Statistical Association},
  year =     {1978},
  OPTkey =   {},
  volume =   {73},
  number =   {},
  pages =    {840--843},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Wei&Smythe&Lin&Park90,
  author =   {L.J. Wei and R.T. Smythe and D.Y. Lin and T.S. Park},
  title =    {Statistical Inference with data-dependent treatment allocation rules},
journal =      {Journal of the American Statistical Association},
  year =     {1990},
  OPTkey =   {},
  volume =   {85},
  number =   {},
  pages =    {156--162},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Zelen69,
  author =   {M. Zelen},
  title =    {Play the winner rule and the controlled clinical trial},
journal =      {Journal of the American Statistical Association},
  year =     {1969},
  OPTkey =   {},
  volume =   {64},
  number =   {},
  pages =    {131--146},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Cheng&Shen05,
  author =   {Y. Cheng and Y. Shen},
  title =    {Bayesian adaptive designs for clinical trials},
journal =      {Biometrika},
  year =     {2005},
  OPTkey =   {},
  volume =   {92},
  number =   {3},
  pages =    {633--646},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Wei79,
  author =   {L.J. Wei},
  title =    {The generalized Polya's urn design for sequential medical trials},
journal =      {Annals of Statistics},
  year =     {1979},
  OPTkey =   {},
  volume =   {7},
  number =   {},
  pages =    {291--296},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}








@article{
Benito03,
   Author = {Benito, J. M. and Lopez, M. and Soriano, V.},
   Title = {Virus load and cytolitic responses in human immunodeficiency virus infection: what is cause and what is effect},
   Journal = {J Infect Dis},
   Volume = {188},
   Number = {5},
   Pages = {794-5; author reply 795-6},
   Note = {0022-1899
Comment
Letter},
 Keywords = {ADP-ribosyl Cyclase/metabolism
Anti-HIV Agents/therapeutic use
Antigens, CD/metabolism
CD4-Positive T-Lymphocytes/*immunology
CD8-Positive T-Lymphocytes/immunology
HIV Infections/drug therapy/*immunology/virology
HIV-1/*physiology
Human
*Viral Load
Virus Replication},
   Year = {2003} }



@article{
DEttorre02,
   Author = {D'Ettorre, G. and Forcina, G. and Andreotti, M. and Sarmati, L. and Palmisano, L. and Galluzzo, C. M. and Nicastri, E. and Mastroianni, C. M. and Vullo, V. and Vella, S. and Andreoni, M.},
   Title = {Discordant response to antiretroviral therapy: {HIV} isolation, genotypic mutations, T-cell proliferation and cytokine production},
   Journal = {Aids},
   Volume = {16},
   Number = {14},
   Pages = {1877-85},
   Note = {0269-9370
Journal Article},
   Abstract = {OBJECTIVE: To study virologic and immunologic factors associated with discordant treatment response in HIV-infected patients receiving highly active antiretroviral therapy (HAART). DESIGN: Study participants included a total of 27 patients: (a) 10 discordant patients (mean CD4+ cell count, 396.1 x 10 cells/l; mean HIV-RNA, 5.4 log copies/ml); (b) seven responder patients (mean CD4+ cell count, 997.5 x 10 cells/l); and (c) 10 failing patients (mean CD4+ cell count 66.5 x 10 cells/l; mean HIV-RNA, 5.4 log copies/ml).(10) (10)METHODS: The HIV-1 isolation rate and biological phenotype, drug resistance genotypic mutations of HIV-1 strains, recall and HIV-1-specific antigen lymphocyte proliferation (LP), and interleukin (IL)-15 production were studied. RESULTS: Virus isolation was obtained in 30% of discordant patients, and in 100% of failing patients. A higher replication constant was reported in discordant patients. No difference in the number of drug resistance mutations and biological phenotypes of HIV-1 was found in discordant patients with respect to failing patients. Discordant patients developed positive LP responses to and HIV-1 p24. LP in response to, HIV-1 p24 and gp160 was positive in responder patients. No significant LP was found in failing patients. Increased levels of IL-15 after stimulation with lipopolysaccaride (LPS) and were found in both discordant patients and responder patients. Conversely, a strong reduction of IL-15 levels was observed in failing patients. CONCLUSION: The present results suggest that decreased virus isolation rate, restoration of both lymphocyte proliferation and IL-15 production are factors involved in the discordant antiretroviral therapy response of HIV-infected patients.},
 Keywords = {Adult
Anti-HIV Agents/*therapeutic use
Antiretroviral Therapy, Highly Active
CD4 Lymphocyte Count
CD8-Positive T-Lymphocytes/drug effects/immunology
Candida albicans
Drug Resistance, Viral
Female
HIV Infections/complications/*drug therapy/immunology/virology
HIV-1/drug effects/genetics/*immunology/isolation & purification
Human
Interleukin-15/*blood
Male
Middle Aged
Mutation
Viral Load
Virus Replication/drug effects},
   Year = {2002} }



@article{
Davenport02,
   Author = {Davenport, M. P. and Zaunders, J. J. and Hazenberg, M. D. and Schuitemaker, H. and van Rij, R. P.},
   Title = {Cell turnover and cell tropism in HIV-1 infection},
   Journal = {Trends Microbiol},
   Volume = {10},
   Number = {6},
   Pages = {275-8},
   Note = {0966-842x
Journal Article},
   Abstract = {Early infection with HIV-1 is dominated by CCR5-tropic (R5, non-syncytium-inducing) viruses. The evolution of CXCR4-tropic (X4, syncytium-inducing) viruses occurs later in the infection and is associated with rapid disease progression. Here, we propose that the tropism of X4 viruses for naive CD4+ T cells is disadvantageous in early infection owing to the low division rate of these cells. In healthy individuals, the division rate of memory cells is nearly ten times higher than that of naive cells and thus the memory-cell tropism of R5 viruses could account for their dominance early in infection. As the division rate of naive T cells increases with CD4+ depletion, X4 viruses come to dominate in late disease.},
 Keywords = {CD4-Positive T-Lymphocytes/*virology
HIV Infections/*immunology/metabolism
HIV-1/*pathogenicity
Human
Immunologic Memory
Macrophages/*virology
Models, Biological
Receptors, CCR5/metabolism
Receptors, CXCR4/metabolism
Tropism},
   Year = {2002} }



@article{
Deeks00,
   Author = {Deeks, S. G. and Barbour, J. D. and Martin, J. N. and Swanson, M. S. and Grant, R. M.},
   Title = {Sustained CD4+ T cell response after virologic failure of protease inhibitor-based regimens in patients with human immunodeficiency virus infection},
   Journal = {J Infect Dis},
   Volume = {181},
   Number = {3},
   Pages = {946-53},
   Note = {0022-1899
Journal Article},
   Abstract = {The relationship between plasma human immunodeficiency virus (HIV) RNA levels and peripheral CD4+ T cell counts was examined in 380 HIV-infected adults receiving long-term protease inhibitor therapy. Patients experiencing virologic failure (persistent HIV RNA >500 copies RNA/mL) generally had CD4+ T cell counts that remained greater than pretherapy baseline levels, at least through 96 weeks of follow-up. The CD4+ T cell response was directly and independently related to degree of viral suppression below the pretreatment baseline. For any given HIV RNA level measured 12 weeks after virologic failure, subsequent CD4+ T cell decline was slower in patients receiving a protease inhibitor-based regimen than in a historical control group of untreated patients. These observations suggest that transient or partial declines in plasma HIV RNA levels can have sustained effects on CD4+ T cell levels.},
 Keywords = {Adult
*CD4 Lymphocyte Count
Female
HIV Infections/*drug therapy/immunology/virology
HIV Protease Inhibitors/*therapeutic use
Human
Male
RNA, Viral/*blood
Support, Non-U.S. Gov't
Support, U.S. Gov't, P.H.S.},
   Year = {2000} }



@article{
Deeks01,
   Author = {Deeks, S. G. and Wrin, T. and Liegler, T. and Hoh, R. and Hayden, M. and Barbour, J. D. and Hellmann, N. S. and Petropoulos, C. J. and McCune, J. M. and Hellerstein, M. K. and Grant, R. M.},
   Title = {Virologic and immunologic consequences of discontinuing combination antiretroviral-drug therapy in HIV-infected patients with detectable viremia},
   Journal = {N Engl J Med},
   Volume = {344},
   Number = {7},
   Pages = {472-80},
   Note = {0028-4793
Clinical Trial
Journal Article
Randomized Controlled Trial},
   Abstract = {BACKGROUND: In many patients with human immunodeficiency virus (HIV) infection, therapy with potent antiretroviral drugs does not result in complete suppression of HIV replication. The effect of cessation of therapy in these patients is unknown. METHODS: Sixteen patients who had a plasma HIV RNA level of more than 2500 copies per milliliter during combination antiretroviral-drug therapy were randomly assigned, in a 2:1 ratio, to discontinue or continue therapy. Plasma HIV RNA levels, CD4 cell counts, and drug susceptibility were measured weekly. Viral replicative capacity was measured at base line and at week 12. RESULTS: Discontinuation of therapy for 12 weeks was associated with a median decrease in the CD4 cell count of 128 cells per cubic millimeter and an increase in the plasma HIV RNA level of 0.84 log copies per milliliter. Virus from all patients with detectable resistance at entry became susceptible to HIV-protease inhibitors within 16 weeks after the discontinuation of therapy. Drug susceptibility began to increase a median of six weeks after the discontinuation of therapy and was temporally associated with increases in plasma HIV RNA levels and decreases in CD4 cell counts. Viral replicative capacity, measured by means of a recombinant-virus assay, was low at entry into the study and increased after therapy was discontinued. Despite the loss of detectable resistance in plasma, resistant virus was cultured from peripheral-blood mononuclear cells in five of nine patients who could be evaluated. Plasma HIV RNA levels, CD4 cell counts, and drug susceptibility remained stable in the patients who continued therapy. CONCLUSIONS: Despite the presence of reduced drug susceptibility, antiretroviral-drug therapy can provide immunologic and virologic benefit. This benefit reflects continued antiviral-drug activity and the maintenance of a viral population with a reduced replicative capacity.},
 Keywords = {Adult
Anti-HIV Agents/pharmacology/*therapeutic use
CD4 Lymphocyte Count
Drug Resistance, Microbial
Drug Therapy, Combination
HIV Infections/*drug therapy/immunology/virology
HIV Protease Inhibitors/pharmacology/*therapeutic use
HIV-1/*drug effects/genetics/isolation & purification
Human
Male
Middle Aged
Proportional Hazards Models
Prospective Studies
RNA, Viral/blood
Support, Non-U.S. Gov't
Support, U.S. Gov't, P.H.S.
Viremia/drug therapy},
   Year = {2001} }



@article{
Deeks01b,
   Author = {Deeks, S. G.},
   Title = {International perspectives on antiretroviral resistance. Nonnucleoside reverse transcriptase inhibitor resistance},
   Journal = {J Acquir Immune Defic Syndr},
   Volume = {26 Suppl 1},
   Pages = {S25-33},
   Note = {1525-4135
Journal Article
Review
Review, Tutorial},
   Abstract = {Although understanding of nonnucleoside reverse transcriptase inhibitor (NNRTI) resistance is less clearly established than that of other classes of antiretroviral drugs, certain facts have been established. The treatment-associated genetic mutation profiles of the available NNRTIs have been mapped, and resistance has been found to develop rapidly after initiation of NNRTI therapy. Despite the chemical diversity of the NNRTIs, cross-resistance among agents of this class is nearly universal. Although the viral replicative capacity (``fitness") of NNRTI-induced viral variants has not been extensively studied, available data suggest that NNRTI-selected mutations confer little damage to viral fitness, and thus a single point mutation produces a strain that is both resistant and fit. Furthermore, with continued therapy, viral evolution persists, creating species with greater numbers of mutations and higher level phenotypic resistance. Taken together, these facts suggest that continued use of NNRTIs after emergence of resistance will produce variants of complex mutational patterns that limit future treatment options, and, therefore, strong consideration should be given to discontinuing NNRTIs after virologic failure is confirmed. This article describes the scientific literature establishing the efficacy and limitations of NNRTI therapy and attempts to define a role for this class of drug in the long-term treatment of HIV-1 disease.},
 Keywords = {Anti-HIV Agents/*pharmacology/therapeutic use
Clinical Trials
Delavirdine/pharmacology/therapeutic use
*Drug Resistance, Microbial
Drug Therapy, Combination
HIV Infections/drug therapy/transmission
HIV-1/*drug effects/genetics/metabolism
HIV-1 Reverse Transcriptase/chemistry/genetics
Human
Nevirapine/pharmacology/therapeutic use
Oxazines/pharmacology/therapeutic use
Phylogeny
Point Mutation/drug effects
Protein Conformation
Reverse Transcriptase Inhibitors/*pharmacology/therapeutic use
Virus Replication/drug effects},
   Year = {2001} }



@article{
Deeks02,
   Author = {Deeks, S. G. and Barbour, J. D. and Grant, R. M. and Martin, J. N.},
   Title = {Duration and predictors of CD4 T-cell gains in patients who continue combination therapy despite detectable plasma viremia},
   Journal = {Aids},
   Volume = {16},
   Number = {2},
   Pages = {201-7},
   Note = {0269-9370
Journal Article},
   Abstract = {BACKGROUND: Sustained elevations in CD4 cell counts commonly occur despite incomplete viral suppression with protease inhibitor-based antiretroviral therapy. OBJECTIVES: To determine the incidence and risk factors associated with return of CD4 cell count to pre-therapy levels in patients experiencing virologic failure of protease inhibitor therapy. DESIGN: This is a clinic-based cohort study of HIV-infected adults who failed to maintain durable viral suppression on a protease inhibitor-based regimen. MAIN OUTCOME MEASURES: Virologic failure was defined as persistent plasma HIV RNA level > 500 copies/ml. Immunologic failure was defined as return of CD4 cell count to pre-therapy levels. RESULTS: A total of 291 patients experienced virologic failure on a protease inhibitor-based regimen and had a treatment-mediated CD4 cell increase above pre-therapy levels at the time of virologic failure. If patient data were censored at the time a successful salvage regimen was initiated, then the median time to immunologic failure after the onset of virologic failure was 3 years. If patient data were also censored at the time therapy was discontinued, then 36.8% of the cohort experienced immunologic failure after 3 years of continuous virologic failure. The change in viral load from a pre-treatment baseline, and not the absolute level of viremia achieved, was a strong and independent predictor of immunologic failure. Discontinuing therapy was associated with immunologic failure independent of viral load changes. CONCLUSION: Reduction in T CD4+ cell numbers may eventually occur during prolonged virologic failure of a protease inhibitor-based regimen and is predicted by the degree of virologic suppression below a pre-therapy 'set-point'.},
 Keywords = {Adult
Antiretroviral Therapy, Highly Active
CD4 Lymphocyte Count
CD4-Positive T-Lymphocytes/cytology/*drug effects
Disease Progression
HIV Infections/blood/*drug therapy/immunology/virology
HIV Protease Inhibitors/*therapeutic use
HIV-1/*drug effects/genetics
Human
Indinavir/therapeutic use
Nelfinavir/therapeutic use
RNA, Viral/blood
Ritonavir/therapeutic use
Saquinavir/therapeutic use
Support, Non-U.S. Gov't
Support, U.S. Gov't, P.H.S.
Time Factors
Treatment Failure
Viremia/blood/*drug therapy/immunology/virology},
   Year = {2002} }



@article{
Deeks03,
   Author = {Deeks, S. G.},
   Title = {Treatment of antiretroviral-drug-resistant HIV-1 infection},
   Journal = {Lancet},
   Volume = {362},
   Number = {9400},
   Pages = {2002-11},
   Note = {1474-547x
Journal Article
Review
Review, Academic},
   Abstract = {Drug-resistant HIV-1 is a cause of growing clinical and public-health concern. In many patients, combination antiretroviral therapy fails to achieve complete viral suppression (virological failure). Continuing viral replication during therapy leads to the accumulation of drug-resistance mutations, resulting in increased viral load and a greater risk of disease progression. Patients with drug-resistant HIV-1 infection have three therapeutic options: a change to a salvage regimen with the aim of fully suppressing viral replication; interruption of therapy; or continuation of a partially effective regimen. The first strategy is preferred for most patients failing their first or perhaps their second regimen. However, the best approach remains unclear for patients who have failed multiple treatment regimens and who have limited options for complete viral suppression. The management of such patients requires a careful understanding of the pathogenesis of drug-resistant HIV-1, the clinical consequences of virological failure, the potential benefits and limitations of diagnostic assays, and the likelihood that agents in development will be effective.},
 Keywords = {Anti-HIV Agents/*immunology/*therapeutic use
Antiretroviral Therapy, Highly Active/methods
Drug Resistance, Viral/genetics/immunology
Drug Therapy, Combination
HIV Infections/*drug therapy/immunology/virology
HIV Protease Inhibitors/immunology/therapeutic use
*HIV-1/drug effects/genetics/immunology
Human
Randomized Controlled Trials
Ritonavir/immunology/therapeutic use
Support, Non-U.S. Gov't
Support, U.S. Gov't, P.H.S.
Treatment Outcome
Viral Load/statistics & numerical data
Virus Replication/drug effects/immunology},
   Year = {2003} }



@article{Deeks04,
   Author = {Deeks, S. G. and Walker, B. D.},
   Title = {The immune response to AIDS virus infection: good, bad, or both?},
   Journal = {J Clin Invest},
   Volume = {113},
   Number = {6},
   Pages = {808-10},
   Note = {0021-9738
Comment
Journal Article},
   Abstract = {A potent antigen-specific T cell response to HIV infection can contribute to the control of viral replication and is therefore beneficial to the host. However, HIV-mediated increases in generalized T cell activation also appear to accelerate both viral replication and CD4+ T cell depletion. A new study in the JCI attempts to experimentally distinguish the beneficial versus harmful aspects of this immune response.},
 Year = {2004} }

@techreport{
DHHS04,
   Author = {DHHS},
   Title = {Guidelines for the use of antiretroviral agents in HIV-1 infected adults and adolescents},
   Institution = {Panel on Clinical Practices for Treatment of HIV Infection, Department of Health and Human Services},
   Month= {March 23},
 Year = {2004} }



@article{
Faure00,
   Author = {Faure, S. and Meyer, L. and Costagliola, D. and Vaneensberghe, C. and Genin, E. and Autran, B. and Delfraissy, J. F. and McDermott, D. H. and Murphy, P. M. and Debre, P. and Theodorou, I. and Combadiere, C.},
   Title = {Rapid progression to AIDS in HIV+ individuals with a structural variant of the chemokine receptor CX3CR1},
   Journal = {Science},
   Volume = {287},
   Number = {5461},
   Pages = {2274-7},
   Note = {0036-8075
Comment
Journal Article},
   Abstract = {Human immunodeficiency virus (HIV) enters cells in vitro via CD4 and a coreceptor. Which of 15 known coreceptors are important in vivo is poorly defined but may be inferred from disease-modifying mutations, as for CCR5. Here two single nucleotide polymorphisms are described in Caucasians in CX3CR1, an HIV coreceptor and leukocyte chemotactic/adhesion receptor for the chemokine fractalkine. HIV-infected patients homozygous for CX3CR1-I249 M280, a variant haplotype affecting two amino acids (isoleucine-249 and methionine-280), progressed to AIDS more rapidly than those with other haplotypes. Functional CX3CR1 analysis showed that fractalkine binding is reduced among patients homozygous for this particular haplotype. Thus, CX3CR1-I249 M280 is a recessive genetic risk factor in HIV/AIDS.},
 Keywords = {Acquired Immunodeficiency Syndrome/genetics/*physiopathology/virology
Case-Control Studies
*Chemokines, CX3C
Chemokines, CXC/metabolism
Chromosomes, Human, Pair 3
Cohort Studies
Disease Progression
European Continental Ancestry Group/genetics
Genotype
HIV/physiology
HIV Infections/genetics/*physiopathology/virology
Haplotypes
Homozygote
Human
Leukocytes, Mononuclear/metabolism
Linkage Disequilibrium
Membrane Proteins/metabolism
Mutation
Polymorphism, Restriction Fragment Length
*Polymorphism, Single Nucleotide
Polymorphism, Single-Stranded Conformational
Receptors, Cytokine/*genetics/*physiology
Receptors, HIV/*genetics/*physiology
Support, Non-U.S. Gov't
Survival Analysis
Variation (Genetics)},
   Year = {2000} }



@article{
Gao01,
   Author = {Gao, X. and Nelson, G. W. and Karacki, P. and Martin, M. P. and Phair, J. and Kaslow, R. and Goedert, J. J. and Buchbinder, S. and Hoots, K. and Vlahov, D. and O'Brien, S. J. and Carrington, M.},
   Title = {Effect of a single amino acid change in MHC class I molecules on the rate of progression to AIDS},
   Journal = {N Engl J Med},
   Volume = {344},
   Number = {22},
   Pages = {1668-75},
   Note = {0028-4793
Journal Article
Multicenter Study},
   Abstract = {BACKGROUND: From studies of genetic polymorphisms and the rate of progression from human immunodeficiency virus type 1 (HIV-1) infection to the acquired immunodeficiency syndrome (AIDS), it appears that the strongest susceptibility is conferred by the major-histocompatibility-complex (MHC) class I type HLA-B*35,Cw*04 allele. However, cytotoxic T-lymphocyte responses have been observed against HIV-1 epitopes presented by HLA-B*3501, the most common HLA-B*35 subtype. We examined subtypes of HLA-B*35 in five cohorts and analyzed the relation of structural differences between HLA-B*35 subtypes to the risk of progression to AIDS. METHODS: Genotyping of HLA class I loci was performed for 850 patients who seroconverted and had known dates of HIV-1 infection. Survival analyses with respect to the rate of progression to AIDS were performed to identify the effects of closely related HLA-B*35 subtypes with different peptide-binding specificities. RESULTS: HLA-B*35 subtypes were divided into two groups according to peptide-binding specificity: the HLA-B*35-PY group, which consists primarily of HLA-B*3501 and binds epitopes with proline in position 2 and tyrosine in position 9; and the more broadly reactive HLA-B*35-Px group, which also binds epitopes with proline in position 2 but can bind several different amino acids (not including tyrosine) in position 9. The influence of HLA-B*35 in accelerating progression to AIDS was completely attributable to HLA-B*35-Px alleles, some of which differ from HLA-B*35-PY alleles by only one amino acid residue. CONCLUSIONS: This analysis shows that, in patients with HIV-1 infection, a single amino acid change in HLA molecules has a substantial effect on the rate of progression to AIDS. The different consequences of HLA-B*35-PY and HLA-B*35-Px in terms of disease progression highlight the importance of the epitope specificities of closely related class I molecules in the immune defense against HIV-1.},
 Keywords = {Acquired Immunodeficiency Syndrome/*genetics
African Continental Ancestry Group/genetics
Alleles
Amino Acid Sequence
Binding Sites/genetics
Disease Progression
Disease-Free Survival
European Continental Ancestry Group/genetics
*Genes, MHC Class I
Genotype
HIV Infections/ethnology/*genetics/immunology
HLA-B35 Antigen/chemistry/*genetics
HLA-C Antigens
Human
Peptides/metabolism
Proportional Hazards Models
Receptors, Peptide/chemistry/genetics/metabolism
Support, U.S. Gov't, P.H.S.},
   Year = {2001} }



@article{
Grabar00,
   Author = {Grabar, S. and Le Moing, V. and Goujard, C. and Leport, C. and Kazatchkine, M. D. and Costagliola, D. and Weiss, L.},
   Title = {Clinical outcome of patients with HIV-1 infection according to immunologic and virologic response after 6 months of highly active antiretroviral therapy},
   Journal = {Ann Intern Med},
   Volume = {133},
   Number = {6},
   Pages = {401-10},
   Note = {0003-4819
Journal Article
Multicenter Study},
   Abstract = {BACKGROUND: The prognostic value of discordant immunologic (CD4 cell increase) and virologic (plasma HIV RNA level decrease) responses to antiretroviral treatment is not known. OBJECTIVE: To study the relation between clinical outcome of HIV-infected patients receiving highly active antiretroviral therapy (HAART) and early immunologic and virologic responses to such therapy. DESIGN: Prospective cohort study. SETTING: 68 hospitals in France. PATIENTS: 2236 protease inhibitor-naive patients. INTERVENTION: Initiation of HAART with one protease inhibitor and two nucleoside analogues between July 1996 and March 1997. MEASUREMENTS: Immunologic and virologic response at 6 months. Multivariate Cox models were used to assess the relation between these responses and progression to a new AIDS-defining event or death. RESULTS: On the basis of 6-month immunologic and virologic responses, patients were classified into four groups: complete response (47.5%), complete nonresponse (16.2%), immunologic response only (19.0%), and virologic response only (17.3%). After month 6 and within a median of 18 months, 69 patients died and 123 experienced a new AIDS-defining event. After adjustment, complete nonresponders and those with only a virologic response had significantly higher risks for clinical progression at 6 months (relative risk, 3.38 [95% CI, 2.28 to 5.02] and 1.98 [CI, 1.26 to 3.10], respectively) than complete responders. The difference between complete responders and those with only an immunologic response at 6 months was weaker and nonsignificant (relative risk, 1.55 [CI, 0.96 to 2.50]). CONCLUSIONS: Immunologic response after 6 months of HAART indicates a favorable clinical outcome in HIV-infected patients regardless of virologic response. This suggests that both immunologic and virologic markers should be used in clinical practice to evaluate treatment response.},
 Keywords = {Adult
CD4 Lymphocyte Count
Disease Progression
Drug Therapy, Combination
Female
HIV Infections/*drug therapy/immunology/virology
HIV Protease Inhibitors/*therapeutic use
*HIV-1/genetics
Human
Male
Multivariate Analysis
Proportional Hazards Models
Prospective Studies
RNA, Viral/blood
Reverse Transcriptase Inhibitors/*therapeutic use
Support, Non-U.S. Gov't
Treatment Outcome
Viral Load},
   Year = {2000} }



@article{
Grueb00,
   Author = {Greub, G. and Ledergerber, B. and Battegay, M. and Grob, P. and Perrin, L. and Furrer, H. and Burgisser, P. and Erb, P. and Boggian, K. and Piffaretti, J. C. and Hirschel, B. and Janin, P. and Francioli, P. and Flepp, M. and Telenti, A.},
   Title = {Clinical progression, survival, and immune recovery during antiretroviral therapy in patients with HIV-1 and hepatitis C virus coinfection: the Swiss HIV Cohort Study},
   Journal = {Lancet},
   Volume = {356},
   Number = {9244},
   Pages = {1800-5},
   Note = {0140-6736
Clinical Trial
Journal Article},
   Abstract = {BACKGROUND: Hepatitis C virus (HCV) infection is highly prevalent among HIV-1-infected individuals, but its contribution to the morbidity and mortality of coinfected patients who receive potent antiretroviral therapy is controversial. We used data from the ongoing Swiss HIV Cohort Study to analyse clinical progression of HIV-1, and the virological and immunological response to potent antiretroviral therapy in HIV-1-infected patients with or without concurrent HCV infection. METHODS: We analysed prospective data on survival, clinical disease progression, suppression of HIV-1 replication, CD4-cell recovery, and frequency of changes in antiretroviral therapy according to HCV status in 3111 patients starting potent antiretroviral therapy. RESULTS: 1157 patients (37.2%) were coinfected with HCV, 1015 of whom (87.7%) had a history of intravenous drug use. In multivariate Cox's regression, the probability of progression to a new AIDS-defining clinical event or to death was independently associated with HCV seropositivity (hazard ratio 1.7 [95% CI 1.26-2.30]), and with active intravenous drug use (1.38 [1.02-1.88]). Virological response to antiretroviral therapy and the probability of treatment change were not associated with HCV serostatus. In contrast, HCV seropositivity was associated with a smaller CD4-cell recovery (hazard ratio for a CD4-cell count increase of at least 50 cells/microL=0.79 [0.72-0.87]). INTERPRETATION: HCV and active intravenous drug use could be important factors in the morbidity and mortality among HIV-1-infected patients, possibly through impaired CD4-cell recovery in HCV seropositive patients receiving potent antiretroviral therapy. These findings are relevant for decisions about optimum timing for HCV treatment in the setting of HIV infection.},
 Keywords = {AIDS-Related Opportunistic Infections/*drug therapy
Adolescent
Adult
Anti-HIV Agents/*therapeutic use
CD4 Lymphocyte Count
Cohort Studies
Disease Progression
Female
Hepatitis C/complications/*drug therapy
Human
Male
Middle Aged
Prospective Studies
Support, Non-U.S. Gov't
Survival Analysis
Switzerland
Viral Load
Viremia/etiology},
   Year = {2000} }



@article{
Katzenstein96,
   Author = {Katzenstein, D. A. and Hammer, S. M. and Hughes, M. D. and Gundacker, H. and Jackson, J. B. and Fiscus, S. and Rasheed, S. and Elbeik, T. and Reichman, R. and Japour, A. and Merigan, T. C. and Hirsch, M. S.},
   Title = {The relation of virologic and immunologic markers to clinical outcomes after nucleoside therapy in HIV-infected adults with 200 to 500 CD4 cells per cubic millimeter. AIDS Clinical Trials Group Study 175 Virology Study Team},
   Journal = {N Engl J Med},
   Volume = {335},
   Number = {15},
   Pages = {1091-8},
   Note = {0028-4793
Clinical Trial
Journal Article
Multicenter Study
Randomized Controlled Trial},
   Abstract = {BACKGROUND: We studied measures of human immunodeficiency virus (HIV) replication, the viral phenotype, and immune function (CD4 cell counts) and the relation of changes in these indicators to clinical outcomes in a subgroup of patients in a controlled trial of early antiretroviral treatment for HIV, the AIDS Clinical Trials Group Study 175. METHODS: The 391 subjects, each of whom entered the study with a single screening CD4 cell count of 200 to 500 per cubic millimeter, were randomly assigned to receive zidovudine alone, didanosine alone, zidovudine plus didanosine, or zidovudine plus zalcitabine. Plasma concentrations of HIV RNA were assessed in 366 subjects, and viral isolates from 332 subjects were assayed for the presence of the syncytium-inducing phenotype. RESULTS: After eight weeks, the mean (+/-SE) decrease from base line in the concentration of HIV RNA, expressed as the change in the base 10 log of the number of copies per milliliter, was 0.26+/-0.06 for patients treated with zidovudine alone, 0.65+/-0.07 for didanosine alone, 0.93+/-0.10 for zidovudine plus didanosine, and 0.89+/-0.06 for zidovudine plus zalcitabine (P<0.001 for each of the pairwise comparisons with zidovudine alone). Multivariate proportional-hazards models showed that higher base-line concentrations of plasma HIV RNA, less suppression of plasma HIV RNA by treatment, and the presence of the syncytium-inducing phenotype were significantly associated with an increased risk of progression to the acquired immunodeficiency syndrome and death. After adjustment for these measures of viral replication and for the viral phenotype, CD4 cell counts were not significant predictors of clinical outcome. CONCLUSIONS: Both the risk of the progression of HIV disease and the efficacy of antiretroviral therapy are strongly associated with the plasma level of HIV RNA and with the viral phenotype. The changes in the plasma concentration of HIV RNA predict the changes in CD4 cell counts and survival after treatment with reverse-transcriptase inhibitors.},
 Keywords = {Adult
Antiviral Agents/*therapeutic use
CD4 Lymphocyte Count
Didanosine/*therapeutic use
Disease Progression
Drug Therapy, Combination
Female
HIV/*genetics/isolation & purification/physiology
HIV Infections/drug therapy/immunology/*virology
Human
Male
Middle Aged
Multivariate Analysis
Phenotype
Proportional Hazards Models
RNA, Viral/*blood
Support, U.S. Gov't, P.H.S.
Treatment Outcome
Virus Replication/drug effects
Zidovudine/*therapeutic use},
   Year = {1996} }



@article{
Kaufmann98,
   Author = {Kaufmann, D. and Pantaleo, G. and Sudre, P. and Telenti, A.},
   Title = {CD4-cell count in HIV-1-infected individuals remaining viraemic with highly active antiretroviral therapy (HAART). Swiss HIV Cohort Study},
   Journal = {Lancet},
   Volume = {351},
   Number = {9104},
   Pages = {723-4},
   Note = {0140-6736
Letter},
 Keywords = {Anti-HIV Agents/*therapeutic use
CD4 Lymphocyte Count
HIV Infections/drug therapy/*immunology
Human
Protease Inhibitors/*therapeutic use
Support, Non-U.S. Gov't
Viremia/drug therapy/*immunology},
   Year = {1998} }



@article{
Kaufmann03,
   Author = {Kaufmann, G. R. and Perrin, L. and Pantaleo, G. and Opravil, M. and Furrer, H. and Telenti, A. and Hirschel, B. and Ledergerber, B. and Vernazza, P. and Bernasconi, E. and Rickenbach, M. and Egger, M. and Battegay, M.},
   Title = {CD4 T-lymphocyte recovery in individuals with advanced HIV-1 infection receiving potent antiretroviral therapy for 4 years: the Swiss HIV Cohort Study},
   Journal = {Arch Intern Med},
   Volume = {163},
   Number = {18},
   Pages = {2187-95},
   Note = {0003-9926
Journal Article},
   Abstract = {BACKGROUND: Highly active antiretroviral therapy (HAART) for human immunodeficiency virus (HIV)-1 infection allows recovery of CD4 T lymphocytes. Few studies have explored the long-term T-lymphocyte responses to HAART. METHODS: Plasma HIV-1 RNA levels and CD4 and CD8 T-lymphocyte counts were longitudinally analyzed over 4 years in 2235 participants of the Swiss HIV Cohort, commencing HAART between 1996 and 1997. The CD4 T-lymphocyte count increase, the percentage of individuals with a CD4 T-lymphocyte count of 500/microL or greater and less than 200/microL, and the determinants of CD4 T-lymphocyte recovery were evaluated in individuals treated with continuous (CONT; n = 985) and discontinuous (DISCONT; n = 1250) HAART. RESULTS: At 4 years, 69.5% of subjects (CONT, 84.5%; DISCONT, 53.6%; P<.001) showed HIV-1 RNA levels below 400 copies/mL, while the median CD4 T-lymphocyte count increased from 190/microL to 423/microL (CONT, 486/microL; DISCONT, 343/microL; P<.001). Of the 2235 participants, 38.8% (CONT, 47.7%; DISCONT, 29.4%; P<.001) reached a CD4 T-lymphocyte count of 500/microL or greater, but in 15.6%, CD4 T-lymphocyte count remained below 200/microL (CONT, 5.9%; DISCONT, 25.9%; P<.001). Larger increases in CD4 T-lymphocyte count were associated with higher baseline HIV-1 RNA, a larger percentage of undetectable HIV-1 RNA levels, lower baseline CD8 T-lymphocyte count, and younger age. Individuals reaching a CD4 T-lymphocyte count of 500/microL or greater at 4 years were characterized by higher nadir and baseline CD4 T-lymphocyte counts and a more sustained reduction of HIV-1 RNA levels. CONCLUSIONS: At 4 years, only 39% of individuals treated with HAART reached a CD4 T-lymphocyte count of 500/microL or greater, and 16% with CD4 T-lymphocyte counts less than 200/microL remained susceptible to opportunistic infections. Treatment interruptions, a poor virologic response, and older age were the major factors negatively affecting the recovery of CD4 T lymphocytes.},
 Keywords = {Adult
*Antiretroviral Therapy, Highly Active
*CD4 Lymphocyte Count
CD8-Positive T-Lymphocytes
Female
HIV Infections/*drug therapy/*immunology
*Hiv-1
Human
Lymphocyte Count
Male
Middle Aged
Prospective Studies
RNA, Viral/*analysis
Support, Non-U.S. Gov't
Viral Load},
   Year = {2003} }



@article{
MartinezPicado99,
   Author = {Martinez-Picado, J. and Savara, A. V. and Sutton, L. and D'Aquila, R. T.},
   Title = {Replicative fitness of protease inhibitor-resistant mutants of human immunodeficiency virus type 1},
   Journal = {J Virol},
   Volume = {73},
   Number = {5},
   Pages = {3744-52},
   Note = {0022-538x
Journal Article},
   Abstract = {The relative replicative fitness of human immunodeficiency virus type 1 (HIV-1) mutants selected by different protease inhibitors (PIs) in vivo was determined. Each mutant was compared to wild type (WT), NL4-3, in the absence of drugs by several methods, including clonal genotyping of cultures infected with two competing viral variants, kinetics of viral antigen production, and viral infectivity/virion particle ratios. A nelfinavir-selected protease D30N substitution substantially decreased replicative capacity relative to WT, while a saquinavir-selected L90M substitution moderately decreased fitness. The D30N mutant virus was also outcompeted by the L90M mutant in the absence of drugs. A major natural polymorphism of the HIV-1 protease, L63P, compensated well for the impairment of fitness caused by L90M but only slightly improved the fitness of D30N. Multiply substituted indinavir-selected mutants M46I/L63P/V82T/I84V and L10R/M46I/L63P/V82T/I84V were just as fit as WT. These results indicate that the mutations which are usually initially selected by nelfinavir and saquinavir, D30N and L90M, respectively, impair fitness. However, additional mutations may improve the replicative capacity of these and other drug-resistant mutants. Hypotheses based on the greater fitness impairment of the nelfinavir-selected D30N mutant are suggested to explain observations that prolonged responses to delayed salvage regimens, including alternate PIs, may be relatively common after nelfinavir failure.},
 Keywords = {Adaptation, Biological
Amino Acid Substitution
Animals
Anti-HIV Agents/*pharmacology
Cells, Cultured
Drug Resistance, Microbial
HIV Protease Inhibitors/*pharmacology
HIV-1/*drug effects/genetics/physiology
Human
Mice
Mutagenesis, Site-Directed
Nelfinavir/*pharmacology
Saquinavir/*pharmacology
Support, Non-U.S. Gov't
Support, U.S. Gov't, P.H.S.
Tumor Cells, Cultured
Virus Replication/*drug effects},
   Year = {1999} }



@article{
Mellors96,
   Author = {Mellors, J. W. and Rinaldo, C. R., Jr. and Gupta, P. and White, R. M. and Todd, J. A. and Kingsley, L. A.},
   Title = {Prognosis in HIV-1 infection predicted by the quantity of virus in plasma},
   Journal = {Science},
   Volume = {272},
   Number = {5265},
   Pages = {1167-70},
   Note = {0036-8075
Comment
Journal Article},
   Abstract = {The relation between viremia and clinical outcome in individuals infected with human immunodeficiency virus-type 1 (HIV-1) has important implications for therapeutic research and clinical care. HIV-1 RNA in plasma was quantified with a branched-DNA signal amplification assay as a measure of viral load in a cohort of 180 seropositive men studied for more than 10 years. The risk of acquired immunodeficiency syndrome (AIDS) and death in study subjects, including those with normal numbers of CD4+ T cells, was directly related to plasma viral load at study entry. Plasma viral load was a better predictor of progression to AIDS and death than was the number of CD4+ T cells.},
 Keywords = {Acquired Immunodeficiency Syndrome/*virology
Antiviral Agents/therapeutic use
Biological Markers/blood
CD4 Lymphocyte Count
CD4-Positive T-Lymphocytes/virology
Cohort Studies
Disease Progression
Follow-Up Studies
HIV Infections/drug therapy/mortality/*virology
HIV-1/genetics/*physiology
Human
Male
Prognosis
Proportional Hazards Models
RNA, Viral/*blood
Support, Non-U.S. Gov't
Support, U.S. Gov't, Non-P.H.S.
Support, U.S. Gov't, P.H.S.
Survival Rate
Time Factors
Viremia/*virology
Virus Replication},
   Year = {1996} }



@article{
Miller00,
   Author = {Miller, V. and Sabin, C. A. and Phillips, A. N. and Rottmann, C. and Rabenau, H. and Weidmann, E. and Rickerts, V. and Findhammer, S. and Helm, E. B. and Staszewski, S.},
   Title = {The impact of protease inhibitor-containing highly active antiretroviral therapy on progression of HIV disease and its relationship to CD4 and viral load},
   Journal = {Aids},
   Volume = {14},
   Number = {14},
   Pages = {2129-36},
   Note = {0269-9370
Clinical Trial
Journal Article},
   Abstract = {OBJECTIVE: To compare the rate of disease progression according to viral load and CD4 cell count in patients receiving or not receiving highly active antiretroviral therapy (HAART), defined as protease inhibitor-containing regimens. DESIGN: An observational study, with prospectively collected data. METHODS: All patients attending the HIV Outpatient clinic as of 1 January 1995 (n = 2083) were included. Follow-up was until the first AIDS-defining event or death. Associations between viral load or CD4 cell count and disease progression were assessed using a person-years approach. Event rates were compared using Poisson regression analysis; a multivariate model was used to assess the independent effects of CD4, viral load and treatment group on event rates and to consider interactions between these variables. RESULTS: The event rates increased with lower CD4 cell count and higher viral load for both treatment groups and were generally lower in the HAART group. In a multivariate analysis, lower CD4 cell counts and higher viral loads remained significantly associated with disease progression, irrespective of treatment group. However, the event rate was significantly lower for the HAART group compared with the control group (relative rate 0.53, P < 0.001). CONCLUSIONS: HAART-treated patients with high viral loads and CD4 cell counts experienced reduced disease progression compared with individuals with the same CD4 cell count and viral load not receiving HAART. Consequently, the short-term prognosis associated with viral load levels and CD4 cell counts may differ in patients on HAART. Whether this effect will be observed with non-protease-inhibitor-containing HAART is not known at this time.},
 Keywords = {Adolescent
Adult
Aged
Antiretroviral Therapy, Highly Active
CD4 Lymphocyte Count
Disease Progression
HIV Infections/*drug therapy/pathology/virology
HIV Protease Inhibitors/*therapeutic use
*HIV-1/isolation & purification
Human
Middle Aged
Prospective Studies
RNA, Viral/analysis
Regression Analysis
Support, Non-U.S. Gov't
Viral Load},
   Year = {2000} }



@article{
Piketty98,
   Author = {Piketty, C. and Castiel, P. and Belec, L. and Batisse, D. and Si Mohamed, A. and Gilquin, J. and Gonzalez-Canali, G. and Jayle, D. and Karmochkine, M. and Weiss, L. and Aboulker, J. P. and Kazatchkine, M. D.},
   Title = {Discrepant responses to triple combination antiretroviral therapy in advanced HIV disease},
   Journal = {Aids},
   Volume = {12},
   Number = {7},
   Pages = {745-50},
   Note = {0269-9370
Journal Article},
   Abstract = {OBJECTIVES: To determine the clinical, virological and immunological outcome in a cohort of unselected patients receiving triple combination therapy for more than 1 year. METHODS: Prospective follow-up of a cohort of 162 unselected, protease inhibitor-naive, antiretroviral-experienced patients with advanced HIV disease, treated with indinavir combined with two nucleoside analogues. RESULTS: The mean CD4 cell count and plasma HIV RNA level in the study group at baseline were 69+/-5 x 10(6)/l and 4.75+/-0.07 log10 copies/ml, respectively. Five per cent of patients died prematurely or were lost to follow-up. Fifty-seven per cent of patients responded to therapy, as assessed by a sustained increase in CD4 cell counts above 50 x 10(6)/l and a decrease in plasma HIV RNA greater than 1 log10 copies/ml, throughout 12.1 months of follow-up. Seventeen per cent of patients were immunological and virological non-responders. Twenty-one per cent of patients exhibited discrepant virological and immunological responses to treatment, of whom one-half failed to exhibit significant increases in CD4 cells despite a virological response to therapy and one-half exhibited increased CD4 cell counts in the absence of significant decrease in plasma viral load. The incidence of AIDS-defining events in the latter group of patients was similar to that of responder patients, whereas their incidence was higher in patients who failed to exhibit a virological and immunological response and those who failed to increase CD4 cells despite a significant decrease in viral load. CONCLUSION: Our observations of discrepant immunological and virological responses to treatment raise the issue of the significance of persistent elevated levels of plasma HIV RNA and of the relevance of measurements of plasma viral load for assessing the efficacy of antiretroviral therapy in patients whose CD4 cell counts increase despite the absence of significant decrease in plasma HIV viral load.},
 Keywords = {Adult
Aged
Anti-HIV Agents/*therapeutic use
Cohort Studies
Drug Therapy, Combination
Female
Follow-Up Studies
HIV Infections/*drug therapy/immunology/physiopathology/virology
HIV Protease Inhibitors/*therapeutic use
Human
Indinavir/*therapeutic use
Lamivudine/*therapeutic use
Male
Middle Aged
Prospective Studies
Reverse Transcriptase Inhibitors/*therapeutic use
Stavudine/*therapeutic use
Support, Non-U.S. Gov't
Treatment Outcome
Zidovudine/*therapeutic use},
   Year = {1998} }



@article{
Piketty01,
   Author = {Piketty, C. and Weiss, L. and Thomas, F. and Mohamed, A. S. and Belec, L. and Kazatchkine, M. D.},
   Title = {Long-term clinical outcome of human immunodeficiency virus-infected patients with discordant immunologic and virologic responses to a protease inhibitor-containing regimen},
   Journal = {J Infect Dis},
   Volume = {183},
   Number = {9},
   Pages = {1328-35},
   Note = {0022-1899
Journal Article},
   Abstract = {Within a prospective cohort of 150 human immunodeficiency virus (HIV)-infected patients who began first-line protease inhibitor therapy in 1996, the outcome of 42 patients with discrepant virologic and immunologic responses to antiretroviral treatment at 12 months was analyzed at 30 months of treatment. The incidence of AIDS-defining events and deaths (14%) in the group of patients with immunologic responses in the absence of a virologic response was higher than that in full-responder patients (2%); yet, the incidence in this group was lower than that in patients with no immunologic response, despite a virologic response (21%), and was lower than that in patients without an immunologic or virologic response (67%; P<.0001, log-rank test). Differences in outcome were significant (relative risk, 6.9; 95% confidence interval, 1.9-39.3) when factors for progression were compared with those of responder patients. The results support the relevance of the CD4 cell marker over plasma HIV load for predicting clinical outcome in patients who do not achieve full immunologic and virologic responses.},
 Keywords = {Adult
Aged
Antiretroviral Therapy, Highly Active
CD4 Lymphocyte Count
Cohort Studies
Disease Progression
Female
HIV Infections/*drug therapy/immunology/virology
HIV Protease Inhibitors/*therapeutic use
Human
Incidence
Longitudinal Studies
Male
Middle Aged
Mortality
Prospective Studies
RNA, Viral/blood
Time Factors
Treatment Outcome
Viral Load},
   Year = {2001} }



@article{
Pilon02,
   Author = {Pilon, A. A. and Lum, J. J. and Sanchez-Dardon, J. and Phenix, B. N. and Douglas, R. and Badley, A. D.},
   Title = {Induction of apoptosis by a nonnucleoside human immunodeficiency virus type 1 reverse transcriptase inhibitor},
   Journal = {Antimicrob Agents Chemother},
   Volume = {46},
   Number = {8},
   Pages = {2687-91},
   Note = {0066-4804
Journal Article},
   Abstract = {Inhibition of human immunodeficiency virus type 1 reverse transcriptase (RT) by both nucleoside and nonnucleoside RT inhibitors profoundly inhibits virus replication. Nucleoside RT inhibitors are known to be toxic, but there is little information regarding the toxicities of nonnucleoside RT inhibitors (NNRTI). We demonstrate that efavirenz (an NNRTI) induces caspase- and mitochondrion-dependent apoptosis of Jurkat T cells and human peripheral blood mononuclear cells. The clinical relevance of these observations is not yet clear.},
 Keywords = {Annexin V/diagnostic use
Apoptosis/*drug effects
Caspases/physiology
Enzyme Inhibitors/diagnostic use
Fluorescein-5-isothiocyanate
Fluorescent Dyes
HIV-1 Reverse Transcriptase/*antagonists & inhibitors
Human
Jurkat Cells
Membrane Potentials/drug effects
Mitochondria/drug effects/physiology
Oxazines/*pharmacology
Reverse Transcriptase Inhibitors/*pharmacology
Support, Non-U.S. Gov't},
   Year = {2002} }



@article{
Price03,
   Author = {Price, D. A. and Scullard, G. and Oxenius, A. and Braganza, R. and Beddows, S. A. and Kazmi, S. and Clarke, J. R. and Johnson, G. E. and Weber, J. N. and Phillips, R. E.},
   Title = {Discordant outcomes following failure of antiretroviral therapy are associated with substantial differences in human immunodeficiency virus-specific cellular immunity},
   Journal = {J Virol},
   Volume = {77},
   Number = {10},
   Pages = {6041-9},
   Note = {0022-538x
Clinical Trial
Journal Article},
   Abstract = {Many individuals chronically infected with human immunodeficiency virus type 1 (HIV-1) experience a recrudescence of plasma virus during continuous combination antiretroviral therapy (ART) due either to the emergence of drug-resistant viruses or to poor compliance. In most cases, virologic failure on ART is associated with a coincident decline in CD4(+) T lymphocyte levels. However, a proportion of discordant individuals retain a stable or even increasing CD4(+) T lymphocyte count despite virological failure. In order to address the nature of these different outcomes, we evaluated virologic and immunologic variables in a prospective, single-blinded, nonrandomized cohort of 53 subjects with chronic HIV-1 infection who had been treated with continuous ART and monitored intensively over a period of 19 months. In all individuals with detectable viremia on ART, multiple drug resistance mutations with similar impacts on viral growth kinetics were detected in the pol gene of circulating plasma virus. Further, C2V3 env gene analysis demonstrated sequences indicative of CCR5 coreceptor usage in the majority of those with detectable plasma viremia. In contrast to this homogeneous virologic pattern, comprehensive screening with a range of antigens derived from HIV-1 revealed substantial immunologic differences. Discordant subjects with stable CD4(+) T lymphocyte counts in the presence of recrudescent virus demonstrated potent virus-specific CD4(+) and CD8(+) T lymphocyte responses. In contrast, subjects with virologic failure associated with declining CD4(+) T lymphocyte counts had substantially weaker HIV-specific CD4(+) T lymphocyte responses and exhibited a trend towards weaker HIV-specific CD8(+) T lymphocyte responses. Importantly the CD4(+) response was sustained over periods as long as 11 months, confirming the stability of the phenomenon. These correlative data lead to the testable hypothesis that the consequences of viral recrudescence during continuous ART are modulated by the HIV-specific cellular immune response.},
 Keywords = {Adult
Amino Acid Sequence
Anti-HIV Agents/pharmacology/*therapeutic use
CD4-Positive T-Lymphocytes/*immunology
CD8-Positive T-Lymphocytes/*immunology
Chronic Disease
Drug Resistance, Viral/genetics
Drug Therapy, Combination
HIV Envelope Protein gp120/chemistry/genetics
HIV Infections/*drug therapy/immunology/physiopathology
HIV-1/*drug effects/genetics/physiology
Human
Lymphocyte Count
Middle Aged
Molecular Sequence Data
Mutation
Peptide Fragments/chemistry/genetics
Prospective Studies
RNA, Viral/blood
Single-Blind Method
Support, Non-U.S. Gov't
*Treatment Failure
Viral Load},
   Year = {2003} }



@article{
Quinones00,
   Author = {Quinones-Mateu, M. E. and Ball, S. C. and Marozsan, A. J. and Torre, V. S. and Albright, J. L. and Vanham, G. and van Der Groen, G. and Colebunders, R. L. and Arts, E. J.},
   Title = {A dual infection/competition assay shows a correlation between ex vivo human immunodeficiency virus type 1 fitness and disease progression},
   Journal = {J Virol},
   Volume = {74},
   Number = {19},
   Pages = {9222-33},
   Note = {0022-538x
Journal Article},
   Abstract = {This study was designed to examine the impact of human immunodeficiency virus type 1 (HIV-1) fitness on disease progression through the use of a dual competition/heteroduplex tracking assay (HTA). Despite numerous studies on the impact of HIV-1 diversity and HIV-specific immune response on disease progression, we still do not have a firm understanding of the long-term pathogenesis of this virus. Strong and early CD8-positive cytotoxic T-cell and CD4-positive T-helper cell responses directed toward HIV-infected cells appear to curb HIV pathogenesis. However, the rate at which the virus infects the CD4(+) T-cell population and possibly destroys the HIV-specific immune response may also alter the rate of disease progression. For HIV-1 fitness studies, we established conditions for dual HIV-1 infections of peripheral blood mononuclear cells (PBMC) and a sensitive HTA to measure relative virus production. A pairwise comparison was then performed to estimate the relative fitness of various non-syncytium-inducing/CCR5-tropic (NSI/R5) and syncytium-inducing/CXCR4-tropic (SI/X4) HIV-1 isolates. Four HIV-1 strains (two NSI/R5 and two SI/X4) with moderate ex vivo fitness were then selected as controls and competed against primary HIV-1 isolates from an HIV-infected Belgian cohort. HIV-1 isolates from long-term survivors (LTS) were outcompeted by control strains and were significantly less fit than HIV-1 isolates from patients with accelerated progression to AIDS (PRO). In addition, NSI/R5 HIV-1 isolates from PRO overgrew control SI/X4 strains, suggesting that not all SI/X4 HIV-1 isolates replicate more efficiently than all NSI/R5 isolates. Finally, there were strong, independent correlations between viral load and the total relative fitness values of HIV-1 isolates from PRO (r = 0.84, P = 0.033) and LTS (r = 0.86, P = 0.028). Separation of the PRO and LTS plots suggest that HIV-1 fitness together with viral load may be a strong predictor for the rate of disease progression.},
 Keywords = {*Biological Assay
HIV Infections/*physiopathology/*virology
*HIV-1/physiology
Human
Predictive Value of Tests
Prognosis
Support, Non-U.S. Gov't
Support, U.S. Gov't, P.H.S.},
   Year = {2000} }



@article{
Racinan02,
   Author = {Rancinan, C. and Neau, D. and Saves, M. and Lawson-Ayayi, S. and Bonnet, F. and Mercie, P. and Dupon, M. and Couzigou, P. and Dabis, F. and Chene, G.},
   Title = {Is hepatitis C virus co-infection associated with survival in HIV-infected patients treated by combination antiretroviral therapy?},
   Journal = {Aids},
   Volume = {16},
   Number = {10},
   Pages = {1357-62},
   Note = {0269-9370
Journal Article},
   Abstract = {OBJECTIVE: To study whether hepatitis C virus (HCV) co-infection or the severe elevation of transaminases is associated with survival after the initiation of antiretroviral combination therapy. DESIGN: Prospective hospital-based cohort (Aquitaine Cohort). METHODS: HIV-infected adults started on an antiretroviral combination before 30 June 1999. HCV infection was defined as antibody detection or positive HCV RNA. Severe elevation of transaminases was defined as a value of aspartate or alanine aminotransferase (AST, ALT) above five times the upper limit of normal values. Survival was studied using a Cox model, including at least baseline HCV status and transaminases as a time-dependent covariate. RESULTS: Overall, 995 patients were analysed, including 576 HCV-positive individuals (58%). At baseline, HCV-positive patients were younger, more often injecting drug users and women, and had more frequently elevated transaminases. A shorter survival was associated with AIDS stage [hazard ratio (HR) versus non-AIDS 1.67; 95% confidence interval (CI) 1.03; 2.68], lower CD4 cell count (HR for 50 cells/mm3 lower 1.33; CI 1.17; 1.51), lower haemoglobin (HR for 1 g/dl lower 1.20; CI 1.07; 1.35), lower platelet count (HR for 10 000 cells/mm3 lower 1.04; CI 1.01; 1.07), and AST during follow-up (HR for > or = 200 IU/l 2.30; CI 1.32; 4.03). HCV co-infection (HR 1.20; CI 0.75; 1.92) was not statistically associated with survival. CONCLUSION: The occurrence of a severe elevation of transaminases was associated with poorer survival, although HCV was not. If liver toxicity may be treatment induced, plasma drug concentrations could guide dosage adjustments of antiretroviral treatments currently prescribed to optimize their use.},
 Keywords = {Acquired Immunodeficiency Syndrome/complications
Age Factors
Anti-HIV Agents/*therapeutic use
Antiretroviral Therapy, Highly Active
Cohort Studies
Comparative Study
Disease Progression
Female
Follow-Up Studies
HIV Infections/blood/*complications/*drug therapy
Hepatitis C/blood/*complications
Human
Male
Proportional Hazards Models
Substance Abuse, Intravenous
Support, Non-U.S. Gov't
Survival Analysis
Transaminases/blood},
   Year = {2002} }



@article{
Roger99,
   Author = {Roger, P. M. and Breittmayer, J. P. and Arlotto, C. and Pugliese, P. and Pradier, C. and Bernard-Pomier, G. and Dellamonica, P. and Bernard, A.},
   Title = {Highly active anti-retroviral therapy (HAART) is associated with a lower level of CD4+ T cell apoptosis in HIV-infected patients},
   Journal = {Clin Exp Immunol},
   Volume = {118},
   Number = {3},
   Pages = {412-6},
   Note = {0009-9104
Journal Article},
   Abstract = {HAART may increase CD4+ T cell counts despite a persistently detectable HIV load. The impact of HAART on apoptosis, which may play a role in the disease process in HIV-infected patients, has not been extensively studied. We performed a study to compare the level of spontaneous T cell apoptosis and anti-retroviral treatments in a cohort of HIV-1-infected patients. Data were obtained from a computerized medical record. Quantification of apoptotic cells was by cytofluorometric technique. From November 1995 to December 1997 we studied T cell apoptosis in 112 HIV-infected patients. Forty patients were classified A, 36 B and 36 C. Thirty patients were naive and 82 received an anti-retroviral treatment, 49 including a protease inhibitor (PI). The median plasma viraemia determined in 63 patients was 3.6 (range 1.3-5.6) log10. The median apoptotic cell count was 22% (range 2-73%) and 12% (range 2-60%) for CD4+ and CD8+ T cells, respectively. We did not observe any correlation between the HIV viraemia and the level of apoptosis of T cell subsets. Patients with HAART showed a lower percentage of apoptotic CD4+ T cells only: 16% (range 2-61%) versus 25% (range 5-73%) for patients receiving two nucleoside analogues (P = 0.02). This effect was significant in stage A patients and remained observable during the whole course of HIV disease. In conclusion, HAART, without any relation to plasma viraemia, is able to reduce apoptosis of CD4+ T cells.},
 Keywords = {Adult
Aged
Anti-HIV Agents/*therapeutic use
*Apoptosis
CD4-Positive T-Lymphocytes/cytology/*drug effects
CD8-Positive T-Lymphocytes/drug effects
Didanosine/therapeutic use
Drug Therapy, Combination
Female
HIV Infections/*drug therapy/immunology/pathology
HIV Protease Inhibitors/therapeutic use
Human
Lamivudine/therapeutic use
Male
Middle Aged
Multivariate Analysis
Retrospective Studies
Stavudine/therapeutic use
Viral Load
Zalcitabine/therapeutic use
Zidovudine/therapeutic use},
   Year = {1999} }



@article{
Stoddart01,
   Author = {Stoddart, C. A. and Liegler, T. J. and Mammano, F. and Linquist-Stepps, V. D. and Hayden, M. S. and Deeks, S. G. and Grant, R. M. and Clavel, F. and McCune, J. M.},
   Title = {Impaired replication of protease inhibitor-resistant HIV-1 in human thymus},
   Journal = {Nat Med},
   Volume = {7},
   Number = {6},
   Pages = {712-8},
   Note = {1078-8956
Journal Article},
   Abstract = {Many HIV-1-infected patients treated with protease inhibitors (PI) develop PI-resistant HIV-1 variants and rebounds in viremia, but their CD4+ T-cell counts often do not fall. We hypothesized that in these patients, T-cell counts remain elevated because PI-resistant virus spares intrathymic T-cell production. To test this, we studied recombinant HIV-1 clones containing wild-type or PI-resistant protease domains, as well as uncloned isolates from patients, in activated peripheral blood mononuclear cells, human thymic organ cultures and human thymus implants in SCID-hu Thy/Liv mice. In most cases, wild-type and PI-resistant HIV-1 isolates replicated to similar degrees in peripheral blood mononuclear cells. However, the replication of PI-resistant but not wild-type HIV-1 isolates was highly impaired in thymocytes. In addition, patients who had PI-resistant HIV-1 had abundant thymus tissue as assessed by computed tomography. We propose that the inability of PI-resistant HIV-1 to replicate efficiently in thymus contributes to the preservation of CD4+ T-cell counts in patients showing virologic rebound on PI therapy.},
 Keywords = {Adult
Animals
CD4 Lymphocyte Count
Drug Resistance, Microbial
Fetal Tissue Transplantation
Flow Cytometry
HIV Core Protein p24/metabolism
HIV Infections/immunology/pathology/*virology
HIV Protease/genetics/*metabolism
HIV Protease Inhibitors/*pharmacology
HIV-1/*drug effects/enzymology/genetics/*physiology
Human
Mice
Mice, SCID
Middle Aged
Organ Culture
Recombination, Genetic
Support, Non-U.S. Gov't
Support, U.S. Gov't, P.H.S.
T-Lymphocytes/*physiology/virology
Thymus Gland/pathology/physiopathology/transplantation/*virology
Viral Load
*Virus Replication},
   Year = {2001} }



@article{
Sufka03,
   Author = {Sufka, S. A. and Ferrari, G. and Gryszowka, V. E. and Wrin, T. and Fiscus, S. A. and Tomaras, G. D. and Staats, H. F. and Patel, D. D. and Sempowski, G. D. and Hellmann, N. S. and Weinhold, K. J. and Hicks, C. B.},
   Title = {Prolonged CD4+ cell/virus load discordance during treatment with protease inhibitor-based highly active antiretroviral therapy: immune response and viral control},
   Journal = {J Infect Dis},
   Volume = {187},
   Number = {7},
   Pages = {1027-37},
   Note = {0022-1899
Clinical Trial
Journal Article},
   Abstract = {Mechanisms that underly discordant CD4+ cell/virus load (VL) responses in patients who receive highly active antiretroviral therapy (HAART) were studied in 30 human immunodeficiency virus (HIV)-positive patients, in 3 groups. Discordant responders maintained CD4+ cell levels >200/mm(3) with stable or increasing trend, despite sustained VLs of 500-5000 copies/mL, for >2 years. Treatment-success patients had CD4+ cell counts >200/mm(3) with stable or increasing trend and VLs <50 copies/mL, for >2 years. Treatment-failure patients initially responded to HAART, followed by decreasing CD4+ cell counts and increasing VLs. Interferon-gamma production to gag and noncytolytic CD8+ cell suppressive activity were greater in discordant responders. Cellular activation was greatest in patients with treatment failure. All discordant responders had non-syncytium-inducing (CCR5-tropic) viruses. Viruses from discordant responders and from patients with treatment failure had extensive resistance mutations; discordant responders had significantly lower viral replication capacities. These findings suggest that discordant responses may be related to enhanced HIV-directed immune responses, diminished cellular activation, decreased viral replication capacity, and preservation of non-syncytium-inducing virus strains.},
 Keywords = {Adult
*Antiretroviral Therapy, Highly Active
*CD4 Lymphocyte Count
Female
HIV/*drug effects
HIV Infections/*drug therapy/*immunology/virology
HIV Protease Inhibitors/*pharmacology/therapeutic use
Human
Male
Middle Aged
Support, Non-U.S. Gov't
Support, U.S. Gov't, P.H.S.
Time Factors
Treatment Failure
*Viral Load
Virus Replication/drug effects},
   Year = {2003} }



@article{
Tebaldi03,
   Author = {Tedaldi, E. M. and Baker, R. K. and Moorman, A. C. and Alzola, C. F. and Furhrer, J. and McCabe, R. E. and Wood, K. C. and Holmberg, S. D.},
   Title = {Influence of coinfection with hepatitis C virus on morbidity and mortality due to human immunodeficiency virus infection in the era of highly active antiretroviral therapy},
   Journal = {Clin Infect Dis},
   Volume = {36},
   Number = {3},
   Pages = {363-7},
   Note = {1537-6591
Journal Article},
   Abstract = {To ascertain the impact of hepatitis C virus (HCV) infection on human immunodeficiency virus (HIV) disease progression and associated death in the era of highly active antiretroviral therapy (HAART), we examined mortality rates, the presence of other diseases, and antiretroviral use in an observational cohort of 823 HIV-infected patients with and without HCV coinfection during the period of January 1996 through June 2001. Analyses were used to compare patient characteristics, comorbid conditions, and survival durations in HIV-infected and HIV-HCV-coinfected patients. HIV-HCV-coinfected persons did not have a statistically greater rate of acquired immunodeficiency syndrome or of renal or cardiovascular disease, but they did have more cases of cirrhosis and transaminase elevations. There were proportionately more deaths in the HIV-HCV-coinfected group. Age, baseline CD4+ cell count, and duration of HAART were significantly associated with survival, but HCV infection was not. HAART use was a strong predictor of increased duration of survival, suggesting that treatment is more important to survival than is HCV coinfection status.},
 Keywords = {Anti-HIV Agents/therapeutic use
*Antiretroviral Therapy, Highly Active
*Hiv
HIV Infections/*complications/drug therapy/epidemiology/mortality
*Hepacivirus
Hepatitis C/*complications/epidemiology/mortality
Human
Morbidity
Mortality
Support, U.S. Gov't, P.H.S.},
   Year = {2003} }




@string{JASA= {Journal of the American Statistical Association}}
@string{JC = {Journal of Classification}}
@string{JSPI = {Journal of Statistical Planning and Inference}}
@string{JRSSB = {Journal of the Royal Statistical Society, Series B}}
@string{PNAS = {Proc. Natl. Acad. Sci.}}

@Article{Wang&Bembom&vanderLaan06,
  author =   {Y. Wang and O. Bembom and M.J. van der Laan},
  title =    {Data adaptive estimation of the treatment specific mean},
  journal =      {Journal of Statistical Planning and Inference},
  year =     {2006},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {also http://www.bepress.com/ucbbiostat/paper159},
  OPTannote =    {}
}
@Article{Sinisi&vanderLaan04,
  author =   {S. Sinisi and M.J. van der Laan},
  title =    {The deletion/substitution/addition algorithm in loss function based estimation:
Applications in Genomics},
  journal =      {Journal of Statistical Methods in Molecular Biology},
  year =     {2004},
  OPTkey =   {},
  volume =   {3},
  number =   {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/sagmb/vol3/iss1/art18},
  OPTannote =    {}
}



@TECHREPORT{Petersen&Deeks&Martin&vanderLaan05,
  author =       {Maya L. Petersen and Steven G. Deeks and Jeffrey N. Martin and Mark J. van der Laan},
  title =        {History-Adjusted Marginal Structural Models: Time-Varying Effect Modification
  and Dynamic Treatment Regimens},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2005},
  type =         {Technical Report 199},
OPTnote =      {http://www.bepress.com/ucbbiostat/paper199},
  month =        {December},
}

@TECHREPORT{vanderLaan&Rubin05,
  author =       {M.J. van der Laan and D. Rubin},
  title =        {Estimating Function Based Cross-Validation and Learning},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2005},
  type =         {Technical Report 180},
OPTnote =      {http://www.bepress.com/ucbbiostat/paper180},
  month =        {},
}

@Article{vanderLaan&Petersen07,
  author =   {M.J. van der Laan and M.L. Petersen},
  title =    {Causal Effect Models for Realistic Individualized Treatment and Intention to Treat Rules},
  journal =      {International Journal of Biostatistics},
  year =     {2007},
  OPTkey =   {},
  volume =   {3},
  number =   {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/ijb/vol3/iss1/art3},
  OPTannote =    {}
}


@TECHREPORT{vanderLaan06,
  author =       {M.J. van der Laan},
  title =        {Causal Effect Models for Intention to Treat and Realistic Individualized
  Treatment Rules},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2006},
  type =         {Technical Report 203},
OPTnote =      {http://www.bepress.com/ucbbiostat/paper203},
  month =        {},
}
@TECHREPORT{vanderLaan08b,
  author =       {M.J. van der Laan},
  title =        {The construction and analysis of adaptive group sequential designs},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2008},
  type =         {Technical Report 232},
OPTnote =      {http://www.bepress.com/ucbbiostat/paper232},
  month =        {March},
}
@TECHREPORT{Moore&vanderLaan07,
  author =       {K.L. Moore and M.J. van der Laan},
  title =        {Covariate adjustment in randomized trials with binary outcomes},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2007},
  type =         {Technical Report 215},
OPTnote =      {http://www.bepress.com/ucbbiostat/paper215},
  month =        {April},
}

@TECHREPORT{vanderLaan&Petersen05,
  author =       {M.J. van der Laan and M.L. Petersen},
  title =        {Direct Effect Models},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2005},
  type =         {Technical Report 187},
OPTnote =      {http://www.bepress.com/ucbbiostat/paper187},
  month =        {},
}
@TECHREPORT{Petersen&vanderLaan06,
  author =       {M.L. Petersen and M.J. van der Laan},
  title =        {Individualized Treatment Rules and Clinical Trials},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2006},
  type =         {Technical Report},
OPTnote =      {},
  month =        {},
}

@Article{vanderLaan&Petersen&Joffe05,
  author =   {M.J. van der Laan and M.L. Petersen and M.M. Joffe},
  title =    {History-Adjusted Marginal Structural Models and Statically-Optimal Dynamic Treatment Regimens},
  journal =      {The International Journal of Biostatistics},
  year =     {2005},
  OPTkey =   {},
  volume =   {1},
  number =   {1},
  pages =    {10-20},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/ijb/vol1/iss1/4},
  OPTannote =    {}
}

@Article{vanderLaan06a,
  author =   {M.J. van der Laan},
  title =    {Statistical Inference for Variable Importance},
  journal =      {International Journal of Biostatistics},
  year =     {2006},
  OPTkey =   {},
  volume =   {2},
  number =   {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/ijb/vol2/iss1/art2},
  OPTannote =    {}
}

@Article{vanderLaan&Birkner&Hubbard05,
  author =   {M.J. van der Laan and M.D. Birkner and A.E. Hubbard},
  title =    {Empirical Bayes and resampling based multiple testing procedure controlling tail probability of the proportion of false positives},
  journal =      {Journal of Statistical Applications in Genetics and Molecular Biology},
  year =     {2005},
  OPTkey =   {},
  volume =   {4},
  number =   {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/sagmb/vol4/iss1/art29},
  OPTannote =    {}
}



@Article{vanderLaan&Dudoit&Pollard04b,
  author =   {M.J. van der Laan and S. Dudoit and K.S. Pollard},
  title =    {Augmentation procedures for control of the generalized family-wise
  error rate and tail probabilities for the proportion of false positives},
journal =      {Journal of Statistical Applications in Genetics and Molecular Biology},
  year =     {2004},
  OPTkey =   {},
  volume =   {3},
  number =   {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/sagmb/vol3/iss1/art15},
  OPTannote =    {}
}
@Article{vanderLaan&Dudoit&Pollard04,
  author =   {S. Dudoit and M.J. van der Laan and K.S. Pollard},
  title =    {Multiple testing. Part II.
  Step-down procedures for control of the family-wise error rate
  },
journal =      {Journal of Statistical Applications in Genetics and Molecular Biology},
  year =     {2004},
  OPTkey =   {},
  volume =   {3},
  number =   {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/sagmb/vol3/iss1/art14},
  OPTannote =    {}
}

@Article{Dudoit&vanderLaan&Pollard04,
  author =   {S. Dudoit and M.J. van der Laan and K.S. Pollard},
  title =    {Multiple testing. Part I. Single-step procedures for control of general Type I error rates},
journal =      {Journal of Statistical Applications in Genetics and Molecular Biology},
  year =     {2004},
  OPTkey =   {},
  volume =   {3},
  number =   {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/sagmb/vol3/iss1/art13},
  OPTannote =    {}
}


@Article{Birkner&Sinisi&vanderLaan05,
  author =   {M.D. Birkner and S.E. Sinisi and M.J. van der Laan},
  title =    {Multiple Testing and Data Adaptive Regression: An Application
  to {HIV}-1 Sequence Data},
  journal =      {Journal of Statistical Applications in Genetics and Molecular Biology},
  year =     {2005},
  OPTkey =   {},
  volume =   {4},
  number =   {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/sagmb/vol4/iss1/art8},
  OPTannote =    {}
}

@TECHREPORT{vanderLaan&Hubbard06,
  author =       {M.J. van der Laan and A.E. Hubbard},
  title =        {Quantile-Function Based Null Distribution in Resampling Based Multiple Testing},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2006},
  type =         {Technical Report},
OPTnote =      {http://www.bepress.com/ucbbiostat/paper198},
  month =        {},
}
@TECHREPORT{Molinaro&vanderLaan04,
  author =       {A. Molinaro and M.J. van der Laan},
  title =        {Deletion/Substitution/Addition Algorithm for Partitioning the Covariate Space in Prediction},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2004},
  type =         {Technical Report},
OPTnote =      {http://www.bepress.com/ucbbiostat/paper162},
  month =        {},
}
@TECHREPORT{Birkner&vanderLaan05,
  author =       {M.D. Birkner and M.J. van der Laan},
  title =        {Application of a Variable Importance Measure Method to {HIV}-1 Sequence Data},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2005},
  type =         {Technical Report},
  month =        {},
}



@TECHREPORT{Neugebauer&vanderLaan05b,
  author =       {R. Neugebauer and M.J. van der Laan},
  title =        {Locally Efficient Estimation of Nonparametric
                    Causal Effects on Mean Outcomes in Longitudinal Studies},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2005},
  number =       {134},
  type =         {Technical Report},
OPTnote =    {http://www.bepress.com/ucbbiostat/paper134, to appear in {JSPI}},
  month =        {},
}
@TECHREPORT{Wang&Petersen&vanderLaan06,
  author =       {Y. Wang and M. Petersen and M.J. van der Laan},
  title =        {A statistical method for diagnosing ETA bias in IPTW estimators},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2006},
  number =       {},
  type =         {Technical Report},
OPTnote =    {},
  month =        {},
}

@TECHREPORT{Moore&vanderLaan07,
  author =       {K.L. Moore and M.J. van der Laan},
  title =        {Covariate adjustment in randomized trials with binary outcomes},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2007},
  type =         {Technical Report 215},
OPTnote =    {http://www.bepress.com/ucbbiostat/paper215},
  month =        {April},
}

@TECHREPORT{vanderLaan&Dudoit&vanderVaart,
  author =       {M.J. van der Laan and S. Dudoit and A.W. van der Vaart},
  title =        {The Cross-Validated Adaptive Epsilon-Net Estimator},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2004},
  type =         {Technical Report 142},
OPTnote =    {http://www.bepress.com/ucbbiostat/paper142},
  month =        {February},
}

@TECHREPORT{vanderLaan&DudoitTechRep130,
  author =       {M.J. van der Laan and S. Dudoit},
  title =        {Unified cross-validation methodology for selection among estimators
  and a general cross-validated adaptive epsilon-net estimator: Finite sample oracle
  inequalities and examples},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2003},
  type =         {Technical Report},
OPTnote =    {http://www.bepress.com/ucbbiostat/paper130},
  month =        {November},
}

@TECHREPORT{Petersen&vanderLaan05,
  author =       {M. Petersen and M.J. van der Laan},
  title =        {Estimation of direct and indirect causal effects in
Epidemiology},
  institution =  {Division of Biostatistics, University of California,
Berkeley},
  year =         {2005},
  type =         {Technical Report},
  month =        {},
}

@TECHREPORT{Petersen&Deeks&Martin&vanderLaan05,
  author =       {M.L. Petersen and S.G. Deeks and J.N. Martin and M.J. van der Laan},
  title =        {History-Adjusted Marginal Structural Models: Time-Varying Effect Modification and Dynamic Treatment Regimens},
  institution =  {Division of Biostatistics, University of California,
Berkeley},
  year =         {2005},
  type =         {Technical Report 199},
OPTnote =      {http://www.bepress.com/ucbbiostat/paper199},
  month =        {},
}

@TECHREPORT{vanderLaan&Petersen04,
  author =       {M.J. van der Laan and M. Petersen},
  title =        {Estimation of direct and indirect causal effects in longitudinal studies},
  institution =  {Division of Biostatistics, University of California,
Berkeley},
  year =         {2004},
  type =         {Technical Report 155},
  month =        {August},
}

@TECHREPORT{vanderLaan&Hubbard&Jewell04,
 author =       {M.J. van der Laan and A.E. Hubbard and N.P. Jewell},
  title =        {Estimation of Treatment Effects in Randomized Trials with Noncompliance and a Dichotomous Outcome},
  institution =  {Division of Biostatistics, University of California,
Berkeley},
  year =         {2004},
  type =         {Technical Report 157},
  OPTnote =      {http://www.bepress.com/ucbbiostat/paper157},
month =        {September},
}
@TECHREPORT{Bein&Hubbard&vanderLaan05,
 author =       {E. Bein and A.E. Hubbard and M.J. van der Laan},
  title =        {Estimating Function Based Cross-Validation in
Estimation of the Causal Effect in Randomized Trials},
  institution =  {Division of Biostatistics, University of California,
Berkeley},
  year =         {2005},
  type =         {Technical Report},
}





@TECHREPORT{vanderLaan&DudoitTechRep130,
  author =       {M.J. van der Laan and S. Dudoit},
  title =        {Unified cross-validation methodology for
selection among estimators and a general cross-validated adaptive
epsilon net estimator: Finite sample oracle inequalities and
examples},
  institution =  {Division of Biostatistics, University of California,
Berkeley},
  year =         {2003},
  type =         {Technical Report 130},
  month =        {Nov.},
}


@TECHREPORT{Molinaroetal05,
  author =       {A.M. Molinaro and M.J. van der Laan and D.H. Moore and K. Kerlikowske},
  title =        {Survival point estimate prediction in matched and non-matched case-control subsample designed studies},
  institution =  {Division of Biostatistics, University of California,
Berkeley},
  year =         {2005},
  note =         {http://www.bepress.com/ucbbiostat/paper149},
}


@TECHREPORT{DudoitetalSIGKDD04,
  author =       {S. Dudoit and M.J. van der Laan and S. Kele\c{s} and A.
M. Molinaro and S. E. Sinisi
and S.L. Teng},
  title =        {Loss-Based Estimation with Cross-Validation:
Applications to Microarray Data
Analysis and Motif Finding.},
  institution =  {Division of Biostatistics, University of California,
Berkeley},
  year =         {2004},
  note =         {to appear in \emph{SIGKDD} Explorations on Microarray Data Mining},
}

@Book{Friedman&Furberg&Demets98,
  author =       {L.M.Friedman and C.D. Furberg and D.L. DeMets},
  title =        {Fundamentals of Clinical Trials},
  publisher =    {Springer-Verlag New York},
  year =         {1998}
}

@Book{ABGK,
  author =       {P.K. Andersen and O. Borgan and R.D. Gill and N. Keiding},
  title =        {Statistical Models Based on Counting Processes},
  publisher =    {Springer-Verlag New York},
  year =         {1993}
}
@Article{Wittes&Brittain90,
  author =   {J. Wittes and E. Brittain},
  title =    {The role of internal pilot studies in increasing efficiency of clinical trials},
journal =      {Statistics in Medicine},
  year =     {1999},
  OPTkey =   {},
  volume =   {9},
  number =   {},
  pages =    {65--72},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

%references for direct and indirect effects:
@InCollection{Robins03,
  author =   {J.M. Robins},
  title =    {Semantics of causal DAG models and the identification of direct and
indirect effects},
  booktitle =    {Highly Structured Stochastic Systems},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher = {Oxford University Press, Oxford},
  year =     {2003},
  editor =   {P. Green, N. Hjort, and S. Richardson},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {70--81},
  OPTnote =      {},
  OPTannote =    {}
}

@InCollection{Hubbard&vanderLaan&Robins99,
  author =   {A. Hubbard and M.J. van der Laan and J.M. Robins},
  title =    {Nonparametric locally ecient
estimation of the treatment specic survival distribution with right censored data
and covariates in observational studies},
  booktitle =    {Statistical Models in Epidemiology, The Environment and Clinical Trials},
  publisher = {Springer Verlag},
  year =     {1999},
editor={M.E. Halloran and D. Berry},
volume={116},
pages={135--178},
  series =   {IMA Volumes in Mathematics and its Applications, Ed. M.E. Halloran and D. Berry}
}

@TechReport{Pearl01,
  author =   {J. Pearl},
  title =    {Cognitive systems Laboratory},
  institution =  {University of California, Los Angeles, Department of Computer Science},
  year =     {2001},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Pearl00,
  author =   {J. Pearl},
  title =    {Causality: Models, Reasoning, and Inference},
  publisher =    {Cambridge University Press, Cambridge},
  year =     {2000},
  OPTkey =   {},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  series =   {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Robins&Greenland92,
  author =   {J.M. Robins and S. Greenland},
  title =    {Identifiability and exchangeability for direct and indirect
effects},
  journal =      {Epidemiology},
  year =     {1992},
  OPTkey =   {},
  volume =   {3},
  number =   {0},
  pages =    {143--155},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{vanderLaan95,
  author =   {M.J. van der Laan},
  title =    {Identity for NPMLE in missing data and biased sampling models},
  journal =      {Bernoulli},
  year =     {1995},
  OPTkey =   {},
  volume =   {1},
  number =   {4},
  pages =    {335--341},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{vanderLaan98,
  author =   {M.J. van der Laan},
  title =    {Identity for NPMLE in Censored Data Models},
  journal =      {Lifetime Data Models},
  year =     {1998},
  OPTkey =   {},
  volume =   {4},
  number =   {0},
  pages =    {83--102},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Klaassen86,
  author =   {C.A.J. Klaassen},
  title =    {Consistent estimation of the influence function of locally asymptotically linear estimators},
  journal =      {Annals of Statistics},
  year =     {1987},
  OPTkey =   {},
  volume =   {15},
  number =   {},
  pages =    {1548--1562},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}





%the next references are for instrumental variable article
@Article{Robins&Rotnitzky04,
  author =   {J.M. Robins and A. Rotnitzky},
  title =    {Estimation of Treatment Effects in Randomized Trials
with Noncompliance and a Dichotomous Outcome using Structural Nested
Mean Models},
  journal =      {Biometrika},
  year =     {2004},
  OPTkey =   {},
  volume =   {0},
  number =   {0},
  pages =    {0},
  OPTmonth =     {},
  OPTnote =      {To Appear},
  OPTannote =    {}
}

@Article{Vandervaart91,
  author =   {A.W. van der Vaart},
  title =    {On differentiable functionals},
  journal =      {Annals of Statistics},
  year =     {1991},
  OPTkey =   {},
  volume =   {19},
  number =   {},
  pages =    {178--204},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}




@Article{Rubin78,
  author =   {D.B. Rubin},
  title =    {Bayesian Inference for causal effects: the role of randomization},
  journal =      {Annals of Statistics},
  year =     {1978},
  OPTkey =   {},
  volume =   {6},
  number =   {},
  pages =    {34--58},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Neyman23,
  author =   {Neyman, J.},
  title =    {On the application of probability theory to agricultural
experiments},
  journal =      {Statistical Science},
  year =     {1990},
  OPTkey =   {},
  volume =   {5},
  number =   {},
  pages =    {465--480},
  OPTmonth =     {},
  OPTnote =      {Translation of 1923 article},
  OPTannote =    {}
}
@Article{Robins86,
  author =   {J.M. Robins},
  title =    {A new approach to causal inference in mortality studies with sustained exposure periods - Application to control of the healthy worker survivor effect},
  journal =      {Mathematical Modelling},
  year =     {1986},
  OPTkey =   {},
  volume =   {7},
  number =   {},
  pages =    {1393--1512},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}





@Article{Robins94,
  author =   {J.M. Robins},
  title =    {Correcting for non-compliance in randomized trials
using structural nested mean models},
  journal =      {Communications in Statistics},
  year =     {1994},
  OPTkey =   {},
  volume =   {23},
  number =   {},
  pages =    {2379--2412},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Vansteelandt03,
  author =   {S. Vansteelandt and E. Goetghebeur},
  title =    {Causal inference with generalized structural  mean
models},
  journal =      {Journal of the Royal Statistical Society, Series B},
  year =     {2003},
  OPTkey =   {},
  volume =   {23},
  number =   {},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {In print},
  OPTannote =    {}
}

@incollection {Robins97a,
   AUTHOR = {Robins, J.M.},
    TITLE = {Structural Nested Failure Time Models},
BOOKTITLE = {The Encyclopedia of Biostatistics},
PUBLISHER = {John Wiley and Sons},
  ADDRESS = {Chichester, UK},
     YEAR = {1997},
   EDITOR = {Armitage, P. and Colton, T. and Andersen, P.K. and Keiding, N.}
}
@article {hernan_brumback_robins,
   AUTHOR = {Hernan, M. A. and Brumback, B. and Robins, J. M.},
    TITLE = {Marginal structural models to estimate the causal effect of zidovudine on the survival of {HIV}-positive men},
  JOURNAL = {Epidemiology},
   VOLUME = {11},
   NUMBER = {5},
     YEAR = {2000},
    PAGES = {561--570}
}
@article {Robins87,
   AUTHOR = {Robins, J.M.},
    TITLE = {Addendum to: ``{A} new approach to causal inference in
             mortality studies with a sustained exposure
             period---application to control of the healthy worker survivor
             effect'' [{M}ath.\ {M}odelling {\bf 7} (1986), no.\ 9-12,
             1393--1512; {M}{R} 87m:92078]},
  JOURNAL = {Comput. Math. Appl.},
 FJOURNAL = {Computers \& Mathematics with Applications. An International
             Journal},
   VOLUME = {14},
     YEAR = {1987},
   NUMBER = {9-12},
    PAGES = {923--945},
     ISSN = {0097-4943},
    CODEN = {CMAPDK},
}

@article {robins_hernan_brumback,
   AUTHOR = {Robins, J. M. and Hernan, M. A. and Brumback, B.},
    TITLE = {Marginal structural models and causal inference in epidemiology},
  JOURNAL = {Epidemiology},
   VOLUME = {11},
   NUMBER = {5},
     YEAR = {2000},
    PAGES = {550--560}
}





@article {Bryan&Yu&vanderLaan03,
   AUTHOR = {Bryan, J. and Yu, Z. and van der Laan, M.J.},
    TITLE = {Analysis of Longitudinal Marginal Structural Models},
  JOURNAL = {Biostatistics},
   VOLUME = {5},
   NUMBER = {3},
     YEAR = {2003},
    PAGES = {361--380}
}

@TechReport{Yu&vanderLaan03,
  author =   {Yu, Z. and van der Laan, M.J.},
  title =    {Double Robust Estimation in Longitudinal Marginal Structural
                    Models},
  institution =  {Division of Biostatistics, University of California,
Berkeley},
  year =     {2003},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {132},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/ucbbiostat/paper132},
  OPTannote =    {}
}

@Article{Neugebauer&vanderLaan05,
  author =   {Neugebauer, R. and van der Laan, M.J.},
  title =    {Why prefer double robust estimates},
  journal =      {Journal of Statistical Planning and Inference},
  year =     {2005},
  OPTkey =   {},
  volume =   {129},
  number =   {1-2},
  pages =    {405--426},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@article {Murphy03,
   AUTHOR = {Murphy, S.A.},
    TITLE = {Optimal dynamic treatment regimes},
  JOURNAL = {Journal of the Royal Statistical Society: Series B},
   VOLUME = {65},
   NUMBER = {2},
     YEAR = {2003},
    PAGES = {?}
}
@article {Robins03a,
   AUTHOR = {Robins, J.M.},
    TITLE = {Discussion of ''{O}ptimal dynamic treatment regimes" by {S}usan {A}. {M}urphy},
  JOURNAL = {Journal of the Royal Statistical Society: Series B},
   VOLUME = {65},
   NUMBER = {2},
     YEAR = {2003},
    PAGES = {355--366}
}

@article {Murphy&vanderLaan&Robins01,
   AUTHOR = {S.A. Murphy and M.J. van der Laan and J.M. Robins},
    TITLE = {Marginal mean models for dynamic treatment regimens},
  JOURNAL = {Journal of the American Statistical Association},
   VOLUME = {96},
   NUMBER = {},
     YEAR = {2001},
    PAGES = {1410--1424}
}
@incollection {Robins98,
    AUTHOR = {Robins, J.M.},
     TITLE = {Marginal structural models versus structural nested models as
              tools for causal inference},
 BOOKTITLE = {Statistical models in epidemiology, the environment, and
              clinical trials (Minneapolis, MN, 1997)},
     PAGES = {95--133},
 PUBLISHER = {Springer},
   ADDRESS = {New York},
      YEAR = {2000},
   MRCLASS = {62N01 (62G08 62P10)},
  MRNUMBER = {2001a:62124},
}
%Robins, J.M. (2003). Discussion of "Optimal dynamic treatment regimes". by Susan A. Murphy.
  %Journal of the Royal Statistical Society: Series B, 65(2):355-366.
@InCollection{Robins97,
  author =   {J.M. Robins},
  title =    {Causal Inference from Complex Longitudinal Data},
  booktitle =    {Latent Variable Modeling and Applications to Causality},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher = {Springer Verlag, New York},
  year =     {1997},
  editor =   {M. Berkane, Editor},
  OPTvolume =    {120},
  OPTnumber =    {},
  OPTseries =    {Lecture Notes in Statistics},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {69--117},
  OPTnote =      {},
  OPTannote =    {}
}

@InCollection{Robins89,
  author =   {J.M. Robins},
  title =    {The analysis of randomized and non-randomized AIDS
treatment trials using a new approach in causal inference in longitudinal studies},
  booktitle =    {Health Service Methodology: A Focus on AIDS},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher = {U.S. Public Health Service, National Center for Health SErvices Research},
  year =     {1989},
  editor =   {L. Sechrest and H. Freeman and A. Mulley},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {Lecture Notes in Statistics},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {Washington D.C.},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {113--159},
  OPTnote =      {},
  OPTannote =    {}
}



@TechReport{Abadie00,
  author =   {A. Abadie},
  title =    {Semiparametric estimation of instrumental variables models for causal effects},
  institution =  {NBER Technical Working Paper},
  year =     {2000},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {260},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Abadie03,
  author =   {A. Abadie},
  title =    {Semiparametric instrumental variable estimation of treatment response models},
  journal =      {Journal of Econometrics},
  year =     {2003},
  OPTkey =   {},
  volume =   {113},
  number =   {},
  pages =    {231-263},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Abadie03,
  author =   {A. Abadie},
  title =    {Semiparametric instrumental variable estimation of treatment response models},
  journal =      {Journal of Econometrics},
  year =     {2003},
  OPTkey =   {},
  volume =   {113},
  number =   {},
  pages =    {231-263},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@TechReport{Wang&Vanderlaan04,
  author =   {Y. Wang and M.J. van der Laan},
  title =    {Data adaptive estimation of the treatment specific mean},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =     {2004},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {159},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/ucbbiostat/paper159},
  OPTannote =    {}
}
@TechReport{Yu&vanderLaan02,
  author =   {Z. Yu and M.J. van der Laan},
  title =    {Construction of counterfactuals and the {G}-computation formula},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =     {2002},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {122},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/ucbbiostat/paper122},
  OPTannote =    {}
}
@TechReport{Yu&Vanderlaan03,
  author =   {Z. Yu and M.J. van der Laan},
  title =    {Measuring treatment effects using semiparametric models},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =     {2003},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {136},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/ucbbiostat/paper136},
  OPTannote =    {}
}

@Article{Angristetal96,
  author =   {J. Angrist and G. Imbens and D.B. Rubin},
  title =    {Identification of causal effects using instrumental variables},
  journal =      {Journal of the American Statistical Association},
  year =     {1996},
  OPTkey =   {},
  volume =   {91},
  number =   {},
  pages =    {444-555},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Robins&Rotnitzky01A,
  author =   {J.M Robins and A. Rotnitzky},
  title =    {Comment on {I}nference for semiparametric models: some questions
  and an answer, by {B}ickel, {P}.{J}. and {K}won, {J}.},
  journal =      {Statistica Sinica},
  year =     {2001},
  OPTkey =   {},
  volume =   {11},
  number =   {},
  pages =    {920-935},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Angrist01,
  author =   {J. Angrist},
  title =    {Estimation of limited dependent variable models with dummy endogenous regressors: simple strategies for empirical practice},
  journal =      {Journal of Business and Economics Statistics},
  year =     {2001},
  OPTkey =   {},
  volume =   {19},
  number =   {},
  pages =    {1--16},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Chamberlain87,
  author =   {G. Chamberlain},
  title =    {Asymptotic efficiency in estimation with conditional moment
restrictions},
  journal =      {Journal of Econometrics},
  year =     {1987},
  OPTkey =   {},
  volume =   {34},
  number =   {},
  pages =    {305--334},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Hiranoetal00,
  author =   {K. Hirano and G. Imbens and D.B. Rubin and X-H. Zhou},
  title =    {Assessing the effects of influenza vaccine in an encouragement design},
  journal =      {Biostatistics},
  year =     {2000},
  OPTkey =   {},
  volume =   {1},
  number =   {},
  pages =    {69--88},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Neyman23,
  author =   {J. Neyman},
  title =    {Sur les applications de la thar des probabilites aux
experiences Agaricales: Essay des principle (1923). Excerpts reprinted (1990) in
English (D. Dabrowska and T. Speed), Trans.},
  journal =      {Statistical Science},
  year =     {1990},
  OPTkey =   {},
  volume =   {5},
  number =   {},
  pages =    {463--472},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



optimal structural nested models for optimal
sequential decisions Proceedings of the 2nd seattle symposium in
biostatistics eds. Lin DY, Heagerty PJ  Springer Verlag Lecture Notes in
Statisitics No. 179  pages 189-326

@InProceedings{Robins05,
  author =   {J.M. Robins},
  title =    {Optimal structural nested models for optimal sequential decisions},
  booktitle =    {Proceedings of the 2nd Seattle symposium in
biostatistics},
  pages =    {189--326},
  year =     {2005},
  editor =   {Lin, D.Y, Heagerty P.J},
  volume =   {179},
  organization = {},
OPTpublisher = {Springer Verlag Lecture Notes in Statistics}
}


@TechReport{Robins05tech,
  author =   {J.M. Robins},
  title =    {Optimal structural nested models for optimal sequential decisions},
  institution =  {Department of Biostatistics, Havard University},
  year =     {2005},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}





@InProceedings{AIC,
  author =   {H. Akaike},
  title =    {Information theory and an extension of the maximum likelihood principle},
  booktitle =    {Second International Symposium on Information Theory},
  pages =    {267-281},
  year =     {1973},
  editor =   {B.N. Petrov and F. Csaki},
  organization = {Budapest: Academiai Kiado}
}


@Article{Balke&Pearl97,
  author =   {A. Balke and J. Pearl},
  title =    {Bound on treatment effects from studies with imperfect compliance},
  journal =      {Journal of the American Statistical Association},
  year =     {1997},
  OPTkey =   {},
  volume =   {92},
  number =   {},
  pages =    {1172--1176},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{Balke&Pearl94,
author =     {A. Balke and J. Pearl},
  title =    {Counterfactual probabilities: Computational methods, bounds, and applications},
  booktitle =    {In Proceedings of the 12th National Conference on Artificial Intelligence},
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {230--237},
  year =     {1994},
  OPTeditor =    {},
  volume =   {I},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {Menlo Park, CA},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {MIT Press},
  OPTnote =      {},
  OPTannote =    {}
}






@Article{Ambroise&McLachlan02,
  author =   {C. Ambroise and G. J. McLachlan},
  title =    {Selection bias in gene extraction on the basis of microarray gene-expression data},
  journal =      PNAS,
  year =     {2002},
  OPTkey =   {},
  volume =   {99},
  number =   {10},
  pages =    {6562--6566},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@InCollection{Arabie&Hubert96,
  author =   {P. Arabie and L. J. Hubert},
  title =    {An overview of combinatorial data analysis},
  booktitle =    {Clustering and Classification},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher = {World Scientific Publishing Co.},
  year =     {1996},
  editor =   {P. Arabie and L. J. Hubert and G. De Soete},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {River Edge, NJ},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {5--63},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{BIC,
  author =   {G. Schwartz},
  title =    {Estimating the Dimension of a Model},
  journal =      {Annals of Statistics},
  year =     {1978},
  volume =   {6},
  pages =    {461-464}
}


@Article{Barnard,
  author =   {M. Barnard},
  title =    {The secular variations of skull characters in four series of Egyptian skulls},
  journal =      {Annals of Eugenics},
  year =     {1935},
  OPTkey =   {},
  volume =   {6},
  OPTnumber =    {},
  pages =    {352--371},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@InProceedings{BenHuretal02,
  author =   {A. Ben-Hur and A. Elisseeff and I. Guyon},
  title =    {A stability based method for discovering structure in clustered data},
  booktitle =    {Pacific Symposium on Biocomputing},
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {6--17},
  year =     {2002},
  OPTeditor =    {},
  volume =   {7},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Benjamini&Hochberg95,
  author =   {Y. Benjamini and Y. Hochberg},
  title =    {Controlling the false discovery rate: a practical and powerful approach to multiple testing},
  journal =      {J. R. Statist. Soc. B},
  year =     {1995},
  OPTkey =   {},
  volume =   {57},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {289--300},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Benjamini&Yekutieli01,
  author =   {Y. Benjamini and D. Yekutieli},
  title =    {The control of the false discovery rate in multiple testing under
   dependency},
  journal =      {Annals of Statistics},
  year =     {2001},
  OPTkey =   {},
  volume =   {29},
  number =   {4},
  pages =    {1165--1188},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Beran88,
  author =   {R. Beran},
  title =    {Balanced simultaneous confidence sets},
  journal =      JASA,
  year =     {1988},
  OPTkey =   {},
  volume =   {83},
  OPTnumber =    {},
  pages =    {679--686},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Bock85,
  author =   {H-H Bock},
  title =    {On some significance tests in cluster analysis},
  journal =      {Journal of Classification},
  year =     {1985},
  OPTkey =   {},
  volume =   {2},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {77--108},
  OPTnote =      {},
  OPTannote =    {}
}



@InCollection{Bock96,
  author =   {H-H Bock},
  title =    {Probability models and hypotheses testing in partitioning cluster analysis},
  booktitle =    {Clustering and Classification},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher = {World Scientific Publishing Co.},
  year =     {1996},
  editor =   {P. Arabie and L. J. Hubert and G. De Soete},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {River Edge, NJ},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {377--453},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Boldricketal02,
  author =   {J. C. Boldrick and A. A. Alizadeh and M. Diehn and S. Dudoit and C. L. Liu and C. E. Belcher and D. Botstein and L. M. Staudt and P. O. Brown
and D. A. Relman},
  title =    {Stereotyped and specific gene expression programs in human innate immue responses to bacteria},
  journal =      PNAS,
  year =     {2002},
  OPTkey =   {},
  volume =   {99},
  number =   {2},
  pages =    {972--977},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Bozdogan00,
  author =   {H. Bozdogan},
  title =    {Akaike's information criterion and recent developments in information complexity},
  journal =      {Journal of Mathematical Psychology},
  year =     {2000},
  volume =   {44},
  pages =    {62-91}
}




@InCollection{Bozdogan93,
  author =   {H. Bozdogan},
  title =    {Choosing the number of component clusters in the mixture model  using a new informational complexity criterion of the inverse Fisher information matrix},
  booktitle =    {Information and Classification},
  publisher = {Heidelberg: Springer Verlag},
  editor = {O. Opitz and B. Lausen and R. Klar},
  year =     {1993},
  series =   {}
}

@Article{Braver,
  author =   {S. L. Braver},
  title =    {On splitting the tails unequally: a new perspective on one-versus two-tailed tests},
  journal =      {Educational and Psychological Measurement},
  year =     {1975},
  OPTkey =   {},
  volume =   {35},
  OPTnumber =    {},
  pages =    {283--301},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Breckenridge89,
  author =   {J. Breckenridge},
  title =    {Replicating cluster analysis: Method, consistency and validity},
  journal =      {Multivariate Behavioral Research},
  year =     {1989},
  OPTkey =   {},
  volume =   {24},
  OPTnumber =    {},
  pages =    {147--161},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Breiman&Spector92,
  author =   {L. Breiman and P. Spector},
  title =    {Submodel Selection and Evaluation in Regression. The
  $X$ Random Case},
  journal =      {International Statistical Review},
  year =     {1992},
  OPTkey =   {},
  volume =   {60},
  OPTnumber =    {},
  pages =    {291--319},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Breiman01,
  author =   {L. Breiman},
  title =    {Statistical modeling: the two cultures},
  journal =      {Statistical Science},
  year =     {2001},
  OPTkey =   {},
  volume =   {16},
  number =   {3},
  pages =    {199--215},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{BreimanAnnals96,
  author =   {L. Breiman},
  title =    {Heuristics of instability and stabilization in model selection},
  journal =      {Annals of Statistics},
  year =     {1996},
  OPTkey =   {},
  volume =   {24},
  number =   {6},
  pages =    {2350--2383},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{BreimanArcing,
  author =   {L. Breiman},
  title =    {Arcing classifiers},
  journal =      {Annals of Statistics},
  year =     {1998},
  OPTkey =   {},
  volume =   {26},
  OPTnumber =    {},
  pages =    {801-824},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{BreimanBagging,
  author =   {L. Breiman},
  title =    {Bagging predictors},
  journal =      {Machine Learning},
  year =     {1996},
  OPTkey =   {},
  volume =   {24},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {123-140},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{BreimanCPD,
  author =   {L. Breiman},
  title =    {Using Convex pseudo-data to increase prediction accuracy},
  institution =  {Department of Statistics, U.C. Berkeley},
  year =     {1998},
  OPTkey =   {},
  OPTtype =      {},
  number =   {513},
  OPTaddress =   {},
  month =    {March},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{BreimanJASA92,
  author =   {L. Breiman},
  title =    {The Little Bootstrap and Other Methods for
  Dimensionality Selection in Regression: $X$-Fixed Prediction Error},
  journal =      JASA,
  year =     {1992},
  OPTkey =   {},
  volume =   {87},
  number =   {419},
  pages =    {738--754},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@TechReport{BreimanOB,
  author =   {L. Breiman},
  title =    {Out-of-bag estimation},
  institution =  {Department of Statistics, U.C. Berkeley},
  year =     {1996},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@TechReport{BreimanRanForests,
  author =   {L. Breiman},
  title =    {Random forests - random features},
  institution =  {Department of Statistics, U.C. Berkeley},
  year =     {1999},
  OPTkey =   {},
  OPTtype =      {},
  number =   {567},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Breimanetal84,
  author =   {L. Breiman and J. H. Friedman and R. Olshen and C. J. Stone},
  title =    {Classification and regression trees},
  publisher =    {Wadsworth International Group},
  year =     {1984},
  OPTkey =   {},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  series =   {The Wadsworth statistics/probability series},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Book{Hastieetal02,
  author =   {T. Hastie and R. Tibshirani and J. Friedman},
  title =    {The Elements of Statistical Learning},
  publisher =    {Springer},
  year =     {2002},
  OPTkey =   {},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  series =   {Springer Series in Statistics},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Broman01,
  author =   {K. W. Broman},
  title =    {Review of statistical methods for QTL mapping in experimental crosses},
  journal =      {Lab Animal},
  year =     {2001},
  OPTkey =   {},
  volume =   {30},
  number =   {7},
  pages =    {44--52},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@PhdThesis{Broman97,
  author =   {K. W. Broman},
  title =    {Identifying quantitative trait loci in experimental crosses},
  school =   {Department of Statistics, U.C. Berkeley},
  year =     {1997},
  OPTkey =   {},
  type =     {Ph.{D}. thesis},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Brown&Koplowitz79,
  author =   {T. A. Brown and J. Koplowitz},
  title =    {The weighted nearest neighbor rule for class dependent sample sizes},
  journal =      {IEEE Transactions on Information Theory},
  year =     {1979},
  OPTkey =   {},
  volume =   {25},
  number =   {5},
  pages =    {617--619},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Buhlmann&Yu,
  author =   {P. Buhlmann and B. Yu},
  title =    {Explaining Bagging.},
  journal =      {Annals of Statistics},
  year =     {(Accepted)},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTpages =     {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Burgessvm98,
  author =   {C. J. C. Burges},
  title =    {A tutorial on support vector machines for pattern recognition},
  journal =      {Data Mining and Knowledge Discovery},
  year =     {1998},
  OPTkey =   {},
  volume =   {2},
  number =   {},
  pages =    {121--167},
  month =    {December},
  OPTnote =      {},
  OPTannote =    {}
}



@article{Burman89,
AUTHOR={P. Burman},
TITLE={A comparative study of ordinary cross-validation, $v$-fold cross-validati
on and the repeated learning testing methods},
JOURNAL={Biometrika},
VOLUME={76},
YEAR={1989},
PAGES={503-514}
}





@TechReport{Buttrey&Karo02,
  author =   {S. E. Buttrey and C. Karo},
  title =    {Using k--neareset neighbor classification in the leaves of a tree},
  institution =  {Naval Postgraduate School, Monterey, CA},
  year =     {2002},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Calinskietal,
  author =   {R. Calinski and J. Harabasz},
  title =    {A dendrite method for cluster analysis},
  journal =      {Communications in Statistics},
  year =     {1974},
  OPTkey =   {},
  volume =   {3},
  OPTnumber =    {},
  pages =    {1--27},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Callowetal00,
  author =   {M. J. Callow and S. Dudoit and E. L. Gong and T. P. Speed and E. M. Rubin},
  title =    {Microarray expression profiling identifies genes with altered expression in {HDL} deficient mice},
  journal =      {Genome Research},
  year =     {2000},
  OPTkey =   {},
  volume =   {10},
  number =   {12},
  OPTmonth =     {},
  pages =    {2022--2029},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Chambers98,
   author = {J. M. Chambers},
   title = {Programming with Data: A Guide to the S Language},
   publisher = {Springer-Verlag New York},
   year = {1998}
}
@Book{Diggleetal2002,
   author = {Peter J. Diggle and P. Heagerty and K-Y Liang and S.L. Zeger},
   title = {Analysis of Longitudinal Data},
   publisher = {Oxford University Press},
   year = {2002 (Second Edition)}
}

@TechReport{ChangLin2001,
  author =       {C.-C. Chang and C.-J. Lin},
  title =        {LIBSVM: a Library for Support Vector Machines (Version 2.31)},
  institution =  {},
  year =         {2001},
  OPTkey =       {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  note =         {\\ {\tt http://www.csie.ntu.edu.tw/~cjlin/papers/libsvm2.ps.gz}},
  OPTannote =    {}
}



@Article{Changetal02,
  author =   {H. Y. Chang and J. T. Chi and S. Dudoit and C. Bondre and M. van de Rijn and D. Botstein D and P. O. Brown},
  title =    {Diversity, topographic differentiation, and positional memory in human fibroblasts},
  journal =      PNAS,
  year =     {2002},
  OPTkey =   {},
  volume =   {99},
  number =   {20},
  pages =    {12877--12882},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Chenetal02,
  author =   {X. Chen and S. T. Cheung and S. So and S. T. Fan and C. Barry and J. Higgins and K.-M. Lai and J. Ji and S. Dudoit and I. O. L. Ng and M. van de Rijn and D. Botstein and P. O. Brown },
  title =    {Gene expression patterns in human liver cancers},
  journal =      {Molecular Biology of the Cell},
  year =     {2002},
  OPTkey =   {},
  volume =   {13},
  number =   {6},
  pages =    {1929--1939},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Cleveland&Devlin88,
  author =   {W. S. Cleveland and S. J. Devlin},
  title =    {Locally-Weighted Regression: An Approach to Regression Analysis by Local Fitting},
  journal =      JASA,
  year =     {1988},
  OPTkey =   {},
  volume =   {83},
  OPTnumber =    {},
  pages =    {596--610},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Cleveland79,
  author =   {W. S. Cleveland},
  title =    {Robust locally weighted regression and smoothing scatterplots},
  journal =      JASA,
  year =     {1979},
  OPTkey =   {},
  volume =   {74},
  number =   {368},
  pages =    {829--836},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Correa&Wolfson99,
  author =   {J. A. Correa and D. B. Wolfson},
  title =    {Length-bias: some characterizations and applications},
  journal =      {Journal of Statistical Computation and Simulation},
  year =     {1999},
  OPTkey =   {},
  volume =   {64},
  Tnumber =      {3},
  pages =    {209--219},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Correaetal02,
  author =   {J. A. Correa and S. Dudoit and D. R. Goldstein},
  title =    {Multiple testing in the survival analysis of microarray data},
  OPTjournal =   {Statistics in Medicine},
  year =     {2002},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTpages =     {},
  OPTmonth =     {},
  note =     {(Submitted)},
  OPTannote =    {}
}


@Article{CortesVapnik95,
  author =   {C. Cortes and V. Vapnik},
  title =    {Support-vector networks},
  journal =      {Machine Learning},
  year =     {1995},
  OPTkey =   {},
  volume =   {20},
  number =   {},
  pages =    {273-297},
  month =    {December},
  OPTnote =      {},
  OPTannote =    {}
}

@InProceedings{Davies&Bouldin,
  author =   {D. Davies and D. Bouldin},
  title =    {A cluster separation measure},
  booktitle =    {IEEE Transactions on Pattern Analysis and Machine Intelligence},
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {224--227},
  year =     {1979},
  OPTeditor =    {},
  volume =   {1},
  OPTnumber =    {PAMI-1},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@article {Davis89,
AUTHOR ={R. B. Davis  and J. R. Anderson},
TITLE ={Exponential survival trees},
JOURNAL = {Statistics in Medicine},
VOLUME = {8},
YEAR ={1989},
NUMBER={},
PAGES = {947-961},
ISSN = {},
CODEN = {},
}




@InCollection{Day96,
  author =   {W. H. E. Day},
  title =    {Complexity theory: {A}n introduction for practitioners of classification},
  booktitle =    {Clustering and Classification},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher = {World Scientific Publishing Co.},
  year =     {1996},
  editor =   {P. Arabie and L. J. Hubert and G. De Soete},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {River Edge, NJ},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {199--233},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Dettling&Buhlmann02,
  author =   {M. Dettling and P. B\"{u}lmann},
  title =    {How to Use Boosting for Tumor Classification with Gene Expression Data},
  journal =      {},
  year =     {2002},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTpages =     {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Dudoit&Fridlyand02II,
  author =   {S. Dudoit and J. Fridlyand},
  title =    {Bagging to improve the accuracy of a clustering procedure},
  OPTjournal =   {Bioinformatics},
  year =     {2002},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTpages =     {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
  }



@InCollection{Dudoit&FridlyandCRC02,
  author =   {S. Dudoit and J. Fridlyand},
  title =    {Classification in microarray experiments},
  booktitle =    {Statistical Analysis of Gene Expression Microarray Data},
  OPTcrossref =  {},
  OPTkey =   {},
  OPTpages =     {},
  publisher =    {Chapman \& Hall/CRC},
  year =     {2002},
  editor =   {T. P. Speed},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTtype =      {},
  OPTchapter =   {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  note =     {(To appear)},
  OPTannote =    {}
}

@Article{Dudoit&FridlyandGenBio02,
  author =   {S. Dudoit and J. Fridlyand},
  title =    {A prediction-based resampling method to estimate the number of clusters in a dataset},
  journal =      {Genome Biology},
  year =     {2002},
  OPTkey =   {},
  volume =   {3},
  number =   {7},
  pages =    {0036.1--0036.21},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@TechReport{Dudoit&FridlyandTechRep600,
  author =   {S. Dudoit and J. Fridlyand},
  title =    {Applications of resampling methods to estimate the number of clusters and to improve the accuracy of a clustering method},
  institution =  {Department of Statistics, Uiversity of California, Berkeley},
  year =     {2001},
  OPTkey =   {},
  OPTtype =      {},
  number =   {600},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {},
  url={stat-www.berkeley.edu/users/sandrine/publications.html},
}

S. Dudoit, M.J. van der Laan (2005),
 Asymptotics of cross-validated
risk estimation in estimator selection and performance assessment.
{\em Statistical Methodology 2}, 2, 131--54.

@Article{Dudoit&vanderLaan05,
  author =   {S. Dudoit and M.J. van der Laan},
  title =    {Asymptotics of cross-validated risk estimation in estimator selection and performance assessment},
  journal =      {Statistical Methodology},
  year =     {2005},
  OPTkey =   {},
  volume =   {2},
  number =   {2},
  OPTmonth =     {},
  pages =    {131--154},
  OPTnote =      {www.bepress.com/ucbbiostat/paper126},
  OPTannote =    {}
}
@Article{Dudoit&SpeedAnnals99,
  author =   {S. Dudoit and T. P. Speed},
  title =    {A score test for linkage using identity by descent data from sibships},
  journal =      {Annals of Statistics},
  year =     {1999},
  OPTkey =   {},
  volume =   {27},
  number =   {3},
  OPTmonth =     {},
  pages =    {943--986},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Dudoit&SpeedBios00,
  author =   {S. Dudoit and T. P. Speed},
  title =    {A score test for the linkage analysis of qualitative and quantitative traits based on identity by descent data on sib-pairs},
  journal =      {Biostatistics},
  year =     {2000},
  OPTkey =   {},
  volume =   {1},
  number =   {1},
  pages =    {1--26},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}




@InCollection{Dudoit&SpeedIMA99,
  author =   {S. Dudoit and T. P. Speed},
  title =    {Triangle constraints for sib-pair identity by descent probabilities under a general multilocus model for disease susceptibility},
  booktitle =    {Statistics in Genetics},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher =    {Springer-Verlag},
  year =     {1999},
  editor =   {M. E. Halloran and S. Geisser},
  volume =   {112},
  OPTnumber =    {},
  series =   {IMA Volumes in Mathematics and its Applications},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {New York},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {181--221},
  OPTnote =      {},
  OPTannote =    {}
}

@InCollection{Dudoit&YangSpringer03,
  author =   {S. Dudoit and Y. H. Yang},
  title =    {Bioconductor {R} packages for exploratory analysis and normalization of c{DNA} microarray data},
  booktitle =    {The Analysis of Gene Expression Data: Methods and Software},
  OPTcrossref =  {},
  OPTkey =   {},
  OPTpages =     {},
  publisher =    {Springer, New York},
  year =     {2003},
  editor =   {G. Parmigiani and E. S. Garrett and R. A. Irizarry and S. L. Zeger},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTtype =      {},
  OPTchapter =   {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{DudoitetalJASA02,
  author =       {S. Dudoit and J. Fridlyand and T. P. Speed},
  title =        {Comparison of Discrimination Methods for the Classification of
 Tumors Using Gene Expression Data},
  journal =      JASA,
  year =         {2002},
  OPTkey =       {},
  volume =    {97},
  number =    {457},
  pages =     {77--87},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{DudoitetalSinica02,
  author =   {S. Dudoit and Y. H. Yang and M. J. Callow and T. P. Speed},
  title =    {Statistical methods for identifying differentially expressed genes in replicated c{DNA} microarray experiments},
  journal =      {Statistica Sinica},
  year =     {2002},
  OPTkey =   {},
  volume =   {12},
  number =   {1},
  pages =    {111--139},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{DudoitetalTechRep110,
  author =   {S. Dudoit and J. P. Shaffer and J. C. Boldrick},
  title =    {Multiple hypothesis testing in microarray experiments},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =     {2002},
  OPTkey =   {},
  OPTtype =      {},
  number =   {110},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {},
  url={www.bepress.com/ucbbiostat/paper110/}

}


@Article{Duffy&Quiroz,
  author =   {D. E. Duffy and A. J. Quiroz},
  title =    {A permutation-based algorithm for block clustering},
  journal =      {Journal of Classification},
  year =     {1991},
  OPTkey =   {},
  volume =   {8},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {65--91},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Dunn58,
  author =   {O. J. Dunn},
  title =    {Estimation of the means of dependent variables},
  journal =      {Annals of Mathematical Statistics},
  year =     {1958},
  OPTkey =   {},
  volume =   {29},
  OPTnumber =    {},
  pages =    {1095-111},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Book{Efron&Tibs93,
  author =   {B. Efron and R. J. Tibshirani},
  ALTeditor =    {},
  title =    {An Introduction to the Bootstrap},
  publisher =    {Chapman \& Hall/CRC},
  year =     {1993},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{EfronetalJASA01,
  author =   {B. Efron and R. Tibshirani and J. D. Storey and V. Tusher},
  title =    {Empirical Bayes analysis of a microarray
experiment},
  journal =      JASA,
  year =     {2001},
  OPTkey =   {},
  volume =   {96},
  OPTnumber =    {},
  pages =    {1151--1160},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@TechReport{EfronetalTechRep01,
  author =   {B. Efron and J. D. Storey and R. Tibshirani},
  title =    {Microarrays, empirical Bayes methods, and false discovery
rates},
  institution =  {Department of Statistics, Stanford University},
  year =     {2001},
  OPTkey =   {},
  OPTtype =      {},
  number =   {2001-218},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Finner99,
  author =   {H. Finner},
  title =    {Stepwise multiple test procedures and control of directional errors},
  journal =      {Annals of Statistics},
  year =     {1999},
  OPTkey =   {},
  volume =   {27},
  OPTnumber =    {},
  pages =    {274--289},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Fisher,
  author =   {R. A. Fisher},
  title =    {The use of multiple measurements in taxonomic problems},
  journal =      {Annals of Eugenics},
  year =     {1936},
  OPTkey =   {},
  volume =   {7},
  OPTnumber =    {},
  pages =    {179-188},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Fisher26,
  author =   {R. A. Fisher},
  title =    {The arrangement of field experiments},
  journal =      {J. Min. Agric. Gr. Br},
  year =     {1926},
  OPTkey =   {},
  volume =   {33},
  OPTnumber =    {},
  pages =    {505--513},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{Fix&Hodges,
  author =   {E. Fix and J. Hodges},
  title =    {Discriminatory analysis, nonparametric discrimination: consistency properties},
  institution =  {Randolph Field, Texas: USAF School of Aviation Medicine},
  year =     {1951},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Fowlkes&Mallows83,
  author =   {E. B. Fowlkes and C. L. Mallows},
  title =    {A method for comparing two hierarchical clusterings},
  journal =      JASA,
  year =     {1983},
  OPTkey =   {},
  volume =   {78},
  OPTnumber =    {383},
  OPTmonth =     {},
  pages =    {553--584},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Fowlkesetal88,
  author =   {E. B. Fowlkes and R. Gnanadesikan and J. R. Kettenring},
  title =    {Variable selection in clustering},
  journal =      JC,
  year =     {1988},
  OPTkey =   {},
  volume =   {5},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {205--228},
  OPTnote =      {},
  OPTannote =    {}
}

@TechReport{Fraley&Raftery98,
  author =   {C. Fraley and A. Raftery},
  title =    {How many clusters? Which clustering method? -- answers via model-based cluster analysis},
  institution =  {Department of Statistics, University of Washington},
  year =     {1998},
  OPTkey =   {},
  OPTtype =      {},
  number =   {329},
  OPTaddress =   {},
  OPTmonth =     {},
  note =     {\url{http://www.stat.washington.edu/www/research/reports/1990s/#1998}},
  OPTannote =    {}
}




@Article{Freund&Schapire97,
  author =   {Y. Freund and R. E. Schapire},
  title =    {A decision-theoretic generalization of on-line learning and an application to boosting},
  journal =      {Journal of Computer and System Sciences},
  year =     {1997},
  OPTkey =   {},
  volume =   {55},
  OPTnumber =    {},
  pages =    {119--139},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@PhdThesis{Fridlyand,
  author =   {J. Fridlyand},
  title =    {Resampling methods for variable selection and classification: applications to genomics},
  school =   {Department of Statistics, U.C. Berkeley},
  year =     {2001},
  OPTkey =   {},
  type =     {Ph.{D}. thesis},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{Friedman94 ,
  author =   {J. H. Friedman},
  title =    {Flexible metric nearest neighbor clasification},
  institution =  {Department of Statistics, Stanford University},
  year =     {1994},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@TechReport{Friedman96a,
  author =   {J. H. Friedman},
  title =    {On bias, variance, 0/1-loss, and the curse--of--dimensionality },
  institution =  {Department of Statistics, Stanford University},
  year =     {1996},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{Friedman96b,
  author =   {J. H. Friedman},
  title =    {Another approach to polychotomous classification},
  institution =  {Department of Statistics, Stanford University},
  year =     {1996},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Friedmanetal00,
  author =   {J. Friedman and T. Hastie and R. Tibshirani},
  title =    {Additive logistic regression: a statistical view of boosting},
  journal =      {Annals of Statistics},
  year =     {2000},
  OPTkey =   {},
  volume =   {28},
  OPTnumber =    {},
  pages =    {337--404},
  OPTmonth =     {},
  note =     {(with discussion)},
  OPTannote =    {}
}

@book {GAM,
   AUTHOR = {T. J. Hastie and R.J. Tibshirani},
    TITLE = {Generalized Additive Models},
PUBLISHER = {Chapman and Hall},
  ADDRESS = {London},
     YEAR = {1990},
    PAGES = {},
     ISBN = {},
}



@Article{Gabriel,
  author =   {K. R. Gabriel},
  title =    {The biplot graphic display of matrices with application to principal component analysis},
  journal =      {Biometrika},
  year =     {1971},
  OPTkey =   {},
  volume =   {58},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {453--467},
  OPTnote =      {},
  OPTannote =    {}
}

@InCollection{Gabriel75,
  author =   {K. R. Gabriel},
  title =    {A comparison of some methods of simultaneous inference in {MANOVA}},
  booktitle =    {Multivariate Statistical Methods: Among-groups covariation; Within-group covariation},
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {61--80},
  OPTpublisher = {},
  year =     {1975},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTtype =      {},
  OPTchapter =   {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@InProceedings{GabrielPun,
  author =       {K. R. Gabriel and F. C. Pun},
  title =        {Binary prediction of weather events with several predictors},
  booktitle =    {Sixth Conference on Probability and Statistics in Atmospheric Science},
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {248--253},
  year =     {1979},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  organization = {American Meterological Society},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}


@Unpublished{Ge&Dudoit,
  author =   {Y. Ge and S. Dudoit},
  title =    {Fast algorithm for resampling-based $p$-value adjustment in multiple testing},
  note =     {(In preparation)},
  OPTkey =   {},
  OPTmonth =     {},
  year =     {2002},
  OPTannote =    {}
}

@Article{Geisser75,
  author =   {S. Geisser},
  title =    {The predictive sample reuse method with applications},
  journal =      {Journal of the American Statistical Association},
  year =     {1975},
  volume =   {70},
  pages =    {320-328}
}

@TechReport{Genovese&Wasserman01,
  author =   {C. Genovese and L. Wasserman},
  title =    {Operating Characteristics and Extensions of the FDR Procedure},
  institution =  {Department of Statistics, Carnegie Mellon},
  year =     {2001},
  OPTkey =   {},
  OPTtype =      {},
  number =   {737},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Gnanadesikan&Kettering95,
  author =   {R. Gnanadesikan and J. R. Kettenring},
  title =    {Weighting and selection of variables for cluster analysis},
  journal =      JC,
  year =     {1995},
  OPTkey =   {},
  volume =   {12},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {113--136},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{GoldsteinetalGenEpi00,
  author =   {D. R. Goldstein and S. Dudoit and T. P. Speed},
  title =    {Power of a score test for quantitative trait linkage analysis of relative pairs.},
  journal =      {Genetic Epidemiology},
  year =     {2000},
  OPTkey =   {},
  volume =   {19},
  number =   {Suppl. 1},
  pages =    {S85--S91},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{GoldsteinetalGenEpi01,
  author =   {D. R. Goldstein and S. Dudoit and T. P. Speed},
  title =    {Power and robustness of a score  test for linkage analysis of quantitative traits using identity by descent data on sib pairs},
  journal =      {Genetic Epidemiology},
  year =     {2001},
  OPTkey =   {},
  volume =   {20},
  number =   {4},
  pages =    {415--431},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@article {Gordon85,
AUTHOR ={L. Gordon and R.A. Olshen},
TITLE ={Tree-structured survival analysis},
JOURNAL = {Cancer Treatment Reports},
VOLUME = {69},
YEAR ={1985},
NUMBER={},
PAGES = {10065-1069},
ISSN = {},
CODEN = {},
}



@InCollection{Gordon96,
  author =   {A. D. Gordon},
  title =    {Hierarchical classification},
  booktitle =    {Clustering and Classification},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher = {World Scientific Publishing Co.},
  year =     {1996},
  editor =   {P. Arabie and L. J. Hubert and G. De Soete},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {River Edge, NJ},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {65--121},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Gower&Hand,
  author = {J. C. Gower and D. J. Hand},
  title =    {Biplots},
  publisher =    {Chapman \& Hall},
  year =     {1996},
  OPTkey =   {},
  OPTeditor =    {},
  OPTvolume =    {},
  number =   {54},
  series =   {Monographs on statistics and applied probability},
  OPTaddress =   {},
  edition =      {1st},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@book {Gyorfi02,
   AUTHOR = {L. Gy\"{o}rfi and M. Kohler and A. Krzy\.{z}ak  and H. Walk},
    TITLE = {A Distribution-Free Theory of Nanparametric Regression},
PUBLISHER = {Springer-Verlag},
  ADDRESS = {New York},
     YEAR = {2002},
    PAGES = {100-102},
     ISBN = {}
}




@Book{Gyorfietal02,
  author =   {L. Gy\"orfi and M. Kohler and A. Krzy\'{z}ak and H. Walk},
  ALTeditor =    {},
  title =    {A distribution-free theory of nonparametric regression},
  publisher =    {Springer-Verlag, New York},
  year =     {2002},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Book{HTF01,
  author =   {T. Hastie and R. Tibshirani and J. H. Friedman},
  ALTeditor =    {},
  title =    {The Elements of Statistical Learning : Data Mining, Inference, and Prediction },
  publisher =    {Springer Verlag},
  year =     {2001},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Hansen01,
  author =   {M. H. Hansen  and B. Yu},
  title =    {Model selection and the principle of minimum description length},
  journal =      {Journal of the American Statistical Association},
  year =     {2001},
  volume =   {96},
  pages =    {746-774}
}

@Article{Hardle85a,
  author =   {W. H{\"a}rdle and J. S. Marron},
  title =    {Asymptotic nonequivalence of some bandwidth selectors in nonparametric regression},
  journal =      {Biometrika},
  year =     {1985},
  volume =   {72},
  pages =    {481--484}
}




@Article{Hardle85b,
  author =   {W. H{\"a}rdle and J. S. Marron},
  title =    {Optimal bandwidth selection in nonparametric regression function estimation},
  journal =      {Annals of Statistics},
  year =     {1985},
  volume =   {13},
  pages =    {1465-1481}
}

@Book{Hardle93,
  author =       {W. H{\"a}rdle},
  title =        {Applied Nonparametric Regression},
  publisher =    {Cambridge University Press},
  pages = {},
  year =         {1993}
}

@Article{Hartigan72,
  author =   {J. A. Hartigan},
  title =    {Direct clustering of a data matrix},
  journal =      {Journal of the American Statistical Association},
  year =     {1972},
  OPTkey =   {},
  volume =   {67},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {123--129},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Hartigan75,
  author =   {J. A. Hartigan},
  title =    {Clustering Algorithms},
  publisher =    {Wiley},
  year =     {1975},
  OPTkey =   {},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Hartigan78,
  author =   {J. Hartigan},
  title =    {Asymptotic distributions for clustering criteria},
  journal =      {Annals of Statistics},
  year =     {1978},
  OPTkey =   {},
  volume =   {6},
  OPTnumber =    {},
  pages =    {117--131},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Hartigan85,
  author =   {J. A. Hartigan},
  title =   {Statistical theory in clustering} ,
  journal =      JC,
  year =     {1985},
  OPTkey =   {},
  volume =   {2},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {63--76},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Hastie&Tibshirani96a,
  author =   {T. Hastie and R. Tibshirani},
  title =    {Discriminant adaptive nearest-nieghbor classification},
  journal =      {IEEE Pattern Recognition and Machine Intelligence},
  year =     {1996},
  OPTkey =   {},
  volume =   {18},
  OPTnumber =    {},
  pages =    {607--616},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{Hastie&Tibshirani96b,
  author =   {T. Hastie and R. Tibshirani},
  title =    {Classification by pairwise coupling},
  institution =  {Department of Statistics, Stanford University},
  year =     {1996},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@article {Hastie90,
   AUTHOR = {T.J. Hastie and  R.J. Tibshirani},
    TITLE = {Exploring the nature of covariate effects in the proportional hazar
ds model},
  JOURNAL = {Biometrics},
   VOLUME = {46},
     YEAR = {1990},
   NUMBER = {4},
    PAGES = {1005-1016},
     ISSN = {},
    CODEN = {},
}


@Book{Hochberg&Tamhane,
  author =   {Y. Hochberg and A. C. Tamhane},
  ALTeditor =    {},
  title =    {Multiple Comparison Procedures},
  publisher =    {Wiley--Interscience},
  year =     {1987},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  series =   {Probability and Mathematical Statistics},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Hochberg88,
  author =   {Y. Hochberg},
  title =    {A sharper Bonferroni procedure for multiple tests of significance},
  journal =      {Biometrika},
  year =     {1988},
  OPTkey =   {},
  volume =   {75},
  OPTnumber =    {},
  pages =    {800--802},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Holm79,
  author =   {S. Holm},
  title =    {A simple sequentially rejective multiple test procedure},
  journal =      {Scand. J. Statist.},
  year =     {1979},
  OPTkey =   {},
  volume =   {6},
  OPTnumber =    {},
  pages =    {65--70},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Hommel&Bernhard99,
  author =   {G. Hommel and G. Bernhard},
  title =    {Bonferroni procedures for logically related hypotheses},
  journal =      {Journal of Statistical Planning and Inference},
  year =     {1999},
  OPTkey =   {},
  volume =   {82},
  OPTnumber =    {},
  pages =    {119--128},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Hommel88,
  author =   {G. Hommel},
  title =    {A stagewise rejective multiple test procedure based on a modified Bonferroni test},
  journal =      {Biometrika},
  year =     {1988},
  OPTkey =   {},
  volume =   {75},
  OPTnumber =    {},
  pages =    {383--386},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Hubert&Arabie85,
  author =   {L. Hubert and P. Arabie},
  title =    {Comparing partitions},
  journal =      JC,
  year =     {1985},
  OPTkey =   {},
  volume =   {2},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {193--218},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Jain&DubesBook,
  author =   {A. K. Jain and R. C. Dubes},
  editor =   {},
  title =    {Algorithms for Clustering Data},
  publisher =    {Prentice-Hall},
  year =     {1988},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {Englewood Cliffs, N. J.},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Jogdeo77,
  author =   {K. Jogdeo},
  title =    {Association and probability inequalities},
  journal =      {Annals of Statistics},
  year =     {1977},
  OPTkey =   {},
  volume =   {5},
  OPTnumber =    {},
  pages =    {495--504},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Kaufman&Rousseeuw90,
  author =   {L. Kaufman and P. J. Rousseeuw},
  ALTeditor =    {},
  title =    {Finding Groups in Data: An Introduction to Cluster Analysis},
  publisher =    {Wiley, New York.},
  year =     {1990},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@article {Keles03,
AUTHOR ={Kele\c{s}, S. and van der Laan, M. and Dudoit,  S.},
TITLE ={Asymptotically Optimal  Model Selection Method for Regression on Censored Outcomes },
JOURNAL = {Technical Report, Division of Biostatistics, UC Berkeley},
VOLUME = {},
YEAR ={2002},
PAGES = {},
ISSN = {},
CODEN = {},
}



@Article{Kohonen90,
  author =   {T. Kohonen},
  title =    {The self-organizing map},
  journal =      {Proc. IEEE},
  year =     {1990},
  OPTkey =   {},
  volume =   {78},
  number =   {9},
  OPTmonth =     {},
  pages =    {1464--1480},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Kohonen95,
  author =   {T. Kohonen},
  title =    {Self-Organizing Maps},
  publisher =    {Springer},
  year =     {1995},
  OPTkey =   {},
  editor =   {T. S. Huang and T. Kohonen and M. R. Schroeder},
  volume =   {30},
  OPTnumber =    {},
  series =   {Springer Series in Information Sciences},
  address =      {Berlin, Heidelberg},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@article {Kooperberg95,
AUTHOR ={C. Kooperberg and C.J.  Stone and Y. K.  Truong},
TITLE ={Hazard Regression},
JOURNAL = {Journal of the American Statistical Association},
VOLUME = {90},
YEAR ={1995},
NUMBER={429},
PAGES = {78-94},
ISSN = {},
CODEN = {},
}



@Article{Koutsoukosetal,
  author =   {A. D. Koutsoukos and L. V. Rubinstein and D. Faraggi and R.M. Simon and S. Kalyandrug and J. N. Weinstein and K.W. Kohn and K.D. Paull},
  title =    {Discrimination techniques applied to the {NCI} in vitro anti-tumor drug screen: predicting biochemical mechanism of action},
  journal =      {Statistics in Medicine},
  year =     {1994},
  OPTkey =   {},
  volume =   {13},
  OPTnumber =    {},
  pages =    {719--730},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Krishnaiah&Reising85,
  author =   {P. R. Krishnaiah and J. M. Reising},
  title =    {Multivariate multiple comparisons},
  journal =      {Encyclopedia of Statistical Sciences},
  year =     {1985},
  OPTkey =   {},
  volume =   {9},
  number =   {6},
  pages =    {88--95},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Krzanowski&Lai,
  author =   {W. Krzanowski and Y. Lai },
  title =    {A criterion for determining the number of groups in a dataset using sum of squares clustering},
  journal =      {Biometrics},
  year =     {1985},
  OPTkey =   {},
  volume =   {44},
  OPTnumber =    {},
  pages =    {23--34},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Laan&Bryan01,
  author =   {M. J. van der Laan and J. Bryan},
  title =    {Gene expression analysis with the parametric bootstrap},
  journal =      {Biostatistics},
  year =     {2001},
  OPTkey =   {},
  volume =   {2},
  number =   {4},
  pages =    {445--461},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Pollard&vanderLaan04,
  author =   {K. S. Pollard and M.J. van der Laan},
  title =    {Choice of Null Distribution in Resampling Based Multiple Testing},
  journal =      JSPI,
  year =     {2004},
  OPTkey =   {},
  OPTvolume =    {125},
  OPTnumber =    {},
  OPTpages =     {85--101},
  OPTmonth =     {},
  note =     {},
  OPTannote =    {}
}


@Article{Laan&PollardJSPI02,
  author =   {M. J. van der Laan and K. S. Pollard},
  title =    {Hybrid clustering of gene expression data with visualization and the bootstrap},
  journal =      JSPI,
  year =     {2002},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTpages =     {},
  OPTmonth =     {},
  note =     {(To appear)},
  OPTannote =    {}
}


@article {Leblanc92,
AUTHOR ={M. Leblanc and J. Crowley},
TITLE ={Relative Risk trees for censored data},
JOURNAL = {Biometrics},
VOLUME = {48},
YEAR ={1992},
NUMBER={},
PAGES = {411-425},
ISSN = {},
CODEN = {},
}





@InProceedings{Leisch02,
  author =   {F. Leisch},
  title =    {Sweave: Dynamic Generation of Statistical Reports Using
                  Literate Data Analysis},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle = {Compstat 2002 --- Proceedings in Computational
                  Statistics},
  Tpages =   {575--580},
  year =     {2002},
  editor =   {Wolfgang H{\"a}rdle and Bernd R{\"o}nz},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  publisher = {Physika Verlag, Heidelberg, Germany},
  note =     {ISBN 3-7908-1517-9},
  OPTannote =    {},
  url =      {http://www.ci.tuwien.ac.at/~leisch/Sweave}
}

@TechReport{Leisch02TR,
  author =   {F. Leisch},
  title =    {Dynamic generation of statistical reports using literate data analysis},
  institution =  {SFB Adaptive Information Systems and Modelling in Economics and Management
Science, Vienna University of Economics and Business Administration},
  year =     {2002},
  OPTkey =   {},
  OPTtype =      {},
  number =   {69},
  OPTaddress =   {},
  month =    {March},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{Leisch99,
  author =   {F. Leisch},
  title =    {Bagged clustering},
  institution =  {SFB Adaptive Information Systems and Modelling in Economics and Management Science, Vienna University of Economics and Business Administration},
  year =     {1999},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  month =    {August},
  note =     {\url{http://www.ci.tuwien.ac.at/~leisch/papers/fl-techrep.html}},
  OPTannote =    {}
}

@Article{Limetal00,
  author =   {T-S Lim and W-Y Loh and Y-S Shih},
  title =    {A comparison of prediction accuracy, complexity, and training time of thiry-three old and new classification algorithms},
  journal =      {Machine Learning},
  year =     {2000},
  OPTkey =   {},
  volume =   {40},
  OPTnumber =    {},
  pages =    {203--229},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Book{Mardiaetal,
  author =   {K. V. Mardia and J. T. Kent and J. M. Bibby},
  title =    {Multivariate Analysis},
  publisher =    {Academic Press, Inc.},
  year =     {1979},
  OPTkey =   {},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {San Diego},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Unpublished{Mayo&Spanos02,
  author =       {D. C. Mayo and A. Spanos},
  title =        {A severe-testing interpretation of {N}eyman-{P}earson methods.  Unpublished manuscript},
  OPTnote =         {},
  OPTkey =       {},
  OPTmonth =     {},
  year =         {2002},
  OPTannote =    {}
}


@Book{McCullagh&Nelder89,
  author =   {P. McCullagh and J. A. Nelder},
  ALTeditor =    {},
  title =    {Generalized Linear Models},
  publisher =    {Chapman \& Hall},
  year =     {1989},
  OPTkey =   {},
  OPTvolume =    {},
  number =   {37},
  series =   {Monographs on Statistics and Applied Probability},
  OPTaddress =   {},
  edition =      {2nd},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Book{McLachlan,
  author =   {G. J. McLachlan},
  OPTeditor =    {},
  title =    {Discriminant analysis and statistical pattern recognition},
  publisher =    {Wiley},
  year =     {1992},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {New York},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{McLachlanetal01,
  author =   {G. J. McLachlan and R. Bean and D. Peel},
  title =    {A mixture model-based approach to the clustering of microarray expression data.},
  journal =      {Bioinformatics},
  year =     {2002},
  OPTkey =   {},
  volume =   {18},
  OPTnumber =    {},
  pages =    {413--422},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{MillerSubsets,
  author =   {A. J. Miller},
  OPTeditor =    {},
  title =    {Subset Selection in Regression},
  publisher =    {Chapman and Hall},
  year =     {1990},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Milligan&Cooper85,
  author =   {G. W. Milligan and M. C. Cooper},
  title =    {An examination of procedures for determining the number of clusters in a data set},
  journal =      {Psychometrika},
  year =     {1985},
  OPTkey =   {},
  volume =   {50},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {159--179},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Milligan&Cooper86,
  author =   {G. W. Milligan and M. C. Cooper},
  title =    {A study of the comparability of external criteria for hierarchical cluster analysis},
  journal =      {Multivariate Behavioral Research},
  year =     {1986},
  OPTkey =   {},
  volume =   {21},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {441--458},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Milligan&Cooper87,
  author =   {G. W. Milligan and M. C. Cooper},
  title =    {Methodology review: {C}lustering methods},
  journal =      {Applied Psychological Measurement},
  year =     {1987},
  OPTkey =   {},
  volume =   {11},
  OPTnumber =    {4},
  OPTmonth =     {December},
  pages =    {329--354},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Milligan89,
  author =   {G. W. Milligan},
  title =    {A study of the beta-flexible clustering method},
  journal =      {Multivariate Behavioral Research},
  year =     {1989},
  OPTkey =   {},
  volume =   {24(2)},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {163--176},
  OPTnote =      {},
  OPTannote =    {}
}


@InCollection{Milligan96,
  author =   {G. W. Milligan},
  title =    {Clustering validation: {R}esults and implications for applied analyses},
  booktitle =    {Clustering and Classification},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher = {World Scientific Publishing Co.},
  year =     {1996},
  editor =   {P. Arabie and L. J. Hubert and G. De Soete},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {River Edge, NJ},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {341--375},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Moreyetal83,
  author =   {L. C. Morey, R. K. Blashfield and H. A. Skinner},
  title =    {A comparison of cluster analysis techniques within a sequential validation framework},
  journal =      {Multivariate Behavioral Research},
  year =     {1983},
  OPTkey =   {},
  volume =   {18},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {309--329},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Morrison90,
  author =   {D. F. Morrison},
  ALTeditor =    {},
  title =    {Multivariate Statistical Methods},
  publisher =    {McGraw-Hill, NY},
  year =     {1990},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  edition =      {3rd},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@InCollection{Murtagh96,
  author =   {F. Murtagh},
  title =    {Neural networks for clustering},
  booktitle =    {Clustering and Classification},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher = {World Scientific Publishing Co.},
  year =     {1996},
  editor =   {P. Arabie and L. J. Hubert and G. De Soete},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {River Edge, NJ},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {235--269},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{PanelDACC,
  author =   {{Panel on Discriminant Analysis, Classification, and Clustering}},
  title =    {Discriminant analysis and clustering},
  journal =      {Statistical Science},
  year =     {1989},
  OPTkey =   {},
  volume =   {4},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {34--69},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{Pavlic&vanderLaanTechRep89,
  author =   {M. Pavlic and M. J. van der Laan},
  title =    {Fitting of mixtures with unspecified number of components using cross-validation distance estimate},
  institution =  {Division of Biostatistics, U.C. Berkeley},
  year =     {2001},
  OPTkey =   {},
  OPTtype =      {},
  number =   {89},
  OPTaddress =   {},
  month =    {February},
  OPTnote =      {},
  OPTannote =    {}
}

@article{Pavlic02,
author  = {M. Pavlic and M. J. van der Laan},
title   = {Fitting of mixtures with unspecified number of components using
cross validation distance estimate},
journal = {Computational Statistics and Data Analysis},
volume  = {41},
issue   = {3-4},
pages   = {413-428},
year    = {2003}
}



@TechReport{Pollard&LaanTechRep107,
  author =   {K. S. Pollard and M. J. van der Laan},
  title =    {A Method to Identify Significant Clusters in Gene Expression Data},
  institution =  {Division of Biostatistics, U.C. Berkeley},
  year =     {2002},
  OPTkey =   {},
  OPTtype =      {},
  number =   {107},
  OPTaddress =   {},
  month =    {April},
  OPTnote =      {},
  OPTannote =    {}
}

@TechReport{Pollard&LaanTechRep121,
  author =   {K. S. Pollard and M. J. van der Laan},
  title =    {Resampling-based methods for identification of significant subsets of genes in expression data},
  institution =  {Division of Biostatistics, U.C. Berkeley},
  year =     {2002},
  OPTkey =   {},
  OPTtype =      {},
  number =   {121},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Ramsey78,
  author =   {P. H. Ramsey},
  title =    {Power differences between pairwise multiple comparisons},
  journal =      JASA,
  year =     {1978},
  OPTkey =   {},
  volume =   {73},
  OPTnumber =    {},
  pages =    {479--485},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Manual{RanForests,
  title =    {Notes on setting up, using, and understanding random forests V3.0},
  OPTkey =   {},
  author =   {L. Breiman},
  OPTorganization = {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  year =     {2001},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Rand,
  author =   {W. M. Rand},
  title =    {Objective criteria for the evaluation of clustering methods},
  journal =      {Journal of the American Statistical Association},
  year =     {1971},
  OPTkey =   {},
  volume =   {66},
  OPTnumber =    {336},
  OPTmonth =     {},
  pages =    {846--850},
  OPTnote =      {},
  OPTannote =    {}
}

@Unpublished{Reineretal01,
  author =   {A. Reiner and D. Yekutieli and Y. Benjamini},
  title =    {Using resampling-based {FDR} controlling multiple test procedures for analyzing microarray gene expression data},
  OPTnote =      {},
  OPTkey =   {},
  OPTmonth =     {},
  year =     {2001},
  OPTannote =    {}
}


@Book{Ripley96,
  author =   {B. D. Ripley},
  title =    {Pattern recognition and neural networks},
  publisher =    {Cambridge University Press},
  year =     {1996},
  OPTkey =   {},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {Cambridge, New York},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}




%very first reference to use trees in survival analysis
@Article{Rissanen78,
  author =   {J. Rissanen},
  title =    {Modelling by shortest data description},
  journal =      {Automatica},
  year =     {1978},
  volume =   {14},
  pages =    {465-471}
}

@Article{Rnews:Dudoit+Yang+Bolstad:2002,
  author       = {S. Dudoit and Y. H.  Yang and B. Bolstad},
  title        = {Using {R} for the Analysis of {DNA} Microarray Data},
  journal      = {R News},
  year         = 2002,
  volume       = 2,
  number       = 1,
  pages        = {24--32},
  month        = {March},
  url          = {CRAN.R-project.org/doc/Rnews/}
}

@article {Robins00a,
AUTHOR ={J. M. Robins and A.  Rotnitzky},
TITLE ={Comment on the {B}ickel and {K}won article, ``{I}nference for semiparametric models: {S}ome questions and an answer''},
JOURNAL = {Statistica Sinica},
VOLUME = {11},
NUMBER={4},
YEAR ={2001},
PAGES = {920-936},
ISSN = {},
CODEN = {}
}


@InProceedings{Robins00c,
  author =   {J.M. Robins},
  title =    {Robust estimation in sequentially ignorable
missing data and causal inference models},
  booktitle =    {Proceedings of the American
Statistical Association},
  pages =    {},
  year =     {2000},
  editor =   {},
  organization = {}
}


@article {Robins00b,
AUTHOR ={J. M. Robins and A.  Rotnitzky and M.J. van der Laan},
TITLE ={Comment on ``{O}n {P}rofile {L}ikelihood" by {S}.{A}. {M}urphy and
{A}.{W}. van der {V}aart},
JOURNAL = {Journal of the American Statistical Association -- Theory and
Methods
},
VOLUME = {450},
YEAR ={2000},
PAGES = {431-435},
ISSN = {},
CODEN = {}
}



@Article{Birge83,
  author =   {L. Birg{\'e}},
  title =    {Approximation dans les espaces m{/'e}triques et th{\'e}orie
  de l'estimation},
  journal =      {Verw. Gebiete},
  year =     {1983},
  OPTkey =   {},
  volume =   {65},
  number =   {},
  OPTmonth =     {},
  pages =    {181--238},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{lecam73,
  author =   {L.M. le Cam},
  title =    {Convergence of estimates under dimensionality restrictions},
  journal =      {Annals of Statistics},
  year =     {1973},
  OPTkey =   {},
  volume =   {22},
  number =   {},
  OPTmonth =     {},
  pages =    {38--53},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Rom90,
  author =   {D. M. Rom},
  title =    {A sequentially rejective test procedure based on a modified {Bonferroni} inequality},
  journal =      {Biometrika},
  year =     {1990},
  OPTkey =   {},
  volume =   {77},
  OPTnumber =    {},
  pages =    {663-665},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{Rosenblatt57,
  author =       {F. Rosenblatt},
  title =        {The perceptron -- a perceiving and recognizing automation},
  institution =  {Cornell Aeronautical Laboratory },
  year =         {1957},
  OPTkey =       {},
  OPTtype =      {},
  number =       {86-460-1},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Ruczinskietal,
  author =   {I. Ruczinski and C. Kooperberg and M. LeBlanc},
  title =    {Logic regression},
  journal =      {},
  year =     {2001},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTpages =     {},
  OPTmonth =     {},
  note =     {Submitted, \url{http://biosun01.biostat.jhsph.edu/~iruczins/html/publications.html}},
  OPTannote =    {}
}

@Article{Saltstone&Stange,
  author =   {R. Saltstone and K. Stange},
  title =    {A computer program to calculate Hubert and Arabie's adjusted Rand index},
  journal =      {Journal of Classification},
  year =     {1996},
  OPTkey =   {},
  volume =   {13},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {169--172},
  OPTnote =      {},
  OPTannote =    {}
}
@TechReport{vanderVaart03,
  author =   {A.W. van der Vaart},
  title =    {Notes on Cross-validation},
  institution =  {Department of Mathematics, Free University, Amsterdam},
  year =     {2003},
  OPTkey =   {},
  OPTtype =      {},
  number =   {},
  OPTaddress =   {},
  OPTmonth =     {},
  note =     {},
  OPTannote =    {Unpublished manuscript}
}

@TechReport{Sarle,
  author =   {W. Sarle},
  title =    {Cubic clustering criterion},
  institution =  {SAS Institute, Inc.},
  year =     {1983},
  OPTkey =   {},
  OPTtype =      {},
  number =   {A-108},
  OPTaddress =   {},
  OPTmonth =     {},
  note =     {\url{http://www.sas.com/service/library/onlinedoc/trindex.html}},
  OPTannote =    {}
}

@TechReport{Sarle&Kuo,
  author =   {W. Sarle and A. Kuo},
  title =    {The MODECLUS Procedures},
  institution =  {SAS Institute, Inc.},
  year =     {1993},
  OPTkey =   {},
  OPTtype =      {},
  number =   {P-256},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Schapireetal,
  author =   {R. E. Schapire and Y. Freund and P. Bartlett and W. S. Lee},
  title =    {Boosting the margin: a new explanation for the effectiveness of voting methods},
  journal =      {Annals of Statistics},
  year =     {1998},
  OPTkey =   {},
  volume =   {26},
  OPTnumber =    {},
  pages =    {1651--1686},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Book{Scheffe,
  author =   {H. Scheff\'{e}},
  ALTeditor =    {},
  title =    {The analysis of variance},
  publisher =    {John Wiley \& Sons},
  year =     {1959},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Scheibler&Schneider,
  author =   {D. Scheibler and W. Schneider},
  title =    {Monte Carlo tests of the accuracy of cluster analysis algorithms: A comparison of hierarchical and nonhierarchical methods},
  journal =      {Multivariate Behavioral Research},
  year =     {},
  OPTkey =   {},
  volume =   {20},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {283--304},
  OPTnote =      {},
  OPTannote =    {}
}


@InProceedings{Schuster81,
  author =   {E. F. Schuster and C. G. Gregory},
  title =    {On the non-consistency of maximum likelihood nonparametric density estimators},
  booktitle =    {Computer Science and Statistics: Proceedings of the 13th Symposium on the interface},
  pages =    {295-298},
  year =     {1981},
  editor =   {Eddy, W.F.},
  organization = {}
}


@Article{Scott81,
  author =   {D. W. Scott and L. E. Factor},
  title =    {Monte Carlo study of three data-based nonparametric density estimators},
  journal =      {Journal of the American Statistical Association},
  year =     {1981},
  volume =   {76},
  pages =    {9-15}
}

@Article{Seeger68,
  author =   {P. Seeger},
  title =    {A note on a method for the analysis of significances en masse},
  journal =      {Technometrics},
  year =     {1968},
  OPTkey =   {},
  volume =   {10},
  number =   {3},
  pages =    {586--593},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Segal88,
  author =   {M. R. Segal},
  title =    {Regression trees for censored data},
  journal =      {Biometrics},
  year =     {1988},
  OPTkey =   {},
  volume =   {44},
  OPTnumber =    {},
  pages =    {35--47},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}





@string{JASA= {Journal of the American Statistical Association}}
@string{JC = {Journal of Classification}}
@string{JSPI = {Journal of Statistical Planning and Inference}}
@string{JRSSB = {Journal of the Royal Statistical Society, Series B}}
@string{PNAS = {Proc. Natl. Acad. Sci.}}

@Article{Shaffer02,
  author =   {J. P. Shaffer},
  title =    {Multiplicity, directional ({T}ype {III}) errors, and
the null hypothesis},
  journal =      {Psychological Methods},
  year =     {2002},
  OPTkey =   {},
  volume =   {7},
  OPTnumber =    {},
  pages =    {356--369},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Shaffer86,
  author =   {J. P. Shaffer},
  title =    {Modified sequentially rejective multiple test procedures},
  journal =      JASA,
  year =     {1986},
  OPTkey =   {},
  volume =   {81},
  OPTnumber =    {},
  pages =    {826--831},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Shaffer95,
  author =   {J. P. Shaffer},
  title =    {Multiple hypothesis testing},
  journal =      {Annu. Rev. Psychol.},
  year =     {1995},
  OPTkey =   {},
  volume =   {46},
  OPTnumber =    {},
  pages =    {561--584},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@article{Shao93,
AUTHOR={Shao, J.},
TITLE={Linear Model Selection by Cross-Validation},
JOURNAL={Journal of the American Statistical Association},
VOLUME={88},
YEAR={1993},
PAGES={486-494}
}




@Article{Sidak67,
  author =   {Z. \v{S}id\'{a}k},
  title =    {Rectangular confidence regions for the means of multivariate normal distributions},
  journal =      JASA,
  year =     {1967},
  OPTkey =   {},
  volume =   {62},
  OPTnumber =    {},
  pages =    {626-633},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Silverman,
  author =   {B. W. Silverman},
  title =    {Smoothed functional principal components analysis by choice of norm},
  journal =      {Annals of Statistics},
  year =     {1996},
  OPTkey =   {},
  volume =   {24},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {1--24},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Silverman84,
  author =   {B. W. Silverman},
  title =    {A fast and efficient cross-validation method for smoothing parameter choice in spline regression},
  journal =      JASA,
  year =     {1984},
  OPTkey =   {},
  volume =   {79},
  number =   {387},
  pages =    {584--589},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}




@Book{Silverman86,
  author =       {B. W. Silverman},
  title =        {Density Estimation for Statistics and Data analysis},
  publisher =    {Chapman \& Hall},
  pages = {},
  year =         {1986}
}

@Article{vanderLaan&Dudoit&Keles04,
  author =   {M.J. van der Laan and S. Dudoit and S. Keles},
  title =    {Asymptotic optimality of likelihood-based cross-validation},
  journal =      {Statistical Applications in Genetics and Molecular Biology},
  year =     {2004},
  OPTkey =   {},
  volume =   {3},
  OPTnumber =    {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/sagmb/vol3/iss1/art4},
  OPTannote =    {}
}
@Article{Simes86,
  author =   {R. J. Simes},
  title =    {An improved Bonferroni procedure for multiple tests of significance},
  journal =      {Biometrika},
  year =     {1986},
  OPTkey =   {},
  volume =   {73},
  OPTnumber =    {},
  pages =    {751--754},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Smyth00,
  author =   {P. Smyth},
  title =    {Model selection of probabilistic clustering using cross-validated likelihood},
  journal =      {Statistics and Computing},
  year =     {2000},
  volume =   {10},
  pages =    {63-72}
}




@Article{Soric89,
  author =   {B. Sori\'{c}},
  title =    {Statistical ``discoveries" and effect-size estimation},
  journal =      JASA,
  year =     {1989},
  OPTkey =   {},
  volume =   {84},
  number =   {406},
  pages =    {608--610},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Stone74,
  author =   {M. Stone},
  title =    {Cross-validatory choice and  assessment of statistical predictions},
  journal =      {Journal of the Royal Statistical Society, Series B},
  year =     {1974},
  volume =   {36},
  pages =    {111-147}
}

@Article{Stone84,
  author =   {C. J. Stone},
  title =    {An asymptotically optimal window selection rule for kernel density estimates},
  journal =      {The Annals of Statistics},
  year =     {1984},
  volume =   {12},
  pages =    {1285-1297}
}

@Article{StoneC84,
  author =   {C. J. Stone},
  title =    {An asymptotically optimal window selection rule for kernel density estimates},
  journal =      {Annals of Statistics},
  year =     {1984},
  OPTkey =   {},
  volume =   {12},
  number =   {4},
  pages =    {1285--1297},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{StoneM74,
  author =   {M. Stone},
  title =    {Cross-validatory choice and assessment of statistics predictions},
  journal =      JRSSB,
  year =     {1974},
  OPTkey =   {},
  volume =   {36},
  number =   {2},
  pages =    {111--147},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}






@Article{StoneM77,
  author =   {M. Stone},
  title =    {Asymptotics for and against cross-validation},
  journal =      {Biometrika},
  year =     {1977},
  OPTkey =   {},
  volume =   {64},
  number =   {1},
  pages =    {29--35},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@TechReport{Storey&TibshiraniTechRep01,
  author =   {J. D. Storey and R. Tibshirani},
  title =    {Estimating false discovery rates under dependence, with applications
to DNA microarrays},
  institution =  {Department of Statistics, Stanford University},
  year =     {2001},
  OPTkey =   {},
  OPTtype =      {},
  number =   {2001-28},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{StoreyJRSSB02,
  author =   {J. D. Storey},
  title =    {A direct approach to false discovery rates},
  journal =      JRSSB,
  year =     {2002},
  OPTkey =   {},
  volume =   {64},
  OPTnumber =    {},
  pages =    {479--498},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{StoreyTechRep01,
  author =   {J. D. Storey},
  title =    {The positive False Discovery Rate: A Bayesian interpretation and the q-value},
  institution =  {Department of Statistics, Stanford University},
  year =     {2001},
  OPTkey =   {},
  OPTtype =      {},
  number =   {2001-12},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{TSH,
  author =   {E. L. Lehmann},
  ALTeditor =    {},
  title =    {Testing Statistical Hypotheses},
  publisher =    {Springer-Verlag, New York},
  year =     {1986},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  edition =      {2nd},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Tibshiranietal02a,
  author =   {R. Tibshirani and T. Hastie and B. Narasimhan and. G. Chu},
  title =    {Diagnosis of multiple cancer types by shrunken centroids of gene expression},
  journal =      PNAS,
  year =     {2002},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTpages =     {},
  OPTmonth =     {},
  note =     {In press},
  OPTannote =    {}
}


@Article{Troendle95,
  author =   {J. F. Troendle},
  title =    {A stepwise resampling method of multiple hypothesis testing},
  journal =      JASA,
  year =     {1995},
  OPTkey =   {},
  volume =   {90},
  OPTnumber =    {},
  pages =    {370--378},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Troendle96,
  author =   {J. F. Troendle},
  title =    {A permutational step-up method of testing multiple outcomes},
  journal =      {Biometrics},
  year =     {1996},
  OPTkey =   {},
  volume =   {52},
  OPTnumber =    {},
  pages =    {846--859},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{VR,
 author = { W. N. Venables and B. D. Ripley },
 title = {Modern Applied Statistics with S--PLUS},
 publisher = {Springer},
 year = {1999}
}


@Book{Vaart96,
  author =       {A. W. van der Vaart  and J. A. Wellner},
  title =        {Weak {C}onvergence and {E}mprical {P}rocesses},
  publisher =    {Springer-Verlag New York},
  pages = {102},
  year =         {1996}
}





@Book{Vaart98,
  author =       {A. W. van der Vaart},
  title =        {Asymptotic Statistics},
  publisher =    {Cambridge University Press},
  pages = {62},
  year =         {1998}
}


@Book{Vapnik,
  author =   {V. N. Vapnik},
  OPTeditor =    {},
  title =    {The nature of statistical learning theory},
  publisher =    {Springer},
  year =     {2000},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  series =   {Statistics for engineering and information science},
  address =      {New York},
  edition =      {2nd},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Vapnik79,
  author =   {V. Vapnik},
  title =    {Estimation of dependences based on empirical data (in Russian)},
  journal =      {Nauka, Moskow},
  year =     {1979},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Book{Vapnik98,
  author =       {V. Vapnik},
  title =        {Statistical Learning Theory},
  publisher =    {Wiley},
  year =         {1998},
  OPTkey =       {},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {New York},
  edition =      {1st},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Book{Venables&Ripley99,
  author =   {W. N. Venables and B. D. Ripley},
  title =    {Modern applied statistics with S-PLUS},
  publisher =    {Springer},
  year =     {1999},
  OPTkey =   {},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  edition =      {3rd},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Westfall&Young93,
  author =   {P. H. Westfall and S. S. Young},
  OPTeditor =    {},
  title =    {Resampling-based multiple testing: {E}xamples and methods for $p$-value adjustment},
  publisher =    {John Wiley \& Sons},
  year =     {1993},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{,
  author =       {},
  title =        {},
  publisher =    {},
  pages = {},
  year =         {}
}


@InCollection{Westfalletal01,
  author =   {P. H. Westfall and D. V. Zaykin and S. S. Young},
  title =    {Multiple tests for genetic effects in association studies},
  booktitle =    {Biostatistical Methods},
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {143--168},
  publisher = {Humana Press, Toloway, NJ},
  year =     {2001},
  editor =   {S. Looney},
  volume =   {184},
  OPTnumber =    {},
  series =   {Methods in Molecular Biology},
  OPTtype =      {},
  OPTchapter =   {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Westonetal2000,
  author =   {J. Weston and S. Mukherjee and  O. Chappelle and  M. Pontil and  T. Poggio and V. Vapnik},
  title =    {Feature Selection for {SVM}s},
  journal =      {Advances in Neural Processing Systems},
  year =     {2001},
  OPTkey =   {},
  volume =   {13},
  number =   {},
  pages =    {668--674},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Wright92,
  author =   {S. P. Wright},
  title =    {Adjusted P-values for simultaneous inference},
  journal =      {Biometrics},
  year =     {1992},
  OPTkey =   {},
  volume =   {48},
  number =   {4},
  pages =    {1005--1013},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{YangetalJCGS02,
  author =   {Y. H. Yang and M. J. Buckley and S. Dudoit and T. P. Speed},
  title =    {Comparison of methods for image analysis on c{DNA} microarray data},
  journal =      {Journal of Computational and Graphical Statistics},
  year =     {2002},
  OPTkey =   {},
  volume =   {11},
  number =   {1},
  pages =    {108--136},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{YangetalNAR02,
  author =   {Y. H. Yang and S. Dudoit and P. Luu and D. M. Lin and V. Peng and J. Ngai and T. P. Speed},
  title =    {Normalization for c{DNA} microarray data: {A} robust composite method addressing single and multiple slide systematic variation},
  journal =      {Nucleic Acids Research},
  year =     {2002},
  OPTkey =   {},
  volume =   {30},
  number =   {4},
  pages =    {e15},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@InProceedings{YangetalSPIE01,
  author =   {Y. H. Yang and S. Dudoit and P. Luu and T. P. Speed},
  title =    {Normalization for c{DNA} microarray data},
  booktitle =    {Microarrays: Optical Technologies and Informatics},
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {141--152},
  year =     {2001},
  editor =   {Michael L. Bittner and Yidong Chen and Andreas N. Dorsel and Edward R. Dougherty},
  volume =   {4266},
  OPTnumber =    {},
  series =   {Proceedings of SPIE},
  address =      {San Jose, CA},
  month =    {May},
  OPTorganization = {SPIE},
  publisher = {SPIE-International Society for Optical Engineering},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Yekutieli&Benjamini99,
  author =   {D. Yekutieli and Y. Benjamini},
  title =    {Resampling-based false discovery rate controlling multiple test procedures for correlated test statistics},
  journal =      JSPI,
  year =     {1999},
  OPTkey =   {},
  volume =   {82},
  OPTnumber =    {},
  pages =    {171--196},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@InCollection{Youden69,
  author =   {W. J. Youden},
  title =    {Measurement agreement comparisons},
  booktitle =    {Precision measurement and calibration: Statistical concepts and procedures},
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {146--151},
  publisher = {National Bureau of Standards, United States Department of Commerce},
  year =     {1969},
  editor =   {H. H. Ku},
  volume =   {1},
  OPTnumber =    {},
  series =   {Special Publication 300},
  type =     {NBS Miscelaneous Publication 248, Proceedings of the 1962 Standards Laboratory Conference},
  OPTchapter =   {},
  OPTaddress =   {},
  OPTedition =   {},
  month =    {February},
  OPTnote =      {},
  OPTannote =    {}
}




@article{Zhang93,
AUTHOR={Zhang, P.},
TITLE={Model selection via multifold cross-validation},
JOURNAL={Annals of Statistics},
VOLUME={21},
YEAR={1993},
PAGES={299-313}
}

@Article{ZhangetalBioinf02,
  author =   {J. Zhang and V. Carey and R. Gentleman},
  title =    {An extensible application for assembling annotation for
genomic data},
  journal =      {Bioinformatics},
  year =     {2002},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {},
  OPTmonth =     {},
  note =     {(In press)},
  OPTannote =    {},
  url = {http://www.R-project.org/}
}







@Book{BKRW,
  author =   {P.J. Bickel and C.A.J. Klaassen and Y. Ritov and J. Wellner},
  title =    {Efficient and Adaptive Estimation for Semiparametric Models},
  publisher =    {Springer-Verlag},
  year =     {1997}
}




@Article{bozdoganaic,
  author =   {H. Bozdogan},
  title =    {Akaike's information criterion and recent developments in information complexity},
  journal =      {Journal of Mathematical Psychology},
  year =     {2000},
  volume =   {44},
  pages =    {62-91}
}



@book {cart,
   AUTHOR = {L. Breiman and J. H. Friedman and R. A. Olshen and C. J. Stone},
    TITLE = {Classification and Regression Trees},
PUBLISHER = {Wadsworth \& Brooks/Cole},
  ADDRESS = {Monterey},
     YEAR = {1984},
    PAGES = {},
     ISBN = {}
}

@book {mark,
 author = {M.J. van der Laan and J.M. Robins},
  title = {Unified methods for censored longitudinal  data and causality},
  publisher = {Springer, New York},
  year =     {2003}
}


@Manual{effsize,
  title =    {Teaching Children to Read},
  OPTkey =   {},
  author =   {{National Reading Panel}},
  organization = {National Institute of Child Health and Human Development, National Institutes of Health},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  year =     {1999},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{gapstats,
  author =   {R. Tibshirani and  G. Walther and T. Hastie.},
  title =    {Estimating the number of clusters in a dataset via the gap statistic},
  institution =  {Department of Biostatistics, Stanford University},
  year =     {2000},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  month =    {March},
  note =     {\url{http://www-stat.stanford.edu/~tibs/research.html}},
  OPTannote =    {}
}




@InProceedings{gillcar,
  author =   {R.D. Gill and M.J. van der Laan and J.M. Robins},
  title =    {Coarsening at random: characterizations, conjectures and counter-examples},
  booktitle =    {Proceedings of the First Seattle Symposium in Biostatistics},
  pages =    {255-94},
  year =     {1997},
  editor =   {D.Y. Lin and T.R. Fleming},
  address =      {New York},
  publisher = {Springer Verlag}
}
@article{Gill&Robins01,
   AUTHOR = {Gill, R. and Robins, J.M.},
    TITLE = {Causal inference in complex longitudinal studies: continuous case},
  JOURNAL = {Ann. Stat.},
 FJOURNAL = {The Annals of Statistics},
   VOLUME = {29},
     YEAR = {2001},
   NUMBER = {6},
    PAGES = {},
     ISSN = {},
    CODEN = {},
  MRCLASS = {},
 MRNUMBER = {},
}


%uses exponential mode at each node
@Article{jacobsen,
  author =   {M. Jacobsen and N. Keiding},
  title =    {Coarsening at random in general sample spaces and random censoring in continuous time},
  journal =      {Annals of Statistics},
  year =     {1995},
  volume =   {23},
  pages =    {774-86}
}

%very first reference to use trees in survival analysis










@Misc{marray,
  OPTkey =   {},
  author =   {S. Dudoit and Y. H. Yang},
  title =    {Normalization and diagnostic plots for cDNA microarray data, {\tt marrayClasses}, {\tt marrayInput}, {\tt marrayNorm}, {\tt marrayPlots}},
  howpublished = {{\tt R} packages},
  OPTmonth =     {},
  year =     {2002},
  OPTnote =      {},
  OPTannote =    {},
  url =          {www.bioconductor.org},
}

@TechReport{mclust98,
  author =   {C. Fraley and A. E. Raftery},
  title =    {MCLUST: Software for Model-Based Cluster Analysis},
  institution =  {Department of Statistics, University of Washington},
  year =     {1998},
  OPTkey =   {},
  OPTtype =      {},
  number =   {342},
  OPTaddress =   {},
  month =    {November},
  OPTnote =      {},
  OPTannote =    {}
}


@Misc{multtest,
  OPTkey =   {},
  author =   {Y. Ge and S. Dudoit},
  title =    {Multiple Testing Procedures, {\tt multtest}},
  howpublished = {{\tt R} package},
  OPTmonth =     {},
  year =     {2002},
  OPTnote =      {},
  OPTannote =    {},
  url =          {www.bioconductor.org},
}

@InProceedings{robins93,
  author =   {J.M. Robins},
  title =    {Information recovery and bias adjustment in proportional hazards regression analysis of randomized trials using surrogate markers},
  booktitle =    {Proceeding of the Biopharmaceutical section},
  pages =    {24-33},
  year =     {1993},
  organization = {American Statistical Association}
}

@InCollection{robrot,
  author =   {J.M. Robins and A. Rotnitzky},
  title =    {Recovery of information and adjustment for dependent censoring using surrogate markers},
  booktitle =    {AIDS Epidemiology},
  publisher = {Bikh\"{a}user},
  year =     {1992},
  series =   {Methodological issues}
}


@Article{robzhao,
  author =   {J.M. Robins and A. Rotnitzky and L.P. Zhao},
  title =    {Estimation of regression coefficients when some regressors are not always observed},
  journal =      {Journal of the American Statistical Association},
  year =     {1994},
  volume =   {89},
  number =   {427},
  pages =    {846-866},
  month =    {September}
}







@Article{Heitjan&Rubin91,
  author =   {D.F. Heitjan and D.B. Rubin},
  title =    {Ignorability and coarse data},
  journal =      {Annals of statistics},
  year =     {1991},
  volume =   {19},
  number =   {4},
  pages =    {2244-2253},
  month =    {December}
}

@Misc{sma,
  OPTkey =   {},
  author =   {S. Dudoit and Y. H. Yang and B. M. Bolstad},
  title =    {Statistical {M}icroarray {A}nalysis, {\tt sma}},
  howpublished = {{\tt R} package},
  OPTmonth =     {},
  year =     {2001},
  note =     {Contributions from Natalie Thorne, Ingrid L\"{o}nnstedt, and Jessica Mar},
  OPTannote =    {},
  url =          {cran.r-project.org/src/contrib/PACKAGES.html\#sma}
}

@PhdThesis{thesis,
  author =   {S. Dudoit},
  title =    {Linkage analysis of complex human traits using identity by descent data},
  school =   {Department of Statistics, University of California, Berkeley},
  year =     {1999},
  OPTkey =   {},
  OPTaddress =   {},
  type =     {Ph.D. thesis},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{vanderVaart&Wellner96,
  author =   {A. van der Vaart and J. Wellner},
  ALTeditor =    {},
  title =    {Weak Convergence and Empirical Processes},
  publisher =    {Springer-Verlag, New York},
  year =     {1996},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@inproceedings{arcones1989boot_mean,
  title={The bootstrap of the mean with arbitrary bootstrap sample size},
  author={Arcones, Miguel A and Gin{\'e}, Evarist},
  booktitle={Annales de l'IHP Probabilit{\'e}s et statistiques},
  volume={25},
  number={4},
  pages={457--481},
  year={1989}
}
@article{gine1989necessary_boot_mean,
  title={Necessary conditions for the bootstrap of the mean},
  author={Gin{\'e}, Evarist and Zinn, Joel},
  journal={The annals of statistics},
  pages={684--691},
  year={1989},
  publisher={JSTOR}
}
@article{arcones1992boot_mestimator,
  title={On the bootstrap of M-estimators and other statistical functionals},
  author={Arcones, Miguel A and Gin{\'e}, Evarist},
  journal={Exploring the limits of bootstrap},
  pages={13--47},
  year={1992},
  publisher={Wiley New York}
}

==> combined.tex <==
@article{vanderLaan17,
	author = {M.J. van der Laan},
	journal = {International Journal of Biostatistics},
	pages = {1106--1118},
	title = {A Generally Efficient Targeted Minimum Loss Based Estimator},
	year = {2017},
}

@techreport{Bibaut&vanderLaan19,
  author =        {A. Bibaut and M.J. van der Laan},
    institution =   {Division of Biostatistics, University of California,
                   Berkeley},
   number={},
  title =         {Fast rates for empirical risk minimization over cadlag functions with bounded sectional variation norm},
  year =          {2019},
  Optnote={ https://arxiv.org/abs/1907.0924},
  }


%- When Adaptive Group Sequential RCT meets Machine Learning W. Zheng, Antoine Chambaz and Mark van der Laan - Effect Modification by Counterfactual Baseline Modifiers: a twist to a familiar storyW. Zheng, Zhehui Luo and Mark van der Laan
%Starmans, R.J.C.M. (2011). Models, Inference and Truth; Probabilistic Reasoning in the Information Era. In Mark.J. Van der Laan & Sherri Rose (Eds.), Targeted Learning; Causal Inference for Observational and Experimental Data (Springer Series in Statistics) (pp. 1-20). Springer.

@preamble{ " \newcommand{\noop}[1]{} " } %

%Benkeser D, van der Laan M (2016). The Highly Adaptive Lasso Estimator. Accepted: Proceedings of the IEEE Conference on Data Science and Advanced Analytics.

@book{vanderLaan&Rose17,
  author =        {M.J. van der Laan and S. Rose},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  title =         {Targeted Learning in Data Science: Causal Inference for Complex Longitudinal Studies},
  year =          {2017},
}

@incollection{Caroneetal17,
	Author = {M. Carone and I. Diaz and M.J. van der Laan},
	Booktitle = {{\rm M.J. van der Laan and S. Rose, } Targeted Learning in Data Science:Causal Inference for complex longitudinal studies},
	Chapter = {26},
	pages={Tbt},
	Publisher = {Springer, New York},
	Title = {Higher order targeted loss-based estimation},
	Year = {2017}}

@article{Benkeser&vanderLaan16,
 author =        {D. Benkeser and M.J. van der Laan},
  journal =       {Proceedings of the IEEE Conference on Data Science and Advanced Analytics},
  title =         {The highly adaptive lasso estimator},
  year =          {2016},
}

@article{Benkeseretal17,
 author =        {D. Benkeser and P. Gilbert and M. van der Laan and M. Carone},
  journal =       {Biometrika},
  title =         {Nonparametric double robust inference for a counterfactual mean},
 note={To appear},
  year =          {2017},
}




@article{Starmans13,
 author =        {R.J.C.M. Starmans},
  journal =       {Stator},
  number =         {24},
  title =         {Picasso, {H}egel and the Era of Big Data (in Dutch)},
  volume =        {2},
  year =          {2013},
}

@article{Starmans&vanderLaan13,
 author =        {R.J.C.M. Starmans and M.J. van der Laan},
  journal =       {Stator},
  number =         {24},
  title =         {Inferential Statistics versus Machine Learning; a Prelude to Reconciliation (in Dutch)},
  volume =        {2},
  year =          {2013},
}



@techreport{Roseetal12,
  author =        {S. Rose and R.J.C.M. Starmans and M.J. van der Laan},
    institution =   {Division of Biostatistics, University of California,
                   Berkeley},
   number={297},
  title =         {Targeted Learning for Causality and Statistical Analysis in Medical Research},
  year =          {2011},
  Optnote={http://biostats.bepress.com/ucbbiostat/paper297},
  }



@incollection{Starmans2012,
  author =        {R.J.C.M. Starmans},
  booktitle =     {Targeted Learning: Causal Inference for Observational and Experimental Studies},
  editor =        {M.J. van der Laan and S. Rose},
  publisher =     {Springer},
  title =         {Models, Inference and Truth: Probabilistic Reasoning in the Information Era},
  pages= {1--20},
  year =          {2011},
      address =       {New York},
}







@incollection{Caroneetal12,
  author =        {M. Carone and M. Petersen and M.J. van der Laan},
  booktitle =     {Interval Censored Time To Event Data: Methods and Applications},
  editor =        {Ding-Geng (Din) Chen, Jianguo Sun, Karl E. Peace (eds)},
  publisher =     {Chapman \& Hall/CRC},
  title =         {Targeted minimum loss based estimation of a casual effect using interval censored time to event data},
  year =          {2012},
      address =       {New York},
}


@article{vanderLaan&Petersen&Zheng13,
 author =        {W. Zheng and M.L. Petersen and M.J. van der Laan},
  journal =       {Journal of Causal Inference},
  number =         {Issue 1},
  pages={83--106},
  title =         {Estimating the Effect of a Community-Based Intervention with Two Communities},
  volume =        {1},
  year =          {2013},
}

@article{Zheng&vanderLaan12a,
 author =        {W. Zheng and M.J. van der Laan},
  journal =       {International Journal of Biostatistics},
  number =         {Issue 1},
  title =         {Targeted Maximum Likelihood Estimation of Natural Direct Effects},
  volume =        {8},
  year =          {2012},
}



@techreport{Zheng&vanderLaan12b,
  author =        {W. Zheng and M.J. van der Laan},
    institution =   {Division of Biostatistics, University of California,
                   Berkeley},
   number={295},
  title =         {Causal Mediation in a Survival Setting with Time-Dependent Mediators},
  year =          {2012},
}


@article{Cotton&Heagerty11,
 author =        {C. Cotton and P. Heagerty},
  journal =       {Stat. Biosc},
  pages =         {28--44},
  title =         {A data augmentation method for estimating the causal effect of adherence to
treatment regimens targeting control of an intermediate measure},
  volume =        {3},
  year =          {2011},
}

@incollection{vanderLaan&Petersen12,
  author =        {M.J. van der Laan and M.L. Petersen},
  booktitle =     {Ensemble Machine Learning: Methods and Applications},
  editor =        {C. Zhang and Y. Ma (eds)},
  publisher =     {Springer},
  title =         {Targeted Learning},
  year =          {2012},
      address =       {New York},
}

@incollection{Zheng&vanderLaan12,
  author =        {W. Zheng and M.J. van der Laan},
  booktitle =     {Targeted Learning: Causal Inference for Observational and Experimental Studies},
  editor =        {M.J. van der Laan and S. Rose},
  publisher =     {Springer},
  title =         {Cross-validated targeted minimum loss based estimation},
  year =          {2011},
      address =       {New York},
}


@techreport{Balzer&vanderLaan13,
  author =        {L.B. Balzer and M.J. van der Laan},
    institution =   {Division of Biostatistics, University of California,
                   Berkeley},
   number={310},
  title =         {Estimating Effects on Rare Outcomes: Knowledge is Power},
  year =          {2013},
}

@techreport{vanderLaan12,
  author =        {M.J. van der Laan},
    institution =   {Division of Biostatistics, University of California,
                   Berkeley, submitted to IJB},
   number={302},
  title =         {Statistical Inference when using Data Adaptive Estimators of Nuisance Parameters},
  year =          {2012},
}

@techreport{Diaz&vanderLaan13,
  author =        {I. Diaz and M.J. van der Laan},
    institution =   {Division of Biostatistics, University of California,
                   Berkeley, submitted to JCI},
   number={306},
  title =         {Targeted Data Adaptive Estimation of the Causal Dose Response Curve},
  year =          {2013},
}


@techreport{vanderLaan&Hubbard13,
  author =        {M.J. van der Laan and A.E. Hubbard and S. Kherad},
    institution =   {Division of Biostatistics, University of California,
                   Berkeley},
   number={314},
  title =         {Statistical Inference for Data Adaptive Target Parameters},
  year =          {2013},
}



@article{Rubin&vanderLaan07,
 author =        {D. Rubin and M.J. van der Laan},
  journal =       {The International Journal of Biostatistics},
  pages =         {http://www.bepress.com/ijb/vol3/iss1/4},
  title =         {A Doubly Robust Censoring Unbiased Trans- formation},
  volume =        {Vol. 3 (1)},
  year =          {2007},
}


@article{Chakrabortietal10,
 author =        {B. Chakraborty and S.A. Murphy and V. Strecher},
  journal =       {Stat. Methods Med. Res.},
  pages =         {317--43},
  title =         {Inference for non-regular parameters in optimal dynamic
treatment regimes},
  volume =        {19},
  year =          {2010},
}

@article{Chakraborti&Murphy13,
 author =        {B. Chakraborty and S.A. Murphy},
  journal =       {Annu. Rev. Stat. Appl.},
  pages =         {1--18},
  title =         {Dynamic treatment regimens},
  volume =        {1},
  year =          {2013},
}


@article{Rubin&vanderLaan12,
  author =        {D.B. Rubin and M.J. van der Laan},
  journal =       {International Journal of Biostatistics},
  pages =         {Issue 1, Article 18},
  title =         {Statistical issues and limitations in personalized medicine research with clinical trials},
  volume =        {8},
  year =          {2012},
}
@article{Wang&vanderLaan11,
  author =        {H. Wang and M.J. van der Laan},
  journal =       {BMC Bioinformatics},
  pages =         {312},
  title =         {Dimension reduction procedure using  targeted variable  importance measurement},
  volume =        {12},
  year =          {2011},
}

@article{Westeretal12,
  author =        {C.W. Wester and O.M. Stitelman and V. De Gruttola and H. Bussmann and R.G. Marlink  and  M.J. van  der  Laan},
  journal =       {AIDS Res Hum Retroviruses},
  pages =         {781--88},
  title =         {Effect modification by sex and  baseline  CD4(+) cell count  among  adults receiving combination antiretroviral therapy in Botswana: Results  from a clinical trial},
  volume =        {28},
  year =          {2012},
}

@book{Polley&vanderLaan12,
  address =       {Available at http://cran.r-project.org/web/packages/SuperLearner/SuperLearner.pdf.
},
  author =        {E. Polley and M.J. van der Laan},
  publisher =     {R package version 2.0-6},
  title =         {Super Learner Prediction},
  year =          {2012},
}

@book{Gruber&vanderLaan12,
  address =       {Available at http://cran.r-project.org/web/packages/tmle/tmle.pdf},
  author =        {S. Gruber and M.J. van der Laan},
  publisher =     {R package version 1.2.0-1},
  title =         {Targeted Maximum Likelihood Estimation},
  year =          {2012},
}

@book{Schwabb&vanderLaan&Petersen12,
  address =       {Available at http://cran.r-project.org/web/packages/ltmle/ltmle.pdf},
  author =        {J. Schwabb and M.J. van der Laan and M.L. Petersen},
  publisher =     { },
  title =         {Longitudinal Targeted Maximum Likelihood Estimation},
  year =          {2012},
}


@article{Banks&Jang&Kwon11,
  author =        {H. Banks and T. Jang and H. Kwon},
  journal =       {Int. J. Pure Appl. Math.},
  pages =         {461--485},
  title =         {Feedback control of HIV antiviral therapy with long measurement time},
  volume =        {66},
  year =          {2011},
}

@book{Bellman57,
  address =       {Princeton, NJ},
  author =        {R. Bellman},
  edition =       {},
  publisher =     {Univ. Press},
  title =         {Dynamic Programming},
  year =          {1957},
}

@article{Benneth&Hauser12,
  author =        {C. Bennett and K. Hauser},
  journal =       {Artif. Intell. Med.},
  pages =         {9--19},
  title =         {Artificial intelligence framework for simulating clinical decision-making: a
Markov decision process approach},
  volume =        {57},
  year =          {2012},
}

%Berger R, Boos D. 1994.Pvalues maximized over a confidence set for the nuisance parameter.J. Am. Stat.Assoc.89:1012Ð16Box G, Hunter W, Hunter J. 1978.Statistics for Experimenters: An Introduction to Design, Data Analysis, andModel Building.NewYork:Wiley

@article{Cai&Tian&Wong&Wei11,
  author =        {T. Cai and L. Tian and P. Wong and L. Wei},
  journal =       {Biostatistics},
  pages =         {270--282},
  title =         {Analysis of randomized comparative clinical trial data for personalized
treatment selections},
  volume =        {12},
  year =          {2011},
}

@article{Chakraborty&Murphy&Strecher10,
  author =        {B. Chakraborty and S. Murphy and V. Strecher},
  journal =       {Stat. Methods Med. Res},
  pages =         {317--343},
  title =         {Inference for non-regular parameters in optimal dynamic
treatment regimes},
  volume =        {19},
  year =          {2010},
}


@article{Dawson&Lavori10,
  author =        {R. Dawson and P. Lavori},
  journal =       {Clin. Trials},
  pages =         {643--652},
  title =         {Sample size calculations for evaluating treatment policies in multi-stage designs},
  volume =        {7},
  year =          {2010},
}

@article{Dawson&Lavori12,
  author =        {R. Dawson and P. Lavori},
  journal =       {Biostatistics},
  pages =         {142--152},
  title =         {Efficient design and inference for multistage randomized trials of individualized
treatment policies},
  volume =        {13},
  year =          {2012},
}

@article{Ernstetal05,
  author =        {D. Ernst and P. Geurts and L. Wehenkel},
  journal =       {J. Mach. Learn. Res.},
  pages =         {503--556},
  title =         {Tree-based batch mode reinforcement learning},
  volume =        {6},
  year =          {2005},
}

@article{Gawedaetal05,
  author =        {A. Gaweda and M. Muezzinoglu and G. Aronoff and A. Jacobs and J. Zurada and M. Brier},
  journal =       {Neural Netw.},
  pages =         {826--34},
  title =         {Individualization of pharmaco-
logical anemia management using reinforcement learning},
  volume =        {18},
  year =          {2005},
}

@article{Goldberg&Kosorok12,
  author =        {Y. Goldberg and M. Kosorok},
  journal =       {Ann. Stat.},
  pages =         {529-60},
  title =         {Q-learning with censored data},
  volume =        {40},
  year =          {2012},
}

@article{Hernanetal06,
  author =        {M.A. Hernan and E. Lanoy and D. Costagliola and J.M. Robins},
  journal =       {Basic Clin. Pharmacol. Toxicol},
  pages =         {237--242},
  title =         {Comparison of dynamic treatment regimes via
inverse probability weighting},
  volume =        {98},
  year =          {2006},
}



@article{Imai&Ratkovicz13,
  author =        {K. Imai and M. Ratkovicz},
  journal =       {Ann. Appl. Stat.},
  pages =         {443-70},
  title =         {Estimating treatment effect heterogeneity in randomized program evaluation},
  volume =        {7},
  year =          {2013},
}

@article{Jones10,
  author =        {H. Jones},
  journal =       {ClinicalTrials.gov data base, updated October 19, 2012},
  pages =         {accessed July 24, 2013},
  title =         {Reinforcement-based treatment for pregnant drug abusers},
  volume =        {Natl. Inst. Health., Bethesda, MD, http://
clinicaltrials.gov/ct2/show/NCT01177982},
  year =          {2010},
}

@article{Kasari09,
  author =        {C. Kasari},
  journal =       {ClinicalTrials.gov database, updated Apr. 26, 2012},
  pages =         {accessed July 24, 2013},
  title =         {Developmental and augmented intervention for facilitating expressive language},
  volume =        {Natl. Inst. Health., Bethesda, MD, http://
clinicaltrials.gov/ct2/show/NCT01013545},
  year =          {2009},
}

@article{Kulkarnietal11,
  author =        {K. Kulkarni and A. Gosavi and S. Murray and K. Grantham},
  journal =       {J. Control Theory Appl.},
  pages =         {421--30},
  title =         {Semi-Markov adaptive critic heuristics with application
to airline revenue management},
  volume =        {9},
  year =          {2011},
}

@article{Laber&Murphy11,
  author =        {E. Laber and S. Murphy},
  journal =       {J. Am. Stat. Assoc.},
  pages =         {904--13},
  title =         {Adaptive confidence intervals for the test error in classification},
  volume =        {106},
  year =          {2011},
}

@article{Lavori&Dawson00,
  author =        {P. Lavori and R. Dawson},
  journal =       {J. R. Stat. Soc. A.},
  pages =         {29--38},
  title =         {A design for testing clinical strategies: biased adaptive within-subject randomiza-
tion},
  volume =        {163},
  year =          {2000},
}
@article{Lavori&Dawson04,
  author =        {P. Lavori and R. Dawson},
  journal =       {Clin. Trials},
  pages =         {9--20},
  title =         {Dynamic treatment regimes: practical design considerations.},
  volume =        {1},
  year =          {2004},
}

@article{Lavori&Dawson08,
  author =        {P. Lavori and R. Dawson},
  journal =       {Annu. Rev. Med.},
  pages =         {443--453},
  title =         {Adaptive treatment strategies in chronic disease},
  volume =        {59},
  year =          {2008},
}

@article{Leeb&Potscher03,
  author =        {H.P. Leeb and B. Potscher},
  journal =       {Econom. Theory},
  pages =         {100-42},
  title =         {The finite-sample distribution of post-model-selection estimators and uniform
versus nonuniform approximations.},
  volume =        {19},
  year =          {2003},
}

@article{Leietal11,
  author =        {H. Lei and I. Nahum-Shani and K. Lynch and D. Oslin and S. Murphy},
  journal =       {Annu. Rev. Clin. Psychol.},
  pages =         {21--48},
  title =         {A ÒSMARTÓ design for building individualized
treatment sequences},
  volume =        {8},
  year =          {2011},
}

@article{Li&Murphy11,
  author =        {Z. Li and S. Murphy},
  journal =       {Biometrika},
  pages =         {503--18},
  title =         {Sample size formulae for two-stage randomized trials with survival outcomes},
  volume =        {98},
  year =          {2011},
}

@article{Lizotteetal10,
  author =        {D. Lizotte and M. Bowling and S. Murphy},
  journal =       {Twenty-Seventh International Conference on Machine Learning
(ICML)},
  pages =         {695--702},
  title =         {Efficient reinforcement learning with multiple reward functions
for randomized clinical trial analysis},
  volume =        {Haifa, Israel: Omnipress},
  year =          {2010},
}

@article{Lizotteetal12,
  author =        {D. Lizotte and M. Bowling and S. Murphy},
  journal =       {J. Mach.
Learn. Res.},
  pages =         {3253--95},
  title =         {Linear fitted-Q iteration with multiple reward functions},
  volume =        {13},
  year =          {2012},
}

@article{Luncefordetal02,
  author =        {J. Lunceford and M. Davidian and A. Tsiatis},
  journal =       {Biometrics},
  pages =         {48--57},
  title =         {Estimation of survival distributions of treatment policies in
two-stage randomization designs in clinical trials},
  volume =        {58},
  year =          {2002},
}

@article{Moodieetal12,
  author =        {E. Moodie and B. Chakraborty and M. Kramer.},
  journal =       {Can. J. Stat.},
  pages =         {629--45},
  title =         {Q-learning for estimating optimal dynamic treatment rules
from observational data},
  volume =        {40},
  year =          {2012},
}

@article{Moodieetal09,
  author =        {E. Moodie and R. Platt and M. Kramer},
  journal =       {J. Am. Stat. Assoc.},
  pages =         {155--65},
  title =         {Estimating response-maximized decision rules with applications to
breastfeeding},
  volume =        {104},
  year =          {2009},
}

@article{Murphy05a,
  author =        {S. Murphy},
  journal =       {J. Mach. Learn. Res.},
  pages =         {1073--97},
  title =         {A generalization error for Q-learning},
  volume =        {6},
  year =          {2005a},
}
@article{Murphy05b,
  author =        {S. Murphy},
  journal =       {Stat. Med.},
  pages =         {1455--81},
  title =         {An experimental design for the development of adaptive treatment strategies},
  volume =        {24},
  year =          {2005b},
}
@article{Murphy&Bingham09,
  author =        {S. Murphy and D. Bingham},
  journal =       {J. Am. Stat. Assoc.},
  pages =         {391--408},
  title =         {Screening experiments for developing dynamic treatment regimes},
  volume =        {24},
  year =          {2005b},
}

@article{Murphyetal01,
  author =        {S. Murphy and M.J. van der Laan and J.M. Robins},
  journal =       {J. Am. Stat. Assoc.},
  pages =         {1410--23},
  title =         {Marginal mean models for
dynamic regimes},
  volume =        {96},
  year =          {2001},
}

@article{Nahum-Shanietal12a,
  author =        {I. Nahum-Shani and M.  Qian and D. Almiral and W.  Pelham and B.  Gnagy B, et al. },
  journal =       {Psychol. Methods},
  pages =         {457--77},
  title =         {Experimental design and primary
data analysis methods for comparing adaptive interventions},
  volume =        {17},
  year =          {2012a},
}

@article{Nahum-Shanietal12b,
  author =        {I. Nahum-Shani and M.  Qian and D. Almiral and W.  Pelham and B.  Gnagy B, et al. },
  journal =       {Psychol. Methods},
  pages =         {478--94},
  title =         {Q-learning: a data analysis method
for constructing adaptive interventions},
  volume =        {17},
  year =          {2012b},
}
@article{Nahum-Shanietal12b,
  author =        {I. Nahum-Shani and M.  Qian and D. Almiral and W.  Pelham and B.  Gnagy B, et al. },
  journal =       {Psychol. Methods},
  pages =         {478--94},
  title =         {Q-learning: a data analysis method
for constructing adaptive interventions},
  volume =        {17},
  year =          {2012b},
}


@article{Navarro-Barrientoseta11,
  author =        {J. Navarro-Barrientos and D. Rivera and L. Collins},
  journal =       {Math. Comput. Model. Dyn. Syst.},
  pages =         {183--203},
  title =         {A dynamical model for describing behavioural interventions
for weight loss and body composition change},
  volume =        {17},
  year =          {2011},
}

@article{Oettingetal11,
  author =        {A. Oetting and J. Levy and R. Weiss and S. Murphy},
  journal =       {In
Causality and Psychopathology: Finding the Determinants of Disorders and
Their Cures},
  pages =         {179--205},
  title =         { Statistical methodology for a SMART design in the development
of adaptive treatment strategies},
  volume =        {ed. PE Shrout, KM Keyes, K Ornstein, New York: Oxford Univ. Press},
  year =          {2011},
}

@article{Orellanaetal10a,
  author =        {L. Orellana and A. Rotnitzky and J.M. Robins},
  journal =       {Int. J. Biostat.},
  pages =         {6:8},
  title =         {Dynamic regime marginal structural mean models for estimation
of optimal dynamic treatment regimes, part I: main content},
  volume =        { },
  year =          {2010a},
}
@article{Orellanaetal10b,
  author =        {L. Orellana and A. Rotnitzky and J.M. Robins},
  journal =       {Int. J. Biostat.},
  pages =         {6:9},
  title =         {Dynamic regime marginal structural mean models for estimation
of optimal dynamic treatment regimes, part I: proofs and additional results},
  volume =        {  },
  year =          {2010b},
}

@article{Ormoneit&Sen02,
  author =        {D. Ormoneit and S. Sen},
  journal =       {Mach. Learn.},
  pages =         {161--78},
  title =         {Kernel-based reinforcement learning},
  volume =        {49},
  year =          {2002},
}

@article{Qian&Murphy11,
  author =        {M. Qian and S. Murphy},
  journal =       {Ann. Stat.},
  pages =         {1180--210},
  title =         {Performance guarantees for individualized treatment rules},
  volume =        {39},
  year =          {2011},
}

@article{Riveraetal07,
  author =        {D. Rivera and M. Pew and L. Collins},
  journal =       {Drug Alcohol Depend.},
  pages =         {S31--40},
  title =         {Using engineering control principles to inform the design of adaptive
interventions: a conceptual introduction},
  volume =        {88},
  year =          {2007},
}

@article{Robins04,
  author =        {J.M. Robins},
  journal =       {Proc. Seattle Symp. Biostat.},
  pages =         {189--326},
  title =         {Optimal structural nested models for optimal sequential decisions},
  volume =        {2nd, ed. D Lin, P Heagerty, New York: Springer},
  year =          {2004},
}

@article{Robinsetal08,
  author =        {J.M. Robins and L. Orellana and A. Rotnitzky},
  journal =       {Stat. Med.},
  pages =         {4678--721},
  title =         {Estimation and extrapolation of optimal treatment and testing
strategies},
  volume =        {27},
  year =          {2008},
}

@article{Rosenbergeretal07,
  author =        {E. Rosenberger and M. Davidian and H. Banks},
  journal =       {Drug Alcohol Depend.},
  pages =         {S41--51},
  title =         {Using mathematical modeling and control to develop structured
treatment interruption strategies for HIV infection},
  volume =        {88},
  year =          {2007},
}

@article{Rosthojetal06,
  author =        {S. Rosth¿j and C. Fullwood and R. Henderson and S. Stewart},
  journal =       {Stat. Med.},
  pages =         {4197--215},
  title =         {Estimation of optimal dynamic anticoagulation
regimes from observational data: a regret-based approach},
  volume ={88},
  year =          {2006},
}

@article{Shortreed&Moodie12,
  author =        {S. Shortreed and E. Moodie},
  journal =       {J.R. Stat. Soc. C.},
  pages =         {577--99},
  title =         {Estimating the optimal dynamic antipsychotic treatment regime: evidence from
the sequential-multiple assignment randomized CATIE Schizophrenia Study},
  volume ={61},
  year =          {2012},
}

@book{Sutton&Barto98,
  address =       {Cambridge, MA},
  author =        {R. Sutton and H. Sung},
  edition =       {},
  publisher =     {MIT  Press},
  title =         {Reinforcement Learning: An Introduction},
  year =          {1998},
}

@article{Thalletal00,
  author =        {P. Thall and R. Millikan and H. Sung},
  journal =       {Stat. Med.},
  pages =         {1011--128},
  title =         {Evaluating multiple treatment courses in clinical trials},
  volume ={30},
  year =          {2000},
}

@article{Thalletal02,
  author =        {P. Thall  and H. Sung and E. Estey},
  journal =       {J. Am. Stat. Assoc.},
  pages =         {29--39},
  title =         {Selecting therapeutic strategies based on efficacy and death in multicourse
clinical trials},
  volume ={39},
  year =          {2002},
}

@article{Thall&Wathen05,
  author =        {P. Thall  and J. Wathen},
  journal =       {Stat. Med.},
  pages =         {1947--64},
  title =         {Covariate-adjusted adaptive randomization in a sarcoma trial with multi-stage
treatments},
  volume ={24},
  year =          {2005},
}

@article{Thalletal07,
  author =        {P. Thall and C. Logothetis and L.C. Pagliaro and S. Wen and M.A.  Brown et al.},
  journal =       {J. Natl. Cancer Inst.},
  pages =         {1613--22},
  title =         {Adaptive therapy for androgen-
independent prostate cancer: a randomized selection trial of four regimens},
  volume ={99},
  year =          {2007},
}

%van der Laan MJ, Petersen ML. 2007a. Causal effect models for realistic individualized treatment andintention to treat rules.Int. J. Biostat.3:3van der Laan MJ, Petersen ML. 2007b. Statistical learning of origin-specific statically optimal individualizedtreatment rules.Int. J. Biostat.3:6

@article{Wagneretal01,
  author =        {E. Wagner and B. Austin and C. Davis and M. Hindmarsh and J. Schaefer and A. Bonomi},
  journal =       {Health Aff.},
  pages =         {64--78},
  title =         {Improving chronic illness care:
translating evidence into action},
  volume ={20},
  year =          {2001},
}

@article{Wahed&Tsiatis04,
  author =        {A. Wahed and A. Tsiatis},
  journal =       {Biometrics},
  pages =         {124--33},
  title =         {Optimal estimator for the survival distribution and related quantities for treatment
policies in two-stage randomized designs in clinical trials},
  volume ={60},
  year =          {2004},
}

@article{Wahed&Tsiatis06,
  author =        {A. Wahed and A. Tsiatis},
  journal =       {Biometrika},
  pages =         {163--77},
  title =         {Semiparametric efficient estimation of survival distributions in two-stage
randomisation designs in clinical trials with censored data},
  volume ={93},
  year =          {2006},
}

@article{Wangetal12,
  author =        {L. Wang and A.  Rotnitzky and X.  Lin and R.  Millikan and P. Thall},
  journal =       {J. Am. Stat. Assoc.},
  pages =         {493--508},
  title =         {Evaluation of viable dynamic treatment regimes in
a sequentially randomized trial of advanced prostate cancer},
  volume ={107},
  year =          {2012},
}

@article{Zhangetal12a,
  author =        {B. Zhang and A. Tsiatis and M. Davidian and M. Zhang and E. Laber},
  journal =       {Stat},
  pages =         {103--14},
  title =         {Estimating optimal treatment regimes from a
classification perspective},
  volume ={1},
  year =          {2012a},
}

@article{Zhangetal12b,
  author =        {B. Zhang and A. Tsiatis and M. Davidian and M. Zhang and E. Laber},
  journal =       {Biometrics},
  pages =         {1010--18},
  title =         {A robust method for estimating optimal treatment regimes},
  volume ={68},
  year =          {2012b},
}
@article{Zhaoetal12,
  author =        {Y. Zhao and D. Zeng and A. Rush and M. Kosorok},
  journal =       {J. Am. Stat. Assoc.},
  pages =         {1106--18},
  title =         {Estimating individual treatment rules using outcome weighted
learning},
  volume ={107},
  year =          {2012},
}

@article{Zhaoetal11,
  author =        {Y. Zhao and D. Zeng and A. Rush and M. Kosorok},
  journal =       {Biometrics},
  pages =         {1422--33},
  title =         {Reinforcement learning strategies for clinical trials in
nonsmall cell lung cancer},
  volume ={67},
  year =          {2011},
}




@techreport{Diaz&vanderLaan2012,
  author =        {I. Diaz and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
number={303},
  title =         {Sensitivity Analysis for Causal Inference Under Unmeasured Confounding and Measurement Error Problems},
  year =          {2012},
  note ={Submitted to IJB, also technical report http://www.bepress.com/ucbbiostat/paper303}
}
@techreport{vanderLaan2012,
  author =        {M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
number={300},
  title =         {Causal Inference for Networks},
  year =          {2012},
  note ={Submitted to JCI, also technical report http://www.bepress.com/ucbbiostat/paper300}
}

@techreport{vanderLaan&Gruber11,
  author =        {M.J. van der Laan and S. Gruber},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
number={290},
  title =         {Targeted Minimum Loss Based Estimation of an Intervention Specific Mean Outcome},
  year =          {2011},
  note ={To appear in IJB, also technical report http://www.bepress.com/ucbbiostat/paper290}
}



@incollection{Marschak53,
  address =       {New York},
  author =        {J. Marschak},
  booktitle =     {Economic measurements for policy and prediction},
  editor =        {W.~C. Hood and T.~C. Koopmans},
  publisher =     {Wiley},
  title =         {Studies in econometric method},
  year =          {1953},
}

@article{Heckman00,
  author =        {J. Heckman},
  journal =       {Q J Econ},
  pages =         {45--97},
  title =         {Causal parameters and policy analysis in economics:
                   A twentieth century retrospective.},
  volume =        {115},
  year =          {2000},
}

@article{Gruber&vanderLaan10,
  author =        {S. Gruber and M.J. van der Laan},
  journal =       {International Journal of Biostatistics},
  pages =         {article 26, www.bepress.com/ijb/vol6/iss1/26},
  title =         {A Targeted Maximum Likelihood Estimator of a Causal Effect on a Bounded Continuous Outcome},
  volume =        {6},
  year =          {2010},
}




@article{Heckman10,
  author =        {J. Heckman},
  journal =       {J Econ Lit},
  pages =         {356--398},
  title =         {Building bridges between structural and program
                   evaluation approaches to evaluating policy.},
  volume =        {48},
  year =          {2010},
}

@article{Bang&Robins05,
author={H. Bang and J.M. Robins},
 journal =       {Biometrics},
  pages =         {962--972},
  title =         {Doubly robust estimation in missing data and causal inference models},
  volume =        {61},
  year =          {2005},
}



@book{Pearson11,
  address =       {London},
  author =        {K. Pearson},
  edition =       {3rd},
  publisher =     {Black},
  title =         {Grammar of science},
  year =          {1911},
}

@article{Rubin74,
  author =        {Donald B. Rubin},
  journal =       {J Educ Psychol},
  number =        {},
  pages =         {688--701},
  title =         {Estimating causal effects of treatments in randomized
                   and nonrandomized studies.},
  volume =        {66},
  year =          {1974},
}

@article{Neyman23,
  author =        {J. Neyman},
  journal =       {Stat Sci},
  number =        {},
  pages =         {465--480},
  title =         {Sur les applications de la theorie des probabilites
                   aux experiences agricoles: Essai des principes ({In
                   Polish}). {E}nglish translation by {D.M.} {D}abrowska and
                   {T.P.} {S}peed (1990)},
  volume =        {5},
  year =          {1923},
}

@book{Pearl09,
  address =       {New York},
  author =        {J. Pearl},
  edition =       {2nd},
  publisher =     {Cambridge},
  title =         {Causality: models, reasoning, and inference},
  year =          {2009},
}

@article{Pearl95,
  author =        {J. Pearl},
  journal =       {Biometrika},
  pages =         {669--710},
  title =         {Causal diagrams for empirical research.},
  volume =        {82},
  year =          {1995},
}

@article{Robins&Greenland92,
  author =        {J.M. Robins and S. Greenland},
  journal =       {Epidemiol},
  pages =         {143--155},
  title =         {Identifiability and exchangeability for direct and
                   indirect effects},
  volume =        {3},
  year =          {1992},
}

@inproceedings{Pearl01b,
  address =       {San Francisco},
  author =        {J. Pearl},
  booktitle =     {Uncertainty in artificial intelligence, Proceedings
                   of the 17th Conference},
  publisher =     {Morgan Kaufmann},
  title =         {Direct and indirect effects.},
  year =          {2001},
}

@article{Baron&Kenny86,
  author =        {R. Baron and D. Kenny},
  journal =       {J Personal Soc Psychol},
  pages =         {1173--1182},
  title =         {The moderator-mediator variable distinction in social
                   psychological research: conceptual, strategic, and
                   statistical considerations.},
  volume =        {51},
  year =          {1986},
}

@book{MacKinnon08,
  address =       {New York},
  author =        {D. {MacKinnon}},
  publisher =     {Erlbaum},
  title =         {Introduction to statistical mediation analysis},
  year =          {2008},
}

@article{MacKinnonetal07,
  author =        {D. {MacKinnon} and C. Lockwood and C. Brown and
                   W. Wang and J. Hoffman},
  journal =       {Clin Trials},
  pages =         {499--513},
  title =         {The intermediate endpoint effect in logistic and
                   probit regression.},
  volume =        {4},
  year =          {2007},
}

@incollection{Pearl10c,
  address =       {},
  author =        {J. Pearl},
  booktitle =     {Statistical causality},
  editor =        {C. Berzuini and P. Dawid and L. Bernardinelli},
  publisher =     {},
  title =         {The mediation formula: a guide to the assessment of
                   causal pathways in nonlinear models.},
  year =          {forthcoming 2011},
}

@article{Pearl10b,
  author =        {J. Pearl},
  journal =       {Int J Biostat},
  pages =         {Article 7},
  title =         {An introduction to causal inference},
  volume =        {6},
  number={2},
  year =          {2010},
}

@article{vanderLaan&Rose10,
  author =        {M.J. van der Laan and S. Rose},
  journal =       {Amstat News},
  pages =         {38--39},
  title =         {Statistics Ready for a Revolution: next Generation of
                   Statisticians Must Build Tools for Massive Data Sets},
  volume =        {399},
  year =          {2010},
}

@techreport{vanderLaan&Dudoit03,
  author =        {M.J. van der Laan and S. Dudoit},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
number={130},
  title =         {Unified cross-validation methodology for selection
                   among estimators and a general cross-validated
                   adaptive epsilon-net estimator: finite sample oracle
                   inequalities and examples},
  year =          {2003},
}




@book{vanderLaan&Robins03,
  author =        {M.J. van der Laan and J.M. Robins},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  title =         {Unified methods for censored longitudinal data and
                   causality},
  year =          {2003},
}

@book{vanderLaan&Rose11,
  author =        {M.J. van der Laan and S. Rose},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  title =         {Targeted Learning: Causal Inference for Observational and Experimental Data},
  year =          {2011},
}

@book{Bickeletal97,
  author =        {P.J. Bickel and C.A.J. Klaassen and Y. Ritov and
                   J. Wellner},
  publisher =     {Springer},
  address={Berlin Heidelberg New York},
  title =         {Efficient and adaptive estimation for semiparametric
                   models},
  year =          {1997},
}

@article{vanderLaan&Rubin06,
  author =        {M.J. van der Laan and Daniel B. Rubin},
  journal =       {Int J Biostat},
  number =        {1},
  pages =         {Article 11},
  title =         {Targeted Maximum Likelihood Learning},
  volume =        {2},
  year =          {2006},
}

@article{Stitelman&vanderLaan11a,
  author =        {O.M. Stitelman and M.J. van der Laan},
  journal =       {Int J Biostat},
  number =        {1},
  title =         {Targeted Maximum Likelihood Estimation of Effect Modification Parameters In Survival Analysis},
  volume =        {7},
  year =          {2011},
}






@article{vanderLaan&Gruber10,
  author =        {M.J. van der Laan and S. Gruber},
  journal =       {Int J Biostat},
  number =        {1},
  title =         {Collaborative Double robust penalized targeted
                   maximum likelihood estimation},
  volume =        {6},
  year =          {2010},
}

@article{Taubes07,
  author =        {G. Taubes},
  journal =       {The New York Times},
  title =         {{Do we really know what makes us healthy?}},
  year =          {2007},
}

@article{USPrev09,
  author =        {{U.S. Preventive Services Task Force}},
  journal =       {Ann Intern Med},
  number =        {10},
  pages =         {716--726},
  title =         {{Screening for breast cancer: U.S. Preventive
                   Services Task Force recommendation statement}},
  volume =        {151},
  year =          {2009},
}

@article{Freedman&Petitti&Robins04,
  author =        {D.A. Freedman and D.B. Petitti and J.M. Robins},
  journal =       {Int J Epidemiol},
  pages =         {43--55},
  title =         {{On the efficacy of screening for breast cancer}},
  volume =        {33},
  year =          {2004},
}

@book{Rothman&Greenland98,
  address =       {Philadelphia},
  author =        {K.J. Rothman and S. Greenland},
  edition =       {2nd},
  publisher =     {Lippincott, Williams \& Wilkins},
  title =         {Modern epidemiology},
  year =          {1998},
}

@book{Jewell04,
  address =       {Boca Raton},
  author =        {N.P. Jewell},
  publisher =     {Chapman \& Hall},
  title =         {Statistics for epidemiology},
  year =          {2004},
}

@book{Freedman05,
  address =       {New York},
  author =        {D.A. Freedman},
  publisher =     {Cambridge},
  title =         {Statistical models: theory and practice},
  year =          {2005},
}

@article{Ioannidis06,
  author =        {J.P.A. Ioannidis},
  journal =       {Neonatal Intensive Care J Perinatol Neonatol},
  number =        {3},
  title =         {{Why most published research findings are false}},
  volume =        {19},
  year =          {2006},
}

@book{Freedman10,
  address =       {New York},
  author =        {D.H. Freedman},
  publisher =     {Little, Brown and Company},
  title =         {Wrong: why experts keep failing us---and how to know
                   when not to trust them},
  year =          {2010},
}

@book{Box&Draper87,
  address =       {Hoboken},
  author =        {G.E.P. Box and N.R. Draper},
  publisher =     {Wiley},
  title =         {Empirical model-building and response surfaces},
  year =          {1987},
}

@article{Robins86,
  author =        {J.M. Robins},
  journal =       {Math Mod},
  number =        {},
  pages =         {1393--1512},
  title =         {A new approach to causal inference in mortality
                   studies with sustained exposure periods--application
                   to control of the healthy worker survivor effect},
  volume =        {7},
  year =          {1986},
}

@article{Tager&Hollenberg&Satariano98,
  author =        {I. Tager and M. Hollenberg and W. Satariano},
  journal =       {Am J Epidemiol},
  pages =         {921--931},
  title =         {{Self-reported leisure-time physical activity and
                   measures of cardiorespiratory fitness in an elderly
                   population}},
  volume =        {147},
  year =          {1998},
}

@manual{RCore,
  address =       {Vienna},
  author =        {{R Development Core Team}},
  organization =  {R Foundation for Statistical Computing},
  title =         {R: a language and environment for statistical
                   computing},
  year =          {2010},
  url =           {http://www.R-project.org},
}

@article{liaw:2002,
  author =        {A. Liaw and M. Wiener},
  journal =       {R News},
  number =        {3},
  pages =         {18--22},
  title =         {Classification and Regression by randomForest},
  volume =        {2},
  year =          {2002},
  url =           {http://CRAN.R-project.org/package=randomForest},
}

@article{randomForests,
  author =        {L. Breiman},
  journal =       {Mach Learn},
  pages =         {5--32},
  title =         {Random Forests},
  volume =        {45},
  year =          {2001},
}

@manual{ipred,
  author =        {A. Peters and T. Hothorn},
  note =          {R package version 0.8-8},
  title =         {ipred: Improved Predictors},
  year =          {2009},
  url =           {http://CRAN.R-project.org/package=ipred},
}

@article{breiman96bagging,
  author =        {L. Breiman},
  journal =       {Mach Learn},
  number =        {2},
  pages =         {123--140},
  title =         {Bagging Predictors},
  volume =        {24},
  year =          {1996},
}

@incollection{gam:1992,
  author =        {T.J. Hastie},
  booktitle =     {Statistical models in {S}},
  editor =        {J.M. Chambers and T.J. Hastie},
  publisher =     {Chapman \& Hall},
  title =         {Generalized additive models},
      address =       {Boca Raton},
  year =          {1992},
}

@book{gams,
  author =        {T.J. Hastie and R.J. Tibshirani},
  publisher =     {Chapman \& Hall},
  title =         {Generalized additive models},
  year =          {1990},
    address =       {Boca Raton},
}

@manual{gbm,
  author =        {G. Ridgeway},
  note =          {R package version 1.6-3},
  title =         {gbm: generalized boosted regression models},
  year =          {2007},
}

@article{friedman:2001,
  author =        {J.H. Friedman},
  journal =       {Ann Stat},
  pages =         {1189-1232},
  title =         {Greedy Function Approximation: a Gradient Boosting
                   Machine},
  volume =        {29},
  year =          {2001},
}

@book{MASS,
  address={Berlin Heidelberg New York},
  author =        {W.N. Venables and B.D. Ripley},
  edition =       {4th},
  publisher =     {Springer},
  title =         {Modern applied statistics with S},
  year =          {2002},
}

@manual{polspline,
  author =        {C. Kooperberg},
  note =          {R package version 1.1.4},
  title =         {polspline: Polynomial spline routines},
  year =          {2009},
  url =           {http://CRAN.R-project.org/package=polspline},
}

@article{MARS,
  author =        {J.H. Friedman},
  journal =       {Ann Stat},
  number =        {1},
  pages =         {1--141},
  title =         {Multivariate Adaptive Regression Splines},
  volume =        {19},
  year =          {1991},
}

@manual{bart,
  author =        {H.A. Chipman and R.E. McCulloch},
  note =          {R package version 0.3-1},
  title =         {BayesTree: {B}ayesian methods for tree-based models},
  year =          {2009},
  url =           {http://CRAN.R-project.org/package=BayesTree},
}

@article{chipman:2009,
  author =        {H.A. Chipman and E.I. George and R.E. McCulloch},
  journal =       {Ann Appl Stat},
  title =         {{BART}: {B}ayesian Additive Regression Trees},
  volume =        {4},
  number={1},
  pages={266--298},
  year =          {2010},
}

@incollection{loess,
  author =        {W.S. Cleveland and E. Groose and W.M. Shyu},
  booktitle =     {Statistical models in {S}},
  editor =        {J.M. Chambers and T.J. Hastie},
  publisher =     {Chapman \& Hall},
  title =         {Local Regression Models},
  year =          {1992},
      address =       {Boca Raton},
}

@techreport{Polley&vanderLaan10,
  author =        {E.C. Polley and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =        {266},
  title =         {Super Learner in Prediction},
  year =          {2010},
}

@book{cook:1994,
  address =       {New York},
  author =        {D. Cook and S. Weisberg},
  publisher =     {Wiley},
  title =         {An introduction to regression graphics},
  year =          {1994},
}

@article{chu:2001,
  author =        {S. Chu},
  journal =       {J Stat Educ},
  number =        {2},
  title =         {Pricing the {C}'s of diamond stones},
  volume =        {9},
  year =          {2001},
}

@book{berndt:1991,
  address =       {New York},
  author =        {E.R. Berndt},
  publisher =     {Addison--Wesley},
  title =         {The practice of econometrics},
  year =          {1991},
}

@article{kibler:1989,
  author =        {D. Kibler and D.W. Aha and M.K. Albert},
  journal =       {Comput Intell},
  pages =         {51},
  title =         {Instance-Based Prediction of Real-Valued Attributes},
  volume =        {5},
  year =          {1989},
}

@book{rosner:1999,
  address =       {Pacific Grove},
  author =        {B. Rosner},
  edition =       {5th},
  publisher =     {Duxbury},
  title =         {Fundamentals of biostatistics},
  year =          {1999},
}

@misc{newman:1998,
  author =        {D.J. Newman and S. Hettich and C.L. Blake and
                   C.J. Merz},
  institution =   {Department of
                   Information and Computer Sciences, University of California, Irvine},
  title =         {{UCI Repository of Machine Learning Databases}},
  year =          {1998},
}

@book{afifi:1979,
  address =       {New York},
  author =        {A. Afifi and S. Azen},
  edition =       {2nd},
  publisher =     {Academic},
  title =         {Statistical analysis: a computer oriented approach},
  year =          {1979},
}

@book{cook:1998,
  address =       {New York},
  author =        {D. Cook},
  publisher =     {Wiley},
  title =         {Regression graphics: ideas for studying regression
                   through graphics},
  year =          {1998},
}

@article{liu:1999,
  author =        {Z. Liu and T. Stengos},
  journal =       {J of Appl Econom},
  pages =         {527--538},
  title =         {Nonlinearities in Cross Country Growth Regressions:
                   a Semiparametric Approach},
  volume =        {14},
  year =          {1999},
}

@article{penrose:1985,
  author =        {K. Penrose and A. Nelson and A. Fisher},
  journal =       {Med Sci Sport Exer},
  pages =         {189},
  title =         {Generalized Body Composition Prediction Equation for
                   Men Using Simple Measurement Techniques},
  volume =        {17},
  year =          {1985},
}

@book{harrell:2001,
  address={Berlin Heidelberg New York},
  author =        {Harrell, Jr., F.E.},
  publisher =     {Springer},
  title =         {Regression modeling strategies with applications to
                   linear models, logistic regression, and survival
                   analysis},
  year =          {2001},
}

@manual{arm,
  author =        {A. Gelman and Y.-S. Su and M. Yajima and J. Hill and
                   M.G. Pittau and J. Kerman and T. Zheng},
  note =          {R package version 1.3-02},
  title =         {arm: data analysis using regression and
                   multilevel/hierarchical models},
  year =          {2010},
  url =           {http://CRAN.R-project.org/package=arm},
}

@article{gelman:2009,
  author =        {A. Gelman and A. Jakulin and M.G. Pittau and
                   Y.-S. Su},
  journal =       {Ann Appl Stat},
  number =        {3},
  pages =         {1360--1383},
  title =         {A Weakly Informative Default Prior Distribution for
                   Logistic and Other Regression Models},
  volume =        {2},
  year =          {2009},
}

@article{friedman:2010,
  author =        {J.H. Friedman and T.J. Hastie and R.J. Tibshirani},
  journal =       {J Stat Softw},
  number =        {1},
  title =         {Regularization Paths for Generalized Linear Models
                   via Coordinate Descent},
  volume =        {33},
  year =          {2010},
}

@manual{glmnet,
  author =        {J.H. Friedman and T.J. Hastie and R.J. Tibshirani},
  note =          {R package version 1.1-5},
  title =         {glmnet: lasso and elastic-net regularized generalized
                   linear models},
  year =          {2010},
  url =           {http://CRAN.R-project.org/package=glmnet},
}

@manual{DSA,
  author =        {R. Neugebauer and J. Bullard},
  note =          {R package version 3.1.3},
  title =         {DSA: Data-adaptive estimation with cross-validation
                   and the D/S/A algorithm},
  year =          {2009},
  url =           {http://www.stat.berkeley.edu/~laan/Software/},
}

@article{SinisivanderLaan04,
  author =        {S.E. Sinisi and M.J. van der Laan},
  journal =       {Stat Appl Genet Mol},
  note =          {Article 18},
  number =        {1},
  title =         {{D}eletion/{S}ubstitution/{A}ddition algorithm in
                   learning with applications in genomics},
  volume =        {3},
  year =          {2004},
}

@manual{svm,
  author =        {E. Dimitriadou and K. Hornik and F. Leisch and
                   D. Meyer and A. Weingessel},
  note =          {R package version 1.5-22},
  title =         {e1071: misc functions of the Department of Statistics
                   (e1071)},
  year =          {2009},
  url =           {http://CRAN.R-project.org/package=e1071},
}

@manual{Chang:2001,
  author =        {C.-C. Chang and C.-J. Lin},
  url =           {http://www.csie.ntu.edu.tw/~cjlin/libsvm},
  title =         {{LIBSVM}: a library for support vector machines},
  year =          {2001},
}

@article{vantveer:2002,
  author =        {L.J. {van't Veer} and H. Dal and M.J. {van de Vijver} and
                   Y.D. He and A.A.M. Hart and M. Mao and H.L. Peterse and
                   K. van der Kooy and M.J. Marton and A.T. Witteveen and
                   G.J. Schreiber and R.M. Kerkhoven and C. Roberts and
                   P.S. Linsley and R. Bernards and S.H. Friend},
  journal =       {Nature},
  pages =         {530--536},
  title =         {Gene Expression Profiling Predicts Clinical Outcome
                   of Breast Cancer},
  volume =        {415},
  year =          {2002},
}

@article{vanderLaan&Polley&Hubbard07,
  author =        {M.J. van der Laan and E.C. Polley and A.E. Hubbard},
  journal =       {Stat Appl Genet Mol},
  pages =        {Article 25},
  title =         {Super Learner},
  volume =        {6},
  year =          {2007},
  number =          {1},
}

@article{Wolpert92,
  author =        {D. H. Wolpert},
  journal =       {Neural Networks},
  pages =         {241--259},
  title =         {Stacked Generalization},
  volume =        {5},
  year =          {1992},
}

@article{Breiman96d,
  author =        {L. Breiman},
  journal =       {Mach Learn},
  pages =         {49--64},
  title =         {Stacked Regressions},
  volume =        {24},
  year =          {1996},
}

@article{Leblanc96,
  author =        {M. LeBlanc and R.J. Tibshirani},
  journal =       {J Am Stat Assoc},
  pages =         {1641--1650},
  title =         {Combining estimates in regression and classification},
  volume =        {91},
  year =          {1996},
}

@article{Stone74,
  author =        {M. Stone},
  journal =       {J R Stat Soc Ser B},
  number =        {2},
  pages =         {111--147},
  title =         {Cross-validatory choice and assessment of statistical
                   predictions},
  volume =        {36},
  year =          {1974},
}

@article{Geisser75,
  author =        {S. Geisser},
  journal =       {J Am Stat Assoc},
  number =        {350},
  pages =         {320--328},
  title =         {The Predictive Sample Reuse Method with Applications},
  volume =        {70},
  year =          {1975},
}

@inproceedings{Tsybakov03,
  author =        {A.B. Tsybakov},
  booktitle =     {COLT},
  editor =        {B. Sch{\"o}lkopf and M.K. Warmuth},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  series =        {Lecture Notes in Computer Science},
  title =         {Optimal rates of aggregation},
  volume =        {2777},
  year =          {2003},
}

@inproceedings{Juditskyetal05,
  author =        {A. Juditsky and A.V. Nazin and A.B. Tsybakov and
                   N. Vayatis},
  booktitle =     {NIPS},
  title =         {Generalization Error Bounds for Aggregation by Mirror
                   Descent with Averaging},
  year =          {2005},
}

@inproceedings{Buneaetal06,
  author =        {F. Bunea and A.B. Tsybakov and M.H. Wegkamp},
  booktitle =     {COLT},
  editor =        {G. Lugosi and H.-U. Simon},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  series =        {Lecture Notes in Computer Science},
  title =         {Aggregation and sparsity via {L}1 penalized least
                   squares},
  volume =        {4005},
  year =          {2006},
}

@article{Buneaetal07,
  author =        {F. Bunea and A.B. Tsybakov and M.H. Wegkamp},
  journal =       {Ann Stat},
  number =        {4},
  pages =         {1674--1697},
  title =         {Aggregation for Gaussian Regression},
  volume =        {35},
  year =          {2007},
}

@inproceedings{Buneaetal07b,
  author =        {F. Bunea and A.B. Tsybakov and M.H. Wegkamp},
  booktitle =     {COLT},
  editor =        {N.H. Bshouty and C. Gentile},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  series =        {Lecture Notes in Computer Science},
  title =         {Sparse density estimation with {L}1 penalties},
  volume =        {4539},
  year =          {2007},
}

@inproceedings{Dalalyan&Tsybakov07,
  author =        {A.S. Dalalyan and A.B. Tsybakov},
  booktitle =     {COLT},
  editor =        {N.H. Bshouty and C. Gentile},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  series =        {Lecture Notes in Computer Science},
  title =         {Aggregation by exponential weighting and sharp oracle
                   inequalities},
  volume =        {4539},
  year =          {2007},
}

@article{Dalalyan&Tsybakov08,
  author =        {A.S. Dalalyan and A.B. Tsybakov},
  journal =       {Mach Learn},
  number =        {1--2},
  pages =         {39--61},
  title =         {Aggregation by exponential weighting, sharp
                   PAC-{B}ayesian bounds and sparsity},
  volume =        {72},
  year =          {2008},
}

@book{Lehmann86,
  author =        {E.L. Lehmann},
  edition =       {2nd},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  title =         {Testing statistical hypotheses},
  year =          {1986},
}

@book{Hastie&Tibshirani&Friedman01,
  author =        {T.J. Hastie and R.J. Tibshirani and J.H. Friedman},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  title =         {The elements of statistical learning: data mining,
                   inference, and prediction},
  year =          {2001},
}

@ inproceedings{Ruczinski&Kooperberg&LeBlanc02,
  author =        {I. Ruczinski and C. Kooperberg and M. LeBlanc},
  booktitle =       {Proceedings of the MSRI workshop on Nonlinear
                   Estimation and Classification},
  editor={D. Denison and M.
                   Hansen and C. Holmes and B. Mallick and B. Yu},
  pages =         {333--344},
  title =         {Logic Regression -- methods and software},
  year =          {2002},
}



@techreport{Birkner&Hubbard&vanderLaan05,
  author =        {M.D. Birkner and A.E. Hubbard and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =        {197},
  title =         {Data Adaptive Pathway Testing},
  year =          {2005},
}

@techreport{Chaffee&Hubbard&vanderLaan10,
  author =        {P. Chaffee and A.E. Hubbard and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =        {263},
  title =         {Permutation-based Pathway Testing using the Super
                   Learner Algorithm},
  year =          {2010},
}

@inproceedings{Polley&vanderLaan09,
  author =        {E.C. Polley and M.J. van der Laan},
  booktitle =     {Design, summarization, analysis \& interpretation
                   of clinical trials with time-to-event endpoints},
  editor =        {K.E. Peace},
  publisher =     {Chapman \& Hall},
  title =         {Predicting Optimal Treatment Assignment Based on
                   Prognostic Factors in Cancer Patients},
address =       {Boca Raton},
  year =          {2009},
}

@article{vanderLaan&Dudoit&vanderVaart06,
  author =        {M.J. van der Laan and S. Dudoit and
                   A.W. van der Vaart},
  journal =       {Stat Decis},
  number =        {3},
  pages =         {373--395},
  title =         {The Cross-Validated Adaptive Epsilon-Net Estimator},
  volume =        {24},
  year =          {2006},
}

@article{vanderVaart&Dudoit&vanderLaan06,
  author =        {A.W. van der Vaart and S. Dudoit and
                   M.J. van der Laan},
  journal =       {Stat Decis},
  number =        {3},
  pages =         {351--371},
  title =         {Oracle Inequalities for Multi-Fold Cross-Validation},
  volume =        {24},
  year =          {2006},
}

@article{vanderLaan&Dudoit&Keles04,
  author =        {M.J. van der Laan and S. Dudoit and S. Kele\c{s}},
  journal =       {Stat Appl Genet Mol},
  pages =         {Article 4},
  title =         {Asymptotic optimality of likelihood-based
                   cross-validation},
  volume =        {3},
  number={1},
  year =          {2004},
}

@article{Dudoit&vanderLaan05,
  author =        {S. Dudoit and M.J. van der Laan},
  journal =       {Stat Methodol},
  number =        {2},
  pages =         {131--154},
  title =         {Asymptotics of cross-validated risk estimation in
                   estimator selection and performance assessment},
  volume =        {2},
  year =          {2005},
}

@techreport{Keles&vanderLaan&Dudoit02,
  author =        {Kele\c{s}, S. and van der Laan, M.J. and Dudoit, S.},
  institution =       {Division of Biostatistics, University of California,
                   Berkeley},
number={124},
  title =         {Asymptotically Optimal Model Selection Method for
                   Regression on Censored Outcomes},
  year =          {2002},
}

@book{Gyorfietal02,
  address={Berlin Heidelberg New York},
  author =        {L. Gy\"{o}rfi and M. Kohler and A. Krzy\.{z}ak and
                   H. Walk},
  pages =         {100--102},
  publisher =     {Springer},
  title =         {A distribution-free theory of nonparametric
                   regression},
  year =          {2002},
}

@article{Stone77,
  author =        {M. Stone},
  journal =       {Biometrika},
  number =        {1},
  pages =         {29--35},
  title =         {Asymptotics for and against cross-validation},
  volume =        {64},
  year =          {1977},
}

@book{Breimanetal84,
  author =        {L. Breiman and J.H. Friedman and R. Olshen and
                   C.J. Stone},
  publisher =     {Chapman \& Hall},
  title =         {Classification and regression trees},
  year =          {1984},
    address =       {Boca Raton},
}

@article{Breiman&Spector92,
  author =        {L. Breiman and P. Spector},
  journal =       {Int Stat Rev},
  pages =         {291--319},
  title =         {Submodel Selection and Evaluation in Regression. {T}he
                   {$X$} Random Case},
  volume =        {60},
  year =          {1992},
}

@book{Efron&Tibshirani93,
  author =        {B. Efron and R. J. Tibshirani},
  publisher =     {Chapman \& Hall},
  title =         {An Introduction to the bootstrap},
  year =          {1993},
      address =       {Boca Raton},
}

@article{Breiman96,
  author =        {L. Breiman},
  journal =       {Ann Stat},
  number =        {6},
  pages =         {2350--2383},
  title =         {Heuristics of instability and stabilization in model
                   selection},
  volume =        {24},
  year =          {1996},
}

@techreport{Breiman96c,
  author =        {L. Breiman},
  institution =   {Department of Statistics, University of California, Berkeley},
  type={Technical {R}eport},
  title =         {Out-of-bag estimation},
  year =          {1996},
}

@book{Ripley96,
  address =       {New York},
  author =        {B.D. Ripley},
  publisher =     {Cambridge},
  title =         {Pattern recognition and neural networks},
  year =          {1996},
}

@article{Breiman98,
  author =        {L. Breiman},
  journal =       {Ann Stat},
  pages =         {801--824},
  title =         {Arcing classifiers},
  volume =        {26},
  year =          {1998},
}

@article{Ambroise&McLachlan02,
  author =        {C. Ambroise and G.J. McLachlan},
  journal =       {Proc Natl Acad Sci},
  number =        {10},
  pages =         {6562--6566},
  title =         {Selection bias in gene extraction on the basis of
                   microarray gene-expression data},
  volume =        {99},
  year =          {2002},
}

@article{Pavlic&vanderLaan03,
  author =        {M. Pavlic and M.J. van der Laan},
  journal =       {Comput Stat Data An},
  pages =         {413--428},
  title =         {Fitting of mixtures with unspecified number of
                   components using cross validation distance estimate},
  volume =        {41},
  year =          {2003},
}

@inproceedings{Akaike73,
  author =        {H. Akaike},
  booktitle =     {Second International Symposium on Information Theory},
  editor =        {B.N. Petrov and F. Csaki},
  organization =  {Academiai Kiado},
  address={Budapest},
  title =         {Information theory and an extension of the maximum
                   likelihood principle},
  year =          {1973},
}

@article{Bozdogan00,
  author =        {H. Bozdogan},
  journal =       {J Math Psychol},
  pages =         {62--91},
  title =         {Akaike's information criterion and recent
                   developments in information complexity},
  volume =        {44},
  year =          {2000},
}

@article{Schwartz78,
  author =        {G. Schwartz},
  journal =       {Ann Stat},
  pages =         {461--464},
  title =         {Estimating the Dimension of a Model},
  volume =        {6},
  year =          {1978},
}

@article{Rissanen78,
  author =        {J. Rissanen},
  journal =       {Automatica},
  pages =         {465--471},
  title =         {Modelling by shortest data description},
  volume =        {14},
  year =          {1978},
}

@incollection{Bozdogan93,
  author =        {H. Bozdogan},
    address={Berlin Heidelberg New York},
  booktitle =     {Information and classification},
  editor =        {O. Opitz and B. Lausen and R. Klar},
  publisher =     {Springer},
  title =         {Choosing the number of component clusters in the
                   mixture model using a new informational complexity
                   criterion of the inverse Fisher information matrix},
  year =          {1993},
}

@article{Snowden&Rose&Mortimer11,
  author =        {J.M. Snowden and S. Rose and K.M. Mortimer},
  journal =       {Am J Epidemiol},
  number =        {00},
  pages =         {000--000},
  title =         {Implementation of G-Computation on a Simulated
                   Data set: demonstration of a Causal Inference
                   Technique},
  volume =        {173},
  year =          {2011},
}

@article{Rose&Snowden&Mortimer11,
author={S. Rose and J.M. Snowden and K.M. Mortimer},
title={Rose et al. Respond to ``{G}-Computation and Standardization in Epidemiology''},
journal={Am J Epidemiol},
volume={173},
number={00},
pages={000--000},
year={2011},
}

@incollection{Robins99b,
  author =        {Robins, J.M.},
  booktitle =     {Statistical models in epidemiology: the environment
                   and clinical trials},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  title =         {Marginal structural models versus structural nested
                   models as tools for causal inference},
  year =          {1999},
}

@article{Hernan&Brumback&Robins00,
  author =        {Hernan, M.A. and Brumback, B. and Robins, J.M.},
  journal =       {Epidemiol},
  number =        {5},
  pages =         {561--570},
  title =         {Marginal structural models to estimate the causal
                   effect of zidovudine on the survival of
                   {HIV}-positive men},
  volume =        {11},
  year =          {2000},
}

@article{Robins&Rotnitzky&vanderLaan00,
  author =        {J.M. Robins and A. Rotnitzky and M.J. van der Laan},
  journal =       {J Am Stat Assoc},
  pages =         {431--435},
  title =         {Comment on ``{O}n profile likelihood"},
  volume =        {450},
  year =          {2000},
}

@inproceedings{Robins00,
  author =        {J.M. Robins},
  booktitle =     {Proceedings of the American Statistical Association},
  editor =        {},
  organization =  {},
  pages =         {},
  title =         {Robust estimation in sequentially ignorable missing
                   data and causal inference models},
  year =          {2000},
}

@article{Robins&Rotnitzky01,
  author =        {J.M. Robins and A. Rotnitzky},
  journal =       {Stat Sinica},
  number =        {4},
  pages =         {920--936},
  title =         {Comment on the {B}ickel and {K}won article,
                   ``{I}nference for semiparametric models: some
                   questions and an answer''},
  volume =        {11},
  year =          {2001},
}

@incollection{Robins&Rotnitzky92,
  author =        {J.M. Robins and A. Rotnitzky},
  booktitle =     {AIDS epidemiology},
  publisher =     {Birkh\"{a}user},
      address={Basel},
  title =         {Recovery of information and adjustment for dependent
                   censoring using surrogate markers},
                   pages={297--331},
  year =          {1992},
}

@article{Robins&Hernan&Brumback00,
  author =        {Robins, J.M. and Hernan, M.A. and Brumback, B.},
  journal =       {Epidemiol},
  number =        {5},
  pages =         {550--560},
  title =         {Marginal structural models and causal inference in
                   epidemiology},
  volume =        {11},
  year =          {2000},
}

@article{Mortimeretal05,
  author =        {K.M. Mortimer and R. Neugebauer and M.J. van der Laan and
                   I.B. Tager},
  journal =       {Am J Epidemiol},
  number =        {4},
  pages =         {382--388},
  title =         {An Application of Model-Fitting Procedures for
                   Marginal Structural Models},
  volume =        {162},
  year =          {2005},
}

@article{Cole&Hernan08,
  author =        {S.R. Cole and M.A. Hernan},
  journal =       {Am J Epidemiol},
  pages =         {656--664},
  title =         {Constructing Inverse Probability Weights for Marginal
                   Structural Models},
  volume =        {168},
  year =          {2008},
}

@article{Bembom&vanderLaan07,
  author =        {O. Bembom and M.J. van der Laan},
  journal =       {Electron J Stat},
volume={1},
pages={574--596},
  title =         {A practical illustration of the importance of
                   realistic individualized treatment rules in causal
                   inference},
  year =          {2007},
}

@article{vanderLaan08,
  author =        {M.J. van der Laan},
  journal =       {Int J Biostat},
  volume={4},
  number={1},
pages={Article 17},
  title =         {Estimation based on case-control designs with known
                   prevalance probability},
  year =          {2008},
}

@article{Rose&vanderLaan08,
  author =        {S. Rose and M.J. van der Laan},
  journal =       {Int J Biostat},
  volume={4},
  number={1},
pages={Article 19},
  title =         {Simple optimal weighting of cases and controls in
                   case-control studies},
  year =          {2008},
}

@article{Rose&vanderLaan09,
  author =        {S. Rose and M.J. van der Laan},
  journal =       {Int J Biostat},
    volume={5},
  number={1},
pages={Article 1},
  title =         {Why match? {I}nvestigating matched case-control study
                   designs with causal effect estimation},
  year =          {2009},
}

@inproceedings{Moore&vanderLaan09,
  author =        {K.L. Moore and M.J. van der Laan},
  booktitle =     {Design, summarization, analysis \& interpretation
                   of clinical trials with time-to-event endpoints},
  editor =        {Karl E. Peace},
        address =       {Boca Raton},
  publisher =     {Chapman \& Hall},
  title =         {Application of Time-to-Event Methods in the
                   Assessment of Safety in Clinical Trials},
  year =          {2009},
}

@article{Moore&vanderLaan092,
  author =        {Moore, K.L. and van der Laan, M.J.},
  journal =       {Stat Med},
  number =        {1},
  pages =         {39--64},
  title =         {Covariate Adjustment in Randomized Trials with Binary
                   Outcomes: targeted Maximum Likelihood Estimation},
  volume =        {28},
  year =          {2009},
}

@article{Moore&vanderLaan093,
  author =        {Moore, K.L. and van der Laan, M.J.},
  journal =       {J Biopharm Stat},
  number =        {6},
  pages =         {1099--1131},
  title =         {Increasing Power in Randomized Trials with Right
                   Censored Outcomes Through Covariate Adjustment},
  volume =        {19},
  year =          {2009},
}

@article{Bembometal09b,
  author =        {O. Bembom and M.L. Petersen and S.-Y. Rhee and
                   W.J. Fessel and S.E. Sinisi and R.W. Shafer and
                   M.J. van der Laan},
  journal =       {Stat Med},
  pages =         {152--72},
  title =         {Biomarker discovery using targeted maximum likelihood
                   estimation: application to the treatment of
                   antiretroviral resistant {HIV} infection},
  volume =        {28},
  year =          {2009},
}

@article{Rosenblumetal09,
  author =        {M. Rosenblum and S.G. Deeks and M.J. van der Laan and
                   D.R. Bangsberg},
  journal =       {PLoS ONE},
  title =         {The Risk of Virologic Failure Decreases with Duration
                   of {HIV} Suppression, at Greater than 50\% Adherence to
                   Antiretroviral Therapy},
  volume =        {4(9): e7196.doi:10.1371/journal.pone.0007196},
  year =          {2009},
}

@article{Gruber&vanderLaan10a,
  author =        {S. Gruber and M.J. van der Laan},
  journal =       {Int J Biostat},
  number =        {1},
  title =         {An application of collaborative targeted maximum
                   likelihood estimation in causal inference and
                   genomics},
  volume =        {6},
  year =          {2010},
}

@article{Rosenblum&vanderLaan10,
  author =        {M. Rosenblum and M.J. van der Laan},
  journal =       {Int J Biostat},
    volume={6},
  number={2},
pages={Article 19},
  title =         {Targeted maximum likelihood estimation of the
                   parameter of a marginal structural model},
  year =          {2010},
}

@book{Dudoit&vanderLaan08,
address={Berlin Heidelberg New York},
  author =        {S. Dudoit and M.J. van der Laan},
  publisher =     {Springer},
  title =         {Resampling based multiple testing with applications
                   to genomics},
  year =          {2008},
}

@article{Robins94,
  author =        {J.M. Robins},
  journal =       {Commun Stat},
  number =        {},
  pages =         {2379--2412},
  title =         {Correcting for noncompliance in randomized trials
                   using structural nested mean models},
  volume =        {23},
  year =          {1994},
}

@article{Robins&Rotnitzky&Zhao95,
  author =        {J.M. Robins and A. Rotnitzky and L.P. Zhao},
  journal =       {J Am Stat Assoc},
  pages =         {106--121},
  title =         {Analysis of semiparametric regression models for
                   repeated outcomes in the presence of missing data.},
  volume =        {90},
  year =          {1995},
}

@article{Scharfstein&Rotnitzky&Robins99,
  author =        {D.O. Scharfstein and A. Rotnitzky and J.M. Robins},
  journal =       {J Am Stat Assoc},
  pages =         {1096-1120 (1121-1146)},
  title =         {Adjusting for Nonignorable Drop-out Using
                   Semiparametric Nonresponse Models, (with Discussion
                   and Rejoinder)},
  volume =        {94},
  year =          {1999},
}

@article{Leon&Tsiatis&Davidian03,
  author =        {S. Leon and A.A. Tsiatis and M. Davidian},
  journal =       {Biometrics},
  pages =         {1046--1055},
  title =         {Semiparametric estimation of treatment effect in a
                   pretest-posttest study},
  volume =        {59},
  year =          {2003},
}

@article{Tan06,
  author =        {Z. Tan},
  journal =       {J Am Stat Assoc},
  pages =         {1619-1637},
  title =         {A distributional approach for causal inference using
                   propensity scores},
  volume =        {101},
  year =          {2006},
}

@book{Tsiatis062,
  address={Berlin Heidelberg New York},
  author =        {A.A. Tsiatis},
  publisher =     {Springer},
  title =         {Semiparametric theory and missing data},
  year =          {2006},
}

@article{Zhang&Tsiatis&Davidian08,
  author =        {M. Zhang and A.A. Tsiatis and M. Davidian},
  journal =       {Biometrics},
  number =        {3},
  pages =         {707--715},
  title =         {Improving efficiency of inferences in randomized
                   clinical trials using auxiliary covariates},
  volume =        {64},
  year =          {2008},
}

@article{Rubin&vanderLaan08,
  author =        {Daniel B. Rubin and M.J. van der Laan},
  journal =       {Int J Biostat},
  title =         {Empirical efficiency maximization: improved locally
                   efficient covariate adjustment in randomized
                   experiments and survival analysis},
  volume =        {4},
  number={1},
  pages={Article 5},
  year =          {2008},
}

@article{Freedman08,
  author =        {D.A. Freedman},
  journal =       {Adv Appl Math},
  pages =         {180--193},
  title =         {On regression adjustments to experimental data},
  volume =        {40},
  year =          {2008},
}

@article{Freedman082,
  author =        {D.A. Freedman},
  journal =       {Ann Appl Stat},
  pages =         {176--96},
  title =         {On regression adjustments to experiments with several
                   treatments},
  volume =        {2},
  year =          {2008},
}

@article{Rosenblum&vanderLaan09,
  author =        {M. Rosenblum and M.J. van der Laan},
  journal =       {Biometrics},
  number =        {3},
  pages =         {937--945},
  title =         {Using Regression Models to Analyze Randomized Trials:
                   asymptotically Valid Hypothesis Tests Despite
                   Incorrectly Specified Models},
  volume =        {65},
  year =          {2009},
}

@book{Hampeletal86,
  author =        {Hampel, F.R. and Ronchetti, E.M. and Rousseeuw, P.J. and
                   Stahel, W.A.},
  address =       {New York},
  publisher =     {Wiley},
  title =         {{Robust statistics: the approach based on influence
                   functions}},
  year =          {1986},
}

@book{vanderVaart98,
  author =        {A.W. van der Vaart},
  publisher =     {Cambridge},
  title =         {Asymptotic statistics},
    address =       {New York},
  year =          {1998},
}

@book{vanderVaart&Wellner96,
  author =        {A.W. van der Vaart and J.A. Wellner},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  title =         {Weak convergence and empirical processes},
  year =          {1996},
}

@article{Rosenbaum&Rubin83,
  author =        {P.R. Rosenbaum and Donald B. Rubin},
  journal =       {Biometrika},
  pages =         {41--55},
  title =         {The central role of the propensity score in
                   observational studies for causal effects},
  volume =        {70},
  year =          {1983},
}

@article{Stitelman&vanderLaan10,
  author =        {O.M. Stitelman and M.J. van der Laan},
Journal={Int J Biostat},
volume={6},
number={1},
pages={Article 21},
  title =         {Collaborative Targeted Maximum Likelihood for
                   Time-to-Event Data},
  year =          {2010},
}


@article{Wedderburn74,
  author =        {R.W.M. Wedderburn},
  journal =       {Biometrika},
  pages =         {439--447},
  title =         {Quasi-likelihood functions, generalized linear
                   models, and the Gauss-Newton method},
  volume =        {61},
  number={3},
  year =          {1974},
}

@article{McCullagh83,
  author =        {P. Mc{C}ullagh},
  journal =       {Ann Stat},
  pages =         {59--67},
  title =         {Quasi-likelihood functions},
  volume =        {11},
  year =          {1983},
}

@article{vanderLaan&Petersen08,
  author =        {M.J. van der Laan and M.L. Petersen},
  journal =       {Int J Biostat},
  number =        {1},
  title =         {Direct effect models},
  volume =        {4},
  pages={Article 23},
  year =          {2008},
}

@techreport{vanderLaan10c,
  author =        {M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =        {268},
  title =         {Estimation of Causal Effects of Community-Based
                   Interventions},
  year =          {2010},
}

@article{Heckman&Ichimura&Todd97,
  author =        {J. Heckman and H. Ichimura and R. Todd},
  journal =       {Rev of Econ Stud},
  pages =         {605--654},
  title =         {Matching as an Econometric Evaluation Estimator:
                   evidence from Evaluating a Job Training Programme},
  volume =        {64},
  year =          {1997},
}

@techreport{Sekhon06,
  author =        {J.S. Sekhon},
  institution =   {University of California,
                   Berkeley},
  type={Technical {R}eport},
  title =         {Alternative balance metrics for bias reduction in
                   matching methods for causal inference},
  year =          {2006},
}

@article{Hansen08,
  author =        {B.B. Hansen},
  journal =       {Biometrika},
  pages =         {481--8},
  title =         {The prognostic analogue of the propensity score},
  volume =        {95},
  year =          {2008},
}

@book{Haignere02,
  address =       {Washington, DC},
  author =        {Haignere, L.},
  edition =       {2nd},
  publisher =     {American Association of University Professors},
  title =         {Paychecks: a guide to conducting salary-equity
                   studies for higher education faculty},
  year =          {2002},
}

@article{Holland88,
  author =        {P.W. Holland},
  journal =       {Stat Sci},
  number =        {2},
  pages =         {186--188.},
  title =         {Comment: Causal Mechanism or Causal Effect: which Is
                   Best for Statistical Science?},
  volume =        {3},
  year =          {1988},
}

@article{Robins98,
  author =        {J.M. Robins},
  journal =       {1997 Proceedings of the American Statistical
                   Association. Section on {B}ayesian Statistical Science},
  pages =         {1--10},
  title =         {Marginal Structural Models},
  year =          {1998},
}

@article{Mossetal04,
  author =        {A.R. Moss and J.A. Hahn and S. Perry and
                   E.D. Charlebois and D. Guzman and R.A. Clark and
                   D.R. Bangsberg},
  journal =       {Clin Infect Dis},
  number =        {8},
  pages =         {1190--1198},
  title =         {Adherence to highly active antiretroviral therapy in
                   the homeless population in {S}an {F}rancisco: a
                   prospective study},
  volume =        {39},
  year =          {2004},
}

@article{Bangsbergetal01,
  author =        {D.R. Bangsberg and F. Hecht and E.D. Charlebois and
                   M. Chesney and A.R. Moss},
  journal =       {AIDS Behav},
  pages =         {275--281},
  title =         {Comparing Objectives Measures of Adherence to HIV
                   Antiretroviral Therapy: electronic Medication
                   Monitors and Unannounced Pill Counts.},
  volume =        {5},
  year =          {2001},
}

@article{Neugebauer&vanderLaan07,
  author =        {R. Neugebauer and M. J. van der Laan},
  journal =       {J Stat Plan Infer},
  number =        {2},
  pages =         {419--434},
  title =         {Nonparametric causal effects based on marginal
                   structural models},
  volume =        {137},
  year =          {2007},
}

@article{Efron87,
  author =        {B. Efron},
  journal =       {J Am Stat Assoc},
  number =        {397},
  pages =         {171--185},
  title =         {Better Bootstrap Confidence Intervals},
  volume =        {82},
  year =          {1987},
}

@article{Kirschetal08,
  author =        {I. Kirsch and B.J. Deacon and T.B. Huedo-Medina and
                   A. Scoboria and T.J. Moore and B.T. Johnson},
  journal =       {PLoS Med},
  number =        {2},
  pages =         {e45. doi:10.1371/journal.pmed.0050045},
  title =         {Initial Severity and Antidepressant Benefits: a
                   Meta-Analysis of Data Submitted to the {Food and Drug
                   Administration}},
  volume =        {5},
  year =          {2008},
}

@article{Baselga01,
  author =        {J. Baselga},
  journal =       {Oncology},
  pages =         {14--21},
  title =         {Herceptin alone or in combination with chemotherapy
                   in the treatment of {HER2}-positive metastatic breast
                   cancer: pivotal trials},
  volume =        {61(S2)},
  year =          {2001},
}

@techreport{Wangetal06,
  author =        {Y. Wang and M.L. Petersen and D.R. Bangsberg and
                   M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =        {211},
  title =         {Diagnosing Bias in the Inverse Probability of
                   Treatment Weighted Estimator Resulting from Violation
                   of Experimental Treatment Assignment.},
  year =          {2006},
}

@article{Robins87,
  author =        {Robins, J.M.},
  journal =       {Comput Math Appl},
  number =        {9--12},
  pages =         {923--945},
  title =         {Addendum to: ``{A} new approach to causal inference
                   in mortality studies with a sustained exposure
                   period---application to control of the healthy worker
                   survivor effect''},
  volume =        {14},
  year =          {1987},
}

@article{Robins872,
  author =        {J.M. Robins},
  journal =       {J Chron Dis (40, Supplement)},
  pages =         {139s--161s},
  title =         {A graphical approach to the identification and
                   estimation of causal parameters in mortality studies
                   with sustained exposure periods},
  volume =        {2},
  year =          {1987},
}

@article{Rosenblum&vanderLaan09b,
  author =        {M. Rosenblum and M.J. van der Laan},
  journal =       {Int J Biostat},
  pages =         {Article 4},
  title =         {Confidence Intervals for the Population Mean Tailored
                   to Small Sample Sizes, with Applications to Survey
                   Sampling},
  volume =        {1},
  year =          {2009},
}

@article{Neugebauer&vanderLaan05,
  author =        {Neugebauer, R. and van der Laan, M.J.},
  journal =       {J Stat Plan Infer},
  number =        {1-2},
  pages =         {405--26},
  title =         {Why prefer double robust estimates},
  volume =        {129},
  year =          {2005},
}

@techreport{Mooreetal09,
  author =        {K.L. Moore and R.S. Neugebauer and M.J. van der Laan and
                   I.B. Tager},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =        {255},
  title =         {Causal Inference in Epidemiological Studies with
                   Strong Confounding},
  year =          {2009},
}

@article{Kish92,
  author =        {L. Kish},
  journal =       {J Off Stat},
  number =        {},
  pages =         {183--200},
  title =         {Weighting for unequal $P_i$},
  volume =        {8},
  year =          {1992},
}

@techreport{Bembom&vanderLaan08,
  author =        {O. Bembom and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =        {230},
  title =         {Data-adaptive selection of the truncation level for
                   Inverse-Probability-of-Treatment-Weighted estimators},
  year =          {2008},
}

@article{Freedman&Berk08,
  author =        {D.A. Freedman and R.A. Berk},
  journal =       {Eval Rev},
  pages =         {392--409},
  title =         {Weighting Regressions by Propensity Scores},
  volume =        {3},
  year =          {2008},
}

@article{Petersenetal10,
  author =        {M.L. Petersen and K.E. Porter and S. Gruber and
                   Y. Wang and M.J. van der Laan},
journal = {Stat Meth Med Res},
  title =         {Diagnosing and responding to violations in the
                   positivity assumption},
     volume =        {published online 28 Oct (doi:
                   10.1177/0962280210386207)},
  year =          {2010},
}

@article{Johnsonetal09,
  author =        {V.A. Johnson and F. Brun-Vezinet and B. Clotet and
                   H.F. Gunthard and D.R. Kuritzkes and D. Pillay and
                   J.M. Schapiro and D.D. Richman},
  journal =       {Top HIV Med},
  number =        {5},
  pages =         {138--45},
  title =         {Update of the drug resistance mutations in {HIV}-1:
                   {D}ecember 2009.},
  volume =        {17},
  year =          {2009},
}

@techreport{Bembometal08b,
  author =        {O. Bembom and W.J. Fessel and R.W. Shafer and
                   M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  type =          {231},
  title =         {Data-adaptive Selection Of The Adjustment Set In
                   Variable Importance Estimation},
  year =          {2008},
}

@techreport{Crumpetal06,
  author =        {R.K. Crump and V.J. Hotz and G.W. Imbens and
                   O.A. Mitnik},
  institution =   {National Bureau of Economic Research},
  number =        {330},
  title =         {Moving the goalposts: addressing limited overlap in
                   the estimation of average treatment effects by
                   changing the estimand},
  year =          {2006},
}

@article{LaLonde86,
  author =        {R.J. LaLonde},
  journal =       {Am Econ Rev},
  pages =         {604--620},
  title =         {Evaluating the Econometric Evaluations of Training
                   Programs with Experimental Data},
  volume =        {76},
  year =          {1986},
}

@article{Dehejia&Wahba99,
  author =        {R. Dehejia and S. Wahba},
  journal =       {J Am Stat Assoc},
  pages =         {1053--1062},
  title =         {Causal Effects in Nonexperimental Studies:
                   reevaluating the Evaluation of Training Programs},
  volume =        {94},
  year =          {1999},
}

@article{vanderLaan&Petersen07,
  author =        {M.J. van der Laan and M.L. Petersen},
  journal =       {Int J Biostat},
  number =        {1},
  pages =         {Article 3},
  title =         {Causal Effect Models for Realistic Individualized
                   Treatment and Intention to Treat Rules},
  volume =        {3},
  year =          {2007},
}

@article{Robins&Orellana&Rotnitzky08,
  author =        {J.M. Robins and L. Orellana and A. Rotnitzky},
  journal =       {Stat Med},
  pages =         {4678--4721},
  title =         {Estimation and extrapolation of optimal treatment and
                   testing strategies},
  volume =        {27},
  year =          {2008},
}

@article{Cochran57,
  author =        {W.G. Cochran},
  journal =       {Biometrics},
  number =        {},
  pages =         {261--281},
  title =         {Analysis of Covariance: its Nature and Uses.},
  volume =        {13},
  year =          {1957},
}

@techreport{Moore&vanderLaan07,
  author =        {K.L. Moore and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  month =         {April},
  number =          {215},
  title =         {Covariate adjustment in randomized trials with binary
                   outcomes},
  year =          {2007},
}

@article{Rosenblum&vanderLaan102,
  author =        {M. Rosenblum and M.J. van der Laan},
  journal =       {Int J Biostat},
  number =        {1},
  pages =         {Article 13},
  title =         {Simple, Efficient Estimators of Treatment Effects in
                   Randomized Trials Using Generalized Linear Models to
                   Leverage Baseline Variables},
  volume =        {6},
  year =          {2010},
}

@article{Freedman083,
  author =        {D.A. Freedman},
  journal =       {Stat Sci},
  pages =         {237--249},
  title =         {Randomization does not justify logistic regression},
  volume =        {23},
  year =          {2008},
}

@article{Yang&Tsiatis01,
  author =        {L. Yang and A.A. Tsiatis},
  journal =       {Am Stat},
  pages =         {29--38},
  title =         {Efficiency study for a treatment effect in a
                   pretest-posttest trial},
  volume =        {56},
  year =          {2001},
}

@book{McCullagh&Nelder89,
  address =       {Boca Raton},
  author =        {P. McCullagh and J.A. Nelder},
  edition =       {2nd},
  publisher =     {Chapman \& Hall},
  title =         {Generalized linear models},
  year =          {1989},
}

@incollection{Gail86,
  address =       {New York},
 author =        {M.H. Gail},
  booktitle =     {Modern Statistical Methods in Chronic Disease
                   Epidemiology},
  editor =        {S.~H. Moolvankar and R.~L.
                   Prentice},
  publisher =     {Wiley},
  title =         {Adjusting for covariates that have the same
                   distribution in exposed and unexposed cohorts},
  year =          {1986},
}

@article{Tsiatisetal08,
  author =        {A.A. Tsiatis and M. Davidian and M. Zhang and X. Lu},
  journal =       {Stat Med},
  pages =         {4658--4677},
  title =         {Covariate adjustment for two-sample treatment
                   comparisons in randomized clinical trials: a
                   principled yet flexible approach},
  volume =        {27},
  year =          {2008},
}

@article{Kochetal98,
  author =        {G.G. Koch and C.M. Tangen and J.W. Jung and
                   I.A. Amara},
  journal =       {Stat Med},
  pages =         {1863--1892},
  title =         {Issues for covariance analysis of dichotomous and
                   ordered categorical data from randomized clinical
                   trials and nonparametric strategies for addressing
                   them},
  volume =        {17},
  year =          {1998},
}

@article{Pococketal02,
  author =        {S.J. Pocock and S.E. Assmann and L.E. Enos and
                   L.E. Kasten},
  journal =       {Stat Med},
  pages =         {2917--2930},
  title =         {Subgroup analysis, covariate adjustment, and baseline
                   comparisons in clinical trial reporting: current
                   practice and problems.},
  volume =        {21},
  year =          {2002},
}

@article{Anderson72,
  author =        {J.A. Anderson},
  journal =       {Biometrika},
  pages =         {19--35},
  title =         {Separate sample logistic discrimination},
  volume =        {59},
  year =          {1972},
}

@article{Robins99,
  author =        {J.M. Robins},
  journal =       {Stat Sci},
  number =        {3},
  pages =         {281--293},
  title =         {[{C}hoice as an Alternative to Control in Observational
                   Studies]: Comment},
  volume =        {14},
  year =          {1999},
}

@article{Manssonetal07,
  author =        {R. Mansson and M.M. Joffe and W. Sun and S. Hennessy},
  journal =       {Am J Epidemiol},
  number =        {3},
  pages =         {332-339},
  title =         {On the Estimation and Use of Propensity Scores in
                   Case-Control and Case-Cohort Studies.},
  volume =        {166},
  year =          {2007},
}

@article{Prentice&Pyke79,
  author =        {R.L. Prentice and R. Pyke},
  journal =       {Biometrika},
  pages =         {403--411},
  title =         {Logistic disease incidence models and case-control
                   studies},
  volume =        {66},
  year =          {1979},
}

@book{Breslow&Day80,
  address =       {Lyon},
  author =        {N.E. Breslow and N.E. Day},
  publisher =     {International Agency for Research on Cancer},
  title =         {Statistical methods in cancer research: {V}olume 1 --
                   {T}he analysis of case-control studies},
  year =          {1980},
}

@article{Breslow96,
  author =        {N.E. Breslow},
  journal =       {J Am Stat Soc},
  pages =         {14--28},
  title =         {Statistics in Epidemiology: the Case-Control Study},
  volume =        {91},
  year =          {1996},
}

@article{Greenland81,
  author =        {S. Greenland},
  journal =       {J Chron Dis},
  pages =         {445--453},
  title =         {Multivariate Estimation of Exposure-Specific
                   Incidence from Case-Control Studies.},
  volume =        {34},
  year =          {1981},
}

@incollection{Holland&Rubin88,
  address =       {Cambridge, MA},
  author =        {P.W. Holland and Donald B. Rubin},
  booktitle =     {Matched sampling for causal effects.},
  editor =        {Donald B. Rubin},
  publisher =     {Cambridge},
  title =         {Causal inference in retrospective studies},
  year =          {1988},
}

@article{Greenland04,
  author =        {S. Greenland},
  journal =       {Am J Epidemiol},
  number =        {4},
  pages =         {301--305},
  title =         {Model-based Estimation of Relative Risks and Other
                   Epidemiologic Measures in Studies of Common Outcomes
                   and in Case-Control Studies.},
  volume =        {160},
  year =          {2004},
}

@article{Newman06,
  author =        {S. Newman},
  journal =       {Epid Persp Innov},
  pages =         {2},
  title =         {Causal analysis of case-control data},
  volume =        {3},
  year =          {2006},
}

@article{Cornfield51,
  author =        {J. Cornfield},
  journal =       {J Nat Cancer Inst},
  pages =         {1269--1275},
  title =         {A method of estimating comparative rates from
                   clinical data. Applications to cancer of the lung,
                   breast, and cervix.},
  volume =        {11},
  year =          {1951},
}

@inproceedings{Cornfield56,
  author =        {J. Cornfield},
    address =       {Berkeley},
  booktitle =     {Proceedings of the 3rd Berkeley symposium, {V}ol
                   IV},
  editor =        {J. Neyman},
  publisher =     {University of California Press},
  title =         {A statistical problem arising from retrospective
                   studies},
  year =          {1956},
}

@article{Prentice&Breslow78,
  author =        {R.L. Prentice and N.E. Breslow},
  journal =       {Biometrika},
  number =        {1},
  pages =         {153--158},
  title =         {Retrospective studies and failure time models.},
  volume =        {65},
  year =          {1978},
}

@article{Moriseetal96,
  author =        {A.P. Morise and G.A. Diamon and R. Detrano and
                   M. Bobbio and Erdogan Gunel},
  journal =       {Med Decis Making},
  pages =         {133--142},
  title =         {The Effect of Disease-prevalence Adjustments on the
                   Accuracy of a Logistic Prediction Model.},
  volume =        {16},
  year =          {1996},
}

@article{Wacholder96,
  author =        {S. Wacholder},
  journal =       {Epidemiol},
  number =        {2},
  pages =         {144--150},
  title =         {The Case-Control Study as Data Missing by Design:
                   estimating Risk Differences.},
  volume =        {7},
  year =          {1996},
}

@article{Rose&vanderLaan11,
  author =        {S. Rose and M.J. van der Laan},
  journal =       {Int J Biostat},
  number =        {17},
  title =         {A Targeted Maximum Likelihood Estimator for Two-Stage
                   Designs},
  volume =        {7},
  year =          {2011},
}

@article{Freedman50,
  author =        {R. Freedman},
  journal =       {Am J of Soc},
  number =        {5},
  pages =         {485--487},
  title =         {Incomplete Matching in Ex Post Facto Studies},
  volume =        {55},
  year =          {1950},
}

@article{Cochran65,
  author =        {W.G. Cochran},
  journal =       {J R Stat Soc Ser A Gen},
  number =        {2},
  pages =         {234--266},
  title =         {The Planning of Observational Studies of Human
                   Populations},
  volume =        {128},
  year =          {1965},
}

@article{Billewicz65,
  author =        {W.Z. Billewicz},
  journal =       {Biometrics},
  number =        {3},
  pages =         {623--644},
  title =         {The Efficiency of Matched Samples: an Empirical
                   Investigation},
  volume =        {21},
  year =          {1965},
}

@article{McKinlay77,
  author =        {S.M. McKinlay},
  journal =       {Biometrics},
  number =        {4},
  pages =         {725--735},
  title =         {Pair-Matching -- A reappraisal of a Popular
                   Technique},
  volume =        {33},
  year =          {1977},
}

@article{Kupperetal81,
  author =        {L.L. Kupper and J.M. Karon and D.G. Kleinbaum and
                   H. Morgenstern and D.K. Lewis},
  journal =       {Biometrics},
  pages =         {271--291},
  title =         {Matching in Epidemiologic Studies: validity and
                   Efficiency Considerations},
  volume =        {37},
  year =          {1981},
}

@article{Costanza95,
  author =        {M.C. Costanza},
  journal =       {Prev Med},
  pages =         {425--433},
  title =         {Matching},
  volume =        {24},
  year =          {1995},
}

@book{Schlesselman82,
  address =       {Oxford},
  author =        {J.J. Schlesselman},
  publisher =     {Oxford},
  title =         {Case-control studies: design, conduct, analysis},
  year =          {1982},
}

@article{Vandenbroukeetal07,
  author =        {J.P. Vandenbrouke and E. von Elm and D.G. Altman and
                   P.C. Gotzsche and C.D. Mulrow and S.J. Pocock and
                   C. Poole and J.J. Schlesselman and
                   M. Egger for the STROBE Initiative},
  journal =       {PLoS Med},
  number =        {10},
  pages =         {1628--1654},
  title =         {Strengthening the Reporting of Observational
                   Studies in Epidemiology ({STROBE}): explanation
                   and Elaboration.},
  volume =        {4},
  year =          {2007},
}

@article{Cochran53,
  author =        {W.G. Cochran},
  journal =       {Am J Public Health},
  pages =         {684--691},
  title =         {Matching in Analytical Studies},
  volume =        {43},
  year =          {1953},
}

@article{Breslowetal78,
  author =        {N.E. Breslow and N.E. Day and K.T. Halvorsen and
                   R.L. Prentice and C. Sabal},
  journal =       {Am J Epidemiol},
  number =        {4},
  pages =         {299--307},
  title =         {Estimation of Multiple Relative Risk Functions in
                   Matched Case-Control Studies},
  volume =        {108},
  year =          {1978},
}

@article{Holford&White&Kelsey78,
  author =        {T.R. Holford and C. White and J.L. Kelsey},
  journal =       {Am J Epidemiol},
  number =        {3},
  pages =         {245--255},
  title =         {Multivariate Analysis for Matched Case-Control
                   Studies},
  volume =        {107},
  year =          {1978},
}

@article{Kannel&McGee&Gordon76,
  author =        {W.B. Kannel and D. McGee and T. Gordon},
  journal =       {Am J Cardiol},
  pages =         {46--51},
  title =         {A general cardiovascular risk profile: the {F}ramingham
                   Study},
  volume =        {38},
  year =          {1976},
}

@article{Andersonetal91,
  author =        {K.M. Anderson and P.W.F. Wilson and P.M. Odell and
                   W.B. Kannel},
  journal =       {Circulation},
  pages =         {356--362},
  title =         {An updated coronary risk profile. A statement for
                   health professionals.},
  volume =        {83},
  year =          {1991},
}

@article{Ramsayetal95,
  author =        {L.E. Ramsay and I.U. Haq and P.R. Jackson and
                   W.W. Yeo},
  journal =       {Lancet},
  number =        {8988},
  pages =         {1467--1471},
  title =         {Sheffield risk and treatment table for cholesterol
                   lowering for primary prevention of coronary heart
                   disease.},
  volume =        {346},
  year =          {1995},
}

@article{Ramsayetal96,
  author =        {L.E. Ramsay and I.U. Haq and P.R. Jackson and
                   W.W. Yeo},
  journal =       {Lancet},
  number =        {9036},
  pages =         {1251},
  title =         {The {S}heffield table for primary prevention of
                   coronary heart disease: corrected.},
  volume =        {348},
  year =          {1996},
}

@article{Wilsonetal98,
  author =        {P.W.F. Wilson and R.B. D'Agostino and D. Levy and
                   A.M. Belanger and H. Silbershatz and W.B. Kannel},
  journal =       {Circulation},
  pages =         {1837--1847},
  title =         {Prediction of coronary heart disease using risk
                   factor categories},
  volume =        {97},
  year =          {1998},
}

@article{Jackson00,
  author =        {R. Jackson},
  journal =       {Br Med J},
  number =        {7236},
  pages =         {709--710},
  title =         {Updated New Zealand cardiovascular disease
                   risk-benefit prediction guide.},
  volume =        {320},
  year =          {2000},
}

@article{Gailetal89,
  author =        {M.H. Gail and L.A. Brinton and D.P. Byar and
                   D.K. Corle and S.B. Green and C. Schairer and
                   J.J. Mulvihill},
  journal =       {J Natl Cancer Inst},
  number =        {24},
  pages =         {1879--1886},
  title =         {Projecting individualized probabilities of developing
                   breast cancer for white females who are being
                   examined annually.},
  volume =        {81},
  year =          {1989},
}

@article{Costantinoetal99,
  author =        {J.P. Costantino and M.H. Gail and D. Pee and
                   S. Anderson and C.K. Redmond and J. Benichou and
                   H.S. Wieand},
  journal =       {J Natl Cancer Inst},
  number =        {18},
  pages =         {1541--1548},
  title =         {Validation studies for models projecting the risk of
                   invasive and total breast cancer incidence.},
  volume =        {91},
  year =          {1999},
}

@article{Tyrer&Duffy&Cuzick04,
  author =        {J. Tyrer and S.W. Duffy and J. Cuzick},
  journal =       {Stat Med},
  number =        {7},
  pages =         {1111--1130},
  title =         {A breast cancer prediction model incorporating
                   familial and personal risk factors},
  volume =        {23},
  year =          {2004},
}

@article{Barlowetal06,
  author =        {W.E. Barlow and E. White and R. Ballard-Barbash and
                   P.M. Vacek and L. Titus-Ernstoff and P.A. Carney and
                   J.A. Tice and D.S. Buist and B.M. Geller and
                   R. Rosenberg and B.C. Yankaskas and K. Kerlikowske},
  journal =       {J Natl Cancer Inst},
  number =        {17},
  pages =         {1204--1214},
  title =         {Prospective breats cancer risk prediction model for
                   women undergoing screening mammography.},
  volume =        {98},
  year =          {2006},
}

@article{Loprinzietal94,
  author =        {C.L. Loprinzi and J.A. Laurie and H.S. Wieand and
                   J.E. Krook and P.J. Novotny and J.W. Kugler and
                   J. Bartel and M. Law and M. Bateman and N.E. Klatt},
  journal =       {J Clin Oncol},
  number =        {3},
  pages =         {601--607},
  title =         {Prospective Evaluation of Prognostic Variables from
                   Patient-Completed Questionnaires, {N}orth {C}entral
                   {C}ancer {T}reatment {G}roup},
  volume =        {12},
  year =          {1994},
}

@manual{Therneau&Lumley09,
  author =        {T. Therneau and T. Lumley},
  note =          {R package version 2.35-8},
  title =         {survival: survival analysis, including penalised
                   likelihood},
  year =          {2009},
  url =           {http://CRAN.R-project.org/package=survival},
}

@article{Tibshirani97,
  author =        {R.J. Tibshirani},
  journal =       {Stat Med},
  pages =         {385--395},
  title =         {The Lasso Method for Variable Selection in the {C}ox
                   Model},
  volume =        {16},
  year =          {1997},
}

@article{Zhang&Lu07,
  author =        {H.H. Zhang and W. Lu},
  journal =       {Biometrika},
  number =        {3},
  pages =         {691--703},
  title =         {Adaptive Lasso for {C}ox's Proportional Hazards Model},
  volume =        {94},
  year =          {2007},
}

@article{Kooperberg&Stone&Truong95,
  author =        {C. Kooperberg and C.J. Stone and Y.K. Truong},
  journal =       {J Am Stat Assoc},
  number =        {429},
  pages =         {78--94},
  title =         {Hazard Regression},
  volume =        {90},
  year =          {1995},
}

@article{Leblanc&Crowley92,
  author =        {M. LeBlanc and J. Crowley},
  journal =       {Biometrics},
  number =        {},
  pages =         {411--425},
  title =         {Relative Risk trees for censored data},
  volume =        {48},
  year =          {1992},
}

@article{Segal88,
  author =        {M.R. Segal},
  journal =       {Biometrics},
  pages =         {35--47},
  title =         {Regression trees for censored data},
  volume =        {44},
  year =          {1988},
}

@article{Hothornetal06,
  author =        {T. Hothorn and P. Buhlmann and S. Dudoit and
                   A.M. Molinaro and M.J. van der Laan},
  journal =       {Biostatistics},
  pages =         {355--373},
  title =         {Survival Ensembles},
  volume =        {7},
  year =          {2006},
}

@article{Ishwaranetal08,
  author =        {H. Ishwaran and U.B. Kogalur and E.H. Blackstone and
                   M.S. Lauer},
  journal =       {Ann Appl Stat},
  number =        {3},
  pages =         {841--860},
  title =         {Random Survival Forests},
  volume =        {2},
  year =          {2008},
}

@article{vanHouwelingenetal06,
  author =        {H.C. van Houwelingen and T. Bruinsma and A.A.M. Hart and
                   L.J. {van't Veer} and L.F.A. Wessels},
  journal =       {Stat Med},
  pages =         {3201--3216},
  title =         {Cross-validated {C}ox Regression on Microarray Gene
                   Expression Data},
  volume =        {25},
  year =          {2006},
}

@techreport{vanderLaan&Rubin07,
  author =        {M.J. van der Laan and Daniel B. Rubin},
    institution =   {Division of Biostatistics, University of California,
                   Berkeley},
   number={226},
  title =         {A note on targeted maximum likelihood and right-censored data},
  year =          {2007},
}

@inproceedings{Robins93,
  author =        {J.M. Robins},
  booktitle =     {Proceedings of the Biopharmaceutical Section},
  organization =  {American Statistical Association},
  title =         {Information recovery and bias adjustment in
                   proportional hazards regression analysis of
                   randomized trials using surrogate markers},
  year =          {1993},
}

@incollection{Hubbard&vanderLaan&Robins99,
  address={Berlin Heidelberg New York},
  author =        {A.E. Hubbard and M.J. van der Laan and J.M. Robins},
  booktitle =     {Statistical models in epidemiology: the environment
                   and clinical trials},
  editor =        {E. Halloran, D. Berry},
   publisher =     {Springer},
  title =         {Nonparametric locally efficient estimation of the
                   treatment specific survival distributions with right
                   censored data and covariates in observational
                   studies},
  year =          {1999},
}

@article{Hernandez&Eijkemans&Steyerberg06,
  author =        {Hern\'{a}ndez, A.V. and Eijkemans, M.J. and
                   Steyerberg, E.W.},
  journal =       {Ann Epidemiol},
  number =        {1},
  pages =         {41--48},
  title =         {Randomized controlled trials With time-to-event
                   outcomes: how much does prespecified covariate
                   adjustment increase power?},
  volume =        {16},
  year =          {2006},
}

@article{Lu&Tsiatis08,
  author =        {Lu, X. and Tsiatis, A.A},
  journal =       {Biometrika},
  number =        {3},
  pages =         {679--694},
  title =         {Improving the efficiency of the log-rank test using
                   auxiliary covariates},
  volume =        {95},
  year =          {2008},
}

@article{Tangen&Koch99,
  author =        {Tangen, C.M. and Koch, G.G.},
  journal =       {J Biopharm Stat},
  number =        {2},
  pages =         {307--338},
  title =         {On-parametric analysis of covariance for hypothesis
                   testing with logrank and {W}ilcoxon scores and
                   survival-rate estimation in a randomized clinical
                   trial},
  volume =        {9},
  year =          {1999},
}

@article{Jiangetal08,
  author =        {Jiang, H. and Symanowski, J. and Paul, S. and Qu, Y. and
                   Zagar, A. and Hong, S.},
  journal =       {Stat Med},
  number =        {28},
  pages =         {5850--5860},
  title =         {The type {I} error and power of nonparametric logrank
                   and {W}ilcoxon tests with adjustment for covariates -- A
                   simulation study},
  volume =        {27},
  year =          {2008},
}

@article{Akazawa&Nakamura&Palesch97,
  author =        {Akazawa, K. and Nakamura, T. and Palesch, Y.},
  journal =       {Stat Med},
  number =        {5},
  pages =         {583--597},
  title =         {Power of logrank test and {C}ox regression model in
                   clinical trials with heterogenous samples},
  volume =        {16},
  year =          {1997},
}

@article{Westeretal10,
  author =        {C.W. Wester and A.M. Thomas and H. Bussmann and
                   S. Moyo and J.M. Gaolathe and V. Novitsky and
                   M. Essex and V. De Gruttola and R.G. Marlink},
  journal =       {AIDS},
  pages =         {S27--S36},
  title =         {Nonnucleoside reverse transcriptase inhibitor
                   outcomes among combination antiretroviral
                   therapy-treated adults in {B}otswana},
  volume =        {24},
  year =          {2010},
}

@book{Andersenetal93,
  author =        {P.K. Andersen and O. Borgan and R.D. Gill and
                   N. Keiding},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  title =         {Statistical models based on counting processes},
  year =          {1993},
}

@techreport{Rudser&LeBlanc&Emerson08,
  author =        {K. Rudser and M. LeBlanc and S.S. Emerson},
  institution={Department of Biostatistics, University of Washington},
  title =         {Estimation for Arbitrary Functionals of Survival},
  number =        {335},
  year =          {2008},
}

@article{vanderLaan10,
  author =        {van der Laan, M.J.},
  journal =       {Int J Biostat},
  pages =          {Article 2},
  number =        {2},
  title =         {Targeted maximum likelihood based causal inference:
                   Part {I}},
  volume =        {6},
  year =          {2010},
}

@article{vanderLaan10b,
  author =        {van der Laan, M.J.},
  journal =       {Int J Biostat},
  pages =          {Article 3},
  number =        {2},
  title =         {Targeted maximum likelihood based causal inference:
                   Part {II}},
  volume =        {6},
  year =          {2010},
}

@article{Sekhon08,
  author =        {J.S. Sekhon},
  journal =       {J Stat Softw},
  title =         {Multivariate and Propensity Score Matching Software
                   with Automated Balance Optimization: the Matching
                   package for {R}},
  year =          {2008},
}

@article{Holland&Reitman77,
  address =       {New York},
  author =        {J.H. Holland and J.S. Reitman},
  journal =       {SIGART Bull},
  pages =         {49--49},
  title =         {Cognitive systems based on adaptive algorithms},
  volume =        {63},
  year =          {1977},
}

@article{Koul&Susarla&vanRyzin81,
  author =        {H. Koul and V. Susarla and J. van Ryzin},
  journal =       {Ann Stat},
  pages =         {1276--88},
  title =         {Regression analysis with randomly right censored
                   data},
  volume =        {9},
  year =          {1981},
}

@article{Keiding&Hols&Green89,
  author =        {N. Keiding and C. Hols and A. Green},
  journal =       {Am J Epidemiol},
  pages =         {588--600},
  title =         {Retrospective estimation of diabetes incidence from
                   information in a current prevalent population and
                   historical mortality},
  volume =        {130},
  year =          {1989},
}

@article{Robins&Rotnitzky&Zhao94,
  author =        {J.M. Robins and A. Rotnitzky and L.P. Zhao},
  journal =       {J Am Stat Assoc},
  month =         {September},
  number =        {427},
  pages =         {846--66},
  title =         {Estimation of regression coefficients when some
                   regressors are not always observed},
  volume =        {89},
  year =          {1994},
}

@article{Robins&Rotnitzky95,
  author =        {Robins, J.M. and A. Rotnitzky},
  journal =       {J Am Stat Assoc},
  pages =         {122--129},
  title =         {Semiparametric Efficiency in Multivariate Regression
                   Models with Missing Data},
  volume =        {90},
  year =          {1995},
}

@article{Kang&Schafer07,
  author =        {J. Kang and J.L. Schafer},
  journal =       {Stat Sci},
  pages =         {523--39},
  title =         {Demystifying Double Robustness: a Comparison of
                   Alternative Strategies for Estimating a Population
                   Mean from Incomplete Data (with discussion)},
  volume =        {22},
  year =          {2007},
}

@article{Robins&Wang00,
  author =        {J.M. Robins and N. Wang},
  journal =       {Biometrika},
  pages =         {113--124},
  title =         {Inference for imputation estimators},
  volume =        {87},
  year =          {2000},
}

@techreport{Bhattacharya&Vogt07,
  author =        {Bhattacharya, J. and Vogt, W.},
  institution =          {National Bureau of
                   Economic Research},
  number={343},
  title =         {Do Instrumental Variables Belong in Propensity
                   Scores?},
  year =          {2007},
}

@techreport{Wooldridge09,
  author =        {Wooldridge, J.},
  institution={Michigan State University},
  type={Technical {R}eport},
  title =         {Should Instrumental Variables be Used as Matching
                   Variables?},
  year =          {2009},
}

@article{Pearl10,
  author =        {Pearl, J.},
  journal =       {Proceedings of Uncertainty in Artificial Intelligence},
  title =         {On a Class of Bias-Amplifying Variables that Endanger
                   Effect Estimates},
  year =          {2010},
}

@article{Holland86,
  author =        {Holland, P.W.},
  journal =       {J Am Stat Assoc},
  number =        {396},
  pages =         {945--960},
  title =         {Statistics and Causal Inference},
  volume =        {81},
  year =          {1986},
}

@book{Rubin06,
  address =       {Cambridge, MA},
  author =        {Donald B. Rubin},
  publisher =     {Cambridge},
  title =         {Matched sampling for causal effects.},
  year =          {2006},
}

@book{Rosenbaum02,
  address={Berlin Heidelberg New York},
  author =        {Rosenbaum, P.R.},
  edition =       {2nd},
  publisher =     {Springer},
  title =         {Observational studies},
  year =          {2002},
}

@article{Rubin97,
  author =        {Rubin, Donald B.},
  journal =       {Ann of Intern Med},
  number =        {8S},
  pages =         {757--763},
  title =         {Estimating causal effects from large data sets using
                   propensity scores},
  volume =        {127},
  year =          {1997},
}

@article{Christakis&Iwashyna03,
  author =        {Christakis, N.A. and Iwashyna, T.I.},
  journal =       {Soc Sci Med},
  number =        {3},
  pages =         {465--475},
  title =         {The Health Impact of Health Care on Families: a
                   matched cohort study of hospice use by decedents and
                   mortality outcomes in surviving, widowed spouses},
  volume =        {57},
  year =          {2003},
}

@article{Dehejia&Wahba02,
  author =        {R. Dehejia and S. Wahba},
  journal =       {Rev Econ Stat},
  number =        {1},
  pages =         {151--161},
  title =         {Propensity Score Matching Methods for Nonexperimental
                   Causal Studies},
  volume =        {84},
  year =          {2002},
}

@article{Galiani&Gertler&Schargrodsky05,
  author =        {Galiani, S. and P. Gertler and E. Schargrodsky},
  journal =       {J Polit Econ},
  number =        {1},
  pages =         {83--120},
  title =         {Water for Life: the Impact of the Privatization of
                   Water Services on Child Mortality},
  volume =        {113},
  year =          {2005},
}

@article{Abadie&Imbens06,
  author =        {Abadie, A. and G.W. Imbens},
  journal =       {Econometrica},
  pages =         {235--267},
  title =         {Large Sample Properties of Matching Estimators for
                   Average Treatment Effects},
  volume =        {74},
  year =          {2006},
}

@article{Herron&Wand07,
  author =        {Herron, M.C. and J. Wand},
  journal =       {Elect Stud},
  number =        {2},
  pages =         {247--261},
  title =         {Assessing Partisan Bias in Voting Technology: the
                   Case of the 2004 {N}ew {H}ampshire Recount},
  volume =        {26},
  year =          {2007},
}

@article{Imai05,
  author =        {K. Imai},
  journal =       {Am Polit Sci Rev},
  number =        {2},
  pages =         {283--300},
  title =         {Do Get-Out-The-Vote Calls Reduce Turnout? The
                   Importance of Statistical Methods for Field
                   Experiments},
  volume =        {99},
  year =          {2005},
}

@incollection{Sekhon08b,
  address =       {New York},
  author =        {Sekhon, J.S.},
  booktitle =     {The Oxford handbook of political methodology},
  editor =        {J.M. Box-Steffensmeier and H.E. Brady and
                   D. Collier},
  publisher =     {Oxford},
  title =         {The {N}eyman-{R}ubin Model of Causal Inference and
                   Estimation via Matching Methods},
  year =          {2008},
}

@article{Morgan&Harding06,
  author =        {Morgan, S.L. and D.J. Harding},
  journal =       {Sociol Meth Res},
  number =        {1},
  pages =         {3--60},
  title =         {Matching Estimators of Causal Effects: prospects and
                   Pitfalls in Theory and Practice},
  volume =        {35},
  year =          {2006},
}

@article{Diprete&Engelhardt04,
  author =        {Diprete, T.A. and H. Engelhardt},
  journal =       {Sociol Meth Res},
  number =        {4},
  pages =         {501--528},
  title =         {Estimating Causal Effects With Matching Methods in
                   the Presence and Absence of Bias Cancellation},
  volume =        {32},
  year =          {2004},
}

@article{Winship&Morgan99,
  author =        {Winship, C. and S.L. Morgan},
  journal =       {Annu Rev Sociol},
  pages =         {659--707},
  title =         {The estimation of causal effects from observational
                   data},
  volume =        {25},
  year =          {1999},
}

@article{Smith97,
  author =        {Smith, H.L.},
  journal =       {Sociol Meth},
  pages =         {305--353},
  title =         {Matching with Multiple Controls to Estimate Treatment
                   Effects in Observational Studies},
  volume =        {27},
  year =          {1997},
}

@article{Rubin02,
  author =        {Rubin, Donald B.},
  journal =       {Health Serv Outcome Res Meth},
  number =        {1},
  pages =         {169--188},
  title =         {Using Propensity Scores to Help Design Observational
                   Studies: application to the Tobacco Litigation},
  volume =        {2},
  year =          {2002},
}

@incollection{Brady08,
  address =       {New York},
  author =        {Brady, H.},
  booktitle =     {The Oxford handbook of political methodology},
  editor =        {J.M. Box-Steffensmeier and H.E. Brady and
                   D. Collier},
  publisher =     {Oxford},
  title =         {Causation and explanation in social science},
  year =          {2008},
}

@article{Freedman06,
  author =        {Freedman, D.A.},
  journal =       {Eval Rev},
  pages =         {691--713},
  title =         {Statistical Models for Causation: what Inferential
                   leverage Do They Provide?},
  volume =        {30},
  year =          {2006},
}

@article{Rubin90,
  author =        {Rubin, Donald B.},
  journal =       {Stat Sci},
  number =        {4},
  pages =         {472--480},
  title =         {Comment: {N}eyman (1923) and Causal Inference in
                   Experiments and Observational Studies},
  volume =        {5},
  year =          {1990},
}

@article{Speed90,
  author =        {T.P. Speed},
  journal =       {Stat Sci},
  number =        {4},
  pages =         {463--464},
  title =         {Introductory Remarks on {N}eyman (1923)},
  volume =        {5},
  year =          {1990},
}

@book{Cox58,
  address =       {New York},
  author =        {Cox, D.R.},
  publisher =     {Wiley},
  title =         {Planning of experiments},
  year =          {1958},
}

@article{Rubin78,
  author =        {Donald B. Rubin},
  journal =       {Ann Stat},
  number =        {},
  pages =         {34--58},
  title =         {Bayesian Inference for causal effects: the role of
                   randomization},
  volume =        {6},
  year =          {1978},
}

@incollection{Rubin75,
  address =       {Alexandria},
  author =        {Rubin, Donald B.},
  booktitle =     {The proceedings of the Social Statistics Section of
                   the American Statistical Association},
  publisher =     {American Statistical Association},
  title =         {Bayesian Inference for Causality: the Importance of
                   Randomization},
  year =          {1975},
}

@article{Rubin08,
  author =        {Rubin, Donald B.},
  journal =       {Ann of Appl Stat},
  number =        {3},
  pages =         {808--840},
  title =         {For Objective Causal Inference, Design Trumps
                   Analysis},
  volume =        {2},
  year =          {2008},
}

@article{Sekhon10,
  author =        {Sekhon, J.S.},
  journal =       {Annu Rev of Polit Sci},
  pages =         {487--508},
  title =         {Opiates for the Matches: matching Methods for Causal
                   Inference},
  volume =        {12},
  year =          {2010},
}

@article{Rubin76,
  author =        {Rubin, Donald B.},
  journal =       {Biometrics},
  number =        {1},
  pages =         {121--132},
  title =         {Multivariate Matching Methods That are Equal Percent
                   Bias Reducing, {II}: maximums on Bias Reduction for
                   Fixed Sample Sizes},
  volume =        {32},
  year =          {1976},
}

@article{Cochran&Rubin73,
  author =        {Cochran, W.G. and Donald B. Rubin},
  journal =       {Sankhya Ser A},
  pages =         {417--446},
  title =         {Controlling Bias in Observational Studies: a Review},
  volume =        {35},
  year =          {1973},
}

@book{Cochran83,
  address =       {New York},
  author =        {Cochran, W.G.},
  note =          {Edited posthumously by L.E. Moses and F. Mosteller},
  publisher =     {Wiley},
  title =         {Planning and analysis of observational studies},
  year =          {1983},
}

@article{Robinsetal07,
  author =        {J.M. Robins and M. Sued and Q. Lei-Gomez and
                   A. Rotnitzky},
  journal =       {Stat Sci},
  pages =         {544--559},
  title =         {Comment: {P}erformance of Double-Robust Estimators When
                   ``Inverse Probability'' Weights Are Highly Variable},
  volume =        {22},
  year =          {2007},
}

@article{Cortes&Vapnik95,
  author =        {C. Cortes and V. Vapnik},
  journal =       {Mach Learn},
  month =         {December},
  pages =         {273--297},
  title =         {Support-vector networks},
  volume =        {20},
  year =          {1995},
}

@techreport{Friedman94,
  author =        {J.H. Friedman},
  institution =   {Department of Statistics, Stanford University},
  type={Technical {R}eport},
  title =         {Flexible metric nearest neighbor classification},
  year =          {1994},
}

@techreport{FDA06,
  author =        {{Food and Drug Administration}},
  institution =   {U.S. Department of Health and Human Services, Food
                   and Drug Administration},
  type={Technical {R}eport},
  title =         {Critical Path Opportunities List},
  year =          {2006},
}

@article{Efronetal04,
  author =        {B. Efron and T. Hastie and I. Johnstone and
                   R. Tibshirani},
  journal =       {Ann Stat (with discussion)},
  number =        {2},
  pages =         {407--499},
  title =         {Least Angle Regression},
  volume =        {32},
  year =          {2004},
}

@techreport{Breiman99,
  author =        {L. Breiman},
  institution =   {Department of Statistics, University of California, Berkeley},
  number =        {567},
  title =         {Random forests - random features},
  year =          {1999},
}

@manual{Breiman01b,
  author =        {L. Breiman},
  title =         {Notes on setting up, using, and understanding random
                   forests V3.0},
  year =          {2001},
}

@article{Golubetal99,
  author =        {T.R. Golub and D.K. Slonim and P. Tamayo and C. Huard and
                   M. Gaasenbeek and J.P. Mesirov and H. Coller and
                   M.L. Loh and J.R. Downing and M.A. Caligiuri and
                   C.D. Bloomfield and E.S. Lander},
  journal =       {Science},
  pages =         {531--537},
  title =         {Molecular classification of cancer: class discovery
                   and class prediction by gene expression monitoring},
  volume =        {286},
  year =          {1999},
}

@article{vanderLaan06a,
  author =        {M.J. van der Laan},
  journal =       {Int J Biostat},
  number =        {1},
  pages =         {Article 2},
  title =         {Statistical Inference for Variable Importance},
  volume =        {2},
  year =          {2006},
}

@article{Robins&Mark&Newey92,
  author =        {J.M. Robins and S.D. Mark and W.K. Newey},
  journal =       {Biometrics},
  number =        {479--495},
  title =         {Estimating exposure effects by modelling the
                   expectation of exposure conditional on confounders},
  volume =        {48},
  year =          {1992},
}

@techreport{Yu&VanderLaan03,
  author =        {Z. Yu and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number={136},
  title =         {Measuring treatment effects using semiparametric
                   models},
  year =          {2003},
}

@techreport{Tuglus&vanderLaan08,
  author =        {C. Tuglus and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
number={233},
  title =         {Targeted Methods for Biomarker Discovery, the Search
                   for a Standard},
  year =          {2008},
}

@book{Hastie&Tibshirani90,
  address =       {London},
  author =        {T.J. Hastie and R.J. Tibshirani},
  publisher =     {Chapman \& Hall},
  title =         {Generalized additive models},
  year =          {1990},
}

@misc{Efron&Hastie07,
  author =        {B. Efron and T. Hastie},
  howpublished =  {R package},
  title =         {lars},
  year =          {2007},
}

@article{Benjamini&Hochberg95,
  author =        {Y. Benjamini and Y. Hochberg},
  journal =       {J R Stat Soc Ser B},
  pages =         {289--300},
  title =         {Controlling the false discovery rate: a practical and
                   powerful approach to multiple testing},
  volume =        {57},
  year =          {1995},
}

@misc{Ge&Dudoit02,
  author =        {Y. Ge and S. Dudoit},
  howpublished =  {R package},
  title =         {Multiple Testing Procedures, multtest},
  year =          {2002},
  url =           {www.bioconductor.org},
}

@article{Tibshirani96,
  author =        {R. Tibshirani},
  journal =       {J R Stat Soc Ser B},
  number =        {1},
  pages =         {267--288},
  title =         {Regression shrinkage and selection via the lasso.},
  volume =        {58},
  year =          {1996},
}

@article{Tuglus&vanderLaan09,
  author =        {C. Tuglus and M.J. van der Laan},
  journal =       {Stat Appl Genet Mol},
  number =        {1},
  pages =         {Article 12},
  title =         {Modified {FDR} Controlling Procedure for Multi-Stage
                   Analyses},
  volume =        {8},
  year =          {2009},
}

@article{Dudoit&Fridlyand&Speed02,
  author =        {S. Dudoit and J. Fridlyand and T. P. Speed},
  journal =       {J Am Stat Assoc},
  number =        {457},
  pages =         {77--87},
  title =         {Comparison of Discrimination Methods for the
                   Classification of Tumors Using Gene Expression Data},
  volume =        {97},
  year =          {2002},
}

@article{Kos&Lah98,
  author =        {J. Kos and T.T. Lah},
  journal =       {Oncol Rep},
  number =        {6},
  pages =         {1349--61},
  title =         {Cysteine proteinases and their endogenous inhibitors:
                   target proteins for prognosis, diagnosis and therapy
                   in cancer (review)},
  volume =        {5},
  year =          {1998},
}

@article{Vitaleetal01,
  author =        {C. Vitale and C. Romagnani and A. Puccetti and
                   D. Olive and R. Costello and L. Chiossone and
                   A. Pitto and A. Bacigalupo and L. Moretta and
                   M.C. Mingari},
  journal =       {Proc Natl Acad Sci},
  pages =         {5764--5769},
  title =         {Surface expression and function of p75/{AIRM}-1 or {CD}33
                   in acute myeloid leukemias: engagement of {CD}33
                   induces apoptosis of leukemic cells},
  volume =        {98},
  year =          {2001},
}

@article{Clappieretal07,
  author =        {E. Clappier and W. Cuccuini and A. Kalota and
                   A. Crinquette and J.M. Cayuela and W.A. Dik and
                   A.W. Langerak and B. Montpellier and B. Nadel and
                   P. Walrafen and O. Delattre and A. Aurias and
                   T. Leblanc and H. Dombret and A.M. Gewirtz and
                   A. Baruchel and F. Sigaux and J. Soulier},
  journal =       {Blood},
  number =        {4},
  pages =         {1251--61},
  title =         {The {C-MYB} locus is involved in chromosomal
                   translocation and genomic duplications in human
                   T-cell acute leukemia ({T-ALL}), the translocation
                   defining a new {T-ALL} subtype in very young children},
  volume =        {110},
  year =          {2007},
}

@article{Lane&Ley03,
  author =        {A.A. Lane and T.J. Ley},
  journal =       {Cell},
  number =        {305-318},
  title =         {Neutrophil elastase cleaves {PML-RAR}-alpha and is
                   important for the development of acute promyelocytic
                   leukemia in mice},
  volume =        {115},
  year =          {2003},
}

@article{Hunger96,
  author =        {S.P. Hunger},
  journal =       {Blood},
  pages =         {1211--1224},
  title =         {Chromosomal translocations involving the {E2A} gene in
                   acute lymphoblastic leukemia: clinical features and
                   molecular pathogenesis.},
  volume =        {87},
  year =          {1996},
}

@article{Nebraletal05,
  author =        {K. Nebral and H.H. Schmidt and O.A. Haas and
                   S. Strehl},
  journal =       {Clin Cancer Res},
  number =        {18},
  pages =         {6489--6494},
  title =         {{NUP}98 Is Fused to Topoisomerase {(DNA)} {II}{beta} 180
                   {kDa} {(TOP2B)} in a Patient with Acute Myeloid Leukemia
                   with a New {t(3;11)(p24;p15)}},
  volume =        {11},
  year =          {2005},
}

@article{Kaufmannetal98b,
  author =        {S.H. Kaufmann and S.D. Gore and C.B. Miller and
                   R.J. Jones and L.A. Zwelling and E. Schneider and
                   P.J. Burke and J.E. Karp},
  journal =       {Leukemia Lymphoma},
  month =         {Apr},
  number =        {3-4},
  pages =         {217--237},
  title =         {Topoisomerase {II} and the response to antileukemic
                   therapy},
  volume =        {29},
  year =          {1998},
}

@article{Kozaretal04,
  author =        {K. Kozar and M.A. Ciemerych and V.I. Rebel and
                   H. Shigematsu and A. Zagozdzon and E. Sicinska and
                   Y. Geng and Q. Yu and S. Bhattacharya and
                   R.T. Bronson and K. Akashi and P. Sicinski},
  journal =       {Cell},
  pages =         {477--491},
  title =         {Mouse development and cell proliferation in the
                   absence of {D}-cyclins},
  volume =        {118},
  year =          {2004},
}

@article{MartinSuberoetal07,
  author =        {J.I. Martin-Subero and R. Ibbotson and W. Klapper and
                   L. Michaux and E. Callet-Bauchu and F. Berger and
                   M.J. Calasanz and C. De Wolf-Peeters and M.J. Dyer and
                   P. Felman and A. Gardiner and R.D. Gascoyne and
                   S. Gesk and L. Harder and D.E. Horsman and M. Kneba and
                   R. Kuppers and A. Majid and N. Parry-Jones and
                   M. Ritgen and M. Salido and F. Sole and G. Thiel and
                   H.H. Wacker and D. Oscier and I. Wlodarska and
                   R. Siebert},
  journal =       {Leukemia},
  number =        {7},
  pages =         {1532--1544},
  title =         {A comprehensive genetic and histopathologic analysis
                   identifies two subgroups of {B}-cell malignancies
                   carrying a t(14;19)(q32;q13) or variant
                   {BCL3}-translocation},
  volume =        {21},
  year =          {2007},
}

@article{Palomeroetal06,
  author =        {T. Palomero and D.T. Odom and J. O'Neil and
                   A.A. Ferrando and A. Margolin and D.S. Neuberg and
                   S.S. Winter and R.S. Larson and W. Li and X.S. Liu and
                   R.A. Young and A.T. Look},
  journal =       {Blood},
  number =        {3},
  pages =         {986--992},
  title =         {Transcriptional regulatory networks downstream of
                   {TAL1/SCL} in {T}-cell acute lymphoblastic leukemia},
  volume =        {108},
  year =          {2006},
}

@article{Wongetal07,
  author =        {H.P. Wong and L. Yu and E.K. Lam and E.K. Tai and
                   W.K. Wu and C.H. Cho},
  journal =       {Toxicol Appl Pharm},
  number =        {3},
  pages =         {261--267},
  title =         {Nicotine promotes cell proliferation via
                   alpha7-nicotinic acetylcholine receptor and
                   catecholamine-synthesizing enzymes-mediated pathway
                   in human colon adenocarcinoma {HT}-29 cells.},
  volume =        {221},
  year =          {2007},
}

@article{Ramaswamyetal03,
  author =        {S. Ramaswamy and K.N. Ross and E.S. Lander and
                   T.R. Golub},
  journal =       {Nat Genet},
  pages =         {49--54},
  title =         {A molecular signature of metastasis in primary solid
                   tumors},
  volume =        {33},
  year =          {2003},
}

@article{Purietal01,
  author =        {R. Puri and A. Tousson and L. Chen and S.S. Kakar},
  journal =       {Cancer Lett},
  pages =         {131--139},
  title =         {Molecular cloning of pituitary tumor transforming
                   gene 1 from ovarian tumors and its expression in
                   tumors},
  volume =        {163},
  year =          {2001},
}

@article{Fujiietal06,
  author =        {T. Fujii and S. Nomoto and K. Koshikawa and Y.Yatabe and
                   O. Teshigawara and T. Mori and S. Inoue and S. Takeda and
                   A. Nakao},
  journal =       {Hepatology},
  pages =         {1267--1275},
  title =         {Overexpression of pituitary tumor transforming gene 1
                   in {HCC} is associated with angiogenesis and poor
                   prognosis},
  volume =        {43},
  year =          {2006},
}

@article{Zhuetal06,
  author =        {X. Zhu and Z. Mao and Y. Na and Y. Guo and X. Wang and
                   D. Xin},
  journal =       {Anticancer Res},
  pages =         {1253--1259},
  title =         {Significance of pituitary tumor transforming gene 1
                   ({PTTG1}) in prostate cancer},
  volume =        {26},
  year =          {2006},
}

@article{Kaufmannetal98a,
  author =        {S.H. Kaufmann and J.E. Karp and P.A. Svingen and
                   S. Krajewski and P.J. Burke and S.D. Gore and
                   J.C. Reed},
  journal =       {Blood},
  number =        {3},
  pages =         {991--1000},
  title =         {Elevated expression of the apoptotic regulator {Mcl}-1
                   at the time of leukemic relapse},
  volume =        {91},
  year =          {1998},
}

@article{Frumanetal99,
  author =        {D.A. Fruman and S.B. Snapper and C.M. Yballe and
                   L. Davidson and J.Y. Yu and F.W. Alt and
                   L.C. Cantley},
  journal =       {Science},
  pages =         {393--397},
  title =         {Impaired {B} cell development and proliferation in
                   absence of phosphoinositide 3-kinase p85-alpha},
  volume =        {283},
  year =          {1999},
}

@article{Tombes&Krystal97,
  author =        {R.M. Tombes and G.W. Krystal},
  journal =       {Biochim Biophys Acta},
  pages =         {281--292},
  title =         {Identification of novel human tumor cell-specific
                   {CaMK-II} variants},
  volume =        {1355},
  year =          {1997},
}

@article{Senturkeretal97,
  author =        {S. Senturker and B. Karahalil and M. Inal and
                   H. Yilmaz and H. Muslumanoglu and G. Gedikoglu and
                   M. Dizdaroglu},
  journal =       {FEBS Letters},
  number =        {3},
  pages =         {286--290},
  title =         {Oxidative {DNA} base damage and antioxidant enzyme
                   levels in childhood acute lymphoblastic leukemia},
  volume =        {416},
  year =          {1997},
}

@article{Komuroetal05,
  author =        {I. Komuro and T. Yasuda and A. Iwamoto and
                   K.S. Akagawa},
  journal =       {J Biol Chem},
  number =        {50},
  pages =         {41137--45},
  title =         {Catalase plays a critical role in the {CSF}-independent
                   survival of human macrophages via regulation of the
                   expression of {BCL}-2 family},
  volume =        {280},
  year =          {2005},
}

@article{Balciunaiteetal05,
  author =        {E. Balciunaite and A. Spektor and N.H. Lents and
                   H. Cam and H. Te Riele and A. Scime and M.A. Rudnicki and
                   R. Young and B.D. Dynlacht},
  journal =       {Mol Cell Biol},
  number =        {18},
  pages =         {8166--78},
  title =         {Pocket protein complexes are recruited to distinct
                   targets in quiescent and proliferating cells},
  volume =        {25},
  year =          {2005},
}

@article{Leoneetal01,
  author =        {G. Leone and R. Sears and E. Huang and R. Rempel and
                   F. Nuckolls and C.H. Park and P. Giangrande and L. Wu and
                   H.I. Saavedra and S.J. Field and M.A. Thompson and
                   H. Yang and Y. Fujiwara and M.E. Greenberg and
                   S. Orkin and C. Smith and J.R. Nevins},
  journal =       {Mol Cell},
  pages =         {105--113},
  title =         {Myc requires distinct {E2F} activities to induce {S}
                   phase and apoptosis},
  volume =        {8},
  year =          {2001},
}

@article{Sax23,
  author =        {Sax, K.},
  journal =       {Genetics},
  title =         {The association of size difference with seed-coat
                   pattern and pigmentation in \textit{Phaseolus
                   vulgaris}},
  year =          {1923},
}

@article{Thoday60,
  author =        {Thoday, J.M.},
  journal =       {Nature},
  title =         {Location of polygenes},
  year =          {1960},
}

@article{Lander&Botstein89,
  author =        {Lander, E.S. and Botstein, D.},
  journal =       {Genetics},
  title =         {Mapping {M}endelian factors underlying quantitative
                   traits using {RFLP} linkage maps},
  year =          {1989},
}

@article{Haley&Knott92,
  author =        {Haley, C.S. and Knott, S.A.},
  journal =       {Heredity},
  title =         {A simple regression method for mapping quantitative
                   trait loci in line crosses using flanking markers},
  year =          {1992},
}

@article{Jansen93,
  author =        {Jansen, R.C.},
  journal =       {Genetics},
  title =         {Interval mapping of multiple quantitative trait loci},
  year =          {1993},
}

@article{Zeng94,
  author =        {Zeng, Z.B.},
  journal =       {Genetics},
  title =         {Precision mapping of quantitative trait loci},
  year =          {1994},
}

@article{Kao&Zeng&Teasdale99,
  author =        {Kao, C.H. and Zeng, Z.B. and Teasdale, R.D.},
  journal =       {Genetics},
  title =         {Multiple interval mapping for quantitative trait
                   loci},
  year =          {1999},
}

@article{Satagopanetal96,
  author =        {Satagopan, J.M. and B.S. Yandell and M.A. Newton and
                   T.C. Osborn},
  journal =       {Genetics},
  title =         {A {B}ayesian approach to detect quantitative trait loci
                   using {M}arkov chain {M}onte {C}arlo},
  year =          {1996},
}

@article{Heath97,
  author =        {Heath, S.C.},
  journal =       {Am J Hum Genet},
  title =         {Markov chain {M}onte {C}arlo segregation and linkage
                   analysis of oligogenic models},
  year =          {1997},
}

@article{Sillanpaa&Arjas98,
  author =        {Sillanpaa, M.J. and Arjas, E.},
  journal =       {Genetics},
  title =         {Bayesian mapping of multiple quantitative trait loci
                   from incomplete inbred line cross data},
  year =          {1998},
}

@article{Leeetal08,
  author =        {Lee, S.S.F. and L. Sun and R. Kustra and S.B. Bull},
  journal =       {Bioinformatics},
  title =         {{EM}-random forest and new measures of variable
                   importance for multi-locus quantitative trait linkage
                   analysis},
  year =          {2008},
}

@article{Wang&Rose&vanderLaan10,
  author =        {H. Wang and S. Rose and M.J. van der Laan},
  journal =       {Stat Prob Lett},
  title =         {Finding quantitative Trait Loci Genes with
                   Collaborative Targeted Maximum Likelihood Learning},
  volume =        {published online 11 Nov (doi:
                   10.1016/j.spl.2010.11.001)},
  year =          {2010},
}

@techreport{Wang&Rose&vanderLaan11,
  author =        {H. Wang and S. Rose and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  type =          {Technical {R}eport},
  title =         {Targeted Methods for Finding Quantitative Trait Loci},
  year =          {2011},
}

@manual{Basten&Weir&Zeng01,
  author =        {C.J. Basten and B.S. Weir and Z.B. Zeng},
  title =         {QTL Cartographer},
  year =          {2001},
  url =           {http://statgen.ncsu.edu/qtlcart/},
}

@article{Masindeetal01,
  author =        {Masinde, G.L. and X. Li and W. Gu and H. Davidson and
                   S. Mohan and D.J. Baylink},
  journal =       {Genome Res},
  title =         {Identification of wound healing/regeneration
                   quantitative trait loci ({QTL}) at multiple time points
                   that explain seventy percent of variance in ({MRL/MpJ
                   and SJL/J}) mice {F2} population},
  year =          {2001},
}

@article{Boyartchuk01,
  author =        {Boyartchuk, V.L. and K.W. Broman and R.E. Mosher and
                   S.E.F. D'Orazio and M.N. Starnbach and W.F. Dietrich},
  journal =       {Nat Genet},
  title =         {Multigenic control of Listeria monocytogenes
                   susceptibility in mice},
  year =          {2001},
}

@article{Broman03,
  author =        {Broman, K.W.},
  journal =       {Genetics},
  title =         {Mapping quantitative trait loci in the case of a
                   spike in the phenotype distribution},
  year =          {2003},
}

@article{Jin&Fine&Yandell07,
  author =        {Jin, C. and J.P. Fine and B.S. Yandell},
  journal =       {J Am Stat Assoc},
  title =         {A unified semiparametric framework for quantitative
                   trait loci analysis, with application to spike
                   phenotypes},
  year =          {2007},
}

@article{Petersenetal08,
  author =        {M.L. Petersen and M.J. van der Laan and S. Napravnik and
                   J.J. Eron and R.D. Moore and S.G. Deeks},
  journal =       {AIDS},
  number =        {16},
  pages =         {2097--106},
  title =         {Long-term consequences of the delay between virologic
                   failure of highly active antiretroviral therapy and
                   regimen modification},
  volume =        {22},
  year =          {2008},
}

@article{Rodgeretal09,
  author =        {A.J. Rodger and Z. Fox and J.D. Lundgren and
                   J.L. Kuller and C. Boesecke and D. Gey and
                   A. Skoutelis and M.B. Goetz and A.N. Phillips and
                     {INSIGHT Strategies for Management of Antiretroviral
  Therapy (SMART) Study Group}},
  journal =       {J Infect Dis},
  number =        {6},
  pages =         {973--83},
  title =         {Activation and coagulation biomarkers are independent
                   predictors of the development of opportunistic
                   disease in patients with {HIV} infection.},
  volume =        {200},
  year =          {2009},
}

@article{Hammeretal08,
  author =        {S.M. Hammer and J.J. Eron and P. Reiss and
                   R.T. Schooley and M.A. Thompson and S. Walmsley and
                   P. Cahn and M.A. Fischl and J.M. Gatell and
                   M.S. Hirsch and D.M. Jacobsen and J.S.G. Montaner and
                   D.D. Richman and P.G. Yeni and P.A. Volberding},
  journal =       {J Am Med Asoc},
  number =        {5},
  pages =         {555--70},
  title =         {Antiretroviral treatment of adult {HIV} infection:
                   2008 recommendations of the {I}nternational {AIDS}
                   {S}ociety-{USA} panel},
  volume =        {300},
  year =          {2008},
}

@article{Stringeretal06,
  author =        {J.S. Stringer and I. Zulu and J. Levy and
                   E.M. Stringer and A. Mwango and B.H. Chi and
                   V. Mtonga and S. Reid and R.A. Cantrell and
                   M. Bulterys and M.S. Saag and R.G. Marlink and
                   A. Mwinga and T.V. Ellerbrock and M. Sinkala},
  journal =       {J Am Med Asoc},
  number =        {7},
  pages =         {782--93},
  title =         {Rapid scale-up of antiretroviral therapy at primary
                   care sites in {Z}ambia: feasibility and early outcomes},
  volume =        {296},
  year =          {2006},
}

@misc{WHO06,
  author =        {{{W}orld {H}ealth {O}rganization}},
  title =         {Antiretroviral therapy for {HIV} infection in adults
                   and adoloescents: recommendations for a public health
                   approach},
  year =          {2006},
}

@article{Reynoldsetal09,
  author =        {S.J. Reynolds and G. Nakigozi and K. Newell and
                   A. Ndyanabo and R. Galiwongo and I. Boaz and
                   T.C. Quinn and R. Gray and M. Wawer and D. Serwadda},
  journal =       {{AIDS}},
  number =        {6},
  pages =         {697--700},
  title =         {Failure of immunologic criteria to appropriately
                   identify antiretroviral treatment failure in {U}ganda},
  volume =        {23},
  year =          {2009},
}

@article{Petersenetal07,
  author =        {M.L Petersen and S.G. Deeks and J.N. Martin and
                   M.J. van der Laan},
  journal =       {Am J Epidemiol},
  number =        {9},
  pages =         {985--993},
  title =         {History-Adjusted Marginal Structural Models to
                   Estimate Time-Varying Effect Modification},
  volume =        {166},
  year =          {2007},
}

@article{Robins&Hernan&Rotnitzky07,
  author =        {J.M. Robins and M.A. Hernan and A. Rotnitzky},
  journal =       {Am J Epidemiol},
  number =        {9},
  pages =         {994--1002},
  title =         {Effect Modification by Time-varying Covariates},
  volume =        {166},
  year =          {2007},
}

@article{vanderLaan&Petersen&Joffe07,
  author =        {M.J. van der Laan and M.L. Petersen and M.M. Joffe},
  journal =       {Am J Epidemiol},
  number =        {9},
  pages =         {1003--1004},
  title =         {Response to Invited Commentary: {P}etersen et. al.
                   Respond to ``{E}ffect Modification by Time-varying
                   Covariates''},
  volume =        {166},
  year =          {2007},
}

@article{vanderLaan&Petersen07b,
  author =        {M.J. van der Laan and M.L. Petersen},
  journal =       {Int J Biostat},
  number =        {1},
  pages =         {Article 6},
  title =         {Statistical Learning of Origin-Specific Statically
                   Optimal Individualized Treatment Rules.},
  volume =        {3},
  year =          {2007},
}

@article{Petersen&Deeks&vanderLaan07,
  author =        {M.L. Petersen and S.G. Deeks and M.J. van der Laan},
  journal =       {Stat Med},
  number =        {25},
  pages =         {4578--601},
  title =         {Individualized Treatment Rules: generating Candidate
                   Clinical Trials.},
  volume =        {26},
  year =          {2007},
}

@article{vanderLaan&Petersen&Joffe05,
  author =        {M.J. van der Laan and M.L. Petersen and M.M. Joffe},
  journal =       {Int J Biostat},
  number =        {1},
  pages =         {10--20},
  title =         {History-Adjusted Marginal Structural Models and
                   Statically-Optimal Dynamic Treatment Regimens},
  volume =        {1},
  year =          {2005},
}

@article{Hernanetal06,
  author =        {M.A. Hernan and E. Lanoy and D. Costagliola and
                   J.M. Robins},
  journal =       {Basic Clin Pharmacol},
  pages =         {237--242},
  title =         {Comparison of dynamic treatment regimes via inverse
                   probability weighting.},
  volume =        {98},
  year =          {2006},
}

@techreport{vanderLaan08b,
  author =        {M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =          {232},
  title =         {The construction and analysis of adaptive group
                   sequential designs},
  year =          {2008},
}

@article{Boivinetal07,
  author =        {Boivin, J. and Bunting, L. and Collins, J.A. and
                   Nygren, K.G.},
  journal =       {Hum Reproduct},
  pages =        {1506--1512},
  title =         {International estimates of infertility prevalence and
                   treatment-seeking: potential need and demand for
                   infertility medical care},
  volume =        {22},
  year =          {2007},
}

@article{Adamsonetal06,
  author =        {Adamson, G.D. and de {M}ouzon, J. and Lancaster, P. and
                   Nygren, K.-G. and Sullivan, E. and
                   Zegers-Hochschild, F.},
  journal =       {Fertil Steril},
  pages =        {1586--1622},
  title =         {World collaborative report on in vitro fertilization,
                   2000},
  volume =        {85},
  year =          {2006},
}

@article{Soullieretal08,
  author =        {Soullier, N. and Bouyer, J. and Pouly J-L. and
                   Guibert, J. and de la {R}ochebrochard},
  journal =       {Hum Reproduct},
  pages =         {187--192},
  title =         {Estimating the success of an in vitro fertilization
                   programme using multiple imputation},
  volume =        {23},
  year =          {2008},
}

@article{delaRochebrochardetal08,
  author =        {de la {R}ochebrochard, E. and Soullier, N. and
                   Peikrishvili, R. and Guibert, J. and Bouyer, J.},
  journal =       {Int J Gynecol Obstet},
  pages =         {74--75},
  title =         {High in vitro fertilization discontinuation rate in
                   {F}rance},
  volume =        {103},
  year =          {2008},
}

@article{delaRochebrochardetal09,
  author =        {de la {R}ochebrochard, E. and Quelen, C. and
                   Peikrishvili, R. and Guibert, J. and Bouyer, J.},
  journal =       {Fertil Steril},
  pages =         {149--156},
  title =         {Long-term outcome of parenthood project during in
                   vitro fertilization and after discontinuation of
                   unscuccessful in vitro fertilization},
  volume =        {92},
  year =          {2009},
}

@book{Schafer97,
  address =       {London},
  author =        {Schafer, J.L.},
  publisher =     {Chapman \& Hall},
  title =         {Analysis of incomplete multivariate data},
  year =          {1997},
}

@book{Little&Rubin02,
  address =       {Hoboken},
  author =        {Little, R.J.A. and Rubin, Donald B.},
  edition =       {2nd},
  publisher =     {Wiley},
  title =         {Statistical analysis with missing data},
  year =          {2002},
}

@techreport{Yu&vanderLaan02,
  author =        {Z. Yu and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number={122},
  title =         {Construction of counterfactuals and the
                   G-computation formula},
  year =          {2002},
}

@article{Gill&Robins01,
  author =        {Gill, R.D. and Robins, J.M.},
  journal =       {Ann Stat},
  number =        {6},
  pages =         {1785--1811},
  title =         {Causal inference in complex longitudinal studies:
                   continuous case},
  volume =        {29},
  year =          {2001},
}

@techreport{DHHS04,
  author =        {{Department of Health and Human Services}},
  institution =   {Panel on Clinical Practices for Treatment of {HIV}
                   Infection},
type={Technical {R}eport},
  title =         {Guidelines for the use of antiretroviral agents in
                   {HIV}-1 infected adults and adolescents},
  year =          {2004},
}

@article{CDC92,
  author =        {{Centers for Disease Control and Prevention}},
  journal =       {Morbid Mortal W Rep},
  pages =         {1--19},
  title =         {{1993 revised classification system for {HIV} infection
                   and expanded surveillance case definition for AIDS
                   among adolescents and adults}},
  volume =        {41},
  year =          {1992},
}

@incollection{Selbyetal05,
  author =        {J.V. Selby and D.H. Smith and E.S. Johnson and
                   M.A. Raebel and G.D. Friedman and B.H. McFarland},
  booktitle =     {Pharmacoepidemiology},
  editor =        {B.L. Strom},
  publisher =     {Wiley},
  title =         {Kaiser {P}ermanente Medical Care Program},
  year =          {2005},
}

@techreport{Neugebauer&Silverberg&vanderLaan10,
  author =        {R. Neugebauer and M.J. Silverberg and
                   M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  type =          {272},
  title =         {Observational Study and Individualized Antiretroviral
                   Therapy Initiation Rules for Reducing Cancer
                   Incidence in {HIV}-Infected Patients},
  year =          {2010},
}




@techreport{Stitelmanetal11,
  author =        {O.M. Stitelman and V. De Gruttola and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  type =          {Technical {R}eport 281, http://www.bepress.com/ucbbiostat/paper281},
  title =         {A General Implementation of TMLE for Longitudinal Data Applied to Causal Inference in Survival Analysis},
  year =          {2011},
}
@techreport{Stitelman&vanderLaan11,
  author =        {O.M. Stitelman and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  type =          {Technical {R}eport},
  title =         {Targeted Maximum Likelihood Estimation of
                   Time-To-Event Parameters With Time-Dependent
                   Covariates},
  year =          {2011},
}

@article{Thalletal07,
  author =        {P.F. Thall and C. Logothetis and L.C. Pagliaro and
                   S. Wen and M.A. Brown and D. Williams and
                   R.E. Millikan},
  journal =       {J Natl Cancer Inst},
  pages =         {1613--22},
  title =         {Adaptive Therapy for Androgen-Independent Prostate
                   Cancer: a randomized Selection Trial of Four
                   Regimens},
  volume =        {99},
  year =          {2007},
}

@article{Bembom&vanderLaan07a,
  author =        {O. Bembom and M.J. van der Laan},
  journal =       {J Natl Cancer Inst},
  pages =         {1577--1582},
  title =         {Comment: Statistical Methods for analyzing sequentially
                   randomized trials},
  volume =        {99(21)},
  year =          {2007},
}

@techreport{Zheng&vanderLaan10,
  author =        {W. Zheng and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =          {273},
  title =         {Asymptotic Theory for Cross-validated Targeted
                   Maximum Likelihood Estimation},
  year =          {2010},
}

@techreport{Zheng&vanderLaan11,
  author =        {W. Zheng and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =          {288},
  title =         {Targeted Maximum Likelihood Estimation of Natural Direct Effect},
  year =          {2011},
}

@book{Robert07,
  address={Berlin Heidelberg New York},
  author =        {Robert, P.C.},
  publisher =     {Springer},
  title =         {{T}he {B}ayesian choice: from
                   decision-thoeretic foundations to
                   computational implementation},
  year =          {2007},
}

@book{Lindley80,
  address =       {Cambridge, MA},
  author =        {Lindley, D.V.},
  publisher =     {Cambridge},
  title =         {{I}ntroduction to probability and statistics from
                   a {B}ayesian point of view, {P}art 2},
  year =          {1980},
}

@article{Golub06,
  author =        {Golub, H.L.},
  journal =       {Stat Med},
  pages =         {3231--3235},
  title =         {The need for more efficient trial designs},
  volume =        {25},
  year =          {2006},
}

@article{Emerson06,
  author =        {Emerson, S.S.},
  journal =       {Stat Med},
  pages =         {3270--3296},
  title =         {Issues in the use of adaptive clinical trial designs},
  volume =        {25},
  year =          {2006},
}

@book{Hu&Rosenberger06,
address = {New York},
  author =        {F. Hu and W.F. Rosenberger},
  publisher =     {Wiley},
  title =         {The theory of response adaptive randomization in
                   clinical trials},
  year =          {2006},
}

@book{Jennison&Turnbull00,
  address =       {Boca Raton},
  author =        {Jennison, C. and Turnbull, B.W.},
  editor =        {},
  publisher =     {Chapman \& Hall},
  title =         {Group sequential methods with applications to
                   clinical trials},
  year =          {2000},
}

@article{Rosenberger96,
  author =        {W.F. Rosenberger},
  journal =       {Stat Sci},
  number =        {},
  pages =         {137--149},
  title =         {New directions in adaptive designs},
  volume =        {11},
  year =          {1996},
}

@techreport{Chambaz&vanderLaan10,
  author =        {Chambaz, A. and van der Laan, M.J.},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
   number={258},
  title =         {Targeting the optimal design in randomized clinical
                   trials with binary outcomes and no covariate},
  year =          {2010},
}

@article{Rosenberger&Vidyashankar&Agarwal01,
  author =        {Rosenberger, W.F. and Vidyashankar, A.N. and
                   Agarwal, D.K.},
  journal =       {J Biopharm Stat},
  number =        {227--236},
  title =         {Covariate-adjusted response-adaptive designs for
                   binary response},
  volume =        {11},
  year =          {2001},
}

@article{Bandyopadhyay&Biswas01,
  author =        {Bandyopadhyay, U. and Biswas, A.},
  journal =       {Biometrika},
  number =        {2},
  pages =         {409--419},
  title =         {Adaptive designs for normal responses with prognostic
                   factors},
  volume =        {88},
  year =          {2001},
}

@article{Atkinson&Biswas05,
  author =        {Atkinson, A.C. and Biswas, A.},
  journal =       {Stat Med},
  number =        {16},
  pages =         {2477--2492},
  title =         {Adaptive biased-coin designs for skewing the
                   allocation proportion in clinical trials with normal
                   responses},
  volume =        {24},
  year =          {2005},
}

@article{Zhangetal07,
  author =        {Zhang, L.-X. and Hu, F.-F. and Cheung, S.H. and
                   Chan, W.S.},
  journal =       {Ann Stat},
  number =        {3},
  pages =         {1166--1182},
  title =         {Asymptotic properties of covariate-adjusted
                   response-adaptive designs},
  volume =        {35},
  year =          {2007},
}

@article{Zhang&Hu09,
  author =        {Zhang, L.-X. and Hu, F.-F.},
  journal =       {Appl Math J Chinese Univ Ser B},
  number =        {1},
  pages =         {1--13},
  title =         {A new family of covariate-adjusted response adaptive
                   designs and their properties},
  volume =        {24},
  year =          {2009},
}

@article{Shao&Yu&Zhong10,
  author =        {Shao, J. and Yu, X. and Bob Zhong, B.},
  journal =       {Biometrika},
  title =         {A theory for testing hypotheses under
                   covariate-adaptive randomization},
  year =          {2010},
}

@article{Gill89,
  author =        {Gill, R.D.},
  journal =       {Scand J Stat},
  title =         {Non- and semiparametric maximum likelihood estimators
                   and the Von {M}ises method (Part 1)},
 number={16},
 pages={97--128},
  year =          {1989},
}

@article{Tan08,
  author =        {Z. Tan},
  journal =       {Int J Biostat},
  pages =         {Article 10},
  title =         {Comment: {I}mproved Local Efficiency and Double
                   Robustness},
  volume =        {4},
  number={1},
  year =          {2008},
}

@techreport{Gruber&vanderLaan11,
  author =        {S. Gruber and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =        {275},
  type =          {Technical Report},
  title =         {{tmle}: an {R} Package for Targeted Maximum Likelihood
                   Estimation},
  year =          {2011},
}

@proceedings{DBLP:conf/colt/2003,
  booktitle =     {COLT},
  editor =        {B. Sch{\"o}lkopf and M.K. Warmuth},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  series =        {Lecture Notes in Computer Science},
  title =         {Computational Learning Theory and Kernel Machines,
                   16th Annual Conference on Computational Learning
                   Theory and 7th Kernel Workshop, COLT/Kernel 2003,
                   Washington, DC, USA, August 24-27, 2003, Proceedings},
  volume =        {2777},
  year =          {2003},
}

@proceedings{DBLP:conf/nips/2005,
  booktitle =     {NIPS},
  title =         {Advances in Neural Information Processing Systems 18
                   [Neural Information Processing Systems, NIPS 2005,
                   December 5-8, 2005, Vancouver, British Columbia,
                   Canada]},
  year =          {2005},
}

@proceedings{DBLP:conf/colt/2006,
  booktitle =     {COLT},
  editor =        {G. Lugosi and H.-U. Simon},
  publisher =     {Springer},
  series =        {Lecture Notes in Computer Science},
    address={Berlin Heidelberg New York},
  title =         {Learning Theory, 19th Annual Conference on Learning
                   Theory, COLT 2006, Pittsburgh, PA, USA, June 22-25,
                   2006, Proceedings},
  volume =        {4005},
  year =          {2006},
}

%% This BibTeX bibliography file was created using BibDesk.
%% http://bibdesk.sourceforge.net/


%% Created for Ivan Diaz at 2011-09-14 16:32:22 -0700


%% Saved with string encoding Unicode (UTF-8)

@article{Rubin76,
  title={Inference and missing data},
  author={Rubin, D.B.},
  journal={Biometrika},
  volume={63},
  number={3},
  pages={581--592},
  year={1976},
  publisher={Biometrika Trust}
}
    @article{Hernan2009,
     title = {Invited commentary: causal diagrams and measurement bias},
     author = {Hern\'an, M. A. and Cole, S. R.},
     journal = {American Journal of Epidemiology},
     volume = {170},
     number = {8},
     pages = {pp. 963-954},
     year = {2009},
    }

    @article{Scharfstein2002,
     title = {Estimation of the Failure Time Distribution in the Presence of Informative Censoring},
     author = {Scharfstein, D. O. and Robins, J. M.},
     journal = {Biometrika},
     volume = {89},
     number = {3},
     pages = {pp. 617-634},
     year = {2002},
     publisher = {Biometrika Trust},
     copyright = {Copyright © 2002 Biometrika Trust},
    }

@article{Rotnitzky2001,
author = {A. Rotnitzky and D. Scharfstein and Su, S. Ting-Li and J. Robins},
title = {Methods for Conducting Sensitivity Analysis of Trials with Potentially Nonignorable Competing Causes of Censoring},
journal = {Biometrics},
volume = {57},
number = {1},
publisher = {Blackwell Publishing Ltd},
issn = {1541-0420},
pages = {103--113},
keywords = {Attrition, Augmented inverse probability of censoring weighted estimation, Curse of dimensionality, Longitudinal data, Noncompliance, Pattern-mixture models, Selection bias, Selection models},
year = {2001},
}
@ARTICLE{Scharfstein1999,
    author = {D. O. Scharfstein and A. Rotnitzky and J. M. Robins},
    title = {Adjusting for Nonignorable Drop-out Using Semiparametric Non-response Models (with discussion)},
    journal = {Journal of the American Statistical Association},
    year = {1999},
    volume = {94},
    pages = {1096--1146}
}

@incollection{Robins1999,
  title={Sensitivity Analysis for Selection Bias and Unmeasured Confounding in Missing Data and Causal Inference Models},
  booktitle={Statistical Models in Epidemiology, the Environment and Clinical Trials},
  author={Robins, J. M. and Rotnitzky, A. and Scharfstein, D. O.},
  series={IMA Volumes in Mathematics and Its Applications},
  year={1999},
  publisher={Springer}
}


@article{Rotnitsky1998,
author = {Rotnitzky, Andrea and Robins, James M. and Scharfstein, Daniel O.},
title = {Semiparametric Regression for Repeated Outcomes with Nonignorable Nonresponse},
journal = {Journal of the American Statistical Association},
volume = {93},
number = {444},
pages = {1321-1339},
year = {1998},
}

@incollection {vanderLaan&Petersen2012,
   author = {van der Laan, Mark J. and Petersen, Maya L.},
   affiliation = {Division of Biostatistics, School of Public Health, University of California, Berkeley, CA, USA},
   title = {Targeted Learning},
   booktitle = {Ensemble Machine Learning},
   editor = {Zhang, Cha and Ma, Yunqian},
   publisher = {Springer US},
   isbn = {978-1-4419-9326-7},
   keyword = {Engineering},
   pages = {117-156},
   year = {2012}
}
@inproceedings{Didelezetal2006,
	Author = {Vanessa Didelez and A. Philip Dawid and Sara Geneletti},
	Bibsource = {DBLP, http://dblp.uni-trier.de},
	Booktitle = {UAI},
	Crossref = {DBLP:conf/uai/2006},
	Date-Added = {2012-04-19 19:44:15 -0700},
	Date-Modified = {2012-04-19 19:48:48 -0700},
	Title = {Direct and Indirect Effects of Sequential Treatments},
	Year = {2006},
	Bdsk-Url-1 = {http://uai.sis.pitt.edu/displayArticleDetails.jsp?mmnu=1&smnu=2&article_id=1276&proceeding_id=22}}


@incollection{korb04,
	Affiliation = {School of Computer Science and Software Engineering, Monash University, Clayton, Victoria 3800, Australia},
	Author = {Korb, Kevin. and Hope, Lucas. and Nicholson, Ann. and Axnick, Karl.},
	Booktitle = {PRICAI 2004: Trends in Artificial Intelligence},
	Date-Added = {2012-04-19 19:07:55 -0700},
	Date-Modified = {2012-04-19 19:07:56 -0700},
	Editor = {Zhang, Chengqi and W. Guesgen, Hans and Yeap, Wai-Kiang},
	Pages = {322-331},
	Publisher = {Springer Berlin / Heidelberg},
	Series = {Lecture Notes in Computer Science},
	Title = {Varieties of Causal Intervention},
	Volume = {3157},
	Year = {2004}}

@article{DawidDidelez2010,
	Author = {A. Philip Dawid and Vanessa Didelez},
	Bibsource = {DBLP, http://dblp.uni-trier.de},
	Date-Added = {2012-04-19 19:34:46 -0700},
	Date-Modified = {2012-04-19 19:38:44 -0700},
	Journal = {CoRR},
	Title = {Identifying the consequences of dynamic treatment strategies: A decision-theoretic overview},
	Volume = {abs/1010.3425},
	Year = {2010},
	Bdsk-Url-1 = {http://arxiv.org/abs/1010.3425}}

@techreport{Diaz12a,
title={Assessing the Causal Effect of Policies: An
Approach Based on Stochastic Interventions},
author={D\'iaz, Iv\'an and van der Laan, Mark},
year={2012},
journal={U.C. Berkeley Division of Biostatistics Working Paper Series}
}

@ARTICLE{Diaz11,
title = {Super Learner Based Conditional Density Estimation with Application to Marginal Structural Models},
author = {D\'iaz, Iv\'an and van der Laan, Mark},
year = {2011},
journal = {The International Journal of Biostatistics},
volume = {7},
number = {1},
pages = {38},
keywords = {Statistical Theory and Methods; causal inference; conditional density; cross validation; efficient estimation; marginal structural models; oracle selector},
}

@article {Diaz12,
author = {Iv\'an D\'iaz and van der Laan, Mark},
title = {Population Intervention Causal Effects Based on Stochastic Interventions},
journal = {Biometrics},
volume = {68},
number = {2},
publisher = {Blackwell Publishing Inc},
issn = {1541-0420},
url = {http://dx.doi.org/10.1111/j.1541-0420.2011.01685.x},
doi = {10.1111/j.1541-0420.2011.01685.x},
pages = {541--549},
keywords = {Causal effect, Counterfactual outcome, Double robustness, Stochastic intervention, Targeted maximum likelihood estimation},
year = {2012},
}
@incollection {Zheng11,
   author = {Zheng, Wenjing and van der Laan, Mark J.},
   affiliation = {Division of Biostatistics, University of California, Berkeley, 101 Haviland Hall, #7358, Berkeley, CA 94720, USA},
   title = {Cross-Validated Targeted Minimum-Loss-Based Estimation},
   booktitle = {Targeted Learning},
   series = {Springer Series in Statistics},
   editor = {Bickel, P. and Diggle, P. and Fienberg, S. and Krickeberg, K. and Olkin, I. and Wermuth, N. and Zeger, S.},
   publisher = {Springer New York},
   isbn = {978-1-4419-9782-1},
   keyword = {Mathematics and Statistics},
   pages = {459-474},
   year = 2011
}

@string{jasa = {Journal of the American Statistical Association}}

@string{jc = {Journal of Classification}}

@string{jrssb = {Journal of the Royal Statistical Society, Series B}}

@string{jspi = {Journal of Statistical Planning and Inference}}

@string{pnas = {Proc. Natl. Acad. Sci.}}

@article{Rubin1974,
    abstract = {Randomization should be employed whenever possible but the use of carefully controlled nonrandomized data to estimate causal effects is a reasonable and necessary procedure in many cases. ({Author/BJG})},
    author = {Rubin, Donald B.},
    citeulike-article-id = {4632390},
    citeulike-linkout-0 = {http://www.eric.ed.gov/ERICWebPortal/detail?accno=EJ118470},
    day = {0},
    journal = {Journal of Educational Psychology},
    keywords = {causality\_detection},
    month = {},
    posted-at = {2009-05-25 17:19:51},
    priority = {2},
    title = {Estimating Causal Effects of Treatments in Randomized and Nonrandomized Studies},
    url = {http://www.eric.ed.gov/ERICWebPortal/detail?accno=EJ118470},
    year = {1974}
}

@article{Mannetal2010,
	Author = {Mann, Jennifer K. AND Balmes, John R. AND Bruckner, Tim A. AND Mortimer, Kathleen M. AND Margolis, Helene G. AND Pratt, Boriana AND Hammond, S. Katharine AND Lurmann, Frederick W. AND Tager, Ira B.},
	Date-Added = {2011-09-14 16:32:02 -0700},
	Date-Modified = {2011-09-14 16:32:19 -0700},
	Doi = {10.1289/ehp.0901292},
	Journal = {Environ Health Perspect},
	Month = {06},
	Number = {10},
	Publisher = {National Institute of Environmental Health Sciences},
	Title = {Short-Term Effects of Air Pollution on Wheeze in Asthmatic Children in Fresno, California},
	Url = {http://dx.doi.org/10.1289%2Fehp.0901292},
	Volume = {118},
	Year = {2010},
	Bdsk-Url-1 = {http://dx.doi.org/10.1289/ehp.0901292}}

@incollection{korb04,
	Affiliation = {School of Computer Science and Software Engineering, Monash University, Clayton, Victoria 3800, Australia},
	Author = {Korb, Kevin. and Hope, Lucas. and Nicholson, Ann. and Axnick, Karl.},
	Booktitle = {PRICAI 2004: Trends in Artificial Intelligence},
	Editor = {Zhang, Chengqi and W. Guesgen, Hans and Yeap, Wai-Kiang},
	Pages = {322-331},
	Publisher = {Springer Berlin / Heidelberg},
	Series = {Lecture Notes in Computer Science},
	Title = {Varieties of Causal Intervention},
	Volume = {3157},
	Year = {2004}}

@article{Petersen10,
	Author = {Petersen, Maya L and Porter, Kristin E. and Gruber, Susan. and Wang, Yue. and van der Laan, Mark J.},
	Issn = {1477-0334},
	Journal = {Stat Methods Med Res},
	Pubmedid = {21030422},
	Title = {Diagnosing and responding to violations in the positivity assumption.},
	Url = {http://www.biomedsearch.com/nih/Diagnosing-responding-to-violations-in/21030422.html},
	Year = {2010},
	Bdsk-Url-1 = {http://www.biomedsearch.com/nih/Diagnosing-responding-to-violations-in/21030422.html}}

@article{Stitelmanetal10,
	Author = {Stitelman, Ori M and Hubbard, Alan E and Jewell, Nicholas P.},
	Publisher = {The Berkeley Electronic Press},
	Title = {The Impact Of Coarsening The Explanatory Variable Of Interest In Making Causal Inferences: Implicit Assumptions Behind Dichotomizing Variables},
	Url = {http://www.bepress.com/ucbbiostat/paper264},
	Year = {2010},
	Bdsk-Url-1 = {http://www.bepress.com/ucbbiostat/paper264}}

@article{Taubman01122009,
	Author = {Taubman, Sarah L and Robins, James M and Mittleman, Murray A and Hern{\'a}n, Miguel A},
	Doi = {10.1093/ije/dyp192},
	Eprint = {http://ije.oxfordjournals.org/content/38/6/1599.full.pdf+html},
	Journal = {International Journal of Epidemiology},
	Number = {6},
	Pages = {1599-1611},
	Title = {Intervening on risk factors for coronary heart disease: an application of the parametric g-formula},
	Url = {http://ije.oxfordjournals.org/content/38/6/1599.abstract},
	Volume = {38},
	Year = {2009},
	Bdsk-Url-1 = {http://ije.oxfordjournals.org/content/38/6/1599.abstract},
	Bdsk-Url-2 = {http://dx.doi.org/10.1093/ije/dyp192}}

@article{Laurenetal10,
	Author = {Cain, Lauren E and Robins, James M and Lanoy, Emilie and Logan, Roger and Costagliola, Dominique and Hern\'an, Miguel A.},
	Journal = {The International Journal of Biostatistics},
	Title = {When to Start Treatment? A Systematic Approach to the Comparison of Dynamic Regimes Using Observational Data},
	Url = {http://www.bepress.com/ijb/vol6/iss2/18},
	Volume = {6},
	Year = {2010},
	Bdsk-Url-1 = {http://www.bepress.com/ijb/vol6/iss2/18}}

@article{Eberhardt&Scheines06,
	Author = {F. Eberhardt and R. Scheines},
	Journal = {Department of Philosophy. Paper 415},
	Title = {Interventions and Causal Inference},
	Url = {http://repository.cmu.edu/philosophy/415},
	Year = {2006},
	Bdsk-Url-1 = {http://repository.cmu.edu/philosophy/415}}

@article{Orellana&Rotnitzky&Robins10,
	Author = {L. Orellana and A. Rotnitzky and J.M. Robins},
	Journal = {The International Journal of Biostatistics},
	Pages = {523-39},
	Title = {Dynamic Regime Marginal Structural Mean Models for Estimation of Optimal Dynamic Treatment Regimes, Part I: Main Content},
	Volume = {6},
	Year = {2010}}

@article{Kang&Shafer07,
	Author = {J. Kang and J. Schafer},
	Journal = {Statistical Science},
	Pages = {523-39},
	Title = {Demystifying Double Robustness: A Comparison of Alternative Strategies for Estimating a Population Mean from Incomplete Data (with discussion)},
	Volume = {22},
	Year = {2007}}

@article{Ridgeway&McCaffrey07,
	Author = {G. Ridgeway and D. McCaffrey},
	Journal = {Statistical Science},
	Pages = {540-43},
	Title = {Comment: Demystifying Double Robustness: A Comparison of Alternative Strategies for Estimating a Population Mean from Incomplete Data (with discussion)},
	Volume = {22},
	Year = {2007}}

@article{Robinsetal07,
	Author = {J. M. Robins and M. Sued and Q. Lei-Gomez and A. Rotnitzky},
	Journal = {Statistical Science},
	Pages = {544-559},
	Title = {Comment: Performance of Double-Robust Estimators When ``Inverse Probability'' Weights Are Highly Variable},
	Volume = {22},
	Year = {2007}}

@article{Tan07,
	Author = {Z. Tan},
	Journal = {Statistical Science},
	Pages = {560-568},
	Title = {Comment: Understanding OR, PS and DR},
	Volume = {22},
	Year = {2007}}
@article {Diaz&vanderLaan1101,
author = {Diaz, Ivan and van der Laan, Mark},
title = {Population Intervention Causal Effects Based on Stochastic Interventions},
journal = {Biometrics},
publisher = {Blackwell Publishing Inc},
issn = {1541-0420},
url = {http://dx.doi.org/10.1111/j.1541-0420.2011.01685.x},
doi = {10.1111/j.1541-0420.2011.01685.x},
pages = {In press.},
keywords = {Causal effect, Counterfactual outcome, Double robustness, Stochastic intervention, Targeted maximum likelihood estimation},
year = {2011},
}


@article{Tsiatis&Davidian07,
	Author = {A. Tsiatis and M. Davidian},
	Journal = {Statistical Science},
	Pages = {569-73},
	Title = {Comment: Demystifying Double Robustness: A Comparison of Alternative Strategies for Estimating a Population Mean from Incomplete Data (with discussion)},
	Volume = {22},
	Year = {2007}}

@article{Kang&Shafer07b,
	Author = {J. Kang and J. Schafer},
	Journal = {Statistical Science},
	Pages = {574-80},
	Title = {Rejoinder: Demystifying Double Robustness: A Comparison of Alternative Strategies for Estimating a Population Mean from Incomplete Data},
	Volume = {22},
	Year = {2007}}

@article{Murphy05,
	Author = {S. Murphy},
	Journal = {Statistics in Medicine},
	Pages = {1455�1481},
	Title = {An experimental design for the development of adaptive treatment strategies},
	Volume = {24},
	Year = {2005}}

@book{Zhang&Ma12,
  title={Ensemble Machine Learning: Methods and Applications},
  author={Zhang, C. and Ma, Y.},
  isbn={9781441993250},
  url={http://books.google.com/books?id=CjAs4stLXhAC},
  year={2012},
  publisher={Springer}
}

@article{Lavori&Dawson00,
	Author = {P. Lavori and R. Dawson},
	Journal = {Journal of the Royal Statistical Society, Series A},
	Pages = {29�38},
	Title = {A design for testing clinical strategies: biased adaptive within-subject randomization},
	Volume = {163},
	Year = {2000}}

@article{Lavori&Dawson04,
	Author = {P. Lavori and R. Dawson},
	Journal = {Clinical trials},
	Pages = {9�20},
	Title = {Dynamic treatment regimes: practical design considerations},
	Volume = {1},
	Year = {2004}}

@article{Thall&Millikan&Sung00,
	Author = {P. Thall and R. Millikan and H.-G. Sung},
	Journal = {Statistics in Medicine},
	Pages = {1011�1028},
	Title = {Evaluating multiple treatment courses in clinical trials},
	Volume = {19},
	Year = {2000}}

@article{Rush&Trivedi&Fava03,
	Author = {A.J. Rush and M. Trivedi and M. Fava},
	Journal = {IV. American Journal of Psychiatry},
	Pages = {237},
	Title = {Depression},
	Volume = {160(2)},
	Year = {2003}}

@article{Schneideretal06,
	Author = {Schneider, L. and Tariot.P.N. and Dagerman, K. and Davis, S. and Hsiao, J. and Ismail, S. and Lebowitz, B. and Lyketsos, C. and Ryan J. and Stroup T. and Sultzer D. and Weintraub, D. and Lieberman, J.},
	Journal = {New England Journal of Medicine},
	Pages = {1525�1538},
	Title = {Effectiveness of atypical antipsychotic drugs in patients with Alzheimer�s disease},
	Volume = {355(15)},
	Year = {2006}}

@article{Swartzetal07,
	Author = {Swartz, M. and Perkins, D. and Stroup, T. and Davis, S. and Capuano, G. and Rosenheck, R. and Reimherr, F. and McGee, M. and Keefe, R. and McEvoy, J. and Hsiao, J. and Lieberman, J.},
	Journal = {American Journal of Psychiatry},
	Pages = {428�436},
	Title = {Effects of antipsychotic medications on psychosocial functioning in patients with chronic shizophrenia: Findings from the nimh catie study},
	Volume = {164},
	Year = {2007}}

@article{Rubin&vanderLaan08,
	Author = {D.B. Rubin and M.J. van der Laan},
	Journal = {The International Journal of Biostatistics},
	Location = {http://www.bepress.com/ijb/vol4/iss1/5},
	Title = {Empirical Efficiency Maximization: Improved Locally Efficient Covariate Adjustment in Randomized Experiments and Survival Analysis},
	Volume = {Vol. 4, Iss. 1, Article 5},
	Year = {2008}}

@article{vanderLaan&Rose&Gruber09,
	Author = {M.J. van der Laan and S. Rose and S. Gruber},
	Journal = {Technical report, working paper series http://www.bepress.com/ucbbiostat/paper254/},
	Title = {Readings on Targeted Maximum Likelihood Estimation},
	Year = {September, 2009}}

@article{Bembometal09,
	Author = {O. Bembom and M.J. van der Laan and T. Haight and I.B. Tager},
	Journal = {Epidemiology},
	Title = {Lifetime and current leisure time physical activity and all-cause mortality in an elderly cohort},
	Year = {2009}}

@article{Bembom&vanderLaan07a,
	Author = {O. Bembom and M.J. van der Laan},
	Journal = {Journal of the National Cancer Institute},
	Pages = {1577-1582},
	Title = {Statistical Methods for analyzing sequentially randomized trials, commentary on JNCI article Adaptive therapy for androgen independent prostate cancer: A Randomized selection trial including four regimens, by Peter F. Thall, C. Logothetis, C. Pagliaro, S. Wen, M.A. Brown, D. Williams, R. Millikan (2007).},
	Volume = {99(21)},
	Year = {2007}}

@article{Rosenblumetal09,
	Author = {M. Rosenblum and S.G. Deeks and M.J. van der Laan and D.R. Bangsberg},
	Journal = {PLoS ONE},
	Title = {The Risk of Virologic Failure Decreases with Duration of HIV Suppression, at Greater than 50\% Adherence to Antiretroviral Therapy},
	Volume = {4(9): e7196.doi:10.1371/journal.pone.0007196},
	Year = {2009}}

@article{Robins&Orallana&Rotnitzky08,
	Author = {J. M. Robins and L. Orallana and A. Rotnitzky},
	Journal = {Statistics in Medicine},
	Pages = {4678-4721},
	Title = {Estimaton and extrapolation of optimal treatment and testing strategies},
	Volume = {27(23)},
	Year = {2008}}

@article{Bembom&vanderLaan07,
	Author = {O. Bembom and M.J. van der Laan},
	Journal = {Electronic Journal of Statistics},
	Title = {A practical illustration of the importance of realistic individualized treatment rules in causal inference},
	Year = {2007}}

@article{Bembometal08,
	Author = {O. Bembom and M.L. Petersen and S.-Y. Rhee and W. J. Fessel and S.E. Sinisi and R.W. Shafer and M.J. van der Laan},
	Journal = {Statistics in Medicine},
	Pages = {http://www3.interscience.wiley.com/journal/121422393/abstract},
	Title = {Biomarker discovery using targeted maximum likelihood estimation: Application to the treatment of antiretroviral resistant HIV infection},
	Year = {2008}}

@article{Tuglus&vanderLaan08,
	Author = {C. Tuglus and M.J. van der Laan},
	Journal = {UC Berkeley Working Paper Series},
	Pages = {http://www.bepress.com/ucbbiostat/paper233/.},
	Title = {Targeted Methods for Biomarker Discovery, the Search for a Standard},
	Year = {2008}}

@article{vanderLaan08,
	Author = {M.J. van der Laan},
	Journal = {The International Journal of Biostatistics},
	Pages = {http://www.bepress.com/ijb/vol4/iss1/17/},
	Title = {Estimation Based on Case-Control Designs with Known Prevalance Probability},
	Year = {2008}}

@article{Rose&vanderLaan08,
	Author = {S. Rose and M.J. van der Laan},
	Journal = {The International Journal of Biostatistics},
	Pages = {http://www.bepress.com/ijb/vol4/iss1/19/.},
	Title = {Simple Optimal Weighting of Cases and Controls in Case-Control Studies},
	Year = {2008}}

@article{Rose&vanderLaan09,
	Author = {S. Rose and M.J. van der Laan},
	Journal = {The International Journal of Biostatistics},
	Pages = {http://www.bepress.com/ijb/vol5/iss1/1/.},
	Title = {Why Match? [Investigating Matched Case-Control Study Designs with Causal Effect Estimation},
	Year = {2009}}

@inproceedings{Moore&vanderLaan09,
	Author = {K.L. Moore and M.J. van der Laan},
	Booktitle = {in Design, Summarization, Analysis \& Interpretation of Clinical Trials with Time-to-Event Endpoints},
	Editor = {Karl E. Peace},
	Publisher = {Chapman and Hall},
	Title = {Application of Time-to-Event Methods in the Assessment of Safety in Clinical Trials},
	Year = {2009}}

@inproceedings{Polley&vanderLaan09,
	Author = {E.C. Polley and M.J. van der Laan},
	Booktitle = {in Design, Summarization, Analysis \& Interpretation of Clinical Trials with Time-to-Event Endpoints},
	Editor = {Karl E. Peace},
	Publisher = {Chapman and Hall},
	Title = {Predicting Optimal Treatment Assignment Based on Prognostic Factors in Cancer Patients},
	Year = {2009}}

@article{vanderVaart&Dudoit&vanderLaan06,
	Author = {A.W. van der Vaart and S. Dudoit and M.J. van der Laan},
	Journal = {Statistics and Decisions},
	Number = {3},
	Pages = {351--371},
	Title = {Oracle Inequalities for Multi-Fold Cross-Validation},
	Volume = {24},
	Year = {2006}}

@article{vanderLaan&Dudoit&vanderVaart06,
	Author = {M.J. van der Laan and S. Dudoit and A.W. van der Vaart},
	Journal = {Statistics and Decisions},
	Number = {3},
	Pages = {373--395},
	Title = {The Cross-Validated Adaptive Epsilon-Net Estimator},
	Volume = {24},
	Year = {2006}}

@article{Rosenbaum&Rubin83,
	Author = {P.R. Rosenbaum and D.B. Rubin},
	Journal = {Biometrika},
	Pages = {41-55},
	Title = {The Central Role of the Propensity Score in Observational Studies for Causal Effects},
	Volume = {70},
	Year = {1983}}

@article{vanderLaan&Polley&Hubbard07,
	Author = {M.J. van der Laan and E. Polley and A. Hubbard},
	Issn = {1},
	Journal = {Statistical Applications in Genetics and Molecular Biology},
	Location = {http://www.bepress.con/sagmb/vol6/iss1/art25},
	Number = {25},
	Title = {Super Learner},
	Volume = {6},
	Year = {2007}}

@article{Sekhon08,
	Author = {J.S. Sekhon},
	Journal = {Journal of Statistical Sotware, Forthcoming},
	Location = {http://ssrn.com/paper=1009044},
	Publisher = {SSRN},
	Title = {Multivariate and Propensity Score Matching Software with Automated Balance Optimization: The Matching package for {R}},
	Year = {2008}}

@article{Zheng&vanderLaan10,
	Author = {Wenjing Zheng and Mark J. van der Laan},
	Journal = {Division of Biostatistics Working Paper Series},
	Location = {http://works.bepress.com/wenjing_zheng/1/},
	Publisher = {U.C. Berkeley},
	Title = {Asymptotic Theory for Cross-validated Targeted Maximum Likelihood Estimation},
	Year = {2010}}

@article{Bembometal08,
	Author = {O. Bembom and J.W. Fessel and R.W. Shafer and M.J. van der Laan},
	Institution = {DigitalCommons@Florida Atlantic University [http://digitalcommons.fau.edu/cgi/oai2.cgi] (United States)},
	Keywords = {General Biostatistics},
	Location = {http://www.scientificcommons.org/36721107},
	Publisher = {The Berkeley Electronic Press},
	Title = {Data-adaptive Selection Of The Adjustment Set In Variable Importance Estimation},
	Url = {http://www.bepress.com/ucbbiostat/paper231},
	Year = {2008},
	Bdsk-Url-1 = {http://www.bepress.com/ucbbiostat/paper231}}

@article{Holland&Reitman77,
	Address = {New York, NY, USA},
	Author = {J.H. Holland and J.S. Reitman},
	Doi = {http://doi.acm.org/10.1145/1045343.1045373},
	Issn = {0163-5719},
	Journal = {SIGART Bull.},
	Pages = {49--49},
	Publisher = {ACM},
	Title = {Cognitive systems based on adaptive algorithms},
	Volume = {63},
	Year = {1977},
	Bdsk-Url-1 = {http://doi.acm.org/10.1145/1045343.1045373}}

@book{Rubin06,
	Address = {Cambridge, MA},
	Author = {D.B. Rubin},
	Publisher = {Cambridge University Press},
	Title = {Matched Sampling for Causal Effects.},
	Year = {2006}}

@incollection{Mansk1&McFadden81,
	Address = {Cambridge, MA},
	Author = {C.F. Manski and D. McFadden},
	Booktitle = {Structural Analysis of Discrete Data with Econometric Applications},
	Editor = {C.F. Manski and D. McFadden},
	Publisher = {The MIT Press},
	Title = {Alternative estimators and sample designs for discrete choice analysis},
	Year = {1981}}

@article{Manski&Lerman77,
	Author = {C.F. Manski and S.R. Lerman},
	Journal = {Econometrica},
	Number = {8},
	Pages = {1977-1988},
	Title = {The Estimation of Choice Probabilities from Choice Based Samples},
	Volume = {45},
	Year = {1977}}

@article{Cosslett81,
	Author = {S.R. Cosslett},
	Journal = {Econometrica},
	Number = {5},
	Pages = {1289-1316},
	Title = {Maximum Likelihood Estimator for Choice-Based Samples},
	Volume = {49},
	Year = {1981}}

@article{Cornfield51,
	Author = {J. Cornfield},
	Journal = {J Nat Cancer Inst},
	Pages = {1269-1275},
	Title = {A method of estimating comparative rates from clinical data. Applications to cancer of the lung, breast, and cervix.},
	Volume = {11},
	Year = {1951}}

@inproceedings{Cornfield56,
	Author = {J. Cornfield},
	Booktitle = {Proceedings of the Third Berkeley Symposium, Volume IV},
	Editor = {J. Neyman},
	Pages = {133-148},
	Publisher = {University of California Press},
	Title = {A statistical problem arising from retrospective studies},
	Year = {1956}}

@article{Benichou&Wacholder94,
	Author = {J. Benichou and S. Wacholder},
	Journal = {Statistics in Medicine},
	Pages = {651-661},
	Title = {A comparison of three approaches to estimate exposure-specific incidence rates from population-based case-control data.},
	Volume = {13},
	Year = {1994}}

@article{Breslow&Robins&Wellner00,
	Author = {N.E. Breslow and J.M. Robins and J.A. Wellner},
	Journal = {Bernoulli},
	Pages = {447--455},
	Title = {On the semi-parametric efficiency of logistic regression under case-control sampling},
	Volume = {6(3)},
	Year = {2000}}

@article{Mansonetal07,
	Author = {R. Mansson, M.M. Joffe, W. Sun, S. Hennessy},
	Journal = {Am J Epidemiol},
	Number = {3},
	Pages = {332-339},
	Title = {On the Estimation and Use of Propensity Scores in Case-Control and Case-Cohort Studies.},
	Volume = {166},
	Year = {2007}}

@article{Anderson79,
	Author = {J.A. Anderson},
	Journal = {Biometrika},
	Pages = {19--35},
	Title = {Separate sample logistic discrimination},
	Volume = {59},
	Year = {1972}}

@article{Prentice&Pyke79,
	Author = {R.L. Prentice and R. Pyke},
	Journal = {Biometrika},
	Pages = {403--411},
	Title = {Logistic disease incidence models and case-control studies},
	Volume = {66},
	Year = {1979}}

@article{Breslow96,
	Author = {N.E. Breslow},
	Journal = {J Am Stat Soc},
	Pages = {14--28},
	Title = {Statistics in Epidemiology: the Case-Control Study},
	Volume = {91},
	Year = {1996}}

@book{Breslow&Day80,
	Address = {Lyon},
	Author = {N.E. Breslow and N.E. Day},
	Publisher = {International Agency for Research on Cancer},
	Title = {Statistical Methods in Cancer Research: Volume 1 -- The analysis of case-control studies},
	Year = {1980}}

@article{Holford&White&Kelsey78,
	Author = {T.R. Holford and C. White and J.L. Kelsey},
	Journal = {Am J Epid},
	Number = {3},
	Pages = {245--255},
	Title = {Multivariate Analysis for Matched Case-Control Studies},
	Volume = {107},
	Year = {1978}}

@article{Breslowetal78,
	Author = {N.E. Breslow and N.E. Day and K.T. Halvorsen and R.L. Prentice and C. Sabal},
	Journal = {Am J Epid},
	Number = {4},
	Pages = {299--307},
	Title = {Estimation of Multiple Relative Risk Functions in Matched Case-Control Studies},
	Volume = {108},
	Year = {1978}}

@book{Schlesselman82,
	Address = {Oxford},
	Author = {J.J. Schlesselman},
	Publisher = {Oxford University Press},
	Title = {Case-Control Studies: Design, Conduct, Analysis},
	Year = {1982}}

@book{Collett91,
	Address = {London},
	Author = {D. Collett},
	Publisher = {Chapman and Hall},
	Title = {Modeling Binary Data},
	Year = {1991}}

@book{Jewell04,
	Address = {Boca Raton},
	Author = {N.P. Jewell},
	Publisher = {Chapman and Hall/CRC},
	Title = {Statistics for Epidemiology},
	Year = {2004}}

@book{Hosmer&Lemeshow00,
	Address = {New York},
	Author = {D.W. Hosmer and S. Lemeshow},
	Edition = {2nd},
	Publisher = {John Wiley and Sons},
	Title = {Applied Logistic Regression},
	Year = {2000}}

@article{Robins99,
	Author = {J.M. Robins},
	Journal = {Statistical Science},
	Number = {3},
	Pages = {281--293},
	Title = {[Choice as an Alternative to Control in Observational Studies]: Comment},
	Volume = {14},
	Year = {1999}}

@article{Newman06,
	Author = {S. Newman},
	Journal = {Epid Persp Innov},
	Pages = {2},
	Title = {Causal Analysis of Case-Control Data},
	Url = {http://www.epi-perspectives.com/content/3/1/2},
	Volume = {3},
	Year = {2006},
	Bdsk-Url-1 = {http://www.epi-perspectives.com/content/3/1/2}}

@article{Zelen&Parker86,
	Author = {M. Zelen and R.A. Parker},
	Journal = {Stat Med},
	Number = {3},
	Pages = {261--269},
	Title = {Case-Control Studies and Bayesian Inference},
	Volume = {5},
	Year = {1986}}

@article{Sinhetal04,
	Author = {S. SInha and B. Mukherjee and M Ghosh},
	Journal = {Biometrics},
	Pages = {41--49},
	Title = {Bayesian Semiparametric Modeling for Matched Case-Control Studies with Multiple Disease States},
	Volume = {60},
	Year = {2004}}

@article{Ritchieetal01,
	Author = {M.D. Ritchie and L.W. Hahn and N. Roodi and L.R. Bailey and W.D. Dupont and F.F. Parl and J.H. Moore},
	Journal = {Am J Hum Genet},
	Number = {1},
	Pages = {138--47},
	Title = {Multifactor-dimensionality reduction reveals high-order interactions among estrogen-metabolism genes in sporadic breast cancer.},
	Volume = {69},
	Year = {2001}}

@article{Mei&Cuccaro&Martin07,
	Author = {H. Mei and M.L. Cuccaro and E.R. Martin},
	Journal = {Am J Hum Genet},
	Number = {6},
	Pages = {1251-61},
	Title = {Multifactor dimensionality reduction-phenomics: a novel method to capture genetic heterogeneity with use of phenotypic variables.},
	Volume = {81},
	Year = {2007}}

@article{Bangsberg&Moss&Deeks04,
	Abstract = {Public health debates about providing HIV antiretroviral therapy to impoverished populations have centred on the relationship between adherence and risk of drug resistance. Recent data indicate that each antiretroviral therapeutic class has a unique adherence-resistance relationship. Resistance to single protease inhibitor therapy occurs most frequently at moderate to high levels of adherence, resistance to non-nucleoside reverse transcriptase inhibitor therapy occurs at low to moderate levels of adherence, and resistance to ritonavir-boosted protease inhibitor therapy is most likely to occur at middle ranges of adherence. These dynamic relationships should be considered in balancing the individual and public health benefits of therapy.},
	Author = {D.R. Bangsberg and A.R. Moss and S.G. Deeks},
	Journal = {J Antimicrob Chemother},
	Keywords = {Anti-HIV Agents/*therapeutic use Developing Countries *Drug Resistance, Viral Humans *Patient Compliance Public Health Research Support, Non-U.S. Gov't Research Support, U.S. Gov't, P.H.S.},
	Note = {0305-7453 (Print) Journal Article Review},
	Number = {5},
	Pages = {696-9},
	Title = {Paradoxes of adherence and drug resistance to {HIV} antiretroviral therapy},
	Volume = {53},
	Year = {2004}}

@article{Scharfstein&Tsiatis&Robins97,
	Author = {D.O. Scharfstein and A.A. Tsiatis and J.M. Robins},
	Journal = {Journal of the American Statistical Association},
	Number = {440},
	Pages = {1342--1350},
	Title = {Semiparametric efficiency and its implications on the design and analysis of group-sequential studies},
	Volume = {92},
	Year = {1997}}

@article{Bembometal07,
	Author = {O. Bembom and M. Petersen and SY Rhee and W.J. Fessel and S.E. Sinisi and R.W. Shafer and M.J. van der Laan},
	Journal = {U.C. Berkeley Division of Biostatistics Working Paper Series},
	Optmonth = {August},
	Optnote = {http://www.bepress.com/ucbbiostat/paper221},
	Title = {Biomarker Discovery Using Targeted Maximum Likelihood Estimation: Application to the Treatment of Antiretroviral Resistant {HIV} Infection},
	Volume = {221},
	Year = {2007}}

@article{vanderLaan&Gruber09,
	Author = {M.J. van der Laan and S. Gruber},
	Journal = {The International Journal of Biostatistics},
	Title = {Collaborative Double robust penalized targeted maximum likelihood estimation},
	Year = {2009}}

@article{vanderLaan&Rubin06,
	Author = {M.J. van der Laan and D. Rubin},
	Journal = {The International Journal of Biostatistics},
	Number = {1},
	Optnote = {http://www.bepress.com/ijb/vol2/iss1/11},
	Title = {Targeted Maximum Likelihood Learning},
	Volume = {2},
	Year = {2006}}

@article{Scharfstein&Tsiatis98,
	Author = {D.O. Scharfstein and A.A. Tsiatis},
	Journal = {Statistics in Medicine},
	Pages = {75--87},
	Title = {The use of simulation and bootstrap in information based group sequential studies},
	Volume = {17},
	Year = {1998}}

@article{Pampallona&Tsiatis&Kim01,
	Author = {S. Pampallona and A.A. Tsiatis and K. Kim},
	Journal = {Drug Informational Journal},
	Pages = {1113-1121},
	Title = {Interim monitoring of group sequential trials using spending functions for the type I and type II error probabilities},
	Volume = {35},
	Year = {2001}}

@article{Tsiatis&Mehta03,
	Author = {A.A. Tsiatis and C. Mehta},
	Journal = {Biometrika},
	Pages = {367-378},
	Title = {On the inefficiency of the adaptive design for monitoring clinical trials},
	Volume = {90},
	Year = {2003}}

@book{tsiatis2006,
	Author = {Tsiatis, A.A.},
	Isbn = {9780387324487},
	Lccn = {2006921164},
	Publisher = {Springer},
	Series = {Springer series in statistics},
	Title = {Semiparametric theory and missing data},
	Url = {http://books.google.com/books?id=xqZFi2EMB40C},
	Year = {2006},
	Bdsk-Url-1 = {http://books.google.com/books?id=xqZFi2EMB40C}}

@article{Banerjee&Tsiatis06,
	Author = {A. Banerjee and A.A. Tsiatis},
	Journal = {Statistics in Medicine},
	Optnote = {In press},
	Title = {Adaptive two-stage designs in phase II clinical trials},
	Year = {2006}}

@article{Tsiatis06,
	Author = {A.A. Tsiatis},
	Journal = {Statistics in Medicine},
	Optnote = {In press},
	Title = {Information based monitoring of clinical trials},
	Year = {2006}}

@article{Lokhnygina&Tsiatis06,
	Author = {Y. Lokhnygina and A.A. Tsiatis},
	Journal = {Journal of Statistical Planning and Inference},
	Optnote = {In press},
	Title = {Optimal two-stage group sequential designs},
	Year = {2006}}

@article{Bauer&Kohne94,
	Author = {P. Bauer and Kohne},
	Journal = {Biometrics},
	Pages = {1029--1041},
	Title = {Evaluation of experiments with adaptive interim analysis},
	Year = {1994}}

@article{Cui&Hung&Wang99,
	Author = {L. Cui and H.M.J. Hung and S-J Wang},
	Journal = {Biometrics},
	Pages = {853--857},
	Title = {Modification of sample size in group sequential trials},
	Year = {1999}}

@article{Jennison&Turnbull03,
	Author = {C. Jennison and B.W. Turnbull},
	Journal = {Statistics in Medicine},
	Pages = {971--993},
	Title = {Mid course sample size modification in clinical trials based on hte observed treatment effect},
	Year = {2003}}

@article{Koyama&Sampson&Gleser04,
	Author = {T. Koyama and A.R. Sampson and L.J. Gleser},
	Journal = {Journal of the Americal Statistical Association},
	Title = {A calculus for design of two stage adaptive procedures},
	Year = {2004}}

@article{Lan&Trost97,
	Author = {K.K.G Lan and D.C. Trost},
	Journal = {Proceedings Biopharm Section},
	Pages = {48-51},
	Title = {Estimation of parameters and sample size re-estimation},
	Year = {1997}}

@article{Lietal02,
	Author = {G. Li and W.J. Shih and T. Xie and J. Lu},
	Journal = {Biostatistics},
	Pages = {277--287},
	Title = {A sample size adjustment procedure for clinical trials based on conditional power},
	Year = {2002}}

@article{Mehta&Tsiatis01,
	Author = {C.R. Mehta and A.A. Tsiatis},
	Journal = {Drug Informational Journal},
	Pages = {1095--1112},
	Title = {Flexible sample size considerations using information based interim monitoring},
	Volume = {35},
	Year = {2001}}

@article{Mulle&Shafer01,
	Author = {H.H. Mulle and H. Shafer},
	Journal = {Biometrics},
	Pages = {886--891},
	Title = {Adaptive group sequential designs for clinical trials: combining the advantages of adaptive and classical group sequential approaches},
	Volume = {57},
	Year = {2001}}

@article{Proschan&Hunsberger95,
	Author = {M.A. Proschan and S.A. Hunsberger},
	Journal = {Biometrics},
	Pages = {1315--1324},
	Title = {Designed extension studies based on conditional power},
	Volume = {51},
	Year = {1995}}

@article{Shen&Fisher99,
	Author = {Y. Shen and L.D. Fisher},
	Journal = {Biometrics},
	Pages = {190--197},
	Title = {Statistical Inference for self-designing clinical trials with a one-sided hypothesis},
	Volume = {55},
	Year = {1999}}

@article{Wittes&Brittain90,
	Author = {J. Wittes and E. Brittain},
	Journal = {Statistics in Medicine},
	Pages = {65--72},
	Title = {The role of internal pilot studies in increasing efficiency of clinical trials},
	Volume = {9},
	Year = {1999}}

@article{Shen&Cheng06,
	Author = {Y. Shen and Y. Cheng},
	Journal = {Biostatistics},
	Optnote = {In Press},
	Title = {Adaptive design: Estimation and Inference with censored data in a semiparametric model},
	Year = {2006}}

@book{Spiegelalter&Abrams&Myles04,
	Author = {D.J. Spiegelalter and K.R. Abrams and J.P. Myles},
	Publisher = {Wiley, Chichester},
	Title = {Bayesian approaches to clinical trials and health care evaluation},
	Year = {2004}}

@book{Berry&Stangl96,
	Author = {D.A. Berry and D.K. Stangl},
	Publisher = {Marcel Dekker, New York},
	Title = {Bayesian biostatistics},
	Year = {1996}}

@article{Berry06,
	Author = {D.A. Berry},
	Journal = {Nature Reviews, Drug Discovery},
	Title = {Bayesian clinical trials},
	Volume = {5},
	Year = {2006}}

@book{Hu&Rosenberger06,
	Author = {F. Hu and W.F. Rosenberger},
	Publisher = {New York Wiley},
	Title = {The theory of response adaptive randomization in clinical trials},
	Year = {2006}}

@book{Dudoit&vanderLaan08,
	Author = {S. Dudoit and M.J. van der Laan},
	Publisher = {Springer Series of Statistics, New York},
	Title = {Resampling based multiple testing with applications to genomics},
	Year = {2008}}

@book{Sen&Singer93,
	Author = {P.K. Sen and J.M. Singer},
	Publisher = {Chapman \& Hall, New York},
	Title = {Large Sample Methods in Statistics: An Introduction with Applications},
	Year = {1993}}

@article{Bai&Hu&Rosenberger02,
	Author = {Z.D. Bai and F. Hu and W.F. Rosenberger},
	Journal = {Annals of Statistics},
	Number = {1},
	Pages = {122--139},
	Title = {Asymptotic properties of adaptive designs for clinical trials with delayed response},
	Volume = {30},
	Year = {2002}}

@article{Andersen&Faries&Tamura94,
	Author = {J. Andersen and D. Faries and R. Tamura},
	Journal = {Communication in Statistical Theory},
	Pages = {309--323},
	Title = {A randomized play-the-winner design for multiarm clinical trials},
	Volume = {23},
	Year = {1994}}

@book{Flournoy&Rosenberger95,
	Author = {N. Flournoy and W.F. Rosenberger},
	Publisher = {Hayward, Institute of Mathematical Statistics},
	Title = {Adaptive Designs},
	Year = {1995}}

@article{Hu&Rosenberger00,
	Author = {F. Hu and W.F. Rosenberger},
	Journal = {Statistics in Medicine},
	Pages = {2067--2075},
	Title = {Analysis of time trends in adaptive designs withi appliation to a neurophysiology experiment},
	Volume = {19},
	Year = {2000}}

@article{Rosenberger96,
	Author = {W.F. Rosenberger},
	Journal = {Statistical Science},
	Pages = {137--149},
	Title = {New directions in adaptive designs},
	Volume = {11},
	Year = {1996}}

@article{Rosenberger&Flournoy&Durham97,
	Author = {W.F. Rosenberger and N. Flournoy and S.D. Durham},
	Journal = {Journal of Statistical Planning and Inference},
	Pages = {69--76},
	Title = {Asymptotic normality of maximum likelihood estimators from multiparameter response driven designs},
	Year = {1997}}

@article{Rosenberger&Grill97,
	Author = {W.F. Rosenberger and S.E. Grill},
	Journal = {Statistics in Medicine},
	Pages = {2245--2260},
	Title = {A sequential design for psychophysical experiments: An application to estimating timing of sensory events},
	Volume = {16},
	Year = {1997}}

@article{Rosenberger&Sriram97,
	Author = {W.F. Rosenberger and T.N. Shiram},
	Journal = {Journal of Statistical Planning and Inference},
	Pages = {309--319},
	Title = {Estimation for an adaptive allocation design},
	Volume = {59},
	Year = {1997}}

@article{Tamuraetal94,
	Author = {R.N. Tamura and D.E. Faries and J.S. Andersen and J.H. Heiligenstein},
	Journal = {Journal of the American Statistical Association},
	Pages = {768--776},
	Title = {A case study of an adaptive clinical trial in the treatment of out-patients with depressive disorder},
	Volume = {89},
	Year = {1994}}

@article{Wei&Durham78,
	Author = {L.J. Wei and S. Durham},
	Journal = {Journal of the American Statistical Association},
	Pages = {840--843},
	Title = {The randomize play-the-winner rule in medical trials},
	Volume = {73},
	Year = {1978}}

@article{Weietal90,
	Author = {L.J. Wei and R.T. Smythe and D.Y. Lin and T.S. Park},
	Journal = {Journal of the American Statistical Association},
	Pages = {156--162},
	Title = {Statistical Inference with data-dependent treatment allocation rules},
	Volume = {85},
	Year = {1990}}

@article{Zelen69,
	Author = {M. Zelen},
	Journal = {Journal of the American Statistical Association},
	Pages = {131--146},
	Title = {Play the winner rule and the controlled clinical trial},
	Volume = {64},
	Year = {1969}}

@article{Cheng&Shen05,
	Author = {Y. Cheng and Y. Shen},
	Journal = {Biometrika},
	Number = {3},
	Pages = {633--646},
	Title = {Bayesian adaptive designs for clinical trials},
	Volume = {92},
	Year = {2005}}

@article{Wei79,
	Author = {L.J. Wei},
	Journal = {Annals of Statistics},
	Pages = {291--296},
	Title = {The generalized Polya's urn design for sequential medical trials},
	Volume = {7},
	Year = {1979}}

@article{Benito&Lopez&Soriano03,
	Author = {Benito, J. M. and Lopez, M. and Soriano, V.},
	Journal = {J Infect Dis},
	Keywords = {ADP-ribosyl Cyclase/metabolism Anti-HIV Agents/therapeutic use Antigens, CD/metabolism CD4-Positive T-Lymphocytes/*immunology CD8-Positive T-Lymphocytes/immunology HIV Infections/drug therapy/*immunology/virology HIV-1/*physiology Human *Viral Load Virus Replication},
	Note = {0022-1899 Comment Letter},
	Number = {5},
	Pages = {794-5; author reply 795-6},
	Title = {Virus load and cytolitic responses in human immunodeficiency virus infection: what is cause and what is effect},
	Volume = {188},
	Year = {2003}}

@article{DEttorreetal02,
	Abstract = {OBJECTIVE: To study virologic and immunologic factors associated with discordant treatment response in HIV-infected patients receiving highly active antiretroviral therapy (HAART). DESIGN: Study participants included a total of 27 patients: (a) 10 discordant patients (mean CD4+ cell count, 396.1 x 10 cells/l; mean HIV-RNA, 5.4 log copies/ml); (b) seven responder patients (mean CD4+ cell count, 997.5 x 10 cells/l); and (c) 10 failing patients (mean CD4+ cell count 66.5 x 10 cells/l; mean HIV-RNA, 5.4 log copies/ml).(10) (10)METHODS: The HIV-1 isolation rate and biological phenotype, drug resistance genotypic mutations of HIV-1 strains, recall and HIV-1-specific antigen lymphocyte proliferation (LP), and interleukin (IL)-15 production were studied. RESULTS: Virus isolation was obtained in 30% of discordant patients, and in 100% of failing patients. A higher replication constant was reported in discordant patients. No difference in the number of drug resistance mutations and biological phenotypes of HIV-1 was found in discordant patients with respect to failing patients. Discordant patients developed positive LP responses to and HIV-1 p24. LP in response to, HIV-1 p24 and gp160 was positive in responder patients. No significant LP was found in failing patients. Increased levels of IL-15 after stimulation with lipopolysaccaride (LPS) and were found in both discordant patients and responder patients. Conversely, a strong reduction of IL-15 levels was observed in failing patients. CONCLUSION: The present results suggest that decreased virus isolation rate, restoration of both lymphocyte proliferation and IL-15 production are factors involved in the discordant antiretroviral therapy response of HIV-infected patients.},
	Author = {D'Ettorre, G. and Forcina, G. and Andreotti, M. and Sarmati, L. and Palmisano, L. and Galluzzo, C. M. and Nicastri, E. and Mastroianni, C. M. and Vullo, V. and Vella, S. and Andreoni, M.},
	Journal = {Aids},
	Keywords = {Adult Anti-HIV Agents/*therapeutic use Antiretroviral Therapy, Highly Active CD4 Lymphocyte Count CD8-Positive T-Lymphocytes/drug effects/immunology Candida albicans Drug Resistance, Viral Female HIV Infections/complications/*drug therapy/immunology/virology HIV-1/drug effects/genetics/*immunology/isolation & purification Human Interleukin-15/*blood Male Middle Aged Mutation Viral Load Virus Replication/drug effects},
	Note = {0269-9370 Journal Article},
	Number = {14},
	Pages = {1877-85},
	Title = {Discordant response to antiretroviral therapy: {HIV} isolation, genotypic mutations, T-cell proliferation and cytokine production},
	Volume = {16},
	Year = {2002}}

@article{Davenportetal02,
	Abstract = {Early infection with HIV-1 is dominated by CCR5-tropic (R5, non-syncytium-inducing) viruses. The evolution of CXCR4-tropic (X4, syncytium-inducing) viruses occurs later in the infection and is associated with rapid disease progression. Here, we propose that the tropism of X4 viruses for naive CD4+ T cells is disadvantageous in early infection owing to the low division rate of these cells. In healthy individuals, the division rate of memory cells is nearly ten times higher than that of naive cells and thus the memory-cell tropism of R5 viruses could account for their dominance early in infection. As the division rate of naive T cells increases with CD4+ depletion, X4 viruses come to dominate in late disease.},
	Author = {Davenport, M. P. and Zaunders, J. J. and Hazenberg, M. D. and Schuitemaker, H. and van Rij, R. P.},
	Journal = {Trends Microbiol},
	Keywords = {CD4-Positive T-Lymphocytes/*virology HIV Infections/*immunology/metabolism HIV-1/*pathogenicity Human Immunologic Memory Macrophages/*virology Models, Biological Receptors, CCR5/metabolism Receptors, CXCR4/metabolism Tropism},
	Note = {0966-842x Journal Article},
	Number = {6},
	Pages = {275-8},
	Title = {Cell turnover and cell tropism in HIV-1 infection},
	Volume = {10},
	Year = {2002}}

@article{Deeksetal00,
	Abstract = {The relationship between plasma human immunodeficiency virus (HIV) RNA levels and peripheral CD4+ T cell counts was examined in 380 HIV-infected adults receiving long-term protease inhibitor therapy. Patients experiencing virologic failure (persistent HIV RNA >500 copies RNA/mL) generally had CD4+ T cell counts that remained greater than pretherapy baseline levels, at least through 96 weeks of follow-up. The CD4+ T cell response was directly and independently related to degree of viral suppression below the pretreatment baseline. For any given HIV RNA level measured 12 weeks after virologic failure, subsequent CD4+ T cell decline was slower in patients receiving a protease inhibitor-based regimen than in a historical control group of untreated patients. These observations suggest that transient or partial declines in plasma HIV RNA levels can have sustained effects on CD4+ T cell levels.},
	Author = {Deeks, S. G. and Barbour, J. D. and Martin, J. N. and Swanson, M. S. and Grant, R. M.},
	Journal = {J Infect Dis},
	Keywords = {Adult *CD4 Lymphocyte Count Female HIV Infections/*drug therapy/immunology/virology HIV Protease Inhibitors/*therapeutic use Human Male RNA, Viral/*blood Support, Non-U.S. Gov't Support, U.S. Gov't, P.H.S.},
	Note = {0022-1899 Journal Article},
	Number = {3},
	Pages = {946-53},
	Title = {Sustained CD4+ T cell response after virologic failure of protease inhibitor-based regimens in patients with human immunodeficiency virus infection},
	Volume = {181},
	Year = {2000}}

@article{Deeksetal01,
	Abstract = {BACKGROUND: In many patients with human immunodeficiency virus (HIV) infection, therapy with potent antiretroviral drugs does not result in complete suppression of HIV replication. The effect of cessation of therapy in these patients is unknown. METHODS: Sixteen patients who had a plasma HIV RNA level of more than 2500 copies per milliliter during combination antiretroviral-drug therapy were randomly assigned, in a 2:1 ratio, to discontinue or continue therapy. Plasma HIV RNA levels, CD4 cell counts, and drug susceptibility were measured weekly. Viral replicative capacity was measured at base line and at week 12. RESULTS: Discontinuation of therapy for 12 weeks was associated with a median decrease in the CD4 cell count of 128 cells per cubic millimeter and an increase in the plasma HIV RNA level of 0.84 log copies per milliliter. Virus from all patients with detectable resistance at entry became susceptible to HIV-protease inhibitors within 16 weeks after the discontinuation of therapy. Drug susceptibility began to increase a median of six weeks after the discontinuation of therapy and was temporally associated with increases in plasma HIV RNA levels and decreases in CD4 cell counts. Viral replicative capacity, measured by means of a recombinant-virus assay, was low at entry into the study and increased after therapy was discontinued. Despite the loss of detectable resistance in plasma, resistant virus was cultured from peripheral-blood mononuclear cells in five of nine patients who could be evaluated. Plasma HIV RNA levels, CD4 cell counts, and drug susceptibility remained stable in the patients who continued therapy. CONCLUSIONS: Despite the presence of reduced drug susceptibility, antiretroviral-drug therapy can provide immunologic and virologic benefit. This benefit reflects continued antiviral-drug activity and the maintenance of a viral population with a reduced replicative capacity.},
	Author = {Deeks, S. G. and Wrin, T. and Liegler, T. and Hoh, R. and Hayden, M. and Barbour, J. D. and Hellmann, N. S. and Petropoulos, C. J. and McCune, J. M. and Hellerstein, M. K. and Grant, R. M.},
	Journal = {N Engl J Med},
	Keywords = {Adult Anti-HIV Agents/pharmacology/*therapeutic use CD4 Lymphocyte Count Drug Resistance, Microbial Drug Therapy, Combination HIV Infections/*drug therapy/immunology/virology HIV Protease Inhibitors/pharmacology/*therapeutic use HIV-1/*drug effects/genetics/isolation & purification Human Male Middle Aged Proportional Hazards Models Prospective Studies RNA, Viral/blood Support, Non-U.S. Gov't Support, U.S. Gov't, P.H.S. Viremia/drug therapy},
	Note = {0028-4793 Clinical Trial Journal Article Randomized Controlled Trial},
	Number = {7},
	Pages = {472-80},
	Title = {Virologic and immunologic consequences of discontinuing combination antiretroviral-drug therapy in HIV-infected patients with detectable viremia},
	Volume = {344},
	Year = {2001}}

@article{Deeks01,
	Abstract = {Although understanding of nonnucleoside reverse transcriptase inhibitor (NNRTI) resistance is less clearly established than that of other classes of antiretroviral drugs, certain facts have been established. The treatment-associated genetic mutation profiles of the available NNRTIs have been mapped, and resistance has been found to develop rapidly after initiation of NNRTI therapy. Despite the chemical diversity of the NNRTIs, cross-resistance among agents of this class is nearly universal. Although the viral replicative capacity (``fitness") of NNRTI-induced viral variants has not been extensively studied, available data suggest that NNRTI-selected mutations confer little damage to viral fitness, and thus a single point mutation produces a strain that is both resistant and fit. Furthermore, with continued therapy, viral evolution persists, creating species with greater numbers of mutations and higher level phenotypic resistance. Taken together, these facts suggest that continued use of NNRTIs after emergence of resistance will produce variants of complex mutational patterns that limit future treatment options, and, therefore, strong consideration should be given to discontinuing NNRTIs after virologic failure is confirmed. This article describes the scientific literature establishing the efficacy and limitations of NNRTI therapy and attempts to define a role for this class of drug in the long-term treatment of HIV-1 disease.},
	Author = {Deeks, S. G.},
	Journal = {J Acquir Immune Defic Syndr},
	Keywords = {Anti-HIV Agents/*pharmacology/therapeutic use Clinical Trials Delavirdine/pharmacology/therapeutic use *Drug Resistance, Microbial Drug Therapy, Combination HIV Infections/drug therapy/transmission HIV-1/*drug effects/genetics/metabolism HIV-1 Reverse Transcriptase/chemistry/genetics Human Nevirapine/pharmacology/therapeutic use Oxazines/pharmacology/therapeutic use Phylogeny Point Mutation/drug effects Protein Conformation Reverse Transcriptase Inhibitors/*pharmacology/therapeutic use Virus Replication/drug effects},
	Note = {1525-4135 Journal Article Review Review, Tutorial},
	Pages = {S25-33},
	Title = {International perspectives on antiretroviral resistance. Nonnucleoside reverse transcriptase inhibitor resistance},
	Volume = {26 Suppl 1},
	Year = {2001}}

@article{Deeksetal02,
	Abstract = {BACKGROUND: Sustained elevations in CD4 cell counts commonly occur despite incomplete viral suppression with protease inhibitor-based antiretroviral therapy. OBJECTIVES: To determine the incidence and risk factors associated with return of CD4 cell count to pre-therapy levels in patients experiencing virologic failure of protease inhibitor therapy. DESIGN: This is a clinic-based cohort study of HIV-infected adults who failed to maintain durable viral suppression on a protease inhibitor-based regimen. MAIN OUTCOME MEASURES: Virologic failure was defined as persistent plasma HIV RNA level > 500 copies/ml. Immunologic failure was defined as return of CD4 cell count to pre-therapy levels. RESULTS: A total of 291 patients experienced virologic failure on a protease inhibitor-based regimen and had a treatment-mediated CD4 cell increase above pre-therapy levels at the time of virologic failure. If patient data were censored at the time a successful salvage regimen was initiated, then the median time to immunologic failure after the onset of virologic failure was 3 years. If patient data were also censored at the time therapy was discontinued, then 36.8% of the cohort experienced immunologic failure after 3 years of continuous virologic failure. The change in viral load from a pre-treatment baseline, and not the absolute level of viremia achieved, was a strong and independent predictor of immunologic failure. Discontinuing therapy was associated with immunologic failure independent of viral load changes. CONCLUSION: Reduction in T CD4+ cell numbers may eventually occur during prolonged virologic failure of a protease inhibitor-based regimen and is predicted by the degree of virologic suppression below a pre-therapy 'set-point'.},
	Author = {Deeks, S. G. and Barbour, J. D. and Grant, R. M. and Martin, J. N.},
	Journal = {Aids},
	Keywords = {Adult Antiretroviral Therapy, Highly Active CD4 Lymphocyte Count CD4-Positive T-Lymphocytes/cytology/*drug effects Disease Progression HIV Infections/blood/*drug therapy/immunology/virology HIV Protease Inhibitors/*therapeutic use HIV-1/*drug effects/genetics Human Indinavir/therapeutic use Nelfinavir/therapeutic use RNA, Viral/blood Ritonavir/therapeutic use Saquinavir/therapeutic use Support, Non-U.S. Gov't Support, U.S. Gov't, P.H.S. Time Factors Treatment Failure Viremia/blood/*drug therapy/immunology/virology},
	Note = {0269-9370 Journal Article},
	Number = {2},
	Pages = {201-7},
	Title = {Duration and predictors of CD4 T-cell gains in patients who continue combination therapy despite detectable plasma viremia},
	Volume = {16},
	Year = {2002}}

@article{Deeks03,
	Abstract = {Drug-resistant HIV-1 is a cause of growing clinical and public-health concern. In many patients, combination antiretroviral therapy fails to achieve complete viral suppression (virological failure). Continuing viral replication during therapy leads to the accumulation of drug-resistance mutations, resulting in increased viral load and a greater risk of disease progression. Patients with drug-resistant HIV-1 infection have three therapeutic options: a change to a salvage regimen with the aim of fully suppressing viral replication; interruption of therapy; or continuation of a partially effective regimen. The first strategy is preferred for most patients failing their first or perhaps their second regimen. However, the best approach remains unclear for patients who have failed multiple treatment regimens and who have limited options for complete viral suppression. The management of such patients requires a careful understanding of the pathogenesis of drug-resistant HIV-1, the clinical consequences of virological failure, the potential benefits and limitations of diagnostic assays, and the likelihood that agents in development will be effective.},
	Author = {Deeks, S. G.},
	Journal = {Lancet},
	Keywords = {Anti-HIV Agents/*immunology/*therapeutic use Antiretroviral Therapy, Highly Active/methods Drug Resistance, Viral/genetics/immunology Drug Therapy, Combination HIV Infections/*drug therapy/immunology/virology HIV Protease Inhibitors/immunology/therapeutic use *HIV-1/drug effects/genetics/immunology Human Randomized Controlled Trials Ritonavir/immunology/therapeutic use Support, Non-U.S. Gov't Support, U.S. Gov't, P.H.S. Treatment Outcome Viral Load/statistics & numerical data Virus Replication/drug effects/immunology},
	Note = {1474-547x Journal Article Review Review, Academic},
	Number = {9400},
	Pages = {2002-11},
	Title = {Treatment of antiretroviral-drug-resistant HIV-1 infection},
	Volume = {362},
	Year = {2003}}

@incollection{robins&Li2008,
address = "Beachwood, Ohio, USA",
author = "Robins, James and Li, Lingling and Tchetgen, Eric and van der Vaart, Aad",
booktitle = "Probability and Statistics: Essays in Honor of David A. Freedman",
doi = "10.1214/193940307000000527",
editor = "Nolan, Deborah and Speed, Terry",
pages = "335--421",
publisher = "Institute of Mathematical Statistics",
series = "Collections",
title = "Higher order influence functions and minimax estimation of nonlinear functionals",
url = "http://dx.doi.org/10.1214/193940307000000527",
volume = "Volume 2",
year = "2008"
}


@article{Deeks&Walker04,
	Abstract = {A potent antigen-specific T cell response to HIV infection can contribute to the control of viral replication and is therefore beneficial to the host. However, HIV-mediated increases in generalized T cell activation also appear to accelerate both viral replication and CD4+ T cell depletion. A new study in the JCI attempts to experimentally distinguish the beneficial versus harmful aspects of this immune response.},
	Author = {Deeks, S. G. and Walker, B. D.},
	Journal = {J Clin Invest},
	Note = {0021-9738 Comment Journal Article},
	Number = {6},
	Pages = {808-10},
	Title = {The immune response to AIDS virus infection: good, bad, or both?},
	Volume = {113},
	Year = {2004}}

@techreport{DHHS04,
	Author = {DHHS},
	Institution = {Panel on Clinical Practices for Treatment of HIV Infection, Department of Health and Human Services},
	Month = {March 23},
	Title = {Guidelines for the use of antiretroviral agents in HIV-1 infected adults and adolescents},
	Year = {2004}}

@article{Faureetal00,
	Abstract = {Human immunodeficiency virus (HIV) enters cells in vitro via CD4 and a coreceptor. Which of 15 known coreceptors are important in vivo is poorly defined but may be inferred from disease-modifying mutations, as for CCR5. Here two single nucleotide polymorphisms are described in Caucasians in CX3CR1, an HIV coreceptor and leukocyte chemotactic/adhesion receptor for the chemokine fractalkine. HIV-infected patients homozygous for CX3CR1-I249 M280, a variant haplotype affecting two amino acids (isoleucine-249 and methionine-280), progressed to AIDS more rapidly than those with other haplotypes. Functional CX3CR1 analysis showed that fractalkine binding is reduced among patients homozygous for this particular haplotype. Thus, CX3CR1-I249 M280 is a recessive genetic risk factor in HIV/AIDS.},
	Author = {Faure, S. and Meyer, L. and Costagliola, D. and Vaneensberghe, C. and Genin, E. and Autran, B. and Delfraissy, J. F. and McDermott, D. H. and Murphy, P. M. and Debre, P. and Theodorou, I. and Combadiere, C.},
	Journal = {Science},
	Keywords = {Acquired Immunodeficiency Syndrome/genetics/*physiopathology/virology Case-Control Studies *Chemokines, CX3C Chemokines, CXC/metabolism Chromosomes, Human, Pair 3 Cohort Studies Disease Progression European Continental Ancestry Group/genetics Genotype HIV/physiology HIV Infections/genetics/*physiopathology/virology Haplotypes Homozygote Human Leukocytes, Mononuclear/metabolism Linkage Disequilibrium Membrane Proteins/metabolism Mutation Polymorphism, Restriction Fragment Length *Polymorphism, Single Nucleotide Polymorphism, Single-Stranded Conformational Receptors, Cytokine/*genetics/*physiology Receptors, HIV/*genetics/*physiology Support, Non-U.S. Gov't Survival Analysis Variation (Genetics)},
	Note = {0036-8075 Comment Journal Article},
	Number = {5461},
	Pages = {2274-7},
	Title = {Rapid progression to AIDS in HIV+ individuals with a structural variant of the chemokine receptor CX3CR1},
	Volume = {287},
	Year = {2000}}

@article{Gaoetal01,
	Abstract = {BACKGROUND: From studies of genetic polymorphisms and the rate of progression from human immunodeficiency virus type 1 (HIV-1) infection to the acquired immunodeficiency syndrome (AIDS), it appears that the strongest susceptibility is conferred by the major-histocompatibility-complex (MHC) class I type HLA-B*35,Cw*04 allele. However, cytotoxic T-lymphocyte responses have been observed against HIV-1 epitopes presented by HLA-B*3501, the most common HLA-B*35 subtype. We examined subtypes of HLA-B*35 in five cohorts and analyzed the relation of structural differences between HLA-B*35 subtypes to the risk of progression to AIDS. METHODS: Genotyping of HLA class I loci was performed for 850 patients who seroconverted and had known dates of HIV-1 infection. Survival analyses with respect to the rate of progression to AIDS were performed to identify the effects of closely related HLA-B*35 subtypes with different peptide-binding specificities. RESULTS: HLA-B*35 subtypes were divided into two groups according to peptide-binding specificity: the HLA-B*35-PY group, which consists primarily of HLA-B*3501 and binds epitopes with proline in position 2 and tyrosine in position 9; and the more broadly reactive HLA-B*35-Px group, which also binds epitopes with proline in position 2 but can bind several different amino acids (not including tyrosine) in position 9. The influence of HLA-B*35 in accelerating progression to AIDS was completely attributable to HLA-B*35-Px alleles, some of which differ from HLA-B*35-PY alleles by only one amino acid residue. CONCLUSIONS: This analysis shows that, in patients with HIV-1 infection, a single amino acid change in HLA molecules has a substantial effect on the rate of progression to AIDS. The different consequences of HLA-B*35-PY and HLA-B*35-Px in terms of disease progression highlight the importance of the epitope specificities of closely related class I molecules in the immune defense against HIV-1.},
	Author = {Gao, X. and Nelson, G. W. and Karacki, P. and Martin, M. P. and Phair, J. and Kaslow, R. and Goedert, J. J. and Buchbinder, S. and Hoots, K. and Vlahov, D. and O'Brien, S. J. and Carrington, M.},
	Journal = {N Engl J Med},
	Keywords = {Acquired Immunodeficiency Syndrome/*genetics African Continental Ancestry Group/genetics Alleles Amino Acid Sequence Binding Sites/genetics Disease Progression Disease-Free Survival European Continental Ancestry Group/genetics *Genes, MHC Class I Genotype HIV Infections/ethnology/*genetics/immunology HLA-B35 Antigen/chemistry/*genetics HLA-C Antigens Human Peptides/metabolism Proportional Hazards Models Receptors, Peptide/chemistry/genetics/metabolism Support, U.S. Gov't, P.H.S.},
	Note = {0028-4793 Journal Article Multicenter Study},
	Number = {22},
	Pages = {1668-75},
	Title = {Effect of a single amino acid change in MHC class I molecules on the rate of progression to AIDS},
	Volume = {344},
	Year = {2001}}

@article{Grabaretal00,
	Abstract = {BACKGROUND: The prognostic value of discordant immunologic (CD4 cell increase) and virologic (plasma HIV RNA level decrease) responses to antiretroviral treatment is not known. OBJECTIVE: To study the relation between clinical outcome of HIV-infected patients receiving highly active antiretroviral therapy (HAART) and early immunologic and virologic responses to such therapy. DESIGN: Prospective cohort study. SETTING: 68 hospitals in France. PATIENTS: 2236 protease inhibitor-naive patients. INTERVENTION: Initiation of HAART with one protease inhibitor and two nucleoside analogues between July 1996 and March 1997. MEASUREMENTS: Immunologic and virologic response at 6 months. Multivariate Cox models were used to assess the relation between these responses and progression to a new AIDS-defining event or death. RESULTS: On the basis of 6-month immunologic and virologic responses, patients were classified into four groups: complete response (47.5%), complete nonresponse (16.2%), immunologic response only (19.0%), and virologic response only (17.3%). After month 6 and within a median of 18 months, 69 patients died and 123 experienced a new AIDS-defining event. After adjustment, complete nonresponders and those with only a virologic response had significantly higher risks for clinical progression at 6 months (relative risk, 3.38 [95% CI, 2.28 to 5.02] and 1.98 [CI, 1.26 to 3.10], respectively) than complete responders. The difference between complete responders and those with only an immunologic response at 6 months was weaker and nonsignificant (relative risk, 1.55 [CI, 0.96 to 2.50]). CONCLUSIONS: Immunologic response after 6 months of HAART indicates a favorable clinical outcome in HIV-infected patients regardless of virologic response. This suggests that both immunologic and virologic markers should be used in clinical practice to evaluate treatment response.},
	Author = {Grabar, S. and Le Moing, V. and Goujard, C. and Leport, C. and Kazatchkine, M. D. and Costagliola, D. and Weiss, L.},
	Journal = {Ann Intern Med},
	Keywords = {Adult CD4 Lymphocyte Count Disease Progression Drug Therapy, Combination Female HIV Infections/*drug therapy/immunology/virology HIV Protease Inhibitors/*therapeutic use *HIV-1/genetics Human Male Multivariate Analysis Proportional Hazards Models Prospective Studies RNA, Viral/blood Reverse Transcriptase Inhibitors/*therapeutic use Support, Non-U.S. Gov't Treatment Outcome Viral Load},
	Note = {0003-4819 Journal Article Multicenter Study},
	Number = {6},
	Pages = {401-10},
	Title = {Clinical outcome of patients with HIV-1 infection according to immunologic and virologic response after 6 months of highly active antiretroviral therapy},
	Volume = {133},
	Year = {2000}}

@article{Gruebetal00,
	Abstract = {BACKGROUND: Hepatitis C virus (HCV) infection is highly prevalent among HIV-1-infected individuals, but its contribution to the morbidity and mortality of coinfected patients who receive potent antiretroviral therapy is controversial. We used data from the ongoing Swiss HIV Cohort Study to analyse clinical progression of HIV-1, and the virological and immunological response to potent antiretroviral therapy in HIV-1-infected patients with or without concurrent HCV infection. METHODS: We analysed prospective data on survival, clinical disease progression, suppression of HIV-1 replication, CD4-cell recovery, and frequency of changes in antiretroviral therapy according to HCV status in 3111 patients starting potent antiretroviral therapy. RESULTS: 1157 patients (37.2%) were coinfected with HCV, 1015 of whom (87.7%) had a history of intravenous drug use. In multivariate Cox's regression, the probability of progression to a new AIDS-defining clinical event or to death was independently associated with HCV seropositivity (hazard ratio 1.7 [95% CI 1.26-2.30]), and with active intravenous drug use (1.38 [1.02-1.88]). Virological response to antiretroviral therapy and the probability of treatment change were not associated with HCV serostatus. In contrast, HCV seropositivity was associated with a smaller CD4-cell recovery (hazard ratio for a CD4-cell count increase of at least 50 cells/microL=0.79 [0.72-0.87]). INTERPRETATION: HCV and active intravenous drug use could be important factors in the morbidity and mortality among HIV-1-infected patients, possibly through impaired CD4-cell recovery in HCV seropositive patients receiving potent antiretroviral therapy. These findings are relevant for decisions about optimum timing for HCV treatment in the setting of HIV infection.},
	Author = {Greub, G. and Ledergerber, B. and Battegay, M. and Grob, P. and Perrin, L. and Furrer, H. and Burgisser, P. and Erb, P. and Boggian, K. and Piffaretti, J. C. and Hirschel, B. and Janin, P. and Francioli, P. and Flepp, M. and Telenti, A.},
	Journal = {Lancet},
	Keywords = {AIDS-Related Opportunistic Infections/*drug therapy Adolescent Adult Anti-HIV Agents/*therapeutic use CD4 Lymphocyte Count Cohort Studies Disease Progression Female Hepatitis C/complications/*drug therapy Human Male Middle Aged Prospective Studies Support, Non-U.S. Gov't Survival Analysis Switzerland Viral Load Viremia/etiology},
	Note = {0140-6736 Clinical Trial Journal Article},
	Number = {9244},
	Pages = {1800-5},
	Title = {Clinical progression, survival, and immune recovery during antiretroviral therapy in patients with HIV-1 and hepatitis C virus coinfection: the Swiss HIV Cohort Study},
	Volume = {356},
	Year = {2000}}

@article{Katzensteinetal96,
	Abstract = {BACKGROUND: We studied measures of human immunodeficiency virus (HIV) replication, the viral phenotype, and immune function (CD4 cell counts) and the relation of changes in these indicators to clinical outcomes in a subgroup of patients in a controlled trial of early antiretroviral treatment for HIV, the AIDS Clinical Trials Group Study 175. METHODS: The 391 subjects, each of whom entered the study with a single screening CD4 cell count of 200 to 500 per cubic millimeter, were randomly assigned to receive zidovudine alone, didanosine alone, zidovudine plus didanosine, or zidovudine plus zalcitabine. Plasma concentrations of HIV RNA were assessed in 366 subjects, and viral isolates from 332 subjects were assayed for the presence of the syncytium-inducing phenotype. RESULTS: After eight weeks, the mean (+/-SE) decrease from base line in the concentration of HIV RNA, expressed as the change in the base 10 log of the number of copies per milliliter, was 0.26+/-0.06 for patients treated with zidovudine alone, 0.65+/-0.07 for didanosine alone, 0.93+/-0.10 for zidovudine plus didanosine, and 0.89+/-0.06 for zidovudine plus zalcitabine (P<0.001 for each of the pairwise comparisons with zidovudine alone). Multivariate proportional-hazards models showed that higher base-line concentrations of plasma HIV RNA, less suppression of plasma HIV RNA by treatment, and the presence of the syncytium-inducing phenotype were significantly associated with an increased risk of progression to the acquired immunodeficiency syndrome and death. After adjustment for these measures of viral replication and for the viral phenotype, CD4 cell counts were not significant predictors of clinical outcome. CONCLUSIONS: Both the risk of the progression of HIV disease and the efficacy of antiretroviral therapy are strongly associated with the plasma level of HIV RNA and with the viral phenotype. The changes in the plasma concentration of HIV RNA predict the changes in CD4 cell counts and survival after treatment with reverse-transcriptase inhibitors.},
	Author = {Katzenstein, D. A. and Hammer, S. M. and Hughes, M. D. and Gundacker, H. and Jackson, J. B. and Fiscus, S. and Rasheed, S. and Elbeik, T. and Reichman, R. and Japour, A. and Merigan, T. C. and Hirsch, M. S.},
	Journal = {N Engl J Med},
	Keywords = {Adult Antiviral Agents/*therapeutic use CD4 Lymphocyte Count Didanosine/*therapeutic use Disease Progression Drug Therapy, Combination Female HIV/*genetics/isolation & purification/physiology HIV Infections/drug therapy/immunology/*virology Human Male Middle Aged Multivariate Analysis Phenotype Proportional Hazards Models RNA, Viral/*blood Support, U.S. Gov't, P.H.S. Treatment Outcome Virus Replication/drug effects Zidovudine/*therapeutic use},
	Note = {0028-4793 Clinical Trial Journal Article Multicenter Study Randomized Controlled Trial},
	Number = {15},
	Pages = {1091-8},
	Title = {The relation of virologic and immunologic markers to clinical outcomes after nucleoside therapy in HIV-infected adults with 200 to 500 CD4 cells per cubic millimeter. AIDS Clinical Trials Group Study 175 Virology Study Team},
	Volume = {335},
	Year = {1996}}

@article{Kaufmannetal98,
	Author = {Kaufmann, D. and Pantaleo, G. and Sudre, P. and Telenti, A.},
	Journal = {Lancet},
	Keywords = {Anti-HIV Agents/*therapeutic use CD4 Lymphocyte Count HIV Infections/drug therapy/*immunology Human Protease Inhibitors/*therapeutic use Support, Non-U.S. Gov't Viremia/drug therapy/*immunology},
	Note = {0140-6736 Letter},
	Number = {9104},
	Pages = {723-4},
	Title = {CD4-cell count in HIV-1-infected individuals remaining viraemic with highly active antiretroviral therapy (HAART). Swiss HIV Cohort Study},
	Volume = {351},
	Year = {1998}}

@article{Kaufmannetal03,
	Abstract = {BACKGROUND: Highly active antiretroviral therapy (HAART) for human immunodeficiency virus (HIV)-1 infection allows recovery of CD4 T lymphocytes. Few studies have explored the long-term T-lymphocyte responses to HAART. METHODS: Plasma HIV-1 RNA levels and CD4 and CD8 T-lymphocyte counts were longitudinally analyzed over 4 years in 2235 participants of the Swiss HIV Cohort, commencing HAART between 1996 and 1997. The CD4 T-lymphocyte count increase, the percentage of individuals with a CD4 T-lymphocyte count of 500/microL or greater and less than 200/microL, and the determinants of CD4 T-lymphocyte recovery were evaluated in individuals treated with continuous (CONT; n = 985) and discontinuous (DISCONT; n = 1250) HAART. RESULTS: At 4 years, 69.5% of subjects (CONT, 84.5%; DISCONT, 53.6%; P<.001) showed HIV-1 RNA levels below 400 copies/mL, while the median CD4 T-lymphocyte count increased from 190/microL to 423/microL (CONT, 486/microL; DISCONT, 343/microL; P<.001). Of the 2235 participants, 38.8% (CONT, 47.7%; DISCONT, 29.4%; P<.001) reached a CD4 T-lymphocyte count of 500/microL or greater, but in 15.6%, CD4 T-lymphocyte count remained below 200/microL (CONT, 5.9%; DISCONT, 25.9%; P<.001). Larger increases in CD4 T-lymphocyte count were associated with higher baseline HIV-1 RNA, a larger percentage of undetectable HIV-1 RNA levels, lower baseline CD8 T-lymphocyte count, and younger age. Individuals reaching a CD4 T-lymphocyte count of 500/microL or greater at 4 years were characterized by higher nadir and baseline CD4 T-lymphocyte counts and a more sustained reduction of HIV-1 RNA levels. CONCLUSIONS: At 4 years, only 39% of individuals treated with HAART reached a CD4 T-lymphocyte count of 500/microL or greater, and 16% with CD4 T-lymphocyte counts less than 200/microL remained susceptible to opportunistic infections. Treatment interruptions, a poor virologic response, and older age were the major factors negatively affecting the recovery of CD4 T lymphocytes.},
	Author = {Kaufmann, G. R. and Perrin, L. and Pantaleo, G. and Opravil, M. and Furrer, H. and Telenti, A. and Hirschel, B. and Ledergerber, B. and Vernazza, P. and Bernasconi, E. and Rickenbach, M. and Egger, M. and Battegay, M.},
	Journal = {Arch Intern Med},
	Keywords = {Adult *Antiretroviral Therapy, Highly Active *CD4 Lymphocyte Count CD8-Positive T-Lymphocytes Female HIV Infections/*drug therapy/*immunology *Hiv-1 Human Lymphocyte Count Male Middle Aged Prospective Studies RNA, Viral/*analysis Support, Non-U.S. Gov't Viral Load},
	Note = {0003-9926 Journal Article},
	Number = {18},
	Pages = {2187-95},
	Title = {CD4 T-lymphocyte recovery in individuals with advanced HIV-1 infection receiving potent antiretroviral therapy for 4 years: the Swiss HIV Cohort Study},
	Volume = {163},
	Year = {2003}}

@article{MartinezPicadoetal99,
	Abstract = {The relative replicative fitness of human immunodeficiency virus type 1 (HIV-1) mutants selected by different protease inhibitors (PIs) in vivo was determined. Each mutant was compared to wild type (WT), NL4-3, in the absence of drugs by several methods, including clonal genotyping of cultures infected with two competing viral variants, kinetics of viral antigen production, and viral infectivity/virion particle ratios. A nelfinavir-selected protease D30N substitution substantially decreased replicative capacity relative to WT, while a saquinavir-selected L90M substitution moderately decreased fitness. The D30N mutant virus was also outcompeted by the L90M mutant in the absence of drugs. A major natural polymorphism of the HIV-1 protease, L63P, compensated well for the impairment of fitness caused by L90M but only slightly improved the fitness of D30N. Multiply substituted indinavir-selected mutants M46I/L63P/V82T/I84V and L10R/M46I/L63P/V82T/I84V were just as fit as WT. These results indicate that the mutations which are usually initially selected by nelfinavir and saquinavir, D30N and L90M, respectively, impair fitness. However, additional mutations may improve the replicative capacity of these and other drug-resistant mutants. Hypotheses based on the greater fitness impairment of the nelfinavir-selected D30N mutant are suggested to explain observations that prolonged responses to delayed salvage regimens, including alternate PIs, may be relatively common after nelfinavir failure.},
	Author = {Martinez-Picado, J. and Savara, A. V. and Sutton, L. and D'Aquila, R. T.},
	Journal = {J Virol},
	Keywords = {Adaptation, Biological Amino Acid Substitution Animals Anti-HIV Agents/*pharmacology Cells, Cultured Drug Resistance, Microbial HIV Protease Inhibitors/*pharmacology HIV-1/*drug effects/genetics/physiology Human Mice Mutagenesis, Site-Directed Nelfinavir/*pharmacology Saquinavir/*pharmacology Support, Non-U.S. Gov't Support, U.S. Gov't, P.H.S. Tumor Cells, Cultured Virus Replication/*drug effects},
	Note = {0022-538x Journal Article},
	Number = {5},
	Pages = {3744-52},
	Title = {Replicative fitness of protease inhibitor-resistant mutants of human immunodeficiency virus type 1},
	Volume = {73},
	Year = {1999}}

@article{Mellorsetal96,
	Abstract = {The relation between viremia and clinical outcome in individuals infected with human immunodeficiency virus-type 1 (HIV-1) has important implications for therapeutic research and clinical care. HIV-1 RNA in plasma was quantified with a branched-DNA signal amplification assay as a measure of viral load in a cohort of 180 seropositive men studied for more than 10 years. The risk of acquired immunodeficiency syndrome (AIDS) and death in study subjects, including those with normal numbers of CD4+ T cells, was directly related to plasma viral load at study entry. Plasma viral load was a better predictor of progression to AIDS and death than was the number of CD4+ T cells.},
	Author = {Mellors, J. W. and Rinaldo, C. R., Jr. and Gupta, P. and White, R. M. and Todd, J. A. and Kingsley, L. A.},
	Journal = {Science},
	Keywords = {Acquired Immunodeficiency Syndrome/*virology Antiviral Agents/therapeutic use Biological Markers/blood CD4 Lymphocyte Count CD4-Positive T-Lymphocytes/virology Cohort Studies Disease Progression Follow-Up Studies HIV Infections/drug therapy/mortality/*virology HIV-1/genetics/*physiology Human Male Prognosis Proportional Hazards Models RNA, Viral/*blood Support, Non-U.S. Gov't Support, U.S. Gov't, Non-P.H.S. Support, U.S. Gov't, P.H.S. Survival Rate Time Factors Viremia/*virology Virus Replication},
	Note = {0036-8075 Comment Journal Article},
	Number = {5265},
	Pages = {1167-70},
	Title = {Prognosis in HIV-1 infection predicted by the quantity of virus in plasma},
	Volume = {272},
	Year = {1996}}

@article{Milleretal00,
	Abstract = {OBJECTIVE: To compare the rate of disease progression according to viral load and CD4 cell count in patients receiving or not receiving highly active antiretroviral therapy (HAART), defined as protease inhibitor-containing regimens. DESIGN: An observational study, with prospectively collected data. METHODS: All patients attending the HIV Outpatient clinic as of 1 January 1995 (n = 2083) were included. Follow-up was until the first AIDS-defining event or death. Associations between viral load or CD4 cell count and disease progression were assessed using a person-years approach. Event rates were compared using Poisson regression analysis; a multivariate model was used to assess the independent effects of CD4, viral load and treatment group on event rates and to consider interactions between these variables. RESULTS: The event rates increased with lower CD4 cell count and higher viral load for both treatment groups and were generally lower in the HAART group. In a multivariate analysis, lower CD4 cell counts and higher viral loads remained significantly associated with disease progression, irrespective of treatment group. However, the event rate was significantly lower for the HAART group compared with the control group (relative rate 0.53, P < 0.001). CONCLUSIONS: HAART-treated patients with high viral loads and CD4 cell counts experienced reduced disease progression compared with individuals with the same CD4 cell count and viral load not receiving HAART. Consequently, the short-term prognosis associated with viral load levels and CD4 cell counts may differ in patients on HAART. Whether this effect will be observed with non-protease-inhibitor-containing HAART is not known at this time.},
	Author = {Miller, V. and Sabin, C. A. and Phillips, A. N. and Rottmann, C. and Rabenau, H. and Weidmann, E. and Rickerts, V. and Findhammer, S. and Helm, E. B. and Staszewski, S.},
	Journal = {Aids},
	Keywords = {Adolescent Adult Aged Antiretroviral Therapy, Highly Active CD4 Lymphocyte Count Disease Progression HIV Infections/*drug therapy/pathology/virology HIV Protease Inhibitors/*therapeutic use *HIV-1/isolation & purification Human Middle Aged Prospective Studies RNA, Viral/analysis Regression Analysis Support, Non-U.S. Gov't Viral Load},
	Note = {0269-9370 Clinical Trial Journal Article},
	Number = {14},
	Pages = {2129-36},
	Title = {The impact of protease inhibitor-containing highly active antiretroviral therapy on progression of HIV disease and its relationship to CD4 and viral load},
	Volume = {14},
	Year = {2000}}

@article{Pikettyetal98,
	Abstract = {OBJECTIVES: To determine the clinical, virological and immunological outcome in a cohort of unselected patients receiving triple combination therapy for more than 1 year. METHODS: Prospective follow-up of a cohort of 162 unselected, protease inhibitor-naive, antiretroviral-experienced patients with advanced HIV disease, treated with indinavir combined with two nucleoside analogues. RESULTS: The mean CD4 cell count and plasma HIV RNA level in the study group at baseline were 69+/-5 x 10(6)/l and 4.75+/-0.07 log10 copies/ml, respectively. Five per cent of patients died prematurely or were lost to follow-up. Fifty-seven per cent of patients responded to therapy, as assessed by a sustained increase in CD4 cell counts above 50 x 10(6)/l and a decrease in plasma HIV RNA greater than 1 log10 copies/ml, throughout 12.1 months of follow-up. Seventeen per cent of patients were immunological and virological non-responders. Twenty-one per cent of patients exhibited discrepant virological and immunological responses to treatment, of whom one-half failed to exhibit significant increases in CD4 cells despite a virological response to therapy and one-half exhibited increased CD4 cell counts in the absence of significant decrease in plasma viral load. The incidence of AIDS-defining events in the latter group of patients was similar to that of responder patients, whereas their incidence was higher in patients who failed to exhibit a virological and immunological response and those who failed to increase CD4 cells despite a significant decrease in viral load. CONCLUSION: Our observations of discrepant immunological and virological responses to treatment raise the issue of the significance of persistent elevated levels of plasma HIV RNA and of the relevance of measurements of plasma viral load for assessing the efficacy of antiretroviral therapy in patients whose CD4 cell counts increase despite the absence of significant decrease in plasma HIV viral load.},
	Author = {Piketty, C. and Castiel, P. and Belec, L. and Batisse, D. and Si Mohamed, A. and Gilquin, J. and Gonzalez-Canali, G. and Jayle, D. and Karmochkine, M. and Weiss, L. and Aboulker, J. P. and Kazatchkine, M. D.},
	Journal = {Aids},
	Keywords = {Adult Aged Anti-HIV Agents/*therapeutic use Cohort Studies Drug Therapy, Combination Female Follow-Up Studies HIV Infections/*drug therapy/immunology/physiopathology/virology HIV Protease Inhibitors/*therapeutic use Human Indinavir/*therapeutic use Lamivudine/*therapeutic use Male Middle Aged Prospective Studies Reverse Transcriptase Inhibitors/*therapeutic use Stavudine/*therapeutic use Support, Non-U.S. Gov't Treatment Outcome Zidovudine/*therapeutic use},
	Note = {0269-9370 Journal Article},
	Number = {7},
	Pages = {745-50},
	Title = {Discrepant responses to triple combination antiretroviral therapy in advanced HIV disease},
	Volume = {12},
	Year = {1998}}

@article{Pikettyetal01,
	Abstract = {Within a prospective cohort of 150 human immunodeficiency virus (HIV)-infected patients who began first-line protease inhibitor therapy in 1996, the outcome of 42 patients with discrepant virologic and immunologic responses to antiretroviral treatment at 12 months was analyzed at 30 months of treatment. The incidence of AIDS-defining events and deaths (14%) in the group of patients with immunologic responses in the absence of a virologic response was higher than that in full-responder patients (2%); yet, the incidence in this group was lower than that in patients with no immunologic response, despite a virologic response (21%), and was lower than that in patients without an immunologic or virologic response (67%; P<.0001, log-rank test). Differences in outcome were significant (relative risk, 6.9; 95% confidence interval, 1.9-39.3) when factors for progression were compared with those of responder patients. The results support the relevance of the CD4 cell marker over plasma HIV load for predicting clinical outcome in patients who do not achieve full immunologic and virologic responses.},
	Author = {Piketty, C. and Weiss, L. and Thomas, F. and Mohamed, A. S. and Belec, L. and Kazatchkine, M. D.},
	Journal = {J Infect Dis},
	Keywords = {Adult Aged Antiretroviral Therapy, Highly Active CD4 Lymphocyte Count Cohort Studies Disease Progression Female HIV Infections/*drug therapy/immunology/virology HIV Protease Inhibitors/*therapeutic use Human Incidence Longitudinal Studies Male Middle Aged Mortality Prospective Studies RNA, Viral/blood Time Factors Treatment Outcome Viral Load},
	Note = {0022-1899 Journal Article},
	Number = {9},
	Pages = {1328-35},
	Title = {Long-term clinical outcome of human immunodeficiency virus-infected patients with discordant immunologic and virologic responses to a protease inhibitor-containing regimen},
	Volume = {183},
	Year = {2001}}

@article{Pilonetal02,
	Abstract = {Inhibition of human immunodeficiency virus type 1 reverse transcriptase (RT) by both nucleoside and nonnucleoside RT inhibitors profoundly inhibits virus replication. Nucleoside RT inhibitors are known to be toxic, but there is little information regarding the toxicities of nonnucleoside RT inhibitors (NNRTI). We demonstrate that efavirenz (an NNRTI) induces caspase- and mitochondrion-dependent apoptosis of Jurkat T cells and human peripheral blood mononuclear cells. The clinical relevance of these observations is not yet clear.},
	Author = {Pilon, A. A. and Lum, J. J. and Sanchez-Dardon, J. and Phenix, B. N. and Douglas, R. and Badley, A. D.},
	Journal = {Antimicrob Agents Chemother},
	Keywords = {Annexin V/diagnostic use Apoptosis/*drug effects Caspases/physiology Enzyme Inhibitors/diagnostic use Fluorescein-5-isothiocyanate Fluorescent Dyes HIV-1 Reverse Transcriptase/*antagonists & inhibitors Human Jurkat Cells Membrane Potentials/drug effects Mitochondria/drug effects/physiology Oxazines/*pharmacology Reverse Transcriptase Inhibitors/*pharmacology Support, Non-U.S. Gov't},
	Note = {0066-4804 Journal Article},
	Number = {8},
	Pages = {2687-91},
	Title = {Induction of apoptosis by a nonnucleoside human immunodeficiency virus type 1 reverse transcriptase inhibitor},
	Volume = {46},
	Year = {2002}}

@article{Priceetal03,
	Abstract = {Many individuals chronically infected with human immunodeficiency virus type 1 (HIV-1) experience a recrudescence of plasma virus during continuous combination antiretroviral therapy (ART) due either to the emergence of drug-resistant viruses or to poor compliance. In most cases, virologic failure on ART is associated with a coincident decline in CD4(+) T lymphocyte levels. However, a proportion of discordant individuals retain a stable or even increasing CD4(+) T lymphocyte count despite virological failure. In order to address the nature of these different outcomes, we evaluated virologic and immunologic variables in a prospective, single-blinded, nonrandomized cohort of 53 subjects with chronic HIV-1 infection who had been treated with continuous ART and monitored intensively over a period of 19 months. In all individuals with detectable viremia on ART, multiple drug resistance mutations with similar impacts on viral growth kinetics were detected in the pol gene of circulating plasma virus. Further, C2V3 env gene analysis demonstrated sequences indicative of CCR5 coreceptor usage in the majority of those with detectable plasma viremia. In contrast to this homogeneous virologic pattern, comprehensive screening with a range of antigens derived from HIV-1 revealed substantial immunologic differences. Discordant subjects with stable CD4(+) T lymphocyte counts in the presence of recrudescent virus demonstrated potent virus-specific CD4(+) and CD8(+) T lymphocyte responses. In contrast, subjects with virologic failure associated with declining CD4(+) T lymphocyte counts had substantially weaker HIV-specific CD4(+) T lymphocyte responses and exhibited a trend towards weaker HIV-specific CD8(+) T lymphocyte responses. Importantly the CD4(+) response was sustained over periods as long as 11 months, confirming the stability of the phenomenon. These correlative data lead to the testable hypothesis that the consequences of viral recrudescence during continuous ART are modulated by the HIV-specific cellular immune response.},
	Author = {Price, D. A. and Scullard, G. and Oxenius, A. and Braganza, R. and Beddows, S. A. and Kazmi, S. and Clarke, J. R. and Johnson, G. E. and Weber, J. N. and Phillips, R. E.},
	Journal = {J Virol},
	Keywords = {Adult Amino Acid Sequence Anti-HIV Agents/pharmacology/*therapeutic use CD4-Positive T-Lymphocytes/*immunology CD8-Positive T-Lymphocytes/*immunology Chronic Disease Drug Resistance, Viral/genetics Drug Therapy, Combination HIV Envelope Protein gp120/chemistry/genetics HIV Infections/*drug therapy/immunology/physiopathology HIV-1/*drug effects/genetics/physiology Human Lymphocyte Count Middle Aged Molecular Sequence Data Mutation Peptide Fragments/chemistry/genetics Prospective Studies RNA, Viral/blood Single-Blind Method Support, Non-U.S. Gov't *Treatment Failure Viral Load},
	Note = {0022-538x Clinical Trial Journal Article},
	Number = {10},
	Pages = {6041-9},
	Title = {Discordant outcomes following failure of antiretroviral therapy are associated with substantial differences in human immunodeficiency virus-specific cellular immunity},
	Volume = {77},
	Year = {2003}}

@article{Quinonesetal00,
	Abstract = {This study was designed to examine the impact of human immunodeficiency virus type 1 (HIV-1) fitness on disease progression through the use of a dual competition/heteroduplex tracking assay (HTA). Despite numerous studies on the impact of HIV-1 diversity and HIV-specific immune response on disease progression, we still do not have a firm understanding of the long-term pathogenesis of this virus. Strong and early CD8-positive cytotoxic T-cell and CD4-positive T-helper cell responses directed toward HIV-infected cells appear to curb HIV pathogenesis. However, the rate at which the virus infects the CD4(+) T-cell population and possibly destroys the HIV-specific immune response may also alter the rate of disease progression. For HIV-1 fitness studies, we established conditions for dual HIV-1 infections of peripheral blood mononuclear cells (PBMC) and a sensitive HTA to measure relative virus production. A pairwise comparison was then performed to estimate the relative fitness of various non-syncytium-inducing/CCR5-tropic (NSI/R5) and syncytium-inducing/CXCR4-tropic (SI/X4) HIV-1 isolates. Four HIV-1 strains (two NSI/R5 and two SI/X4) with moderate ex vivo fitness were then selected as controls and competed against primary HIV-1 isolates from an HIV-infected Belgian cohort. HIV-1 isolates from long-term survivors (LTS) were outcompeted by control strains and were significantly less fit than HIV-1 isolates from patients with accelerated progression to AIDS (PRO). In addition, NSI/R5 HIV-1 isolates from PRO overgrew control SI/X4 strains, suggesting that not all SI/X4 HIV-1 isolates replicate more efficiently than all NSI/R5 isolates. Finally, there were strong, independent correlations between viral load and the total relative fitness values of HIV-1 isolates from PRO (r = 0.84, P = 0.033) and LTS (r = 0.86, P = 0.028). Separation of the PRO and LTS plots suggest that HIV-1 fitness together with viral load may be a strong predictor for the rate of disease progression.},
	Author = {Quinones-Mateu, M. E. and Ball, S. C. and Marozsan, A. J. and Torre, V. S. and Albright, J. L. and Vanham, G. and van Der Groen, G. and Colebunders, R. L. and Arts, E. J.},
	Journal = {J Virol},
	Keywords = {*Biological Assay HIV Infections/*physiopathology/*virology *HIV-1/physiology Human Predictive Value of Tests Prognosis Support, Non-U.S. Gov't Support, U.S. Gov't, P.H.S.},
	Note = {0022-538x Journal Article},
	Number = {19},
	Pages = {9222-33},
	Title = {A dual infection/competition assay shows a correlation between ex vivo human immunodeficiency virus type 1 fitness and disease progression},
	Volume = {74},
	Year = {2000}}

@article{Racinanetal02,
	Abstract = {OBJECTIVE: To study whether hepatitis C virus (HCV) co-infection or the severe elevation of transaminases is associated with survival after the initiation of antiretroviral combination therapy. DESIGN: Prospective hospital-based cohort (Aquitaine Cohort). METHODS: HIV-infected adults started on an antiretroviral combination before 30 June 1999. HCV infection was defined as antibody detection or positive HCV RNA. Severe elevation of transaminases was defined as a value of aspartate or alanine aminotransferase (AST, ALT) above five times the upper limit of normal values. Survival was studied using a Cox model, including at least baseline HCV status and transaminases as a time-dependent covariate. RESULTS: Overall, 995 patients were analysed, including 576 HCV-positive individuals (58%). At baseline, HCV-positive patients were younger, more often injecting drug users and women, and had more frequently elevated transaminases. A shorter survival was associated with AIDS stage [hazard ratio (HR) versus non-AIDS 1.67; 95% confidence interval (CI) 1.03; 2.68], lower CD4 cell count (HR for 50 cells/mm3 lower 1.33; CI 1.17; 1.51), lower haemoglobin (HR for 1 g/dl lower 1.20; CI 1.07; 1.35), lower platelet count (HR for 10 000 cells/mm3 lower 1.04; CI 1.01; 1.07), and AST during follow-up (HR for > or = 200 IU/l 2.30; CI 1.32; 4.03). HCV co-infection (HR 1.20; CI 0.75; 1.92) was not statistically associated with survival. CONCLUSION: The occurrence of a severe elevation of transaminases was associated with poorer survival, although HCV was not. If liver toxicity may be treatment induced, plasma drug concentrations could guide dosage adjustments of antiretroviral treatments currently prescribed to optimize their use.},
	Author = {Rancinan, C. and Neau, D. and Saves, M. and Lawson-Ayayi, S. and Bonnet, F. and Mercie, P. and Dupon, M. and Couzigou, P. and Dabis, F. and Chene, G.},
	Journal = {Aids},
	Keywords = {Acquired Immunodeficiency Syndrome/complications Age Factors Anti-HIV Agents/*therapeutic use Antiretroviral Therapy, Highly Active Cohort Studies Comparative Study Disease Progression Female Follow-Up Studies HIV Infections/blood/*complications/*drug therapy Hepatitis C/blood/*complications Human Male Proportional Hazards Models Substance Abuse, Intravenous Support, Non-U.S. Gov't Survival Analysis Transaminases/blood},
	Note = {0269-9370 Journal Article},
	Number = {10},
	Pages = {1357-62},
	Title = {Is hepatitis C virus co-infection associated with survival in HIV-infected patients treated by combination antiretroviral therapy?},
	Volume = {16},
	Year = {2002}}

@article{Rogeretal99,
	Abstract = {HAART may increase CD4+ T cell counts despite a persistently detectable HIV load. The impact of HAART on apoptosis, which may play a role in the disease process in HIV-infected patients, has not been extensively studied. We performed a study to compare the level of spontaneous T cell apoptosis and anti-retroviral treatments in a cohort of HIV-1-infected patients. Data were obtained from a computerized medical record. Quantification of apoptotic cells was by cytofluorometric technique. From November 1995 to December 1997 we studied T cell apoptosis in 112 HIV-infected patients. Forty patients were classified A, 36 B and 36 C. Thirty patients were naive and 82 received an anti-retroviral treatment, 49 including a protease inhibitor (PI). The median plasma viraemia determined in 63 patients was 3.6 (range 1.3-5.6) log10. The median apoptotic cell count was 22% (range 2-73%) and 12% (range 2-60%) for CD4+ and CD8+ T cells, respectively. We did not observe any correlation between the HIV viraemia and the level of apoptosis of T cell subsets. Patients with HAART showed a lower percentage of apoptotic CD4+ T cells only: 16% (range 2-61%) versus 25% (range 5-73%) for patients receiving two nucleoside analogues (P = 0.02). This effect was significant in stage A patients and remained observable during the whole course of HIV disease. In conclusion, HAART, without any relation to plasma viraemia, is able to reduce apoptosis of CD4+ T cells.},
	Author = {Roger, P. M. and Breittmayer, J. P. and Arlotto, C. and Pugliese, P. and Pradier, C. and Bernard-Pomier, G. and Dellamonica, P. and Bernard, A.},
	Journal = {Clin Exp Immunol},
	Keywords = {Adult Aged Anti-HIV Agents/*therapeutic use *Apoptosis CD4-Positive T-Lymphocytes/cytology/*drug effects CD8-Positive T-Lymphocytes/drug effects Didanosine/therapeutic use Drug Therapy, Combination Female HIV Infections/*drug therapy/immunology/pathology HIV Protease Inhibitors/therapeutic use Human Lamivudine/therapeutic use Male Middle Aged Multivariate Analysis Retrospective Studies Stavudine/therapeutic use Viral Load Zalcitabine/therapeutic use Zidovudine/therapeutic use},
	Note = {0009-9104 Journal Article},
	Number = {3},
	Pages = {412-6},
	Title = {Highly active anti-retroviral therapy (HAART) is associated with a lower level of CD4+ T cell apoptosis in HIV-infected patients},
	Volume = {118},
	Year = {1999}}

@article{Stoddaretalt01,
	Abstract = {Many HIV-1-infected patients treated with protease inhibitors (PI) develop PI-resistant HIV-1 variants and rebounds in viremia, but their CD4+ T-cell counts often do not fall. We hypothesized that in these patients, T-cell counts remain elevated because PI-resistant virus spares intrathymic T-cell production. To test this, we studied recombinant HIV-1 clones containing wild-type or PI-resistant protease domains, as well as uncloned isolates from patients, in activated peripheral blood mononuclear cells, human thymic organ cultures and human thymus implants in SCID-hu Thy/Liv mice. In most cases, wild-type and PI-resistant HIV-1 isolates replicated to similar degrees in peripheral blood mononuclear cells. However, the replication of PI-resistant but not wild-type HIV-1 isolates was highly impaired in thymocytes. In addition, patients who had PI-resistant HIV-1 had abundant thymus tissue as assessed by computed tomography. We propose that the inability of PI-resistant HIV-1 to replicate efficiently in thymus contributes to the preservation of CD4+ T-cell counts in patients showing virologic rebound on PI therapy.},
	Author = {Stoddart, C. A. and Liegler, T. J. and Mammano, F. and Linquist-Stepps, V. D. and Hayden, M. S. and Deeks, S. G. and Grant, R. M. and Clavel, F. and McCune, J. M.},
	Journal = {Nat Med},
	Keywords = {Adult Animals CD4 Lymphocyte Count Drug Resistance, Microbial Fetal Tissue Transplantation Flow Cytometry HIV Core Protein p24/metabolism HIV Infections/immunology/pathology/*virology HIV Protease/genetics/*metabolism HIV Protease Inhibitors/*pharmacology HIV-1/*drug effects/enzymology/genetics/*physiology Human Mice Mice, SCID Middle Aged Organ Culture Recombination, Genetic Support, Non-U.S. Gov't Support, U.S. Gov't, P.H.S. T-Lymphocytes/*physiology/virology Thymus Gland/pathology/physiopathology/transplantation/*virology Viral Load *Virus Replication},
	Note = {1078-8956 Journal Article},
	Number = {6},
	Pages = {712-8},
	Title = {Impaired replication of protease inhibitor-resistant HIV-1 in human thymus},
	Volume = {7},
	Year = {2001}}

@article{Sufkaetal03,
	Abstract = {Mechanisms that underly discordant CD4+ cell/virus load (VL) responses in patients who receive highly active antiretroviral therapy (HAART) were studied in 30 human immunodeficiency virus (HIV)-positive patients, in 3 groups. Discordant responders maintained CD4+ cell levels >200/mm(3) with stable or increasing trend, despite sustained VLs of 500-5000 copies/mL, for >2 years. Treatment-success patients had CD4+ cell counts >200/mm(3) with stable or increasing trend and VLs <50 copies/mL, for >2 years. Treatment-failure patients initially responded to HAART, followed by decreasing CD4+ cell counts and increasing VLs. Interferon-gamma production to gag and noncytolytic CD8+ cell suppressive activity were greater in discordant responders. Cellular activation was greatest in patients with treatment failure. All discordant responders had non-syncytium-inducing (CCR5-tropic) viruses. Viruses from discordant responders and from patients with treatment failure had extensive resistance mutations; discordant responders had significantly lower viral replication capacities. These findings suggest that discordant responses may be related to enhanced HIV-directed immune responses, diminished cellular activation, decreased viral replication capacity, and preservation of non-syncytium-inducing virus strains.},
	Author = {Sufka, S. A. and Ferrari, G. and Gryszowka, V. E. and Wrin, T. and Fiscus, S. A. and Tomaras, G. D. and Staats, H. F. and Patel, D. D. and Sempowski, G. D. and Hellmann, N. S. and Weinhold, K. J. and Hicks, C. B.},
	Journal = {J Infect Dis},
	Keywords = {Adult *Antiretroviral Therapy, Highly Active *CD4 Lymphocyte Count Female HIV/*drug effects HIV Infections/*drug therapy/*immunology/virology HIV Protease Inhibitors/*pharmacology/therapeutic use Human Male Middle Aged Support, Non-U.S. Gov't Support, U.S. Gov't, P.H.S. Time Factors Treatment Failure *Viral Load Virus Replication/drug effects},
	Note = {0022-1899 Clinical Trial Journal Article},
	Number = {7},
	Pages = {1027-37},
	Title = {Prolonged CD4+ cell/virus load discordance during treatment with protease inhibitor-based highly active antiretroviral therapy: immune response and viral control},
	Volume = {187},
	Year = {2003}}

@article{Tebaldietal03,
	Abstract = {To ascertain the impact of hepatitis C virus (HCV) infection on human immunodeficiency virus (HIV) disease progression and associated death in the era of highly active antiretroviral therapy (HAART), we examined mortality rates, the presence of other diseases, and antiretroviral use in an observational cohort of 823 HIV-infected patients with and without HCV coinfection during the period of January 1996 through June 2001. Analyses were used to compare patient characteristics, comorbid conditions, and survival durations in HIV-infected and HIV-HCV-coinfected patients. HIV-HCV-coinfected persons did not have a statistically greater rate of acquired immunodeficiency syndrome or of renal or cardiovascular disease, but they did have more cases of cirrhosis and transaminase elevations. There were proportionately more deaths in the HIV-HCV-coinfected group. Age, baseline CD4+ cell count, and duration of HAART were significantly associated with survival, but HCV infection was not. HAART use was a strong predictor of increased duration of survival, suggesting that treatment is more important to survival than is HCV coinfection status.},
	Author = {Tedaldi, E. M. and Baker, R. K. and Moorman, A. C. and Alzola, C. F. and Furhrer, J. and McCabe, R. E. and Wood, K. C. and Holmberg, S. D.},
	Journal = {Clin Infect Dis},
	Keywords = {Anti-HIV Agents/therapeutic use *Antiretroviral Therapy, Highly Active *Hiv HIV Infections/*complications/drug therapy/epidemiology/mortality *Hepacivirus Hepatitis C/*complications/epidemiology/mortality Human Morbidity Mortality Support, U.S. Gov't, P.H.S.},
	Note = {1537-6591 Journal Article},
	Number = {3},
	Pages = {363-7},
	Title = {Influence of coinfection with hepatitis C virus on morbidity and mortality due to human immunodeficiency virus infection in the era of highly active antiretroviral therapy},
	Volume = {36},
	Year = {2003}}

@article{Wang&Bembom&vanderLaan06,
	Author = {Y. Wang and O. Bembom and M.J. van der Laan},
	Journal = {Journal of Statistical Planning and Inference},
	Optnote = {also http://www.bepress.com/ucbbiostat/paper159},
	Title = {Data adaptive estimation of the treatment specific mean},
	Year = {2006}}

@article{Sinisi&vanderLaan04,
	Author = {S. Sinisi and M.J. van der Laan},
	Journal = {Journal of Statistical Methods in Molecular Biology},
	Number = {1},
	Optnote = {http://www.bepress.com/sagmb/vol3/iss1/art18},
	Title = {The deletion/substitution/addition algorithm in loss function based estimation: Applications in Genomics},
	Volume = {3},
	Year = {2004}}

@techreport{Petersenetal05,
	Author = {M. L. Petersen and S.G. Deeks and J. N. Martin and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Month = {December},
	Optnote = {http://www.bepress.com/ucbbiostat/paper199},
	Title = {History-Adjusted Marginal Structural Models: Time-Varying Effect Modification and Dynamic Treatment Regimens},
	Type = {Technical Report 199},
	Year = {2005}}

@techreport{vanderLaan&Rubin05,
	Author = {M.J. van der Laan and D. Rubin},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper180},
	Title = {Estimating Function Based Cross-Validation and Learning},
	Type = {Technical Report 180},
	Year = {2005}}

@article{vanderLaan&Petersen07,
	Author = {M.J. van der Laan and M.L. Petersen},
	Journal = {International Journal of Biostatistics},
	Number = {1},
	Optnote = {http://www.bepress.com/ijb/vol3/iss1/art3},
	Title = {Causal Effect Models for Realistic Individualized Treatment and Intention to Treat Rules},
	Volume = {3},
	Year = {2007}}

@techreport{vanderLaan06,
	Author = {M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper203},
	Title = {Causal Effect Models for Intention to Treat and Realistic Individualized Treatment Rules},
	Type = {Technical Report 203},
	Year = {2006}}

@techreport{vanderLaan08b,
	Author = {M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Month = {March},
	Optnote = {http://www.bepress.com/ucbbiostat/paper232},
	Title = {The construction and analysis of adaptive group sequential designs},
	Type = {Technical Report 232},
	Year = {2008}}

@techreport{Moore&vanderLaan07,
	Author = {K.L. Moore and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Month = {April},
	Optnote = {http://www.bepress.com/ucbbiostat/paper215},
	Title = {Covariate adjustment in randomized trials with binary outcomes},
	Type = {Technical Report 215},
	Year = {2007}}

@techreport{vanderLaan&Petersen05,
	Author = {M.J. van der Laan and M.L. Petersen},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper187},
	Title = {Direct Effect Models},
	Type = {Technical Report 187},
	Year = {2005}}

@techreport{Petersen&vanderLaan06,
	Author = {M.L. Petersen and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Title = {Individualized Treatment Rules and Clinical Trials},
	Type = {Technical Report},
	Year = {2006}}

@article{vanderLaan&Petersen&Joffe05,
	Author = {M.J. van der Laan and M.L. Petersen and M.M. Joffe},
	Journal = {The International Journal of Biostatistics},
	Number = {1},
	Optnote = {http://www.bepress.com/ijb/vol1/iss1/4},
	Pages = {10-20},
	Title = {History-Adjusted Marginal Structural Models and Statically-Optimal Dynamic Treatment Regimens},
	Volume = {1},
	Year = {2005}}

@article{vanderLaan06a,
	Author = {M.J. van der Laan},
	Journal = {International Journal of Biostatistics},
	Number = {1},
	Optnote = {http://www.bepress.com/ijb/vol2/iss1/art2},
	Title = {Statistical Inference for Variable Importance},
	Volume = {2},
	Year = {2006}}

@article{vanderLaan&Birkner&Hubbard05,
	Author = {M.J. van der Laan and M.D. Birkner and A.E. Hubbard},
	Journal = {Journal of Statistical Applications in Genetics and Molecular Biology},
	Number = {1},
	Optnote = {http://www.bepress.com/sagmb/vol4/iss1/art29},
	Title = {Empirical Bayes and resampling based multiple testing procedure controlling tail probability of the proportion of false positives},
	Volume = {4},
	Year = {2005}}

@article{vanderLaan&Dudoit&Pollard04b,
	Author = {M.J. van der Laan and S. Dudoit and K.S. Pollard},
	Journal = {Journal of Statistical Applications in Genetics and Molecular Biology},
	Number = {1},
	Optnote = {http://www.bepress.com/sagmb/vol3/iss1/art15},
	Title = {Augmentation procedures for control of the generalized family-wise error rate and tail probabilities for the proportion of false positives},
	Volume = {3},
	Year = {2004}}

@article{vanderLaan&Dudoit&Pollard04,
	Author = {S. Dudoit and M.J. van der Laan and K.S. Pollard},
	Journal = {Journal of Statistical Applications in Genetics and Molecular Biology},
	Number = {1},
	Optnote = {http://www.bepress.com/sagmb/vol3/iss1/art14},
	Title = {Multiple testing. Part II. Step-down procedures for control of the family-wise error rate},
	Volume = {3},
	Year = {2004}}

@article{Dudoit&vanderLaan&Pollard04,
	Author = {S. Dudoit and M.J. van der Laan and K.S. Pollard},
	Journal = {Journal of Statistical Applications in Genetics and Molecular Biology},
	Number = {1},
	Optnote = {http://www.bepress.com/sagmb/vol3/iss1/art13},
	Title = {Multiple testing. Part I. Single-step procedures for control of general Type I error rates},
	Volume = {3},
	Year = {2004}}

@article{Birkner&Sinisi&vanderLaan05,
	Author = {M.D. Birkner and S.E. Sinisi and M.J. van der Laan},
	Journal = {Journal of Statistical Applications in Genetics and Molecular Biology},
	Number = {1},
	Optnote = {http://www.bepress.com/sagmb/vol4/iss1/art8},
	Title = {Multiple Testing and Data Adaptive Regression: An Application to {HIV}-1 Sequence Data},
	Volume = {4},
	Year = {2005}}

@techreport{vanderLaan&Hubbard06,
	Author = {M.J. van der Laan and A.E. Hubbard},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper198},
	Title = {Quantile-Function Based Null Distribution in Resampling Based Multiple Testing},
	Type = {Technical Report},
	Year = {2006}}

@techreport{Molinaro&vanderLaan04,
	Author = {A. Molinaro and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper162},
	Title = {Deletion/Substitution/Addition Algorithm for Partitioning the Covariate Space in Prediction},
	Type = {Technical Report},
	Year = {2004}}

@techreport{Birkner&vanderLaan05,
	Author = {M.D. Birkner and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Title = {Application of a Variable Importance Measure Method to {HIV}-1 Sequence Data},
	Type = {Technical Report},
	Year = {2005}}

@article{Neugebauer2007419,
	Author = {Romain Neugebauer and Mark van der Laan},
	Doi = {DOI: 10.1016/j.jspi.2005.12.008},
	Issn = {0378-3758},
	Journal = {Journal of Statistical Planning and Inference},
	Number = {2},
	Pages = {419 - 434},
	Title = {Nonparametric causal effects based on marginal structural models},
	Url = {http://www.sciencedirect.com/science/article/pii/S0378375806000334},
	Volume = {137},
	Year = {2007},
	Bdsk-Url-1 = {http://www.sciencedirect.com/science/article/pii/S0378375806000334},
	Bdsk-Url-2 = {http://dx.doi.org/10.1016/j.jspi.2005.12.008}}

@techreport{Neugebauer&vanderLaan05b,
	Author = {R. Neugebauer and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {134},
	Optnote = {http://www.bepress.com/ucbbiostat/paper134, to appear in {JSPI}},
	Title = {Locally Efficient Estimation of Nonparametric Causal Effects on Mean Outcomes in Longitudinal Studies},
	Type = {Technical Report},
	Year = {2005}}

@techreport{Wang&Petersen&vanderLaan06,
	Author = {Y. Wang and M. Petersen and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Title = {A statistical method for diagnosing ETA bias in IPTW estimators},
	Type = {Technical Report},
	Year = {2006}}

@techreport{vanderLaan&Dudoit&vanderVaart,
	Author = {M.J. van der Laan and S. Dudoit and A.W. van der Vaart},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Month = {February},
	Optnote = {http://www.bepress.com/ucbbiostat/paper142},
	Title = {The Cross-Validated Adaptive Epsilon-Net Estimator},
	Type = {Technical Report 142},
	Year = {2004}}

@techreport{vanderLaan&Dudoit03,
	Author = {M.J. van der Laan and S. Dudoit},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Month = {November},
	Optnote = {http://www.bepress.com/ucbbiostat/paper130},
	Title = {Unified cross-validation methodology for selection among estimators and a general cross-validated adaptive epsilon-net estimator: Finite sample oracle inequalities and examples},
	Type = {Technical Report},
	Year = {2003}}

@techreport{Petersen&vanderLaan05,
	Author = {M. Petersen and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Title = {Estimation of direct and indirect causal effects in Epidemiology},
	Type = {Technical Report},
	Year = {2005}}

@techreport{vanderLaan&Petersen04,
	Author = {M.J. van der Laan and M. Petersen},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Month = {August},
	Title = {Estimation of direct and indirect causal effects in longitudinal studies},
	Type = {Technical Report 155},
	Year = {2004}}

@techreport{vanderLaan&Hubbard&Jewell04,
	Author = {M.J. van der Laan and A.E. Hubbard and N.P. Jewell},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Month = {September},
	Optnote = {http://www.bepress.com/ucbbiostat/paper157},
	Title = {Estimation of Treatment Effects in Randomized Trials with Noncompliance and a Dichotomous Outcome},
	Type = {Technical Report 157},
	Year = {2004}}

@techreport{Bein&Hubbard&vanderLaan05,
	Author = {E. Bein and A.E. Hubbard and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Title = {Estimating Function Based Cross-Validation in Estimation of the Causal Effect in Randomized Trials},
	Type = {Technical Report},
	Year = {2005}}

@techreport{Molinaroetal05,
	Author = {A.M. Molinaro and M.J. van der Laan and D.H. Moore and K. Kerlikowske},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Note = {http://www.bepress.com/ucbbiostat/paper149},
	Title = {Survival point estimate prediction in matched and non-matched case-control subsample designed studies},
	Year = {2005}}

@techreport{Dudoitetal04,
	Author = {S. Dudoit and M.J. van der Laan and S. Kele\c{s} and A. M. Molinaro and S. E. Sinisi and S.L. Teng},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Note = {to appear in \emph{SIGKDD} Explorations on Microarray Data Mining},
	Title = {Loss-Based Estimation with Cross-Validation: Applications to Microarray Data Analysis and Motif Finding.},
	Year = {2004}}

@book{Friedman&Furberg&Demets98,
	Author = {L.M.Friedman and C.D. Furberg and D.L. DeMets},
	Publisher = {Springer-Verlag New York},
	Title = {Fundamentals of Clinical Trials},
	Year = {1998}}

@book{Andersenetal93,
	Author = {P.K. Andersen and O. Borgan and R.D. Gill and N. Keiding},
	Publisher = {Springer-Verlag New York},
	Title = {Statistical Models Based on Counting Processes},
	Year = {1993}}

@article{Wittes&Brittain90,
	Author = {J. Wittes and E. Brittain},
	Journal = {Statistics in Medicine},
	Pages = {65--72},
	Title = {The role of internal pilot studies in increasing efficiency of clinical trials},
	Volume = {9},
	Year = {1999}}

@incollection{Robins03,
	Author = {J.M. Robins},
	Booktitle = {Highly Structured Stochastic Systems},
	Editor = {P. Green, N. Hjort, and S. Richardson},
	Pages = {70--81},
	Publisher = {Oxford University Press, Oxford},
	Title = {Semantics of causal DAG models and the identification of direct and indirect effects},
	Year = {2003}}

@techreport{Pearl01,
	Author = {J. Pearl},
	Institution = {University of California, Los Angeles, Department of Computer Science},
	Title = {Cognitive systems Laboratory},
	Year = {2001}}

@book{Pearl00,
	Author = {J. Pearl},
	Publisher = {Cambridge University Press, Cambridge},
	Title = {Causality: Models, Reasoning, and Inference},
	Year = {2000}}

@article{Robins&Greenland92,
	Author = {J.M. Robins and S. Greenland},
	Journal = {Epidemiology},
	Number = {0},
	Pages = {143--155},
	Title = {Identifiability and exchangeability for direct and indirect effects},
	Volume = {3},
	Year = {1992}}

@article{vanderLaan95,
	Author = {M.J. van der Laan},
	Journal = {Bernoulli},
	Number = {4},
	Pages = {335--341},
	Title = {Identity for NPMLE in missing data and biased sampling models},
	Volume = {1},
	Year = {1995}}

@article{vanderLaan98,
	Author = {M.J. van der Laan},
	Journal = {Lifetime Data Models},
	Number = {0},
	Pages = {83--102},
	Title = {Identity for NPMLE in Censored Data Models},
	Volume = {4},
	Year = {1998}}

@article{Klaassen86,
	Author = {C.A.J. Klaassen},
	Journal = {Annals of Statistics},
	Pages = {1548--1562},
	Title = {Consistent estimation of the influence function of locally asymptotically linear estimators},
	Volume = {15},
	Year = {1987}}

@article{Robins&Rotnitzky04,
	Author = {J.M. Robins and A. Rotnitzky},
	Journal = {Biometrika},
	Number = {0},
	Optnote = {To Appear},
	Pages = {0},
	Title = {Estimation of Treatment Effects in Randomized Trials with Noncompliance and a Dichotomous Outcome using Structural Nested Mean Models},
	Volume = {0},
	Year = {2004}}

@article{vanderVaart91,
	Author = {A.W. van der Vaart},
	Journal = {Annals of Statistics},
	Pages = {178--204},
	Title = {On differentiable functionals},
	Volume = {19},
	Year = {1991}}

@article{Rubin78,
	Author = {D.B. Rubin},
	Journal = {Annals of Statistics},
	Pages = {34--58},
	Title = {Bayesian Inference for causal effects: the role of randomization},
	Volume = {6},
	Year = {1978}}

@article{Neyman23,
	Author = {Neyman, J.},
	Journal = {Statistical Science},
	Optnote = {Translation of 1923 article},
	Pages = {465--480},
	Title = {On the application of probability theory to agricultural experiments},
	Volume = {5},
	Year = {1990}}

@article{Robins86,
	Author = {J.M. Robins},
	Journal = {Mathematical Modelling},
	Pages = {1393--1512},
	Title = {A new approach to causal inference in mortality studies with sustained exposure periods - Application to control of the healthy worker survivor effect},
	Volume = {7},
	Year = {1986}}

@article{Robins94,
	Author = {J.M. Robins},
	Journal = {Communications in Statistics},
	Pages = {2379--2412},
	Title = {Correcting for non-compliance in randomized trials using structural nested mean models},
	Volume = {23},
	Year = {1994}}

@article{Vansteelandt&Goetghebeur03,
	Author = {S. Vansteelandt and E. Goetghebeur},
	Journal = {Journal of the Royal Statistical Society, Series B},
	Optnote = {In print},
	Title = {Causal inference with generalized structural mean models},
	Volume = {23},
	Year = {2003}}

@incollection{Robins97a,
	Address = {Chichester, UK},
	Author = {Robins, J.M.},
	Booktitle = {The Encyclopedia of Biostatistics},
	Editor = {Armitage, P. and Colton, T. and Andersen, P.K. and Keiding, N.},
	Publisher = {John Wiley and Sons},
	Title = {Structural Nested Failure Time Models},
	Year = {1997}}

@article{Hernan&Brumback&Robins,
	Author = {Hernan, M. A. and Brumback, B. and Robins, J. M.},
	Journal = {Epidemiology},
	Number = {5},
	Pages = {561--570},
	Title = {Marginal structural models to estimate the causal effect of zidovudine on the survival of {HIV}-positive men},
	Volume = {11},
	Year = {2000}}

@article{Robins87,
	Author = {Robins, J.M.},
	Coden = {CMAPDK},
	Fjournal = {Computers \& Mathematics with Applications. An International Journal},
	Issn = {0097-4943},
	Journal = {Comput. Math. Appl.},
	Number = {9-12},
	Pages = {923--945},
	Title = {Addendum to: ``{A} new approach to causal inference in mortality studies with a sustained exposure period---application to control of the healthy worker survivor effect'' [{M}ath.\ {M}odelling {\bf 7} (1986), no.\ 9-12, 1393--1512; {M}{R} 87m:92078]},
	Volume = {14},
	Year = {1987}}

@article{Robins&Hernan&Brumback00,
	Author = {Robins, J. M. and Hernan, M. A. and Brumback, B.},
	Journal = {Epidemiology},
	Number = {5},
	Pages = {550--560},
	Title = {Marginal structural models and causal inference in epidemiology},
	Volume = {11},
	Year = {2000}}

@article{Bryan&Yu&vanderLaan03,
	Author = {Bryan, J. and Yu, Z. and van der Laan, M.J.},
	Journal = {Biostatistics},
	Number = {3},
	Pages = {361--380},
	Title = {Analysis of Longitudinal Marginal Structural Models},
	Volume = {5},
	Year = {2003}}

@techreport{Yu&vanderLaan03b,
	Author = {Yu, Z. and van der Laan, M.J.},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper132},
	Optnumber = {132},
	Title = {Double Robust Estimation in Longitudinal Marginal Structural Models},
	Year = {2003}}

@article{Neugebauer&vanderLaan05,
	Author = {Neugebauer, R. and van der Laan, M.J.},
	Journal = {Journal of Statistical Planning and Inference},
	Number = {1-2},
	Pages = {405--26},
	Title = {Why prefer double robust estimates},
	Volume = {129},
	Year = {2005}}

@article{Murphy03,
	Author = {Murphy, S.A.},
	Journal = {Journal of the Royal Statistical Society: Series B},
	Number = {2},
	Pages = {331-66},
	Title = {Optimal dynamic treatment regimes},
	Volume = {65},
	Year = {2003}}

@article{Robins03a,
	Author = {Robins, J.M.},
	Journal = {Journal of the Royal Statistical Society: Series B},
	Number = {2},
	Pages = {355--66},
	Title = {Discussion of ``Optimal dynamic treatment regimes" by Susan A. Murphy},
	Volume = {65},
	Year = {2003}}

@article{Murphy&vanderLaan&Robins01,
	Author = {S.A. Murphy and M.J. van der Laan and J.M. Robins},
	Journal = {Journal of the American Statistical Association},
	Pages = {1410--1424},
	Title = {Marginal mean models for dynamic treatment regimens},
	Volume = {96},
	Year = {2001}}

@incollection{Robins98,
	Address = {New York},
	Author = {Robins, J.M.},
	Booktitle = {Statistical models in epidemiology, the environment, and clinical trials (Minneapolis, MN, 1997)},
	Mrclass = {62N01 (62G08 62P10)},
	Mrnumber = {2001a:62124},
	Pages = {95--133},
	Publisher = {Springer},
	Title = {Marginal structural models versus structural nested models as tools for causal inference},
	Year = {2000}}

@incollection{Robins97,
	Author = {J.M. Robins},
	Booktitle = {Latent Variable Modeling and Applications to Causality},
	Editor = {M. Berkane, Editor},
	Optseries = {Lecture Notes in Statistics},
	Optvolume = {120},
	Pages = {69--117},
	Publisher = {Springer Verlag, New York},
	Title = {Causal Inference from Complex Longitudinal Data},
	Year = {1997}}

@incollection{Robins89,
	Address = {Washington D.C.},
	Author = {J.M. Robins},
	Booktitle = {Health Service Methodology: A Focus on AIDS},
	Editor = {L. Sechrest and H. Freeman and A. Mulley},
	Optseries = {Lecture Notes in Statistics},
	Pages = {113--159},
	Publisher = {U.S. Public Health Service, National Center for Health SErvices Research},
	Title = {The analysis of randomized and non-randomized AIDS treatment trials using a new approach in causal inference in longitudinal studies},
	Year = {1989}}

@techreport{Abadie00,
	Author = {A. Abadie},
	Institution = {NBER Technical Working Paper},
	Optnumber = {260},
	Title = {Semiparametric estimation of instrumental variables models for causal effects},
	Year = {2000}}

@article{Abadie03,
	Author = {A. Abadie},
	Journal = {Journal of Econometrics},
	Pages = {231-263},
	Title = {Semiparametric instrumental variable estimation of treatment response models},
	Volume = {113},
	Year = {2003}}

@article{Abadie03,
	Author = {A. Abadie},
	Journal = {Journal of Econometrics},
	Pages = {231-263},
	Title = {Semiparametric instrumental variable estimation of treatment response models},
	Volume = {113},
	Year = {2003}}

@techreport{Wang&Vanderlaan04,
	Author = {Y. Wang and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper159},
	Optnumber = {159},
	Title = {Data adaptive estimation of the treatment specific mean},
	Year = {2004}}

@techreport{Yu&Vanderlaan02,
	Author = {Z. Yu and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper122},
	Optnumber = {122},
	Title = {Construction of counterfactuals and the {G}-computation formula},
	Year = {2002}}

@techreport{Yu&Vanderlaan03,
	Author = {Z. Yu and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper136},
	Optnumber = {136},
	Title = {Measuring treatment effects using semiparametric models},
	Year = {2003}}

@article{Angristetal&Imbens&Rubin96,
	Author = {J. Angrist and G. Imbens and D.B. Rubin},
	Journal = {Journal of the American Statistical Association},
	Pages = {444-555},
	Title = {Identification of causal effects using instrumental variables},
	Volume = {91},
	Year = {1996}}

@article{Robins&Rotnitzky01A,
	Author = {J.M Robins and A. Rotnitzky},
	Journal = {Statistica Sinica},
	Pages = {920-935},
	Title = {Comment on {I}nference for semiparametric models: some questions and an answer, by {B}ickel, {P}.{J}. and {K}won, {J}.},
	Volume = {11},
	Year = {2001}}

@article{Angrist01,
	Author = {J. Angrist},
	Journal = {Journal of Business and Economics Statistics},
	Pages = {1--16},
	Title = {Estimation of limited dependent variable models with dummy endogenous regressors: simple strategies for empirical practice},
	Volume = {19},
	Year = {2001}}

@article{Chamberlain87,
	Author = {G. Chamberlain},
	Journal = {Journal of Econometrics},
	Pages = {305--334},
	Title = {Asymptotic efficiency in estimation with conditional moment restrictions},
	Volume = {34},
	Year = {1987}}

@article{Hiranoetal00,
	Author = {K. Hirano and G. Imbens and D.B. Rubin and X-H. Zhou},
	Journal = {Biostatistics},
	Pages = {69--88},
	Title = {Assessing the effects of influenza vaccine in an encouragement design},
	Volume = {1},
	Year = {2000}}

@article{Neyman23,
	Author = {J. Neyman},
	Journal = {Statistical Science},
	Pages = {463--472},
	Title = {Sur les applications de la thar des probabilites aux experiences Agaricales: Essay des principle (1923). Excerpts reprinted (1990) in English (D. Dabrowska and T. Speed), Trans.},
	Volume = {5},
	Year = {1990}}

@inproceedings{Robins05,
	Author = {J.M. Robins},
	Booktitle = {Proceedings of the 2nd Seattle symposium in biostatistics},
	Editor = {Lin, D.Y, Heagerty P.J},
	Optpublisher = {Springer Verlag Lecture Notes in Statistics},
	Pages = {189--326},
	Title = {Optimal structural nested models for optimal sequential decisions},
	Volume = {179},
	Year = {2005}}

@techreport{Robins05b,
	Author = {J.M. Robins},
	Institution = {Department of Biostatistics, Havard University},
	Title = {Optimal structural nested models for optimal sequential decisions},
	Year = {2005}}

@inproceedings{Akaike73,
	Author = {H. Akaike},
	Booktitle = {Second International Symposium on Information Theory},
	Editor = {B.N. Petrov and F. Csaki},
	Organization = {Budapest: Academiai Kiado},
	Pages = {267-281},
	Title = {Information theory and an extension of the maximum likelihood principle},
	Year = {1973}}

@article{Balke&Pearl97,
	Author = {A. Balke and J. Pearl},
	Journal = {Journal of the American Statistical Association},
	Pages = {1172--1176},
	Title = {Bound on treatment effects from studies with imperfect compliance},
	Volume = {92},
	Year = {1997}}

@inproceedings{Balke&Pearl94,
	Author = {A. Balke and J. Pearl},
	Booktitle = {In Proceedings of the 12th National Conference on Artificial Intelligence},
	Optaddress = {Menlo Park, CA},
	Optpublisher = {MIT Press},
	Pages = {230--237},
	Title = {Counterfactual probabilities: Computational methods, bounds, and applications},
	Volume = {I},
	Year = {1994}}

@article{Ambroise&McLachlan02,
	Author = {C. Ambroise and G. J. McLachlan},
	Journal = PNAS,
	Number = {10},
	Pages = {6562--6566},
	Title = {Selection bias in gene extraction on the basis of microarray gene-expression data},
	Volume = {99},
	Year = {2002}}

@incollection{Arabie&Hubert96,
	Address = {River Edge, NJ},
	Author = {P. Arabie and L. J. Hubert},
	Booktitle = {Clustering and Classification},
	Editor = {P. Arabie and L. J. Hubert and G. De Soete},
	Pages = {5--63},
	Publisher = {World Scientific Publishing Co.},
	Title = {An overview of combinatorial data analysis},
	Year = {1996}}

@article{Schwartz78,
	Author = {G. Schwartz},
	Journal = {Annals of Statistics},
	Pages = {461-464},
	Title = {Estimating the Dimension of a Model},
	Volume = {6},
	Year = {1978}}

@article{Barnard35,
	Author = {M. Barnard},
	Journal = {Annals of Eugenics},
	Pages = {352--371},
	Title = {The secular variations of skull characters in four series of Egyptian skulls},
	Volume = {6},
	Year = {1935}}

@inproceedings{BenHur&Elisseeff&Guyon02,
	Author = {A. Ben-Hur and A. Elisseeff and I. Guyon},
	Booktitle = {Pacific Symposium on Biocomputing},
	Pages = {6--17},
	Title = {A stability based method for discovering structure in clustered data},
	Volume = {7},
	Year = {2002}}

@article{Benjamini&Hochberg95,
	Author = {Y. Benjamini and Y. Hochberg},
	Journal = {J. R. Statist. Soc. B},
	Pages = {289--300},
	Title = {Controlling the false discovery rate: a practical and powerful approach to multiple testing},
	Volume = {57},
	Year = {1995}}

@article{Benjamini&Yekutieli01,
	Author = {Y. Benjamini and D. Yekutieli},
	Journal = {Annals of Statistics},
	Number = {4},
	Pages = {1165--1188},
	Title = {The control of the false discovery rate in multiple testing under dependency},
	Volume = {29},
	Year = {2001}}

@article{Beran88,
	Author = {R. Beran},
	Journal = JASA,
	Pages = {679--686},
	Title = {Balanced simultaneous confidence sets},
	Volume = {83},
	Year = {1988}}

@article{Bock85,
	Author = {H-H Bock},
	Journal = {Journal of Classification},
	Pages = {77--108},
	Title = {On some significance tests in cluster analysis},
	Volume = {2},
	Year = {1985}}

@incollection{Bock96,
	Address = {River Edge, NJ},
	Author = {H-H Bock},
	Booktitle = {Clustering and Classification},
	Editor = {P. Arabie and L. J. Hubert and G. De Soete},
	Pages = {377--453},
	Publisher = {World Scientific Publishing Co.},
	Title = {Probability models and hypotheses testing in partitioning cluster analysis},
	Year = {1996}}

@article{Boldricketal02,
	Author = {J. C. Boldrick and A. A. Alizadeh and M. Diehn and S. Dudoit and C. L. Liu and C. E. Belcher and D. Botstein and L. M. Staudt and P. O. Brown and D. A. Relman},
	Journal = PNAS,
	Number = {2},
	Pages = {972--977},
	Title = {Stereotyped and specific gene expression programs in human innate immue responses to bacteria},
	Volume = {99},
	Year = {2002}}

@article{Bozdogan00,
	Author = {H. Bozdogan},
	Journal = {Journal of Mathematical Psychology},
	Pages = {62-91},
	Title = {Akaike's information criterion and recent developments in information complexity},
	Volume = {44},
	Year = {2000}}

@incollection{Bozdogan93,
	Author = {H. Bozdogan},
	Booktitle = {Information and Classification},
	Editor = {O. Opitz and B. Lausen and R. Klar},
	Publisher = {Heidelberg: Springer Verlag},
	Title = {Choosing the number of component clusters in the mixture model using a new informational complexity criterion of the inverse Fisher information matrix},
	Year = {1993}}

@article{Braver,
	Author = {S. L. Braver},
	Journal = {Educational and Psychological Measurement},
	Pages = {283--301},
	Title = {On splitting the tails unequally: a new perspective on one-versus two-tailed tests},
	Volume = {35},
	Year = {1975}}

@article{Breckenridge89,
	Author = {J. Breckenridge},
	Journal = {Multivariate Behavioral Research},
	Pages = {147--161},
	Title = {Replicating cluster analysis: Method, consistency and validity},
	Volume = {24},
	Year = {1989}}

@article{Breiman&Spector92,
	Author = {L. Breiman and P. Spector},
	Journal = {International Statistical Review},
	Pages = {291--319},
	Title = {Submodel Selection and Evaluation in Regression. The $X$ Random Case},
	Volume = {60},
	Year = {1992}}

@article{Breiman01,
	Author = {L. Breiman},
	Journal = {Statistical Science},
	Number = {3},
	Pages = {199--215},
	Title = {Statistical modeling: the two cultures},
	Volume = {16},
	Year = {2001}}

@article{Breiman96,
	Author = {L. Breiman},
	Journal = {Annals of Statistics},
	Number = {6},
	Pages = {2350--2383},
	Title = {Heuristics of instability and stabilization in model selection},
	Volume = {24},
	Year = {1996}}

@article{Breiman98,
	Author = {L. Breiman},
	Journal = {Annals of Statistics},
	Pages = {801-824},
	Title = {Arcing classifiers},
	Volume = {26},
	Year = {1998}}

@article{Breiman96b,
	Author = {L. Breiman},
	Journal = {Machine Learning},
	Pages = {123-140},
	Title = {Bagging predictors},
	Volume = {24},
	Year = {1996}}

@techreport{Breiman98b,
	Author = {L. Breiman},
	Institution = {Department of Statistics, U.C. Berkeley},
	Month = {March},
	Number = {513},
	Title = {Using Convex pseudo-data to increase prediction accuracy},
	Year = {1998}}

@article{Breiman92,
	Author = {L. Breiman},
	Journal = JASA,
	Number = {419},
	Pages = {738--754},
	Title = {The Little Bootstrap and Other Methods for Dimensionality Selection in Regression: $X$-Fixed Prediction Error},
	Volume = {87},
	Year = {1992}}

@techreport{Breiman96c,
	Author = {L. Breiman},
	Institution = {Department of Statistics, U.C. Berkeley},
	Title = {Out-of-bag estimation},
	Year = {1996}}

@techreport{Breiman99,
	Author = {L. Breiman},
	Institution = {Department of Statistics, U.C. Berkeley},
	Number = {567},
	Title = {Random forests - random features},
	Year = {1999}}

@book{Breimanetal84,
	Author = {L. Breiman and J. H. Friedman and R. Olshen and C. J. Stone},
	Publisher = {Wadsworth International Group},
	Series = {The Wadsworth statistics/probability series},
	Title = {Classification and regression trees},
	Year = {1984}}

@book{Hastie&Tibshirani&Friedman02,
	Author = {T. Hastie and R. Tibshirani and J. Friedman},
	Publisher = {Springer},
	Series = {Springer Series in Statistics},
	Title = {The Elements of Statistical Learning},
	Year = {2002}}

@article{Broman01,
	Author = {K. W. Broman},
	Journal = {Lab Animal},
	Number = {7},
	Pages = {44--52},
	Title = {Review of statistical methods for QTL mapping in experimental crosses},
	Volume = {30},
	Year = {2001}}

@phdthesis{Broman97,
	Author = {K. W. Broman},
	School = {Department of Statistics, U.C. Berkeley},
	Title = {Identifying quantitative trait loci in experimental crosses},
	Type = {Ph.{D}. thesis},
	Year = {1997}}

@article{Brown&Koplowitz79,
	Author = {T. A. Brown and J. Koplowitz},
	Journal = {IEEE Transactions on Information Theory},
	Number = {5},
	Pages = {617--619},
	Title = {The weighted nearest neighbor rule for class dependent sample sizes},
	Volume = {25},
	Year = {1979}}

@article{Buhlmann&Yu,
	Author = {P. Buhlmann and B. Yu},
	Journal = {Annals of Statistics},
	Title = {Explaining Bagging.},
	Year = {(Accepted)}}

@article{Burges98,
	Author = {C. J. C. Burges},
	Journal = {Data Mining and Knowledge Discovery},
	Month = {December},
	Pages = {121--167},
	Title = {A tutorial on support vector machines for pattern recognition},
	Volume = {2},
	Year = {1998}}

@article{Burman89,
	Author = {P. Burman},
	Journal = {Biometrika},
	Pages = {503-514},
	Title = {A comparative study of ordinary cross-validation, $v$-fold cross-validati on and the repeated learning testing methods},
	Volume = {76},
	Year = {1989}}

@techreport{Buttrey&Karo02,
	Author = {S. E. Buttrey and C. Karo},
	Institution = {Naval Postgraduate School, Monterey, CA},
	Title = {Using k--neareset neighbor classification in the leaves of a tree},
	Year = {2002}}

@article{Calinski&Harabasz74l,
	Author = {R. Calinski and J. Harabasz},
	Journal = {Communications in Statistics},
	Pages = {1--27},
	Title = {A dendrite method for cluster analysis},
	Volume = {3},
	Year = {1974}}

@article{Callowetal00,
	Author = {M. J. Callow and S. Dudoit and E. L. Gong and T. P. Speed and E. M. Rubin},
	Journal = {Genome Research},
	Number = {12},
	Pages = {2022--2029},
	Title = {Microarray expression profiling identifies genes with altered expression in {HDL} deficient mice},
	Volume = {10},
	Year = {2000}}

@book{Chambers98,
	Author = {J. M. Chambers},
	Publisher = {Springer-Verlag New York},
	Title = {Programming with Data: A Guide to the S Language},
	Year = {1998}}

@book{Diggleetal02,
	Author = {Peter J. Diggle and P. Heagerty and K-Y Liang and S.L. Zeger},
	Publisher = {Oxford University Press},
	Title = {Analysis of Longitudinal Data},
	Year = {2002 (Second Edition)}}

@techreport{Chang&Lin01,
	Author = {C.-C. Chang and C.-J. Lin},
	Note = {\\ {\tt http://www.csie.ntu.edu.tw/~cjlin/papers/libsvm2.ps.gz}},
	Title = {LIBSVM: a Library for Support Vector Machines (Version 2.31)},
	Year = {2001}}

@article{Changetal02,
	Author = {H. Y. Chang and J. T. Chi and S. Dudoit and C. Bondre and M. van de Rijn and D. Botstein D and P. O. Brown},
	Journal = PNAS,
	Number = {20},
	Pages = {12877--12882},
	Title = {Diversity, topographic differentiation, and positional memory in human fibroblasts},
	Volume = {99},
	Year = {2002}}

@article{Chenetal02,
	Author = {X. Chen and S. T. Cheung and S. So and S. T. Fan and C. Barry and J. Higgins and K.-M. Lai and J. Ji and S. Dudoit and I. O. L. Ng and M. van de Rijn and D. Botstein and P. O. Brown},
	Journal = {Molecular Biology of the Cell},
	Number = {6},
	Pages = {1929--1939},
	Title = {Gene expression patterns in human liver cancers},
	Volume = {13},
	Year = {2002}}

@article{Cleveland&Devlin88,
	Author = {W. S. Cleveland and S. J. Devlin},
	Journal = JASA,
	Pages = {596--610},
	Title = {Locally-Weighted Regression: An Approach to Regression Analysis by Local Fitting},
	Volume = {83},
	Year = {1988}}

@article{Cleveland79,
	Author = {W. S. Cleveland},
	Journal = JASA,
	Number = {368},
	Pages = {829--836},
	Title = {Robust locally weighted regression and smoothing scatterplots},
	Volume = {74},
	Year = {1979}}

@article{Correa&Wolfson99,
	Author = {J. A. Correa and D. B. Wolfson},
	Journal = {Journal of Statistical Computation and Simulation},
	Pages = {209--219},
	Title = {Length-bias: some characterizations and applications},
	Tnumber = {3},
	Volume = {64},
	Year = {1999}}

@article{Correa&Dudoit&Goldstein02,
	Author = {J. A. Correa and S. Dudoit and D. R. Goldstein},
	Note = {(Submitted)},
	Optjournal = {Statistics in Medicine},
	Title = {Multiple testing in the survival analysis of microarray data},
	Year = {2002}}

@article{Cortes&Vapnik95,
	Author = {C. Cortes and V. Vapnik},
	Journal = {Machine Learning},
	Month = {December},
	Pages = {273-297},
	Title = {Support-vector networks},
	Volume = {20},
	Year = {1995}}

@inproceedings{Davies&Bouldin79,
	Author = {D. Davies and D. Bouldin},
	Booktitle = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
	Optnumber = {PAMI-1},
	Pages = {224--227},
	Title = {A cluster separation measure},
	Volume = {1},
	Year = {1979}}

@article{Davis&Anderson89,
	Author = {R. B. Davis and J. R. Anderson},
	Journal = {Statistics in Medicine},
	Pages = {947-961},
	Title = {Exponential survival trees},
	Volume = {8},
	Year = {1989}}

@incollection{Day96,
	Address = {River Edge, NJ},
	Author = {W. H. E. Day},
	Booktitle = {Clustering and Classification},
	Editor = {P. Arabie and L. J. Hubert and G. De Soete},
	Pages = {199--233},
	Publisher = {World Scientific Publishing Co.},
	Title = {Complexity theory: {A}n introduction for practitioners of classification},
	Year = {1996}}

@article{Dettling&Buhlmann02,
	Author = {M. Dettling and P. B\"{u}hlmann},
	Title = {How to Use Boosting for Tumor Classification with Gene Expression Data},
	Year = {2002}}

@article{Dudoit&Fridlyand02,
	Author = {S. Dudoit and J. Fridlyand},
	Optjournal = {Bioinformatics},
	Title = {Bagging to improve the accuracy of a clustering procedure},
	Year = {2002}}

@incollection{Dudoit&Fridlyand02b,
	Author = {S. Dudoit and J. Fridlyand},
	Booktitle = {Statistical Analysis of Gene Expression Microarray Data},
	Editor = {T. P. Speed},
	Note = {(To appear)},
	Publisher = {Chapman \& Hall/CRC},
	Title = {Classification in microarray experiments},
	Year = {2002}}

@article{Dudoit&Fridlyand02c,
	Author = {S. Dudoit and J. Fridlyand},
	Journal = {Genome Biology},
	Number = {7},
	Pages = {0036.1--0036.21},
	Title = {A prediction-based resampling method to estimate the number of clusters in a dataset},
	Volume = {3},
	Year = {2002}}

@techreport{Dudoit&Fridlyand01,
	Author = {S. Dudoit and J. Fridlyand},
	Institution = {Department of Statistics, Uiversity of California, Berkeley},
	Number = {600},
	Title = {Applications of resampling methods to estimate the number of clusters and to improve the accuracy of a clustering method},
	Url = {stat-www.berkeley.edu/users/sandrine/publications.html},
	Year = {2001},
	Bdsk-Url-1 = {stat-www.berkeley.edu/users/sandrine/publications.html}}

@article{Dudoit&vanderLaan05,
	Author = {S. Dudoit and M.J. van der Laan},
	Journal = {Statistical Methodology},
	Number = {2},
	Optnote = {www.bepress.com/ucbbiostat/paper126},
	Pages = {131--154},
	Title = {Asymptotics of cross-validated risk estimation in estimator selection and performance assessment},
	Volume = {2},
	Year = {2005}}

@article{Dudoit&Speed99,
	Author = {S. Dudoit and T. P. Speed},
	Journal = {Annals of Statistics},
	Number = {3},
	Pages = {943--986},
	Title = {A score test for linkage using identity by descent data from sibships},
	Volume = {27},
	Year = {1999}}

@article{Dudoit&Speed00,
	Author = {S. Dudoit and T. P. Speed},
	Journal = {Biostatistics},
	Number = {1},
	Pages = {1--26},
	Title = {A score test for the linkage analysis of qualitative and quantitative traits based on identity by descent data on sib-pairs},
	Volume = {1},
	Year = {2000}}

@incollection{Dudoit&Speed99b,
	Address = {New York},
	Author = {S. Dudoit and T. P. Speed},
	Booktitle = {Statistics in Genetics},
	Editor = {M. E. Halloran and S. Geisser},
	Pages = {181--221},
	Publisher = {Springer-Verlag},
	Series = {IMA Volumes in Mathematics and its Applications},
	Title = {Triangle constraints for sib-pair identity by descent probabilities under a general multilocus model for disease susceptibility},
	Volume = {112},
	Year = {1999}}

@incollection{Dudoit&Yang03,
	Author = {S. Dudoit and Y. H. Yang},
	Booktitle = {The Analysis of Gene Expression Data: Methods and Software},
	Editor = {G. Parmigiani and E. S. Garrett and R. A. Irizarry and S. L. Zeger},
	Publisher = {Springer, New York},
	Title = {Bioconductor {R} packages for exploratory analysis and normalization of c{DNA} microarray data},
	Year = {2003}}

@article{Dudoit&Fridlyand&Speed02,
	Author = {S. Dudoit and J. Fridlyand and T. P. Speed},
	Journal = JASA,
	Number = {457},
	Pages = {77--87},
	Title = {Comparison of Discrimination Methods for the Classification of Tumors Using Gene Expression Data},
	Volume = {97},
	Year = {2002}}

@article{Dudoitetal02,
	Author = {S. Dudoit and Y. H. Yang and M. J. Callow and T. P. Speed},
	Journal = {Statistica Sinica},
	Number = {1},
	Pages = {111--139},
	Title = {Statistical methods for identifying differentially expressed genes in replicated c{DNA} microarray experiments},
	Volume = {12},
	Year = {2002}}

@techreport{Dudoit&Shaffer&Boldrick02,
	Author = {S. Dudoit and J. P. Shaffer and J. C. Boldrick},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {110},
	Title = {Multiple hypothesis testing in microarray experiments},
	Url = {www.bepress.com/ucbbiostat/paper110/},
	Year = {2002},
	Bdsk-Url-1 = {www.bepress.com/ucbbiostat/paper110/}}

@article{Duffy&Quiroz91,
	Author = {D. E. Duffy and A. J. Quiroz},
	Journal = {Journal of Classification},
	Pages = {65--91},
	Title = {A permutation-based algorithm for block clustering},
	Volume = {8},
	Year = {1991}}

@article{Dunn58,
	Author = {O. J. Dunn},
	Journal = {Annals of Mathematical Statistics},
	Pages = {1095-111},
	Title = {Estimation of the means of dependent variables},
	Volume = {29},
	Year = {1958}}

@book{Efron&Tibshirani93,
	Author = {B. Efron and R. J. Tibshirani},
	Publisher = {Chapman \& Hall/CRC},
	Title = {An Introduction to the Bootstrap},
	Year = {1993}}

@article{EfronetalJASA01,
	Author = {B. Efron and R. Tibshirani and J. D. Storey and V. Tusher},
	Journal = JASA,
	Pages = {1151--1160},
	Title = {Empirical Bayes analysis of a microarray experiment},
	Volume = {96},
	Year = {2001}}

@techreport{Efron&Storey&Tibshirani01,
	Author = {B. Efron and J. D. Storey and R. Tibshirani},
	Institution = {Department of Statistics, Stanford University},
	Number = {2001-218},
	Title = {Microarrays, empirical Bayes methods, and false discovery rates},
	Year = {2001}}

@article{Finner99,
	Author = {H. Finner},
	Journal = {Annals of Statistics},
	Pages = {274--289},
	Title = {Stepwise multiple test procedures and control of directional errors},
	Volume = {27},
	Year = {1999}}

@article{Fisher36,
	Author = {R. A. Fisher},
	Journal = {Annals of Eugenics},
	Pages = {179-188},
	Title = {The use of multiple measurements in taxonomic problems},
	Volume = {7},
	Year = {1936}}

@article{Fisher26,
	Author = {R. A. Fisher},
	Journal = {J. Min. Agric. Gr. Br},
	Pages = {505--513},
	Title = {The arrangement of field experiments},
	Volume = {33},
	Year = {1926}}

@techreport{Fix&Hodges51,
	Author = {E. Fix and J. Hodges},
	Institution = {Randolph Field, Texas: USAF School of Aviation Medicine},
	Title = {Discriminatory analysis, nonparametric discrimination: consistency properties},
	Year = {1951}}

@article{Fowlkes&Mallows83,
	Author = {E. B. Fowlkes and C. L. Mallows},
	Journal = JASA,
	Optnumber = {383},
	Pages = {553--584},
	Title = {A method for comparing two hierarchical clusterings},
	Volume = {78},
	Year = {1983}}

@article{Fowlkes&Gnanadesikan&Kettenring88,
	Author = {E. B. Fowlkes and R. Gnanadesikan and J. R. Kettenring},
	Journal = JC,
	Pages = {205--228},
	Title = {Variable selection in clustering},
	Volume = {5},
	Year = {1988}}

@techreport{Fraley&Raftery98,
	Author = {C. Fraley and A. Raftery},
	Institution = {Department of Statistics, University of Washington},
	Note = {\url{http://www.stat.washington.edu/www/research/reports/1990s/#1998}},
	Number = {329},
	Title = {How many clusters? Which clustering method? -- answers via model-based cluster analysis},
	Year = {1998}}

@article{Freund&Schapire97,
	Author = {Y. Freund and R. E. Schapire},
	Journal = {Journal of Computer and System Sciences},
	Pages = {119--139},
	Title = {A decision-theoretic generalization of on-line learning and an application to boosting},
	Volume = {55},
	Year = {1997}}

@phdthesis{Fridlyand01,
	Author = {J. Fridlyand},
	School = {Department of Statistics, U.C. Berkeley},
	Title = {Resampling methods for variable selection and classification: applications to genomics},
	Type = {Ph.{D}. thesis},
	Year = {2001}}

@techreport{Friedman94,
	Author = {J. H. Friedman},
	Institution = {Department of Statistics, Stanford University},
	Title = {Flexible metric nearest neighbor clasification},
	Year = {1994}}

@techreport{Friedman96a,
	Author = {J. H. Friedman},
	Institution = {Department of Statistics, Stanford University},
	Title = {On bias, variance, 0/1-loss, and the curse--of--dimensionality},
	Year = {1996}}

@techreport{Friedman96b,
	Author = {J. H. Friedman},
	Institution = {Department of Statistics, Stanford University},
	Title = {Another approach to polychotomous classification},
	Year = {1996}}

@article{Friedman&Hastie&Tibshirani00,
	Author = {J. Friedman and T. Hastie and R. Tibshirani},
	Journal = {Annals of Statistics},
	Note = {(with discussion)},
	Pages = {337--404},
	Title = {Additive logistic regression: a statistical view of boosting},
	Volume = {28},
	Year = {2000}}

@book{Hastie&Tibshirani90,
	Address = {London},
	Author = {T. J. Hastie and R.J. Tibshirani},
	Publisher = {Chapman and Hall},
	Title = {Generalized Additive Models},
	Year = {1990}}

@article{Gabriel71,
	Author = {K. R. Gabriel},
	Journal = {Biometrika},
	Pages = {453--467},
	Title = {The biplot graphic display of matrices with application to principal component analysis},
	Volume = {58},
	Year = {1971}}

@incollection{Gabriel75,
	Author = {K. R. Gabriel},
	Booktitle = {Multivariate Statistical Methods: Among-groups covariation; Within-group covariation},
	Pages = {61--80},
	Title = {A comparison of some methods of simultaneous inference in {MANOVA}},
	Year = {1975}}

@inproceedings{Gabriel&Pun79,
	Author = {K. R. Gabriel and F. C. Pun},
	Booktitle = {Sixth Conference on Probability and Statistics in Atmospheric Science},
	Organization = {American Meterological Society},
	Pages = {248--253},
	Title = {Binary prediction of weather events with several predictors},
	Year = {1979}}

@unpublished{Ge&Dudoit02,
	Author = {Y. Ge and S. Dudoit},
	Note = {(In preparation)},
	Title = {Fast algorithm for resampling-based $p$-value adjustment in multiple testing},
	Year = {2002}}

@article{Geisser75,
	Author = {S. Geisser},
	Journal = {Journal of the American Statistical Association},
	Pages = {320-328},
	Title = {The predictive sample reuse method with applications},
	Volume = {70},
	Year = {1975}}

@techreport{Genovese&Wasserman01,
	Author = {C. Genovese and L. Wasserman},
	Institution = {Department of Statistics, Carnegie Mellon},
	Number = {737},
	Title = {Operating Characteristics and Extensions of the FDR Procedure},
	Year = {2001}}

@article{Gnanadesikan&Kettenring95,
	Author = {R. Gnanadesikan and J. R. Kettenring},
	Journal = JC,
	Pages = {113--136},
	Title = {Weighting and selection of variables for cluster analysis},
	Volume = {12},
	Year = {1995}}

@article{Goldstein&Dudoit&Speed00,
	Author = {D. R. Goldstein and S. Dudoit and T. P. Speed},
	Journal = {Genetic Epidemiology},
	Number = {Suppl. 1},
	Pages = {S85--S91},
	Title = {Power of a score test for quantitative trait linkage analysis of relative pairs.},
	Volume = {19},
	Year = {2000}}

@article{Goldstein&Dudoit&Sped01,
	Author = {D. R. Goldstein and S. Dudoit and T. P. Speed},
	Journal = {Genetic Epidemiology},
	Number = {4},
	Pages = {415--431},
	Title = {Power and robustness of a score test for linkage analysis of quantitative traits using identity by descent data on sib pairs},
	Volume = {20},
	Year = {2001}}

@article{Gordon&Olshen85,
	Author = {L. Gordon and R.A. Olshen},
	Journal = {Cancer Treatment Reports},
	Pages = {10065-1069},
	Title = {Tree-structured survival analysis},
	Volume = {69},
	Year = {1985}}

@incollection{Gordon96,
	Address = {River Edge, NJ},
	Author = {A. D. Gordon},
	Booktitle = {Clustering and Classification},
	Editor = {P. Arabie and L. J. Hubert and G. De Soete},
	Pages = {65--121},
	Publisher = {World Scientific Publishing Co.},
	Title = {Hierarchical classification},
	Year = {1996}}

@book{Gower&Hand96,
	Author = {J. C. Gower and D. J. Hand},
	Edition = {1st},
	Number = {54},
	Publisher = {Chapman \& Hall},
	Series = {Monographs on statistics and applied probability},
	Title = {Biplots},
	Year = {1996}}

@book{Gyorfietal02,
	Address = {New York},
	Author = {L. Gy\"{o}rfi and M. Kohler and A. Krzy\.{z}ak and H. Walk},
	Pages = {100-102},
	Publisher = {Springer-Verlag},
	Title = {A Distribution-Free Theory of Nanparametric Regression},
	Year = {2002}}

@book{Gyorfietal02b,
	Author = {L. Gy\"orfi and M. Kohler and A. Krzy\'{z}ak and H. Walk},
	Publisher = {Springer-Verlag, New York},
	Title = {A distribution-free theory of nonparametric regression},
	Year = {2002}}

@book{Hastie&Tibshirani&Friedman01,
	Author = {T. Hastie and R. Tibshirani and J. H. Friedman},
	Publisher = {Springer Verlag},
	Title = {The Elements of Statistical Learning : Data Mining, Inference, and Prediction},
	Year = {2001}}

@article{Hansen&Yu01,
	Author = {M. H. Hansen and B. Yu},
	Journal = {Journal of the American Statistical Association},
	Pages = {746-774},
	Title = {Model selection and the principle of minimum description length},
	Volume = {96},
	Year = {2001}}

@article{Hardle&Marron85a,
	Author = {W. H{\"a}rdle and J. S. Marron},
	Journal = {Biometrika},
	Pages = {481--484},
	Title = {Asymptotic nonequivalence of some bandwidth selectors in nonparametric regression},
	Volume = {72},
	Year = {1985}}

@article{Hardle&Marron85b,
	Author = {W. H{\"a}rdle and J. S. Marron},
	Journal = {Annals of Statistics},
	Pages = {1465-1481},
	Title = {Optimal bandwidth selection in nonparametric regression function estimation},
	Volume = {13},
	Year = {1985}}

@book{Hardle93,
	Author = {W. H{\"a}rdle},
	Publisher = {Cambridge University Press},
	Title = {Applied Nonparametric Regression},
	Year = {1993}}

@article{Hartigan72,
	Author = {J. A. Hartigan},
	Journal = {Journal of the American Statistical Association},
	Pages = {123--129},
	Title = {Direct clustering of a data matrix},
	Volume = {67},
	Year = {1972}}

@book{Hartigan75,
	Author = {J. A. Hartigan},
	Publisher = {Wiley},
	Title = {Clustering Algorithms},
	Year = {1975}}

@article{Hartigan78,
	Author = {J. Hartigan},
	Journal = {Annals of Statistics},
	Pages = {117--131},
	Title = {Asymptotic distributions for clustering criteria},
	Volume = {6},
	Year = {1978}}

@article{Hartigan85,
	Author = {J. A. Hartigan},
	Journal = JC,
	Pages = {63--76},
	Title = {Statistical theory in clustering},
	Volume = {2},
	Year = {1985}}

@article{Hastie&Tibshirani96a,
	Author = {T. Hastie and R. Tibshirani},
	Journal = {IEEE Pattern Recognition and Machine Intelligence},
	Pages = {607--616},
	Title = {Discriminant adaptive nearest-nieghbor classification},
	Volume = {18},
	Year = {1996}}

@techreport{Hastie&Tibshirani96b,
	Author = {T. Hastie and R. Tibshirani},
	Institution = {Department of Statistics, Stanford University},
	Title = {Classification by pairwise coupling},
	Year = {1996}}

@article{Hastie&Tibshirani90,
	Author = {T.J. Hastie and R.J. Tibshirani},
	Journal = {Biometrics},
	Number = {4},
	Pages = {1005-1016},
	Title = {Exploring the nature of covariate effects in the proportional hazar ds model},
	Volume = {46},
	Year = {1990}}

@book{Hochberg&Tamhane87,
	Author = {Y. Hochberg and A. C. Tamhane},
	Publisher = {Wiley--Interscience},
	Series = {Probability and Mathematical Statistics},
	Title = {Multiple Comparison Procedures},
	Year = {1987}}

@article{Hochberg88,
	Author = {Y. Hochberg},
	Journal = {Biometrika},
	Pages = {800--802},
	Title = {A sharper Bonferroni procedure for multiple tests of significance},
	Volume = {75},
	Year = {1988}}

@article{Holm79,
	Author = {S. Holm},
	Journal = {Scand. J. Statist.},
	Pages = {65--70},
	Title = {A simple sequentially rejective multiple test procedure},
	Volume = {6},
	Year = {1979}}

@article{Hommel&Bernhard99,
	Author = {G. Hommel and G. Bernhard},
	Journal = {Journal of Statistical Planning and Inference},
	Pages = {119--128},
	Title = {Bonferroni procedures for logically related hypotheses},
	Volume = {82},
	Year = {1999}}

@article{Hommel88,
	Author = {G. Hommel},
	Journal = {Biometrika},
	Pages = {383--386},
	Title = {A stagewise rejective multiple test procedure based on a modified Bonferroni test},
	Volume = {75},
	Year = {1988}}

@article{Hubert&Arabie85,
	Author = {L. Hubert and P. Arabie},
	Journal = JC,
	Pages = {193--218},
	Title = {Comparing partitions},
	Volume = {2},
	Year = {1985}}

@book{Jain&Dubes88,
	Address = {Englewood Cliffs, N. J.},
	Author = {A. K. Jain and R. C. Dubes},
	Publisher = {Prentice-Hall},
	Title = {Algorithms for Clustering Data},
	Year = {1988}}

@article{Jogdeo77,
	Author = {K. Jogdeo},
	Journal = {Annals of Statistics},
	Pages = {495--504},
	Title = {Association and probability inequalities},
	Volume = {5},
	Year = {1977}}

@book{Kaufman&Rousseeuw90,
	Author = {L. Kaufman and P. J. Rousseeuw},
	Publisher = {Wiley, New York.},
	Title = {Finding Groups in Data: An Introduction to Cluster Analysis},
	Year = {1990}}

@article{Keles&vanderLaan&Dudoit03,
	Author = {Kele\c{s}, S. and van der Laan, M. and Dudoit, S.},
	Journal = {Technical Report, Division of Biostatistics, UC Berkeley},
	Title = {Asymptotically Optimal Model Selection Method for Regression on Censored Outcomes},
	Year = {2002}}

@article{Kohonen90,
	Author = {T. Kohonen},
	Journal = {Proc. IEEE},
	Number = {9},
	Pages = {1464--1480},
	Title = {The self-organizing map},
	Volume = {78},
	Year = {1990}}

@book{Kohonen95,
	Address = {Berlin, Heidelberg},
	Author = {T. Kohonen},
	Editor = {T. S. Huang and T. Kohonen and M. R. Schroeder},
	Publisher = {Springer},
	Series = {Springer Series in Information Sciences},
	Title = {Self-Organizing Maps},
	Volume = {30},
	Year = {1995}}

@article{Kooperberg&Stone&Truong95,
	Author = {C. Kooperberg and C.J. Stone and Y. K. Truong},
	Journal = {Journal of the American Statistical Association},
	Number = {429},
	Pages = {78-94},
	Title = {Hazard Regression},
	Volume = {90},
	Year = {1995}}

@article{Koutsoukosetal94,
	Author = {A. D. Koutsoukos and L. V. Rubinstein and D. Faraggi and R.M. Simon and S. Kalyandrug and J. N. Weinstein and K.W. Kohn and K.D. Paull},
	Journal = {Statistics in Medicine},
	Pages = {719--730},
	Title = {Discrimination techniques applied to the {NCI} in vitro anti-tumor drug screen: predicting biochemical mechanism of action},
	Volume = {13},
	Year = {1994}}

@article{Krishnaiah&Reising85,
	Author = {P. R. Krishnaiah and J. M. Reising},
	Journal = {Encyclopedia of Statistical Sciences},
	Number = {6},
	Pages = {88--95},
	Title = {Multivariate multiple comparisons},
	Volume = {9},
	Year = {1985}}

@article{Krzanowski&Lai85,
	Author = {W. Krzanowski and Y. Lai},
	Journal = {Biometrics},
	Pages = {23--34},
	Title = {A criterion for determining the number of groups in a dataset using sum of squares clustering},
	Volume = {44},
	Year = {1985}}

@article{Laan&Bryan01,
	Author = {M. J. van der Laan and J. Bryan},
	Journal = {Biostatistics},
	Number = {4},
	Pages = {445--461},
	Title = {Gene expression analysis with the parametric bootstrap},
	Volume = {2},
	Year = {2001}}

@article{Pollard&vanderLaan04,
	Author = {K. S. Pollard and M.J. van der Laan},
	Journal = JSPI,
	Optpages = {85--101},
	Optvolume = {125},
	Title = {Choice of Null Distribution in Resampling Based Multiple Testing},
	Year = {2004}}

@article{vanderLaan&Pollard02,
	Author = {M. J. van der Laan and K. S. Pollard},
	Journal = JSPI,
	Note = {(To appear)},
	Title = {Hybrid clustering of gene expression data with visualization and the bootstrap},
	Year = {2002}}

@article{Leblanc&Crowley92,
	Author = {M. Leblanc and J. Crowley},
	Journal = {Biometrics},
	Pages = {411-425},
	Title = {Relative Risk trees for censored data},
	Volume = {48},
	Year = {1992}}

@inproceedings{Leisch02,
	Author = {F. Leisch},
	Booktitle = {Compstat 2002 --- Proceedings in Computational Statistics},
	Editor = {Wolfgang H{\"a}rdle and Bernd R{\"o}nz},
	Note = {ISBN 3-7908-1517-9},
	Publisher = {Physika Verlag, Heidelberg, Germany},
	Title = {Sweave: Dynamic Generation of Statistical Reports Using Literate Data Analysis},
	Tpages = {575--580},
	Url = {http://www.ci.tuwien.ac.at/~leisch/Sweave},
	Year = {2002},
	Bdsk-Url-1 = {http://www.ci.tuwien.ac.at/~leisch/Sweave}}

@techreport{Leisch02Tb,
	Author = {F. Leisch},
	Institution = {SFB Adaptive Information Systems and Modelling in Economics and Management Science, Vienna University of Economics and Business Administration},
	Month = {March},
	Number = {69},
	Title = {Dynamic generation of statistical reports using literate data analysis},
	Year = {2002}}

@techreport{Leisch99,
	Author = {F. Leisch},
	Institution = {SFB Adaptive Information Systems and Modelling in Economics and Management Science, Vienna University of Economics and Business Administration},
	Month = {August},
	Note = {\url{http://www.ci.tuwien.ac.at/~leisch/papers/fl-techrep.html}},
	Title = {Bagged clustering},
	Year = {1999}}

@article{Lim&Low&Shih00,
	Author = {T-S Lim and W-Y Loh and Y-S Shih},
	Journal = {Machine Learning},
	Pages = {203--229},
	Title = {A comparison of prediction accuracy, complexity, and training time of thiry-three old and new classification algorithms},
	Volume = {40},
	Year = {2000}}

@book{Mardia&Kent&Bibby79,
	Address = {San Diego},
	Author = {K. V. Mardia and J. T. Kent and J. M. Bibby},
	Publisher = {Academic Press, Inc.},
	Title = {Multivariate Analysis},
	Year = {1979}}

@unpublished{Mayo&Spanos02,
	Author = {D. C. Mayo and A. Spanos},
	Title = {A severe-testing interpretation of {N}eyman-{P}earson methods. Unpublished manuscript},
	Year = {2002}}

@book{McCullagh&Nelder89,
	Author = {P. McCullagh and J. A. Nelder},
	Edition = {2nd},
	Number = {37},
	Publisher = {Chapman \& Hall},
	Series = {Monographs on Statistics and Applied Probability},
	Title = {Generalized Linear Models},
	Year = {1989}}

@book{McLachlan92,
	Address = {New York},
	Author = {G. J. McLachlan},
	Publisher = {Wiley},
	Title = {Discriminant analysis and statistical pattern recognition},
	Year = {1992}}

@article{McLachlan&Bean&Peel01,
	Author = {G. J. McLachlan and R. Bean and D. Peel},
	Journal = {Bioinformatics},
	Pages = {413--422},
	Title = {A mixture model-based approach to the clustering of microarray expression data.},
	Volume = {18},
	Year = {2002}}

@book{Miller90,
	Author = {A. J. Miller},
	Publisher = {Chapman and Hall},
	Title = {Subset Selection in Regression},
	Year = {1990}}

@article{Milligan&Cooper85,
	Author = {G. W. Milligan and M. C. Cooper},
	Journal = {Psychometrika},
	Pages = {159--179},
	Title = {An examination of procedures for determining the number of clusters in a data set},
	Volume = {50},
	Year = {1985}}

@article{Milligan&Cooper86,
	Author = {G. W. Milligan and M. C. Cooper},
	Journal = {Multivariate Behavioral Research},
	Pages = {441--458},
	Title = {A study of the comparability of external criteria for hierarchical cluster analysis},
	Volume = {21},
	Year = {1986}}

@article{Milligan&Cooper87,
	Author = {G. W. Milligan and M. C. Cooper},
	Journal = {Applied Psychological Measurement},
	Optmonth = {December},
	Optnumber = {4},
	Pages = {329--354},
	Title = {Methodology review: {C}lustering methods},
	Volume = {11},
	Year = {1987}}

@article{Milligan89,
	Author = {G. W. Milligan},
	Journal = {Multivariate Behavioral Research},
	Pages = {163--176},
	Title = {A study of the beta-flexible clustering method},
	Volume = {24(2)},
	Year = {1989}}

@incollection{Milligan96,
	Address = {River Edge, NJ},
	Author = {G. W. Milligan},
	Booktitle = {Clustering and Classification},
	Editor = {P. Arabie and L. J. Hubert and G. De Soete},
	Pages = {341--375},
	Publisher = {World Scientific Publishing Co.},
	Title = {Clustering validation: {R}esults and implications for applied analyses},
	Year = {1996}}

@article{Morey&Blashfield&Skinnerl83,
	Author = {L. C. Morey, R. K. Blashfield and H. A. Skinner},
	Journal = {Multivariate Behavioral Research},
	Pages = {309--329},
	Title = {A comparison of cluster analysis techniques within a sequential validation framework},
	Volume = {18},
	Year = {1983}}

@book{Morrison90,
	Author = {D. F. Morrison},
	Edition = {3rd},
	Publisher = {McGraw-Hill, NY},
	Title = {Multivariate Statistical Methods},
	Year = {1990}}

@incollection{Murtagh96,
	Address = {River Edge, NJ},
	Author = {F. Murtagh},
	Booktitle = {Clustering and Classification},
	Editor = {P. Arabie and L. J. Hubert and G. De Soete},
	Pages = {235--269},
	Publisher = {World Scientific Publishing Co.},
	Title = {Neural networks for clustering},
	Year = {1996}}

@article{PanelDACC89,
	Author = {{Panel on Discriminant Analysis, Classification, and Clustering}},
	Journal = {Statistical Science},
	Pages = {34--69},
	Title = {Discriminant analysis and clustering},
	Volume = {4},
	Year = {1989}}

@techreport{Pavlic&vanderLaan89,
	Author = {M. Pavlic and M. J. van der Laan},
	Institution = {Division of Biostatistics, U.C. Berkeley},
	Month = {February},
	Number = {89},
	Title = {Fitting of mixtures with unspecified number of components using cross-validation distance estimate},
	Year = {2001}}

@article{Pavlic&vanderLaan02,
	Author = {M. Pavlic and M. J. van der Laan},
	Issue = {3-4},
	Journal = {Computational Statistics and Data Analysis},
	Pages = {413-428},
	Title = {Fitting of mixtures with unspecified number of components using cross validation distance estimate},
	Volume = {41},
	Year = {2003}}

@techreport{Pollard&vanderLaan02,
	Author = {K. S. Pollard and M. J. van der Laan},
	Institution = {Division of Biostatistics, U.C. Berkeley},
	Month = {April},
	Number = {107},
	Title = {A Method to Identify Significant Clusters in Gene Expression Data},
	Year = {2002}}

@techreport{Pollard&vanderLaan02b,
	Author = {K. S. Pollard and M. J. van der Laan},
	Institution = {Division of Biostatistics, U.C. Berkeley},
	Number = {121},
	Title = {Resampling-based methods for identification of significant subsets of genes in expression data},
	Year = {2002}}

@article{Ramsey78,
	Author = {P. H. Ramsey},
	Journal = JASA,
	Pages = {479--485},
	Title = {Power differences between pairwise multiple comparisons},
	Volume = {73},
	Year = {1978}}

@manual{Breiman01b,
	Author = {L. Breiman},
	Title = {Notes on setting up, using, and understanding random forests V3.0},
	Year = {2001}}

@article{Rand71,
	Author = {W. M. Rand},
	Journal = {Journal of the American Statistical Association},
	Optnumber = {336},
	Pages = {846--850},
	Title = {Objective criteria for the evaluation of clustering methods},
	Volume = {66},
	Year = {1971}}

@unpublished{Reiner&Yekutieli&Benjaminil01,
	Author = {A. Reiner and D. Yekutieli and Y. Benjamini},
	Title = {Using resampling-based {FDR} controlling multiple test procedures for analyzing microarray gene expression data},
	Year = {2001}}

@book{Ripley96,
	Address = {Cambridge, New York},
	Author = {B. D. Ripley},
	Publisher = {Cambridge University Press},
	Title = {Pattern recognition and neural networks},
	Year = {1996}}

@article{Rissanen78,
	Author = {J. Rissanen},
	Journal = {Automatica},
	Pages = {465-471},
	Title = {Modelling by shortest data description},
	Volume = {14},
	Year = {1978}}

@article{Rnews:Dudoit&Yang&Bolstad02,
	Author = {S. Dudoit and Y. H. Yang and B. Bolstad},
	Journal = {R News},
	Month = {March},
	Number = 1,
	Pages = {24--32},
	Title = {Using {R} for the Analysis of {DNA} Microarray Data},
	Url = {CRAN.R-project.org/doc/Rnews/},
	Volume = 2,
	Year = 2002,
	Bdsk-Url-1 = {CRAN.R-project.org/doc/Rnews/}}

@article{Robins&Botnitzky00,
	Author = {J. M. Robins and A. Rotnitzky},
	Journal = {Statistica Sinica},
	Number = {4},
	Pages = {920-936},
	Title = {Comment on the {B}ickel and {K}won article, ``{I}nference for semiparametric models: {S}ome questions and an answer''},
	Volume = {11},
	Year = {2001}}

@inproceedings{Robins00,
	Author = {J.M. Robins},
	Booktitle = {Proceedings of the American Statistical Association},
	Title = {Robust estimation in sequentially ignorable missing data and causal inference models},
	Year = {2000}}

@article{Robins&Rotnitzky&vanderLaan00,
	Author = {J. M. Robins and A. Rotnitzky and M.J. van der Laan},
	Journal = {Journal of the American Statistical Association -- Theory and Methods},
	Pages = {431-435},
	Title = {Comment on ``{O}n {P}rofile {L}ikelihood" by {S}.{A}. {M}urphy and {A}.{W}. van der {V}aart},
	Volume = {450},
	Year = {2000}}

@article{Birge83,
	Author = {L. Birg{\'e}},
	Journal = {Verw. Gebiete},
	Pages = {181--238},
	Title = {Approximation dans les espaces m{/'e}triques et th{\'e}orie de l'estimation},
	Volume = {65},
	Year = {1983}}

@article{lecam73,
	Author = {L.M. le Cam},
	Journal = {Annals of Statistics},
	Pages = {38--53},
	Title = {Convergence of estimates under dimensionality restrictions},
	Volume = {22},
	Year = {1973}}

@article{Rom90,
	Author = {D. M. Rom},
	Journal = {Biometrika},
	Pages = {663-665},
	Title = {A sequentially rejective test procedure based on a modified {Bonferroni} inequality},
	Volume = {77},
	Year = {1990}}

@techreport{Rosenblatt57,
	Author = {F. Rosenblatt},
	Institution = {Cornell Aeronautical Laboratory},
	Number = {86-460-1},
	Title = {The perceptron -- a perceiving and recognizing automation},
	Year = {1957}}

@article{Ruczinskietal&Kooperberg&LeBlanc01,
	Author = {I. Ruczinski and C. Kooperberg and M. LeBlanc},
	Note = {Submitted, \url{http://biosun01.biostat.jhsph.edu/~iruczins/html/publications.html}},
	Title = {Logic regression},
	Year = {2001}}

@article{Saltstone&Stange96,
	Author = {R. Saltstone and K. Stange},
	Journal = {Journal of Classification},
	Pages = {169--172},
	Title = {A computer program to calculate Hubert and Arabie's adjusted Rand index},
	Volume = {13},
	Year = {1996}}

@techreport{vanderVaart03,
	Author = {A.W. van der Vaart},
	Institution = {Department of Mathematics, Free University, Amsterdam},
	Optannote = {Unpublished manuscript},
	Title = {Notes on Cross-validation},
	Year = {2003}}

@techreport{Sarle83,
	Author = {W. Sarle},
	Institution = {SAS Institute, Inc.},
	Note = {\url{http://www.sas.com/service/library/onlinedoc/trindex.html}},
	Number = {A-108},
	Title = {Cubic clustering criterion},
	Year = {1983}}

@techreport{Sarle&Kuo93,
	Author = {W. Sarle and A. Kuo},
	Institution = {SAS Institute, Inc.},
	Number = {P-256},
	Title = {The MODECLUS Procedures},
	Year = {1993}}

@article{Schapireetal98,
	Author = {R. E. Schapire and Y. Freund and P. Bartlett and W. S. Lee},
	Journal = {Annals of Statistics},
	Pages = {1651--1686},
	Title = {Boosting the margin: a new explanation for the effectiveness of voting methods},
	Volume = {26},
	Year = {1998}}

@book{Scheffe59,
	Author = {H. Scheff\'{e}},
	Publisher = {John Wiley \& Sons},
	Title = {The analysis of variance},
	Year = {1959}}

@article{Scheibler&Schneider85,
	Author = {D. Scheibler and W. Schneider},
	Journal = {Multivariate Behavioral Research},
	Pages = {283--304},
	Title = {Monte Carlo tests of the accuracy of cluster analysis algorithms: A comparison of hierarchical and nonhierarchical methods},
	Volume = {20},
	Year = {1985}}

@inproceedings{Schuster&Gregory81,
	Author = {E. F. Schuster and C. G. Gregory},
	Booktitle = {Computer Science and Statistics: Proceedings of the 13th Symposium on the interface},
	Editor = {Eddy, W.F.},
	Pages = {295-298},
	Title = {On the non-consistency of maximum likelihood nonparametric density estimators},
	Year = {1981}}

@article{Scott&Factor81,
	Author = {D. W. Scott and L. E. Factor},
	Journal = {Journal of the American Statistical Association},
	Pages = {9-15},
	Title = {Monte Carlo study of three data-based nonparametric density estimators},
	Volume = {76},
	Year = {1981}}

@article{Seeger68,
	Author = {P. Seeger},
	Journal = {Technometrics},
	Number = {3},
	Pages = {586--593},
	Title = {A note on a method for the analysis of significances en masse},
	Volume = {10},
	Year = {1968}}

@article{Segal88,
	Author = {M. R. Segal},
	Journal = {Biometrics},
	Pages = {35--47},
	Title = {Regression trees for censored data},
	Volume = {44},
	Year = {1988}}

@article{Shaffer02,
	Author = {J. P. Shaffer},
	Journal = {Psychological Methods},
	Pages = {356--369},
	Title = {Multiplicity, directional ({T}ype {III}) errors, and the null hypothesis},
	Volume = {7},
	Year = {2002}}

@article{Shaffer86,
	Author = {J. P. Shaffer},
	Journal = JASA,
	Pages = {826--831},
	Title = {Modified sequentially rejective multiple test procedures},
	Volume = {81},
	Year = {1986}}

@article{Shaffer95,
	Author = {J. P. Shaffer},
	Journal = {Annu. Rev. Psychol.},
	Pages = {561--584},
	Title = {Multiple hypothesis testing},
	Volume = {46},
	Year = {1995}}

@article{Shao93,
	Author = {Shao, J.},
	Journal = {Journal of the American Statistical Association},
	Pages = {486-494},
	Title = {Linear Model Selection by Cross-Validation},
	Volume = {88},
	Year = {1993}}

@article{Sidak67,
	Author = {Z. \v{S}id\'{a}k},
	Journal = JASA,
	Pages = {626-633},
	Title = {Rectangular confidence regions for the means of multivariate normal distributions},
	Volume = {62},
	Year = {1967}}

@article{Silverman96,
	Author = {B. W. Silverman},
	Journal = {Annals of Statistics},
	Pages = {1--24},
	Title = {Smoothed functional principal components analysis by choice of norm},
	Volume = {24},
	Year = {1996}}

@article{Silverman84,
	Author = {B. W. Silverman},
	Journal = JASA,
	Number = {387},
	Pages = {584--589},
	Title = {A fast and efficient cross-validation method for smoothing parameter choice in spline regression},
	Volume = {79},
	Year = {1984}}

@book{Silverman86,
	Author = {B. W. Silverman},
	Publisher = {Chapman \& Hall},
	Title = {Density Estimation for Statistics and Data analysis},
	Year = {1986}}

@article{vanderLaan&Dudoit&Keles04,
	Author = {M.J. van der Laan and S. Dudoit and S. Keles},
	Journal = {Statistical Applications in Genetics and Molecular Biology},
	Optnote = {http://www.bepress.com/sagmb/vol3/iss1/art4},
	Optnumber = {1},
	Title = {Asymptotic optimality of likelihood-based cross-validation},
	Volume = {3},
	Year = {2004}}

@article{Simes86,
	Author = {R. J. Simes},
	Journal = {Biometrika},
	Pages = {751--754},
	Title = {An improved Bonferroni procedure for multiple tests of significance},
	Volume = {73},
	Year = {1986}}

@article{Smyth00,
	Author = {P. Smyth},
	Journal = {Statistics and Computing},
	Pages = {63-72},
	Title = {Model selection of probabilistic clustering using cross-validated likelihood},
	Volume = {10},
	Year = {2000}}

@article{Soric89,
	Author = {B. Sori\'{c}},
	Journal = JASA,
	Number = {406},
	Pages = {608--610},
	Title = {Statistical ``discoveries" and effect-size estimation},
	Volume = {84},
	Year = {1989}}

@article{Stone74,
	Author = {M. Stone},
	Journal = {Journal of the Royal Statistical Society, Series B},
	Pages = {111-147},
	Title = {Cross-validatory choice and assessment of statistical predictions},
	Volume = {36},
	Year = {1974}}

@article{Stone84,
	Author = {C. J. Stone},
	Journal = {Annals of Statistics},
	Number = {4},
	Pages = {1285--1297},
	Title = {An asymptotically optimal window selection rule for kernel density estimates},
	Volume = {12},
	Year = {1984}}

@article{Stone74,
	Author = {M. Stone},
	Journal = JRSSB,
	Number = {2},
	Pages = {111--147},
	Title = {Cross-validatory choice and assessment of statistics predictions},
	Volume = {36},
	Year = {1974}}

@article{Stone77,
	Author = {M. Stone},
	Journal = {Biometrika},
	Number = {1},
	Pages = {29--35},
	Title = {Asymptotics for and against cross-validation},
	Volume = {64},
	Year = {1977}}

@techreport{Storey&Tibshirani01,
	Author = {J. D. Storey and R. Tibshirani},
	Institution = {Department of Statistics, Stanford University},
	Number = {2001-28},
	Title = {Estimating false discovery rates under dependence, with applications to DNA microarrays},
	Year = {2001}}

@article{Storey02,
	Author = {J. D. Storey},
	Journal = JRSSB,
	Pages = {479--498},
	Title = {A direct approach to false discovery rates},
	Volume = {64},
	Year = {2002}}

@techreport{Storey01,
	Author = {J. D. Storey},
	Institution = {Department of Statistics, Stanford University},
	Number = {2001-12},
	Title = {The positive False Discovery Rate: A Bayesian interpretation and the q-value},
	Year = {2001}}

@book{Lehmann86,
	Author = {E. L. Lehmann},
	Edition = {2nd},
	Publisher = {Springer-Verlag, New York},
	Title = {Testing Statistical Hypotheses},
	Year = {1986}}

@article{Tibshiranietal02a,
	Author = {R. Tibshirani and T. Hastie and B. Narasimhan and. G. Chu},
	Journal = PNAS,
	Note = {In press},
	Title = {Diagnosis of multiple cancer types by shrunken centroids of gene expression},
	Year = {2002}}

@article{Troendle95,
	Author = {J. F. Troendle},
	Journal = JASA,
	Pages = {370--378},
	Title = {A stepwise resampling method of multiple hypothesis testing},
	Volume = {90},
	Year = {1995}}

@article{Troendle96,
	Author = {J. F. Troendle},
	Journal = {Biometrics},
	Pages = {846--859},
	Title = {A permutational step-up method of testing multiple outcomes},
	Volume = {52},
	Year = {1996}}

@book{vanderVaart&Wellner96,
	Author = {A. W. van der Vaart and J. A. Wellner},
	Pages = {102},
	Publisher = {Springer-Verlag New York},
	Title = {Weak {C}onvergence and {E}mprical {P}rocesses},
	Year = {1996}}

@book{vanderVaart98,
	Author = {A. W. van der Vaart},
	Pages = {62},
	Publisher = {Cambridge University Press},
	Title = {Asymptotic Statistics},
	Year = {1998}}

@book{Vapnik00,
	Address = {New York},
	Author = {V. N. Vapnik},
	Edition = {2nd},
	Publisher = {Springer},
	Series = {Statistics for engineering and information science},
	Title = {The nature of statistical learning theory},
	Year = {2000}}

@article{Vapnik79,
	Author = {V. Vapnik},
	Journal = {Nauka, Moskow},
	Title = {Estimation of dependences based on empirical data (in Russian)},
	Year = {1979}}

@book{Vapnik98,
	Address = {New York},
	Author = {V. Vapnik},
	Edition = {1st},
	Publisher = {Wiley},
	Title = {Statistical Learning Theory},
	Year = {1998}}

@book{Venables&Ripley99,
	Author = {W. N. Venables and B. D. Ripley},
	Edition = {3rd},
	Publisher = {Springer},
	Title = {Modern applied statistics with S-PLUS},
	Year = {1999}}

@book{Westfall&Young93,
	Author = {P. H. Westfall and S. S. Young},
	Publisher = {John Wiley \& Sons},
	Title = {Resampling-based multiple testing: {E}xamples and methods for $p$-value adjustment},
	Year = {1993}}

@incollection{Westfalletal&Zaykin&Young01,
	Author = {P. H. Westfall and D. V. Zaykin and S. S. Young},
	Booktitle = {Biostatistical Methods},
	Editor = {S. Looney},
	Pages = {143--168},
	Publisher = {Humana Press, Toloway, NJ},
	Series = {Methods in Molecular Biology},
	Title = {Multiple tests for genetic effects in association studies},
	Volume = {184},
	Year = {2001}}

@article{Westonetal2000,
	Author = {J. Weston and S. Mukherjee and O. Chappelle and M. Pontil and T. Poggio and V. Vapnik},
	Journal = {Advances in Neural Processing Systems},
	Pages = {668--674},
	Title = {Feature Selection for {SVM}s},
	Volume = {13},
	Year = {2001}}

@article{Wright92,
	Author = {S. P. Wright},
	Journal = {Biometrics},
	Number = {4},
	Pages = {1005--1013},
	Title = {Adjusted P-values for simultaneous inference},
	Volume = {48},
	Year = {1992}}

@article{Yangetal02,
	Author = {Y. H. Yang and M. J. Buckley and S. Dudoit and T. P. Speed},
	Journal = {Journal of Computational and Graphical Statistics},
	Number = {1},
	Pages = {108--136},
	Title = {Comparison of methods for image analysis on c{DNA} microarray data},
	Volume = {11},
	Year = {2002}}

@article{Yangetal02b,
	Author = {Y. H. Yang and S. Dudoit and P. Luu and D. M. Lin and V. Peng and J. Ngai and T. P. Speed},
	Journal = {Nucleic Acids Research},
	Number = {4},
	Pages = {e15},
	Title = {Normalization for c{DNA} microarray data: {A} robust composite method addressing single and multiple slide systematic variation},
	Volume = {30},
	Year = {2002}}

@inproceedings{Yangetal01,
	Address = {San Jose, CA},
	Author = {Y. H. Yang and S. Dudoit and P. Luu and T. P. Speed},
	Booktitle = {Microarrays: Optical Technologies and Informatics},
	Editor = {Michael L. Bittner and Yidong Chen and Andreas N. Dorsel and Edward R. Dougherty},
	Month = {May},
	Optorganization = {SPIE},
	Pages = {141--152},
	Publisher = {SPIE-International Society for Optical Engineering},
	Series = {Proceedings of SPIE},
	Title = {Normalization for c{DNA} microarray data},
	Volume = {4266},
	Year = {2001}}

@article{Yekutieli&Benjamini99,
	Author = {D. Yekutieli and Y. Benjamini},
	Journal = JSPI,
	Pages = {171--196},
	Title = {Resampling-based false discovery rate controlling multiple test procedures for correlated test statistics},
	Volume = {82},
	Year = {1999}}

@incollection{Youden69,
	Author = {W. J. Youden},
	Booktitle = {Precision measurement and calibration: Statistical concepts and procedures},
	Editor = {H. H. Ku},
	Month = {February},
	Pages = {146--151},
	Publisher = {National Bureau of Standards, United States Department of Commerce},
	Series = {Special Publication 300},
	Title = {Measurement agreement comparisons},
	Type = {NBS Miscelaneous Publication 248, Proceedings of the 1962 Standards Laboratory Conference},
	Volume = {1},
	Year = {1969}}

@article{Zhang93,
	Author = {Zhang, P.},
	Journal = {Annals of Statistics},
	Pages = {299-313},
	Title = {Model selection via multifold cross-validation},
	Volume = {21},
	Year = {1993}}

@article{Zhang&Carey&Gentleman02,
	Author = {J. Zhang and V. Carey and R. Gentleman},
	Journal = {Bioinformatics},
	Note = {(In press)},
	Title = {An extensible application for assembling annotation for genomic data},
	Url = {http://www.R-project.org/},
	Year = {2002},
	Bdsk-Url-1 = {http://www.R-project.org/}}

@book{Bickeletal97,
	Author = {P.J. Bickel and C.A.J. Klaassen and Y. Ritov and J. Wellner},
	Publisher = {Springer-Verlag},
	Title = {Efficient and Adaptive Estimation for Semiparametric Models},
	Year = {1997}}

@article{Bozdogan00,
	Author = {H. Bozdogan},
	Journal = {Journal of Mathematical Psychology},
	Pages = {62-91},
	Title = {Akaike's information criterion and recent developments in information complexity},
	Volume = {44},
	Year = {2000}}

@book{Breimanetal84,
	Address = {Monterey},
	Author = {L. Breiman and J. H. Friedman and R. A. Olshen and C. J. Stone},
	Publisher = {Wadsworth \& Brooks/Cole},
	Title = {Classification and Regression Trees},
	Year = {1984}}

@book{vanderlaan&Robins03,
	Author = {M.J. van der Laan and J.M. Robins},
	Publisher = {Springer, New York},
	Title = {Unified methods for censored longitudinal data and causality},
	Year = {2003}}

@manual{effsize,
	Author = {{National Reading Panel}},
	Organization = {National Institute of Child Health and Human Development, National Institutes of Health},
	Title = {Teaching Children to Read},
	Year = {1999}}

@techreport{Tibshirani&Walther&Hastie00,
	Author = {R. Tibshirani and G. Walther and T. Hastie.},
	Institution = {Department of Biostatistics, Stanford University},
	Month = {March},
	Note = {\url{http://www-stat.stanford.edu/~tibs/research.html}},
	Title = {Estimating the number of clusters in a dataset via the gap statistic},
	Year = {2000}}

@inproceedings{Gill&vanderLaan&Robins97,
	Address = {New York},
	Author = {R.D. Gill and M.J. van der Laan and J.M. Robins},
	Booktitle = {Proceedings of the First Seattle Symposium in Biostatistics},
	Editor = {D.Y. Lin and T.R. Fleming},
	Pages = {255-94},
	Publisher = {Springer Verlag},
	Title = {Coarsening at random: characterizations, conjectures and counter-examples},
	Year = {1997}}

@article{Gill&Robins01,
	Author = {Gill, R. and Robins, J.M.},
	Fjournal = {The Annals of Statistics},
	Journal = {Ann. Stat.},
	Number = {6},
	Title = {Causal inference in complex longitudinal studies: continuous case},
	Volume = {29},
	Year = {2001}}

@article{Jacobsen&Keiding95,
	Author = {M. Jacobsen and N. Keiding},
	Journal = {Annals of Statistics},
	Pages = {774-86},
	Title = {Coarsening at random in general sample spaces and random censoring in continuous time},
	Volume = {23},
	Year = {1995}}

@misc{Dudoit&Yang02,
	Author = {S. Dudoit and Y. H. Yang},
	Howpublished = {{\tt R} packages},
	Title = {Normalization and diagnostic plots for cDNA microarray data, {\tt marrayClasses}, {\tt marrayInput}, {\tt marrayNorm}, {\tt marrayPlots}},
	Url = {www.bioconductor.org},
	Year = {2002},
	Bdsk-Url-1 = {www.bioconductor.org}}

@techreport{Fraley&Raftery98,
	Author = {C. Fraley and A. E. Raftery},
	Institution = {Department of Statistics, University of Washington},
	Month = {November},
	Number = {342},
	Title = {MCLUST: Software for Model-Based Cluster Analysis},
	Year = {1998}}

@misc{Ge&Dudoit02,
	Author = {Y. Ge and S. Dudoit},
	Howpublished = {{\tt R} package},
	Title = {Multiple Testing Procedures, {\tt multtest}},
	Url = {www.bioconductor.org},
	Year = {2002},
	Bdsk-Url-1 = {www.bioconductor.org}}

@inproceedings{Robins93,
	Author = {J.M. Robins},
	Booktitle = {Proceeding of the Biopharmaceutical section},
	Organization = {American Statistical Association},
	Pages = {24-33},
	Title = {Information recovery and bias adjustment in proportional hazards regression analysis of randomized trials using surrogate markers},
	Year = {1993}}

@incollection{Robins&Rotnitzky92,
	Author = {J.M. Robins and A. Rotnitzky},
	Booktitle = {AIDS Epidemiology},
	Publisher = {Bikh\"{a}user},
	Series = {Methodological issues},
	Title = {Recovery of information and adjustment for dependent censoring using surrogate markers},
	Year = {1992}}

@article{Robins&Rotnitzky&Zhao94,
	Author = {J.M. Robins and A. Rotnitzky and L.P. Zhao},
	Journal = {Journal of the American Statistical Association},
	Month = {September},
	Number = {427},
	Pages = {846-866},
	Title = {Estimation of regression coefficients when some regressors are not always observed},
	Volume = {89},
	Year = {1994}}

@article{Heitjan&Rubin91,
	Author = {D.F. Heitjan and D.B. Rubin},
	Journal = {Annals of statistics},
	Month = {December},
	Number = {4},
	Pages = {2244-2253},
	Title = {Ignorability and coarse data},
	Volume = {19},
	Year = {1991}}

@misc{Dudoit&Yang&Bolstad01,
	Author = {S. Dudoit and Y. H. Yang and B. M. Bolstad},
	Howpublished = {{\tt R} package},
	Note = {Contributions from Natalie Thorne, Ingrid L\"{o}nnstedt, and Jessica Mar},
	Title = {Statistical {M}icroarray {A}nalysis, {\tt sma}},
	Url = {cran.r-project.org/src/contrib/PACKAGES.html\#sma},
	Year = {2001},
	Bdsk-Url-1 = {cran.r-project.org/src/contrib/PACKAGES.html%5C#sma}}

@phdthesis{Dudoit99,
	Author = {S. Dudoit},
	School = {Department of Statistics, University of California, Berkeley},
	Title = {Linkage analysis of complex human traits using identity by descent data},
	Type = {Ph.D. thesis},
	Year = {1999}}

@book{vanderVaart&Wellner96,
	Author = {A. van der Vaart and J. Wellner},
	Publisher = {Springer-Verlag, New York},
	Title = {Weak Convergence and Empirical Processes},
	Year = {1996}}

@book{Robert07,
	Address = {New York},
	Author = {Robert, P. C.},
	Publisher = {Springer},
	Title = {{T}he {B}ayesian {C}hoice: {F}rom {D}ecision-{T}hoeretic {F}oundations to {C}omputational {I}mplementation},
	Year = {2007}}

@book{Lindley80,
	Address = {Cambridge},
	Author = {Lindley, D. V.},
	Publisher = {Cambridge University Press},
	Title = {{I}ntroduction to {P}robability and {S}tatistics from a {B}ayesian {P}oint of {V}iew, Part 2},
	Year = {1965}}

@article{Tager&Hollenberg&Satariano98,
	Author = {I.B. Tager and M. Hollenberg and W. Satariano},
	Publisher = {American Journal of Epidemiology},
	Title = {Self-reported leisure-time physical activity and measures of cardiorespiratory fitness in an elderly population},
	Year = {1998}}

@techreport{Hubbard&vanderLaan05,
	Author = {A.E. Hubbard and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper191},
	Title = {Population Intervention Models in Causal Inference},
	Type = {Technical Report 191},
	Year = {2005}}

@manual{Ghalanos&Theussl10,
	Author = {A. Ghalanos and S. Theussl},
	Title = {Rsolnp: General Non-linear Optimization Using Augmented Lagrange Multiplier Method. R package},
	Year = {2010}}

@phdthesis{Ye87,
	Author = {Yinyu Ye},
	School = {Department of EES, Stanford University},
	Title = {Interior Algorithms for Linear, Quadratic, and Linearly Constrained Non-Linear Programming},
	Year = {1987}}

@book{vanderLaan&Rose11,
	Address = {New York},
	Author = {M.J. van der Laan and S. Rose},
	Publisher = {Springer},
	Title = {Targeted Learning: Causal Inference for Observational and Experimental Data},
	Year = {2011}}

@book{Kullback59,
	Author = {S. Kullback},
	year = {1959},
	Title = {Information Theory and Statistics},
	Publisher = {John Wiley \& Sons}
	Address = {New York}
}

@incollection {vandervaart02,
   author = {van der Vaart, Aad},
   title = {Semiparameric Statistics},
   booktitle = {Lectures on Probability Theory and Statistics},
   series = {Lecture Notes in Mathematics},
   publisher = {Springer Berlin / Heidelberg},
   keyword = {Mathematics and Statistics},
   pages = {331-457},
   volume = {1781},
   note = {},
   year = {2002}
}

%A. Donner and N. Klar. Design and Analysis of Cluster Randomization Trials in Health Research. Arnold, London, 2000.
%R.J. Hayes and L.H. Moulton. Cluster randomised trials. Chapman & Hall/CRC, Boca Raton, 2009.
%MJ Campbell, A. Donner, and N. Klar. Developments in cluster randomized trials and Statistics in Medicine. Statistics in Medicine, 26(1):2Ð19, 2007. doi: 10.1002/sim.2731.

@article{Robins&Ritov97,
title={Towards a curse of dimensionality appropriate asymptotic theory for semi parametric models},
author={J.M. Robins and Y. Ritov},
year={1997},
journal={Statistics in Medicine},
volume={16},
pages={285--319},
}

@article{vanderLaan&Gruber15,
title={One-step targeted minimum loss-based estimation based on universal least favorable one-dimensional submodels},
author={M.J. van der Laan and S. Gruber},
year={2015},
journal={to appear in International Journal of Biostatistics},
volume={},
pages={},
}


@article{Neuhaus71,
title={On weak convergence of stochastic processes with multidimensional time parameter},
author={G. Neuhaus},
year={1971},
journal={Annals of Statistics},
volume={42},
pages={1285--1295},
}


@article{vanderVaart&Wellner11,
title={A local maximal inequality under uniform entropy},
author={A.W. van der Vaart and J.A. Wellner},
year={2011},
journal={Electronic Journal of Statistics},
volume={5},
pages={192--203},
note={ISSN: 1935-7524, DOI: 10.1214/11-EJS605},
}


@article{Porteretal11,
title={The relative performance of targeted maximum likelihood estimators},
author={K.E. Porter and S. Gruber and M. J. van der Laan and J. S. Sekhon},
year= {2011},
journal={Int J Biostat.},
volume={Jan 1, 2011; 7(1): Article 31.},
note={Published online Aug 17, 2011. doi:  10.2202/1557-4679.1308. Also available at: U.C. Berkeley Division of Biostatistics Working Paper Series. Working Paper 279, http://www.bepress.com/ucbbiostat/paper279},
}

@incollection{Sekhonetal12,
	Address = {New York Dordrecht Heidelberg London},
	Author = {J.S. Sekhon and S. Gruber and K.E. Porter and M.J. van der Laan},
	Booktitle = {Targeted Learning: Causal Inference for Observational and Experimental Data},
	Date-Added = {2012-08-24 11:01:37 -0700},
	Date-Modified = {2012-08-24 11:02:54 -0700},
	Editor = {van der Laan, M.J. and Rose, S.},
	Keywords = {Chpt3},
	Publisher = {Springer},
	Title = {Propensity score-based estimators and C-TMLE},
	Year = {2012}}


@incollection{Robinsetal08,
year={2008},
isbn={DOI:
10.1214/1939403070000005, arXiv:0805.3040v1},
booktitle={Essays in Honor of David A. Freedman
},
series={IMS, Collections Probability and Statistics},
title={Higher order influence functions and minimax estimation of non-linear functionals},
publisher={Springer New York},
author={J.M. Robins and L. Li and E. Tchetgen and A.W. van der Vaart},
pages={335-421},
language={English}
}

@techreport{vanderLaan15,
  author =        {M.J. van der Laan},
  institution =   {UC Berkeley},
number={300},
  title =         {A generally efficient targeted minimum loss-based estimator },
  year =          {2015},
  note ={http://biostats.bepress.com/ucbbiostat/paper343, 2015}
}

@techreport{vanderLaan12network,
  author =        {M.J. van der Laan},
  institution =   {UC Berkeley},
number={300},
  title =         {Causal Inference for Networks},
  year =          {2012},
  note ={http://biostats.bepress.com/ucbbiostat/paper300,to appear in Journal of Causal Inference}
}

@techreport{vanderLaanetal13,
  author =        {M.J. van der Laan and A.E. Hubbard and S. Kherad},
  institution =   {UC Berkeley},
number={314},
  title =         {Statistical Inference for Data Adaptive Target Parameters},
  year =          {June 2013},
  note ={http://biostats.bepress.com/ucbbiostat/paper314, Revised for Biometrics}
}

@techreport{vanderLaan13,
  author =        {M.J. van der Laan},
  institution =   {UC Berkeley},
number={317},
  title =         {Targeted Learning of an Optimal Dynamic Treatment and Statistical Inference for its Mean Outcome},
  year =          {2013},
  note ={http://biostats.bepress.com/ucbbiostat/paper317, to appear in Journal of Causal Inference}
}



@techreport{Balzer@vanderLaan13,
  author =        {L. Balzer and M.J. van der Laan},
  institution =   {UC Berkeley},
number={310},
  title =         {Estimating effects on rare outcomes: Knowledge is Power},
  year =          {2013},
  note ={Revised for Biometrics}
}


@article{Schnitzeretal13,
title = {Targeted minimum loss based estimator that outperforms a given estimator},
author = {M. Schnitzer,   E. Moodie, M.J. van der Laan, R. Platt, M. Klei3},
year = {2013},
journal = {to appear in Biometrics
},
volume = {},
number = {},
pages = {http://biostats.bepress.com/ucbbiostat/paper304},
}

@article{Rotnitzkyetal12,
title = {Improved double-robust estimation in missing data and causal inference models},
author = {A. Rotnitzky and Q. Lei and M. Sued and J. M. Robins},
year = {2012},
journal = {Biometrika},
volume = {99},
number = {2},
pages = {439--456, doi:  10.1093/biomet/ass013},
}

@article{Gruber&vanderLaan12,
title = {Targeted minimum loss based estimator that outperforms a given estimator},
author = {S. Gruber and M.J. van der Laan},
year = {2012},
journal = {The International Journal of Biostatistics},
volume = {8},
number = {1},
pages = {Article 11, doi: 10.1515/1557-4679.1332},
}

@techreport{Sapp&vanderLaan13,
  author =        {S. Sapp and M.J. van der Laan and K. Page},
  institution =   {UC Berkeley},
number={307},
  title =         {Targeted Estimation of Variable Importance Measures with Interval-Censored Outcomes},
  year =          {2013},
  note ={Submitted to IJB}
}


@techreport{Neugebaueretal13,
  author =        {R. Neugebauer and J.A. Schmittdiel and M.J. van der Laan},
  institution =   {The Agency for Healthcare Research and Quality},
number={No. HHSA29020050016I},
  title =         {Targeted Learning in real-world comparative effectiveness research with time-varying interventions},
  year =          {2013},
  note ={http://diabetestranslation.org/en/news_publications/Reports}
}


@article{Diaz11,
title = {Super Learner Based Conditional Density Estimation with Application to Marginal Structural Models},
author = {D\'iaz, Iv\'an and van der Laan, Mark},
year = {2011},
journal = {The International Journal of Biostatistics},
volume = {7},
number = {1},
pages = {38},
}

@article {Diaz12,
author = {Iv\'an D\'iaz and van der Laan, Mark},
title = {Population Intervention Causal Effects Based on Stochastic Interventions},
journal = {Biometrics},
volume = {68},
number = {2},
publisher = {Blackwell Publishing Inc},
issn = {1541-0420},
pages = {541--549},
keywords = {Causal effect, Counterfactual outcome, Double robustness, Stochastic intervention, Targeted maximum likelihood estimation},
year = {2012},
}

@article{Diaz13a,
title={Sensitivity Analysis for Causal Inference Under Unmeasured Confounding and Measurement Error Problems},
author={D{\'\i}az, Iv{\'a}n and van der Laan, Mark J},
year= {{2013}, In press},
journal={International Journal of Biostatistics}
}

@article{Diaz13b,
title={Assessing the Causal Effect of Policies: An Example Using Stochastic Interventions},
author={D{\'\i}az, Iv{\'a}n and van der Laan, Mark J},
year= {{2013}, In press},
journal={International Journal of Biostatistics}
}

@incollection{Starmans11,
year={2011},
isbn={978-1-4419-9781-4},
booktitle={Targeted Learning},
series={Springer Series in Statistics},
title={Models, Inference, and Truth},
publisher={Springer New York},
author={R. Starmans},
pages={1-20},
language={English}
}
@incollection{Diaz11a,
year={2011},
isbn={978-1-4419-9781-4},
booktitle={Targeted Learning},
series={Springer Series in Statistics},
title={Targeted Bayesian Learning},
publisher={Springer New York},
author={Iv\'an D\'iaz and Hubbard, Alan E. and van der Laan, Mark J.},
pages={475--493},
language={English}
}



@article{Diaz13c,
title={Targeted Data Adaptive Estimation of the Causal Dose Response Curve},
author={D{\'\i}az, I. and van der Laan, M. J.},
year= {2013},
journal={Journal of Causal Inference},
Volume={1 (2)},
pages={171--192}
}

@article{ndeu,
  title={Identification and efficient estimation of the natural direct effect among the untreated},
  author={Lendle, Samuel D and Subbaraman, Meenakshi S and van der Laan, Mark J},
  journal={Biometrics},
  pages={1--8},
  year={2013},
  publisher={Wiley Online Library}
}

@article{tmle_safety,
  title={Targeted maximum likelihood estimation in safety analysis},
  author={Lendle, Samuel D and Fireman, Bruce and van der Laan, Mark J},
  journal={Journal of clinical epidemiology},
  volume={66},
  number={8},
  pages={S91--S98},
  year={2013},
  publisher={Elsevier}
}

@article{subbaraman2013cravings,
  title={Cravings as a mediator and moderator of drinking outcomes in the COMBINE study},
  author={Subbaraman, Meenakshi Sabina and Lendle, Samuel and Laan, Mark and Kaskutas, Lee Ann and Ahern, Jennifer},
  journal={Addiction},
  year={2013},
  publisher={Wiley Online Library}
}

@article{bsatmle,
  title={Balancing Score Adjusted Targeted Minimum Loss-based Estimation},
  author={Lendle, Samuel D and Fireman, Bruce and van der Laan, Mark J},
  year={2013},
  publisher={bepress}
}
@article{brooks2013,
author = "Jordan Brooks and Mark J {van der Laan} and Daniel E Singer and Alan S Go",
institution = "Division of Biostatistics, University of California",
title = "Targeted Minimum Loss-Based Estimation of Causal Effects in Right-Censored Survival Data with Time-Dependent Covariates: Warfarin, Stroke, and Death in Atrial Fibrillation",
journal = {Journal of Causal Inference},
year = {2013},
volume = {1},
issue	 = {2},
page = {235-254},
doi = {10.1515/jci-2013-0001}
}

@article{brooks2012,
author = "Jordan Brooks and Mark J {van der Laan} and Alan S Go",
institution = "Division of Biostatistics, University of California",
title = "Targeted Maximum Likelihood Estimation for Prediction Calibration",
journal = {International Journal of Biostatistics},
year = "2012"
volume = {8},
issue	 = {1},
article = {30},
doi = {10.1515/1557-4679.1385}
}@techreport{Chambazetal13,
  author =        {A. Chambaz and N. Pierre and M.J. van der Laan},
  institution =   {UC Berkeley},
number={292},
  title =         {Estimation of a Non-Parametric Variable Importance Measure of a Continuous Exposure},
  year =          {2013},
  note ={to appear in Electronic Journal of Applied Statistics}
}




@techreport{Aronow&Samii13,
  author =        {P.M. Aronow and C. Samii},
  institution =   {Yale University and New York University},
number={},
  title =         {Estimating average causal effects under general interference},
  year =          {2013},
  note ={Unpublished manuscript}
}



@book{Carringtonetal05,
  address =       {},
  author =        {P.J. Carrington and J. Scott and S. Wasserman},
  edition =       {},
  publisher =     {Cambridge University Press},
  title =         {Models and Methods in Social Network Analysis (Structural Analysis in the Social Sciences)},
  year =          {2005},
}



@article{Bakshyetal12,
	Author = {E. Bakshy and D. Eckles and R. Yan and I. Rosenn},
	Journal = {EC 2012: Proceedings of the ACM Conference on Electronic Commerce},
	Month = {},
	Volume={ACM. http://arxiv.org/abs/1206.4327},
	Title = {Social influence in social advertising: Evidence from field experiments},
	Year = {2012}
}

@article{Airoldietal13,
	Author = {E. M. Airoldi and P. Toulis and E. Kao and D.B. Rubin},
	Journal = {Proceedings of the 30 th International Conference on Ma-
chine Learning, Atlanta, Georgia, USA, 2013},
	Month = {},
	Volume={JMLR: W\&CP volume 28},
	Title = {Estimation of causal peer influence effects},
	Year = {2013}
}


@article{Gruber&vanderLaan12a,
	Author = {S. Gruber and M.J. van der Laan},
	Journal = {Statistical Methods in Medical Research},
	Month = {February},
	Title = {Consistent causal effect estimation under dual misspecification and implications for confounder selection procedure},
	Year = {2012}
}
@article{vanderLaan&Balzer&Petersen13,
	Author = {M.J. van der Laan and L.B. Balzer and M.L. Petersen},
	Journal = {Journal of Statistical Research},
	Month = {},
	Pages={113-156},
	Volume={46(2)},
	Title = {Adaptive Matching in Randomized Trials and Observational Studies},
	Year = {2013}
}


@incollection{vanderLaan&Petersen12,
	Author = {M.J. van der Laan and M.L. Petersen},
	Booktitle = {Ensemble Machine Learning},
	Chapter = {pages 117--156, ISBN 978-1-4419-9326-7},
	Publisher = {Springer, New York},
	Title = {Targeted Learning},
	Year = {2012}}


@incollection{Zheng&vanderLaan11,
	Author = {W. Zheng and M.J. van der Laan},
	Booktitle = {{\rm M.J. van der Laan and S. Rose, } Targeted Learning:Causal Inference for Observational and Experimental Data},
	Chapter = {21},
	pages={459-474},
	Publisher = {Springer, New York},
	Title = {Cross-validated Targeted Minimum Loss Based Estimation},
	Year = {2011}}

@incollection{Wang&Rose&vanderLaan11,
	Author = {H. Wang and S. Rose and M.J. van der Laan},
	Booktitle = {{\rm M.J. van der Laan and S. Rose, } Targeted Learning:Causal Inference for Observational and Experimental Data},
	Chapter = {23},
	Publisher = {Springer, New York},
	Title = {Finding Quantitative Trait Loci Genes},
	Year = {2011}}

	@incollection{Tuglus&vanderLaan11,
	Author = {C. Tuglus and M.J. van der Laan},
	Booktitle = {{\rm M.J. van der Laan and S. Rose, } Targeted Learning:Causal Inference for Observational and Experimental Data},
	Chapter = {22},
	Publisher = {Springer, New York},
	Title = {Targeted Methods for Biomarker Discoveries},
	Year = {2011}}

@incollection{Polley&Rose&vanderLaan11,
	Author = {E.C. Polley and S. Rose and M.J. van der Laan},
	Booktitle = {{\rm M.J. van der Laan and S. Rose, } Targeted Learning:Causal Inference for Observational and Experimental Data},
	Chapter = {3},
	Publisher = {Springer, New York},
	Title = {Super Learning},
	Year = {2011}}

@book{vanderLaan96b,
  address =       {Amsterdam},
  author =        {M.J. van der Laan},
  edition =       {CWI tract 114},
  publisher =     {Centre of Computer Science and Mathematics},
  title =         {Efficient and Inefficient Estimation in Semiparametric Models},
  year =          {1996},
}
@book{Donner&Klar00,
  address =       {London},
  author =        {A. Donner and N. Klar},
  edition =       {},
  publisher =     {Arnold},
  title =         {Design and Analysis of Cluster Randomization Trials in Health Research},
  year =          {2000},
}

@book{Hayes&Moulton09,
  address =       {Boca Raton},
  author =        {R.J. Hayes and L.H. Moulton},
  edition =       {},
  publisher =     {Chapman \& Hall/CRC},
  title =         {Cluster Randomized Trials},
  year =          {2009},
}
@book{vanderLaan&Rose12,
  address =       {New York},
  author =        {M.J. van der Laan and S. Rose},
  edition =       {},
  publisher =     {Springer},
  title =         {Targeted Learning: Causal Inference for Observational and Experimental Data},
  year =          {2012},
}
@book{Murray98,
  address =       {Oxford},
  author =        {D.M. Murray},
  edition =       {},
  publisher =     {Oxford University Press},
  title =         {Design and Analysis of Community Randomized Trials},
  year =          {1998},
}
 @article{Campbelletal07,
  author =        {M.J. Campbell and A. Donner and N. Klar},
  journal =       {Statistics in Medicine},
  pages =         {2--19, doi: 10.1002/sim.2731},
  title =         {Developments in cluster randomized trials and statistics in medicine},
  volume =        {26},
  year =          {2007},
}
 @article{Klar&Donner97,
  author =        {N. Klar and A. Donner},
  journal =       {Statistics in Medicine},
  pages =         {1753--1764},
  title =         {The merits of matching in community intervention trials: a cautionary tale},
  volume =        {16(15)},
  year =          {1997},
}


 @article{Raudenbush&Martinez&Spybrook07,
  author =        {S.W. Raudenbush and A. Martinez and J. Spybrook},
  journal =       {Educational Evaluation and Policy Analysis},
  pages =         {5--29},
  title =         {Developments in cluster randomized trials and statistics in medicine},
  volume =        {29},
  year =          {2007},
}

@article{Freedman&Green&Byar90,
  author =        {L.S. Freedman and S.B. Green and D.P. Byar},
  journal =       {Statistics in Medicine},
  pages =         {943--952},
  title =         {Assessing the gain in efficiency due to matching in a community intervention study},
  volume =        {9},
  year =          {1990},
}
@article{Gill&vanderLaan&Wellner95,
  author =        {R.D. Gill and M.J. van der Laan and J.A. Wellner},
  journal =       {Annales de l'Institut Henri Poincar{\'e}},
  pages =         {545--597},
  title =         {Inefficient estimators of the bivariate survival function for three models},
  volume =        {31},
  year =          {1995},
}
@article{Freedmanetal97,
  author =        {L. Freedman and M. Gail and S. Green and D. Corle},
  journal =       {Controlled clinical trials},
  pages =         {131--139, doi:10.1016/S0197-2456(96)00115-8},
  title =         {The efficiency of the matched-pairs design of the community intervention trial for smoking cessation (COMMIT)},
  volume =        {18(2)},
  year =          {1997},
}

@article{Toftageretal11,
  author =        {M. Toftager and L.B. Christiansen and P.L. Kristensen and J. Troelsen},
  journal =       {BMC Public Health},
  pages =         {711--777},
  title =         {SPACE for physical activity-a multicomponent intervention study: study design and baseline findings from a cluster randomized controlled trial},
  volume =        {10},
  year =          {2011},
}

@article{Koetheetal10,
  author =        {J.R. Koethe and A.O. Westfall and D.K. Luhanga and G.M. Clark and J.D. Goldman and P.L Mulenga and R.A. Cantrell and B.H. Chi and I. Zulu and M.S. Saag and J. S. Stringer},
  journal =       {PlLoS One},
  pages =         {5(3):e9680},
  title =         {A cluster randomized trial of routine HIV-1 viral load monitoring in Zambia},
  volume =        {5},
  year =          {2010},
}

@article{Watsonetal04,
  author =        {L. Watson and R. Small and S. Brown and W. Dawson and J. Lumley},
  journal =       {Journal of Controlled Clinical Trials},
  pages =         {235--250},
  title =         {Mounting a community-randomized trial: sample size, matching, selection, and randomization issues in PRISM},
  volume =        {3},
  year =          {2004},
}

@article{Gailetal92,
  author =        {M.H. Gail and D.P. Byar and T.F. Pechacek and D.K. Corle},
  journal =       {Controlled clinical trials},
  pages =         {6-21},
  title =         {Aspects of statistical design for the community intervention trial for smoking cessation},
  volume =        {13},
  year =          {1992},
}

@article{Commit91,
  author =        {COMMIT Research Group},
  journal =       {Journal of National Cancer Institute},
  pages =         {1620-1628},
  title =         {Summary of design and intervention},
  volume =        {83(22)},
  year =          {1991},
}

 @article{Imai&King&Nall09,
  author =        {Kosuke Imai and G. King and C. Nall},
  journal =       {Statistical Science},
  pages =         {29--53},
  title =         {The essential role of pair matching in cluster randomized experiments with applicationto the Mexican Universal Health Insurance Evaluation},
  volume =        {24 (1)},
  year =          {2009},
}


@article{Imai08,
  author =        {K. Imai},
  journal =       {Statistics in Medicine},
  pages =         {4857--4873},
  title =         {Variance identification and efficiency analysis in randomized experiments under the matched-pair design},
  volume =        {27(24)},
  year =          {2008},
}



@techreport{vanderLaan&Gruber11,
  author =        {M.J. van der Laan and S. Gruber},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
number={290},
  title =         {Targeted Minimum Loss Based Estimation of an Intervention Specific Mean Outcome},
  year =          {2011},
  note ={To appear  in IJB, also technical report http://www.bepress.com/ucbbiostat/paper290 }
}

@techreport{vanderLaan08,
  author =        {M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
number={232},
  title =         {The construction and analysis of adaptive group sequential designs},
  year =          {2008},
  note ={http://www.bepress.com/ucbbiostat/paper234 }
}


@techreport{Balzer&Petersen&vanderLaan12,
  author =        {L.B. Balzer and M.L. Petersen and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
number={294},
  title =         {Why match in individually and cluster randomized trials},
  year =          {2012},
  note ={To appear  in Statistics in Medicine, also technical report http://www.bepress.com/ucbbiostat/paper294}
}



@incollection{Marschak53,
  address =       {New York},
  author =        {J. Marschak},
  booktitle =     {Economic measurements for policy and prediction},
  editor =        {W.~C. Hood and T.~C. Koopmans},
  publisher =     {Wiley},
  title =         {Studies in econometric method},
  year =          {1953},
}

@article{Heckman00,
  author =        {J. Heckman},
  journal =       {Q J Econ},
  pages =         {45--97},
  title =         {Causal parameters and policy analysis in economics:
                   A twentieth century retrospective.},
  volume =        {115},
  year =          {2000},
}

@article{Gruber&vanderLaan10,
  author =        {S. Gruber and M.J. van der Laan},
  journal =       {International Journal of Biostatistics},
  pages =         {article 26, www.bepress.com/ijb/vol6/iss1/26},
  title =         {A Targeted Maximum Likelihood Estimator of a Causal Effect on a Bounded Continuous Outcome},
  volume =        {6},
  year =          {2010},
}




@article{Heckman10,
  author =        {J. Heckman},
  journal =       {J Econ Lit},
  pages =         {356--398},
  title =         {Building bridges between structural and program
                   evaluation approaches to evaluating policy.},
  volume =        {48},
  year =          {2010},
}

@article{Bang&Robins05,
author={H. Bang and J.M. Robins},
 journal =       {Biometrics},
  pages =         {962--972},
  title =         {Doubly robust estimation in missing data and causal inference models},
  volume =        {61},
  year =          {2005},
}



@book{Pearson11,
  address =       {London},
  author =        {K. Pearson},
  edition =       {3rd},
  publisher =     {Black},
  title =         {Grammar of science},
  year =          {1911},
}

@article{Rubin74,
  author =        {Donald B. Rubin},
  journal =       {J Educ Psychol},
  number =        {},
  pages =         {688--701},
  title =         {Estimating causal effects of treatments in randomized
                   and nonrandomized studies.},
  volume =        {66},
  year =          {1974},
}

@article{Neyman23,
  author =        {J. Neyman},
  journal =       {Stat Sci},
  number =        {},
  pages =         {465--480},
  title =         {Sur les applications de la theorie des probabilites
                   aux experiences agricoles: Essai des principes ({In
                   Polish}). {E}nglish translation by {D.M.} {D}abrowska and
                   {T.P.} {S}peed (1990)},
  volume =        {5},
  year =          {1923},
}

@book{Pearl09,
  address =       {New York},
  author =        {J. Pearl},
  edition =       {2nd},
  publisher =     {Cambridge},
  title =         {Causality: models, reasoning, and inference},
  year =          {2009},
}

@article{Pearl95,
  author =        {J. Pearl},
  journal =       {Biometrika},
  pages =         {669--710},
  title =         {Causal diagrams for empirical research.},
  volume =        {82},
  year =          {1995},
}

@article{Robins&Greenland92,
  author =        {J.M. Robins and S. Greenland},
  journal =       {Epidemiol},
  pages =         {143--155},
  title =         {Identifiability and exchangeability for direct and
                   indirect effects},
  volume =        {3},
  year =          {1992},
}

@inproceedings{Pearl01b,
  address =       {San Francisco},
  author =        {J. Pearl},
  booktitle =     {Uncertainty in artificial intelligence, Proceedings
                   of the 17th Conference},
  publisher =     {Morgan Kaufmann},
  title =         {Direct and indirect effects.},
  year =          {2001},
}

@article{Baron&Kenny86,
  author =        {R. Baron and D. Kenny},
  journal =       {J Personal Soc Psychol},
  pages =         {1173--1182},
  title =         {The moderator-mediator variable distinction in social
                   psychological research: conceptual, strategic, and
                   statistical considerations.},
  volume =        {51},
  year =          {1986},
}

@book{MacKinnon08,
  address =       {New York},
  author =        {D. {MacKinnon}},
  publisher =     {Erlbaum},
  title =         {Introduction to statistical mediation analysis},
  year =          {2008},
}

@article{MacKinnonetal07,
  author =        {D. {MacKinnon} and C. Lockwood and C. Brown and
                   W. Wang and J. Hoffman},
  journal =       {Clin Trials},
  pages =         {499--513},
  title =         {The intermediate endpoint effect in logistic and
                   probit regression.},
  volume =        {4},
  year =          {2007},
}

@incollection{Pearl10c,
  address =       {},
  author =        {J. Pearl},
  booktitle =     {Statistical causality},
  editor =        {C. Berzuini and P. Dawid and L. Bernardinelli},
  publisher =     {},
  title =         {The mediation formula: a guide to the assessment of
                   causal pathways in nonlinear models.},
  year =          {forthcoming 2011},
}

@article{Pearl10b,
  author =        {J. Pearl},
  journal =       {Int J Biostat},
  pages =         {Article 7},
  title =         {An introduction to causal inference},
  volume =        {6},
  number={2},
  year =          {2010},
}

@article{vanderLaan&Rose10,
  author =        {M.J. van der Laan and S. Rose},
  journal =       {Amstat News},
  pages =         {38--39},
  title =         {Statistics Ready for a Revolution: next Generation of
                   Statisticians Must Build Tools for Massive Data Sets},
  volume =        {399},
  year =          {2010},
}

@techreport{vanderLaan&Dudoit03,
  author =        {M.J. van der Laan and S. Dudoit},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
number={130},
  title =         {Unified cross-validation methodology for selection
                   among estimators and a general cross-validated
                   adaptive epsilon-net estimator: finite sample oracle
                   inequalities and examples},
  year =          {2003},
}




@book{vanderLaan&Robins03,
  author =        {M.J. van der Laan and J.M. Robins},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  title =         {Unified methods for censored longitudinal data and
                   causality},
  year =          {2003},
}

@book{vanderLaan&Rose11,
  author =        {M.J. van der Laan and S. Rose},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  title =         {Targeted Learning: Causal Inference for Observational and Experimental Data},
  year =          {2011},
}
@book{Bickeletal97,
  author =        {P.J. Bickel and C.A.J. Klaassen and Y. Ritov and
                   J. Wellner},
  publisher =     {Springer},
  address={Berlin Heidelberg New York},
  title =         {Efficient and adaptive estimation for semiparametric
                   models},
  year =          {1997},
}

@article{vanderLaan&Rubin06,
  author =        {M.J. van der Laan and Daniel B. Rubin},
  journal =       {Int J Biostat},
  number =        {1},
  pages =         {Article 11},
  title =         {Targeted Maximum Likelihood Learning},
  volume =        {2},
  year =          {2006},
}

@article{Stitelman&vanderLaan11a,
  author =        {O.M. Stitelman and M.J. van der Laan},
  journal =       {Int J Biostat},
  number =        {1},
  title =         {Targeted Maximum Likelihood Estimation of Effect Modification Parameters In Survival Analysis},
  volume =        {7},
  year =          {2011},
}






@article{vanderLaan&Gruber10,
  author =        {M.J. van der Laan and S. Gruber},
  journal =       {Int J Biostat},
  number =        {1},
  title =         {Collaborative Double robust penalized targeted
                   maximum likelihood estimation},
  volume =        {6},
  year =          {2010},
}

@article{Taubes07,
  author =        {G. Taubes},
  journal =       {The New York Times},
  title =         {{Do we really know what makes us healthy?}},
  year =          {2007},
}

@article{USPrev09,
  author =        {{U.S. Preventive Services Task Force}},
  journal =       {Ann Intern Med},
  number =        {10},
  pages =         {716--726},
  title =         {{Screening for breast cancer: U.S. Preventive
                   Services Task Force recommendation statement}},
  volume =        {151},
  year =          {2009},
}

@article{Freedman&Petitti&Robins04,
  author =        {D.A. Freedman and D.B. Petitti and J.M. Robins},
  journal =       {Int J Epidemiol},
  pages =         {43--55},
  title =         {{On the efficacy of screening for breast cancer}},
  volume =        {33},
  year =          {2004},
}

@book{Rothman&Greenland98,
  address =       {Philadelphia},
  author =        {K.J. Rothman and S. Greenland},
  edition =       {2nd},
  publisher =     {Lippincott, Williams \& Wilkins},
  title =         {Modern epidemiology},
  year =          {1998},
}

@book{Jewell04,
  address =       {Boca Raton},
  author =        {N.P. Jewell},
  publisher =     {Chapman \& Hall},
  title =         {Statistics for epidemiology},
  year =          {2004},
}

@book{Freedman05,
  address =       {New York},
  author =        {D.A. Freedman},
  publisher =     {Cambridge},
  title =         {Statistical models: theory and practice},
  year =          {2005},
}

@article{Ioannidis06,
  author =        {J.P.A. Ioannidis},
  journal =       {Neonatal Intensive Care J Perinatol Neonatol},
  number =        {3},
  title =         {{Why most published research findings are false}},
  volume =        {19},
  year =          {2006},
}

@book{Freedman10,
  address =       {New York},
  author =        {D.H. Freedman},
  publisher =     {Little, Brown and Company},
  title =         {Wrong: why experts keep failing us---and how to know
                   when not to trust them},
  year =          {2010},
}

@book{Box&Draper87,
  address =       {Hoboken},
  author =        {G.E.P. Box and N.R. Draper},
  publisher =     {Wiley},
  title =         {Empirical model-building and response surfaces},
  year =          {1987},
}

@article{Robins86,
  author =        {J.M. Robins},
  journal =       {Math Mod},
  number =        {},
  pages =         {1393--1512},
  title =         {A new approach to causal inference in mortality
                   studies with sustained exposure periods--application
                   to control of the healthy worker survivor effect},
  volume =        {7},
  year =          {1986},
}

@article{Tager&Hollenberg&Satariano98,
  author =        {I. Tager and M. Hollenberg and W. Satariano},
  journal =       {Am J Epidemiol},
  pages =         {921--931},
  title =         {{Self-reported leisure-time physical activity and
                   measures of cardiorespiratory fitness in an elderly
                   population}},
  volume =        {147},
  year =          {1998},
}

@manual{RCore,
  address =       {Vienna},
  author =        {{R Development Core Team}},
  organization =  {R Foundation for Statistical Computing},
  title =         {R: a language and environment for statistical
                   computing},
  year =          {2010},
  url =           {http://www.R-project.org},
}

@article{liaw:2002,
  author =        {A. Liaw and M. Wiener},
  journal =       {R News},
  number =        {3},
  pages =         {18--22},
  title =         {Classification and Regression by randomForest},
  volume =        {2},
  year =          {2002},
  url =           {http://CRAN.R-project.org/package=randomForest},
}

@article{randomForests,
  author =        {L. Breiman},
  journal =       {Mach Learn},
  pages =         {5--32},
  title =         {Random Forests},
  volume =        {45},
  year =          {2001},
}

@manual{ipred,
  author =        {A. Peters and T. Hothorn},
  note =          {R package version 0.8-8},
  title =         {ipred: Improved Predictors},
  year =          {2009},
  url =           {http://CRAN.R-project.org/package=ipred},
}

@article{breiman96bagging,
  author =        {L. Breiman},
  journal =       {Mach Learn},
  number =        {2},
  pages =         {123--140},
  title =         {Bagging Predictors},
  volume =        {24},
  year =          {1996},
}

@incollection{gam:1992,
  author =        {T.J. Hastie},
  booktitle =     {Statistical models in {S}},
  editor =        {J.M. Chambers and T.J. Hastie},
  publisher =     {Chapman \& Hall},
  title =         {Generalized additive models},
      address =       {Boca Raton},
  year =          {1992},
}

@book{gams,
  author =        {T.J. Hastie and R.J. Tibshirani},
  publisher =     {Chapman \& Hall},
  title =         {Generalized additive models},
  year =          {1990},
    address =       {Boca Raton},
}

@manual{gbm,
  author =        {G. Ridgeway},
  note =          {R package version 1.6-3},
  title =         {gbm: generalized boosted regression models},
  year =          {2007},
}

@article{friedman:2001,
  author =        {J.H. Friedman},
  journal =       {Ann Stat},
  pages =         {1189-1232},
  title =         {Greedy Function Approximation: a Gradient Boosting
                   Machine},
  volume =        {29},
  year =          {2001},
}

@book{MASS,
  address={Berlin Heidelberg New York},
  author =        {W.N. Venables and B.D. Ripley},
  edition =       {4th},
  publisher =     {Springer},
  title =         {Modern applied statistics with S},
  year =          {2002},
}

@manual{polspline,
  author =        {C. Kooperberg},
  note =          {R package version 1.1.4},
  title =         {polspline: Polynomial spline routines},
  year =          {2009},
  url =           {http://CRAN.R-project.org/package=polspline},
}

@article{MARS,
  author =        {J.H. Friedman},
  journal =       {Ann Stat},
  number =        {1},
  pages =         {1--141},
  title =         {Multivariate Adaptive Regression Splines},
  volume =        {19},
  year =          {1991},
}

@manual{bart,
  author =        {H.A. Chipman and R.E. McCulloch},
  note =          {R package version 0.3-1},
  title =         {BayesTree: {B}ayesian methods for tree-based models},
  year =          {2009},
  url =           {http://CRAN.R-project.org/package=BayesTree},
}

@article{chipman:2009,
  author =        {H.A. Chipman and E.I. George and R.E. McCulloch},
  journal =       {Ann Appl Stat},
  title =         {{BART}: {B}ayesian Additive Regression Trees},
  volume =        {4},
  number={1},
  pages={266--298},
  year =          {2010},
}

@incollection{loess,
  author =        {W.S. Cleveland and E. Groose and W.M. Shyu},
  booktitle =     {Statistical models in {S}},
  editor =        {J.M. Chambers and T.J. Hastie},
  publisher =     {Chapman \& Hall},
  title =         {Local Regression Models},
  year =          {1992},
      address =       {Boca Raton},
}

@techreport{Polley&vanderLaan10,
  author =        {E.C. Polley and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =        {266},
  title =         {Super Learner in Prediction},
  year =          {2010},
}

@book{cook:1994,
  address =       {New York},
  author =        {D. Cook and S. Weisberg},
  publisher =     {Wiley},
  title =         {An introduction to regression graphics},
  year =          {1994},
}

@article{chu:2001,
  author =        {S. Chu},
  journal =       {J Stat Educ},
  number =        {2},
  title =         {Pricing the {C}'s of diamond stones},
  volume =        {9},
  year =          {2001},
}

@book{berndt:1991,
  address =       {New York},
  author =        {E.R. Berndt},
  publisher =     {Addison--Wesley},
  title =         {The practice of econometrics},
  year =          {1991},
}

@article{kibler:1989,
  author =        {D. Kibler and D.W. Aha and M.K. Albert},
  journal =       {Comput Intell},
  pages =         {51},
  title =         {Instance-Based Prediction of Real-Valued Attributes},
  volume =        {5},
  year =          {1989},
}

@book{rosner:1999,
  address =       {Pacific Grove},
  author =        {B. Rosner},
  edition =       {5th},
  publisher =     {Duxbury},
  title =         {Fundamentals of biostatistics},
  year =          {1999},
}

@misc{newman:1998,
  author =        {D.J. Newman and S. Hettich and C.L. Blake and
                   C.J. Merz},
  institution =   {Department of
                   Information and Computer Sciences, University of California, Irvine},
  title =         {{UCI Repository of Machine Learning Databases}},
  year =          {1998},
}

@book{afifi:1979,
  address =       {New York},
  author =        {A. Afifi and S. Azen},
  edition =       {2nd},
  publisher =     {Academic},
  title =         {Statistical analysis: a computer oriented approach},
  year =          {1979},
}

@book{cook:1998,
  address =       {New York},
  author =        {D. Cook},
  publisher =     {Wiley},
  title =         {Regression graphics: ideas for studying regression
                   through graphics},
  year =          {1998},
}

@article{liu:1999,
  author =        {Z. Liu and T. Stengos},
  journal =       {J of Appl Econom},
  pages =         {527--538},
  title =         {Nonlinearities in Cross Country Growth Regressions:
                   a Semiparametric Approach},
  volume =        {14},
  year =          {1999},
}

@article{penrose:1985,
  author =        {K. Penrose and A. Nelson and A. Fisher},
  journal =       {Med Sci Sport Exer},
  pages =         {189},
  title =         {Generalized Body Composition Prediction Equation for
                   Men Using Simple Measurement Techniques},
  volume =        {17},
  year =          {1985},
}

@book{harrell:2001,
  address={Berlin Heidelberg New York},
  author =        {Harrell, Jr., F.E.},
  publisher =     {Springer},
  title =         {Regression modeling strategies with applications to
                   linear models, logistic regression, and survival
                   analysis},
  year =          {2001},
}

@manual{arm,
  author =        {A. Gelman and Y.-S. Su and M. Yajima and J. Hill and
                   M.G. Pittau and J. Kerman and T. Zheng},
  note =          {R package version 1.3-02},
  title =         {arm: data analysis using regression and
                   multilevel/hierarchical models},
  year =          {2010},
  url =           {http://CRAN.R-project.org/package=arm},
}

@article{gelman:2009,
  author =        {A. Gelman and A. Jakulin and M.G. Pittau and
                   Y.-S. Su},
  journal =       {Ann Appl Stat},
  number =        {3},
  pages =         {1360--1383},
  title =         {A Weakly Informative Default Prior Distribution for
                   Logistic and Other Regression Models},
  volume =        {2},
  year =          {2009},
}

@article{friedman:2010,
  author =        {J.H. Friedman and T.J. Hastie and R.J. Tibshirani},
  journal =       {J Stat Softw},
  number =        {1},
  title =         {Regularization Paths for Generalized Linear Models
                   via Coordinate Descent},
  volume =        {33},
  year =          {2010},
}

@manual{glmnet,
  author =        {J.H. Friedman and T.J. Hastie and R.J. Tibshirani},
  note =          {R package version 1.1-5},
  title =         {glmnet: lasso and elastic-net regularized generalized
                   linear models},
  year =          {2010},
  url =           {http://CRAN.R-project.org/package=glmnet},
}

@manual{DSA,
  author =        {R. Neugebauer and J. Bullard},
  note =          {R package version 3.1.3},
  title =         {DSA: Data-adaptive estimation with cross-validation
                   and the D/S/A algorithm},
  year =          {2009},
  url =           {http://www.stat.berkeley.edu/~laan/Software/},
}

@article{SinisivanderLaan04,
  author =        {S.E. Sinisi and M.J. van der Laan},
  journal =       {Stat Appl Genet Mol},
  note =          {Article 18},
  number =        {1},
  title =         {{D}eletion/{S}ubstitution/{A}ddition algorithm in
                   learning with applications in genomics},
  volume =        {3},
  year =          {2004},
}

@manual{svm,
  author =        {E. Dimitriadou and K. Hornik and F. Leisch and
                   D. Meyer and A. Weingessel},
  note =          {R package version 1.5-22},
  title =         {e1071: misc functions of the Department of Statistics
                   (e1071)},
  year =          {2009},
  url =           {http://CRAN.R-project.org/package=e1071},
}

@manual{Chang:2001,
  author =        {C.-C. Chang and C.-J. Lin},
  url =           {http://www.csie.ntu.edu.tw/~cjlin/libsvm},
  title =         {{LIBSVM}: a library for support vector machines},
  year =          {2001},
}

@article{vantveer:2002,
  author =        {L.J. {van't Veer} and H. Dal and M.J. {van de Vijver} and
                   Y.D. He and A.A.M. Hart and M. Mao and H.L. Peterse and
                   K. van der Kooy and M.J. Marton and A.T. Witteveen and
                   G.J. Schreiber and R.M. Kerkhoven and C. Roberts and
                   P.S. Linsley and R. Bernards and S.H. Friend},
  journal =       {Nature},
  pages =         {530--536},
  title =         {Gene Expression Profiling Predicts Clinical Outcome
                   of Breast Cancer},
  volume =        {415},
  year =          {2002},
}

@article{vanderLaan&Polley&Hubbard07,
  author =        {M.J. van der Laan and E.C. Polley and A.E. Hubbard},
  journal =       {Stat Appl Genet Mol},
  pages =        {Article 25},
  title =         {Super Learner},
  volume =        {6},
  year =          {2007},
  number =          {1},
}

@article{Wolpert92,
  author =        {D. H. Wolpert},
  journal =       {Neural Networks},
  pages =         {241--259},
  title =         {Stacked Generalization},
  volume =        {5},
  year =          {1992},
}

@article{Breiman96d,
  author =        {L. Breiman},
  journal =       {Mach Learn},
  pages =         {49--64},
  title =         {Stacked Regressions},
  volume =        {24},
  year =          {1996},
}

@article{Leblanc96,
  author =        {M. LeBlanc and R.J. Tibshirani},
  journal =       {J Am Stat Assoc},
  pages =         {1641--1650},
  title =         {Combining estimates in regression and classification},
  volume =        {91},
  year =          {1996},
}

@article{Stone74,
  author =        {M. Stone},
  journal =       {J R Stat Soc Ser B},
  number =        {2},
  pages =         {111--147},
  title =         {Cross-validatory choice and assessment of statistical
                   predictions},
  volume =        {36},
  year =          {1974},
}

@article{Geisser75,
  author =        {S. Geisser},
  journal =       {J Am Stat Assoc},
  number =        {350},
  pages =         {320--328},
  title =         {The Predictive Sample Reuse Method with Applications},
  volume =        {70},
  year =          {1975},
}

@inproceedings{Tsybakov03,
  author =        {A.B. Tsybakov},
  booktitle =     {COLT},
  editor =        {B. Sch{\"o}lkopf and M.K. Warmuth},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  series =        {Lecture Notes in Computer Science},
  title =         {Optimal rates of aggregation},
  volume =        {2777},
  year =          {2003},
}

@inproceedings{Juditskyetal05,
  author =        {A. Juditsky and A.V. Nazin and A.B. Tsybakov and
                   N. Vayatis},
  booktitle =     {NIPS},
  title =         {Generalization Error Bounds for Aggregation by Mirror
                   Descent with Averaging},
  year =          {2005},
}

@inproceedings{Buneaetal06,
  author =        {F. Bunea and A.B. Tsybakov and M.H. Wegkamp},
  booktitle =     {COLT},
  editor =        {G. Lugosi and H.-U. Simon},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  series =        {Lecture Notes in Computer Science},
  title =         {Aggregation and sparsity via {L}1 penalized least
                   squares},
  volume =        {4005},
  year =          {2006},
}

@article{Buneaetal07,
  author =        {F. Bunea and A.B. Tsybakov and M.H. Wegkamp},
  journal =       {Ann Stat},
  number =        {4},
  pages =         {1674--1697},
  title =         {Aggregation for Gaussian Regression},
  volume =        {35},
  year =          {2007},
}

@inproceedings{Buneaetal07b,
  author =        {F. Bunea and A.B. Tsybakov and M.H. Wegkamp},
  booktitle =     {COLT},
  editor =        {N.H. Bshouty and C. Gentile},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  series =        {Lecture Notes in Computer Science},
  title =         {Sparse density estimation with {L}1 penalties},
  volume =        {4539},
  year =          {2007},
}

@inproceedings{Dalalyan&Tsybakov07,
  author =        {A.S. Dalalyan and A.B. Tsybakov},
  booktitle =     {COLT},
  editor =        {N.H. Bshouty and C. Gentile},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  series =        {Lecture Notes in Computer Science},
  title =         {Aggregation by exponential weighting and sharp oracle
                   inequalities},
  volume =        {4539},
  year =          {2007},
}

@article{Dalalyan&Tsybakov08,
  author =        {A.S. Dalalyan and A.B. Tsybakov},
  journal =       {Mach Learn},
  number =        {1--2},
  pages =         {39--61},
  title =         {Aggregation by exponential weighting, sharp
                   PAC-{B}ayesian bounds and sparsity},
  volume =        {72},
  year =          {2008},
}

@book{Lehmann86,
  author =        {E.L. Lehmann},
  edition =       {2nd},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  title =         {Testing statistical hypotheses},
  year =          {1986},
}

@book{Hastie&Tibshirani&Friedman01,
  author =        {T.J. Hastie and R.J. Tibshirani and J.H. Friedman},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  title =         {The elements of statistical learning: data mining,
                   inference, and prediction},
  year =          {2001},
}

@ inproceedings{Ruczinski&Kooperberg&LeBlanc02,
  author =        {I. Ruczinski and C. Kooperberg and M. LeBlanc},
  booktitle =       {Proceedings of the MSRI workshop on Nonlinear
                   Estimation and Classification},
  editor={D. Denison and M.
                   Hansen and C. Holmes and B. Mallick and B. Yu},
  pages =         {333--344},
  title =         {Logic Regression -- methods and software},
  year =          {2002},
}



@techreport{Birkner&Hubbard&vanderLaan05,
  author =        {M.D. Birkner and A.E. Hubbard and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =        {197},
  title =         {Data Adaptive Pathway Testing},
  year =          {2005},
}

@techreport{Chaffee&Hubbard&vanderLaan10,
  author =        {P. Chaffee and A.E. Hubbard and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =        {263},
  title =         {Permutation-based Pathway Testing using the Super
                   Learner Algorithm},
  year =          {2010},
}
@incollection{Polleyetal12,
	Address = {New York Dordrecht Heidelberg London},
	Author = {E.C. Polley and Sherri Rose and M.J. van der Laan},
	Booktitle = {Targeted Learning: Causal Inference for Observational and Experimental Data},
	Date-Added = {2012-08-24 11:01:37 -0700},
	Date-Modified = {2012-08-24 11:02:54 -0700},
	Editor = {van der Laan, M.J. and Rose, S.},
	Keywords = {Chpt3},
	Publisher = {Springer},
	Title = {Super Learning},
	Year = {2012}}

	@inproceedings{Polley&vanderLaan09,
  author =        {E.C. Polley and M.J. van der Laan},
  booktitle =     {Design, summarization, analysis \& interpretation
                   of clinical trials with time-to-event endpoints},
  editor =        {K.E. Peace},
  publisher =     {Chapman \& Hall},
  title =         {Predicting Optimal Treatment Assignment Based on
                   Prognostic Factors in Cancer Patients},
address =       {Boca Raton},
  year =          {2009},
}

@article{vanderLaan&Dudoit&vanderVaart06,
  author =        {M.J. van der Laan and S. Dudoit and
                   A.W. van der Vaart},
  journal =       {Stat Decis},
  number =        {3},
  pages =         {373--395},
  title =         {The Cross-Validated Adaptive Epsilon-Net Estimator},
  volume =        {24},
  year =          {2006},
}

@article{vanderVaart&Dudoit&vanderLaan06,
  author =        {A.W. van der Vaart and S. Dudoit and
                   M.J. van der Laan},
  journal =       {Stat Decis},
  number =        {3},
  pages =         {351--371},
  title =         {Oracle Inequalities for Multi-Fold Cross-Validation},
  volume =        {24},
  year =          {2006},
}

@article{vanderLaan&Dudoit&Keles04,
  author =        {M.J. van der Laan and S. Dudoit and S. Kele\c{s}},
  journal =       {Stat Appl Genet Mol},
  pages =         {Article 4},
  title =         {Asymptotic optimality of likelihood-based
                   cross-validation},
  volume =        {3},
  number={1},
  year =          {2004},
}

@article{Dudoit&vanderLaan05,
  author =        {S. Dudoit and M.J. van der Laan},
  journal =       {Stat Methodol},
  number =        {2},
  pages =         {131--154},
  title =         {Asymptotics of cross-validated risk estimation in
                   estimator selection and performance assessment},
  volume =        {2},
  year =          {2005},
}

@techreport{Keles&vanderLaan&Dudoit02,
  author =        {Kele\c{s}, S. and van der Laan, M.J. and Dudoit, S.},
  institution =       {Division of Biostatistics, University of California,
                   Berkeley},
number={124},
  title =         {Asymptotically Optimal Model Selection Method for
                   Regression on Censored Outcomes},
  year =          {2002},
}

@book{Gyorfietal02,
  address={Berlin Heidelberg New York},
  author =        {L. Gy\"{o}rfi and M. Kohler and A. Krzy\.{z}ak and
                   H. Walk},
  pages =         {100--102},
  publisher =     {Springer},
  title =         {A distribution-free theory of nonparametric
                   regression},
  year =          {2002},
}

@article{Stone77,
  author =        {M. Stone},
  journal =       {Biometrika},
  number =        {1},
  pages =         {29--35},
  title =         {Asymptotics for and against cross-validation},
  volume =        {64},
  year =          {1977},
}

@book{Breimanetal84,
  author =        {L. Breiman and J.H. Friedman and R. Olshen and
                   C.J. Stone},
  publisher =     {Chapman \& Hall},
  title =         {Classification and regression trees},
  year =          {1984},
    address =       {Boca Raton},
}

@article{Breiman&Spector92,
  author =        {L. Breiman and P. Spector},
  journal =       {Int Stat Rev},
  pages =         {291--319},
  title =         {Submodel Selection and Evaluation in Regression. {T}he
                   {$X$} Random Case},
  volume =        {60},
  year =          {1992},
}

@book{Efron&Tibshirani93,
  author =        {B. Efron and R. J. Tibshirani},
  publisher =     {Chapman \& Hall},
  title =         {An Introduction to the bootstrap},
  year =          {1993},
      address =       {Boca Raton},
}

@article{Breiman96,
  author =        {L. Breiman},
  journal =       {Ann Stat},
  number =        {6},
  pages =         {2350--2383},
  title =         {Heuristics of instability and stabilization in model
                   selection},
  volume =        {24},
  year =          {1996},
}

@techreport{Breiman96c,
  author =        {L. Breiman},
  institution =   {Department of Statistics, University of California, Berkeley},
  type={Technical {R}eport},
  title =         {Out-of-bag estimation},
  year =          {1996},
}

@book{Ripley96,
  address =       {New York},
  author =        {B.D. Ripley},
  publisher =     {Cambridge},
  title =         {Pattern recognition and neural networks},
  year =          {1996},
}

@article{Breiman98,
  author =        {L. Breiman},
  journal =       {Ann Stat},
  pages =         {801--824},
  title =         {Arcing classifiers},
  volume =        {26},
  year =          {1998},
}

@article{Ambroise&McLachlan02,
  author =        {C. Ambroise and G.J. McLachlan},
  journal =       {Proc Natl Acad Sci},
  number =        {10},
  pages =         {6562--6566},
  title =         {Selection bias in gene extraction on the basis of
                   microarray gene-expression data},
  volume =        {99},
  year =          {2002},
}

@article{Pavlic&vanderLaan03,
  author =        {M. Pavlic and M.J. van der Laan},
  journal =       {Comput Stat Data An},
  pages =         {413--428},
  title =         {Fitting of mixtures with unspecified number of
                   components using cross validation distance estimate},
  volume =        {41},
  year =          {2003},
}

@inproceedings{Akaike73,
  author =        {H. Akaike},
  booktitle =     {Second International Symposium on Information Theory},
  editor =        {B.N. Petrov and F. Csaki},
  organization =  {Academiai Kiado},
  address={Budapest},
  title =         {Information theory and an extension of the maximum
                   likelihood principle},
  year =          {1973},
}

@article{Bozdogan00,
  author =        {H. Bozdogan},
  journal =       {J Math Psychol},
  pages =         {62--91},
  title =         {Akaike's information criterion and recent
                   developments in information complexity},
  volume =        {44},
  year =          {2000},
}

@article{Schwartz78,
  author =        {G. Schwartz},
  journal =       {Ann Stat},
  pages =         {461--464},
  title =         {Estimating the Dimension of a Model},
  volume =        {6},
  year =          {1978},
}

@article{Rissanen78,
  author =        {J. Rissanen},
  journal =       {Automatica},
  pages =         {465--471},
  title =         {Modelling by shortest data description},
  volume =        {14},
  year =          {1978},
}

@incollection{Bozdogan93,
  author =        {H. Bozdogan},
    address={Berlin Heidelberg New York},
  booktitle =     {Information and classification},
  editor =        {O. Opitz and B. Lausen and R. Klar},
  publisher =     {Springer},
  title =         {Choosing the number of component clusters in the
                   mixture model using a new informational complexity
                   criterion of the inverse Fisher information matrix},
  year =          {1993},
}

@article{Snowden&Rose&Mortimer11,
  author =        {J.M. Snowden and S. Rose and K.M. Mortimer},
  journal =       {Am J Epidemiol},
  number =        {00},
  pages =         {000--000},
  title =         {Implementation of G-Computation on a Simulated
                   Data set: demonstration of a Causal Inference
                   Technique},
  volume =        {173},
  year =          {2011},
}

@article{Rose&Snowden&Mortimer11,
author={S. Rose and J.M. Snowden and K.M. Mortimer},
title={Rose et al. Respond to ``{G}-Computation and Standardization in Epidemiology''},
journal={Am J Epidemiol},
volume={173},
number={00},
pages={000--000},
year={2011},
}

@incollection{Robins99b,
  author =        {Robins, J.M.},
  booktitle =     {Statistical models in epidemiology: the environment
                   and clinical trials},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  title =         {Marginal structural models versus structural nested
                   models as tools for causal inference},
  year =          {1999},
}

@article{Hernan&Brumback&Robins00,
  author =        {Hernan, M.A. and Brumback, B. and Robins, J.M.},
  journal =       {Epidemiol},
  number =        {5},
  pages =         {561--570},
  title =         {Marginal structural models to estimate the causal
                   effect of zidovudine on the survival of
                   {HIV}-positive men},
  volume =        {11},
  year =          {2000},
}

@article{Robins&Rotnitzky&vanderLaan00,
  author =        {J.M. Robins and A. Rotnitzky and M.J. van der Laan},
  journal =       {J Am Stat Assoc},
  pages =         {431--435},
  title =         {Comment on ``{O}n profile likelihood"},
  volume =        {450},
  year =          {2000},
}

@inproceedings{Robins00,
  author =        {J.M. Robins},
  booktitle =     {Proceedings of the American Statistical Association},
  editor =        {},
  organization =  {},
  pages =         {},
  title =         {Robust estimation in sequentially ignorable missing
                   data and causal inference models},
  year =          {2000},
}

@article{Robins&Rotnitzky01,
  author =        {J.M. Robins and A. Rotnitzky},
  journal =       {Stat Sinica},
  number =        {4},
  pages =         {920--936},
  title =         {Comment on the {B}ickel and {K}won article,
                   ``{I}nference for semiparametric models: some
                   questions and an answer''},
  volume =        {11},
  year =          {2001},
}

@article{Dawid&Didelez10,
  author =        {P. Dawid and V. Didelez},
  journal =       {Statist. Surv.},
  number =        {},
  pages =         {184--231},
  title =         {Identifying the consequences of dynamic treatment strategies: A decision-theoretic overview},
  volume =        {4},
  year =          {2010},
}



@incollection{Robins&Rotnitzky92,
  author =        {J.M. Robins and A. Rotnitzky},
  booktitle =     {AIDS epidemiology},
  editor ={Jewell N., Dietz K., Farewell V.},
  pages={296--231},
  publisher =     {Birkh\"{a}user},
      address={Basel},
  title =         {Recovery of information and adjustment for dependent
                   censoring using surrogate markers},
  year =          {1992},
}

@article{Robins&Hernan&Brumback00,
  author =        {Robins, J.M. and Hernan, M.A. and Brumback, B.},
  journal =       {Epidemiol},
  number =        {5},
  pages =         {550--560},
  title =         {Marginal structural models and causal inference in
                   epidemiology},
  volume =        {11},
  year =          {2000},
}

@article{Mortimeretal05,
  author =        {K.M. Mortimer and R. Neugebauer and M.J. van der Laan and
                   I.B. Tager},
  journal =       {Am J Epidemiol},
  number =        {4},
  pages =         {382--388},
  title =         {An Application of Model-Fitting Procedures for
                   Marginal Structural Models},
  volume =        {162},
  year =          {2005},
}

@article{Cole&Hernan08,
  author =        {S.R. Cole and M.A. Hernan},
  journal =       {Am J Epidemiol},
  pages =         {656--664},
  title =         {Constructing Inverse Probability Weights for Marginal
                   Structural Models},
  volume =        {168},
  year =          {2008},
}

@article{Bembom&vanderLaan07,
  author =        {O. Bembom and M.J. van der Laan},
  journal =       {Electron J Stat},
volume={1},
pages={574--596},
  title =         {A practical illustration of the importance of
                   realistic individualized treatment rules in causal
                   inference},
  year =          {2007},
}

@article{vanderLaan08,
  author =        {M.J. van der Laan},
  journal =       {Int J Biostat},
  volume={4},
  number={1},
pages={Article 17},
  title =         {Estimation based on case-control designs with known
                   prevalance probability},
  year =          {2008},
}

@article{Rose&vanderLaan08,
  author =        {S. Rose and M.J. van der Laan},
  journal =       {Int J Biostat},
  volume={4},
  number={1},
pages={Article 19},
  title =         {Simple optimal weighting of cases and controls in
                   case-control studies},
  year =          {2008},
}

@article{Rose&vanderLaan09,
  author =        {S. Rose and M.J. van der Laan},
  journal =       {Int J Biostat},
    volume={5},
  number={1},
pages={Article 1},
  title =         {Why match? {I}nvestigating matched case-control study
                   designs with causal effect estimation},
  year =          {2009},
}

@inproceedings{Moore&vanderLaan09,
  author =        {K.L. Moore and M.J. van der Laan},
  booktitle =     {Design, summarization, analysis \& interpretation
                   of clinical trials with time-to-event endpoints},
  editor =        {Karl E. Peace},
        address =       {Boca Raton},
  publisher =     {Chapman \& Hall},
  title =         {Application of Time-to-Event Methods in the
                   Assessment of Safety in Clinical Trials},
  year =          {2009},
}

@article{Moore&vanderLaan092,
  author =        {Moore, K.L. and van der Laan, M.J.},
  journal =       {Stat Med},
  number =        {1},
  pages =         {39--64},
  title =         {Covariate Adjustment in Randomized Trials with Binary
                   Outcomes: targeted Maximum Likelihood Estimation},
  volume =        {28},
  year =          {2009},
}

@article{Moore&vanderLaan093,
  author =        {Moore, K.L. and van der Laan, M.J.},
  journal =       {J Biopharm Stat},
  number =        {6},
  pages =         {1099--1131},
  title =         {Increasing Power in Randomized Trials with Right
                   Censored Outcomes Through Covariate Adjustment},
  volume =        {19},
  year =          {2009},
}

@article{Bembometal09b,
  author =        {O. Bembom and M.L. Petersen and S.-Y. Rhee and
                   W.J. Fessel and S.E. Sinisi and R.W. Shafer and
                   M.J. van der Laan},
  journal =       {Stat Med},
  pages =         {152--72},
  title =         {Biomarker discovery using targeted maximum likelihood
                   estimation: application to the treatment of
                   antiretroviral resistant {HIV} infection},
  volume =        {28},
  year =          {2009},
}

@article{Rosenblumetal09,
  author =        {M. Rosenblum and S.G. Deeks and M.J. van der Laan and
                   D.R. Bangsberg},
  journal =       {PLoS ONE},
  title =         {The Risk of Virologic Failure Decreases with Duration
                   of {HIV} Suppression, at Greater than 50\% Adherence to
                   Antiretroviral Therapy},
  volume =        {4(9): e7196.doi:10.1371/journal.pone.0007196},
  year =          {2009},
}

@article{Gruber&vanderLaan10a,
  author =        {S. Gruber and M.J. van der Laan},
  journal =       {Int J Biostat},
  number =        {1},
  title =         {An application of collaborative targeted maximum
                   likelihood estimation in causal inference and
                   genomics},
  volume =        {6},
  year =          {2010},
}

@article{Rosenblum&vanderLaan10,
  author =        {M. Rosenblum and M.J. van der Laan},
  journal =       {Int J Biostat},
    volume={6},
  number={2},
pages={Article 19},
  title =         {Targeted maximum likelihood estimation of the
                   parameter of a marginal structural model},
  year =          {2010},
}

@book{Dudoit&vanderLaan08,
address={Berlin Heidelberg New York},
  author =        {S. Dudoit and M.J. van der Laan},
  publisher =     {Springer},
  title =         {Resampling based multiple testing with applications
                   to genomics},
  year =          {2008},
}

@article{Robins94,
  author =        {J.M. Robins},
  journal =       {Commun Stat},
  number =        {},
  pages =         {2379--2412},
  title =         {Correcting for noncompliance in randomized trials
                   using structural nested mean models},
  volume =        {23},
  year =          {1994},
}

@article{Robins&Rotnitzky&Zhao95,
  author =        {J.M. Robins and A. Rotnitzky and L.P. Zhao},
  journal =       {J Am Stat Assoc},
  pages =         {106--121},
  title =         {Analysis of semiparametric regression models for
                   repeated outcomes in the presence of missing data.},
  volume =        {90},
  year =          {1995},
}

@article{Scharfstein&Rotnitzky&Robins99,
  author =        {D.O. Scharfstein and A. Rotnitzky and J.M. Robins},
  journal =       {J Am Stat Assoc},
  pages =         {1096-1120 (1121-1146)},
  title =         {Adjusting for Nonignorable Drop-out Using
                   Semiparametric Nonresponse Models, (with Discussion
                   and Rejoinder)},
  volume =        {94},
  year =          {1999},
}

@article{Leon&Tsiatis&Davidian03,
  author =        {S. Leon and A.A. Tsiatis and M. Davidian},
  journal =       {Biometrics},
  pages =         {1046--1055},
  title =         {Semiparametric estimation of treatment effect in a
                   pretest-posttest study},
  volume =        {59},
  year =          {2003},
}

@article{Tan06,
  author =        {Z. Tan},
  journal =       {J Am Stat Assoc},
  pages =         {1619-1637},
  title =         {A distributional approach for causal inference using
                   propensity scores},
  volume =        {101},
  year =          {2006},
}

@book{Tsiatis062,
  address={Berlin Heidelberg New York},
  author =        {A.A. Tsiatis},
  publisher =     {Springer},
  title =         {Semiparametric theory and missing data},
  year =          {2006},
}

@article{Zhang&Tsiatis&Davidian08,
  author =        {M. Zhang and A.A. Tsiatis and M. Davidian},
  journal =       {Biometrics},
  number =        {3},
  pages =         {707--715},
  title =         {Improving efficiency of inferences in randomized
                   clinical trials using auxiliary covariates},
  volume =        {64},
  year =          {2008},
}

@article{Rubin&vanderLaan08,
  author =        {Daniel B. Rubin and M.J. van der Laan},
  journal =       {Int J Biostat},
  title =         {Empirical efficiency maximization: improved locally
                   efficient covariate adjustment in randomized
                   experiments and survival analysis},
  volume =        {4},
  number={1},
  pages={Article 5},
  year =          {2008},
}

@article{Freedman08,
  author =        {D.A. Freedman},
  journal =       {Adv Appl Math},
  pages =         {180--193},
  title =         {On regression adjustments to experimental data},
  volume =        {40},
  year =          {2008},
}

@article{Freedman082,
  author =        {D.A. Freedman},
  journal =       {Ann Appl Stat},
  pages =         {176--96},
  title =         {On regression adjustments to experiments with several
                   treatments},
  volume =        {2},
  year =          {2008},
}

@article{Rosenblum&vanderLaan09,
  author =        {M. Rosenblum and M.J. van der Laan},
  journal =       {Biometrics},
  number =        {3},
  pages =         {937--945},
  title =         {Using Regression Models to Analyze Randomized Trials:
                   asymptotically Valid Hypothesis Tests Despite
                   Incorrectly Specified Models},
  volume =        {65},
  year =          {2009},
}

@book{Hampeletal86,
  author =        {Hampel, F.R. and Ronchetti, E.M. and Rousseeuw, P.J. and
                   Stahel, W.A.},
  address =       {New York},
  publisher =     {Wiley},
  title =         {{Robust statistics: the approach based on influence
                   functions}},
  year =          {1986},
}

@book{vanderVaart98,
  author =        {A.W. van der Vaart},
  publisher =     {Cambridge},
  title =         {Asymptotic statistics},
    address =       {New York},
  year =          {1998},
}

@book{vanderVaart&Wellner96,
  author =        {A.W. van der Vaart and J.A. Wellner},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  title =         {Weak convergence and empirical processes},
  year =          {1996},
}

@article{Rosenbaum&Rubin83,
  author =        {P.R. Rosenbaum and Donald B. Rubin},
  journal =       {Biometrika},
  pages =         {41--55},
  title =         {The central role of the propensity score in
                   observational studies for causal effects},
  volume =        {70},
  year =          {1983},
}

@article{Stitelman&vanderLaan10,
  author =        {O.M. Stitelman and M.J. van der Laan},
Journal={Int J Biostat},
volume={6},
number={1},
pages={Article 21},
  title =         {Collaborative Targeted Maximum Likelihood for
                   Time-to-Event Data},
  year =          {2010},
}


@article{Wedderburn74,
  author =        {R.W.M. Wedderburn},
  journal =       {Biometrika},
  pages =         {439--447},
  title =         {Quasi-likelihood functions, generalized linear
                   models, and the Gauss-Newton method},
  volume =        {61},
  number={3},
  year =          {1974},
}

@article{McCullagh83,
  author =        {P. Mc{C}ullagh},
  journal =       {Ann Stat},
  pages =         {59--67},
  title =         {Quasi-likelihood functions},
  volume =        {11},
  year =          {1983},
}

@article{vanderLaan&Petersen08,
  author =        {M.J. van der Laan and M.L. Petersen},
  journal =       {Int J Biostat},
  number =        {1},
  title =         {Direct effect models},
  volume =        {4},
  pages={Article 23},
  year =          {2008},
}

@techreport{vanderLaan10c,
  author =        {M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =        {268},
  title =         {Estimation of Causal Effects of Community-Based
                   Interventions},
  year =          {2010},
}

@article{Heckman&Ichimura&Todd97,
  author =        {J. Heckman and H. Ichimura and R. Todd},
  journal =       {Rev of Econ Stud},
  pages =         {605--654},
  title =         {Matching as an Econometric Evaluation Estimator:
                   evidence from Evaluating a Job Training Programme},
  volume =        {64},
  year =          {1997},
}

@techreport{Sekhon06,
  author =        {J.S. Sekhon},
  institution =   {University of California,
                   Berkeley},
  type={Technical {R}eport},
  title =         {Alternative balance metrics for bias reduction in
                   matching methods for causal inference},
  year =          {2006},
}

@article{Hansen08,
  author =        {B.B. Hansen},
  journal =       {Biometrika},
  pages =         {481--8},
  title =         {The prognostic analogue of the propensity score},
  volume =        {95},
  year =          {2008},
}

@book{Haignere02,
  address =       {Washington, DC},
  author =        {Haignere, L.},
  edition =       {2nd},
  publisher =     {American Association of University Professors},
  title =         {Paychecks: a guide to conducting salary-equity
                   studies for higher education faculty},
  year =          {2002},
}

@article{Holland88,
  author =        {P.W. Holland},
  journal =       {Stat Sci},
  number =        {2},
  pages =         {186--188.},
  title =         {Comment: Causal Mechanism or Causal Effect: which Is
                   Best for Statistical Science?},
  volume =        {3},
  year =          {1988},
}

@article{Robins98,
  author =        {J.M. Robins},
  journal =       {1997 Proceedings of the American Statistical
                   Association. Section on {B}ayesian Statistical Science},
  pages =         {1--10},
  title =         {Marginal Structural Models},
  year =          {1998},
}

@article{Mossetal04,
  author =        {A.R. Moss and J.A. Hahn and S. Perry and
                   E.D. Charlebois and D. Guzman and R.A. Clark and
                   D.R. Bangsberg},
  journal =       {Clin Infect Dis},
  number =        {8},
  pages =         {1190--1198},
  title =         {Adherence to highly active antiretroviral therapy in
                   the homeless population in {S}an {F}rancisco: a
                   prospective study},
  volume =        {39},
  year =          {2004},
}

@article{Bangsbergetal01,
  author =        {D.R. Bangsberg and F. Hecht and E.D. Charlebois and
                   M. Chesney and A.R. Moss},
  journal =       {AIDS Behav},
  pages =         {275--281},
  title =         {Comparing Objectives Measures of Adherence to HIV
                   Antiretroviral Therapy: electronic Medication
                   Monitors and Unannounced Pill Counts.},
  volume =        {5},
  year =          {2001},
}

@article{Neugebauer&vanderLaan07,
  author =        {R. Neugebauer and M. J. van der Laan},
  journal =       {J Stat Plan Infer},
  number =        {2},
  pages =         {419--434},
  title =         {Nonparametric causal effects based on marginal
                   structural models},
  volume =        {137},
  year =          {2007},
}

@article{Efron87,
  author =        {B. Efron},
  journal =       {J Am Stat Assoc},
  number =        {397},
  pages =         {171--185},
  title =         {Better Bootstrap Confidence Intervals},
  volume =        {82},
  year =          {1987},
}

@article{Kirschetal08,
  author =        {I. Kirsch and B.J. Deacon and T.B. Huedo-Medina and
                   A. Scoboria and T.J. Moore and B.T. Johnson},
  journal =       {PLoS Med},
  number =        {2},
  pages =         {e45. doi:10.1371/journal.pmed.0050045},
  title =         {Initial Severity and Antidepressant Benefits: a
                   Meta-Analysis of Data Submitted to the {Food and Drug
                   Administration}},
  volume =        {5},
  year =          {2008},
}

@article{Baselga01,
  author =        {J. Baselga},
  journal =       {Oncology},
  pages =         {14--21},
  title =         {Herceptin alone or in combination with chemotherapy
                   in the treatment of {HER2}-positive metastatic breast
                   cancer: pivotal trials},
  volume =        {61(S2)},
  year =          {2001},
}

@techreport{Wangetal06,
  author =        {Y. Wang and M.L. Petersen and D.R. Bangsberg and
                   M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =        {211},
  title =         {Diagnosing Bias in the Inverse Probability of
                   Treatment Weighted Estimator Resulting from Violation
                   of Experimental Treatment Assignment.},
  year =          {2006},
}

@article{Robins87,
  author =        {Robins, J.M.},
  journal =       {Comput Math Appl},
  number =        {9--12},
  pages =         {923--945},
  title =         {Addendum to: ``{A} new approach to causal inference
                   in mortality studies with a sustained exposure
                   period---application to control of the healthy worker
                   survivor effect''},
  volume =        {14},
  year =          {1987},
}



@article{Robins872,
  author =        {J.M. Robins},
  journal =       {J Chron Dis (40, Supplement)},
  pages =         {139s--161s},
  title =         {A graphical approach to the identification and
                   estimation of causal parameters in mortality studies
                   with sustained exposure periods},
  volume =        {2},
  year =          {1987},
}

@article{Rosenblum&vanderLaan09b,
  author =        {M. Rosenblum and M.J. van der Laan},
  journal =       {Int J Biostat},
  pages =         {Article 4},
  title =         {Confidence Intervals for the Population Mean Tailored
                   to Small Sample Sizes, with Applications to Survey
                   Sampling},
  volume =        {1},
  year =          {2009},
}

@article{Neugebauer&vanderLaan05,
  author =        {Neugebauer, R. and van der Laan, M.J.},
  journal =       {J Stat Plan Infer},
  number =        {1-2},
  pages =         {405--26},
  title =         {Why prefer double robust estimates},
  volume =        {129},
  year =          {2005},
}

@techreport{Mooreetal09,
  author =        {K.L. Moore and R.S. Neugebauer and M.J. van der Laan and
                   I.B. Tager},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =        {255},
  title =         {Causal Inference in Epidemiological Studies with
                   Strong Confounding},
  year =          {2009},
}

@article{Kish92,
  author =        {L. Kish},
  journal =       {J Off Stat},
  number =        {},
  pages =         {183--200},
  title =         {Weighting for unequal $P_i$},
  volume =        {8},
  year =          {1992},
}

@techreport{Bembom&vanderLaan08,
  author =        {O. Bembom and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =        {230},
  title =         {Data-adaptive selection of the truncation level for
                   Inverse-Probability-of-Treatment-Weighted estimators},
  year =          {2008},
}

@article{Freedman&Berk08,
  author =        {D.A. Freedman and R.A. Berk},
  journal =       {Eval Rev},
  pages =         {392--409},
  title =         {Weighting Regressions by Propensity Scores},
  volume =        {3},
  year =          {2008},
}

@article{Petersenetal10,
  author =        {M.L. Petersen and K.E. Porter and S. Gruber and
                   Y. Wang and M.J. van der Laan},
journal = {Stat Meth Med Res},
  title =         {Diagnosing and responding to violations in the
                   positivity assumption},
     volume =        {published online 28 Oct (doi:
                   10.1177/0962280210386207)},
  year =          {2010},
}

@article{Johnsonetal09,
  author =        {V.A. Johnson and F. Brun-Vezinet and B. Clotet and
                   H.F. Gunthard and D.R. Kuritzkes and D. Pillay and
                   J.M. Schapiro and D.D. Richman},
  journal =       {Top HIV Med},
  number =        {5},
  pages =         {138--45},
  title =         {Update of the drug resistance mutations in {HIV}-1:
                   {D}ecember 2009.},
  volume =        {17},
  year =          {2009},
}

@techreport{Bembometal08b,
  author =        {O. Bembom and W.J. Fessel and R.W. Shafer and
                   M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  type =          {231},
  title =         {Data-adaptive Selection Of The Adjustment Set In
                   Variable Importance Estimation},
  year =          {2008},
}

@techreport{Crumpetal06,
  author =        {R.K. Crump and V.J. Hotz and G.W. Imbens and
                   O.A. Mitnik},
  institution =   {National Bureau of Economic Research},
  number =        {330},
  title =         {Moving the goalposts: addressing limited overlap in
                   the estimation of average treatment effects by
                   changing the estimand},
  year =          {2006},
}

@article{LaLonde86,
  author =        {R.J. LaLonde},
  journal =       {Am Econ Rev},
  pages =         {604--620},
  title =         {Evaluating the Econometric Evaluations of Training
                   Programs with Experimental Data},
  volume =        {76},
  year =          {1986},
}

@article{Dehejia&Wahba99,
  author =        {R. Dehejia and S. Wahba},
  journal =       {J Am Stat Assoc},
  pages =         {1053--1062},
  title =         {Causal Effects in Nonexperimental Studies:
                   reevaluating the Evaluation of Training Programs},
  volume =        {94},
  year =          {1999},
}

@article{vanderLaan&Petersen07,
  author =        {M.J. van der Laan and M.L. Petersen},
  journal =       {Int J Biostat},
  number =        {1},
  pages =         {Article 3},
  title =         {Causal Effect Models for Realistic Individualized
                   Treatment and Intention to Treat Rules},
  volume =        {3},
  year =          {2007},
}

@article{Robins&Orellana&Rotnitzky08,
  author =        {J.M. Robins and L. Orellana and A. Rotnitzky},
  journal =       {Stat Med},
  pages =         {4678--4721},
  title =         {Estimation and extrapolation of optimal treatment and
                   testing strategies},
  volume =        {27},
  year =          {2008},
}

@article{Cochran57,
  author =        {W.G. Cochran},
  journal =       {Biometrics},
  number =        {},
  pages =         {261--281},
  title =         {Analysis of Covariance: its Nature and Uses.},
  volume =        {13},
  year =          {1957},
}

@techreport{Moore&vanderLaan07,
  author =        {K.L. Moore and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  month =         {April},
  number =          {215},
  title =         {Covariate adjustment in randomized trials with binary
                   outcomes},
  year =          {2007},
}

@article{Rosenblum&vanderLaan102,
  author =        {M. Rosenblum and M.J. van der Laan},
  journal =       {Int J Biostat},
  number =        {1},
  pages =         {Article 13},
  title =         {Simple, Efficient Estimators of Treatment Effects in
                   Randomized Trials Using Generalized Linear Models to
                   Leverage Baseline Variables},
  volume =        {6},
  year =          {2010},
}

@article{Freedman083,
  author =        {D.A. Freedman},
  journal =       {Stat Sci},
  pages =         {237--249},
  title =         {Randomization does not justify logistic regression},
  volume =        {23},
  year =          {2008},
}

@article{Yang&Tsiatis01,
  author =        {L. Yang and A.A. Tsiatis},
  journal =       {Am Stat},
  pages =         {29--38},
  title =         {Efficiency study for a treatment effect in a
                   pretest-posttest trial},
  volume =        {56},
  year =          {2001},
}

@book{McCullagh&Nelder89,
  address =       {Boca Raton},
  author =        {P. McCullagh and J.A. Nelder},
  edition =       {2nd},
  publisher =     {Chapman \& Hall},
  title =         {Generalized linear models},
  year =          {1989},
}

@incollection{Gail86,
  address =       {New York},
 author =        {M.H. Gail},
  booktitle =     {Modern Statistical Methods in Chronic Disease
                   Epidemiology},
  editor =        {S.~H. Moolvankar and R.~L.
                   Prentice},
  publisher =     {Wiley},
  title =         {Adjusting for covariates that have the same
                   distribution in exposed and unexposed cohorts},
  year =          {1986},
}

@article{Tsiatisetal08,
  author =        {A.A. Tsiatis and M. Davidian and M. Zhang and X. Lu},
  journal =       {Stat Med},
  pages =         {4658--4677},
  title =         {Covariate adjustment for two-sample treatment
                   comparisons in randomized clinical trials: a
                   principled yet flexible approach},
  volume =        {27},
  year =          {2008},
}

@article{Kochetal98,
  author =        {G.G. Koch and C.M. Tangen and J.W. Jung and
                   I.A. Amara},
  journal =       {Stat Med},
  pages =         {1863--1892},
  title =         {Issues for covariance analysis of dichotomous and
                   ordered categorical data from randomized clinical
                   trials and nonparametric strategies for addressing
                   them},
  volume =        {17},
  year =          {1998},
}

@article{Pococketal02,
  author =        {S.J. Pocock and S.E. Assmann and L.E. Enos and
                   L.E. Kasten},
  journal =       {Stat Med},
  pages =         {2917--2930},
  title =         {Subgroup analysis, covariate adjustment, and baseline
                   comparisons in clinical trial reporting: current
                   practice and problems.},
  volume =        {21},
  year =          {2002},
}

@article{Anderson72,
  author =        {J.A. Anderson},
  journal =       {Biometrika},
  pages =         {19--35},
  title =         {Separate sample logistic discrimination},
  volume =        {59},
  year =          {1972},
}

@article{Robins99,
  author =        {J.M. Robins},
  journal =       {Stat Sci},
  number =        {3},
  pages =         {281--293},
  title =         {[{C}hoice as an Alternative to Control in Observational
                   Studies]: Comment},
  volume =        {14},
  year =          {1999},
}

@article{Manssonetal07,
  author =        {R. Mansson and M.M. Joffe and W. Sun and S. Hennessy},
  journal =       {Am J Epidemiol},
  number =        {3},
  pages =         {332-339},
  title =         {On the Estimation and Use of Propensity Scores in
                   Case-Control and Case-Cohort Studies.},
  volume =        {166},
  year =          {2007},
}

@article{Prentice&Pyke79,
  author =        {R.L. Prentice and R. Pyke},
  journal =       {Biometrika},
  pages =         {403--411},
  title =         {Logistic disease incidence models and case-control
                   studies},
  volume =        {66},
  year =          {1979},
}

@book{Breslow&Day80,
  address =       {Lyon},
  author =        {N.E. Breslow and N.E. Day},
  publisher =     {International Agency for Research on Cancer},
  title =         {Statistical methods in cancer research: {V}olume 1 --
                   {T}he analysis of case-control studies},
  year =          {1980},
}

@article{Breslow96,
  author =        {N.E. Breslow},
  journal =       {J Am Stat Soc},
  pages =         {14--28},
  title =         {Statistics in Epidemiology: the Case-Control Study},
  volume =        {91},
  year =          {1996},
}

@article{Greenland81,
  author =        {S. Greenland},
  journal =       {J Chron Dis},
  pages =         {445--453},
  title =         {Multivariate Estimation of Exposure-Specific
                   Incidence from Case-Control Studies.},
  volume =        {34},
  year =          {1981},
}

@incollection{Holland&Rubin88,
  address =       {Cambridge, MA},
  author =        {P.W. Holland and Donald B. Rubin},
  booktitle =     {Matched sampling for causal effects.},
  editor =        {Donald B. Rubin},
  publisher =     {Cambridge},
  title =         {Causal inference in retrospective studies},
  year =          {1988},
}

@article{Greenland04,
  author =        {S. Greenland},
  journal =       {Am J Epidemiol},
  number =        {4},
  pages =         {301--305},
  title =         {Model-based Estimation of Relative Risks and Other
                   Epidemiologic Measures in Studies of Common Outcomes
                   and in Case-Control Studies.},
  volume =        {160},
  year =          {2004},
}

@article{Newman06,
  author =        {S. Newman},
  journal =       {Epid Persp Innov},
  pages =         {2},
  title =         {Causal analysis of case-control data},
  volume =        {3},
  year =          {2006},
}

@article{Cornfield51,
  author =        {J. Cornfield},
  journal =       {J Nat Cancer Inst},
  pages =         {1269--1275},
  title =         {A method of estimating comparative rates from
                   clinical data. Applications to cancer of the lung,
                   breast, and cervix.},
  volume =        {11},
  year =          {1951},
}

@inproceedings{Cornfield56,
  author =        {J. Cornfield},
    address =       {Berkeley},
  booktitle =     {Proceedings of the 3rd Berkeley symposium, {V}ol
                   IV},
  editor =        {J. Neyman},
  publisher =     {University of California Press},
  title =         {A statistical problem arising from retrospective
                   studies},
  year =          {1956},
}

@article{Prentice&Breslow78,
  author =        {R.L. Prentice and N.E. Breslow},
  journal =       {Biometrika},
  number =        {1},
  pages =         {153--158},
  title =         {Retrospective studies and failure time models.},
  volume =        {65},
  year =          {1978},
}

@article{Moriseetal96,
  author =        {A.P. Morise and G.A. Diamon and R. Detrano and
                   M. Bobbio and Erdogan Gunel},
  journal =       {Med Decis Making},
  pages =         {133--142},
  title =         {The Effect of Disease-prevalence Adjustments on the
                   Accuracy of a Logistic Prediction Model.},
  volume =        {16},
  year =          {1996},
}

@article{Wacholder96,
  author =        {S. Wacholder},
  journal =       {Epidemiol},
  number =        {2},
  pages =         {144--150},
  title =         {The Case-Control Study as Data Missing by Design:
                   estimating Risk Differences.},
  volume =        {7},
  year =          {1996},
}

@article{Rose&vanderLaan11,
  author =        {S. Rose and M.J. van der Laan},
  journal =       {Int J Biostat},
  number =        {17},
  title =         {A Targeted Maximum Likelihood Estimator for Two-Stage
                   Designs},
  volume =        {7},
  year =          {2011},
}

@article{Freedman50,
  author =        {R. Freedman},
  journal =       {Am J of Soc},
  number =        {5},
  pages =         {485--487},
  title =         {Incomplete Matching in Ex Post Facto Studies},
  volume =        {55},
  year =          {1950},
}

@article{Cochran65,
  author =        {W.G. Cochran},
  journal =       {J R Stat Soc Ser A Gen},
  number =        {2},
  pages =         {234--266},
  title =         {The Planning of Observational Studies of Human
                   Populations},
  volume =        {128},
  year =          {1965},
}

@article{Billewicz65,
  author =        {W.Z. Billewicz},
  journal =       {Biometrics},
  number =        {3},
  pages =         {623--644},
  title =         {The Efficiency of Matched Samples: an Empirical
                   Investigation},
  volume =        {21},
  year =          {1965},
}

@article{McKinlay77,
  author =        {S.M. McKinlay},
  journal =       {Biometrics},
  number =        {4},
  pages =         {725--735},
  title =         {Pair-Matching -- A reappraisal of a Popular
                   Technique},
  volume =        {33},
  year =          {1977},
}

@article{Kupperetal81,
  author =        {L.L. Kupper and J.M. Karon and D.G. Kleinbaum and
                   H. Morgenstern and D.K. Lewis},
  journal =       {Biometrics},
  pages =         {271--291},
  title =         {Matching in Epidemiologic Studies: validity and
                   Efficiency Considerations},
  volume =        {37},
  year =          {1981},
}

@article{Costanza95,
  author =        {M.C. Costanza},
  journal =       {Prev Med},
  pages =         {425--433},
  title =         {Matching},
  volume =        {24},
  year =          {1995},
}

@book{Schlesselman82,
  address =       {Oxford},
  author =        {J.J. Schlesselman},
  publisher =     {Oxford},
  title =         {Case-control studies: design, conduct, analysis},
  year =          {1982},
}

@article{Vandenbroukeetal07,
  author =        {J.P. Vandenbrouke and E. von Elm and D.G. Altman and
                   P.C. Gotzsche and C.D. Mulrow and S.J. Pocock and
                   C. Poole and J.J. Schlesselman and
                   M. Egger for the STROBE Initiative},
  journal =       {PLoS Med},
  number =        {10},
  pages =         {1628--1654},
  title =         {Strengthening the Reporting of Observational
                   Studies in Epidemiology ({STROBE}): explanation
                   and Elaboration.},
  volume =        {4},
  year =          {2007},
}

@article{Cochran53,
  author =        {W.G. Cochran},
  journal =       {Am J Public Health},
  pages =         {684--691},
  title =         {Matching in Analytical Studies},
  volume =        {43},
  year =          {1953},
}

@article{Breslowetal78,
  author =        {N.E. Breslow and N.E. Day and K.T. Halvorsen and
                   R.L. Prentice and C. Sabal},
  journal =       {Am J Epidemiol},
  number =        {4},
  pages =         {299--307},
  title =         {Estimation of Multiple Relative Risk Functions in
                   Matched Case-Control Studies},
  volume =        {108},
  year =          {1978},
}

@article{Holford&White&Kelsey78,
  author =        {T.R. Holford and C. White and J.L. Kelsey},
  journal =       {Am J Epidemiol},
  number =        {3},
  pages =         {245--255},
  title =         {Multivariate Analysis for Matched Case-Control
                   Studies},
  volume =        {107},
  year =          {1978},
}

@article{Kannel&McGee&Gordon76,
  author =        {W.B. Kannel and D. McGee and T. Gordon},
  journal =       {Am J Cardiol},
  pages =         {46--51},
  title =         {A general cardiovascular risk profile: the {F}ramingham
                   Study},
  volume =        {38},
  year =          {1976},
}

@article{Andersonetal91,
  author =        {K.M. Anderson and P.W.F. Wilson and P.M. Odell and
                   W.B. Kannel},
  journal =       {Circulation},
  pages =         {356--362},
  title =         {An updated coronary risk profile. A statement for
                   health professionals.},
  volume =        {83},
  year =          {1991},
}

@article{Ramsayetal95,
  author =        {L.E. Ramsay and I.U. Haq and P.R. Jackson and
                   W.W. Yeo},
  journal =       {Lancet},
  number =        {8988},
  pages =         {1467--1471},
  title =         {Sheffield risk and treatment table for cholesterol
                   lowering for primary prevention of coronary heart
                   disease.},
  volume =        {346},
  year =          {1995},
}

@article{Ramsayetal96,
  author =        {L.E. Ramsay and I.U. Haq and P.R. Jackson and
                   W.W. Yeo},
  journal =       {Lancet},
  number =        {9036},
  pages =         {1251},
  title =         {The {S}heffield table for primary prevention of
                   coronary heart disease: corrected.},
  volume =        {348},
  year =          {1996},
}

@article{Wilsonetal98,
  author =        {P.W.F. Wilson and R.B. D'Agostino and D. Levy and
                   A.M. Belanger and H. Silbershatz and W.B. Kannel},
  journal =       {Circulation},
  pages =         {1837--1847},
  title =         {Prediction of coronary heart disease using risk
                   factor categories},
  volume =        {97},
  year =          {1998},
}

@article{Jackson00,
  author =        {R. Jackson},
  journal =       {Br Med J},
  number =        {7236},
  pages =         {709--710},
  title =         {Updated New Zealand cardiovascular disease
                   risk-benefit prediction guide.},
  volume =        {320},
  year =          {2000},
}

@article{Gailetal89,
  author =        {M.H. Gail and L.A. Brinton and D.P. Byar and
                   D.K. Corle and S.B. Green and C. Schairer and
                   J.J. Mulvihill},
  journal =       {J Natl Cancer Inst},
  number =        {24},
  pages =         {1879--1886},
  title =         {Projecting individualized probabilities of developing
                   breast cancer for white females who are being
                   examined annually.},
  volume =        {81},
  year =          {1989},
}

@article{Costantinoetal99,
  author =        {J.P. Costantino and M.H. Gail and D. Pee and
                   S. Anderson and C.K. Redmond and J. Benichou and
                   H.S. Wieand},
  journal =       {J Natl Cancer Inst},
  number =        {18},
  pages =         {1541--1548},
  title =         {Validation studies for models projecting the risk of
                   invasive and total breast cancer incidence.},
  volume =        {91},
  year =          {1999},
}

@article{Tyrer&Duffy&Cuzick04,
  author =        {J. Tyrer and S.W. Duffy and J. Cuzick},
  journal =       {Stat Med},
  number =        {7},
  pages =         {1111--1130},
  title =         {A breast cancer prediction model incorporating
                   familial and personal risk factors},
  volume =        {23},
  year =          {2004},
}

@article{Barlowetal06,
  author =        {W.E. Barlow and E. White and R. Ballard-Barbash and
                   P.M. Vacek and L. Titus-Ernstoff and P.A. Carney and
                   J.A. Tice and D.S. Buist and B.M. Geller and
                   R. Rosenberg and B.C. Yankaskas and K. Kerlikowske},
  journal =       {J Natl Cancer Inst},
  number =        {17},
  pages =         {1204--1214},
  title =         {Prospective breats cancer risk prediction model for
                   women undergoing screening mammography.},
  volume =        {98},
  year =          {2006},
}

@article{Loprinzietal94,
  author =        {C.L. Loprinzi and J.A. Laurie and H.S. Wieand and
                   J.E. Krook and P.J. Novotny and J.W. Kugler and
                   J. Bartel and M. Law and M. Bateman and N.E. Klatt},
  journal =       {J Clin Oncol},
  number =        {3},
  pages =         {601--607},
  title =         {Prospective Evaluation of Prognostic Variables from
                   Patient-Completed Questionnaires, {N}orth {C}entral
                   {C}ancer {T}reatment {G}roup},
  volume =        {12},
  year =          {1994},
}

@manual{Therneau&Lumley09,
  author =        {T. Therneau and T. Lumley},
  note =          {R package version 2.35-8},
  title =         {survival: survival analysis, including penalised
                   likelihood},
  year =          {2009},
  url =           {http://CRAN.R-project.org/package=survival},
}

@article{Tibshirani97,
  author =        {R.J. Tibshirani},
  journal =       {Stat Med},
  pages =         {385--395},
  title =         {The Lasso Method for Variable Selection in the {C}ox
                   Model},
  volume =        {16},
  year =          {1997},
}

@article{Zhang&Lu07,
  author =        {H.H. Zhang and W. Lu},
  journal =       {Biometrika},
  number =        {3},
  pages =         {691--703},
  title =         {Adaptive Lasso for {C}ox's Proportional Hazards Model},
  volume =        {94},
  year =          {2007},
}

@article{Kooperberg&Stone&Truong95,
  author =        {C. Kooperberg and C.J. Stone and Y.K. Truong},
  journal =       {J Am Stat Assoc},
  number =        {429},
  pages =         {78--94},
  title =         {Hazard Regression},
  volume =        {90},
  year =          {1995},
}

@article{Leblanc&Crowley92,
  author =        {M. LeBlanc and J. Crowley},
  journal =       {Biometrics},
  number =        {},
  pages =         {411--425},
  title =         {Relative Risk trees for censored data},
  volume =        {48},
  year =          {1992},
}

@article{Segal88,
  author =        {M.R. Segal},
  journal =       {Biometrics},
  pages =         {35--47},
  title =         {Regression trees for censored data},
  volume =        {44},
  year =          {1988},
}

@article{Hothornetal06,
  author =        {T. Hothorn and P. Buhlmann and S. Dudoit and
                   A.M. Molinaro and M.J. van der Laan},
  journal =       {Biostatistics},
  pages =         {355--373},
  title =         {Survival Ensembles},
  volume =        {7},
  year =          {2006},
}

@article{Ishwaranetal08,
  author =        {H. Ishwaran and U.B. Kogalur and E.H. Blackstone and
                   M.S. Lauer},
  journal =       {Ann Appl Stat},
  number =        {3},
  pages =         {841--860},
  title =         {Random Survival Forests},
  volume =        {2},
  year =          {2008},
}

@article{vanHouwelingenetal06,
  author =        {H.C. van Houwelingen and T. Bruinsma and A.A.M. Hart and
                   L.J. {van't Veer} and L.F.A. Wessels},
  journal =       {Stat Med},
  pages =         {3201--3216},
  title =         {Cross-validated {C}ox Regression on Microarray Gene
                   Expression Data},
  volume =        {25},
  year =          {2006},
}

@techreport{vanderLaan&Rubin07,
  author =        {M.J. van der Laan and Daniel B. Rubin},
    institution =   {Division of Biostatistics, University of California,
                   Berkeley},
   number={226},
  title =         {A note on targeted maximum likelihood and right-censored data},
  year =          {2007},
}

@inproceedings{Robins93,
  author =        {J.M. Robins},
  booktitle =     {Proceedings of the Biopharmaceutical Section},
  organization =  {American Statistical Association},
  title =         {Information recovery and bias adjustment in
                   proportional hazards regression analysis of
                   randomized trials using surrogate markers},
  year =          {1993},
}

@incollection{Hubbard&vanderLaan&Robins99,
  address={Berlin Heidelberg New York},
  author =        {A.E. Hubbard and M.J. van der Laan and J.M. Robins},
  booktitle =     {Statistical models in epidemiology: the environment
                   and clinical trials},
  editor =        {E. Halloran, D. Berry},
   publisher =     {Springer},
  title =         {Nonparametric locally efficient estimation of the
                   treatment specific survival distributions with right
                   censored data and covariates in observational
                   studies},
  year =          {1999},
}

@article{Hernandez&Eijkemans&Steyerberg06,
  author =        {Hern\'{a}ndez, A.V. and Eijkemans, M.J. and
                   Steyerberg, E.W.},
  journal =       {Ann Epidemiol},
  number =        {1},
  pages =         {41--48},
  title =         {Randomized controlled trials With time-to-event
                   outcomes: how much does prespecified covariate
                   adjustment increase power?},
  volume =        {16},
  year =          {2006},
}

@article{Lu&Tsiatis08,
  author =        {Lu, X. and Tsiatis, A.A},
  journal =       {Biometrika},
  number =        {3},
  pages =         {679--694},
  title =         {Improving the efficiency of the log-rank test using
                   auxiliary covariates},
  volume =        {95},
  year =          {2008},
}

@article{Tangen&Koch99,
  author =        {Tangen, C.M. and Koch, G.G.},
  journal =       {J Biopharm Stat},
  number =        {2},
  pages =         {307--338},
  title =         {On-parametric analysis of covariance for hypothesis
                   testing with logrank and {W}ilcoxon scores and
                   survival-rate estimation in a randomized clinical
                   trial},
  volume =        {9},
  year =          {1999},
}

@article{Jiangetal08,
  author =        {Jiang, H. and Symanowski, J. and Paul, S. and Qu, Y. and
                   Zagar, A. and Hong, S.},
  journal =       {Stat Med},
  number =        {28},
  pages =         {5850--5860},
  title =         {The type {I} error and power of nonparametric logrank
                   and {W}ilcoxon tests with adjustment for covariates -- A
                   simulation study},
  volume =        {27},
  year =          {2008},
}

@article{Akazawa&Nakamura&Palesch97,
  author =        {Akazawa, K. and Nakamura, T. and Palesch, Y.},
  journal =       {Stat Med},
  number =        {5},
  pages =         {583--597},
  title =         {Power of logrank test and {C}ox regression model in
                   clinical trials with heterogenous samples},
  volume =        {16},
  year =          {1997},
}

@article{Westeretal10,
  author =        {C.W. Wester and A.M. Thomas and H. Bussmann and
                   S. Moyo and J.M. Gaolathe and V. Novitsky and
                   M. Essex and V. De Gruttola and R.G. Marlink},
  journal =       {AIDS},
  pages =         {S27--S36},
  title =         {Nonnucleoside reverse transcriptase inhibitor
                   outcomes among combination antiretroviral
                   therapy-treated adults in {B}otswana},
  volume =        {24},
  year =          {2010},
}

@book{Andersenetal93,
  author =        {P.K. Andersen and O. Borgan and R.D. Gill and
                   N. Keiding},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  title =         {Statistical models based on counting processes},
  year =          {1993},
}

@techreport{Rudser&LeBlanc&Emerson08,
  author =        {K. Rudser and M. LeBlanc and S.S. Emerson},
  institution={Department of Biostatistics, University of Washington},
  title =         {Estimation for Arbitrary Functionals of Survival},
  number =        {335},
  year =          {2008},
}

@article{vanderLaan10,
  author =        {van der Laan, M.J.},
  journal =       {Int J Biostat},
  pages =          {Article 2},
  number =        {2},
  title =         {Targeted maximum likelihood based causal inference:
                   Part {I}},
  volume =        {6},
  year =          {2010},
}

@article{vanderLaan10b,
  author =        {van der Laan, M.J.},
  journal =       {Int J Biostat},
  pages =          {Article 3},
  number =        {2},
  title =         {Targeted maximum likelihood based causal inference:
                   Part {II}},
  volume =        {6},
  year =          {2010},
}

@article{Sekhon08,
  author =        {J.S. Sekhon},
  journal =       {J Stat Softw},
  title =         {Multivariate and Propensity Score Matching Software
                   with Automated Balance Optimization: the Matching
                   package for {R}},
  year =          {2008},
}

@article{Holland&Reitman77,
  address =       {New York},
  author =        {J.H. Holland and J.S. Reitman},
  journal =       {SIGART Bull},
  pages =         {49--49},
  title =         {Cognitive systems based on adaptive algorithms},
  volume =        {63},
  year =          {1977},
}

@article{Koul&Susarla&vanRyzin81,
  author =        {H. Koul and V. Susarla and J. van Ryzin},
  journal =       {Ann Stat},
  pages =         {1276--88},
  title =         {Regression analysis with randomly right censored
                   data},
  volume =        {9},
  year =          {1981},
}

@article{Keiding&Hols&Green89,
  author =        {N. Keiding and C. Hols and A. Green},
  journal =       {Am J Epidemiol},
  pages =         {588--600},
  title =         {Retrospective estimation of diabetes incidence from
                   information in a current prevalent population and
                   historical mortality},
  volume =        {130},
  year =          {1989},
}

@article{Robins&Rotnitzky&Zhao94,
  author =        {J.M. Robins and A. Rotnitzky and L.P. Zhao},
  journal =       {J Am Stat Assoc},
  month =         {September},
  number =        {427},
  pages =         {846--66},
  title =         {Estimation of regression coefficients when some
                   regressors are not always observed},
  volume =        {89},
  year =          {1994},
}

@article{Robins&Rotnitzky95,
  author =        {Robins, J.M. and A. Rotnitzky},
  journal =       {J Am Stat Assoc},
  pages =         {122--129},
  title =         {Semiparametric Efficiency in Multivariate Regression
                   Models with Missing Data},
  volume =        {90},
  year =          {1995},
}

@article{Kang&Schafer07,
  author =        {J. Kang and J.L. Schafer},
  journal =       {Stat Sci},
  pages =         {523--39},
  title =         {Demystifying Double Robustness: a Comparison of
                   Alternative Strategies for Estimating a Population
                   Mean from Incomplete Data (with discussion)},
  volume =        {22},
  year =          {2007},
}

@article{Robins&Wang00,
  author =        {J.M. Robins and N. Wang},
  journal =       {Biometrika},
  pages =         {113--124},
  title =         {Inference for imputation estimators},
  volume =        {87},
  year =          {2000},
}

@techreport{Bhattacharya&Vogt07,
  author =        {Bhattacharya, J. and Vogt, W.},
  institution =          {National Bureau of
                   Economic Research},
  number={343},
  title =         {Do Instrumental Variables Belong in Propensity
                   Scores?},
  year =          {2007},
}

@techreport{Wooldridge09,
  author =        {Wooldridge, J.},
  institution={Michigan State University},
  type={Technical {R}eport},
  title =         {Should Instrumental Variables be Used as Matching
                   Variables?},
  year =          {2009},
}

@article{Pearl10,
  author =        {Pearl, J.},
  journal =       {Proceedings of Uncertainty in Artificial Intelligence},
  title =         {On a Class of Bias-Amplifying Variables that Endanger
                   Effect Estimates},
  year =          {2010},
}

@article{Holland86,
  author =        {Holland, P.W.},
  journal =       {J Am Stat Assoc},
  number =        {396},
  pages =         {945--960},
  title =         {Statistics and Causal Inference},
  volume =        {81},
  year =          {1986},
}

@book{Rubin06,
  address =       {Cambridge, MA},
  author =        {Donald B. Rubin},
  publisher =     {Cambridge},
  title =         {Matched sampling for causal effects.},
  year =          {2006},
}

@book{Rosenbaum02,
  address={Berlin Heidelberg New York},
  author =        {Rosenbaum, P.R.},
  edition =       {2nd},
  publisher =     {Springer},
  title =         {Observational studies},
  year =          {2002},
}

@article{Rubin97,
  author =        {Rubin, Donald B.},
  journal =       {Ann of Intern Med},
  number =        {8S},
  pages =         {757--763},
  title =         {Estimating causal effects from large data sets using
                   propensity scores},
  volume =        {127},
  year =          {1997},
}

@article{Christakis&Iwashyna03,
  author =        {Christakis, N.A. and Iwashyna, T.I.},
  journal =       {Soc Sci Med},
  number =        {3},
  pages =         {465--475},
  title =         {The Health Impact of Health Care on Families: a
                   matched cohort study of hospice use by decedents and
                   mortality outcomes in surviving, widowed spouses},
  volume =        {57},
  year =          {2003},
}

@article{Dehejia&Wahba02,
  author =        {R. Dehejia and S. Wahba},
  journal =       {Rev Econ Stat},
  number =        {1},
  pages =         {151--161},
  title =         {Propensity Score Matching Methods for Nonexperimental
                   Causal Studies},
  volume =        {84},
  year =          {2002},
}

@article{Galiani&Gertler&Schargrodsky05,
  author =        {Galiani, S. and P. Gertler and E. Schargrodsky},
  journal =       {J Polit Econ},
  number =        {1},
  pages =         {83--120},
  title =         {Water for Life: the Impact of the Privatization of
                   Water Services on Child Mortality},
  volume =        {113},
  year =          {2005},
}

@article{Abadie&Imbens06,
  author =        {Abadie, A. and G.W. Imbens},
  journal =       {Econometrica},
  pages =         {235--267},
  title =         {Large Sample Properties of Matching Estimators for
                   Average Treatment Effects},
  volume =        {74},
  year =          {2006},
}

@article{Herron&Wand07,
  author =        {Herron, M.C. and J. Wand},
  journal =       {Elect Stud},
  number =        {2},
  pages =         {247--261},
  title =         {Assessing Partisan Bias in Voting Technology: the
                   Case of the 2004 {N}ew {H}ampshire Recount},
  volume =        {26},
  year =          {2007},
}

@article{Imai05,
  author =        {K. Imai},
  journal =       {Am Polit Sci Rev},
  number =        {2},
  pages =         {283--300},
  title =         {Do Get-Out-The-Vote Calls Reduce Turnout? The
                   Importance of Statistical Methods for Field
                   Experiments},
  volume =        {99},
  year =          {2005},
}

@incollection{Sekhon08b,
  address =       {New York},
  author =        {Sekhon, J.S.},
  booktitle =     {The Oxford handbook of political methodology},
  editor =        {J.M. Box-Steffensmeier and H.E. Brady and
                   D. Collier},
  publisher =     {Oxford},
  title =         {The {N}eyman-{R}ubin Model of Causal Inference and
                   Estimation via Matching Methods},
  year =          {2008},
}

@article{Morgan&Harding06,
  author =        {Morgan, S.L. and D.J. Harding},
  journal =       {Sociol Meth Res},
  number =        {1},
  pages =         {3--60},
  title =         {Matching Estimators of Causal Effects: prospects and
                   Pitfalls in Theory and Practice},
  volume =        {35},
  year =          {2006},
}

@article{Diprete&Engelhardt04,
  author =        {Diprete, T.A. and H. Engelhardt},
  journal =       {Sociol Meth Res},
  number =        {4},
  pages =         {501--528},
  title =         {Estimating Causal Effects With Matching Methods in
                   the Presence and Absence of Bias Cancellation},
  volume =        {32},
  year =          {2004},
}

@article{Winship&Morgan99,
  author =        {Winship, C. and S.L. Morgan},
  journal =       {Annu Rev Sociol},
  pages =         {659--707},
  title =         {The estimation of causal effects from observational
                   data},
  volume =        {25},
  year =          {1999},
}

@article{Smith97,
  author =        {Smith, H.L.},
  journal =       {Sociol Meth},
  pages =         {305--353},
  title =         {Matching with Multiple Controls to Estimate Treatment
                   Effects in Observational Studies},
  volume =        {27},
  year =          {1997},
}

@article{Rubin02,
  author =        {Rubin, Donald B.},
  journal =       {Health Serv Outcome Res Meth},
  number =        {1},
  pages =         {169--188},
  title =         {Using Propensity Scores to Help Design Observational
                   Studies: application to the Tobacco Litigation},
  volume =        {2},
  year =          {2002},
}

@incollection{Brady08,
  address =       {New York},
  author =        {Brady, H.},
  booktitle =     {The Oxford handbook of political methodology},
  editor =        {J.M. Box-Steffensmeier and H.E. Brady and
                   D. Collier},
  publisher =     {Oxford},
  title =         {Causation and explanation in social science},
  year =          {2008},
}

@article{Freedman06,
  author =        {Freedman, D.A.},
  journal =       {Eval Rev},
  pages =         {691--713},
  title =         {Statistical Models for Causation: what Inferential
                   leverage Do They Provide?},
  volume =        {30},
  year =          {2006},
}

@article{Rubin90,
  author =        {Rubin, Donald B.},
  journal =       {Stat Sci},
  number =        {4},
  pages =         {472--480},
  title =         {Comment: {N}eyman (1923) and Causal Inference in
                   Experiments and Observational Studies},
  volume =        {5},
  year =          {1990},
}

@article{Speed90,
  author =        {T.P. Speed},
  journal =       {Stat Sci},
  number =        {4},
  pages =         {463--464},
  title =         {Introductory Remarks on {N}eyman (1923)},
  volume =        {5},
  year =          {1990},
}

@book{Cox58,
  address =       {New York},
  author =        {Cox, D.R.},
  publisher =     {Wiley},
  title =         {Planning of experiments},
  year =          {1958},
}

@article{Rubin78,
  author =        {Donald B. Rubin},
  journal =       {Ann Stat},
  number =        {},
  pages =         {34--58},
  title =         {Bayesian Inference for causal effects: the role of
                   randomization},
  volume =        {6},
  year =          {1978},
}

@incollection{Rubin75,
  address =       {Alexandria},
  author =        {Rubin, Donald B.},
  booktitle =     {The proceedings of the Social Statistics Section of
                   the American Statistical Association},
  publisher =     {American Statistical Association},
  title =         {Bayesian Inference for Causality: the Importance of
                   Randomization},
  year =          {1975},
}

@article{Rubin08,
  author =        {Rubin, Donald B.},
  journal =       {Ann of Appl Stat},
  number =        {3},
  pages =         {808--840},
  title =         {For Objective Causal Inference, Design Trumps
                   Analysis},
  volume =        {2},
  year =          {2008},
}

@article{Sekhon10,
  author =        {Sekhon, J.S.},
  journal =       {Annu Rev of Polit Sci},
  pages =         {487--508},
  title =         {Opiates for the Matches: matching Methods for Causal
                   Inference},
  volume =        {12},
  year =          {2010},
}

@article{Rubin76,
  author =        {Rubin, Donald B.},
  journal =       {Biometrics},
  number =        {1},
  pages =         {121--132},
  title =         {Multivariate Matching Methods That are Equal Percent
                   Bias Reducing, {II}: maximums on Bias Reduction for
                   Fixed Sample Sizes},
  volume =        {32},
  year =          {1976},
}

@article{Cochran&Rubin73,
  author =        {Cochran, W.G. and Donald B. Rubin},
  journal =       {Sankhya Ser A},
  pages =         {417--446},
  title =         {Controlling Bias in Observational Studies: a Review},
  volume =        {35},
  year =          {1973},
}

@book{Cochran83,
  address =       {New York},
  author =        {Cochran, W.G.},
  note =          {Edited posthumously by L.E. Moses and F. Mosteller},
  publisher =     {Wiley},
  title =         {Planning and analysis of observational studies},
  year =          {1983},
}

@article{Robinsetal07,
  author =        {J.M. Robins and M. Sued and Q. Lei-Gomez and
                   A. Rotnitzky},
  journal =       {Stat Sci},
  pages =         {544--559},
  title =         {Comment: {P}erformance of Double-Robust Estimators When
                   ``Inverse Probability'' Weights Are Highly Variable},
  volume =        {22},
  year =          {2007},
}

@article{Cortes&Vapnik95,
  author =        {C. Cortes and V. Vapnik},
  journal =       {Mach Learn},
  month =         {December},
  pages =         {273--297},
  title =         {Support-vector networks},
  volume =        {20},
  year =          {1995},
}

@techreport{Friedman94,
  author =        {J.H. Friedman},
  institution =   {Department of Statistics, Stanford University},
  type={Technical {R}eport},
  title =         {Flexible metric nearest neighbor classification},
  year =          {1994},
}

@techreport{FDA06,
  author =        {{Food and Drug Administration}},
  institution =   {U.S. Department of Health and Human Services, Food
                   and Drug Administration},
  type={Technical {R}eport},
  title =         {Critical Path Opportunities List},
  year =          {2006},
}

@article{Efronetal04,
  author =        {B. Efron and T. Hastie and I. Johnstone and
                   R. Tibshirani},
  journal =       {Ann Stat (with discussion)},
  number =        {2},
  pages =         {407--499},
  title =         {Least Angle Regression},
  volume =        {32},
  year =          {2004},
}

@techreport{Breiman99,
  author =        {L. Breiman},
  institution =   {Department of Statistics, University of California, Berkeley},
  number =        {567},
  title =         {Random forests - random features},
  year =          {1999},
}

@manual{Breiman01b,
  author =        {L. Breiman},
  title =         {Notes on setting up, using, and understanding random
                   forests V3.0},
  year =          {2001},
}

@article{Golubetal99,
  author =        {T.R. Golub and D.K. Slonim and P. Tamayo and C. Huard and
                   M. Gaasenbeek and J.P. Mesirov and H. Coller and
                   M.L. Loh and J.R. Downing and M.A. Caligiuri and
                   C.D. Bloomfield and E.S. Lander},
  journal =       {Science},
  pages =         {531--537},
  title =         {Molecular classification of cancer: class discovery
                   and class prediction by gene expression monitoring},
  volume =        {286},
  year =          {1999},
}

@article{vanderLaan06a,
  author =        {M.J. van der Laan},
  journal =       {Int J Biostat},
  number =        {1},
  pages =         {Article 2},
  title =         {Statistical Inference for Variable Importance},
  volume =        {2},
  year =          {2006},
}

@article{Robins&Mark&Newey92,
  author =        {J.M. Robins and S.D. Mark and W.K. Newey},
  journal =       {Biometrics},
  number =        {479--495},
  title =         {Estimating exposure effects by modelling the
                   expectation of exposure conditional on confounders},
  volume =        {48},
  year =          {1992},
}

@techreport{Yu&VanderLaan03,
  author =        {Z. Yu and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number={136},
  title =         {Measuring treatment effects using semiparametric
                   models},
  year =          {2003},
}

@techreport{Tuglus&vanderLaan08,
  author =        {C. Tuglus and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
number={233},
  title =         {Targeted Methods for Biomarker Discovery, the Search
                   for a Standard},
  year =          {2008},
}

@book{Hastie&Tibshirani90,
  address =       {London},
  author =        {T.J. Hastie and R.J. Tibshirani},
  publisher =     {Chapman \& Hall},
  title =         {Generalized additive models},
  year =          {1990},
}

@misc{Efron&Hastie07,
  author =        {B. Efron and T. Hastie},
  howpublished =  {R package},
  title =         {lars},
  year =          {2007},
}

@article{Benjamini&Hochberg95,
  author =        {Y. Benjamini and Y. Hochberg},
  journal =       {J R Stat Soc Ser B},
  pages =         {289--300},
  title =         {Controlling the false discovery rate: a practical and
                   powerful approach to multiple testing},
  volume =        {57},
  year =          {1995},
}

@misc{Ge&Dudoit02,
  author =        {Y. Ge and S. Dudoit},
  howpublished =  {R package},
  title =         {Multiple Testing Procedures, multtest},
  year =          {2002},
  url =           {www.bioconductor.org},
}

@article{Tibshirani96,
  author =        {R. Tibshirani},
  journal =       {J R Stat Soc Ser B},
  number =        {1},
  pages =         {267--288},
  title =         {Regression shrinkage and selection via the lasso.},
  volume =        {58},
  year =          {1996},
}

@article{Tuglus&vanderLaan09,
  author =        {C. Tuglus and M.J. van der Laan},
  journal =       {Stat Appl Genet Mol},
  number =        {1},
  pages =         {Article 12},
  title =         {Modified {FDR} Controlling Procedure for Multi-Stage
                   Analyses},
  volume =        {8},
  year =          {2009},
}

@article{Dudoit&Fridlyand&Speed02,
  author =        {S. Dudoit and J. Fridlyand and T. P. Speed},
  journal =       {J Am Stat Assoc},
  number =        {457},
  pages =         {77--87},
  title =         {Comparison of Discrimination Methods for the
                   Classification of Tumors Using Gene Expression Data},
  volume =        {97},
  year =          {2002},
}

@article{Kos&Lah98,
  author =        {J. Kos and T.T. Lah},
  journal =       {Oncol Rep},
  number =        {6},
  pages =         {1349--61},
  title =         {Cysteine proteinases and their endogenous inhibitors:
                   target proteins for prognosis, diagnosis and therapy
                   in cancer (review)},
  volume =        {5},
  year =          {1998},
}

@article{Vitaleetal01,
  author =        {C. Vitale and C. Romagnani and A. Puccetti and
                   D. Olive and R. Costello and L. Chiossone and
                   A. Pitto and A. Bacigalupo and L. Moretta and
                   M.C. Mingari},
  journal =       {Proc Natl Acad Sci},
  pages =         {5764--5769},
  title =         {Surface expression and function of p75/{AIRM}-1 or {CD}33
                   in acute myeloid leukemias: engagement of {CD}33
                   induces apoptosis of leukemic cells},
  volume =        {98},
  year =          {2001},
}

@article{Clappieretal07,
  author =        {E. Clappier and W. Cuccuini and A. Kalota and
                   A. Crinquette and J.M. Cayuela and W.A. Dik and
                   A.W. Langerak and B. Montpellier and B. Nadel and
                   P. Walrafen and O. Delattre and A. Aurias and
                   T. Leblanc and H. Dombret and A.M. Gewirtz and
                   A. Baruchel and F. Sigaux and J. Soulier},
  journal =       {Blood},
  number =        {4},
  pages =         {1251--61},
  title =         {The {C-MYB} locus is involved in chromosomal
                   translocation and genomic duplications in human
                   T-cell acute leukemia ({T-ALL}), the translocation
                   defining a new {T-ALL} subtype in very young children},
  volume =        {110},
  year =          {2007},
}

@article{Lane&Ley03,
  author =        {A.A. Lane and T.J. Ley},
  journal =       {Cell},
  number =        {305-318},
  title =         {Neutrophil elastase cleaves {PML-RAR}-alpha and is
                   important for the development of acute promyelocytic
                   leukemia in mice},
  volume =        {115},
  year =          {2003},
}

@article{Hunger96,
  author =        {S.P. Hunger},
  journal =       {Blood},
  pages =         {1211--1224},
  title =         {Chromosomal translocations involving the {E2A} gene in
                   acute lymphoblastic leukemia: clinical features and
                   molecular pathogenesis.},
  volume =        {87},
  year =          {1996},
}

@article{Nebraletal05,
  author =        {K. Nebral and H.H. Schmidt and O.A. Haas and
                   S. Strehl},
  journal =       {Clin Cancer Res},
  number =        {18},
  pages =         {6489--6494},
  title =         {{NUP}98 Is Fused to Topoisomerase {(DNA)} {II}{beta} 180
                   {kDa} {(TOP2B)} in a Patient with Acute Myeloid Leukemia
                   with a New {t(3;11)(p24;p15)}},
  volume =        {11},
  year =          {2005},
}

@article{Kaufmannetal98b,
  author =        {S.H. Kaufmann and S.D. Gore and C.B. Miller and
                   R.J. Jones and L.A. Zwelling and E. Schneider and
                   P.J. Burke and J.E. Karp},
  journal =       {Leukemia Lymphoma},
  month =         {Apr},
  number =        {3-4},
  pages =         {217--237},
  title =         {Topoisomerase {II} and the response to antileukemic
                   therapy},
  volume =        {29},
  year =          {1998},
}

@article{Kozaretal04,
  author =        {K. Kozar and M.A. Ciemerych and V.I. Rebel and
                   H. Shigematsu and A. Zagozdzon and E. Sicinska and
                   Y. Geng and Q. Yu and S. Bhattacharya and
                   R.T. Bronson and K. Akashi and P. Sicinski},
  journal =       {Cell},
  pages =         {477--491},
  title =         {Mouse development and cell proliferation in the
                   absence of {D}-cyclins},
  volume =        {118},
  year =          {2004},
}

@article{MartinSuberoetal07,
  author =        {J.I. Martin-Subero and R. Ibbotson and W. Klapper and
                   L. Michaux and E. Callet-Bauchu and F. Berger and
                   M.J. Calasanz and C. De Wolf-Peeters and M.J. Dyer and
                   P. Felman and A. Gardiner and R.D. Gascoyne and
                   S. Gesk and L. Harder and D.E. Horsman and M. Kneba and
                   R. Kuppers and A. Majid and N. Parry-Jones and
                   M. Ritgen and M. Salido and F. Sole and G. Thiel and
                   H.H. Wacker and D. Oscier and I. Wlodarska and
                   R. Siebert},
  journal =       {Leukemia},
  number =        {7},
  pages =         {1532--1544},
  title =         {A comprehensive genetic and histopathologic analysis
                   identifies two subgroups of {B}-cell malignancies
                   carrying a t(14;19)(q32;q13) or variant
                   {BCL3}-translocation},
  volume =        {21},
  year =          {2007},
}

@article{Palomeroetal06,
  author =        {T. Palomero and D.T. Odom and J. O'Neil and
                   A.A. Ferrando and A. Margolin and D.S. Neuberg and
                   S.S. Winter and R.S. Larson and W. Li and X.S. Liu and
                   R.A. Young and A.T. Look},
  journal =       {Blood},
  number =        {3},
  pages =         {986--992},
  title =         {Transcriptional regulatory networks downstream of
                   {TAL1/SCL} in {T}-cell acute lymphoblastic leukemia},
  volume =        {108},
  year =          {2006},
}

@article{Wongetal07,
  author =        {H.P. Wong and L. Yu and E.K. Lam and E.K. Tai and
                   W.K. Wu and C.H. Cho},
  journal =       {Toxicol Appl Pharm},
  number =        {3},
  pages =         {261--267},
  title =         {Nicotine promotes cell proliferation via
                   alpha7-nicotinic acetylcholine receptor and
                   catecholamine-synthesizing enzymes-mediated pathway
                   in human colon adenocarcinoma {HT}-29 cells.},
  volume =        {221},
  year =          {2007},
}

@article{Ramaswamyetal03,
  author =        {S. Ramaswamy and K.N. Ross and E.S. Lander and
                   T.R. Golub},
  journal =       {Nat Genet},
  pages =         {49--54},
  title =         {A molecular signature of metastasis in primary solid
                   tumors},
  volume =        {33},
  year =          {2003},
}

@article{Purietal01,
  author =        {R. Puri and A. Tousson and L. Chen and S.S. Kakar},
  journal =       {Cancer Lett},
  pages =         {131--139},
  title =         {Molecular cloning of pituitary tumor transforming
                   gene 1 from ovarian tumors and its expression in
                   tumors},
  volume =        {163},
  year =          {2001},
}

@article{Fujiietal06,
  author =        {T. Fujii and S. Nomoto and K. Koshikawa and Y.Yatabe and
                   O. Teshigawara and T. Mori and S. Inoue and S. Takeda and
                   A. Nakao},
  journal =       {Hepatology},
  pages =         {1267--1275},
  title =         {Overexpression of pituitary tumor transforming gene 1
                   in {HCC} is associated with angiogenesis and poor
                   prognosis},
  volume =        {43},
  year =          {2006},
}

@article{Zhuetal06,
  author =        {X. Zhu and Z. Mao and Y. Na and Y. Guo and X. Wang and
                   D. Xin},
  journal =       {Anticancer Res},
  pages =         {1253--1259},
  title =         {Significance of pituitary tumor transforming gene 1
                   ({PTTG1}) in prostate cancer},
  volume =        {26},
  year =          {2006},
}

@article{Kaufmannetal98a,
  author =        {S.H. Kaufmann and J.E. Karp and P.A. Svingen and
                   S. Krajewski and P.J. Burke and S.D. Gore and
                   J.C. Reed},
  journal =       {Blood},
  number =        {3},
  pages =         {991--1000},
  title =         {Elevated expression of the apoptotic regulator {Mcl}-1
                   at the time of leukemic relapse},
  volume =        {91},
  year =          {1998},
}

@article{Frumanetal99,
  author =        {D.A. Fruman and S.B. Snapper and C.M. Yballe and
                   L. Davidson and J.Y. Yu and F.W. Alt and
                   L.C. Cantley},
  journal =       {Science},
  pages =         {393--397},
  title =         {Impaired {B} cell development and proliferation in
                   absence of phosphoinositide 3-kinase p85-alpha},
  volume =        {283},
  year =          {1999},
}

@article{Tombes&Krystal97,
  author =        {R.M. Tombes and G.W. Krystal},
  journal =       {Biochim Biophys Acta},
  pages =         {281--292},
  title =         {Identification of novel human tumor cell-specific
                   {CaMK-II} variants},
  volume =        {1355},
  year =          {1997},
}

@article{Senturkeretal97,
  author =        {S. Senturker and B. Karahalil and M. Inal and
                   H. Yilmaz and H. Muslumanoglu and G. Gedikoglu and
                   M. Dizdaroglu},
  journal =       {FEBS Letters},
  number =        {3},
  pages =         {286--290},
  title =         {Oxidative {DNA} base damage and antioxidant enzyme
                   levels in childhood acute lymphoblastic leukemia},
  volume =        {416},
  year =          {1997},
}

@article{Komuroetal05,
  author =        {I. Komuro and T. Yasuda and A. Iwamoto and
                   K.S. Akagawa},
  journal =       {J Biol Chem},
  number =        {50},
  pages =         {41137--45},
  title =         {Catalase plays a critical role in the {CSF}-independent
                   survival of human macrophages via regulation of the
                   expression of {BCL}-2 family},
  volume =        {280},
  year =          {2005},
}

@article{Balciunaiteetal05,
  author =        {E. Balciunaite and A. Spektor and N.H. Lents and
                   H. Cam and H. Te Riele and A. Scime and M.A. Rudnicki and
                   R. Young and B.D. Dynlacht},
  journal =       {Mol Cell Biol},
  number =        {18},
  pages =         {8166--78},
  title =         {Pocket protein complexes are recruited to distinct
                   targets in quiescent and proliferating cells},
  volume =        {25},
  year =          {2005},
}

@article{Leoneetal01,
  author =        {G. Leone and R. Sears and E. Huang and R. Rempel and
                   F. Nuckolls and C.H. Park and P. Giangrande and L. Wu and
                   H.I. Saavedra and S.J. Field and M.A. Thompson and
                   H. Yang and Y. Fujiwara and M.E. Greenberg and
                   S. Orkin and C. Smith and J.R. Nevins},
  journal =       {Mol Cell},
  pages =         {105--113},
  title =         {Myc requires distinct {E2F} activities to induce {S}
                   phase and apoptosis},
  volume =        {8},
  year =          {2001},
}

@article{Sax23,
  author =        {Sax, K.},
  journal =       {Genetics},
  title =         {The association of size difference with seed-coat
                   pattern and pigmentation in \textit{Phaseolus
                   vulgaris}},
  year =          {1923},
}

@article{Thoday60,
  author =        {Thoday, J.M.},
  journal =       {Nature},
  title =         {Location of polygenes},
  year =          {1960},
}

@article{Lander&Botstein89,
  author =        {Lander, E.S. and Botstein, D.},
  journal =       {Genetics},
  title =         {Mapping {M}endelian factors underlying quantitative
                   traits using {RFLP} linkage maps},
  year =          {1989},
}

@article{Haley&Knott92,
  author =        {Haley, C.S. and Knott, S.A.},
  journal =       {Heredity},
  title =         {A simple regression method for mapping quantitative
                   trait loci in line crosses using flanking markers},
  year =          {1992},
}

@article{Jansen93,
  author =        {Jansen, R.C.},
  journal =       {Genetics},
  title =         {Interval mapping of multiple quantitative trait loci},
  year =          {1993},
}

@article{Zeng94,
  author =        {Zeng, Z.B.},
  journal =       {Genetics},
  title =         {Precision mapping of quantitative trait loci},
  year =          {1994},
}

@article{Kao&Zeng&Teasdale99,
  author =        {Kao, C.H. and Zeng, Z.B. and Teasdale, R.D.},
  journal =       {Genetics},
  title =         {Multiple interval mapping for quantitative trait
                   loci},
  year =          {1999},
}

@article{Satagopanetal96,
  author =        {Satagopan, J.M. and B.S. Yandell and M.A. Newton and
                   T.C. Osborn},
  journal =       {Genetics},
  title =         {A {B}ayesian approach to detect quantitative trait loci
                   using {M}arkov chain {M}onte {C}arlo},
  year =          {1996},
}

@article{Heath97,
  author =        {Heath, S.C.},
  journal =       {Am J Hum Genet},
  title =         {Markov chain {M}onte {C}arlo segregation and linkage
                   analysis of oligogenic models},
  year =          {1997},
}

@article{Sillanpaa&Arjas98,
  author =        {Sillanpaa, M.J. and Arjas, E.},
  journal =       {Genetics},
  title =         {Bayesian mapping of multiple quantitative trait loci
                   from incomplete inbred line cross data},
  year =          {1998},
}

@article{Leeetal08,
  author =        {Lee, S.S.F. and L. Sun and R. Kustra and S.B. Bull},
  journal =       {Bioinformatics},
  title =         {{EM}-random forest and new measures of variable
                   importance for multi-locus quantitative trait linkage
                   analysis},
  year =          {2008},
}

@article{Wang&Rose&vanderLaan10,
  author =        {H. Wang and S. Rose and M.J. van der Laan},
  journal =       {Stat Prob Lett},
  title =         {Finding quantitative Trait Loci Genes with
                   Collaborative Targeted Maximum Likelihood Learning},
  volume =        {published online 11 Nov (doi:
                   10.1016/j.spl.2010.11.001)},
  year =          {2010},
}

@techreport{Wang&Rose&vanderLaan11,
  author =        {H. Wang and S. Rose and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  type =          {Technical {R}eport},
  title =         {Targeted Methods for Finding Quantitative Trait Loci},
  year =          {2011},
}

@manual{Basten&Weir&Zeng01,
  author =        {C.J. Basten and B.S. Weir and Z.B. Zeng},
  title =         {QTL Cartographer},
  year =          {2001},
  url =           {http://statgen.ncsu.edu/qtlcart/},
}

@article{Masindeetal01,
  author =        {Masinde, G.L. and X. Li and W. Gu and H. Davidson and
                   S. Mohan and D.J. Baylink},
  journal =       {Genome Res},
  title =         {Identification of wound healing/regeneration
                   quantitative trait loci ({QTL}) at multiple time points
                   that explain seventy percent of variance in ({MRL/MpJ
                   and SJL/J}) mice {F2} population},
  year =          {2001},
}

@article{Boyartchuk01,
  author =        {Boyartchuk, V.L. and K.W. Broman and R.E. Mosher and
                   S.E.F. D'Orazio and M.N. Starnbach and W.F. Dietrich},
  journal =       {Nat Genet},
  title =         {Multigenic control of Listeria monocytogenes
                   susceptibility in mice},
  year =          {2001},
}

@article{Broman03,
  author =        {Broman, K.W.},
  journal =       {Genetics},
  title =         {Mapping quantitative trait loci in the case of a
                   spike in the phenotype distribution},
  year =          {2003},
}

@article{Jin&Fine&Yandell07,
  author =        {Jin, C. and J.P. Fine and B.S. Yandell},
  journal =       {J Am Stat Assoc},
  title =         {A unified semiparametric framework for quantitative
                   trait loci analysis, with application to spike
                   phenotypes},
  year =          {2007},
}

@article{Petersenetal08,
  author =        {M.L. Petersen and M.J. van der Laan and S. Napravnik and
                   J.J. Eron and R.D. Moore and S.G. Deeks},
  journal =       {AIDS},
  number =        {16},
  pages =         {2097--106},
  title =         {Long-term consequences of the delay between virologic
                   failure of highly active antiretroviral therapy and
                   regimen modification},
  volume =        {22},
  year =          {2008},
}

@article{Rodgeretal09,
  author =        {A.J. Rodger and Z. Fox and J.D. Lundgren and
                   J.L. Kuller and C. Boesecke and D. Gey and
                   A. Skoutelis and M.B. Goetz and A.N. Phillips and
                     {INSIGHT Strategies for Management of Antiretroviral
  Therapy (SMART) Study Group}},
  journal =       {J Infect Dis},
  number =        {6},
  pages =         {973--83},
  title =         {Activation and coagulation biomarkers are independent
                   predictors of the development of opportunistic
                   disease in patients with {HIV} infection.},
  volume =        {200},
  year =          {2009},
}

@article{Hammeretal08,
  author =        {S.M. Hammer and J.J. Eron and P. Reiss and
                   R.T. Schooley and M.A. Thompson and S. Walmsley and
                   P. Cahn and M.A. Fischl and J.M. Gatell and
                   M.S. Hirsch and D.M. Jacobsen and J.S.G. Montaner and
                   D.D. Richman and P.G. Yeni and P.A. Volberding},
  journal =       {J Am Med Asoc},
  number =        {5},
  pages =         {555--70},
  title =         {Antiretroviral treatment of adult {HIV} infection:
                   2008 recommendations of the {I}nternational {AIDS}
                   {S}ociety-{USA} panel},
  volume =        {300},
  year =          {2008},
}

@article{Stringeretal06,
  author =        {J.S. Stringer and I. Zulu and J. Levy and
                   E.M. Stringer and A. Mwango and B.H. Chi and
                   V. Mtonga and S. Reid and R.A. Cantrell and
                   M. Bulterys and M.S. Saag and R.G. Marlink and
                   A. Mwinga and T.V. Ellerbrock and M. Sinkala},
  journal =       {J Am Med Asoc},
  number =        {7},
  pages =         {782--93},
  title =         {Rapid scale-up of antiretroviral therapy at primary
                   care sites in {Z}ambia: feasibility and early outcomes},
  volume =        {296},
  year =          {2006},
}

@misc{WHO06,
  author =        {{{W}orld {H}ealth {O}rganization}},
  title =         {Antiretroviral therapy for {HIV} infection in adults
                   and adoloescents: recommendations for a public health
                   approach},
  year =          {2006},
}

@article{Reynoldsetal09,
  author =        {S.J. Reynolds and G. Nakigozi and K. Newell and
                   A. Ndyanabo and R. Galiwongo and I. Boaz and
                   T.C. Quinn and R. Gray and M. Wawer and D. Serwadda},
  journal =       {{AIDS}},
  number =        {6},
  pages =         {697--700},
  title =         {Failure of immunologic criteria to appropriately
                   identify antiretroviral treatment failure in {U}ganda},
  volume =        {23},
  year =          {2009},
}

@article{Petersenetal07,
  author =        {M.L Petersen and S.G. Deeks and J.N. Martin and
                   M.J. van der Laan},
  journal =       {Am J Epidemiol},
  number =        {9},
  pages =         {985--993},
  title =         {History-Adjusted Marginal Structural Models to
                   Estimate Time-Varying Effect Modification},
  volume =        {166},
  year =          {2007},
}

@article{Robins&Hernan&Rotnitzky07,
  author =        {J.M. Robins and M.A. Hernan and A. Rotnitzky},
  journal =       {Am J Epidemiol},
  number =        {9},
  pages =         {994--1002},
  title =         {Effect Modification by Time-varying Covariates},
  volume =        {166},
  year =          {2007},
}

@article{vanderLaan&Petersen&Joffe07,
  author =        {M.J. van der Laan and M.L. Petersen and M.M. Joffe},
  journal =       {Am J Epidemiol},
  number =        {9},
  pages =         {1003--1004},
  title =         {Response to Invited Commentary: {P}etersen et. al.
                   Respond to ``{E}ffect Modification by Time-varying
                   Covariates''},
  volume =        {166},
  year =          {2007},
}

@article{vanderLaan&Petersen07b,
  author =        {M.J. van der Laan and M.L. Petersen},
  journal =       {Int J Biostat},
  number =        {1},
  pages =         {Article 6},
  title =         {Statistical Learning of Origin-Specific Statically
                   Optimal Individualized Treatment Rules.},
  volume =        {3},
  year =          {2007},
}

@article{Petersen&Deeks&vanderLaan07,
  author =        {M.L. Petersen and S.G. Deeks and M.J. van der Laan},
  journal =       {Stat Med},
  number =        {25},
  pages =         {4578--601},
  title =         {Individualized Treatment Rules: generating Candidate
                   Clinical Trials.},
  volume =        {26},
  year =          {2007},
}

@article{vanderLaan&Petersen&Joffe05,
  author =        {M.J. van der Laan and M.L. Petersen and M.M. Joffe},
  journal =       {Int J Biostat},
  number =        {1},
  pages =         {10--20},
  title =         {History-Adjusted Marginal Structural Models and
                   Statically-Optimal Dynamic Treatment Regimens},
  volume =        {1},
  year =          {2005},
}

@article{Hernanetal06,
  author =        {M.A. Hernan and E. Lanoy and D. Costagliola and
                   J.M. Robins},
  journal =       {Basic Clin Pharmacol},
  pages =         {237--242},
  title =         {Comparison of dynamic treatment regimes via inverse
                   probability weighting.},
  volume =        {98},
  year =          {2006},
}

@techreport{vanderLaan08b,
  author =        {M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =          {232},
  title =         {The construction and analysis of adaptive group
                   sequential designs},
  year =          {2008},
}

@article{Boivinetal07,
  author =        {Boivin, J. and Bunting, L. and Collins, J.A. and
                   Nygren, K.G.},
  journal =       {Hum Reproduct},
  pages =        {1506--1512},
  title =         {International estimates of infertility prevalence and
                   treatment-seeking: potential need and demand for
                   infertility medical care},
  volume =        {22},
  year =          {2007},
}

@article{Adamsonetal06,
  author =        {Adamson, G.D. and de {M}ouzon, J. and Lancaster, P. and
                   Nygren, K.-G. and Sullivan, E. and
                   Zegers-Hochschild, F.},
  journal =       {Fertil Steril},
  pages =        {1586--1622},
  title =         {World collaborative report on in vitro fertilization,
                   2000},
  volume =        {85},
  year =          {2006},
}

@article{Soullieretal08,
  author =        {Soullier, N. and Bouyer, J. and Pouly J-L. and
                   Guibert, J. and de la {R}ochebrochard},
  journal =       {Hum Reproduct},
  pages =         {187--192},
  title =         {Estimating the success of an in vitro fertilization
                   programme using multiple imputation},
  volume =        {23},
  year =          {2008},
}

@article{delaRochebrochardetal08,
  author =        {de la {R}ochebrochard, E. and Soullier, N. and
                   Peikrishvili, R. and Guibert, J. and Bouyer, J.},
  journal =       {Int J Gynecol Obstet},
  pages =         {74--75},
  title =         {High in vitro fertilization discontinuation rate in
                   {F}rance},
  volume =        {103},
  year =          {2008},
}

@article{delaRochebrochardetal09,
  author =        {de la {R}ochebrochard, E. and Quelen, C. and
                   Peikrishvili, R. and Guibert, J. and Bouyer, J.},
  journal =       {Fertil Steril},
  pages =         {149--156},
  title =         {Long-term outcome of parenthood project during in
                   vitro fertilization and after discontinuation of
                   unscuccessful in vitro fertilization},
  volume =        {92},
  year =          {2009},
}

@book{Schafer97,
  address =       {London},
  author =        {Schafer, J.L.},
  publisher =     {Chapman \& Hall},
  title =         {Analysis of incomplete multivariate data},
  year =          {1997},
}

@book{Little&Rubin02,
  address =       {Hoboken},
  author =        {Little, R.J.A. and Rubin, Donald B.},
  edition =       {2nd},
  publisher =     {Wiley},
  title =         {Statistical analysis with missing data},
  year =          {2002},
}

@techreport{Yu&vanderLaan02,
  author =        {Z. Yu and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number={122},
  title =         {Construction of counterfactuals and the
                   G-computation formula},
  year =          {2002},
}

@article{Gill&Robins01,
  author =        {Gill, R.D. and Robins, J.M.},
  journal =       {Ann Stat},
  number =        {6},
  pages =         {1785--1811},
  title =         {Causal inference in complex longitudinal studies:
                   continuous case},
  volume =        {29},
  year =          {2001},
}

@techreport{DHHS04,
  author =        {{Department of Health and Human Services}},
  institution =   {Panel on Clinical Practices for Treatment of {HIV}
                   Infection},
type={Technical {R}eport},
  title =         {Guidelines for the use of antiretroviral agents in
                   {HIV}-1 infected adults and adolescents},
  year =          {2004},
}

@article{CDC92,
  author =        {{Centers for Disease Control and Prevention}},
  journal =       {Morbid Mortal W Rep},
  pages =         {1--19},
  title =         {{1993 revised classification system for {HIV} infection
                   and expanded surveillance case definition for AIDS
                   among adolescents and adults}},
  volume =        {41},
  year =          {1992},
}

@incollection{Selbyetal05,
  author =        {J.V. Selby and D.H. Smith and E.S. Johnson and
                   M.A. Raebel and G.D. Friedman and B.H. McFarland},
  booktitle =     {Pharmacoepidemiology},
  editor =        {B.L. Strom},
  publisher =     {Wiley},
  title =         {Kaiser {P}ermanente Medical Care Program},
  year =          {2005},
}

@techreport{Neugebauer&Silverberg&vanderLaan10,
  author =        {R. Neugebauer and M.J. Silverberg and
                   M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  type =          {272},
  title =         {Observational Study and Individualized Antiretroviral
                   Therapy Initiation Rules for Reducing Cancer
                   Incidence in {HIV}-Infected Patients},
  year =          {2010},
}




@techreport{Stitelmanetal11,
  author =        {O.M. Stitelman and V. De Gruttola and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  type =          {Technical {R}eport 281, http://www.bepress.com/ucbbiostat/paper281},
  title =         {A General Implementation of TMLE for Longitudinal Data Applied to Causal Inference in Survival Analysis},
  year =          {2011},
}
@techreport{Stitelman&vanderLaan11,
  author =        {O.M. Stitelman and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  type =          {Technical {R}eport},
  title =         {Targeted Maximum Likelihood Estimation of
                   Time-To-Event Parameters With Time-Dependent
                   Covariates},
  year =          {2011},
}

@article{Thalletal07,
  author =        {P.F. Thall and C. Logothetis and L.C. Pagliaro and
                   S. Wen and M.A. Brown and D. Williams and
                   R.E. Millikan},
  journal =       {J Natl Cancer Inst},
  pages =         {1613--22},
  title =         {Adaptive Therapy for Androgen-Independent Prostate
                   Cancer: a randomized Selection Trial of Four
                   Regimens},
  volume =        {99},
  year =          {2007},
}

@article{Bembom&vanderLaan07a,
  author =        {O. Bembom and M.J. van der Laan},
  journal =       {J Natl Cancer Inst},
  pages =         {1577--1582},
  title =         {Comment: Statistical Methods for analyzing sequentially
                   randomized trials},
  volume =        {99(21)},
  year =          {2007},
}

@techreport{Zheng&vanderLaan10,
  author =        {W. Zheng and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =          {273},
  title =         {Asymptotic Theory for Cross-validated Targeted
                   Maximum Likelihood Estimation},
  year =          {2010},
}

@techreport{Zheng&vanderLaan11,
  author =        {W. Zheng and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =          {288},
  title =         {Targeted Maximum Likelihood Estimation of Natural Direct Effect},
  year =          {2011},
}

@book{Robert07,
  address={Berlin Heidelberg New York},
  author =        {Robert, P.C.},
  publisher =     {Springer},
  title =         {{T}he {B}ayesian choice: from
                   decision-thoeretic foundations to
                   computational implementation},
  year =          {2007},
}

@book{Lindley80,
  address =       {Cambridge, MA},
  author =        {Lindley, D.V.},
  publisher =     {Cambridge},
  title =         {{I}ntroduction to probability and statistics from
                   a {B}ayesian point of view, {P}art 2},
  year =          {1980},
}

@article{Golub06,
  author =        {Golub, H.L.},
  journal =       {Stat Med},
  pages =         {3231--3235},
  title =         {The need for more efficient trial designs},
  volume =        {25},
  year =          {2006},
}

@article{Emerson06,
  author =        {Emerson, S.S.},
  journal =       {Stat Med},
  pages =         {3270--3296},
  title =         {Issues in the use of adaptive clinical trial designs},
  volume =        {25},
  year =          {2006},
}

@book{Hu&Rosenberger06,
address = {New York},
  author =        {F. Hu and W.F. Rosenberger},
  publisher =     {Wiley},
  title =         {The theory of response adaptive randomization in
                   clinical trials},
  year =          {2006},
}

@book{Jennison&Turnbull00,
  address =       {Boca Raton},
  author =        {Jennison, C. and Turnbull, B.W.},
  editor =        {},
  publisher =     {Chapman \& Hall},
  title =         {Group sequential methods with applications to
                   clinical trials},
  year =          {2000},
}

@article{Rosenberger96,
  author =        {W.F. Rosenberger},
  journal =       {Stat Sci},
  number =        {},
  pages =         {137--149},
  title =         {New directions in adaptive designs},
  volume =        {11},
  year =          {1996},
}

@techreport{Chambaz&vanderLaan10,
  author =        {Chambaz, A. and van der Laan, M.J.},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
   number={258},
  title =         {Targeting the optimal design in randomized clinical
                   trials with binary outcomes and no covariate},
  year =          {2010},
}

@article{Rosenberger&Vidyashankar&Agarwal01,
  author =        {Rosenberger, W.F. and Vidyashankar, A.N. and
                   Agarwal, D.K.},
  journal =       {J Biopharm Stat},
  number =        {227--236},
  title =         {Covariate-adjusted response-adaptive designs for
                   binary response},
  volume =        {11},
  year =          {2001},
}

@article{Bandyopadhyay&Biswas01,
  author =        {Bandyopadhyay, U. and Biswas, A.},
  journal =       {Biometrika},
  number =        {2},
  pages =         {409--419},
  title =         {Adaptive designs for normal responses with prognostic
                   factors},
  volume =        {88},
  year =          {2001},
}

@article{Atkinson&Biswas05,
  author =        {Atkinson, A.C. and Biswas, A.},
  journal =       {Stat Med},
  number =        {16},
  pages =         {2477--2492},
  title =         {Adaptive biased-coin designs for skewing the
                   allocation proportion in clinical trials with normal
                   responses},
  volume =        {24},
  year =          {2005},
}

@article{Zhangetal07,
  author =        {Zhang, L.-X. and Hu, F.-F. and Cheung, S.H. and
                   Chan, W.S.},
  journal =       {Ann Stat},
  number =        {3},
  pages =         {1166--1182},
  title =         {Asymptotic properties of covariate-adjusted
                   response-adaptive designs},
  volume =        {35},
  year =          {2007},
}

@article{Zhang&Hu09,
  author =        {Zhang, L.-X. and Hu, F.-F.},
  journal =       {Appl Math J Chinese Univ Ser B},
  number =        {1},
  pages =         {1--13},
  title =         {A new family of covariate-adjusted response adaptive
                   designs and their properties},
  volume =        {24},
  year =          {2009},
}

@article{Shao&Yu&Zhong10,
  author =        {Shao, J. and Yu, X. and Bob Zhong, B.},
  journal =       {Biometrika},
  title =         {A theory for testing hypotheses under
                   covariate-adaptive randomization},
  year =          {2010},
}

@article{Gill89,
  author =        {Gill, R.D.},
  journal =       {Scand J Stat},
  title =         {Non- and semiparametric maximum likelihood estimators
                   and the Von {M}ises method (Part 1)},
  year =          {1989},
}

@article{Tan08,
  author =        {Z. Tan},
  journal =       {Int J Biostat},
  pages =         {Article 10},
  title =         {Comment: {I}mproved Local Efficiency and Double
                   Robustness},
  volume =        {4},
  number={1},
  year =          {2008},
}

@techreport{Gruber&vanderLaan11,
  author =        {S. Gruber and M.J. van der Laan},
  institution =   {Division of Biostatistics, University of California,
                   Berkeley},
  number =        {275},
  type =          {Technical Report},
  title =         {{tmle}: an {R} Package for Targeted Maximum Likelihood
                   Estimation},
  year =          {2011},
}

@proceedings{DBLP:conf/colt/2003,
  booktitle =     {COLT},
  editor =        {B. Sch{\"o}lkopf and M.K. Warmuth},
  publisher =     {Springer},
    address={Berlin Heidelberg New York},
  series =        {Lecture Notes in Computer Science},
  title =         {Computational Learning Theory and Kernel Machines,
                   16th Annual Conference on Computational Learning
                   Theory and 7th Kernel Workshop, COLT/Kernel 2003,
                   Washington, DC, USA, August 24-27, 2003, Proceedings},
  volume =        {2777},
  year =          {2003},
}

@proceedings{DBLP:conf/nips/2005,
  booktitle =     {NIPS},
  title =         {Advances in Neural Information Processing Systems 18
                   [Neural Information Processing Systems, NIPS 2005,
                   December 5-8, 2005, Vancouver, British Columbia,
                   Canada]},
  year =          {2005},
}

@proceedings{DBLP:conf/colt/2006,
  booktitle =     {COLT},
  editor =        {G. Lugosi and H.-U. Simon},
  publisher =     {Springer},
  series =        {Lecture Notes in Computer Science},
    address={Berlin Heidelberg New York},
  title =         {Learning Theory, 19th Annual Conference on Learning
                   Theory, COLT 2006, Pittsburgh, PA, USA, June 22-25,
                   2006, Proceedings},
  volume =        {4005},
  year =          {2006},
}



@ARTICLE{Diaz11,
title = {Super Learner Based Conditional Density Estimation with Application to Marginal Structural Models},
author = {D\'iaz, Iv\'an and van der Laan, Mark},
year = {2011},
journal = {The International Journal of Biostatistics},
volume = {7},
number = {1},
pages = {38},
}

@article {Diaz12,
author = {Iv\'an D\'iaz and van der Laan, Mark},
title = {Population Intervention Causal Effects Based on Stochastic Interventions},
journal = {Biometrics},
volume = {68},
number = {2},
publisher = {Blackwell Publishing Inc},
issn = {1541-0420},
pages = {541--549},
keywords = {Causal effect, Counterfactual outcome, Double robustness, Stochastic intervention, Targeted maximum likelihood estimation},
year = {2012},
}

@article{Diaz13,
title={Sensitivity Analysis for Causal Inference Under Unmeasured Confounding and Measurement Error Problems},
author={D{\'\i}az, Iv{\'a}n and van der Laan, Mark J},
year= {\noop{2013}In press},
journal={International Journal of Biostatistics}
}

@article{Diaz13,
title={Assessing the Causal Effect of Policies: An Example Using Stochastic Interventions},
author={D{\'\i}az, Iv{\'a}n and van der Laan, Mark J},
year= {\noop{2013}In press},
journal={International Journal of Biostatistics}
}


@incollection{Diaz11a,
year={2011},
isbn={978-1-4419-9781-4},
booktitle={Targeted Learning},
series={Springer Series in Statistics},
title={Targeted Bayesian Learning},
publisher={Springer New York},
author={Iv\'an D\'iaz and Hubbard, Alan E. and van der Laan, Mark J.},
pages={475-493},
language={English}
}

@article{Diaz13,
title={Targeted Data Adaptive Estimation of the Causal Dose Response Curve},
author={D{\'\i}az, Iv{\'a}n and van der Laan, Mark J},
year= {\noop{2013}In press},
journal={Journal of Causal Inference},
}


@ARTICLE{Diaz11,
title = {Super Learner Based Conditional Density Estimation with Application to Marginal Structural Models},
author = {D\'iaz, Iv\'an and van der Laan, Mark},
year = {2011},
journal = {The International Journal of Biostatistics},
volume = {7},
number = {1},
pages = {38},
}

@article {Diaz12,
author = {Iv\'an D\'iaz and van der Laan, Mark},
title = {Population Intervention Causal Effects Based on Stochastic Interventions},
journal = {Biometrics},
volume = {68},
number = {2},
publisher = {Blackwell Publishing Inc},
issn = {1541-0420},
pages = {541--549},
keywords = {Causal effect, Counterfactual outcome, Double robustness, Stochastic intervention, Targeted maximum likelihood estimation},
year = {2012},
}

@article{Diaz13,
title={Sensitivity Analysis for Causal Inference Under Unmeasured Confounding and Measurement Error Problems},
author={D{\'\i}az, Iv{\'a}n and van der Laan, Mark J},
year= {\noop{2013}In press},
journal={International Journal of Biostatistics}
}

@article{Diaz13,
title={Assessing the Causal Effect of Policies: An Example Using Stochastic Interventions},
author={D{\'\i}az, Iv{\'a}n and van der Laan, Mark J},
year= {\noop{2013}In press},
journal={International Journal of Biostatistics}
}


@incollection{Diaz11a,
year={2011},
isbn={978-1-4419-9781-4},
booktitle={Targeted Learning},
series={Springer Series in Statistics},
title={Targeted Bayesian Learning},
publisher={Springer New York},
author={Iv\'an D\'iaz and Hubbard, Alan E. and van der Laan, Mark J.},
pages={475-493},
language={English}
}

@article{Diaz13,
title={Targeted Data Adaptive Estimation of the Causal Dose Response Curve},
author={D{\'\i}az, Iv{\'a}n and van der Laan, Mark J},
year= {\noop{2013}In press},
journal={Journal of Causal Inference},
}


@ARTICLE{Diaz11,
title = {Super Learner Based Conditional Density Estimation with Application to Marginal Structural Models},
author = {D\'iaz, Iv\'an and van der Laan, Mark},
year = {2011},
journal = {The International Journal of Biostatistics},
volume = {7},
number = {1},
pages = {38},
}

@article {Diaz12,
author = {Iv\'an D\'iaz and van der Laan, Mark},
title = {Population Intervention Causal Effects Based on Stochastic Interventions},
journal = {Biometrics},
volume = {68},
number = {2},
publisher = {Blackwell Publishing Inc},
issn = {1541-0420},
pages = {541--549},
keywords = {Causal effect, Counterfactual outcome, Double robustness, Stochastic intervention, Targeted maximum likelihood estimation},
year = {2012},
}

@article{Diaz13,
title={Sensitivity Analysis for Causal Inference Under Unmeasured Confounding and Measurement Error Problems},
author={D{\'\i}az, Iv{\'a}n and van der Laan, Mark J},
year= {\noop{2013}In press},
journal={International Journal of Biostatistics}
}

@article{Diaz13,
title={Assessing the Causal Effect of Policies: An Example Using Stochastic Interventions},
author={D{\'\i}az, Iv{\'a}n and van der Laan, Mark J},
year= {\noop{2013}In press},
journal={International Journal of Biostatistics}
}


@incollection{Diaz11a,
year={2011},
isbn={978-1-4419-9781-4},
booktitle={Targeted Learning},
series={Springer Series in Statistics},
title={Targeted Bayesian Learning},
publisher={Springer New York},
author={Iv\'an D\'iaz and Hubbard, Alan E. and van der Laan, Mark J.},
pages={475-493},
language={English}
}

@article{Diaz13,
title={Targeted Data Adaptive Estimation of the Causal Dose Response Curve},
author={D{\'\i}az, I. and van der Laan, M. J.},
year= {2013},
journal={Journal of Causal Inference},
volume={1},
number={2},
pages={171--192},
}



@ARTICLE{Diaz11,
title = {Super Learner Based Conditional Density Estimation with Application to Marginal Structural Models},
author = {D\'iaz, Iv\'an and van der Laan, Mark},
year = {2011},
journal = {The International Journal of Biostatistics},
volume = {7},
number = {1},
pages = {38},
}

@article {Diaz12,
author = {Iv\'an D\'iaz and van der Laan, Mark},
title = {Population Intervention Causal Effects Based on Stochastic Interventions},
journal = {Biometrics},
volume = {68},
number = {2},
publisher = {Blackwell Publishing Inc},
issn = {1541-0420},
pages = {541--549},
keywords = {Causal effect, Counterfactual outcome, Double robustness, Stochastic intervention, Targeted maximum likelihood estimation},
year = {2012},
}

@article{Diaz13,
title={Sensitivity Analysis for Causal Inference Under Unmeasured Confounding and Measurement Error Problems},
author={D{\'\i}az, Iv{\'a}n and van der Laan, Mark J},
year= {\noop{2013}In press},
journal={International Journal of Biostatistics}
}

@article{Diaz13,
title={Assessing the Causal Effect of Policies: An Example Using Stochastic Interventions},
author={D{\'\i}az, Iv{\'a}n and van der Laan, Mark J},
year= {\noop{2013}In press},
journal={International Journal of Biostatistics}
}


@incollection{Diaz11a,
year={2011},
isbn={978-1-4419-9781-4},
booktitle={Targeted Learning},
series={Springer Series in Statistics},
title={Targeted Bayesian Learning},
publisher={Springer New York},
author={Iv\'an D\'iaz and Hubbard, Alan E. and van der Laan, Mark J.},
pages={475-493},
language={English}
}

@article{Diaz13,
title={Targeted Data Adaptive Estimation of the Causal Dose Response Curve},
author={D{\'\i}az, Iv{\'a}n and van der Laan, Mark J},
year= {\noop{2013}In press},
journal={Journal of Causal Inference},
}
%% This BibTeX bibliography file was created using BibDesk.
%% http://bibdesk.sourceforge.net/


%% Created for Laura Balzer at 2012-08-26 21:21:41 -0700


%% Saved with string encoding Unicode (UTF-8)

@article{Chambaz&vanderLaan11a,
Title={Targeting The Optimal Design In Randomized Clinical Trials With Binary Outcomes And No Covariate, Theoretical Study},	Author = {A. Chambaz and M.J. van der Laan},
	Journal = {Int J Biostat},
	Note = {Working paper 258, www.bepress.com/ucbbiostat},
	Number = {1},
	Pages = {1-32},
	Volume = {7},
	Year = {2011}}

	@article{Chambaz&vanderLaan11b,
Title={Targeting The Optimal Design In Randomized Clinical Trials With Binary Outcomes And No Covariate, Simulation Study},	Author = {A. Chambaz and M.J. van der Laan},
	Journal = {Int J Biostat},
	Note = {Working paper 258,www.bepress.com/ucbbiostat},
	Number = {1},
	Pages = {33-},
	Volume = {7},
	Year = {2011}}


@article{Dawid&Didelez10,
Title={Identifying the consequences of dynamic treatment strategies: A decision theoretic overview},
Author = {A. Dawid and V. Didelez},
	Journal = {Statistics Surveys},
	Note = {},
	Number = {4},
	Pages = {184--231},
	Volume = {},
	Year = {2010}}

@inproceedings{Polley2009,
	Address = {Boca Raton},
	Author = {E.C. Polley and M.J. van der Laan},
	Booktitle = {Design and Analysis Clinical Trials with Time-to-Event Endpoints},
	Date-Added = {2012-08-26 20:23:48 -0700},
	Date-Modified = {2012-08-26 20:25:05 -0700},
	Editor = {Karl E. Peace},
	Keywords = {App},
	Publisher = {Chapman \& Hall/CRC},
	Title = {Selecting Optimal Treatments Based on Predictive Factors},
	Year = {2009}}

@article{Arnold2009,
	Author = {B. Arnold and B. Arana and D. M\"{a}usezahl and A. Hubbard and J.M. Colford},
	Date-Added = {2012-08-26 20:07:08 -0700},
	Date-Modified = {2012-08-26 20:08:37 -0700},
	Journal = {Int J Biostat},
	Note = {PMCID: PMC2786251},
	Number = {6},
	Pages = {1651-1661},
	Title = {Evaluation of a pre-existing, 3-year household water treatment and handwashing intervention in rural Guatemala},
	Volume = {38},
	Year = {2009}}

@article{Odden2011,
	Author = {M.C. Odden and I.B. Tager and M.J. van der Laan and J.A Delaney and C.A. Peralta and R. Katz and M.J. Sarnak and B.M. Psaty and M.G. Shlipak},
	Date-Added = {2012-08-26 20:00:36 -0700},
	Date-Modified = {2012-08-26 20:02:31 -0700},
	Journal = {Int J Biostat},
	Keywords = {App},
	Note = {PMCID: PMC3204667},
	Number = {1},
	Pages = {Article 34},
	Title = {Antihypertensive medication use and change in kidney function in elderly adults: a marginal structural model analysis},
	Volume = {7},
	Year = {2011}}

@unpublished{Josh2012,
	Author = {M. Petersen and J. Schwab and M. van der Laan},
	Date-Added = {2012-08-26 16:32:16 -0700},
	Date-Modified = {2012-08-26 21:08:43 -0700},
	Note = {Unpublished, Division of Biostatistics, University of California, Berkeley},
	Title = {Estimating the impact of clinic-based interventions},
	Year = {2012}}

@book{Bickel1993,
	Address = {Baltimore},
	Author = {Bickel, P.J. and Klaassen, C.A.J. and Ritov, Y. and Wellner, J.A.},
	Date-Added = {2012-08-26 15:53:44 -0700},
	Date-Modified = {2012-08-26 15:55:11 -0700},
	Keywords = {book},
	Publisher = {Johns Hopkins University Press},
	Title = {{Efficient and Adaptive Estimation for Semiparametric Models}},
	Year = {1993}}

@article{Rosenblum2011,
	Author = {M. Rosenblum and M.J. van der Laan},
	Date-Added = {2012-08-26 01:25:31 -0700},
	Date-Modified = {2012-08-26 01:30:42 -0700},
	Journal = {Biometrika},
	Number = {4},
	Pages = {845--860},
	Title = {Optimizing randomized trial designs to distinguish which subpopulations benefit from treatment},
	Volume = {98},
	Year = {2011}}

@unpublished{Geeven2012,
	Author = {G. Geeven and M.J. van der Laan and M.C.M. de Gunst},
	Date-Added = {2012-08-26 01:09:47 -0700},
	Date-Modified = {2012-08-26 21:05:35 -0700},
	Keywords = {unpub},
	Note = {Unpublished, Division of Biostatistics, University of California, Berkeley},
	Title = {Comparison of targeted maximum likelihood and shrinkage estimators of parameters in gene networks},
	Year = {2012}}

@unpublished{Brooks2012,
	Author = {J. Brooks and M.J. van der Laan},
	Date-Added = {2012-08-26 01:08:46 -0700},
	Date-Modified = {2012-08-26 21:05:29 -0700},
	Note = {Unpublished, Division of Biostatistics, University of California, Berkeley},
	Title = {Targeted Maximum Likelihood Estimation for Prediction Calibration},
	Year = {2012}}

@article{Tuglus2011,
	Author = {C. Tuglus and M.J. van der Laan},
	Date-Added = {2012-08-26 00:51:25 -0700},
	Date-Modified = {2012-08-26 00:52:39 -0700},
	Journal = {Stat Appl Genet Mol Biol},
	Keywords = {App},
	Note = {PMCID: PMC3122882},
	Number = {1},
	Pages = {Article 2},
	Title = {Repeated measures semiparametric regression using targeted maximum likelihood methodology with application to transcription factor activity discovery},
	Volume = {10},
	Year = {2011}}

@article{Wang2011,
	Author = {H. Wang and M.J. van der Laan},
	Date-Added = {2012-08-26 00:41:51 -0700},
	Date-Modified = {2012-08-26 00:42:47 -0700},
	Journal = {BMC Bioinformatics},
	Keywords = {App},
	Note = {PMCID: PMC3166941},
	Number = {312},
	Title = {Dimension Reduction Procedure Using Targeted Variable Importance Measurement},
	Volume = {12},
	Year = {2011}}

@article{Moore2011,
	Author = {K.L. Moore and R. Neugebauer and T. Valappil and M.J. van der Laan},
	Date-Added = {2012-08-26 00:17:52 -0700},
	Date-Modified = {2012-08-26 00:19:34 -0700},
	Journal = {Stat Med},
	Note = {PMID: 21751231},
	Number = {19},
	Pages = {2389--2408},
	Title = {Robust extraction of covariate information to improve estimation efficiency in randomized trials},
	Volume = {30},
	Year = {2011}}

@article{Chaffee2012,
	Author = {P.H. Chaffee and M.J. van der Laan},
	Date-Added = {2012-08-25 23:46:42 -0700},
	Date-Modified = {2012-08-25 23:47:53 -0700},
	Journal = {Int J Biostat},
	Keywords = {Simulation},
	Note = {PMID: 22740582},
	Number = {1},
	Pages = {Article 14},
	Title = {Targeted maximum likelihood estimation for dynamic treatment regimes in sequentially randomized controlled trials},
	Volume = {8},
	Year = {2012}}

@article{Atkinson2010,
	Author = {R.W. Atkinson and G.W. Fuller and H.R. Anderson and R.M. Harrison and B. Armstrong},
	Date-Added = {2012-08-25 22:10:07 -0700},
	Date-Modified = {2012-08-25 22:11:33 -0700},
	Journal = {Epidemiology},
	Keywords = {Aim3},
	Note = {PMID: 20502338},
	Number = {4},
	Pages = {501-511},
	Title = {Urban ambient particle metrics and health:a time-series analysis},
	Volume = {21},
	Year = {2010}}

@article{Catalano2006,
	Author = {R. Catalano and T. Bruckner and A.R. Marks and B. Eskenazi},
	Date-Added = {2012-08-25 22:03:01 -0700},
	Date-Modified = {2012-08-25 22:04:09 -0700},
	Journal = {Hum Reprod},
	Keywords = {Aim3},
	Note = {PMID: 16936298},
	Number = {12},
	Pages = {3127-3131},
	Title = {Exogenous shocks to the human sex ratio: the case of {S}eptember 11, 2001 in {N}ew {Y}ork {C}ity},
	Volume = {21},
	Year = {2006}}

@article{Eskenazi2007,
	Author = {B. Eskenazi and A.R. Marks and R. Catalano and T. Bruckner and P.G. Toniolo},
	Date-Added = {2012-08-25 21:57:52 -0700},
	Date-Modified = {2012-08-25 21:59:23 -0700},
	Journal = {Hum Reprod},
	Keywords = {Aim3},
	Number = {11},
	Pages = {3013-3020},
	Title = {Low birthweight in {N}ew {Y}ork {C}ity and upstate {N}ew {Y}ork following the events of {S}eptember 11th},
	Volume = {22},
	Year = {2007}}

@article{Diaz&vanderLaan12,
	Author = {I. Diaz and M.J. van der Laan},
	Date-Added = {},
	Date-Modified = {},
	Journal = {Biometrics, to appear},
	Keywords = {},
	Number = {},
	Pages = {},
	Title = {Population intervention causal effects based on stochastic interventions},
	Volume = {},
	Year = {2012}}

@article{Imbens2007,
	Author = {G.W. Imbens and T. Lemieux},
	Date-Added = {2012-08-25 21:48:32 -0700},
	Date-Modified = {2012-08-25 21:55:33 -0700},
	Journal = {J Econom},
	Keywords = {Aim3},
	Number = {2},
	Pages = {615--635},
	Title = {Regression discontinuity designs: {A} guide to practice},
	Volume = {142},
	Year = {2008}}

@article{Imbens2009,
	Author = {G.W. Imbens and J.M. Wooldridge},
	Date-Added = {2012-08-25 20:46:14 -0700},
	Date-Modified = {2012-08-25 20:46:57 -0700},
	Journal = {J Econ Lit},
	Keywords = {Aim3},
	Number = {1},
	Pages = {5-86},
	Title = {Recent Developments in the Econometrics of Program Evaluation},
	Volume = {47},
	Year = {2009}}

@article{Sobel2006,
	Author = {M.E. Sobel},
	Date-Added = {2012-08-25 17:38:58 -0700},
	Date-Modified = {2012-08-26 20:36:23 -0700},
	Journal = {J Am Stat Assoc Asoc},
	Keywords = {Aim2},
	Number = {476},
	Pages = {1398--1407},
	Title = {What Do Randomized Studies of Housing Mobility Demonstrate?: {C}ausal inference in the face of interference},
	Volume = {101},
	Year = {2006}}

@article{Hong2006,
	Author = {G. Hong and S.W. Raudenbush},
	Date-Added = {2012-08-25 17:31:23 -0700},
	Date-Modified = {2012-08-25 17:49:36 -0700},
	Journal = {J Am Stat Assoc},
	Keywords = {Aim2},
	Number = {475},
	Pages = {901--910},
	Title = {Evaluating Kindergarten Retention Policy: {A} Case Study of Causal Inference for Multilevel Observational Data},
	Volume = {101},
	Year = {2006}}

@article{Halloran&Struchiner95,
	Author = {M.E. Halloran and C.J. Struchiner},
	Date-Added = {2012-08-25 17:27:15 -0700},
	Date-Modified = {2012-08-25 17:28:57 -0700},
	Journal = {Epidemiology},
	Keywords = {Aim2},
	Note = {PMID: 7742400},
	Number = {2},
	Pages = {142-151},
	Title = {Causal inference in infectious diseases},
	Volume = {6},
	Year = {1995}}

@article{Hudgens&Halloran08,
	Author = {M.G. Hudgens and M.E. Halloran},
	Date-Added = {2012-08-25 15:30:45 -0700},
	Date-Modified = {2012-08-25 15:32:14 -0700},
	Journal = {J Am Stat Assoc},
	Keywords = {Aim2},
	Note = {PMCID: PMC2600548},
	Number = {482},
	Pages = {832--842},
	Title = {Toward {C}ausal {I}nference {W}ith {I}nterference},
	Volume = {103},
	Year = {2008},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAZgAAAAAAZgAAgAADE1hY2ludG9zaCBIRAAAAAAAAAAAAAAAAAAAAMobz/1IKwAABsaXyhAyMDA4X0h1ZGdlbnMucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAHSNyEzF6XmgAAAAAAAAAAAAEAAgAACSAAAAAAAAAAAAAAAAAAAAAKTGl0ZXJhdHVyZQAQAAgAAMocMm0AAAARAAgAAMxe+goAAAABABAGxpfKAAxX9QAMUlIAAAAeAAIAPE1hY2ludG9zaCBIRDpVc2VyczpsYXVyYTpEZXNrdG9wOkxpdGVyYXR1cmU6MjAwOF9IdWRnZW5zLnBkZgAOACIAEAAyADAAMAA4AF8ASAB1AGQAZwBlAG4AcwAuAHAAZABmAA8AGgAMAE0AYQBjAGkAbgB0AG8AcwBoACAASABEABIAL1VzZXJzL2xhdXJhL0Rlc2t0b3AvTGl0ZXJhdHVyZS8yMDA4X0h1ZGdlbnMucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAeLi4vTGl0ZXJhdHVyZS8yMDA4X0h1ZGdlbnMucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAjwCPgJDAkwCVwJbAmkCcAJ5ApoCnwKiAq8CtAAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAALG}}

@article{Tchetgen&vanderWeele12,
	Author = {E.J. {Tchetgen Tchetgen} and T.J. VanderWeele},
	Date-Added = {2012-08-25 15:28:32 -0700},
	Date-Modified = {2012-08-25 17:48:19 -0700},
	Journal = {Stat Meth Med Res},
	Keywords = {Aim2},
	Note = {PMID: 21068053},
	Number = {1},
	Pages = {55-75},
	Title = {On causal inference in the presence of interference},
	Volume = {21},
	Year = {2012}}

@article{vanderWeeleetal12,
	Author = {T.J. VanderWeele and J.P. Vandenbrouke and E.J. {Tchetgen Tchetgen} and J.M. Robins},
	Date-Added = {2012-08-25 13:41:16 -0700},
	Date-Modified = {2012-08-25 17:52:19 -0700},
	Journal = {Epidemiology},
	Keywords = {Aim2},
	Note = {PMID: 22317812},
	Number = {3},
	Pages = {285--292},
	Title = {A mapping between interactions and interference: implications for vaccine trials},
	Volume = {23},
	Year = {2012},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAagAAAAAAagAAgAADE1hY2ludG9zaCBIRAAAAAAAAAAAAAAAAAAAAMobz/1IKwAABsaXyhQyMDEyX1ZhbmRlcldlZWxlLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAHSPAnzF6GJQAAAAAAAAAAAAEAAgAACSAAAAAAAAAAAAAAAAAAAAAKTGl0ZXJhdHVyZQAQAAgAAMocMm0AAAARAAgAAMxe6JUAAAABABAGxpfKAAxX9QAMUlIAAAAeAAIAQE1hY2ludG9zaCBIRDpVc2VyczpsYXVyYTpEZXNrdG9wOkxpdGVyYXR1cmU6MjAxMl9WYW5kZXJXZWVsZS5wZGYADgAqABQAMgAwADEAMgBfAFYAYQBuAGQAZQByAFcAZQBlAGwAZQAuAHAAZABmAA8AGgAMAE0AYQBjAGkAbgB0AG8AcwBoACAASABEABIAM1VzZXJzL2xhdXJhL0Rlc2t0b3AvTGl0ZXJhdHVyZS8yMDEyX1ZhbmRlcldlZWxlLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QIi4uL0xpdGVyYXR1cmUvMjAxMl9WYW5kZXJXZWVsZS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACTAJOAlMCXAJnAmsCeQKAAokCrgKzArYCwwLIAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAto=}}

@book{Fitzmaurice2004,
	Address = {Hoboken},
	Author = {G.M. Fitzmaurice and N.M. Laird and J.H. Ware},
	Date-Added = {2012-08-25 13:17:30 -0700},
	Date-Modified = {2012-08-25 13:20:50 -0700},
	Keywords = {book},
	Publisher = {John Wiley \& Sons},
	Title = {Applied {L}ongitudinal {A}nalysis},
	Year = {2004}}

@booklet{UNAIDS,
	Address = {Johannesburg, Republic of South Africa},
	Author = {{UNAIDS RST-ESA}},
	Date-Added = {2012-08-24 17:33:29 -0700},
	Date-Modified = {2012-08-24 17:42:29 -0700},
	Keywords = {HIV},
	Note = {Avaliable at \url{http://www.unaidsrstesa.org/media-corner/factsheets/high-level-meeting-aids-implication-estern-and-southern-africa}},
	Title = {High level meeting on {AIDS}: {I}mplication for {E}aster and {S}outhern {A}frica},
	Year = {2012},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAX4AAAAAAX4AAgAADE1hY2ludG9zaCBIRAAAAAAAAAAAAAAAAAAAAMobz/1IKwAABq+JbwpVTkFJRFMucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAHRmOizF1rYQAAAAAAAAAAAAEAAgAACSAAAAAAAAAAAAAAAAAAAAAJR3JhbnQyMDEyAAAQAAgAAMocMm0AAAARAAgAAMxdzdEAAAABABAGr4lvAAxX9QAMUlIAAAAeAAIANU1hY2ludG9zaCBIRDpVc2VyczpsYXVyYTpEZXNrdG9wOkdyYW50MjAxMjpVTkFJRFMucGRmAAAOABYACgBVAE4AQQBJAEQAUwAuAHAAZABmAA8AGgAMAE0AYQBjAGkAbgB0AG8AcwBoACAASABEABIAKFVzZXJzL2xhdXJhL0Rlc2t0b3AvR3JhbnQyMDEyL1VOQUlEUy5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdFpVTkFJRFMucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAiICJAIpAjICPQJBAk8CVgJfAmoCbwJyAn8ChAAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKW}}

@conference{Zheng2011community,
	Address = {Ann Habor, MI},
	Author = {W. Zheng and M.J. van der Laan and M.L. Petersen},
	Booktitle = {Atlantic Causal Inference Conference},
	Date-Added = {2012-08-24 14:08:26 -0700},
	Date-Modified = {2012-08-24 14:11:36 -0700},
	Keywords = {Community},
	Title = {Causal inference for community based studies with few communities},
	Year = {2011}}

@conference{Balzer2012wnar,
	Address = {Fort Collins, CO},
	Author = {L. Balzer and M. Petersen and J. Schwab and M. van der Laan},
	Booktitle = {WNAR},
	Date-Added = {2012-08-24 11:58:45 -0700},
	Date-Modified = {2012-08-24 12:04:14 -0700},
	Keywords = {community},
	Title = {Estimating the impact of community-level interventions: {T}he {SEARCH} {T}rial and {HIV} {P}revention in {S}ub-{S}aharan {A}frica},
	Year = {2012}}

@incollection{Chpt24,
	Address = {New York Dordrecht Heidelberg London},
	Author = {M.L. Petersen and M.J. van der Laan},
	Booktitle = {Targeted Learning: Causal Inference for Observational and Experimental Data},
	Date-Added = {2012-08-24 11:01:37 -0700},
	Date-Modified = {2012-08-24 11:02:54 -0700},
	Editor = {van der Laan, M.J. and Rose, S.},
	Keywords = {Chpt4},
	Publisher = {Springer},
	Title = {Case {S}tudy: {L}ongitudinal {HIV} {C}ohort {D}ata},
	Year = {2011}}

@incollection{vanderLaan2012sl,
	Address = {New York Dordrecht Heidelberg London},
	Author = {M.J. van der Laan and M.L. Petersen},
	Booktitle = {{Ensemble Machine Learning}},
	Date-Added = {2012-08-24 10:43:01 -0700},
	Date-Modified = {2012-08-24 10:50:07 -0700},
	Editor = {C. Zhang and Y. Ma},
	Keywords = {Superlearner},
	Publisher = {Springer},
	Title = {Targeted {L}earning},
	Year = {2012}}

@incollection{Chpt6,
	Address = {New York Dordrecht Heidelberg London},
	Author = {S. Rose and M.J. van der Laan},
	Booktitle = {Targeted Learning: Causal Inference for Observational and Experimental Data},
	Date-Added = {2012-08-24 10:19:20 -0700},
	Date-Modified = {2012-08-24 10:20:25 -0700},
	Editor = {van der Laan, M.J. and Rose, S.},
	Keywords = {Chpt6},
	Publisher = {Springer},
	Title = {Why {TMLE}?},
	Year = {2011}}

@techreport{Pearl2010transport,
	Author = {J. Pearl and E. Bareinboim},
	Date-Added = {2012-08-24 09:47:13 -0700},
	Date-Modified = {2012-08-24 09:48:55 -0700},
	Institution = {Computer Science Department, University of California, Los Angeles},
	Keywords = {Other},
	Number = {R-372},
	Title = {Transportability across studies: {A} formal approach},
	Url = {ftp://www.mmss.cs.ucla.edu/pub/stat_ser/r372.pdf},
	Year = {2012},
	Bdsk-Url-1 = {ftp://www.mmss.cs.ucla.edu/pub/stat_ser/r372.pdf}}

@article{VanderWeele2009,
	Author = {T.J. VanderWeele},
	Date-Added = {2012-08-23 18:19:15 -0700},
	Date-Modified = {2012-08-23 18:20:15 -0700},
	Journal = {Epidemiology},
	Keywords = {Aim2},
	Note = {PMID: 19234398},
	Number = {1},
	Pages = {18-26},
	Title = {Marginal structural models for the estimation of direct and indirect effects},
	Volume = {20},
	Year = {2009}}

@article{Petersen2006b,
	Author = {M.L. Petersen and S.E. Sinisi and M.J. van der Laan},
	Date-Added = {2012-08-23 18:16:52 -0700},
	Date-Modified = {2012-08-23 18:18:16 -0700},
	Journal = {Epidemiology},
	Keywords = {Aim2},
	Note = {PMID: 16617276},
	Number = {3},
	Pages = {276--284},
	Title = {Estimation of direct causal effects},
	Volume = {17},
	Year = {2006}}

@article{Cain2010,
	Author = {L.E. Cain and J.M. Robins and E. Lanoy and R. Logan and D. Costagliola and M.A. Hern\'{a}n},
	Date-Added = {2012-08-23 18:13:50 -0700},
	Date-Modified = {2012-08-26 21:02:08 -0700},
	Journal = {Int J Biostat},
	Keywords = {Aim1},
	Note = {PMCID: PMC3406513},
	Number = {2},
	Pages = {Article 18},
	Title = {When to start treatment? {A} systematic approach to the comparison of dynamic regimes using observational data},
	Volume = {6},
	Year = {2010}}

@article{Hernan2009b,
	Author = {M.A. Hern\'{a}n and J.M. Robins},
	Date-Added = {2012-08-23 18:07:50 -0700},
	Date-Modified = {2012-08-23 18:09:24 -0700},
	Journal = {N Engl J Med},
	Keywords = {Aim1},
	Note = {PMID: 19701984},
	Number = {8},
	Pages = {823--824},
	Title = {{Comment on: Early versus deferred antiretroviral therapy for HIV on survival}},
	Volume = {361},
	Year = {2009}}

@article{Kitahata2009,
	Date-Added = {2012-08-23 18:04:16 -0700},
	Date-Modified = {2012-08-23 18:05:43 -0700},
	Journal = {N Engl J Med},
	Keywords = {Aim1},
	Note = {PMCID: PMC2854555},
	Number = {18},
	Pages = {1815--1826},
	Title = {{Effect of early versus deferred antiretroviral therapy for HIV on survival}},
	Volume = {360},
	Year = {2009}}

@article{Bodnar2004,
	Author = {L.M. Bodnar and M. Davidian and A.M. Siega-Riz and A.A. Tsiatis},
	Date-Added = {2012-08-23 18:00:22 -0700},
	Date-Modified = {2012-08-23 18:00:22 -0700},
	Journal = {Am J Epidemiol},
	Keywords = {Aim1},
	Note = {PMID: 15128604},
	Number = {10},
	Pages = {926--934},
	Title = {{Marginal Structural Models for Analyzing Causal Effects of Time-dependent Treatments: An Application in Perinatal Epidemiology}},
	Volume = {159},
	Year = {2004}}

@article{Hernan2009,
	Author = {M.A. Hern\'{a}n and S.R. Cole},
	Date-Added = {2012-08-23 17:31:04 -0700},
	Date-Modified = {2012-08-23 17:32:34 -0700},
	Journal = {Am J Epidemiol},
	Keywords = {Roadmap},
	Note = {PMCID: PMC2765368},
	Number = {8},
	Pages = {959--962 with discussion 963-963},
	Title = {{Invited Commentary: Causal diagrams and measurement bias}},
	Volume = {170},
	Year = {2009}}

@incollection{Robins2009,
	Address = {Boca Raton, FL},
	Author = {J.M. Robins and M.A. Hern\'{a}n},
	Booktitle = {{Longitudinal Data Analysis}},
	Chapter = {23},
	Date-Added = {2012-08-23 17:26:46 -0700},
	Date-Modified = {2012-08-23 17:43:10 -0700},
	Editor = {G. Fitzmaurice and M. Davidian and G. Verbeke and G. Molenberghs},
	Keywords = {Aim2},
	Publisher = {Chapman \& Hall/CRC},
	Title = {{Estimation of the causal effects of time-varying exposures}},
	Year = {2009}}

@article{Hernan2006b,
	Author = {M.A. Hern\'{a}n and J.M. Robins},
	Date-Added = {2012-08-23 17:07:52 -0700},
	Date-Modified = {2012-08-23 17:09:25 -0700},
	Journal = {J Epidemiol Community Health},
	Keywords = {Aim2},
	Note = {PMCID: PMC2652882},
	Number = {7},
	Pages = {578--586},
	Title = {Estimating causal effects from epidemiological data},
	Volume = {60},
	Year = {2006}}

@article{Munoz2011,
	Annote = {DOI: 10.2202/1557-4679.1356},
	Author = {I. D\'{i}az Munoz and M.J. van der Laan},
	Date-Added = {2012-08-23 16:58:00 -0700},
	Date-Modified = {2012-08-26 21:03:47 -0700},
	Journal = {Int J Biostat},
	Keywords = {Superlearner},
	Note = {PMID: 22718677},
	Pages = {Article 38},
	Title = {Super learner based conditional density estimation with application to marginal structural models},
	Volume = {7},
	Year = {2011}}

@article{Houssaini2012,
	Author = {A. Houssa\"{i}ni and L. Assoumou and A.G. Marcelin and J.M. Calvez and P. Flandre},
	Date-Added = {2012-08-23 16:54:44 -0700},
	Date-Modified = {2012-08-23 16:57:15 -0700},
	Journal = {AIDS Res Treat},
	Keywords = {Superlearner},
	Note = {PMCID: PMC3324131},
	Number = {Article ID 478467},
	Pages = {Epub},
	Title = {{Investigation of Super Learner Methodology on HIV-1 Small Sample: Application on Jaguar Trial Data}},
	Volume = {2012},
	Year = {2012}}

@article{Sinisi2007,
	Annote = {. doi:  10.2202/1544-6115.1240},
	Author = {S.E. Sinisi and E.C. Polley and M.L. Petersen and M.J. van der Laan},
	Date-Added = {2012-08-23 14:06:15 -0700},
	Date-Modified = {2012-08-23 16:51:18 -0700},
	Journal = {Stat Appl Genet Mol},
	Keywords = {Superlearner},
	Note = {PMCID: PMC2473869},
	Number = {Article 7},
	Pages = {Epub},
	Read = {0},
	Title = {{Super learning: an application to the prediction of HIV-1 drug resistance}},
	Volume = {6},
	Year = {2007}}

@article{Petersen2006,
	Author = {M.L. Petersen and Y. Wang and M.J. van der Laan and D.R. Bangsberg},
	Date-Added = {2012-08-23 13:56:04 -0700},
	Date-Modified = {2012-08-23 14:04:00 -0700},
	Journal = {J Acquir Immune Defic Syndr},
	Keywords = {Aim1},
	Note = {PMID: 17133209},
	Number = {Suppl 1},
	Pages = {S96--S103},
	Title = {{Assessing the effectiveness of antiretroviral adherence interventions. Using marginal structural models to replicate the findings of randomized controlled trials}},
	Volume = {43},
	Year = {2006}}

@article{Hernan2004,
	Author = {M.A. Hern\'{a}n and S. Hern\'{a}ndez-D\'{i}az and J.M. Robins},
	Date-Added = {2012-08-23 10:56:44 -0700},
	Date-Modified = {2012-08-23 10:58:39 -0700},
	Journal = {Epidemiology},
	Keywords = {Roadmap},
	Note = {PMID: 15308962},
	Number = {5},
	Pages = {615--625},
	Title = {A structural approach to selection bias},
	Volume = {15},
	Year = {2004}}

@article{Robins1999,
	Author = {J.M. Robins},
	Date-Added = {2012-08-23 10:53:51 -0700},
	Date-Modified = {2012-08-23 10:55:18 -0700},
	Journal = {Synthese},
	Keywords = {Roadmap + MSM},
	Number = {1-2},
	Pages = {151-179},
	Title = {{Association, Causation, and Marginal Structural Models}},
	Volume = {121},
	Year = {1999}}

@article{Greenland1999,
	Author = {S. Greenland and J. Pearl and J.M. Robins},
	Date-Added = {2012-08-23 10:33:03 -0700},
	Date-Modified = {2012-08-23 10:34:19 -0700},
	Journal = {Epidemiology},
	Keywords = {Roadmap},
	Note = {PMID: 9888278},
	Number = {1},
	Pages = {37--48},
	Title = {Causal diagrams for empirical research.},
	Volume = {10},
	Year = {1999}}

@article{Pearl2009b,
	Author = {J. Pearl},
	Date-Added = {2012-08-23 10:29:27 -0700},
	Date-Modified = {2012-08-26 20:45:51 -0700},
	Journal = {Statist Surv},
	Keywords = {Roadmap},
	Pages = {96--146},
	Title = {{Causal inference in statistics: An overview}},
	Volume = {3},
	Year = {2009},
	Bdsk-Url-1 = {http://www.i-journals.org/ss/viewarticle.php?id=57}}

@incollection{GreenlandPearl2007,
	Address = {Thousand Oaks},
	Author = {S. Greenland and J. Pearl},
	Booktitle = {Encyclopedia of Epidemiology},
	Date-Added = {2012-08-23 10:11:07 -0700},
	Date-Modified = {2012-08-26 20:45:23 -0700},
	Editor = {S. Boslaugh},
	Keywords = {Roadmap},
	Pages = {149--156},
	Publisher = {SAGE Publications},
	Title = {Causal Diagrams},
	Volume = {1},
	Year = {2007}}

@incollection{Pearl2012,
	Address = {New York},
	Annote = {Technical report available at ftp://pike.cs.ucla.edu/pub/stat_ser/r370.pdf},
	Author = {J. Pearl},
	Booktitle = {Handbook of Structural Equation Modeling},
	Chapter = {5},
	Date-Added = {2012-08-23 09:41:04 -0700},
	Date-Modified = {2012-08-26 20:46:32 -0700},
	Editor = {R. Hoyle},
	Institution = {Computer Science Department, University of California, Los Angeles},
	Keywords = {Roadmap},
	Pages = {68--91},
	Publisher = {Guilford Press},
	Title = {The Causal Foundations of Structural Equation Modeling},
	Volume = {R-370},
	Year = {2012}}

@article{Lighthouse2012,
	Annote = {http://www.ncbi.nlm.nih.gov/pubmed/22808948},
	Author = {C. Feldacker and H. Tweya and O. Keiser and R. Weigel and M. Kalulu and L. Fenner and M. Egger and E. Manda and J.B. Mwafilaso and C. Kamba and S. Phiri},
	Date-Added = {2012-08-22 22:26:03 -0700},
	Date-Modified = {2012-08-22 22:29:06 -0700},
	Journal = {Trop Med Int Health},
	Keywords = {HIV},
	Note = {PMID: 22808948},
	Title = {{Characteristics of adults and children diagnosed with tuberculosis in Lilongwe, Malawi: findings from an integrated HIV/TB clinic}},
	Volume = {Epub ahead of print},
	Year = {2012}}

@conference{LREC2010,
	Address = {Presentation \# THAE0305, Vienna, Austria},
	Author = {K. Wools-Kaloustian and R. Kosgei and S. Kimaiyo and P. Braitstein and E. Sang and B. Musick and C. Yiannoutsos and A. Siika},
	Booktitle = {{XVIII International AIDS Conference}},
	Date-Added = {2012-08-22 22:21:13 -0700},
	Date-Modified = {2012-08-26 20:35:11 -0700},
	Keywords = {HIV},
	Title = {{Low risk express care: A nurse-centered model for the management of stable patients on combination antiretroviral therapy (cART)}},
	Year = {2010}}

@article{Young2011,
	Author = {J.G. Young and L.E. Cain and J.M. Robins and E.J. O'Reilly and M.A. Hern\'{a}n},
	Date-Added = {2012-08-22 22:11:06 -0700},
	Date-Modified = {2012-08-26 20:34:12 -0700},
	Journal = {Stat Biosci},
	Keywords = {Aim1},
	Pages = {119-143},
	Title = {Comparative Effectiveness of Dynamic Treatment Regimes: An Application of the Parametric G-Formula},
	Volume = {3},
	Year = {2011}}

@article{Taubman2009,
	Author = {S.L. Taubman and J.M. Robins and M.A. Mittleman and M.A. Hern\'{a}n},
	Date-Added = {2012-08-22 21:46:33 -0700},
	Date-Modified = {2012-08-22 22:09:34 -0700},
	Journal = {Int J Epidemiol},
	Keywords = {Aim1},
	Note = {PMCID: PMC2786249},
	Number = {6},
	Pages = {1599--1611},
	Title = {Intervening on risk factors for coronary heart disease: an application of the parametric g-formula},
	Volume = {38},
	Year = {2009}}

@article{Cain2011,
	Author = {{HIV-CAUSAL Collaboration} and L.E. Cain and R. Logan and J.M. Robins and J.A. Sterne and C. Sabin and L. Bansi and A. Justice and J. Goulet and A. van Sighem and F. de Wolf and H.C. Bucher and V. von Wyl and A. Esteve and J. Casabona and J. del Amo and S. Moreno and R. Seng and L. Meyer and S. Perez-Hoyos and R. Muga and S. Lodi and E. Lanoy and D. Costagliola and M.A. Hern\'{a}n},
	Date-Added = {2012-08-22 21:36:52 -0700},
	Date-Modified = {2012-08-22 21:43:12 -0700},
	Journal = {Ann Intern Med},
	Keywords = {Aim1},
	Note = {PMID: 21502648},
	Number = {8},
	Pages = {509-515},
	Title = {{When to initiate combined antiretroviral therapy to reduce mortality and AIDS-defining illness in HIV-infected persons in developed countries: an observational study}},
	Volume = {154},
	Year = {2011}}

@article{DART2010,
	Author = {{DART Trial Team}},
	Date-Added = {2012-08-22 21:23:22 -0700},
	Date-Modified = {2012-08-22 21:24:46 -0700},
	Journal = {Lancet},
	Keywords = {HIV},
	Note = {PMCID: PMC280572},
	Number = {9709},
	Pages = {123-131},
	Title = {{Routine versus clinically driven laboratory monitoring of HIV antiretroviral therapy in Africa (DART): a randomised non-inferiority trial}},
	Volume = {375},
	Year = {2010}}

@conference{Saag2012,
	Address = {Paper \#87, Seattle, WA},
	Author = {M. Saag and A. Westfall and D. Luhanga and P. Mulenga and B. Chi and L. Mulenga and R. Cantrell and A. Mwango and J. Koethe and J. Stringer},
	Booktitle = {CROI},
	Date-Added = {2012-08-22 21:18:33 -0700},
	Date-Modified = {2012-08-26 20:32:56 -0700},
	Keywords = {HIV},
	Title = {A Cluster Randomized Trial of Routine vs Discretionary Viral Load Monitoring among Adults Starting {ART}: {Z}ambia.},
	Year = {2012}}

@article{Cohen2011,
	Author = {M.S. Cohen and Y.Q. Chen and M. McCauley and T. Gamble and M.C. Hosseinipour and N. Kumarasamy and J.G. Hakim and J. Kumwenda and B. Grinsztejn and J.H. Pilotto and S.V. Godbole and S. Mehendale and S. Chariyalertsak and B.R. Santos and K.H. Mayer and I.F. Hoffman and S.H. Eshleman and E. Piwowar-Manning and L. Wang and J. Makhema and L.A. Mills and G. de Bruyn and I. Sanne and J. Eron and J. Gallant and D. Havlir and S. Swindells and H. Ribaudo and V. Elharrar and D. Burns and T.E. Taha and K. Nielsen-Saines and D. Celentano and M. Essex and T.R. Fleming},
	Date-Added = {2012-08-22 11:31:09 -0700},
	Date-Modified = {2012-08-22 21:04:10 -0700},
	Journal = {N Engl J Med},
	Keywords = {HIV},
	Note = {PMCID: PMC3200068},
	Number = {6},
	Pages = {493-505},
	Title = {{Prevention of HIV-1 infection with early antiretroviral therapy}},
	Volume = {365},
	Year = {2011}}

@article{Green2008,
	Author = {L.W. Green},
	Date-Added = {2012-08-22 11:23:38 -0700},
	Date-Modified = {2012-08-22 11:25:49 -0700},
	Journal = {Fam Pract},
	Keywords = {HIV},
	Note = {PMID: 18794201},
	Number = {Suppl1},
	Pages = {i20-i24},
	Title = {{Making research relevant: if it is an evidence-based practice, where's the practice-based evidence?}},
	Volume = {25},
	Year = {2006}}

@article{Jamshidian2011,
	Author = {F. Jamshidian and A.E. Hubbard and N.P. Jewell},
	Date-Added = {2012-08-22 09:29:55 -0700},
	Date-Modified = {2012-08-26 21:04:37 -0700},
	Journal = {Stat Meth Med Res},
	Keywords = {Application},
	Note = {PMID: 21908418},
	Title = {Accounting for perception, placebo and unmasking effects in estimating treatment effects in randomised clinical trials},
	Year = {2011},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAagAAAAAAagAAgAADE1hY2ludG9zaCBIRAAAAAAAAAAAAAAAAAAAAMobz/1IKwAABsaXyhQyMDExXyBKYW1zaGlkaWFuLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAHPD5UzFpW1AAAAAAAAAAAAAEAAgAACSAAAAAAAAAAAAAAAAAAAAAKTGl0ZXJhdHVyZQAQAAgAAMocMm0AAAARAAgAAMxauUQAAAABABAGxpfKAAxX9QAMUlIAAAAeAAIAQE1hY2ludG9zaCBIRDpVc2VyczpsYXVyYTpEZXNrdG9wOkxpdGVyYXR1cmU6MjAxMV8gSmFtc2hpZGlhbi5wZGYADgAqABQAMgAwADEAMQBfACAASgBhAG0AcwBoAGkAZABpAGEAbgAuAHAAZABmAA8AGgAMAE0AYQBjAGkAbgB0AG8AcwBoACAASABEABIAM1VzZXJzL2xhdXJhL0Rlc2t0b3AvTGl0ZXJhdHVyZS8yMDExXyBKYW1zaGlkaWFuLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QIi4uL0xpdGVyYXR1cmUvMjAxMV8gSmFtc2hpZGlhbi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACTAJOAlMCXAJnAmsCeQKAAokCrgKzArYCwwLIAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAto=}}

@article{Gruber2012,
	Author = {S. Gruber and M.J. van der Laan},
	Date-Added = {2012-08-22 09:24:55 -0700},
	Date-Modified = {2012-08-24 13:51:01 -0700},
	Journal = {Int J Biostat},
	Keywords = {TMLE},
	Note = {PMID: 22628356},
	Number = {1},
	Pages = {Article 11},
	Title = {Targeted minimum loss based estimator that outperforms a given estimator},
	Volume = {8},
	Year = {2012}}

@incollection{HubbardJewellvanderLaan11,
	Address = {New York Dordrecht Heidelberg London},
	Author = {A.E. Hubbard and N.P. Jewell and M.J. van der Laan},
	Booktitle = {Targeted Learning: Causal Inference for Observational and Experimental Data},
	Date-Added = {2012-08-22 09:17:35 -0700},
	Date-Modified = {2012-08-22 09:20:29 -0700},
	Editor = {van der Laan, M.J. and Rose, S.},
	Keywords = {Chpt8},
	Publisher = {Springer},
	Title = {{Direct Effects and Effect Among the Treated}},
	Year = {2011}}

@incollection{MunozHubbardVdL11,
	Address = {New York Dordrecht Heidelberg London},
	Author = {I.D. Mu\~{n}oz and M. van der Laan},
	Booktitle = {Targeted Learning: Causal Inference for Observational and Experimental Data},
	Date-Added = {2012-08-22 09:14:07 -0700},
	Date-Modified = {2012-08-22 09:15:41 -0700},
	Editor = {van der Laan, M.J. and Rose, S.},
	Keywords = {Chpt28},
	Publisher = {Springer},
	Title = {{Targeted Bayesian Learning}},
	Year = {2011}}

@article{Hubbard2010,
	Author = {A.E. Hubbard and J. Ahern and N.L. Fleischer and M. van der Laan and S.A. Lippman and N. Jewell and T. Bruckner and W.A. Satariano},
	Date-Added = {2012-08-22 08:50:55 -0700},
	Date-Modified = {2012-08-24 10:10:42 -0700},
	Journal = {Epidemiology},
	Keywords = {Community},
	Note = {PMID: 20220526},
	Number = {4},
	Pages = {467-474},
	Title = {To {GEE} or Not to {GEE} Comparing Population Average and Mixed Models for Estimating the Associations Between Neighborhood Risk Factors and Health},
	Volume = {21},
	Year = {2010}}

@article{Oakes2004,
	Author = {J.M. Oakes},
	Date-Added = {2012-08-22 08:48:00 -0700},
	Date-Modified = {2012-08-22 08:49:35 -0700},
	Journal = {Soc Sci Med},
	Keywords = {Community},
	Note = {PMID: 15020009},
	Number = {10},
	Pages = {1929-1952},
	Title = {The (mis)estimation of neighborhood effects: causal inference for a practicable social epidemiology (with discussion)},
	Volume = {58},
	Year = {2004}}

@article{LiangZeger86,
	Author = {K.Y. Liang and S.L. Zeger},
	Date-Added = {2012-08-22 08:41:06 -0700},
	Date-Modified = {2012-08-22 08:46:50 -0700},
	Journal = {Biometrika},
	Keywords = {Community},
	Number = {1},
	Pages = {13-22},
	Title = {{Longitudinal Data Analysis Using Generalized Linear Models}},
	Url = {http://www.jstor.org/stable/2336267},
	Volume = {73},
	Year = {1986},
	Bdsk-Url-1 = {http://www.jstor.org/stable/2336267}}

@article{LairdWare82,
	Author = {N.M. Laird and J.H. Ware},
	Date-Added = {2012-08-22 08:37:25 -0700},
	Date-Modified = {2012-08-22 08:47:14 -0700},
	Journal = {Biometrics},
	Keywords = {Community},
	Note = {PMID: 7168798},
	Number = {4},
	Pages = {963--974},
	Title = {Random-effects models for longitudinal data},
	Volume = {38},
	Year = {1982}}

@article{ZegerLiangAlbert88,
	Author = {S.L. Zeger and K.Y. Liang and P.S. Albert},
	Date-Added = {2012-08-22 08:35:18 -0700},
	Date-Modified = {2012-08-22 08:46:59 -0700},
	Journal = {Biometrics},
	Keywords = {Community},
	Note = {PMID: 3233245},
	Number = {4},
	Pages = {1049-1060},
	Title = {Models for longitudinal data: a generalized estimating equation approach},
	Volume = {44},
	Year = {1988}}

@article{Wester2012,
	Author = {C.W. Wester and O.M. Stitelman and V. De Gruttola and H. Bussmann and R.G. Marlink and M.J. van der Laan},
	Date-Added = {2012-08-22 08:27:34 -0700},
	Date-Modified = {2012-08-26 21:00:48 -0700},
	Journal = {AIDS Res Hum Retroviruses},
	Keywords = {Application},
	Note = {PMID: 22309114},
	Number = {9},
	Pages = {781-788},
	Title = {Effect Modification by Sex and Baseline {CD4}(+) Cell Count Among Adults Receiving Combination Antiretroviral Therapy in {B}otswana: Results from a Clinical Trial},
	Volume = {28},
	Year = {2012}}

@manual{tmlePackage,
	Author = {S. Gruber and M. van der Laan},
	Date-Added = {2012-08-22 07:17:24 -0700},
	Date-Modified = {2012-08-26 21:18:22 -0700},
	Keywords = {R tmle},
	Note = {R package version 1.2.0-1, Available at \url{http://cran.r-project.org/web/packages/tmle/tmle.pdf}},
	Title = {{Targeted Maximum Likelihood Estimation}},
	Year = {2012}}

@manual{SuperLearnerPackage,
	Author = {E. Polley and M. van der Laan},
	Date-Added = {2012-08-22 07:14:31 -0700},
	Date-Modified = {2012-08-26 21:16:59 -0700},
	Keywords = {Superlearner},
	Note = {R package version 2.0-6, Available at \url{http://cran.r-project.org/web/packages/SuperLearner/SuperLearner.pdf}},
	Title = {{Super Learner Prediction}},
	Year = {2012},
	Bdsk-Url-1 = {http://cran.r-project.org/web/packages/SuperLearner/SuperLearner.pdf}}

@techreport{vanderLaan&Petersen12b,
	Author = {M.J. van der Laan, L. Balzer and M.L. Petersen},
	Date-Added = {2012-08-21 19:16:35 -0700},
	Date-Modified = {2012-08-26 21:15:43 -0700},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Keywords = {Allocation},
	Note = {Available at \url{http://biostats.bepress.com/ucbbiostat/paper296/}},
	Number = {296},
	Title = {Randomized Trials and Observational Studies in which Treatment Allocation Depends on the Baseline Characteristics of all Sampled Units},
	Year = {2012}}

@article{Munoz2012,
	Author = {I. D\'{i}az Munoz and M. van der Laan},
	Date-Added = {2012-08-21 19:12:50 -0700},
	Date-Modified = {2012-08-26 20:59:07 -0700},
	Journal = {Biometrics},
	Keywords = {Stochastic},
	Note = {PMID: 21977966},
	Number = {2},
	Pages = {541-549},
	Title = {Population Intervention Causal Effects Based on Stochastic Interventions},
	Volume = {68},
	Year = {2012}}

@inproceedings{Didelezetal06,
	Address = {Cambridge, MA},
	Author = {V. Didelez and A.P. Dawid and S. Geneletti},
	Booktitle = {{Proceedings of the 22nd Annual Conference on Uncertainty in Artificial Intelligence}},
	Date-Added = {2012-08-21 19:09:44 -0700},
	Date-Modified = {2012-08-26 21:14:54 -0700},
	Keywords = {Stochastic},
	Pages = {138--146},
	Title = {{Direct and Indirect Effects of Sequential Treatments}},
	Year = {2006}}

@techreport{Zheng&vanderLaan12,
	Author = {W. Zheng and M.J. van der Laan},
	Date-Added = {2012-08-21 19:05:33 -0700},
	Date-Modified = {2012-08-26 21:11:53 -0700},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Keywords = {NDE-long},
	Note = {Available at \url{http://biostats.bepress.com/ucbbiostat/paper295/}},
	Number = {295},
	Title = {Causal Mediation in a Survival Setting with Time-Dependent Mediators},
	Year = {2012}}

@article{Zheng2012,
	Author = {W. Zheng and M.J. van der Laan},
	Date-Added = {2012-08-21 19:02:52 -0700},
	Date-Modified = {2012-08-26 01:05:10 -0700},
	Journal = {Int J Biostat},
	Keywords = {NDE},
	Note = {PMID: 22499725},
	Number = {1},
	Pages = {1--40},
	Title = {Targeted maximum likelihood estimation for natural direct effects},
	Volume = {8},
	Year = {2012}}

@article{Schnitzer2012,
	Author = {M.E. Schnitzer and E.E. Moodie and R.W. Platt},
	Date-Added = {2012-08-21 18:59:59 -0700},
	Date-Modified = {2012-08-26 21:01:32 -0700},
	Journal = {Biostatistics},
	Keywords = {tmle},
	Note = {PMID: 22797173},
	Title = {Targeted maximum likelihood estimation for marginal time-dependent treatment effects under density misspecification},
	Year = {2012}}

@article{vanderLaan&Gruber12,
	Author = {M.J. van der Laan and S. Gruber},
	Date-Added = {2012-08-21 18:54:29 -0700},
	Date-Modified = {2012-08-24 11:33:54 -0700},
	Journal = {Int J Biostat},
	Keywords = {TMLE},
	Note = {PMID: 22611591},
	Number = {1},
	Title = {Targeted minimum loss based estimation of causal effects of multiple time point interventions},
	Volume = {8},
	Year = {2012},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAawAAAAAAawAAgAADE1hY2ludG9zaCBIRAAAAAAAAAAAAAAAAAAAAMobz/1IKwAABsaXyhUyMDEyX3ZkTFRvd2VyVE1MRS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAHO3ATzFpBoQAAAAAAAAAAAAEAAgAACSAAAAAAAAAAAAAAAAAAAAAKTGl0ZXJhdHVyZQAQAAgAAMocMm0AAAARAAgAAMxapBEAAAABABAGxpfKAAxX9QAMUlIAAAAeAAIAQU1hY2ludG9zaCBIRDpVc2VyczpsYXVyYTpEZXNrdG9wOkxpdGVyYXR1cmU6MjAxMl92ZExUb3dlclRNTEUucGRmAAAOACwAFQAyADAAMQAyAF8AdgBkAEwAVABvAHcAZQByAFQATQBMAEUALgBwAGQAZgAPABoADABNAGEAYwBpAG4AdABvAHMAaAAgAEgARAASADRVc2Vycy9sYXVyYS9EZXNrdG9wL0xpdGVyYXR1cmUvMjAxMl92ZExUb3dlclRNTEUucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfECMuLi9MaXRlcmF0dXJlLzIwMTJfdmRMVG93ZXJUTUxFLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAJQAlICVwJgAmsCbwJ9AoQCjQKzArgCuwLIAs0AAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAC3w==}}

@article{Porter2011,
	Author = {K.E. Porter and S. Gruber and M.J. van der Laan and J.S. Sekhon},
	Date-Added = {2012-08-21 18:45:58 -0700},
	Date-Modified = {2012-08-24 10:56:49 -0700},
	Journal = {Int J Biostat},
	Keywords = {TMLE},
	Note = {PMCID: PMC3173607},
	Number = {1},
	Pages = {Article 31},
	Title = {The relative performance of targeted maximum likelihood estimators},
	Volume = {7},
	Year = {2011},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAZQAAAAAAZQAAgAADE1hY2ludG9zaCBIRAAAAAAAAAAAAAAAAAAAAMobz/1IKwAABsaXyg8yMDEwX1BvcnRlci5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAHOgUYzFmHbQAAAAAAAAAAAAEAAgAACSAAAAAAAAAAAAAAAAAAAAAKTGl0ZXJhdHVyZQAQAAgAAMocMm0AAAARAAgAAMxZ6d0AAAABABAGxpfKAAxX9QAMUlIAAAAeAAIAO01hY2ludG9zaCBIRDpVc2VyczpsYXVyYTpEZXNrdG9wOkxpdGVyYXR1cmU6MjAxMF9Qb3J0ZXIucGRmAAAOACAADwAyADAAMQAwAF8AUABvAHIAdABlAHIALgBwAGQAZgAPABoADABNAGEAYwBpAG4AdABvAHMAaAAgAEgARAASAC5Vc2Vycy9sYXVyYS9EZXNrdG9wL0xpdGVyYXR1cmUvMjAxMF9Qb3J0ZXIucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi9MaXRlcmF0dXJlLzIwMTBfUG9ydGVyLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAI4AjoCPwJIAlMCVwJlAmwCdQKVApoCnQKqAq8AAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACwQ==}}

@article{Gruber2012ctmle,
	Author = {S. Gruber and M.J. van der Laan},
	Date-Added = {2012-08-21 18:30:43 -0700},
	Date-Modified = {2012-08-24 11:27:09 -0700},
	Journal = {Stat Meth Med Res},
	Keywords = {TMLE},
	Note = {PMID: 22368176},
	Title = {Consistent causal effect estimation under dual misspecification and implications for confounder selection procedures},
	Year = {2012}}

@article{Moore2012,
	Author = {K.L. Moore and R. Neugebauer and M.J. van der Laan and I.B. Tager},
	Date-Added = {2012-08-21 18:06:06 -0700},
	Date-Modified = {2012-08-22 22:16:22 -0700},
	Journal = {Stat Med},
	Keywords = {Aim1},
	Note = {PMID: 22362629},
	Number = {13},
	Pages = {1380--1404},
	Title = {Causal inference in epidemiological studies with strong confounding},
	Volume = {31},
	Year = {2012}}

@incollection{GruberVanderLaan2011,
	Address = {New York Dordrecht Heidelberg London},
	Author = {S. Gruber and M.J. van der Laan},
	Booktitle = {Targeted Learning: Causal Inference for Observational and Experimental Data},
	Date-Added = {2012-08-21 17:57:04 -0700},
	Date-Modified = {2012-08-22 07:57:20 -0700},
	Editor = {van der Laan, M.J. and Rose, S.},
	Keywords = {Chpt19},
	Publisher = {Springer},
	Title = {{C-TMLE of an Additive Point Treatment Effect}},
	Year = {2011}}

@article{Moodie2011,
	Author = {E.E. Moodie and D.A. Stephens},
	Date-Added = {2012-08-21 17:46:11 -0700},
	Date-Modified = {2012-08-23 17:34:11 -0700},
	Journal = {Int J Public Health},
	Keywords = {Aim1},
	Note = {PMID: 20931349},
	Number = {1},
	Pages = {117-119},
	Title = {{Marginal Structural Models: unbiased estimation for longitudinal studies}},
	Volume = {56},
	Year = {2011}}

@unpublished{Balzer2012,
	Author = {L.B. Balzer and M.L. Petersen and M.J. van der Laan},
	Date-Added = {2012-08-21 17:40:53 -0700},
	Date-Modified = {2012-08-26 21:05:25 -0700},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Keywords = {Superlearner},
	Note = {Unpublished, Division of Biostatistics, University of California, Berkeley},
	Title = {Adaptive estimation with few independent units},
	Year = {2012}}

@incollection{Rosenblum11,
	Address = {New York Dordrecht Heidelberg London},
	Author = {M. Rosenblum},
	Booktitle = {Targeted Learning: Causal Inference for Observational and Experimental Data},
	Date-Added = {2012-08-21 17:37:05 -0700},
	Date-Modified = {2012-08-22 08:12:21 -0700},
	Editor = {van der Laan, M.J. and Rose, S.},
	Keywords = {Chpt9},
	Publisher = {Springer},
	Title = {{Marginal Structural Models}},
	Year = {2011}}

@incollection{Chpt10,
	Address = {New York Dordrecht Heidelberg London},
	Author = {M.L. Petersen and K.E. Porter and S. Gruber and Y. Wang and M.J. van der Laan},
	Booktitle = {Targeted Learning: Causal Inference for Observational and Experimental Data},
	Date-Added = {2012-08-21 17:34:18 -0700},
	Date-Modified = {2012-08-24 11:19:47 -0700},
	Editor = {van der Laan, M.J. and Rose, S.},
	Keywords = {Chpt10},
	Publisher = {Springer},
	Title = {Positivity},
	Year = {2011}}

@incollection{Chpt3,
	Address = {New York Dordrecht Heidelberg London},
	Author = {E.C. Polley and S. Rose and M.J. van der Laan},
	Booktitle = {Targeted Learning: Causal Inference for Observational and Experimental Data},
	Date-Added = {2012-08-21 17:32:12 -0700},
	Date-Modified = {2012-08-24 12:09:45 -0700},
	Editor = {van der Laan, M.J. and Rose, S.},
	Keywords = {Chpt3},
	Publisher = {Springer},
	Title = {{Super Learner}},
	Year = {2011}}

@unpublished{Petersen&vanderLaan12,
	Author = {M.L. Petersen and M.J. van der Laan},
	Date-Added = {2012-08-21 17:22:48 -0700},
	Date-Modified = {2012-08-26 20:39:05 -0700},
	Keywords = {Roadmap},
	Note = {Unpublished, Division of Biostatistics, University of California, Berkeley},
	Title = {A General Roadmap for the Estimation of Causal Effects},
	Year = {2012}}

@article{Gsponer2012,
	Author = {T. Gsponer and M. Petersen and M. Egger and S. Phiri and M.H. Maathuis and P. Musondad and H. Tweya and K. Peter and B.H. Chi and O. Keiser and {IeDEA Southern Africa}},
	Date-Added = {2012-08-21 17:15:06 -0700},
	Date-Modified = {2012-08-24 11:58:18 -0700},
	Journal = {{AIDS}},
	Keywords = {HIV},
	Note = {PMID: 22089376},
	Number = {1},
	Pages = {57--65},
	Title = {{The causal effect of switching to second-line ART in programmes without access to routine viral load monitoring}},
	Volume = {36},
	Year = {2012}}

@book{Hernan&Robins13,
	Author = {M.A. Hern\'{a}n and J.M. Robins},
	Date-Added = {2012-08-21 17:06:54 -0700},
	Date-Modified = {2012-08-26 20:30:31 -0700},
	Keywords = {Book},
	Note = {Unpublished},
	Publisher = {Chapman \& Hall/CRC},
	Title = {{Causal Inference}},
	Year = {2012}}

@article{Petersen2012,
	Author = {M.L. Petersen and K.E. Porter and S. Gruber and Y. Wang and M.J. van der Laan},
	Date-Added = {2012-08-21 16:51:22 -0700},
	Date-Modified = {2012-08-22 22:15:34 -0700},
	Journal = {Stat Meth Med Res},
	Keywords = {Aim1},
	Note = {PMID: 21030422},
	Number = {1},
	Pages = {31--54},
	Title = {Diagnosing and responding to violations in the positivity assumption},
	Volume = {21},
	Year = {2012}}

@book{Donner&Klar00,
	Address = {London},
	Author = {A. Donner and N. Klar},
	Date-Modified = {2012-08-22 08:06:45 -0700},
	Keywords = {Community},
	Publisher = {Arnold},
	Title = {Design and Analysis of Cluster Randomization Trials in Health Research},
	Year = {2000}}

@book{Hayes2009,
	Address = {Boca Raton},
	Author = {R.J. Hayes and L.H. Moulton},
	Date-Modified = {2012-08-25 22:52:13 -0700},
	Publisher = {Chapman \& Hall/CRC},
	Title = {Cluster Randomized Trials},
	Year = {2009}}

@book{vanderLaanRose2011,
	Address = {New York Dordrecht Heidelberg London},
	Author = {M.J. van der Laan and S. Rose},
	Date-Modified = {2012-08-22 21:07:34 -0700},
	Keywords = {Book},
	Publisher = {Springer},
	Title = {{Targeted Learning: Causal Inference for Observational and Experimental Data}},
	Year = {2011}}

@book{Murray98,
	Address = {Oxford},
	Author = {D.M. Murray},
	Date-Modified = {2012-08-22 08:09:26 -0700},
	Keywords = {Community},
	Publisher = {Oxford University Press},
	Title = {Design and Analysis of Community Randomized Trials},
	Year = {1998}}

@article{Campbell&Donner&Klar07,
	Author = {M.J. Campbell and A. Donner and N. Klar},
	Journal = {Statistics in Medicine},
	Pages = {2--19, doi: 10.1002/sim.2731},
	Title = {Developments in cluster randomized trials and statistics in medicine},
	Volume = {26},
	Year = {2007}}

@article{Klar&Donner97,
	Author = {N. Klar and A. Donner},
	Date-Modified = {2012-08-22 08:08:30 -0700},
	Journal = {Statistics in Medicine},
	Keywords = {Community},
	Pages = {1753--1764},
	Title = {The merits of matching in community intervention trials: a cautionary tale},
	Volume = {16(15)},
	Year = {1997}}

@article{Raudenbush&Martinez&Spybrook07,
	Author = {S.W. Raudenbush and A. Martinez and J. Spybrook},
	Journal = {Educational Evaluation and Policy Analysis},
	Pages = {5--29},
	Title = {Developments in cluster randomized trials and statistics in medicine},
	Volume = {29},
	Year = {2007}}

@article{Freedman&Green&Byar90,
	Author = {L.S. Freedman and S.B. Green and D.P. Byar},
	Journal = {Statistics in Medicine},
	Pages = {943--952},
	Title = {Assessing the gain in efficiency due to matching in a community intervention study},
	Volume = {9},
	Year = {1990}}

@article{Freedmanetal97,
	Author = {L. Freedman and M. Gail and S. Green and D. Corle},
	Journal = {Controlled clinical trials},
	Pages = {131--139, doi:10.1016/S0197-2456(96)00115-8},
	Title = {The efficiency of the matched-pairs design of the community intervention trial for smoking cessation (COMMIT)},
	Volume = {18(2)},
	Year = {1997}}

@article{Toftageretal11,
	Author = {M. Toftager and L.B. Christiansen and P.L. Kristensen and J. Troelsen},
	Journal = {BMC Public Health},
	Pages = {711--777},
	Title = {SPACE for physical activity-a multicomponent intervention study: study design and baseline findings from a cluster randomized controlled trial},
	Volume = {10},
	Year = {2011}}

@article{Koetheetal10,
	Author = {J.R. Koethe and A.O. Westfall and D.K. Luhanga and G.M. Clark and J.D. Goldman and P.L Mulenga and R.A. Cantrell and B.H. Chi and I. Zulu and M.S. Saag and J. S. Stringer},
	Journal = {PlLoS One},
	Pages = {5(3):e9680},
	Title = {A cluster randomized trial of routine HIV-1 viral load monitoring in Zambia},
	Volume = {5},
	Year = {2010}}

@article{Watsonetal04,
	Author = {L. Watson and R. Small and S. Brown and W. Dawson and J. Lumley},
	Journal = {Journal of Controlled Clinical Trials},
	Pages = {235--250},
	Title = {Mounting a community-randomized trial: sample size, matching, selection, and randomization issues in PRISM},
	Volume = {3},
	Year = {2004}}

@article{Gailetal92,
	Author = {M.H. Gail and D.P. Byar and T.F. Pechacek and D.K. Corle},
	Journal = {Controlled clinical trials},
	Pages = {6-21},
	Title = {Aspects of statistical design for the community intervention trial for smoking cessation},
	Volume = {13},
	Year = {1992}}

@article{Commit91,
	Author = {COMMIT Research Group},
	Journal = {Journal of National Cancer Institute},
	Pages = {1620-1628},
	Title = {Summary of design and intervention},
	Volume = {83(22)},
	Year = {1991}}

@article{Imai&King&Nall09,
	Author = {Kosuke Imai and G. King and C. Nall},
	Journal = {Statistical Science},
	Pages = {29--53},
	Title = {The essential role of pair matching in cluster randomized experiments with applicationto the Mexican Universal Health Insurance Evaluation},
	Volume = {24 (1)},
	Year = {2009}}

@article{Imai08,
	Author = {K. Imai},
	Journal = {Statistics in Medicine},
	Pages = {4857--4873},
	Title = {Variance identification and efficiency analysis in randomized experiments under the matched-pair design},
	Volume = {27(24)},
	Year = {2008}}

@techreport{vanderLaan2011,
	Author = {M.J. van der Laan and S. Gruber},
	Date-Modified = {2012-08-26 20:48:45 -0700},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Keywords = {TMLE},
	Note = {Available at \url{http://www.bepress.com/ucbbiostat/paper290}; To appear in Int J. Biostat},
	Number = {290},
	Title = {Targeted Minimum Loss Based Estimation of an Intervention Specific Mean Outcome},
	Year = {2011}}

@techreport{vanderLaan08,
	Author = {M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Note = {http://www.bepress.com/ucbbiostat/paper234},
	Number = {232},
	Title = {The construction and analysis of adaptive group sequential designs},
	Year = {2008}}

@techreport{Balzer&Petersen&vanderLaan12,
	Author = {L.B. Balzer and M.L. Petersen and M.J. van der Laan},
	Date-Modified = {2012-08-21 17:14:20 -0700},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Note = {Under Review at Statistics in Medicine; Technical report available at http://www.bepress.com/ucbbiostat/paper294},
	Number = {294},
	Title = {{Why Match in Individually and Cluster Randomized Trials?}},
	Year = {2012}}

@incollection{Marschak53,
	Address = {New York},
	Author = {J. Marschak},
	Booktitle = {Economic measurements for policy and prediction},
	Editor = {W.~C. Hood and T.~C. Koopmans},
	Publisher = {Wiley},
	Title = {Studies in econometric method},
	Year = {1953}}

@article{Heckman00,
	Author = {J. Heckman},
	Journal = {Q J Econ},
	Pages = {45--97},
	Title = {Causal parameters and policy analysis in economics: A twentieth century retrospective.},
	Volume = {115},
	Year = {2000}}

@article{Gruber2010,
	Author = {S. Gruber and M.J. van der Laan},
	Date-Modified = {2012-08-26 00:48:08 -0700},
	Journal = {Int J BiostatBiostatistics},
	Keywords = {App},
	Note = {PMCID: PMC3126669},
	Number = {1},
	Pages = {Article 26},
	Title = {A Targeted Maximum Likelihood Estimator of a Causal Effect on a Bounded Continuous Outcome},
	Volume = {6},
	Year = {2010}}

@article{Heckman10,
	Author = {J. Heckman},
	Journal = {J Econ Lit},
	Pages = {356--398},
	Title = {Building bridges between structural and program evaluation approaches to evaluating policy.},
	Volume = {48},
	Year = {2010}}

@article{Bang&Robins05,
	Author = {H. Bang and J.M. Robins},
	Journal = {Biometrics},
	Pages = {962--972},
	Title = {Doubly robust estimation in missing data and causal inference models},
	Volume = {61},
	Year = {2005}}

@book{Pearson11,
	Address = {London},
	Author = {K. Pearson},
	Edition = {3rd},
	Publisher = {Black},
	Title = {Grammar of science},
	Year = {1911}}

@article{Rubin74,
	Author = {Donald B. Rubin},
	Journal = {J Educ Psychol},
	Pages = {688--701},
	Title = {Estimating causal effects of treatments in randomized and nonrandomized studies.},
	Volume = {66},
	Year = {1974}}

@article{Neyman23,
	Author = {J. Neyman},
	Journal = {Stat Sci},
	Pages = {465--480},
	Title = {Sur les applications de la theorie des probabilites aux experiences agricoles: Essai des principes ({In Polish}). {E}nglish translation by {D.M.} {D}abrowska and {T.P.} {S}peed (1990)},
	Volume = {5},
	Year = {1923}}

@book{Pearl2009,
	Address = {New York},
	Author = {J. Pearl},
	Date-Modified = {2012-08-22 21:06:39 -0700},
	Edition = {2nd},
	Keywords = {Book},
	Publisher = {Cambridge University Press},
	Title = {{Causality: Models, Reasoning and Inference}},
	Year = {2009}}

@article{Pearl95,
	Author = {J. Pearl},
	Journal = {Biometrika},
	Pages = {669--710},
	Title = {Causal diagrams for empirical research.},
	Volume = {82},
	Year = {1995}}

@article{RobinsGreenland1992,
	Author = {J.M. Robins and S. Greenland},
	Date-Modified = {2012-08-26 16:42:09 -0700},
	Journal = {Epidemiol},
	Keywords = {DE},
	Note = {PMID: 1576220},
	Pages = {143--155},
	Title = {Identifiability and exchangeability for direct and indirect effects},
	Volume = {3},
	Year = {1992}}

@inproceedings{Pearl2001,
	Address = {San Francisco},
	Author = {J. Pearl},
	Booktitle = {Proceedings of the Seventeenth Conference on Uncertainty in artificial intelligence},
	Date-Modified = {2012-08-26 20:43:51 -0700},
	Pages = {411--420},
	Publisher = {Morgan Kaufmann},
	Title = {Direct and indirect effects},
	Year = {2001}}

@article{Baron&Kenny86,
	Author = {R. Baron and D. Kenny},
	Journal = {J Personal Soc Psychol},
	Pages = {1173--1182},
	Title = {The moderator-mediator variable distinction in social psychological research: conceptual, strategic, and statistical considerations.},
	Volume = {51},
	Year = {1986}}

@book{MacKinnon08,
	Address = {New York},
	Author = {D. {MacKinnon}},
	Publisher = {Erlbaum},
	Title = {Introduction to statistical mediation analysis},
	Year = {2008}}

@article{MacKinnonetal07,
	Author = {D. {MacKinnon} and C. Lockwood and C. Brown and W. Wang and J. Hoffman},
	Journal = {Clin Trials},
	Pages = {499--513},
	Title = {The intermediate endpoint effect in logistic and probit regression.},
	Volume = {4},
	Year = {2007}}

@incollection{Pearl10c,
	Author = {J. Pearl},
	Booktitle = {Statistical causality},
	Editor = {C. Berzuini and P. Dawid and L. Bernardinelli},
	Title = {The mediation formula: a guide to the assessment of causal pathways in nonlinear models.},
	Year = {forthcoming 2011}}

@article{Pearl2010,
	Author = {J. Pearl},
	Date-Modified = {2012-08-26 20:46:05 -0700},
	Journal = {Int J Biostat},
	Keywords = {Roadmap},
	Note = {PMCID: PMC2836213},
	Number = {2},
	Pages = {Article 7},
	Title = {An Introduction to Causal Inference},
	Volume = {6},
	Year = {2010}}

@article{vanderLaan&Rose10,
	Author = {M.J. van der Laan and S. Rose},
	Journal = {Amstat News},
	Pages = {38--39},
	Title = {Statistics Ready for a Revolution: next Generation of Statisticians Must Build Tools for Massive Data Sets},
	Volume = {399},
	Year = {2010}}

@techreport{vanderLaan2003,
	Author = {M.J. van der Laan and S. Dudoit},
	Date-Modified = {2012-08-26 20:51:01 -0700},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Keywords = {Superlearner},
	Note = {Available at \url{http://biostats.bepress.com/ucbbiostat/paper130}},
	Number = {130},
	Title = {Unified Cross-Validation Methodology For Selection Among Estimators and a General Cross-Validated Adaptive Epsilon-Net Estimator: Finite Sample Oracle Inequalities and Examples},
	Year = {2003}}

@book{vanderLaanRobins2003,
	Address = {New York Berlin Heidelberg},
	Author = {M.J. van der Laan and J.M. Robins},
	Date-Modified = {2012-08-22 21:07:29 -0700},
	Keywords = {Book},
	Publisher = {Springer-Verlag},
	Title = {{Unified Methods for Censored Longitudinal Data and Causality}},
	Year = {2003}}

@book{Bickel1997,
	Address = {Berlin Heidelberg New York},
	Author = {P.J. Bickel and C.A.J. Klaassen and Y. Ritov and J. Wellner},
	Date-Modified = {2012-08-26 15:51:23 -0700},
	Publisher = {Springer},
	Title = {Efficient and adaptive estimation for semiparametric models},
	Year = {1997}}

@article{vanderLaan2006,
	Author = {M.J. van der Laan and Daniel B. Rubin},
	Date-Modified = {2012-08-26 20:31:54 -0700},
	Journal = {Int J Biostat},
	Keywords = {TMLE},
	Number = {1},
	Pages = {Article 11},
	Title = {Targeted Maximum Likelihood Learning},
	Volume = {2},
	Year = {2006}}

@article{Stitelman2011b,
	Author = {O.M. Stitelman and M.J. van der Laan},
	Date-Modified = {2012-08-26 00:54:24 -0700},
	Journal = {Int J Biostat},
	Keywords = {App},
	Note = {PMCID: PMC3083138},
	Number = {1},
	Pages = {19},
	Read = {1},
	Title = {Targeted Maximum Likelihood Estimation of Effect Modification Parameters In Survival Analysis},
	Volume = {7},
	Year = {2011}}

@article{vanderLaan2010ctmle,
	Author = {M.J. van der Laan and S. Gruber},
	Date-Modified = {2012-08-24 11:26:51 -0700},
	Journal = {Int J Biostat},
	Keywords = {TMLE},
	Note = {PMCID: PMC2898626},
	Number = {1},
	Title = {Collaborative double robust penalized targeted maximum likelihood estimation},
	Volume = {6},
	Year = {2010}}

@article{Taubes07,
	Author = {G. Taubes},
	Journal = {The New York Times},
	Title = {{Do we really know what makes us healthy?}},
	Year = {2007}}

@article{USPrev09,
	Author = {{U.S. Preventive Services Task Force}},
	Journal = {Ann Intern Med},
	Number = {10},
	Pages = {716--726},
	Title = {{Screening for breast cancer: U.S. Preventive Services Task Force recommendation statement}},
	Volume = {151},
	Year = {2009}}

@article{Freedman&Petitti&Robins04,
	Author = {D.A. Freedman and D.B. Petitti and J.M. Robins},
	Journal = {Int J Epidemiol},
	Pages = {43--55},
	Title = {{On the efficacy of screening for breast cancer}},
	Volume = {33},
	Year = {2004}}

@book{Rothman&Greenland98,
	Address = {Philadelphia},
	Author = {K.J. Rothman and S. Greenland},
	Edition = {2nd},
	Publisher = {Lippincott, Williams \& Wilkins},
	Title = {Modern epidemiology},
	Year = {1998}}

@book{Jewell04,
	Address = {Boca Raton},
	Author = {N.P. Jewell},
	Publisher = {Chapman \& Hall},
	Title = {Statistics for epidemiology},
	Year = {2004}}

@book{Freedman05,
	Address = {New York},
	Author = {D.A. Freedman},
	Publisher = {Cambridge},
	Title = {Statistical models: theory and practice},
	Year = {2005}}

@article{Ioannidis06,
	Author = {J.P.A. Ioannidis},
	Journal = {Neonatal Intensive Care J Perinatol Neonatol},
	Number = {3},
	Title = {{Why most published research findings are false}},
	Volume = {19},
	Year = {2006}}

@book{Freedman10,
	Address = {New York},
	Author = {D.H. Freedman},
	Publisher = {Little, Brown and Company},
	Title = {Wrong: why experts keep failing us---and how to know when not to trust them},
	Year = {2010}}

@book{Box&Draper87,
	Address = {Hoboken},
	Author = {G.E.P. Box and N.R. Draper},
	Publisher = {Wiley},
	Title = {Empirical model-building and response surfaces},
	Year = {1987}}

@article{Robins1986,
	Author = {J.M. Robins},
	Date-Modified = {2012-08-26 14:52:27 -0700},
	Journal = {Math Mod},
	Pages = {1393--1512},
	Title = {A new approach to causal inference in mortality studies with sustained exposure periods--application to control of the healthy worker survivor effect},
	Volume = {7},
	Year = {1986}}

@article{Tager&Hollenberg&Satariano98,
	Author = {I. Tager and M. Hollenberg and W. Satariano},
	Journal = {Am J Epidemiol},
	Pages = {921--931},
	Title = {{Self-reported leisure-time physical activity and measures of cardiorespiratory fitness in an elderly population}},
	Volume = {147},
	Year = {1998}}

@manual{RCore,
	Address = {Vienna},
	Author = {{R Development Core Team}},
	Date-Modified = {2012-08-22 08:11:48 -0700},
	Keywords = {R},
	Organization = {R Foundation for Statistical Computing},
	Title = {R: a language and environment for statistical computing},
	Url = {http://www.R-project.org},
	Year = {2010},
	Bdsk-Url-1 = {http://www.R-project.org}}

@article{liaw:2002,
	Author = {A. Liaw and M. Wiener},
	Journal = {R News},
	Number = {3},
	Pages = {18--22},
	Title = {Classification and Regression by randomForest},
	Url = {http://CRAN.R-project.org/package=randomForest},
	Volume = {2},
	Year = {2002},
	Bdsk-Url-1 = {http://CRAN.R-project.org/package=randomForest}}

@article{randomForests,
	Author = {L. Breiman},
	Journal = {Mach Learn},
	Pages = {5--32},
	Title = {Random Forests},
	Volume = {45},
	Year = {2001}}

@manual{ipred,
	Author = {A. Peters and T. Hothorn},
	Note = {R package version 0.8-8},
	Title = {ipred: Improved Predictors},
	Url = {http://CRAN.R-project.org/package=ipred},
	Year = {2009},
	Bdsk-Url-1 = {http://CRAN.R-project.org/package=ipred}}

@article{breiman96bagging,
	Author = {L. Breiman},
	Journal = {Mach Learn},
	Number = {2},
	Pages = {123--140},
	Title = {Bagging Predictors},
	Volume = {24},
	Year = {1996}}

@incollection{gam:1992,
	Address = {Boca Raton},
	Author = {T.J. Hastie},
	Booktitle = {Statistical models in {S}},
	Editor = {J.M. Chambers and T.J. Hastie},
	Publisher = {Chapman \& Hall},
	Title = {Generalized additive models},
	Year = {1992}}

@book{gams,
	Address = {Boca Raton},
	Author = {T.J. Hastie and R.J. Tibshirani},
	Publisher = {Chapman \& Hall},
	Title = {Generalized additive models},
	Year = {1990}}

@manual{gbm,
	Author = {G. Ridgeway},
	Note = {R package version 1.6-3},
	Title = {gbm: generalized boosted regression models},
	Year = {2007}}

@article{friedman:2001,
	Author = {J.H. Friedman},
	Journal = {Ann Stat},
	Pages = {1189-1232},
	Title = {Greedy Function Approximation: a Gradient Boosting Machine},
	Volume = {29},
	Year = {2001}}

@book{MASS,
	Address = {Berlin Heidelberg New York},
	Author = {W.N. Venables and B.D. Ripley},
	Edition = {4th},
	Publisher = {Springer},
	Title = {Modern applied statistics with S},
	Year = {2002}}

@manual{polspline,
	Author = {C. Kooperberg},
	Note = {R package version 1.1.4},
	Title = {polspline: Polynomial spline routines},
	Url = {http://CRAN.R-project.org/package=polspline},
	Year = {2009},
	Bdsk-Url-1 = {http://CRAN.R-project.org/package=polspline}}

@article{MARS,
	Author = {J.H. Friedman},
	Journal = {Ann Stat},
	Number = {1},
	Pages = {1--141},
	Title = {Multivariate Adaptive Regression Splines},
	Volume = {19},
	Year = {1991}}

@manual{bart,
	Author = {H.A. Chipman and R.E. McCulloch},
	Note = {R package version 0.3-1},
	Title = {BayesTree: {B}ayesian methods for tree-based models},
	Url = {http://CRAN.R-project.org/package=BayesTree},
	Year = {2009},
	Bdsk-Url-1 = {http://CRAN.R-project.org/package=BayesTree}}

@article{chipman:2009,
	Author = {H.A. Chipman and E.I. George and R.E. McCulloch},
	Journal = {Ann Appl Stat},
	Number = {1},
	Pages = {266--298},
	Title = {{BART}: {B}ayesian Additive Regression Trees},
	Volume = {4},
	Year = {2010}}

@incollection{loess,
	Address = {Boca Raton},
	Author = {W.S. Cleveland and E. Groose and W.M. Shyu},
	Booktitle = {Statistical models in {S}},
	Editor = {J.M. Chambers and T.J. Hastie},
	Publisher = {Chapman \& Hall},
	Title = {Local Regression Models},
	Year = {1992}}

@techreport{Polley2010,
	Author = {E.C. Polley and M.J. van der Laan},
	Date-Modified = {2012-08-26 21:10:49 -0700},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Keywords = {Superlearner},
	Note = {Available at \url{http://www.bepress.com/ucbbiostat/paper266/}},
	Number = {266},
	Title = {Super Learner in Prediction},
	Year = {2010}}

@book{cook:1994,
	Address = {New York},
	Author = {D. Cook and S. Weisberg},
	Publisher = {Wiley},
	Title = {An introduction to regression graphics},
	Year = {1994}}

@article{chu:2001,
	Author = {S. Chu},
	Journal = {J Stat Educ},
	Number = {2},
	Title = {Pricing the {C}'s of diamond stones},
	Volume = {9},
	Year = {2001}}

@book{berndt:1991,
	Address = {New York},
	Author = {E.R. Berndt},
	Publisher = {Addison--Wesley},
	Title = {The practice of econometrics},
	Year = {1991}}

@article{kibler:1989,
	Author = {D. Kibler and D.W. Aha and M.K. Albert},
	Journal = {Comput Intell},
	Pages = {51},
	Title = {Instance-Based Prediction of Real-Valued Attributes},
	Volume = {5},
	Year = {1989}}

@book{rosner:1999,
	Address = {Pacific Grove},
	Author = {B. Rosner},
	Edition = {5th},
	Publisher = {Duxbury},
	Title = {Fundamentals of biostatistics},
	Year = {1999}}

@misc{newman:1998,
	Author = {D.J. Newman and S. Hettich and C.L. Blake and C.J. Merz},
	Institution = {Department of Information and Computer Sciences, University of California, Irvine},
	Title = {{UCI Repository of Machine Learning Databases}},
	Year = {1998}}

@book{afifi:1979,
	Address = {New York},
	Author = {A. Afifi and S. Azen},
	Edition = {2nd},
	Publisher = {Academic},
	Title = {Statistical analysis: a computer oriented approach},
	Year = {1979}}

@book{cook:1998,
	Address = {New York},
	Author = {D. Cook},
	Publisher = {Wiley},
	Title = {Regression graphics: ideas for studying regression through graphics},
	Year = {1998}}

@article{liu:1999,
	Author = {Z. Liu and T. Stengos},
	Journal = {J of Appl Econom},
	Pages = {527--538},
	Title = {Nonlinearities in Cross Country Growth Regressions: a Semiparametric Approach},
	Volume = {14},
	Year = {1999}}

@article{penrose:1985,
	Author = {K. Penrose and A. Nelson and A. Fisher},
	Journal = {Med Sci Sport Exer},
	Pages = {189},
	Title = {Generalized Body Composition Prediction Equation for Men Using Simple Measurement Techniques},
	Volume = {17},
	Year = {1985}}

@book{harrell:2001,
	Address = {Berlin Heidelberg New York},
	Author = {Harrell, Jr., F.E.},
	Publisher = {Springer},
	Title = {Regression modeling strategies with applications to linear models, logistic regression, and survival analysis},
	Year = {2001}}

@manual{arm,
	Author = {A. Gelman and Y.-S. Su and M. Yajima and J. Hill and M.G. Pittau and J. Kerman and T. Zheng},
	Note = {R package version 1.3-02},
	Title = {arm: data analysis using regression and multilevel/hierarchical models},
	Url = {http://CRAN.R-project.org/package=arm},
	Year = {2010},
	Bdsk-Url-1 = {http://CRAN.R-project.org/package=arm}}

@article{gelman:2009,
	Author = {A. Gelman and A. Jakulin and M.G. Pittau and Y.-S. Su},
	Journal = {Ann Appl Stat},
	Number = {3},
	Pages = {1360--1383},
	Title = {A Weakly Informative Default Prior Distribution for Logistic and Other Regression Models},
	Volume = {2},
	Year = {2009}}

@article{friedman:2010,
	Author = {J.H. Friedman and T.J. Hastie and R.J. Tibshirani},
	Journal = {J Stat Softw},
	Number = {1},
	Title = {Regularization Paths for Generalized Linear Models via Coordinate Descent},
	Volume = {33},
	Year = {2010}}

@manual{glmnet,
	Author = {J.H. Friedman and T.J. Hastie and R.J. Tibshirani},
	Note = {R package version 1.1-5},
	Title = {glmnet: lasso and elastic-net regularized generalized linear models},
	Url = {http://CRAN.R-project.org/package=glmnet},
	Year = {2010},
	Bdsk-Url-1 = {http://CRAN.R-project.org/package=glmnet}}

@manual{DSA,
	Author = {R. Neugebauer and J. Bullard},
	Note = {R package version 3.1.3},
	Title = {DSA: Data-adaptive estimation with cross-validation and the D/S/A algorithm},
	Url = {http://www.stat.berkeley.edu/~laan/Software/},
	Year = {2009},
	Bdsk-Url-1 = {http://www.stat.berkeley.edu/~laan/Software/}}

@article{SinisivanderLaan04,
	Author = {S.E. Sinisi and M.J. van der Laan},
	Journal = {Stat Appl Genet Mol},
	Note = {Article 18},
	Number = {1},
	Title = {{D}eletion/{S}ubstitution/{A}ddition algorithm in learning with applications in genomics},
	Volume = {3},
	Year = {2004}}

@manual{svm,
	Author = {E. Dimitriadou and K. Hornik and F. Leisch and D. Meyer and A. Weingessel},
	Note = {R package version 1.5-22},
	Title = {e1071: misc functions of the Department of Statistics (e1071)},
	Url = {http://CRAN.R-project.org/package=e1071},
	Year = {2009},
	Bdsk-Url-1 = {http://CRAN.R-project.org/package=e1071}}

@manual{Chang:2001,
	Author = {C.-C. Chang and C.-J. Lin},
	Title = {{LIBSVM}: a library for support vector machines},
	Url = {http://www.csie.ntu.edu.tw/~cjlin/libsvm},
	Year = {2001},
	Bdsk-Url-1 = {http://www.csie.ntu.edu.tw/~cjlin/libsvm}}

@article{vantveer:2002,
	Author = {L.J. {van't Veer} and H. Dal and M.J. {van de Vijver} and Y.D. He and A.A.M. Hart and M. Mao and H.L. Peterse and K. van der Kooy and M.J. Marton and A.T. Witteveen and G.J. Schreiber and R.M. Kerkhoven and C. Roberts and P.S. Linsley and R. Bernards and S.H. Friend},
	Journal = {Nature},
	Pages = {530--536},
	Title = {Gene Expression Profiling Predicts Clinical Outcome of Breast Cancer},
	Volume = {415},
	Year = {2002}}

@article{vanderLaan2007,
	Author = {M.J. van der Laan and E.C. Polley and A.E. Hubbard},
	Date-Modified = {2012-08-23 17:06:55 -0700},
	Journal = {Stat Appl Genet Mol},
	Keywords = {Superlearner},
	Note = {PMID: 17910531},
	Number = {1},
	Pages = {Article 25},
	Title = {Super Learner},
	Volume = {6},
	Year = {2007}}

@article{Wolpert92,
	Author = {D. H. Wolpert},
	Journal = {Neural Networks},
	Pages = {241--259},
	Title = {Stacked Generalization},
	Volume = {5},
	Year = {1992}}

@article{Breiman96d,
	Author = {L. Breiman},
	Journal = {Mach Learn},
	Pages = {49--64},
	Title = {Stacked Regressions},
	Volume = {24},
	Year = {1996}}

@article{Leblanc96,
	Author = {M. LeBlanc and R.J. Tibshirani},
	Journal = {J Am Stat Assoc},
	Pages = {1641--1650},
	Title = {Combining estimates in regression and classification},
	Volume = {91},
	Year = {1996}}

@article{Stone74,
	Author = {M. Stone},
	Journal = {J R Stat Soc Ser B},
	Number = {2},
	Pages = {111--147},
	Title = {Cross-validatory choice and assessment of statistical predictions},
	Volume = {36},
	Year = {1974}}

@article{Geisser75,
	Author = {S. Geisser},
	Journal = {J Am Stat Assoc},
	Number = {350},
	Pages = {320--328},
	Title = {The Predictive Sample Reuse Method with Applications},
	Volume = {70},
	Year = {1975}}

@inproceedings{Tsybakov03,
	Address = {Berlin Heidelberg New York},
	Author = {A.B. Tsybakov},
	Booktitle = {COLT},
	Editor = {B. Sch{\"o}lkopf and M.K. Warmuth},
	Publisher = {Springer},
	Series = {Lecture Notes in Computer Science},
	Title = {Optimal rates of aggregation},
	Volume = {2777},
	Year = {2003}}

@inproceedings{Juditskyetal05,
	Author = {A. Juditsky and A.V. Nazin and A.B. Tsybakov and N. Vayatis},
	Booktitle = {NIPS},
	Title = {Generalization Error Bounds for Aggregation by Mirror Descent with Averaging},
	Year = {2005}}

@inproceedings{Buneaetal06,
	Address = {Berlin Heidelberg New York},
	Author = {F. Bunea and A.B. Tsybakov and M.H. Wegkamp},
	Booktitle = {COLT},
	Editor = {G. Lugosi and H.-U. Simon},
	Publisher = {Springer},
	Series = {Lecture Notes in Computer Science},
	Title = {Aggregation and sparsity via {L}1 penalized least squares},
	Volume = {4005},
	Year = {2006}}

@article{Buneaetal07,
	Author = {F. Bunea and A.B. Tsybakov and M.H. Wegkamp},
	Journal = {Ann Stat},
	Number = {4},
	Pages = {1674--1697},
	Title = {Aggregation for Gaussian Regression},
	Volume = {35},
	Year = {2007}}

@inproceedings{Buneaetal07b,
	Address = {Berlin Heidelberg New York},
	Author = {F. Bunea and A.B. Tsybakov and M.H. Wegkamp},
	Booktitle = {COLT},
	Editor = {N.H. Bshouty and C. Gentile},
	Publisher = {Springer},
	Series = {Lecture Notes in Computer Science},
	Title = {Sparse density estimation with {L}1 penalties},
	Volume = {4539},
	Year = {2007}}

@inproceedings{Dalalyan&Tsybakov07,
	Address = {Berlin Heidelberg New York},
	Author = {A.S. Dalalyan and A.B. Tsybakov},
	Booktitle = {COLT},
	Editor = {N.H. Bshouty and C. Gentile},
	Publisher = {Springer},
	Series = {Lecture Notes in Computer Science},
	Title = {Aggregation by exponential weighting and sharp oracle inequalities},
	Volume = {4539},
	Year = {2007}}

@article{Dalalyan&Tsybakov08,
	Author = {A.S. Dalalyan and A.B. Tsybakov},
	Journal = {Mach Learn},
	Number = {1--2},
	Pages = {39--61},
	Title = {Aggregation by exponential weighting, sharp PAC-{B}ayesian bounds and sparsity},
	Volume = {72},
	Year = {2008}}

@book{Lehmann86,
	Address = {Berlin Heidelberg New York},
	Author = {E.L. Lehmann},
	Edition = {2nd},
	Publisher = {Springer},
	Title = {Testing statistical hypotheses},
	Year = {1986}}

@book{Hastie&Tibshirani&Friedman01,
	Address = {Berlin Heidelberg New York},
	Author = {T.J. Hastie and R.J. Tibshirani and J.H. Friedman},
	Date-Modified = {2012-08-23 17:04:42 -0700},
	Publisher = {Springer},
	Title = {{The Elements of Statistical Learning: Data Mining, Inference, and Prediction}},
	Year = {2001}}

@inproceedings{Ruczinski&Kooperberg&LeBlanc02,
	Author = {I. Ruczinski and C. Kooperberg and M. LeBlanc},
	Booktitle = {Proceedings of the MSRI workshop on Nonlinear Estimation and Classification},
	Editor = {D. Denison and M. Hansen and C. Holmes and B. Mallick and B. Yu},
	Pages = {333--344},
	Title = {Logic Regression -- methods and software},
	Year = {2002}}

@techreport{Birkner&Hubbard&vanderLaan05,
	Author = {M.D. Birkner and A.E. Hubbard and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {197},
	Title = {Data Adaptive Pathway Testing},
	Year = {2005}}

@techreport{Chaffee&Hubbard&vanderLaan10,
	Author = {P. Chaffee and A.E. Hubbard and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {263},
	Title = {Permutation-based Pathway Testing using the Super Learner Algorithm},
	Year = {2010}}

@inproceedings{Polley&vanderLaan09,
	Address = {Boca Raton},
	Author = {E.C. Polley and M.J. van der Laan},
	Booktitle = {Design, summarization, analysis \& interpretation of clinical trials with time-to-event endpoints},
	Editor = {K.E. Peace},
	Publisher = {Chapman \& Hall},
	Title = {Predicting Optimal Treatment Assignment Based on Prognostic Factors in Cancer Patients},
	Year = {2009}}

@article{vanderLaan&Dudoit&vanderVaart06,
	Author = {M.J. van der Laan and S. Dudoit and A.W. van der Vaart},
	Journal = {Stat Decis},
	Number = {3},
	Pages = {373--395},
	Title = {The Cross-Validated Adaptive Epsilon-Net Estimator},
	Volume = {24},
	Year = {2006}}

@article{vanderVaart&Dudoit&vanderLaan06,
	Author = {A.W. van der Vaart and S. Dudoit and M.J. van der Laan},
	Journal = {Stat Decis},
	Number = {3},
	Pages = {351--371},
	Title = {Oracle Inequalities for Multi-Fold Cross-Validation},
	Volume = {24},
	Year = {2006}}

@article{vanderLaan&Dudoit&Keles04,
	Author = {M.J. van der Laan and S. Dudoit and S. Kele\c{s}},
	Journal = {Stat Appl Genet Mol},
	Number = {1},
	Pages = {Article 4},
	Title = {Asymptotic optimality of likelihood-based cross-validation},
	Volume = {3},
	Year = {2004}}

@article{Dudoit&vanderLaan05,
	Author = {S. Dudoit and M.J. van der Laan},
	Journal = {Stat Methodol},
	Number = {2},
	Pages = {131--154},
	Title = {Asymptotics of cross-validated risk estimation in estimator selection and performance assessment},
	Volume = {2},
	Year = {2005}}

@techreport{Keles&vanderLaan&Dudoit02,
	Author = {Kele\c{s}, S. and van der Laan, M.J. and Dudoit, S.},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {124},
	Title = {Asymptotically Optimal Model Selection Method for Regression on Censored Outcomes},
	Year = {2002}}

@book{Gyorfietal02,
	Address = {Berlin Heidelberg New York},
	Author = {L. Gy\"{o}rfi and M. Kohler and A. Krzy\.{z}ak and H. Walk},
	Pages = {100--102},
	Publisher = {Springer},
	Title = {A distribution-free theory of nonparametric regression},
	Year = {2002}}

@article{Stone77,
	Author = {M. Stone},
	Journal = {Biometrika},
	Number = {1},
	Pages = {29--35},
	Title = {Asymptotics for and against cross-validation},
	Volume = {64},
	Year = {1977}}

@book{Breimanetal84,
	Address = {Boca Raton},
	Author = {L. Breiman and J.H. Friedman and R. Olshen and C.J. Stone},
	Publisher = {Chapman \& Hall},
	Title = {Classification and regression trees},
	Year = {1984}}

@article{Breiman&Spector92,
	Author = {L. Breiman and P. Spector},
	Journal = {Int Stat Rev},
	Pages = {291--319},
	Title = {Submodel Selection and Evaluation in Regression. {T}he {$X$} Random Case},
	Volume = {60},
	Year = {1992}}

@book{Efron&Tibshirani93,
	Address = {Boca Raton},
	Author = {B. Efron and R. J. Tibshirani},
	Publisher = {Chapman \& Hall},
	Title = {An Introduction to the bootstrap},
	Year = {1993}}

@article{Breiman96,
	Author = {L. Breiman},
	Journal = {Ann Stat},
	Number = {6},
	Pages = {2350--2383},
	Title = {Heuristics of instability and stabilization in model selection},
	Volume = {24},
	Year = {1996}}

@techreport{Breiman96c,
	Author = {L. Breiman},
	Institution = {Department of Statistics, University of California, Berkeley},
	Title = {Out-of-bag estimation},
	Type = {Technical {R}eport},
	Year = {1996}}

@book{Ripley96,
	Address = {New York},
	Author = {B.D. Ripley},
	Publisher = {Cambridge},
	Title = {Pattern recognition and neural networks},
	Year = {1996}}

@article{Breiman98,
	Author = {L. Breiman},
	Journal = {Ann Stat},
	Pages = {801--824},
	Title = {Arcing classifiers},
	Volume = {26},
	Year = {1998}}

@article{Ambroise&McLachlan02,
	Author = {C. Ambroise and G.J. McLachlan},
	Journal = {Proc Natl Acad Sci},
	Number = {10},
	Pages = {6562--6566},
	Title = {Selection bias in gene extraction on the basis of microarray gene-expression data},
	Volume = {99},
	Year = {2002}}

@article{Pavlic&vanderLaan03,
	Author = {M. Pavlic and M.J. van der Laan},
	Journal = {Comput Stat Data An},
	Pages = {413--428},
	Title = {Fitting of mixtures with unspecified number of components using cross validation distance estimate},
	Volume = {41},
	Year = {2003}}

@inproceedings{Akaike73,
	Address = {Budapest},
	Author = {H. Akaike},
	Booktitle = {Second International Symposium on Information Theory},
	Editor = {B.N. Petrov and F. Csaki},
	Organization = {Academiai Kiado},
	Title = {Information theory and an extension of the maximum likelihood principle},
	Year = {1973}}

@article{Bozdogan00,
	Author = {H. Bozdogan},
	Journal = {J Math Psychol},
	Pages = {62--91},
	Title = {Akaike's information criterion and recent developments in information complexity},
	Volume = {44},
	Year = {2000}}

@article{Schwartz78,
	Author = {G. Schwartz},
	Journal = {Ann Stat},
	Pages = {461--464},
	Title = {Estimating the Dimension of a Model},
	Volume = {6},
	Year = {1978}}

@article{Rissanen78,
	Author = {J. Rissanen},
	Journal = {Automatica},
	Pages = {465--471},
	Title = {Modelling by shortest data description},
	Volume = {14},
	Year = {1978}}

@incollection{Bozdogan93,
	Address = {Berlin Heidelberg New York},
	Author = {H. Bozdogan},
	Booktitle = {Information and classification},
	Editor = {O. Opitz and B. Lausen and R. Klar},
	Publisher = {Springer},
	Title = {Choosing the number of component clusters in the mixture model using a new informational complexity criterion of the inverse Fisher information matrix},
	Year = {1993}}

@article{Snowden&Rose&Mortimer11,
	Author = {J.M. Snowden and S. Rose and K.M. Mortimer},
	Journal = {Am J Epidemiol},
	Number = {00},
	Pages = {000--000},
	Title = {Implementation of G-Computation on a Simulated Data set: demonstration of a Causal Inference Technique},
	Volume = {173},
	Year = {2011}}

@article{Rose&Snowden&Mortimer11,
	Author = {S. Rose and J.M. Snowden and K.M. Mortimer},
	Journal = {Am J Epidemiol},
	Number = {00},
	Pages = {000--000},
	Title = {Rose et al. Respond to ``{G}-Computation and Standardization in Epidemiology''},
	Volume = {173},
	Year = {2011}}

@incollection{Robins99b,
	Address = {Berlin Heidelberg New York},
	Author = {Robins, J.M.},
	Booktitle = {Statistical models in epidemiology: the environment and clinical trials},
	Publisher = {Springer},
	Title = {Marginal structural models versus structural nested models as tools for causal inference},
	Year = {1999}}

@article{Hernan2000,
	Author = {M.A. Hern\'{a}n and B. Brumback and J.M. Robins},
	Date-Modified = {2012-08-23 11:06:09 -0700},
	Journal = {Epidemiol},
	Keywords = {Roadmap + MSM},
	Note = {PMID: 10955409},
	Number = {5},
	Pages = {561--570},
	Title = {Marginal structural models to estimate the causal effect of zidovudine on the survival of {HIV}-positive men},
	Volume = {11},
	Year = {2000}}

@article{Robins&Rotnitzky&vanderLaan00,
	Author = {J.M. Robins and A. Rotnitzky and M.J. van der Laan},
	Journal = {J Am Stat Assoc},
	Pages = {431--435},
	Title = {Comment on ``{O}n profile likelihood"},
	Volume = {450},
	Year = {2000}}

@inproceedings{Robins2000b,
	Address = {Alexandria, VA},
	Author = {J.M. Robins},
	Booktitle = {1999 Proceedings of the American Statistical Association},
	Date-Modified = {2012-08-26 20:55:09 -0700},
	Pages = {6-10},
	Publisher = {American Statistical Association},
	Title = {Robust estimation in sequentially ignorable missing data and causal inference models},
	Year = {2000}}

@article{Robins&Rotnitzky01,
	Author = {J.M. Robins and A. Rotnitzky},
	Journal = {Stat Sinica},
	Number = {4},
	Pages = {920--936},
	Title = {Comment on the {B}ickel and {K}won article, ``{I}nference for semiparametric models: some questions and an answer''},
	Volume = {11},
	Year = {2001}}

@incollection{Robins&Rotnitzky92,
	Address = {Basel},
	Author = {J.M. Robins and A. Rotnitzky},
	Booktitle = {AIDS epidemiology},
	Publisher = {Birkh\"{a}user},
	Title = {Recovery of information and adjustment for dependent censoring using surrogate markers},
	Year = {1992}}

@article{Robins2000,
	Author = {J.M. Robins and M.A. Hern\'{a}n and B. Brumback},
	Date-Modified = {2012-08-23 10:26:28 -0700},
	Journal = {Epidemiology},
	Keywords = {Roadmap},
	Note = {PMID: 10955408},
	Number = {5},
	Pages = {550--560},
	Title = {Marginal structural models and causal inference in epidemiology},
	Volume = {11},
	Year = {2000}}

@article{Mortimeretal05,
	Author = {K.M. Mortimer and R. Neugebauer and M.J. van der Laan and I.B. Tager},
	Journal = {Am J Epidemiol},
	Number = {4},
	Pages = {382--388},
	Title = {An Application of Model-Fitting Procedures for Marginal Structural Models},
	Volume = {162},
	Year = {2005}}

@article{Cole2008,
	Annote = {http://www.ncbi.nlm.nih.gov/pmc/articles/PMC2732954/},
	Author = {S.R. Cole and M.A. Hern\'{a}n},
	Date-Modified = {2012-08-26 20:34:41 -0700},
	Journal = {Am J Epidemiol},
	Keywords = {Aim1},
	Note = {PMCID: PMC2732954},
	Number = {6},
	Pages = {656--664},
	Title = {Constructing Inverse Probability Weights for Marginal Structural Models},
	Volume = {168},
	Year = {2008}}

@article{Bembom2007,
	Author = {O. Bembom and M.J. van der Laan},
	Date-Modified = {2012-08-23 18:03:30 -0700},
	Journal = {Electron J Stat},
	Keywords = {Aim1},
	Note = {PMCID: PMC2600532},
	Pages = {574--596},
	Title = {A practical illustration of the importance of realistic individualized treatment rules in causal inference},
	Volume = {1},
	Year = {2007}}

@article{vanderLaan2008casecontrol,
	Author = {M.J. van der Laan},
	Date-Modified = {2012-08-24 09:45:10 -0700},
	Journal = {Int J Biostat},
	Keywords = {Application},
	Note = {PMID: 22462152},
	Number = {1},
	Pages = {Article 17},
	Title = {Estimation based on case-control designs with known prevalance probability},
	Volume = {4},
	Year = {2008}}

@article{Rose2008,
	Author = {S. Rose and M.J. van der Laan},
	Date-Modified = {2012-08-24 09:43:57 -0700},
	Journal = {Int J Biostat},
	Keywords = {Application},
	Note = {PMCID: PMC2835459},
	Number = {1},
	Pages = {Article 19},
	Title = {Simple optimal weighting of cases and controls in case-control studies},
	Volume = {4},
	Year = {2008}}

@article{Rose2009,
	Author = {S. Rose and M.J. van der Laan},
	Date-Modified = {2012-08-24 09:43:07 -0700},
	Journal = {Int J Biostat},
	Keywords = {Application},
	Note = {PMCID: PMC2827892},
	Number = {1},
	Pages = {Article 1},
	Title = {Why match? {I}nvestigating matched case-control study designs with causal effect estimation},
	Volume = {5},
	Year = {2009}}

@inproceedings{Moore2009c,
	Address = {Boca Raton},
	Author = {K.L. Moore and M.J. van der Laan},
	Booktitle = {Design and Analysis Clinical Trials with Time-to-Event Endpoints},
	Date-Modified = {2012-08-26 20:23:23 -0700},
	Editor = {Karl E. Peace},
	Keywords = {App},
	Publisher = {Chapman \& Hall/CRC},
	Title = {Application of Time-to-Event Methods in the Assessment of Safety in Clinical Trials},
	Year = {2009}}

@article{Moore2009,
	Author = {Moore, K.L. and van der Laan, M.J.},
	Date-Modified = {2012-08-26 00:15:23 -0700},
	Journal = {Stat Med},
	Keywords = {Application},
	Note = {PMCID: PMC2857590},
	Number = {1},
	Pages = {39--64},
	Title = {Covariate Adjustment in Randomized Trials with Binary Outcomes: {T}argeted Maximum Likelihood Estimation},
	Volume = {28},
	Year = {2009}}

@article{Moore2009b,
	Author = {Moore, K.L. and van der Laan, M.J.},
	Date-Modified = {2012-08-26 00:22:36 -0700},
	Journal = {J Biopharm Stat},
	Keywords = {Application},
	Note = {PMID: 20183467},
	Number = {6},
	Pages = {1099--1131},
	Title = {Increasing Power in Randomized Trials with Right Censored Outcomes Through Covariate Adjustment},
	Volume = {19},
	Year = {2009}}

@article{Bembom2009,
	Author = {O. Bembom and M.L. Petersen and S.-Y. Rhee and W.J. Fessel and S.E. Sinisi and R.W. Shafer and M.J. van der Laan},
	Date-Modified = {2012-08-24 10:55:57 -0700},
	Journal = {Stat Med},
	Keywords = {Application},
	Note = {PMID: 18825650},
	Number = {1},
	Pages = {152--721},
	Title = {Biomarker discovery using targeted maximum likelihood estimation: application to the treatment of antiretroviral resistant {HIV} infection},
	Volume = {28},
	Year = {2009}}

@article{Rosenblum2009,
	Author = {M. Rosenblum and S.G. Deeks and M.J. van der Laan and D.R. Bangsberg},
	Date-Modified = {2012-08-26 00:27:48 -0700},
	Journal = {PLoS ONE},
	Keywords = {Application},
	Note = {PMCID: PMC2747009},
	Number = {9},
	Pages = {e7196},
	Title = {The Risk of Virologic Failure Decreases with Duration of {HIV} Suppression, at Greater than 50\% Adherence to Antiretroviral Therapy},
	Volume = {4},
	Year = {2009}}

@article{Gruber2010ctmle,
	Author = {S. Gruber and M.J. van der Laan},
	Date-Modified = {2012-08-24 11:27:25 -0700},
	Journal = {Int J Biostat},
	Keywords = {TMLE},
	Note = {PMCID: PMC3126668},
	Number = {1},
	Title = {An application of collaborative targeted maximum likelihood estimation in causal inference and genomics},
	Volume = {6},
	Year = {2010},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAZQAAAAAAZQAAgAADE1hY2ludG9zaCBIRAAAAAAAAAAAAAAAAAAAAMobz/1IKwAABsaXyg8yMDEwX0dydWJlci5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAHROAxzF0WKwAAAAAAAAAAAAEAAgAACSAAAAAAAAAAAAAAAAAAAAAKTGl0ZXJhdHVyZQAQAAgAAMocMm0AAAARAAgAAMxdeJsAAAABABAGxpfKAAxX9QAMUlIAAAAeAAIAO01hY2ludG9zaCBIRDpVc2VyczpsYXVyYTpEZXNrdG9wOkxpdGVyYXR1cmU6MjAxMF9HcnViZXIucGRmAAAOACAADwAyADAAMQAwAF8ARwByAHUAYgBlAHIALgBwAGQAZgAPABoADABNAGEAYwBpAG4AdABvAHMAaAAgAEgARAASAC5Vc2Vycy9sYXVyYS9EZXNrdG9wL0xpdGVyYXR1cmUvMjAxMF9HcnViZXIucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi9MaXRlcmF0dXJlLzIwMTBfR3J1YmVyLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAI4AjoCPwJIAlMCVwJlAmwCdQKVApoCnQKqAq8AAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACwQ==}}

@article{Rosenblum2010,
	Author = {M. Rosenblum and M.J. van der Laan},
	Date-Modified = {2012-08-23 17:02:41 -0700},
	Journal = {Int J Biostat},
	Keywords = {MSM},
	Note = {PMCID: PMC3126671},
	Number = {2},
	Pages = {Article 19},
	Title = {Targeted maximum likelihood estimation of the parameter of a marginal structural model},
	Volume = {6},
	Year = {2010}}

@book{Dudoit&vanderLaan08,
	Address = {Berlin Heidelberg New York},
	Author = {S. Dudoit and M.J. van der Laan},
	Publisher = {Springer},
	Title = {Resampling based multiple testing with applications to genomics},
	Year = {2008}}

@article{Robins94,
	Author = {J.M. Robins},
	Journal = {Commun Stat},
	Pages = {2379--2412},
	Title = {Correcting for noncompliance in randomized trials using structural nested mean models},
	Volume = {23},
	Year = {1994}}

@article{Robins&Rotnitzky&Zhao95,
	Author = {J.M. Robins and A. Rotnitzky and L.P. Zhao},
	Journal = {J Am Stat Assoc},
	Pages = {106--121},
	Title = {Analysis of semiparametric regression models for repeated outcomes in the presence of missing data.},
	Volume = {90},
	Year = {1995}}

@article{Scharfstein&Rotnitzky&Robins99,
	Author = {D.O. Scharfstein and A. Rotnitzky and J.M. Robins},
	Journal = {J Am Stat Assoc},
	Pages = {1096-1120 (1121-1146)},
	Title = {Adjusting for Nonignorable Drop-out Using Semiparametric Nonresponse Models, (with Discussion and Rejoinder)},
	Volume = {94},
	Year = {1999}}

@article{Leon&Tsiatis&Davidian03,
	Author = {S. Leon and A.A. Tsiatis and M. Davidian},
	Journal = {Biometrics},
	Pages = {1046--1055},
	Title = {Semiparametric estimation of treatment effect in a pretest-posttest study},
	Volume = {59},
	Year = {2003}}

@article{Tan06,
	Author = {Z. Tan},
	Journal = {J Am Stat Assoc},
	Pages = {1619-1637},
	Title = {A distributional approach for causal inference using propensity scores},
	Volume = {101},
	Year = {2006}}

@book{Tsiatis2006,
	Address = {Berlin Heidelberg New York},
	Author = {A.A. Tsiatis},
	Date-Modified = {2012-08-22 21:08:28 -0700},
	Keywords = {Book},
	Publisher = {Springer},
	Title = {{Semiparametric Theory and Missing Data}},
	Year = {2006}}

@article{Zhang&Tsiatis&Davidian08,
	Author = {M. Zhang and A.A. Tsiatis and M. Davidian},
	Journal = {Biometrics},
	Number = {3},
	Pages = {707--715},
	Title = {Improving efficiency of inferences in randomized clinical trials using auxiliary covariates},
	Volume = {64},
	Year = {2008}}

@article{Rubin&vanderLaan08,
	Author = {Daniel B. Rubin and M.J. van der Laan},
	Journal = {Int J Biostat},
	Number = {1},
	Pages = {Article 5},
	Title = {Empirical efficiency maximization: improved locally efficient covariate adjustment in randomized experiments and survival analysis},
	Volume = {4},
	Year = {2008}}

@article{Freedman08,
	Author = {D.A. Freedman},
	Journal = {Adv Appl Math},
	Pages = {180--193},
	Title = {On regression adjustments to experimental data},
	Volume = {40},
	Year = {2008}}

@article{Freedman082,
	Author = {D.A. Freedman},
	Journal = {Ann Appl Stat},
	Pages = {176--96},
	Title = {On regression adjustments to experiments with several treatments},
	Volume = {2},
	Year = {2008}}

@article{Rosenblum2009b,
	Author = {M. Rosenblum and M.J. van der Laan},
	Date-Modified = {2012-08-26 01:20:38 -0700},
	Journal = {Biometrics},
	Keywords = {App},
	Note = {PMCID: PMC2748134},
	Number = {3},
	Pages = {937--945},
	Title = {Using Regression Models to Analyze Randomized Trials: asymptotically Valid Hypothesis Tests Despite Incorrectly Specified Models},
	Volume = {65},
	Year = {2009}}

@book{Hampeletal86,
	Address = {New York},
	Author = {Hampel, F.R. and Ronchetti, E.M. and Rousseeuw, P.J. and Stahel, W.A.},
	Publisher = {Wiley},
	Title = {{Robust statistics: the approach based on influence functions}},
	Year = {1986}}

@book{vanderVaart98,
	Address = {New York},
	Author = {A.W. van der Vaart},
	Publisher = {Cambridge},
	Title = {Asymptotic statistics},
	Year = {1998}}

@book{vanderVaartWellner1996,
	Address = {Berlin Heidelberg New York},
	Author = {A.W. van der Vaart and J.A. Wellner},
	Date-Modified = {2012-08-24 12:13:06 -0700},
	Publisher = {Springer},
	Title = {Weak convergence and empirical processes},
	Year = {1996}}

@article{Rosenbaum&Rubin83,
	Author = {P.R. Rosenbaum and Donald B. Rubin},
	Journal = {Biometrika},
	Pages = {41--55},
	Title = {The central role of the propensity score in observational studies for causal effects},
	Volume = {70},
	Year = {1983}}

@article{Stitelman2010ctmle,
	Author = {O.M. Stitelman and M.J. van der Laan},
	Date-Modified = {2012-08-24 11:27:04 -0700},
	Journal = {Int J Biostat},
	Keywords = {TMLE},
	Note = {PMID: 21969976},
	Number = {1},
	Pages = {Article 21},
	Title = {Collaborative targeted maximum likelihood for time to event data},
	Volume = {6},
	Year = {2010}}

@article{Wedderburn74,
	Author = {R.W.M. Wedderburn},
	Journal = {Biometrika},
	Number = {3},
	Pages = {439--447},
	Title = {Quasi-likelihood functions, generalized linear models, and the Gauss-Newton method},
	Volume = {61},
	Year = {1974}}

@article{McCullagh83,
	Author = {P. Mc{C}ullagh},
	Journal = {Ann Stat},
	Pages = {59--67},
	Title = {Quasi-likelihood functions},
	Volume = {11},
	Year = {1983}}

@article{vanderLaan2008de,
	Author = {M.J. van der Laan and M.L. Petersen},
	Date-Modified = {2012-08-24 13:46:46 -0700},
	Journal = {Int J Biostat},
	Keywords = {NDE},
	Note = {PMID: 22462121},
	Number = {1},
	Pages = {Article 23},
	Title = {Direct effect models},
	Volume = {4},
	Year = {2008}}

@techreport{vanderLaan2010community,
	Author = {M.J. van der Laan},
	Date-Modified = {2012-08-26 21:16:04 -0700},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Keywords = {Community},
	Note = {Available at \url{http://biostats.bepress.com/ucbbiostat/paper268/}},
	Number = {268},
	Title = {Estimation of Causal Effects of Community-Based Interventions},
	Year = {2010}}

@article{Heckman&Ichimura&Todd97,
	Author = {J. Heckman and H. Ichimura and R. Todd},
	Journal = {Rev of Econ Stud},
	Pages = {605--654},
	Title = {Matching as an Econometric Evaluation Estimator: evidence from Evaluating a Job Training Programme},
	Volume = {64},
	Year = {1997}}

@techreport{Sekhon06,
	Author = {J.S. Sekhon},
	Institution = {University of California, Berkeley},
	Title = {Alternative balance metrics for bias reduction in matching methods for causal inference},
	Type = {Technical {R}eport},
	Year = {2006}}

@article{Hansen08,
	Author = {B.B. Hansen},
	Journal = {Biometrika},
	Pages = {481--8},
	Title = {The prognostic analogue of the propensity score},
	Volume = {95},
	Year = {2008}}

@book{Haignere02,
	Address = {Washington, DC},
	Author = {Haignere, L.},
	Edition = {2nd},
	Publisher = {American Association of University Professors},
	Title = {Paychecks: a guide to conducting salary-equity studies for higher education faculty},
	Year = {2002}}

@article{Holland88,
	Author = {P.W. Holland},
	Journal = {Stat Sci},
	Number = {2},
	Pages = {186--188.},
	Title = {Comment: Causal Mechanism or Causal Effect: which Is Best for Statistical Science?},
	Volume = {3},
	Year = {1988}}

@article{Robins98,
	Author = {J.M. Robins},
	Journal = {1997 Proceedings of the American Statistical Association. Section on {B}ayesian Statistical Science},
	Pages = {1--10},
	Title = {Marginal Structural Models},
	Year = {1998}}

@article{Mossetal04,
	Author = {A.R. Moss and J.A. Hahn and S. Perry and E.D. Charlebois and D. Guzman and R.A. Clark and D.R. Bangsberg},
	Journal = {Clin Infect Dis},
	Number = {8},
	Pages = {1190--1198},
	Title = {Adherence to highly active antiretroviral therapy in the homeless population in {S}an {F}rancisco: a prospective study},
	Volume = {39},
	Year = {2004}}

@article{Bangsbergetal01,
	Author = {D.R. Bangsberg and F. Hecht and E.D. Charlebois and M. Chesney and A.R. Moss},
	Journal = {AIDS Behav},
	Pages = {275--281},
	Title = {Comparing Objectives Measures of Adherence to HIV Antiretroviral Therapy: electronic Medication Monitors and Unannounced Pill Counts.},
	Volume = {5},
	Year = {2001}}

@article{Neugebauer2007,
	Author = {R. Neugebauer and M. J. van der Laan},
	Date-Modified = {2012-08-26 20:45:08 -0700},
	Journal = {J Stat Plan Infer},
	Keywords = {Roadmap + MSM},
	Number = {2},
	Pages = {419--434},
	Title = {Nonparametric causal effects based on marginal structural models},
	Volume = {137},
	Year = {2007},
	Bdsk-Url-1 = {http://www.sciencedirect.com/science/article/pii/S0378375806000334}}

@article{Efron87,
	Author = {B. Efron},
	Journal = {J Am Stat Assoc},
	Number = {397},
	Pages = {171--185},
	Title = {Better Bootstrap Confidence Intervals},
	Volume = {82},
	Year = {1987}}

@article{Kirschetal08,
	Author = {I. Kirsch and B.J. Deacon and T.B. Huedo-Medina and A. Scoboria and T.J. Moore and B.T. Johnson},
	Journal = {PLoS Med},
	Number = {2},
	Pages = {e45. doi:10.1371/journal.pmed.0050045},
	Title = {Initial Severity and Antidepressant Benefits: a Meta-Analysis of Data Submitted to the {Food and Drug Administration}},
	Volume = {5},
	Year = {2008}}

@article{Baselga01,
	Author = {J. Baselga},
	Journal = {Oncology},
	Pages = {14--21},
	Title = {Herceptin alone or in combination with chemotherapy in the treatment of {HER2}-positive metastatic breast cancer: pivotal trials},
	Volume = {61(S2)},
	Year = {2001}}

@techreport{Wangetal06,
	Author = {Y. Wang and M.L. Petersen and D.R. Bangsberg and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {211},
	Title = {Diagnosing Bias in the Inverse Probability of Treatment Weighted Estimator Resulting from Violation of Experimental Treatment Assignment.},
	Year = {2006}}

@article{Robins87,
	Author = {Robins, J.M.},
	Journal = {Comput Math Appl},
	Number = {9--12},
	Pages = {923--945},
	Title = {Addendum to: ``{A} new approach to causal inference in mortality studies with a sustained exposure period---application to control of the healthy worker survivor effect''},
	Volume = {14},
	Year = {1987}}

@article{Robins872,
	Author = {J.M. Robins},
	Journal = {J Chron Dis (40, Supplement)},
	Pages = {139s--161s},
	Title = {A graphical approach to the identification and estimation of causal parameters in mortality studies with sustained exposure periods},
	Volume = {2},
	Year = {1987}}

@article{Rosenblum&vanderLaan09b,
	Author = {M. Rosenblum and M.J. van der Laan},
	Journal = {Int J Biostat},
	Pages = {Article 4},
	Title = {Confidence Intervals for the Population Mean Tailored to Small Sample Sizes, with Applications to Survey Sampling},
	Volume = {1},
	Year = {2009}}

@article{Neugebauer2005,
	Author = {Neugebauer, R. and van der Laan, M.J.},
	Date-Modified = {2012-08-26 21:21:41 -0700},
	Journal = {J Stat Plan Infer},
	Number = {1-2},
	Pages = {405--26},
	Title = {Why prefer double robust estimates in causal inference?},
	Volume = {129},
	Year = {2005}}

@techreport{Mooreetal09,
	Author = {K.L. Moore and R.S. Neugebauer and M.J. van der Laan and I.B. Tager},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {255},
	Title = {Causal Inference in Epidemiological Studies with Strong Confounding},
	Year = {2009}}

@article{Kish92,
	Author = {L. Kish},
	Journal = {J Off Stat},
	Pages = {183--200},
	Title = {Weighting for unequal $P_i$},
	Volume = {8},
	Year = {1992}}

@techreport{Bembom2008,
	Author = {O. Bembom and M.J. van der Laan},
	Date-Modified = {2012-08-26 21:02:51 -0700},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Keywords = {Aim1},
	Note = {Available at \url{http://biostats.bepress.com/ucbbiostat/paper230}},
	Number = {230},
	Title = {Data-adaptive selection of the truncation level for Inverse-Probability-of-Treatment-Weighted estimators},
	Year = {2008},
	Bdsk-Url-1 = {http://biostats.bepress.com/ucbbiostat/paper230}}

@article{Freedman&Berk08,
	Author = {D.A. Freedman and R.A. Berk},
	Journal = {Eval Rev},
	Pages = {392--409},
	Title = {Weighting Regressions by Propensity Scores},
	Volume = {3},
	Year = {2008}}

@article{Petersenetal10,
	Author = {M.L. Petersen and K.E. Porter and S. Gruber and Y. Wang and M.J. van der Laan},
	Journal = {Stat Meth Med Res},
	Title = {Diagnosing and responding to violations in the positivity assumption},
	Volume = {published online 28 Oct (doi: 10.1177/0962280210386207)},
	Year = {2010}}

@article{Johnsonetal09,
	Author = {V.A. Johnson and F. Brun-Vezinet and B. Clotet and H.F. Gunthard and D.R. Kuritzkes and D. Pillay and J.M. Schapiro and D.D. Richman},
	Journal = {Top HIV Med},
	Number = {5},
	Pages = {138--45},
	Title = {Update of the drug resistance mutations in {HIV}-1: {D}ecember 2009.},
	Volume = {17},
	Year = {2009}}

@techreport{Bembometal08b,
	Author = {O. Bembom and W.J. Fessel and R.W. Shafer and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Title = {Data-adaptive Selection Of The Adjustment Set In Variable Importance Estimation},
	Type = {231},
	Year = {2008}}

@techreport{Crumpetal06,
	Author = {R.K. Crump and V.J. Hotz and G.W. Imbens and O.A. Mitnik},
	Institution = {National Bureau of Economic Research},
	Number = {330},
	Title = {Moving the goalposts: addressing limited overlap in the estimation of average treatment effects by changing the estimand},
	Year = {2006}}

@article{LaLonde86,
	Author = {R.J. LaLonde},
	Journal = {Am Econ Rev},
	Pages = {604--620},
	Title = {Evaluating the Econometric Evaluations of Training Programs with Experimental Data},
	Volume = {76},
	Year = {1986}}

@article{Dehejia&Wahba99,
	Author = {R. Dehejia and S. Wahba},
	Journal = {J Am Stat Assoc},
	Pages = {1053--1062},
	Title = {Causal Effects in Nonexperimental Studies: reevaluating the Evaluation of Training Programs},
	Volume = {94},
	Year = {1999}}

@article{vanderLaan2007indvtxt,
	Author = {M.J. van der Laan and M.L. Petersen},
	Date-Modified = {2012-08-26 20:33:40 -0700},
	Journal = {Int J Biostat},
	Keywords = {Aim1},
	Note = {PMCID: PMC2613338},
	Number = {1},
	Pages = {Article 3},
	Title = {Causal Effect Models for Realistic Individualized Treatment and Intention to Treat Rules},
	Volume = {3},
	Year = {2007}}

@article{Robins2008,
	Author = {J.M. Robins and L. Orellana and A. Rotnitzky},
	Date-Modified = {2012-08-22 21:31:41 -0700},
	Journal = {Stat Med},
	Keywords = {Aim1},
	Note = {PMID: 18646286},
	Number = {23},
	Pages = {4678--4721},
	Title = {Estimation and extrapolation of optimal treatment and testing strategies},
	Volume = {27},
	Year = {2008}}

@article{Cochran57,
	Author = {W.G. Cochran},
	Journal = {Biometrics},
	Pages = {261--281},
	Title = {Analysis of Covariance: its Nature and Uses.},
	Volume = {13},
	Year = {1957}}

@techreport{Moore&vanderLaan07,
	Author = {K.L. Moore and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Month = {April},
	Number = {215},
	Title = {Covariate adjustment in randomized trials with binary outcomes},
	Year = {2007}}

@article{Rosenblum2010b,
	Author = {M. Rosenblum and M.J. van der Laan},
	Date-Modified = {2012-08-26 00:37:20 -0700},
	Journal = {Int J Biostat},
	Keywords = {Application},
	Note = {PMCID: PMC2898625},
	Number = {1},
	Pages = {Article 13},
	Title = {Simple, Efficient Estimators of Treatment Effects in Randomized Trials Using Generalized Linear Models to Leverage Baseline Variables},
	Volume = {6},
	Year = {2010}}

@article{Freedman083,
	Author = {D.A. Freedman},
	Journal = {Stat Sci},
	Pages = {237--249},
	Title = {Randomization does not justify logistic regression},
	Volume = {23},
	Year = {2008}}

@article{Yang&Tsiatis01,
	Author = {L. Yang and A.A. Tsiatis},
	Journal = {Am Stat},
	Pages = {29--38},
	Title = {Efficiency study for a treatment effect in a pretest-posttest trial},
	Volume = {56},
	Year = {2001}}

@book{McCullagh&Nelder89,
	Address = {Boca Raton},
	Author = {P. McCullagh and J.A. Nelder},
	Edition = {2nd},
	Publisher = {Chapman \& Hall},
	Title = {Generalized linear models},
	Year = {1989}}

@incollection{Gail86,
	Address = {New York},
	Author = {M.H. Gail},
	Booktitle = {Modern Statistical Methods in Chronic Disease Epidemiology},
	Editor = {S.~H. Moolvankar and R.~L. Prentice},
	Publisher = {Wiley},
	Title = {Adjusting for covariates that have the same distribution in exposed and unexposed cohorts},
	Year = {1986}}

@article{Tsiatisetal08,
	Author = {A.A. Tsiatis and M. Davidian and M. Zhang and X. Lu},
	Journal = {Stat Med},
	Pages = {4658--4677},
	Title = {Covariate adjustment for two-sample treatment comparisons in randomized clinical trials: a principled yet flexible approach},
	Volume = {27},
	Year = {2008}}

@article{Kochetal98,
	Author = {G.G. Koch and C.M. Tangen and J.W. Jung and I.A. Amara},
	Journal = {Stat Med},
	Pages = {1863--1892},
	Title = {Issues for covariance analysis of dichotomous and ordered categorical data from randomized clinical trials and nonparametric strategies for addressing them},
	Volume = {17},
	Year = {1998}}

@article{Pococketal02,
	Author = {S.J. Pocock and S.E. Assmann and L.E. Enos and L.E. Kasten},
	Journal = {Stat Med},
	Pages = {2917--2930},
	Title = {Subgroup analysis, covariate adjustment, and baseline comparisons in clinical trial reporting: current practice and problems.},
	Volume = {21},
	Year = {2002}}

@article{Anderson72,
	Author = {J.A. Anderson},
	Journal = {Biometrika},
	Pages = {19--35},
	Title = {Separate sample logistic discrimination},
	Volume = {59},
	Year = {1972}}

@article{Robins99,
	Author = {J.M. Robins},
	Journal = {Stat Sci},
	Number = {3},
	Pages = {281--293},
	Title = {[{C}hoice as an Alternative to Control in Observational Studies]: Comment},
	Volume = {14},
	Year = {1999}}

@article{Manssonetal07,
	Author = {R. Mansson and M.M. Joffe and W. Sun and S. Hennessy},
	Journal = {Am J Epidemiol},
	Number = {3},
	Pages = {332-339},
	Title = {On the Estimation and Use of Propensity Scores in Case-Control and Case-Cohort Studies.},
	Volume = {166},
	Year = {2007}}

@article{Prentice&Pyke79,
	Author = {R.L. Prentice and R. Pyke},
	Journal = {Biometrika},
	Pages = {403--411},
	Title = {Logistic disease incidence models and case-control studies},
	Volume = {66},
	Year = {1979}}

@book{Breslow&Day80,
	Address = {Lyon},
	Author = {N.E. Breslow and N.E. Day},
	Publisher = {International Agency for Research on Cancer},
	Title = {Statistical methods in cancer research: {V}olume 1 -- {T}he analysis of case-control studies},
	Year = {1980}}

@article{Breslow96,
	Author = {N.E. Breslow},
	Journal = {J Am Stat Soc},
	Pages = {14--28},
	Title = {Statistics in Epidemiology: the Case-Control Study},
	Volume = {91},
	Year = {1996}}

@article{Greenland81,
	Author = {S. Greenland},
	Journal = {J Chron Dis},
	Pages = {445--453},
	Title = {Multivariate Estimation of Exposure-Specific Incidence from Case-Control Studies.},
	Volume = {34},
	Year = {1981}}

@incollection{Holland&Rubin88,
	Address = {Cambridge, MA},
	Author = {P.W. Holland and Donald B. Rubin},
	Booktitle = {Matched sampling for causal effects.},
	Editor = {Donald B. Rubin},
	Publisher = {Cambridge},
	Title = {Causal inference in retrospective studies},
	Year = {1988}}

@article{Greenland04,
	Author = {S. Greenland},
	Journal = {Am J Epidemiol},
	Number = {4},
	Pages = {301--305},
	Title = {Model-based Estimation of Relative Risks and Other Epidemiologic Measures in Studies of Common Outcomes and in Case-Control Studies.},
	Volume = {160},
	Year = {2004}}

@article{Newman06,
	Author = {S. Newman},
	Journal = {Epid Persp Innov},
	Pages = {2},
	Title = {Causal analysis of case-control data},
	Volume = {3},
	Year = {2006}}

@article{Cornfield51,
	Author = {J. Cornfield},
	Journal = {J Nat Cancer Inst},
	Pages = {1269--1275},
	Title = {A method of estimating comparative rates from clinical data. Applications to cancer of the lung, breast, and cervix.},
	Volume = {11},
	Year = {1951}}

@inproceedings{Cornfield56,
	Address = {Berkeley},
	Author = {J. Cornfield},
	Booktitle = {Proceedings of the 3rd Berkeley symposium, {V}ol IV},
	Editor = {J. Neyman},
	Publisher = {University of California Press},
	Title = {A statistical problem arising from retrospective studies},
	Year = {1956}}

@article{Prentice&Breslow78,
	Author = {R.L. Prentice and N.E. Breslow},
	Journal = {Biometrika},
	Number = {1},
	Pages = {153--158},
	Title = {Retrospective studies and failure time models.},
	Volume = {65},
	Year = {1978}}

@article{Moriseetal96,
	Author = {A.P. Morise and G.A. Diamon and R. Detrano and M. Bobbio and Erdogan Gunel},
	Journal = {Med Decis Making},
	Pages = {133--142},
	Title = {The Effect of Disease-prevalence Adjustments on the Accuracy of a Logistic Prediction Model.},
	Volume = {16},
	Year = {1996}}

@article{Wacholder96,
	Author = {S. Wacholder},
	Journal = {Epidemiol},
	Number = {2},
	Pages = {144--150},
	Title = {The Case-Control Study as Data Missing by Design: estimating Risk Differences.},
	Volume = {7},
	Year = {1996}}

@article{Rose2011,
	Author = {S. Rose and M.J. van der Laan},
	Date-Modified = {2012-08-26 00:49:30 -0700},
	Journal = {Int J Biostat},
	Keywords = {App},
	Note = {PMCID: PMC3083136},
	Number = {17},
	Title = {A Targeted Maximum Likelihood Estimator for Two-Stage Designs},
	Volume = {7},
	Year = {2011}}

@article{Freedman50,
	Author = {R. Freedman},
	Journal = {Am J of Soc},
	Number = {5},
	Pages = {485--487},
	Title = {Incomplete Matching in Ex Post Facto Studies},
	Volume = {55},
	Year = {1950}}

@article{Cochran65,
	Author = {W.G. Cochran},
	Journal = {J R Stat Soc Ser A Gen},
	Number = {2},
	Pages = {234--266},
	Title = {The Planning of Observational Studies of Human Populations},
	Volume = {128},
	Year = {1965}}

@article{Billewicz65,
	Author = {W.Z. Billewicz},
	Journal = {Biometrics},
	Number = {3},
	Pages = {623--644},
	Title = {The Efficiency of Matched Samples: an Empirical Investigation},
	Volume = {21},
	Year = {1965}}

@article{McKinlay77,
	Author = {S.M. McKinlay},
	Journal = {Biometrics},
	Number = {4},
	Pages = {725--735},
	Title = {Pair-Matching -- A reappraisal of a Popular Technique},
	Volume = {33},
	Year = {1977}}

@article{Kupperetal81,
	Author = {L.L. Kupper and J.M. Karon and D.G. Kleinbaum and H. Morgenstern and D.K. Lewis},
	Journal = {Biometrics},
	Pages = {271--291},
	Title = {Matching in Epidemiologic Studies: validity and Efficiency Considerations},
	Volume = {37},
	Year = {1981}}

@article{Costanza95,
	Author = {M.C. Costanza},
	Journal = {Prev Med},
	Pages = {425--433},
	Title = {Matching},
	Volume = {24},
	Year = {1995}}

@book{Schlesselman82,
	Address = {Oxford},
	Author = {J.J. Schlesselman},
	Publisher = {Oxford},
	Title = {Case-control studies: design, conduct, analysis},
	Year = {1982}}

@article{Vandenbroukeetal07,
	Author = {J.P. Vandenbrouke and E. von Elm and D.G. Altman and P.C. Gotzsche and C.D. Mulrow and S.J. Pocock and C. Poole and J.J. Schlesselman and M. Egger for the STROBE Initiative},
	Journal = {PLoS Med},
	Number = {10},
	Pages = {1628--1654},
	Title = {Strengthening the Reporting of Observational Studies in Epidemiology ({STROBE}): explanation and Elaboration.},
	Volume = {4},
	Year = {2007}}

@article{Cochran53,
	Author = {W.G. Cochran},
	Journal = {Am J Public Health},
	Pages = {684--691},
	Title = {Matching in Analytical Studies},
	Volume = {43},
	Year = {1953}}

@article{Breslowetal78,
	Author = {N.E. Breslow and N.E. Day and K.T. Halvorsen and R.L. Prentice and C. Sabal},
	Journal = {Am J Epidemiol},
	Number = {4},
	Pages = {299--307},
	Title = {Estimation of Multiple Relative Risk Functions in Matched Case-Control Studies},
	Volume = {108},
	Year = {1978}}

@article{Holford&White&Kelsey78,
	Author = {T.R. Holford and C. White and J.L. Kelsey},
	Journal = {Am J Epidemiol},
	Number = {3},
	Pages = {245--255},
	Title = {Multivariate Analysis for Matched Case-Control Studies},
	Volume = {107},
	Year = {1978}}

@article{Kannel&McGee&Gordon76,
	Author = {W.B. Kannel and D. McGee and T. Gordon},
	Journal = {Am J Cardiol},
	Pages = {46--51},
	Title = {A general cardiovascular risk profile: the {F}ramingham Study},
	Volume = {38},
	Year = {1976}}

@article{Andersonetal91,
	Author = {K.M. Anderson and P.W.F. Wilson and P.M. Odell and W.B. Kannel},
	Journal = {Circulation},
	Pages = {356--362},
	Title = {An updated coronary risk profile. A statement for health professionals.},
	Volume = {83},
	Year = {1991}}

@article{Ramsayetal95,
	Author = {L.E. Ramsay and I.U. Haq and P.R. Jackson and W.W. Yeo},
	Journal = {Lancet},
	Number = {8988},
	Pages = {1467--1471},
	Title = {Sheffield risk and treatment table for cholesterol lowering for primary prevention of coronary heart disease.},
	Volume = {346},
	Year = {1995}}

@article{Ramsayetal96,
	Author = {L.E. Ramsay and I.U. Haq and P.R. Jackson and W.W. Yeo},
	Journal = {Lancet},
	Number = {9036},
	Pages = {1251},
	Title = {The {S}heffield table for primary prevention of coronary heart disease: corrected.},
	Volume = {348},
	Year = {1996}}

@article{Wilsonetal98,
	Author = {P.W.F. Wilson and R.B. D'Agostino and D. Levy and A.M. Belanger and H. Silbershatz and W.B. Kannel},
	Journal = {Circulation},
	Pages = {1837--1847},
	Title = {Prediction of coronary heart disease using risk factor categories},
	Volume = {97},
	Year = {1998}}

@article{Jackson00,
	Author = {R. Jackson},
	Journal = {Br Med J},
	Number = {7236},
	Pages = {709--710},
	Title = {Updated New Zealand cardiovascular disease risk-benefit prediction guide.},
	Volume = {320},
	Year = {2000}}

@article{Gailetal89,
	Author = {M.H. Gail and L.A. Brinton and D.P. Byar and D.K. Corle and S.B. Green and C. Schairer and J.J. Mulvihill},
	Journal = {J Natl Cancer Inst},
	Number = {24},
	Pages = {1879--1886},
	Title = {Projecting individualized probabilities of developing breast cancer for white females who are being examined annually.},
	Volume = {81},
	Year = {1989}}

@article{Costantinoetal99,
	Author = {J.P. Costantino and M.H. Gail and D. Pee and S. Anderson and C.K. Redmond and J. Benichou and H.S. Wieand},
	Journal = {J Natl Cancer Inst},
	Number = {18},
	Pages = {1541--1548},
	Title = {Validation studies for models projecting the risk of invasive and total breast cancer incidence.},
	Volume = {91},
	Year = {1999}}

@article{Tyrer&Duffy&Cuzick04,
	Author = {J. Tyrer and S.W. Duffy and J. Cuzick},
	Journal = {Stat Med},
	Number = {7},
	Pages = {1111--1130},
	Title = {A breast cancer prediction model incorporating familial and personal risk factors},
	Volume = {23},
	Year = {2004}}

@article{Barlowetal06,
	Author = {W.E. Barlow and E. White and R. Ballard-Barbash and P.M. Vacek and L. Titus-Ernstoff and P.A. Carney and J.A. Tice and D.S. Buist and B.M. Geller and R. Rosenberg and B.C. Yankaskas and K. Kerlikowske},
	Journal = {J Natl Cancer Inst},
	Number = {17},
	Pages = {1204--1214},
	Title = {Prospective breats cancer risk prediction model for women undergoing screening mammography.},
	Volume = {98},
	Year = {2006}}

@article{Loprinzietal94,
	Author = {C.L. Loprinzi and J.A. Laurie and H.S. Wieand and J.E. Krook and P.J. Novotny and J.W. Kugler and J. Bartel and M. Law and M. Bateman and N.E. Klatt},
	Journal = {J Clin Oncol},
	Number = {3},
	Pages = {601--607},
	Title = {Prospective Evaluation of Prognostic Variables from Patient-Completed Questionnaires, {N}orth {C}entral {C}ancer {T}reatment {G}roup},
	Volume = {12},
	Year = {1994}}

@manual{Therneau&Lumley09,
	Author = {T. Therneau and T. Lumley},
	Note = {R package version 2.35-8},
	Title = {survival: survival analysis, including penalised likelihood},
	Url = {http://CRAN.R-project.org/package=survival},
	Year = {2009},
	Bdsk-Url-1 = {http://CRAN.R-project.org/package=survival}}

@article{Tibshirani97,
	Author = {R.J. Tibshirani},
	Journal = {Stat Med},
	Pages = {385--395},
	Title = {The Lasso Method for Variable Selection in the {C}ox Model},
	Volume = {16},
	Year = {1997}}

@article{Zhang&Lu07,
	Author = {H.H. Zhang and W. Lu},
	Journal = {Biometrika},
	Number = {3},
	Pages = {691--703},
	Title = {Adaptive Lasso for {C}ox's Proportional Hazards Model},
	Volume = {94},
	Year = {2007}}

@article{Kooperberg&Stone&Truong95,
	Author = {C. Kooperberg and C.J. Stone and Y.K. Truong},
	Journal = {J Am Stat Assoc},
	Number = {429},
	Pages = {78--94},
	Title = {Hazard Regression},
	Volume = {90},
	Year = {1995}}

@article{Leblanc&Crowley92,
	Author = {M. LeBlanc and J. Crowley},
	Journal = {Biometrics},
	Pages = {411--425},
	Title = {Relative Risk trees for censored data},
	Volume = {48},
	Year = {1992}}

@article{Segal88,
	Author = {M.R. Segal},
	Journal = {Biometrics},
	Pages = {35--47},
	Title = {Regression trees for censored data},
	Volume = {44},
	Year = {1988}}

@article{Hothornetal06,
	Author = {T. Hothorn and P. Buhlmann and S. Dudoit and A.M. Molinaro and M.J. van der Laan},
	Journal = {Biostatistics},
	Pages = {355--373},
	Title = {Survival Ensembles},
	Volume = {7},
	Year = {2006}}

@article{Ishwaranetal08,
	Author = {H. Ishwaran and U.B. Kogalur and E.H. Blackstone and M.S. Lauer},
	Journal = {Ann Appl Stat},
	Number = {3},
	Pages = {841--860},
	Title = {Random Survival Forests},
	Volume = {2},
	Year = {2008}}

@article{vanHouwelingenetal06,
	Author = {H.C. van Houwelingen and T. Bruinsma and A.A.M. Hart and L.J. {van't Veer} and L.F.A. Wessels},
	Journal = {Stat Med},
	Pages = {3201--3216},
	Title = {Cross-validated {C}ox Regression on Microarray Gene Expression Data},
	Volume = {25},
	Year = {2006}}

@techreport{vanderLaan&Rubin07,
	Author = {M.J. van der Laan and Daniel B. Rubin},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {226},
	Title = {A note on targeted maximum likelihood and right-censored data},
	Year = {2007}}

@inproceedings{Robins93,
	Author = {J.M. Robins},
	Booktitle = {Proceedings of the Biopharmaceutical Section},
	Organization = {American Statistical Association},
	Title = {Information recovery and bias adjustment in proportional hazards regression analysis of randomized trials using surrogate markers},
	Year = {1993}}

@incollection{Hubbard&vanderLaan&Robins99,
	Address = {Berlin Heidelberg New York},
	Author = {A.E. Hubbard and M.J. van der Laan and J.M. Robins},
	Booktitle = {Statistical models in epidemiology: the environment and clinical trials},
	Editor = {E. Halloran, D. Berry},
	Publisher = {Springer},
	Title = {Nonparametric locally efficient estimation of the treatment specific survival distributions with right censored data and covariates in observational studies},
	Year = {1999}}

@article{Hernandez&Eijkemans&Steyerberg06,
	Author = {Hern\'{a}ndez, A.V. and Eijkemans, M.J. and Steyerberg, E.W.},
	Journal = {Ann Epidemiol},
	Number = {1},
	Pages = {41--48},
	Title = {Randomized controlled trials With time-to-event outcomes: how much does prespecified covariate adjustment increase power?},
	Volume = {16},
	Year = {2006}}

@article{Lu&Tsiatis08,
	Author = {Lu, X. and Tsiatis, A.A},
	Journal = {Biometrika},
	Number = {3},
	Pages = {679--694},
	Title = {Improving the efficiency of the log-rank test using auxiliary covariates},
	Volume = {95},
	Year = {2008}}

@article{Tangen&Koch99,
	Author = {Tangen, C.M. and Koch, G.G.},
	Journal = {J Biopharm Stat},
	Number = {2},
	Pages = {307--338},
	Title = {On-parametric analysis of covariance for hypothesis testing with logrank and {W}ilcoxon scores and survival-rate estimation in a randomized clinical trial},
	Volume = {9},
	Year = {1999}}

@article{Jiangetal08,
	Author = {Jiang, H. and Symanowski, J. and Paul, S. and Qu, Y. and Zagar, A. and Hong, S.},
	Journal = {Stat Med},
	Number = {28},
	Pages = {5850--5860},
	Title = {The type {I} error and power of nonparametric logrank and {W}ilcoxon tests with adjustment for covariates -- A simulation study},
	Volume = {27},
	Year = {2008}}

@article{Akazawa&Nakamura&Palesch97,
	Author = {Akazawa, K. and Nakamura, T. and Palesch, Y.},
	Journal = {Stat Med},
	Number = {5},
	Pages = {583--597},
	Title = {Power of logrank test and {C}ox regression model in clinical trials with heterogenous samples},
	Volume = {16},
	Year = {1997}}

@article{Westeretal10,
	Author = {C.W. Wester and A.M. Thomas and H. Bussmann and S. Moyo and J.M. Gaolathe and V. Novitsky and M. Essex and V. De Gruttola and R.G. Marlink},
	Journal = {AIDS},
	Pages = {S27--S36},
	Title = {Nonnucleoside reverse transcriptase inhibitor outcomes among combination antiretroviral therapy-treated adults in {B}otswana},
	Volume = {24},
	Year = {2010}}

@book{Andersenetal93,
	Address = {Berlin Heidelberg New York},
	Author = {P.K. Andersen and O. Borgan and R.D. Gill and N. Keiding},
	Publisher = {Springer},
	Title = {Statistical models based on counting processes},
	Year = {1993}}

@techreport{Rudser&LeBlanc&Emerson08,
	Author = {K. Rudser and M. LeBlanc and S.S. Emerson},
	Institution = {Department of Biostatistics, University of Washington},
	Number = {335},
	Title = {Estimation for Arbitrary Functionals of Survival},
	Year = {2008}}

@article{vanderLaan10,
	Author = {van der Laan, M.J.},
	Date-Modified = {2012-08-24 10:54:39 -0700},
	Journal = {Int J Biostat},
	Keywords = {tmle},
	Note = {PMID: 21969992},
	Number = {2},
	Pages = {Article 2},
	Title = {Targeted maximum likelihood based causal inference: Part {I}},
	Volume = {6},
	Year = {2010}}

@article{vanderLaan10b,
	Author = {van der Laan, M.J.},
	Date-Modified = {2012-08-24 10:54:44 -0700},
	Journal = {Int J Biostat},
	Keywords = {tmle},
	Note = {PMCID: PMC3126672},
	Number = {2},
	Pages = {Article 3},
	Title = {Targeted maximum likelihood based causal inference: Part {II}},
	Volume = {6},
	Year = {2010}}

@article{Sekhon08,
	Author = {J.S. Sekhon},
	Journal = {J Stat Softw},
	Title = {Multivariate and Propensity Score Matching Software with Automated Balance Optimization: the Matching package for {R}},
	Year = {2008}}

@article{Holland&Reitman77,
	Address = {New York},
	Author = {J.H. Holland and J.S. Reitman},
	Journal = {SIGART Bull},
	Pages = {49--49},
	Title = {Cognitive systems based on adaptive algorithms},
	Volume = {63},
	Year = {1977}}

@article{Koul&Susarla&vanRyzin81,
	Author = {H. Koul and V. Susarla and J. van Ryzin},
	Journal = {Ann Stat},
	Pages = {1276--88},
	Title = {Regression analysis with randomly right censored data},
	Volume = {9},
	Year = {1981}}

@article{Keiding&Hols&Green89,
	Author = {N. Keiding and C. Hols and A. Green},
	Journal = {Am J Epidemiol},
	Pages = {588--600},
	Title = {Retrospective estimation of diabetes incidence from information in a current prevalent population and historical mortality},
	Volume = {130},
	Year = {1989}}

@article{Robins&Rotnitzky&Zhao94,
	Author = {J.M. Robins and A. Rotnitzky and L.P. Zhao},
	Journal = {J Am Stat Assoc},
	Month = {September},
	Number = {427},
	Pages = {846--66},
	Title = {Estimation of regression coefficients when some regressors are not always observed},
	Volume = {89},
	Year = {1994}}

@article{Robins&Rotnitzky95,
	Author = {Robins, J.M. and A. Rotnitzky},
	Journal = {J Am Stat Assoc},
	Pages = {122--129},
	Title = {Semiparametric Efficiency in Multivariate Regression Models with Missing Data},
	Volume = {90},
	Year = {1995}}

@article{Kang&Schafer07,
	Author = {J. Kang and J.L. Schafer},
	Journal = {Stat Sci},
	Pages = {523--39},
	Title = {Demystifying Double Robustness: a Comparison of Alternative Strategies for Estimating a Population Mean from Incomplete Data (with discussion)},
	Volume = {22},
	Year = {2007}}

@article{Robins&Wang00,
	Author = {J.M. Robins and N. Wang},
	Journal = {Biometrika},
	Pages = {113--124},
	Title = {Inference for imputation estimators},
	Volume = {87},
	Year = {2000}}

@techreport{Bhattacharya&Vogt07,
	Author = {Bhattacharya, J. and Vogt, W.},
	Institution = {National Bureau of Economic Research},
	Number = {343},
	Title = {Do Instrumental Variables Belong in Propensity Scores?},
	Year = {2007}}

@techreport{Wooldridge09,
	Author = {Wooldridge, J.},
	Institution = {Michigan State University},
	Title = {Should Instrumental Variables be Used as Matching Variables?},
	Type = {Technical {R}eport},
	Year = {2009}}

@article{Pearl10,
	Author = {Pearl, J.},
	Journal = {Proceedings of Uncertainty in Artificial Intelligence},
	Title = {On a Class of Bias-Amplifying Variables that Endanger Effect Estimates},
	Year = {2010}}

@article{Holland86,
	Author = {Holland, P.W.},
	Journal = {J Am Stat Assoc},
	Number = {396},
	Pages = {945--960},
	Title = {Statistics and Causal Inference},
	Volume = {81},
	Year = {1986}}

@book{Rubin06,
	Address = {Cambridge, MA},
	Author = {Donald B. Rubin},
	Publisher = {Cambridge},
	Title = {Matched sampling for causal effects.},
	Year = {2006}}

@book{Rosenbaum02,
	Address = {Berlin Heidelberg New York},
	Author = {Rosenbaum, P.R.},
	Edition = {2nd},
	Publisher = {Springer},
	Title = {Observational studies},
	Year = {2002}}

@article{Rubin97,
	Author = {Rubin, Donald B.},
	Journal = {Ann of Intern Med},
	Number = {8S},
	Pages = {757--763},
	Title = {Estimating causal effects from large data sets using propensity scores},
	Volume = {127},
	Year = {1997}}

@article{Christakis&Iwashyna03,
	Author = {Christakis, N.A. and Iwashyna, T.I.},
	Journal = {Soc Sci Med},
	Number = {3},
	Pages = {465--475},
	Title = {The Health Impact of Health Care on Families: a matched cohort study of hospice use by decedents and mortality outcomes in surviving, widowed spouses},
	Volume = {57},
	Year = {2003}}

@article{Dehejia&Wahba02,
	Author = {R. Dehejia and S. Wahba},
	Journal = {Rev Econ Stat},
	Number = {1},
	Pages = {151--161},
	Title = {Propensity Score Matching Methods for Nonexperimental Causal Studies},
	Volume = {84},
	Year = {2002}}

@article{Galiani&Gertler&Schargrodsky05,
	Author = {Galiani, S. and P. Gertler and E. Schargrodsky},
	Journal = {J Polit Econ},
	Number = {1},
	Pages = {83--120},
	Title = {Water for Life: the Impact of the Privatization of Water Services on Child Mortality},
	Volume = {113},
	Year = {2005}}

@article{Abadie&Imbens06,
	Author = {Abadie, A. and G.W. Imbens},
	Journal = {Econometrica},
	Pages = {235--267},
	Title = {Large Sample Properties of Matching Estimators for Average Treatment Effects},
	Volume = {74},
	Year = {2006}}

@article{Herron&Wand07,
	Author = {Herron, M.C. and J. Wand},
	Journal = {Elect Stud},
	Number = {2},
	Pages = {247--261},
	Title = {Assessing Partisan Bias in Voting Technology: the Case of the 2004 {N}ew {H}ampshire Recount},
	Volume = {26},
	Year = {2007}}

@article{Imai05,
	Author = {K. Imai},
	Journal = {Am Polit Sci Rev},
	Number = {2},
	Pages = {283--300},
	Title = {Do Get-Out-The-Vote Calls Reduce Turnout? The Importance of Statistical Methods for Field Experiments},
	Volume = {99},
	Year = {2005}}

@incollection{Sekhon08b,
	Address = {New York},
	Author = {Sekhon, J.S.},
	Booktitle = {The Oxford handbook of political methodology},
	Editor = {J.M. Box-Steffensmeier and H.E. Brady and D. Collier},
	Publisher = {Oxford},
	Title = {The {N}eyman-{R}ubin Model of Causal Inference and Estimation via Matching Methods},
	Year = {2008}}

@article{Morgan&Harding06,
	Author = {Morgan, S.L. and D.J. Harding},
	Journal = {Sociol Meth Res},
	Number = {1},
	Pages = {3--60},
	Title = {Matching Estimators of Causal Effects: prospects and Pitfalls in Theory and Practice},
	Volume = {35},
	Year = {2006}}

@article{Diprete&Engelhardt04,
	Author = {Diprete, T.A. and H. Engelhardt},
	Journal = {Sociol Meth Res},
	Number = {4},
	Pages = {501--528},
	Title = {Estimating Causal Effects With Matching Methods in the Presence and Absence of Bias Cancellation},
	Volume = {32},
	Year = {2004}}

@article{Winship&Morgan99,
	Author = {Winship, C. and S.L. Morgan},
	Journal = {Annu Rev Sociol},
	Pages = {659--707},
	Title = {The estimation of causal effects from observational data},
	Volume = {25},
	Year = {1999}}

@article{Smith97,
	Author = {Smith, H.L.},
	Journal = {Sociol Meth},
	Pages = {305--353},
	Title = {Matching with Multiple Controls to Estimate Treatment Effects in Observational Studies},
	Volume = {27},
	Year = {1997}}

@article{Rubin02,
	Author = {Rubin, Donald B.},
	Journal = {Health Serv Outcome Res Meth},
	Number = {1},
	Pages = {169--188},
	Title = {Using Propensity Scores to Help Design Observational Studies: application to the Tobacco Litigation},
	Volume = {2},
	Year = {2002}}

@incollection{Brady08,
	Address = {New York},
	Author = {Brady, H.},
	Booktitle = {The Oxford handbook of political methodology},
	Editor = {J.M. Box-Steffensmeier and H.E. Brady and D. Collier},
	Publisher = {Oxford},
	Title = {Causation and explanation in social science},
	Year = {2008}}

@article{Freedman06,
	Author = {Freedman, D.A.},
	Journal = {Eval Rev},
	Pages = {691--713},
	Title = {Statistical Models for Causation: what Inferential leverage Do They Provide?},
	Volume = {30},
	Year = {2006}}

@article{Rubin90,
	Author = {Rubin, Donald B.},
	Journal = {Stat Sci},
	Number = {4},
	Pages = {472--480},
	Title = {Comment: {N}eyman (1923) and Causal Inference in Experiments and Observational Studies},
	Volume = {5},
	Year = {1990}}

@article{Speed90,
	Author = {T.P. Speed},
	Journal = {Stat Sci},
	Number = {4},
	Pages = {463--464},
	Title = {Introductory Remarks on {N}eyman (1923)},
	Volume = {5},
	Year = {1990}}

@book{Cox58,
	Address = {New York},
	Author = {Cox, D.R.},
	Publisher = {Wiley},
	Title = {Planning of experiments},
	Year = {1958}}

@article{Rubin78,
	Author = {Donald B. Rubin},
	Journal = {Ann Stat},
	Pages = {34--58},
	Title = {Bayesian Inference for causal effects: the role of randomization},
	Volume = {6},
	Year = {1978}}

@incollection{Rubin75,
	Address = {Alexandria},
	Author = {Rubin, Donald B.},
	Booktitle = {The proceedings of the Social Statistics Section of the American Statistical Association},
	Publisher = {American Statistical Association},
	Title = {Bayesian Inference for Causality: the Importance of Randomization},
	Year = {1975}}

@article{Rubin08,
	Author = {Rubin, Donald B.},
	Journal = {Ann of Appl Stat},
	Number = {3},
	Pages = {808--840},
	Title = {For Objective Causal Inference, Design Trumps Analysis},
	Volume = {2},
	Year = {2008}}

@article{Sekhon10,
	Author = {Sekhon, J.S.},
	Journal = {Annu Rev of Polit Sci},
	Pages = {487--508},
	Title = {Opiates for the Matches: matching Methods for Causal Inference},
	Volume = {12},
	Year = {2010}}

@article{Rubin76,
	Author = {Rubin, Donald B.},
	Journal = {Biometrics},
	Number = {1},
	Pages = {121--132},
	Title = {Multivariate Matching Methods That are Equal Percent Bias Reducing, {II}: maximums on Bias Reduction for Fixed Sample Sizes},
	Volume = {32},
	Year = {1976}}

@article{Cochran&Rubin73,
	Author = {Cochran, W.G. and Donald B. Rubin},
	Journal = {Sankhya Ser A},
	Pages = {417--446},
	Title = {Controlling Bias in Observational Studies: a Review},
	Volume = {35},
	Year = {1973}}

@book{Cochran83,
	Address = {New York},
	Author = {Cochran, W.G.},
	Note = {Edited posthumously by L.E. Moses and F. Mosteller},
	Publisher = {Wiley},
	Title = {Planning and analysis of observational studies},
	Year = {1983}}

@article{Robinsetal07,
	Author = {J.M. Robins and M. Sued and Q. Lei-Gomez and A. Rotnitzky},
	Journal = {Stat Sci},
	Pages = {544--559},
	Title = {Comment: {P}erformance of Double-Robust Estimators When ``Inverse Probability'' Weights Are Highly Variable},
	Volume = {22},
	Year = {2007}}

@article{Cortes&Vapnik95,
	Author = {C. Cortes and V. Vapnik},
	Journal = {Mach Learn},
	Month = {December},
	Pages = {273--297},
	Title = {Support-vector networks},
	Volume = {20},
	Year = {1995}}

@techreport{Friedman94,
	Author = {J.H. Friedman},
	Institution = {Department of Statistics, Stanford University},
	Title = {Flexible metric nearest neighbor classification},
	Type = {Technical {R}eport},
	Year = {1994}}

@techreport{FDA06,
	Author = {{Food and Drug Administration}},
	Institution = {U.S. Department of Health and Human Services, Food and Drug Administration},
	Title = {Critical Path Opportunities List},
	Type = {Technical {R}eport},
	Year = {2006}}

@article{Efronetal04,
	Author = {B. Efron and T. Hastie and I. Johnstone and R. Tibshirani},
	Journal = {Ann Stat (with discussion)},
	Number = {2},
	Pages = {407--499},
	Title = {Least Angle Regression},
	Volume = {32},
	Year = {2004}}

@techreport{Breiman99,
	Author = {L. Breiman},
	Institution = {Department of Statistics, University of California, Berkeley},
	Number = {567},
	Title = {Random forests - random features},
	Year = {1999}}

@manual{Breiman01b,
	Author = {L. Breiman},
	Title = {Notes on setting up, using, and understanding random forests V3.0},
	Year = {2001}}

@article{Golubetal99,
	Author = {T.R. Golub and D.K. Slonim and P. Tamayo and C. Huard and M. Gaasenbeek and J.P. Mesirov and H. Coller and M.L. Loh and J.R. Downing and M.A. Caligiuri and C.D. Bloomfield and E.S. Lander},
	Journal = {Science},
	Pages = {531--537},
	Title = {Molecular classification of cancer: class discovery and class prediction by gene expression monitoring},
	Volume = {286},
	Year = {1999}}

@article{vanderLaan06a,
	Author = {M.J. van der Laan},
	Journal = {Int J Biostat},
	Number = {1},
	Pages = {Article 2},
	Title = {Statistical Inference for Variable Importance},
	Volume = {2},
	Year = {2006}}

@article{Robins&Mark&Newey92,
	Author = {J.M. Robins and S.D. Mark and W.K. Newey},
	Journal = {Biometrics},
	Number = {479--495},
	Title = {Estimating exposure effects by modelling the expectation of exposure conditional on confounders},
	Volume = {48},
	Year = {1992}}

@techreport{Yu&VanderLaan03,
	Author = {Z. Yu and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {136},
	Title = {Measuring treatment effects using semiparametric models},
	Year = {2003}}

@techreport{Tuglus&vanderLaan08,
	Author = {C. Tuglus and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {233},
	Title = {Targeted Methods for Biomarker Discovery, the Search for a Standard},
	Year = {2008}}

@book{Hastie&Tibshirani90,
	Address = {London},
	Author = {T.J. Hastie and R.J. Tibshirani},
	Publisher = {Chapman \& Hall},
	Title = {Generalized additive models},
	Year = {1990}}

@misc{Efron&Hastie07,
	Author = {B. Efron and T. Hastie},
	Howpublished = {R package},
	Title = {lars},
	Year = {2007}}

@article{Benjamini&Hochberg95,
	Author = {Y. Benjamini and Y. Hochberg},
	Journal = {J R Stat Soc Ser B},
	Pages = {289--300},
	Title = {Controlling the false discovery rate: a practical and powerful approach to multiple testing},
	Volume = {57},
	Year = {1995}}

@misc{Ge&Dudoit02,
	Author = {Y. Ge and S. Dudoit},
	Howpublished = {R package},
	Title = {Multiple Testing Procedures, multtest},
	Url = {www.bioconductor.org},
	Year = {2002},
	Bdsk-Url-1 = {www.bioconductor.org}}

@article{Tibshirani96,
	Author = {R. Tibshirani},
	Journal = {J R Stat Soc Ser B},
	Number = {1},
	Pages = {267--288},
	Title = {Regression shrinkage and selection via the lasso.},
	Volume = {58},
	Year = {1996}}

@article{Tuglus&vanderLaan09,
	Author = {C. Tuglus and M.J. van der Laan},
	Journal = {Stat Appl Genet Mol},
	Number = {1},
	Pages = {Article 12},
	Title = {Modified {FDR} Controlling Procedure for Multi-Stage Analyses},
	Volume = {8},
	Year = {2009}}

@article{Dudoit&Fridlyand&Speed02,
	Author = {S. Dudoit and J. Fridlyand and T. P. Speed},
	Journal = {J Am Stat Assoc},
	Number = {457},
	Pages = {77--87},
	Title = {Comparison of Discrimination Methods for the Classification of Tumors Using Gene Expression Data},
	Volume = {97},
	Year = {2002}}

@article{Kos&Lah98,
	Author = {J. Kos and T.T. Lah},
	Journal = {Oncol Rep},
	Number = {6},
	Pages = {1349--61},
	Title = {Cysteine proteinases and their endogenous inhibitors: target proteins for prognosis, diagnosis and therapy in cancer (review)},
	Volume = {5},
	Year = {1998}}

@article{Vitaleetal01,
	Author = {C. Vitale and C. Romagnani and A. Puccetti and D. Olive and R. Costello and L. Chiossone and A. Pitto and A. Bacigalupo and L. Moretta and M.C. Mingari},
	Journal = {Proc Natl Acad Sci},
	Pages = {5764--5769},
	Title = {Surface expression and function of p75/{AIRM}-1 or {CD}33 in acute myeloid leukemias: engagement of {CD}33 induces apoptosis of leukemic cells},
	Volume = {98},
	Year = {2001}}

@article{Clappieretal07,
	Author = {E. Clappier and W. Cuccuini and A. Kalota and A. Crinquette and J.M. Cayuela and W.A. Dik and A.W. Langerak and B. Montpellier and B. Nadel and P. Walrafen and O. Delattre and A. Aurias and T. Leblanc and H. Dombret and A.M. Gewirtz and A. Baruchel and F. Sigaux and J. Soulier},
	Journal = {Blood},
	Number = {4},
	Pages = {1251--61},
	Title = {The {C-MYB} locus is involved in chromosomal translocation and genomic duplications in human T-cell acute leukemia ({T-ALL}), the translocation defining a new {T-ALL} subtype in very young children},
	Volume = {110},
	Year = {2007}}

@article{Lane&Ley03,
	Author = {A.A. Lane and T.J. Ley},
	Journal = {Cell},
	Number = {305-318},
	Title = {Neutrophil elastase cleaves {PML-RAR}-alpha and is important for the development of acute promyelocytic leukemia in mice},
	Volume = {115},
	Year = {2003}}

@article{Hunger96,
	Author = {S.P. Hunger},
	Journal = {Blood},
	Pages = {1211--1224},
	Title = {Chromosomal translocations involving the {E2A} gene in acute lymphoblastic leukemia: clinical features and molecular pathogenesis.},
	Volume = {87},
	Year = {1996}}

@article{Nebraletal05,
	Author = {K. Nebral and H.H. Schmidt and O.A. Haas and S. Strehl},
	Journal = {Clin Cancer Res},
	Number = {18},
	Pages = {6489--6494},
	Title = {{NUP}98 Is Fused to Topoisomerase {(DNA)} {II}{beta} 180 {kDa} {(TOP2B)} in a Patient with Acute Myeloid Leukemia with a New {t(3;11)(p24;p15)}},
	Volume = {11},
	Year = {2005}}

@article{Kaufmannetal98b,
	Author = {S.H. Kaufmann and S.D. Gore and C.B. Miller and R.J. Jones and L.A. Zwelling and E. Schneider and P.J. Burke and J.E. Karp},
	Journal = {Leukemia Lymphoma},
	Month = {Apr},
	Number = {3-4},
	Pages = {217--237},
	Title = {Topoisomerase {II} and the response to antileukemic therapy},
	Volume = {29},
	Year = {1998}}

@article{Kozaretal04,
	Author = {K. Kozar and M.A. Ciemerych and V.I. Rebel and H. Shigematsu and A. Zagozdzon and E. Sicinska and Y. Geng and Q. Yu and S. Bhattacharya and R.T. Bronson and K. Akashi and P. Sicinski},
	Journal = {Cell},
	Pages = {477--491},
	Title = {Mouse development and cell proliferation in the absence of {D}-cyclins},
	Volume = {118},
	Year = {2004}}

@article{MartinSuberoetal07,
	Author = {J.I. Martin-Subero and R. Ibbotson and W. Klapper and L. Michaux and E. Callet-Bauchu and F. Berger and M.J. Calasanz and C. De Wolf-Peeters and M.J. Dyer and P. Felman and A. Gardiner and R.D. Gascoyne and S. Gesk and L. Harder and D.E. Horsman and M. Kneba and R. Kuppers and A. Majid and N. Parry-Jones and M. Ritgen and M. Salido and F. Sole and G. Thiel and H.H. Wacker and D. Oscier and I. Wlodarska and R. Siebert},
	Journal = {Leukemia},
	Number = {7},
	Pages = {1532--1544},
	Title = {A comprehensive genetic and histopathologic analysis identifies two subgroups of {B}-cell malignancies carrying a t(14;19)(q32;q13) or variant {BCL3}-translocation},
	Volume = {21},
	Year = {2007}}

@article{Palomeroetal06,
	Author = {T. Palomero and D.T. Odom and J. O'Neil and A.A. Ferrando and A. Margolin and D.S. Neuberg and S.S. Winter and R.S. Larson and W. Li and X.S. Liu and R.A. Young and A.T. Look},
	Journal = {Blood},
	Number = {3},
	Pages = {986--992},
	Title = {Transcriptional regulatory networks downstream of {TAL1/SCL} in {T}-cell acute lymphoblastic leukemia},
	Volume = {108},
	Year = {2006}}

@article{Wongetal07,
	Author = {H.P. Wong and L. Yu and E.K. Lam and E.K. Tai and W.K. Wu and C.H. Cho},
	Journal = {Toxicol Appl Pharm},
	Number = {3},
	Pages = {261--267},
	Title = {Nicotine promotes cell proliferation via alpha7-nicotinic acetylcholine receptor and catecholamine-synthesizing enzymes-mediated pathway in human colon adenocarcinoma {HT}-29 cells.},
	Volume = {221},
	Year = {2007}}

@article{Ramaswamyetal03,
	Author = {S. Ramaswamy and K.N. Ross and E.S. Lander and T.R. Golub},
	Journal = {Nat Genet},
	Pages = {49--54},
	Title = {A molecular signature of metastasis in primary solid tumors},
	Volume = {33},
	Year = {2003}}

@article{Purietal01,
	Author = {R. Puri and A. Tousson and L. Chen and S.S. Kakar},
	Journal = {Cancer Lett},
	Pages = {131--139},
	Title = {Molecular cloning of pituitary tumor transforming gene 1 from ovarian tumors and its expression in tumors},
	Volume = {163},
	Year = {2001}}

@article{Fujiietal06,
	Author = {T. Fujii and S. Nomoto and K. Koshikawa and Y.Yatabe and O. Teshigawara and T. Mori and S. Inoue and S. Takeda and A. Nakao},
	Journal = {Hepatology},
	Pages = {1267--1275},
	Title = {Overexpression of pituitary tumor transforming gene 1 in {HCC} is associated with angiogenesis and poor prognosis},
	Volume = {43},
	Year = {2006}}

@article{Zhuetal06,
	Author = {X. Zhu and Z. Mao and Y. Na and Y. Guo and X. Wang and D. Xin},
	Journal = {Anticancer Res},
	Pages = {1253--1259},
	Title = {Significance of pituitary tumor transforming gene 1 ({PTTG1}) in prostate cancer},
	Volume = {26},
	Year = {2006}}

@article{Kaufmannetal98a,
	Author = {S.H. Kaufmann and J.E. Karp and P.A. Svingen and S. Krajewski and P.J. Burke and S.D. Gore and J.C. Reed},
	Journal = {Blood},
	Number = {3},
	Pages = {991--1000},
	Title = {Elevated expression of the apoptotic regulator {Mcl}-1 at the time of leukemic relapse},
	Volume = {91},
	Year = {1998}}

@article{Frumanetal99,
	Author = {D.A. Fruman and S.B. Snapper and C.M. Yballe and L. Davidson and J.Y. Yu and F.W. Alt and L.C. Cantley},
	Journal = {Science},
	Pages = {393--397},
	Title = {Impaired {B} cell development and proliferation in absence of phosphoinositide 3-kinase p85-alpha},
	Volume = {283},
	Year = {1999}}

@article{Tombes&Krystal97,
	Author = {R.M. Tombes and G.W. Krystal},
	Journal = {Biochim Biophys Acta},
	Pages = {281--292},
	Title = {Identification of novel human tumor cell-specific {CaMK-II} variants},
	Volume = {1355},
	Year = {1997}}

@article{Senturkeretal97,
	Author = {S. Senturker and B. Karahalil and M. Inal and H. Yilmaz and H. Muslumanoglu and G. Gedikoglu and M. Dizdaroglu},
	Journal = {FEBS Letters},
	Number = {3},
	Pages = {286--290},
	Title = {Oxidative {DNA} base damage and antioxidant enzyme levels in childhood acute lymphoblastic leukemia},
	Volume = {416},
	Year = {1997}}

@article{Komuroetal05,
	Author = {I. Komuro and T. Yasuda and A. Iwamoto and K.S. Akagawa},
	Journal = {J Biol Chem},
	Number = {50},
	Pages = {41137--45},
	Title = {Catalase plays a critical role in the {CSF}-independent survival of human macrophages via regulation of the expression of {BCL}-2 family},
	Volume = {280},
	Year = {2005}}

@article{Balciunaiteetal05,
	Author = {E. Balciunaite and A. Spektor and N.H. Lents and H. Cam and H. Te Riele and A. Scime and M.A. Rudnicki and R. Young and B.D. Dynlacht},
	Journal = {Mol Cell Biol},
	Number = {18},
	Pages = {8166--78},
	Title = {Pocket protein complexes are recruited to distinct targets in quiescent and proliferating cells},
	Volume = {25},
	Year = {2005}}

@article{Leoneetal01,
	Author = {G. Leone and R. Sears and E. Huang and R. Rempel and F. Nuckolls and C.H. Park and P. Giangrande and L. Wu and H.I. Saavedra and S.J. Field and M.A. Thompson and H. Yang and Y. Fujiwara and M.E. Greenberg and S. Orkin and C. Smith and J.R. Nevins},
	Journal = {Mol Cell},
	Pages = {105--113},
	Title = {Myc requires distinct {E2F} activities to induce {S} phase and apoptosis},
	Volume = {8},
	Year = {2001}}

@article{Sax23,
	Author = {Sax, K.},
	Journal = {Genetics},
	Title = {The association of size difference with seed-coat pattern and pigmentation in \textit{Phaseolus vulgaris}},
	Year = {1923}}

@article{Thoday60,
	Author = {Thoday, J.M.},
	Journal = {Nature},
	Title = {Location of polygenes},
	Year = {1960}}

@article{Lander&Botstein89,
	Author = {Lander, E.S. and Botstein, D.},
	Journal = {Genetics},
	Title = {Mapping {M}endelian factors underlying quantitative traits using {RFLP} linkage maps},
	Year = {1989}}

@article{Haley&Knott92,
	Author = {Haley, C.S. and Knott, S.A.},
	Journal = {Heredity},
	Title = {A simple regression method for mapping quantitative trait loci in line crosses using flanking markers},
	Year = {1992}}

@article{Jansen93,
	Author = {Jansen, R.C.},
	Journal = {Genetics},
	Title = {Interval mapping of multiple quantitative trait loci},
	Year = {1993}}

@article{Zeng94,
	Author = {Zeng, Z.B.},
	Journal = {Genetics},
	Title = {Precision mapping of quantitative trait loci},
	Year = {1994}}

@article{Kao&Zeng&Teasdale99,
	Author = {Kao, C.H. and Zeng, Z.B. and Teasdale, R.D.},
	Journal = {Genetics},
	Title = {Multiple interval mapping for quantitative trait loci},
	Year = {1999}}

@article{Satagopanetal96,
	Author = {Satagopan, J.M. and B.S. Yandell and M.A. Newton and T.C. Osborn},
	Journal = {Genetics},
	Title = {A {B}ayesian approach to detect quantitative trait loci using {M}arkov chain {M}onte {C}arlo},
	Year = {1996}}

@article{Heath97,
	Author = {Heath, S.C.},
	Journal = {Am J Hum Genet},
	Title = {Markov chain {M}onte {C}arlo segregation and linkage analysis of oligogenic models},
	Year = {1997}}

@article{Sillanpaa&Arjas98,
	Author = {Sillanpaa, M.J. and Arjas, E.},
	Journal = {Genetics},
	Title = {Bayesian mapping of multiple quantitative trait loci from incomplete inbred line cross data},
	Year = {1998}}

@article{Leeetal08,
	Author = {Lee, S.S.F. and L. Sun and R. Kustra and S.B. Bull},
	Journal = {Bioinformatics},
	Title = {{EM}-random forest and new measures of variable importance for multi-locus quantitative trait linkage analysis},
	Year = {2008}}

@article{Wang2011ctmle,
	Author = {H. Wang and S. Rose and M.J. van der Laan},
	Date-Modified = {2012-08-26 00:45:19 -0700},
	Journal = {Stat Prob Lett},
	Keywords = {App},
	Note = {PMCID: PMC3090625},
	Number = {7},
	Pages = {792--796},
	Title = {{F}inding {Q}uantitative {T}rait {L}oci {G}enes with {C}ollaborative {T}argeted {M}aximum {L}ikelihood {L}earning},
	Volume = {81},
	Year = {2011}}

@techreport{Wang&Rose&vanderLaan11,
	Author = {H. Wang and S. Rose and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Title = {Targeted Methods for Finding Quantitative Trait Loci},
	Type = {Technical {R}eport},
	Year = {2011}}

@manual{Basten&Weir&Zeng01,
	Author = {C.J. Basten and B.S. Weir and Z.B. Zeng},
	Title = {QTL Cartographer},
	Url = {http://statgen.ncsu.edu/qtlcart/},
	Year = {2001},
	Bdsk-Url-1 = {http://statgen.ncsu.edu/qtlcart/}}

@article{Masindeetal01,
	Author = {Masinde, G.L. and X. Li and W. Gu and H. Davidson and S. Mohan and D.J. Baylink},
	Journal = {Genome Res},
	Title = {Identification of wound healing/regeneration quantitative trait loci ({QTL}) at multiple time points that explain seventy percent of variance in ({MRL/MpJ and SJL/J}) mice {F2} population},
	Year = {2001}}

@article{Boyartchuk01,
	Author = {Boyartchuk, V.L. and K.W. Broman and R.E. Mosher and S.E.F. D'Orazio and M.N. Starnbach and W.F. Dietrich},
	Journal = {Nat Genet},
	Title = {Multigenic control of Listeria monocytogenes susceptibility in mice},
	Year = {2001}}

@article{Broman03,
	Author = {Broman, K.W.},
	Journal = {Genetics},
	Title = {Mapping quantitative trait loci in the case of a spike in the phenotype distribution},
	Year = {2003}}

@article{Jin&Fine&Yandell07,
	Author = {Jin, C. and J.P. Fine and B.S. Yandell},
	Journal = {J Am Stat Assoc},
	Title = {A unified semiparametric framework for quantitative trait loci analysis, with application to spike phenotypes},
	Year = {2007}}

@article{Petersenetal08,
	Author = {M.L. Petersen and M.J. van der Laan and S. Napravnik and J.J. Eron and R.D. Moore and S.G. Deeks},
	Journal = {AIDS},
	Number = {16},
	Pages = {2097--106},
	Title = {Long-term consequences of the delay between virologic failure of highly active antiretroviral therapy and regimen modification},
	Volume = {22},
	Year = {2008}}

@article{Rodgeretal09,
	Author = {A.J. Rodger and Z. Fox and J.D. Lundgren and J.L. Kuller and C. Boesecke and D. Gey and A. Skoutelis and M.B. Goetz and A.N. Phillips and {INSIGHT Strategies for Management of Antiretroviral Therapy (SMART) Study Group}},
	Journal = {J Infect Dis},
	Number = {6},
	Pages = {973--83},
	Title = {Activation and coagulation biomarkers are independent predictors of the development of opportunistic disease in patients with {HIV} infection.},
	Volume = {200},
	Year = {2009}}

@article{Hammeretal08,
	Author = {S.M. Hammer and J.J. Eron and P. Reiss and R.T. Schooley and M.A. Thompson and S. Walmsley and P. Cahn and M.A. Fischl and J.M. Gatell and M.S. Hirsch and D.M. Jacobsen and J.S.G. Montaner and D.D. Richman and P.G. Yeni and P.A. Volberding},
	Journal = {J Am Med Asoc},
	Number = {5},
	Pages = {555--70},
	Title = {Antiretroviral treatment of adult {HIV} infection: 2008 recommendations of the {I}nternational {AIDS} {S}ociety-{USA} panel},
	Volume = {300},
	Year = {2008}}

@article{Stringeretal06,
	Author = {J.S. Stringer and I. Zulu and J. Levy and E.M. Stringer and A. Mwango and B.H. Chi and V. Mtonga and S. Reid and R.A. Cantrell and M. Bulterys and M.S. Saag and R.G. Marlink and A. Mwinga and T.V. Ellerbrock and M. Sinkala},
	Journal = {J Am Med Asoc},
	Number = {7},
	Pages = {782--93},
	Title = {Rapid scale-up of antiretroviral therapy at primary care sites in {Z}ambia: feasibility and early outcomes},
	Volume = {296},
	Year = {2006}}

@misc{WHO06,
	Author = {{{W}orld {H}ealth {O}rganization}},
	Title = {Antiretroviral therapy for {HIV} infection in adults and adoloescents: recommendations for a public health approach},
	Year = {2006}}

@article{Reynoldsetal09,
	Author = {S.J. Reynolds and G. Nakigozi and K. Newell and A. Ndyanabo and R. Galiwongo and I. Boaz and T.C. Quinn and R. Gray and M. Wawer and D. Serwadda},
	Journal = {{AIDS}},
	Number = {6},
	Pages = {697--700},
	Title = {Failure of immunologic criteria to appropriately identify antiretroviral treatment failure in {U}ganda},
	Volume = {23},
	Year = {2009}}

@article{Petersen2007,
	Author = {M.L Petersen and S.G. Deeks and J.N. Martin and M.J. van der Laan},
	Date-Modified = {2012-08-25 23:33:55 -0700},
	Journal = {Am J Epidemiol},
	Keywords = {Aim1},
	Note = {PMCID: PMC2561999},
	Number = {9},
	Pages = {985--993},
	Title = {History-adjusted Marginal Structural Models for Estimating Time-varying Effect Modification},
	Volume = {166},
	Year = {2007}}

@article{Robins&Hernan&Rotnitzky07,
	Author = {J.M. Robins and M.A. Hernan and A. Rotnitzky},
	Journal = {Am J Epidemiol},
	Number = {9},
	Pages = {994--1002},
	Title = {Effect Modification by Time-varying Covariates},
	Volume = {166},
	Year = {2007}}

@article{vanderLaan&Petersen&Joffe07,
	Author = {M.J. van der Laan and M.L. Petersen and M.M. Joffe},
	Journal = {Am J Epidemiol},
	Number = {9},
	Pages = {1003--1004},
	Title = {Response to Invited Commentary: {P}etersen et. al. Respond to ``{E}ffect Modification by Time-varying Covariates''},
	Volume = {166},
	Year = {2007}}

@article{vanderLaan&Petersen07b,
	Author = {M.J. van der Laan and M.L. Petersen},
	Journal = {Int J Biostat},
	Number = {1},
	Pages = {Article 6},
	Title = {Statistical Learning of Origin-Specific Statically Optimal Individualized Treatment Rules.},
	Volume = {3},
	Year = {2007}}

@article{Petersen&Deeks&vanderLaan07,
	Author = {M.L. Petersen and S.G. Deeks and M.J. van der Laan},
	Date-Modified = {2012-08-20 22:22:11 -0700},
	Journal = {Stat Med},
	Note = {PubMed Central PMCID: PMC2442037},
	Number = {25},
	Pages = {4578--601},
	Title = {{Individualized treatment rules: Generating candidate clinical trials}},
	Volume = {26},
	Year = {2007}}

@article{vanderLaan2005,
	Author = {M.J. van der Laan and M.L. Petersen and M.M. Joffe},
	Date-Modified = {2012-08-24 09:41:11 -0700},
	Journal = {Int J Biostat},
	Keywords = {Aim1},
	Number = {1},
	Pages = {10--20},
	Title = {{History-Adjusted Marginal Structural Models and Statically-Optimal Dynamic Treatment Regimens}},
	Volume = {1},
	Year = {2005}}

@article{Hernan2006,
	Author = {M.A. Hern\'{a}n and E. Lanoy and D. Costagliola and J.M. Robins},
	Date-Modified = {2012-08-23 18:01:19 -0700},
	Journal = {Basic Clin Pharmacol Toxicol},
	Keywords = {Aim1},
	Note = {PMID: 16611197},
	Number = {3},
	Pages = {237--242},
	Title = {Comparison of dynamic treatment regimes via inverse probability weighting},
	Volume = {98},
	Year = {2006}}

@techreport{vanderLaan08b,
	Author = {M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {232},
	Title = {The construction and analysis of adaptive group sequential designs},
	Year = {2008}}

@article{Boivinetal07,
	Author = {Boivin, J. and Bunting, L. and Collins, J.A. and Nygren, K.G.},
	Journal = {Hum Reproduct},
	Pages = {1506--1512},
	Title = {International estimates of infertility prevalence and treatment-seeking: potential need and demand for infertility medical care},
	Volume = {22},
	Year = {2007}}

@article{Adamsonetal06,
	Author = {Adamson, G.D. and de {M}ouzon, J. and Lancaster, P. and Nygren, K.-G. and Sullivan, E. and Zegers-Hochschild, F.},
	Journal = {Fertil Steril},
	Pages = {1586--1622},
	Title = {World collaborative report on in vitro fertilization, 2000},
	Volume = {85},
	Year = {2006}}

@article{Soullieretal08,
	Author = {Soullier, N. and Bouyer, J. and Pouly J-L. and Guibert, J. and de la {R}ochebrochard},
	Journal = {Hum Reproduct},
	Pages = {187--192},
	Title = {Estimating the success of an in vitro fertilization programme using multiple imputation},
	Volume = {23},
	Year = {2008}}

@article{delaRochebrochardetal08,
	Author = {de la {R}ochebrochard, E. and Soullier, N. and Peikrishvili, R. and Guibert, J. and Bouyer, J.},
	Journal = {Int J Gynecol Obstet},
	Pages = {74--75},
	Title = {High in vitro fertilization discontinuation rate in {F}rance},
	Volume = {103},
	Year = {2008}}

@article{delaRochebrochardetal09,
	Author = {de la {R}ochebrochard, E. and Quelen, C. and Peikrishvili, R. and Guibert, J. and Bouyer, J.},
	Journal = {Fertil Steril},
	Pages = {149--156},
	Title = {Long-term outcome of parenthood project during in vitro fertilization and after discontinuation of unscuccessful in vitro fertilization},
	Volume = {92},
	Year = {2009}}

@book{Schafer97,
	Address = {London},
	Author = {Schafer, J.L.},
	Publisher = {Chapman \& Hall},
	Title = {Analysis of incomplete multivariate data},
	Year = {1997}}

@book{Little&Rubin02,
	Address = {Hoboken},
	Author = {Little, R.J.A. and Rubin, Donald B.},
	Edition = {2nd},
	Publisher = {Wiley},
	Title = {Statistical analysis with missing data},
	Year = {2002}}

@techreport{Yu&vanderLaan02,
	Author = {Z. Yu and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {122},
	Title = {Construction of counterfactuals and the G-computation formula},
	Year = {2002}}

@article{Gill&Robins01,
	Author = {Gill, R.D. and Robins, J.M.},
	Journal = {Ann Stat},
	Number = {6},
	Pages = {1785--1811},
	Title = {Causal inference in complex longitudinal studies: continuous case},
	Volume = {29},
	Year = {2001}}

@techreport{DHHS04,
	Author = {{Department of Health and Human Services}},
	Institution = {Panel on Clinical Practices for Treatment of {HIV} Infection},
	Title = {Guidelines for the use of antiretroviral agents in {HIV}-1 infected adults and adolescents},
	Type = {Technical {R}eport},
	Year = {2004}}

@article{CDC92,
	Author = {{Centers for Disease Control and Prevention}},
	Journal = {Morbid Mortal W Rep},
	Pages = {1--19},
	Title = {{1993 revised classification system for {HIV} infection and expanded surveillance case definition for AIDS among adolescents and adults}},
	Volume = {41},
	Year = {1992}}

@incollection{Selbyetal05,
	Author = {J.V. Selby and D.H. Smith and E.S. Johnson and M.A. Raebel and G.D. Friedman and B.H. McFarland},
	Booktitle = {Pharmacoepidemiology},
	Editor = {B.L. Strom},
	Publisher = {Wiley},
	Title = {Kaiser {P}ermanente Medical Care Program},
	Year = {2005}}

@techreport{Neugebauer&Silverberg&vanderLaan10,
	Author = {R. Neugebauer and M.J. Silverberg and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Title = {Observational Study and Individualized Antiretroviral Therapy Initiation Rules for Reducing Cancer Incidence in {HIV}-Infected Patients},
	Type = {272},
	Year = {2010}}

@techreport{Stitelman2011,
	Author = {O.M. Stitelman and V. De Gruttola and M.J. van der Laan},
	Date-Modified = {2012-08-26 20:56:50 -0700},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Keywords = {tmle},
	Note = {Available at \url{http://www.bepress.com/ucbbiostat/paper281}; To appear in Int J. Biostat},
	Number = {281},
	Title = {A General Implementation of TMLE for Longitudinal Data Applied to Causal Inference in Survival Analysis},
	Year = {2011}}

@techreport{Stitelman2011a,
	Author = {O.M. Stitelman and M.J. van der Laan},
	Date-Modified = {2012-08-24 11:37:04 -0700},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Title = {Targeted Maximum Likelihood Estimation of Time-To-Event Parameters With Time-Dependent Covariates},
	Type = {Technical {R}eport},
	Year = {2011}}

@article{Thalletal07,
	Author = {P.F. Thall and C. Logothetis and L.C. Pagliaro and S. Wen and M.A. Brown and D. Williams and R.E. Millikan},
	Journal = {J Natl Cancer Inst},
	Pages = {1613--22},
	Title = {Adaptive Therapy for Androgen-Independent Prostate Cancer: a randomized Selection Trial of Four Regimens},
	Volume = {99},
	Year = {2007}}

@article{Bembom&vanderLaan07a,
	Author = {O. Bembom and M.J. van der Laan},
	Journal = {J Natl Cancer Inst},
	Pages = {1577--1582},
	Title = {Comment: Statistical Methods for analyzing sequentially randomized trials},
	Volume = {99(21)},
	Year = {2007}}

@techreport{Zheng&vanderLaan10,
	Author = {W. Zheng and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {273},
	Title = {Asymptotic Theory for Cross-validated Targeted Maximum Likelihood Estimation},
	Year = {2010}}

@techreport{Zheng&vanderLaan11,
	Author = {W. Zheng and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {288},
	Title = {Targeted Maximum Likelihood Estimation of Natural Direct Effect},
	Year = {2011}}

@book{Robert07,
	Address = {Berlin Heidelberg New York},
	Author = {Robert, P.C.},
	Publisher = {Springer},
	Title = {{T}he {B}ayesian choice: from decision-thoeretic foundations to computational implementation},
	Year = {2007}}

@book{Lindley80,
	Address = {Cambridge, MA},
	Author = {Lindley, D.V.},
	Publisher = {Cambridge},
	Title = {{I}ntroduction to probability and statistics from a {B}ayesian point of view, {P}art 2},
	Year = {1980}}

@article{Golub06,
	Author = {Golub, H.L.},
	Journal = {Stat Med},
	Pages = {3231--3235},
	Title = {The need for more efficient trial designs},
	Volume = {25},
	Year = {2006}}

@article{Emerson06,
	Author = {Emerson, S.S.},
	Journal = {Stat Med},
	Pages = {3270--3296},
	Title = {Issues in the use of adaptive clinical trial designs},
	Volume = {25},
	Year = {2006}}

@book{Hu&Rosenberger06,
	Address = {New York},
	Author = {F. Hu and W.F. Rosenberger},
	Publisher = {Wiley},
	Title = {The theory of response adaptive randomization in clinical trials},
	Year = {2006}}

@book{Jennison&Turnbull00,
	Address = {Boca Raton},
	Author = {Jennison, C. and Turnbull, B.W.},
	Publisher = {Chapman \& Hall},
	Title = {Group sequential methods with applications to clinical trials},
	Year = {2000}}

@article{Rosenberger96,
	Author = {W.F. Rosenberger},
	Journal = {Stat Sci},
	Pages = {137--149},
	Title = {New directions in adaptive designs},
	Volume = {11},
	Year = {1996}}

@techreport{Chambaz10,
	Author = {Chambaz, A. and van der Laan, M.J.},
	Date-Modified = {2012-08-26 20:55:57 -0700},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Keywords = {App},
	Note = {Available at \url{http://biostats.bepress.com/ucbbiostat/paper258/}},
	Number = {258},
	Title = {Targeting the optimal design in randomized clinical trials with binary outcomes and no covariate},
	Year = {2010}}

@article{Rosenberger&Vidyashankar&Agarwal01,
	Author = {Rosenberger, W.F. and Vidyashankar, A.N. and Agarwal, D.K.},
	Journal = {J Biopharm Stat},
	Number = {227--236},
	Title = {Covariate-adjusted response-adaptive designs for binary response},
	Volume = {11},
	Year = {2001}}

@article{Bandyopadhyay&Biswas01,
	Author = {Bandyopadhyay, U. and Biswas, A.},
	Journal = {Biometrika},
	Number = {2},
	Pages = {409--419},
	Title = {Adaptive designs for normal responses with prognostic factors},
	Volume = {88},
	Year = {2001}}

@article{Atkinson&Biswas05,
	Author = {Atkinson, A.C. and Biswas, A.},
	Journal = {Stat Med},
	Number = {16},
	Pages = {2477--2492},
	Title = {Adaptive biased-coin designs for skewing the allocation proportion in clinical trials with normal responses},
	Volume = {24},
	Year = {2005}}

@article{Zhangetal07,
	Author = {Zhang, L.-X. and Hu, F.-F. and Cheung, S.H. and Chan, W.S.},
	Journal = {Ann Stat},
	Number = {3},
	Pages = {1166--1182},
	Title = {Asymptotic properties of covariate-adjusted response-adaptive designs},
	Volume = {35},
	Year = {2007}}

@article{Zhang&Hu09,
	Author = {Zhang, L.-X. and Hu, F.-F.},
	Journal = {Appl Math J Chinese Univ Ser B},
	Number = {1},
	Pages = {1--13},
	Title = {A new family of covariate-adjusted response adaptive designs and their properties},
	Volume = {24},
	Year = {2009}}

@article{Shao&Yu&Zhong10,
	Author = {Shao, J. and Yu, X. and Bob Zhong, B.},
	Journal = {Biometrika},
	Title = {A theory for testing hypotheses under covariate-adaptive randomization},
	Year = {2010}}

@article{Gill89,
	Author = {Gill, R.D.},
	Journal = {Scand J Stat},
	Title = {Non- and semiparametric maximum likelihood estimators and the Von Mises method (Part 1)},
	Year = {1989}}

@article{Tan08,
	Author = {Z. Tan},
	Journal = {Int J Biostat},
	Number = {1},
	Pages = {Article 10},
	Title = {Comment: {I}mproved Local Efficiency and Double Robustness},
	Volume = {4},
	Year = {2008}}

@techreport{tmlePackageb,
	Author = {S. Gruber and M.J. van der Laan},
	Date-Modified = {2012-08-26 21:19:43 -0700},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Keywords = {tmle},
	Note = {Available at \url{http://biostats.bepress.com/ucbbiostat/paper275/}},
	Number = {275},
	Title = {{tmle}: an {R} Package for Targeted Maximum Likelihood Estimation},
	Year = {2011}}

@proceedings{DBLP:conf/colt/2003,
	Address = {Berlin Heidelberg New York},
	Booktitle = {COLT},
	Editor = {B. Sch{\"o}lkopf and M.K. Warmuth},
	Publisher = {Springer},
	Series = {Lecture Notes in Computer Science},
	Title = {Computational Learning Theory and Kernel Machines, 16th Annual Conference on Computational Learning Theory and 7th Kernel Workshop, COLT/Kernel 2003, Washington, DC, USA, August 24-27, 2003, Proceedings},
	Volume = {2777},
	Year = {2003}}

@proceedings{DBLP:conf/nips/2005,
	Booktitle = {NIPS},
	Title = {Advances in Neural Information Processing Systems 18 [Neural Information Processing Systems, NIPS 2005, December 5-8, 2005, Vancouver, British Columbia, Canada]},
	Year = {2005}}

@proceedings{DBLP:conf/colt/2006,
	Address = {Berlin Heidelberg New York},
	Booktitle = {COLT},
	Editor = {G. Lugosi and H.-U. Simon},
	Publisher = {Springer},
	Series = {Lecture Notes in Computer Science},
	Title = {Learning Theory, 19th Annual Conference on Learning Theory, COLT 2006, Pittsburgh, PA, USA, June 22-25, 2006, Proceedings},
	Volume = {4005},
	Year = {2006}}

%% This BibTeX bibliography file was created using BibDesk.
%% http://bibdesk.sourceforge.net/


%% Created for Susan Gruber at 2012-01-03 21:41:54 -0500


%% Saved with string encoding Unicode (UTF-8)


@string{jasa = {Journal of the American Statistical Association}}

@string{jc = {Journal of Classification}}

@string{jrssb = {Journal of the Royal Statistical Society, Series B}}

@string{jspi = {Journal of Statistical Planning and Inference}}

@string{pnas = {Proc. Natl. Acad. Sci.}}

@article{Xiao&Abrahamowicz&Moodie10,
	Author = {Y. Xiao, M. Abrahamowicz, E.E.M. Moodie},
	Journal = {The International Journal of Biostatistics},
	Title = {Accuracy of Conventional and Marginal Structural Cox Model Estimators: A Simulation Study},
	Volume = {6},
	Issue = {2},
	Article={13},
	Year = {2010}
}

@article{Moore&vanderLaan092,
  author =        {Moore, K.L. and van der Laan, M.J.},
  journal =       {Stat Med},
  number =        {1},
  pages =         {39--64},
  title =         {Covariate Adjustment in Randomized Trials with Binary
                   Outcomes: targeted Maximum Likelihood Estimation},
  volume =        {28},
  year =          {2009},
}

@article{Gruber&vanderLaanTygacil,
  author = {S. Gruber and M.J. van der Laan},
  journal = {Biometrics},
  title = {An Application of Targeted Maximum Likelihood Estimation to the Meta-Analysis of Safety Data},
  Year = {2012 (in press)}
  }

@article{Hahn04,
	Author = {J. Hahn},
	Date-Added = {2012-01-03 21:40:45 -0500},
	Date-Modified = {2012-01-03 21:41:54 -0500},
	Journal = {Rev Econ Stat},
	Pages = {73-76},
	Title = {Functional restriction and efficiency in causal inference},
	Volume = {86},
	Year = {2004}}

@techreport{DiazHubbard&vanderLaan10,
	Author = {I. Diaz Munoz and A. E. Hubbard and M. J. van der Laan},
	Date-Added = {2011-12-29 11:12:37 -0500},
	Date-Modified = {2011-12-29 11:13:20 -0500},
	Institution = {UC Berkeley Division of Biostatistics Working Paper Series},
	Month = {October},
	Number = {270},
	Title = {Targeted Bayesian Learning},
	Type = {Working Paper},
	Year = {2010}}

@article{Abadie&Imbens11,
	Author = {A. Abadie and G.W. Imbens},
	Journal = {Journal of Business and Economic Statistics},
	Number = {1},
	Pages = {1-11},
	Title = {Bias-Corrected Matching Estimators for Average Treatment Effects},
	Volume = {29},
	Year = {2011}}

@article{Hernan10,
	Author = {The HIV-CAUSAL Collaboration},
	Date = {2010///},
	Date-Added = {2011-12-11 13:32:38 -0500},
	Date-Modified = {2011-12-11 13:33:01 -0500},
	Id = {00002030-201001020-00017},
	Isbn = {0269-9370},
	Journal = {AIDS},
	Number = {1},
	Title = {The effect of combined antiretroviral therapy on the overall mortality of {HIV}-infected individuals},
	Ty = {JOUR},
	Volume = {24},
	Year = {2010}}

@article{Newey90,
	Author = {W. K. Newey},
	Issue = {2},
	Journal = {Journal of Applied Econometrics},
	Pages = {99-135},
	Title = {Semiparametric Efficiency Bounds},
	Volume = {5},
	Year = {1990}}

@article{Robins&Mark&Newey92,
	Author = {J.M. Robins, S.D. Mark, W.K. Newey},
	Journal = {Biometrics},
	Volume = {48},
	pages = {479-95},
	Month = {June},
	Year = {1992},
	Title = {Estimating Exposure Effects by Modelling the Expectation of Exposure Conditional on Confounders}}

@article{Porteretal11,
	Author = {K.E. Porter and S. Gruber and M.J. van der Laan and J. S. Sekhon},
	Date-Added = {2011-12-08 18:06:10 -0500},
	Date-Modified = {2011-12-08 18:08:07 -0500},
	Journal = {The International Journal of Biostatistics},
	Number = {31},
	Issue = {1},
	Pages = {1-34},
	Title = {The Relative Performance of Targeted Maximum Likelihood Estimators},
	Volume = {7},
	Year = {2011}}

@article{Petersenetal10,
	Author = {M.L. Petersen and K.E. Porter and S. Gruber and Y. Wang and M.J. van der Laan},
	Date-Added = {2011-12-08 18:04:58 -0500},
	Date-Modified = {2011-12-08 18:04:58 -0500},
	Journal = {Stat Meth Med Res},
	Title = {Diagnosing and responding to violations in the positivity assumption},
	Volume = {published online 28 Oct (doi: 10.1177/0962280210386207)},
	Year = {2010}}

@techreport{Polley&vanderLaan10,
	Author = {E. C. Polley and M. J. van der Laan},
	Date-Added = {2011-07-11 21:14:27 -0700},
	Date-Modified = {2011-07-11 21:16:20 -0700},
	Institution = {U.C. Berkeley Division of Biostatistics Working Paper Series},
	Number = {200},
	Title = {Super Learner in Prediction},
	Year = {2010}}

@article{Breiman01c,
	Author = {L. Breiman},
	Date-Added = {2011-07-11 21:01:09 -0700},
	Date-Modified = {2011-07-11 21:02:03 -0700},
	Journal = {Machine Learning},
	Number = {1},
	Pages = {5-32},
	Title = {Random Forests},
	Volume = {45},
	Year = {2001}}

@techreport{Gruber&vanderLaan10c,
	Author = {S. Gruber and M.J. van der Laan},
	Date-Added = {2011-04-03 23:22:01 -0700},
	Date-Modified = {2011-04-03 23:22:01 -0700},
	Institution = {UC Berkeley},
	Number = {265},
	Title = {A Targeted Maximum Likelihood Estimator of a Causal Effect on a Bounded Continuous Outcome},
	Year = {2010}}

@book{Pearl00,
	Author = {J. Pearl},
	Date-Added = {2011-04-03 23:19:36 -0700},
	Date-Modified = {2011-04-03 23:19:36 -0700},
	Publisher = {Cambridge University Press, Cambridge},
	Title = {Causality: Models, Reasoning, and Inference},
	Year = {2000}}

@article{Imai&vanDyk04,
	Author = {K. Imai and D.A. van Dyk},
	Journal={Journal of the American Statistical Association},
	Volume={99},
	pages={854-66},
	year={2004},
	title={Causal inference with general treatment regimes: generalizing the propensity score}}


@article{Rotnitzkyetal12,
	Author = {A. Rotnitzky and Q. Lei and M. Sued and J. Robins},
	Journal={Biometrika},
	Volume = {99},
	Issue = {2},
	pages = {439-56},
	Title = {Improved Double-Robust Estimation in missing data and causal inference models},
	Year = {2012}}


@misc{Rotnitzkyetal11,
	Author = {A. Rotnitzky and Q. Lei and M. Sued and J. Robins},
	Date-Added = {2011-04-02 21:41:14 -0700},
	Date-Modified = {2011-04-03 23:25:42 -0700},
	Howpublished = {ENAR 2011 Spring Meeting},
	Month = {March},
	Title = {Enhanced Double-Robust Locally- Efficient Estimation in Regression Models for Longitudinal Studies},
	Year = {2011}}

@article{Rotnitzky&Li&Li10,
	Author = {A. Rotnitzky and L. Li and X. Li},
	Date-Added = {2011-03-14 17:15:47 -0700},
	Date-Modified = {2011-03-15 10:47:49 -0700},
	Journal = {Biometrika},
	Number = {4},
	Pages = {997-1001},
	Title = {A note on overadjustment in inverse probability weighted estimation},
	Type = {article},
	Volume = {97},
	Year = {2010}}

@manual{trustPKG,
	Author = {C. J. Geyer},
	Date-Added = {2011-03-07 21:04:15 -0800},
	Date-Modified = {2011-03-07 21:04:15 -0800},
	Note = {R package version 0.1-2},
	Title = {trust: Trust Region Optimization},
	Url = {http://CRAN.R-project.org/package=trust},
	Year = {2009},
	Bdsk-Url-1 = {http://CRAN.R-project.org/package=trust}}

@manual{alabamaPKG,
	Author = {R. Varadhan},
	Date-Added = {2011-03-07 21:04:06 -0800},
	Date-Modified = {2011-03-07 21:04:06 -0800},
	Note = {R package version 2010.10-1},
	Title = {alabama: Constrained nonlinear optimization},
	Url = {http://CRAN.R-project.org/package=alabama},
	Year = {2010},
	Bdsk-Url-1 = {http://CRAN.R-project.org/package=alabama}}

@article{Bembometal09b,
	Author = {O. Bembom and M.L. Petersen and S.-Y. Rhee and W. J. Fessel and S.E. Sinisi and R.W. Shafer and M.J. van der Laan},
	Date-Added = {2011-02-28 15:57:47 -0800},
	Date-Modified = {2011-02-28 15:57:47 -0800},
	Issue = {1},
	Journal = {Statistics in Medicine},
	Pages = {152-72},
	Title = {Biomarker discovery using targeted maximum likelihood estimation: Application to the treatment of antiretroviral resistant {HIV} infection},
	Volume = {28},
	Year = {2009}}

@article{Holland77,
	Address = {New York, NY, USA},
	Author = {J.H. Holland and J.S. Reitman},
	Date-Added = {2011-02-28 15:57:47 -0800},
	Date-Modified = {2011-02-28 15:57:47 -0800},
	Doi = {http://doi.acm.org/10.1145/1045343.1045373},
	Issn = {0163-5719},
	Journal = {SIGART Bull.},
	Pages = {49--49},
	Publisher = {ACM},
	Title = {Cognitive systems based on adaptive algorithms},
	Volume = {63},
	Year = {1977},
	Bdsk-Url-1 = {http://doi.acm.org/10.1145/1045343.1045373}}

@article{Abadie&Imbens06,
	Author = {A. Abadie and G.W. Imbens},
	Date-Added = {2011-02-28 15:57:47 -0800},
	Date-Modified = {2011-02-28 15:57:47 -0800},
	Issue = {1},
	Journal = {Econometrica},
	Pages = {235-67},
	Title = {Large Sample Properties of Matching Estimators for Average Treatment Effects},
	Volume = {74},
	Year = {2006}}

@article{hernan&brumback&robins03,
	Author = {Hernan, M. A. and Brumback, B. and Robins, J. M.},
	Date-Added = {2011-02-28 15:57:47 -0800},
	Date-Modified = {2011-02-28 15:57:47 -0800},
	Journal = {Epidemiology},
	Number = {5},
	Pages = {561--570},
	Title = {Marginal structural models to estimate the causal effect of zidovudine on the survival of {HIV}-positive men},
	Volume = {11},
	Year = {2000}}

@techreport{Bembom&Fessel&Shafer&vanderLaan08,
	Author = {O. Bembom and J.W. Fessel and R.W. Shafer and M.J. van der Laan},
	Date-Added = {2011-02-28 15:57:47 -0800},
	Date-Modified = {2011-02-28 15:57:47 -0800},
	Institution = {DigitalCommons@Florida Atlantic University [http://digitalcommons.fau.edu/cgi/oai2.cgi] (United States)},
	Keywords = {General Biostatistics},
	Location = {http://www.scientificcommons.org/36721107},
	Publisher = {The Berkeley Electronic Press},
	Title = {Data-adaptive Selection Of The Adjustment Set In Variable Importance Estimation},
	Url = {http://www.bepress.com/ucbbiostat/paper231},
	Year = {2008},
	Bdsk-Url-1 = {http://www.bepress.com/ucbbiostat/paper231}}

@article{vanderLaan&Gruber09,
	Author = {M.J. van der Laan and S. Gruber},
	Date-Added = {2011-02-22 20:50:28 -0800},
	Date-Modified = {2011-02-22 20:50:28 -0800},
	Journal = {The International Journal of Biostatistics},
	Title = {Collaborative Double robust penalized targeted maximum likelihood estimation},
	Year = {2009}}

@manual{HmiscPKG,
	Author = {F.E. {Harrell Jr}},
	Date-Added = {2011-02-22 20:48:50 -0800},
	Date-Modified = {2011-02-22 20:48:50 -0800},
	Note = {R package version 3.8-3},
	Title = {Hmisc: Harrell Miscellaneous},
	Url = {http://CRAN.R-project.org/package=Hmisc},
	Year = {2010},
	Bdsk-Url-1 = {http://CRAN.R-project.org/package=Hmisc}}

@article{Freedman&Berk08,
	Author = {D.A. Freedman and R.A. Berk},
	Date-Added = {2011-02-22 20:47:43 -0800},
	Date-Modified = {2011-03-13 16:18:51 -0700},
	Issue = {4},
	Journal = {Evaluation Review},
	Pages = {392-409},
	Title = {Weighting Regressions by Propensity Scores},
	Volume = {32},
	Year = {2008}}

@article{Shpitser08,
	Author = {I. Shpitser and J. Pearl},
	Journal = {Journal of Machine Learning Research},
	Pages = {1941-79},
	Title = {Complete Identification Methods for the Causal Hierarchy},
	Volume = {9},
	Year = {2008}}

@article{Tan08,
	Author = {Z. Tan},
	Date-Added = {2011-02-22 20:42:13 -0800},
	Date-Modified = {2011-02-22 20:42:13 -0800},
	Issue = {2},
	Journal = {Biometrika},
	Pages = {1-22},
	Title = {Bounded, efficient, and doubly robust estimation with inverse weighting},
	Volume = {94},
	Year = {2008}}

@article{McCullagh83,
	Author = {P. Mc{C}ullagh},
	Date-Added = {2011-02-22 20:42:13 -0800},
	Date-Modified = {2011-02-22 20:42:13 -0800},
	Issue = {1},
	Journal = {The Annals of Statistics},
	Pages = {59-67},
	Title = {Quasi-likelihood functions},
	Volume = {11},
	Year = {1983}}

@article{Dehejia&Wahba02,
	Author = {R.H. Dehejia and S. Wahba},
	Date-Added = {2011-02-22 20:42:13 -0800},
	Date-Modified = {2011-02-22 20:42:13 -0800},
	Journal = {The Review of Economics and Statistics},
	Pages = {151-61},
	Title = {Propensity Score Matching Methods for Nonexperimental Causal Studies},
	Volume = {84},
	Year = {2002}}

@article{Stukeletal07,
	Author = {T.A. Stukel and E.S. Fisher and D.E. Wennberg and D.A.Alter and D.J.Gottlieb and M.J. Vermeulen},
	Date-Added = {2011-02-22 20:42:13 -0800},
	Date-Modified = {2011-02-22 20:42:13 -0800},
	Journal = {JAMA},
	Pages = {278-85},
	Title = {Analysis of Observational Studies in the Presence of Treatment Selection Bias: Effects of Invasive Cardiac Management on {AMI} Survival Using Propensity Score and Instrumental Variable Methods},
	Volume = {297},
	Year = {2007}}

@book{mark,
	Author = {M.J. van der Laan and J.M. Robins},
	Date-Added = {2011-02-22 20:42:13 -0800},
	Date-Modified = {2011-02-22 20:42:13 -0800},
	Publisher = {Springer, New York},
	Title = {Unified methods for censored longitudinal data and causality},
	Year = {2003}}

@book{vanderLaan&Rose11,
	Author = {M.J. van der Laan and S. Rose},
	Publisher = {Springer, New York},
	Title = {Targeted Learning: Prediction and Causal Inference for Observational and Experimental Data},
	Year = {2011}}

@incollection{KS_vanderLaan&Rose11,
	Author = {J.S. Sekhon and S. Gruber and K. Porter and M.J. van der Laan},
	Booktitle = {{\rm M.J. van der Laan and S. Rose, } Targeted Learning: Prediction and Causal Inference for Observational and Experimental Data},
	Chapter = {21},
	Publisher = {Springer, New York},
	Title = {Propensity-Score-Based Estimators and {C-TMLE}},
	Year = {2011}}


	@incollection{RosenblumTMLEChapter,
	Author = {M. Rosenblum},
	Booktitle = {{\rm M.J. van der Laan and S. Rose, } Targeted Learning: Prediction and Causal Inference for Observational and Experimental Data},
	Chapter = {9},
	Publisher = {Springer, New York},
	Title = {Marginal Structural Models},
	Year = {2011}}

	@incollection{GruberCTMLEChapter,
	Author = {S. Gruber and M.J. van der Laan},
	Booktitle = {{\rm M.J. van der Laan and S. Rose, } C-TMLE of an Additive Point Treatment Effect},
	Chapter = {19},
	Publisher = {Springer, New York},
	Title = {Marginal Structural Models},
	Year = {2011}}


	@incollection{AntoineTMLEChapter,
	Author = {A. Chambaz},
	Booktitle = {{\rm M.J. van der Laan and S. Rose, } Targeted Learning: Prediction and Causal Inference for Observational and Experimental Data},
	Chapter = {29},
	Publisher = {Springer, New York},
	Title = {TMLE in Adaptive Group Sequential Covariate-Adjusted RCTs},
	Year = {2011}}





@article{Stitelman&vanderLaan10,
	Author = {O.M. Stitelman and M.J. van der Laan},
	Date-Added = {2011-02-22 20:35:37 -0800},
	Date-Modified = {2011-12-08 18:09:52 -0500},
	Journal = {The International Journal of Biostatistics},
	Number = {1},
	Title = {Collaborative Targeted Maximum Likelihood for Time to Event Data},
	Volume = {6},
	Year = {2010}}

@article{Breslow74,
	Author = {Breslow, N.},
	Date-Added = {2010-06-28 13:31:45 -0700},
	Date-Modified = {2010-06-28 13:33:19 -0700},
	Journal = {Biometrics},
	Month = {March},
	Number = {1},
	Pages = {89-99},
	Title = {Covariance Analysis of Censored Survival Data},
	Volume = {30},
	Year = {1974}}

@article{Effronetal02,
	Author = {Efron, B. and Hastie H. and Johnstone and Tibshirani},
	Date-Added = {2010-05-27 13:34:30 -0700},
	Date-Modified = {2010-05-27 13:36:40 -0700},
	Journal = {The Annals of Statistics},
	Title = {Least Angle Regression (with discussion)},
	Year = {2003}}

@manual{RDCT10,
	Address = {Vienna, Austria},
	Author = {R Development Core Team},
	Date-Added = {2010-05-27 13:15:41 -0700},
	Date-Modified = {2010-05-27 13:18:22 -0700},
	Organization = {R Foundation for Statistical Computing},
	Title = {{R}: A Language and Environment for Statistical Computing},
	Url = {http://www.R-project.org},
	Year = {2010},
	Bdsk-Url-1 = {http://www.R-project.org}}


@manual{RDCT12,
	Address = {Vienna, Austria},
	Author = {{R Development Core Team}},
	Date-Added = {2010-05-27 13:15:41 -0700},
	Date-Modified = {2010-05-27 13:18:22 -0700},
	Organization = {{R} Foundation for Statistical Computing},
	Title = {{R}: A Language and Environment for Statistical Computing},
	Url = {http://www.R-project.org},
	Year = {2012},
	Bdsk-Url-1 = {http://www.R-project.org}}

  @Manual{RDCT11,
    title = {R: A Language and Environment for Statistical Computing},
    author = {{R Development Core Team}},
    organization = {R Foundation for Statistical Computing},
    address = {Vienna, Austria},
    year = {2011},
    note = {{ISBN} 3-900051-07-0},
    url = {http://www.R-project.org/},
  }

@manual{bartPKG,
	Author = {Hugh Chipman and Robert McCulloch},
	Note = {{R} package version~0.3-1.1},
	Title = {{BayesTree}: Bayesian Methods for Tree Based Models},
	Url = {http://CRAN.R-project.org/package=BayesTree},
	Year = {2010},
	Bdsk-Url-1 = {http://CRAN.R-project.org/package=BayesTree}}

@manual{SLPKG,
	Author = {E.C. Polley},
	Note = {{R}~package version~1.1-17},
	Title = {{SuperLearner}: {S}uper {L}earner Prediction},
	Url = {http://www.stat.berkeley.edu/~ecpolley/SL/},
	Year = {2010},
	Bdsk-Url-1 = {http://www.stat.berkeley.edu/~ecpolley/SL/}}

@manual{caretPKG,
	Author = {M. Kuhn and J. Wing and S. Weston and A. Williams and C. Keefer and A. Engelhardt},
	Note = {{R} package version~4.72},
	Title = {{caret}: Classification and Regression Training},
	Url = {http://CRAN.R-project.org/package=caret},
	Year = {2010},
	Bdsk-Url-1 = {http://CRAN.R-project.org/package=caret}}

@manual{TMLEPKG,
	Author = {S. Gruber},
	Note = {{R}~package version~1.2.0},
	Title = {{tmle}: Targeted Maximum Likelihood Estimation},
	Url = {http://CRAN.R-project.org/package=tmle},
	Year = {2012},
	Bdsk-Url-1 = {http://CRAN.R-project.org/package=tmle}}

@manual{CTMLEPKG,
	Author = {S. Gruber},
	Note = {{R}~software version~0.5},
	Title = {Collaborative Targeted Maximum Likelihood Estimation},
	Url = {http://www.stat.berkeley.edu/~laan/Software/},
	Year = {2010},
	Bdsk-Url-1 = {http://www.stat.berkeley.edu/~laan/Software/}}

@article{SL_jss,
	Author = {E.C. Polley and M.J. van der Laan},
	Note = {submitted...},
	Title = {Super Learner},
	Year = {2011}}

@manual{ipredPKG,
	Author = {A. Peters and T. Hothorn},
	Note = {{R} package version~0.8-8},
	Title = {{ipred}: Improved Predictors},
	Url = {http://CRAN.R-project.org/package=ipred},
	Year = {2009},
	Bdsk-Url-1 = {http://CRAN.R-project.org/package=ipred}}

@manual{dsaPKG,
	Author = {R. Neugebauer and J. Bullard},
	Note = {{R} package version~3.1.4},
	Title = {{DSA}: Deletion/Substitution/Addition Algorithm},
	Url = {http://www.stat.berkeley.edu/~laan/Software/},
	Year = {2010},
	Bdsk-Url-1 = {http://www.stat.berkeley.edu/~laan/Software/}}

@manual{earthPKG,
	Author = {S. Milborrow},
	Note = {{R} package version~2.4-0},
	Title = {{earth}: Multivariate Adaptive Regression Spline Models},
	Url = {http://CRAN.R-project.org/package=earth},
	Year = {2009},
	Bdsk-Url-1 = {http://CRAN.R-project.org/package=earth}}

@book{nnetPKG,
	Address = {New York},
	Author = {W. N. Venables and B. D. Ripley},
	Edition = {4th},
	Note = {ISBN 0-387-95457-0},
	Publisher = {Springer},
	Title = {Modern Applied Statistics with S},
	Url = {http://www.stats.ox.ac.uk/pub/MASS4},
	Year = {2002},
	Bdsk-Url-1 = {http://www.stats.ox.ac.uk/pub/MASS4}}

@manual{e1071PKG,
	Author = {E. Dimitriadou and K. Hornik and F. Leisch and D. Meyer and and A. Weingessel},
	Note = {{R} package version~1.5-24},
	Title = {{e1071}: Misc Functions of the Department of Statistics (e1071), TU Wien},
	Url = {http://CRAN.R-project.org/package=e1071},
	Year = {2010},
	Bdsk-Url-1 = {http://CRAN.R-project.org/package=e1071}}

@manual{gamPKG,
	Author = {T.J. Hastie},
	Note = {{R} package version~1.01},
	Title = {{gam}: Generalized Additive Models},
	Url = {http://CRAN.R-project.org/package=gam},
	Year = {2009},
	Bdsk-Url-1 = {http://CRAN.R-project.org/package=gam}}

@article{Zhang&Yu98,
	Author = {Zhang, J and Yu, KF},
	Date-Added = {2010-05-26 14:58:38 -0700},
	Date-Modified = {2010-05-26 15:00:17 -0700},
	Journal = {JAMA},
	Pages = {1690-1},
	Title = {What's relative risk? A method of correcting the odds ratio in cohort studies of common outcomes},
	Volume = {280},
	Year = {1998}}

@article{Zocchettietal97,
	Author = {Zocchetti, C and Consonni, D and Bertazzi, P A},
	Date-Added = {2010-05-26 14:54:07 -0700},
	Date-Modified = {2010-05-26 14:57:40 -0700},
	Journal = {International Journal of Epidemiology},
	Pages = {220-223},
	Title = {Relationship between prevalence rate ratios and odds ratios in cross-sectional studies},
	Volume = {26},
	Year = {1997}}

@article{Greenland03,
	Author = {Greenland, S},
	Date-Added = {2010-05-26 14:39:43 -0700},
	Date-Modified = {2010-05-26 14:41:15 -0700},
	Journal = {Am J Epidemiol},
	Number = {4},
	Pages = {301-305},
	Title = {Model-based Estimation of Relative Risks and Other Epidemiologic Measures in Studies of Common Outcomes and in Case-Control Studies},
	Volume = {160},
	Year = {2003}}

@article{Hogueetal83,
	Author = {Hogue, C.J.R. and Gaylor, DW and Schulz, KF},
	Date-Added = {2010-05-26 14:32:50 -0700},
	Date-Modified = {2010-05-26 14:34:43 -0700},
	Journal = {Am J Epidemiol},
	Number = {3},
	Pages = {396-407},
	Title = {Estimators of Relative Risk for Case-Control Studies},
	Volume = {118},
	Year = {1983}}

@article{Carteretal05,
	Author = {Carter, RE and Lipsitz, SR and Tilley, BC},
	Date-Added = {2010-05-26 13:07:18 -0700},
	Date-Modified = {2010-05-26 13:08:31 -0700},
	Title = {Quasi-likelihood estimation for relative risk regression models}}

@article{McNuttetal01,
	Author = {McNutt, Louise-Anne and hu, Chuntao and Xue, Xiaonana and Hafner, Paul},
	Date-Added = {2010-05-26 12:38:16 -0700},
	Date-Modified = {2010-05-26 12:40:01 -0700},
	Journal = {Am J Epidemiol},
	Number = {10},
	Pages = {940-943},
	Title = {Estimating the Relative Risk in Cohort Studies and Clinical Trials of Common Outcomes},
	Volume = {157},
	Year = {2003}}

@article{Zou04,
	Author = {Zou, G.},
	Date-Added = {2010-05-26 11:56:32 -0700},
	Date-Modified = {2010-05-26 11:57:29 -0700},
	Journal = {Am J Epidemiol},
	Pages = {702-6},
	Title = {A modified Poisson regresion approach to prospective studies with binary data},
	Volume = {159},
	Year = {2004}}

@article{Zocchettietal95,
	Author = {Zocchett, C and Consonni, Dario and Bertazzi, Pier Alberto},
	Date-Added = {2010-05-26 11:50:39 -0700},
	Date-Modified = {2010-05-26 11:52:18 -0700},
	Journal = {Int J Epidemiol},
	Pages = {1064-1105},
	Title = {RE: Estimation of prevalence rate ratios from cross-sectional data (letter)},
	Volume = {24},
	Year = {1995}}

@article{Skovetal98,
	Author = {Skov, T and Deddens, J.A. and Petersen, M.R.},
	Date-Added = {2010-05-26 11:47:20 -0700},
	Date-Modified = {2010-05-26 11:50:06 -0700},
	Journal = {Int J Epidemiol},
	Pages = {91-95},
	Title = {Prevalence proportion ratios: estimation and hypothesis testing},
	Volume = {27},
	Year = {1998}}

@proceedings{Deddensetal08,
	Address = {Cary, NC},
	Author = {Deddens, J.A. and Petersen, M.R. and Lei, X.},
	Date-Added = {2010-05-24 14:27:56 -0700},
	Date-Modified = {2010-05-24 14:31:49 -0700},
	Number = {270-28},
	Organization = {SAS Institute},
	Publisher = {Proceedings of the 28th Annual SAS Users Group International Conference, March 30-April 2, 2003},
	Title = {Estimation of prevalence ratios when PROC GENMOD does not converge},
	Year = {2003}}

@article{Lee&Chia98,
	Author = {Lee, J and Chia, KS},
	Date-Added = {2010-05-24 14:06:12 -0700},
	Date-Modified = {2010-05-24 14:07:51 -0700},
	Journal = {Br J Ind Med},
	Pages = {861-2},
	Title = {Estimation of prevalence rate ratios for cross-sectional data: an example in occupational epidemiology},
	Volume = {50},
	Year = {1993}}

@article{Lee94,
	Author = {Lee, J.},
	Date-Added = {2010-05-24 14:04:58 -0700},
	Date-Modified = {2010-05-24 14:09:36 -0700},
	Journal = {Int J Epidemiol},
	Pages = {201-3},
	Title = {Odds ratio or relative risk for cross-sectional data?},
	Volume = {23},
	Year = {1994}}

@article{Wacholder86,
	Author = {Wacholder, S},
	Date-Added = {2010-05-24 13:59:47 -0700},
	Date-Modified = {2010-05-24 14:01:31 -0700},
	Journal = {Am J Epidemiol},
	Pages = {174-84},
	Title = {Binomial regression in {GLIM}, estimating risk ratios and risk differences.},
	Volume = {123},
	Year = {1986}}

@techreport{Lumleyetal06,
	Author = {Lumley, Thomas and Kronmal, Richard and Ma, Shuangge},
	Date-Added = {2010-05-24 13:27:04 -0700},
	Date-Modified = {2010-05-24 13:29:21 -0700},
	Institution = {University of Washington},
	Number = {293},
	Title = {Relative Risk Regresssion in Medical Research: Models, Contrasts, Estimators, and Algorithms},
	Year = {2006}}

@article{Barros&Hirakata03,
	Author = {Barros, Alu{\'\i}sio J D and Hirakata, V{\^a}nia N},
	Date-Added = {2010-05-24 13:25:16 -0700},
	Date-Modified = {2010-05-24 13:25:16 -0700},
	Doi = {10.1186/1471-2288-3-21},
	Journal = {BMC Med Res Methodol},
	Journal-Full = {BMC medical research methodology},
	Mesh = {Cross-Sectional Studies; Empirical Research; Humans; Linear Models; Logistic Models; Models, Statistical; Odds Ratio; Poisson Distribution; Prevalence; Proportional Hazards Models},
	Month = {Oct},
	Pages = {21},
	Pmc = {PMC521200},
	Pmid = {14567763},
	Pst = {epublish},
	Title = {Alternatives for logistic regression in cross-sectional studies: an empirical comparison of models that directly estimate the prevalence ratio},
	Volume = {3},
	Year = {2003},
	Bdsk-Url-1 = {http://dx.doi.org/10.1186/1471-2288-3-21}}

@article{Neutra&Drolette78,
	Author = {Neutra, R R and Drolette, M E},
	Date-Added = {2009-10-05 15:02:58 -0700},
	Date-Modified = {2009-10-05 15:02:58 -0700},
	Journal = {Am J Epidemiol},
	Journal-Full = {American journal of epidemiology},
	Mesh = {Biometry; Communicable Diseases; Environmental Exposure; Humans; Methods; Models, Theoretical; Probability Theory; Retrospective Studies},
	Month = {Sep},
	Number = {3},
	Pages = {214-22},
	Pmid = {707490},
	Title = {Estimating exposure-specific disease rates from case-control studies using Bayes' theorem},
	Volume = {108},
	Year = {1978}}

@article{Miettinen76,
	Author = {Miettinen, Olli S},
	Date-Added = {2009-10-05 13:42:11 -0700},
	Date-Modified = {2009-10-05 13:43:23 -0700},
	Journal = {American Journal of Epidemiology},
	Pages = {226-35.},
	Title = {Estimability and estimation in case-referent studies},
	Volume = {103},
	Year = {1976}}

@book{Checkowayetaletal04,
	Author = {Harvey Checkoway and Neil Pearce and David Kriebel},
	Date-Added = {2009-10-05 14:34:34 -0700},
	Date-Modified = {2009-10-05 14:36:29 -0700},
	Publisher = {Oxford University Press},
	Title = {Research Methods in Occupational Epidemiology},
	Year = {2004}}

@article{Kang&Schafer07,
	Author = {J. Kang and J. Schafer},
	Journal = {Statistical Science},
	Pages = {523-39},
	Title = {Demystifying Double Robustness: A Comparison of Alternative Strategies for Estimating a Population Mean from Incomplete Data (with discussion)},
	Volume = {22},
	Year = {2007}}

@article{Robinsetal07,
	Author = {J. M. Robins and M. Sued and Q. Lei-Gomez and A. Rotnitzky},
	Journal = {Statistical Science},
	Pages = {544-559},
	Title = {Comment: Performance of Double-Robust Estimators When ``Inverse Probability'' Weights Are Highly Variable},
	Volume = {22},
	Year = {2007}}

@article{Tan07,
	Author = {Z. Tan},
	Journal = {Statistical Science},
	Pages = {560-568},
	Title = {Comment: Understanding {OR}, {PS} and {DR}},
	Volume = {22},
	Year = {2007}}

@article{Neugebauer&vanderLaan05,
	Author = {R. Neugebauer and M.J. van der Laan},
	Journal = {Journal of Statistical Planning and Inference},
	Pages = {405--426},
	Title = {Why prefer double robust estimators in causal inference?},
	Volume = {129, Issues 1-2},
	Year = {2005}}

@article{vanderLaan&Petersen07,
	Author = {M.J. van der Laan and M.L. Petersen},
	Journal = {The International Journal of Biostatistics},
	Title = {Causal Effect Models for Realistic Individualized Treatment and Intention to Treat Rules},
	Volume = {3, Issue 1, Article 3},
	Year = {2007}}

@article{Tsiatis&Davidian07,
	Author = {A. Tsiatis and M. Davidian},
	Journal = {Statistical Science},
	Pages = {569-73},
	Title = {Comment: Demystifying Double Robustness: A Comparison of Alternative Strategies for Estimating a Population Mean from Incomplete Data (with discussion)},
	Volume = {22},
	Year = {2007}}

@article{Kang&Shafer07b,
	Author = {J. Kang and J. Schafer},
	Journal = {Statistical Science},
	Pages = {574-80},
	Title = {Rejoinder: Demystifying Double Robustness: A Comparison of Alternative Strategies for Estimating a Population Mean from Incomplete Data},
	Volume = {22},
	Year = {2007}}

@article{Schafer99,
	Author = {J.L. Schafer},
	Issue = {1},
	Journal = {Stat Methods Med Res},
	Month = {March},
	Pages = {3-15},
	Title = {Multiple imputation: a primer},
	Volume = {8},
	Year = {1999}}

@article{Pearl10a,
	Author = {J. Pearl},
	Journal = {The International Journal of Biostatistics},
	Number = {2},
	Title = {An Introduction to Causal Inference},
	Volume = {6},
	Year = {2010}}

@article{Hampel74,
	Author = {F.R. Hampel},
	Journal = {Journal of the American Statistical Association},
	Number = {346},
	Pages = {383-93},
	Title = {The Influence Curve and Its Role in Robust Estimation},
	Volume = {69},
	Year = {1974}}

@article{Murphy05,
	Author = {S. Murphy},
	Journal = {Statistics in Medicine},
	Title = {An experimental design for the development of adaptive treatment strategies},
	Volume = {24},
	Year = {2005}}

@article{Lavori&Dawson00,
	Author = {P. Lavori and R. Dawson},
	Journal = {Journal of the Royal Statistical Society, Series A},
	Title = {A design for testing clinical strategies: biased adaptive within-subject randomization},
	Volume = {163},
	Year = {2000}}

@article{Lavori&Dawson04,
	Author = {P. Lavori and R. Dawson},
	Journal = {Clinical trials},
	Title = {Dynamic treatment regimes: practical design considerations},
	Volume = {1},
	Year = {2004}}

@article{Thall&Millikan&Sung00,
	Author = {P. Thall and R. Millikan and H.-G. Sung},
	Journal = {Statistics in Medicine},
	Title = {Evaluating multiple treatment courses in clinical trials},
	Volume = {19},
	Year = {2000}}

@article{Rush&Trivedi&Fava03,
	Author = {A.J. Rush and M. Trivedi and M. Fava},
	Journal = {IV. American Journal of Psychiatry},
	Pages = {237},
	Title = {Depression},
	Volume = {160(2)},
	Year = {2003}}

@article{Schneideretal06,
	Author = {Schneider, L. and Tariot.P.N. and Dagerman, K. and Davis, S. and Hsiao, J. and Ismail, S. and Lebowitz, B. and Lyketsos, C. and Ryan J. and Stroup T. and Sultzer D. and Weintraub, D. and Lieberman, J.},
	Journal = {New England Journal of Medicine},
	Volume = {355(15)},
	Year = {2006}}

@article{Swartzetal07,
	Author = {Swartz, M. and Perkins, D. and Stroup, T. and Davis, S. and Capuano, G. and Rosenheck, R. and Reimherr, F. and McGee, M. and Keefe, R. and McEvoy, J. and Hsiao, J. and Lieberman, J.},
	Journal = {American Journal of Psychiatry},
	Title = {Effects of antipsychotic medications on psychosocial functioning in patients with chronic shizophrenia: Findings from the nimh catie study},
	Volume = {164},
	Year = {2007}}

@article{Rubin&vanderLaan08,
	Author = {D.B. Rubin and M.J. van der Laan},
	Journal = {The International Journal of Biostatistics},
	Location = {http://www.bepress.com/ijb/vol4/iss1/5},
	Title = {Empirical Efficiency Maximization: Improved Locally Efficient Covariate Adjustment in Randomized Experiments and Survival Analysis},
	Volume = {Vol. 4, Iss. 1, Article 5},
	Year = {2008}}

@article{vanderLaan&Rubin07,
	Author = {M.J. van der Laan and D.B. Rubin},
	Journal = {Technical report, working paper series http://www.bepress.com/ucbbiostat/paper226},
	Title = {A Note on Targeted Maximum Likelihood and Right Censored Data},
	Year = {2007}}

@article{vanderLaan&Rose&Gruber09,
	Author = {M.J. van der Laan and S. Rose and S. Gruber},
	Journal = {U.C. Berkeley Division of Biostatistics Working Paper Series, Paper 254},
	Title = {Readings in Targeted Maximum Likelihood Estimation},
	Year = {2009}}

@article{Bembometal09,
	Author = {O. Bembom and M.J. van der Laan and T. Haight and I.B. Tager},
	Journal = {Epidemiology},
	Title = {Lifetime and current leisure time physical activity and all-cause mortality in an elderly cohort},
	Year = {2009}}

@article{Bembom&vanderLaan07a,
	Author = {O. Bembom and M.J. van der Laan},
	Journal = {Journal of the National Cancer Institute},
	Pages = {1577-1582},
	Title = {Statistical Methods for analyzing sequentially randomized trials, commentary on JNCI article Adaptive therapy for androgen independent prostate cancer: A Randomized selection trial including four regimens, by Peter F. Thall, C. Logothetis, C. Pagliaro, S. Wen, M.A. Brown, D. Williams, R. Millikan (2007).},
	Volume = {99(21)},
	Year = {2007}}

@article{Rosenblumetal09,
	Author = {M. Rosenblum and S.G. Deeks and M.J. van der Laan and D.R. Bangsberg},
	Journal = {PLoS ONE},
	Title = {The Risk of Virologic Failure Decreases with Duration of HIV Suppression, at Greater than 50\% Adherence to Antiretroviral Therapy},
	Volume = {4(9): e7196.doi:10.1371/journal.pone.0007196},
	Year = {2009}}

@article{Robins&Orallana&Rotnitzky08,
	Author = {J. M. Robins and L. Orallana and A. Rotnitzky},
	Journal = {Statistics in Medicine},
	Pages = {4678-4721},
	Title = {Estimaton and extrapolation of optimal treatment and testing strategies},
	Volume = {27(23)},
	Year = {2008}}

@article{Bembom&vanderLaan07,
	Author = {O. Bembom and M.J. van der Laan},
	Journal = {Electronic Journal of Statistics},
	Pages = {http://www.i-journals.org/ejs/viewarticle.php?id=105&layout=abstract},
	Title = {A practical illustration of the importance of realistic individualized treatment rules in causal inference},
	Year = {2007}}

@article{Bembometal08,
	Author = {O. Bembom and M.L. Petersen and S.-Y. Rhee and W. J. Fessel and S.E. Sinisi and R.W. Shafer and M.J. van der Laan},
	Journal = {Statistics in Medicine},
	Pages = {http://www3.interscience.wiley.com/journal/121422393/abstract},
	Title = {Biomarker discovery using targeted maximum likelihood estimation: Application to the treatment of antiretroviral resistant HIV infection},
	Year = {2008}}

@article{Tuglus&vanderLaan08,
	Author = {C. Tuglus and M.J. van der Laan},
	Journal = {UC Berkeley Working Paper Series},
	Pages = {http://www.bepress.com/ucbbiostat/paper233/.},
	Title = {Targeted Methods for Biomarker Discovery, the Search for a Standard},
	Year = {2008}}

@article{vanderLaan08,
	Author = {M.J. van der Laan},
	Journal = {The International Journal of Biostatistics},
	Pages = {http://www.bepress.com/ijb/vol4/iss1/17/},
	Title = {Estimation Based on Case-Control Designs with Known Prevalance Probability},
	Year = {2008}}

@article{Rose&vanderLaan08,
	Author = {S. Rose and M.J. van der Laan},
	Journal = {The International Journal of Biostatistics},
	Pages = {http://www.bepress.com/ijb/vol4/iss1/19/.},
	Title = {Simple Optimal Weighting of Cases and Controls in Case-Control Studies},
	Year = {2008}}

@article{Rose&vanderLaan09,
	Author = {S. Rose and M.J. van der Laan},
	Journal = {The International Journal of Biostatistics},
	Pages = {http://www.bepress.com/ijb/vol5/iss1/1/.},
	Title = {Why Match? [Investigating Matched Case-Control Study Designs with Causal Effect Estimation},
	Year = {2009}}

@inproceedings{Moore&vanderLaan09,
	Author = {K.L. Moore and M.J. van der Laan},
	Booktitle = {in Design, Summarization, Analysis \& Interpretation of Clinical Trials with Time-to-Event Endpoints},
	Editor = {Karl E. Peace},
	Publisher = {Chapman and Hall},
	Title = {Application of Time-to-Event Methods in the Assessment of Safety in Clinical Trials},
	Year = {2009}}

@inproceedings{Polley&vanderLaan09,
	Author = {E.C. Polley and M.J. van der Laan},
	Booktitle = {in Design, Summarization, Analysis \& Interpretation of Clinical Trials with Time-to-Event Endpoints},
	Editor = {Karl E. Peace},
	Publisher = {Chapman and Hall},
	Title = {Predicting Optimal Treatment Assignment Based on Prognostic Factors in Cancer Patients},
	Year = {2009}}

@article{vanderVaart&Dudoit&vanderLaan06,
	Author = {A.W. van der Vaart and S. Dudoit and M.J. van der Laan},
	Journal = {Statistics and Decisions},
	Number = {3},
	Pages = {351--371},
	Title = {Oracle Inequalities for Multi-Fold Cross-Validation},
	Volume = {24},
	Year = {2006}}

@article{vanderLaan&Dudoit&vanderVaart06,
	Author = {M.J. van der Laan and S. Dudoit and A.W. van der Vaart},
	Journal = {Statistics and Decisions},
	Number = {3},
	Pages = {373--395},
	Title = {The Cross-Validated Adaptive Epsilon-Net Estimator},
	Volume = {24},
	Year = {2006}}

@article{Rosenbaum&Rubin83,
	Author = {P.R. Rosenbaum and D.B. Rubin},
	Journal = {Biometrika},
	Pages = {41-55},
	Title = {The Central Role of the Propensity Score in Observational Studies for Causal Effects},
	Volume = {70},
	Year = {1983}}

@article{vanderLaan&Polley&Hubbard07,
	Author = {M.J. van der Laan and E. Polley and A. Hubbard},
	Issn = {1},
	Journal = {Statistical Applications in Genetics and Molecular Biology},
	Location = {http://www.bepress.con/sagmb/vol6/iss1/art25},
	Number = {25},
	Title = {{S}uper {L}earner},
	Volume = {6},
	Year = {2007}}

@article{Sekhon08,
	Author = {J.S. Sekhon},
	Journal = {Journal of Statistical Sotware, Forthcoming},
	Location = {http://ssrn.com/paper=1009044},
	Publisher = {SSRN},
	Title = {Multivariate and Propensity Score Matching Software with Automated Balance Optimization: The Matching package for {R}},
	Year = {2008}}

@article{Bembometal08b,
	Author = {O. Bembom and J.W. Fessel and R.W. Shafer and M.J. van der Laan},
	Institution = {DigitalCommons\@Florida Atlantic University [http://digitalcommons.fau.edu/cgi/oai2.cgi] (United States)},
	Keywords = {General Biostatistics},
	Location = {http://www.scientificcommons.org/36721107},
	Publisher = {The Berkeley Electronic Press},
	Title = {Data-adaptive Selection Of The Adjustment Set In Variable Importance Estimation},
	Url = {http://www.bepress.com/ucbbiostat/paper231},
	Year = {2008},
	Bdsk-Url-1 = {http://www.bepress.com/ucbbiostat/paper231}}

@article{Holland&Reitman77,
	Address = {New York, NY, USA},
	Author = {J.H. Holland and J.S. Reitman},
	Doi = {http://doi.acm.org/10.1145/1045343.1045373},
	Issn = {0163-5719},
	Journal = {SIGART Bull.},
	Pages = {49--49},
	Publisher = {ACM},
	Title = {Cognitive systems based on adaptive algorithms},
	Volume = {63},
	Year = {1977},
	Bdsk-Url-1 = {http://doi.acm.org/10.1145/1045343.1045373}}

@book{Rubin06,
	Address = {Cambridge, MA},
	Author = {D.B. Rubin},
	Publisher = {Cambridge University Press},
	Title = {Matched Sampling for Causal Effects.},
	Year = {2006}}

@incollection{Mansk1&McFadden81,
	Address = {Cambridge, MA},
	Author = {C.F. Manski and D. McFadden},
	Booktitle = {Structural Analysis of Discrete Data with Econometric Applications},
	Editor = {C.F. Manski and D. McFadden},
	Publisher = {The MIT Press},
	Title = {Alternative estimators and sample designs for discrete choice analysis},
	Year = {1981}}

@article{Manski&Lerman77,
	Author = {C.F. Manski and S.R. Lerman},
	Journal = {Econometrica},
	Number = {8},
	Pages = {1977-1988},
	Title = {The Estimation of Choice Probabilities from Choice Based Samples},
	Volume = {45},
	Year = {1977}}

@article{Cosslett81,
	Author = {S.R. Cosslett},
	Journal = {Econometrica},
	Number = {5},
	Pages = {1289-1316},
	Title = {Maximum Likelihood Estimator for Choice-Based Samples},
	Volume = {49},
	Year = {1981}}

@article{Cornfield51,
	Author = {J. Cornfield},
	Journal = {J Nat Cancer Inst},
	Pages = {1269-1275},
	Title = {A method of estimating comparative rates from clinical data. Applications to cancer of the lung, breast, and cervix.},
	Volume = {11},
	Year = {1951}}

@inproceedings{Cornfield56,
	Author = {J. Cornfield},
	Booktitle = {Proceedings of the Third Berkeley Symposium, Volume IV},
	Editor = {J. Neyman},
	Pages = {133-148},
	Publisher = {University of California Press},
	Title = {A statistical problem arising from retrospective studies},
	Year = {1956}}

@article{Benichou&Wacholder94,
	Author = {J. Benichou and S. Wacholder},
	Journal = {Statistics in Medicine},
	Pages = {651-661},
	Title = {A comparison of three approaches to estimate exposure-specific incidence rates from population-based case-control data.},
	Volume = {13},
	Year = {1994}}

@article{Breslow&Robins&Wellner00,
	Author = {N.E. Breslow and J.M. Robins and J.A. Wellner},
	Journal = {Bernoulli},
	Pages = {447--455},
	Title = {On the semi-parametric efficiency of logistic regression under case-control sampling},
	Volume = {6(3)},
	Year = {2000}}

@article{Mansonetal07,
	Author = {R. Mansson, M.M. Joffe, W. Sun, S. Hennessy},
	Journal = {Am J Epidemiol},
	Number = {3},
	Pages = {332-339},
	Title = {On the Estimation and Use of Propensity Scores in Case-Control and Case-Cohort Studies.},
	Volume = {166},
	Year = {2007}}

@article{Anderson79,
	Author = {J.A. Anderson},
	Journal = {Biometrika},
	Pages = {19--35},
	Title = {Separate sample logistic discrimination},
	Volume = {59},
	Year = {1972}}

@article{Prentice&Pyke79,
	Author = {R.L. Prentice and R. Pyke},
	Journal = {Biometrika},
	Pages = {403--411},
	Title = {Logistic disease incidence models and case-control studies},
	Volume = {66},
	Year = {1979}}

@article{Breslow96,
	Author = {N.E. Breslow},
	Journal = {J Am Stat Soc},
	Pages = {14--28},
	Title = {Statistics in Epidemiology: the Case-Control Study},
	Volume = {91},
	Year = {1996}}

@book{Breslow&Day80,
	Address = {Lyon},
	Author = {N.E. Breslow and N.E. Day},
	Publisher = {International Agency for Research on Cancer},
	Title = {Statistical Methods in Cancer Research: Volume 1 -- The analysis of case-control studies},
	Year = {1980}}

@article{Holford&White&Kelsey78,
	Author = {T.R. Holford and C. White and J.L. Kelsey},
	Journal = {Am J Epid},
	Number = {3},
	Pages = {245--255},
	Title = {Multivariate Analysis for Matched Case-Control Studies},
	Volume = {107},
	Year = {1978}}

@article{Breslowetal78,
	Author = {N.E. Breslow and N.E. Day and K.T. Halvorsen and R.L. Prentice and C. Sabal},
	Journal = {Am J Epid},
	Number = {4},
	Pages = {299--307},
	Title = {Estimation of Multiple Relative Risk Functions in Matched Case-Control Studies},
	Volume = {108},
	Year = {1978}}

@book{Schlesselman82,
	Address = {Oxford},
	Author = {J.J. Schlesselman},
	Publisher = {Oxford University Press},
	Title = {Case-Control Studies: Design, Conduct, Analysis},
	Year = {1982}}

@book{Collett91,
	Address = {London},
	Author = {D. Collett},
	Publisher = {Chapman and Hall},
	Title = {Modeling Binary Data},
	Year = {1991}}

@book{Jewell04,
	Address = {Boca Raton},
	Author = {N.P. Jewell},
	Publisher = {Chapman and Hall/CRC},
	Title = {Statistics for Epidemiology},
	Year = {2004}}

@book{Hosmer&Lemeshow00,
	Address = {New York},
	Author = {D.W. Hosmer and S. Lemeshow},
	Edition = {2nd},
	Publisher = {John Wiley and Sons},
	Title = {Applied Logistic Regression},
	Year = {2000}}

@article{Robins99,
	Author = {J.M. Robins},
	Journal = {Statistical Science},
	Number = {3},
	Pages = {281--293},
	Title = {[Choice as an Alternative to Control in Observational Studies]: Comment},
	Volume = {14},
	Year = {1999}}

@article{Newman06,
	Author = {S. Newman},
	Journal = {Epid Persp Innov},
	Pages = {2},
	Title = {Causal Analysis of Case-Control Data},
	Url = {http://www.epi-perspectives.com/content/3/1/2},
	Volume = {3},
	Year = {2006},
	Bdsk-Url-1 = {http://www.epi-perspectives.com/content/3/1/2}}

@article{Zelen&Parker86,
	Author = {M. Zelen and R.A. Parker},
	Journal = {Stat Med},
	Number = {3},
	Pages = {261--269},
	Title = {Case-Control Studies and Bayesian Inference},
	Volume = {5},
	Year = {1986}}

@article{Sinhetal04,
	Author = {S. SInha and B. Mukherjee and M Ghosh},
	Journal = {Biometrics},
	Pages = {41--49},
	Title = {Bayesian Semiparametric Modeling for Matched Case-Control Studies with Multiple Disease States},
	Volume = {60},
	Year = {2004}}

@article{Ritchieetal01,
	Author = {M.D. Ritchie and L.W. Hahn and N. Roodi and L.R. Bailey and W.D. Dupont and F.F. Parl and J.H. Moore},
	Journal = {Am J Hum Genet},
	Number = {1},
	Pages = {138--47},
	Title = {Multifactor-dimensionality reduction reveals high-order interactions among estrogen-metabolism genes in sporadic breast cancer.},
	Volume = {69},
	Year = {2001}}

@article{Mei&Cuccaro&Martin07,
	Author = {H. Mei and M.L. Cuccaro and E.R. Martin},
	Journal = {Am J Hum Genet},
	Number = {6},
	Pages = {1251-61},
	Title = {Multifactor dimensionality reduction-phenomics: a novel method to capture genetic heterogeneity with use of phenotypic variables.},
	Volume = {81},
	Year = {2007}}

@article{Bangsberg&Moss&Deeks04,
	Abstract = {Public health debates about providing HIV antiretroviral therapy to impoverished populations have centred on the relationship between adherence and risk of drug resistance. Recent data indicate that each antiretroviral therapeutic class has a unique adherence-resistance relationship. Resistance to single protease inhibitor therapy occurs most frequently at moderate to high levels of adherence, resistance to non-nucleoside reverse transcriptase inhibitor therapy occurs at low to moderate levels of adherence, and resistance to ritonavir-boosted protease inhibitor therapy is most likely to occur at middle ranges of adherence. These dynamic relationships should be considered in balancing the individual and public health benefits of therapy.},
	Author = {D.R. Bangsberg and A.R. Moss and S.G. Deeks},
	Journal = {J Antimicrob Chemother},
	Keywords = {Anti-HIV Agents/*therapeutic use Developing Countries *Drug Resistance, Viral Humans *Patient Compliance Public Health Research Support, Non-U.S. Gov't Research Support, U.S. Gov't, P.H.S.},
	Note = {0305-7453 (Print) Journal Article Review},
	Number = {5},
	Pages = {696-9},
	Title = {Paradoxes of adherence and drug resistance to {HIV} antiretroviral therapy},
	Volume = {53},
	Year = {2004}}

@article{Scharfstein&Tsiatis&Robins97,
	Author = {D.O. Scharfstein and A.A. Tsiatis and J.M. Robins},
	Journal = {Journal of the American Statistical Association},
	Number = {440},
	Pages = {1342--1350},
	Title = {Semiparametric efficiency and its implications on the design and analysis of group-sequential studies},
	Volume = {92},
	Year = {1997}}

@article{Bembometal07,
	Author = {O. Bembom and M. Petersen and SY Rhee and W.J. Fessel and S.E. Sinisi and R.W. Shafer 	 and M.J. van der Laan},
	Journal = {U.C. Berkeley Division of Biostatistics Working Paper Series},
	Optmonth = {August},
	Optnote = {http://www.bepress.com/ucbbiostat/paper221},
	Title = {Biomarker Discovery Using Targeted Maximum Likelihood Estimation: Application to the Treatment of Antiretroviral Resistant {HIV} Infection},
	Volume = {221},
	Year = {2007}}


@article{vanderLaan&Gruber12,
	Author = {M.J. van der Laan and S. Gruber},
	Journal = {The International Journal of Biostatistics},
	Title = {Targeted Minimum Loss Based Estimation of an Intervention Specific Mean},
	Volume = {in press},
	Year = {2012}}

@article{vanderLaan&Gruber12a,
	Author = {M.J. van der Laan and S. Gruber},
	Journal = {The International Journal of Biostatistics},
	Title = {Targeted Minimum Loss Based Estimation of Causal Effects of Multiple Time Point Interventions},
	Volume = {8},
	Year = {2012}}

@article{Gruber&vanderLaan12b,
	Author = {S. Gruber and M.J. van der Laan},
	Journal = {The International Journal of Biostatistics},
	Title = {Targeted Minimum Loss Based Estimation of a Causal Effect on an Outcome with Known Conditional Bounds},
	Volume = {8},
	Year = {2012}}

@techreport{Polley&vanderLaan10,
	Author = {E.C. Polley and M.J. van der Laan},
	Title = {Super Learner in Prediction},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper266},
	Year = {2010}}




@techreport{Stitelman&DeGruttola&vanderLaan11,
	Author = {O. M. Stitelman and  V. De Gruttola and M. J. van der Laan},
	Title = {A General Implementation of TMLE for Longitudinal Data Applied to Causal Inference in Survival Analysis},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper281},
	Month = {April},
	Year = {2011}
}




@techreport{tmleTR12,
	Author = {S. Gruber and M.J. van der Laan },
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper275},
	Title = {tmle: An {R} Package for Targeted Maximum Likelihood Estimation},
	Type = {Technical Report 275},
	Year = {revised: 2012}}

@techreport{vanderLaan&Gruber11TR,
	Author = {M.J. van der Laan and S. Gruber},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper290},
	Title = {Targeted Maximum Loss Based Estimation of an Intervention Specific Mean},
	Type = {Technical Report 290},
	Year = {2011}}

@article{vanderLaan&Gruber10,
	Author = {M.J. van der Laan and S. Gruber},
	Journal = {The International Journal of Biostatistics},
	Month = {January},
	Number = {1},
	Title = {Collaborative Double Robust Penalized Targeted Maximum Likelihood Estimation},
	Volume = {6},
	Year = {2010}}

@article{vanderLaan&Rubin06,
	Author = {M.J. van der Laan and D. Rubin},
	Journal = {The International Journal of Biostatistics},
	Number = {1},
	Optnote = {http://www.bepress.com/ijb/vol2/iss1/11},
	Title = {Targeted Maximum Likelihood Learning},
	Volume = {2},
	Year = {2006}}

@techreport{vanderLaan&Rubin06TR,
	Author = {M.J. van der Laan and D. Rubin},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper199},
	Title = {Targeted Maximum Likelihood Learning},
	Type = {Technical Report 213},
	Year = {2006}}

@article{Scharfstein&Tsiatis98,
	Author = {D.O. Scharfstein and A.A. Tsiatis},
	Journal = {Statistics in Medicine},
	Pages = {75--87},
	Title = {The use of simulation and bootstrap in information based group sequential studies},
	Volume = {17},
	Year = {1998}}

@article{Pampallona&Tsiatis&Kim01,
	Author = {S. Pampallona and A.A. Tsiatis and K. Kim},
	Journal = {Drug Informational Journal},
	Pages = {1113-1121},
	Title = {Interim monitoring of group sequential trials using spending functions for the type I and type II error probabilities},
	Volume = {35},
	Year = {2001}}

@article{Tsiatis&Mehta03,
	Author = {A.A. Tsiatis and C. Mehta},
	Journal = {Biometrika},
	Pages = {367-378},
	Title = {On the inefficiency of the adaptive design for monitoring clinical trials},
	Volume = {90},
	Year = {2003}}

@article{Banerjee&Tsiatis06,
	Author = {A. Banerjee and A.A. Tsiatis},
	Journal = {Statistics in Medicine},
	Optnote = {In press},
	Title = {Adaptive two-stage designs in phase II clinical trials},
	Year = {2006}}

@article{Tsiatis06,
	Author = {A.A. Tsiatis},
	Journal = {Statistics in Medicine},
	Optnote = {In press},
	Title = {Information based monitoring of clinical trials},
	Year = {2006}}

@article{Lokhnygina&Tsiatis06,
	Author = {Y. Lokhnygina and A.A. Tsiatis},
	Journal = {Journal of Statistical Planning and Inference},
	Optnote = {In press},
	Title = {Optimal two-stage group sequential designs},
	Year = {2006}}

@article{Bauer&Kohne94,
	Author = {P. Bauer and Kohne},
	Journal = {Biometrics},
	Pages = {1029--1041},
	Title = {Evaluation of experiments with adaptive interim analysis},
	Year = {1994}}

@article{Cui&Hung&Wang99,
	Author = {L. Cui and H.M.J. Hung and S-J Wang},
	Journal = {Biometrics},
	Pages = {853--857},
	Title = {Modification of sample size in group sequential trials},
	Year = {1999}}

@article{Jennison&Turnbull03,
	Author = {C. Jennison and B.W. Turnbull},
	Journal = {Statistics in Medicine},
	Pages = {971--993},
	Title = {Mid course sample size modification in clinical trials based on hte observed treatment effect},
	Year = {2003}}

@article{Koyama&Sampson&Gleser04,
	Author = {T. Koyama and A.R. Sampson and L.J. Gleser},
	Journal = {Journal of the Americal Statistical Association},
	Title = {A calculus for design of two stage adaptive procedures},
	Year = {2004}}

@article{Lan&Trost97,
	Author = {K.K.G Lan and D.C. Trost},
	Journal = {Proceedings Biopharm Section},
	Pages = {48-51},
	Title = {Estimation of parameters and sample size re-estimation},
	Year = {1997}}

@article{Lietal02,
	Author = {G. Li and W.J. Shih and T. Xie and J. Lu},
	Journal = {Biostatistics},
	Pages = {277--287},
	Title = {A sample size adjustment procedure for clinical trials based on conditional power},
	Year = {2002}}

@article{Mehta&Tsiatis01,
	Author = {C.R. Mehta and A.A. Tsiatis},
	Journal = {Drug Informational Journal},
	Pages = {1095--1112},
	Title = {Flexible sample size considerations using information based interim monitoring},
	Volume = {35},
	Year = {2001}}

@article{Mulle&Shafer01,
	Author = {H.H. Mulle and H. Shafer},
	Journal = {Biometrics},
	Pages = {886--891},
	Title = {Adaptive group sequential designs for clinical trials: combining the advantages of adaptive and classical group sequential approaches},
	Volume = {57},
	Year = {2001}}

@article{Proschan&Hunsberger95,
	Author = {M.A. Proschan and S.A. Hunsberger},
	Journal = {Biometrics},
	Pages = {1315--1324},
	Title = {Designed extension studies based on conditional power},
	Volume = {51},
	Year = {1995}}

@article{Shen&Fisher99,
	Author = {Y. Shen and L.D. Fisher},
	Journal = {Biometrics},
	Pages = {190--197},
	Title = {Statistical Inference for self-designing clinical trials with a one-sided hypothesis},
	Volume = {55},
	Year = {1999}}

@article{Wittes&Brittain90,
	Author = {J. Wittes and E. Brittain},
	Journal = {Statistics in Medicine},
	Pages = {65--72},
	Title = {The role of internal pilot studies in increasing efficiency of clinical trials},
	Volume = {9},
	Year = {1999}}

@article{Shen&Cheng06,
	Author = {Y. Shen and Y. Cheng},
	Journal = {Biostatistics},
	Optnote = {In Press},
	Title = {Adaptive design: Estimation and Inference with censored data in a semiparametric model},
	Year = {2006}}

@book{Spiegelalter&Abrams&Myles04,
	Author = {D.J. Spiegelalter and K.R. Abrams and J.P. Myles},
	Publisher = {Wiley, Chichester},
	Title = {Bayesian approaches to clinical trials and health care evaluation},
	Year = {2004}}

@book{Berry&Stangl96,
	Author = {D.A. Berry and D.K. Stangl},
	Publisher = {Marcel Dekker, New York},
	Title = {Bayesian biostatistics},
	Year = {1996}}

@article{Berry06,
	Author = {D.A. Berry},
	Journal = {Nature Reviews, Drug Discovery},
	Title = {Bayesian clinical trials},
	Volume = {5},
	Year = {2006}}

@book{Hu&Rosenberger06,
	Author = {F. Hu and W.F. Rosenberger},
	Publisher = {New York Wiley},
	Title = {The theory of response adaptive randomization in clinical trials},
	Year = {2006}}

@book{Dudoit&vanderLaan08,
	Author = {S. Dudoit and M.J. van der Laan},
	Publisher = {Springer Series of Statistics, New York},
	Title = {Resampling based multiple testing with applications to genomics},
	Year = {2008}}

@book{Sen&Singer93,
	Author = {P.K. Sen and J.M. Singer},
	Publisher = {Chapman \& Hall, New York},
	Title = {Large Sample Methods in Statistics: An Introduction with Applications},
	Year = {1993}}

@article{Bai&Hu&Rosenberger02,
	Author = {Z.D. Bai and F. Hu and W.F. Rosenberger},
	Journal = {The Annals of Statistics},
	Number = {1},
	Pages = {122--139},
	Title = {Asymptotic properties of adaptive designs for clinical trials with delayed response},
	Volume = {30},
	Year = {2002}}

@article{Andersen&Faries&Tamura94,
	Author = {J. Andersen and D. Faries and R. Tamura},
	Journal = {Communication in Statistical Theory},
	Pages = {309--323},
	Title = {A randomized play-the-winner design for multiarm clinical trials},
	Volume = {23},
	Year = {1994}}

@book{Flournoy&Rosenberger95,
	Author = {N. Flournoy and W.F. Rosenberger},
	Publisher = {Hayward, Institute of Mathematical Statistics},
	Title = {Adaptive Designs},
	Year = {1995}}

@article{Hu&Rosenberger00,
	Author = {F. Hu and W.F. Rosenberger},
	Journal = {Statistics in Medicine},
	Pages = {2067--2075},
	Title = {Analysis of time trends in adaptive designs withi appliation to a neurophysiology experiment},
	Volume = {19},
	Year = {2000}}

@article{Rosenberger96,
	Author = {W.F. Rosenberger},
	Journal = {Statistical Science},
	Pages = {137--149},
	Title = {New directions in adaptive designs},
	Volume = {11},
	Year = {1996}}

@article{Rosenberger&Flournoy&Durham97,
	Author = {W.F. Rosenberger and N. Flournoy and S.D. Durham},
	Journal = {Journal of Statistical Planning and Inference},
	Pages = {69--76},
	Title = {Asymptotic normality of maximum likelihood estimators from multiparameter response driven designs},
	Year = {1997}}

@article{Rosenberger&Grill97,
	Author = {W.F. Rosenberger and S.E. Grill},
	Journal = {Statistics in Medicine},
	Pages = {2245--2260},
	Title = {A sequential design for psychophysical experiments: An application to estimating timing of sensory events},
	Volume = {16},
	Year = {1997}}

@article{Rosenberger&Sriram97,
	Author = {W.F. Rosenberger and T.N. Shiram},
	Journal = {Journal of Statistical Planning and Inference},
	Pages = {309--319},
	Title = {Estimation for an adaptive allocation design},
	Volume = {59},
	Year = {1997}}

@article{Tamuraetal94,
	Author = {R.N. Tamura and D.E. Faries and J.S. Andersen and J.H. Heiligenstein},
	Journal = {Journal of the American Statistical Association},
	Pages = {768--776},
	Title = {A case study of an adaptive clinical trial in the treatment of out-patients with depressive disorder},
	Volume = {89},
	Year = {1994}}

@article{Wei&Durham78,
	Author = {L.J. Wei and S. Durham},
	Journal = {Journal of the American Statistical Association},
	Pages = {840--843},
	Title = {The randomize play-the-winner rule in medical trials},
	Volume = {73},
	Year = {1978}}

@article{Weietal90,
	Author = {L.J. Wei and R.T. Smythe and D.Y. Lin and T.S. Park},
	Journal = {Journal of the American Statistical Association},
	Pages = {156--162},
	Title = {Statistical Inference with data-dependent treatment allocation rules},
	Volume = {85},
	Year = {1990}}

@article{Zelen69,
	Author = {M. Zelen},
	Journal = {Journal of the American Statistical Association},
	Pages = {131--146},
	Title = {Play the winner rule and the controlled clinical trial},
	Volume = {64},
	Year = {1969}}

@article{Cheng&Shen05,
	Author = {Y. Cheng and Y. Shen},
	Journal = {Biometrika},
	Number = {3},
	Pages = {633--646},
	Title = {Bayesian adaptive designs for clinical trials},
	Volume = {92},
	Year = {2005}}

@article{Wei79,
	Author = {L.J. Wei},
	Journal = {The Annals of Statistics},
	Pages = {291--296},
	Title = {The generalized Polya's urn design for sequential medical trials},
	Volume = {7},
	Year = {1979}}

@article{Benito&Lopez&Soriano03,
	Author = {Benito, J. M. and Lopez, M. and Soriano, V.},
	Journal = {J Infect Dis},
	Keywords = {ADP-ribosyl Cyclase/metabolism Anti-HIV Agents/therapeutic use Antigens, CD/metabolism CD4-Positive T-Lymphocytes/*immunology CD8-Positive T-Lymphocytes/immunology HIV Infections/drug therapy/*immunology/virology HIV-1/*physiology Human *Viral Load Virus Replication},
	Note = {0022-1899 Comment Letter},
	Number = {5},
	Pages = {794-5; author reply 795-6},
	Title = {Virus load and cytolitic responses in human immunodeficiency virus infection: what is cause and what is effect},
	Volume = {188},
	Year = {2003}}

@article{DEttorreetal02,
	Abstract = {OBJECTIVE: To study virologic and immunologic factors associated with discordant treatment response in HIV-infected patients receiving highly active antiretroviral therapy (HAART). DESIGN: Study participants included a total of 27 patients: (a) 10 discordant patients (mean CD4+ cell count, 396.1 x 10 cells/l; mean HIV-RNA, 5.4 log copies/ml); (b) seven responder patients (mean CD4+ cell count, 997.5 x 10 cells/l); and (c) 10 failing patients (mean CD4+ cell count 66.5 x 10 cells/l; mean HIV-RNA, 5.4 log copies/ml).(10) (10)METHODS: The HIV-1 isolation rate and biological phenotype, drug resistance genotypic mutations of HIV-1 strains, recall and HIV-1-specific antigen lymphocyte proliferation (LP), and interleukin (IL)-15 production were studied. RESULTS: Virus isolation was obtained in 30% of discordant patients, and in 100% of failing patients. A higher replication constant was reported in discordant patients. No difference in the number of drug resistance mutations and biological phenotypes of HIV-1 was found in discordant patients with respect to failing patients. Discordant patients developed positive LP responses to and HIV-1 p24. LP in response to, HIV-1 p24 and gp160 was positive in responder patients. No significant LP was found in failing patients. Increased levels of IL-15 after stimulation with lipopolysaccaride (LPS) and were found in both discordant patients and responder patients. Conversely, a strong reduction of IL-15 levels was observed in failing patients. CONCLUSION: The present results suggest that decreased virus isolation rate, restoration of both lymphocyte proliferation and IL-15 production are factors involved in the discordant antiretroviral therapy response of HIV-infected patients.},
	Author = {D'Ettorre, G. and Forcina, G. and Andreotti, M. and Sarmati, L. and Palmisano, L. and Galluzzo, C. M. and Nicastri, E. and Mastroianni, C. M. and Vullo, V. and Vella, S. and Andreoni, M.},
	Journal = {Aids},
	Keywords = {Adult Anti-HIV Agents/*therapeutic use Antiretroviral Therapy, Highly Active CD4 Lymphocyte Count CD8-Positive T-Lymphocytes/drug effects/immunology Candida albicans Drug Resistance, Viral Female HIV Infections/complications/*drug therapy/immunology/virology HIV-1/drug effects/genetics/*immunology/isolation & purification Human Interleukin-15/*blood Male Middle Aged Mutation Viral Load Virus Replication/drug effects},
	Note = {0269-9370 Journal Article},
	Number = {14},
	Pages = {1877-85},
	Title = {Discordant response to antiretroviral therapy: {HIV} isolation, genotypic mutations, T-cell proliferation and cytokine production},
	Volume = {16},
	Year = {2002}}

@article{Davenportetal02,
	Abstract = {Early infection with HIV-1 is dominated by CCR5-tropic (R5, non-syncytium-inducing) viruses. The evolution of CXCR4-tropic (X4, syncytium-inducing) viruses occurs later in the infection and is associated with rapid disease progression. Here, we propose that the tropism of X4 viruses for naive CD4+ T cells is disadvantageous in early infection owing to the low division rate of these cells. In healthy individuals, the division rate of memory cells is nearly ten times higher than that of naive cells and thus the memory-cell tropism of R5 viruses could account for their dominance early in infection. As the division rate of naive T cells increases with CD4+ depletion, X4 viruses come to dominate in late disease.},
	Author = {Davenport, M. P. and Zaunders, J. J. and Hazenberg, M. D. and Schuitemaker, H. and van Rij, R. P.},
	Journal = {Trends Microbiol},
	Keywords = {CD4-Positive T-Lymphocytes/*virology HIV Infections/*immunology/metabolism HIV-1/*pathogenicity Human Immunologic Memory Macrophages/*virology Models, Biological Receptors, CCR5/metabolism Receptors, CXCR4/metabolism Tropism},
	Note = {0966-842x Journal Article},
	Number = {6},
	Pages = {275-8},
	Title = {Cell turnover and cell tropism in HIV-1 infection},
	Volume = {10},
	Year = {2002}}

@article{Deeksetal00,
	Abstract = {The relationship between plasma human immunodeficiency virus (HIV) RNA levels and peripheral CD4+ T cell counts was examined in 380 HIV-infected adults receiving long-term protease inhibitor therapy. Patients experiencing virologic failure (persistent HIV RNA >500 copies RNA/mL) generally had CD4+ T cell counts that remained greater than pretherapy baseline levels, at least through 96 weeks of follow-up. The CD4+ T cell response was directly and independently related to degree of viral suppression below the pretreatment baseline. For any given HIV RNA level measured 12 weeks after virologic failure, subsequent CD4+ T cell decline was slower in patients receiving a protease inhibitor-based regimen than in a historical control group of untreated patients. These observations suggest that transient or partial declines in plasma HIV RNA levels can have sustained effects on CD4+ T cell levels.},
	Author = {Deeks, S. G. and Barbour, J. D. and Martin, J. N. and Swanson, M. S. and Grant, R. M.},
	Journal = {J Infect Dis},
	Keywords = {Adult *CD4 Lymphocyte Count Female HIV Infections/*drug therapy/immunology/virology HIV Protease Inhibitors/*therapeutic use Human Male RNA, Viral/*blood Support, Non-U.S. Gov't Support, U.S. Gov't, P.H.S.},
	Note = {0022-1899 Journal Article},
	Number = {3},
	Pages = {946-53},
	Title = {Sustained CD4+ T cell response after virologic failure of protease inhibitor-based regimens in patients with human immunodeficiency virus infection},
	Volume = {181},
	Year = {2000}}

@article{Deeksetal01,
	Abstract = {BACKGROUND: In many patients with human immunodeficiency virus (HIV) infection, therapy with potent antiretroviral drugs does not result in complete suppression of HIV replication. The effect of cessation of therapy in these patients is unknown. METHODS: Sixteen patients who had a plasma HIV RNA level of more than 2500 copies per milliliter during combination antiretroviral-drug therapy were randomly assigned, in a 2:1 ratio, to discontinue or continue therapy. Plasma HIV RNA levels, CD4 cell counts, and drug susceptibility were measured weekly. Viral replicative capacity was measured at base line and at week 12. RESULTS: Discontinuation of therapy for 12 weeks was associated with a median decrease in the CD4 cell count of 128 cells per cubic millimeter and an increase in the plasma HIV RNA level of 0.84 log copies per milliliter. Virus from all patients with detectable resistance at entry became susceptible to HIV-protease inhibitors within 16 weeks after the discontinuation of therapy. Drug susceptibility began to increase a median of six weeks after the discontinuation of therapy and was temporally associated with increases in plasma HIV RNA levels and decreases in CD4 cell counts. Viral replicative capacity, measured by means of a recombinant-virus assay, was low at entry into the study and increased after therapy was discontinued. Despite the loss of detectable resistance in plasma, resistant virus was cultured from peripheral-blood mononuclear cells in five of nine patients who could be evaluated. Plasma HIV RNA levels, CD4 cell counts, and drug susceptibility remained stable in the patients who continued therapy. CONCLUSIONS: Despite the presence of reduced drug susceptibility, antiretroviral-drug therapy can provide immunologic and virologic benefit. This benefit reflects continued antiviral-drug activity and the maintenance of a viral population with a reduced replicative capacity.},
	Author = {Deeks, S. G. and Wrin, T. and Liegler, T. and Hoh, R. and Hayden, M. and Barbour, J. D. and Hellmann, N. S. and Petropoulos, C. J. and McCune, J. M. and Hellerstein, M. K. and Grant, R. M.},
	Journal = {N Engl J Med},
	Keywords = {Adult Anti-HIV Agents/pharmacology/*therapeutic use CD4 Lymphocyte Count Drug Resistance, Microbial Drug Therapy, Combination HIV Infections/*drug therapy/immunology/virology HIV Protease Inhibitors/pharmacology/*therapeutic use HIV-1/*drug effects/genetics/isolation & purification Human Male Middle Aged Proportional Hazards Models Prospective Studies RNA, Viral/blood Support, Non-U.S. Gov't Support, U.S. Gov't, P.H.S. Viremia/drug therapy},
	Note = {0028-4793 Clinical Trial Journal Article Randomized Controlled Trial},
	Number = {7},
	Pages = {472-80},
	Title = {Virologic and immunologic consequences of discontinuing combination antiretroviral-drug therapy in HIV-infected patients with detectable viremia},
	Volume = {344},
	Year = {2001}}

@article{Deeks01,
	Abstract = {Although understanding of nonnucleoside reverse transcriptase inhibitor (NNRTI) resistance is less clearly established than that of other classes of antiretroviral drugs, certain facts have been established. The treatment-associated genetic mutation profiles of the available NNRTIs have been mapped, and resistance has been found to develop rapidly after initiation of NNRTI therapy. Despite the chemical diversity of the NNRTIs, cross-resistance among agents of this class is nearly universal. Although the viral replicative capacity (``fitness") of NNRTI-induced viral variants has not been extensively studied, available data suggest that NNRTI-selected mutations confer little damage to viral fitness, and thus a single point mutation produces a strain that is both resistant and fit. Furthermore, with continued therapy, viral evolution persists, creating species with greater numbers of mutations and higher level phenotypic resistance. Taken together, these facts suggest that continued use of NNRTIs after emergence of resistance will produce variants of complex mutational patterns that limit future treatment options, and, therefore, strong consideration should be given to discontinuing NNRTIs after virologic failure is confirmed. This article describes the scientific literature establishing the efficacy and limitations of NNRTI therapy and attempts to define a role for this class of drug in the long-term treatment of HIV-1 disease.},
	Author = {Deeks, S. G.},
	Journal = {J Acquir Immune Defic Syndr},
	Keywords = {Anti-HIV Agents/*pharmacology/therapeutic use Clinical Trials Delavirdine/pharmacology/therapeutic use *Drug Resistance, Microbial Drug Therapy, Combination HIV Infections/drug therapy/transmission HIV-1/*drug effects/genetics/metabolism HIV-1 Reverse Transcriptase/chemistry/genetics Human Nevirapine/pharmacology/therapeutic use Oxazines/pharmacology/therapeutic use Phylogeny Point Mutation/drug effects Protein Conformation Reverse Transcriptase Inhibitors/*pharmacology/therapeutic use Virus Replication/drug effects},
	Note = {1525-4135 Journal Article Review Review, Tutorial},
	Pages = {S25-33},
	Title = {International perspectives on antiretroviral resistance. Nonnucleoside reverse transcriptase inhibitor resistance},
	Volume = {26 Suppl 1},
	Year = {2001}}

@article{Deeksetal02,
	Abstract = {BACKGROUND: Sustained elevations in CD4 cell counts commonly occur despite incomplete viral suppression with protease inhibitor-based antiretroviral therapy. OBJECTIVES: To determine the incidence and risk factors associated with return of CD4 cell count to pre-therapy levels in patients experiencing virologic failure of protease inhibitor therapy. DESIGN: This is a clinic-based cohort study of HIV-infected adults who failed to maintain durable viral suppression on a protease inhibitor-based regimen. MAIN OUTCOME MEASURES: Virologic failure was defined as persistent plasma HIV RNA level > 500 copies/ml. Immunologic failure was defined as return of CD4 cell count to pre-therapy levels. RESULTS: A total of 291 patients experienced virologic failure on a protease inhibitor-based regimen and had a treatment-mediated CD4 cell increase above pre-therapy levels at the time of virologic failure. If patient data were censored at the time a successful salvage regimen was initiated, then the median time to immunologic failure after the onset of virologic failure was 3 years. If patient data were also censored at the time therapy was discontinued, then 36.8% of the cohort experienced immunologic failure after 3 years of continuous virologic failure. The change in viral load from a pre-treatment baseline, and not the absolute level of viremia achieved, was a strong and independent predictor of immunologic failure. Discontinuing therapy was associated with immunologic failure independent of viral load changes. CONCLUSION: Reduction in T CD4+ cell numbers may eventually occur during prolonged virologic failure of a protease inhibitor-based regimen and is predicted by the degree of virologic suppression below a pre-therapy 'set-point'.},
	Author = {Deeks, S. G. and Barbour, J. D. and Grant, R. M. and Martin, J. N.},
	Journal = {Aids},
	Keywords = {Adult Antiretroviral Therapy, Highly Active CD4 Lymphocyte Count CD4-Positive T-Lymphocytes/cytology/*drug effects Disease Progression HIV Infections/blood/*drug therapy/immunology/virology HIV Protease Inhibitors/*therapeutic use HIV-1/*drug effects/genetics Human Indinavir/therapeutic use Nelfinavir/therapeutic use RNA, Viral/blood Ritonavir/therapeutic use Saquinavir/therapeutic use Support, Non-U.S. Gov't Support, U.S. Gov't, P.H.S. Time Factors Treatment Failure Viremia/blood/*drug therapy/immunology/virology},
	Note = {0269-9370 Journal Article},
	Number = {2},
	Pages = {201-7},
	Title = {Duration and predictors of CD4 T-cell gains in patients who continue combination therapy despite detectable plasma viremia},
	Volume = {16},
	Year = {2002}}

@article{Deeks03,
	Abstract = {Drug-resistant HIV-1 is a cause of growing clinical and public-health concern. In many patients, combination antiretroviral therapy fails to achieve complete viral suppression (virological failure). Continuing viral replication during therapy leads to the accumulation of drug-resistance mutations, resulting in increased viral load and a greater risk of disease progression. Patients with drug-resistant HIV-1 infection have three therapeutic options: a change to a salvage regimen with the aim of fully suppressing viral replication; interruption of therapy; or continuation of a partially effective regimen. The first strategy is preferred for most patients failing their first or perhaps their second regimen. However, the best approach remains unclear for patients who have failed multiple treatment regimens and who have limited options for complete viral suppression. The management of such patients requires a careful understanding of the pathogenesis of drug-resistant HIV-1, the clinical consequences of virological failure, the potential benefits and limitations of diagnostic assays, and the likelihood that agents in development will be effective.},
	Author = {Deeks, S. G.},
	Journal = {Lancet},
	Keywords = {Anti-HIV Agents/*immunology/*therapeutic use Antiretroviral Therapy, Highly Active/methods Drug Resistance, Viral/genetics/immunology Drug Therapy, Combination HIV Infections/*drug therapy/immunology/virology HIV Protease Inhibitors/immunology/therapeutic use *HIV-1/drug effects/genetics/immunology Human Randomized Controlled Trials Ritonavir/immunology/therapeutic use Support, Non-U.S. Gov't Support, U.S. Gov't, P.H.S. Treatment Outcome Viral Load/statistics & numerical data Virus Replication/drug effects/immunology},
	Note = {1474-547x Journal Article Review Review, Academic},
	Number = {9400},
	Pages = {2002-11},
	Title = {Treatment of antiretroviral-drug-resistant HIV-1 infection},
	Volume = {362},
	Year = {2003}}

@article{Deeks&Walker04,
	Abstract = {A potent antigen-specific T cell response to HIV infection can contribute to the control of viral replication and is therefore beneficial to the host. However, HIV-mediated increases in generalized T cell activation also appear to accelerate both viral replication and CD4+ T cell depletion. A new study in the JCI attempts to experimentally distinguish the beneficial versus harmful aspects of this immune response.},
	Author = {Deeks, S. G. and Walker, B. D.},
	Journal = {J Clin Invest},
	Note = {0021-9738 Comment Journal Article},
	Number = {6},
	Pages = {808-10},
	Title = {The immune response to AIDS virus infection: good, bad, or both?},
	Volume = {113},
	Year = {2004}}

@techreport{DHHS04,
	Author = {DHHS},
	Institution = {Panel on Clinical Practices for Treatment of HIV Infection, Department of Health and Human Services},
	Month = {March 23},
	Title = {Guidelines for the use of antiretroviral agents in HIV-1 infected adults and adolescents},
	Year = {2004}}

@article{Faureetal00,
	Abstract = {Human immunodeficiency virus (HIV) enters cells in vitro via CD4 and a coreceptor. Which of 15 known coreceptors are important in vivo is poorly defined but may be inferred from disease-modifying mutations, as for CCR5. Here two single nucleotide polymorphisms are described in Caucasians in CX3CR1, an HIV coreceptor and leukocyte chemotactic/adhesion receptor for the chemokine fractalkine. HIV-infected patients homozygous for CX3CR1-I249 M280, a variant haplotype affecting two amino acids (isoleucine-249 and methionine-280), progressed to AIDS more rapidly than those with other haplotypes. Functional CX3CR1 analysis showed that fractalkine binding is reduced among patients homozygous for this particular haplotype. Thus, CX3CR1-I249 M280 is a recessive genetic risk factor in HIV/AIDS.},
	Author = {Faure, S. and Meyer, L. and Costagliola, D. and Vaneensberghe, C. and Genin, E. and Autran, B. and Delfraissy, J. F. and McDermott, D. H. and Murphy, P. M. and Debre, P. and Theodorou, I. and Combadiere, C.},
	Journal = {Science},
	Keywords = {Acquired Immunodeficiency Syndrome/genetics/*physiopathology/virology Case-Control Studies *Chemokines, CX3C Chemokines, CXC/metabolism Chromosomes, Human, Pair 3 Cohort Studies Disease Progression European Continental Ancestry Group/genetics Genotype HIV/physiology HIV Infections/genetics/*physiopathology/virology Haplotypes Homozygote Human Leukocytes, Mononuclear/metabolism Linkage Disequilibrium Membrane Proteins/metabolism Mutation Polymorphism, Restriction Fragment Length *Polymorphism, Single Nucleotide Polymorphism, Single-Stranded Conformational Receptors, Cytokine/*genetics/*physiology Receptors, HIV/*genetics/*physiology Support, Non-U.S. Gov't Survival Analysis Variation (Genetics)},
	Note = {0036-8075 Comment Journal Article},
	Number = {5461},
	Pages = {2274-7},
	Title = {Rapid progression to AIDS in HIV+ individuals with a structural variant of the chemokine receptor CX3CR1},
	Volume = {287},
	Year = {2000}}

@article{Gaoetal01,
	Abstract = {BACKGROUND: From studies of genetic polymorphisms and the rate of progression from human immunodeficiency virus type 1 (HIV-1) infection to the acquired immunodeficiency syndrome (AIDS), it appears that the strongest susceptibility is conferred by the major-histocompatibility-complex (MHC) class I type HLA-B*35,Cw*04 allele. However, cytotoxic T-lymphocyte responses have been observed against HIV-1 epitopes presented by HLA-B*3501, the most common HLA-B*35 subtype. We examined subtypes of HLA-B*35 in five cohorts and analyzed the relation of structural differences between HLA-B*35 subtypes to the risk of progression to AIDS. METHODS: Genotyping of HLA class I loci was performed for 850 patients who seroconverted and had known dates of HIV-1 infection. Survival analyses with respect to the rate of progression to AIDS were performed to identify the effects of closely related HLA-B*35 subtypes with different peptide-binding specificities. RESULTS: HLA-B*35 subtypes were divided into two groups according to peptide-binding specificity: the HLA-B*35-PY group, which consists primarily of HLA-B*3501 and binds epitopes with proline in position 2 and tyrosine in position 9; and the more broadly reactive HLA-B*35-Px group, which also binds epitopes with proline in position 2 but can bind several different amino acids (not including tyrosine) in position 9. The influence of HLA-B*35 in accelerating progression to AIDS was completely attributable to HLA-B*35-Px alleles, some of which differ from HLA-B*35-PY alleles by only one amino acid residue. CONCLUSIONS: This analysis shows that, in patients with HIV-1 infection, a single amino acid change in HLA molecules has a substantial effect on the rate of progression to AIDS. The different consequences of HLA-B*35-PY and HLA-B*35-Px in terms of disease progression highlight the importance of the epitope specificities of closely related class I molecules in the immune defense against HIV-1.},
	Author = {Gao, X. and Nelson, G. W. and Karacki, P. and Martin, M. P. and Phair, J. and Kaslow, R. and Goedert, J. J. and Buchbinder, S. and Hoots, K. and Vlahov, D. and O'Brien, S. J. and Carrington, M.},
	Journal = {N Engl J Med},
	Keywords = {Acquired Immunodeficiency Syndrome/*genetics African Continental Ancestry Group/genetics Alleles Amino Acid Sequence Binding Sites/genetics Disease Progression Disease-Free Survival European Continental Ancestry Group/genetics *Genes, MHC Class I Genotype HIV Infections/ethnology/*genetics/immunology HLA-B35 Antigen/chemistry/*genetics HLA-C Antigens Human Peptides/metabolism Proportional Hazards Models Receptors, Peptide/chemistry/genetics/metabolism Support, U.S. Gov't, P.H.S.},
	Note = {0028-4793 Journal Article Multicenter Study},
	Number = {22},
	Pages = {1668-75},
	Title = {Effect of a single amino acid change in MHC class I molecules on the rate of progression to AIDS},
	Volume = {344},
	Year = {2001}}

@article{Grabaretal00,
	Abstract = {BACKGROUND: The prognostic value of discordant immunologic (CD4 cell increase) and virologic (plasma HIV RNA level decrease) responses to antiretroviral treatment is not known. OBJECTIVE: To study the relation between clinical outcome of HIV-infected patients receiving highly active antiretroviral therapy (HAART) and early immunologic and virologic responses to such therapy. DESIGN: Prospective cohort study. SETTING: 68 hospitals in France. PATIENTS: 2236 protease inhibitor-naive patients. INTERVENTION: Initiation of HAART with one protease inhibitor and two nucleoside analogues between July 1996 and March 1997. MEASUREMENTS: Immunologic and virologic response at 6 months. Multivariate Cox models were used to assess the relation between these responses and progression to a new AIDS-defining event or death. RESULTS: On the basis of 6-month immunologic and virologic responses, patients were classified into four groups: complete response (47.5%), complete nonresponse (16.2%), immunologic response only (19.0%), and virologic response only (17.3%). After month 6 and within a median of 18 months, 69 patients died and 123 experienced a new AIDS-defining event. After adjustment, complete nonresponders and those with only a virologic response had significantly higher risks for clinical progression at 6 months (relative risk, 3.38 [95% CI, 2.28 to 5.02] and 1.98 [CI, 1.26 to 3.10], respectively) than complete responders. The difference between complete responders and those with only an immunologic response at 6 months was weaker and nonsignificant (relative risk, 1.55 [CI, 0.96 to 2.50]). CONCLUSIONS: Immunologic response after 6 months of HAART indicates a favorable clinical outcome in HIV-infected patients regardless of virologic response. This suggests that both immunologic and virologic markers should be used in clinical practice to evaluate treatment response.},
	Author = {Grabar, S. and Le Moing, V. and Goujard, C. and Leport, C. and Kazatchkine, M. D. and Costagliola, D. and Weiss, L.},
	Journal = {Ann Intern Med},
	Keywords = {Adult CD4 Lymphocyte Count Disease Progression Drug Therapy, Combination Female HIV Infections/*drug therapy/immunology/virology HIV Protease Inhibitors/*therapeutic use *HIV-1/genetics Human Male Multivariate Analysis Proportional Hazards Models Prospective Studies RNA, Viral/blood Reverse Transcriptase Inhibitors/*therapeutic use Support, Non-U.S. Gov't Treatment Outcome Viral Load},
	Note = {0003-4819 Journal Article Multicenter Study},
	Number = {6},
	Pages = {401-10},
	Title = {Clinical outcome of patients with HIV-1 infection according to immunologic and virologic response after 6 months of highly active antiretroviral therapy},
	Volume = {133},
	Year = {2000}}

@article{Gruebetal00,
	Abstract = {BACKGROUND: Hepatitis C virus (HCV) infection is highly prevalent among HIV-1-infected individuals, but its contribution to the morbidity and mortality of coinfected patients who receive potent antiretroviral therapy is controversial. We used data from the ongoing Swiss HIV Cohort Study to analyse clinical progression of HIV-1, and the virological and immunological response to potent antiretroviral therapy in HIV-1-infected patients with or without concurrent HCV infection. METHODS: We analysed prospective data on survival, clinical disease progression, suppression of HIV-1 replication, CD4-cell recovery, and frequency of changes in antiretroviral therapy according to HCV status in 3111 patients starting potent antiretroviral therapy. RESULTS: 1157 patients (37.2%) were coinfected with HCV, 1015 of whom (87.7%) had a history of intravenous drug use. In multivariate Cox's regression, the probability of progression to a new AIDS-defining clinical event or to death was independently associated with HCV seropositivity (hazard ratio 1.7 [95% CI 1.26-2.30]), and with active intravenous drug use (1.38 [1.02-1.88]). Virological response to antiretroviral therapy and the probability of treatment change were not associated with HCV serostatus. In contrast, HCV seropositivity was associated with a smaller CD4-cell recovery (hazard ratio for a CD4-cell count increase of at least 50 cells/microL=0.79 [0.72-0.87]). INTERPRETATION: HCV and active intravenous drug use could be important factors in the morbidity and mortality among HIV-1-infected patients, possibly through impaired CD4-cell recovery in HCV seropositive patients receiving potent antiretroviral therapy. These findings are relevant for decisions about optimum timing for HCV treatment in the setting of HIV infection.},
	Author = {Greub, G. and Ledergerber, B. and Battegay, M. and Grob, P. and Perrin, L. and Furrer, H. and Burgisser, P. and Erb, P. and Boggian, K. and Piffaretti, J. C. and Hirschel, B. and Janin, P. and Francioli, P. and Flepp, M. and Telenti, A.},
	Journal = {Lancet},
	Keywords = {AIDS-Related Opportunistic Infections/*drug therapy Adolescent Adult Anti-HIV Agents/*therapeutic use CD4 Lymphocyte Count Cohort Studies Disease Progression Female Hepatitis C/complications/*drug therapy Human Male Middle Aged Prospective Studies Support, Non-U.S. Gov't Survival Analysis Switzerland Viral Load Viremia/etiology},
	Note = {0140-6736 Clinical Trial Journal Article},
	Number = {9244},
	Pages = {1800-5},
	Title = {Clinical progression, survival, and immune recovery during antiretroviral therapy in patients with HIV-1 and hepatitis C virus coinfection: the Swiss HIV Cohort Study},
	Volume = {356},
	Year = {2000}}

@article{Katzensteinetal96,
	Abstract = {BACKGROUND: We studied measures of human immunodeficiency virus (HIV) replication, the viral phenotype, and immune function (CD4 cell counts) and the relation of changes in these indicators to clinical outcomes in a subgroup of patients in a controlled trial of early antiretroviral treatment for HIV, the AIDS Clinical Trials Group Study 175. METHODS: The 391 subjects, each of whom entered the study with a single screening CD4 cell count of 200 to 500 per cubic millimeter, were randomly assigned to receive zidovudine alone, didanosine alone, zidovudine plus didanosine, or zidovudine plus zalcitabine. Plasma concentrations of HIV RNA were assessed in 366 subjects, and viral isolates from 332 subjects were assayed for the presence of the syncytium-inducing phenotype. RESULTS: After eight weeks, the mean (+/-SE) decrease from base line in the concentration of HIV RNA, expressed as the change in the base 10 log of the number of copies per milliliter, was 0.26+/-0.06 for patients treated with zidovudine alone, 0.65+/-0.07 for didanosine alone, 0.93+/-0.10 for zidovudine plus didanosine, and 0.89+/-0.06 for zidovudine plus zalcitabine (P<0.001 for each of the pairwise comparisons with zidovudine alone). Multivariate proportional-hazards models showed that higher base-line concentrations of plasma HIV RNA, less suppression of plasma HIV RNA by treatment, and the presence of the syncytium-inducing phenotype were significantly associated with an increased risk of progression to the acquired immunodeficiency syndrome and death. After adjustment for these measures of viral replication and for the viral phenotype, CD4 cell counts were not significant predictors of clinical outcome. CONCLUSIONS: Both the risk of the progression of HIV disease and the efficacy of antiretroviral therapy are strongly associated with the plasma level of HIV RNA and with the viral phenotype. The changes in the plasma concentration of HIV RNA predict the changes in CD4 cell counts and survival after treatment with reverse-transcriptase inhibitors.},
	Author = {Katzenstein, D. A. and Hammer, S. M. and Hughes, M. D. and Gundacker, H. and Jackson, J. B. and Fiscus, S. and Rasheed, S. and Elbeik, T. and Reichman, R. and Japour, A. and Merigan, T. C. and Hirsch, M. S.},
	Journal = {N Engl J Med},
	Keywords = {Adult Antiviral Agents/*therapeutic use CD4 Lymphocyte Count Didanosine/*therapeutic use Disease Progression Drug Therapy, Combination Female HIV/*genetics/isolation & purification/physiology HIV Infections/drug therapy/immunology/*virology Human Male Middle Aged Multivariate Analysis Phenotype Proportional Hazards Models RNA, Viral/*blood Support, U.S. Gov't, P.H.S. Treatment Outcome Virus Replication/drug effects Zidovudine/*therapeutic use},
	Note = {0028-4793 Clinical Trial Journal Article Multicenter Study Randomized Controlled Trial},
	Number = {15},
	Pages = {1091-8},
	Title = {The relation of virologic and immunologic markers to clinical outcomes after nucleoside therapy in HIV-infected adults with 200 to 500 CD4 cells per cubic millimeter. AIDS Clinical Trials Group Study 175 Virology Study Team},
	Volume = {335},
	Year = {1996}}

@article{Kaufmannetal98,
	Author = {Kaufmann, D. and Pantaleo, G. and Sudre, P. and Telenti, A.},
	Journal = {Lancet},
	Keywords = {Anti-HIV Agents/*therapeutic use CD4 Lymphocyte Count HIV Infections/drug therapy/*immunology Human Protease Inhibitors/*therapeutic use Support, Non-U.S. Gov't Viremia/drug therapy/*immunology},
	Note = {0140-6736 Letter},
	Number = {9104},
	Pages = {723-4},
	Title = {CD4-cell count in HIV-1-infected individuals remaining viraemic with highly active antiretroviral therapy (HAART). Swiss HIV Cohort Study},
	Volume = {351},
	Year = {1998}}

@article{Kaufmannetal03,
	Abstract = {BACKGROUND: Highly active antiretroviral therapy (HAART) for human immunodeficiency virus (HIV)-1 infection allows recovery of CD4 T lymphocytes. Few studies have explored the long-term T-lymphocyte responses to HAART. METHODS: Plasma HIV-1 RNA levels and CD4 and CD8 T-lymphocyte counts were longitudinally analyzed over 4 years in 2235 participants of the Swiss HIV Cohort, commencing HAART between 1996 and 1997. The CD4 T-lymphocyte count increase, the percentage of individuals with a CD4 T-lymphocyte count of 500/microL or greater and less than 200/microL, and the determinants of CD4 T-lymphocyte recovery were evaluated in individuals treated with continuous (CONT; n = 985) and discontinuous (DISCONT; n = 1250) HAART. RESULTS: At 4 years, 69.5% of subjects (CONT, 84.5%; DISCONT, 53.6%; P<.001) showed HIV-1 RNA levels below 400 copies/mL, while the median CD4 T-lymphocyte count increased from 190/microL to 423/microL (CONT, 486/microL; DISCONT, 343/microL; P<.001). Of the 2235 participants, 38.8% (CONT, 47.7%; DISCONT, 29.4%; P<.001) reached a CD4 T-lymphocyte count of 500/microL or greater, but in 15.6%, CD4 T-lymphocyte count remained below 200/microL (CONT, 5.9%; DISCONT, 25.9%; P<.001). Larger increases in CD4 T-lymphocyte count were associated with higher baseline HIV-1 RNA, a larger percentage of undetectable HIV-1 RNA levels, lower baseline CD8 T-lymphocyte count, and younger age. Individuals reaching a CD4 T-lymphocyte count of 500/microL or greater at 4 years were characterized by higher nadir and baseline CD4 T-lymphocyte counts and a more sustained reduction of HIV-1 RNA levels. CONCLUSIONS: At 4 years, only 39% of individuals treated with HAART reached a CD4 T-lymphocyte count of 500/microL or greater, and 16% with CD4 T-lymphocyte counts less than 200/microL remained susceptible to opportunistic infections. Treatment interruptions, a poor virologic response, and older age were the major factors negatively affecting the recovery of CD4 T lymphocytes.},
	Author = {Kaufmann, G. R. and Perrin, L. and Pantaleo, G. and Opravil, M. and Furrer, H. and Telenti, A. and Hirschel, B. and Ledergerber, B. and Vernazza, P. and Bernasconi, E. and Rickenbach, M. and Egger, M. and Battegay, M.},
	Journal = {Arch Intern Med},
	Keywords = {Adult *Antiretroviral Therapy, Highly Active *CD4 Lymphocyte Count CD8-Positive T-Lymphocytes Female HIV Infections/*drug therapy/*immunology *Hiv-1 Human Lymphocyte Count Male Middle Aged Prospective Studies RNA, Viral/*analysis Support, Non-U.S. Gov't Viral Load},
	Note = {0003-9926 Journal Article},
	Number = {18},
	Pages = {2187-95},
	Title = {CD4 T-lymphocyte recovery in individuals with advanced HIV-1 infection receiving potent antiretroviral therapy for 4 years: the Swiss HIV Cohort Study},
	Volume = {163},
	Year = {2003}}

@article{MartinezPicadoetal99,
	Abstract = {The relative replicative fitness of human immunodeficiency virus type 1 (HIV-1) mutants selected by different protease inhibitors (PIs) in vivo was determined. Each mutant was compared to wild type (WT), NL4-3, in the absence of drugs by several methods, including clonal genotyping of cultures infected with two competing viral variants, kinetics of viral antigen production, and viral infectivity/virion particle ratios. A nelfinavir-selected protease D30N substitution substantially decreased replicative capacity relative to WT, while a saquinavir-selected L90M substitution moderately decreased fitness. The D30N mutant virus was also outcompeted by the L90M mutant in the absence of drugs. A major natural polymorphism of the HIV-1 protease, L63P, compensated well for the impairment of fitness caused by L90M but only slightly improved the fitness of D30N. Multiply substituted indinavir-selected mutants M46I/L63P/V82T/I84V and L10R/M46I/L63P/V82T/I84V were just as fit as WT. These results indicate that the mutations which are usually initially selected by nelfinavir and saquinavir, D30N and L90M, respectively, impair fitness. However, additional mutations may improve the replicative capacity of these and other drug-resistant mutants. Hypotheses based on the greater fitness impairment of the nelfinavir-selected D30N mutant are suggested to explain observations that prolonged responses to delayed salvage regimens, including alternate PIs, may be relatively common after nelfinavir failure.},
	Author = {Martinez-Picado, J. and Savara, A. V. and Sutton, L. and D'Aquila, R. T.},
	Journal = {J Virol},
	Keywords = {Adaptation, Biological Amino Acid Substitution Animals Anti-HIV Agents/*pharmacology Cells, Cultured Drug Resistance, Microbial HIV Protease Inhibitors/*pharmacology HIV-1/*drug effects/genetics/physiology Human Mice Mutagenesis, Site-Directed Nelfinavir/*pharmacology Saquinavir/*pharmacology Support, Non-U.S. Gov't Support, U.S. Gov't, P.H.S. Tumor Cells, Cultured Virus Replication/*drug effects},
	Note = {0022-538x Journal Article},
	Number = {5},
	Pages = {3744-52},
	Title = {Replicative fitness of protease inhibitor-resistant mutants of human immunodeficiency virus type 1},
	Volume = {73},
	Year = {1999}}

@article{Mellorsetal96,
	Abstract = {The relation between viremia and clinical outcome in individuals infected with human immunodeficiency virus-type 1 (HIV-1) has important implications for therapeutic research and clinical care. HIV-1 RNA in plasma was quantified with a branched-DNA signal amplification assay as a measure of viral load in a cohort of 180 seropositive men studied for more than 10 years. The risk of acquired immunodeficiency syndrome (AIDS) and death in study subjects, including those with normal numbers of CD4+ T cells, was directly related to plasma viral load at study entry. Plasma viral load was a better predictor of progression to AIDS and death than was the number of CD4+ T cells.},
	Author = {Mellors, J. W. and Rinaldo, C. R., Jr. and Gupta, P. and White, R. M. and Todd, J. A. and Kingsley, L. A.},
	Journal = {Science},
	Keywords = {Acquired Immunodeficiency Syndrome/*virology Antiviral Agents/therapeutic use Biological Markers/blood CD4 Lymphocyte Count CD4-Positive T-Lymphocytes/virology Cohort Studies Disease Progression Follow-Up Studies HIV Infections/drug therapy/mortality/*virology HIV-1/genetics/*physiology Human Male Prognosis Proportional Hazards Models RNA, Viral/*blood Support, Non-U.S. Gov't Support, U.S. Gov't, Non-P.H.S. Support, U.S. Gov't, P.H.S. Survival Rate Time Factors Viremia/*virology Virus Replication},
	Note = {0036-8075 Comment Journal Article},
	Number = {5265},
	Pages = {1167-70},
	Title = {Prognosis in HIV-1 infection predicted by the quantity of virus in plasma},
	Volume = {272},
	Year = {1996}}

@article{Milleretal00,
	Abstract = {OBJECTIVE: To compare the rate of disease progression according to viral load and CD4 cell count in patients receiving or not receiving highly active antiretroviral therapy (HAART), defined as protease inhibitor-containing regimens. DESIGN: An observational study, with prospectively collected data. METHODS: All patients attending the HIV Outpatient clinic as of 1 January 1995 (n = 2083) were included. Follow-up was until the first AIDS-defining event or death. Associations between viral load or CD4 cell count and disease progression were assessed using a person-years approach. Event rates were compared using Poisson regression analysis; a multivariate model was used to assess the independent effects of CD4, viral load and treatment group on event rates and to consider interactions between these variables. RESULTS: The event rates increased with lower CD4 cell count and higher viral load for both treatment groups and were generally lower in the HAART group. In a multivariate analysis, lower CD4 cell counts and higher viral loads remained significantly associated with disease progression, irrespective of treatment group. However, the event rate was significantly lower for the HAART group compared with the control group (relative rate 0.53, P < 0.001). CONCLUSIONS: HAART-treated patients with high viral loads and CD4 cell counts experienced reduced disease progression compared with individuals with the same CD4 cell count and viral load not receiving HAART. Consequently, the short-term prognosis associated with viral load levels and CD4 cell counts may differ in patients on HAART. Whether this effect will be observed with non-protease-inhibitor-containing HAART is not known at this time.},
	Author = {Miller, V. and Sabin, C. A. and Phillips, A. N. and Rottmann, C. and Rabenau, H. and Weidmann, E. and Rickerts, V. and Findhammer, S. and Helm, E. B. and Staszewski, S.},
	Journal = {Aids},
	Keywords = {Adolescent Adult Aged Antiretroviral Therapy, Highly Active CD4 Lymphocyte Count Disease Progression HIV Infections/*drug therapy/pathology/virology HIV Protease Inhibitors/*therapeutic use *HIV-1/isolation & purification Human Middle Aged Prospective Studies RNA, Viral/analysis Regression Analysis Support, Non-U.S. Gov't Viral Load},
	Note = {0269-9370 Clinical Trial Journal Article},
	Number = {14},
	Pages = {2129-36},
	Title = {The impact of protease inhibitor-containing highly active antiretroviral therapy on progression of HIV disease and its relationship to CD4 and viral load},
	Volume = {14},
	Year = {2000}}

@article{Pikettyetal98,
	Abstract = {OBJECTIVES: To determine the clinical, virological and immunological outcome in a cohort of unselected patients receiving triple combination therapy for more than 1 year. METHODS: Prospective follow-up of a cohort of 162 unselected, protease inhibitor-naive, antiretroviral-experienced patients with advanced HIV disease, treated with indinavir combined with two nucleoside analogues. RESULTS: The mean CD4 cell count and plasma HIV RNA level in the study group at baseline were 69+/-5 x 10(6)/l and 4.75+/-0.07 log10 copies/ml, respectively. Five per cent of patients died prematurely or were lost to follow-up. Fifty-seven per cent of patients responded to therapy, as assessed by a sustained increase in CD4 cell counts above 50 x 10(6)/l and a decrease in plasma HIV RNA greater than 1 log10 copies/ml, throughout 12.1 months of follow-up. Seventeen per cent of patients were immunological and virological non-responders. Twenty-one per cent of patients exhibited discrepant virological and immunological responses to treatment, of whom one-half failed to exhibit significant increases in CD4 cells despite a virological response to therapy and one-half exhibited increased CD4 cell counts in the absence of significant decrease in plasma viral load. The incidence of AIDS-defining events in the latter group of patients was similar to that of responder patients, whereas their incidence was higher in patients who failed to exhibit a virological and immunological response and those who failed to increase CD4 cells despite a significant decrease in viral load. CONCLUSION: Our observations of discrepant immunological and virological responses to treatment raise the issue of the significance of persistent elevated levels of plasma HIV RNA and of the relevance of measurements of plasma viral load for assessing the efficacy of antiretroviral therapy in patients whose CD4 cell counts increase despite the absence of significant decrease in plasma HIV viral load.},
	Author = {Piketty, C. and Castiel, P. and Belec, L. and Batisse, D. and Si Mohamed, A. and Gilquin, J. and Gonzalez-Canali, G. and Jayle, D. and Karmochkine, M. and Weiss, L. and Aboulker, J. P. and Kazatchkine, M. D.},
	Journal = {Aids},
	Keywords = {Adult Aged Anti-HIV Agents/*therapeutic use Cohort Studies Drug Therapy, Combination Female Follow-Up Studies HIV Infections/*drug therapy/immunology/physiopathology/virology HIV Protease Inhibitors/*therapeutic use Human Indinavir/*therapeutic use Lamivudine/*therapeutic use Male Middle Aged Prospective Studies Reverse Transcriptase Inhibitors/*therapeutic use Stavudine/*therapeutic use Support, Non-U.S. Gov't Treatment Outcome Zidovudine/*therapeutic use},
	Note = {0269-9370 Journal Article},
	Number = {7},
	Pages = {745-50},
	Title = {Discrepant responses to triple combination antiretroviral therapy in advanced HIV disease},
	Volume = {12},
	Year = {1998}}

@article{Pikettyetal01,
	Abstract = {Within a prospective cohort of 150 human immunodeficiency virus (HIV)-infected patients who began first-line protease inhibitor therapy in 1996, the outcome of 42 patients with discrepant virologic and immunologic responses to antiretroviral treatment at 12 months was analyzed at 30 months of treatment. The incidence of AIDS-defining events and deaths (14%) in the group of patients with immunologic responses in the absence of a virologic response was higher than that in full-responder patients (2%); yet, the incidence in this group was lower than that in patients with no immunologic response, despite a virologic response (21%), and was lower than that in patients without an immunologic or virologic response (67%; P<.0001, log-rank test). Differences in outcome were significant (relative risk, 6.9; 95% confidence interval, 1.9-39.3) when factors for progression were compared with those of responder patients. The results support the relevance of the CD4 cell marker over plasma HIV load for predicting clinical outcome in patients who do not achieve full immunologic and virologic responses.},
	Author = {Piketty, C. and Weiss, L. and Thomas, F. and Mohamed, A. S. and Belec, L. and Kazatchkine, M. D.},
	Journal = {J Infect Dis},
	Keywords = {Adult Aged Antiretroviral Therapy, Highly Active CD4 Lymphocyte Count Cohort Studies Disease Progression Female HIV Infections/*drug therapy/immunology/virology HIV Protease Inhibitors/*therapeutic use Human Incidence Longitudinal Studies Male Middle Aged Mortality Prospective Studies RNA, Viral/blood Time Factors Treatment Outcome Viral Load},
	Note = {0022-1899 Journal Article},
	Number = {9},
	Pages = {1328-35},
	Title = {Long-term clinical outcome of human immunodeficiency virus-infected patients with discordant immunologic and virologic responses to a protease inhibitor-containing regimen},
	Volume = {183},
	Year = {2001}}

@article{Pilonetal02,
	Abstract = {Inhibition of human immunodeficiency virus type 1 reverse transcriptase (RT) by both nucleoside and nonnucleoside RT inhibitors profoundly inhibits virus replication. Nucleoside RT inhibitors are known to be toxic, but there is little information regarding the toxicities of nonnucleoside RT inhibitors (NNRTI). We demonstrate that efavirenz (an NNRTI) induces caspase- and mitochondrion-dependent apoptosis of Jurkat T cells and human peripheral blood mononuclear cells. The clinical relevance of these observations is not yet clear.},
	Author = {Pilon, A. A. and Lum, J. J. and Sanchez-Dardon, J. and Phenix, B. N. and Douglas, R. and Badley, A. D.},
	Journal = {Antimicrob Agents Chemother},
	Keywords = {Annexin V/diagnostic use Apoptosis/*drug effects Caspases/physiology Enzyme Inhibitors/diagnostic use Fluorescein-5-isothiocyanate Fluorescent Dyes HIV-1 Reverse Transcriptase/*antagonists & inhibitors Human Jurkat Cells Membrane Potentials/drug effects Mitochondria/drug effects/physiology Oxazines/*pharmacology Reverse Transcriptase Inhibitors/*pharmacology Support, Non-U.S. Gov't},
	Note = {0066-4804 Journal Article},
	Number = {8},
	Pages = {2687-91},
	Title = {Induction of apoptosis by a nonnucleoside human immunodeficiency virus type 1 reverse transcriptase inhibitor},
	Volume = {46},
	Year = {2002}}

@article{Priceetal03,
	Abstract = {Many individuals chronically infected with human immunodeficiency virus type 1 (HIV-1) experience a recrudescence of plasma virus during continuous combination antiretroviral therapy (ART) due either to the emergence of drug-resistant viruses or to poor compliance. In most cases, virologic failure on ART is associated with a coincident decline in CD4(+) T lymphocyte levels. However, a proportion of discordant individuals retain a stable or even increasing CD4(+) T lymphocyte count despite virological failure. In order to address the nature of these different outcomes, we evaluated virologic and immunologic variables in a prospective, single-blinded, nonrandomized cohort of 53 subjects with chronic HIV-1 infection who had been treated with continuous ART and monitored intensively over a period of 19 months. In all individuals with detectable viremia on ART, multiple drug resistance mutations with similar impacts on viral growth kinetics were detected in the pol gene of circulating plasma virus. Further, C2V3 env gene analysis demonstrated sequences indicative of CCR5 coreceptor usage in the majority of those with detectable plasma viremia. In contrast to this homogeneous virologic pattern, comprehensive screening with a range of antigens derived from HIV-1 revealed substantial immunologic differences. Discordant subjects with stable CD4(+) T lymphocyte counts in the presence of recrudescent virus demonstrated potent virus-specific CD4(+) and CD8(+) T lymphocyte responses. In contrast, subjects with virologic failure associated with declining CD4(+) T lymphocyte counts had substantially weaker HIV-specific CD4(+) T lymphocyte responses and exhibited a trend towards weaker HIV-specific CD8(+) T lymphocyte responses. Importantly the CD4(+) response was sustained over periods as long as 11 months, confirming the stability of the phenomenon. These correlative data lead to the testable hypothesis that the consequences of viral recrudescence during continuous ART are modulated by the HIV-specific cellular immune response.},
	Author = {Price, D. A. and Scullard, G. and Oxenius, A. and Braganza, R. and Beddows, S. A. and Kazmi, S. and Clarke, J. R. and Johnson, G. E. and Weber, J. N. and Phillips, R. E.},
	Journal = {J Virol},
	Keywords = {Adult Amino Acid Sequence Anti-HIV Agents/pharmacology/*therapeutic use CD4-Positive T-Lymphocytes/*immunology CD8-Positive T-Lymphocytes/*immunology Chronic Disease Drug Resistance, Viral/genetics Drug Therapy, Combination HIV Envelope Protein gp120/chemistry/genetics HIV Infections/*drug therapy/immunology/physiopathology HIV-1/*drug effects/genetics/physiology Human Lymphocyte Count Middle Aged Molecular Sequence Data Mutation Peptide Fragments/chemistry/genetics Prospective Studies RNA, Viral/blood Single-Blind Method Support, Non-U.S. Gov't *Treatment Failure Viral Load},
	Note = {0022-538x Clinical Trial Journal Article},
	Number = {10},
	Pages = {6041-9},
	Title = {Discordant outcomes following failure of antiretroviral therapy are associated with substantial differences in human immunodeficiency virus-specific cellular immunity},
	Volume = {77},
	Year = {2003}}

@article{Quinonesetal00,
	Abstract = {This study was designed to examine the impact of human immunodeficiency virus type 1 (HIV-1) fitness on disease progression through the use of a dual competition/heteroduplex tracking assay (HTA). Despite numerous studies on the impact of HIV-1 diversity and HIV-specific immune response on disease progression, we still do not have a firm understanding of the long-term pathogenesis of this virus. Strong and early CD8-positive cytotoxic T-cell and CD4-positive T-helper cell responses directed toward HIV-infected cells appear to curb HIV pathogenesis. However, the rate at which the virus infects the CD4(+) T-cell population and possibly destroys the HIV-specific immune response may also alter the rate of disease progression. For HIV-1 fitness studies, we established conditions for dual HIV-1 infections of peripheral blood mononuclear cells (PBMC) and a sensitive HTA to measure relative virus production. A pairwise comparison was then performed to estimate the relative fitness of various non-syncytium-inducing/CCR5-tropic (NSI/R5) and syncytium-inducing/CXCR4-tropic (SI/X4) HIV-1 isolates. Four HIV-1 strains (two NSI/R5 and two SI/X4) with moderate ex vivo fitness were then selected as controls and competed against primary HIV-1 isolates from an HIV-infected Belgian cohort. HIV-1 isolates from long-term survivors (LTS) were outcompeted by control strains and were significantly less fit than HIV-1 isolates from patients with accelerated progression to AIDS (PRO). In addition, NSI/R5 HIV-1 isolates from PRO overgrew control SI/X4 strains, suggesting that not all SI/X4 HIV-1 isolates replicate more efficiently than all NSI/R5 isolates. Finally, there were strong, independent correlations between viral load and the total relative fitness values of HIV-1 isolates from PRO (r = 0.84, P = 0.033) and LTS (r = 0.86, P = 0.028). Separation of the PRO and LTS plots suggest that HIV-1 fitness together with viral load may be a strong predictor for the rate of disease progression.},
	Author = {Quinones-Mateu, M. E. and Ball, S. C. and Marozsan, A. J. and Torre, V. S. and Albright, J. L. and Vanham, G. and van Der Groen, G. and Colebunders, R. L. and Arts, E. J.},
	Journal = {J Virol},
	Keywords = {*Biological Assay HIV Infections/*physiopathology/*virology *HIV-1/physiology Human Predictive Value of Tests Prognosis Support, Non-U.S. Gov't Support, U.S. Gov't, P.H.S.},
	Note = {0022-538x Journal Article},
	Number = {19},
	Pages = {9222-33},
	Title = {A dual infection/competition assay shows a correlation between ex vivo human immunodeficiency virus type 1 fitness and disease progression},
	Volume = {74},
	Year = {2000}}

@article{Racinanetal02,
	Abstract = {OBJECTIVE: To study whether hepatitis C virus (HCV) co-infection or the severe elevation of transaminases is associated with survival after the initiation of antiretroviral combination therapy. DESIGN: Prospective hospital-based cohort (Aquitaine Cohort). METHODS: HIV-infected adults started on an antiretroviral combination before 30 June 1999. HCV infection was defined as antibody detection or positive HCV RNA. Severe elevation of transaminases was defined as a value of aspartate or alanine aminotransferase (AST, ALT) above five times the upper limit of normal values. Survival was studied using a Cox model, including at least baseline HCV status and transaminases as a time-dependent covariate. RESULTS: Overall, 995 patients were analysed, including 576 HCV-positive individuals (58%). At baseline, HCV-positive patients were younger, more often injecting drug users and women, and had more frequently elevated transaminases. A shorter survival was associated with AIDS stage [hazard ratio (HR) versus non-AIDS 1.67; 95% confidence interval (CI) 1.03; 2.68], lower CD4 cell count (HR for 50 cells/mm3 lower 1.33; CI 1.17; 1.51), lower haemoglobin (HR for 1 g/dl lower 1.20; CI 1.07; 1.35), lower platelet count (HR for 10 000 cells/mm3 lower 1.04; CI 1.01; 1.07), and AST during follow-up (HR for > or = 200 IU/l 2.30; CI 1.32; 4.03). HCV co-infection (HR 1.20; CI 0.75; 1.92) was not statistically associated with survival. CONCLUSION: The occurrence of a severe elevation of transaminases was associated with poorer survival, although HCV was not. If liver toxicity may be treatment induced, plasma drug concentrations could guide dosage adjustments of antiretroviral treatments currently prescribed to optimize their use.},
	Author = {Rancinan, C. and Neau, D. and Saves, M. and Lawson-Ayayi, S. and Bonnet, F. and Mercie, P. and Dupon, M. and Couzigou, P. and Dabis, F. and Chene, G.},
	Journal = {Aids},
	Keywords = {Acquired Immunodeficiency Syndrome/complications Age Factors Anti-HIV Agents/*therapeutic use Antiretroviral Therapy, Highly Active Cohort Studies Comparative Study Disease Progression Female Follow-Up Studies HIV Infections/blood/*complications/*drug therapy Hepatitis C/blood/*complications Human Male Proportional Hazards Models Substance Abuse, Intravenous Support, Non-U.S. Gov't Survival Analysis Transaminases/blood},
	Note = {0269-9370 Journal Article},
	Number = {10},
	Pages = {1357-62},
	Title = {Is hepatitis C virus co-infection associated with survival in HIV-infected patients treated by combination antiretroviral therapy?},
	Volume = {16},
	Year = {2002}}

@article{Rogeretal99,
	Abstract = {HAART may increase CD4+ T cell counts despite a persistently detectable HIV load. The impact of HAART on apoptosis, which may play a role in the disease process in HIV-infected patients, has not been extensively studied. We performed a study to compare the level of spontaneous T cell apoptosis and anti-retroviral treatments in a cohort of HIV-1-infected patients. Data were obtained from a computerized medical record. Quantification of apoptotic cells was by cytofluorometric technique. From November 1995 to December 1997 we studied T cell apoptosis in 112 HIV-infected patients. Forty patients were classified A, 36 B and 36 C. Thirty patients were naive and 82 received an anti-retroviral treatment, 49 including a protease inhibitor (PI). The median plasma viraemia determined in 63 patients was 3.6 (range 1.3-5.6) log10. The median apoptotic cell count was 22% (range 2-73%) and 12% (range 2-60%) for CD4+ and CD8+ T cells, respectively. We did not observe any correlation between the HIV viraemia and the level of apoptosis of T cell subsets. Patients with HAART showed a lower percentage of apoptotic CD4+ T cells only: 16% (range 2-61%) versus 25% (range 5-73%) for patients receiving two nucleoside analogues (P = 0.02). This effect was significant in stage A patients and remained observable during the whole course of HIV disease. In conclusion, HAART, without any relation to plasma viraemia, is able to reduce apoptosis of CD4+ T cells.},
	Author = {Roger, P. M. and Breittmayer, J. P. and Arlotto, C. and Pugliese, P. and Pradier, C. and Bernard-Pomier, G. and Dellamonica, P. and Bernard, A.},
	Journal = {Clin Exp Immunol},
	Keywords = {Adult Aged Anti-HIV Agents/*therapeutic use *Apoptosis CD4-Positive T-Lymphocytes/cytology/*drug effects CD8-Positive T-Lymphocytes/drug effects Didanosine/therapeutic use Drug Therapy, Combination Female HIV Infections/*drug therapy/immunology/pathology HIV Protease Inhibitors/therapeutic use Human Lamivudine/therapeutic use Male Middle Aged Multivariate Analysis Retrospective Studies Stavudine/therapeutic use Viral Load Zalcitabine/therapeutic use Zidovudine/therapeutic use},
	Note = {0009-9104 Journal Article},
	Number = {3},
	Pages = {412-6},
	Title = {Highly active anti-retroviral therapy (HAART) is associated with a lower level of CD4+ T cell apoptosis in HIV-infected patients},
	Volume = {118},
	Year = {1999}}

@article{Stoddaretalt01,
	Abstract = {Many HIV-1-infected patients treated with protease inhibitors (PI) develop PI-resistant HIV-1 variants and rebounds in viremia, but their CD4+ T-cell counts often do not fall. We hypothesized that in these patients, T-cell counts remain elevated because PI-resistant virus spares intrathymic T-cell production. To test this, we studied recombinant HIV-1 clones containing wild-type or PI-resistant protease domains, as well as uncloned isolates from patients, in activated peripheral blood mononuclear cells, human thymic organ cultures and human thymus implants in SCID-hu Thy/Liv mice. In most cases, wild-type and PI-resistant HIV-1 isolates replicated to similar degrees in peripheral blood mononuclear cells. However, the replication of PI-resistant but not wild-type HIV-1 isolates was highly impaired in thymocytes. In addition, patients who had PI-resistant HIV-1 had abundant thymus tissue as assessed by computed tomography. We propose that the inability of PI-resistant HIV-1 to replicate efficiently in thymus contributes to the preservation of CD4+ T-cell counts in patients showing virologic rebound on PI therapy.},
	Author = {Stoddart, C. A. and Liegler, T. J. and Mammano, F. and Linquist-Stepps, V. D. and Hayden, M. S. and Deeks, S. G. and Grant, R. M. and Clavel, F. and McCune, J. M.},
	Journal = {Nat Med},
	Keywords = {Adult Animals CD4 Lymphocyte Count Drug Resistance, Microbial Fetal Tissue Transplantation Flow Cytometry HIV Core Protein p24/metabolism HIV Infections/immunology/pathology/*virology HIV Protease/genetics/*metabolism HIV Protease Inhibitors/*pharmacology HIV-1/*drug effects/enzymology/genetics/*physiology Human Mice Mice, SCID Middle Aged Organ Culture Recombination, Genetic Support, Non-U.S. Gov't Support, U.S. Gov't, P.H.S. T-Lymphocytes/*physiology/virology Thymus Gland/pathology/physiopathology/transplantation/*virology Viral Load *Virus Replication},
	Note = {1078-8956 Journal Article},
	Number = {6},
	Pages = {712-8},
	Title = {Impaired replication of protease inhibitor-resistant HIV-1 in human thymus},
	Volume = {7},
	Year = {2001}}

@article{Sufkaetal03,
	Abstract = {Mechanisms that underly discordant CD4+ cell/virus load (VL) responses in patients who receive highly active antiretroviral therapy (HAART) were studied in 30 human immunodeficiency virus (HIV)-positive patients, in 3 groups. Discordant responders maintained CD4+ cell levels >200/mm(3) with stable or increasing trend, despite sustained VLs of 500-5000 copies/mL, for >2 years. Treatment-success patients had CD4+ cell counts >200/mm(3) with stable or increasing trend and VLs <50 copies/mL, for >2 years. Treatment-failure patients initially responded to HAART, followed by decreasing CD4+ cell counts and increasing VLs. Interferon-gamma production to gag and noncytolytic CD8+ cell suppressive activity were greater in discordant responders. Cellular activation was greatest in patients with treatment failure. All discordant responders had non-syncytium-inducing (CCR5-tropic) viruses. Viruses from discordant responders and from patients with treatment failure had extensive resistance mutations; discordant responders had significantly lower viral replication capacities. These findings suggest that discordant responses may be related to enhanced HIV-directed immune responses, diminished cellular activation, decreased viral replication capacity, and preservation of non-syncytium-inducing virus strains.},
	Author = {Sufka, S. A. and Ferrari, G. and Gryszowka, V. E. and Wrin, T. and Fiscus, S. A. and Tomaras, G. D. and Staats, H. F. and Patel, D. D. and Sempowski, G. D. and Hellmann, N. S. and Weinhold, K. J. and Hicks, C. B.},
	Journal = {J Infect Dis},
	Keywords = {Adult *Antiretroviral Therapy, Highly Active *CD4 Lymphocyte Count Female HIV/*drug effects HIV Infections/*drug therapy/*immunology/virology HIV Protease Inhibitors/*pharmacology/therapeutic use Human Male Middle Aged Support, Non-U.S. Gov't Support, U.S. Gov't, P.H.S. Time Factors Treatment Failure *Viral Load Virus Replication/drug effects},
	Note = {0022-1899 Clinical Trial Journal Article},
	Number = {7},
	Pages = {1027-37},
	Title = {Prolonged CD4+ cell/virus load discordance during treatment with protease inhibitor-based highly active antiretroviral therapy: immune response and viral control},
	Volume = {187},
	Year = {2003}}

@article{Tebaldietal03,
	Abstract = {To ascertain the impact of hepatitis C virus (HCV) infection on human immunodeficiency virus (HIV) disease progression and associated death in the era of highly active antiretroviral therapy (HAART), we examined mortality rates, the presence of other diseases, and antiretroviral use in an observational cohort of 823 HIV-infected patients with and without HCV coinfection during the period of January 1996 through June 2001. Analyses were used to compare patient characteristics, comorbid conditions, and survival durations in HIV-infected and HIV-HCV-coinfected patients. HIV-HCV-coinfected persons did not have a statistically greater rate of acquired immunodeficiency syndrome or of renal or cardiovascular disease, but they did have more cases of cirrhosis and transaminase elevations. There were proportionately more deaths in the HIV-HCV-coinfected group. Age, baseline CD4+ cell count, and duration of HAART were significantly associated with survival, but HCV infection was not. HAART use was a strong predictor of increased duration of survival, suggesting that treatment is more important to survival than is HCV coinfection status.},
	Author = {Tedaldi, E. M. and Baker, R. K. and Moorman, A. C. and Alzola, C. F. and Furhrer, J. and McCabe, R. E. and Wood, K. C. and Holmberg, S. D.},
	Journal = {Clin Infect Dis},
	Keywords = {Anti-HIV Agents/therapeutic use *Antiretroviral Therapy, Highly Active *Hiv HIV Infections/*complications/drug therapy/epidemiology/mortality *Hepacivirus Hepatitis C/*complications/epidemiology/mortality Human Morbidity Mortality Support, U.S. Gov't, P.H.S.},
	Note = {1537-6591 Journal Article},
	Number = {3},
	Pages = {363-7},
	Title = {Influence of coinfection with hepatitis C virus on morbidity and mortality due to human immunodeficiency virus infection in the era of highly active antiretroviral therapy},
	Volume = {36},
	Year = {2003}}

@article{Wang&Bembom&vanderLaan06,
	Author = {Y. Wang and O. Bembom and M.J. van der Laan},
	Journal = {Journal of Statistical Planning and Inference},
	Optnote = {also http://www.bepress.com/ucbbiostat/paper159},
	Title = {Data adaptive estimation of the treatment specific mean},
	Year = {2006}}

@article{Sinisi&vanderLaan04,
	Author = {S. Sinisi and M.J. van der Laan},
	Journal = {Journal of Statistical Methods in Molecular Biology},
	Optnote = {http://www.bepress.com/sagmb/vol3/iss1/art18},
	Title = {The {D}eletion/{S}ubstitution/{A}ddition Algorithm in Loss Function Based Estimation: Applications in Genomics},
	Volume = {3},
	Year = {2004}}

@techreport{Petersenetal05,
	Author = {M. L. Petersen and S.G. Deeks and J. N. Martin and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Month = {December},
	Optnote = {http://www.bepress.com/ucbbiostat/paper199},
	Title = {History-Adjusted Marginal Structural Models: Time-Varying Effect Modification and Dynamic Treatment Regimens},
	Type = {Technical Report 199},
	Year = {2005}}

@techreport{vanderLaan&Rubin05,
	Author = {M.J. van der Laan and D. Rubin},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper180},
	Title = {Estimating Function Based Cross-Validation and Learning},
	Type = {Technical Report 180},
	Year = {2005}}

@article{Chambaz&Rousseau08,
	Author = {A. Chambaz and J. Rousseau},
	Issue = {2},
	Journal = {The Annals of Statistics},
	Pages = {938-62},
	Title = {Bounds for Bayesian order identification with application to mixtures},
	Volume = {36},
	Year = {2008}}

@techreport{Gruber&vanderLaan09,
	Author = {S. Gruber and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper252},
	Title = {Targeted Maximum Likelihood Estimation: A Gentle Introduction},
	Type = {Technical Report 252},
	Year = {2009}}

@techreport{vanderLaan06,
	Author = {M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper203},
	Title = {Causal Effect Models for Intention to Treat and Realistic Individualized Treatment Rules},
	Type = {Technical Report 203},
	Year = {2006}}

@techreport{vanderLaan08b,
	Author = {M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Month = {March},
	Optnote = {http://www.bepress.com/ucbbiostat/paper232},
	Title = {The construction and analysis of adaptive group sequential designs},
	Type = {Technical Report 232},
	Year = {2008}}

@techreport{Moore&vanderLaan07,
	Author = {K.L. Moore and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Month = {April},
	Optnote = {http://www.bepress.com/ucbbiostat/paper215},
	Title = {Covariate adjustment in randomized trials with binary outcomes},
	Type = {Technical Report 215},
	Year = {2007}}

@techreport{vanderLaan&Petersen05,
	Author = {M.J. van der Laan and M.L. Petersen},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper187},
	Title = {Direct Effect Models},
	Type = {Technical Report 187},
	Year = {2005}}

@techreport{Petersen&vanderLaan06,
	Author = {M.L. Petersen and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Title = {Individualized Treatment Rules and Clinical Trials},
	Type = {Technical Report},
	Year = {2006}}

@article{vanderLaan&Petersen&Joffe05,
	Author = {M.J. van der Laan and M.L. Petersen and M.M. Joffe},
	Journal = {The International Journal of Biostatistics},
	Number = {1},
	Optnote = {http://www.bepress.com/ijb/vol1/iss1/4},
	Pages = {10-20},
	Title = {History-Adjusted Marginal Structural Models and Statically-Optimal Dynamic Treatment Regimens},
	Volume = {1},
	Year = {2005}}

@article{vanderLaan06a,
	Author = {M.J. van der Laan},
	Journal = {International Journal of Biostatistics},
	Number = {1},
	Optnote = {http://www.bepress.com/ijb/vol2/iss1/art2},
	Title = {Statistical Inference for Variable Importance},
	Volume = {2},
	Year = {2006}}

@article{vanderLaan&Birkner&Hubbard05,
	Author = {M.J. van der Laan and M.D. Birkner and A.E. Hubbard},
	Journal = {Journal of Statistical Applications in Genetics and Molecular Biology},
	Number = {1},
	Optnote = {http://www.bepress.com/sagmb/vol4/iss1/art29},
	Title = {Empirical Bayes and resampling based multiple testing procedure controlling tail probability of the proportion of false positives},
	Volume = {4},
	Year = {2005}}

@article{vanderLaan&Dudoit&Pollard04b,
	Author = {M.J. van der Laan and S. Dudoit and K.S. Pollard},
	Journal = {Journal of Statistical Applications in Genetics and Molecular Biology},
	Number = {1},
	Optnote = {http://www.bepress.com/sagmb/vol3/iss1/art15},
	Title = {Augmentation procedures for control of the generalized family-wise error rate and tail probabilities for the proportion of false positives},
	Volume = {3},
	Year = {2004}}

@article{vanderLaan&Dudoit&Pollard04,
	Author = {S. Dudoit and M.J. van der Laan and K.S. Pollard},
	Journal = {Journal of Statistical Applications in Genetics and Molecular Biology},
	Number = {1},
	Optnote = {http://www.bepress.com/sagmb/vol3/iss1/art14},
	Title = {Multiple testing. Part II. Step-down procedures for control of the family-wise error rate},
	Volume = {3},
	Year = {2004}}

@article{Dudoit&vanderLaan&Pollard04,
	Author = {S. Dudoit and M.J. van der Laan and K.S. Pollard},
	Journal = {Journal of Statistical Applications in Genetics and Molecular Biology},
	Number = {1},
	Optnote = {http://www.bepress.com/sagmb/vol3/iss1/art13},
	Title = {Multiple testing. Part I. Single-step procedures for control of general Type I error rates},
	Volume = {3},
	Year = {2004}}

@article{Birkner&Sinisi&vanderLaan05,
	Author = {M.D. Birkner and S.E. Sinisi and M.J. van der Laan},
	Journal = {Journal of Statistical Applications in Genetics and Molecular Biology},
	Number = {1},
	Optnote = {http://www.bepress.com/sagmb/vol4/iss1/art8},
	Title = {Multiple Testing and Data Adaptive Regression: An Application to {HIV}-1 Sequence Data},
	Volume = {4},
	Year = {2005}}

@techreport{vanderLaan&Hubbard06,
	Author = {M.J. van der Laan and A.E. Hubbard},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper198},
	Title = {Quantile-Function Based Null Distribution in Resampling Based Multiple Testing},
	Type = {Technical Report},
	Year = {2006}}

@techreport{Molinaro&vanderLaan04,
	Author = {A. Molinaro and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper162},
	Title = {Deletion/Substitution/Addition Algorithm for Partitioning the Covariate Space in Prediction},
	Type = {Technical Report},
	Year = {2004}}

@techreport{Birkner&vanderLaan05,
	Author = {M.D. Birkner and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Title = {Application of a Variable Importance Measure Method to {HIV}-1 Sequence Data},
	Type = {Technical Report},
	Year = {2005}}

@techreport{Neugebauer&vanderLaan05b,
	Author = {R. Neugebauer and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {134},
	Optnote = {http://www.bepress.com/ucbbiostat/paper134, to appear in {JSPI}},
	Title = {Locally Efficient Estimation of Nonparametric Causal Effects on Mean Outcomes in Longitudinal Studies},
	Type = {Technical Report},
	Year = {2005}}

@techreport{Wang&Petersen&vanderLaan06,
	Author = {Y. Wang and M. Petersen and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Title = {A statistical method for diagnosing {ETA} bias in {IPTW} estimators},
	Type = {Technical Report},
	Year = {2006}}

@techreport{vanderLaan&Dudoit&vanderVaart,
	Author = {M.J. van der Laan and S. Dudoit and A.W. van der Vaart},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Month = {February},
	Optnote = {http://www.bepress.com/ucbbiostat/paper142},
	Title = {The Cross-Validated Adaptive Epsilon-Net Estimator},
	Type = {Technical Report 142},
	Year = {2004}}

@techreport{vanderLaan&Dudoit03,
	Author = {M.J. van der Laan and S. Dudoit},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Month = {November},
	Optnote = {http://www.bepress.com/ucbbiostat/paper130},
	Title = {Unified cross-validation methodology for selection among estimators and a general cross-validated adaptive epsilon-net estimator: Finite sample oracle inequalities and examples},
	Type = {Technical Report},
	Year = {2003}}

@techreport{Petersen&vanderLaan05,
	Author = {M. Petersen and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Title = {Estimation of direct and indirect causal effects in Epidemiology},
	Type = {Technical Report},
	Year = {2005}}

@techreport{vanderLaan&Petersen04,
	Author = {M.J. van der Laan and M. Petersen},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Month = {August},
	Title = {Estimation of direct and indirect causal effects in longitudinal studies},
	Type = {Technical Report 155},
	Year = {2004}}

@techreport{vanderLaan&Hubbard&Jewell04,
	Author = {M.J. van der Laan and A.E. Hubbard and N.P. Jewell},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Month = {September},
	Optnote = {http://www.bepress.com/ucbbiostat/paper157},
	Title = {Estimation of Treatment Effects in Randomized Trials with Noncompliance and a Dichotomous Outcome},
	Type = {Technical Report 157},
	Year = {2004}}

@techreport{Bein&Hubbard&vanderLaan05,
	Author = {E. Bein and A.E. Hubbard and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Title = {Estimating Function Based Cross-Validation in Estimation of the Causal Effect in Randomized Trials},
	Type = {Technical Report},
	Year = {2005}}

@techreport{Molinaroetal05,
	Author = {A.M. Molinaro and M.J. van der Laan and D.H. Moore and K. Kerlikowske},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Note = {http://www.bepress.com/ucbbiostat/paper149},
	Title = {Survival point estimate prediction in matched and non-matched case-control subsample designed studies},
	Year = {2005}}

@techreport{Dudoitetal04,
	Author = {S. Dudoit and M.J. van der Laan and S. Kele\c{s} and A. M. Molinaro and S. E. Sinisi and S.L. Teng},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Note = {to appear in \emph{SIGKDD} Explorations on Microarray Data Mining},
	Title = {Loss-Based Estimation with Cross-Validation: Applications to Microarray Data Analysis and Motif Finding.},
	Year = {2004}}

@book{Friedman&Furberg&Demets98,
	Author = {L.M.Friedman and C.D. Furberg and D.L. DeMets},
	Publisher = {Springer-Verlag New York},
	Title = {Fundamentals of Clinical Trials},
	Year = {1998}}

@book{Andersenetal93,
	Author = {P.K. Andersen and O. Borgan and R.D. Gill and N. Keiding},
	Publisher = {Springer-Verlag New York},
	Title = {Statistical Models Based on Counting Processes},
	Year = {1993}}

@incollection{Robins03,
	Author = {J.M. Robins},
	Booktitle = {Highly Structured Stochastic Systems},
	Editor = {P. Green, N. Hjort, and S. Richardson},
	Pages = {70--81},
	Publisher = {Oxford University Press, Oxford},
	Title = {Semantics of causal DAG models and the identification of direct and indirect effects},
	Year = {2003}}

@techreport{Pearl01,
	Author = {J. Pearl},
	Institution = {University of California, Los Angeles, Department of Computer Science},
	Title = {Cognitive systems Laboratory},
	Year = {2001}}

@techreport{Pearl10b,
	Author = {J. Pearl},
	Institution = {University of California, Los Angeles, Department of Computer Science},
	Month = {August},
	Number = {R-370},
	Title = {The Causal Foundations of Structural Equation Modeling},
	Year = {2010}}

@book{Pearl09,
	Author = {J. Pearl},
	Date-Modified = {2011-04-03 23:20:08 -0700},
	Edition = {2nd},
	Publisher = {Cambridge University Press, Cambridge},
	Title = {Causality: Models, Reasoning, and Inference},
	Year = {2000}}

@article{Robins&Greenland92,
	Author = {J.M. Robins and S. Greenland},
	Journal = {Epidemiology},
	Number = {0},
	Pages = {143--155},
	Title = {Identifiability and exchangeability for direct and indirect effects},
	Volume = {3},
	Year = {1992}}

@article{vanderLaan95,
	Author = {M.J. van der Laan},
	Journal = {Bernoulli},
	Number = {4},
	Pages = {335--341},
	Title = {Identity for NPMLE in missing data and biased sampling models},
	Volume = {1},
	Year = {1995}}

@article{vanderLaan98,
	Author = {M.J. van der Laan},
	Journal = {Lifetime Data Models},
	Number = {0},
	Pages = {83--102},
	Title = {Identity for NPMLE in Censored Data Models},
	Volume = {4},
	Year = {1998}}

@article{Klaassen86,
	Author = {C.A.J. Klaassen},
	Journal = {The Annals of Statistics},
	Pages = {1548--1562},
	Title = {Consistent estimation of the influence function of locally asymptotically linear estimators},
	Volume = {15},
	Year = {1987}}

@article{Robins&Rotnitzky04,
	Author = {J.M. Robins and A. Rotnitzky},
	Journal = {Biometrika},
	Number = {0},
	Optnote = {To Appear},
	Pages = {0},
	Title = {Estimation of Treatment Effects in Randomized Trials with Noncompliance and a Dichotomous Outcome using Structural Nested Mean Models},
	Volume = {0},
	Year = {2004}}

@article{vanderVaart91,
	Author = {A.W. van der Vaart},
	Journal = {The Annals of Statistics},
	Pages = {178--204},
	Title = {On differentiable functionals},
	Volume = {19},
	Year = {1991}}

@article{Rubin78,
	Author = {D.B. Rubin},
	Journal = {The Annals of Statistics},
	Pages = {34--58},
	Title = {Bayesian Inference for causal effects: the role of randomization},
	Volume = {6},
	Year = {1978}}

@article{Neyman23,
	Author = {Neyman, J.},
	Journal = {Statistical Science},
	Optnote = {Translation of 1923 article},
	Pages = {465--480},
	Title = {On the application of probability theory to agricultural experiments},
	Volume = {5},
	Year = {1990}}

@article{Robins86,
	Author = {J.M. Robins},
	Journal = {Mathematical Modelling},
	Pages = {1393--1512},
	Title = {A New Approach to Causal Inference in Mortality Studies with Sustained Exposure Periods - Application to Control of the Healthy Worker Survivor Effect},
	Volume = {7},
	Year = {1986}}

@article{Robins94,
	Author = {J.M. Robins},
	Journal = {Communications in Statistics},
	Pages = {2379--2412},
	Title = {Correcting for non-compliance in randomized trials using structural nested mean models},
	Volume = {23},
	Year = {1994}}


@inproceedings{Robins00c,
	Author = {J.M. Robins},
	Booktitle = {Proceedings of the American Statistical Association: Section on Bayesian Statistical Science},
	Pages = {6-10},
	Title = {Robust Estimation in Sequentially Ignorable Missing Data and Causal Inference Models},
	Year = {2000}}

@article{Stuart10,
	Author = {B.K. Lee and J. Lessler and E.A. Stuart},
	Issue = {3},
	Journal = {Statistics in Medicine},
	Pages = {337-46},
	Title = {Improved propensity score weighting using machine learning},
	Volume = {29},
	Year = {2009}}

@article{Leeetal10,
	Author = {B.K. Lee and J. Lessler and E.A. Stuart},
	Issue = {3},
	Journal = {Statistics in Medicine},
	Pages = {337-46},
	Volume = {29},
	Year = {2009}}


@article{Schneeweiss09,
	Author = {S. Schneeweiss and J.A. Rassen and R. J. Glynn and J. Avorn and H. Mogun and M. A. Brookhart},
	Journal = {Epidemiology},
	Title = {High-dimensional propensity score adjustment in studies of treatment effects using health care claims data},
	Volume = {20(4)},
	pages={512--522},
	Optnote={doi:  10.1097/EDE.0b013e3181a663cc},	Year = {2009}}

@article{Brookhart11,
	Author = {D. Westreich and S.R. Cole and M.J. Funk and M.A. Brookhart and T Sturmer},
	Journal = {Pharmacoepidemiology and Drug Safety},
	Pages = {317-20},
	Title = {The role of the c-statistic in variable selection for propensity scores},
	Volume = {20},
	Year = 2011}

@article{Westreichetal11,
	Author = {D. Westreich and S.R. Cole and M.J. Funk and M.A. Brookhart and T Sturmer},
	Journal = {Pharmacoepidemiology and Drug Safety},
	Pages = {317-20},
	Title = {The role of the c-statistic in variable selection for propensity scores},
	Volume = {20},
	Year = 2011}


@article{Vansteelandt10,
	Author = {S. Vansteelandt and M. Bekaert and G. Claeskens},
	Journal = {Statistical Methods in Medical Research},
	Title = {On model selection and model misspecification in causal inference},
	Volume={21(1)},
	pages={7--30},
	Optnote={doi: 10.1177/0962280210387717},	Year = {2010}}

@article{Vansteelandt&Goetghebeur03,
	Author = {S. Vansteelandt and E. Goetghebeur},
	Journal = {Journal of the Royal Statistical Society, Series B},
	Optnote = {In print},
	Title = {Causal inference with generalized structural mean models},
	Volume = {23},
	Year = {2003}}

@incollection{Robins97a,
	Address = {Chichester, UK},
	Author = {Robins, J.M.},
	Booktitle = {The Encyclopedia of Biostatistics},
	Editor = {Armitage, P. and Colton, T. and Andersen, P.K. and Keiding, N.},
	Publisher = {John Wiley and Sons},
	Title = {Structural Nested Failure Time Models},
	Year = {1997}}



@article{RobinsMSM97,
	Author = {Robins, J. M.},
	Title = {Marginal structural models},
	Journal = {1997 Proceedings of the American Statistical Association Section on Bayesian Statistical Science},
	Pages = {1-10},
	Year = {1997}
}

@article{Hernan&Brumback&Robins,
	Author = {Hernan, M. A. and Brumback, B. and Robins, J. M.},
	Journal = {Epidemiology},
	Number = {5},
	Pages = {561--570},
	Title = {Marginal Structural Models to Estimate the Causal Effect of Zidovudine on the Survival of {HIV}-Positive Men},
	Volume = {11},
	Year = {2000}}

@article{Robins87,
	Author = {Robins, J.M.},
	Coden = {CMAPDK},
	Fjournal = {Computers \& Mathematics with Applications. An International Journal},
	Issn = {0097-4943},
	Journal = {Comput. Math. Appl.},
	Number = {9-12},
	Pages = {923--945},
	Title = {Addendum to: ``{A} new approach to causal inference in mortality studies with a sustained exposure period---application to control of the healthy worker survivor effect'' [{M}ath.\ {M}odelling {\bf 7} (1986), no.\ 9-12, 1393--1512; {M}{R} 87m:92078]},
	Volume = {14},
	Year = {1987}}

@article{Robins&Hernan&Brumback00,
	Author = {Robins, J. M. and Hernan, M. A. and Brumback, B.},
	Journal = {Epidemiology},
	Number = {5},
	Pages = {550--560},
	Title = {Marginal Structural Models and Causal Inference in Epidemiology},
	Volume = {11},
	Year = {2000}}

@article{Bryan&Yu&vanderLaan03,
	Author = {Bryan, J. and Yu, Z. and van der Laan, M.J.},
	Journal = {Biostatistics},
	Number = {3},
	Pages = {361--380},
	Title = {Analysis of Longitudinal Marginal Structural Models},
	Volume = {5},
	Year = {2003}}

@techreport{Yu&vanderLaan03b,
	Author = {Yu, Z. and van der Laan, M.J.},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper132},
	Optnumber = {132},
	Title = {Double Robust Estimation in Longitudinal Marginal Structural Models},
	Year = {2003}}

@article{Murphy03,
	Author = {Murphy, S.A.},
	Journal = {Journal of the Royal Statistical Society: Series B},
	Number = {2},
	Pages = {331-66},
	Title = {Optimal dynamic treatment regimes},
	Volume = {65},
	Year = {2003}}

@article{Robins03a,
	Author = {Robins, J.M.},
	Journal = {Journal of the Royal Statistical Society: Series B},
	Number = {2},
	Pages = {355--66},
	Title = {Discussion of ``Optimal dynamic treatment regimes" by Susan A. Murphy},
	Volume = {65},
	Year = {2003}}

@article{Murphy&vanderLaan&Robins01,
	Author = {S.A. Murphy and M.J. van der Laan and J.M. Robins},
	Journal = {Journal of the American Statistical Association},
	Pages = {1410--1424},
	Title = {Marginal mean models for dynamic treatment regimens},
	Volume = {96},
	Year = {2001}}



@incollection{Robins98,
	Address = {New York},
	Author = {Robins, J.M.},
	Booktitle = {Statistical Models in Epidemiology, the Environment, and Clinical Trials (Minneapolis, MN, 1997)},
	Mrclass = {62N01 (62G08 62P10)},
	Mrnumber = {2001a:62124},
	Pages = {95-133},
	Publisher = {Springer-Verlag},
	Title = {Marginal Structural Models versus Structural Nested Models as Tools for Causal Inference},
	Year = {2000}}

@incollection{Robins97,
	Author = {J.M. Robins},
	Booktitle = {Latent Variable Modeling and Applications to Causality},
	Editor = {M. Berkane, Editor},
	Optseries = {Lecture Notes in Statistics},
	Optvolume = {120},
	Pages = {69--117},
	Publisher = {Springer-Verlag, New York},
	Title = {Causal Inference from Complex Longitudinal Data},
	Year = {1997}}

@incollection{Robins89,
	Address = {Washington D.C.},
	Author = {J.M. Robins},
	Booktitle = {Health Service Methodology: A Focus on AIDS},
	Editor = {L. Sechrest and H. Freeman and A. Mulley},
	Optseries = {Lecture Notes in Statistics},
	Pages = {113--159},
	Publisher = {U.S. Public Health Service, National Center for Health SErvices Research},
	Title = {The analysis of randomized and non-randomized AIDS treatment trials using a new approach in causal inference in longitudinal studies},
	Year = {1989}}

@techreport{Abadie00,
	Author = {A. Abadie},
	Institution = {NBER Technical Working Paper},
	Optnumber = {260},
	Title = {Semiparametric estimation of instrumental variables models for causal effects},
	Year = {2000}}

@article{Abadie03,
	Author = {A. Abadie},
	Journal = {Journal of Econometrics},
	Pages = {231-263},
	Title = {Semiparametric instrumental variable estimation of treatment response models},
	Volume = {113},
	Year = {2003}}

@techreport{Wang&Vanderlaan04,
	Author = {Y. Wang and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper159},
	Optnumber = {159},
	Title = {Data adaptive estimation of the treatment specific mean},
	Year = {2004}}

@techreport{Yu&Vanderlaan02,
	Author = {Z. Yu and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper122},
	Optnumber = {122},
	Title = {Construction of counterfactuals and the {G}-computation formula},
	Year = {2002}}

@techreport{Yu&Vanderlaan03,
	Author = {Z. Yu and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper136},
	Optnumber = {136},
	Title = {Measuring treatment effects using semiparametric models},
	Year = {2003}}

@article{Angristetal&Imbens&Rubin96,
	Author = {J. Angrist and G. Imbens and D.B. Rubin},
	Journal = {Journal of the American Statistical Association},
	Pages = {444-555},
	Title = {Identification of causal effects using instrumental variables},
	Volume = {91},
	Year = {1996}}

@article{Robins&Rotnitzky01A,
	Author = {J.M Robins and A. Rotnitzky},
	Journal = {Statistica Sinica},
	Pages = {920-935},
	Title = {Comment on {I}nference for Semiparametric Models: Some Questions and an Answer, by {B}ickel, {P}.{J}. and {K}won, {J}.},
	Volume = {11},
	Year = {2001}}

@article{Rubin96,
	Author = {D.B. Rubin},
	Journal = {Journal of the American Statistical Association},
	Month = {June},
	Number = {434},
	Pages = {473-89},
	Title = {Multiple Imputation After 18+ Years},
	Volume = {91},
	Year = {1996}}

@article{Angrist01,
	Author = {J. Angrist},
	Journal = {Journal of Business and Economics Statistics},
	Pages = {1--16},
	Title = {Estimation of limited dependent variable models with dummy endogenous regressors: simple strategies for empirical practice},
	Volume = {19},
	Year = {2001}}

@article{Chamberlain87,
	Author = {G. Chamberlain},
	Journal = {Journal of Econometrics},
	Pages = {305--334},
	Title = {Asymptotic efficiency in estimation with conditional moment restrictions},
	Volume = {34},
	Year = {1987}}

@article{Hiranoetal00,
	Author = {K. Hirano and G. Imbens and D.B. Rubin and X-H. Zhou},
	Journal = {Biostatistics},
	Pages = {69--88},
	Title = {Assessing the effects of influenza vaccine in an encouragement design},
	Volume = {1},
	Year = {2000}}

@inproceedings{Robins05,
	Author = {J.M. Robins},
	Booktitle = {Proceedings of the 2nd Seattle symposium in biostatistics},
	Editor = {Lin, D.Y, Heagerty P.J},
	Optpublisher = {Springer-Verlag Lecture Notes in Statistics},
	Pages = {189--326},
	Title = {Optimal structural nested models for optimal sequential decisions},
	Volume = {179},
	Year = {2005}}

@techreport{Robins05b,
	Author = {J.M. Robins},
	Institution = {Department of Biostatistics, Havard University},
	Title = {Optimal structural nested models for optimal sequential decisions},
	Year = {2005}}

@inproceedings{Akaike73,
	Author = {H. Akaike},
	Booktitle = {Second International Symposium on Information Theory},
	Editor = {B.N. Petrov and F. Csaki},
	Organization = {Budapest: Academiai Kiado},
	Pages = {267-281},
	Title = {Information theory and an extension of the maximum likelihood principle},
	Year = {1973}}

@article{Balke&Pearl97,
	Author = {A. Balke and J. Pearl},
	Journal = {Journal of the American Statistical Association},
	Pages = {1172--1176},
	Title = {Bound on treatment effects from studies with imperfect compliance},
	Volume = {92},
	Year = {1997}}

@inproceedings{Balke&Pearl94,
	Author = {A. Balke and J. Pearl},
	Booktitle = {In Proceedings of the 12th National Conference on Artificial Intelligence},
	Optaddress = {Menlo Park, CA},
	Optpublisher = {MIT Press},
	Pages = {230--237},
	Title = {Counterfactual probabilities: Computational methods, bounds, and applications},
	Volume = {I},
	Year = {1994}}

@article{Ambroise&McLachlan02,
	Author = {C. Ambroise and G. J. McLachlan},
	Journal = PNAS,
	Number = {10},
	Pages = {6562--6566},
	Title = {Selection bias in gene extraction on the basis of microarray gene-expression data},
	Volume = {99},
	Year = {2002}}

@incollection{Arabie&Hubert96,
	Address = {River Edge, NJ},
	Author = {P. Arabie and L. J. Hubert},
	Booktitle = {Clustering and Classification},
	Editor = {P. Arabie and L. J. Hubert and G. De Soete},
	Pages = {5--63},
	Publisher = {World Scientific Publishing Co.},
	Title = {An overview of combinatorial data analysis},
	Year = {1996}}

@article{Schwartz78,
	Author = {G. Schwartz},
	Journal = {The Annals of Statistics},
	Pages = {461-464},
	Title = {Estimating the Dimension of a Model},
	Volume = {6},
	Year = {1978}}

@article{Barnard35,
	Author = {M. Barnard},
	Journal = {Annals of Eugenics},
	Pages = {352--371},
	Title = {The secular variations of skull characters in four series of Egyptian skulls},
	Volume = {6},
	Year = {1935}}

@inproceedings{BenHur&Elisseeff&Guyon02,
	Author = {A. Ben-Hur and A. Elisseeff and I. Guyon},
	Booktitle = {Pacific Symposium on Biocomputing},
	Pages = {6--17},
	Title = {A stability based method for discovering structure in clustered data},
	Volume = {7},
	Year = {2002}}

@article{Benjamini&Hochberg95,
	Author = {Y. Benjamini and Y. Hochberg},
	Journal = {J. R. Statist. Soc. B},
	Pages = {289--300},
	Title = {Controlling the false discovery rate: a practical and powerful approach to multiple testing},
	Volume = {57},
	Year = {1995}}

@article{Benjamini&Yekutieli01,
	Author = {Y. Benjamini and D. Yekutieli},
	Journal = {The Annals of Statistics},
	Number = {4},
	Pages = {1165--1188},
	Title = {The control of the false discovery rate in multiple testing under dependency},
	Volume = {29},
	Year = {2001}}

@article{Beran88,
	Author = {R. Beran},
	Journal = JASA,
	Pages = {679--686},
	Title = {Balanced simultaneous confidence sets},
	Volume = {83},
	Year = {1988}}

@article{Bock85,
	Author = {H-H Bock},
	Journal = {Journal of Classification},
	Pages = {77--108},
	Title = {On some significance tests in cluster analysis},
	Volume = {2},
	Year = {1985}}

@incollection{Bock96,
	Address = {River Edge, NJ},
	Author = {H-H Bock},
	Booktitle = {Clustering and Classification},
	Editor = {P. Arabie and L. J. Hubert and G. De Soete},
	Pages = {377--453},
	Publisher = {World Scientific Publishing Co.},
	Title = {Probability models and hypotheses testing in partitioning cluster analysis},
	Year = {1996}}

@article{Boldricketal02,
	Author = {J. C. Boldrick and A. A. Alizadeh and M. Diehn and S. Dudoit and C. L. Liu and C. E. Belcher and D. Botstein and L. M. Staudt and P. O. Brown and D. A. Relman},
	Journal = PNAS,
	Number = {2},
	Pages = {972--977},
	Title = {Stereotyped and specific gene expression programs in human innate immue responses to bacteria},
	Volume = {99},
	Year = {2002}}

@article{Bozdogan00,
	Author = {H. Bozdogan},
	Journal = {Journal of Mathematical Psychology},
	Pages = {62-91},
	Title = {Akaike's information criterion and recent developments in information complexity},
	Volume = {44},
	Year = {2000}}

@incollection{Bozdogan93,
	Author = {H. Bozdogan},
	Booktitle = {Information and Classification},
	Editor = {O. Opitz and B. Lausen and R. Klar},
	Publisher = {Heidelberg: Springer-Verlag},
	Title = {Choosing the number of component clusters in the mixture model using a new informational complexity criterion of the inverse Fisher information matrix},
	Year = {1993}}

@article{Braver,
	Author = {S. L. Braver},
	Journal = {Educational and Psychological Measurement},
	Pages = {283--301},
	Title = {On splitting the tails unequally: a new perspective on one-versus two-tailed tests},
	Volume = {35},
	Year = {1975}}

@article{Breckenridge89,
	Author = {J. Breckenridge},
	Journal = {Multivariate Behavioral Research},
	Pages = {147--161},
	Title = {Replicating cluster analysis: Method, consistency and validity},
	Volume = {24},
	Year = {1989}}

@article{Breiman&Spector92,
	Author = {L. Breiman and P. Spector},
	Journal = {International Statistical Review},
	Pages = {291--319},
	Title = {Submodel Selection and Evaluation in Regression. The $X$ Random Case},
	Volume = {60},
	Year = {1992}}

@article{Breiman01,
	Author = {L. Breiman},
	Journal = {Statistical Science},
	Number = {3},
	Pages = {199--215},
	Title = {Statistical modeling: the two cultures},
	Volume = {16},
	Year = {2001}}

@article{Breiman96,
	Author = {L. Breiman},
	Journal = {The Annals of Statistics},
	Number = {6},
	Pages = {2350--2383},
	Title = {Heuristics of instability and stabilization in model selection},
	Volume = {24},
	Year = {1996}}

@article{Breiman98,
	Author = {L. Breiman},
	Journal = {The Annals of Statistics},
	Pages = {801-824},
	Title = {Arcing classifiers},
	Volume = {26},
	Year = {1998}}

@article{Breiman96b,
	Author = {L. Breiman},
	Journal = {Machine Learning},
	Pages = {123-140},
	Title = {Bagging predictors},
	Volume = {24},
	Year = {1996}}

@techreport{Breiman98b,
	Author = {L. Breiman},
	Institution = {Department of Statistics, U.C. Berkeley},
	Month = {March},
	Number = {513},
	Title = {Using Convex pseudo-data to increase prediction accuracy},
	Year = {1998}}

@article{Breiman92,
	Author = {L. Breiman},
	Journal = JASA,
	Number = {419},
	Pages = {738--754},
	Title = {The Little Bootstrap and Other Methods for Dimensionality Selection in Regression: $X$-Fixed Prediction Error},
	Volume = {87},
	Year = {1992}}

@techreport{Breiman96c,
	Author = {L. Breiman},
	Institution = {Department of Statistics, U.C. Berkeley},
	Title = {Out-of-bag estimation},
	Year = {1996}}

@techreport{Breiman99,
	Author = {L. Breiman},
	Institution = {Department of Statistics, U.C. Berkeley},
	Number = {567},
	Title = {Random forests - random features},
	Year = {1999}}

@book{Little&Rubin87,
	Author = { R.J.A. Little and D. B. Rubin},
	Publisher = {Wiley},
	Series = {Wiley Series in Probability and Mathematical Statistics},
	Title = {Statistical Analysis With Missing Data},
	Year = {1987}}

@book{Breimanetal84,
	Author = {L. Breiman and J. H. Friedman and R. Olshen and C. J. Stone},
	Publisher = {Wadsworth International Group},
	Series = {The Wadsworth statistics/probability series},
	Title = {Classification and regression trees},
	Year = {1984}}

@book{Hastie&Tibshirani&Friedman02,
	Author = {T. Hastie and R. Tibshirani and J. Friedman},
	Publisher = {Springer},
	Series = {Springer Series in Statistics},
	Title = {The Elements of Statistical Learning},
	Year = {2002}}

@article{Broman01,
	Author = {K. W. Broman},
	Journal = {Lab Animal},
	Number = {7},
	Pages = {44--52},
	Title = {Review of statistical methods for QTL mapping in experimental crosses},
	Volume = {30},
	Year = {2001}}

@phdthesis{Broman97,
	Author = {K. W. Broman},
	School = {Department of Statistics, U.C. Berkeley},
	Title = {Identifying quantitative trait loci in experimental crosses},
	Type = {Ph.{D}. thesis},
	Year = {1997}}

@article{Brown&Koplowitz79,
	Author = {T. A. Brown and J. Koplowitz},
	Journal = {IEEE Transactions on Information Theory},
	Number = {5},
	Pages = {617--619},
	Title = {The weighted nearest neighbor rule for class dependent sample sizes},
	Volume = {25},
	Year = {1979}}

@article{Buhlmann&Yu,
	Author = {P. Buhlmann and B. Yu},
	Journal = {The Annals of Statistics},
	Title = {Explaining Bagging.},
	Year = {(Accepted)}}

@article{Burges98,
	Author = {C. J. C. Burges},
	Journal = {Data Mining and Knowledge Discovery},
	Month = {December},
	Pages = {121--167},
	Title = {A tutorial on support vector machines for pattern recognition},
	Volume = {2},
	Year = {1998}}

@article{Burman89,
	Author = {P. Burman},
	Journal = {Biometrika},
	Pages = {503-514},
	Title = {A comparative study of ordinary cross-validation, $v$-fold cross-validati on and the repeated learning testing methods},
	Volume = {76},
	Year = {1989}}

@techreport{Buttrey&Karo02,
	Author = {S. E. Buttrey and C. Karo},
	Institution = {Naval Postgraduate School, Monterey, CA},
	Title = {Using k--neareset neighbor classification in the leaves of a tree},
	Year = {2002}}

@article{Calinski&Harabasz74l,
	Author = {R. Calinski and J. Harabasz},
	Journal = {Communications in Statistics},
	Pages = {1--27},
	Title = {A dendrite method for cluster analysis},
	Volume = {3},
	Year = {1974}}

@article{Callowetal00,
	Author = {M. J. Callow and S. Dudoit and E. L. Gong and T. P. Speed and E. M. Rubin},
	Journal = {Genome Research},
	Number = {12},
	Pages = {2022--2029},
	Title = {Microarray expression profiling identifies genes with altered expression in {HDL} deficient mice},
	Volume = {10},
	Year = {2000}}

@book{Chambers98,
	Author = {J. M. Chambers},
	Publisher = {Springer-Verlag New York},
	Title = {Programming with Data: A Guide to the S Language},
	Year = {1998}}

@book{Diggleetal02,
	Author = {Peter J. Diggle and P. Heagerty and K-Y Liang and S.L. Zeger},
	Publisher = {Oxford University Press},
	Title = {Analysis of Longitudinal Data},
	Year = {2002 (Second Edition)}}

@techreport{Chang&Lin01,
	Author = {C.-C. Chang and C.-J. Lin},
	Note = {\\ {\tt http://www.csie.ntu.edu.tw/~cjlin/papers/libsvm2.ps.gz}},
	Title = {{LIBSVM}: a Library for Support Vector Machines (Version 2.31)},
	Year = {2001}}

@article{Changetal02,
	Author = {H. Y. Chang and J. T. Chi and S. Dudoit and C. Bondre and M. van de Rijn and D. Botstein D and P. O. Brown},
	Journal = PNAS,
	Number = {20},
	Pages = {12877--12882},
	Title = {Diversity, topographic differentiation, and positional memory in human fibroblasts},
	Volume = {99},
	Year = {2002}}

@article{Chenetal02,
	Author = {X. Chen and S. T. Cheung and S. So and S. T. Fan and C. Barry and J. Higgins and K.-M. Lai and J. Ji and S. Dudoit and I. O. L. Ng and M. van de Rijn and D. Botstein and P. O. Brown},
	Journal = {Molecular Biology of the Cell},
	Number = {6},
	Pages = {1929--1939},
	Title = {Gene expression patterns in human liver cancers},
	Volume = {13},
	Year = {2002}}

@incollection{Cleveland&Grosse&Shyu92,
	Author = {W. S. Cleveland, E. Grosse and W. M. Shyu},
	Booktitle = {Statistical Models in S},
	Chapter = {6},
	Editor = {J. M. Chambers and T. J. Hastie},
	Publisher = {Wadsworth \& Brooks/Cole},
	Title = {Local regression models},
	Year = 1992}

@article{Cleveland&Devlin88,
	Author = {W. S. Cleveland and S. J. Devlin},
	Journal = JASA,
	Pages = {596--610},
	Title = {Locally-Weighted Regression: An Approach to Regression Analysis by Local Fitting},
	Volume = {83},
	Year = {1988}}

@article{Cleveland79,
	Author = {W. S. Cleveland},
	Journal = JASA,
	Number = {368},
	Pages = {829--836},
	Title = {Robust locally weighted regression and smoothing scatterplots},
	Volume = {74},
	Year = {1979}}

@article{Correa&Wolfson99,
	Author = {J. A. Correa and D. B. Wolfson},
	Journal = {Journal of Statistical Computation and Simulation},
	Pages = {209--219},
	Title = {Length-bias: some characterizations and applications},
	Tnumber = {3},
	Volume = {64},
	Year = {1999}}

@article{Correa&Dudoit&Goldstein02,
	Author = {J. A. Correa and S. Dudoit and D. R. Goldstein},
	Note = {(Submitted)},
	Optjournal = {Statistics in Medicine},
	Title = {Multiple testing in the survival analysis of microarray data},
	Year = {2002}}

@article{Cortes&Vapnik95,
	Author = {C. Cortes and V. Vapnik},
	Journal = {Machine Learning},
	Month = {December},
	Pages = {273-297},
	Title = {Support-vector networks},
	Volume = {20},
	Year = {1995}}

@inproceedings{Davies&Bouldin79,
	Author = {D. Davies and D. Bouldin},
	Booktitle = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
	Optnumber = {PAMI-1},
	Pages = {224--227},
	Title = {A cluster separation measure},
	Volume = {1},
	Year = {1979}}

@article{Davis&Anderson89,
	Author = {R. B. Davis and J. R. Anderson},
	Journal = {Statistics in Medicine},
	Pages = {947-961},
	Title = {Exponential survival trees},
	Volume = {8},
	Year = {1989}}

@incollection{Day96,
	Address = {River Edge, NJ},
	Author = {W. H. E. Day},
	Booktitle = {Clustering and Classification},
	Editor = {P. Arabie and L. J. Hubert and G. De Soete},
	Pages = {199--233},
	Publisher = {World Scientific Publishing Co.},
	Title = {Complexity theory: {A}n introduction for practitioners of classification},
	Year = {1996}}

@article{Dettling&Buhlmann02,
	Author = {M. Dettling and P. B\"{u}hlmann},
	Title = {How to Use Boosting for Tumor Classification with Gene Expression Data},
	Year = {2002}}

@article{Dudoit&Fridlyand02,
	Author = {S. Dudoit and J. Fridlyand},
	Optjournal = {Bioinformatics},
	Title = {Bagging to improve the accuracy of a clustering procedure},
	Year = {2002}}

@incollection{Dudoit&Fridlyand02b,
	Author = {S. Dudoit and J. Fridlyand},
	Booktitle = {Statistical Analysis of Gene Expression Microarray Data},
	Editor = {T. P. Speed},
	Note = {(To appear)},
	Publisher = {Chapman \& Hall/CRC},
	Title = {Classification in microarray experiments},
	Year = {2002}}

@article{Dudoit&Fridlyand02c,
	Author = {S. Dudoit and J. Fridlyand},
	Journal = {Genome Biology},
	Number = {7},
	Pages = {0036.1--0036.21},
	Title = {A prediction-based resampling method to estimate the number of clusters in a dataset},
	Volume = {3},
	Year = {2002}}

@techreport{Dudoit&Fridlyand01,
	Author = {S. Dudoit and J. Fridlyand},
	Institution = {Department of Statistics, Uiversity of California, Berkeley},
	Number = {600},
	Title = {Applications of resampling methods to estimate the number of clusters and to improve the accuracy of a clustering method},
	Url = {stat-www.berkeley.edu/users/sandrine/publications.html},
	Year = {2001},
	Bdsk-Url-1 = {stat-www.berkeley.edu/users/sandrine/publications.html}}

@article{Dudoit&vanderLaan05,
	Author = {S. Dudoit and M.J. van der Laan},
	Journal = {Statistical Methodology},
	Number = {2},
	Optnote = {www.bepress.com/ucbbiostat/paper126},
	Pages = {131--154},
	Title = {Asymptotics of cross-validated risk estimation in estimator selection and performance assessment},
	Volume = {2},
	Year = {2005}}

@article{Dudoit&Speed99,
	Author = {S. Dudoit and T. P. Speed},
	Journal = {The Annals of Statistics},
	Number = {3},
	Pages = {943--986},
	Title = {A score test for linkage using identity by descent data from sibships},
	Volume = {27},
	Year = {1999}}

@article{Dudoit&Speed00,
	Author = {S. Dudoit and T. P. Speed},
	Journal = {Biostatistics},
	Number = {1},
	Pages = {1--26},
	Title = {A score test for the linkage analysis of qualitative and quantitative traits based on identity by descent data on sib-pairs},
	Volume = {1},
	Year = {2000}}

@incollection{Dudoit&Speed99b,
	Address = {New York},
	Author = {S. Dudoit and T. P. Speed},
	Booktitle = {Statistics in Genetics},
	Editor = {M. E. Halloran and S. Geisser},
	Pages = {181--221},
	Publisher = {Springer-Verlag},
	Series = {IMA Volumes in Mathematics and its Applications},
	Title = {Triangle constraints for sib-pair identity by descent probabilities under a general multilocus model for disease susceptibility},
	Volume = {112},
	Year = {1999}}

@incollection{Dudoit&Yang03,
	Author = {S. Dudoit and Y. H. Yang},
	Booktitle = {The Analysis of Gene Expression Data: Methods and Software},
	Editor = {G. Parmigiani and E. S. Garrett and R. A. Irizarry and S. L. Zeger},
	Publisher = {Springer-Verlag, New York},
	Title = {Bioconductor {R} packages for exploratory analysis and normalization of c{DNA} microarray data},
	Year = {2003}}

@article{Dudoit&Fridlyand&Speed02,
	Author = {S. Dudoit and J. Fridlyand and T. P. Speed},
	Journal = JASA,
	Number = {457},
	Pages = {77--87},
	Title = {Comparison of Discrimination Methods for the Classification of Tumors Using Gene Expression Data},
	Volume = {97},
	Year = {2002}}

@article{Dudoitetal02,
	Author = {S. Dudoit and Y. H. Yang and M. J. Callow and T. P. Speed},
	Journal = {Statistica Sinica},
	Number = {1},
	Pages = {111--139},
	Title = {Statistical methods for identifying differentially expressed genes in replicated c{DNA} microarray experiments},
	Volume = {12},
	Year = {2002}}

@techreport{Dudoit&Shaffer&Boldrick02,
	Author = {S. Dudoit and J. P. Shaffer and J. C. Boldrick},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {110},
	Title = {Multiple hypothesis testing in microarray experiments},
	Url = {www.bepress.com/ucbbiostat/paper110/},
	Year = {2002},
	Bdsk-Url-1 = {www.bepress.com/ucbbiostat/paper110/}}

@article{Duffy&Quiroz91,
	Author = {D. E. Duffy and A. J. Quiroz},
	Journal = {Journal of Classification},
	Pages = {65--91},
	Title = {A permutation-based algorithm for block clustering},
	Volume = {8},
	Year = {1991}}

@article{Dunn58,
	Author = {O. J. Dunn},
	Journal = {Annals of Mathematical Statistics},
	Pages = {1095-111},
	Title = {Estimation of the means of dependent variables},
	Volume = {29},
	Year = {1958}}

@book{Efron&Tibshirani93,
	Author = {B. Efron and R. J. Tibshirani},
	Publisher = {Chapman \& Hall/CRC},
	Title = {An Introduction to the Bootstrap},
	Year = {1993}}

@article{EfronetalJASA01,
	Author = {B. Efron and R. Tibshirani and J. D. Storey and V. Tusher},
	Journal = JASA,
	Pages = {1151--1160},
	Title = {Empirical Bayes analysis of a microarray experiment},
	Volume = {96},
	Year = {2001}}

@techreport{Efron&Storey&Tibshirani01,
	Author = {B. Efron and J. D. Storey and R. Tibshirani},
	Institution = {Department of Statistics, Stanford University},
	Number = {2001-218},
	Title = {Microarrays, empirical Bayes methods, and false discovery rates},
	Year = {2001}}

@article{Finner99,
	Author = {H. Finner},
	Journal = {The Annals of Statistics},
	Pages = {274--289},
	Title = {Stepwise multiple test procedures and control of directional errors},
	Volume = {27},
	Year = {1999}}

@article{Fisher36,
	Author = {R. A. Fisher},
	Journal = {Annals of Eugenics},
	Pages = {179-188},
	Title = {The use of multiple measurements in taxonomic problems},
	Volume = {7},
	Year = {1936}}

@article{Fisher26,
	Author = {R. A. Fisher},
	Journal = {J. Min. Agric. Gr. Br},
	Pages = {505--513},
	Title = {The arrangement of field experiments},
	Volume = {33},
	Year = {1926}}

@techreport{Fix&Hodges51,
	Author = {E. Fix and J. Hodges},
	Institution = {Randolph Field, Texas: USAF School of Aviation Medicine},
	Title = {Discriminatory analysis, nonparametric discrimination: consistency properties},
	Year = {1951}}

@article{Fowlkes&Mallows83,
	Author = {E. B. Fowlkes and C. L. Mallows},
	Journal = JASA,
	Optnumber = {383},
	Pages = {553--584},
	Title = {A method for comparing two hierarchical clusterings},
	Volume = {78},
	Year = {1983}}

@article{Fowlkes&Gnanadesikan&Kettenring88,
	Author = {E. B. Fowlkes and R. Gnanadesikan and J. R. Kettenring},
	Journal = JC,
	Pages = {205--228},
	Title = {Variable selection in clustering},
	Volume = {5},
	Year = {1988}}

@techreport{Fraley&Raftery98,
	Author = {C. Fraley and A. Raftery},
	Institution = {Department of Statistics, University of Washington},
	Note = {\url{http://www.stat.washington.edu/www/research/reports/1990s/#1998}},
	Number = {329},
	Title = {How many clusters? Which clustering method? -- answers via model-based cluster analysis},
	Year = {1998}}

@article{Freund&Schapire97,
	Author = {Y. Freund and R. E. Schapire},
	Journal = {Journal of Computer and System Sciences},
	Pages = {119--139},
	Title = {A decision-theoretic generalization of on-line learning and an application to boosting},
	Volume = {55},
	Year = {1997}}

@phdthesis{Fridlyand01,
	Author = {J. Fridlyand},
	School = {Department of Statistics, U.C. Berkeley},
	Title = {Resampling methods for variable selection and classification: applications to genomics},
	Type = {Ph.{D}. thesis},
	Year = {2001}}

@article{Friedman91,
	Abstract = {A new method is presented for flexible regression modeling of high dimensional data. The model takes the form of an expansion in product spline basis functions, where the number of basis functions as well as the parameters associated with each one (product degree and knot locations) are automatically determined by the data. This procedure is motivated by the recursive partitioning approach to regression and shares its attractive properties. Unlike recursive partitioning, however, this method produces continuous models with continuous derivatives. It has more power and flexibility to model relationships that are nearly additive or involve interactions in at most a few variables. In addition, the model can be represented in a form that separately identifies the additive contributions and those associated with the different multivariable interactions.},
	Author = {Friedman, Jerome H.},
	Copyright = {Copyright � 1991 Institute of Mathematical Statistics},
	Issn = {00905364},
	Journal = {The Annals of Statistics},
	Jstor_Formatteddate = {Mar., 1991},
	Language = {English},
	Number = {1},
	Pages = {pp. 1-67},
	Publisher = {Institute of Mathematical Statistics},
	Title = {Multivariate Adaptive Regression Splines},
	Url = {http://www.jstor.org/stable/2241837},
	Volume = {19},
	Year = {1991},
	Bdsk-Url-1 = {http://www.jstor.org/stable/2241837}}

@techreport{Friedman93,
	Author = {J. H. Friedman},
	Institution = {Department of Statistics, Stanford University},
	Title = {Fast {MARS}},
	Year = {1993}}

@techreport{Friedman94,
	Author = {J. H. Friedman},
	Institution = {Department of Statistics, Stanford University},
	Title = {Flexible metric nearest neighbor classification},
	Year = {1994}}

@techreport{Friedman96a,
	Author = {J. H. Friedman},
	Institution = {Department of Statistics, Stanford University},
	Title = {On bias, variance, 0/1-loss, and the curse--of--dimensionality},
	Year = {1996}}

@techreport{Friedman96b,
	Author = {J. H. Friedman},
	Institution = {Department of Statistics, Stanford University},
	Title = {Another approach to polychotomous classification},
	Year = {1996}}

@article{Friedman&Hastie&Tibshirani00,
	Author = {J. Friedman and T. Hastie and R. Tibshirani},
	Journal = {The Annals of Statistics},
	Note = {(with discussion)},
	Pages = {337--404},
	Title = {Additive logistic regression: a statistical view of boosting},
	Volume = {28},
	Year = {2000}}

@book{Hastie&Tibshirani90,
	Address = {London},
	Author = {T. J. Hastie and R.J. Tibshirani},
	Publisher = {Chapman and Hall},
	Title = {Generalized Additive Models},
	Year = {1990}}

@article{Gabriel71,
	Author = {K. R. Gabriel},
	Journal = {Biometrika},
	Pages = {453--467},
	Title = {The biplot graphic display of matrices with application to principal component analysis},
	Volume = {58},
	Year = {1971}}

@incollection{Gabriel75,
	Author = {K. R. Gabriel},
	Booktitle = {Multivariate Statistical Methods: Among-groups covariation; Within-group covariation},
	Pages = {61--80},
	Title = {A comparison of some methods of simultaneous inference in {MANOVA}},
	Year = {1975}}

@inproceedings{Gabriel&Pun79,
	Author = {K. R. Gabriel and F. C. Pun},
	Booktitle = {Sixth Conference on Probability and Statistics in Atmospheric Science},
	Organization = {American Meterological Society},
	Pages = {248--253},
	Title = {Binary prediction of weather events with several predictors},
	Year = {1979}}

@unpublished{Ge&Dudoit02,
	Author = {Y. Ge and S. Dudoit},
	Note = {(In preparation)},
	Title = {Fast algorithm for resampling-based $p$-value adjustment in multiple testing},
	Year = {2002}}

@article{Geisser75,
	Author = {S. Geisser},
	Journal = {Journal of the American Statistical Association},
	Pages = {320-328},
	Title = {The predictive sample reuse method with applications},
	Volume = {70},
	Year = {1975}}

@techreport{Genovese&Wasserman01,
	Author = {C. Genovese and L. Wasserman},
	Institution = {Department of Statistics, Carnegie Mellon},
	Number = {737},
	Title = {Operating Characteristics and Extensions of the FDR Procedure},
	Year = {2001}}

@article{Gnanadesikan&Kettenring95,
	Author = {R. Gnanadesikan and J. R. Kettenring},
	Journal = JC,
	Pages = {113--136},
	Title = {Weighting and selection of variables for cluster analysis},
	Volume = {12},
	Year = {1995}}

@article{Goldstein&Dudoit&Speed00,
	Author = {D. R. Goldstein and S. Dudoit and T. P. Speed},
	Journal = {Genetic Epidemiology},
	Number = {Suppl. 1},
	Pages = {S85--S91},
	Title = {Power of a score test for quantitative trait linkage analysis of relative pairs.},
	Volume = {19},
	Year = {2000}}

@article{Goldstein&Dudoit&Sped01,
	Author = {D. R. Goldstein and S. Dudoit and T. P. Speed},
	Journal = {Genetic Epidemiology},
	Number = {4},
	Pages = {415--431},
	Title = {Power and robustness of a score test for linkage analysis of quantitative traits using identity by descent data on sib pairs},
	Volume = {20},
	Year = {2001}}

@article{Gordon&Olshen85,
	Author = {L. Gordon and R.A. Olshen},
	Journal = {Cancer Treatment Reports},
	Pages = {10065-1069},
	Title = {Tree-structured survival analysis},
	Volume = {69},
	Year = {1985}}

@incollection{Gordon96,
	Address = {River Edge, NJ},
	Author = {A. D. Gordon},
	Booktitle = {Clustering and Classification},
	Editor = {P. Arabie and L. J. Hubert and G. De Soete},
	Pages = {65--121},
	Publisher = {World Scientific Publishing Co.},
	Title = {Hierarchical classification},
	Year = {1996}}

@book{Gower&Hand96,
	Author = {J. C. Gower and D. J. Hand},
	Edition = {1st},
	Number = {54},
	Publisher = {Chapman \& Hall},
	Series = {Monographs on statistics and applied probability},
	Title = {Biplots},
	Year = {1996}}

@book{Gyorfietal02,
	Address = {New York},
	Author = {L. Gy\"{o}rfi and M. Kohler and A. Krzy\.{z}ak and H. Walk},
	Pages = {100-102},
	Publisher = {Springer-Verlag},
	Title = {A Distribution-Free Theory of Nanparametric Regression},
	Year = {2002}}

@book{Gyorfietal02b,
	Author = {L. Gy\"orfi and M. Kohler and A. Krzy\'{z}ak and H. Walk},
	Publisher = {Springer-Verlag, New York},
	Title = {A distribution-free theory of nonparametric regression},
	Year = {2002}}

@book{Hastie&Tibshirani&Friedman01,
	Author = {T. Hastie and R. Tibshirani and J. H. Friedman},
	Publisher = {Springer-Verlag},
	Title = {The Elements of Statistical Learning : Data Mining, Inference, and Prediction},
	Year = {2001}}

@article{Hansen&Yu01,
	Author = {M. H. Hansen and B. Yu},
	Journal = {Journal of the American Statistical Association},
	Pages = {746-774},
	Title = {Model selection and the principle of minimum description length},
	Volume = {96},
	Year = {2001}}

@article{Hardle&Marron85a,
	Author = {W. H{\"a}rdle and J. S. Marron},
	Journal = {Biometrika},
	Pages = {481--484},
	Title = {Asymptotic nonequivalence of some bandwidth selectors in nonparametric regression},
	Volume = {72},
	Year = {1985}}

@article{Hardle&Marron85b,
	Author = {W. H{\"a}rdle and J. S. Marron},
	Journal = {The Annals of Statistics},
	Pages = {1465-1481},
	Title = {Optimal bandwidth selection in nonparametric regression function estimation},
	Volume = {13},
	Year = {1985}}

@book{Hardle93,
	Author = {W. H{\"a}rdle},
	Publisher = {Cambridge University Press},
	Title = {Applied Nonparametric Regression},
	Year = {1993}}

@article{Hartigan72,
	Author = {J. A. Hartigan},
	Journal = {Journal of the American Statistical Association},
	Pages = {123--129},
	Title = {Direct clustering of a data matrix},
	Volume = {67},
	Year = {1972}}

@book{Hartigan75,
	Author = {J. A. Hartigan},
	Publisher = {Wiley},
	Title = {Clustering Algorithms},
	Year = {1975}}

@article{Hartigan78,
	Author = {J. Hartigan},
	Journal = {The Annals of Statistics},
	Pages = {117--131},
	Title = {Asymptotic distributions for clustering criteria},
	Volume = {6},
	Year = {1978}}

@article{Hartigan85,
	Author = {J. A. Hartigan},
	Journal = JC,
	Pages = {63--76},
	Title = {Statistical theory in clustering},
	Volume = {2},
	Year = {1985}}

@incollection{Hastie&Pregibon92,
	Author = {T.J. Hastie and D. Pregibon},
	Booktitle = {Statistical Models in S},
	Chapter = {6},
	Editor = {J. M. Chambers and T. J. Hastie},
	Publisher = {Wadsworth \& Brooks/Cole},
	Title = {Generalized linear models},
	Year = {1992}}

@article{Hastie&Tibshirani96a,
	Author = {T. Hastie and R. Tibshirani},
	Journal = {IEEE Pattern Recognition and Machine Intelligence},
	Pages = {607--616},
	Title = {Discriminant adaptive nearest-nieghbor classification},
	Volume = {18},
	Year = {1996}}

@techreport{Hastie&Tibshirani96b,
	Author = {T. Hastie and R. Tibshirani},
	Institution = {Department of Statistics, Stanford University},
	Title = {Classification by pairwise coupling},
	Year = {1996}}

@article{Hastie&Tibshirani90b,
	Author = {T.J. Hastie and R.J. Tibshirani},
	Date-Modified = {2011-02-22 20:11:53 -0800},
	Journal = {Biometrics},
	Number = {4},
	Pages = {1005-1016},
	Title = {Exploring the nature of covariate effects in the proportional hazar ds model},
	Volume = {46},
	Year = {1990}}

@e{Hochberg&Tamhane87,
	Author = {Y. Hochberg and A. C. Tamhane},
	Publisher = {Wiley--Interscience},
	Series = {Probability and Mathematical Statistics},
	Title = {Multiple Comparison Procedures},
	Year = {1987}}

@article{Hochberg88,
	Author = {Y. Hochberg},
	Journal = {Biometrika},
	Pages = {800--802},
	Title = {A sharper Bonferroni procedure for multiple tests of significance},
	Volume = {75},
	Year = {1988}}

@article{Holm79,
	Author = {S. Holm},
	Journal = {Scand. J. Statist.},
	Pages = {65--70},
	Title = {A simple sequentially rejective multiple test procedure},
	Volume = {6},
	Year = {1979}}

@article{Hommel&Bernhard99,
	Author = {G. Hommel and G. Bernhard},
	Journal = {Journal of Statistical Planning and Inference},
	Pages = {119--128},
	Title = {Bonferroni procedures for logically related hypotheses},
	Volume = {82},
	Year = {1999}}

@article{Hommel88,
	Author = {G. Hommel},
	Journal = {Biometrika},
	Pages = {383--386},
	Title = {A stagewise rejective multiple test procedure based on a modified Bonferroni test},
	Volume = {75},
	Year = {1988}}

@article{Hubert&Arabie85,
	Author = {L. Hubert and P. Arabie},
	Journal = JC,
	Pages = {193--218},
	Title = {Comparing partitions},
	Volume = {2},
	Year = {1985}}

@book{Jain&Dubes88,
	Address = {Englewood Cliffs, N. J.},
	Author = {A. K. Jain and R. C. Dubes},
	Publisher = {Prentice-Hall},
	Title = {Algorithms for Clustering Data},
	Year = {1988}}

@article{Jogdeo77,
	Author = {K. Jogdeo},
	Journal = {The Annals of Statistics},
	Pages = {495--504},
	Title = {Association and probability inequalities},
	Volume = {5},
	Year = {1977}}

@book{Kaufman&Rousseeuw90,
	Author = {L. Kaufman and P. J. Rousseeuw},
	Publisher = {Wiley, New York.},
	Title = {Finding Groups in Data: An Introduction to Cluster Analysis},
	Year = {1990}}

@article{Keles&vanderLaan&Dudoit03,
	Author = {Kele\c{s}, S. and van der Laan, M. and Dudoit, S.},
	Journal = {Technical Report, Division of Biostatistics, UC Berkeley},
	Title = {Asymptotically Optimal Model Selection Method for Regression on Censored Outcomes},
	Year = {2002}}

@article{Kohonen90,
	Author = {T. Kohonen},
	Journal = {Proc. IEEE},
	Number = {9},
	Pages = {1464--1480},
	Title = {The self-organizing map},
	Volume = {78},
	Year = {1990}}

@book{Kohonen95,
	Address = {Berlin, Heidelberg},
	Author = {T. Kohonen},
	Editor = {T. S. Huang and T. Kohonen and M. R. Schroeder},
	Publisher = {Springer-Verlag},
	Series = {Springer Series in Information Sciences},
	Title = {Self-Organizing Maps},
	Volume = {30},
	Year = {1995}}

@article{Kooperberg&Stone&Truong95,
	Author = {C. Kooperberg and C.J. Stone and Y. K. Truong},
	Journal = {Journal of the American Statistical Association},
	Number = {429},
	Pages = {78-94},
	Title = {Hazard Regression},
	Volume = {90},
	Year = {1995}}

@article{Koutsoukosetal94,
	Author = {A. D. Koutsoukos and L. V. Rubinstein and D. Faraggi and R.M. Simon and S. Kalyandrug and J. N. Weinstein and K.W. Kohn and K.D. Paull},
	Journal = {Statistics in Medicine},
	Pages = {719--730},
	Title = {Discrimination techniques applied to the {NCI} in vitro anti-tumor drug screen: predicting biochemical mechanism of action},
	Volume = {13},
	Year = {1994}}

@article{Krishnaiah&Reising85,
	Author = {P. R. Krishnaiah and J. M. Reising},
	Journal = {Encyclopedia of Statistical Sciences},
	Number = {6},
	Pages = {88--95},
	Title = {Multivariate multiple comparisons},
	Volume = {9},
	Year = {1985}}

@article{Krzanowski&Lai85,
	Author = {W. Krzanowski and Y. Lai},
	Journal = {Biometrics},
	Pages = {23--34},
	Title = {A criterion for determining the number of groups in a dataset using sum of squares clustering},
	Volume = {44},
	Year = {1985}}

@article{Laan&Bryan01,
	Author = {M. J. van der Laan and J. Bryan},
	Journal = {Biostatistics},
	Number = {4},
	Pages = {445--461},
	Title = {Gene expression analysis with the parametric bootstrap},
	Volume = {2},
	Year = {2001}}

@article{Pollard&vanderLaan04,
	Author = {K. S. Pollard and M.J. van der Laan},
	Journal = JSPI,
	Optpages = {85--101},
	Optvolume = {125},
	Title = {Choice of Null Distribution in Resampling Based Multiple Testing},
	Year = {2004}}

@article{vanderLaan&Pollard02,
	Author = {M. J. van der Laan and K. S. Pollard},
	Journal = JSPI,
	Note = {(To appear)},
	Title = {Hybrid clustering of gene expression data with visualization and the bootstrap},
	Year = {2002}}

@article{Leblanc&Crowley92,
	Author = {M. Leblanc and J. Crowley},
	Journal = {Biometrics},
	Pages = {411-425},
	Title = {Relative Risk trees for censored data},
	Volume = {48},
	Year = {1992}}

@inproceedings{Leisch02,
	Author = {F. Leisch},
	Booktitle = {Compstat 2002 --- Proceedings in Computational Statistics},
	Editor = {Wolfgang H{\"a}rdle and Bernd R{\"o}nz},
	Note = {ISBN 3-7908-1517-9},
	Publisher = {Physika Verlag, Heidelberg, Germany},
	Title = {Sweave: Dynamic Generation of Statistical Reports Using Literate Data Analysis},
	Tpages = {575--580},
	Url = {http://www.ci.tuwien.ac.at/~leisch/Sweave},
	Year = {2002},
	Bdsk-Url-1 = {http://www.ci.tuwien.ac.at/~leisch/Sweave}}

@techreport{Leisch02Tb,
	Author = {F. Leisch},
	Institution = {SFB Adaptive Information Systems and Modelling in Economics and Management Science, Vienna University of Economics and Business Administration},
	Month = {March},
	Number = {69},
	Title = {Dynamic generation of statistical reports using literate data analysis},
	Year = {2002}}

@techreport{Leisch99,
	Author = {F. Leisch},
	Institution = {SFB Adaptive Information Systems and Modelling in Economics and Management Science, Vienna University of Economics and Business Administration},
	Month = {August},
	Note = {\url{http://www.ci.tuwien.ac.at/~leisch/papers/fl-techrep.html}},
	Title = {Bagged clustering},
	Year = {1999}}

@article{Lim&Low&Shih00,
	Author = {T-S Lim and W-Y Loh and Y-S Shih},
	Journal = {Machine Learning},
	Pages = {203--229},
	Title = {A comparison of prediction accuracy, complexity, and training time of thiry-three old and new classification algorithms},
	Volume = {40},
	Year = {2000}}

@book{Mardia&Kent&Bibby79,
	Address = {San Diego},
	Author = {K. V. Mardia and J. T. Kent and J. M. Bibby},
	Publisher = {Academic Press, Inc.},
	Title = {Multivariate Analysis},
	Year = {1979}}

@unpublished{Mayo&Spanos02,
	Author = {D. C. Mayo and A. Spanos},
	Title = {A severe-testing interpretation of {N}eyman-{P}earson methods. Unpublished manuscript},
	Year = {2002}}

@book{McCullagh&Nelder89,
	Author = {P. McCullagh and J. A. Nelder},
	Edition = {2nd},
	Number = {37},
	Publisher = {Chapman \& Hall},
	Series = {Monographs on Statistics and Applied Probability},
	Title = {Generalized Linear Models},
	Year = {1989}}

@book{McLachlan92,
	Address = {New York},
	Author = {G. J. McLachlan},
	Publisher = {Wiley},
	Title = {Discriminant analysis and statistical pattern recognition},
	Year = {1992}}

@article{McLachlan&Bean&Peel01,
	Author = {G. J. McLachlan and R. Bean and D. Peel},
	Journal = {Bioinformatics},
	Pages = {413--422},
	Title = {A mixture model-based approach to the clustering of microarray expression data.},
	Volume = {18},
	Year = {2002}}

@book{Miller90,
	Author = {A. J. Miller},
	Publisher = {Chapman and Hall},
	Title = {Subset Selection in Regression},
	Year = {1990}}

@article{Milligan&Cooper85,
	Author = {G. W. Milligan and M. C. Cooper},
	Journal = {Psychometrika},
	Pages = {159--179},
	Title = {An examination of procedures for determining the number of clusters in a data set},
	Volume = {50},
	Year = {1985}}

@article{Milligan&Cooper86,
	Author = {G. W. Milligan and M. C. Cooper},
	Journal = {Multivariate Behavioral Research},
	Pages = {441--458},
	Title = {A study of the comparability of external criteria for hierarchical cluster analysis},
	Volume = {21},
	Year = {1986}}

@article{Milligan&Cooper87,
	Author = {G. W. Milligan and M. C. Cooper},
	Journal = {Applied Psychological Measurement},
	Optmonth = {December},
	Optnumber = {4},
	Pages = {329--354},
	Title = {Methodology review: {C}lustering methods},
	Volume = {11},
	Year = {1987}}

@article{Milligan89,
	Author = {G. W. Milligan},
	Journal = {Multivariate Behavioral Research},
	Pages = {163--176},
	Title = {A study of the beta-flexible clustering method},
	Volume = {24(2)},
	Year = {1989}}

@incollection{Milligan96,
	Address = {River Edge, NJ},
	Author = {G. W. Milligan},
	Booktitle = {Clustering and Classification},
	Editor = {P. Arabie and L. J. Hubert and G. De Soete},
	Pages = {341--375},
	Publisher = {World Scientific Publishing Co.},
	Title = {Clustering validation: {R}esults and implications for applied analyses},
	Year = {1996}}

@article{Morey&Blashfield&Skinnerl83,
	Author = {L. C. Morey, R. K. Blashfield and H. A. Skinner},
	Journal = {Multivariate Behavioral Research},
	Pages = {309--329},
	Title = {A comparison of cluster analysis techniques within a sequential validation framework},
	Volume = {18},
	Year = {1983}}

@book{Morrison90,
	Author = {D. F. Morrison},
	Edition = {3rd},
	Publisher = {McGraw-Hill, NY},
	Title = {Multivariate Statistical Methods},
	Year = {1990}}

@incollection{Murtagh96,
	Address = {River Edge, NJ},
	Author = {F. Murtagh},
	Booktitle = {Clustering and Classification},
	Editor = {P. Arabie and L. J. Hubert and G. De Soete},
	Pages = {235--269},
	Publisher = {World Scientific Publishing Co.},
	Title = {Neural networks for clustering},
	Year = {1996}}

@article{PanelDACC89,
	Author = {{Panel on Discriminant Analysis, Classification, and Clustering}},
	Journal = {Statistical Science},
	Pages = {34--69},
	Title = {Discriminant analysis and clustering},
	Volume = {4},
	Year = {1989}}

@techreport{Pavlic&vanderLaan89,
	Author = {M. Pavlic and M. J. van der Laan},
	Institution = {Division of Biostatistics, U.C. Berkeley},
	Month = {February},
	Number = {89},
	Title = {Fitting of mixtures with unspecified number of components using cross-validation distance estimate},
	Year = {2001}}

@article{Pavlic&vanderLaan02,
	Author = {M. Pavlic and M. J. van der Laan},
	Issue = {3-4},
	Journal = {Computational Statistics and Data Analysis},
	Pages = {413-428},
	Title = {Fitting of mixtures with unspecified number of components using cross validation distance estimate},
	Volume = {41},
	Year = {2003}}

@techreport{Pollard&vanderLaan02,
	Author = {K. S. Pollard and M. J. van der Laan},
	Institution = {Division of Biostatistics, U.C. Berkeley},
	Month = {April},
	Number = {107},
	Title = {A Method to Identify Significant Clusters in Gene Expression Data},
	Year = {2002}}

@techreport{Pollard&vanderLaan02b,
	Author = {K. S. Pollard and M. J. van der Laan},
	Institution = {Division of Biostatistics, U.C. Berkeley},
	Number = {121},
	Title = {Resampling-based methods for identification of significant subsets of genes in expression data},
	Year = {2002}}

@article{Ramsey78,
	Author = {P. H. Ramsey},
	Journal = JASA,
	Pages = {479--485},
	Title = {Power differences between pairwise multiple comparisons},
	Volume = {73},
	Year = {1978}}

@manual{Breiman01b,
	Author = {L. Breiman},
	Title = {Notes on setting up, using, and understanding random forests V3.0},
	Year = {2001}}

@article{Rand71,
	Author = {W. M. Rand},
	Journal = {Journal of the American Statistical Association},
	Optnumber = {336},
	Pages = {846--850},
	Title = {Objective criteria for the evaluation of clustering methods},
	Volume = {66},
	Year = {1971}}

@unpublished{Reiner&Yekutieli&Benjaminil01,
	Author = {A. Reiner and D. Yekutieli and Y. Benjamini},
	Title = {Using resampling-based {FDR} controlling multiple test procedures for analyzing microarray gene expression data},
	Year = {2001}}

@book{Ripley96,
	Address = {Cambridge, New York},
	Author = {B. D. Ripley},
	Publisher = {Cambridge University Press},
	Title = {Pattern recognition and neural networks},
	Year = {1996}}

@book{Rosner99,
	Address = {Pacific Grove, CA},
	Author = {B. Rosner},
	Publisher = {Duxbury Press},
	Title = {Fundamentals of Biostatistics, 5th Ed.},
	Year = {1999}}

@misc{FEVdata,
	Author = {B. Rosner},
	Note = {Submitted by M.J. Kahn, Wheaton College, Norton, MA},
	Optnote = {accessed 12/20/2010},
	Title = {FEV dataset},
	Year = {1999}}

@article{Kahn05,
	Author = {M. Kahn},
	Journal = {The Journal of Statistical Education},
	Number = {2},
	Title = {An Exhalent Problem for Teaching Statistics},
	Volume = {13},
	Year = {2005}}

@article{Rissanen78,
	Author = {J. Rissanen},
	Journal = {Automatica},
	Pages = {465-471},
	Title = {Modelling by shortest data description},
	Volume = {14},
	Year = {1978}}

@article{Rnews:Dudoit&Yang&Bolstad02,
	Author = {S. Dudoit and Y. H. Yang and B. Bolstad},
	Journal = {R News},
	Month = {March},
	Number = 1,
	Pages = {24--32},
	Title = {Using {R} for the Analysis of {DNA} Microarray Data},
	Url = {CRAN.R-project.org/doc/Rnews/},
	Volume = 2,
	Year = 2002,
	Bdsk-Url-1 = {CRAN.R-project.org/doc/Rnews/}}

@article{Robins&Rotnitzky00,
	Author = {J. M. Robins and A. Rotnitzky},
	Journal = {Statistica Sinica},
	Number = {4},
	Pages = {920-936},
	Title = {Comment on the {B}ickel and {K}won article, `{I}nference for Semiparametric Models: {S}ome Questions and an Answer'},
	Volume = {11},
	Year = {2001}}

@inproceedings{Robins00,
	Author = {J.M. Robins},
	Booktitle = {Proceedings of the American Statistical Association},
	Title = {Robust estimation in sequentially ignorable missing data and causal inference models},
	Year = {2000}}

@article{Robins00a,
	Author = {J. M. Robins and A. Rotnitzky},
	Journal = {Statistica Sinica},
	Number = {4},
	Pages = {920-936},
	Title = {Comment on the {B}ickel and {K}won article, `{I}nference for Semiparametric Models: {S}ome Questions and an Answer'},
	Volume = {11},
	Year = {2001}}

@article{Rubin74,
	Author = {D.B. Rubin},
	Journal = {Journal of Educational Psychology},
	Pages = {688-701},
	Title = {Estimating Causal Effects of Treatments in Randomized and Nonrandomized Studies},
	Volume = {64},
	Year = {1974}}

@article{Robins00b,
	Author = {J. M. Robins and A. Rotnitzky and M.J. van der Laan},
	Journal = {Journal of the American Statistical Association -- Theory and Methods},
	Pages = {431-435},
	Title = {Comment on ``{O}n {P}rofile {L}ikelihood" by {S}.{A}. {M}urphy and {A}.{W}. van der {V}aart},
	Volume = {450},
	Year = {2000}}

@article{hernan_brumback_robins,
	Author = {Hernan, M. A. and Brumback, B. and Robins, J. M.},
	Journal = {Epidemiology},
	Number = {5},
	Pages = {561--570},
	Title = {Marginal Structural Models to Estimate the Causal Effect of Zidovudine on the Survival of {HIV}-Positive Men},
	Volume = {11},
	Year = {2000}}

@article{Robins&Rotnitzky&vanderLaan00,
	Author = {J. M. Robins and A. Rotnitzky and M.J. van der Laan},
	Journal = {Journal of the American Statistical Association -- Theory and Methods},
	Pages = {431-435},
	Title = {Comment on ``{O}n {P}rofile {L}ikelihood" by {S}.{A}. {M}urphy and {A}.{W}. van der {V}aart},
	Volume = {450},
	Year = {2000}}

@article{Birge83,
	Author = {L. Birg{\'e}},
	Journal = {Verw. Gebiete},
	Pages = {181--238},
	Title = {Approximation dans les espaces m{/'e}triques et th{\'e}orie de l'estimation},
	Volume = {65},
	Year = {1983}}

@article{lecam73,
	Author = {L.M. le Cam},
	Journal = {The Annals of Statistics},
	Pages = {38--53},
	Title = {Convergence of estimates under dimensionality restrictions},
	Volume = {22},
	Year = {1973}}

@article{Rom90,
	Author = {D. M. Rom},
	Journal = {Biometrika},
	Pages = {663-665},
	Title = {A sequentially rejective test procedure based on a modified {Bonferroni} inequality},
	Volume = {77},
	Year = {1990}}

@techreport{Rosenblatt57,
	Author = {F. Rosenblatt},
	Institution = {Cornell Aeronautical Laboratory},
	Number = {86-460-1},
	Title = {The perceptron -- a perceiving and recognizing automation},
	Year = {1957}}

@article{Ruczinskietal&Kooperberg&LeBlanc01,
	Author = {I. Ruczinski and C. Kooperberg and M. LeBlanc},
	Note = {Submitted, \url{http://biosun01.biostat.jhsph.edu/~iruczins/html/publications.html}},
	Title = {Logic regression},
	Year = {2001}}

@article{Saltstone&Stange96,
	Author = {R. Saltstone and K. Stange},
	Journal = {Journal of Classification},
	Pages = {169--172},
	Title = {A computer program to calculate Hubert and Arabie's adjusted Rand index},
	Volume = {13},
	Year = {1996}}

@techreport{vanderVaart03,
	Author = {A.W. van der Vaart},
	Institution = {Department of Mathematics, Free University, Amsterdam},
	Optannote = {Unpublished manuscript},
	Title = {Notes on Cross-validation},
	Year = {2003}}

@techreport{Sarle83,
	Author = {W. Sarle},
	Institution = {SAS Institute, Inc.},
	Note = {\url{http://www.sas.com/service/library/onlinedoc/trindex.html}},
	Number = {A-108},
	Title = {Cubic clustering criterion},
	Year = {1983}}

@techreport{Sarle&Kuo93,
	Author = {W. Sarle and A. Kuo},
	Institution = {SAS Institute, Inc.},
	Number = {P-256},
	Title = {The MODECLUS Procedures},
	Year = {1993}}

@article{Schapireetal98,
	Author = {R. E. Schapire and Y. Freund and P. Bartlett and W. S. Lee},
	Journal = {The Annals of Statistics},
	Pages = {1651--1686},
	Title = {Boosting the margin: a new explanation for the effectiveness of voting methods},
	Volume = {26},
	Year = {1998}}

@book{Scheffe59,
	Author = {H. Scheff\'{e}},
	Publisher = {John Wiley \& Sons},
	Title = {The analysis of variance},
	Year = {1959}}

@article{Scheibler&Schneider85,
	Author = {D. Scheibler and W. Schneider},
	Journal = {Multivariate Behavioral Research},
	Pages = {283--304},
	Title = {Monte Carlo tests of the accuracy of cluster analysis algorithms: A comparison of hierarchical and nonhierarchical methods},
	Volume = {20},
	Year = {1985}}

@inproceedings{Schuster&Gregory81,
	Author = {E. F. Schuster and C. G. Gregory},
	Booktitle = {Computer Science and Statistics: Proceedings of the 13th Symposium on the interface},
	Editor = {Eddy, W.F.},
	Pages = {295-298},
	Title = {On the non-consistency of maximum likelihood nonparametric density estimators},
	Year = {1981}}

@article{Scott&Factor81,
	Author = {D. W. Scott and L. E. Factor},
	Journal = {Journal of the American Statistical Association},
	Pages = {9-15},
	Title = {Monte Carlo study of three data-based nonparametric density estimators},
	Volume = {76},
	Year = {1981}}

@article{Seeger68,
	Author = {P. Seeger},
	Journal = {Technometrics},
	Number = {3},
	Pages = {586--593},
	Title = {A note on a method for the analysis of significances en masse},
	Volume = {10},
	Year = {1968}}

@article{Segal88,
	Author = {M. R. Segal},
	Journal = {Biometrics},
	Pages = {35--47},
	Title = {Regression trees for censored data},
	Volume = {44},
	Year = {1988}}

@article{Shaffer02,
	Author = {J. P. Shaffer},
	Journal = {Psychological Methods},
	Pages = {356--369},
	Title = {Multiplicity, directional ({T}ype {III}) errors, and the null hypothesis},
	Volume = {7},
	Year = {2002}}

@article{Shaffer86,
	Author = {J. P. Shaffer},
	Journal = JASA,
	Pages = {826--831},
	Title = {Modified sequentially rejective multiple test procedures},
	Volume = {81},
	Year = {1986}}

@article{Shaffer95,
	Author = {J. P. Shaffer},
	Journal = {Annu. Rev. Psychol.},
	Pages = {561--584},
	Title = {Multiple hypothesis testing},
	Volume = {46},
	Year = {1995}}

@article{Shao93,
	Author = {Shao, J.},
	Journal = {Journal of the American Statistical Association},
	Pages = {486-494},
	Title = {Linear Model Selection by Cross-Validation},
	Volume = {88},
	Year = {1993}}

@article{Sidak67,
	Author = {Z. \v{S}id\'{a}k},
	Journal = JASA,
	Pages = {626-633},
	Title = {Rectangular confidence regions for the means of multivariate normal distributions},
	Volume = {62},
	Year = {1967}}

@article{Silverman96,
	Author = {B. W. Silverman},
	Journal = {The Annals of Statistics},
	Pages = {1--24},
	Title = {Smoothed functional principal components analysis by choice of norm},
	Volume = {24},
	Year = {1996}}

@article{Silverman84,
	Author = {B. W. Silverman},
	Journal = JASA,
	Number = {387},
	Pages = {584--589},
	Title = {A fast and efficient cross-validation method for smoothing parameter choice in spline regression},
	Volume = {79},
	Year = {1984}}

@book{Silverman86,
	Author = {B. W. Silverman},
	Publisher = {Chapman \& Hall},
	Title = {Density Estimation for Statistics and Data analysis},
	Year = {1986}}

@article{vanderLaan&Dudoit&Keles04,
	Author = {M.J. van der Laan and S. Dudoit and S. Keles},
	Journal = {Statistical Applications in Genetics and Molecular Biology},
	Optnote = {http://www.bepress.com/sagmb/vol3/iss1/art4},
	Optnumber = {1},
	Title = {Asymptotic optimality of likelihood-based cross-validation},
	Volume = {3},
	Year = {2004}}

@article{Simes86,
	Author = {R. J. Simes},
	Journal = {Biometrika},
	Pages = {751--754},
	Title = {An improved Bonferroni procedure for multiple tests of significance},
	Volume = {73},
	Year = {1986}}

@article{Smyth00,
	Author = {P. Smyth},
	Journal = {Statistics and Computing},
	Pages = {63-72},
	Title = {Model selection of probabilistic clustering using cross-validated likelihood},
	Volume = {10},
	Year = {2000}}

@article{Soric89,
	Author = {B. Sori\'{c}},
	Journal = JASA,
	Number = {406},
	Pages = {608--610},
	Title = {Statistical ``discoveries" and effect-size estimation},
	Volume = {84},
	Year = {1989}}

@article{Stone84,
	Author = {C. J. Stone},
	Journal = {The Annals of Statistics},
	Number = {4},
	Pages = {1285--1297},
	Title = {An asymptotically optimal window selection rule for kernel density estimates},
	Volume = {12},
	Year = {1984}}

@article{Stone74,
	Author = {M. Stone},
	Journal = JRSSB,
	Number = {2},
	Pages = {111--147},
	Title = {Cross-validatory choice and assessment of statistics predictions},
	Volume = {36},
	Year = {1974}}

@article{Stone77,
	Author = {M. Stone},
	Journal = {Biometrika},
	Number = {1},
	Pages = {29--35},
	Title = {Asymptotics for and against cross-validation},
	Volume = {64},
	Year = {1977}}

@techreport{Storey&Tibshirani01,
	Author = {J. D. Storey and R. Tibshirani},
	Institution = {Department of Statistics, Stanford University},
	Number = {2001-28},
	Title = {Estimating false discovery rates under dependence, with applications to DNA microarrays},
	Year = {2001}}

@article{Storey02,
	Author = {J. D. Storey},
	Journal = JRSSB,
	Pages = {479--498},
	Title = {A direct approach to false discovery rates},
	Volume = {64},
	Year = {2002}}

@techreport{Storey01,
	Author = {J. D. Storey},
	Institution = {Department of Statistics, Stanford University},
	Number = {2001-12},
	Title = {The positive False Discovery Rate: A Bayesian interpretation and the q-value},
	Year = {2001}}

@book{Lehmann86,
	Author = {E. L. Lehmann},
	Edition = {2nd},
	Publisher = {Springer-Verlag, New York},
	Title = {Testing Statistical Hypotheses},
	Year = {1986}}

@article{Tibshiranietal02a,
	Author = {R. Tibshirani and T. Hastie and B. Narasimhan and. G. Chu},
	Journal = PNAS,
	Note = {In press},
	Title = {Diagnosis of multiple cancer types by shrunken centroids of gene expression},
	Year = {2002}}

@article{Troendle95,
	Author = {J. F. Troendle},
	Journal = JASA,
	Pages = {370--378},
	Title = {A stepwise resampling method of multiple hypothesis testing},
	Volume = {90},
	Year = {1995}}

@article{Troendle96,
	Author = {J. F. Troendle},
	Journal = {Biometrics},
	Pages = {846--859},
	Title = {A permutational step-up method of testing multiple outcomes},
	Volume = {52},
	Year = {1996}}

@book{vanderVaart&Wellner96,
	Author = {A. W. van der Vaart and J. A. Wellner},
	Pages = {102},
	Publisher = {Springer-Verlag New York},
	Title = {Weak {C}onvergence and {E}mprical {P}rocesses},
	Year = {1996}}

@book{vanderVaart98,
	Author = {A. W. van der Vaart},
	Pages = {62},
	Publisher = {Cambridge University Press},
	Title = {Asymptotic Statistics},
	Year = {1998}}

@book{Vapnik00,
	Address = {New York},
	Author = {V. N. Vapnik},
	Edition = {2nd},
	Publisher = {Springer-Verlag},
	Series = {Statistics for engineering and information science},
	Title = {The nature of statistical learning theory},
	Year = {2000}}

@article{Vapnik79,
	Author = {V. Vapnik},
	Journal = {Nauka, Moskow},
	Title = {Estimation of dependences based on empirical data (in Russian)},
	Year = {1979}}

@book{Vapnik98,
	Address = {New York},
	Author = {V. Vapnik},
	Edition = {1st},
	Publisher = {Wiley},
	Title = {Statistical Learning Theory},
	Year = {1998}}

@book{Venables&Ripley99,
	Author = {W. N. Venables and B. D. Ripley},
	Edition = {3rd},
	Publisher = {Springer-Verlag},
	Title = {Modern applied statistics with S-PLUS},
	Year = {1999}}

@book{Venables&Ripley02,
	Address = {New York},
	Author = {W. N. Venables and B. D. Ripley},
	Edition = {4th},
	Publisher = {Springer-Verlag},
	Title = {Modern Applied Statistics with S},
	Year = {2002}}

@book{Westfall&Young93,
	Author = {P. H. Westfall and S. S. Young},
	Publisher = {John Wiley \& Sons},
	Title = {Resampling-based multiple testing: {E}xamples and methods for $p$-value adjustment},
	Year = {1993}}

@incollection{Westfalletal&Zaykin&Young01,
	Author = {P. H. Westfall and D. V. Zaykin and S. S. Young},
	Booktitle = {Biostatistical Methods},
	Editor = {S. Looney},
	Pages = {143--168},
	Publisher = {Humana Press, Toloway, NJ},
	Series = {Methods in Molecular Biology},
	Title = {Multiple tests for genetic effects in association studies},
	Volume = {184},
	Year = {2001}}

@article{Westonetal2000,
	Author = {J. Weston and S. Mukherjee and O. Chappelle and M. Pontil and T. Poggio and V. Vapnik},
	Journal = {Advances in Neural Processing Systems},
	Pages = {668--674},
	Title = {Feature Selection for {SVM}s},
	Volume = {13},
	Year = {2001}}

@article{Wright92,
	Author = {S. P. Wright},
	Journal = {Biometrics},
	Number = {4},
	Pages = {1005--1013},
	Title = {Adjusted P-values for simultaneous inference},
	Volume = {48},
	Year = {1992}}

@article{Yangetal02,
	Author = {Y. H. Yang and M. J. Buckley and S. Dudoit and T. P. Speed},
	Journal = {Journal of Computational and Graphical Statistics},
	Number = {1},
	Pages = {108--136},
	Title = {Comparison of methods for image analysis on c{DNA} microarray data},
	Volume = {11},
	Year = {2002}}

@article{Yangetal02b,
	Author = {Y. H. Yang and S. Dudoit and P. Luu and D. M. Lin and V. Peng and J. Ngai and T. P. Speed},
	Journal = {Nucleic Acids Research},
	Number = {4},
	Pages = {e15},
	Title = {Normalization for c{DNA} microarray data: {A} robust composite method addressing single and multiple slide systematic variation},
	Volume = {30},
	Year = {2002}}

@inproceedings{Yangetal01,
	Address = {San Jose, CA},
	Author = {Y. H. Yang and S. Dudoit and P. Luu and T. P. Speed},
	Booktitle = {Microarrays: Optical Technologies and Informatics},
	Editor = {Michael L. Bittner and Yidong Chen and Andreas N. Dorsel and Edward R. Dougherty},
	Month = {May},
	Optorganization = {SPIE},
	Pages = {141--152},
	Publisher = {SPIE-International Society for Optical Engineering},
	Series = {Proceedings of SPIE},
	Title = {Normalization for c{DNA} microarray data},
	Volume = {4266},
	Year = {2001}}

@article{Yekutieli&Benjamini99,
	Author = {D. Yekutieli and Y. Benjamini},
	Journal = JSPI,
	Pages = {171--196},
	Title = {Resampling-based false discovery rate controlling multiple test procedures for correlated test statistics},
	Volume = {82},
	Year = {1999}}

@incollection{Youden69,
	Author = {W. J. Youden},
	Booktitle = {Precision measurement and calibration: Statistical concepts and procedures},
	Editor = {H. H. Ku},
	Month = {February},
	Pages = {146--151},
	Publisher = {National Bureau of Standards, United States Department of Commerce},
	Series = {Special Publication 300},
	Title = {Measurement agreement comparisons},
	Type = {NBS Miscelaneous Publication 248, Proceedings of the 1962 Standards Laboratory Conference},
	Volume = {1},
	Year = {1969}}

@article{Zhang93,
	Author = {Zhang, P.},
	Journal = {The Annals of Statistics},
	Pages = {299-313},
	Title = {Model selection via multifold cross-validation},
	Volume = {21},
	Year = {1993}}

@article{Zhang&Carey&Gentleman02,
	Author = {J. Zhang and V. Carey and R. Gentleman},
	Journal = {Bioinformatics},
	Note = {(In press)},
	Title = {An extensible application for assembling annotation for genomic data},
	Url = {http://www.R-project.org/},
	Year = {2002},
	Bdsk-Url-1 = {http://www.R-project.org/}}

@article{Gradyetal09,
	Author = {D. Grady and J. Macer and M. Kristof and H. Shen and M. Tagliaferri and J. Creasman},
	Issue = {5},
	Journal = {Menopause},
	Pages = {932-6},
	Title = {Is a shorter hot flash diary just as good as a 7-day diary?},
	Volume = {16},
	Year = {2009}}

@book{Bickeletal97,
	Author = {P.J. Bickel and C.A.J. Klaassen and Y. Ritov and J. Wellner},
	Publisher = {Springer-Verlag},
	Title = {Efficient and Adaptive Estimation for Semiparametric Models},
	Year = {1997}}

@book{vanderLaan&Robins03,
	Author = {M.J. van der Laan and J.M. Robins},
	Publisher = {Springer-Verlag, New York},
	Title = {Unified Methods for Censored Longitudinal Data and Causality},
	Year = {2003}}

@manual{effsize,
	Author = {{National Reading Panel}},
	Organization = {National Institute of Child Health and Human Development, National Institutes of Health},
	Title = {Teaching Children to Read},
	Year = {1999}}

@techreport{Tibshirani&Walther&Hastie00,
	Author = {R. Tibshirani and G. Walther and T. Hastie.},
	Institution = {Department of Biostatistics, Stanford University},
	Month = {March},
	Note = {\url{http://www-stat.stanford.edu/~tibs/research.html}},
	Title = {Estimating the number of clusters in a dataset via the gap statistic},
	Year = {2000}}

@inproceedings{Gill&vanderLaan&Robins97,
	Address = {New York},
	Author = {R.D. Gill and M.J. van der Laan and J.M. Robins},
	Booktitle = {Proceedings of the First Seattle Symposium in Biostatistics},
	Editor = {D.Y. Lin and T.R. Fleming},
	Pages = {255-94},
	Publisher = {Springer-Verlag},
	Title = {Coarsening At Random: Characterizations, Conjectures and Counter-Examples},
	Year = {1997}}

@article{Gill&Robins01,
	Author = {Gill, R. and Robins, J.M.},
	Fjournal = {The Annals of Statistics},
	Journal = {Ann. Stat.},
	Number = {6},
	Title = {Causal inference in complex longitudinal studies: continuous case},
	Volume = {29},
	Year = {2001}}

@article{Jacobsen&Keiding95,
	Author = {M. Jacobsen and N. Keiding},
	Journal = {The Annals of Statistics},
	Pages = {774-86},
	Title = {Coarsening at Random in General Sample Spaces and Random Censoring in Continuous Time},
	Volume = {23},
	Year = {1995}}

@misc{Dudoit&Yang02,
	Author = {S. Dudoit and Y. H. Yang},
	Howpublished = {{\tt R} packages},
	Title = {Normalization and diagnostic plots for cDNA microarray data, {\tt marrayClasses}, {\tt marrayInput}, {\tt marrayNorm}, {\tt marrayPlots}},
	Url = {www.bioconductor.org},
	Year = {2002},
	Bdsk-Url-1 = {www.bioconductor.org}}

@techreport{Fraley&Raftery98b,
	Author = {C. Fraley and A. E. Raftery},
	Date-Modified = {2011-02-22 20:11:02 -0800},
	Institution = {Department of Statistics, University of Washington},
	Month = {November},
	Number = {342},
	Title = {MCLUST: Software for Model-Based Cluster Analysis},
	Year = {1998}}

@misc{Ge&Dudoit02b,
	Author = {Y. Ge and S. Dudoit},
	Date-Modified = {2011-02-22 20:11:23 -0800},
	Howpublished = {{\tt R} package},
	Title = {Multiple Testing Procedures, {\tt multtest}},
	Url = {www.bioconductor.org},
	Year = {2002},
	Bdsk-Url-1 = {www.bioconductor.org}}

@article{Robins&Rotnitzky95,
	Author = {J.M. Robins and A. Rotnitzky},
	Journal = {Journal of the American Statistical Association},
	Month = {March},
	Number = {429},
	Pages = {122-9},
	Title = {Semiparametric Efficiency in Multivariate Regression Models with Missing Data},
	Volume = {90},
	Year = {1995}}


@inproceedings{Robins93,
	Author = {J.M. Robins},
	Booktitle = {Proceeding of the Biopharmaceutical section},
	Organization = {American Statistical Association},
	Pages = {24-33},
	Title = {Information recovery and bias adjustment in proportional hazards regression analysis of randomized trials using surrogate markers},
	Year = {1993}}

@incollection{Robins&Rotnitzky92,
	Author = {J.M. Robins and A. Rotnitzky},
	Booktitle = {AIDS Epidemiology},
	Publisher = {Bikh\"{a}user},
	Series = {Methodological issues},
	Title = {Recovery of information and adjustment for dependent censoring using surrogate markers},
	Year = {1992}}

@article{Robins&Rotnitzky&Zhao94,
	Author = {J.M. Robins and A. Rotnitzky and L.P. Zhao},
	Journal = {Journal of the American Statistical Association},
	Month = {September},
	Number = {427},
	Pages = {846-66},
	Title = {Estimation of regression coefficients when some regressors are not always observed},
	Volume = {89},
	Year = {1994}}

@article{Hubbard&vanderLaan08,
	Author = {A.E. Hubbard and M.J. van der Laan},
	Journal = {Biometrika},
	Number = {1},
	Pages = {35-47},
	Title = {Population intervention models in causal inference},
	Volume = {95},
	Year = {2008}}

@article{Heitjan&Rubin91,
	Author = {D.F. Heitjan and D.B. Rubin},
	Journal = {The Annals of Statistics},
	Month = {December},
	Number = {4},
	Pages = {2244-2253},
	Title = {Ignorability and Coarse Data},
	Volume = {19},
	Year = {1991}}

@misc{Dudoit&Yang&Bolstad01,
	Author = {S. Dudoit and Y. H. Yang and B. M. Bolstad},
	Howpublished = {{\tt R} package},
	Note = {Contributions from Natalie Thorne, Ingrid L\"{o}nnstedt, and Jessica Mar},
	Title = {Statistical {M}icroarray {A}nalysis, {\tt sma}},
	Url = {cran.r-project.org/src/contrib/PACKAGES.html\#sma},
	Year = {2001},
	Bdsk-Url-1 = {cran.r-project.org/src/contrib/PACKAGES.html%5C#sma}}

@phdthesis{Dudoit99,
	Author = {S. Dudoit},
	School = {Department of Statistics, University of California, Berkeley},
	Title = {Linkage analysis of complex human traits using identity by descent data},
	Type = {Ph.D. thesis},
	Year = {1999}}

@article{Rosenblum&vanderLaan10,
	Author = {M. Rosenblum and M.J. van der Laan},
	Journal = {The International Journal of Biostatistics},
	Number = {19},
	Title = {Targeted Maximum Likelihood Estimation of the Parameter of a Marginal Structural Model},
	Volume = {6},
	Year = {2010}}

@article{Gruber&vanderLaan10a,
	Author = {S. Gruber and M.J. van der Laan},
	Issue = {26},
	Journal = {The International Journal of Biostatistics},
	Number = {1},
	Title = {A Targeted Maximum Likelihood Estimator of a Causal Effect on a Bounded Continuous Outcome},
	Volume = {6},
	Year = {2010}}

@article{Gruber&vanderLaan10b,
	Author = {S. Gruber and M.J. van der Laan},
	Issue = {18},
	Journal = {The International Journal of Biostatistics},
	Number = {1},
	Title = {An Application of Collaborative Targeted Maximum Likelihood Estimation in Causal Inference and Genomics},
	Volume = {6},
	Year = {2010}}

@unpublished{bhattacharya.vogt.zbias,
	Author = {Bhattacharya, J. and Vogt, W},
	Note = {NBER Technical Working Paper 343, National Bureau of Economic Research, MA.},
	Title = {Do Instrumental Variables Belong in Propensity Scores?},
	Year = {2007}}

@unpublished{wooldridge.zbias,
	Author = {Wooldridge, J.},
	Note = {Tech.\ Rep.\ Michigan State University, MI.},
	Title = {Should Instrumental Variables be Used as Matching Variables?},
	Year = {2009}}

@article{pearl.zbias,
	Author = {Pearl, Judea},
	Journal = {Proceedings of UAI},
	Note = {forthcoming},
	Title = {On a Class of Bias-Amplifying Variables that Endanger Effect Estimates},
	Year = {2010}}

@unpublished{Bhattacharya&Vogt07,
	Author = {Bhattacharya, J. and Vogt, W},
	Note = {NBER Technical Working Paper 343, National Bureau of Economic Research, MA.},
	Title = {Do Instrumental Variables Belong in Propensity Scores?},
	Year = {2007}}

@unpublished{Wooldridge09,
	Author = {Wooldridge, J.},
	Note = {Tech.\ Rep.\ Michigan State University, MI.},
	Title = {Should Instrumental Variables be Used as Matching Variables?},
	Year = {2009}}

@article{Bang&Robins05,
	Author = {Bang, H. and J. M. Robins},
	Journal = {Biometrics},
	Pages = {962-72},
	Title = {Doubly Robust Estimation in Missing Data and Causal Inference Models},
	Volume = {61},
	Year = {2005}}

@article{Pearl10,
	Author = {Pearl, J.},
	Journal = {Proceedings of UAI},
	Note = {forthcoming},
	Title = {On a Class of Bias-Amplifying Variables that Endanger Effect Estimates},
	Year = {{2010}}}

@article{Scharfstein&Rotnitzky&Robins99,
	Author = {Scharfstein, D.O. and Rotnitzky, A. and Robins, J.M.},
	Journal = {Journal of the American Statistical Association},
	Number = {448},
	Pages = {1096-1120 (1121-1146)},
	Title = {Adjusting for Non-Ignorable Drop-out Using Semiparametric Nonresponse Models, (with Discussion and Rejoinder)},
	Volume = {94},
	Year = {{1999}}}

@article{Scharfstein99,
	Author = {Scharfstein, D.O. and Rotnitzky, A. and Robins, J.M.},
	Journal = {Journal of the American Statistical Association},
	Number = {448},
	Pages = {1096-1120 (1121-1146)},
	Title = {Adjusting for Non-Ignorable Drop-out Using Semiparametric Nonresponse Models, (with Discussion and Rejoinder)},
	Volume = {94},
	Year = {{1999}}}

@article{Robins1999,
	Author = {Robins, J.M.},
	Journal = {Statistics in Medicine},
	Number = {21},
	Pages = {1663-1680},
	Title = {Commentary on Using Inverse Weighting and Predictive Inference to Estimate the Effecs of Time-Varying Treatments on the Discrete-time Hazard},
	Year = {{1999}}}

@techreport{Wang06,
	Author = {Y. Wang and M. Petersen and D. Bangsberg and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {211},
	Optnote = {http://www.bepress.com/ucbbiostat/paper211},
	Opturl = {www.bepress.com/ucbbiostat/paper211/},
	Title = {Diagnosing Bias in the Inverse Probability of Treatment Weighted Estimator Resulting from Violation of Experimental Treatment Assignment.},
	Year = {2006}}

@techreport{Moore09,
	Author = {K.L. Moore and R.S. Neugebauer and M.J. van der Laan and I.B. Tager},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {255},
	Optmonth = {Oct},
	Title = {Causal Inference in Epidemiological Studies with Strong Confounding},
	Url = {www.bepress.com/ucbbiostat/paper255/},
	Year = {2009},
	Bdsk-Url-1 = {www.bepress.com/ucbbiostat/paper255/}}

@article{Cole&Hernan08,
	Author = {S.R. Cole and M.A. Hernan},
	Journal = {American Journal of Epidemiology},
	Pages = {656-664},
	Title = {Constructing Inverse Probability Weights for Marginal Structural Models},
	Volume = {168},
	Year = {2008}}

@article{Kish92,
	Author = {L. Kish},
	Journal = {Journal of Official Statistics},
	Pages = {183--200},
	Title = {Weighting for unequal {P}$_i$},
	Volume = {8},
	Year = {1992}}

@techreport{Bembom.trunc,
	Author = {O. Bembom and M.J. van der Laan},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Number = {230},
	Title = {Data-adaptive selection of the truncation level for Inverse-Probability-of-Treatment-Weighted estimators},
	Url = {www.bepress.com/ucbbiostat/paper230/},
	Year = {2008},
	Bdsk-Url-1 = {www.bepress.com/ucbbiostat/paper230/}}

@article{Ridgeway&McCaffrey07,
	Author = {G. Ridgeway and D.F. McCaffrey},
	Journal = {Statistical Science},
	Pages = {540-443},
	Title = {Comment: Demystifying Double Robustness: A Comparison of Alternative Strategies for Estimating a Population Mean from Incomplete Data},
	Volume = {22:4},
	Year = {2007}}

@article{Robinsetal1994b,
	Author = {J.M. Robins, A. Rotnitzky and L.P. Zhao},
	Journal = {J. Am. Statist. Assoc.},
	Pages = {846-66},
	Title = {Estimation of Regression Coefficients When Some Regressors are Not Always Observed},
	Volume = {89},
	Year = {1994}}

@article{Tan10,
	Author = {Z. Tan},
	Date-Modified = {2011-03-07 21:06:22 -0800},
	Journal = {Biometrika},
	Pages = {661-682},
	Title = {Bounded, efficient and doubly robust estimation with inverse weighting},
	Volume = {97,3},
	Year = {2010}}

@article{Tan06,
	Author = {Z. Tan},
	Date-Modified = {2011-03-07 21:06:16 -0800},
	Journal = {J. Am. Statist. Assoc.},
	Pages = {1619-37},
	Title = {A distributional approach for causal inference using propensity scores},
	Volume = {101},
	Year = {2006}}

@article{Cao&Tsiatis&Davidian09,
	Author = {W. Cao and A.A. Tsiatis and M. Davidian},
	Date-Modified = {2011-03-07 21:06:41 -0800},
	Journal = {Biometrika},
	Pages = {723-734},
	Title = {Improving efficiency and robustness of the doubly robust estimator for a population mean with incomplete data},
	Volume = {96,3},
	Year = {2009}}

@misc{Gruber&vanderLaanWNAR11,
	Author = {S. Gruber and M.J. van der Laan},
	Date-Added = {2011-12-08},
	Date-Modified = {2011-12-08},
	Howpublished = {WNAR 2011 Spring Meeting},
	Month = {June},
	Title = {Collaborative Targeted Maximum Likelihood Estimation},
	Year = {2011}}

@misc{Rotnitzky11,
	Author = {A. Rotnitzky},
	Date-Added = {2011-04-02 21:38:04 -0700},
	Date-Modified = {2011-04-02 21:41:08 -0700},
	Howpublished = {ENAR 2011 Spring Meeting},
	Month = {March},
	Title = {Enhanced Double-Robust Locally- Efficient Estimation in Regression Models for Longitudinal Studies},
	Year = {2011}}

@article{Gruber&vanderLaan12Outperforms,
	Author = {S. Gruber and M.J. van der Laan},
	Date-Modified = {2011-12-13 12:08:39 -0500},
	Journal = {The International Journal of Biostatistics},
	Volume = {8},
	Issue = {1},
	Title = {Targeted minimum loss based estimator that outperforms a given estimator},
	Year = {2012}}

@article{Wedderburn74,
	Author = {R.W.M. Wedderburn},
	Date-Modified = {2011-03-07 21:46:06 -0800},
	Issue = {3},
	Journal = {Biometrika},
	Title = {Quasi-likelihood functions, generalized linear models, and the {G}auss-{N}ewton method},
	Volume = {61},
	Year = {1974}}

@article{Robins&Wang2000,
	Author = {J.M. Robins and N. Wang},
	Journal = {Biometrika},
	Pages = {113-124},
	Title = {Inference for imputation estimators},
	Volume = {87},
	Year = {2000}}

@article{Petersen&Schwab&vanderLaan13,
  title={Targeted maximum likelihood estimation of dynamic and static marginal Structural Working Models},
  author={M. Petersen and J. Schwab and S. Gruber and N. Blaser and M. Schomaker and M.J. van der Laan},
  journal={Journal of Causal Inference},
  volume={2},
  Issue={2},
  pages={147--185},
  year={2013}
  note={DOI: https://doi.org/10.1515/jci-2013-0007},
  }









@article{Sobel06,
  title={What Do Randomized Studies of Housing Mobility Demonstrate? Causal Inference in the Face of Interference},
  author={M. Sobel},
  journal={Journal of the American Statistical Association},
  volume={101},
  pages={1398--1407},
  year={2006}
  }

@techreport{vanderLaan&Gruber11TR,
	Author = {M.J. van der Laan and S. Gruber},
	Institution = {Division of Biostatistics, University of California, Berkeley},
	Optnote = {http://www.bepress.com/ucbbiostat/paper290},
	Title = {Targeted Maximum Loss Based Estimation of an Intervention Specific Mean},
	Type = {Technical Report 290},
	Year = {2011}}
@article{Raudenbush&Bryk86,
  author = {S.W. Raudenbush and A.S. Bryk},
  title= {A hierarchical model
for studying school effects. Sociology of Education},
  journal = {Sociology of Education},
  volume = {59},
  issue = {},
  pages = {1--17},
  year = {1986}
}

@techreport{vanderLaan08,
	Author = {Mark J. van der Laan},
	Date-Added = {2008-03},
	Institution = {University of California, Berkeley},
	Number = {232, www.bepress.com/ucbbiostat/paper232},
	Title = {The Construction and Analysis of Adaptive Group Sequential Designs},
	Year = {2008}}

@book{Raudenbush&Bryk02,
author={S.W. Raudenbush and A.S. Bryk},
title={Hierarchical linear models: Application and data analysis methods},
publisher={Newbury
Park: Sage.},
year={2002}
}



@book{vanderLaan96,
author={M.J. van der Laan},
title={Efficient and Inefficient Estimation in Semiparametric Models},
publisher={Center for Mathematics and Computer Science, CWI-tract 114},
year={1996}
}

@article{Raudenbush&Liu00,
author={ S.W. Raudenbush and X. Liu},
titlte={Statistical power and
optimal design for multisite randomized trials},
journal={Psychological
Methods},
volume={5},
pages={199Ð213},
year={2000}
}


 @article{Raudenbush&Sampson99a,
 author={S.W. Raudenbush and  R.J. Sampson},
  title={Assessing direct
and indirect effects in multilevel designs with latent
variables},
  journal={Sociological Methods \& Research},
  volume={28},
  pages={123Ð153},
  year={1999}
   }

  @inCollection{Raudenbush&Sampson99b,
 author={S.W. Raudenbush and  R.J. Sampson},
title={Ecometrics: Toward a science of assessing ecological settings, with
application to the systematic social observation of neighbor-
hoods. In M. P. Becker (Ed.)},
 booktitle={Sociological methodology},
OPTvolume={29},
 pages={1Ð41},
 publisher={Boston, MA: Blackwell},
 year={1999}
 }

 @article{Raudenbush&Whillms95,
 author={S.W. Raudenbush and J.D. Whillms},
 title={The estimation of
school effects},
 journal={Journal of Educational and Behavioral
Statistics},
 volume={20},
 pages={307Ð335},
 year={1995}
 }

@article{Coleman58,
author={J.S. Coleman},
title={Relational analysis: The study of social
organizations with survey methods},
journal={Human Organization},
volume={17},
pages={28Ð36},
year={1958}
}

@article{Colemanetal66,
author={J.S.
Coleman and E.Q. Campbell and C.J. Hobson and J. McPartland and
A.M. Mood and F.D. Weinfeld and R.L. York},
title={Equality of educational opportunity. Washington, DC:
Government Printing OfÞce},
journal={Journal of the Royal Statistical Society, Series A},
volume={156},
pages={9Ð38},
year={1966}
}


@article{Aitkin&Longford86,
author={M. Aitkin and N. Longford},
title={Statistical modeling issues
in school effectiveness studies},
journal={Journal of the Royal
Statistical Society, Series A},
volume={149},
pages={1Ð43},
year={1986}
}

@book{Rubin06,
author={D.B. Rubin},
title={Matched Sampling for Causal Effects.},
publisher={Cambridge University Press},
address={Cambridge, MA},
year={2006},
}

@book{Goldstein95,
author={H. Goldstein},
title={Multilevel statistical models},
publisher={London:
Edward Arnold},
year={1995}
}

@article{McMichael99,
author={A.J. McMichael},
title={Prisoners of the proximate: Loosening
the constraints on epidemiology in an age of change},
journal={American Journal of Epidemiology},
volume={149},
pages={887Ð897},
year={1999}
}

@article{Susser99,
author={M. Susser},
title={Should the epidemiologist be a social
scientist or a molecular biologist?},
journal={International Journal of
Epidemiology},
volume={28},
pages={1019Ð1022},
year={1999}
}

@article{Berkmanetal00,
author={L.F. Berkman and T. Glass and I. Brissette and T.E. Seeman},
title={From social integration to health: Durkheim
in the new millennium},
journal={Social Science \& Medicine},
volume={51},
pages={843Ð857},
year={2000}
}

@article{Krieger01,
author={N. Krieger},
title={Theories for social epidemiology in the 21st
century: An ecosocial perspective},
journal={International Journal of
Epidemiology},
volume={30},
pages={668Ð677},
year={2001}
}

@book{Parsons51,
author={T. Parsons},
title={The social system},
publisher={New York: Free Press},
year={1951}
}

@book{Starr82,
author={P. Starr},
title={The social transformation of American medicine},
publisher={New York: Basic Books},
year={1982}
}

@article{Rose85,
author={G. Rose},
title={Sick individuals and sick populations},
journal={International Journal of Epidemiology},
volume={14},
pages={32Ð38},
year={1985}
}

@article{Clarketal91,
author={J. Clark and D.A. Potter and J.B. McKinlay},
title={Bringing
social structure back into clinical decision making},
journal={Social
Science \& Medicine},
volume={32},
pages={853Ð866},
year={1991}
}

@article{Barr95,
author={D.A. Barr},
title={The effects of organizational structure on
primary care outcomes under managed care},
journal={Annals of
Internal Medicine},
volume={122},
pages={353Ð359},
year={1995}
}


@article{McKinlay96,
author={J.B. McKinlay},
title={Some contributions from the social
system to gender inequalities in heart disease},
journal={Journal of
Health and Social Behavior},
volume={37},
pages={1Ð26},
year={1996}
}



@article{Feldmanetal97,
author={H.A. Feldman and J. B. McKinlay and D.A. Potter and K.M. Freund and
R.B. Burns and M.A. Moskowitz and L.E. Kasten},
title={Nonmedical inßuences on medical decision making: An
experimental technique using videotapes, factorial
design, and survey sampling},
journal={Health Services Research},
volume={32},
pages={343Ð366},
year={1997}
}

@article{Hook01,
author={E.B. Hook},
title={(Letter to Editor) RE: Neighborhood social
environment and risk of death: Multilevel evidence from the
Alameda County Study},
journal={American Journal of Epidemiology},
volume={151},
pages={1132Ð1133},
year={2001}
}

@article{Draper95,
author={D. Draper},
title={Inference and hierarchical modeling in the
social sciences},
journal={Journal of Educational and Behavioral
Statistics},
volume={20},
pages={115Ð147},
year={1995}
}

@article{Lindley&Smith72,
author={D. Lindley and A. Smith},
title={Bayes estimation for linear
models},
journal={Journal of the Royal Statistical Society, Series B},
volume={34},
pages={1Ð41},
year={1972}
}


@article{Dempsteretal77,
author={A.P. Dempster and N.M. Laird and D.B. Rubin},
title={Maximum
likelihood from incomplete data via the EM algorithm},
journal={Journal of the Royal Statistical Society, Series B},
volume={39},
pages={1Ð8},
year={1977}
}

@article{Laird&Ware82,
author={
N.M. Laird and J.H. Ware},
title={Random-effects models for
longitudinal data},
journal={Biometrics},
volume={38},
pages={963Ð974},
year={1982}
}


@inCollection{Masonetal84,
author={W.M. Mason and G.Y. Wong and B. Entwisle},
title={Contextual
analysis through the multilevel Linear Model. In S.
Leinhardt (Ed.)},
booktitle={Sociological methodology: 1983Ð1984},
publisher={San
Francisco: Jossey-Bass},
year={1984}
}




@book{Goldstein87,
author={H. Goldstein},
title={Multilevel statistical models in educational
and social research},
publisher={London: Edward Arnold},
year={1987}
}



@book{Bryk&Raudenbush92,
author={A.S. Bryk and S.W. Raudenbush},
title= {Hierarchical linear
models},
publisher={Newbury Park: Sage},
year={1992}
}


@book{Verbeke&Molenbergs97,
author={G. Verbeke and G. Molenbergs},
title={Linear mixed models in practice: A SAS oriented approach},
publisher={New York: Springer},
year={1997}
}



@article{Singer98,
author={J.D. Singer},
title={Using SAS proc mixed to Þt multilevel
models, hierarchical models, and individual growth models},
journal={Journal of Educational and Behavioral Statistics},
volume={24},
pages={323Ð355},
year={1998}
}


@article{Kreftetal94,
author={I.G.G. Kreft and J. de Leeuw and R. van der Leeden},
title={Review of Þve multilevel analysis programs: BMDP-5,
GENMOD, HLM, ML3, VARCL. },
journal={American Statistician},
volume={48},
pages={324Ð335},
year={1994}
}

@inCollection{Deleeuw&Kreft01,
author={J. De Leeuw and I.G.G. Kreft},
title={Software for multilevel
analysis},
booktitle={In H. Goldstein (Ed.), Multilevel modelling of
health statistics},
pages={187Ð204},
publisher={New York: Wiley},
year={2001}
}


@book{Susser73,
author={M. Susser},
title={Causal thinking in health sciences: Concepts
and strategies of epidemiology},
publisher={New York: Oxford},
year={1973}
}

@inCollection{Freedman91,
author={D. Freedman},
title={Statistical models and shoe leather (with
discussion). In P. V. Marsden (Ed.)},
booktitle={Sociological methodol-
ogy},
OPTvol={21},
publisher={San Francisco: Jossey-Banks},
year={1991}
}

@article{Freedman97,
author={D. Freedman},
title={From association to causation via
regression (with comments). In S. P. Turner (Ed.)},
booktitle={Causality in crisis? Statistical methods and the search for causal
knowledge in the social sciences},
OPTpages={113Ð182},
publisher={Notre Dame,
IN: Notre Dame University Press},
year={1997}
}


@article{Greenland90,
author={S. Greenland},
title={Randomization, statistics, and causal
inference},
journal={Epidemiology},
volume={1},
pages={421Ð429},
year={1990}
}


@article{Greenland96,
author={S. Greenland},
title={Basic methods for sensitivity analysis of
biases},
journal={International Journal of Epidemiology},
volume={25},
pages={1107Ð1116},
year={1996}
}

@article{Greenland00,
author={S. Greenland},
title={Principles of multilevel modelling},
journal={International Journal of Epidemiology},
volume={29},
pages={158Ð167},
year={2000}
}

@article{Greenland01,
author={S. Greenland},
title={Ecologic versus individual-level sources of
bias in ecologic estimates of contextual health effects},
journal={International Journal of Epidemiology},
volume={30},
pages={1343Ð1350},
year={2001}
}

@article{Greenland02,
author={S. Greenland},
title={A review of multilevel theory for
ecological analyses},
journal={Statistics in Medicine},
volume={21},
pages={389Ð395},
year={2002}
}

@article{Greenland&Morgenstern01,
author={S. Greenland and H. Morgenstern},
title={Confounding in
health research},
journal={Annual Review of Public Health},
volume={22},
pages={189Ð212},
year={2001}
}

@article{Greenlandetal99,
author={S. Greenland and J. Pearl and J.M. Robins},
title= {Causal
diagrams for epidemiologic research},
journal={Epidemiology},
volume={10},
pages={37Ð48},
year={1999}
}


@article{Manski93,
author={C.F. Manski},
title={IdentiÞcation of endogenous social
effects: The reßection problem},
journal={Review of Economic Studies},
volume={60},
pages={531Ð542},
year={1993}
}


@inCollection{Manski93b,
author={C.F. Manski},
title={IdentiÞcation problems in the social
sciences. In P. V. Marsden (Ed.)},
booktitle={Sociological methodology},
publisher={San Francisco: Jossey-Banks},
year={1993}
}


@article{Halloran&Struchiner95,
author={M.E. Halloran and C.J. Struchiner},
title={Causal inference in
infectious diseases},
journal={Epidemiology},
volume={6},
pages={142Ð151},
year={1995}
}

@article{Morgenstern95,
author={H. Morgenstern},
title={Ecologic studies in epidemiology:
Concepts, principles, and methods},
journal={Annual Review of Public
Health},
volume={16},
pages={61Ð81},
year={1995}
}

@inCollection{Sobel95,
author={M.E.Sobel},
title={Causal inference in the social and
behavioral sciences},
booktitle={In M. E. Sobel (Ed.), Handbook of
statistical modeling for the social and behavioral sciences},
pages={1Ð38},
publisher={New York: Plenum.},
year={1995}
}


@article{Kaufman&Cooper99,
author={J.S. Kaufman and R.S. Cooper},
title={Seeking causal
explanations in social epidemiology},
journal={American Journal of
Epidemiology},
volume={150},
pages={113Ð120},
year={1995}
}

@article{Kaufman&Poole00,
author={J.S. Kaufman and C. Poole},
title={Looking back on causal
thinking in the health sciences},
journal={Annual Review of Public
Health},
volume={21},
pages={101Ð119},
year={2000}
}

@article{Kaufman&Kaufman01,
author={J. S. Kaufman and S. Kaufman},
title={Assessment of
structured socioeconomic effects on health},
journal={Epidemiology},
volume={12},
pages={157Ð167},
year={2001}
}

@article{Robins01,
author={J.M. Robins},
title={Data, design, and background knowledge
in etiologic inference},
journal={Epidemiology},
volume={12},
pages={313Ð320},
year={2001}
}


@article{Maldonado&Greenland02,
author={G. Maldonado and S. Greenland},
title={Estimating causal effects},
journal={International Journal of Epidemiology},
volume={31},
pages={422Ð438},
year={2002}
}

@book{Campbell&Stanley63,
author={D.T. Campbell and J.C. Stanley},
title={Experimental and
quasi-experimental designs for research},
publisher={Hopewell, NJ:
Houghton Mifßin},
year={1963}
}

@article{Cochran65,
author={W.G. Cochran},
title={The planning of observational studies
of human populations},
journal={Journal of the Royal Statistical
Society, Series A},
volume={128},
pages={243Ð265},
year={1965}
}

@article{McKinlay75,
author={S.M. McKinlay},
title={The design and analysis of the
observational studyÑa review},
journal={Journal of the American
Statistical Association},
volume={70},
pages={503Ð523},
year={1975}
}

@article{Heckman79,
author={J.J. Heckman},
title={Sample selection bias as a speciÞcation
error},
journal={Econometrica},
volume={47},
pages={153Ð162},
year={1979}
}


@article{Leamer83,
author={E. Leamer},
title={LetÕs take the con out of econometrics},
journal={American Economic Review},
volume={73},
pages={32Ð43},
year={1983}
}

@inCollection{Smith90,
author={H.L. Smith},
title={SpeciÞcation problems in experimental and
nonexperimental social research},
booktitle={In C. C. Clogg (Ed.), Sociological methodology},
volume={20},
publisher={Oxford: Basil},
year={1990}
}

@article{Rubin91,
author={D.B. Rubin},
title={Practical implications of modes of
statistical inference for causal effects and the critical role
of the assignment mechanism},
journal={Biometrics},
volume={47},
pages={1213Ð1234},
year={1991}
}

@inCollection{Clogg&Haritou97,
author={C.C. Clogg and A. Haritou},
title={The regression method for causal inference and a dilemma confronting this method},
booktitle={In S. P. Turner (Ed.), Causality in crisis? Statistical methods
and the search for causal knowledge in the social sciences},
pages={83Ð112},
publisher={Notre Dame, IN: Notre Dame University Press},
year={1997}
}

@article{Copas&Li97,
author={J.B. Copas and H.G. Li},
title={Inference for non-random
samples (with discussion)},
journal={Journal of the Royal Statistical
Society, Series B},
volume={59},
pages={55Ð95},
year={1997}
}

@inCollection{Freedman97,
author={D. Freedman},
title={From association to causation via
regression (with comments)},
booktitle={In S. P. Turner (Ed.), Causality
in crisis? Statistical methods and the search for causal
knowledge in the social sciences},
pages={113Ð182},
publisher={Notre Dame,
IN: Notre Dame University Press},
year={1997}
}

@article{Winship&Morgan99,
author={C. Winship and S.L.  Morgan},
title={The estimation of causal
effects from observational data},
journal={Annual Review of Sociology},
volume={25},
pages={659Ð707},
year={1999}
}

@book{Pearl00,
author={J. Pearl},
title={Causality: Models, reasoning, and inference},
publisher={ New York: Cambridge University Press},
year={2000}
}

@book{Rosenbaum02,
author={P.R. Rosenbaum},
title={Observational studies},
publisher={New York:
Springer},
year={2002}
}


@article{Charltonetal85,
author={J.R. Charlton and M.F. DÕSouza and M. Tooley and R. Silver},
title={A community trial strategy for evaluating treatment
for symptomatic conditions},
journal={Statistics in Medicine},
volume={4},
pages={11Ð21},
year={1985}
}

@article{Meyeretal91,
author={L. Meyer and N. Job-Spira and J. Bouyer and E. Bouvet and A. Spira},
title={Prevention of sexually transmitted diseases: A
randomised community trial},
journal={Journal of Epidemiology and
Community Health},
volume={45},
pages={152Ð158},
year={1991}
}


@article{Shipleyetal95,
author={R.H. Shipley and T.D. Hartwell and W.D. Austin and A.C. Clayton and L.C. Stanley },
title={Community stop-smoking contests
in the COMMIT trial: Relationship of participation to
costs},
journal={Community intervention trials. Preventive Medicine},
volume={ 24},
pages={286Ð292},
year={1995}
}

@article{Holderetal97,
author={H.D. Holder and R.F. Saltz and A.J. Treno and J.W. Grube and R.B. Voas},
title={Evaluation design for a community prevention
trial. An environmental approach to reduce alcohol-
involved trauma},
journal={Evaluation Review},
volume={21},
pages={140Ð165},
year={1997}
}

@article{Feldmanetal98,
author={H.A. Feldman and M.A. Proschan and D.M. Murray and D.C. Goff and M.
Stylianou and E. Dulberg and P.G. McGovern and W. Chan and N.C.
Mann and V. Bittner},
title={Statistical design of
REACT (Rapid Early Action for Coronary Treatment), a
multisite community trial with continual data collection},
journal={Controlled Clinicial Trials},
volume={19},
pages={391Ð403},
year={1998}
}

@article{LeFortetal98,
author={S.M. LeFort and K. Gray-Donald and K.M. Rowat and M.E. Jeans},
title={Randomized controlled trial of a community-based
psychoeducation program for the self-management of
chronic pain},
journal={Pain},
volume={74},
pages={297Ð306},
year={1998}
}


@article{Perskyetal99,
author={V. Persky and L. Coover and E. Hernandez and A. Contreras and J. Slezak and J. Piorkowski and L. Curtis and M. Turyk and V. Ramakrishnan and  P. Scheff},
title={Chicago community-based asthma
intervention trial: Feasibility of delivering peer education in
an inner-city population},
journal={Chest},
volume={116},
pages={216SÐ223S},
year={1999}
}

@article{Biglanetal00,
author={A. Biglan and K. Smolkowski and T. Duncan and C. Black},
title={A randomised controlled trial of a community
intervention to prevent adolescent tobacco use},
journal={Tobacco
Control},
volume={9},
pages={24Ð32},
year={2000}
}


@article{Luepkeretal00,
author={R.V. Luepker and J.M. Raczynski and S. Osganian and R.J Goldberg and
Jr. J.R.  Finnegan and J.R. Hedges and Jr. D.C. Goff and M.S.
Eisenberg and J.G. Zapka and H.A. Feldman and D.R. Labarthe and P.G. McGovern and C.E. Cornell and M.A. Proschan and D.G. Simons-Morton},
title={Effect of a community
intervention on patient delay and emergency medical service
use in acute coronary heart disease: The rapid early action
for coronary treatment (REACT) trial},
journal={JAMA},
volume={284},
pages={60Ð67},
year={2000}
}


@Article{Oakes04,
  author = {J.M. Oakes},
  title= {The (mis)estimation of neigborhood effects: causal inference for a practicable social epidemiology },
  journal = {Social Science and Medicine},
  volume = {58},
  issue = {},
  pages = {1929--1952},
  year = {2004}
}

@Article{Abadie&Imbens06,
  author = {A. Abadie and G.W. Imbens},
  title= {Large Sample Properties of Matching Estimators for Average Treatment Effects},
  journal = {Econometrica},
  volume = {74},
  issue = {1},
  pages = {235-67},
  year = {2006}
}

@Article{Greenland&Morgenstern90,
  author = {S. Greenland and H. Morgenstern},
  title= {Matching and Efficiency in Cohort Studies},
  journal = {American Journal of Epidemiology},
  volume = {131},
  issue = {1},
  pages = {151-159},
  year = {1990}
}

@Article{Costanza95,
  author = {M. Costanza},
  title= {Theoretical Epidemiology, Matching},
  journal = {Preventive Medicine},
  volume = {24},
  issue = {},
  pages = {425-433},
  year = {1995}
}

@Article{Joffe&Rosenbaum99,
  author = {M.M. Joffe and P.R. Rosenbaum},
  title= {Invited Commentary: Propensity Scores},
  journal = {American Journal of Epidemiology},
  volume = {150},
  issue = {4},
  pages = {327-333},
  year = {1999}
}


@article{Neugebauer&vanderLaan07,
author={R. Neugebauer, M. J. van der Laan},
title={ Nonparametric Causal E?ects based on
marginal structural models},
journal={Journal of Statistical Planning and Inference},
year={2007},
volume={137},
pages={419Ð434},
}




@article{Murphy05,
author={S. Murphy},
title={An experimental design for the development of adaptive treatment strategies},
journal={Statistics in Medicine},
year={2005},
volume={24},
pages={1455Ð1481},
}

@article{Lavori&Dawson00,
author={P. Lavori and R. Dawson},
title={A design for testing clinical strategies: biased adaptive within-subject
randomization},
journal={Journal of the Royal Statistical Society, Series A},
volume={163},
pages={29Ð38},
year={2000},
}

@article{Lavori&Dawson04,
author={P. Lavori  and R. Dawson},
title={Dynamic treatment regimes: practical design considerations},
journal={Clinical trials},
volume={1},
pages={9Ð20},
year={2004},
}

@article{Thalletal00,
author={P. Thall and R. Millikan and H.-G. Sung},
title={Evaluating multiple treatment courses in clinical trials},
journal={Statistics in Medicine},
volume={19},
pages={1011Ð1028},
year={2000},
}

@article{Rushetal03,
author={A.J. Rush and M. Trivedi and M. Fava},
title={Depression},
journal={IV. American Journal of Psychiatry},
volume={160(2)},
pages={237},
year={2003},
}

@article{Schneideretal06,
author={Schneider, L. and Tariot.P.N. and Dagerman, K. and Davis, S. and Hsiao, J. and Ismail, S. and Lebowitz, B. and Lyketsos, C. and Ryan
J. and Stroup T. and Sultzer D. and Weintraub, D. and Lieberman, J.},
title= {E?ectiveness of atypical antipsychotic
drugs in patients with AlzheimerÕs disease},
journal={New England Journal of Medicine},
volume={355(15)},
pages={1525Ð1538},
year={2006},
}

@article{Swartzetal07,
author={Swartz, M. and Perkins, D. and Stroup, T. and Davis, S. and Capuano, G. and Rosenheck, R. and Reimherr, F. and McGee, M. and Keefe,
R. and McEvoy, J. and Hsiao, J. and Lieberman, J.},
title={Effects of antipsychotic medications on psychosocial
functioning in patients with chronic shizophrenia: Findings from the nimh catie study},
year={2007},
journal={American Journal
of Psychiatry},
volume={164},
pages={428Ð436},
}

@article{Rubin&vanderLaan08,
author={D.B. Rubin and M.J. van der Laan},
title={Empirical Efficiency Maximization: Improved Locally Efficient Covariate Adjustment in Randomized Experiments and Survival Analysis},
year={2008},
journal={The International Journal of Biostatistics},
volume={Vol. 4, Iss. 1, Article 5},
location={http://www.bepress.com/ijb/vol4/iss1/5},
}


@article{vanderLaan&Rose&Gruber09,
author={M.J. van der Laan and S. Rose and S. Gruber},
title={Readings on Targeted Maximum Likelihood Estimation},
year={September, 2009},
journal={Technical report, working paper series http://www.bepress.com/ucbbiostat/paper254/},
}

@article{Bembometal09,
author={O. Bembom and M.J. van der Laan and T. Haight and I.B. Tager},
title={Lifetime and
current leisure time physical activity and all-cause mortality in an elderly cohort},
year={2009},
journal={Epidemiology},
volume={},
pages={},
}

@article{Bembom&vanderLaan07a,
author={Oliver Bembom and Mark van der Laan},
title={Statistical Methods for analyzing sequentially randomized trials, commentary on JNCI article Adaptive therapy for androgen independent prostate cancer: A Randomized selection trial including four regimens, by Peter F. Thall, C. Logothetis, C. Pagliaro, S. Wen, M.A. Brown, D. Williams, R. Millikan (2007). },
journal={Journal of the National Cancer Institute},
year={2007},
volume={99(21)},
pages={1577-1582},
 }

@article{Rosenblumetal09,
author={M. Rosenblum and S.G. Deeks and M.J. van der Laan and D.R. Bangsberg},
title={The Risk
of Virologic Failure Decreases with Duration of HIV Suppression, at Greater
than 50\% Adherence to Antiretroviral Therapy},
year={2009},
journal={PLoS ONE},
volume={4(9): e7196.doi:10.1371/journal.pone.0007196},
}



@article{Robinsetal08,
author={J. Robins and L. Orallana and A. Rotnitzky},
title={Estimaton and extrapolation of optimal treatment and  testing strategies},
journal={Statistics in Medicine},
year={2008},
volume={27(23)},
pages={ 4678-4721},
}


@article{Bembom&vanderLaan07,
author= {O. Bembom and M.J. van der Laan},
title={A practical illustration of the importance of realistic individualized treatment rules in causal inference},
journal={Electronic Journal of Statistics},
year={2007},
pages={http://www.i-journals.org/ejs/viewarticle.php?id=105&layout=abstract},
}

@article{Bembometal08,
author={O. Bembom and M.L. Petersen and S.-Y. Rhee and W. J. Fessel and S.E. Sinisi and R.W. Shafer and M.J. van der Laan},
title ={Biomarker discovery using targeted maximum likelihood estimation: Application to the treatment of antiretroviral resistant HIV infection},
journal={Statistics in Medicine},
year={2008},
pages={http://www3.interscience.wiley.com/journal/121422393/abstract},
}

@article{Cassel76,
author={J. Cassel},
title={The contribution of the social environment to host resistance},
journal={American Journal of Epidemiology},
volume={104},
pages={107--123},
year={1976}
}

@article{Tuglus&vanderLaan08,
author={C. Tuglus and M.J. van der Laan},
title={Targeted Methods for Biomarker Discovery, the Search for a Standard},
journal={UC Berkeley Working Paper Series},
year={2008},
pages={http://www.bepress.com/ucbbiostat/paper233/.},
}

@article{vanderLaan08,
author={M.J. van der Laan},
title={Estimation Based on Case-Control Designs with Known Prevalance Probability},
journal={The International Journal of Biostatistics},
year={2008},
volume={http://www.bepress.com/ijb/vol4/iss1/17/},
}

@article{Rose&vanderLaan08,
author={S. Rose and M.J. van der Laan},
title={Simple Optimal Weighting of Cases and Controls in Case-Control Studies},
journal={The International Journal of Biostatistics},
year={2008},
pages={http://www.bepress.com/ijb/vol4/iss1/19/.},
}

@article{Rose&vanderLaan09,
author={S. Rose and M.J. van der Laan},
title={Why Match? Investigating Matched Case-Control Study Designs with Causal Effect Estimation},
journal={The International Journal of Biostatistics},
year={2009},
pages={http://www.bepress.com/ijb/vol5/iss1/1/.},
}


@inproceedings{Moore&vanderLaan09,
author={K.L. Moore and M.J. van der Laan},
title={Application of Time-to-Event Methods in the Assessment of Safety in Clinical Trials},
booktitle={in Design, Summarization, Analysis \& Interpretation of Clinical Trials with Time-to-Event Endpoints},
year={2009},
editor={Karl E. Peace},
publisher={Chapman and Hall},
}

@inproceedings{Polley&vanderLaan09,
author={E.C. Polley and M.J. van der Laan},
title={Predicting Optimal Treatment Assignment Based on Prognostic Factors in Cancer Patients},
booktitle={in Design, Summarization, Analysis \& Interpretation of Clinical Trials with Time-to-Event Endpoints},
year={2009},
editor={Karl E. Peace},
publisher={Chapman and Hall},
}


@article{vanderVaart&Dudoit&vanderLaan06,
  author =       {A.W. van der Vaart and S. Dudoit and M.J. van der Laan},
  title =        {Oracle Inequalities for Multi-Fold Cross-Validation},
   journal = {Statistics and Decisions},
   volume={24},
 number={3},
 year={2006},
 pages={351--371},
}

@article{vanderLaan&Dudoit&vanderVaart06,
  author =       {M.J. van der Laan and S. Dudoit and A.W. van der Vaart},
  title =        {The Cross-Validated Adaptive Epsilon-Net Estimator},
   journal = {Statistics and Decisions},
   volume={24},
 number={3},
 year={2006},
 pages={373--395},
}

 @article{Rosenbaum&Rubin83,
 author={P.R. Rosenbaum and D.B. Rubin},
 title={The Central Role of the Propensity Score in Observational Studies for Causal Effects},
 journal={Biometrika},
 volume={70},
 year={1983},
 pages={41-55}
 }

@article{vanderLaan&Polley&Hubbard07,
 author = {M.J. van der Laan and E. Polley and A. Hubbard},
 title = {Super Learner},
 journal = {Statistical Applications in Genetics and Molecular Biology},
 volume = {6},
 number ={25},
 year = {2007},
 issn = {1},
 location={http://www.bepress.con/sagmb/vol6/iss1/art25},
 }

 @article{Sekhon08,
 author={J.S. Sekhon},
 title= {Multivariate and Propensity Score Matching
 Software with Automated Balance Optimization: The Matching package for {R}},
 journal = {Journal of Statistical Sotware, Forthcoming},
 publisher={SSRN},
location = {http://ssrn.com/paper=1009044},
year={2008}
}

@article{Bembom&Fessel&Shafer&vanderLaan08,
	location = {http://www.scientificcommons.org/36721107},
	title = {Data-adaptive Selection Of The Adjustment Set In Variable Importance Estimation},
	author = {O. Bembom and J.W. Fessel and R.W. Shafer  and M.J. van der Laan},
	year = {2008},
	keywords = {General Biostatistics},
	publisher = {The Berkeley Electronic Press},
	url = {http://www.bepress.com/ucbbiostat/paper231},
	institution = {DigitalCommons@Florida Atlantic University [http://digitalcommons.fau.edu/cgi/oai2.cgi] (United States)},
}

@article{Holland77,
 author = {J.H. Holland and J.S. Reitman},
 title = {Cognitive systems based on adaptive algorithms},
 journal = {SIGART Bull.},
 volume = {63},
 year = {1977},
 issn = {0163-5719},
 pages = {49--49},
 doi = {http://doi.acm.org/10.1145/1045343.1045373},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

@book{Rubin06,
author={D.B. Rubin},
title={Matched Sampling for Causal Effects.},
publisher={Cambridge University Press},
address={Cambridge, MA},
year={2006},
}

@incollection{Mans81,
author={C.F. Manski and D. McFadden},
title={Alternative estimators and sample designs for discrete choice analysis},
booktitle={Structural Analysis of Discrete Data with Econometric Applications},
publisher={The MIT Press},
address={Cambridge, MA},
year={1981},
editor={C.F. Manski and D. McFadden},
}

@article{Mans77,
author={C.F. Manski and S.R. Lerman},
title={The Estimation of Choice Probabilities from Choice Based Samples},
journal={Econometrica},
volume={45},
number={8},
pages={1977-1988},
year={1977},
}

@article{Coss81,
author={S.R. Cosslett},
title={Maximum Likelihood Estimator for Choice-Based Samples},
journal={Econometrica},
volume={49},
number={5},
pages={1289-1316},
year={1981},
}


@article{Corn51,
author={J. Cornfield},
title={A method of estimating comparative rates from clinical data.  Applications to cancer of the lung, breast, and cervix.},
journal={J Nat Cancer Inst},
volume={11},
pages={1269-1275},
year={1951},
}

@inproceedings{Corn56,
author={J. Cornfield},
title={A statistical problem arising from retrospective studies},
booktitle={Proceedings of the Third Berkeley Symposium, Volume IV},
year={1956},
editor={J. Neyman},
pages={133-148},
publisher={University of California Press},
}

@article{Beni94,
author={J. Benichou and S. Wacholder},
title={A comparison of three approaches to estimate exposure-specific incidence rates from population-based case-control data.},
journal={Statistics in Medicine},
volume={13},
pages={651-661},
year={1994},
}
@article{Breslow&Robins&Wellner00,
author={N.E. Breslow and J.M. Robins and J.A. Wellner},
title={On the semi-parametric efficiency of logistic regression under case-control sampling},
journal={Bernoulli},
volume={6(3)},
pages={447--455},
year={2000},
}
@article{Mansonetal07,
author = {R. Mansson, M.M. Joffe, W. Sun, S. Hennessy},
title = {On the Estimation and Use of Propensity Scores in Case-Control and Case-Cohort Studies.},
journal = {Am J Epidemiol},
volume = {166},
number = {3},
pages = {332-339},
year = {2007},
}

@article{And79,
author={J.A. Anderson},
title={Separate sample logistic discrimination},
journal={Biometrika},
volume={59},
pages={19--35},
year={1972},
}

@article{Prentice&Pike79,
author={R.L. Prentice and R. Pyke},
title={Logistic disease incidence models and case-control studies},
journal={Biometrika},
volume={66},
pages={403--411},
year={1979},
}

@article{Breslow96,
author={N.E. Breslow},
title={Statistics in Epidemiology: the Case-Control Study},
journal={J Am Stat Soc},
volume={91},
pages={14--28},
year={1996},
}

@book{Breslow&Day80,
author={N.E. Breslow and N.E. Day},
title={Statistical Methods in Cancer Research:  Volume 1 -- The analysis of case-control studies},
publisher={International Agency for Research on Cancer},
address={Lyon},
year={1980},
}

@article{Holfordetal78,
author={T.R. Holford and C. White and J.L. Kelsey},
title={Multivariate Analysis for Matched Case-Control Studies},
journal={Am J Epid},
volume={107},
number={3},
pages={245--255},
year={1978},
}

@article{Breslowetal78,
author={N.E. Breslow and N.E. Day and K.T. Halvorsen and R.L. Prentice and C. Sabal},
title={Estimation of Multiple Relative Risk Functions in Matched Case-Control Studies},
journal={Am J Epid},
volume={108},
number={4},
pages={299--307},
year={1978},
}

@book{Schlesselman82,
author={J.J. Schlesselman},
title={Case-Control Studies:  Design, Conduct, Analysis},
publisher={Oxford University Press},
address={Oxford},
year={1982},
}

@book{Collett91,
author={D. Collett},
title={Modeling Binary Data},
publisher={Chapman and Hall},
address={London},
year={1991},
}

@book{Jewell04,
author={N.P. Jewell},
title={Statistics for Epidemiology},
publisher={Chapman and Hall/CRC},
address={Boca Raton},
year={2004},
}

@book{Hosmer&Lemeshow00,
author={D.W. Hosmer and S. Lemeshow},
title={Applied Logistic Regression},
edition={2nd},
publisher={John Wiley and Sons},
address={New York},
year={2000},
}

@article{Robins99,
author={J.M. Robins},
title={[Choice as an Alternative to Control in Observational Studies]:  Comment},
journal={Statistical Science},
volume={14},
number={3},
pages={281--293},
year={1999},
}

@article{Newman06,
author={S. Newman},
title={Causal Analysis of Case-Control Data},
journal={Epid Persp Innov},
volume={3},
pages={2},
url={http://www.epi-perspectives.com/content/3/1/2},
year={2006},
}

@article{Zele86,
author={M. Zelen and R.A. Parker},
title={Case-Control Studies and Bayesian Inference},
journal={Stat Med},
volume={5},
number={3},
pages={261--269},
year={1986},
}

@article{Sinh04,
author={S. SInha and B. Mukherjee and M Ghosh},
title={Bayesian Semiparametric Modeling for Matched Case-Control Studies with Multiple Disease States},
journal={Biometrics},
volume={60},
pages={41--49},
year={2004},
}

@article{Ritc01,
author = {M.D. Ritchie and L.W. Hahn and N. Roodi and L.R. Bailey and W.D. Dupont and F.F. Parl and J.H. Moore},
title = {Multifactor-dimensionality reduction reveals high-order interactions among estrogen-metabolism genes in sporadic breast cancer.},
journal = {Am J Hum Genet},
volume = {69},
number = {1},
pages = {138--47},
year = {2001},
}

@article{Mei07,
author = {H. Mei and M.L. Cuccaro and E.R. Martin},
title = {Multifactor dimensionality reduction-phenomics: a novel method to capture genetic heterogeneity with use of phenotypic variables.},
journal = {Am J Hum Genet},
volume = {81},
number = {6},
pages = {1251-61},
year = {2007},
}




@article{
Bangsberg04,
   Author = {D.R. Bangsberg and A.R. Moss and S.G. Deeks},
   Title = {Paradoxes of adherence and drug resistance to {HIV} antiretroviral therapy},
   Journal = {J Antimicrob Chemother},
   Volume = {53},
   Number = {5},
   Pages = {696-9},
   Note = {0305-7453 (Print)
Journal Article
Review},
   Abstract = {Public health debates about providing HIV antiretroviral therapy to impoverished populations have centred on the relationship between adherence and risk of drug resistance. Recent data indicate that each antiretroviral therapeutic class has a unique adherence-resistance relationship. Resistance to single protease inhibitor therapy occurs most frequently at moderate to high levels of adherence, resistance to non-nucleoside reverse transcriptase inhibitor therapy occurs at low to moderate levels of adherence, and resistance to ritonavir-boosted protease inhibitor therapy is most likely to occur at middle ranges of adherence. These dynamic relationships should be considered in balancing the individual and public health benefits of therapy.},
 Keywords = {Anti-HIV Agents/*therapeutic use
Developing Countries
*Drug Resistance, Viral
Humans
*Patient Compliance
Public Health
Research Support, Non-U.S. Gov't
Research Support, U.S. Gov't, P.H.S.},
   Year = {2004} }


@Article{Scharfstein&Tsiatis&Robins97,
  author =   {D.O. Scharfstein and A.A. Tsiatis and J.M. Robins},
  title =    {Semiparametric efficiency and its implications on the design and analysis of group-sequential studies},
journal =      {Journal of the American Statistical Association},
  year =     {1997},
  OPTkey =   {},
  volume =   {92},
  number =   {440},
  pages =    {1342--1350},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Bembom&Petersen07,
   author={O. Bembom and M. Petersen and SY Rhee and W.J. Fessel and S.E. Sinisi and R.W. Shafer 	     and M.J. van der Laan},
   title={Biomarker Discovery Using Targeted Maximum Likelihood Estimation: Application to the  Treatment of Antiretroviral Resistant {HIV} Infection},
   journal= {U.C. Berkeley Division of Biostatistics Working Paper Series},
   year={2007},
  volume={221},
   OPTmonth={August},
  OPTnote={http://www.bepress.com/ucbbiostat/paper221}
}

@Article{vanderLaan&Gruber09,
  author=  {M.J. van der Laan and S. Gruber},
  title={Collaborative Double robust penalized targeted maximum likelihood estimation},
  journal={The International Journal of Biostatistics},
  year={2010},
  volume={},
 }
@Article{Gruber&vanderLaan09,
  author=  {S. Gruber and M.J. van der Laan},
  title={An application of collaborative targeted maximum likelihood estimation in causal inference and genomics},
  journal={The International Journal of Biostatistics},
  year={2010},
  volume={},
 }
@Article{vanderLaan&Rubin06,
  author =   {M.J. van der Laan and D. Rubin},
  title =    {Targeted Maximum Likelihood Learning},
journal =      {The International Journal of Biostatistics},
  year =     {2006},
  OPTkey =   {},
  volume =   {2},
  number =   {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/ijb/vol2/iss1/11},
  OPTannote =    {}
}


@Article{Scharfstein&Tsiatis98,
  author =   {D.O. Scharfstein and A.A. Tsiatis},
  title =    {The use of simulation and bootstrap in information based group sequential studies},
journal =      {Statistics in Medicine},
  year =     {1998},
  OPTkey =   {},
  volume =   {17},
  number =   {},
  pages =    {75--87},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Pampallona&Tsiatis&Kim01,
  author =   {S. Pampallona and A.A. Tsiatis and K. Kim},
  title =    {Interim monitoring of group sequential trials using spending functions for the type I and type II error probabilities},
journal =      {Drug Informational Journal},
  year =     {2001},
  OPTkey =   {},
  volume =   {35},
  number =   {},
  pages =    {1113-1121},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Tsiatis&Mehta03,
  author =   {A.A. Tsiatis and C. Mehta},
  title =    {On the inefficiency of the adaptive design for monitoring clinical trials},
journal =      {Biometrika},
  year =     {2003},
  OPTkey =   {},
  volume =   {90},
  number =   {},
  pages =    {367-378},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Banerjee&Tsiatis06,
  author =   {A. Banerjee and A.A. Tsiatis},
  title =    {Adaptive two-stage designs in phase II clinical trials},
journal =      {Statistics in Medicine},
  year =     {2006},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {In press},
  OPTannote =    {}
}
@Article{Tsiatis06,
  author =   {A.A. Tsiatis},
  title =    {Information based monitoring of clinical trials},
journal =      {Statistics in Medicine},
  year =     {2006},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {In press},
  OPTannote =    {}
}

@Article{Lokhnygina&Tsiatis06,
  author =   {Y. Lokhnygina and A.A. Tsiatis},
  title =    {Optimal two-stage group sequential designs},
journal =      {Journal of Statistical Planning and Inference},
  year =     {2006},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {},
  OPTnote =      {In press},
  OPTannote =    {}
}

  @Article{Bauer&Kohne94,
  author =   {P. Bauer and Kohne},
  title =    {Evaluation of experiments with adaptive interim analysis},
journal =      {Biometrics},
  year =     {1994},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {1029--1041},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Cui&Hung&Wang99,
  author =   {L. Cui and H.M.J. Wang and S-J Wang},
  title =    {Modification of sample size in group sequential trials},
journal =      {Biometrics},
  year =     {1999},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {853--857},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Jennison&Turnbull03,
  author =   {C. Jennison and B.W. Turnbull},
  title =    {Mid course sample size modification in clinical trials based on hte observed treatment effect},
journal =      {Statistics in Medicine},
  year =     {2003},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {971--993},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Koyama&Sampson&Gleser04,
  author =   {T. Koyama and A.R. Sampson and L.J. Gleser},
  title =    {A calculus for design of two stage adaptive procedures},
journal =      {Journal of the Americal Statistical Association},
  year =     {2004},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Lan&Trost97,
  author =   {K.K.G Lan and D.C. Trost},
  title =    {Estimation of parameters and sample size re-estimation},
journal =      {Proceedings Biopharm Section},
  year =     {1997},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {48-51},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Li&Shih&Xie&Lu02,
  author =   {G. Li and W.J. Shih and T. Xie and J. Lu},
  title =    {A sample size adjustment procedure for clinical trials based on conditional power},
journal =      {Biostatistics},
  year =     {2002},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {277--287},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Mehta&Tsiatis01,
  author =   {C.R. Mehta and A.A. Tsiatis},
  title =    {Flexible sample size considerations using information based interim monitoring},
journal =      {Drug Informational Journal},
  year =     {2001},
  OPTkey =   {},
  volume =   {35},
  number =   {},
  pages =    {1095--1112},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Mulle&Shafer01,
  author =   {H.H. Mulle and H. Shafer},
  title =    {Adaptive group sequential designs for clinical trials: combining the advantages of adaptive and classical group sequential approaches},
journal =      {Biometrics},
  year =     {2001},
  OPTkey =   {},
  volume =   {57},
  number =   {},
  pages =    {886--891},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Proschan&Hunsberger95,
  author =   {M.A. Proschan and S.A. Hunsberger},
  title =    {Designed extension studies based on conditional power},
journal =      {Biometrics},
  year =     {1995},
  OPTkey =   {},
  volume =   {51},
  number =   {},
  pages =    {1315--1324},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Shen&Fisher99,
  author =   {Y. Shen and L.D. Fisher},
  title =    {Statistical Inference for self-designing clinical trials with a one-sided hypothesis},
journal =      {Biometrics},
  year =     {1999},
  OPTkey =   {},
  volume =   {55},
  number =   {},
  pages =    {190--197},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Wittes&Brittain90,
  author =   {J. Wittes and E. Brittain},
  title =    {The role of internal pilot studies in increasing efficiency of clinical trials},
journal =      {Statistics in Medicine},
  year =     {1999},
  OPTkey =   {},
  volume =   {9},
  number =   {},
  pages =    {65--72},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Shen&Cheng06,
  author =   {Y. Shen and Y. Cheng},
  title =    {Adaptive design: Estimation and Inference with censored data in a semiparametric model},
journal =      {Biostatistics},
  year =     {2006},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {In Press},
  OPTannote =    {}
}

%next reference for adaptive allocation of treatments

@Book{Spiegelalteretal04,
  author =       {D.J. Spiegelalter and K.R. Abrams and J.P. Myles},
  title =        {Bayesian approaches to clinical trials and health care evaluation},
  publisher =    {Wiley, Chichester},
  year =         {2004}
}
@Book{Berry&Stangl96,
  author =       {D.A. Berry and D.K. Stangl},
  title =        {Bayesian biostatistics},
  publisher =    {Marcel Dekker, New York},
  year =         {1996}
}


@Article{Berry06,
  author =   {D.A. Berry},
  title =    {Bayesian clinical trials},
journal =      {Nature Reviews, Drug Discovery},
  year =     {2006},
  OPTkey =   {},
  volume =   {5},
  number =   {},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

%D. A. Berry, Bayesian clinical trials, Nature Reviews, Drug
%Recovery, vol 5, january 2006.


@Book{Hu&Rosenberger06,
  author =       {F. Hu and W.F. Rosenberger},
  title =        {The theory of response adaptive randomization in clinical trials},
  publisher =    {New York Wiley},
  year =         {2006}
}

@Book{Dudoit&vanderLaan08,
  author =       {S. Dudoit and M.J. van der Laan},
  title =        {Resampling based multiple testing with applications to genomics},
  publisher =    {Springer Series of Statistics, New York},
  year =         {2008}
}

@Book{Sen&Singer93,
  author =       {P.K. Sen and J.M. Singer},
  title =        {Large Sample Methods in Statistics: An Introduction with Applications},
  publisher =    {Chapman \& Hall, New York},
  year =         {1993}
}


@Article{Bai&Hu&Rosenberger02,
  author =   {Z.D. Bai and F. Hu and W.F. Rosenberger},
  title =    {Asymptotic properties of adaptive designs for clinical trials with delayed response},
journal =      {Annals of Statistics},
  year =     {2002},
  OPTkey =   {},
  volume =   {30},
  number =   {1},
  pages =    {122--139},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Andersen&Faries&Tamura94,
  author =   {J. Andersen and D. Faries and R. Tamura},
  title =    {A randomized play-the-winner design for multiarm clinical trials},
journal =      {Communication in Statistical Theory},
  year =     {1994},
  OPTkey =   {},
  volume =   {23},
  number =   {},
  pages =    {309--323},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Flournoy&Rosenberger95,
  author =       {N. Flournoy and W.F. Rosenberger},
  title =        {Adaptive Designs},
  publisher =    {Hayward, Institute of Mathematical Statistics},
  year =         {1995}
}

@Article{Hu&Rosenberger00,
  author =   {F. Hu and W.F. Rosenberger},
  title =    {Analysis of time trends in adaptive designs withi appliation to a neurophysiology experiment},
journal =      {Statistics in Medicine},
  year =     {2000},
  OPTkey =   {},
  volume =   {19},
  number =   {},
  pages =    {2067--2075},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Rosenberger96,
  author =   {W.F. Rosenberger},
  title =    {New directions in adaptive designs},
journal =      {Statistical Science},
  year =     {1996},
  OPTkey =   {},
  volume =   {11},
  number =   {},
  pages =    {137--149},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Rosenberger&Flournoy&Durham97,
  author =   {W.F. Rosenberger and N. Flournoy and S.D. Durham},
  title =    {Asymptotic normality of maximum likelihood estimators
  from multiparameter response driven designs},
journal =      {Journal of Statistical Planning and Inference},
  year =     {1997},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {69--76},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Rosenberger&Grill97,
  author =   {W.F. Rosenberger and S.E. Grill},
  title =    {A sequential design for psychophysical experiments: An application to estimating timing of sensory events},
journal =      {Statistics in Medicine},
  year =     {1997},
  OPTkey =   {},
  volume =   {16},
  number =   {},
  pages =    {2245--2260},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Rosenberger&Sriram97,
  author =   {W.F. Rosenberger and T.N. Shiram},
  title =    {Estimation for an adaptive allocation design},
journal =      {Journal of Statistical Planning and Inference},
  year =     {1997},
  OPTkey =   {},
  volume =   {59},
  number =   {},
  pages =    {309--319},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Tamura&Faries&Andersen&Heiligenstein94,
  author =   {R.N. Tamura and D.E. Faries and J.S. Andersen and J.H. Heiligenstein},
  title =    {A case study of an adaptive clinical trial in the treatment of out-patients with depressive disorder},
journal =      {Journal of the American Statistical Association},
  year =     {1994},
  OPTkey =   {},
  volume =   {89},
  number =   {},
  pages =    {768--776},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Wei&Durham78,
  author =   {L.J. Wei and S. Durham},
  title =    {The randomize play-the-winner rule in medical trials},
journal =      {Journal of the American Statistical Association},
  year =     {1978},
  OPTkey =   {},
  volume =   {73},
  number =   {},
  pages =    {840--843},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Wei&Smythe&Lin&Park90,
  author =   {L.J. Wei and R.T. Smythe and D.Y. Lin and T.S. Park},
  title =    {Statistical Inference with data-dependent treatment allocation rules},
journal =      {Journal of the American Statistical Association},
  year =     {1990},
  OPTkey =   {},
  volume =   {85},
  number =   {},
  pages =    {156--162},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Zelen69,
  author =   {M. Zelen},
  title =    {Play the winner rule and the controlled clinical trial},
journal =      {Journal of the American Statistical Association},
  year =     {1969},
  OPTkey =   {},
  volume =   {64},
  number =   {},
  pages =    {131--146},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Cheng&Shen05,
  author =   {Y. Cheng and Y. Shen},
  title =    {Bayesian adaptive designs for clinical trials},
journal =      {Biometrika},
  year =     {2005},
  OPTkey =   {},
  volume =   {92},
  number =   {3},
  pages =    {633--646},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Wei79,
  author =   {L.J. Wei},
  title =    {The generalized Polya's urn design for sequential medical trials},
journal =      {Annals of Statistics},
  year =     {1979},
  OPTkey =   {},
  volume =   {7},
  number =   {},
  pages =    {291--296},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}








@article{
Benito03,
   Author = {Benito, J. M. and Lopez, M. and Soriano, V.},
   Title = {Virus load and cytolitic responses in human immunodeficiency virus infection: what is cause and what is effect},
   Journal = {J Infect Dis},
   Volume = {188},
   Number = {5},
   Pages = {794-5; author reply 795-6},
   Note = {0022-1899
Comment
Letter},
 Keywords = {ADP-ribosyl Cyclase/metabolism
Anti-HIV Agents/therapeutic use
Antigens, CD/metabolism
CD4-Positive T-Lymphocytes/*immunology
CD8-Positive T-Lymphocytes/immunology
HIV Infections/drug therapy/*immunology/virology
HIV-1/*physiology
Human
*Viral Load
Virus Replication},
   Year = {2003} }



@article{
DEttorre02,
   Author = {D'Ettorre, G. and Forcina, G. and Andreotti, M. and Sarmati, L. and Palmisano, L. and Galluzzo, C. M. and Nicastri, E. and Mastroianni, C. M. and Vullo, V. and Vella, S. and Andreoni, M.},
   Title = {Discordant response to antiretroviral therapy: {HIV} isolation, genotypic mutations, T-cell proliferation and cytokine production},
   Journal = {Aids},
   Volume = {16},
   Number = {14},
   Pages = {1877-85},
   Note = {0269-9370
Journal Article},
   Abstract = {OBJECTIVE: To study virologic and immunologic factors associated with discordant treatment response in HIV-infected patients receiving highly active antiretroviral therapy (HAART). DESIGN: Study participants included a total of 27 patients: (a) 10 discordant patients (mean CD4+ cell count, 396.1 x 10 cells/l; mean HIV-RNA, 5.4 log copies/ml); (b) seven responder patients (mean CD4+ cell count, 997.5 x 10 cells/l); and (c) 10 failing patients (mean CD4+ cell count 66.5 x 10 cells/l; mean HIV-RNA, 5.4 log copies/ml).(10) (10)METHODS: The HIV-1 isolation rate and biological phenotype, drug resistance genotypic mutations of HIV-1 strains, recall and HIV-1-specific antigen lymphocyte proliferation (LP), and interleukin (IL)-15 production were studied. RESULTS: Virus isolation was obtained in 30% of discordant patients, and in 100% of failing patients. A higher replication constant was reported in discordant patients. No difference in the number of drug resistance mutations and biological phenotypes of HIV-1 was found in discordant patients with respect to failing patients. Discordant patients developed positive LP responses to and HIV-1 p24. LP in response to, HIV-1 p24 and gp160 was positive in responder patients. No significant LP was found in failing patients. Increased levels of IL-15 after stimulation with lipopolysaccaride (LPS) and were found in both discordant patients and responder patients. Conversely, a strong reduction of IL-15 levels was observed in failing patients. CONCLUSION: The present results suggest that decreased virus isolation rate, restoration of both lymphocyte proliferation and IL-15 production are factors involved in the discordant antiretroviral therapy response of HIV-infected patients.},
 Keywords = {Adult
Anti-HIV Agents/*therapeutic use
Antiretroviral Therapy, Highly Active
CD4 Lymphocyte Count
CD8-Positive T-Lymphocytes/drug effects/immunology
Candida albicans
Drug Resistance, Viral
Female
HIV Infections/complications/*drug therapy/immunology/virology
HIV-1/drug effects/genetics/*immunology/isolation & purification
Human
Interleukin-15/*blood
Male
Middle Aged
Mutation
Viral Load
Virus Replication/drug effects},
   Year = {2002} }



@article{
Davenport02,
   Author = {Davenport, M. P. and Zaunders, J. J. and Hazenberg, M. D. and Schuitemaker, H. and van Rij, R. P.},
   Title = {Cell turnover and cell tropism in HIV-1 infection},
   Journal = {Trends Microbiol},
   Volume = {10},
   Number = {6},
   Pages = {275-8},
   Note = {0966-842x
Journal Article},
   Abstract = {Early infection with HIV-1 is dominated by CCR5-tropic (R5, non-syncytium-inducing) viruses. The evolution of CXCR4-tropic (X4, syncytium-inducing) viruses occurs later in the infection and is associated with rapid disease progression. Here, we propose that the tropism of X4 viruses for naive CD4+ T cells is disadvantageous in early infection owing to the low division rate of these cells. In healthy individuals, the division rate of memory cells is nearly ten times higher than that of naive cells and thus the memory-cell tropism of R5 viruses could account for their dominance early in infection. As the division rate of naive T cells increases with CD4+ depletion, X4 viruses come to dominate in late disease.},
 Keywords = {CD4-Positive T-Lymphocytes/*virology
HIV Infections/*immunology/metabolism
HIV-1/*pathogenicity
Human
Immunologic Memory
Macrophages/*virology
Models, Biological
Receptors, CCR5/metabolism
Receptors, CXCR4/metabolism
Tropism},
   Year = {2002} }



@article{
Deeks00,
   Author = {Deeks, S. G. and Barbour, J. D. and Martin, J. N. and Swanson, M. S. and Grant, R. M.},
   Title = {Sustained CD4+ T cell response after virologic failure of protease inhibitor-based regimens in patients with human immunodeficiency virus infection},
   Journal = {J Infect Dis},
   Volume = {181},
   Number = {3},
   Pages = {946-53},
   Note = {0022-1899
Journal Article},
   Abstract = {The relationship between plasma human immunodeficiency virus (HIV) RNA levels and peripheral CD4+ T cell counts was examined in 380 HIV-infected adults receiving long-term protease inhibitor therapy. Patients experiencing virologic failure (persistent HIV RNA >500 copies RNA/mL) generally had CD4+ T cell counts that remained greater than pretherapy baseline levels, at least through 96 weeks of follow-up. The CD4+ T cell response was directly and independently related to degree of viral suppression below the pretreatment baseline. For any given HIV RNA level measured 12 weeks after virologic failure, subsequent CD4+ T cell decline was slower in patients receiving a protease inhibitor-based regimen than in a historical control group of untreated patients. These observations suggest that transient or partial declines in plasma HIV RNA levels can have sustained effects on CD4+ T cell levels.},
 Keywords = {Adult
*CD4 Lymphocyte Count
Female
HIV Infections/*drug therapy/immunology/virology
HIV Protease Inhibitors/*therapeutic use
Human
Male
RNA, Viral/*blood
Support, Non-U.S. Gov't
Support, U.S. Gov't, P.H.S.},
   Year = {2000} }



@article{
Deeks01,
   Author = {Deeks, S. G. and Wrin, T. and Liegler, T. and Hoh, R. and Hayden, M. and Barbour, J. D. and Hellmann, N. S. and Petropoulos, C. J. and McCune, J. M. and Hellerstein, M. K. and Grant, R. M.},
   Title = {Virologic and immunologic consequences of discontinuing combination antiretroviral-drug therapy in HIV-infected patients with detectable viremia},
   Journal = {N Engl J Med},
   Volume = {344},
   Number = {7},
   Pages = {472-80},
   Note = {0028-4793
Clinical Trial
Journal Article
Randomized Controlled Trial},
   Abstract = {BACKGROUND: In many patients with human immunodeficiency virus (HIV) infection, therapy with potent antiretroviral drugs does not result in complete suppression of HIV replication. The effect of cessation of therapy in these patients is unknown. METHODS: Sixteen patients who had a plasma HIV RNA level of more than 2500 copies per milliliter during combination antiretroviral-drug therapy were randomly assigned, in a 2:1 ratio, to discontinue or continue therapy. Plasma HIV RNA levels, CD4 cell counts, and drug susceptibility were measured weekly. Viral replicative capacity was measured at base line and at week 12. RESULTS: Discontinuation of therapy for 12 weeks was associated with a median decrease in the CD4 cell count of 128 cells per cubic millimeter and an increase in the plasma HIV RNA level of 0.84 log copies per milliliter. Virus from all patients with detectable resistance at entry became susceptible to HIV-protease inhibitors within 16 weeks after the discontinuation of therapy. Drug susceptibility began to increase a median of six weeks after the discontinuation of therapy and was temporally associated with increases in plasma HIV RNA levels and decreases in CD4 cell counts. Viral replicative capacity, measured by means of a recombinant-virus assay, was low at entry into the study and increased after therapy was discontinued. Despite the loss of detectable resistance in plasma, resistant virus was cultured from peripheral-blood mononuclear cells in five of nine patients who could be evaluated. Plasma HIV RNA levels, CD4 cell counts, and drug susceptibility remained stable in the patients who continued therapy. CONCLUSIONS: Despite the presence of reduced drug susceptibility, antiretroviral-drug therapy can provide immunologic and virologic benefit. This benefit reflects continued antiviral-drug activity and the maintenance of a viral population with a reduced replicative capacity.},
 Keywords = {Adult
Anti-HIV Agents/pharmacology/*therapeutic use
CD4 Lymphocyte Count
Drug Resistance, Microbial
Drug Therapy, Combination
HIV Infections/*drug therapy/immunology/virology
HIV Protease Inhibitors/pharmacology/*therapeutic use
HIV-1/*drug effects/genetics/isolation & purification
Human
Male
Middle Aged
Proportional Hazards Models
Prospective Studies
RNA, Viral/blood
Support, Non-U.S. Gov't
Support, U.S. Gov't, P.H.S.
Viremia/drug therapy},
   Year = {2001} }



@article{
Deeks01b,
   Author = {Deeks, S. G.},
   Title = {International perspectives on antiretroviral resistance. Nonnucleoside reverse transcriptase inhibitor resistance},
   Journal = {J Acquir Immune Defic Syndr},
   Volume = {26 Suppl 1},
   Pages = {S25-33},
   Note = {1525-4135
Journal Article
Review
Review, Tutorial},
   Abstract = {Although understanding of nonnucleoside reverse transcriptase inhibitor (NNRTI) resistance is less clearly established than that of other classes of antiretroviral drugs, certain facts have been established. The treatment-associated genetic mutation profiles of the available NNRTIs have been mapped, and resistance has been found to develop rapidly after initiation of NNRTI therapy. Despite the chemical diversity of the NNRTIs, cross-resistance among agents of this class is nearly universal. Although the viral replicative capacity (``fitness") of NNRTI-induced viral variants has not been extensively studied, available data suggest that NNRTI-selected mutations confer little damage to viral fitness, and thus a single point mutation produces a strain that is both resistant and fit. Furthermore, with continued therapy, viral evolution persists, creating species with greater numbers of mutations and higher level phenotypic resistance. Taken together, these facts suggest that continued use of NNRTIs after emergence of resistance will produce variants of complex mutational patterns that limit future treatment options, and, therefore, strong consideration should be given to discontinuing NNRTIs after virologic failure is confirmed. This article describes the scientific literature establishing the efficacy and limitations of NNRTI therapy and attempts to define a role for this class of drug in the long-term treatment of HIV-1 disease.},
 Keywords = {Anti-HIV Agents/*pharmacology/therapeutic use
Clinical Trials
Delavirdine/pharmacology/therapeutic use
*Drug Resistance, Microbial
Drug Therapy, Combination
HIV Infections/drug therapy/transmission
HIV-1/*drug effects/genetics/metabolism
HIV-1 Reverse Transcriptase/chemistry/genetics
Human
Nevirapine/pharmacology/therapeutic use
Oxazines/pharmacology/therapeutic use
Phylogeny
Point Mutation/drug effects
Protein Conformation
Reverse Transcriptase Inhibitors/*pharmacology/therapeutic use
Virus Replication/drug effects},
   Year = {2001} }



@article{
Deeks02,
   Author = {Deeks, S. G. and Barbour, J. D. and Grant, R. M. and Martin, J. N.},
   Title = {Duration and predictors of CD4 T-cell gains in patients who continue combination therapy despite detectable plasma viremia},
   Journal = {Aids},
   Volume = {16},
   Number = {2},
   Pages = {201-7},
   Note = {0269-9370
Journal Article},
   Abstract = {BACKGROUND: Sustained elevations in CD4 cell counts commonly occur despite incomplete viral suppression with protease inhibitor-based antiretroviral therapy. OBJECTIVES: To determine the incidence and risk factors associated with return of CD4 cell count to pre-therapy levels in patients experiencing virologic failure of protease inhibitor therapy. DESIGN: This is a clinic-based cohort study of HIV-infected adults who failed to maintain durable viral suppression on a protease inhibitor-based regimen. MAIN OUTCOME MEASURES: Virologic failure was defined as persistent plasma HIV RNA level > 500 copies/ml. Immunologic failure was defined as return of CD4 cell count to pre-therapy levels. RESULTS: A total of 291 patients experienced virologic failure on a protease inhibitor-based regimen and had a treatment-mediated CD4 cell increase above pre-therapy levels at the time of virologic failure. If patient data were censored at the time a successful salvage regimen was initiated, then the median time to immunologic failure after the onset of virologic failure was 3 years. If patient data were also censored at the time therapy was discontinued, then 36.8% of the cohort experienced immunologic failure after 3 years of continuous virologic failure. The change in viral load from a pre-treatment baseline, and not the absolute level of viremia achieved, was a strong and independent predictor of immunologic failure. Discontinuing therapy was associated with immunologic failure independent of viral load changes. CONCLUSION: Reduction in T CD4+ cell numbers may eventually occur during prolonged virologic failure of a protease inhibitor-based regimen and is predicted by the degree of virologic suppression below a pre-therapy 'set-point'.},
 Keywords = {Adult
Antiretroviral Therapy, Highly Active
CD4 Lymphocyte Count
CD4-Positive T-Lymphocytes/cytology/*drug effects
Disease Progression
HIV Infections/blood/*drug therapy/immunology/virology
HIV Protease Inhibitors/*therapeutic use
HIV-1/*drug effects/genetics
Human
Indinavir/therapeutic use
Nelfinavir/therapeutic use
RNA, Viral/blood
Ritonavir/therapeutic use
Saquinavir/therapeutic use
Support, Non-U.S. Gov't
Support, U.S. Gov't, P.H.S.
Time Factors
Treatment Failure
Viremia/blood/*drug therapy/immunology/virology},
   Year = {2002} }



@article{
Deeks03,
   Author = {Deeks, S. G.},
   Title = {Treatment of antiretroviral-drug-resistant HIV-1 infection},
   Journal = {Lancet},
   Volume = {362},
   Number = {9400},
   Pages = {2002-11},
   Note = {1474-547x
Journal Article
Review
Review, Academic},
   Abstract = {Drug-resistant HIV-1 is a cause of growing clinical and public-health concern. In many patients, combination antiretroviral therapy fails to achieve complete viral suppression (virological failure). Continuing viral replication during therapy leads to the accumulation of drug-resistance mutations, resulting in increased viral load and a greater risk of disease progression. Patients with drug-resistant HIV-1 infection have three therapeutic options: a change to a salvage regimen with the aim of fully suppressing viral replication; interruption of therapy; or continuation of a partially effective regimen. The first strategy is preferred for most patients failing their first or perhaps their second regimen. However, the best approach remains unclear for patients who have failed multiple treatment regimens and who have limited options for complete viral suppression. The management of such patients requires a careful understanding of the pathogenesis of drug-resistant HIV-1, the clinical consequences of virological failure, the potential benefits and limitations of diagnostic assays, and the likelihood that agents in development will be effective.},
 Keywords = {Anti-HIV Agents/*immunology/*therapeutic use
Antiretroviral Therapy, Highly Active/methods
Drug Resistance, Viral/genetics/immunology
Drug Therapy, Combination
HIV Infections/*drug therapy/immunology/virology
HIV Protease Inhibitors/immunology/therapeutic use
*HIV-1/drug effects/genetics/immunology
Human
Randomized Controlled Trials
Ritonavir/immunology/therapeutic use
Support, Non-U.S. Gov't
Support, U.S. Gov't, P.H.S.
Treatment Outcome
Viral Load/statistics & numerical data
Virus Replication/drug effects/immunology},
   Year = {2003} }



@article{Deeks04,
   Author = {Deeks, S. G. and Walker, B. D.},
   Title = {The immune response to AIDS virus infection: good, bad, or both?},
   Journal = {J Clin Invest},
   Volume = {113},
   Number = {6},
   Pages = {808-10},
   Note = {0021-9738
Comment
Journal Article},
   Abstract = {A potent antigen-specific T cell response to HIV infection can contribute to the control of viral replication and is therefore beneficial to the host. However, HIV-mediated increases in generalized T cell activation also appear to accelerate both viral replication and CD4+ T cell depletion. A new study in the JCI attempts to experimentally distinguish the beneficial versus harmful aspects of this immune response.},
 Year = {2004} }

@techreport{
DHHS04,
   Author = {DHHS},
   Title = {Guidelines for the use of antiretroviral agents in HIV-1 infected adults and adolescents},
   Institution = {Panel on Clinical Practices for Treatment of HIV Infection, Department of Health and Human Services},
   Month= {March 23},
 Year = {2004} }



@article{
Faure00,
   Author = {Faure, S. and Meyer, L. and Costagliola, D. and Vaneensberghe, C. and Genin, E. and Autran, B. and Delfraissy, J. F. and McDermott, D. H. and Murphy, P. M. and Debre, P. and Theodorou, I. and Combadiere, C.},
   Title = {Rapid progression to AIDS in HIV+ individuals with a structural variant of the chemokine receptor CX3CR1},
   Journal = {Science},
   Volume = {287},
   Number = {5461},
   Pages = {2274-7},
   Note = {0036-8075
Comment
Journal Article},
   Abstract = {Human immunodeficiency virus (HIV) enters cells in vitro via CD4 and a coreceptor. Which of 15 known coreceptors are important in vivo is poorly defined but may be inferred from disease-modifying mutations, as for CCR5. Here two single nucleotide polymorphisms are described in Caucasians in CX3CR1, an HIV coreceptor and leukocyte chemotactic/adhesion receptor for the chemokine fractalkine. HIV-infected patients homozygous for CX3CR1-I249 M280, a variant haplotype affecting two amino acids (isoleucine-249 and methionine-280), progressed to AIDS more rapidly than those with other haplotypes. Functional CX3CR1 analysis showed that fractalkine binding is reduced among patients homozygous for this particular haplotype. Thus, CX3CR1-I249 M280 is a recessive genetic risk factor in HIV/AIDS.},
 Keywords = {Acquired Immunodeficiency Syndrome/genetics/*physiopathology/virology
Case-Control Studies
*Chemokines, CX3C
Chemokines, CXC/metabolism
Chromosomes, Human, Pair 3
Cohort Studies
Disease Progression
European Continental Ancestry Group/genetics
Genotype
HIV/physiology
HIV Infections/genetics/*physiopathology/virology
Haplotypes
Homozygote
Human
Leukocytes, Mononuclear/metabolism
Linkage Disequilibrium
Membrane Proteins/metabolism
Mutation
Polymorphism, Restriction Fragment Length
*Polymorphism, Single Nucleotide
Polymorphism, Single-Stranded Conformational
Receptors, Cytokine/*genetics/*physiology
Receptors, HIV/*genetics/*physiology
Support, Non-U.S. Gov't
Survival Analysis
Variation (Genetics)},
   Year = {2000} }



@article{
Gao01,
   Author = {Gao, X. and Nelson, G. W. and Karacki, P. and Martin, M. P. and Phair, J. and Kaslow, R. and Goedert, J. J. and Buchbinder, S. and Hoots, K. and Vlahov, D. and O'Brien, S. J. and Carrington, M.},
   Title = {Effect of a single amino acid change in MHC class I molecules on the rate of progression to AIDS},
   Journal = {N Engl J Med},
   Volume = {344},
   Number = {22},
   Pages = {1668-75},
   Note = {0028-4793
Journal Article
Multicenter Study},
   Abstract = {BACKGROUND: From studies of genetic polymorphisms and the rate of progression from human immunodeficiency virus type 1 (HIV-1) infection to the acquired immunodeficiency syndrome (AIDS), it appears that the strongest susceptibility is conferred by the major-histocompatibility-complex (MHC) class I type HLA-B*35,Cw*04 allele. However, cytotoxic T-lymphocyte responses have been observed against HIV-1 epitopes presented by HLA-B*3501, the most common HLA-B*35 subtype. We examined subtypes of HLA-B*35 in five cohorts and analyzed the relation of structural differences between HLA-B*35 subtypes to the risk of progression to AIDS. METHODS: Genotyping of HLA class I loci was performed for 850 patients who seroconverted and had known dates of HIV-1 infection. Survival analyses with respect to the rate of progression to AIDS were performed to identify the effects of closely related HLA-B*35 subtypes with different peptide-binding specificities. RESULTS: HLA-B*35 subtypes were divided into two groups according to peptide-binding specificity: the HLA-B*35-PY group, which consists primarily of HLA-B*3501 and binds epitopes with proline in position 2 and tyrosine in position 9; and the more broadly reactive HLA-B*35-Px group, which also binds epitopes with proline in position 2 but can bind several different amino acids (not including tyrosine) in position 9. The influence of HLA-B*35 in accelerating progression to AIDS was completely attributable to HLA-B*35-Px alleles, some of which differ from HLA-B*35-PY alleles by only one amino acid residue. CONCLUSIONS: This analysis shows that, in patients with HIV-1 infection, a single amino acid change in HLA molecules has a substantial effect on the rate of progression to AIDS. The different consequences of HLA-B*35-PY and HLA-B*35-Px in terms of disease progression highlight the importance of the epitope specificities of closely related class I molecules in the immune defense against HIV-1.},
 Keywords = {Acquired Immunodeficiency Syndrome/*genetics
African Continental Ancestry Group/genetics
Alleles
Amino Acid Sequence
Binding Sites/genetics
Disease Progression
Disease-Free Survival
European Continental Ancestry Group/genetics
*Genes, MHC Class I
Genotype
HIV Infections/ethnology/*genetics/immunology
HLA-B35 Antigen/chemistry/*genetics
HLA-C Antigens
Human
Peptides/metabolism
Proportional Hazards Models
Receptors, Peptide/chemistry/genetics/metabolism
Support, U.S. Gov't, P.H.S.},
   Year = {2001} }



@article{
Grabar00,
   Author = {Grabar, S. and Le Moing, V. and Goujard, C. and Leport, C. and Kazatchkine, M. D. and Costagliola, D. and Weiss, L.},
   Title = {Clinical outcome of patients with HIV-1 infection according to immunologic and virologic response after 6 months of highly active antiretroviral therapy},
   Journal = {Ann Intern Med},
   Volume = {133},
   Number = {6},
   Pages = {401-10},
   Note = {0003-4819
Journal Article
Multicenter Study},
   Abstract = {BACKGROUND: The prognostic value of discordant immunologic (CD4 cell increase) and virologic (plasma HIV RNA level decrease) responses to antiretroviral treatment is not known. OBJECTIVE: To study the relation between clinical outcome of HIV-infected patients receiving highly active antiretroviral therapy (HAART) and early immunologic and virologic responses to such therapy. DESIGN: Prospective cohort study. SETTING: 68 hospitals in France. PATIENTS: 2236 protease inhibitor-naive patients. INTERVENTION: Initiation of HAART with one protease inhibitor and two nucleoside analogues between July 1996 and March 1997. MEASUREMENTS: Immunologic and virologic response at 6 months. Multivariate Cox models were used to assess the relation between these responses and progression to a new AIDS-defining event or death. RESULTS: On the basis of 6-month immunologic and virologic responses, patients were classified into four groups: complete response (47.5%), complete nonresponse (16.2%), immunologic response only (19.0%), and virologic response only (17.3%). After month 6 and within a median of 18 months, 69 patients died and 123 experienced a new AIDS-defining event. After adjustment, complete nonresponders and those with only a virologic response had significantly higher risks for clinical progression at 6 months (relative risk, 3.38 [95% CI, 2.28 to 5.02] and 1.98 [CI, 1.26 to 3.10], respectively) than complete responders. The difference between complete responders and those with only an immunologic response at 6 months was weaker and nonsignificant (relative risk, 1.55 [CI, 0.96 to 2.50]). CONCLUSIONS: Immunologic response after 6 months of HAART indicates a favorable clinical outcome in HIV-infected patients regardless of virologic response. This suggests that both immunologic and virologic markers should be used in clinical practice to evaluate treatment response.},
 Keywords = {Adult
CD4 Lymphocyte Count
Disease Progression
Drug Therapy, Combination
Female
HIV Infections/*drug therapy/immunology/virology
HIV Protease Inhibitors/*therapeutic use
*HIV-1/genetics
Human
Male
Multivariate Analysis
Proportional Hazards Models
Prospective Studies
RNA, Viral/blood
Reverse Transcriptase Inhibitors/*therapeutic use
Support, Non-U.S. Gov't
Treatment Outcome
Viral Load},
   Year = {2000} }



@article{
Grueb00,
   Author = {Greub, G. and Ledergerber, B. and Battegay, M. and Grob, P. and Perrin, L. and Furrer, H. and Burgisser, P. and Erb, P. and Boggian, K. and Piffaretti, J. C. and Hirschel, B. and Janin, P. and Francioli, P. and Flepp, M. and Telenti, A.},
   Title = {Clinical progression, survival, and immune recovery during antiretroviral therapy in patients with HIV-1 and hepatitis C virus coinfection: the Swiss HIV Cohort Study},
   Journal = {Lancet},
   Volume = {356},
   Number = {9244},
   Pages = {1800-5},
   Note = {0140-6736
Clinical Trial
Journal Article},
   Abstract = {BACKGROUND: Hepatitis C virus (HCV) infection is highly prevalent among HIV-1-infected individuals, but its contribution to the morbidity and mortality of coinfected patients who receive potent antiretroviral therapy is controversial. We used data from the ongoing Swiss HIV Cohort Study to analyse clinical progression of HIV-1, and the virological and immunological response to potent antiretroviral therapy in HIV-1-infected patients with or without concurrent HCV infection. METHODS: We analysed prospective data on survival, clinical disease progression, suppression of HIV-1 replication, CD4-cell recovery, and frequency of changes in antiretroviral therapy according to HCV status in 3111 patients starting potent antiretroviral therapy. RESULTS: 1157 patients (37.2%) were coinfected with HCV, 1015 of whom (87.7%) had a history of intravenous drug use. In multivariate Cox's regression, the probability of progression to a new AIDS-defining clinical event or to death was independently associated with HCV seropositivity (hazard ratio 1.7 [95% CI 1.26-2.30]), and with active intravenous drug use (1.38 [1.02-1.88]). Virological response to antiretroviral therapy and the probability of treatment change were not associated with HCV serostatus. In contrast, HCV seropositivity was associated with a smaller CD4-cell recovery (hazard ratio for a CD4-cell count increase of at least 50 cells/microL=0.79 [0.72-0.87]). INTERPRETATION: HCV and active intravenous drug use could be important factors in the morbidity and mortality among HIV-1-infected patients, possibly through impaired CD4-cell recovery in HCV seropositive patients receiving potent antiretroviral therapy. These findings are relevant for decisions about optimum timing for HCV treatment in the setting of HIV infection.},
 Keywords = {AIDS-Related Opportunistic Infections/*drug therapy
Adolescent
Adult
Anti-HIV Agents/*therapeutic use
CD4 Lymphocyte Count
Cohort Studies
Disease Progression
Female
Hepatitis C/complications/*drug therapy
Human
Male
Middle Aged
Prospective Studies
Support, Non-U.S. Gov't
Survival Analysis
Switzerland
Viral Load
Viremia/etiology},
   Year = {2000} }



@article{
Katzenstein96,
   Author = {Katzenstein, D. A. and Hammer, S. M. and Hughes, M. D. and Gundacker, H. and Jackson, J. B. and Fiscus, S. and Rasheed, S. and Elbeik, T. and Reichman, R. and Japour, A. and Merigan, T. C. and Hirsch, M. S.},
   Title = {The relation of virologic and immunologic markers to clinical outcomes after nucleoside therapy in HIV-infected adults with 200 to 500 CD4 cells per cubic millimeter. AIDS Clinical Trials Group Study 175 Virology Study Team},
   Journal = {N Engl J Med},
   Volume = {335},
   Number = {15},
   Pages = {1091-8},
   Note = {0028-4793
Clinical Trial
Journal Article
Multicenter Study
Randomized Controlled Trial},
   Abstract = {BACKGROUND: We studied measures of human immunodeficiency virus (HIV) replication, the viral phenotype, and immune function (CD4 cell counts) and the relation of changes in these indicators to clinical outcomes in a subgroup of patients in a controlled trial of early antiretroviral treatment for HIV, the AIDS Clinical Trials Group Study 175. METHODS: The 391 subjects, each of whom entered the study with a single screening CD4 cell count of 200 to 500 per cubic millimeter, were randomly assigned to receive zidovudine alone, didanosine alone, zidovudine plus didanosine, or zidovudine plus zalcitabine. Plasma concentrations of HIV RNA were assessed in 366 subjects, and viral isolates from 332 subjects were assayed for the presence of the syncytium-inducing phenotype. RESULTS: After eight weeks, the mean (+/-SE) decrease from base line in the concentration of HIV RNA, expressed as the change in the base 10 log of the number of copies per milliliter, was 0.26+/-0.06 for patients treated with zidovudine alone, 0.65+/-0.07 for didanosine alone, 0.93+/-0.10 for zidovudine plus didanosine, and 0.89+/-0.06 for zidovudine plus zalcitabine (P<0.001 for each of the pairwise comparisons with zidovudine alone). Multivariate proportional-hazards models showed that higher base-line concentrations of plasma HIV RNA, less suppression of plasma HIV RNA by treatment, and the presence of the syncytium-inducing phenotype were significantly associated with an increased risk of progression to the acquired immunodeficiency syndrome and death. After adjustment for these measures of viral replication and for the viral phenotype, CD4 cell counts were not significant predictors of clinical outcome. CONCLUSIONS: Both the risk of the progression of HIV disease and the efficacy of antiretroviral therapy are strongly associated with the plasma level of HIV RNA and with the viral phenotype. The changes in the plasma concentration of HIV RNA predict the changes in CD4 cell counts and survival after treatment with reverse-transcriptase inhibitors.},
 Keywords = {Adult
Antiviral Agents/*therapeutic use
CD4 Lymphocyte Count
Didanosine/*therapeutic use
Disease Progression
Drug Therapy, Combination
Female
HIV/*genetics/isolation & purification/physiology
HIV Infections/drug therapy/immunology/*virology
Human
Male
Middle Aged
Multivariate Analysis
Phenotype
Proportional Hazards Models
RNA, Viral/*blood
Support, U.S. Gov't, P.H.S.
Treatment Outcome
Virus Replication/drug effects
Zidovudine/*therapeutic use},
   Year = {1996} }



@article{
Kaufmann98,
   Author = {Kaufmann, D. and Pantaleo, G. and Sudre, P. and Telenti, A.},
   Title = {CD4-cell count in HIV-1-infected individuals remaining viraemic with highly active antiretroviral therapy (HAART). Swiss HIV Cohort Study},
   Journal = {Lancet},
   Volume = {351},
   Number = {9104},
   Pages = {723-4},
   Note = {0140-6736
Letter},
 Keywords = {Anti-HIV Agents/*therapeutic use
CD4 Lymphocyte Count
HIV Infections/drug therapy/*immunology
Human
Protease Inhibitors/*therapeutic use
Support, Non-U.S. Gov't
Viremia/drug therapy/*immunology},
   Year = {1998} }



@article{
Kaufmann03,
   Author = {Kaufmann, G. R. and Perrin, L. and Pantaleo, G. and Opravil, M. and Furrer, H. and Telenti, A. and Hirschel, B. and Ledergerber, B. and Vernazza, P. and Bernasconi, E. and Rickenbach, M. and Egger, M. and Battegay, M.},
   Title = {CD4 T-lymphocyte recovery in individuals with advanced HIV-1 infection receiving potent antiretroviral therapy for 4 years: the Swiss HIV Cohort Study},
   Journal = {Arch Intern Med},
   Volume = {163},
   Number = {18},
   Pages = {2187-95},
   Note = {0003-9926
Journal Article},
   Abstract = {BACKGROUND: Highly active antiretroviral therapy (HAART) for human immunodeficiency virus (HIV)-1 infection allows recovery of CD4 T lymphocytes. Few studies have explored the long-term T-lymphocyte responses to HAART. METHODS: Plasma HIV-1 RNA levels and CD4 and CD8 T-lymphocyte counts were longitudinally analyzed over 4 years in 2235 participants of the Swiss HIV Cohort, commencing HAART between 1996 and 1997. The CD4 T-lymphocyte count increase, the percentage of individuals with a CD4 T-lymphocyte count of 500/microL or greater and less than 200/microL, and the determinants of CD4 T-lymphocyte recovery were evaluated in individuals treated with continuous (CONT; n = 985) and discontinuous (DISCONT; n = 1250) HAART. RESULTS: At 4 years, 69.5% of subjects (CONT, 84.5%; DISCONT, 53.6%; P<.001) showed HIV-1 RNA levels below 400 copies/mL, while the median CD4 T-lymphocyte count increased from 190/microL to 423/microL (CONT, 486/microL; DISCONT, 343/microL; P<.001). Of the 2235 participants, 38.8% (CONT, 47.7%; DISCONT, 29.4%; P<.001) reached a CD4 T-lymphocyte count of 500/microL or greater, but in 15.6%, CD4 T-lymphocyte count remained below 200/microL (CONT, 5.9%; DISCONT, 25.9%; P<.001). Larger increases in CD4 T-lymphocyte count were associated with higher baseline HIV-1 RNA, a larger percentage of undetectable HIV-1 RNA levels, lower baseline CD8 T-lymphocyte count, and younger age. Individuals reaching a CD4 T-lymphocyte count of 500/microL or greater at 4 years were characterized by higher nadir and baseline CD4 T-lymphocyte counts and a more sustained reduction of HIV-1 RNA levels. CONCLUSIONS: At 4 years, only 39% of individuals treated with HAART reached a CD4 T-lymphocyte count of 500/microL or greater, and 16% with CD4 T-lymphocyte counts less than 200/microL remained susceptible to opportunistic infections. Treatment interruptions, a poor virologic response, and older age were the major factors negatively affecting the recovery of CD4 T lymphocytes.},
 Keywords = {Adult
*Antiretroviral Therapy, Highly Active
*CD4 Lymphocyte Count
CD8-Positive T-Lymphocytes
Female
HIV Infections/*drug therapy/*immunology
*Hiv-1
Human
Lymphocyte Count
Male
Middle Aged
Prospective Studies
RNA, Viral/*analysis
Support, Non-U.S. Gov't
Viral Load},
   Year = {2003} }



@article{
MartinezPicado99,
   Author = {Martinez-Picado, J. and Savara, A. V. and Sutton, L. and D'Aquila, R. T.},
   Title = {Replicative fitness of protease inhibitor-resistant mutants of human immunodeficiency virus type 1},
   Journal = {J Virol},
   Volume = {73},
   Number = {5},
   Pages = {3744-52},
   Note = {0022-538x
Journal Article},
   Abstract = {The relative replicative fitness of human immunodeficiency virus type 1 (HIV-1) mutants selected by different protease inhibitors (PIs) in vivo was determined. Each mutant was compared to wild type (WT), NL4-3, in the absence of drugs by several methods, including clonal genotyping of cultures infected with two competing viral variants, kinetics of viral antigen production, and viral infectivity/virion particle ratios. A nelfinavir-selected protease D30N substitution substantially decreased replicative capacity relative to WT, while a saquinavir-selected L90M substitution moderately decreased fitness. The D30N mutant virus was also outcompeted by the L90M mutant in the absence of drugs. A major natural polymorphism of the HIV-1 protease, L63P, compensated well for the impairment of fitness caused by L90M but only slightly improved the fitness of D30N. Multiply substituted indinavir-selected mutants M46I/L63P/V82T/I84V and L10R/M46I/L63P/V82T/I84V were just as fit as WT. These results indicate that the mutations which are usually initially selected by nelfinavir and saquinavir, D30N and L90M, respectively, impair fitness. However, additional mutations may improve the replicative capacity of these and other drug-resistant mutants. Hypotheses based on the greater fitness impairment of the nelfinavir-selected D30N mutant are suggested to explain observations that prolonged responses to delayed salvage regimens, including alternate PIs, may be relatively common after nelfinavir failure.},
 Keywords = {Adaptation, Biological
Amino Acid Substitution
Animals
Anti-HIV Agents/*pharmacology
Cells, Cultured
Drug Resistance, Microbial
HIV Protease Inhibitors/*pharmacology
HIV-1/*drug effects/genetics/physiology
Human
Mice
Mutagenesis, Site-Directed
Nelfinavir/*pharmacology
Saquinavir/*pharmacology
Support, Non-U.S. Gov't
Support, U.S. Gov't, P.H.S.
Tumor Cells, Cultured
Virus Replication/*drug effects},
   Year = {1999} }



@article{
Mellors96,
   Author = {Mellors, J. W. and Rinaldo, C. R., Jr. and Gupta, P. and White, R. M. and Todd, J. A. and Kingsley, L. A.},
   Title = {Prognosis in HIV-1 infection predicted by the quantity of virus in plasma},
   Journal = {Science},
   Volume = {272},
   Number = {5265},
   Pages = {1167-70},
   Note = {0036-8075
Comment
Journal Article},
   Abstract = {The relation between viremia and clinical outcome in individuals infected with human immunodeficiency virus-type 1 (HIV-1) has important implications for therapeutic research and clinical care. HIV-1 RNA in plasma was quantified with a branched-DNA signal amplification assay as a measure of viral load in a cohort of 180 seropositive men studied for more than 10 years. The risk of acquired immunodeficiency syndrome (AIDS) and death in study subjects, including those with normal numbers of CD4+ T cells, was directly related to plasma viral load at study entry. Plasma viral load was a better predictor of progression to AIDS and death than was the number of CD4+ T cells.},
 Keywords = {Acquired Immunodeficiency Syndrome/*virology
Antiviral Agents/therapeutic use
Biological Markers/blood
CD4 Lymphocyte Count
CD4-Positive T-Lymphocytes/virology
Cohort Studies
Disease Progression
Follow-Up Studies
HIV Infections/drug therapy/mortality/*virology
HIV-1/genetics/*physiology
Human
Male
Prognosis
Proportional Hazards Models
RNA, Viral/*blood
Support, Non-U.S. Gov't
Support, U.S. Gov't, Non-P.H.S.
Support, U.S. Gov't, P.H.S.
Survival Rate
Time Factors
Viremia/*virology
Virus Replication},
   Year = {1996} }



@article{
Miller00,
   Author = {Miller, V. and Sabin, C. A. and Phillips, A. N. and Rottmann, C. and Rabenau, H. and Weidmann, E. and Rickerts, V. and Findhammer, S. and Helm, E. B. and Staszewski, S.},
   Title = {The impact of protease inhibitor-containing highly active antiretroviral therapy on progression of HIV disease and its relationship to CD4 and viral load},
   Journal = {Aids},
   Volume = {14},
   Number = {14},
   Pages = {2129-36},
   Note = {0269-9370
Clinical Trial
Journal Article},
   Abstract = {OBJECTIVE: To compare the rate of disease progression according to viral load and CD4 cell count in patients receiving or not receiving highly active antiretroviral therapy (HAART), defined as protease inhibitor-containing regimens. DESIGN: An observational study, with prospectively collected data. METHODS: All patients attending the HIV Outpatient clinic as of 1 January 1995 (n = 2083) were included. Follow-up was until the first AIDS-defining event or death. Associations between viral load or CD4 cell count and disease progression were assessed using a person-years approach. Event rates were compared using Poisson regression analysis; a multivariate model was used to assess the independent effects of CD4, viral load and treatment group on event rates and to consider interactions between these variables. RESULTS: The event rates increased with lower CD4 cell count and higher viral load for both treatment groups and were generally lower in the HAART group. In a multivariate analysis, lower CD4 cell counts and higher viral loads remained significantly associated with disease progression, irrespective of treatment group. However, the event rate was significantly lower for the HAART group compared with the control group (relative rate 0.53, P < 0.001). CONCLUSIONS: HAART-treated patients with high viral loads and CD4 cell counts experienced reduced disease progression compared with individuals with the same CD4 cell count and viral load not receiving HAART. Consequently, the short-term prognosis associated with viral load levels and CD4 cell counts may differ in patients on HAART. Whether this effect will be observed with non-protease-inhibitor-containing HAART is not known at this time.},
 Keywords = {Adolescent
Adult
Aged
Antiretroviral Therapy, Highly Active
CD4 Lymphocyte Count
Disease Progression
HIV Infections/*drug therapy/pathology/virology
HIV Protease Inhibitors/*therapeutic use
*HIV-1/isolation & purification
Human
Middle Aged
Prospective Studies
RNA, Viral/analysis
Regression Analysis
Support, Non-U.S. Gov't
Viral Load},
   Year = {2000} }



@article{
Piketty98,
   Author = {Piketty, C. and Castiel, P. and Belec, L. and Batisse, D. and Si Mohamed, A. and Gilquin, J. and Gonzalez-Canali, G. and Jayle, D. and Karmochkine, M. and Weiss, L. and Aboulker, J. P. and Kazatchkine, M. D.},
   Title = {Discrepant responses to triple combination antiretroviral therapy in advanced HIV disease},
   Journal = {Aids},
   Volume = {12},
   Number = {7},
   Pages = {745-50},
   Note = {0269-9370
Journal Article},
   Abstract = {OBJECTIVES: To determine the clinical, virological and immunological outcome in a cohort of unselected patients receiving triple combination therapy for more than 1 year. METHODS: Prospective follow-up of a cohort of 162 unselected, protease inhibitor-naive, antiretroviral-experienced patients with advanced HIV disease, treated with indinavir combined with two nucleoside analogues. RESULTS: The mean CD4 cell count and plasma HIV RNA level in the study group at baseline were 69+/-5 x 10(6)/l and 4.75+/-0.07 log10 copies/ml, respectively. Five per cent of patients died prematurely or were lost to follow-up. Fifty-seven per cent of patients responded to therapy, as assessed by a sustained increase in CD4 cell counts above 50 x 10(6)/l and a decrease in plasma HIV RNA greater than 1 log10 copies/ml, throughout 12.1 months of follow-up. Seventeen per cent of patients were immunological and virological non-responders. Twenty-one per cent of patients exhibited discrepant virological and immunological responses to treatment, of whom one-half failed to exhibit significant increases in CD4 cells despite a virological response to therapy and one-half exhibited increased CD4 cell counts in the absence of significant decrease in plasma viral load. The incidence of AIDS-defining events in the latter group of patients was similar to that of responder patients, whereas their incidence was higher in patients who failed to exhibit a virological and immunological response and those who failed to increase CD4 cells despite a significant decrease in viral load. CONCLUSION: Our observations of discrepant immunological and virological responses to treatment raise the issue of the significance of persistent elevated levels of plasma HIV RNA and of the relevance of measurements of plasma viral load for assessing the efficacy of antiretroviral therapy in patients whose CD4 cell counts increase despite the absence of significant decrease in plasma HIV viral load.},
 Keywords = {Adult
Aged
Anti-HIV Agents/*therapeutic use
Cohort Studies
Drug Therapy, Combination
Female
Follow-Up Studies
HIV Infections/*drug therapy/immunology/physiopathology/virology
HIV Protease Inhibitors/*therapeutic use
Human
Indinavir/*therapeutic use
Lamivudine/*therapeutic use
Male
Middle Aged
Prospective Studies
Reverse Transcriptase Inhibitors/*therapeutic use
Stavudine/*therapeutic use
Support, Non-U.S. Gov't
Treatment Outcome
Zidovudine/*therapeutic use},
   Year = {1998} }



@article{
Piketty01,
   Author = {Piketty, C. and Weiss, L. and Thomas, F. and Mohamed, A. S. and Belec, L. and Kazatchkine, M. D.},
   Title = {Long-term clinical outcome of human immunodeficiency virus-infected patients with discordant immunologic and virologic responses to a protease inhibitor-containing regimen},
   Journal = {J Infect Dis},
   Volume = {183},
   Number = {9},
   Pages = {1328-35},
   Note = {0022-1899
Journal Article},
   Abstract = {Within a prospective cohort of 150 human immunodeficiency virus (HIV)-infected patients who began first-line protease inhibitor therapy in 1996, the outcome of 42 patients with discrepant virologic and immunologic responses to antiretroviral treatment at 12 months was analyzed at 30 months of treatment. The incidence of AIDS-defining events and deaths (14%) in the group of patients with immunologic responses in the absence of a virologic response was higher than that in full-responder patients (2%); yet, the incidence in this group was lower than that in patients with no immunologic response, despite a virologic response (21%), and was lower than that in patients without an immunologic or virologic response (67%; P<.0001, log-rank test). Differences in outcome were significant (relative risk, 6.9; 95% confidence interval, 1.9-39.3) when factors for progression were compared with those of responder patients. The results support the relevance of the CD4 cell marker over plasma HIV load for predicting clinical outcome in patients who do not achieve full immunologic and virologic responses.},
 Keywords = {Adult
Aged
Antiretroviral Therapy, Highly Active
CD4 Lymphocyte Count
Cohort Studies
Disease Progression
Female
HIV Infections/*drug therapy/immunology/virology
HIV Protease Inhibitors/*therapeutic use
Human
Incidence
Longitudinal Studies
Male
Middle Aged
Mortality
Prospective Studies
RNA, Viral/blood
Time Factors
Treatment Outcome
Viral Load},
   Year = {2001} }



@article{
Pilon02,
   Author = {Pilon, A. A. and Lum, J. J. and Sanchez-Dardon, J. and Phenix, B. N. and Douglas, R. and Badley, A. D.},
   Title = {Induction of apoptosis by a nonnucleoside human immunodeficiency virus type 1 reverse transcriptase inhibitor},
   Journal = {Antimicrob Agents Chemother},
   Volume = {46},
   Number = {8},
   Pages = {2687-91},
   Note = {0066-4804
Journal Article},
   Abstract = {Inhibition of human immunodeficiency virus type 1 reverse transcriptase (RT) by both nucleoside and nonnucleoside RT inhibitors profoundly inhibits virus replication. Nucleoside RT inhibitors are known to be toxic, but there is little information regarding the toxicities of nonnucleoside RT inhibitors (NNRTI). We demonstrate that efavirenz (an NNRTI) induces caspase- and mitochondrion-dependent apoptosis of Jurkat T cells and human peripheral blood mononuclear cells. The clinical relevance of these observations is not yet clear.},
 Keywords = {Annexin V/diagnostic use
Apoptosis/*drug effects
Caspases/physiology
Enzyme Inhibitors/diagnostic use
Fluorescein-5-isothiocyanate
Fluorescent Dyes
HIV-1 Reverse Transcriptase/*antagonists & inhibitors
Human
Jurkat Cells
Membrane Potentials/drug effects
Mitochondria/drug effects/physiology
Oxazines/*pharmacology
Reverse Transcriptase Inhibitors/*pharmacology
Support, Non-U.S. Gov't},
   Year = {2002} }



@article{
Price03,
   Author = {Price, D. A. and Scullard, G. and Oxenius, A. and Braganza, R. and Beddows, S. A. and Kazmi, S. and Clarke, J. R. and Johnson, G. E. and Weber, J. N. and Phillips, R. E.},
   Title = {Discordant outcomes following failure of antiretroviral therapy are associated with substantial differences in human immunodeficiency virus-specific cellular immunity},
   Journal = {J Virol},
   Volume = {77},
   Number = {10},
   Pages = {6041-9},
   Note = {0022-538x
Clinical Trial
Journal Article},
   Abstract = {Many individuals chronically infected with human immunodeficiency virus type 1 (HIV-1) experience a recrudescence of plasma virus during continuous combination antiretroviral therapy (ART) due either to the emergence of drug-resistant viruses or to poor compliance. In most cases, virologic failure on ART is associated with a coincident decline in CD4(+) T lymphocyte levels. However, a proportion of discordant individuals retain a stable or even increasing CD4(+) T lymphocyte count despite virological failure. In order to address the nature of these different outcomes, we evaluated virologic and immunologic variables in a prospective, single-blinded, nonrandomized cohort of 53 subjects with chronic HIV-1 infection who had been treated with continuous ART and monitored intensively over a period of 19 months. In all individuals with detectable viremia on ART, multiple drug resistance mutations with similar impacts on viral growth kinetics were detected in the pol gene of circulating plasma virus. Further, C2V3 env gene analysis demonstrated sequences indicative of CCR5 coreceptor usage in the majority of those with detectable plasma viremia. In contrast to this homogeneous virologic pattern, comprehensive screening with a range of antigens derived from HIV-1 revealed substantial immunologic differences. Discordant subjects with stable CD4(+) T lymphocyte counts in the presence of recrudescent virus demonstrated potent virus-specific CD4(+) and CD8(+) T lymphocyte responses. In contrast, subjects with virologic failure associated with declining CD4(+) T lymphocyte counts had substantially weaker HIV-specific CD4(+) T lymphocyte responses and exhibited a trend towards weaker HIV-specific CD8(+) T lymphocyte responses. Importantly the CD4(+) response was sustained over periods as long as 11 months, confirming the stability of the phenomenon. These correlative data lead to the testable hypothesis that the consequences of viral recrudescence during continuous ART are modulated by the HIV-specific cellular immune response.},
 Keywords = {Adult
Amino Acid Sequence
Anti-HIV Agents/pharmacology/*therapeutic use
CD4-Positive T-Lymphocytes/*immunology
CD8-Positive T-Lymphocytes/*immunology
Chronic Disease
Drug Resistance, Viral/genetics
Drug Therapy, Combination
HIV Envelope Protein gp120/chemistry/genetics
HIV Infections/*drug therapy/immunology/physiopathology
HIV-1/*drug effects/genetics/physiology
Human
Lymphocyte Count
Middle Aged
Molecular Sequence Data
Mutation
Peptide Fragments/chemistry/genetics
Prospective Studies
RNA, Viral/blood
Single-Blind Method
Support, Non-U.S. Gov't
*Treatment Failure
Viral Load},
   Year = {2003} }



@article{
Quinones00,
   Author = {Quinones-Mateu, M. E. and Ball, S. C. and Marozsan, A. J. and Torre, V. S. and Albright, J. L. and Vanham, G. and van Der Groen, G. and Colebunders, R. L. and Arts, E. J.},
   Title = {A dual infection/competition assay shows a correlation between ex vivo human immunodeficiency virus type 1 fitness and disease progression},
   Journal = {J Virol},
   Volume = {74},
   Number = {19},
   Pages = {9222-33},
   Note = {0022-538x
Journal Article},
   Abstract = {This study was designed to examine the impact of human immunodeficiency virus type 1 (HIV-1) fitness on disease progression through the use of a dual competition/heteroduplex tracking assay (HTA). Despite numerous studies on the impact of HIV-1 diversity and HIV-specific immune response on disease progression, we still do not have a firm understanding of the long-term pathogenesis of this virus. Strong and early CD8-positive cytotoxic T-cell and CD4-positive T-helper cell responses directed toward HIV-infected cells appear to curb HIV pathogenesis. However, the rate at which the virus infects the CD4(+) T-cell population and possibly destroys the HIV-specific immune response may also alter the rate of disease progression. For HIV-1 fitness studies, we established conditions for dual HIV-1 infections of peripheral blood mononuclear cells (PBMC) and a sensitive HTA to measure relative virus production. A pairwise comparison was then performed to estimate the relative fitness of various non-syncytium-inducing/CCR5-tropic (NSI/R5) and syncytium-inducing/CXCR4-tropic (SI/X4) HIV-1 isolates. Four HIV-1 strains (two NSI/R5 and two SI/X4) with moderate ex vivo fitness were then selected as controls and competed against primary HIV-1 isolates from an HIV-infected Belgian cohort. HIV-1 isolates from long-term survivors (LTS) were outcompeted by control strains and were significantly less fit than HIV-1 isolates from patients with accelerated progression to AIDS (PRO). In addition, NSI/R5 HIV-1 isolates from PRO overgrew control SI/X4 strains, suggesting that not all SI/X4 HIV-1 isolates replicate more efficiently than all NSI/R5 isolates. Finally, there were strong, independent correlations between viral load and the total relative fitness values of HIV-1 isolates from PRO (r = 0.84, P = 0.033) and LTS (r = 0.86, P = 0.028). Separation of the PRO and LTS plots suggest that HIV-1 fitness together with viral load may be a strong predictor for the rate of disease progression.},
 Keywords = {*Biological Assay
HIV Infections/*physiopathology/*virology
*HIV-1/physiology
Human
Predictive Value of Tests
Prognosis
Support, Non-U.S. Gov't
Support, U.S. Gov't, P.H.S.},
   Year = {2000} }



@article{
Racinan02,
   Author = {Rancinan, C. and Neau, D. and Saves, M. and Lawson-Ayayi, S. and Bonnet, F. and Mercie, P. and Dupon, M. and Couzigou, P. and Dabis, F. and Chene, G.},
   Title = {Is hepatitis C virus co-infection associated with survival in HIV-infected patients treated by combination antiretroviral therapy?},
   Journal = {Aids},
   Volume = {16},
   Number = {10},
   Pages = {1357-62},
   Note = {0269-9370
Journal Article},
   Abstract = {OBJECTIVE: To study whether hepatitis C virus (HCV) co-infection or the severe elevation of transaminases is associated with survival after the initiation of antiretroviral combination therapy. DESIGN: Prospective hospital-based cohort (Aquitaine Cohort). METHODS: HIV-infected adults started on an antiretroviral combination before 30 June 1999. HCV infection was defined as antibody detection or positive HCV RNA. Severe elevation of transaminases was defined as a value of aspartate or alanine aminotransferase (AST, ALT) above five times the upper limit of normal values. Survival was studied using a Cox model, including at least baseline HCV status and transaminases as a time-dependent covariate. RESULTS: Overall, 995 patients were analysed, including 576 HCV-positive individuals (58%). At baseline, HCV-positive patients were younger, more often injecting drug users and women, and had more frequently elevated transaminases. A shorter survival was associated with AIDS stage [hazard ratio (HR) versus non-AIDS 1.67; 95% confidence interval (CI) 1.03; 2.68], lower CD4 cell count (HR for 50 cells/mm3 lower 1.33; CI 1.17; 1.51), lower haemoglobin (HR for 1 g/dl lower 1.20; CI 1.07; 1.35), lower platelet count (HR for 10 000 cells/mm3 lower 1.04; CI 1.01; 1.07), and AST during follow-up (HR for > or = 200 IU/l 2.30; CI 1.32; 4.03). HCV co-infection (HR 1.20; CI 0.75; 1.92) was not statistically associated with survival. CONCLUSION: The occurrence of a severe elevation of transaminases was associated with poorer survival, although HCV was not. If liver toxicity may be treatment induced, plasma drug concentrations could guide dosage adjustments of antiretroviral treatments currently prescribed to optimize their use.},
 Keywords = {Acquired Immunodeficiency Syndrome/complications
Age Factors
Anti-HIV Agents/*therapeutic use
Antiretroviral Therapy, Highly Active
Cohort Studies
Comparative Study
Disease Progression
Female
Follow-Up Studies
HIV Infections/blood/*complications/*drug therapy
Hepatitis C/blood/*complications
Human
Male
Proportional Hazards Models
Substance Abuse, Intravenous
Support, Non-U.S. Gov't
Survival Analysis
Transaminases/blood},
   Year = {2002} }



@article{
Roger99,
   Author = {Roger, P. M. and Breittmayer, J. P. and Arlotto, C. and Pugliese, P. and Pradier, C. and Bernard-Pomier, G. and Dellamonica, P. and Bernard, A.},
   Title = {Highly active anti-retroviral therapy (HAART) is associated with a lower level of CD4+ T cell apoptosis in HIV-infected patients},
   Journal = {Clin Exp Immunol},
   Volume = {118},
   Number = {3},
   Pages = {412-6},
   Note = {0009-9104
Journal Article},
   Abstract = {HAART may increase CD4+ T cell counts despite a persistently detectable HIV load. The impact of HAART on apoptosis, which may play a role in the disease process in HIV-infected patients, has not been extensively studied. We performed a study to compare the level of spontaneous T cell apoptosis and anti-retroviral treatments in a cohort of HIV-1-infected patients. Data were obtained from a computerized medical record. Quantification of apoptotic cells was by cytofluorometric technique. From November 1995 to December 1997 we studied T cell apoptosis in 112 HIV-infected patients. Forty patients were classified A, 36 B and 36 C. Thirty patients were naive and 82 received an anti-retroviral treatment, 49 including a protease inhibitor (PI). The median plasma viraemia determined in 63 patients was 3.6 (range 1.3-5.6) log10. The median apoptotic cell count was 22% (range 2-73%) and 12% (range 2-60%) for CD4+ and CD8+ T cells, respectively. We did not observe any correlation between the HIV viraemia and the level of apoptosis of T cell subsets. Patients with HAART showed a lower percentage of apoptotic CD4+ T cells only: 16% (range 2-61%) versus 25% (range 5-73%) for patients receiving two nucleoside analogues (P = 0.02). This effect was significant in stage A patients and remained observable during the whole course of HIV disease. In conclusion, HAART, without any relation to plasma viraemia, is able to reduce apoptosis of CD4+ T cells.},
 Keywords = {Adult
Aged
Anti-HIV Agents/*therapeutic use
*Apoptosis
CD4-Positive T-Lymphocytes/cytology/*drug effects
CD8-Positive T-Lymphocytes/drug effects
Didanosine/therapeutic use
Drug Therapy, Combination
Female
HIV Infections/*drug therapy/immunology/pathology
HIV Protease Inhibitors/therapeutic use
Human
Lamivudine/therapeutic use
Male
Middle Aged
Multivariate Analysis
Retrospective Studies
Stavudine/therapeutic use
Viral Load
Zalcitabine/therapeutic use
Zidovudine/therapeutic use},
   Year = {1999} }



@article{
Stoddart01,
   Author = {Stoddart, C. A. and Liegler, T. J. and Mammano, F. and Linquist-Stepps, V. D. and Hayden, M. S. and Deeks, S. G. and Grant, R. M. and Clavel, F. and McCune, J. M.},
   Title = {Impaired replication of protease inhibitor-resistant HIV-1 in human thymus},
   Journal = {Nat Med},
   Volume = {7},
   Number = {6},
   Pages = {712-8},
   Note = {1078-8956
Journal Article},
   Abstract = {Many HIV-1-infected patients treated with protease inhibitors (PI) develop PI-resistant HIV-1 variants and rebounds in viremia, but their CD4+ T-cell counts often do not fall. We hypothesized that in these patients, T-cell counts remain elevated because PI-resistant virus spares intrathymic T-cell production. To test this, we studied recombinant HIV-1 clones containing wild-type or PI-resistant protease domains, as well as uncloned isolates from patients, in activated peripheral blood mononuclear cells, human thymic organ cultures and human thymus implants in SCID-hu Thy/Liv mice. In most cases, wild-type and PI-resistant HIV-1 isolates replicated to similar degrees in peripheral blood mononuclear cells. However, the replication of PI-resistant but not wild-type HIV-1 isolates was highly impaired in thymocytes. In addition, patients who had PI-resistant HIV-1 had abundant thymus tissue as assessed by computed tomography. We propose that the inability of PI-resistant HIV-1 to replicate efficiently in thymus contributes to the preservation of CD4+ T-cell counts in patients showing virologic rebound on PI therapy.},
 Keywords = {Adult
Animals
CD4 Lymphocyte Count
Drug Resistance, Microbial
Fetal Tissue Transplantation
Flow Cytometry
HIV Core Protein p24/metabolism
HIV Infections/immunology/pathology/*virology
HIV Protease/genetics/*metabolism
HIV Protease Inhibitors/*pharmacology
HIV-1/*drug effects/enzymology/genetics/*physiology
Human
Mice
Mice, SCID
Middle Aged
Organ Culture
Recombination, Genetic
Support, Non-U.S. Gov't
Support, U.S. Gov't, P.H.S.
T-Lymphocytes/*physiology/virology
Thymus Gland/pathology/physiopathology/transplantation/*virology
Viral Load
*Virus Replication},
   Year = {2001} }



@article{
Sufka03,
   Author = {Sufka, S. A. and Ferrari, G. and Gryszowka, V. E. and Wrin, T. and Fiscus, S. A. and Tomaras, G. D. and Staats, H. F. and Patel, D. D. and Sempowski, G. D. and Hellmann, N. S. and Weinhold, K. J. and Hicks, C. B.},
   Title = {Prolonged CD4+ cell/virus load discordance during treatment with protease inhibitor-based highly active antiretroviral therapy: immune response and viral control},
   Journal = {J Infect Dis},
   Volume = {187},
   Number = {7},
   Pages = {1027-37},
   Note = {0022-1899
Clinical Trial
Journal Article},
   Abstract = {Mechanisms that underly discordant CD4+ cell/virus load (VL) responses in patients who receive highly active antiretroviral therapy (HAART) were studied in 30 human immunodeficiency virus (HIV)-positive patients, in 3 groups. Discordant responders maintained CD4+ cell levels >200/mm(3) with stable or increasing trend, despite sustained VLs of 500-5000 copies/mL, for >2 years. Treatment-success patients had CD4+ cell counts >200/mm(3) with stable or increasing trend and VLs <50 copies/mL, for >2 years. Treatment-failure patients initially responded to HAART, followed by decreasing CD4+ cell counts and increasing VLs. Interferon-gamma production to gag and noncytolytic CD8+ cell suppressive activity were greater in discordant responders. Cellular activation was greatest in patients with treatment failure. All discordant responders had non-syncytium-inducing (CCR5-tropic) viruses. Viruses from discordant responders and from patients with treatment failure had extensive resistance mutations; discordant responders had significantly lower viral replication capacities. These findings suggest that discordant responses may be related to enhanced HIV-directed immune responses, diminished cellular activation, decreased viral replication capacity, and preservation of non-syncytium-inducing virus strains.},
 Keywords = {Adult
*Antiretroviral Therapy, Highly Active
*CD4 Lymphocyte Count
Female
HIV/*drug effects
HIV Infections/*drug therapy/*immunology/virology
HIV Protease Inhibitors/*pharmacology/therapeutic use
Human
Male
Middle Aged
Support, Non-U.S. Gov't
Support, U.S. Gov't, P.H.S.
Time Factors
Treatment Failure
*Viral Load
Virus Replication/drug effects},
   Year = {2003} }



@article{
Tebaldi03,
   Author = {Tedaldi, E. M. and Baker, R. K. and Moorman, A. C. and Alzola, C. F. and Furhrer, J. and McCabe, R. E. and Wood, K. C. and Holmberg, S. D.},
   Title = {Influence of coinfection with hepatitis C virus on morbidity and mortality due to human immunodeficiency virus infection in the era of highly active antiretroviral therapy},
   Journal = {Clin Infect Dis},
   Volume = {36},
   Number = {3},
   Pages = {363-7},
   Note = {1537-6591
Journal Article},
   Abstract = {To ascertain the impact of hepatitis C virus (HCV) infection on human immunodeficiency virus (HIV) disease progression and associated death in the era of highly active antiretroviral therapy (HAART), we examined mortality rates, the presence of other diseases, and antiretroviral use in an observational cohort of 823 HIV-infected patients with and without HCV coinfection during the period of January 1996 through June 2001. Analyses were used to compare patient characteristics, comorbid conditions, and survival durations in HIV-infected and HIV-HCV-coinfected patients. HIV-HCV-coinfected persons did not have a statistically greater rate of acquired immunodeficiency syndrome or of renal or cardiovascular disease, but they did have more cases of cirrhosis and transaminase elevations. There were proportionately more deaths in the HIV-HCV-coinfected group. Age, baseline CD4+ cell count, and duration of HAART were significantly associated with survival, but HCV infection was not. HAART use was a strong predictor of increased duration of survival, suggesting that treatment is more important to survival than is HCV coinfection status.},
 Keywords = {Anti-HIV Agents/therapeutic use
*Antiretroviral Therapy, Highly Active
*Hiv
HIV Infections/*complications/drug therapy/epidemiology/mortality
*Hepacivirus
Hepatitis C/*complications/epidemiology/mortality
Human
Morbidity
Mortality
Support, U.S. Gov't, P.H.S.},
   Year = {2003} }




@string{JASA= {Journal of the American Statistical Association}}
@string{JC = {Journal of Classification}}
@string{JSPI = {Journal of Statistical Planning and Inference}}
@string{JRSSB = {Journal of the Royal Statistical Society, Series B}}
@string{PNAS = {Proc. Natl. Acad. Sci.}}

@Article{Wang&Bembom&vanderLaan06,
  author =   {Y. Wang and O. Bembom and M.J. van der Laan},
  title =    {Data adaptive estimation of the treatment specific mean},
  journal =      {Journal of Statistical Planning and Inference},
  year =     {2006},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {also http://www.bepress.com/ucbbiostat/paper159},
  OPTannote =    {}
}
@Article{Sinisi&vanderLaan04,
  author =   {S. Sinisi and M.J. van der Laan},
  title =    {The deletion/substitution/addition algorithm in loss function based estimation:
Applications in Genomics},
  journal =      {Journal of Statistical Methods in Molecular Biology},
  year =     {2004},
  OPTkey =   {},
  volume =   {3},
  number =   {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/sagmb/vol3/iss1/art18},
  OPTannote =    {}
}



@TECHREPORT{Petersen&Deeks&Martin&vanderLaan05,
  author =       {Maya L. Petersen and Steven G. Deeks and Jeffrey N. Martin and Mark J. van der Laan},
  title =        {History-Adjusted Marginal Structural Models: Time-Varying Effect Modification
  and Dynamic Treatment Regimens},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2005},
  type =         {Technical Report 199},
OPTnote =      {http://www.bepress.com/ucbbiostat/paper199},
  month =        {December},
}

@TECHREPORT{vanderLaan&Rubin05,
  author =       {M.J. van der Laan and D. Rubin},
  title =        {Estimating Function Based Cross-Validation and Learning},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2005},
  type =         {Technical Report 180},
OPTnote =      {http://www.bepress.com/ucbbiostat/paper180},
  month =        {},
}

@Article{vanderLaan&Petersen07,
  author =   {M.J. van der Laan and M.L. Petersen},
  title =    {Causal Effect Models for Realistic Individualized Treatment and Intention to Treat Rules},
  journal =      {International Journal of Biostatistics},
  year =     {2007},
  OPTkey =   {},
  volume =   {3},
  number =   {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/ijb/vol3/iss1/art3},
  OPTannote =    {}
}


@TECHREPORT{vanderLaan06,
  author =       {M.J. van der Laan},
  title =        {Causal Effect Models for Intention to Treat and Realistic Individualized
  Treatment Rules},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2006},
  type =         {Technical Report 203},
OPTnote =      {http://www.bepress.com/ucbbiostat/paper203},
  month =        {},
}
@TECHREPORT{vanderLaan08b,
  author =       {M.J. van der Laan},
  title =        {The construction and analysis of adaptive group sequential designs},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2008},
  type =         {Technical Report 232},
OPTnote =      {http://www.bepress.com/ucbbiostat/paper232},
  month =        {March},
}
@TECHREPORT{Moore&vanderLaan07,
  author =       {K.L. Moore and M.J. van der Laan},
  title =        {Covariate adjustment in randomized trials with binary outcomes},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2007},
  type =         {Technical Report 215},
OPTnote =      {http://www.bepress.com/ucbbiostat/paper215},
  month =        {April},
}

@TECHREPORT{vanderLaan&Petersen05,
  author =       {M.J. van der Laan and M.L. Petersen},
  title =        {Direct Effect Models},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2005},
  type =         {Technical Report 187},
OPTnote =      {http://www.bepress.com/ucbbiostat/paper187},
  month =        {},
}
@TECHREPORT{Petersen&vanderLaan06,
  author =       {M.L. Petersen and M.J. van der Laan},
  title =        {Individualized Treatment Rules and Clinical Trials},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2006},
  type =         {Technical Report},
OPTnote =      {},
  month =        {},
}

@Article{vanderLaan&Petersen&Joffe05,
  author =   {M.J. van der Laan and M.L. Petersen and M.M. Joffe},
  title =    {History-Adjusted Marginal Structural Models and Statically-Optimal Dynamic Treatment Regimens},
  journal =      {The International Journal of Biostatistics},
  year =     {2005},
  OPTkey =   {},
  volume =   {1},
  number =   {1},
  pages =    {10-20},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/ijb/vol1/iss1/4},
  OPTannote =    {}
}

@Article{vanderLaan06a,
  author =   {M.J. van der Laan},
  title =    {Statistical Inference for Variable Importance},
  journal =      {International Journal of Biostatistics},
  year =     {2006},
  OPTkey =   {},
  volume =   {2},
  number =   {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/ijb/vol2/iss1/art2},
  OPTannote =    {}
}

@Article{vanderLaan&Birkner&Hubbard05,
  author =   {M.J. van der Laan and M.D. Birkner and A.E. Hubbard},
  title =    {Empirical Bayes and resampling based multiple testing procedure controlling tail probability of the proportion of false positives},
  journal =      {Journal of Statistical Applications in Genetics and Molecular Biology},
  year =     {2005},
  OPTkey =   {},
  volume =   {4},
  number =   {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/sagmb/vol4/iss1/art29},
  OPTannote =    {}
}



@Article{vanderLaan&Dudoit&Pollard04b,
  author =   {M.J. van der Laan and S. Dudoit and K.S. Pollard},
  title =    {Augmentation procedures for control of the generalized family-wise
  error rate and tail probabilities for the proportion of false positives},
journal =      {Journal of Statistical Applications in Genetics and Molecular Biology},
  year =     {2004},
  OPTkey =   {},
  volume =   {3},
  number =   {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/sagmb/vol3/iss1/art15},
  OPTannote =    {}
}
@Article{vanderLaan&Dudoit&Pollard04,
  author =   {S. Dudoit and M.J. van der Laan and K.S. Pollard},
  title =    {Multiple testing. Part II.
  Step-down procedures for control of the family-wise error rate
  },
journal =      {Journal of Statistical Applications in Genetics and Molecular Biology},
  year =     {2004},
  OPTkey =   {},
  volume =   {3},
  number =   {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/sagmb/vol3/iss1/art14},
  OPTannote =    {}
}

@Article{Dudoit&vanderLaan&Pollard04,
  author =   {S. Dudoit and M.J. van der Laan and K.S. Pollard},
  title =    {Multiple testing. Part I. Single-step procedures for control of general Type I error rates},
journal =      {Journal of Statistical Applications in Genetics and Molecular Biology},
  year =     {2004},
  OPTkey =   {},
  volume =   {3},
  number =   {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/sagmb/vol3/iss1/art13},
  OPTannote =    {}
}


@Article{Birkner&Sinisi&vanderLaan05,
  author =   {M.D. Birkner and S.E. Sinisi and M.J. van der Laan},
  title =    {Multiple Testing and Data Adaptive Regression: An Application
  to {HIV}-1 Sequence Data},
  journal =      {Journal of Statistical Applications in Genetics and Molecular Biology},
  year =     {2005},
  OPTkey =   {},
  volume =   {4},
  number =   {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/sagmb/vol4/iss1/art8},
  OPTannote =    {}
}

@TECHREPORT{vanderLaan&Hubbard06,
  author =       {M.J. van der Laan and A.E. Hubbard},
  title =        {Quantile-Function Based Null Distribution in Resampling Based Multiple Testing},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2006},
  type =         {Technical Report},
OPTnote =      {http://www.bepress.com/ucbbiostat/paper198},
  month =        {},
}
@TECHREPORT{Molinaro&vanderLaan04,
  author =       {A. Molinaro and M.J. van der Laan},
  title =        {Deletion/Substitution/Addition Algorithm for Partitioning the Covariate Space in Prediction},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2004},
  type =         {Technical Report},
OPTnote =      {http://www.bepress.com/ucbbiostat/paper162},
  month =        {},
}
@TECHREPORT{Birkner&vanderLaan05,
  author =       {M.D. Birkner and M.J. van der Laan},
  title =        {Application of a Variable Importance Measure Method to {HIV}-1 Sequence Data},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2005},
  type =         {Technical Report},
  month =        {},
}



@TECHREPORT{Neugebauer&vanderLaan05b,
  author =       {R. Neugebauer and M.J. van der Laan},
  title =        {Locally Efficient Estimation of Nonparametric
                    Causal Effects on Mean Outcomes in Longitudinal Studies},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2005},
  number =       {134},
  type =         {Technical Report},
OPTnote =    {http://www.bepress.com/ucbbiostat/paper134, to appear in {JSPI}},
  month =        {},
}
@TECHREPORT{Wang&Petersen&vanderLaan06,
  author =       {Y. Wang and M. Petersen and M.J. van der Laan},
  title =        {A statistical method for diagnosing ETA bias in IPTW estimators},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2006},
  number =       {},
  type =         {Technical Report},
OPTnote =    {},
  month =        {},
}

@TECHREPORT{Moore&vanderLaan07,
  author =       {K.L. Moore and M.J. van der Laan},
  title =        {Covariate adjustment in randomized trials with binary outcomes},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2007},
  type =         {Technical Report 215},
OPTnote =    {http://www.bepress.com/ucbbiostat/paper215},
  month =        {April},
}

@TECHREPORT{vanderLaan&Dudoit&vanderVaart,
  author =       {M.J. van der Laan and S. Dudoit and A.W. van der Vaart},
  title =        {The Cross-Validated Adaptive Epsilon-Net Estimator},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2004},
  type =         {Technical Report 142},
OPTnote =    {http://www.bepress.com/ucbbiostat/paper142},
  month =        {February},
}

@TECHREPORT{vanderLaan&DudoitTechRep130,
  author =       {M.J. van der Laan and S. Dudoit},
  title =        {Unified cross-validation methodology for selection among estimators
  and a general cross-validated adaptive epsilon-net estimator: Finite sample oracle
  inequalities and examples},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2003},
  type =         {Technical Report},
OPTnote =    {http://www.bepress.com/ucbbiostat/paper130},
  month =        {November},
}

@TECHREPORT{Petersen&vanderLaan05,
  author =       {M. Petersen and M.J. van der Laan},
  title =        {Estimation of direct and indirect causal effects in
Epidemiology},
  institution =  {Division of Biostatistics, University of California,
Berkeley},
  year =         {2005},
  type =         {Technical Report},
  month =        {},
}

@TECHREPORT{Petersen&Deeks&Martin&vanderLaan05,
  author =       {M.L. Petersen and S.G. Deeks and J.N. Martin and M.J. van der Laan},
  title =        {History-Adjusted Marginal Structural Models: Time-Varying Effect Modification and Dynamic Treatment Regimens},
  institution =  {Division of Biostatistics, University of California,
Berkeley},
  year =         {2005},
  type =         {Technical Report 199},
OPTnote =      {http://www.bepress.com/ucbbiostat/paper199},
  month =        {},
}

@TECHREPORT{vanderLaan&Petersen04,
  author =       {M.J. van der Laan and M. Petersen},
  title =        {Estimation of direct and indirect causal effects in longitudinal studies},
  institution =  {Division of Biostatistics, University of California,
Berkeley},
  year =         {2004},
  type =         {Technical Report 155},
  month =        {August},
}

@TECHREPORT{vanderLaan&Hubbard&Jewell04,
 author =       {M.J. van der Laan and A.E. Hubbard and N.P. Jewell},
  title =        {Estimation of Treatment Effects in Randomized Trials with Noncompliance and a Dichotomous Outcome},
  institution =  {Division of Biostatistics, University of California,
Berkeley},
  year =         {2004},
  type =         {Technical Report 157},
  OPTnote =      {http://www.bepress.com/ucbbiostat/paper157},
month =        {September},
}
@TECHREPORT{Bein&Hubbard&vanderLaan05,
 author =       {E. Bein and A.E. Hubbard and M.J. van der Laan},
  title =        {Estimating Function Based Cross-Validation in
Estimation of the Causal Effect in Randomized Trials},
  institution =  {Division of Biostatistics, University of California,
Berkeley},
  year =         {2005},
  type =         {Technical Report},
}





@TECHREPORT{vanderLaan&DudoitTechRep130,
  author =       {M.J. van der Laan and S. Dudoit},
  title =        {Unified cross-validation methodology for
selection among estimators and a general cross-validated adaptive
epsilon net estimator: Finite sample oracle inequalities and
examples},
  institution =  {Division of Biostatistics, University of California,
Berkeley},
  year =         {2003},
  type =         {Technical Report 130},
  month =        {Nov.},
}


@TECHREPORT{Molinaroetal05,
  author =       {A.M. Molinaro and M.J. van der Laan and D.H. Moore and K. Kerlikowske},
  title =        {Survival point estimate prediction in matched and non-matched case-control subsample designed studies},
  institution =  {Division of Biostatistics, University of California,
Berkeley},
  year =         {2005},
  note =         {http://www.bepress.com/ucbbiostat/paper149},
}


@TECHREPORT{DudoitetalSIGKDD04,
  author =       {S. Dudoit and M.J. van der Laan and S. Kele\c{s} and A.
M. Molinaro and S. E. Sinisi
and S.L. Teng},
  title =        {Loss-Based Estimation with Cross-Validation:
Applications to Microarray Data
Analysis and Motif Finding.},
  institution =  {Division of Biostatistics, University of California,
Berkeley},
  year =         {2004},
  note =         {to appear in \emph{SIGKDD} Explorations on Microarray Data Mining},
}

@Book{Friedman&Furberg&Demets98,
  author =       {L.M.Friedman and C.D. Furberg and D.L. DeMets},
  title =        {Fundamentals of Clinical Trials},
  publisher =    {Springer-Verlag New York},
  year =         {1998}
}

@Book{ABGK,
  author =       {P.K. Andersen and O. Borgan and R.D. Gill and N. Keiding},
  title =        {Statistical Models Based on Counting Processes},
  publisher =    {Springer-Verlag New York},
  year =         {1993}
}
@Article{Wittes&Brittain90,
  author =   {J. Wittes and E. Brittain},
  title =    {The role of internal pilot studies in increasing efficiency of clinical trials},
journal =      {Statistics in Medicine},
  year =     {1999},
  OPTkey =   {},
  volume =   {9},
  number =   {},
  pages =    {65--72},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

%references for direct and indirect effects:
@InCollection{Robins03,
  author =   {J.M. Robins},
  title =    {Semantics of causal DAG models and the identification of direct and
indirect effects},
  booktitle =    {Highly Structured Stochastic Systems},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher = {Oxford University Press, Oxford},
  year =     {2003},
  editor =   {P. Green, N. Hjort, and S. Richardson},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {70--81},
  OPTnote =      {},
  OPTannote =    {}
}

@InCollection{Hubbard&vanderLaan&Robins99,
  author =   {A. Hubbard and M.J. van der Laan and J.M. Robins},
  title =    {Nonparametric locally ecient
estimation of the treatment specic survival distribution with right censored data
and covariates in observational studies},
  booktitle =    {Statistical Models in Epidemiology, The Environment and Clinical Trials},
  publisher = {Springer Verlag},
  year =     {1999},
editor={M.E. Halloran and D. Berry},
volume={116},
pages={135--178},
  series =   {IMA Volumes in Mathematics and its Applications, Ed. M.E. Halloran and D. Berry}
}

@TechReport{Pearl01,
  author =   {J. Pearl},
  title =    {Cognitive systems Laboratory},
  institution =  {University of California, Los Angeles, Department of Computer Science},
  year =     {2001},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Pearl00,
  author =   {J. Pearl},
  title =    {Causality: Models, Reasoning, and Inference},
  publisher =    {Cambridge University Press, Cambridge},
  year =     {2000},
  OPTkey =   {},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  series =   {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Robins&Greenland92,
  author =   {J.M. Robins and S. Greenland},
  title =    {Identifiability and exchangeability for direct and indirect
effects},
  journal =      {Epidemiology},
  year =     {1992},
  OPTkey =   {},
  volume =   {3},
  number =   {0},
  pages =    {143--155},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{vanderLaan95,
  author =   {M.J. van der Laan},
  title =    {Identity for NPMLE in missing data and biased sampling models},
  journal =      {Bernoulli},
  year =     {1995},
  OPTkey =   {},
  volume =   {1},
  number =   {4},
  pages =    {335--341},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{vanderLaan98,
  author =   {M.J. van der Laan},
  title =    {Identity for NPMLE in Censored Data Models},
  journal =      {Lifetime Data Models},
  year =     {1998},
  OPTkey =   {},
  volume =   {4},
  number =   {0},
  pages =    {83--102},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Klaassen86,
  author =   {C.A.J. Klaassen},
  title =    {Consistent estimation of the influence function of locally asymptotically linear estimators},
  journal =      {Annals of Statistics},
  year =     {1987},
  OPTkey =   {},
  volume =   {15},
  number =   {},
  pages =    {1548--1562},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}





%the next references are for instrumental variable article
@Article{Robins&Rotnitzky04,
  author =   {J.M. Robins and A. Rotnitzky},
  title =    {Estimation of Treatment Effects in Randomized Trials
with Noncompliance and a Dichotomous Outcome using Structural Nested
Mean Models},
  journal =      {Biometrika},
  year =     {2004},
  OPTkey =   {},
  volume =   {0},
  number =   {0},
  pages =    {0},
  OPTmonth =     {},
  OPTnote =      {To Appear},
  OPTannote =    {}
}

@Article{Vandervaart91,
  author =   {A.W. van der Vaart},
  title =    {On differentiable functionals},
  journal =      {Annals of Statistics},
  year =     {1991},
  OPTkey =   {},
  volume =   {19},
  number =   {},
  pages =    {178--204},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}




@Article{Rubin78,
  author =   {D.B. Rubin},
  title =    {Bayesian Inference for causal effects: the role of randomization},
  journal =      {Annals of Statistics},
  year =     {1978},
  OPTkey =   {},
  volume =   {6},
  number =   {},
  pages =    {34--58},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Neyman23,
  author =   {Neyman, J.},
  title =    {On the application of probability theory to agricultural
experiments},
  journal =      {Statistical Science},
  year =     {1990},
  OPTkey =   {},
  volume =   {5},
  number =   {},
  pages =    {465--480},
  OPTmonth =     {},
  OPTnote =      {Translation of 1923 article},
  OPTannote =    {}
}
@Article{Robins86,
  author =   {J.M. Robins},
  title =    {A new approach to causal inference in mortality studies with sustained exposure periods - Application to control of the healthy worker survivor effect},
  journal =      {Mathematical Modelling},
  year =     {1986},
  OPTkey =   {},
  volume =   {7},
  number =   {},
  pages =    {1393--1512},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}





@Article{Robins94,
  author =   {J.M. Robins},
  title =    {Correcting for non-compliance in randomized trials
using structural nested mean models},
  journal =      {Communications in Statistics},
  year =     {1994},
  OPTkey =   {},
  volume =   {23},
  number =   {},
  pages =    {2379--2412},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Vansteelandt03,
  author =   {S. Vansteelandt and E. Goetghebeur},
  title =    {Causal inference with generalized structural  mean
models},
  journal =      {Journal of the Royal Statistical Society, Series B},
  year =     {2003},
  OPTkey =   {},
  volume =   {23},
  number =   {},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {In print},
  OPTannote =    {}
}

@incollection {Robins97a,
   AUTHOR = {Robins, J.M.},
    TITLE = {Structural Nested Failure Time Models},
BOOKTITLE = {The Encyclopedia of Biostatistics},
PUBLISHER = {John Wiley and Sons},
  ADDRESS = {Chichester, UK},
     YEAR = {1997},
   EDITOR = {Armitage, P. and Colton, T. and Andersen, P.K. and Keiding, N.}
}
@article {hernan_brumback_robins,
   AUTHOR = {Hernan, M. A. and Brumback, B. and Robins, J. M.},
    TITLE = {Marginal structural models to estimate the causal effect of zidovudine on the survival of {HIV}-positive men},
  JOURNAL = {Epidemiology},
   VOLUME = {11},
   NUMBER = {5},
     YEAR = {2000},
    PAGES = {561--570}
}
@article {Robins87,
   AUTHOR = {Robins, J.M.},
    TITLE = {Addendum to: ``{A} new approach to causal inference in
             mortality studies with a sustained exposure
             period---application to control of the healthy worker survivor
             effect'' [{M}ath.\ {M}odelling {\bf 7} (1986), no.\ 9-12,
             1393--1512; {M}{R} 87m:92078]},
  JOURNAL = {Comput. Math. Appl.},
 FJOURNAL = {Computers \& Mathematics with Applications. An International
             Journal},
   VOLUME = {14},
     YEAR = {1987},
   NUMBER = {9-12},
    PAGES = {923--945},
     ISSN = {0097-4943},
    CODEN = {CMAPDK},
}

@article {robins_hernan_brumback,
   AUTHOR = {Robins, J. M. and Hernan, M. A. and Brumback, B.},
    TITLE = {Marginal structural models and causal inference in epidemiology},
  JOURNAL = {Epidemiology},
   VOLUME = {11},
   NUMBER = {5},
     YEAR = {2000},
    PAGES = {550--560}
}





@article {Bryan&Yu&vanderLaan03,
   AUTHOR = {Bryan, J. and Yu, Z. and van der Laan, M.J.},
    TITLE = {Analysis of Longitudinal Marginal Structural Models},
  JOURNAL = {Biostatistics},
   VOLUME = {5},
   NUMBER = {3},
     YEAR = {2003},
    PAGES = {361--380}
}

@TechReport{Yu&vanderLaan03,
  author =   {Yu, Z. and van der Laan, M.J.},
  title =    {Double Robust Estimation in Longitudinal Marginal Structural
                    Models},
  institution =  {Division of Biostatistics, University of California,
Berkeley},
  year =     {2003},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {132},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/ucbbiostat/paper132},
  OPTannote =    {}
}

@Article{Neugebauer&vanderLaan05,
  author =   {Neugebauer, R. and van der Laan, M.J.},
  title =    {Why prefer double robust estimates},
  journal =      {Journal of Statistical Planning and Inference},
  year =     {2005},
  OPTkey =   {},
  volume =   {129},
  number =   {1-2},
  pages =    {405--426},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@article {Murphy03,
   AUTHOR = {Murphy, S.A.},
    TITLE = {Optimal dynamic treatment regimes},
  JOURNAL = {Journal of the Royal Statistical Society: Series B},
   VOLUME = {65},
   NUMBER = {2},
     YEAR = {2003},
    PAGES = {?}
}
@article {Robins03a,
   AUTHOR = {Robins, J.M.},
    TITLE = {Discussion of ''{O}ptimal dynamic treatment regimes" by {S}usan {A}. {M}urphy},
  JOURNAL = {Journal of the Royal Statistical Society: Series B},
   VOLUME = {65},
   NUMBER = {2},
     YEAR = {2003},
    PAGES = {355--366}
}

@article {Murphy&vanderLaan&Robins01,
   AUTHOR = {S.A. Murphy and M.J. van der Laan and J.M. Robins},
    TITLE = {Marginal mean models for dynamic treatment regimens},
  JOURNAL = {Journal of the American Statistical Association},
   VOLUME = {96},
   NUMBER = {},
     YEAR = {2001},
    PAGES = {1410--1424}
}
@incollection {Robins98,
    AUTHOR = {Robins, J.M.},
     TITLE = {Marginal structural models versus structural nested models as
              tools for causal inference},
 BOOKTITLE = {Statistical models in epidemiology, the environment, and
              clinical trials (Minneapolis, MN, 1997)},
     PAGES = {95--133},
 PUBLISHER = {Springer},
   ADDRESS = {New York},
      YEAR = {2000},
   MRCLASS = {62N01 (62G08 62P10)},
  MRNUMBER = {2001a:62124},
}
%Robins, J.M. (2003). Discussion of "Optimal dynamic treatment regimes". by Susan A. Murphy.
  %Journal of the Royal Statistical Society: Series B, 65(2):355-366.
@InCollection{Robins97,
  author =   {J.M. Robins},
  title =    {Causal Inference from Complex Longitudinal Data},
  booktitle =    {Latent Variable Modeling and Applications to Causality},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher = {Springer Verlag, New York},
  year =     {1997},
  editor =   {M. Berkane, Editor},
  OPTvolume =    {120},
  OPTnumber =    {},
  OPTseries =    {Lecture Notes in Statistics},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {69--117},
  OPTnote =      {},
  OPTannote =    {}
}

@InCollection{Robins89,
  author =   {J.M. Robins},
  title =    {The analysis of randomized and non-randomized AIDS
treatment trials using a new approach in causal inference in longitudinal studies},
  booktitle =    {Health Service Methodology: A Focus on AIDS},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher = {U.S. Public Health Service, National Center for Health SErvices Research},
  year =     {1989},
  editor =   {L. Sechrest and H. Freeman and A. Mulley},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {Lecture Notes in Statistics},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {Washington D.C.},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {113--159},
  OPTnote =      {},
  OPTannote =    {}
}



@TechReport{Abadie00,
  author =   {A. Abadie},
  title =    {Semiparametric estimation of instrumental variables models for causal effects},
  institution =  {NBER Technical Working Paper},
  year =     {2000},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {260},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Abadie03,
  author =   {A. Abadie},
  title =    {Semiparametric instrumental variable estimation of treatment response models},
  journal =      {Journal of Econometrics},
  year =     {2003},
  OPTkey =   {},
  volume =   {113},
  number =   {},
  pages =    {231-263},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Abadie03,
  author =   {A. Abadie},
  title =    {Semiparametric instrumental variable estimation of treatment response models},
  journal =      {Journal of Econometrics},
  year =     {2003},
  OPTkey =   {},
  volume =   {113},
  number =   {},
  pages =    {231-263},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@TechReport{Wang&Vanderlaan04,
  author =   {Y. Wang and M.J. van der Laan},
  title =    {Data adaptive estimation of the treatment specific mean},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =     {2004},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {159},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/ucbbiostat/paper159},
  OPTannote =    {}
}
@TechReport{Yu&vanderLaan02,
  author =   {Z. Yu and M.J. van der Laan},
  title =    {Construction of counterfactuals and the {G}-computation formula},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =     {2002},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {122},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/ucbbiostat/paper122},
  OPTannote =    {}
}
@TechReport{Yu&Vanderlaan03,
  author =   {Z. Yu and M.J. van der Laan},
  title =    {Measuring treatment effects using semiparametric models},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =     {2003},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {136},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/ucbbiostat/paper136},
  OPTannote =    {}
}

@Article{Angristetal96,
  author =   {J. Angrist and G. Imbens and D.B. Rubin},
  title =    {Identification of causal effects using instrumental variables},
  journal =      {Journal of the American Statistical Association},
  year =     {1996},
  OPTkey =   {},
  volume =   {91},
  number =   {},
  pages =    {444-555},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Robins&Rotnitzky01A,
  author =   {J.M Robins and A. Rotnitzky},
  title =    {Comment on {I}nference for semiparametric models: some questions
  and an answer, by {B}ickel, {P}.{J}. and {K}won, {J}.},
  journal =      {Statistica Sinica},
  year =     {2001},
  OPTkey =   {},
  volume =   {11},
  number =   {},
  pages =    {920-935},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Angrist01,
  author =   {J. Angrist},
  title =    {Estimation of limited dependent variable models with dummy endogenous regressors: simple strategies for empirical practice},
  journal =      {Journal of Business and Economics Statistics},
  year =     {2001},
  OPTkey =   {},
  volume =   {19},
  number =   {},
  pages =    {1--16},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Chamberlain87,
  author =   {G. Chamberlain},
  title =    {Asymptotic efficiency in estimation with conditional moment
restrictions},
  journal =      {Journal of Econometrics},
  year =     {1987},
  OPTkey =   {},
  volume =   {34},
  number =   {},
  pages =    {305--334},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Hiranoetal00,
  author =   {K. Hirano and G. Imbens and D.B. Rubin and X-H. Zhou},
  title =    {Assessing the effects of influenza vaccine in an encouragement design},
  journal =      {Biostatistics},
  year =     {2000},
  OPTkey =   {},
  volume =   {1},
  number =   {},
  pages =    {69--88},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Neyman23,
  author =   {J. Neyman},
  title =    {Sur les applications de la thar des probabilites aux
experiences Agaricales: Essay des principle (1923). Excerpts reprinted (1990) in
English (D. Dabrowska and T. Speed), Trans.},
  journal =      {Statistical Science},
  year =     {1990},
  OPTkey =   {},
  volume =   {5},
  number =   {},
  pages =    {463--472},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



optimal structural nested models for optimal
sequential decisions Proceedings of the 2nd seattle symposium in
biostatistics eds. Lin DY, Heagerty PJ  Springer Verlag Lecture Notes in
Statisitics No. 179  pages 189-326

@InProceedings{Robins05,
  author =   {J.M. Robins},
  title =    {Optimal structural nested models for optimal sequential decisions},
  booktitle =    {Proceedings of the 2nd Seattle symposium in
biostatistics},
  pages =    {189--326},
  year =     {2005},
  editor =   {Lin, D.Y, Heagerty P.J},
  volume =   {179},
  organization = {},
OPTpublisher = {Springer Verlag Lecture Notes in Statistics}
}


@TechReport{Robins05tech,
  author =   {J.M. Robins},
  title =    {Optimal structural nested models for optimal sequential decisions},
  institution =  {Department of Biostatistics, Havard University},
  year =     {2005},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}





@InProceedings{AIC,
  author =   {H. Akaike},
  title =    {Information theory and an extension of the maximum likelihood principle},
  booktitle =    {Second International Symposium on Information Theory},
  pages =    {267-281},
  year =     {1973},
  editor =   {B.N. Petrov and F. Csaki},
  organization = {Budapest: Academiai Kiado}
}


@Article{Balke&Pearl97,
  author =   {A. Balke and J. Pearl},
  title =    {Bound on treatment effects from studies with imperfect compliance},
  journal =      {Journal of the American Statistical Association},
  year =     {1997},
  OPTkey =   {},
  volume =   {92},
  number =   {},
  pages =    {1172--1176},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{Balke&Pearl94,
author =     {A. Balke and J. Pearl},
  title =    {Counterfactual probabilities: Computational methods, bounds, and applications},
  booktitle =    {In Proceedings of the 12th National Conference on Artificial Intelligence},
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {230--237},
  year =     {1994},
  OPTeditor =    {},
  volume =   {I},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {Menlo Park, CA},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {MIT Press},
  OPTnote =      {},
  OPTannote =    {}
}






@Article{Ambroise&McLachlan02,
  author =   {C. Ambroise and G. J. McLachlan},
  title =    {Selection bias in gene extraction on the basis of microarray gene-expression data},
  journal =      PNAS,
  year =     {2002},
  OPTkey =   {},
  volume =   {99},
  number =   {10},
  pages =    {6562--6566},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@InCollection{Arabie&Hubert96,
  author =   {P. Arabie and L. J. Hubert},
  title =    {An overview of combinatorial data analysis},
  booktitle =    {Clustering and Classification},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher = {World Scientific Publishing Co.},
  year =     {1996},
  editor =   {P. Arabie and L. J. Hubert and G. De Soete},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {River Edge, NJ},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {5--63},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{BIC,
  author =   {G. Schwartz},
  title =    {Estimating the Dimension of a Model},
  journal =      {Annals of Statistics},
  year =     {1978},
  volume =   {6},
  pages =    {461-464}
}


@Article{Barnard,
  author =   {M. Barnard},
  title =    {The secular variations of skull characters in four series of Egyptian skulls},
  journal =      {Annals of Eugenics},
  year =     {1935},
  OPTkey =   {},
  volume =   {6},
  OPTnumber =    {},
  pages =    {352--371},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@InProceedings{BenHuretal02,
  author =   {A. Ben-Hur and A. Elisseeff and I. Guyon},
  title =    {A stability based method for discovering structure in clustered data},
  booktitle =    {Pacific Symposium on Biocomputing},
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {6--17},
  year =     {2002},
  OPTeditor =    {},
  volume =   {7},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Benjamini&Hochberg95,
  author =   {Y. Benjamini and Y. Hochberg},
  title =    {Controlling the false discovery rate: a practical and powerful approach to multiple testing},
  journal =      {J. R. Statist. Soc. B},
  year =     {1995},
  OPTkey =   {},
  volume =   {57},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {289--300},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Benjamini&Yekutieli01,
  author =   {Y. Benjamini and D. Yekutieli},
  title =    {The control of the false discovery rate in multiple testing under
   dependency},
  journal =      {Annals of Statistics},
  year =     {2001},
  OPTkey =   {},
  volume =   {29},
  number =   {4},
  pages =    {1165--1188},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Beran88,
  author =   {R. Beran},
  title =    {Balanced simultaneous confidence sets},
  journal =      JASA,
  year =     {1988},
  OPTkey =   {},
  volume =   {83},
  OPTnumber =    {},
  pages =    {679--686},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Bock85,
  author =   {H-H Bock},
  title =    {On some significance tests in cluster analysis},
  journal =      {Journal of Classification},
  year =     {1985},
  OPTkey =   {},
  volume =   {2},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {77--108},
  OPTnote =      {},
  OPTannote =    {}
}



@InCollection{Bock96,
  author =   {H-H Bock},
  title =    {Probability models and hypotheses testing in partitioning cluster analysis},
  booktitle =    {Clustering and Classification},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher = {World Scientific Publishing Co.},
  year =     {1996},
  editor =   {P. Arabie and L. J. Hubert and G. De Soete},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {River Edge, NJ},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {377--453},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Boldricketal02,
  author =   {J. C. Boldrick and A. A. Alizadeh and M. Diehn and S. Dudoit and C. L. Liu and C. E. Belcher and D. Botstein and L. M. Staudt and P. O. Brown
and D. A. Relman},
  title =    {Stereotyped and specific gene expression programs in human innate immue responses to bacteria},
  journal =      PNAS,
  year =     {2002},
  OPTkey =   {},
  volume =   {99},
  number =   {2},
  pages =    {972--977},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Bozdogan00,
  author =   {H. Bozdogan},
  title =    {Akaike's information criterion and recent developments in information complexity},
  journal =      {Journal of Mathematical Psychology},
  year =     {2000},
  volume =   {44},
  pages =    {62-91}
}




@InCollection{Bozdogan93,
  author =   {H. Bozdogan},
  title =    {Choosing the number of component clusters in the mixture model  using a new informational complexity criterion of the inverse Fisher information matrix},
  booktitle =    {Information and Classification},
  publisher = {Heidelberg: Springer Verlag},
  editor = {O. Opitz and B. Lausen and R. Klar},
  year =     {1993},
  series =   {}
}

@Article{Braver,
  author =   {S. L. Braver},
  title =    {On splitting the tails unequally: a new perspective on one-versus two-tailed tests},
  journal =      {Educational and Psychological Measurement},
  year =     {1975},
  OPTkey =   {},
  volume =   {35},
  OPTnumber =    {},
  pages =    {283--301},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Breckenridge89,
  author =   {J. Breckenridge},
  title =    {Replicating cluster analysis: Method, consistency and validity},
  journal =      {Multivariate Behavioral Research},
  year =     {1989},
  OPTkey =   {},
  volume =   {24},
  OPTnumber =    {},
  pages =    {147--161},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Breiman&Spector92,
  author =   {L. Breiman and P. Spector},
  title =    {Submodel Selection and Evaluation in Regression. The
  $X$ Random Case},
  journal =      {International Statistical Review},
  year =     {1992},
  OPTkey =   {},
  volume =   {60},
  OPTnumber =    {},
  pages =    {291--319},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Breiman01,
  author =   {L. Breiman},
  title =    {Statistical modeling: the two cultures},
  journal =      {Statistical Science},
  year =     {2001},
  OPTkey =   {},
  volume =   {16},
  number =   {3},
  pages =    {199--215},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{BreimanAnnals96,
  author =   {L. Breiman},
  title =    {Heuristics of instability and stabilization in model selection},
  journal =      {Annals of Statistics},
  year =     {1996},
  OPTkey =   {},
  volume =   {24},
  number =   {6},
  pages =    {2350--2383},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{BreimanArcing,
  author =   {L. Breiman},
  title =    {Arcing classifiers},
  journal =      {Annals of Statistics},
  year =     {1998},
  OPTkey =   {},
  volume =   {26},
  OPTnumber =    {},
  pages =    {801-824},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{BreimanBagging,
  author =   {L. Breiman},
  title =    {Bagging predictors},
  journal =      {Machine Learning},
  year =     {1996},
  OPTkey =   {},
  volume =   {24},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {123-140},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{BreimanCPD,
  author =   {L. Breiman},
  title =    {Using Convex pseudo-data to increase prediction accuracy},
  institution =  {Department of Statistics, U.C. Berkeley},
  year =     {1998},
  OPTkey =   {},
  OPTtype =      {},
  number =   {513},
  OPTaddress =   {},
  month =    {March},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{BreimanJASA92,
  author =   {L. Breiman},
  title =    {The Little Bootstrap and Other Methods for
  Dimensionality Selection in Regression: $X$-Fixed Prediction Error},
  journal =      JASA,
  year =     {1992},
  OPTkey =   {},
  volume =   {87},
  number =   {419},
  pages =    {738--754},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@TechReport{BreimanOB,
  author =   {L. Breiman},
  title =    {Out-of-bag estimation},
  institution =  {Department of Statistics, U.C. Berkeley},
  year =     {1996},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@TechReport{BreimanRanForests,
  author =   {L. Breiman},
  title =    {Random forests - random features},
  institution =  {Department of Statistics, U.C. Berkeley},
  year =     {1999},
  OPTkey =   {},
  OPTtype =      {},
  number =   {567},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Breimanetal84,
  author =   {L. Breiman and J. H. Friedman and R. Olshen and C. J. Stone},
  title =    {Classification and regression trees},
  publisher =    {Wadsworth International Group},
  year =     {1984},
  OPTkey =   {},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  series =   {The Wadsworth statistics/probability series},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Book{Hastieetal02,
  author =   {T. Hastie and R. Tibshirani and J. Friedman},
  title =    {The Elements of Statistical Learning},
  publisher =    {Springer},
  year =     {2002},
  OPTkey =   {},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  series =   {Springer Series in Statistics},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Broman01,
  author =   {K. W. Broman},
  title =    {Review of statistical methods for QTL mapping in experimental crosses},
  journal =      {Lab Animal},
  year =     {2001},
  OPTkey =   {},
  volume =   {30},
  number =   {7},
  pages =    {44--52},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@PhdThesis{Broman97,
  author =   {K. W. Broman},
  title =    {Identifying quantitative trait loci in experimental crosses},
  school =   {Department of Statistics, U.C. Berkeley},
  year =     {1997},
  OPTkey =   {},
  type =     {Ph.{D}. thesis},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Brown&Koplowitz79,
  author =   {T. A. Brown and J. Koplowitz},
  title =    {The weighted nearest neighbor rule for class dependent sample sizes},
  journal =      {IEEE Transactions on Information Theory},
  year =     {1979},
  OPTkey =   {},
  volume =   {25},
  number =   {5},
  pages =    {617--619},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Buhlmann&Yu,
  author =   {P. Buhlmann and B. Yu},
  title =    {Explaining Bagging.},
  journal =      {Annals of Statistics},
  year =     {(Accepted)},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTpages =     {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Burgessvm98,
  author =   {C. J. C. Burges},
  title =    {A tutorial on support vector machines for pattern recognition},
  journal =      {Data Mining and Knowledge Discovery},
  year =     {1998},
  OPTkey =   {},
  volume =   {2},
  number =   {},
  pages =    {121--167},
  month =    {December},
  OPTnote =      {},
  OPTannote =    {}
}



@article{Burman89,
AUTHOR={P. Burman},
TITLE={A comparative study of ordinary cross-validation, $v$-fold cross-validati
on and the repeated learning testing methods},
JOURNAL={Biometrika},
VOLUME={76},
YEAR={1989},
PAGES={503-514}
}





@TechReport{Buttrey&Karo02,
  author =   {S. E. Buttrey and C. Karo},
  title =    {Using k--neareset neighbor classification in the leaves of a tree},
  institution =  {Naval Postgraduate School, Monterey, CA},
  year =     {2002},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Calinskietal,
  author =   {R. Calinski and J. Harabasz},
  title =    {A dendrite method for cluster analysis},
  journal =      {Communications in Statistics},
  year =     {1974},
  OPTkey =   {},
  volume =   {3},
  OPTnumber =    {},
  pages =    {1--27},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Callowetal00,
  author =   {M. J. Callow and S. Dudoit and E. L. Gong and T. P. Speed and E. M. Rubin},
  title =    {Microarray expression profiling identifies genes with altered expression in {HDL} deficient mice},
  journal =      {Genome Research},
  year =     {2000},
  OPTkey =   {},
  volume =   {10},
  number =   {12},
  OPTmonth =     {},
  pages =    {2022--2029},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Chambers98,
   author = {J. M. Chambers},
   title = {Programming with Data: A Guide to the S Language},
   publisher = {Springer-Verlag New York},
   year = {1998}
}
@Book{Diggleetal2002,
   author = {Peter J. Diggle and P. Heagerty and K-Y Liang and S.L. Zeger},
   title = {Analysis of Longitudinal Data},
   publisher = {Oxford University Press},
   year = {2002 (Second Edition)}
}

@TechReport{ChangLin2001,
  author =       {C.-C. Chang and C.-J. Lin},
  title =        {LIBSVM: a Library for Support Vector Machines (Version 2.31)},
  institution =  {},
  year =         {2001},
  OPTkey =       {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  note =         {\\ {\tt http://www.csie.ntu.edu.tw/~cjlin/papers/libsvm2.ps.gz}},
  OPTannote =    {}
}



@Article{Changetal02,
  author =   {H. Y. Chang and J. T. Chi and S. Dudoit and C. Bondre and M. van de Rijn and D. Botstein D and P. O. Brown},
  title =    {Diversity, topographic differentiation, and positional memory in human fibroblasts},
  journal =      PNAS,
  year =     {2002},
  OPTkey =   {},
  volume =   {99},
  number =   {20},
  pages =    {12877--12882},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Chenetal02,
  author =   {X. Chen and S. T. Cheung and S. So and S. T. Fan and C. Barry and J. Higgins and K.-M. Lai and J. Ji and S. Dudoit and I. O. L. Ng and M. van de Rijn and D. Botstein and P. O. Brown },
  title =    {Gene expression patterns in human liver cancers},
  journal =      {Molecular Biology of the Cell},
  year =     {2002},
  OPTkey =   {},
  volume =   {13},
  number =   {6},
  pages =    {1929--1939},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Cleveland&Devlin88,
  author =   {W. S. Cleveland and S. J. Devlin},
  title =    {Locally-Weighted Regression: An Approach to Regression Analysis by Local Fitting},
  journal =      JASA,
  year =     {1988},
  OPTkey =   {},
  volume =   {83},
  OPTnumber =    {},
  pages =    {596--610},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Cleveland79,
  author =   {W. S. Cleveland},
  title =    {Robust locally weighted regression and smoothing scatterplots},
  journal =      JASA,
  year =     {1979},
  OPTkey =   {},
  volume =   {74},
  number =   {368},
  pages =    {829--836},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Correa&Wolfson99,
  author =   {J. A. Correa and D. B. Wolfson},
  title =    {Length-bias: some characterizations and applications},
  journal =      {Journal of Statistical Computation and Simulation},
  year =     {1999},
  OPTkey =   {},
  volume =   {64},
  Tnumber =      {3},
  pages =    {209--219},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Correaetal02,
  author =   {J. A. Correa and S. Dudoit and D. R. Goldstein},
  title =    {Multiple testing in the survival analysis of microarray data},
  OPTjournal =   {Statistics in Medicine},
  year =     {2002},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTpages =     {},
  OPTmonth =     {},
  note =     {(Submitted)},
  OPTannote =    {}
}


@Article{CortesVapnik95,
  author =   {C. Cortes and V. Vapnik},
  title =    {Support-vector networks},
  journal =      {Machine Learning},
  year =     {1995},
  OPTkey =   {},
  volume =   {20},
  number =   {},
  pages =    {273-297},
  month =    {December},
  OPTnote =      {},
  OPTannote =    {}
}

@InProceedings{Davies&Bouldin,
  author =   {D. Davies and D. Bouldin},
  title =    {A cluster separation measure},
  booktitle =    {IEEE Transactions on Pattern Analysis and Machine Intelligence},
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {224--227},
  year =     {1979},
  OPTeditor =    {},
  volume =   {1},
  OPTnumber =    {PAMI-1},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@article {Davis89,
AUTHOR ={R. B. Davis  and J. R. Anderson},
TITLE ={Exponential survival trees},
JOURNAL = {Statistics in Medicine},
VOLUME = {8},
YEAR ={1989},
NUMBER={},
PAGES = {947-961},
ISSN = {},
CODEN = {},
}




@InCollection{Day96,
  author =   {W. H. E. Day},
  title =    {Complexity theory: {A}n introduction for practitioners of classification},
  booktitle =    {Clustering and Classification},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher = {World Scientific Publishing Co.},
  year =     {1996},
  editor =   {P. Arabie and L. J. Hubert and G. De Soete},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {River Edge, NJ},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {199--233},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Dettling&Buhlmann02,
  author =   {M. Dettling and P. B\"{u}lmann},
  title =    {How to Use Boosting for Tumor Classification with Gene Expression Data},
  journal =      {},
  year =     {2002},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTpages =     {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Dudoit&Fridlyand02II,
  author =   {S. Dudoit and J. Fridlyand},
  title =    {Bagging to improve the accuracy of a clustering procedure},
  OPTjournal =   {Bioinformatics},
  year =     {2002},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTpages =     {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
  }



@InCollection{Dudoit&FridlyandCRC02,
  author =   {S. Dudoit and J. Fridlyand},
  title =    {Classification in microarray experiments},
  booktitle =    {Statistical Analysis of Gene Expression Microarray Data},
  OPTcrossref =  {},
  OPTkey =   {},
  OPTpages =     {},
  publisher =    {Chapman \& Hall/CRC},
  year =     {2002},
  editor =   {T. P. Speed},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTtype =      {},
  OPTchapter =   {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  note =     {(To appear)},
  OPTannote =    {}
}

@Article{Dudoit&FridlyandGenBio02,
  author =   {S. Dudoit and J. Fridlyand},
  title =    {A prediction-based resampling method to estimate the number of clusters in a dataset},
  journal =      {Genome Biology},
  year =     {2002},
  OPTkey =   {},
  volume =   {3},
  number =   {7},
  pages =    {0036.1--0036.21},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@TechReport{Dudoit&FridlyandTechRep600,
  author =   {S. Dudoit and J. Fridlyand},
  title =    {Applications of resampling methods to estimate the number of clusters and to improve the accuracy of a clustering method},
  institution =  {Department of Statistics, Uiversity of California, Berkeley},
  year =     {2001},
  OPTkey =   {},
  OPTtype =      {},
  number =   {600},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {},
  url={stat-www.berkeley.edu/users/sandrine/publications.html},
}

S. Dudoit, M.J. van der Laan (2005),
 Asymptotics of cross-validated
risk estimation in estimator selection and performance assessment.
{\em Statistical Methodology 2}, 2, 131--54.

@Article{Dudoit&vanderLaan05,
  author =   {S. Dudoit and M.J. van der Laan},
  title =    {Asymptotics of cross-validated risk estimation in estimator selection and performance assessment},
  journal =      {Statistical Methodology},
  year =     {2005},
  OPTkey =   {},
  volume =   {2},
  number =   {2},
  OPTmonth =     {},
  pages =    {131--154},
  OPTnote =      {www.bepress.com/ucbbiostat/paper126},
  OPTannote =    {}
}
@Article{Dudoit&SpeedAnnals99,
  author =   {S. Dudoit and T. P. Speed},
  title =    {A score test for linkage using identity by descent data from sibships},
  journal =      {Annals of Statistics},
  year =     {1999},
  OPTkey =   {},
  volume =   {27},
  number =   {3},
  OPTmonth =     {},
  pages =    {943--986},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Dudoit&SpeedBios00,
  author =   {S. Dudoit and T. P. Speed},
  title =    {A score test for the linkage analysis of qualitative and quantitative traits based on identity by descent data on sib-pairs},
  journal =      {Biostatistics},
  year =     {2000},
  OPTkey =   {},
  volume =   {1},
  number =   {1},
  pages =    {1--26},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}




@InCollection{Dudoit&SpeedIMA99,
  author =   {S. Dudoit and T. P. Speed},
  title =    {Triangle constraints for sib-pair identity by descent probabilities under a general multilocus model for disease susceptibility},
  booktitle =    {Statistics in Genetics},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher =    {Springer-Verlag},
  year =     {1999},
  editor =   {M. E. Halloran and S. Geisser},
  volume =   {112},
  OPTnumber =    {},
  series =   {IMA Volumes in Mathematics and its Applications},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {New York},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {181--221},
  OPTnote =      {},
  OPTannote =    {}
}

@InCollection{Dudoit&YangSpringer03,
  author =   {S. Dudoit and Y. H. Yang},
  title =    {Bioconductor {R} packages for exploratory analysis and normalization of c{DNA} microarray data},
  booktitle =    {The Analysis of Gene Expression Data: Methods and Software},
  OPTcrossref =  {},
  OPTkey =   {},
  OPTpages =     {},
  publisher =    {Springer, New York},
  year =     {2003},
  editor =   {G. Parmigiani and E. S. Garrett and R. A. Irizarry and S. L. Zeger},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTtype =      {},
  OPTchapter =   {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{DudoitetalJASA02,
  author =       {S. Dudoit and J. Fridlyand and T. P. Speed},
  title =        {Comparison of Discrimination Methods for the Classification of
 Tumors Using Gene Expression Data},
  journal =      JASA,
  year =         {2002},
  OPTkey =       {},
  volume =    {97},
  number =    {457},
  pages =     {77--87},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{DudoitetalSinica02,
  author =   {S. Dudoit and Y. H. Yang and M. J. Callow and T. P. Speed},
  title =    {Statistical methods for identifying differentially expressed genes in replicated c{DNA} microarray experiments},
  journal =      {Statistica Sinica},
  year =     {2002},
  OPTkey =   {},
  volume =   {12},
  number =   {1},
  pages =    {111--139},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{DudoitetalTechRep110,
  author =   {S. Dudoit and J. P. Shaffer and J. C. Boldrick},
  title =    {Multiple hypothesis testing in microarray experiments},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =     {2002},
  OPTkey =   {},
  OPTtype =      {},
  number =   {110},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {},
  url={www.bepress.com/ucbbiostat/paper110/}

}


@Article{Duffy&Quiroz,
  author =   {D. E. Duffy and A. J. Quiroz},
  title =    {A permutation-based algorithm for block clustering},
  journal =      {Journal of Classification},
  year =     {1991},
  OPTkey =   {},
  volume =   {8},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {65--91},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Dunn58,
  author =   {O. J. Dunn},
  title =    {Estimation of the means of dependent variables},
  journal =      {Annals of Mathematical Statistics},
  year =     {1958},
  OPTkey =   {},
  volume =   {29},
  OPTnumber =    {},
  pages =    {1095-111},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Book{Efron&Tibs93,
  author =   {B. Efron and R. J. Tibshirani},
  ALTeditor =    {},
  title =    {An Introduction to the Bootstrap},
  publisher =    {Chapman \& Hall/CRC},
  year =     {1993},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{EfronetalJASA01,
  author =   {B. Efron and R. Tibshirani and J. D. Storey and V. Tusher},
  title =    {Empirical Bayes analysis of a microarray
experiment},
  journal =      JASA,
  year =     {2001},
  OPTkey =   {},
  volume =   {96},
  OPTnumber =    {},
  pages =    {1151--1160},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@TechReport{EfronetalTechRep01,
  author =   {B. Efron and J. D. Storey and R. Tibshirani},
  title =    {Microarrays, empirical Bayes methods, and false discovery
rates},
  institution =  {Department of Statistics, Stanford University},
  year =     {2001},
  OPTkey =   {},
  OPTtype =      {},
  number =   {2001-218},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Finner99,
  author =   {H. Finner},
  title =    {Stepwise multiple test procedures and control of directional errors},
  journal =      {Annals of Statistics},
  year =     {1999},
  OPTkey =   {},
  volume =   {27},
  OPTnumber =    {},
  pages =    {274--289},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Fisher,
  author =   {R. A. Fisher},
  title =    {The use of multiple measurements in taxonomic problems},
  journal =      {Annals of Eugenics},
  year =     {1936},
  OPTkey =   {},
  volume =   {7},
  OPTnumber =    {},
  pages =    {179-188},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Fisher26,
  author =   {R. A. Fisher},
  title =    {The arrangement of field experiments},
  journal =      {J. Min. Agric. Gr. Br},
  year =     {1926},
  OPTkey =   {},
  volume =   {33},
  OPTnumber =    {},
  pages =    {505--513},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{Fix&Hodges,
  author =   {E. Fix and J. Hodges},
  title =    {Discriminatory analysis, nonparametric discrimination: consistency properties},
  institution =  {Randolph Field, Texas: USAF School of Aviation Medicine},
  year =     {1951},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Fowlkes&Mallows83,
  author =   {E. B. Fowlkes and C. L. Mallows},
  title =    {A method for comparing two hierarchical clusterings},
  journal =      JASA,
  year =     {1983},
  OPTkey =   {},
  volume =   {78},
  OPTnumber =    {383},
  OPTmonth =     {},
  pages =    {553--584},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Fowlkesetal88,
  author =   {E. B. Fowlkes and R. Gnanadesikan and J. R. Kettenring},
  title =    {Variable selection in clustering},
  journal =      JC,
  year =     {1988},
  OPTkey =   {},
  volume =   {5},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {205--228},
  OPTnote =      {},
  OPTannote =    {}
}

@TechReport{Fraley&Raftery98,
  author =   {C. Fraley and A. Raftery},
  title =    {How many clusters? Which clustering method? -- answers via model-based cluster analysis},
  institution =  {Department of Statistics, University of Washington},
  year =     {1998},
  OPTkey =   {},
  OPTtype =      {},
  number =   {329},
  OPTaddress =   {},
  OPTmonth =     {},
  note =     {\url{http://www.stat.washington.edu/www/research/reports/1990s/#1998}},
  OPTannote =    {}
}




@Article{Freund&Schapire97,
  author =   {Y. Freund and R. E. Schapire},
  title =    {A decision-theoretic generalization of on-line learning and an application to boosting},
  journal =      {Journal of Computer and System Sciences},
  year =     {1997},
  OPTkey =   {},
  volume =   {55},
  OPTnumber =    {},
  pages =    {119--139},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@PhdThesis{Fridlyand,
  author =   {J. Fridlyand},
  title =    {Resampling methods for variable selection and classification: applications to genomics},
  school =   {Department of Statistics, U.C. Berkeley},
  year =     {2001},
  OPTkey =   {},
  type =     {Ph.{D}. thesis},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{Friedman94 ,
  author =   {J. H. Friedman},
  title =    {Flexible metric nearest neighbor clasification},
  institution =  {Department of Statistics, Stanford University},
  year =     {1994},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@TechReport{Friedman96a,
  author =   {J. H. Friedman},
  title =    {On bias, variance, 0/1-loss, and the curse--of--dimensionality },
  institution =  {Department of Statistics, Stanford University},
  year =     {1996},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{Friedman96b,
  author =   {J. H. Friedman},
  title =    {Another approach to polychotomous classification},
  institution =  {Department of Statistics, Stanford University},
  year =     {1996},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Friedmanetal00,
  author =   {J. Friedman and T. Hastie and R. Tibshirani},
  title =    {Additive logistic regression: a statistical view of boosting},
  journal =      {Annals of Statistics},
  year =     {2000},
  OPTkey =   {},
  volume =   {28},
  OPTnumber =    {},
  pages =    {337--404},
  OPTmonth =     {},
  note =     {(with discussion)},
  OPTannote =    {}
}

@book {GAM,
   AUTHOR = {T. J. Hastie and R.J. Tibshirani},
    TITLE = {Generalized Additive Models},
PUBLISHER = {Chapman and Hall},
  ADDRESS = {London},
     YEAR = {1990},
    PAGES = {},
     ISBN = {},
}



@Article{Gabriel,
  author =   {K. R. Gabriel},
  title =    {The biplot graphic display of matrices with application to principal component analysis},
  journal =      {Biometrika},
  year =     {1971},
  OPTkey =   {},
  volume =   {58},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {453--467},
  OPTnote =      {},
  OPTannote =    {}
}

@InCollection{Gabriel75,
  author =   {K. R. Gabriel},
  title =    {A comparison of some methods of simultaneous inference in {MANOVA}},
  booktitle =    {Multivariate Statistical Methods: Among-groups covariation; Within-group covariation},
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {61--80},
  OPTpublisher = {},
  year =     {1975},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTtype =      {},
  OPTchapter =   {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@InProceedings{GabrielPun,
  author =       {K. R. Gabriel and F. C. Pun},
  title =        {Binary prediction of weather events with several predictors},
  booktitle =    {Sixth Conference on Probability and Statistics in Atmospheric Science},
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {248--253},
  year =     {1979},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  organization = {American Meterological Society},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}


@Unpublished{Ge&Dudoit,
  author =   {Y. Ge and S. Dudoit},
  title =    {Fast algorithm for resampling-based $p$-value adjustment in multiple testing},
  note =     {(In preparation)},
  OPTkey =   {},
  OPTmonth =     {},
  year =     {2002},
  OPTannote =    {}
}

@Article{Geisser75,
  author =   {S. Geisser},
  title =    {The predictive sample reuse method with applications},
  journal =      {Journal of the American Statistical Association},
  year =     {1975},
  volume =   {70},
  pages =    {320-328}
}

@TechReport{Genovese&Wasserman01,
  author =   {C. Genovese and L. Wasserman},
  title =    {Operating Characteristics and Extensions of the FDR Procedure},
  institution =  {Department of Statistics, Carnegie Mellon},
  year =     {2001},
  OPTkey =   {},
  OPTtype =      {},
  number =   {737},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Gnanadesikan&Kettering95,
  author =   {R. Gnanadesikan and J. R. Kettenring},
  title =    {Weighting and selection of variables for cluster analysis},
  journal =      JC,
  year =     {1995},
  OPTkey =   {},
  volume =   {12},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {113--136},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{GoldsteinetalGenEpi00,
  author =   {D. R. Goldstein and S. Dudoit and T. P. Speed},
  title =    {Power of a score test for quantitative trait linkage analysis of relative pairs.},
  journal =      {Genetic Epidemiology},
  year =     {2000},
  OPTkey =   {},
  volume =   {19},
  number =   {Suppl. 1},
  pages =    {S85--S91},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{GoldsteinetalGenEpi01,
  author =   {D. R. Goldstein and S. Dudoit and T. P. Speed},
  title =    {Power and robustness of a score  test for linkage analysis of quantitative traits using identity by descent data on sib pairs},
  journal =      {Genetic Epidemiology},
  year =     {2001},
  OPTkey =   {},
  volume =   {20},
  number =   {4},
  pages =    {415--431},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@article {Gordon85,
AUTHOR ={L. Gordon and R.A. Olshen},
TITLE ={Tree-structured survival analysis},
JOURNAL = {Cancer Treatment Reports},
VOLUME = {69},
YEAR ={1985},
NUMBER={},
PAGES = {10065-1069},
ISSN = {},
CODEN = {},
}



@InCollection{Gordon96,
  author =   {A. D. Gordon},
  title =    {Hierarchical classification},
  booktitle =    {Clustering and Classification},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher = {World Scientific Publishing Co.},
  year =     {1996},
  editor =   {P. Arabie and L. J. Hubert and G. De Soete},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {River Edge, NJ},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {65--121},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Gower&Hand,
  author = {J. C. Gower and D. J. Hand},
  title =    {Biplots},
  publisher =    {Chapman \& Hall},
  year =     {1996},
  OPTkey =   {},
  OPTeditor =    {},
  OPTvolume =    {},
  number =   {54},
  series =   {Monographs on statistics and applied probability},
  OPTaddress =   {},
  edition =      {1st},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@book {Gyorfi02,
   AUTHOR = {L. Gy\"{o}rfi and M. Kohler and A. Krzy\.{z}ak  and H. Walk},
    TITLE = {A Distribution-Free Theory of Nanparametric Regression},
PUBLISHER = {Springer-Verlag},
  ADDRESS = {New York},
     YEAR = {2002},
    PAGES = {100-102},
     ISBN = {}
}




@Book{Gyorfietal02,
  author =   {L. Gy\"orfi and M. Kohler and A. Krzy\'{z}ak and H. Walk},
  ALTeditor =    {},
  title =    {A distribution-free theory of nonparametric regression},
  publisher =    {Springer-Verlag, New York},
  year =     {2002},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Book{HTF01,
  author =   {T. Hastie and R. Tibshirani and J. H. Friedman},
  ALTeditor =    {},
  title =    {The Elements of Statistical Learning : Data Mining, Inference, and Prediction },
  publisher =    {Springer Verlag},
  year =     {2001},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Hansen01,
  author =   {M. H. Hansen  and B. Yu},
  title =    {Model selection and the principle of minimum description length},
  journal =      {Journal of the American Statistical Association},
  year =     {2001},
  volume =   {96},
  pages =    {746-774}
}

@Article{Hardle85a,
  author =   {W. H{\"a}rdle and J. S. Marron},
  title =    {Asymptotic nonequivalence of some bandwidth selectors in nonparametric regression},
  journal =      {Biometrika},
  year =     {1985},
  volume =   {72},
  pages =    {481--484}
}




@Article{Hardle85b,
  author =   {W. H{\"a}rdle and J. S. Marron},
  title =    {Optimal bandwidth selection in nonparametric regression function estimation},
  journal =      {Annals of Statistics},
  year =     {1985},
  volume =   {13},
  pages =    {1465-1481}
}

@Book{Hardle93,
  author =       {W. H{\"a}rdle},
  title =        {Applied Nonparametric Regression},
  publisher =    {Cambridge University Press},
  pages = {},
  year =         {1993}
}

@Article{Hartigan72,
  author =   {J. A. Hartigan},
  title =    {Direct clustering of a data matrix},
  journal =      {Journal of the American Statistical Association},
  year =     {1972},
  OPTkey =   {},
  volume =   {67},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {123--129},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Hartigan75,
  author =   {J. A. Hartigan},
  title =    {Clustering Algorithms},
  publisher =    {Wiley},
  year =     {1975},
  OPTkey =   {},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Hartigan78,
  author =   {J. Hartigan},
  title =    {Asymptotic distributions for clustering criteria},
  journal =      {Annals of Statistics},
  year =     {1978},
  OPTkey =   {},
  volume =   {6},
  OPTnumber =    {},
  pages =    {117--131},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Hartigan85,
  author =   {J. A. Hartigan},
  title =   {Statistical theory in clustering} ,
  journal =      JC,
  year =     {1985},
  OPTkey =   {},
  volume =   {2},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {63--76},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Hastie&Tibshirani96a,
  author =   {T. Hastie and R. Tibshirani},
  title =    {Discriminant adaptive nearest-nieghbor classification},
  journal =      {IEEE Pattern Recognition and Machine Intelligence},
  year =     {1996},
  OPTkey =   {},
  volume =   {18},
  OPTnumber =    {},
  pages =    {607--616},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{Hastie&Tibshirani96b,
  author =   {T. Hastie and R. Tibshirani},
  title =    {Classification by pairwise coupling},
  institution =  {Department of Statistics, Stanford University},
  year =     {1996},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@article {Hastie90,
   AUTHOR = {T.J. Hastie and  R.J. Tibshirani},
    TITLE = {Exploring the nature of covariate effects in the proportional hazar
ds model},
  JOURNAL = {Biometrics},
   VOLUME = {46},
     YEAR = {1990},
   NUMBER = {4},
    PAGES = {1005-1016},
     ISSN = {},
    CODEN = {},
}


@Book{Hochberg&Tamhane,
  author =   {Y. Hochberg and A. C. Tamhane},
  ALTeditor =    {},
  title =    {Multiple Comparison Procedures},
  publisher =    {Wiley--Interscience},
  year =     {1987},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  series =   {Probability and Mathematical Statistics},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Hochberg88,
  author =   {Y. Hochberg},
  title =    {A sharper Bonferroni procedure for multiple tests of significance},
  journal =      {Biometrika},
  year =     {1988},
  OPTkey =   {},
  volume =   {75},
  OPTnumber =    {},
  pages =    {800--802},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Holm79,
  author =   {S. Holm},
  title =    {A simple sequentially rejective multiple test procedure},
  journal =      {Scand. J. Statist.},
  year =     {1979},
  OPTkey =   {},
  volume =   {6},
  OPTnumber =    {},
  pages =    {65--70},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Hommel&Bernhard99,
  author =   {G. Hommel and G. Bernhard},
  title =    {Bonferroni procedures for logically related hypotheses},
  journal =      {Journal of Statistical Planning and Inference},
  year =     {1999},
  OPTkey =   {},
  volume =   {82},
  OPTnumber =    {},
  pages =    {119--128},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Hommel88,
  author =   {G. Hommel},
  title =    {A stagewise rejective multiple test procedure based on a modified Bonferroni test},
  journal =      {Biometrika},
  year =     {1988},
  OPTkey =   {},
  volume =   {75},
  OPTnumber =    {},
  pages =    {383--386},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Hubert&Arabie85,
  author =   {L. Hubert and P. Arabie},
  title =    {Comparing partitions},
  journal =      JC,
  year =     {1985},
  OPTkey =   {},
  volume =   {2},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {193--218},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Jain&DubesBook,
  author =   {A. K. Jain and R. C. Dubes},
  editor =   {},
  title =    {Algorithms for Clustering Data},
  publisher =    {Prentice-Hall},
  year =     {1988},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {Englewood Cliffs, N. J.},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Jogdeo77,
  author =   {K. Jogdeo},
  title =    {Association and probability inequalities},
  journal =      {Annals of Statistics},
  year =     {1977},
  OPTkey =   {},
  volume =   {5},
  OPTnumber =    {},
  pages =    {495--504},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Kaufman&Rousseeuw90,
  author =   {L. Kaufman and P. J. Rousseeuw},
  ALTeditor =    {},
  title =    {Finding Groups in Data: An Introduction to Cluster Analysis},
  publisher =    {Wiley, New York.},
  year =     {1990},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@article {Keles03,
AUTHOR ={Kele\c{s}, S. and van der Laan, M. and Dudoit,  S.},
TITLE ={Asymptotically Optimal  Model Selection Method for Regression on Censored Outcomes },
JOURNAL = {Technical Report, Division of Biostatistics, UC Berkeley},
VOLUME = {},
YEAR ={2002},
PAGES = {},
ISSN = {},
CODEN = {},
}



@Article{Kohonen90,
  author =   {T. Kohonen},
  title =    {The self-organizing map},
  journal =      {Proc. IEEE},
  year =     {1990},
  OPTkey =   {},
  volume =   {78},
  number =   {9},
  OPTmonth =     {},
  pages =    {1464--1480},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Kohonen95,
  author =   {T. Kohonen},
  title =    {Self-Organizing Maps},
  publisher =    {Springer},
  year =     {1995},
  OPTkey =   {},
  editor =   {T. S. Huang and T. Kohonen and M. R. Schroeder},
  volume =   {30},
  OPTnumber =    {},
  series =   {Springer Series in Information Sciences},
  address =      {Berlin, Heidelberg},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@article {Kooperberg95,
AUTHOR ={C. Kooperberg and C.J.  Stone and Y. K.  Truong},
TITLE ={Hazard Regression},
JOURNAL = {Journal of the American Statistical Association},
VOLUME = {90},
YEAR ={1995},
NUMBER={429},
PAGES = {78-94},
ISSN = {},
CODEN = {},
}



@Article{Koutsoukosetal,
  author =   {A. D. Koutsoukos and L. V. Rubinstein and D. Faraggi and R.M. Simon and S. Kalyandrug and J. N. Weinstein and K.W. Kohn and K.D. Paull},
  title =    {Discrimination techniques applied to the {NCI} in vitro anti-tumor drug screen: predicting biochemical mechanism of action},
  journal =      {Statistics in Medicine},
  year =     {1994},
  OPTkey =   {},
  volume =   {13},
  OPTnumber =    {},
  pages =    {719--730},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Krishnaiah&Reising85,
  author =   {P. R. Krishnaiah and J. M. Reising},
  title =    {Multivariate multiple comparisons},
  journal =      {Encyclopedia of Statistical Sciences},
  year =     {1985},
  OPTkey =   {},
  volume =   {9},
  number =   {6},
  pages =    {88--95},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Krzanowski&Lai,
  author =   {W. Krzanowski and Y. Lai },
  title =    {A criterion for determining the number of groups in a dataset using sum of squares clustering},
  journal =      {Biometrics},
  year =     {1985},
  OPTkey =   {},
  volume =   {44},
  OPTnumber =    {},
  pages =    {23--34},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Laan&Bryan01,
  author =   {M. J. van der Laan and J. Bryan},
  title =    {Gene expression analysis with the parametric bootstrap},
  journal =      {Biostatistics},
  year =     {2001},
  OPTkey =   {},
  volume =   {2},
  number =   {4},
  pages =    {445--461},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Pollard&vanderLaan04,
  author =   {K. S. Pollard and M.J. van der Laan},
  title =    {Choice of Null Distribution in Resampling Based Multiple Testing},
  journal =      JSPI,
  year =     {2004},
  OPTkey =   {},
  OPTvolume =    {125},
  OPTnumber =    {},
  OPTpages =     {85--101},
  OPTmonth =     {},
  note =     {},
  OPTannote =    {}
}


@Article{Laan&PollardJSPI02,
  author =   {M. J. van der Laan and K. S. Pollard},
  title =    {Hybrid clustering of gene expression data with visualization and the bootstrap},
  journal =      JSPI,
  year =     {2002},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTpages =     {},
  OPTmonth =     {},
  note =     {(To appear)},
  OPTannote =    {}
}


@article {Leblanc92,
AUTHOR ={M. Leblanc and J. Crowley},
TITLE ={Relative Risk trees for censored data},
JOURNAL = {Biometrics},
VOLUME = {48},
YEAR ={1992},
NUMBER={},
PAGES = {411-425},
ISSN = {},
CODEN = {},
}





@InProceedings{Leisch02,
  author =   {F. Leisch},
  title =    {Sweave: Dynamic Generation of Statistical Reports Using
                  Literate Data Analysis},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle = {Compstat 2002 --- Proceedings in Computational
                  Statistics},
  Tpages =   {575--580},
  year =     {2002},
  editor =   {Wolfgang H{\"a}rdle and Bernd R{\"o}nz},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  publisher = {Physika Verlag, Heidelberg, Germany},
  note =     {ISBN 3-7908-1517-9},
  OPTannote =    {},
  url =      {http://www.ci.tuwien.ac.at/~leisch/Sweave}
}

@TechReport{Leisch02TR,
  author =   {F. Leisch},
  title =    {Dynamic generation of statistical reports using literate data analysis},
  institution =  {SFB Adaptive Information Systems and Modelling in Economics and Management
Science, Vienna University of Economics and Business Administration},
  year =     {2002},
  OPTkey =   {},
  OPTtype =      {},
  number =   {69},
  OPTaddress =   {},
  month =    {March},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{Leisch99,
  author =   {F. Leisch},
  title =    {Bagged clustering},
  institution =  {SFB Adaptive Information Systems and Modelling in Economics and Management Science, Vienna University of Economics and Business Administration},
  year =     {1999},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  month =    {August},
  note =     {\url{http://www.ci.tuwien.ac.at/~leisch/papers/fl-techrep.html}},
  OPTannote =    {}
}

@Article{Limetal00,
  author =   {T-S Lim and W-Y Loh and Y-S Shih},
  title =    {A comparison of prediction accuracy, complexity, and training time of thiry-three old and new classification algorithms},
  journal =      {Machine Learning},
  year =     {2000},
  OPTkey =   {},
  volume =   {40},
  OPTnumber =    {},
  pages =    {203--229},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Book{Mardiaetal,
  author =   {K. V. Mardia and J. T. Kent and J. M. Bibby},
  title =    {Multivariate Analysis},
  publisher =    {Academic Press, Inc.},
  year =     {1979},
  OPTkey =   {},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {San Diego},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Unpublished{Mayo&Spanos02,
  author =       {D. C. Mayo and A. Spanos},
  title =        {A severe-testing interpretation of {N}eyman-{P}earson methods.  Unpublished manuscript},
  OPTnote =         {},
  OPTkey =       {},
  OPTmonth =     {},
  year =         {2002},
  OPTannote =    {}
}


@Book{McCullagh&Nelder89,
  author =   {P. McCullagh and J. A. Nelder},
  ALTeditor =    {},
  title =    {Generalized Linear Models},
  publisher =    {Chapman \& Hall},
  year =     {1989},
  OPTkey =   {},
  OPTvolume =    {},
  number =   {37},
  series =   {Monographs on Statistics and Applied Probability},
  OPTaddress =   {},
  edition =      {2nd},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Book{McLachlan,
  author =   {G. J. McLachlan},
  OPTeditor =    {},
  title =    {Discriminant analysis and statistical pattern recognition},
  publisher =    {Wiley},
  year =     {1992},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {New York},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{McLachlanetal01,
  author =   {G. J. McLachlan and R. Bean and D. Peel},
  title =    {A mixture model-based approach to the clustering of microarray expression data.},
  journal =      {Bioinformatics},
  year =     {2002},
  OPTkey =   {},
  volume =   {18},
  OPTnumber =    {},
  pages =    {413--422},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{MillerSubsets,
  author =   {A. J. Miller},
  OPTeditor =    {},
  title =    {Subset Selection in Regression},
  publisher =    {Chapman and Hall},
  year =     {1990},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Milligan&Cooper85,
  author =   {G. W. Milligan and M. C. Cooper},
  title =    {An examination of procedures for determining the number of clusters in a data set},
  journal =      {Psychometrika},
  year =     {1985},
  OPTkey =   {},
  volume =   {50},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {159--179},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Milligan&Cooper86,
  author =   {G. W. Milligan and M. C. Cooper},
  title =    {A study of the comparability of external criteria for hierarchical cluster analysis},
  journal =      {Multivariate Behavioral Research},
  year =     {1986},
  OPTkey =   {},
  volume =   {21},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {441--458},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Milligan&Cooper87,
  author =   {G. W. Milligan and M. C. Cooper},
  title =    {Methodology review: {C}lustering methods},
  journal =      {Applied Psychological Measurement},
  year =     {1987},
  OPTkey =   {},
  volume =   {11},
  OPTnumber =    {4},
  OPTmonth =     {December},
  pages =    {329--354},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Milligan89,
  author =   {G. W. Milligan},
  title =    {A study of the beta-flexible clustering method},
  journal =      {Multivariate Behavioral Research},
  year =     {1989},
  OPTkey =   {},
  volume =   {24(2)},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {163--176},
  OPTnote =      {},
  OPTannote =    {}
}


@InCollection{Milligan96,
  author =   {G. W. Milligan},
  title =    {Clustering validation: {R}esults and implications for applied analyses},
  booktitle =    {Clustering and Classification},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher = {World Scientific Publishing Co.},
  year =     {1996},
  editor =   {P. Arabie and L. J. Hubert and G. De Soete},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {River Edge, NJ},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {341--375},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Moreyetal83,
  author =   {L. C. Morey, R. K. Blashfield and H. A. Skinner},
  title =    {A comparison of cluster analysis techniques within a sequential validation framework},
  journal =      {Multivariate Behavioral Research},
  year =     {1983},
  OPTkey =   {},
  volume =   {18},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {309--329},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Morrison90,
  author =   {D. F. Morrison},
  ALTeditor =    {},
  title =    {Multivariate Statistical Methods},
  publisher =    {McGraw-Hill, NY},
  year =     {1990},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  edition =      {3rd},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@InCollection{Murtagh96,
  author =   {F. Murtagh},
  title =    {Neural networks for clustering},
  booktitle =    {Clustering and Classification},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher = {World Scientific Publishing Co.},
  year =     {1996},
  editor =   {P. Arabie and L. J. Hubert and G. De Soete},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {River Edge, NJ},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {235--269},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{PanelDACC,
  author =   {{Panel on Discriminant Analysis, Classification, and Clustering}},
  title =    {Discriminant analysis and clustering},
  journal =      {Statistical Science},
  year =     {1989},
  OPTkey =   {},
  volume =   {4},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {34--69},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{Pavlic&vanderLaanTechRep89,
  author =   {M. Pavlic and M. J. van der Laan},
  title =    {Fitting of mixtures with unspecified number of components using cross-validation distance estimate},
  institution =  {Division of Biostatistics, U.C. Berkeley},
  year =     {2001},
  OPTkey =   {},
  OPTtype =      {},
  number =   {89},
  OPTaddress =   {},
  month =    {February},
  OPTnote =      {},
  OPTannote =    {}
}

@article{Pavlic02,
author  = {M. Pavlic and M. J. van der Laan},
title   = {Fitting of mixtures with unspecified number of components using
cross validation distance estimate},
journal = {Computational Statistics and Data Analysis},
volume  = {41},
issue   = {3-4},
pages   = {413-428},
year    = {2003}
}



@TechReport{Pollard&LaanTechRep107,
  author =   {K. S. Pollard and M. J. van der Laan},
  title =    {A Method to Identify Significant Clusters in Gene Expression Data},
  institution =  {Division of Biostatistics, U.C. Berkeley},
  year =     {2002},
  OPTkey =   {},
  OPTtype =      {},
  number =   {107},
  OPTaddress =   {},
  month =    {April},
  OPTnote =      {},
  OPTannote =    {}
}

@TechReport{Pollard&LaanTechRep121,
  author =   {K. S. Pollard and M. J. van der Laan},
  title =    {Resampling-based methods for identification of significant subsets of genes in expression data},
  institution =  {Division of Biostatistics, U.C. Berkeley},
  year =     {2002},
  OPTkey =   {},
  OPTtype =      {},
  number =   {121},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Ramsey78,
  author =   {P. H. Ramsey},
  title =    {Power differences between pairwise multiple comparisons},
  journal =      JASA,
  year =     {1978},
  OPTkey =   {},
  volume =   {73},
  OPTnumber =    {},
  pages =    {479--485},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Manual{RanForests,
  title =    {Notes on setting up, using, and understanding random forests V3.0},
  OPTkey =   {},
  author =   {L. Breiman},
  OPTorganization = {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  year =     {2001},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Rand,
  author =   {W. M. Rand},
  title =    {Objective criteria for the evaluation of clustering methods},
  journal =      {Journal of the American Statistical Association},
  year =     {1971},
  OPTkey =   {},
  volume =   {66},
  OPTnumber =    {336},
  OPTmonth =     {},
  pages =    {846--850},
  OPTnote =      {},
  OPTannote =    {}
}

@Unpublished{Reineretal01,
  author =   {A. Reiner and D. Yekutieli and Y. Benjamini},
  title =    {Using resampling-based {FDR} controlling multiple test procedures for analyzing microarray gene expression data},
  OPTnote =      {},
  OPTkey =   {},
  OPTmonth =     {},
  year =     {2001},
  OPTannote =    {}
}


@Book{Ripley96,
  author =   {B. D. Ripley},
  title =    {Pattern recognition and neural networks},
  publisher =    {Cambridge University Press},
  year =     {1996},
  OPTkey =   {},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {Cambridge, New York},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}




%very first reference to use trees in survival analysis
@Article{Rissanen78,
  author =   {J. Rissanen},
  title =    {Modelling by shortest data description},
  journal =      {Automatica},
  year =     {1978},
  volume =   {14},
  pages =    {465-471}
}

@Article{Rnews:Dudoit+Yang+Bolstad:2002,
  author       = {S. Dudoit and Y. H.  Yang and B. Bolstad},
  title        = {Using {R} for the Analysis of {DNA} Microarray Data},
  journal      = {R News},
  year         = 2002,
  volume       = 2,
  number       = 1,
  pages        = {24--32},
  month        = {March},
  url          = {CRAN.R-project.org/doc/Rnews/}
}

@article {Robins00a,
AUTHOR ={J. M. Robins and A.  Rotnitzky},
TITLE ={Comment on the {B}ickel and {K}won article, ``{I}nference for semiparametric models: {S}ome questions and an answer''},
JOURNAL = {Statistica Sinica},
VOLUME = {11},
NUMBER={4},
YEAR ={2001},
PAGES = {920-936},
ISSN = {},
CODEN = {}
}


@InProceedings{Robins00c,
  author =   {J.M. Robins},
  title =    {Robust estimation in sequentially ignorable
missing data and causal inference models},
  booktitle =    {Proceedings of the American
Statistical Association},
  pages =    {},
  year =     {2000},
  editor =   {},
  organization = {}
}


@article {Robins00b,
AUTHOR ={J. M. Robins and A.  Rotnitzky and M.J. van der Laan},
TITLE ={Comment on ``{O}n {P}rofile {L}ikelihood" by {S}.{A}. {M}urphy and
{A}.{W}. van der {V}aart},
JOURNAL = {Journal of the American Statistical Association -- Theory and
Methods
},
VOLUME = {450},
YEAR ={2000},
PAGES = {431-435},
ISSN = {},
CODEN = {}
}



@Article{Birge83,
  author =   {L. Birg{\'e}},
  title =    {Approximation dans les espaces m{/'e}triques et th{\'e}orie
  de l'estimation},
  journal =      {Verw. Gebiete},
  year =     {1983},
  OPTkey =   {},
  volume =   {65},
  number =   {},
  OPTmonth =     {},
  pages =    {181--238},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{lecam73,
  author =   {L.M. le Cam},
  title =    {Convergence of estimates under dimensionality restrictions},
  journal =      {Annals of Statistics},
  year =     {1973},
  OPTkey =   {},
  volume =   {22},
  number =   {},
  OPTmonth =     {},
  pages =    {38--53},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Rom90,
  author =   {D. M. Rom},
  title =    {A sequentially rejective test procedure based on a modified {Bonferroni} inequality},
  journal =      {Biometrika},
  year =     {1990},
  OPTkey =   {},
  volume =   {77},
  OPTnumber =    {},
  pages =    {663-665},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{Rosenblatt57,
  author =       {F. Rosenblatt},
  title =        {The perceptron -- a perceiving and recognizing automation},
  institution =  {Cornell Aeronautical Laboratory },
  year =         {1957},
  OPTkey =       {},
  OPTtype =      {},
  number =       {86-460-1},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Ruczinskietal,
  author =   {I. Ruczinski and C. Kooperberg and M. LeBlanc},
  title =    {Logic regression},
  journal =      {},
  year =     {2001},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTpages =     {},
  OPTmonth =     {},
  note =     {Submitted, \url{http://biosun01.biostat.jhsph.edu/~iruczins/html/publications.html}},
  OPTannote =    {}
}

@Article{Saltstone&Stange,
  author =   {R. Saltstone and K. Stange},
  title =    {A computer program to calculate Hubert and Arabie's adjusted Rand index},
  journal =      {Journal of Classification},
  year =     {1996},
  OPTkey =   {},
  volume =   {13},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {169--172},
  OPTnote =      {},
  OPTannote =    {}
}
@TechReport{vanderVaart03,
  author =   {A.W. van der Vaart},
  title =    {Notes on Cross-validation},
  institution =  {Department of Mathematics, Free University, Amsterdam},
  year =     {2003},
  OPTkey =   {},
  OPTtype =      {},
  number =   {},
  OPTaddress =   {},
  OPTmonth =     {},
  note =     {},
  OPTannote =    {Unpublished manuscript}
}

@TechReport{Sarle,
  author =   {W. Sarle},
  title =    {Cubic clustering criterion},
  institution =  {SAS Institute, Inc.},
  year =     {1983},
  OPTkey =   {},
  OPTtype =      {},
  number =   {A-108},
  OPTaddress =   {},
  OPTmonth =     {},
  note =     {\url{http://www.sas.com/service/library/onlinedoc/trindex.html}},
  OPTannote =    {}
}

@TechReport{Sarle&Kuo,
  author =   {W. Sarle and A. Kuo},
  title =    {The MODECLUS Procedures},
  institution =  {SAS Institute, Inc.},
  year =     {1993},
  OPTkey =   {},
  OPTtype =      {},
  number =   {P-256},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Schapireetal,
  author =   {R. E. Schapire and Y. Freund and P. Bartlett and W. S. Lee},
  title =    {Boosting the margin: a new explanation for the effectiveness of voting methods},
  journal =      {Annals of Statistics},
  year =     {1998},
  OPTkey =   {},
  volume =   {26},
  OPTnumber =    {},
  pages =    {1651--1686},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Book{Scheffe,
  author =   {H. Scheff\'{e}},
  ALTeditor =    {},
  title =    {The analysis of variance},
  publisher =    {John Wiley \& Sons},
  year =     {1959},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Scheibler&Schneider,
  author =   {D. Scheibler and W. Schneider},
  title =    {Monte Carlo tests of the accuracy of cluster analysis algorithms: A comparison of hierarchical and nonhierarchical methods},
  journal =      {Multivariate Behavioral Research},
  year =     {},
  OPTkey =   {},
  volume =   {20},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {283--304},
  OPTnote =      {},
  OPTannote =    {}
}


@InProceedings{Schuster81,
  author =   {E. F. Schuster and C. G. Gregory},
  title =    {On the non-consistency of maximum likelihood nonparametric density estimators},
  booktitle =    {Computer Science and Statistics: Proceedings of the 13th Symposium on the interface},
  pages =    {295-298},
  year =     {1981},
  editor =   {Eddy, W.F.},
  organization = {}
}


@Article{Scott81,
  author =   {D. W. Scott and L. E. Factor},
  title =    {Monte Carlo study of three data-based nonparametric density estimators},
  journal =      {Journal of the American Statistical Association},
  year =     {1981},
  volume =   {76},
  pages =    {9-15}
}

@Article{Seeger68,
  author =   {P. Seeger},
  title =    {A note on a method for the analysis of significances en masse},
  journal =      {Technometrics},
  year =     {1968},
  OPTkey =   {},
  volume =   {10},
  number =   {3},
  pages =    {586--593},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Segal88,
  author =   {M. R. Segal},
  title =    {Regression trees for censored data},
  journal =      {Biometrics},
  year =     {1988},
  OPTkey =   {},
  volume =   {44},
  OPTnumber =    {},
  pages =    {35--47},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}





@string{JASA= {Journal of the American Statistical Association}}
@string{JC = {Journal of Classification}}
@string{JSPI = {Journal of Statistical Planning and Inference}}
@string{JRSSB = {Journal of the Royal Statistical Society, Series B}}
@string{PNAS = {Proc. Natl. Acad. Sci.}}

@Article{Shaffer02,
  author =   {J. P. Shaffer},
  title =    {Multiplicity, directional ({T}ype {III}) errors, and
the null hypothesis},
  journal =      {Psychological Methods},
  year =     {2002},
  OPTkey =   {},
  volume =   {7},
  OPTnumber =    {},
  pages =    {356--369},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Shaffer86,
  author =   {J. P. Shaffer},
  title =    {Modified sequentially rejective multiple test procedures},
  journal =      JASA,
  year =     {1986},
  OPTkey =   {},
  volume =   {81},
  OPTnumber =    {},
  pages =    {826--831},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Shaffer95,
  author =   {J. P. Shaffer},
  title =    {Multiple hypothesis testing},
  journal =      {Annu. Rev. Psychol.},
  year =     {1995},
  OPTkey =   {},
  volume =   {46},
  OPTnumber =    {},
  pages =    {561--584},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@article{Shao93,
AUTHOR={Shao, J.},
TITLE={Linear Model Selection by Cross-Validation},
JOURNAL={Journal of the American Statistical Association},
VOLUME={88},
YEAR={1993},
PAGES={486-494}
}




@Article{Sidak67,
  author =   {Z. \v{S}id\'{a}k},
  title =    {Rectangular confidence regions for the means of multivariate normal distributions},
  journal =      JASA,
  year =     {1967},
  OPTkey =   {},
  volume =   {62},
  OPTnumber =    {},
  pages =    {626-633},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Silverman,
  author =   {B. W. Silverman},
  title =    {Smoothed functional principal components analysis by choice of norm},
  journal =      {Annals of Statistics},
  year =     {1996},
  OPTkey =   {},
  volume =   {24},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {1--24},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Silverman84,
  author =   {B. W. Silverman},
  title =    {A fast and efficient cross-validation method for smoothing parameter choice in spline regression},
  journal =      JASA,
  year =     {1984},
  OPTkey =   {},
  volume =   {79},
  number =   {387},
  pages =    {584--589},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}




@Book{Silverman86,
  author =       {B. W. Silverman},
  title =        {Density Estimation for Statistics and Data analysis},
  publisher =    {Chapman \& Hall},
  pages = {},
  year =         {1986}
}

@Article{vanderLaan&Dudoit&Keles04,
  author =   {M.J. van der Laan and S. Dudoit and S. Keles},
  title =    {Asymptotic optimality of likelihood-based cross-validation},
  journal =      {Statistical Applications in Genetics and Molecular Biology},
  year =     {2004},
  OPTkey =   {},
  volume =   {3},
  OPTnumber =    {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/sagmb/vol3/iss1/art4},
  OPTannote =    {}
}
@Article{Simes86,
  author =   {R. J. Simes},
  title =    {An improved Bonferroni procedure for multiple tests of significance},
  journal =      {Biometrika},
  year =     {1986},
  OPTkey =   {},
  volume =   {73},
  OPTnumber =    {},
  pages =    {751--754},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Smyth00,
  author =   {P. Smyth},
  title =    {Model selection of probabilistic clustering using cross-validated likelihood},
  journal =      {Statistics and Computing},
  year =     {2000},
  volume =   {10},
  pages =    {63-72}
}




@Article{Soric89,
  author =   {B. Sori\'{c}},
  title =    {Statistical ``discoveries" and effect-size estimation},
  journal =      JASA,
  year =     {1989},
  OPTkey =   {},
  volume =   {84},
  number =   {406},
  pages =    {608--610},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Stone74,
  author =   {M. Stone},
  title =    {Cross-validatory choice and  assessment of statistical predictions},
  journal =      {Journal of the Royal Statistical Society, Series B},
  year =     {1974},
  volume =   {36},
  pages =    {111-147}
}

@Article{Stone84,
  author =   {C. J. Stone},
  title =    {An asymptotically optimal window selection rule for kernel density estimates},
  journal =      {The Annals of Statistics},
  year =     {1984},
  volume =   {12},
  pages =    {1285-1297}
}

@Article{StoneC84,
  author =   {C. J. Stone},
  title =    {An asymptotically optimal window selection rule for kernel density estimates},
  journal =      {Annals of Statistics},
  year =     {1984},
  OPTkey =   {},
  volume =   {12},
  number =   {4},
  pages =    {1285--1297},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{StoneM74,
  author =   {M. Stone},
  title =    {Cross-validatory choice and assessment of statistics predictions},
  journal =      JRSSB,
  year =     {1974},
  OPTkey =   {},
  volume =   {36},
  number =   {2},
  pages =    {111--147},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}






@Article{StoneM77,
  author =   {M. Stone},
  title =    {Asymptotics for and against cross-validation},
  journal =      {Biometrika},
  year =     {1977},
  OPTkey =   {},
  volume =   {64},
  number =   {1},
  pages =    {29--35},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@TechReport{Storey&TibshiraniTechRep01,
  author =   {J. D. Storey and R. Tibshirani},
  title =    {Estimating false discovery rates under dependence, with applications
to DNA microarrays},
  institution =  {Department of Statistics, Stanford University},
  year =     {2001},
  OPTkey =   {},
  OPTtype =      {},
  number =   {2001-28},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{StoreyJRSSB02,
  author =   {J. D. Storey},
  title =    {A direct approach to false discovery rates},
  journal =      JRSSB,
  year =     {2002},
  OPTkey =   {},
  volume =   {64},
  OPTnumber =    {},
  pages =    {479--498},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{StoreyTechRep01,
  author =   {J. D. Storey},
  title =    {The positive False Discovery Rate: A Bayesian interpretation and the q-value},
  institution =  {Department of Statistics, Stanford University},
  year =     {2001},
  OPTkey =   {},
  OPTtype =      {},
  number =   {2001-12},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{TSH,
  author =   {E. L. Lehmann},
  ALTeditor =    {},
  title =    {Testing Statistical Hypotheses},
  publisher =    {Springer-Verlag, New York},
  year =     {1986},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  edition =      {2nd},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Tibshiranietal02a,
  author =   {R. Tibshirani and T. Hastie and B. Narasimhan and. G. Chu},
  title =    {Diagnosis of multiple cancer types by shrunken centroids of gene expression},
  journal =      PNAS,
  year =     {2002},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTpages =     {},
  OPTmonth =     {},
  note =     {In press},
  OPTannote =    {}
}


@Article{Troendle95,
  author =   {J. F. Troendle},
  title =    {A stepwise resampling method of multiple hypothesis testing},
  journal =      JASA,
  year =     {1995},
  OPTkey =   {},
  volume =   {90},
  OPTnumber =    {},
  pages =    {370--378},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Troendle96,
  author =   {J. F. Troendle},
  title =    {A permutational step-up method of testing multiple outcomes},
  journal =      {Biometrics},
  year =     {1996},
  OPTkey =   {},
  volume =   {52},
  OPTnumber =    {},
  pages =    {846--859},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{VR,
 author = { W. N. Venables and B. D. Ripley },
 title = {Modern Applied Statistics with S--PLUS},
 publisher = {Springer},
 year = {1999}
}


@Book{Vaart96,
  author =       {A. W. van der Vaart  and J. A. Wellner},
  title =        {Weak {C}onvergence and {E}mprical {P}rocesses},
  publisher =    {Springer-Verlag New York},
  pages = {102},
  year =         {1996}
}





@Book{Vaart98,
  author =       {A. W. van der Vaart},
  title =        {Asymptotic Statistics},
  publisher =    {Cambridge University Press},
  pages = {62},
  year =         {1998}
}


@Book{Vapnik,
  author =   {V. N. Vapnik},
  OPTeditor =    {},
  title =    {The nature of statistical learning theory},
  publisher =    {Springer},
  year =     {2000},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  series =   {Statistics for engineering and information science},
  address =      {New York},
  edition =      {2nd},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Vapnik79,
  author =   {V. Vapnik},
  title =    {Estimation of dependences based on empirical data (in Russian)},
  journal =      {Nauka, Moskow},
  year =     {1979},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Book{Vapnik98,
  author =       {V. Vapnik},
  title =        {Statistical Learning Theory},
  publisher =    {Wiley},
  year =         {1998},
  OPTkey =       {},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {New York},
  edition =      {1st},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Book{Venables&Ripley99,
  author =   {W. N. Venables and B. D. Ripley},
  title =    {Modern applied statistics with S-PLUS},
  publisher =    {Springer},
  year =     {1999},
  OPTkey =   {},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  edition =      {3rd},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Westfall&Young93,
  author =   {P. H. Westfall and S. S. Young},
  OPTeditor =    {},
  title =    {Resampling-based multiple testing: {E}xamples and methods for $p$-value adjustment},
  publisher =    {John Wiley \& Sons},
  year =     {1993},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{,
  author =       {},
  title =        {},
  publisher =    {},
  pages = {},
  year =         {}
}


@InCollection{Westfalletal01,
  author =   {P. H. Westfall and D. V. Zaykin and S. S. Young},
  title =    {Multiple tests for genetic effects in association studies},
  booktitle =    {Biostatistical Methods},
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {143--168},
  publisher = {Humana Press, Toloway, NJ},
  year =     {2001},
  editor =   {S. Looney},
  volume =   {184},
  OPTnumber =    {},
  series =   {Methods in Molecular Biology},
  OPTtype =      {},
  OPTchapter =   {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Westonetal2000,
  author =   {J. Weston and S. Mukherjee and  O. Chappelle and  M. Pontil and  T. Poggio and V. Vapnik},
  title =    {Feature Selection for {SVM}s},
  journal =      {Advances in Neural Processing Systems},
  year =     {2001},
  OPTkey =   {},
  volume =   {13},
  number =   {},
  pages =    {668--674},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Wright92,
  author =   {S. P. Wright},
  title =    {Adjusted P-values for simultaneous inference},
  journal =      {Biometrics},
  year =     {1992},
  OPTkey =   {},
  volume =   {48},
  number =   {4},
  pages =    {1005--1013},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{YangetalJCGS02,
  author =   {Y. H. Yang and M. J. Buckley and S. Dudoit and T. P. Speed},
  title =    {Comparison of methods for image analysis on c{DNA} microarray data},
  journal =      {Journal of Computational and Graphical Statistics},
  year =     {2002},
  OPTkey =   {},
  volume =   {11},
  number =   {1},
  pages =    {108--136},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{YangetalNAR02,
  author =   {Y. H. Yang and S. Dudoit and P. Luu and D. M. Lin and V. Peng and J. Ngai and T. P. Speed},
  title =    {Normalization for c{DNA} microarray data: {A} robust composite method addressing single and multiple slide systematic variation},
  journal =      {Nucleic Acids Research},
  year =     {2002},
  OPTkey =   {},
  volume =   {30},
  number =   {4},
  pages =    {e15},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@InProceedings{YangetalSPIE01,
  author =   {Y. H. Yang and S. Dudoit and P. Luu and T. P. Speed},
  title =    {Normalization for c{DNA} microarray data},
  booktitle =    {Microarrays: Optical Technologies and Informatics},
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {141--152},
  year =     {2001},
  editor =   {Michael L. Bittner and Yidong Chen and Andreas N. Dorsel and Edward R. Dougherty},
  volume =   {4266},
  OPTnumber =    {},
  series =   {Proceedings of SPIE},
  address =      {San Jose, CA},
  month =    {May},
  OPTorganization = {SPIE},
  publisher = {SPIE-International Society for Optical Engineering},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Yekutieli&Benjamini99,
  author =   {D. Yekutieli and Y. Benjamini},
  title =    {Resampling-based false discovery rate controlling multiple test procedures for correlated test statistics},
  journal =      JSPI,
  year =     {1999},
  OPTkey =   {},
  volume =   {82},
  OPTnumber =    {},
  pages =    {171--196},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@InCollection{Youden69,
  author =   {W. J. Youden},
  title =    {Measurement agreement comparisons},
  booktitle =    {Precision measurement and calibration: Statistical concepts and procedures},
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {146--151},
  publisher = {National Bureau of Standards, United States Department of Commerce},
  year =     {1969},
  editor =   {H. H. Ku},
  volume =   {1},
  OPTnumber =    {},
  series =   {Special Publication 300},
  type =     {NBS Miscelaneous Publication 248, Proceedings of the 1962 Standards Laboratory Conference},
  OPTchapter =   {},
  OPTaddress =   {},
  OPTedition =   {},
  month =    {February},
  OPTnote =      {},
  OPTannote =    {}
}




@article{Zhang93,
AUTHOR={Zhang, P.},
TITLE={Model selection via multifold cross-validation},
JOURNAL={Annals of Statistics},
VOLUME={21},
YEAR={1993},
PAGES={299-313}
}

@Article{ZhangetalBioinf02,
  author =   {J. Zhang and V. Carey and R. Gentleman},
  title =    {An extensible application for assembling annotation for
genomic data},
  journal =      {Bioinformatics},
  year =     {2002},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {},
  OPTmonth =     {},
  note =     {(In press)},
  OPTannote =    {},
  url = {http://www.R-project.org/}
}



@Book{vanderVaart98,
  author =   {A.W. van der Vaart},
  title =    {Asymptotic Statistics},
  publisher =    {Cambridge University Press},
  year =     {1998}
}




@Book{BKRW,
  author =   {P.J. Bickel and C.A.J. Klaassen and Y. Ritov and J. Wellner},
  title =    {Efficient and Adaptive Estimation for Semiparametric Models},
  publisher =    {Springer-Verlag},
  year =     {1997}
}




@Article{bozdoganaic,
  author =   {H. Bozdogan},
  title =    {Akaike's information criterion and recent developments in information complexity},
  journal =      {Journal of Mathematical Psychology},
  year =     {2000},
  volume =   {44},
  pages =    {62-91}
}



@book {cart,
   AUTHOR = {L. Breiman and J. H. Friedman and R. A. Olshen and C. J. Stone},
    TITLE = {Classification and Regression Trees},
PUBLISHER = {Wadsworth \& Brooks/Cole},
  ADDRESS = {Monterey},
     YEAR = {1984},
    PAGES = {},
     ISBN = {}
}

@book {mark,
 author = {M.J. van der Laan and J.M. Robins},
  title = {Unified methods for censored longitudinal  data and causality},
  publisher = {Springer, New York},
  year =     {2003}
}


@Manual{effsize,
  title =    {Teaching Children to Read},
  OPTkey =   {},
  author =   {{National Reading Panel}},
  organization = {National Institute of Child Health and Human Development, National Institutes of Health},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  year =     {1999},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{gapstats,
  author =   {R. Tibshirani and  G. Walther and T. Hastie.},
  title =    {Estimating the number of clusters in a dataset via the gap statistic},
  institution =  {Department of Biostatistics, Stanford University},
  year =     {2000},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  month =    {March},
  note =     {\url{http://www-stat.stanford.edu/~tibs/research.html}},
  OPTannote =    {}
}




@InProceedings{gillcar,
  author =   {R.D. Gill and M.J. van der Laan and J.M. Robins},
  title =    {Coarsening at random: characterizations, conjectures and counter-examples},
  booktitle =    {Proceedings of the First Seattle Symposium in Biostatistics},
  pages =    {255-94},
  year =     {1997},
  editor =   {D.Y. Lin and T.R. Fleming},
  address =      {New York},
  publisher = {Springer Verlag}
}
@article{Gill&Robins01,
   AUTHOR = {Gill, R. and Robins, J.M.},
    TITLE = {Causal inference in complex longitudinal studies: continuous case},
  JOURNAL = {Ann. Stat.},
 FJOURNAL = {The Annals of Statistics},
   VOLUME = {29},
     YEAR = {2001},
   NUMBER = {6},
    PAGES = {},
     ISSN = {},
    CODEN = {},
  MRCLASS = {},
 MRNUMBER = {},
}


%uses exponential mode at each node
@Article{jacobsen,
  author =   {M. Jacobsen and N. Keiding},
  title =    {Coarsening at random in general sample spaces and random censoring in continuous time},
  journal =      {Annals of Statistics},
  year =     {1995},
  volume =   {23},
  pages =    {774-86}
}

%very first reference to use trees in survival analysis










@Misc{marray,
  OPTkey =   {},
  author =   {S. Dudoit and Y. H. Yang},
  title =    {Normalization and diagnostic plots for cDNA microarray data, {\tt marrayClasses}, {\tt marrayInput}, {\tt marrayNorm}, {\tt marrayPlots}},
  howpublished = {{\tt R} packages},
  OPTmonth =     {},
  year =     {2002},
  OPTnote =      {},
  OPTannote =    {},
  url =          {www.bioconductor.org},
}

@TechReport{mclust98,
  author =   {C. Fraley and A. E. Raftery},
  title =    {MCLUST: Software for Model-Based Cluster Analysis},
  institution =  {Department of Statistics, University of Washington},
  year =     {1998},
  OPTkey =   {},
  OPTtype =      {},
  number =   {342},
  OPTaddress =   {},
  month =    {November},
  OPTnote =      {},
  OPTannote =    {}
}


@Misc{multtest,
  OPTkey =   {},
  author =   {Y. Ge and S. Dudoit},
  title =    {Multiple Testing Procedures, {\tt multtest}},
  howpublished = {{\tt R} package},
  OPTmonth =     {},
  year =     {2002},
  OPTnote =      {},
  OPTannote =    {},
  url =          {www.bioconductor.org},
}

@InProceedings{robins93,
  author =   {J.M. Robins},
  title =    {Information recovery and bias adjustment in proportional hazards regression analysis of randomized trials using surrogate markers},
  booktitle =    {Proceeding of the Biopharmaceutical section},
  pages =    {24-33},
  year =     {1993},
  organization = {American Statistical Association}
}

@InCollection{robrot,
  author =   {J.M. Robins and A. Rotnitzky},
  title =    {Recovery of information and adjustment for dependent censoring using surrogate markers},
  booktitle =    {AIDS Epidemiology},
  publisher = {Bikh\"{a}user},
  year =     {1992},
  series =   {Methodological issues}
}


@Article{robzhao,
  author =   {J.M. Robins and A. Rotnitzky and L.P. Zhao},
  title =    {Estimation of regression coefficients when some regressors are not always observed},
  journal =      {Journal of the American Statistical Association},
  year =     {1994},
  volume =   {89},
  number =   {427},
  pages =    {846-866},
  month =    {September}
}







@Article{Heitjan&Rubin91,
  author =   {D.F. Heitjan and D.B. Rubin},
  title =    {Ignorability and coarse data},
  journal =      {Annals of statistics},
  year =     {1991},
  volume =   {19},
  number =   {4},
  pages =    {2244-2253},
  month =    {December}
}

@Misc{sma,
  OPTkey =   {},
  author =   {S. Dudoit and Y. H. Yang and B. M. Bolstad},
  title =    {Statistical {M}icroarray {A}nalysis, {\tt sma}},
  howpublished = {{\tt R} package},
  OPTmonth =     {},
  year =     {2001},
  note =     {Contributions from Natalie Thorne, Ingrid L\"{o}nnstedt, and Jessica Mar},
  OPTannote =    {},
  url =          {cran.r-project.org/src/contrib/PACKAGES.html\#sma}
}

@PhdThesis{thesis,
  author =   {S. Dudoit},
  title =    {Linkage analysis of complex human traits using identity by descent data},
  school =   {Department of Statistics, University of California, Berkeley},
  year =     {1999},
  OPTkey =   {},
  OPTaddress =   {},
  type =     {Ph.D. thesis},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{vanderVaart&Wellner96,
  author =   {A. van der Vaart and J. Wellner},
  ALTeditor =    {},
  title =    {Weak Convergence and Empirical Processes},
  publisher =    {Springer-Verlag, New York},
  year =     {1996},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@article{Raudenbush&Bryk86,
  author = {S.W. Raudenbush and A.S. Bryk},
  title= {A hierarchical model
for studying school effects. Sociology of Education},
  journal = {Sociology of Education},
  volume = {59},
  issue = {},
  pages = {1--17},
  year = {1986}
}

@techreport{vanderLaan08,
	Author = {Mark J. van der Laan},
	Date-Added = {2008-03},
	Institution = {University of California, Berkeley},
	Number = {232, www.bepress.com/ucbbiostat/paper232},
	Title = {The Construction and Analysis of Adaptive Group Sequential Designs},
	Year = {2008}}

@book{Raudenbush&Bryk02,
author={S.W. Raudenbush and A.S. Bryk},
title={Hierarchical linear models: Application and data analysis methods},
publisher={Newbury
Park: Sage.},
year={2002}
}


@article{Raudenbush&Liu00,
author={ S.W. Raudenbush and X. Liu},
titlte={Statistical power and
optimal design for multisite randomized trials},
journal={Psychological
Methods},
volume={5},
pages={199Ð213},
year={2000}
}


 @article{Raudenbush&Sampson99a,
 author={S.W. Raudenbush and  R.J. Sampson},
  title={Assessing direct
and indirect effects in multilevel designs with latent
variables},
  journal={Sociological Methods \& Research},
  volume={28},
  pages={123Ð153},
  year={1999}
   }

  @inCollection{Raudenbush&Sampson99b,
 author={S.W. Raudenbush and  R.J. Sampson},
title={Ecometrics: Toward a science of assessing ecological settings, with
application to the systematic social observation of neighbor-
hoods. In M. P. Becker (Ed.)},
 booktitle={Sociological methodology},
OPTvolume={29},
 pages={1Ð41},
 publisher={Boston, MA: Blackwell},
 year={1999}
 }

 @article{Raudenbush&Whillms95,
 author={S.W. Raudenbush and J.D. Whillms},
 title={The estimation of
school effects},
 journal={Journal of Educational and Behavioral
Statistics},
 volume={20},
 pages={307Ð335},
 year={1995}
 }

@article{Coleman58,
author={J.S. Coleman},
title={Relational analysis: The study of social
organizations with survey methods},
journal={Human Organization},
volume={17},
pages={28Ð36},
year={1958}
}

@article{Colemanetal66,
author={J.S.
Coleman and E.Q. Campbell and C.J. Hobson and J. McPartland and
A.M. Mood and F.D. Weinfeld and R.L. York},
title={Equality of educational opportunity. Washington, DC:
Government Printing OfÞce},
journal={Journal of the Royal Statistical Society, Series A},
volume={156},
pages={9Ð38},
year={1966}
}


@article{Aitkin&Longford86,
author={M. Aitkin and N. Longford},
title={Statistical modeling issues
in school effectiveness studies},
journal={Journal of the Royal
Statistical Society, Series A},
volume={149},
pages={1Ð43},
year={1986}
}

@book{Rubin06,
author={D.B. Rubin},
title={Matched Sampling for Causal Effects.},
publisher={Cambridge University Press},
address={Cambridge, MA},
year={2006},
}

@book{Goldstein95,
author={H. Goldstein},
title={Multilevel statistical models},
publisher={London:
Edward Arnold},
year={1995}
}

@article{McMichael99,
author={A.J. McMichael},
title={Prisoners of the proximate: Loosening
the constraints on epidemiology in an age of change},
journal={American Journal of Epidemiology},
volume={149},
pages={887Ð897},
year={1999}
}

@article{Susser99,
author={M. Susser},
title={Should the epidemiologist be a social
scientist or a molecular biologist?},
journal={International Journal of
Epidemiology},
volume={28},
pages={1019Ð1022},
year={1999}
}

@article{Berkmanetal00,
author={L.F. Berkman and T. Glass and I. Brissette and T.E. Seeman},
title={From social integration to health: Durkheim
in the new millennium},
journal={Social Science \& Medicine},
volume={51},
pages={843Ð857},
year={2000}
}

@article{Krieger01,
author={N. Krieger},
title={Theories for social epidemiology in the 21st
century: An ecosocial perspective},
journal={International Journal of
Epidemiology},
volume={30},
pages={668Ð677},
year={2001}
}

@book{Parsons51,
author={T. Parsons},
title={The social system},
publisher={New York: Free Press},
year={1951}
}

@book{Starr82,
author={P. Starr},
title={The social transformation of American medicine},
publisher={New York: Basic Books},
year={1982}
}

@article{Rose85,
author={G. Rose},
title={Sick individuals and sick populations},
journal={International Journal of Epidemiology},
volume={14},
pages={32Ð38},
year={1985}
}

@article{Clarketal91,
author={J. Clark and D.A. Potter and J.B. McKinlay},
title={Bringing
social structure back into clinical decision making},
journal={Social
Science \& Medicine},
volume={32},
pages={853Ð866},
year={1991}
}

@article{Barr95,
author={D.A. Barr},
title={The effects of organizational structure on
primary care outcomes under managed care},
journal={Annals of
Internal Medicine},
volume={122},
pages={353Ð359},
year={1995}
}


@article{McKinlay96,
author={J.B. McKinlay},
title={Some contributions from the social
system to gender inequalities in heart disease},
journal={Journal of
Health and Social Behavior},
volume={37},
pages={1Ð26},
year={1996}
}



@article{Feldmanetal97,
author={H.A. Feldman and J. B. McKinlay and D.A. Potter and K.M. Freund and
R.B. Burns and M.A. Moskowitz and L.E. Kasten},
title={Nonmedical inßuences on medical decision making: An
experimental technique using videotapes, factorial
design, and survey sampling},
journal={Health Services Research},
volume={32},
pages={343Ð366},
year={1997}
}

@article{Hook01,
author={E.B. Hook},
title={(Letter to Editor) RE: Neighborhood social
environment and risk of death: Multilevel evidence from the
Alameda County Study},
journal={American Journal of Epidemiology},
volume={151},
pages={1132Ð1133},
year={2001}
}

@article{Draper95,
author={D. Draper},
title={Inference and hierarchical modeling in the
social sciences},
journal={Journal of Educational and Behavioral
Statistics},
volume={20},
pages={115Ð147},
year={1995}
}

@article{Lindley&Smith72,
author={D. Lindley and A. Smith},
title={Bayes estimation for linear
models},
journal={Journal of the Royal Statistical Society, Series B},
volume={34},
pages={1Ð41},
year={1972}
}


@article{Dempsteretal77,
author={A.P. Dempster and N.M. Laird and D.B. Rubin},
title={Maximum
likelihood from incomplete data via the EM algorithm},
journal={Journal of the Royal Statistical Society, Series B},
volume={39},
pages={1Ð8},
year={1977}
}

@article{Laird&Ware82,
author={
N.M. Laird and J.H. Ware},
title={Random-effects models for
longitudinal data},
journal={Biometrics},
volume={38},
pages={963Ð974},
year={1982}
}


@inCollection{Masonetal84,
author={W.M. Mason and G.Y. Wong and B. Entwisle},
title={Contextual
analysis through the multilevel Linear Model. In S.
Leinhardt (Ed.)},
booktitle={Sociological methodology: 1983Ð1984},
publisher={San
Francisco: Jossey-Bass},
year={1984}
}




@book{Goldstein87,
author={H. Goldstein},
title={Multilevel statistical models in educational
and social research},
publisher={London: Edward Arnold},
year={1987}
}



@book{Bryk&Raudenbush92,
author={A.S. Bryk and S.W. Raudenbush},
title= {Hierarchical linear
models},
publisher={Newbury Park: Sage},
year={1992}
}


@book{Verbeke&Molenbergs97,
author={G. Verbeke and G. Molenbergs},
title={Linear mixed models in practice: A SAS oriented approach},
publisher={New York: Springer},
year={1997}
}



@article{Singer98,
author={J.D. Singer},
title={Using SAS proc mixed to Þt multilevel
models, hierarchical models, and individual growth models},
journal={Journal of Educational and Behavioral Statistics},
volume={24},
pages={323Ð355},
year={1998}
}


@article{Kreftetal94,
author={I.G.G. Kreft and J. de Leeuw and R. van der Leeden},
title={Review of Þve multilevel analysis programs: BMDP-5,
GENMOD, HLM, ML3, VARCL. },
journal={American Statistician},
volume={48},
pages={324Ð335},
year={1994}
}

@inCollection{Deleeuw&Kreft01,
author={J. De Leeuw and I.G.G. Kreft},
title={Software for multilevel
analysis},
booktitle={In H. Goldstein (Ed.), Multilevel modelling of
health statistics},
pages={187Ð204},
publisher={New York: Wiley},
year={2001}
}


@book{Susser73,
author={M. Susser},
title={Causal thinking in health sciences: Concepts
and strategies of epidemiology},
publisher={New York: Oxford},
year={1973}
}

@inCollection{Freedman91,
author={D. Freedman},
title={Statistical models and shoe leather (with
discussion). In P. V. Marsden (Ed.)},
booktitle={Sociological methodol-
ogy},
OPTvol={21},
publisher={San Francisco: Jossey-Banks},
year={1991}
}

@article{Freedman97,
author={D. Freedman},
title={From association to causation via
regression (with comments). In S. P. Turner (Ed.)},
booktitle={Causality in crisis? Statistical methods and the search for causal
knowledge in the social sciences},
OPTpages={113Ð182},
publisher={Notre Dame,
IN: Notre Dame University Press},
year={1997}
}


@article{Greenland90,
author={S. Greenland},
title={Randomization, statistics, and causal
inference},
journal={Epidemiology},
volume={1},
pages={421Ð429},
year={1990}
}


@article{Greenland96,
author={S. Greenland},
title={Basic methods for sensitivity analysis of
biases},
journal={International Journal of Epidemiology},
volume={25},
pages={1107Ð1116},
year={1996}
}

@article{Greenland00,
author={S. Greenland},
title={Principles of multilevel modelling},
journal={International Journal of Epidemiology},
volume={29},
pages={158Ð167},
year={2000}
}

@article{Greenland01,
author={S. Greenland},
title={Ecologic versus individual-level sources of
bias in ecologic estimates of contextual health effects},
journal={International Journal of Epidemiology},
volume={30},
pages={1343Ð1350},
year={2001}
}

@article{Greenland02,
author={S. Greenland},
title={A review of multilevel theory for
ecological analyses},
journal={Statistics in Medicine},
volume={21},
pages={389Ð395},
year={2002}
}

@article{Greenland&Morgenstern01,
author={S. Greenland and H. Morgenstern},
title={Confounding in
health research},
journal={Annual Review of Public Health},
volume={22},
pages={189Ð212},
year={2001}
}

@article{Greenlandetal99,
author={S. Greenland and J. Pearl and J.M. Robins},
title= {Causal
diagrams for epidemiologic research},
journal={Epidemiology},
volume={10},
pages={37Ð48},
year={1999}
}


@article{Manski93,
author={C.F. Manski},
title={IdentiÞcation of endogenous social
effects: The reßection problem},
journal={Review of Economic Studies},
volume={60},
pages={531Ð542},
year={1993}
}


@inCollection{Manski93b,
author={C.F. Manski},
title={IdentiÞcation problems in the social
sciences. In P. V. Marsden (Ed.)},
booktitle={Sociological methodology},
publisher={San Francisco: Jossey-Banks},
year={1993}
}


@article{Halloran&Struchiner95,
author={M.E. Halloran and C.J. Struchiner},
title={Causal inference in
infectious diseases},
journal={Epidemiology},
volume={6},
pages={142Ð151},
year={1995}
}

@article{Morgenstern95,
author={H. Morgenstern},
title={Ecologic studies in epidemiology:
Concepts, principles, and methods},
journal={Annual Review of Public
Health},
volume={16},
pages={61Ð81},
year={1995}
}

@inCollection{Sobel95,
author={M.E.Sobel},
title={Causal inference in the social and
behavioral sciences},
booktitle={In M. E. Sobel (Ed.), Handbook of
statistical modeling for the social and behavioral sciences},
pages={1Ð38},
publisher={New York: Plenum.},
year={1995}
}


@article{Kaufman&Cooper99,
author={J.S. Kaufman and R.S. Cooper},
title={Seeking causal
explanations in social epidemiology},
journal={American Journal of
Epidemiology},
volume={150},
pages={113Ð120},
year={1995}
}

@article{Kaufman&Poole00,
author={J.S. Kaufman and C. Poole},
title={Looking back on causal
thinking in the health sciences},
journal={Annual Review of Public
Health},
volume={21},
pages={101Ð119},
year={2000}
}

@article{Kaufman&Kaufman01,
author={J. S. Kaufman and S. Kaufman},
title={Assessment of
structured socioeconomic effects on health},
journal={Epidemiology},
volume={12},
pages={157Ð167},
year={2001}
}

@article{Robins01,
author={J.M. Robins},
title={Data, design, and background knowledge
in etiologic inference},
journal={Epidemiology},
volume={12},
pages={313Ð320},
year={2001}
}


@article{Maldonado&Greenland02,
author={G. Maldonado and S. Greenland},
title={Estimating causal effects},
journal={International Journal of Epidemiology},
volume={31},
pages={422Ð438},
year={2002}
}

@book{Campbell&Stanley63,
author={D.T. Campbell and J.C. Stanley},
title={Experimental and
quasi-experimental designs for research},
publisher={Hopewell, NJ:
Houghton Mifßin},
year={1963}
}

@article{Cochran65,
author={W.G. Cochran},
title={The planning of observational studies
of human populations},
journal={Journal of the Royal Statistical
Society, Series A},
volume={128},
pages={243Ð265},
year={1965}
}

@article{McKinlay75,
author={S.M. McKinlay},
title={The design and analysis of the
observational studyÑa review},
journal={Journal of the American
Statistical Association},
volume={70},
pages={503Ð523},
year={1975}
}

@article{Heckman79,
author={J.J. Heckman},
title={Sample selection bias as a speciÞcation
error},
journal={Econometrica},
volume={47},
pages={153Ð162},
year={1979}
}


@article{Leamer83,
author={E. Leamer},
title={LetÕs take the con out of econometrics},
journal={American Economic Review},
volume={73},
pages={32Ð43},
year={1983}
}

@inCollection{Smith90,
author={H.L. Smith},
title={SpeciÞcation problems in experimental and
nonexperimental social research},
booktitle={In C. C. Clogg (Ed.), Sociological methodology},
volume={20},
publisher={Oxford: Basil},
year={1990}
}

@article{Rubin91,
author={D.B. Rubin},
title={Practical implications of modes of
statistical inference for causal effects and the critical role
of the assignment mechanism},
journal={Biometrics},
volume={47},
pages={1213Ð1234},
year={1991}
}

@inCollection{Clogg&Haritou97,
author={C.C. Clogg and A. Haritou},
title={The regression method for causal inference and a dilemma confronting this method},
booktitle={In S. P. Turner (Ed.), Causality in crisis? Statistical methods
and the search for causal knowledge in the social sciences},
pages={83Ð112},
publisher={Notre Dame, IN: Notre Dame University Press},
year={1997}
}

@article{Copas&Li97,
author={J.B. Copas and H.G. Li},
title={Inference for non-random
samples (with discussion)},
journal={Journal of the Royal Statistical
Society, Series B},
volume={59},
pages={55Ð95},
year={1997}
}

@inCollection{Freedman97,
author={D. Freedman},
title={From association to causation via
regression (with comments)},
booktitle={In S. P. Turner (Ed.), Causality
in crisis? Statistical methods and the search for causal
knowledge in the social sciences},
pages={113Ð182},
publisher={Notre Dame,
IN: Notre Dame University Press},
year={1997}
}

@article{Winship&Morgan99,
author={C. Winship and S.L.  Morgan},
title={The estimation of causal
effects from observational data},
journal={Annual Review of Sociology},
volume={25},
pages={659Ð707},
year={1999}
}

@book{Pearl00,
author={J. Pearl},
title={Causality: Models, reasoning, and inference},
publisher={ New York: Cambridge University Press},
year={2000}
}

@book{Rosenbaum02,
author={P.R. Rosenbaum},
title={Observational studies},
publisher={New York:
Springer},
year={2002}
}


@article{Charltonetal85,
author={J.R. Charlton and M.F. DÕSouza and M. Tooley and R. Silver},
title={A community trial strategy for evaluating treatment
for symptomatic conditions},
journal={Statistics in Medicine},
volume={4},
pages={11Ð21},
year={1985}
}

@article{Meyeretal91,
author={L. Meyer and N. Job-Spira and J. Bouyer and E. Bouvet and A. Spira},
title={Prevention of sexually transmitted diseases: A
randomised community trial},
journal={Journal of Epidemiology and
Community Health},
volume={45},
pages={152Ð158},
year={1991}
}


@article{Shipleyetal95,
author={R.H. Shipley and T.D. Hartwell and W.D. Austin and A.C. Clayton and L.C. Stanley },
title={Community stop-smoking contests
in the COMMIT trial: Relationship of participation to
costs},
journal={Community intervention trials. Preventive Medicine},
volume={ 24},
pages={286Ð292},
year={1995}
}

@article{Holderetal97,
author={H.D. Holder and R.F. Saltz and A.J. Treno and J.W. Grube and R.B. Voas},
title={Evaluation design for a community prevention
trial. An environmental approach to reduce alcohol-
involved trauma},
journal={Evaluation Review},
volume={21},
pages={140Ð165},
year={1997}
}

@article{Feldmanetal98,
author={H.A. Feldman and M.A. Proschan and D.M. Murray and D.C. Goff and M.
Stylianou and E. Dulberg and P.G. McGovern and W. Chan and N.C.
Mann and V. Bittner},
title={Statistical design of
REACT (Rapid Early Action for Coronary Treatment), a
multisite community trial with continual data collection},
journal={Controlled Clinicial Trials},
volume={19},
pages={391Ð403},
year={1998}
}

@article{LeFortetal98,
author={S.M. LeFort and K. Gray-Donald and K.M. Rowat and M.E. Jeans},
title={Randomized controlled trial of a community-based
psychoeducation program for the self-management of
chronic pain},
journal={Pain},
volume={74},
pages={297Ð306},
year={1998}
}


@article{Perskyetal99,
author={V. Persky and L. Coover and E. Hernandez and A. Contreras and J. Slezak and J. Piorkowski and L. Curtis and M. Turyk and V. Ramakrishnan and  P. Scheff},
title={Chicago community-based asthma
intervention trial: Feasibility of delivering peer education in
an inner-city population},
journal={Chest},
volume={116},
pages={216SÐ223S},
year={1999}
}

@article{Biglanetal00,
author={A. Biglan and K. Smolkowski and T. Duncan and C. Black},
title={A randomised controlled trial of a community
intervention to prevent adolescent tobacco use},
journal={Tobacco
Control},
volume={9},
pages={24Ð32},
year={2000}
}


@article{Luepkeretal00,
author={R.V. Luepker and J.M. Raczynski and S. Osganian and R.J Goldberg and
Jr. J.R.  Finnegan and J.R. Hedges and Jr. D.C. Goff and M.S.
Eisenberg and J.G. Zapka and H.A. Feldman and D.R. Labarthe and P.G. McGovern and C.E. Cornell and M.A. Proschan and D.G. Simons-Morton},
title={Effect of a community
intervention on patient delay and emergency medical service
use in acute coronary heart disease: The rapid early action
for coronary treatment (REACT) trial},
journal={JAMA},
volume={284},
pages={60Ð67},
year={2000}
}


@Article{Oakes04,
  author = {J.M. Oakes},
  title= {The (mis)estimation of neigborhood effects: causal inference for a practicable social epidemiology },
  journal = {Social Science and Medicine},
  volume = {58},
  issue = {},
  pages = {1929--1952},
  year = {2004}
}

@Article{Abadie&Imbens06,
  author = {A. Abadie and G.W. Imbens},
  title= {Large Sample Properties of Matching Estimators for Average Treatment Effects},
  journal = {Econometrica},
  volume = {74},
  issue = {1},
  pages = {235-67},
  year = {2006}
}

@Article{Greenland&Morgenstern90,
  author = {S. Greenland and H. Morgenstern},
  title= {Matching and Efficiency in Cohort Studies},
  journal = {American Journal of Epidemiology},
  volume = {131},
  issue = {1},
  pages = {151-159},
  year = {1990}
}

@Article{Costanza95,
  author = {M. Costanza},
  title= {Theoretical Epidemiology, Matching},
  journal = {Preventive Medicine},
  volume = {24},
  issue = {},
  pages = {425-433},
  year = {1995}
}

@Article{Joffe&Rosenbaum99,
  author = {M.M. Joffe and P.R. Rosenbaum},
  title= {Invited Commentary: Propensity Scores},
  journal = {American Journal of Epidemiology},
  volume = {150},
  issue = {4},
  pages = {327-333},
  year = {1999}
}


@article{Neugebauer&vanderLaan07,
author={R. Neugebauer, M. J. van der Laan},
title={ Nonparametric Causal E?ects based on
marginal structural models},
journal={Journal of Statistical Planning and Inference},
year={2007},
volume={137},
pages={419Ð434},
}




@article{Murphy05,
author={S. Murphy},
title={An experimental design for the development of adaptive treatment strategies},
journal={Statistics in Medicine},
year={2005},
volume={24},
pages={1455Ð1481},
}

@article{Lavori&Dawson00,
author={P. Lavori and R. Dawson},
title={A design for testing clinical strategies: biased adaptive within-subject
randomization},
journal={Journal of the Royal Statistical Society, Series A},
volume={163},
pages={29Ð38},
year={2000},
}

@article{Lavori&Dawson04,
author={P. Lavori  and R. Dawson},
title={Dynamic treatment regimes: practical design considerations},
journal={Clinical trials},
volume={1},
pages={9Ð20},
year={2004},
}

@article{Thalletal00,
author={P. Thall and R. Millikan and H.-G. Sung},
title={Evaluating multiple treatment courses in clinical trials},
journal={Statistics in Medicine},
volume={19},
pages={1011Ð1028},
year={2000},
}

@article{Rushetal03,
author={A.J. Rush and M. Trivedi and M. Fava},
title={Depression},
journal={IV. American Journal of Psychiatry},
volume={160(2)},
pages={237},
year={2003},
}

@article{Schneideretal06,
author={Schneider, L. and Tariot.P.N. and Dagerman, K. and Davis, S. and Hsiao, J. and Ismail, S. and Lebowitz, B. and Lyketsos, C. and Ryan
J. and Stroup T. and Sultzer D. and Weintraub, D. and Lieberman, J.},
title= {E?ectiveness of atypical antipsychotic
drugs in patients with AlzheimerÕs disease},
journal={New England Journal of Medicine},
volume={355(15)},
pages={1525Ð1538},
year={2006},
}

@article{Swartzetal07,
author={Swartz, M. and Perkins, D. and Stroup, T. and Davis, S. and Capuano, G. and Rosenheck, R. and Reimherr, F. and McGee, M. and Keefe,
R. and McEvoy, J. and Hsiao, J. and Lieberman, J.},
title={Effects of antipsychotic medications on psychosocial
functioning in patients with chronic shizophrenia: Findings from the nimh catie study},
year={2007},
journal={American Journal
of Psychiatry},
volume={164},
pages={428Ð436},
}

@article{Rubin&vanderLaan08,
author={D.B. Rubin and M.J. van der Laan},
title={Empirical Efficiency Maximization: Improved Locally Efficient Covariate Adjustment in Randomized Experiments and Survival Analysis},
year={2008},
journal={The International Journal of Biostatistics},
volume={Vol. 4, Iss. 1, Article 5},
location={http://www.bepress.com/ijb/vol4/iss1/5},
}


@article{vanderLaan&Rose&Gruber09,
author={M.J. van der Laan and S. Rose and S. Gruber},
title={Readings on Targeted Maximum Likelihood Estimation},
year={September, 2009},
journal={Technical report, working paper series http://www.bepress.com/ucbbiostat/paper254/},
}

@article{Bembometal09,
author={O. Bembom and M.J. van der Laan and T. Haight and I.B. Tager},
title={Lifetime and
current leisure time physical activity and all-cause mortality in an elderly cohort},
year={2009},
journal={Epidemiology},
volume={},
pages={},
}

@article{Bembom&vanderLaan07a,
author={Oliver Bembom and Mark van der Laan},
title={Statistical Methods for analyzing sequentially randomized trials, commentary on JNCI article Adaptive therapy for androgen independent prostate cancer: A Randomized selection trial including four regimens, by Peter F. Thall, C. Logothetis, C. Pagliaro, S. Wen, M.A. Brown, D. Williams, R. Millikan (2007). },
journal={Journal of the National Cancer Institute},
year={2007},
volume={99(21)},
pages={1577-1582},
 }

@article{Rosenblumetal09,
author={M. Rosenblum and S.G. Deeks and M.J. van der Laan and D.R. Bangsberg},
title={The Risk
of Virologic Failure Decreases with Duration of HIV Suppression, at Greater
than 50\% Adherence to Antiretroviral Therapy},
year={2009},
journal={PLoS ONE},
volume={4(9): e7196.doi:10.1371/journal.pone.0007196},
}



@article{Robinsetal08,
author={J. Robins and L. Orallana and A. Rotnitzky},
title={Estimaton and extrapolation of optimal treatment and  testing strategies},
journal={Statistics in Medicine},
year={2008},
volume={27(23)},
pages={ 4678-4721},
}


@article{Bembom&vanderLaan07,
author= {O. Bembom and M.J. van der Laan},
title={A practical illustration of the importance of realistic individualized treatment rules in causal inference},
journal={Electronic Journal of Statistics},
year={2007},
pages={http://www.i-journals.org/ejs/viewarticle.php?id=105&layout=abstract},
}

@article{Bembometal08,
author={O. Bembom and M.L. Petersen and S.-Y. Rhee and W. J. Fessel and S.E. Sinisi and R.W. Shafer and M.J. van der Laan},
title ={Biomarker discovery using targeted maximum likelihood estimation: Application to the treatment of antiretroviral resistant HIV infection},
journal={Statistics in Medicine},
year={2008},
pages={http://www3.interscience.wiley.com/journal/121422393/abstract},
}

@article{Cassel76,
author={J. Cassel},
title={The contribution of the social environment to host resistance},
journal={American Journal of Epidemiology},
volume={104},
pages={107--123},
year={1976}
}

@article{Tuglus&vanderLaan08,
author={C. Tuglus and M.J. van der Laan},
title={Targeted Methods for Biomarker Discovery, the Search for a Standard},
journal={UC Berkeley Working Paper Series},
year={2008},
pages={http://www.bepress.com/ucbbiostat/paper233/.},
}

@article{vanderLaan08,
author={M.J. van der Laan},
title={Estimation Based on Case-Control Designs with Known Prevalance Probability},
journal={The International Journal of Biostatistics},
year={2008},
pages={http://www.bepress.com/ijb/vol4/iss1/17/},
}

@article{Rose&vanderLaan08,
author={S. Rose and M.J. van der Laan},
title={Simple Optimal Weighting of Cases and Controls in Case-Control Studies},
journal={The International Journal of Biostatistics},
year={2008},
pages={http://www.bepress.com/ijb/vol4/iss1/19/.},
}

@article{Rose&vanderLaan09,
author={S. Rose and M.J. van der Laan},
title={Why Match? Investigating Matched Case-Control Study Designs with Causal Effect Estimation},
journal={The International Journal of Biostatistics},
year={2009},
pages={http://www.bepress.com/ijb/vol5/iss1/1/.},
}


@inproceedings{Moore&vanderLaan09,
author={K.L. Moore and M.J. van der Laan},
title={Application of Time-to-Event Methods in the Assessment of Safety in Clinical Trials},
booktitle={in Design, Summarization, Analysis \& Interpretation of Clinical Trials with Time-to-Event Endpoints},
year={2009},
editor={Karl E. Peace},
publisher={Chapman and Hall},
}

@inproceedings{Polley&vanderLaan09,
author={E.C. Polley and M.J. van der Laan},
title={Predicting Optimal Treatment Assignment Based on Prognostic Factors in Cancer Patients},
booktitle={in Design, Summarization, Analysis \& Interpretation of Clinical Trials with Time-to-Event Endpoints},
year={2009},
editor={Karl E. Peace},
publisher={Chapman and Hall},
}


@article{vanderVaart&Dudoit&vanderLaan06,
  author =       {A.W. van der Vaart and S. Dudoit and M.J. van der Laan},
  title =        {Oracle Inequalities for Multi-Fold Cross-Validation},
   journal = {Statistics and Decisions},
   volume={24},
 number={3},
 year={2006},
 pages={351--371},
}

@article{vanderLaan&Dudoit&vanderVaart06,
  author =       {M.J. van der Laan and S. Dudoit and A.W. van der Vaart},
  title =        {The Cross-Validated Adaptive Epsilon-Net Estimator},
   journal = {Statistics and Decisions},
   volume={24},
 number={3},
 year={2006},
 pages={373--395},
}

 @article{Rosenbaum&Rubin83,
 author={P.R. Rosenbaum and D.B. Rubin},
 title={The Central Role of the Propensity Score in Observational Studies for Causal Effects},
 journal={Biometrika},
 volume={70},
 year={1983},
 pages={41-55}
 }

@article{vanderLaan&Polley&Hubbard07,
 author = {M.J. van der Laan and E. Polley and A. Hubbard},
 title = {Super Learner},
 journal = {Statistical Applications in Genetics and Molecular Biology},
 volume = {6},
 number ={25},
 year = {2007},
 issn = {1},
 location={http://www.bepress.con/sagmb/vol6/iss1/art25},
 }

 @article{Sekhon08,
 author={J.S. Sekhon},
 title= {Multivariate and Propensity Score Matching
 Software with Automated Balance Optimization: The Matching package for {R}},
 journal = {Journal of Statistical Sotware, Forthcoming},
 publisher={SSRN},
location = {http://ssrn.com/paper=1009044},
year={2008}
}

@article{Bembom&Fessel&Shafer&vanderLaan08,
	location = {http://www.scientificcommons.org/36721107},
	title = {Data-adaptive Selection Of The Adjustment Set In Variable Importance Estimation},
	author = {O. Bembom and J.W. Fessel and R.W. Shafer  and M.J. van der Laan},
	year = {2008},
	keywords = {General Biostatistics},
	publisher = {The Berkeley Electronic Press},
	url = {http://www.bepress.com/ucbbiostat/paper231},
	institution = {DigitalCommons@Florida Atlantic University [http://digitalcommons.fau.edu/cgi/oai2.cgi] (United States)},
}

@article{Holland77,
 author = {J.H. Holland and J.S. Reitman},
 title = {Cognitive systems based on adaptive algorithms},
 journal = {SIGART Bull.},
 volume = {63},
 year = {1977},
 issn = {0163-5719},
 pages = {49--49},
 doi = {http://doi.acm.org/10.1145/1045343.1045373},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

@book{Rubin06,
author={D.B. Rubin},
title={Matched Sampling for Causal Effects.},
publisher={Cambridge University Press},
address={Cambridge, MA},
year={2006},
}

@incollection{Mans81,
author={C.F. Manski and D. McFadden},
title={Alternative estimators and sample designs for discrete choice analysis},
booktitle={Structural Analysis of Discrete Data with Econometric Applications},
publisher={The MIT Press},
address={Cambridge, MA},
year={1981},
editor={C.F. Manski and D. McFadden},
}

@article{Mans77,
author={C.F. Manski and S.R. Lerman},
title={The Estimation of Choice Probabilities from Choice Based Samples},
journal={Econometrica},
volume={45},
number={8},
pages={1977-1988},
year={1977},
}

@article{Coss81,
author={S.R. Cosslett},
title={Maximum Likelihood Estimator for Choice-Based Samples},
journal={Econometrica},
volume={49},
number={5},
pages={1289-1316},
year={1981},
}


@article{Corn51,
author={J. Cornfield},
title={A method of estimating comparative rates from clinical data.  Applications to cancer of the lung, breast, and cervix.},
journal={J Nat Cancer Inst},
volume={11},
pages={1269-1275},
year={1951},
}

@inproceedings{Corn56,
author={J. Cornfield},
title={A statistical problem arising from retrospective studies},
booktitle={Proceedings of the Third Berkeley Symposium, Volume IV},
year={1956},
editor={J. Neyman},
pages={133-148},
publisher={University of California Press},
}

@article{Beni94,
author={J. Benichou and S. Wacholder},
title={A comparison of three approaches to estimate exposure-specific incidence rates from population-based case-control data.},
journal={Statistics in Medicine},
volume={13},
pages={651-661},
year={1994},
}
@article{Breslow&Robins&Wellner00,
author={N.E. Breslow and J.M. Robins and J.A. Wellner},
title={On the semi-parametric efficiency of logistic regression under case-control sampling},
journal={Bernoulli},
volume={6(3)},
pages={447--455},
year={2000},
}
@article{Mansonetal07,
author = {R. Mansson, M.M. Joffe, W. Sun, S. Hennessy},
title = {On the Estimation and Use of Propensity Scores in Case-Control and Case-Cohort Studies.},
journal = {Am J Epidemiol},
volume = {166},
number = {3},
pages = {332-339},
year = {2007},
}

@article{And79,
author={J.A. Anderson},
title={Separate sample logistic discrimination},
journal={Biometrika},
volume={59},
pages={19--35},
year={1972},
}

@article{Prentice&Pike79,
author={R.L. Prentice and R. Pyke},
title={Logistic disease incidence models and case-control studies},
journal={Biometrika},
volume={66},
pages={403--411},
year={1979},
}

@article{Breslow96,
author={N.E. Breslow},
title={Statistics in Epidemiology: the Case-Control Study},
journal={J Am Stat Soc},
volume={91},
pages={14--28},
year={1996},
}

@book{Breslow&Day80,
author={N.E. Breslow and N.E. Day},
title={Statistical Methods in Cancer Research:  Volume 1 -- The analysis of case-control studies},
publisher={International Agency for Research on Cancer},
address={Lyon},
year={1980},
}

@article{Holfordetal78,
author={T.R. Holford and C. White and J.L. Kelsey},
title={Multivariate Analysis for Matched Case-Control Studies},
journal={Am J Epid},
volume={107},
number={3},
pages={245--255},
year={1978},
}

@article{Breslowetal78,
author={N.E. Breslow and N.E. Day and K.T. Halvorsen and R.L. Prentice and C. Sabal},
title={Estimation of Multiple Relative Risk Functions in Matched Case-Control Studies},
journal={Am J Epid},
volume={108},
number={4},
pages={299--307},
year={1978},
}

@book{Schlesselman82,
author={J.J. Schlesselman},
title={Case-Control Studies:  Design, Conduct, Analysis},
publisher={Oxford University Press},
address={Oxford},
year={1982},
}

@book{Collett91,
author={D. Collett},
title={Modeling Binary Data},
publisher={Chapman and Hall},
address={London},
year={1991},
}

@book{Jewell04,
author={N.P. Jewell},
title={Statistics for Epidemiology},
publisher={Chapman and Hall/CRC},
address={Boca Raton},
year={2004},
}

@book{Hosmer&Lemeshow00,
author={D.W. Hosmer and S. Lemeshow},
title={Applied Logistic Regression},
edition={2nd},
publisher={John Wiley and Sons},
address={New York},
year={2000},
}

@article{Robins99,
author={J.M. Robins},
title={[Choice as an Alternative to Control in Observational Studies]:  Comment},
journal={Statistical Science},
volume={14},
number={3},
pages={281--293},
year={1999},
}

@article{Newman06,
author={S. Newman},
title={Causal Analysis of Case-Control Data},
journal={Epid Persp Innov},
volume={3},
pages={2},
url={http://www.epi-perspectives.com/content/3/1/2},
year={2006},
}

@article{Zele86,
author={M. Zelen and R.A. Parker},
title={Case-Control Studies and Bayesian Inference},
journal={Stat Med},
volume={5},
number={3},
pages={261--269},
year={1986},
}

@article{Sinh04,
author={S. SInha and B. Mukherjee and M Ghosh},
title={Bayesian Semiparametric Modeling for Matched Case-Control Studies with Multiple Disease States},
journal={Biometrics},
volume={60},
pages={41--49},
year={2004},
}

@article{Ritc01,
author = {M.D. Ritchie and L.W. Hahn and N. Roodi and L.R. Bailey and W.D. Dupont and F.F. Parl and J.H. Moore},
title = {Multifactor-dimensionality reduction reveals high-order interactions among estrogen-metabolism genes in sporadic breast cancer.},
journal = {Am J Hum Genet},
volume = {69},
number = {1},
pages = {138--47},
year = {2001},
}

@article{Mei07,
author = {H. Mei and M.L. Cuccaro and E.R. Martin},
title = {Multifactor dimensionality reduction-phenomics: a novel method to capture genetic heterogeneity with use of phenotypic variables.},
journal = {Am J Hum Genet},
volume = {81},
number = {6},
pages = {1251-61},
year = {2007},
}




@article{
Bangsberg04,
   Author = {D.R. Bangsberg and A.R. Moss and S.G. Deeks},
   Title = {Paradoxes of adherence and drug resistance to {HIV} antiretroviral therapy},
   Journal = {J Antimicrob Chemother},
   Volume = {53},
   Number = {5},
   Pages = {696-9},
   Note = {0305-7453 (Print)
Journal Article
Review},
   Abstract = {Public health debates about providing HIV antiretroviral therapy to impoverished populations have centred on the relationship between adherence and risk of drug resistance. Recent data indicate that each antiretroviral therapeutic class has a unique adherence-resistance relationship. Resistance to single protease inhibitor therapy occurs most frequently at moderate to high levels of adherence, resistance to non-nucleoside reverse transcriptase inhibitor therapy occurs at low to moderate levels of adherence, and resistance to ritonavir-boosted protease inhibitor therapy is most likely to occur at middle ranges of adherence. These dynamic relationships should be considered in balancing the individual and public health benefits of therapy.},
 Keywords = {Anti-HIV Agents/*therapeutic use
Developing Countries
*Drug Resistance, Viral
Humans
*Patient Compliance
Public Health
Research Support, Non-U.S. Gov't
Research Support, U.S. Gov't, P.H.S.},
   Year = {2004} }


@Article{Scharfstein&Tsiatis&Robins97,
  author =   {D.O. Scharfstein and A.A. Tsiatis and J.M. Robins},
  title =    {Semiparametric efficiency and its implications on the design and analysis of group-sequential studies},
journal =      {Journal of the American Statistical Association},
  year =     {1997},
  OPTkey =   {},
  volume =   {92},
  number =   {440},
  pages =    {1342--1350},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Bembom&Petersen07,
   author={O. Bembom and M. Petersen and SY Rhee and W.J. Fessel and S.E. Sinisi and R.W. Shafer 	     and M.J. van der Laan},
   title={Biomarker Discovery Using Targeted Maximum Likelihood Estimation: Application to the  Treatment of Antiretroviral Resistant {HIV} Infection},
   journal= {U.C. Berkeley Division of Biostatistics Working Paper Series},
   year={2007},
  volume={221},
   OPTmonth={August},
  OPTnote={http://www.bepress.com/ucbbiostat/paper221}
}

@Article{vanderLaan&Gruber09,
  author=  {M.J. van der Laan and S. Gruber},
  title={Collaborative Double robust penalized targeted maximum likelihood estimation},
  journal={The International Journal of Biostatistics},
  year={2010},
  volume={},
 }
@Article{Gruber&vanderLaan09,
  author=  {S. Gruber and M.J. van der Laan},
  title={An application of collaborative targeted maximum likelihood estimation in causal inference and genomics},
  journal={The International Journal of Biostatistics},
  year={2010},
  volume={},
 }
@Article{vanderLaan&Rubin06,
  author =   {M.J. van der Laan and D. Rubin},
  title =    {Targeted Maximum Likelihood Learning},
journal =      {The International Journal of Biostatistics},
  year =     {2006},
  OPTkey =   {},
  volume =   {2},
  number =   {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/ijb/vol2/iss1/11},
  OPTannote =    {}
}


@Article{Scharfstein&Tsiatis98,
  author =   {D.O. Scharfstein and A.A. Tsiatis},
  title =    {The use of simulation and bootstrap in information based group sequential studies},
journal =      {Statistics in Medicine},
  year =     {1998},
  OPTkey =   {},
  volume =   {17},
  number =   {},
  pages =    {75--87},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Pampallona&Tsiatis&Kim01,
  author =   {S. Pampallona and A.A. Tsiatis and K. Kim},
  title =    {Interim monitoring of group sequential trials using spending functions for the type I and type II error probabilities},
journal =      {Drug Informational Journal},
  year =     {2001},
  OPTkey =   {},
  volume =   {35},
  number =   {},
  pages =    {1113-1121},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Tsiatis&Mehta03,
  author =   {A.A. Tsiatis and C. Mehta},
  title =    {On the inefficiency of the adaptive design for monitoring clinical trials},
journal =      {Biometrika},
  year =     {2003},
  OPTkey =   {},
  volume =   {90},
  number =   {},
  pages =    {367-378},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Banerjee&Tsiatis06,
  author =   {A. Banerjee and A.A. Tsiatis},
  title =    {Adaptive two-stage designs in phase II clinical trials},
journal =      {Statistics in Medicine},
  year =     {2006},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {In press},
  OPTannote =    {}
}
@Article{Tsiatis06,
  author =   {A.A. Tsiatis},
  title =    {Information based monitoring of clinical trials},
journal =      {Statistics in Medicine},
  year =     {2006},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {In press},
  OPTannote =    {}
}

@Article{Lokhnygina&Tsiatis06,
  author =   {Y. Lokhnygina and A.A. Tsiatis},
  title =    {Optimal two-stage group sequential designs},
journal =      {Journal of Statistical Planning and Inference},
  year =     {2006},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {},
  OPTnote =      {In press},
  OPTannote =    {}
}

  @Article{Bauer&Kohne94,
  author =   {P. Bauer and Kohne},
  title =    {Evaluation of experiments with adaptive interim analysis},
journal =      {Biometrics},
  year =     {1994},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {1029--1041},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Cui&Hung&Wang99,
  author =   {L. Cui and H.M.J. Wang and S-J Wang},
  title =    {Modification of sample size in group sequential trials},
journal =      {Biometrics},
  year =     {1999},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {853--857},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Jennison&Turnbull03,
  author =   {C. Jennison and B.W. Turnbull},
  title =    {Mid course sample size modification in clinical trials based on hte observed treatment effect},
journal =      {Statistics in Medicine},
  year =     {2003},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {971--993},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Koyama&Sampson&Gleser04,
  author =   {T. Koyama and A.R. Sampson and L.J. Gleser},
  title =    {A calculus for design of two stage adaptive procedures},
journal =      {Journal of the Americal Statistical Association},
  year =     {2004},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Lan&Trost97,
  author =   {K.K.G Lan and D.C. Trost},
  title =    {Estimation of parameters and sample size re-estimation},
journal =      {Proceedings Biopharm Section},
  year =     {1997},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {48-51},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Li&Shih&Xie&Lu02,
  author =   {G. Li and W.J. Shih and T. Xie and J. Lu},
  title =    {A sample size adjustment procedure for clinical trials based on conditional power},
journal =      {Biostatistics},
  year =     {2002},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {277--287},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Mehta&Tsiatis01,
  author =   {C.R. Mehta and A.A. Tsiatis},
  title =    {Flexible sample size considerations using information based interim monitoring},
journal =      {Drug Informational Journal},
  year =     {2001},
  OPTkey =   {},
  volume =   {35},
  number =   {},
  pages =    {1095--1112},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Mulle&Shafer01,
  author =   {H.H. Mulle and H. Shafer},
  title =    {Adaptive group sequential designs for clinical trials: combining the advantages of adaptive and classical group sequential approaches},
journal =      {Biometrics},
  year =     {2001},
  OPTkey =   {},
  volume =   {57},
  number =   {},
  pages =    {886--891},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Proschan&Hunsberger95,
  author =   {M.A. Proschan and S.A. Hunsberger},
  title =    {Designed extension studies based on conditional power},
journal =      {Biometrics},
  year =     {1995},
  OPTkey =   {},
  volume =   {51},
  number =   {},
  pages =    {1315--1324},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Shen&Fisher99,
  author =   {Y. Shen and L.D. Fisher},
  title =    {Statistical Inference for self-designing clinical trials with a one-sided hypothesis},
journal =      {Biometrics},
  year =     {1999},
  OPTkey =   {},
  volume =   {55},
  number =   {},
  pages =    {190--197},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Wittes&Brittain90,
  author =   {J. Wittes and E. Brittain},
  title =    {The role of internal pilot studies in increasing efficiency of clinical trials},
journal =      {Statistics in Medicine},
  year =     {1999},
  OPTkey =   {},
  volume =   {9},
  number =   {},
  pages =    {65--72},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Shen&Cheng06,
  author =   {Y. Shen and Y. Cheng},
  title =    {Adaptive design: Estimation and Inference with censored data in a semiparametric model},
journal =      {Biostatistics},
  year =     {2006},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {In Press},
  OPTannote =    {}
}

%next reference for adaptive allocation of treatments

@Book{Spiegelalteretal04,
  author =       {D.J. Spiegelalter and K.R. Abrams and J.P. Myles},
  title =        {Bayesian approaches to clinical trials and health care evaluation},
  publisher =    {Wiley, Chichester},
  year =         {2004}
}
@Book{Berry&Stangl96,
  author =       {D.A. Berry and D.K. Stangl},
  title =        {Bayesian biostatistics},
  publisher =    {Marcel Dekker, New York},
  year =         {1996}
}


@Article{Berry06,
  author =   {D.A. Berry},
  title =    {Bayesian clinical trials},
journal =      {Nature Reviews, Drug Discovery},
  year =     {2006},
  OPTkey =   {},
  volume =   {5},
  number =   {},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

%D. A. Berry, Bayesian clinical trials, Nature Reviews, Drug
%Recovery, vol 5, january 2006.


@Book{Hu&Rosenberger06,
  author =       {F. Hu and W.F. Rosenberger},
  title =        {The theory of response adaptive randomization in clinical trials},
  publisher =    {New York Wiley},
  year =         {2006}
}

@Book{Dudoit&vanderLaan08,
  author =       {S. Dudoit and M.J. van der Laan},
  title =        {Resampling based multiple testing with applications to genomics},
  publisher =    {Springer Series of Statistics, New York},
  year =         {2008}
}

@Book{Sen&Singer93,
  author =       {P.K. Sen and J.M. Singer},
  title =        {Large Sample Methods in Statistics: An Introduction with Applications},
  publisher =    {Chapman \& Hall, New York},
  year =         {1993}
}


@Article{Bai&Hu&Rosenberger02,
  author =   {Z.D. Bai and F. Hu and W.F. Rosenberger},
  title =    {Asymptotic properties of adaptive designs for clinical trials with delayed response},
journal =      {Annals of Statistics},
  year =     {2002},
  OPTkey =   {},
  volume =   {30},
  number =   {1},
  pages =    {122--139},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Andersen&Faries&Tamura94,
  author =   {J. Andersen and D. Faries and R. Tamura},
  title =    {A randomized play-the-winner design for multiarm clinical trials},
journal =      {Communication in Statistical Theory},
  year =     {1994},
  OPTkey =   {},
  volume =   {23},
  number =   {},
  pages =    {309--323},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Flournoy&Rosenberger95,
  author =       {N. Flournoy and W.F. Rosenberger},
  title =        {Adaptive Designs},
  publisher =    {Hayward, Institute of Mathematical Statistics},
  year =         {1995}
}

@Article{Hu&Rosenberger00,
  author =   {F. Hu and W.F. Rosenberger},
  title =    {Analysis of time trends in adaptive designs withi appliation to a neurophysiology experiment},
journal =      {Statistics in Medicine},
  year =     {2000},
  OPTkey =   {},
  volume =   {19},
  number =   {},
  pages =    {2067--2075},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Rosenberger96,
  author =   {W.F. Rosenberger},
  title =    {New directions in adaptive designs},
journal =      {Statistical Science},
  year =     {1996},
  OPTkey =   {},
  volume =   {11},
  number =   {},
  pages =    {137--149},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Rosenberger&Flournoy&Durham97,
  author =   {W.F. Rosenberger and N. Flournoy and S.D. Durham},
  title =    {Asymptotic normality of maximum likelihood estimators
  from multiparameter response driven designs},
journal =      {Journal of Statistical Planning and Inference},
  year =     {1997},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {69--76},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Rosenberger&Grill97,
  author =   {W.F. Rosenberger and S.E. Grill},
  title =    {A sequential design for psychophysical experiments: An application to estimating timing of sensory events},
journal =      {Statistics in Medicine},
  year =     {1997},
  OPTkey =   {},
  volume =   {16},
  number =   {},
  pages =    {2245--2260},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Rosenberger&Sriram97,
  author =   {W.F. Rosenberger and T.N. Shiram},
  title =    {Estimation for an adaptive allocation design},
journal =      {Journal of Statistical Planning and Inference},
  year =     {1997},
  OPTkey =   {},
  volume =   {59},
  number =   {},
  pages =    {309--319},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Tamura&Faries&Andersen&Heiligenstein94,
  author =   {R.N. Tamura and D.E. Faries and J.S. Andersen and J.H. Heiligenstein},
  title =    {A case study of an adaptive clinical trial in the treatment of out-patients with depressive disorder},
journal =      {Journal of the American Statistical Association},
  year =     {1994},
  OPTkey =   {},
  volume =   {89},
  number =   {},
  pages =    {768--776},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Wei&Durham78,
  author =   {L.J. Wei and S. Durham},
  title =    {The randomize play-the-winner rule in medical trials},
journal =      {Journal of the American Statistical Association},
  year =     {1978},
  OPTkey =   {},
  volume =   {73},
  number =   {},
  pages =    {840--843},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Wei&Smythe&Lin&Park90,
  author =   {L.J. Wei and R.T. Smythe and D.Y. Lin and T.S. Park},
  title =    {Statistical Inference with data-dependent treatment allocation rules},
journal =      {Journal of the American Statistical Association},
  year =     {1990},
  OPTkey =   {},
  volume =   {85},
  number =   {},
  pages =    {156--162},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Zelen69,
  author =   {M. Zelen},
  title =    {Play the winner rule and the controlled clinical trial},
journal =      {Journal of the American Statistical Association},
  year =     {1969},
  OPTkey =   {},
  volume =   {64},
  number =   {},
  pages =    {131--146},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Cheng&Shen05,
  author =   {Y. Cheng and Y. Shen},
  title =    {Bayesian adaptive designs for clinical trials},
journal =      {Biometrika},
  year =     {2005},
  OPTkey =   {},
  volume =   {92},
  number =   {3},
  pages =    {633--646},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Wei79,
  author =   {L.J. Wei},
  title =    {The generalized Polya's urn design for sequential medical trials},
journal =      {Annals of Statistics},
  year =     {1979},
  OPTkey =   {},
  volume =   {7},
  number =   {},
  pages =    {291--296},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}








@article{
Benito03,
   Author = {Benito, J. M. and Lopez, M. and Soriano, V.},
   Title = {Virus load and cytolitic responses in human immunodeficiency virus infection: what is cause and what is effect},
   Journal = {J Infect Dis},
   Volume = {188},
   Number = {5},
   Pages = {794-5; author reply 795-6},
   Note = {0022-1899
Comment
Letter},
 Keywords = {ADP-ribosyl Cyclase/metabolism
Anti-HIV Agents/therapeutic use
Antigens, CD/metabolism
CD4-Positive T-Lymphocytes/*immunology
CD8-Positive T-Lymphocytes/immunology
HIV Infections/drug therapy/*immunology/virology
HIV-1/*physiology
Human
*Viral Load
Virus Replication},
   Year = {2003} }



@article{
DEttorre02,
   Author = {D'Ettorre, G. and Forcina, G. and Andreotti, M. and Sarmati, L. and Palmisano, L. and Galluzzo, C. M. and Nicastri, E. and Mastroianni, C. M. and Vullo, V. and Vella, S. and Andreoni, M.},
   Title = {Discordant response to antiretroviral therapy: {HIV} isolation, genotypic mutations, T-cell proliferation and cytokine production},
   Journal = {Aids},
   Volume = {16},
   Number = {14},
   Pages = {1877-85},
   Note = {0269-9370
Journal Article},
   Abstract = {OBJECTIVE: To study virologic and immunologic factors associated with discordant treatment response in HIV-infected patients receiving highly active antiretroviral therapy (HAART). DESIGN: Study participants included a total of 27 patients: (a) 10 discordant patients (mean CD4+ cell count, 396.1 x 10 cells/l; mean HIV-RNA, 5.4 log copies/ml); (b) seven responder patients (mean CD4+ cell count, 997.5 x 10 cells/l); and (c) 10 failing patients (mean CD4+ cell count 66.5 x 10 cells/l; mean HIV-RNA, 5.4 log copies/ml).(10) (10)METHODS: The HIV-1 isolation rate and biological phenotype, drug resistance genotypic mutations of HIV-1 strains, recall and HIV-1-specific antigen lymphocyte proliferation (LP), and interleukin (IL)-15 production were studied. RESULTS: Virus isolation was obtained in 30% of discordant patients, and in 100% of failing patients. A higher replication constant was reported in discordant patients. No difference in the number of drug resistance mutations and biological phenotypes of HIV-1 was found in discordant patients with respect to failing patients. Discordant patients developed positive LP responses to and HIV-1 p24. LP in response to, HIV-1 p24 and gp160 was positive in responder patients. No significant LP was found in failing patients. Increased levels of IL-15 after stimulation with lipopolysaccaride (LPS) and were found in both discordant patients and responder patients. Conversely, a strong reduction of IL-15 levels was observed in failing patients. CONCLUSION: The present results suggest that decreased virus isolation rate, restoration of both lymphocyte proliferation and IL-15 production are factors involved in the discordant antiretroviral therapy response of HIV-infected patients.},
 Keywords = {Adult
Anti-HIV Agents/*therapeutic use
Antiretroviral Therapy, Highly Active
CD4 Lymphocyte Count
CD8-Positive T-Lymphocytes/drug effects/immunology
Candida albicans
Drug Resistance, Viral
Female
HIV Infections/complications/*drug therapy/immunology/virology
HIV-1/drug effects/genetics/*immunology/isolation & purification
Human
Interleukin-15/*blood
Male
Middle Aged
Mutation
Viral Load
Virus Replication/drug effects},
   Year = {2002} }



@article{
Davenport02,
   Author = {Davenport, M. P. and Zaunders, J. J. and Hazenberg, M. D. and Schuitemaker, H. and van Rij, R. P.},
   Title = {Cell turnover and cell tropism in HIV-1 infection},
   Journal = {Trends Microbiol},
   Volume = {10},
   Number = {6},
   Pages = {275-8},
   Note = {0966-842x
Journal Article},
   Abstract = {Early infection with HIV-1 is dominated by CCR5-tropic (R5, non-syncytium-inducing) viruses. The evolution of CXCR4-tropic (X4, syncytium-inducing) viruses occurs later in the infection and is associated with rapid disease progression. Here, we propose that the tropism of X4 viruses for naive CD4+ T cells is disadvantageous in early infection owing to the low division rate of these cells. In healthy individuals, the division rate of memory cells is nearly ten times higher than that of naive cells and thus the memory-cell tropism of R5 viruses could account for their dominance early in infection. As the division rate of naive T cells increases with CD4+ depletion, X4 viruses come to dominate in late disease.},
 Keywords = {CD4-Positive T-Lymphocytes/*virology
HIV Infections/*immunology/metabolism
HIV-1/*pathogenicity
Human
Immunologic Memory
Macrophages/*virology
Models, Biological
Receptors, CCR5/metabolism
Receptors, CXCR4/metabolism
Tropism},
   Year = {2002} }



@article{
Deeks00,
   Author = {Deeks, S. G. and Barbour, J. D. and Martin, J. N. and Swanson, M. S. and Grant, R. M.},
   Title = {Sustained CD4+ T cell response after virologic failure of protease inhibitor-based regimens in patients with human immunodeficiency virus infection},
   Journal = {J Infect Dis},
   Volume = {181},
   Number = {3},
   Pages = {946-53},
   Note = {0022-1899
Journal Article},
   Abstract = {The relationship between plasma human immunodeficiency virus (HIV) RNA levels and peripheral CD4+ T cell counts was examined in 380 HIV-infected adults receiving long-term protease inhibitor therapy. Patients experiencing virologic failure (persistent HIV RNA >500 copies RNA/mL) generally had CD4+ T cell counts that remained greater than pretherapy baseline levels, at least through 96 weeks of follow-up. The CD4+ T cell response was directly and independently related to degree of viral suppression below the pretreatment baseline. For any given HIV RNA level measured 12 weeks after virologic failure, subsequent CD4+ T cell decline was slower in patients receiving a protease inhibitor-based regimen than in a historical control group of untreated patients. These observations suggest that transient or partial declines in plasma HIV RNA levels can have sustained effects on CD4+ T cell levels.},
 Keywords = {Adult
*CD4 Lymphocyte Count
Female
HIV Infections/*drug therapy/immunology/virology
HIV Protease Inhibitors/*therapeutic use
Human
Male
RNA, Viral/*blood
Support, Non-U.S. Gov't
Support, U.S. Gov't, P.H.S.},
   Year = {2000} }



@article{
Deeks01,
   Author = {Deeks, S. G. and Wrin, T. and Liegler, T. and Hoh, R. and Hayden, M. and Barbour, J. D. and Hellmann, N. S. and Petropoulos, C. J. and McCune, J. M. and Hellerstein, M. K. and Grant, R. M.},
   Title = {Virologic and immunologic consequences of discontinuing combination antiretroviral-drug therapy in HIV-infected patients with detectable viremia},
   Journal = {N Engl J Med},
   Volume = {344},
   Number = {7},
   Pages = {472-80},
   Note = {0028-4793
Clinical Trial
Journal Article
Randomized Controlled Trial},
   Abstract = {BACKGROUND: In many patients with human immunodeficiency virus (HIV) infection, therapy with potent antiretroviral drugs does not result in complete suppression of HIV replication. The effect of cessation of therapy in these patients is unknown. METHODS: Sixteen patients who had a plasma HIV RNA level of more than 2500 copies per milliliter during combination antiretroviral-drug therapy were randomly assigned, in a 2:1 ratio, to discontinue or continue therapy. Plasma HIV RNA levels, CD4 cell counts, and drug susceptibility were measured weekly. Viral replicative capacity was measured at base line and at week 12. RESULTS: Discontinuation of therapy for 12 weeks was associated with a median decrease in the CD4 cell count of 128 cells per cubic millimeter and an increase in the plasma HIV RNA level of 0.84 log copies per milliliter. Virus from all patients with detectable resistance at entry became susceptible to HIV-protease inhibitors within 16 weeks after the discontinuation of therapy. Drug susceptibility began to increase a median of six weeks after the discontinuation of therapy and was temporally associated with increases in plasma HIV RNA levels and decreases in CD4 cell counts. Viral replicative capacity, measured by means of a recombinant-virus assay, was low at entry into the study and increased after therapy was discontinued. Despite the loss of detectable resistance in plasma, resistant virus was cultured from peripheral-blood mononuclear cells in five of nine patients who could be evaluated. Plasma HIV RNA levels, CD4 cell counts, and drug susceptibility remained stable in the patients who continued therapy. CONCLUSIONS: Despite the presence of reduced drug susceptibility, antiretroviral-drug therapy can provide immunologic and virologic benefit. This benefit reflects continued antiviral-drug activity and the maintenance of a viral population with a reduced replicative capacity.},
 Keywords = {Adult
Anti-HIV Agents/pharmacology/*therapeutic use
CD4 Lymphocyte Count
Drug Resistance, Microbial
Drug Therapy, Combination
HIV Infections/*drug therapy/immunology/virology
HIV Protease Inhibitors/pharmacology/*therapeutic use
HIV-1/*drug effects/genetics/isolation & purification
Human
Male
Middle Aged
Proportional Hazards Models
Prospective Studies
RNA, Viral/blood
Support, Non-U.S. Gov't
Support, U.S. Gov't, P.H.S.
Viremia/drug therapy},
   Year = {2001} }



@article{
Deeks01b,
   Author = {Deeks, S. G.},
   Title = {International perspectives on antiretroviral resistance. Nonnucleoside reverse transcriptase inhibitor resistance},
   Journal = {J Acquir Immune Defic Syndr},
   Volume = {26 Suppl 1},
   Pages = {S25-33},
   Note = {1525-4135
Journal Article
Review
Review, Tutorial},
   Abstract = {Although understanding of nonnucleoside reverse transcriptase inhibitor (NNRTI) resistance is less clearly established than that of other classes of antiretroviral drugs, certain facts have been established. The treatment-associated genetic mutation profiles of the available NNRTIs have been mapped, and resistance has been found to develop rapidly after initiation of NNRTI therapy. Despite the chemical diversity of the NNRTIs, cross-resistance among agents of this class is nearly universal. Although the viral replicative capacity (``fitness") of NNRTI-induced viral variants has not been extensively studied, available data suggest that NNRTI-selected mutations confer little damage to viral fitness, and thus a single point mutation produces a strain that is both resistant and fit. Furthermore, with continued therapy, viral evolution persists, creating species with greater numbers of mutations and higher level phenotypic resistance. Taken together, these facts suggest that continued use of NNRTIs after emergence of resistance will produce variants of complex mutational patterns that limit future treatment options, and, therefore, strong consideration should be given to discontinuing NNRTIs after virologic failure is confirmed. This article describes the scientific literature establishing the efficacy and limitations of NNRTI therapy and attempts to define a role for this class of drug in the long-term treatment of HIV-1 disease.},
 Keywords = {Anti-HIV Agents/*pharmacology/therapeutic use
Clinical Trials
Delavirdine/pharmacology/therapeutic use
*Drug Resistance, Microbial
Drug Therapy, Combination
HIV Infections/drug therapy/transmission
HIV-1/*drug effects/genetics/metabolism
HIV-1 Reverse Transcriptase/chemistry/genetics
Human
Nevirapine/pharmacology/therapeutic use
Oxazines/pharmacology/therapeutic use
Phylogeny
Point Mutation/drug effects
Protein Conformation
Reverse Transcriptase Inhibitors/*pharmacology/therapeutic use
Virus Replication/drug effects},
   Year = {2001} }



@article{
Deeks02,
   Author = {Deeks, S. G. and Barbour, J. D. and Grant, R. M. and Martin, J. N.},
   Title = {Duration and predictors of CD4 T-cell gains in patients who continue combination therapy despite detectable plasma viremia},
   Journal = {Aids},
   Volume = {16},
   Number = {2},
   Pages = {201-7},
   Note = {0269-9370
Journal Article},
   Abstract = {BACKGROUND: Sustained elevations in CD4 cell counts commonly occur despite incomplete viral suppression with protease inhibitor-based antiretroviral therapy. OBJECTIVES: To determine the incidence and risk factors associated with return of CD4 cell count to pre-therapy levels in patients experiencing virologic failure of protease inhibitor therapy. DESIGN: This is a clinic-based cohort study of HIV-infected adults who failed to maintain durable viral suppression on a protease inhibitor-based regimen. MAIN OUTCOME MEASURES: Virologic failure was defined as persistent plasma HIV RNA level > 500 copies/ml. Immunologic failure was defined as return of CD4 cell count to pre-therapy levels. RESULTS: A total of 291 patients experienced virologic failure on a protease inhibitor-based regimen and had a treatment-mediated CD4 cell increase above pre-therapy levels at the time of virologic failure. If patient data were censored at the time a successful salvage regimen was initiated, then the median time to immunologic failure after the onset of virologic failure was 3 years. If patient data were also censored at the time therapy was discontinued, then 36.8% of the cohort experienced immunologic failure after 3 years of continuous virologic failure. The change in viral load from a pre-treatment baseline, and not the absolute level of viremia achieved, was a strong and independent predictor of immunologic failure. Discontinuing therapy was associated with immunologic failure independent of viral load changes. CONCLUSION: Reduction in T CD4+ cell numbers may eventually occur during prolonged virologic failure of a protease inhibitor-based regimen and is predicted by the degree of virologic suppression below a pre-therapy 'set-point'.},
 Keywords = {Adult
Antiretroviral Therapy, Highly Active
CD4 Lymphocyte Count
CD4-Positive T-Lymphocytes/cytology/*drug effects
Disease Progression
HIV Infections/blood/*drug therapy/immunology/virology
HIV Protease Inhibitors/*therapeutic use
HIV-1/*drug effects/genetics
Human
Indinavir/therapeutic use
Nelfinavir/therapeutic use
RNA, Viral/blood
Ritonavir/therapeutic use
Saquinavir/therapeutic use
Support, Non-U.S. Gov't
Support, U.S. Gov't, P.H.S.
Time Factors
Treatment Failure
Viremia/blood/*drug therapy/immunology/virology},
   Year = {2002} }



@article{
Deeks03,
   Author = {Deeks, S. G.},
   Title = {Treatment of antiretroviral-drug-resistant HIV-1 infection},
   Journal = {Lancet},
   Volume = {362},
   Number = {9400},
   Pages = {2002-11},
   Note = {1474-547x
Journal Article
Review
Review, Academic},
   Abstract = {Drug-resistant HIV-1 is a cause of growing clinical and public-health concern. In many patients, combination antiretroviral therapy fails to achieve complete viral suppression (virological failure). Continuing viral replication during therapy leads to the accumulation of drug-resistance mutations, resulting in increased viral load and a greater risk of disease progression. Patients with drug-resistant HIV-1 infection have three therapeutic options: a change to a salvage regimen with the aim of fully suppressing viral replication; interruption of therapy; or continuation of a partially effective regimen. The first strategy is preferred for most patients failing their first or perhaps their second regimen. However, the best approach remains unclear for patients who have failed multiple treatment regimens and who have limited options for complete viral suppression. The management of such patients requires a careful understanding of the pathogenesis of drug-resistant HIV-1, the clinical consequences of virological failure, the potential benefits and limitations of diagnostic assays, and the likelihood that agents in development will be effective.},
 Keywords = {Anti-HIV Agents/*immunology/*therapeutic use
Antiretroviral Therapy, Highly Active/methods
Drug Resistance, Viral/genetics/immunology
Drug Therapy, Combination
HIV Infections/*drug therapy/immunology/virology
HIV Protease Inhibitors/immunology/therapeutic use
*HIV-1/drug effects/genetics/immunology
Human
Randomized Controlled Trials
Ritonavir/immunology/therapeutic use
Support, Non-U.S. Gov't
Support, U.S. Gov't, P.H.S.
Treatment Outcome
Viral Load/statistics & numerical data
Virus Replication/drug effects/immunology},
   Year = {2003} }



@article{Deeks04,
   Author = {Deeks, S. G. and Walker, B. D.},
   Title = {The immune response to AIDS virus infection: good, bad, or both?},
   Journal = {J Clin Invest},
   Volume = {113},
   Number = {6},
   Pages = {808-10},
   Note = {0021-9738
Comment
Journal Article},
   Abstract = {A potent antigen-specific T cell response to HIV infection can contribute to the control of viral replication and is therefore beneficial to the host. However, HIV-mediated increases in generalized T cell activation also appear to accelerate both viral replication and CD4+ T cell depletion. A new study in the JCI attempts to experimentally distinguish the beneficial versus harmful aspects of this immune response.},
 Year = {2004} }

@techreport{
DHHS04,
   Author = {DHHS},
   Title = {Guidelines for the use of antiretroviral agents in HIV-1 infected adults and adolescents},
   Institution = {Panel on Clinical Practices for Treatment of HIV Infection, Department of Health and Human Services},
   Month= {March 23},
 Year = {2004} }



@article{
Faure00,
   Author = {Faure, S. and Meyer, L. and Costagliola, D. and Vaneensberghe, C. and Genin, E. and Autran, B. and Delfraissy, J. F. and McDermott, D. H. and Murphy, P. M. and Debre, P. and Theodorou, I. and Combadiere, C.},
   Title = {Rapid progression to AIDS in HIV+ individuals with a structural variant of the chemokine receptor CX3CR1},
   Journal = {Science},
   Volume = {287},
   Number = {5461},
   Pages = {2274-7},
   Note = {0036-8075
Comment
Journal Article},
   Abstract = {Human immunodeficiency virus (HIV) enters cells in vitro via CD4 and a coreceptor. Which of 15 known coreceptors are important in vivo is poorly defined but may be inferred from disease-modifying mutations, as for CCR5. Here two single nucleotide polymorphisms are described in Caucasians in CX3CR1, an HIV coreceptor and leukocyte chemotactic/adhesion receptor for the chemokine fractalkine. HIV-infected patients homozygous for CX3CR1-I249 M280, a variant haplotype affecting two amino acids (isoleucine-249 and methionine-280), progressed to AIDS more rapidly than those with other haplotypes. Functional CX3CR1 analysis showed that fractalkine binding is reduced among patients homozygous for this particular haplotype. Thus, CX3CR1-I249 M280 is a recessive genetic risk factor in HIV/AIDS.},
 Keywords = {Acquired Immunodeficiency Syndrome/genetics/*physiopathology/virology
Case-Control Studies
*Chemokines, CX3C
Chemokines, CXC/metabolism
Chromosomes, Human, Pair 3
Cohort Studies
Disease Progression
European Continental Ancestry Group/genetics
Genotype
HIV/physiology
HIV Infections/genetics/*physiopathology/virology
Haplotypes
Homozygote
Human
Leukocytes, Mononuclear/metabolism
Linkage Disequilibrium
Membrane Proteins/metabolism
Mutation
Polymorphism, Restriction Fragment Length
*Polymorphism, Single Nucleotide
Polymorphism, Single-Stranded Conformational
Receptors, Cytokine/*genetics/*physiology
Receptors, HIV/*genetics/*physiology
Support, Non-U.S. Gov't
Survival Analysis
Variation (Genetics)},
   Year = {2000} }



@article{
Gao01,
   Author = {Gao, X. and Nelson, G. W. and Karacki, P. and Martin, M. P. and Phair, J. and Kaslow, R. and Goedert, J. J. and Buchbinder, S. and Hoots, K. and Vlahov, D. and O'Brien, S. J. and Carrington, M.},
   Title = {Effect of a single amino acid change in MHC class I molecules on the rate of progression to AIDS},
   Journal = {N Engl J Med},
   Volume = {344},
   Number = {22},
   Pages = {1668-75},
   Note = {0028-4793
Journal Article
Multicenter Study},
   Abstract = {BACKGROUND: From studies of genetic polymorphisms and the rate of progression from human immunodeficiency virus type 1 (HIV-1) infection to the acquired immunodeficiency syndrome (AIDS), it appears that the strongest susceptibility is conferred by the major-histocompatibility-complex (MHC) class I type HLA-B*35,Cw*04 allele. However, cytotoxic T-lymphocyte responses have been observed against HIV-1 epitopes presented by HLA-B*3501, the most common HLA-B*35 subtype. We examined subtypes of HLA-B*35 in five cohorts and analyzed the relation of structural differences between HLA-B*35 subtypes to the risk of progression to AIDS. METHODS: Genotyping of HLA class I loci was performed for 850 patients who seroconverted and had known dates of HIV-1 infection. Survival analyses with respect to the rate of progression to AIDS were performed to identify the effects of closely related HLA-B*35 subtypes with different peptide-binding specificities. RESULTS: HLA-B*35 subtypes were divided into two groups according to peptide-binding specificity: the HLA-B*35-PY group, which consists primarily of HLA-B*3501 and binds epitopes with proline in position 2 and tyrosine in position 9; and the more broadly reactive HLA-B*35-Px group, which also binds epitopes with proline in position 2 but can bind several different amino acids (not including tyrosine) in position 9. The influence of HLA-B*35 in accelerating progression to AIDS was completely attributable to HLA-B*35-Px alleles, some of which differ from HLA-B*35-PY alleles by only one amino acid residue. CONCLUSIONS: This analysis shows that, in patients with HIV-1 infection, a single amino acid change in HLA molecules has a substantial effect on the rate of progression to AIDS. The different consequences of HLA-B*35-PY and HLA-B*35-Px in terms of disease progression highlight the importance of the epitope specificities of closely related class I molecules in the immune defense against HIV-1.},
 Keywords = {Acquired Immunodeficiency Syndrome/*genetics
African Continental Ancestry Group/genetics
Alleles
Amino Acid Sequence
Binding Sites/genetics
Disease Progression
Disease-Free Survival
European Continental Ancestry Group/genetics
*Genes, MHC Class I
Genotype
HIV Infections/ethnology/*genetics/immunology
HLA-B35 Antigen/chemistry/*genetics
HLA-C Antigens
Human
Peptides/metabolism
Proportional Hazards Models
Receptors, Peptide/chemistry/genetics/metabolism
Support, U.S. Gov't, P.H.S.},
   Year = {2001} }



@article{
Grabar00,
   Author = {Grabar, S. and Le Moing, V. and Goujard, C. and Leport, C. and Kazatchkine, M. D. and Costagliola, D. and Weiss, L.},
   Title = {Clinical outcome of patients with HIV-1 infection according to immunologic and virologic response after 6 months of highly active antiretroviral therapy},
   Journal = {Ann Intern Med},
   Volume = {133},
   Number = {6},
   Pages = {401-10},
   Note = {0003-4819
Journal Article
Multicenter Study},
   Abstract = {BACKGROUND: The prognostic value of discordant immunologic (CD4 cell increase) and virologic (plasma HIV RNA level decrease) responses to antiretroviral treatment is not known. OBJECTIVE: To study the relation between clinical outcome of HIV-infected patients receiving highly active antiretroviral therapy (HAART) and early immunologic and virologic responses to such therapy. DESIGN: Prospective cohort study. SETTING: 68 hospitals in France. PATIENTS: 2236 protease inhibitor-naive patients. INTERVENTION: Initiation of HAART with one protease inhibitor and two nucleoside analogues between July 1996 and March 1997. MEASUREMENTS: Immunologic and virologic response at 6 months. Multivariate Cox models were used to assess the relation between these responses and progression to a new AIDS-defining event or death. RESULTS: On the basis of 6-month immunologic and virologic responses, patients were classified into four groups: complete response (47.5%), complete nonresponse (16.2%), immunologic response only (19.0%), and virologic response only (17.3%). After month 6 and within a median of 18 months, 69 patients died and 123 experienced a new AIDS-defining event. After adjustment, complete nonresponders and those with only a virologic response had significantly higher risks for clinical progression at 6 months (relative risk, 3.38 [95% CI, 2.28 to 5.02] and 1.98 [CI, 1.26 to 3.10], respectively) than complete responders. The difference between complete responders and those with only an immunologic response at 6 months was weaker and nonsignificant (relative risk, 1.55 [CI, 0.96 to 2.50]). CONCLUSIONS: Immunologic response after 6 months of HAART indicates a favorable clinical outcome in HIV-infected patients regardless of virologic response. This suggests that both immunologic and virologic markers should be used in clinical practice to evaluate treatment response.},
 Keywords = {Adult
CD4 Lymphocyte Count
Disease Progression
Drug Therapy, Combination
Female
HIV Infections/*drug therapy/immunology/virology
HIV Protease Inhibitors/*therapeutic use
*HIV-1/genetics
Human
Male
Multivariate Analysis
Proportional Hazards Models
Prospective Studies
RNA, Viral/blood
Reverse Transcriptase Inhibitors/*therapeutic use
Support, Non-U.S. Gov't
Treatment Outcome
Viral Load},
   Year = {2000} }



@article{
Grueb00,
   Author = {Greub, G. and Ledergerber, B. and Battegay, M. and Grob, P. and Perrin, L. and Furrer, H. and Burgisser, P. and Erb, P. and Boggian, K. and Piffaretti, J. C. and Hirschel, B. and Janin, P. and Francioli, P. and Flepp, M. and Telenti, A.},
   Title = {Clinical progression, survival, and immune recovery during antiretroviral therapy in patients with HIV-1 and hepatitis C virus coinfection: the Swiss HIV Cohort Study},
   Journal = {Lancet},
   Volume = {356},
   Number = {9244},
   Pages = {1800-5},
   Note = {0140-6736
Clinical Trial
Journal Article},
   Abstract = {BACKGROUND: Hepatitis C virus (HCV) infection is highly prevalent among HIV-1-infected individuals, but its contribution to the morbidity and mortality of coinfected patients who receive potent antiretroviral therapy is controversial. We used data from the ongoing Swiss HIV Cohort Study to analyse clinical progression of HIV-1, and the virological and immunological response to potent antiretroviral therapy in HIV-1-infected patients with or without concurrent HCV infection. METHODS: We analysed prospective data on survival, clinical disease progression, suppression of HIV-1 replication, CD4-cell recovery, and frequency of changes in antiretroviral therapy according to HCV status in 3111 patients starting potent antiretroviral therapy. RESULTS: 1157 patients (37.2%) were coinfected with HCV, 1015 of whom (87.7%) had a history of intravenous drug use. In multivariate Cox's regression, the probability of progression to a new AIDS-defining clinical event or to death was independently associated with HCV seropositivity (hazard ratio 1.7 [95% CI 1.26-2.30]), and with active intravenous drug use (1.38 [1.02-1.88]). Virological response to antiretroviral therapy and the probability of treatment change were not associated with HCV serostatus. In contrast, HCV seropositivity was associated with a smaller CD4-cell recovery (hazard ratio for a CD4-cell count increase of at least 50 cells/microL=0.79 [0.72-0.87]). INTERPRETATION: HCV and active intravenous drug use could be important factors in the morbidity and mortality among HIV-1-infected patients, possibly through impaired CD4-cell recovery in HCV seropositive patients receiving potent antiretroviral therapy. These findings are relevant for decisions about optimum timing for HCV treatment in the setting of HIV infection.},
 Keywords = {AIDS-Related Opportunistic Infections/*drug therapy
Adolescent
Adult
Anti-HIV Agents/*therapeutic use
CD4 Lymphocyte Count
Cohort Studies
Disease Progression
Female
Hepatitis C/complications/*drug therapy
Human
Male
Middle Aged
Prospective Studies
Support, Non-U.S. Gov't
Survival Analysis
Switzerland
Viral Load
Viremia/etiology},
   Year = {2000} }



@article{
Katzenstein96,
   Author = {Katzenstein, D. A. and Hammer, S. M. and Hughes, M. D. and Gundacker, H. and Jackson, J. B. and Fiscus, S. and Rasheed, S. and Elbeik, T. and Reichman, R. and Japour, A. and Merigan, T. C. and Hirsch, M. S.},
   Title = {The relation of virologic and immunologic markers to clinical outcomes after nucleoside therapy in HIV-infected adults with 200 to 500 CD4 cells per cubic millimeter. AIDS Clinical Trials Group Study 175 Virology Study Team},
   Journal = {N Engl J Med},
   Volume = {335},
   Number = {15},
   Pages = {1091-8},
   Note = {0028-4793
Clinical Trial
Journal Article
Multicenter Study
Randomized Controlled Trial},
   Abstract = {BACKGROUND: We studied measures of human immunodeficiency virus (HIV) replication, the viral phenotype, and immune function (CD4 cell counts) and the relation of changes in these indicators to clinical outcomes in a subgroup of patients in a controlled trial of early antiretroviral treatment for HIV, the AIDS Clinical Trials Group Study 175. METHODS: The 391 subjects, each of whom entered the study with a single screening CD4 cell count of 200 to 500 per cubic millimeter, were randomly assigned to receive zidovudine alone, didanosine alone, zidovudine plus didanosine, or zidovudine plus zalcitabine. Plasma concentrations of HIV RNA were assessed in 366 subjects, and viral isolates from 332 subjects were assayed for the presence of the syncytium-inducing phenotype. RESULTS: After eight weeks, the mean (+/-SE) decrease from base line in the concentration of HIV RNA, expressed as the change in the base 10 log of the number of copies per milliliter, was 0.26+/-0.06 for patients treated with zidovudine alone, 0.65+/-0.07 for didanosine alone, 0.93+/-0.10 for zidovudine plus didanosine, and 0.89+/-0.06 for zidovudine plus zalcitabine (P<0.001 for each of the pairwise comparisons with zidovudine alone). Multivariate proportional-hazards models showed that higher base-line concentrations of plasma HIV RNA, less suppression of plasma HIV RNA by treatment, and the presence of the syncytium-inducing phenotype were significantly associated with an increased risk of progression to the acquired immunodeficiency syndrome and death. After adjustment for these measures of viral replication and for the viral phenotype, CD4 cell counts were not significant predictors of clinical outcome. CONCLUSIONS: Both the risk of the progression of HIV disease and the efficacy of antiretroviral therapy are strongly associated with the plasma level of HIV RNA and with the viral phenotype. The changes in the plasma concentration of HIV RNA predict the changes in CD4 cell counts and survival after treatment with reverse-transcriptase inhibitors.},
 Keywords = {Adult
Antiviral Agents/*therapeutic use
CD4 Lymphocyte Count
Didanosine/*therapeutic use
Disease Progression
Drug Therapy, Combination
Female
HIV/*genetics/isolation & purification/physiology
HIV Infections/drug therapy/immunology/*virology
Human
Male
Middle Aged
Multivariate Analysis
Phenotype
Proportional Hazards Models
RNA, Viral/*blood
Support, U.S. Gov't, P.H.S.
Treatment Outcome
Virus Replication/drug effects
Zidovudine/*therapeutic use},
   Year = {1996} }



@article{
Kaufmann98,
   Author = {Kaufmann, D. and Pantaleo, G. and Sudre, P. and Telenti, A.},
   Title = {CD4-cell count in HIV-1-infected individuals remaining viraemic with highly active antiretroviral therapy (HAART). Swiss HIV Cohort Study},
   Journal = {Lancet},
   Volume = {351},
   Number = {9104},
   Pages = {723-4},
   Note = {0140-6736
Letter},
 Keywords = {Anti-HIV Agents/*therapeutic use
CD4 Lymphocyte Count
HIV Infections/drug therapy/*immunology
Human
Protease Inhibitors/*therapeutic use
Support, Non-U.S. Gov't
Viremia/drug therapy/*immunology},
   Year = {1998} }



@article{
Kaufmann03,
   Author = {Kaufmann, G. R. and Perrin, L. and Pantaleo, G. and Opravil, M. and Furrer, H. and Telenti, A. and Hirschel, B. and Ledergerber, B. and Vernazza, P. and Bernasconi, E. and Rickenbach, M. and Egger, M. and Battegay, M.},
   Title = {CD4 T-lymphocyte recovery in individuals with advanced HIV-1 infection receiving potent antiretroviral therapy for 4 years: the Swiss HIV Cohort Study},
   Journal = {Arch Intern Med},
   Volume = {163},
   Number = {18},
   Pages = {2187-95},
   Note = {0003-9926
Journal Article},
   Abstract = {BACKGROUND: Highly active antiretroviral therapy (HAART) for human immunodeficiency virus (HIV)-1 infection allows recovery of CD4 T lymphocytes. Few studies have explored the long-term T-lymphocyte responses to HAART. METHODS: Plasma HIV-1 RNA levels and CD4 and CD8 T-lymphocyte counts were longitudinally analyzed over 4 years in 2235 participants of the Swiss HIV Cohort, commencing HAART between 1996 and 1997. The CD4 T-lymphocyte count increase, the percentage of individuals with a CD4 T-lymphocyte count of 500/microL or greater and less than 200/microL, and the determinants of CD4 T-lymphocyte recovery were evaluated in individuals treated with continuous (CONT; n = 985) and discontinuous (DISCONT; n = 1250) HAART. RESULTS: At 4 years, 69.5% of subjects (CONT, 84.5%; DISCONT, 53.6%; P<.001) showed HIV-1 RNA levels below 400 copies/mL, while the median CD4 T-lymphocyte count increased from 190/microL to 423/microL (CONT, 486/microL; DISCONT, 343/microL; P<.001). Of the 2235 participants, 38.8% (CONT, 47.7%; DISCONT, 29.4%; P<.001) reached a CD4 T-lymphocyte count of 500/microL or greater, but in 15.6%, CD4 T-lymphocyte count remained below 200/microL (CONT, 5.9%; DISCONT, 25.9%; P<.001). Larger increases in CD4 T-lymphocyte count were associated with higher baseline HIV-1 RNA, a larger percentage of undetectable HIV-1 RNA levels, lower baseline CD8 T-lymphocyte count, and younger age. Individuals reaching a CD4 T-lymphocyte count of 500/microL or greater at 4 years were characterized by higher nadir and baseline CD4 T-lymphocyte counts and a more sustained reduction of HIV-1 RNA levels. CONCLUSIONS: At 4 years, only 39% of individuals treated with HAART reached a CD4 T-lymphocyte count of 500/microL or greater, and 16% with CD4 T-lymphocyte counts less than 200/microL remained susceptible to opportunistic infections. Treatment interruptions, a poor virologic response, and older age were the major factors negatively affecting the recovery of CD4 T lymphocytes.},
 Keywords = {Adult
*Antiretroviral Therapy, Highly Active
*CD4 Lymphocyte Count
CD8-Positive T-Lymphocytes
Female
HIV Infections/*drug therapy/*immunology
*Hiv-1
Human
Lymphocyte Count
Male
Middle Aged
Prospective Studies
RNA, Viral/*analysis
Support, Non-U.S. Gov't
Viral Load},
   Year = {2003} }



@article{
MartinezPicado99,
   Author = {Martinez-Picado, J. and Savara, A. V. and Sutton, L. and D'Aquila, R. T.},
   Title = {Replicative fitness of protease inhibitor-resistant mutants of human immunodeficiency virus type 1},
   Journal = {J Virol},
   Volume = {73},
   Number = {5},
   Pages = {3744-52},
   Note = {0022-538x
Journal Article},
   Abstract = {The relative replicative fitness of human immunodeficiency virus type 1 (HIV-1) mutants selected by different protease inhibitors (PIs) in vivo was determined. Each mutant was compared to wild type (WT), NL4-3, in the absence of drugs by several methods, including clonal genotyping of cultures infected with two competing viral variants, kinetics of viral antigen production, and viral infectivity/virion particle ratios. A nelfinavir-selected protease D30N substitution substantially decreased replicative capacity relative to WT, while a saquinavir-selected L90M substitution moderately decreased fitness. The D30N mutant virus was also outcompeted by the L90M mutant in the absence of drugs. A major natural polymorphism of the HIV-1 protease, L63P, compensated well for the impairment of fitness caused by L90M but only slightly improved the fitness of D30N. Multiply substituted indinavir-selected mutants M46I/L63P/V82T/I84V and L10R/M46I/L63P/V82T/I84V were just as fit as WT. These results indicate that the mutations which are usually initially selected by nelfinavir and saquinavir, D30N and L90M, respectively, impair fitness. However, additional mutations may improve the replicative capacity of these and other drug-resistant mutants. Hypotheses based on the greater fitness impairment of the nelfinavir-selected D30N mutant are suggested to explain observations that prolonged responses to delayed salvage regimens, including alternate PIs, may be relatively common after nelfinavir failure.},
 Keywords = {Adaptation, Biological
Amino Acid Substitution
Animals
Anti-HIV Agents/*pharmacology
Cells, Cultured
Drug Resistance, Microbial
HIV Protease Inhibitors/*pharmacology
HIV-1/*drug effects/genetics/physiology
Human
Mice
Mutagenesis, Site-Directed
Nelfinavir/*pharmacology
Saquinavir/*pharmacology
Support, Non-U.S. Gov't
Support, U.S. Gov't, P.H.S.
Tumor Cells, Cultured
Virus Replication/*drug effects},
   Year = {1999} }



@article{
Mellors96,
   Author = {Mellors, J. W. and Rinaldo, C. R., Jr. and Gupta, P. and White, R. M. and Todd, J. A. and Kingsley, L. A.},
   Title = {Prognosis in HIV-1 infection predicted by the quantity of virus in plasma},
   Journal = {Science},
   Volume = {272},
   Number = {5265},
   Pages = {1167-70},
   Note = {0036-8075
Comment
Journal Article},
   Abstract = {The relation between viremia and clinical outcome in individuals infected with human immunodeficiency virus-type 1 (HIV-1) has important implications for therapeutic research and clinical care. HIV-1 RNA in plasma was quantified with a branched-DNA signal amplification assay as a measure of viral load in a cohort of 180 seropositive men studied for more than 10 years. The risk of acquired immunodeficiency syndrome (AIDS) and death in study subjects, including those with normal numbers of CD4+ T cells, was directly related to plasma viral load at study entry. Plasma viral load was a better predictor of progression to AIDS and death than was the number of CD4+ T cells.},
 Keywords = {Acquired Immunodeficiency Syndrome/*virology
Antiviral Agents/therapeutic use
Biological Markers/blood
CD4 Lymphocyte Count
CD4-Positive T-Lymphocytes/virology
Cohort Studies
Disease Progression
Follow-Up Studies
HIV Infections/drug therapy/mortality/*virology
HIV-1/genetics/*physiology
Human
Male
Prognosis
Proportional Hazards Models
RNA, Viral/*blood
Support, Non-U.S. Gov't
Support, U.S. Gov't, Non-P.H.S.
Support, U.S. Gov't, P.H.S.
Survival Rate
Time Factors
Viremia/*virology
Virus Replication},
   Year = {1996} }



@article{
Miller00,
   Author = {Miller, V. and Sabin, C. A. and Phillips, A. N. and Rottmann, C. and Rabenau, H. and Weidmann, E. and Rickerts, V. and Findhammer, S. and Helm, E. B. and Staszewski, S.},
   Title = {The impact of protease inhibitor-containing highly active antiretroviral therapy on progression of HIV disease and its relationship to CD4 and viral load},
   Journal = {Aids},
   Volume = {14},
   Number = {14},
   Pages = {2129-36},
   Note = {0269-9370
Clinical Trial
Journal Article},
   Abstract = {OBJECTIVE: To compare the rate of disease progression according to viral load and CD4 cell count in patients receiving or not receiving highly active antiretroviral therapy (HAART), defined as protease inhibitor-containing regimens. DESIGN: An observational study, with prospectively collected data. METHODS: All patients attending the HIV Outpatient clinic as of 1 January 1995 (n = 2083) were included. Follow-up was until the first AIDS-defining event or death. Associations between viral load or CD4 cell count and disease progression were assessed using a person-years approach. Event rates were compared using Poisson regression analysis; a multivariate model was used to assess the independent effects of CD4, viral load and treatment group on event rates and to consider interactions between these variables. RESULTS: The event rates increased with lower CD4 cell count and higher viral load for both treatment groups and were generally lower in the HAART group. In a multivariate analysis, lower CD4 cell counts and higher viral loads remained significantly associated with disease progression, irrespective of treatment group. However, the event rate was significantly lower for the HAART group compared with the control group (relative rate 0.53, P < 0.001). CONCLUSIONS: HAART-treated patients with high viral loads and CD4 cell counts experienced reduced disease progression compared with individuals with the same CD4 cell count and viral load not receiving HAART. Consequently, the short-term prognosis associated with viral load levels and CD4 cell counts may differ in patients on HAART. Whether this effect will be observed with non-protease-inhibitor-containing HAART is not known at this time.},
 Keywords = {Adolescent
Adult
Aged
Antiretroviral Therapy, Highly Active
CD4 Lymphocyte Count
Disease Progression
HIV Infections/*drug therapy/pathology/virology
HIV Protease Inhibitors/*therapeutic use
*HIV-1/isolation & purification
Human
Middle Aged
Prospective Studies
RNA, Viral/analysis
Regression Analysis
Support, Non-U.S. Gov't
Viral Load},
   Year = {2000} }



@article{
Piketty98,
   Author = {Piketty, C. and Castiel, P. and Belec, L. and Batisse, D. and Si Mohamed, A. and Gilquin, J. and Gonzalez-Canali, G. and Jayle, D. and Karmochkine, M. and Weiss, L. and Aboulker, J. P. and Kazatchkine, M. D.},
   Title = {Discrepant responses to triple combination antiretroviral therapy in advanced HIV disease},
   Journal = {Aids},
   Volume = {12},
   Number = {7},
   Pages = {745-50},
   Note = {0269-9370
Journal Article},
   Abstract = {OBJECTIVES: To determine the clinical, virological and immunological outcome in a cohort of unselected patients receiving triple combination therapy for more than 1 year. METHODS: Prospective follow-up of a cohort of 162 unselected, protease inhibitor-naive, antiretroviral-experienced patients with advanced HIV disease, treated with indinavir combined with two nucleoside analogues. RESULTS: The mean CD4 cell count and plasma HIV RNA level in the study group at baseline were 69+/-5 x 10(6)/l and 4.75+/-0.07 log10 copies/ml, respectively. Five per cent of patients died prematurely or were lost to follow-up. Fifty-seven per cent of patients responded to therapy, as assessed by a sustained increase in CD4 cell counts above 50 x 10(6)/l and a decrease in plasma HIV RNA greater than 1 log10 copies/ml, throughout 12.1 months of follow-up. Seventeen per cent of patients were immunological and virological non-responders. Twenty-one per cent of patients exhibited discrepant virological and immunological responses to treatment, of whom one-half failed to exhibit significant increases in CD4 cells despite a virological response to therapy and one-half exhibited increased CD4 cell counts in the absence of significant decrease in plasma viral load. The incidence of AIDS-defining events in the latter group of patients was similar to that of responder patients, whereas their incidence was higher in patients who failed to exhibit a virological and immunological response and those who failed to increase CD4 cells despite a significant decrease in viral load. CONCLUSION: Our observations of discrepant immunological and virological responses to treatment raise the issue of the significance of persistent elevated levels of plasma HIV RNA and of the relevance of measurements of plasma viral load for assessing the efficacy of antiretroviral therapy in patients whose CD4 cell counts increase despite the absence of significant decrease in plasma HIV viral load.},
 Keywords = {Adult
Aged
Anti-HIV Agents/*therapeutic use
Cohort Studies
Drug Therapy, Combination
Female
Follow-Up Studies
HIV Infections/*drug therapy/immunology/physiopathology/virology
HIV Protease Inhibitors/*therapeutic use
Human
Indinavir/*therapeutic use
Lamivudine/*therapeutic use
Male
Middle Aged
Prospective Studies
Reverse Transcriptase Inhibitors/*therapeutic use
Stavudine/*therapeutic use
Support, Non-U.S. Gov't
Treatment Outcome
Zidovudine/*therapeutic use},
   Year = {1998} }



@article{
Piketty01,
   Author = {Piketty, C. and Weiss, L. and Thomas, F. and Mohamed, A. S. and Belec, L. and Kazatchkine, M. D.},
   Title = {Long-term clinical outcome of human immunodeficiency virus-infected patients with discordant immunologic and virologic responses to a protease inhibitor-containing regimen},
   Journal = {J Infect Dis},
   Volume = {183},
   Number = {9},
   Pages = {1328-35},
   Note = {0022-1899
Journal Article},
   Abstract = {Within a prospective cohort of 150 human immunodeficiency virus (HIV)-infected patients who began first-line protease inhibitor therapy in 1996, the outcome of 42 patients with discrepant virologic and immunologic responses to antiretroviral treatment at 12 months was analyzed at 30 months of treatment. The incidence of AIDS-defining events and deaths (14%) in the group of patients with immunologic responses in the absence of a virologic response was higher than that in full-responder patients (2%); yet, the incidence in this group was lower than that in patients with no immunologic response, despite a virologic response (21%), and was lower than that in patients without an immunologic or virologic response (67%; P<.0001, log-rank test). Differences in outcome were significant (relative risk, 6.9; 95% confidence interval, 1.9-39.3) when factors for progression were compared with those of responder patients. The results support the relevance of the CD4 cell marker over plasma HIV load for predicting clinical outcome in patients who do not achieve full immunologic and virologic responses.},
 Keywords = {Adult
Aged
Antiretroviral Therapy, Highly Active
CD4 Lymphocyte Count
Cohort Studies
Disease Progression
Female
HIV Infections/*drug therapy/immunology/virology
HIV Protease Inhibitors/*therapeutic use
Human
Incidence
Longitudinal Studies
Male
Middle Aged
Mortality
Prospective Studies
RNA, Viral/blood
Time Factors
Treatment Outcome
Viral Load},
   Year = {2001} }



@article{
Pilon02,
   Author = {Pilon, A. A. and Lum, J. J. and Sanchez-Dardon, J. and Phenix, B. N. and Douglas, R. and Badley, A. D.},
   Title = {Induction of apoptosis by a nonnucleoside human immunodeficiency virus type 1 reverse transcriptase inhibitor},
   Journal = {Antimicrob Agents Chemother},
   Volume = {46},
   Number = {8},
   Pages = {2687-91},
   Note = {0066-4804
Journal Article},
   Abstract = {Inhibition of human immunodeficiency virus type 1 reverse transcriptase (RT) by both nucleoside and nonnucleoside RT inhibitors profoundly inhibits virus replication. Nucleoside RT inhibitors are known to be toxic, but there is little information regarding the toxicities of nonnucleoside RT inhibitors (NNRTI). We demonstrate that efavirenz (an NNRTI) induces caspase- and mitochondrion-dependent apoptosis of Jurkat T cells and human peripheral blood mononuclear cells. The clinical relevance of these observations is not yet clear.},
 Keywords = {Annexin V/diagnostic use
Apoptosis/*drug effects
Caspases/physiology
Enzyme Inhibitors/diagnostic use
Fluorescein-5-isothiocyanate
Fluorescent Dyes
HIV-1 Reverse Transcriptase/*antagonists & inhibitors
Human
Jurkat Cells
Membrane Potentials/drug effects
Mitochondria/drug effects/physiology
Oxazines/*pharmacology
Reverse Transcriptase Inhibitors/*pharmacology
Support, Non-U.S. Gov't},
   Year = {2002} }



@article{
Price03,
   Author = {Price, D. A. and Scullard, G. and Oxenius, A. and Braganza, R. and Beddows, S. A. and Kazmi, S. and Clarke, J. R. and Johnson, G. E. and Weber, J. N. and Phillips, R. E.},
   Title = {Discordant outcomes following failure of antiretroviral therapy are associated with substantial differences in human immunodeficiency virus-specific cellular immunity},
   Journal = {J Virol},
   Volume = {77},
   Number = {10},
   Pages = {6041-9},
   Note = {0022-538x
Clinical Trial
Journal Article},
   Abstract = {Many individuals chronically infected with human immunodeficiency virus type 1 (HIV-1) experience a recrudescence of plasma virus during continuous combination antiretroviral therapy (ART) due either to the emergence of drug-resistant viruses or to poor compliance. In most cases, virologic failure on ART is associated with a coincident decline in CD4(+) T lymphocyte levels. However, a proportion of discordant individuals retain a stable or even increasing CD4(+) T lymphocyte count despite virological failure. In order to address the nature of these different outcomes, we evaluated virologic and immunologic variables in a prospective, single-blinded, nonrandomized cohort of 53 subjects with chronic HIV-1 infection who had been treated with continuous ART and monitored intensively over a period of 19 months. In all individuals with detectable viremia on ART, multiple drug resistance mutations with similar impacts on viral growth kinetics were detected in the pol gene of circulating plasma virus. Further, C2V3 env gene analysis demonstrated sequences indicative of CCR5 coreceptor usage in the majority of those with detectable plasma viremia. In contrast to this homogeneous virologic pattern, comprehensive screening with a range of antigens derived from HIV-1 revealed substantial immunologic differences. Discordant subjects with stable CD4(+) T lymphocyte counts in the presence of recrudescent virus demonstrated potent virus-specific CD4(+) and CD8(+) T lymphocyte responses. In contrast, subjects with virologic failure associated with declining CD4(+) T lymphocyte counts had substantially weaker HIV-specific CD4(+) T lymphocyte responses and exhibited a trend towards weaker HIV-specific CD8(+) T lymphocyte responses. Importantly the CD4(+) response was sustained over periods as long as 11 months, confirming the stability of the phenomenon. These correlative data lead to the testable hypothesis that the consequences of viral recrudescence during continuous ART are modulated by the HIV-specific cellular immune response.},
 Keywords = {Adult
Amino Acid Sequence
Anti-HIV Agents/pharmacology/*therapeutic use
CD4-Positive T-Lymphocytes/*immunology
CD8-Positive T-Lymphocytes/*immunology
Chronic Disease
Drug Resistance, Viral/genetics
Drug Therapy, Combination
HIV Envelope Protein gp120/chemistry/genetics
HIV Infections/*drug therapy/immunology/physiopathology
HIV-1/*drug effects/genetics/physiology
Human
Lymphocyte Count
Middle Aged
Molecular Sequence Data
Mutation
Peptide Fragments/chemistry/genetics
Prospective Studies
RNA, Viral/blood
Single-Blind Method
Support, Non-U.S. Gov't
*Treatment Failure
Viral Load},
   Year = {2003} }



@article{
Quinones00,
   Author = {Quinones-Mateu, M. E. and Ball, S. C. and Marozsan, A. J. and Torre, V. S. and Albright, J. L. and Vanham, G. and van Der Groen, G. and Colebunders, R. L. and Arts, E. J.},
   Title = {A dual infection/competition assay shows a correlation between ex vivo human immunodeficiency virus type 1 fitness and disease progression},
   Journal = {J Virol},
   Volume = {74},
   Number = {19},
   Pages = {9222-33},
   Note = {0022-538x
Journal Article},
   Abstract = {This study was designed to examine the impact of human immunodeficiency virus type 1 (HIV-1) fitness on disease progression through the use of a dual competition/heteroduplex tracking assay (HTA). Despite numerous studies on the impact of HIV-1 diversity and HIV-specific immune response on disease progression, we still do not have a firm understanding of the long-term pathogenesis of this virus. Strong and early CD8-positive cytotoxic T-cell and CD4-positive T-helper cell responses directed toward HIV-infected cells appear to curb HIV pathogenesis. However, the rate at which the virus infects the CD4(+) T-cell population and possibly destroys the HIV-specific immune response may also alter the rate of disease progression. For HIV-1 fitness studies, we established conditions for dual HIV-1 infections of peripheral blood mononuclear cells (PBMC) and a sensitive HTA to measure relative virus production. A pairwise comparison was then performed to estimate the relative fitness of various non-syncytium-inducing/CCR5-tropic (NSI/R5) and syncytium-inducing/CXCR4-tropic (SI/X4) HIV-1 isolates. Four HIV-1 strains (two NSI/R5 and two SI/X4) with moderate ex vivo fitness were then selected as controls and competed against primary HIV-1 isolates from an HIV-infected Belgian cohort. HIV-1 isolates from long-term survivors (LTS) were outcompeted by control strains and were significantly less fit than HIV-1 isolates from patients with accelerated progression to AIDS (PRO). In addition, NSI/R5 HIV-1 isolates from PRO overgrew control SI/X4 strains, suggesting that not all SI/X4 HIV-1 isolates replicate more efficiently than all NSI/R5 isolates. Finally, there were strong, independent correlations between viral load and the total relative fitness values of HIV-1 isolates from PRO (r = 0.84, P = 0.033) and LTS (r = 0.86, P = 0.028). Separation of the PRO and LTS plots suggest that HIV-1 fitness together with viral load may be a strong predictor for the rate of disease progression.},
 Keywords = {*Biological Assay
HIV Infections/*physiopathology/*virology
*HIV-1/physiology
Human
Predictive Value of Tests
Prognosis
Support, Non-U.S. Gov't
Support, U.S. Gov't, P.H.S.},
   Year = {2000} }



@article{
Racinan02,
   Author = {Rancinan, C. and Neau, D. and Saves, M. and Lawson-Ayayi, S. and Bonnet, F. and Mercie, P. and Dupon, M. and Couzigou, P. and Dabis, F. and Chene, G.},
   Title = {Is hepatitis C virus co-infection associated with survival in HIV-infected patients treated by combination antiretroviral therapy?},
   Journal = {Aids},
   Volume = {16},
   Number = {10},
   Pages = {1357-62},
   Note = {0269-9370
Journal Article},
   Abstract = {OBJECTIVE: To study whether hepatitis C virus (HCV) co-infection or the severe elevation of transaminases is associated with survival after the initiation of antiretroviral combination therapy. DESIGN: Prospective hospital-based cohort (Aquitaine Cohort). METHODS: HIV-infected adults started on an antiretroviral combination before 30 June 1999. HCV infection was defined as antibody detection or positive HCV RNA. Severe elevation of transaminases was defined as a value of aspartate or alanine aminotransferase (AST, ALT) above five times the upper limit of normal values. Survival was studied using a Cox model, including at least baseline HCV status and transaminases as a time-dependent covariate. RESULTS: Overall, 995 patients were analysed, including 576 HCV-positive individuals (58%). At baseline, HCV-positive patients were younger, more often injecting drug users and women, and had more frequently elevated transaminases. A shorter survival was associated with AIDS stage [hazard ratio (HR) versus non-AIDS 1.67; 95% confidence interval (CI) 1.03; 2.68], lower CD4 cell count (HR for 50 cells/mm3 lower 1.33; CI 1.17; 1.51), lower haemoglobin (HR for 1 g/dl lower 1.20; CI 1.07; 1.35), lower platelet count (HR for 10 000 cells/mm3 lower 1.04; CI 1.01; 1.07), and AST during follow-up (HR for > or = 200 IU/l 2.30; CI 1.32; 4.03). HCV co-infection (HR 1.20; CI 0.75; 1.92) was not statistically associated with survival. CONCLUSION: The occurrence of a severe elevation of transaminases was associated with poorer survival, although HCV was not. If liver toxicity may be treatment induced, plasma drug concentrations could guide dosage adjustments of antiretroviral treatments currently prescribed to optimize their use.},
 Keywords = {Acquired Immunodeficiency Syndrome/complications
Age Factors
Anti-HIV Agents/*therapeutic use
Antiretroviral Therapy, Highly Active
Cohort Studies
Comparative Study
Disease Progression
Female
Follow-Up Studies
HIV Infections/blood/*complications/*drug therapy
Hepatitis C/blood/*complications
Human
Male
Proportional Hazards Models
Substance Abuse, Intravenous
Support, Non-U.S. Gov't
Survival Analysis
Transaminases/blood},
   Year = {2002} }



@article{
Roger99,
   Author = {Roger, P. M. and Breittmayer, J. P. and Arlotto, C. and Pugliese, P. and Pradier, C. and Bernard-Pomier, G. and Dellamonica, P. and Bernard, A.},
   Title = {Highly active anti-retroviral therapy (HAART) is associated with a lower level of CD4+ T cell apoptosis in HIV-infected patients},
   Journal = {Clin Exp Immunol},
   Volume = {118},
   Number = {3},
   Pages = {412-6},
   Note = {0009-9104
Journal Article},
   Abstract = {HAART may increase CD4+ T cell counts despite a persistently detectable HIV load. The impact of HAART on apoptosis, which may play a role in the disease process in HIV-infected patients, has not been extensively studied. We performed a study to compare the level of spontaneous T cell apoptosis and anti-retroviral treatments in a cohort of HIV-1-infected patients. Data were obtained from a computerized medical record. Quantification of apoptotic cells was by cytofluorometric technique. From November 1995 to December 1997 we studied T cell apoptosis in 112 HIV-infected patients. Forty patients were classified A, 36 B and 36 C. Thirty patients were naive and 82 received an anti-retroviral treatment, 49 including a protease inhibitor (PI). The median plasma viraemia determined in 63 patients was 3.6 (range 1.3-5.6) log10. The median apoptotic cell count was 22% (range 2-73%) and 12% (range 2-60%) for CD4+ and CD8+ T cells, respectively. We did not observe any correlation between the HIV viraemia and the level of apoptosis of T cell subsets. Patients with HAART showed a lower percentage of apoptotic CD4+ T cells only: 16% (range 2-61%) versus 25% (range 5-73%) for patients receiving two nucleoside analogues (P = 0.02). This effect was significant in stage A patients and remained observable during the whole course of HIV disease. In conclusion, HAART, without any relation to plasma viraemia, is able to reduce apoptosis of CD4+ T cells.},
 Keywords = {Adult
Aged
Anti-HIV Agents/*therapeutic use
*Apoptosis
CD4-Positive T-Lymphocytes/cytology/*drug effects
CD8-Positive T-Lymphocytes/drug effects
Didanosine/therapeutic use
Drug Therapy, Combination
Female
HIV Infections/*drug therapy/immunology/pathology
HIV Protease Inhibitors/therapeutic use
Human
Lamivudine/therapeutic use
Male
Middle Aged
Multivariate Analysis
Retrospective Studies
Stavudine/therapeutic use
Viral Load
Zalcitabine/therapeutic use
Zidovudine/therapeutic use},
   Year = {1999} }



@article{
Stoddart01,
   Author = {Stoddart, C. A. and Liegler, T. J. and Mammano, F. and Linquist-Stepps, V. D. and Hayden, M. S. and Deeks, S. G. and Grant, R. M. and Clavel, F. and McCune, J. M.},
   Title = {Impaired replication of protease inhibitor-resistant HIV-1 in human thymus},
   Journal = {Nat Med},
   Volume = {7},
   Number = {6},
   Pages = {712-8},
   Note = {1078-8956
Journal Article},
   Abstract = {Many HIV-1-infected patients treated with protease inhibitors (PI) develop PI-resistant HIV-1 variants and rebounds in viremia, but their CD4+ T-cell counts often do not fall. We hypothesized that in these patients, T-cell counts remain elevated because PI-resistant virus spares intrathymic T-cell production. To test this, we studied recombinant HIV-1 clones containing wild-type or PI-resistant protease domains, as well as uncloned isolates from patients, in activated peripheral blood mononuclear cells, human thymic organ cultures and human thymus implants in SCID-hu Thy/Liv mice. In most cases, wild-type and PI-resistant HIV-1 isolates replicated to similar degrees in peripheral blood mononuclear cells. However, the replication of PI-resistant but not wild-type HIV-1 isolates was highly impaired in thymocytes. In addition, patients who had PI-resistant HIV-1 had abundant thymus tissue as assessed by computed tomography. We propose that the inability of PI-resistant HIV-1 to replicate efficiently in thymus contributes to the preservation of CD4+ T-cell counts in patients showing virologic rebound on PI therapy.},
 Keywords = {Adult
Animals
CD4 Lymphocyte Count
Drug Resistance, Microbial
Fetal Tissue Transplantation
Flow Cytometry
HIV Core Protein p24/metabolism
HIV Infections/immunology/pathology/*virology
HIV Protease/genetics/*metabolism
HIV Protease Inhibitors/*pharmacology
HIV-1/*drug effects/enzymology/genetics/*physiology
Human
Mice
Mice, SCID
Middle Aged
Organ Culture
Recombination, Genetic
Support, Non-U.S. Gov't
Support, U.S. Gov't, P.H.S.
T-Lymphocytes/*physiology/virology
Thymus Gland/pathology/physiopathology/transplantation/*virology
Viral Load
*Virus Replication},
   Year = {2001} }



@article{
Sufka03,
   Author = {Sufka, S. A. and Ferrari, G. and Gryszowka, V. E. and Wrin, T. and Fiscus, S. A. and Tomaras, G. D. and Staats, H. F. and Patel, D. D. and Sempowski, G. D. and Hellmann, N. S. and Weinhold, K. J. and Hicks, C. B.},
   Title = {Prolonged CD4+ cell/virus load discordance during treatment with protease inhibitor-based highly active antiretroviral therapy: immune response and viral control},
   Journal = {J Infect Dis},
   Volume = {187},
   Number = {7},
   Pages = {1027-37},
   Note = {0022-1899
Clinical Trial
Journal Article},
   Abstract = {Mechanisms that underly discordant CD4+ cell/virus load (VL) responses in patients who receive highly active antiretroviral therapy (HAART) were studied in 30 human immunodeficiency virus (HIV)-positive patients, in 3 groups. Discordant responders maintained CD4+ cell levels >200/mm(3) with stable or increasing trend, despite sustained VLs of 500-5000 copies/mL, for >2 years. Treatment-success patients had CD4+ cell counts >200/mm(3) with stable or increasing trend and VLs <50 copies/mL, for >2 years. Treatment-failure patients initially responded to HAART, followed by decreasing CD4+ cell counts and increasing VLs. Interferon-gamma production to gag and noncytolytic CD8+ cell suppressive activity were greater in discordant responders. Cellular activation was greatest in patients with treatment failure. All discordant responders had non-syncytium-inducing (CCR5-tropic) viruses. Viruses from discordant responders and from patients with treatment failure had extensive resistance mutations; discordant responders had significantly lower viral replication capacities. These findings suggest that discordant responses may be related to enhanced HIV-directed immune responses, diminished cellular activation, decreased viral replication capacity, and preservation of non-syncytium-inducing virus strains.},
 Keywords = {Adult
*Antiretroviral Therapy, Highly Active
*CD4 Lymphocyte Count
Female
HIV/*drug effects
HIV Infections/*drug therapy/*immunology/virology
HIV Protease Inhibitors/*pharmacology/therapeutic use
Human
Male
Middle Aged
Support, Non-U.S. Gov't
Support, U.S. Gov't, P.H.S.
Time Factors
Treatment Failure
*Viral Load
Virus Replication/drug effects},
   Year = {2003} }



@article{
Tebaldi03,
   Author = {Tedaldi, E. M. and Baker, R. K. and Moorman, A. C. and Alzola, C. F. and Furhrer, J. and McCabe, R. E. and Wood, K. C. and Holmberg, S. D.},
   Title = {Influence of coinfection with hepatitis C virus on morbidity and mortality due to human immunodeficiency virus infection in the era of highly active antiretroviral therapy},
   Journal = {Clin Infect Dis},
   Volume = {36},
   Number = {3},
   Pages = {363-7},
   Note = {1537-6591
Journal Article},
   Abstract = {To ascertain the impact of hepatitis C virus (HCV) infection on human immunodeficiency virus (HIV) disease progression and associated death in the era of highly active antiretroviral therapy (HAART), we examined mortality rates, the presence of other diseases, and antiretroviral use in an observational cohort of 823 HIV-infected patients with and without HCV coinfection during the period of January 1996 through June 2001. Analyses were used to compare patient characteristics, comorbid conditions, and survival durations in HIV-infected and HIV-HCV-coinfected patients. HIV-HCV-coinfected persons did not have a statistically greater rate of acquired immunodeficiency syndrome or of renal or cardiovascular disease, but they did have more cases of cirrhosis and transaminase elevations. There were proportionately more deaths in the HIV-HCV-coinfected group. Age, baseline CD4+ cell count, and duration of HAART were significantly associated with survival, but HCV infection was not. HAART use was a strong predictor of increased duration of survival, suggesting that treatment is more important to survival than is HCV coinfection status.},
 Keywords = {Anti-HIV Agents/therapeutic use
*Antiretroviral Therapy, Highly Active
*Hiv
HIV Infections/*complications/drug therapy/epidemiology/mortality
*Hepacivirus
Hepatitis C/*complications/epidemiology/mortality
Human
Morbidity
Mortality
Support, U.S. Gov't, P.H.S.},
   Year = {2003} }




@string{JASA= {Journal of the American Statistical Association}}
@string{JC = {Journal of Classification}}
@string{JSPI = {Journal of Statistical Planning and Inference}}
@string{JRSSB = {Journal of the Royal Statistical Society, Series B}}
@string{PNAS = {Proc. Natl. Acad. Sci.}}

@Article{Wang&Bembom&vanderLaan06,
  author =   {Y. Wang and O. Bembom and M.J. van der Laan},
  title =    {Data adaptive estimation of the treatment specific mean},
  journal =      {Journal of Statistical Planning and Inference},
  year =     {2006},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {also http://www.bepress.com/ucbbiostat/paper159},
  OPTannote =    {}
}
@Article{Sinisi&vanderLaan04,
  author =   {S. Sinisi and M.J. van der Laan},
  title =    {The deletion/substitution/addition algorithm in loss function based estimation:
Applications in Genomics},
  journal =      {Journal of Statistical Methods in Molecular Biology},
  year =     {2004},
  OPTkey =   {},
  volume =   {3},
  number =   {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/sagmb/vol3/iss1/art18},
  OPTannote =    {}
}



@TECHREPORT{Petersen&Deeks&Martin&vanderLaan05,
  author =       {Maya L. Petersen and Steven G. Deeks and Jeffrey N. Martin and Mark J. van der Laan},
  title =        {History-Adjusted Marginal Structural Models: Time-Varying Effect Modification
  and Dynamic Treatment Regimens},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2005},
  type =         {Technical Report 199},
OPTnote =      {http://www.bepress.com/ucbbiostat/paper199},
  month =        {December},
}

@TECHREPORT{vanderLaan&Rubin05,
  author =       {M.J. van der Laan and D. Rubin},
  title =        {Estimating Function Based Cross-Validation and Learning},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2005},
  type =         {Technical Report 180},
OPTnote =      {http://www.bepress.com/ucbbiostat/paper180},
  month =        {},
}

@Article{vanderLaan&Petersen07,
  author =   {M.J. van der Laan and M.L. Petersen},
  title =    {Causal Effect Models for Realistic Individualized Treatment and Intention to Treat Rules},
  journal =      {International Journal of Biostatistics},
  year =     {2007},
  OPTkey =   {},
  volume =   {3},
  number =   {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/ijb/vol3/iss1/art3},
  OPTannote =    {}
}


@TECHREPORT{vanderLaan06,
  author =       {M.J. van der Laan},
  title =        {Causal Effect Models for Intention to Treat and Realistic Individualized
  Treatment Rules},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2006},
  type =         {Technical Report 203},
OPTnote =      {http://www.bepress.com/ucbbiostat/paper203},
  month =        {},
}
@TECHREPORT{vanderLaan08b,
  author =       {M.J. van der Laan},
  title =        {The construction and analysis of adaptive group sequential designs},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2008},
  type =         {Technical Report 232},
OPTnote =      {http://www.bepress.com/ucbbiostat/paper232},
  month =        {March},
}
@TECHREPORT{Moore&vanderLaan07,
  author =       {K.L. Moore and M.J. van der Laan},
  title =        {Covariate adjustment in randomized trials with binary outcomes},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2007},
  type =         {Technical Report 215},
OPTnote =      {http://www.bepress.com/ucbbiostat/paper215},
  month =        {April},
}

@TECHREPORT{vanderLaan&Petersen05,
  author =       {M.J. van der Laan and M.L. Petersen},
  title =        {Direct Effect Models},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2005},
  type =         {Technical Report 187},
OPTnote =      {http://www.bepress.com/ucbbiostat/paper187},
  month =        {},
}
@TECHREPORT{Petersen&vanderLaan06,
  author =       {M.L. Petersen and M.J. van der Laan},
  title =        {Individualized Treatment Rules and Clinical Trials},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2006},
  type =         {Technical Report},
OPTnote =      {},
  month =        {},
}

@Article{vanderLaan&Petersen&Joffe05,
  author =   {M.J. van der Laan and M.L. Petersen and M.M. Joffe},
  title =    {History-Adjusted Marginal Structural Models and Statically-Optimal Dynamic Treatment Regimens},
  journal =      {The International Journal of Biostatistics},
  year =     {2005},
  OPTkey =   {},
  volume =   {1},
  number =   {1},
  pages =    {10-20},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/ijb/vol1/iss1/4},
  OPTannote =    {}
}

@Article{vanderLaan06a,
  author =   {M.J. van der Laan},
  title =    {Statistical Inference for Variable Importance},
  journal =      {International Journal of Biostatistics},
  year =     {2006},
  OPTkey =   {},
  volume =   {2},
  number =   {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/ijb/vol2/iss1/art2},
  OPTannote =    {}
}

@Article{vanderLaan&Birkner&Hubbard05,
  author =   {M.J. van der Laan and M.D. Birkner and A.E. Hubbard},
  title =    {Empirical Bayes and resampling based multiple testing procedure controlling tail probability of the proportion of false positives},
  journal =      {Journal of Statistical Applications in Genetics and Molecular Biology},
  year =     {2005},
  OPTkey =   {},
  volume =   {4},
  number =   {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/sagmb/vol4/iss1/art29},
  OPTannote =    {}
}



@Article{vanderLaan&Dudoit&Pollard04b,
  author =   {M.J. van der Laan and S. Dudoit and K.S. Pollard},
  title =    {Augmentation procedures for control of the generalized family-wise
  error rate and tail probabilities for the proportion of false positives},
journal =      {Journal of Statistical Applications in Genetics and Molecular Biology},
  year =     {2004},
  OPTkey =   {},
  volume =   {3},
  number =   {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/sagmb/vol3/iss1/art15},
  OPTannote =    {}
}
@Article{vanderLaan&Dudoit&Pollard04,
  author =   {S. Dudoit and M.J. van der Laan and K.S. Pollard},
  title =    {Multiple testing. Part II.
  Step-down procedures for control of the family-wise error rate
  },
journal =      {Journal of Statistical Applications in Genetics and Molecular Biology},
  year =     {2004},
  OPTkey =   {},
  volume =   {3},
  number =   {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/sagmb/vol3/iss1/art14},
  OPTannote =    {}
}

@Article{Dudoit&vanderLaan&Pollard04,
  author =   {S. Dudoit and M.J. van der Laan and K.S. Pollard},
  title =    {Multiple testing. Part I. Single-step procedures for control of general Type I error rates},
journal =      {Journal of Statistical Applications in Genetics and Molecular Biology},
  year =     {2004},
  OPTkey =   {},
  volume =   {3},
  number =   {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/sagmb/vol3/iss1/art13},
  OPTannote =    {}
}


@Article{Birkner&Sinisi&vanderLaan05,
  author =   {M.D. Birkner and S.E. Sinisi and M.J. van der Laan},
  title =    {Multiple Testing and Data Adaptive Regression: An Application
  to {HIV}-1 Sequence Data},
  journal =      {Journal of Statistical Applications in Genetics and Molecular Biology},
  year =     {2005},
  OPTkey =   {},
  volume =   {4},
  number =   {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/sagmb/vol4/iss1/art8},
  OPTannote =    {}
}

@TECHREPORT{vanderLaan&Hubbard06,
  author =       {M.J. van der Laan and A.E. Hubbard},
  title =        {Quantile-Function Based Null Distribution in Resampling Based Multiple Testing},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2006},
  type =         {Technical Report},
OPTnote =      {http://www.bepress.com/ucbbiostat/paper198},
  month =        {},
}
@TECHREPORT{Molinaro&vanderLaan04,
  author =       {A. Molinaro and M.J. van der Laan},
  title =        {Deletion/Substitution/Addition Algorithm for Partitioning the Covariate Space in Prediction},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2004},
  type =         {Technical Report},
OPTnote =      {http://www.bepress.com/ucbbiostat/paper162},
  month =        {},
}
@TECHREPORT{Birkner&vanderLaan05,
  author =       {M.D. Birkner and M.J. van der Laan},
  title =        {Application of a Variable Importance Measure Method to {HIV}-1 Sequence Data},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2005},
  type =         {Technical Report},
  month =        {},
}



@TECHREPORT{Neugebauer&vanderLaan05b,
  author =       {R. Neugebauer and M.J. van der Laan},
  title =        {Locally Efficient Estimation of Nonparametric
                    Causal Effects on Mean Outcomes in Longitudinal Studies},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2005},
  number =       {134},
  type =         {Technical Report},
OPTnote =    {http://www.bepress.com/ucbbiostat/paper134, to appear in {JSPI}},
  month =        {},
}
@TECHREPORT{Wang&Petersen&vanderLaan06,
  author =       {Y. Wang and M. Petersen and M.J. van der Laan},
  title =        {A statistical method for diagnosing ETA bias in IPTW estimators},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2006},
  number =       {},
  type =         {Technical Report},
OPTnote =    {},
  month =        {},
}

@TECHREPORT{Moore&vanderLaan07,
  author =       {K.L. Moore and M.J. van der Laan},
  title =        {Covariate adjustment in randomized trials with binary outcomes},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2007},
  type =         {Technical Report 215},
OPTnote =    {http://www.bepress.com/ucbbiostat/paper215},
  month =        {April},
}

@TECHREPORT{vanderLaan&Dudoit&vanderVaart,
  author =       {M.J. van der Laan and S. Dudoit and A.W. van der Vaart},
  title =        {The Cross-Validated Adaptive Epsilon-Net Estimator},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2004},
  type =         {Technical Report 142},
OPTnote =    {http://www.bepress.com/ucbbiostat/paper142},
  month =        {February},
}

@TECHREPORT{vanderLaan&DudoitTechRep130,
  author =       {M.J. van der Laan and S. Dudoit},
  title =        {Unified cross-validation methodology for selection among estimators
  and a general cross-validated adaptive epsilon-net estimator: Finite sample oracle
  inequalities and examples},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =         {2003},
  type =         {Technical Report},
OPTnote =    {http://www.bepress.com/ucbbiostat/paper130},
  month =        {November},
}

@TECHREPORT{Petersen&vanderLaan05,
  author =       {M. Petersen and M.J. van der Laan},
  title =        {Estimation of direct and indirect causal effects in
Epidemiology},
  institution =  {Division of Biostatistics, University of California,
Berkeley},
  year =         {2005},
  type =         {Technical Report},
  month =        {},
}

@TECHREPORT{Petersen&Deeks&Martin&vanderLaan05,
  author =       {M.L. Petersen and S.G. Deeks and J.N. Martin and M.J. van der Laan},
  title =        {History-Adjusted Marginal Structural Models: Time-Varying Effect Modification and Dynamic Treatment Regimens},
  institution =  {Division of Biostatistics, University of California,
Berkeley},
  year =         {2005},
  type =         {Technical Report 199},
OPTnote =      {http://www.bepress.com/ucbbiostat/paper199},
  month =        {},
}

@TECHREPORT{vanderLaan&Petersen04,
  author =       {M.J. van der Laan and M. Petersen},
  title =        {Estimation of direct and indirect causal effects in longitudinal studies},
  institution =  {Division of Biostatistics, University of California,
Berkeley},
  year =         {2004},
  type =         {Technical Report 155},
  month =        {August},
}

@TECHREPORT{vanderLaan&Hubbard&Jewell04,
 author =       {M.J. van der Laan and A.E. Hubbard and N.P. Jewell},
  title =        {Estimation of Treatment Effects in Randomized Trials with Noncompliance and a Dichotomous Outcome},
  institution =  {Division of Biostatistics, University of California,
Berkeley},
  year =         {2004},
  type =         {Technical Report 157},
  OPTnote =      {http://www.bepress.com/ucbbiostat/paper157},
month =        {September},
}
@TECHREPORT{Bein&Hubbard&vanderLaan05,
 author =       {E. Bein and A.E. Hubbard and M.J. van der Laan},
  title =        {Estimating Function Based Cross-Validation in
Estimation of the Causal Effect in Randomized Trials},
  institution =  {Division of Biostatistics, University of California,
Berkeley},
  year =         {2005},
  type =         {Technical Report},
}





@TECHREPORT{vanderLaan&DudoitTechRep130,
  author =       {M.J. van der Laan and S. Dudoit},
  title =        {Unified cross-validation methodology for
selection among estimators and a general cross-validated adaptive
epsilon net estimator: Finite sample oracle inequalities and
examples},
  institution =  {Division of Biostatistics, University of California,
Berkeley},
  year =         {2003},
  type =         {Technical Report 130},
  month =        {Nov.},
}


@TECHREPORT{Molinaroetal05,
  author =       {A.M. Molinaro and M.J. van der Laan and D.H. Moore and K. Kerlikowske},
  title =        {Survival point estimate prediction in matched and non-matched case-control subsample designed studies},
  institution =  {Division of Biostatistics, University of California,
Berkeley},
  year =         {2005},
  note =         {http://www.bepress.com/ucbbiostat/paper149},
}


@TECHREPORT{DudoitetalSIGKDD04,
  author =       {S. Dudoit and M.J. van der Laan and S. Kele\c{s} and A.
M. Molinaro and S. E. Sinisi
and S.L. Teng},
  title =        {Loss-Based Estimation with Cross-Validation:
Applications to Microarray Data
Analysis and Motif Finding.},
  institution =  {Division of Biostatistics, University of California,
Berkeley},
  year =         {2004},
  note =         {to appear in \emph{SIGKDD} Explorations on Microarray Data Mining},
}

@Book{Friedman&Furberg&Demets98,
  author =       {L.M.Friedman and C.D. Furberg and D.L. DeMets},
  title =        {Fundamentals of Clinical Trials},
  publisher =    {Springer-Verlag New York},
  year =         {1998}
}

@Book{ABGK,
  author =       {P.K. Andersen and O. Borgan and R.D. Gill and N. Keiding},
  title =        {Statistical Models Based on Counting Processes},
  publisher =    {Springer-Verlag New York},
  year =         {1993}
}
@Article{Wittes&Brittain90,
  author =   {J. Wittes and E. Brittain},
  title =    {The role of internal pilot studies in increasing efficiency of clinical trials},
journal =      {Statistics in Medicine},
  year =     {1999},
  OPTkey =   {},
  volume =   {9},
  number =   {},
  pages =    {65--72},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

%references for direct and indirect effects:
@InCollection{Robins03,
  author =   {J.M. Robins},
  title =    {Semantics of causal DAG models and the identification of direct and
indirect effects},
  booktitle =    {Highly Structured Stochastic Systems},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher = {Oxford University Press, Oxford},
  year =     {2003},
  editor =   {P. Green, N. Hjort, and S. Richardson},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {70--81},
  OPTnote =      {},
  OPTannote =    {}
}

@InCollection{Hubbard&vanderLaan&Robins99,
  author =   {A. Hubbard and M.J. van der Laan and J.M. Robins},
  title =    {Nonparametric locally ecient
estimation of the treatment specic survival distribution with right censored data
and covariates in observational studies},
  booktitle =    {Statistical Models in Epidemiology, The Environment and Clinical Trials},
  publisher = {Springer Verlag},
  year =     {1999},
editor={M.E. Halloran and D. Berry},
volume={116},
pages={135--178},
  series =   {IMA Volumes in Mathematics and its Applications, Ed. M.E. Halloran and D. Berry}
}

@TechReport{Pearl01,
  author =   {J. Pearl},
  title =    {Cognitive systems Laboratory},
  institution =  {University of California, Los Angeles, Department of Computer Science},
  year =     {2001},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Pearl00,
  author =   {J. Pearl},
  title =    {Causality: Models, Reasoning, and Inference},
  publisher =    {Cambridge University Press, Cambridge},
  year =     {2000},
  OPTkey =   {},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  series =   {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Robins&Greenland92,
  author =   {J.M. Robins and S. Greenland},
  title =    {Identifiability and exchangeability for direct and indirect
effects},
  journal =      {Epidemiology},
  year =     {1992},
  OPTkey =   {},
  volume =   {3},
  number =   {0},
  pages =    {143--155},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{vanderLaan95,
  author =   {M.J. van der Laan},
  title =    {Identity for NPMLE in missing data and biased sampling models},
  journal =      {Bernoulli},
  year =     {1995},
  OPTkey =   {},
  volume =   {1},
  number =   {4},
  pages =    {335--341},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{vanderLaan98,
  author =   {M.J. van der Laan},
  title =    {Identity for NPMLE in Censored Data Models},
  journal =      {Lifetime Data Models},
  year =     {1998},
  OPTkey =   {},
  volume =   {4},
  number =   {0},
  pages =    {83--102},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Klaassen86,
  author =   {C.A.J. Klaassen},
  title =    {Consistent estimation of the influence function of locally asymptotically linear estimators},
  journal =      {Annals of Statistics},
  year =     {1987},
  OPTkey =   {},
  volume =   {15},
  number =   {},
  pages =    {1548--1562},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}





%the next references are for instrumental variable article
@Article{Robins&Rotnitzky04,
  author =   {J.M. Robins and A. Rotnitzky},
  title =    {Estimation of Treatment Effects in Randomized Trials
with Noncompliance and a Dichotomous Outcome using Structural Nested
Mean Models},
  journal =      {Biometrika},
  year =     {2004},
  OPTkey =   {},
  volume =   {0},
  number =   {0},
  pages =    {0},
  OPTmonth =     {},
  OPTnote =      {To Appear},
  OPTannote =    {}
}

@Article{Vandervaart91,
  author =   {A.W. van der Vaart},
  title =    {On differentiable functionals},
  journal =      {Annals of Statistics},
  year =     {1991},
  OPTkey =   {},
  volume =   {19},
  number =   {},
  pages =    {178--204},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}




@Article{Rubin78,
  author =   {D.B. Rubin},
  title =    {Bayesian Inference for causal effects: the role of randomization},
  journal =      {Annals of Statistics},
  year =     {1978},
  OPTkey =   {},
  volume =   {6},
  number =   {},
  pages =    {34--58},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Neyman23,
  author =   {Neyman, J.},
  title =    {On the application of probability theory to agricultural
experiments},
  journal =      {Statistical Science},
  year =     {1990},
  OPTkey =   {},
  volume =   {5},
  number =   {},
  pages =    {465--480},
  OPTmonth =     {},
  OPTnote =      {Translation of 1923 article},
  OPTannote =    {}
}
@Article{Robins86,
  author =   {J.M. Robins},
  title =    {A new approach to causal inference in mortality studies with sustained exposure periods - Application to control of the healthy worker survivor effect},
  journal =      {Mathematical Modelling},
  year =     {1986},
  OPTkey =   {},
  volume =   {7},
  number =   {},
  pages =    {1393--1512},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}





@Article{Robins94,
  author =   {J.M. Robins},
  title =    {Correcting for non-compliance in randomized trials
using structural nested mean models},
  journal =      {Communications in Statistics},
  year =     {1994},
  OPTkey =   {},
  volume =   {23},
  number =   {},
  pages =    {2379--2412},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Vansteelandt03,
  author =   {S. Vansteelandt and E. Goetghebeur},
  title =    {Causal inference with generalized structural  mean
models},
  journal =      {Journal of the Royal Statistical Society, Series B},
  year =     {2003},
  OPTkey =   {},
  volume =   {23},
  number =   {},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {In print},
  OPTannote =    {}
}

@incollection {Robins97a,
   AUTHOR = {Robins, J.M.},
    TITLE = {Structural Nested Failure Time Models},
BOOKTITLE = {The Encyclopedia of Biostatistics},
PUBLISHER = {John Wiley and Sons},
  ADDRESS = {Chichester, UK},
     YEAR = {1997},
   EDITOR = {Armitage, P. and Colton, T. and Andersen, P.K. and Keiding, N.}
}
@article {hernan_brumback_robins,
   AUTHOR = {Hernan, M. A. and Brumback, B. and Robins, J. M.},
    TITLE = {Marginal structural models to estimate the causal effect of zidovudine on the survival of {HIV}-positive men},
  JOURNAL = {Epidemiology},
   VOLUME = {11},
   NUMBER = {5},
     YEAR = {2000},
    PAGES = {561--570}
}
@article {Robins87,
   AUTHOR = {Robins, J.M.},
    TITLE = {Addendum to: ``{A} new approach to causal inference in
             mortality studies with a sustained exposure
             period---application to control of the healthy worker survivor
             effect'' [{M}ath.\ {M}odelling {\bf 7} (1986), no.\ 9-12,
             1393--1512; {M}{R} 87m:92078]},
  JOURNAL = {Comput. Math. Appl.},
 FJOURNAL = {Computers \& Mathematics with Applications. An International
             Journal},
   VOLUME = {14},
     YEAR = {1987},
   NUMBER = {9-12},
    PAGES = {923--945},
     ISSN = {0097-4943},
    CODEN = {CMAPDK},
}

@article {robins_hernan_brumback,
   AUTHOR = {Robins, J. M. and Hernan, M. A. and Brumback, B.},
    TITLE = {Marginal structural models and causal inference in epidemiology},
  JOURNAL = {Epidemiology},
   VOLUME = {11},
   NUMBER = {5},
     YEAR = {2000},
    PAGES = {550--560}
}





@article {Bryan&Yu&vanderLaan03,
   AUTHOR = {Bryan, J. and Yu, Z. and van der Laan, M.J.},
    TITLE = {Analysis of Longitudinal Marginal Structural Models},
  JOURNAL = {Biostatistics},
   VOLUME = {5},
   NUMBER = {3},
     YEAR = {2003},
    PAGES = {361--380}
}

@TechReport{Yu&vanderLaan03,
  author =   {Yu, Z. and van der Laan, M.J.},
  title =    {Double Robust Estimation in Longitudinal Marginal Structural
                    Models},
  institution =  {Division of Biostatistics, University of California,
Berkeley},
  year =     {2003},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {132},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/ucbbiostat/paper132},
  OPTannote =    {}
}

@Article{Neugebauer&vanderLaan05,
  author =   {Neugebauer, R. and van der Laan, M.J.},
  title =    {Why prefer double robust estimates},
  journal =      {Journal of Statistical Planning and Inference},
  year =     {2005},
  OPTkey =   {},
  volume =   {129},
  number =   {1-2},
  pages =    {405--426},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@article {Murphy03,
   AUTHOR = {Murphy, S.A.},
    TITLE = {Optimal dynamic treatment regimes},
  JOURNAL = {Journal of the Royal Statistical Society: Series B},
   VOLUME = {65},
   NUMBER = {2},
     YEAR = {2003},
    PAGES = {?}
}
@article {Robins03a,
   AUTHOR = {Robins, J.M.},
    TITLE = {Discussion of ''{O}ptimal dynamic treatment regimes" by {S}usan {A}. {M}urphy},
  JOURNAL = {Journal of the Royal Statistical Society: Series B},
   VOLUME = {65},
   NUMBER = {2},
     YEAR = {2003},
    PAGES = {355--366}
}

@article {Murphy&vanderLaan&Robins01,
   AUTHOR = {S.A. Murphy and M.J. van der Laan and J.M. Robins},
    TITLE = {Marginal mean models for dynamic treatment regimens},
  JOURNAL = {Journal of the American Statistical Association},
   VOLUME = {96},
   NUMBER = {},
     YEAR = {2001},
    PAGES = {1410--1424}
}
@incollection {Robins98,
    AUTHOR = {Robins, J.M.},
     TITLE = {Marginal structural models versus structural nested models as
              tools for causal inference},
 BOOKTITLE = {Statistical models in epidemiology, the environment, and
              clinical trials (Minneapolis, MN, 1997)},
     PAGES = {95--133},
 PUBLISHER = {Springer},
   ADDRESS = {New York},
      YEAR = {2000},
   MRCLASS = {62N01 (62G08 62P10)},
  MRNUMBER = {2001a:62124},
}
%Robins, J.M. (2003). Discussion of "Optimal dynamic treatment regimes". by Susan A. Murphy.
  %Journal of the Royal Statistical Society: Series B, 65(2):355-366.
@InCollection{Robins97,
  author =   {J.M. Robins},
  title =    {Causal Inference from Complex Longitudinal Data},
  booktitle =    {Latent Variable Modeling and Applications to Causality},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher = {Springer Verlag, New York},
  year =     {1997},
  editor =   {M. Berkane, Editor},
  OPTvolume =    {120},
  OPTnumber =    {},
  OPTseries =    {Lecture Notes in Statistics},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {69--117},
  OPTnote =      {},
  OPTannote =    {}
}

@InCollection{Robins89,
  author =   {J.M. Robins},
  title =    {The analysis of randomized and non-randomized AIDS
treatment trials using a new approach in causal inference in longitudinal studies},
  booktitle =    {Health Service Methodology: A Focus on AIDS},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher = {U.S. Public Health Service, National Center for Health SErvices Research},
  year =     {1989},
  editor =   {L. Sechrest and H. Freeman and A. Mulley},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {Lecture Notes in Statistics},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {Washington D.C.},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {113--159},
  OPTnote =      {},
  OPTannote =    {}
}



@TechReport{Abadie00,
  author =   {A. Abadie},
  title =    {Semiparametric estimation of instrumental variables models for causal effects},
  institution =  {NBER Technical Working Paper},
  year =     {2000},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {260},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Abadie03,
  author =   {A. Abadie},
  title =    {Semiparametric instrumental variable estimation of treatment response models},
  journal =      {Journal of Econometrics},
  year =     {2003},
  OPTkey =   {},
  volume =   {113},
  number =   {},
  pages =    {231-263},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Abadie03,
  author =   {A. Abadie},
  title =    {Semiparametric instrumental variable estimation of treatment response models},
  journal =      {Journal of Econometrics},
  year =     {2003},
  OPTkey =   {},
  volume =   {113},
  number =   {},
  pages =    {231-263},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@TechReport{Wang&Vanderlaan04,
  author =   {Y. Wang and M.J. van der Laan},
  title =    {Data adaptive estimation of the treatment specific mean},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =     {2004},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {159},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/ucbbiostat/paper159},
  OPTannote =    {}
}
@TechReport{Yu&vanderLaan02,
  author =   {Z. Yu and M.J. van der Laan},
  title =    {Construction of counterfactuals and the {G}-computation formula},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =     {2002},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {122},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/ucbbiostat/paper122},
  OPTannote =    {}
}
@TechReport{Yu&Vanderlaan03,
  author =   {Z. Yu and M.J. van der Laan},
  title =    {Measuring treatment effects using semiparametric models},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =     {2003},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {136},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/ucbbiostat/paper136},
  OPTannote =    {}
}

@Article{Angristetal96,
  author =   {J. Angrist and G. Imbens and D.B. Rubin},
  title =    {Identification of causal effects using instrumental variables},
  journal =      {Journal of the American Statistical Association},
  year =     {1996},
  OPTkey =   {},
  volume =   {91},
  number =   {},
  pages =    {444-555},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Robins&Rotnitzky01A,
  author =   {J.M Robins and A. Rotnitzky},
  title =    {Comment on {I}nference for semiparametric models: some questions
  and an answer, by {B}ickel, {P}.{J}. and {K}won, {J}.},
  journal =      {Statistica Sinica},
  year =     {2001},
  OPTkey =   {},
  volume =   {11},
  number =   {},
  pages =    {920-935},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Angrist01,
  author =   {J. Angrist},
  title =    {Estimation of limited dependent variable models with dummy endogenous regressors: simple strategies for empirical practice},
  journal =      {Journal of Business and Economics Statistics},
  year =     {2001},
  OPTkey =   {},
  volume =   {19},
  number =   {},
  pages =    {1--16},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Chamberlain87,
  author =   {G. Chamberlain},
  title =    {Asymptotic efficiency in estimation with conditional moment
restrictions},
  journal =      {Journal of Econometrics},
  year =     {1987},
  OPTkey =   {},
  volume =   {34},
  number =   {},
  pages =    {305--334},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Hiranoetal00,
  author =   {K. Hirano and G. Imbens and D.B. Rubin and X-H. Zhou},
  title =    {Assessing the effects of influenza vaccine in an encouragement design},
  journal =      {Biostatistics},
  year =     {2000},
  OPTkey =   {},
  volume =   {1},
  number =   {},
  pages =    {69--88},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Neyman23,
  author =   {J. Neyman},
  title =    {Sur les applications de la thar des probabilites aux
experiences Agaricales: Essay des principle (1923). Excerpts reprinted (1990) in
English (D. Dabrowska and T. Speed), Trans.},
  journal =      {Statistical Science},
  year =     {1990},
  OPTkey =   {},
  volume =   {5},
  number =   {},
  pages =    {463--472},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



optimal structural nested models for optimal
sequential decisions Proceedings of the 2nd seattle symposium in
biostatistics eds. Lin DY, Heagerty PJ  Springer Verlag Lecture Notes in
Statisitics No. 179  pages 189-326

@InProceedings{Robins05,
  author =   {J.M. Robins},
  title =    {Optimal structural nested models for optimal sequential decisions},
  booktitle =    {Proceedings of the 2nd Seattle symposium in
biostatistics},
  pages =    {189--326},
  year =     {2005},
  editor =   {Lin, D.Y, Heagerty P.J},
  volume =   {179},
  organization = {},
OPTpublisher = {Springer Verlag Lecture Notes in Statistics}
}


@TechReport{Robins05tech,
  author =   {J.M. Robins},
  title =    {Optimal structural nested models for optimal sequential decisions},
  institution =  {Department of Biostatistics, Havard University},
  year =     {2005},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}





@InProceedings{AIC,
  author =   {H. Akaike},
  title =    {Information theory and an extension of the maximum likelihood principle},
  booktitle =    {Second International Symposium on Information Theory},
  pages =    {267-281},
  year =     {1973},
  editor =   {B.N. Petrov and F. Csaki},
  organization = {Budapest: Academiai Kiado}
}


@Article{Balke&Pearl97,
  author =   {A. Balke and J. Pearl},
  title =    {Bound on treatment effects from studies with imperfect compliance},
  journal =      {Journal of the American Statistical Association},
  year =     {1997},
  OPTkey =   {},
  volume =   {92},
  number =   {},
  pages =    {1172--1176},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{Balke&Pearl94,
author =     {A. Balke and J. Pearl},
  title =    {Counterfactual probabilities: Computational methods, bounds, and applications},
  booktitle =    {In Proceedings of the 12th National Conference on Artificial Intelligence},
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {230--237},
  year =     {1994},
  OPTeditor =    {},
  volume =   {I},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {Menlo Park, CA},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {MIT Press},
  OPTnote =      {},
  OPTannote =    {}
}






@Article{Ambroise&McLachlan02,
  author =   {C. Ambroise and G. J. McLachlan},
  title =    {Selection bias in gene extraction on the basis of microarray gene-expression data},
  journal =      PNAS,
  year =     {2002},
  OPTkey =   {},
  volume =   {99},
  number =   {10},
  pages =    {6562--6566},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@InCollection{Arabie&Hubert96,
  author =   {P. Arabie and L. J. Hubert},
  title =    {An overview of combinatorial data analysis},
  booktitle =    {Clustering and Classification},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher = {World Scientific Publishing Co.},
  year =     {1996},
  editor =   {P. Arabie and L. J. Hubert and G. De Soete},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {River Edge, NJ},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {5--63},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{BIC,
  author =   {G. Schwartz},
  title =    {Estimating the Dimension of a Model},
  journal =      {Annals of Statistics},
  year =     {1978},
  volume =   {6},
  pages =    {461-464}
}


@Article{Barnard,
  author =   {M. Barnard},
  title =    {The secular variations of skull characters in four series of Egyptian skulls},
  journal =      {Annals of Eugenics},
  year =     {1935},
  OPTkey =   {},
  volume =   {6},
  OPTnumber =    {},
  pages =    {352--371},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@InProceedings{BenHuretal02,
  author =   {A. Ben-Hur and A. Elisseeff and I. Guyon},
  title =    {A stability based method for discovering structure in clustered data},
  booktitle =    {Pacific Symposium on Biocomputing},
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {6--17},
  year =     {2002},
  OPTeditor =    {},
  volume =   {7},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Benjamini&Hochberg95,
  author =   {Y. Benjamini and Y. Hochberg},
  title =    {Controlling the false discovery rate: a practical and powerful approach to multiple testing},
  journal =      {J. R. Statist. Soc. B},
  year =     {1995},
  OPTkey =   {},
  volume =   {57},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {289--300},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Benjamini&Yekutieli01,
  author =   {Y. Benjamini and D. Yekutieli},
  title =    {The control of the false discovery rate in multiple testing under
   dependency},
  journal =      {Annals of Statistics},
  year =     {2001},
  OPTkey =   {},
  volume =   {29},
  number =   {4},
  pages =    {1165--1188},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Beran88,
  author =   {R. Beran},
  title =    {Balanced simultaneous confidence sets},
  journal =      JASA,
  year =     {1988},
  OPTkey =   {},
  volume =   {83},
  OPTnumber =    {},
  pages =    {679--686},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Bock85,
  author =   {H-H Bock},
  title =    {On some significance tests in cluster analysis},
  journal =      {Journal of Classification},
  year =     {1985},
  OPTkey =   {},
  volume =   {2},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {77--108},
  OPTnote =      {},
  OPTannote =    {}
}



@InCollection{Bock96,
  author =   {H-H Bock},
  title =    {Probability models and hypotheses testing in partitioning cluster analysis},
  booktitle =    {Clustering and Classification},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher = {World Scientific Publishing Co.},
  year =     {1996},
  editor =   {P. Arabie and L. J. Hubert and G. De Soete},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {River Edge, NJ},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {377--453},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Boldricketal02,
  author =   {J. C. Boldrick and A. A. Alizadeh and M. Diehn and S. Dudoit and C. L. Liu and C. E. Belcher and D. Botstein and L. M. Staudt and P. O. Brown
and D. A. Relman},
  title =    {Stereotyped and specific gene expression programs in human innate immue responses to bacteria},
  journal =      PNAS,
  year =     {2002},
  OPTkey =   {},
  volume =   {99},
  number =   {2},
  pages =    {972--977},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Bozdogan00,
  author =   {H. Bozdogan},
  title =    {Akaike's information criterion and recent developments in information complexity},
  journal =      {Journal of Mathematical Psychology},
  year =     {2000},
  volume =   {44},
  pages =    {62-91}
}




@InCollection{Bozdogan93,
  author =   {H. Bozdogan},
  title =    {Choosing the number of component clusters in the mixture model  using a new informational complexity criterion of the inverse Fisher information matrix},
  booktitle =    {Information and Classification},
  publisher = {Heidelberg: Springer Verlag},
  editor = {O. Opitz and B. Lausen and R. Klar},
  year =     {1993},
  series =   {}
}

@Article{Braver,
  author =   {S. L. Braver},
  title =    {On splitting the tails unequally: a new perspective on one-versus two-tailed tests},
  journal =      {Educational and Psychological Measurement},
  year =     {1975},
  OPTkey =   {},
  volume =   {35},
  OPTnumber =    {},
  pages =    {283--301},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Breckenridge89,
  author =   {J. Breckenridge},
  title =    {Replicating cluster analysis: Method, consistency and validity},
  journal =      {Multivariate Behavioral Research},
  year =     {1989},
  OPTkey =   {},
  volume =   {24},
  OPTnumber =    {},
  pages =    {147--161},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Breiman&Spector92,
  author =   {L. Breiman and P. Spector},
  title =    {Submodel Selection and Evaluation in Regression. The
  $X$ Random Case},
  journal =      {International Statistical Review},
  year =     {1992},
  OPTkey =   {},
  volume =   {60},
  OPTnumber =    {},
  pages =    {291--319},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Breiman01,
  author =   {L. Breiman},
  title =    {Statistical modeling: the two cultures},
  journal =      {Statistical Science},
  year =     {2001},
  OPTkey =   {},
  volume =   {16},
  number =   {3},
  pages =    {199--215},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{BreimanAnnals96,
  author =   {L. Breiman},
  title =    {Heuristics of instability and stabilization in model selection},
  journal =      {Annals of Statistics},
  year =     {1996},
  OPTkey =   {},
  volume =   {24},
  number =   {6},
  pages =    {2350--2383},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{BreimanArcing,
  author =   {L. Breiman},
  title =    {Arcing classifiers},
  journal =      {Annals of Statistics},
  year =     {1998},
  OPTkey =   {},
  volume =   {26},
  OPTnumber =    {},
  pages =    {801-824},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{BreimanBagging,
  author =   {L. Breiman},
  title =    {Bagging predictors},
  journal =      {Machine Learning},
  year =     {1996},
  OPTkey =   {},
  volume =   {24},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {123-140},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{BreimanCPD,
  author =   {L. Breiman},
  title =    {Using Convex pseudo-data to increase prediction accuracy},
  institution =  {Department of Statistics, U.C. Berkeley},
  year =     {1998},
  OPTkey =   {},
  OPTtype =      {},
  number =   {513},
  OPTaddress =   {},
  month =    {March},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{BreimanJASA92,
  author =   {L. Breiman},
  title =    {The Little Bootstrap and Other Methods for
  Dimensionality Selection in Regression: $X$-Fixed Prediction Error},
  journal =      JASA,
  year =     {1992},
  OPTkey =   {},
  volume =   {87},
  number =   {419},
  pages =    {738--754},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@TechReport{BreimanOB,
  author =   {L. Breiman},
  title =    {Out-of-bag estimation},
  institution =  {Department of Statistics, U.C. Berkeley},
  year =     {1996},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@TechReport{BreimanRanForests,
  author =   {L. Breiman},
  title =    {Random forests - random features},
  institution =  {Department of Statistics, U.C. Berkeley},
  year =     {1999},
  OPTkey =   {},
  OPTtype =      {},
  number =   {567},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Breimanetal84,
  author =   {L. Breiman and J. H. Friedman and R. Olshen and C. J. Stone},
  title =    {Classification and regression trees},
  publisher =    {Wadsworth International Group},
  year =     {1984},
  OPTkey =   {},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  series =   {The Wadsworth statistics/probability series},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Book{Hastieetal02,
  author =   {T. Hastie and R. Tibshirani and J. Friedman},
  title =    {The Elements of Statistical Learning},
  publisher =    {Springer},
  year =     {2002},
  OPTkey =   {},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  series =   {Springer Series in Statistics},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Broman01,
  author =   {K. W. Broman},
  title =    {Review of statistical methods for QTL mapping in experimental crosses},
  journal =      {Lab Animal},
  year =     {2001},
  OPTkey =   {},
  volume =   {30},
  number =   {7},
  pages =    {44--52},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@PhdThesis{Broman97,
  author =   {K. W. Broman},
  title =    {Identifying quantitative trait loci in experimental crosses},
  school =   {Department of Statistics, U.C. Berkeley},
  year =     {1997},
  OPTkey =   {},
  type =     {Ph.{D}. thesis},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Brown&Koplowitz79,
  author =   {T. A. Brown and J. Koplowitz},
  title =    {The weighted nearest neighbor rule for class dependent sample sizes},
  journal =      {IEEE Transactions on Information Theory},
  year =     {1979},
  OPTkey =   {},
  volume =   {25},
  number =   {5},
  pages =    {617--619},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Buhlmann&Yu,
  author =   {P. Buhlmann and B. Yu},
  title =    {Explaining Bagging.},
  journal =      {Annals of Statistics},
  year =     {(Accepted)},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTpages =     {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Burgessvm98,
  author =   {C. J. C. Burges},
  title =    {A tutorial on support vector machines for pattern recognition},
  journal =      {Data Mining and Knowledge Discovery},
  year =     {1998},
  OPTkey =   {},
  volume =   {2},
  number =   {},
  pages =    {121--167},
  month =    {December},
  OPTnote =      {},
  OPTannote =    {}
}



@article{Burman89,
AUTHOR={P. Burman},
TITLE={A comparative study of ordinary cross-validation, $v$-fold cross-validati
on and the repeated learning testing methods},
JOURNAL={Biometrika},
VOLUME={76},
YEAR={1989},
PAGES={503-514}
}





@TechReport{Buttrey&Karo02,
  author =   {S. E. Buttrey and C. Karo},
  title =    {Using k--neareset neighbor classification in the leaves of a tree},
  institution =  {Naval Postgraduate School, Monterey, CA},
  year =     {2002},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Calinskietal,
  author =   {R. Calinski and J. Harabasz},
  title =    {A dendrite method for cluster analysis},
  journal =      {Communications in Statistics},
  year =     {1974},
  OPTkey =   {},
  volume =   {3},
  OPTnumber =    {},
  pages =    {1--27},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Callowetal00,
  author =   {M. J. Callow and S. Dudoit and E. L. Gong and T. P. Speed and E. M. Rubin},
  title =    {Microarray expression profiling identifies genes with altered expression in {HDL} deficient mice},
  journal =      {Genome Research},
  year =     {2000},
  OPTkey =   {},
  volume =   {10},
  number =   {12},
  OPTmonth =     {},
  pages =    {2022--2029},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Chambers98,
   author = {J. M. Chambers},
   title = {Programming with Data: A Guide to the S Language},
   publisher = {Springer-Verlag New York},
   year = {1998}
}
@Book{Diggleetal2002,
   author = {Peter J. Diggle and P. Heagerty and K-Y Liang and S.L. Zeger},
   title = {Analysis of Longitudinal Data},
   publisher = {Oxford University Press},
   year = {2002 (Second Edition)}
}

@TechReport{ChangLin2001,
  author =       {C.-C. Chang and C.-J. Lin},
  title =        {LIBSVM: a Library for Support Vector Machines (Version 2.31)},
  institution =  {},
  year =         {2001},
  OPTkey =       {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  note =         {\\ {\tt http://www.csie.ntu.edu.tw/~cjlin/papers/libsvm2.ps.gz}},
  OPTannote =    {}
}



@Article{Changetal02,
  author =   {H. Y. Chang and J. T. Chi and S. Dudoit and C. Bondre and M. van de Rijn and D. Botstein D and P. O. Brown},
  title =    {Diversity, topographic differentiation, and positional memory in human fibroblasts},
  journal =      PNAS,
  year =     {2002},
  OPTkey =   {},
  volume =   {99},
  number =   {20},
  pages =    {12877--12882},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Chenetal02,
  author =   {X. Chen and S. T. Cheung and S. So and S. T. Fan and C. Barry and J. Higgins and K.-M. Lai and J. Ji and S. Dudoit and I. O. L. Ng and M. van de Rijn and D. Botstein and P. O. Brown },
  title =    {Gene expression patterns in human liver cancers},
  journal =      {Molecular Biology of the Cell},
  year =     {2002},
  OPTkey =   {},
  volume =   {13},
  number =   {6},
  pages =    {1929--1939},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Cleveland&Devlin88,
  author =   {W. S. Cleveland and S. J. Devlin},
  title =    {Locally-Weighted Regression: An Approach to Regression Analysis by Local Fitting},
  journal =      JASA,
  year =     {1988},
  OPTkey =   {},
  volume =   {83},
  OPTnumber =    {},
  pages =    {596--610},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Cleveland79,
  author =   {W. S. Cleveland},
  title =    {Robust locally weighted regression and smoothing scatterplots},
  journal =      JASA,
  year =     {1979},
  OPTkey =   {},
  volume =   {74},
  number =   {368},
  pages =    {829--836},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Correa&Wolfson99,
  author =   {J. A. Correa and D. B. Wolfson},
  title =    {Length-bias: some characterizations and applications},
  journal =      {Journal of Statistical Computation and Simulation},
  year =     {1999},
  OPTkey =   {},
  volume =   {64},
  Tnumber =      {3},
  pages =    {209--219},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Correaetal02,
  author =   {J. A. Correa and S. Dudoit and D. R. Goldstein},
  title =    {Multiple testing in the survival analysis of microarray data},
  OPTjournal =   {Statistics in Medicine},
  year =     {2002},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTpages =     {},
  OPTmonth =     {},
  note =     {(Submitted)},
  OPTannote =    {}
}


@Article{CortesVapnik95,
  author =   {C. Cortes and V. Vapnik},
  title =    {Support-vector networks},
  journal =      {Machine Learning},
  year =     {1995},
  OPTkey =   {},
  volume =   {20},
  number =   {},
  pages =    {273-297},
  month =    {December},
  OPTnote =      {},
  OPTannote =    {}
}

@InProceedings{Davies&Bouldin,
  author =   {D. Davies and D. Bouldin},
  title =    {A cluster separation measure},
  booktitle =    {IEEE Transactions on Pattern Analysis and Machine Intelligence},
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {224--227},
  year =     {1979},
  OPTeditor =    {},
  volume =   {1},
  OPTnumber =    {PAMI-1},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@article {Davis89,
AUTHOR ={R. B. Davis  and J. R. Anderson},
TITLE ={Exponential survival trees},
JOURNAL = {Statistics in Medicine},
VOLUME = {8},
YEAR ={1989},
NUMBER={},
PAGES = {947-961},
ISSN = {},
CODEN = {},
}




@InCollection{Day96,
  author =   {W. H. E. Day},
  title =    {Complexity theory: {A}n introduction for practitioners of classification},
  booktitle =    {Clustering and Classification},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher = {World Scientific Publishing Co.},
  year =     {1996},
  editor =   {P. Arabie and L. J. Hubert and G. De Soete},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {River Edge, NJ},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {199--233},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Dettling&Buhlmann02,
  author =   {M. Dettling and P. B\"{u}lmann},
  title =    {How to Use Boosting for Tumor Classification with Gene Expression Data},
  journal =      {},
  year =     {2002},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTpages =     {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Dudoit&Fridlyand02II,
  author =   {S. Dudoit and J. Fridlyand},
  title =    {Bagging to improve the accuracy of a clustering procedure},
  OPTjournal =   {Bioinformatics},
  year =     {2002},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTpages =     {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
  }



@InCollection{Dudoit&FridlyandCRC02,
  author =   {S. Dudoit and J. Fridlyand},
  title =    {Classification in microarray experiments},
  booktitle =    {Statistical Analysis of Gene Expression Microarray Data},
  OPTcrossref =  {},
  OPTkey =   {},
  OPTpages =     {},
  publisher =    {Chapman \& Hall/CRC},
  year =     {2002},
  editor =   {T. P. Speed},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTtype =      {},
  OPTchapter =   {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  note =     {(To appear)},
  OPTannote =    {}
}

@Article{Dudoit&FridlyandGenBio02,
  author =   {S. Dudoit and J. Fridlyand},
  title =    {A prediction-based resampling method to estimate the number of clusters in a dataset},
  journal =      {Genome Biology},
  year =     {2002},
  OPTkey =   {},
  volume =   {3},
  number =   {7},
  pages =    {0036.1--0036.21},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@TechReport{Dudoit&FridlyandTechRep600,
  author =   {S. Dudoit and J. Fridlyand},
  title =    {Applications of resampling methods to estimate the number of clusters and to improve the accuracy of a clustering method},
  institution =  {Department of Statistics, Uiversity of California, Berkeley},
  year =     {2001},
  OPTkey =   {},
  OPTtype =      {},
  number =   {600},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {},
  url={stat-www.berkeley.edu/users/sandrine/publications.html},
}

S. Dudoit, M.J. van der Laan (2005),
 Asymptotics of cross-validated
risk estimation in estimator selection and performance assessment.
{\em Statistical Methodology 2}, 2, 131--54.

@Article{Dudoit&vanderLaan05,
  author =   {S. Dudoit and M.J. van der Laan},
  title =    {Asymptotics of cross-validated risk estimation in estimator selection and performance assessment},
  journal =      {Statistical Methodology},
  year =     {2005},
  OPTkey =   {},
  volume =   {2},
  number =   {2},
  OPTmonth =     {},
  pages =    {131--154},
  OPTnote =      {www.bepress.com/ucbbiostat/paper126},
  OPTannote =    {}
}
@Article{Dudoit&SpeedAnnals99,
  author =   {S. Dudoit and T. P. Speed},
  title =    {A score test for linkage using identity by descent data from sibships},
  journal =      {Annals of Statistics},
  year =     {1999},
  OPTkey =   {},
  volume =   {27},
  number =   {3},
  OPTmonth =     {},
  pages =    {943--986},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Dudoit&SpeedBios00,
  author =   {S. Dudoit and T. P. Speed},
  title =    {A score test for the linkage analysis of qualitative and quantitative traits based on identity by descent data on sib-pairs},
  journal =      {Biostatistics},
  year =     {2000},
  OPTkey =   {},
  volume =   {1},
  number =   {1},
  pages =    {1--26},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}




@InCollection{Dudoit&SpeedIMA99,
  author =   {S. Dudoit and T. P. Speed},
  title =    {Triangle constraints for sib-pair identity by descent probabilities under a general multilocus model for disease susceptibility},
  booktitle =    {Statistics in Genetics},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher =    {Springer-Verlag},
  year =     {1999},
  editor =   {M. E. Halloran and S. Geisser},
  volume =   {112},
  OPTnumber =    {},
  series =   {IMA Volumes in Mathematics and its Applications},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {New York},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {181--221},
  OPTnote =      {},
  OPTannote =    {}
}

@InCollection{Dudoit&YangSpringer03,
  author =   {S. Dudoit and Y. H. Yang},
  title =    {Bioconductor {R} packages for exploratory analysis and normalization of c{DNA} microarray data},
  booktitle =    {The Analysis of Gene Expression Data: Methods and Software},
  OPTcrossref =  {},
  OPTkey =   {},
  OPTpages =     {},
  publisher =    {Springer, New York},
  year =     {2003},
  editor =   {G. Parmigiani and E. S. Garrett and R. A. Irizarry and S. L. Zeger},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTtype =      {},
  OPTchapter =   {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{DudoitetalJASA02,
  author =       {S. Dudoit and J. Fridlyand and T. P. Speed},
  title =        {Comparison of Discrimination Methods for the Classification of
 Tumors Using Gene Expression Data},
  journal =      JASA,
  year =         {2002},
  OPTkey =       {},
  volume =    {97},
  number =    {457},
  pages =     {77--87},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{DudoitetalSinica02,
  author =   {S. Dudoit and Y. H. Yang and M. J. Callow and T. P. Speed},
  title =    {Statistical methods for identifying differentially expressed genes in replicated c{DNA} microarray experiments},
  journal =      {Statistica Sinica},
  year =     {2002},
  OPTkey =   {},
  volume =   {12},
  number =   {1},
  pages =    {111--139},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{DudoitetalTechRep110,
  author =   {S. Dudoit and J. P. Shaffer and J. C. Boldrick},
  title =    {Multiple hypothesis testing in microarray experiments},
  institution =  {Division of Biostatistics, University of California, Berkeley},
  year =     {2002},
  OPTkey =   {},
  OPTtype =      {},
  number =   {110},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {},
  url={www.bepress.com/ucbbiostat/paper110/}

}


@Article{Duffy&Quiroz,
  author =   {D. E. Duffy and A. J. Quiroz},
  title =    {A permutation-based algorithm for block clustering},
  journal =      {Journal of Classification},
  year =     {1991},
  OPTkey =   {},
  volume =   {8},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {65--91},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Dunn58,
  author =   {O. J. Dunn},
  title =    {Estimation of the means of dependent variables},
  journal =      {Annals of Mathematical Statistics},
  year =     {1958},
  OPTkey =   {},
  volume =   {29},
  OPTnumber =    {},
  pages =    {1095-111},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Book{Efron&Tibs93,
  author =   {B. Efron and R. J. Tibshirani},
  ALTeditor =    {},
  title =    {An Introduction to the Bootstrap},
  publisher =    {Chapman \& Hall/CRC},
  year =     {1993},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{EfronetalJASA01,
  author =   {B. Efron and R. Tibshirani and J. D. Storey and V. Tusher},
  title =    {Empirical Bayes analysis of a microarray
experiment},
  journal =      JASA,
  year =     {2001},
  OPTkey =   {},
  volume =   {96},
  OPTnumber =    {},
  pages =    {1151--1160},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@TechReport{EfronetalTechRep01,
  author =   {B. Efron and J. D. Storey and R. Tibshirani},
  title =    {Microarrays, empirical Bayes methods, and false discovery
rates},
  institution =  {Department of Statistics, Stanford University},
  year =     {2001},
  OPTkey =   {},
  OPTtype =      {},
  number =   {2001-218},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Finner99,
  author =   {H. Finner},
  title =    {Stepwise multiple test procedures and control of directional errors},
  journal =      {Annals of Statistics},
  year =     {1999},
  OPTkey =   {},
  volume =   {27},
  OPTnumber =    {},
  pages =    {274--289},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Fisher,
  author =   {R. A. Fisher},
  title =    {The use of multiple measurements in taxonomic problems},
  journal =      {Annals of Eugenics},
  year =     {1936},
  OPTkey =   {},
  volume =   {7},
  OPTnumber =    {},
  pages =    {179-188},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Fisher26,
  author =   {R. A. Fisher},
  title =    {The arrangement of field experiments},
  journal =      {J. Min. Agric. Gr. Br},
  year =     {1926},
  OPTkey =   {},
  volume =   {33},
  OPTnumber =    {},
  pages =    {505--513},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{Fix&Hodges,
  author =   {E. Fix and J. Hodges},
  title =    {Discriminatory analysis, nonparametric discrimination: consistency properties},
  institution =  {Randolph Field, Texas: USAF School of Aviation Medicine},
  year =     {1951},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Fowlkes&Mallows83,
  author =   {E. B. Fowlkes and C. L. Mallows},
  title =    {A method for comparing two hierarchical clusterings},
  journal =      JASA,
  year =     {1983},
  OPTkey =   {},
  volume =   {78},
  OPTnumber =    {383},
  OPTmonth =     {},
  pages =    {553--584},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Fowlkesetal88,
  author =   {E. B. Fowlkes and R. Gnanadesikan and J. R. Kettenring},
  title =    {Variable selection in clustering},
  journal =      JC,
  year =     {1988},
  OPTkey =   {},
  volume =   {5},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {205--228},
  OPTnote =      {},
  OPTannote =    {}
}

@TechReport{Fraley&Raftery98,
  author =   {C. Fraley and A. Raftery},
  title =    {How many clusters? Which clustering method? -- answers via model-based cluster analysis},
  institution =  {Department of Statistics, University of Washington},
  year =     {1998},
  OPTkey =   {},
  OPTtype =      {},
  number =   {329},
  OPTaddress =   {},
  OPTmonth =     {},
  note =     {\url{http://www.stat.washington.edu/www/research/reports/1990s/#1998}},
  OPTannote =    {}
}




@Article{Freund&Schapire97,
  author =   {Y. Freund and R. E. Schapire},
  title =    {A decision-theoretic generalization of on-line learning and an application to boosting},
  journal =      {Journal of Computer and System Sciences},
  year =     {1997},
  OPTkey =   {},
  volume =   {55},
  OPTnumber =    {},
  pages =    {119--139},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@PhdThesis{Fridlyand,
  author =   {J. Fridlyand},
  title =    {Resampling methods for variable selection and classification: applications to genomics},
  school =   {Department of Statistics, U.C. Berkeley},
  year =     {2001},
  OPTkey =   {},
  type =     {Ph.{D}. thesis},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{Friedman94 ,
  author =   {J. H. Friedman},
  title =    {Flexible metric nearest neighbor clasification},
  institution =  {Department of Statistics, Stanford University},
  year =     {1994},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@TechReport{Friedman96a,
  author =   {J. H. Friedman},
  title =    {On bias, variance, 0/1-loss, and the curse--of--dimensionality },
  institution =  {Department of Statistics, Stanford University},
  year =     {1996},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{Friedman96b,
  author =   {J. H. Friedman},
  title =    {Another approach to polychotomous classification},
  institution =  {Department of Statistics, Stanford University},
  year =     {1996},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Friedmanetal00,
  author =   {J. Friedman and T. Hastie and R. Tibshirani},
  title =    {Additive logistic regression: a statistical view of boosting},
  journal =      {Annals of Statistics},
  year =     {2000},
  OPTkey =   {},
  volume =   {28},
  OPTnumber =    {},
  pages =    {337--404},
  OPTmonth =     {},
  note =     {(with discussion)},
  OPTannote =    {}
}

@book {GAM,
   AUTHOR = {T. J. Hastie and R.J. Tibshirani},
    TITLE = {Generalized Additive Models},
PUBLISHER = {Chapman and Hall},
  ADDRESS = {London},
     YEAR = {1990},
    PAGES = {},
     ISBN = {},
}



@Article{Gabriel,
  author =   {K. R. Gabriel},
  title =    {The biplot graphic display of matrices with application to principal component analysis},
  journal =      {Biometrika},
  year =     {1971},
  OPTkey =   {},
  volume =   {58},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {453--467},
  OPTnote =      {},
  OPTannote =    {}
}

@InCollection{Gabriel75,
  author =   {K. R. Gabriel},
  title =    {A comparison of some methods of simultaneous inference in {MANOVA}},
  booktitle =    {Multivariate Statistical Methods: Among-groups covariation; Within-group covariation},
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {61--80},
  OPTpublisher = {},
  year =     {1975},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTtype =      {},
  OPTchapter =   {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@InProceedings{GabrielPun,
  author =       {K. R. Gabriel and F. C. Pun},
  title =        {Binary prediction of weather events with several predictors},
  booktitle =    {Sixth Conference on Probability and Statistics in Atmospheric Science},
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {248--253},
  year =     {1979},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  organization = {American Meterological Society},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}


@Unpublished{Ge&Dudoit,
  author =   {Y. Ge and S. Dudoit},
  title =    {Fast algorithm for resampling-based $p$-value adjustment in multiple testing},
  note =     {(In preparation)},
  OPTkey =   {},
  OPTmonth =     {},
  year =     {2002},
  OPTannote =    {}
}

@Article{Geisser75,
  author =   {S. Geisser},
  title =    {The predictive sample reuse method with applications},
  journal =      {Journal of the American Statistical Association},
  year =     {1975},
  volume =   {70},
  pages =    {320-328}
}

@TechReport{Genovese&Wasserman01,
  author =   {C. Genovese and L. Wasserman},
  title =    {Operating Characteristics and Extensions of the FDR Procedure},
  institution =  {Department of Statistics, Carnegie Mellon},
  year =     {2001},
  OPTkey =   {},
  OPTtype =      {},
  number =   {737},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Gnanadesikan&Kettering95,
  author =   {R. Gnanadesikan and J. R. Kettenring},
  title =    {Weighting and selection of variables for cluster analysis},
  journal =      JC,
  year =     {1995},
  OPTkey =   {},
  volume =   {12},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {113--136},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{GoldsteinetalGenEpi00,
  author =   {D. R. Goldstein and S. Dudoit and T. P. Speed},
  title =    {Power of a score test for quantitative trait linkage analysis of relative pairs.},
  journal =      {Genetic Epidemiology},
  year =     {2000},
  OPTkey =   {},
  volume =   {19},
  number =   {Suppl. 1},
  pages =    {S85--S91},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{GoldsteinetalGenEpi01,
  author =   {D. R. Goldstein and S. Dudoit and T. P. Speed},
  title =    {Power and robustness of a score  test for linkage analysis of quantitative traits using identity by descent data on sib pairs},
  journal =      {Genetic Epidemiology},
  year =     {2001},
  OPTkey =   {},
  volume =   {20},
  number =   {4},
  pages =    {415--431},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@article {Gordon85,
AUTHOR ={L. Gordon and R.A. Olshen},
TITLE ={Tree-structured survival analysis},
JOURNAL = {Cancer Treatment Reports},
VOLUME = {69},
YEAR ={1985},
NUMBER={},
PAGES = {10065-1069},
ISSN = {},
CODEN = {},
}



@InCollection{Gordon96,
  author =   {A. D. Gordon},
  title =    {Hierarchical classification},
  booktitle =    {Clustering and Classification},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher = {World Scientific Publishing Co.},
  year =     {1996},
  editor =   {P. Arabie and L. J. Hubert and G. De Soete},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {River Edge, NJ},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {65--121},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Gower&Hand,
  author = {J. C. Gower and D. J. Hand},
  title =    {Biplots},
  publisher =    {Chapman \& Hall},
  year =     {1996},
  OPTkey =   {},
  OPTeditor =    {},
  OPTvolume =    {},
  number =   {54},
  series =   {Monographs on statistics and applied probability},
  OPTaddress =   {},
  edition =      {1st},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@book {Gyorfi02,
   AUTHOR = {L. Gy\"{o}rfi and M. Kohler and A. Krzy\.{z}ak  and H. Walk},
    TITLE = {A Distribution-Free Theory of Nanparametric Regression},
PUBLISHER = {Springer-Verlag},
  ADDRESS = {New York},
     YEAR = {2002},
    PAGES = {100-102},
     ISBN = {}
}




@Book{Gyorfietal02,
  author =   {L. Gy\"orfi and M. Kohler and A. Krzy\'{z}ak and H. Walk},
  ALTeditor =    {},
  title =    {A distribution-free theory of nonparametric regression},
  publisher =    {Springer-Verlag, New York},
  year =     {2002},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Book{HTF01,
  author =   {T. Hastie and R. Tibshirani and J. H. Friedman},
  ALTeditor =    {},
  title =    {The Elements of Statistical Learning : Data Mining, Inference, and Prediction },
  publisher =    {Springer Verlag},
  year =     {2001},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Hansen01,
  author =   {M. H. Hansen  and B. Yu},
  title =    {Model selection and the principle of minimum description length},
  journal =      {Journal of the American Statistical Association},
  year =     {2001},
  volume =   {96},
  pages =    {746-774}
}

@Article{Hardle85a,
  author =   {W. H{\"a}rdle and J. S. Marron},
  title =    {Asymptotic nonequivalence of some bandwidth selectors in nonparametric regression},
  journal =      {Biometrika},
  year =     {1985},
  volume =   {72},
  pages =    {481--484}
}




@Article{Hardle85b,
  author =   {W. H{\"a}rdle and J. S. Marron},
  title =    {Optimal bandwidth selection in nonparametric regression function estimation},
  journal =      {Annals of Statistics},
  year =     {1985},
  volume =   {13},
  pages =    {1465-1481}
}

@Book{Hardle93,
  author =       {W. H{\"a}rdle},
  title =        {Applied Nonparametric Regression},
  publisher =    {Cambridge University Press},
  pages = {},
  year =         {1993}
}

@Article{Hartigan72,
  author =   {J. A. Hartigan},
  title =    {Direct clustering of a data matrix},
  journal =      {Journal of the American Statistical Association},
  year =     {1972},
  OPTkey =   {},
  volume =   {67},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {123--129},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Hartigan75,
  author =   {J. A. Hartigan},
  title =    {Clustering Algorithms},
  publisher =    {Wiley},
  year =     {1975},
  OPTkey =   {},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Hartigan78,
  author =   {J. Hartigan},
  title =    {Asymptotic distributions for clustering criteria},
  journal =      {Annals of Statistics},
  year =     {1978},
  OPTkey =   {},
  volume =   {6},
  OPTnumber =    {},
  pages =    {117--131},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Hartigan85,
  author =   {J. A. Hartigan},
  title =   {Statistical theory in clustering} ,
  journal =      JC,
  year =     {1985},
  OPTkey =   {},
  volume =   {2},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {63--76},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Hastie&Tibshirani96a,
  author =   {T. Hastie and R. Tibshirani},
  title =    {Discriminant adaptive nearest-nieghbor classification},
  journal =      {IEEE Pattern Recognition and Machine Intelligence},
  year =     {1996},
  OPTkey =   {},
  volume =   {18},
  OPTnumber =    {},
  pages =    {607--616},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{Hastie&Tibshirani96b,
  author =   {T. Hastie and R. Tibshirani},
  title =    {Classification by pairwise coupling},
  institution =  {Department of Statistics, Stanford University},
  year =     {1996},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@article {Hastie90,
   AUTHOR = {T.J. Hastie and  R.J. Tibshirani},
    TITLE = {Exploring the nature of covariate effects in the proportional hazar
ds model},
  JOURNAL = {Biometrics},
   VOLUME = {46},
     YEAR = {1990},
   NUMBER = {4},
    PAGES = {1005-1016},
     ISSN = {},
    CODEN = {},
}


@Book{Hochberg&Tamhane,
  author =   {Y. Hochberg and A. C. Tamhane},
  ALTeditor =    {},
  title =    {Multiple Comparison Procedures},
  publisher =    {Wiley--Interscience},
  year =     {1987},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  series =   {Probability and Mathematical Statistics},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Hochberg88,
  author =   {Y. Hochberg},
  title =    {A sharper Bonferroni procedure for multiple tests of significance},
  journal =      {Biometrika},
  year =     {1988},
  OPTkey =   {},
  volume =   {75},
  OPTnumber =    {},
  pages =    {800--802},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Holm79,
  author =   {S. Holm},
  title =    {A simple sequentially rejective multiple test procedure},
  journal =      {Scand. J. Statist.},
  year =     {1979},
  OPTkey =   {},
  volume =   {6},
  OPTnumber =    {},
  pages =    {65--70},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Hommel&Bernhard99,
  author =   {G. Hommel and G. Bernhard},
  title =    {Bonferroni procedures for logically related hypotheses},
  journal =      {Journal of Statistical Planning and Inference},
  year =     {1999},
  OPTkey =   {},
  volume =   {82},
  OPTnumber =    {},
  pages =    {119--128},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Hommel88,
  author =   {G. Hommel},
  title =    {A stagewise rejective multiple test procedure based on a modified Bonferroni test},
  journal =      {Biometrika},
  year =     {1988},
  OPTkey =   {},
  volume =   {75},
  OPTnumber =    {},
  pages =    {383--386},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Hubert&Arabie85,
  author =   {L. Hubert and P. Arabie},
  title =    {Comparing partitions},
  journal =      JC,
  year =     {1985},
  OPTkey =   {},
  volume =   {2},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {193--218},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Jain&DubesBook,
  author =   {A. K. Jain and R. C. Dubes},
  editor =   {},
  title =    {Algorithms for Clustering Data},
  publisher =    {Prentice-Hall},
  year =     {1988},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {Englewood Cliffs, N. J.},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Jogdeo77,
  author =   {K. Jogdeo},
  title =    {Association and probability inequalities},
  journal =      {Annals of Statistics},
  year =     {1977},
  OPTkey =   {},
  volume =   {5},
  OPTnumber =    {},
  pages =    {495--504},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Kaufman&Rousseeuw90,
  author =   {L. Kaufman and P. J. Rousseeuw},
  ALTeditor =    {},
  title =    {Finding Groups in Data: An Introduction to Cluster Analysis},
  publisher =    {Wiley, New York.},
  year =     {1990},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@article {Keles03,
AUTHOR ={Kele\c{s}, S. and van der Laan, M. and Dudoit,  S.},
TITLE ={Asymptotically Optimal  Model Selection Method for Regression on Censored Outcomes },
JOURNAL = {Technical Report, Division of Biostatistics, UC Berkeley},
VOLUME = {},
YEAR ={2002},
PAGES = {},
ISSN = {},
CODEN = {},
}



@Article{Kohonen90,
  author =   {T. Kohonen},
  title =    {The self-organizing map},
  journal =      {Proc. IEEE},
  year =     {1990},
  OPTkey =   {},
  volume =   {78},
  number =   {9},
  OPTmonth =     {},
  pages =    {1464--1480},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Kohonen95,
  author =   {T. Kohonen},
  title =    {Self-Organizing Maps},
  publisher =    {Springer},
  year =     {1995},
  OPTkey =   {},
  editor =   {T. S. Huang and T. Kohonen and M. R. Schroeder},
  volume =   {30},
  OPTnumber =    {},
  series =   {Springer Series in Information Sciences},
  address =      {Berlin, Heidelberg},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@article {Kooperberg95,
AUTHOR ={C. Kooperberg and C.J.  Stone and Y. K.  Truong},
TITLE ={Hazard Regression},
JOURNAL = {Journal of the American Statistical Association},
VOLUME = {90},
YEAR ={1995},
NUMBER={429},
PAGES = {78-94},
ISSN = {},
CODEN = {},
}



@Article{Koutsoukosetal,
  author =   {A. D. Koutsoukos and L. V. Rubinstein and D. Faraggi and R.M. Simon and S. Kalyandrug and J. N. Weinstein and K.W. Kohn and K.D. Paull},
  title =    {Discrimination techniques applied to the {NCI} in vitro anti-tumor drug screen: predicting biochemical mechanism of action},
  journal =      {Statistics in Medicine},
  year =     {1994},
  OPTkey =   {},
  volume =   {13},
  OPTnumber =    {},
  pages =    {719--730},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Krishnaiah&Reising85,
  author =   {P. R. Krishnaiah and J. M. Reising},
  title =    {Multivariate multiple comparisons},
  journal =      {Encyclopedia of Statistical Sciences},
  year =     {1985},
  OPTkey =   {},
  volume =   {9},
  number =   {6},
  pages =    {88--95},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Krzanowski&Lai,
  author =   {W. Krzanowski and Y. Lai },
  title =    {A criterion for determining the number of groups in a dataset using sum of squares clustering},
  journal =      {Biometrics},
  year =     {1985},
  OPTkey =   {},
  volume =   {44},
  OPTnumber =    {},
  pages =    {23--34},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Laan&Bryan01,
  author =   {M. J. van der Laan and J. Bryan},
  title =    {Gene expression analysis with the parametric bootstrap},
  journal =      {Biostatistics},
  year =     {2001},
  OPTkey =   {},
  volume =   {2},
  number =   {4},
  pages =    {445--461},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Pollard&vanderLaan04,
  author =   {K. S. Pollard and M.J. van der Laan},
  title =    {Choice of Null Distribution in Resampling Based Multiple Testing},
  journal =      JSPI,
  year =     {2004},
  OPTkey =   {},
  OPTvolume =    {125},
  OPTnumber =    {},
  OPTpages =     {85--101},
  OPTmonth =     {},
  note =     {},
  OPTannote =    {}
}


@Article{Laan&PollardJSPI02,
  author =   {M. J. van der Laan and K. S. Pollard},
  title =    {Hybrid clustering of gene expression data with visualization and the bootstrap},
  journal =      JSPI,
  year =     {2002},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTpages =     {},
  OPTmonth =     {},
  note =     {(To appear)},
  OPTannote =    {}
}


@article {Leblanc92,
AUTHOR ={M. Leblanc and J. Crowley},
TITLE ={Relative Risk trees for censored data},
JOURNAL = {Biometrics},
VOLUME = {48},
YEAR ={1992},
NUMBER={},
PAGES = {411-425},
ISSN = {},
CODEN = {},
}





@InProceedings{Leisch02,
  author =   {F. Leisch},
  title =    {Sweave: Dynamic Generation of Statistical Reports Using
                  Literate Data Analysis},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle = {Compstat 2002 --- Proceedings in Computational
                  Statistics},
  Tpages =   {575--580},
  year =     {2002},
  editor =   {Wolfgang H{\"a}rdle and Bernd R{\"o}nz},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  publisher = {Physika Verlag, Heidelberg, Germany},
  note =     {ISBN 3-7908-1517-9},
  OPTannote =    {},
  url =      {http://www.ci.tuwien.ac.at/~leisch/Sweave}
}

@TechReport{Leisch02TR,
  author =   {F. Leisch},
  title =    {Dynamic generation of statistical reports using literate data analysis},
  institution =  {SFB Adaptive Information Systems and Modelling in Economics and Management
Science, Vienna University of Economics and Business Administration},
  year =     {2002},
  OPTkey =   {},
  OPTtype =      {},
  number =   {69},
  OPTaddress =   {},
  month =    {March},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{Leisch99,
  author =   {F. Leisch},
  title =    {Bagged clustering},
  institution =  {SFB Adaptive Information Systems and Modelling in Economics and Management Science, Vienna University of Economics and Business Administration},
  year =     {1999},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  month =    {August},
  note =     {\url{http://www.ci.tuwien.ac.at/~leisch/papers/fl-techrep.html}},
  OPTannote =    {}
}

@Article{Limetal00,
  author =   {T-S Lim and W-Y Loh and Y-S Shih},
  title =    {A comparison of prediction accuracy, complexity, and training time of thiry-three old and new classification algorithms},
  journal =      {Machine Learning},
  year =     {2000},
  OPTkey =   {},
  volume =   {40},
  OPTnumber =    {},
  pages =    {203--229},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Book{Mardiaetal,
  author =   {K. V. Mardia and J. T. Kent and J. M. Bibby},
  title =    {Multivariate Analysis},
  publisher =    {Academic Press, Inc.},
  year =     {1979},
  OPTkey =   {},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {San Diego},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Unpublished{Mayo&Spanos02,
  author =       {D. C. Mayo and A. Spanos},
  title =        {A severe-testing interpretation of {N}eyman-{P}earson methods.  Unpublished manuscript},
  OPTnote =         {},
  OPTkey =       {},
  OPTmonth =     {},
  year =         {2002},
  OPTannote =    {}
}


@Book{McCullagh&Nelder89,
  author =   {P. McCullagh and J. A. Nelder},
  ALTeditor =    {},
  title =    {Generalized Linear Models},
  publisher =    {Chapman \& Hall},
  year =     {1989},
  OPTkey =   {},
  OPTvolume =    {},
  number =   {37},
  series =   {Monographs on Statistics and Applied Probability},
  OPTaddress =   {},
  edition =      {2nd},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Book{McLachlan,
  author =   {G. J. McLachlan},
  OPTeditor =    {},
  title =    {Discriminant analysis and statistical pattern recognition},
  publisher =    {Wiley},
  year =     {1992},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {New York},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{McLachlanetal01,
  author =   {G. J. McLachlan and R. Bean and D. Peel},
  title =    {A mixture model-based approach to the clustering of microarray expression data.},
  journal =      {Bioinformatics},
  year =     {2002},
  OPTkey =   {},
  volume =   {18},
  OPTnumber =    {},
  pages =    {413--422},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{MillerSubsets,
  author =   {A. J. Miller},
  OPTeditor =    {},
  title =    {Subset Selection in Regression},
  publisher =    {Chapman and Hall},
  year =     {1990},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Milligan&Cooper85,
  author =   {G. W. Milligan and M. C. Cooper},
  title =    {An examination of procedures for determining the number of clusters in a data set},
  journal =      {Psychometrika},
  year =     {1985},
  OPTkey =   {},
  volume =   {50},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {159--179},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Milligan&Cooper86,
  author =   {G. W. Milligan and M. C. Cooper},
  title =    {A study of the comparability of external criteria for hierarchical cluster analysis},
  journal =      {Multivariate Behavioral Research},
  year =     {1986},
  OPTkey =   {},
  volume =   {21},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {441--458},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Milligan&Cooper87,
  author =   {G. W. Milligan and M. C. Cooper},
  title =    {Methodology review: {C}lustering methods},
  journal =      {Applied Psychological Measurement},
  year =     {1987},
  OPTkey =   {},
  volume =   {11},
  OPTnumber =    {4},
  OPTmonth =     {December},
  pages =    {329--354},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Milligan89,
  author =   {G. W. Milligan},
  title =    {A study of the beta-flexible clustering method},
  journal =      {Multivariate Behavioral Research},
  year =     {1989},
  OPTkey =   {},
  volume =   {24(2)},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {163--176},
  OPTnote =      {},
  OPTannote =    {}
}


@InCollection{Milligan96,
  author =   {G. W. Milligan},
  title =    {Clustering validation: {R}esults and implications for applied analyses},
  booktitle =    {Clustering and Classification},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher = {World Scientific Publishing Co.},
  year =     {1996},
  editor =   {P. Arabie and L. J. Hubert and G. De Soete},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {River Edge, NJ},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {341--375},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Moreyetal83,
  author =   {L. C. Morey, R. K. Blashfield and H. A. Skinner},
  title =    {A comparison of cluster analysis techniques within a sequential validation framework},
  journal =      {Multivariate Behavioral Research},
  year =     {1983},
  OPTkey =   {},
  volume =   {18},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {309--329},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Morrison90,
  author =   {D. F. Morrison},
  ALTeditor =    {},
  title =    {Multivariate Statistical Methods},
  publisher =    {McGraw-Hill, NY},
  year =     {1990},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  edition =      {3rd},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@InCollection{Murtagh96,
  author =   {F. Murtagh},
  title =    {Neural networks for clustering},
  booktitle =    {Clustering and Classification},
  OPTcrossref =  {},
  OPTkey =   {},
  publisher = {World Scientific Publishing Co.},
  year =     {1996},
  editor =   {P. Arabie and L. J. Hubert and G. De Soete},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTchapter =   {},
  OPTtype =      {},
  address =      {River Edge, NJ},
  OPTedition =   {},
  OPTmonth =     {},
  pages =    {235--269},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{PanelDACC,
  author =   {{Panel on Discriminant Analysis, Classification, and Clustering}},
  title =    {Discriminant analysis and clustering},
  journal =      {Statistical Science},
  year =     {1989},
  OPTkey =   {},
  volume =   {4},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {34--69},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{Pavlic&vanderLaanTechRep89,
  author =   {M. Pavlic and M. J. van der Laan},
  title =    {Fitting of mixtures with unspecified number of components using cross-validation distance estimate},
  institution =  {Division of Biostatistics, U.C. Berkeley},
  year =     {2001},
  OPTkey =   {},
  OPTtype =      {},
  number =   {89},
  OPTaddress =   {},
  month =    {February},
  OPTnote =      {},
  OPTannote =    {}
}

@article{Pavlic02,
author  = {M. Pavlic and M. J. van der Laan},
title   = {Fitting of mixtures with unspecified number of components using
cross validation distance estimate},
journal = {Computational Statistics and Data Analysis},
volume  = {41},
issue   = {3-4},
pages   = {413-428},
year    = {2003}
}



@TechReport{Pollard&LaanTechRep107,
  author =   {K. S. Pollard and M. J. van der Laan},
  title =    {A Method to Identify Significant Clusters in Gene Expression Data},
  institution =  {Division of Biostatistics, U.C. Berkeley},
  year =     {2002},
  OPTkey =   {},
  OPTtype =      {},
  number =   {107},
  OPTaddress =   {},
  month =    {April},
  OPTnote =      {},
  OPTannote =    {}
}

@TechReport{Pollard&LaanTechRep121,
  author =   {K. S. Pollard and M. J. van der Laan},
  title =    {Resampling-based methods for identification of significant subsets of genes in expression data},
  institution =  {Division of Biostatistics, U.C. Berkeley},
  year =     {2002},
  OPTkey =   {},
  OPTtype =      {},
  number =   {121},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Ramsey78,
  author =   {P. H. Ramsey},
  title =    {Power differences between pairwise multiple comparisons},
  journal =      JASA,
  year =     {1978},
  OPTkey =   {},
  volume =   {73},
  OPTnumber =    {},
  pages =    {479--485},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Manual{RanForests,
  title =    {Notes on setting up, using, and understanding random forests V3.0},
  OPTkey =   {},
  author =   {L. Breiman},
  OPTorganization = {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  year =     {2001},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Rand,
  author =   {W. M. Rand},
  title =    {Objective criteria for the evaluation of clustering methods},
  journal =      {Journal of the American Statistical Association},
  year =     {1971},
  OPTkey =   {},
  volume =   {66},
  OPTnumber =    {336},
  OPTmonth =     {},
  pages =    {846--850},
  OPTnote =      {},
  OPTannote =    {}
}

@Unpublished{Reineretal01,
  author =   {A. Reiner and D. Yekutieli and Y. Benjamini},
  title =    {Using resampling-based {FDR} controlling multiple test procedures for analyzing microarray gene expression data},
  OPTnote =      {},
  OPTkey =   {},
  OPTmonth =     {},
  year =     {2001},
  OPTannote =    {}
}


@Book{Ripley96,
  author =   {B. D. Ripley},
  title =    {Pattern recognition and neural networks},
  publisher =    {Cambridge University Press},
  year =     {1996},
  OPTkey =   {},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {Cambridge, New York},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}




%very first reference to use trees in survival analysis
@Article{Rissanen78,
  author =   {J. Rissanen},
  title =    {Modelling by shortest data description},
  journal =      {Automatica},
  year =     {1978},
  volume =   {14},
  pages =    {465-471}
}

@Article{Rnews:Dudoit+Yang+Bolstad:2002,
  author       = {S. Dudoit and Y. H.  Yang and B. Bolstad},
  title        = {Using {R} for the Analysis of {DNA} Microarray Data},
  journal      = {R News},
  year         = 2002,
  volume       = 2,
  number       = 1,
  pages        = {24--32},
  month        = {March},
  url          = {CRAN.R-project.org/doc/Rnews/}
}

@article {Robins00a,
AUTHOR ={J. M. Robins and A.  Rotnitzky},
TITLE ={Comment on the {B}ickel and {K}won article, ``{I}nference for semiparametric models: {S}ome questions and an answer''},
JOURNAL = {Statistica Sinica},
VOLUME = {11},
NUMBER={4},
YEAR ={2001},
PAGES = {920-936},
ISSN = {},
CODEN = {}
}


@InProceedings{Robins00c,
  author =   {J.M. Robins},
  title =    {Robust estimation in sequentially ignorable
missing data and causal inference models},
  booktitle =    {Proceedings of the American
Statistical Association},
  pages =    {},
  year =     {2000},
  editor =   {},
  organization = {}
}


@article {Robins00b,
AUTHOR ={J. M. Robins and A.  Rotnitzky and M.J. van der Laan},
TITLE ={Comment on ``{O}n {P}rofile {L}ikelihood" by {S}.{A}. {M}urphy and
{A}.{W}. van der {V}aart},
JOURNAL = {Journal of the American Statistical Association -- Theory and
Methods
},
VOLUME = {450},
YEAR ={2000},
PAGES = {431-435},
ISSN = {},
CODEN = {}
}



@Article{Birge83,
  author =   {L. Birg{\'e}},
  title =    {Approximation dans les espaces m{/'e}triques et th{\'e}orie
  de l'estimation},
  journal =      {Verw. Gebiete},
  year =     {1983},
  OPTkey =   {},
  volume =   {65},
  number =   {},
  OPTmonth =     {},
  pages =    {181--238},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{lecam73,
  author =   {L.M. le Cam},
  title =    {Convergence of estimates under dimensionality restrictions},
  journal =      {Annals of Statistics},
  year =     {1973},
  OPTkey =   {},
  volume =   {22},
  number =   {},
  OPTmonth =     {},
  pages =    {38--53},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Rom90,
  author =   {D. M. Rom},
  title =    {A sequentially rejective test procedure based on a modified {Bonferroni} inequality},
  journal =      {Biometrika},
  year =     {1990},
  OPTkey =   {},
  volume =   {77},
  OPTnumber =    {},
  pages =    {663-665},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{Rosenblatt57,
  author =       {F. Rosenblatt},
  title =        {The perceptron -- a perceiving and recognizing automation},
  institution =  {Cornell Aeronautical Laboratory },
  year =         {1957},
  OPTkey =       {},
  OPTtype =      {},
  number =       {86-460-1},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Ruczinskietal,
  author =   {I. Ruczinski and C. Kooperberg and M. LeBlanc},
  title =    {Logic regression},
  journal =      {},
  year =     {2001},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTpages =     {},
  OPTmonth =     {},
  note =     {Submitted, \url{http://biosun01.biostat.jhsph.edu/~iruczins/html/publications.html}},
  OPTannote =    {}
}

@Article{Saltstone&Stange,
  author =   {R. Saltstone and K. Stange},
  title =    {A computer program to calculate Hubert and Arabie's adjusted Rand index},
  journal =      {Journal of Classification},
  year =     {1996},
  OPTkey =   {},
  volume =   {13},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {169--172},
  OPTnote =      {},
  OPTannote =    {}
}
@TechReport{vanderVaart03,
  author =   {A.W. van der Vaart},
  title =    {Notes on Cross-validation},
  institution =  {Department of Mathematics, Free University, Amsterdam},
  year =     {2003},
  OPTkey =   {},
  OPTtype =      {},
  number =   {},
  OPTaddress =   {},
  OPTmonth =     {},
  note =     {},
  OPTannote =    {Unpublished manuscript}
}

@TechReport{Sarle,
  author =   {W. Sarle},
  title =    {Cubic clustering criterion},
  institution =  {SAS Institute, Inc.},
  year =     {1983},
  OPTkey =   {},
  OPTtype =      {},
  number =   {A-108},
  OPTaddress =   {},
  OPTmonth =     {},
  note =     {\url{http://www.sas.com/service/library/onlinedoc/trindex.html}},
  OPTannote =    {}
}

@TechReport{Sarle&Kuo,
  author =   {W. Sarle and A. Kuo},
  title =    {The MODECLUS Procedures},
  institution =  {SAS Institute, Inc.},
  year =     {1993},
  OPTkey =   {},
  OPTtype =      {},
  number =   {P-256},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Schapireetal,
  author =   {R. E. Schapire and Y. Freund and P. Bartlett and W. S. Lee},
  title =    {Boosting the margin: a new explanation for the effectiveness of voting methods},
  journal =      {Annals of Statistics},
  year =     {1998},
  OPTkey =   {},
  volume =   {26},
  OPTnumber =    {},
  pages =    {1651--1686},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Book{Scheffe,
  author =   {H. Scheff\'{e}},
  ALTeditor =    {},
  title =    {The analysis of variance},
  publisher =    {John Wiley \& Sons},
  year =     {1959},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Scheibler&Schneider,
  author =   {D. Scheibler and W. Schneider},
  title =    {Monte Carlo tests of the accuracy of cluster analysis algorithms: A comparison of hierarchical and nonhierarchical methods},
  journal =      {Multivariate Behavioral Research},
  year =     {},
  OPTkey =   {},
  volume =   {20},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {283--304},
  OPTnote =      {},
  OPTannote =    {}
}


@InProceedings{Schuster81,
  author =   {E. F. Schuster and C. G. Gregory},
  title =    {On the non-consistency of maximum likelihood nonparametric density estimators},
  booktitle =    {Computer Science and Statistics: Proceedings of the 13th Symposium on the interface},
  pages =    {295-298},
  year =     {1981},
  editor =   {Eddy, W.F.},
  organization = {}
}


@Article{Scott81,
  author =   {D. W. Scott and L. E. Factor},
  title =    {Monte Carlo study of three data-based nonparametric density estimators},
  journal =      {Journal of the American Statistical Association},
  year =     {1981},
  volume =   {76},
  pages =    {9-15}
}

@Article{Seeger68,
  author =   {P. Seeger},
  title =    {A note on a method for the analysis of significances en masse},
  journal =      {Technometrics},
  year =     {1968},
  OPTkey =   {},
  volume =   {10},
  number =   {3},
  pages =    {586--593},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Segal88,
  author =   {M. R. Segal},
  title =    {Regression trees for censored data},
  journal =      {Biometrics},
  year =     {1988},
  OPTkey =   {},
  volume =   {44},
  OPTnumber =    {},
  pages =    {35--47},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}





@string{JASA= {Journal of the American Statistical Association}}
@string{JC = {Journal of Classification}}
@string{JSPI = {Journal of Statistical Planning and Inference}}
@string{JRSSB = {Journal of the Royal Statistical Society, Series B}}
@string{PNAS = {Proc. Natl. Acad. Sci.}}

@Article{Shaffer02,
  author =   {J. P. Shaffer},
  title =    {Multiplicity, directional ({T}ype {III}) errors, and
the null hypothesis},
  journal =      {Psychological Methods},
  year =     {2002},
  OPTkey =   {},
  volume =   {7},
  OPTnumber =    {},
  pages =    {356--369},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Shaffer86,
  author =   {J. P. Shaffer},
  title =    {Modified sequentially rejective multiple test procedures},
  journal =      JASA,
  year =     {1986},
  OPTkey =   {},
  volume =   {81},
  OPTnumber =    {},
  pages =    {826--831},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Shaffer95,
  author =   {J. P. Shaffer},
  title =    {Multiple hypothesis testing},
  journal =      {Annu. Rev. Psychol.},
  year =     {1995},
  OPTkey =   {},
  volume =   {46},
  OPTnumber =    {},
  pages =    {561--584},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@article{Shao93,
AUTHOR={Shao, J.},
TITLE={Linear Model Selection by Cross-Validation},
JOURNAL={Journal of the American Statistical Association},
VOLUME={88},
YEAR={1993},
PAGES={486-494}
}




@Article{Sidak67,
  author =   {Z. \v{S}id\'{a}k},
  title =    {Rectangular confidence regions for the means of multivariate normal distributions},
  journal =      JASA,
  year =     {1967},
  OPTkey =   {},
  volume =   {62},
  OPTnumber =    {},
  pages =    {626-633},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Silverman,
  author =   {B. W. Silverman},
  title =    {Smoothed functional principal components analysis by choice of norm},
  journal =      {Annals of Statistics},
  year =     {1996},
  OPTkey =   {},
  volume =   {24},
  OPTnumber =    {},
  OPTmonth =     {},
  pages =    {1--24},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Silverman84,
  author =   {B. W. Silverman},
  title =    {A fast and efficient cross-validation method for smoothing parameter choice in spline regression},
  journal =      JASA,
  year =     {1984},
  OPTkey =   {},
  volume =   {79},
  number =   {387},
  pages =    {584--589},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}




@Book{Silverman86,
  author =       {B. W. Silverman},
  title =        {Density Estimation for Statistics and Data analysis},
  publisher =    {Chapman \& Hall},
  pages = {},
  year =         {1986}
}

@Article{vanderLaan&Dudoit&Keles04,
  author =   {M.J. van der Laan and S. Dudoit and S. Keles},
  title =    {Asymptotic optimality of likelihood-based cross-validation},
  journal =      {Statistical Applications in Genetics and Molecular Biology},
  year =     {2004},
  OPTkey =   {},
  volume =   {3},
  OPTnumber =    {1},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {http://www.bepress.com/sagmb/vol3/iss1/art4},
  OPTannote =    {}
}
@Article{Simes86,
  author =   {R. J. Simes},
  title =    {An improved Bonferroni procedure for multiple tests of significance},
  journal =      {Biometrika},
  year =     {1986},
  OPTkey =   {},
  volume =   {73},
  OPTnumber =    {},
  pages =    {751--754},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{Smyth00,
  author =   {P. Smyth},
  title =    {Model selection of probabilistic clustering using cross-validated likelihood},
  journal =      {Statistics and Computing},
  year =     {2000},
  volume =   {10},
  pages =    {63-72}
}




@Article{Soric89,
  author =   {B. Sori\'{c}},
  title =    {Statistical ``discoveries" and effect-size estimation},
  journal =      JASA,
  year =     {1989},
  OPTkey =   {},
  volume =   {84},
  number =   {406},
  pages =    {608--610},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Stone74,
  author =   {M. Stone},
  title =    {Cross-validatory choice and  assessment of statistical predictions},
  journal =      {Journal of the Royal Statistical Society, Series B},
  year =     {1974},
  volume =   {36},
  pages =    {111-147}
}

@Article{Stone84,
  author =   {C. J. Stone},
  title =    {An asymptotically optimal window selection rule for kernel density estimates},
  journal =      {The Annals of Statistics},
  year =     {1984},
  volume =   {12},
  pages =    {1285-1297}
}

@Article{StoneC84,
  author =   {C. J. Stone},
  title =    {An asymptotically optimal window selection rule for kernel density estimates},
  journal =      {Annals of Statistics},
  year =     {1984},
  OPTkey =   {},
  volume =   {12},
  number =   {4},
  pages =    {1285--1297},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{StoneM74,
  author =   {M. Stone},
  title =    {Cross-validatory choice and assessment of statistics predictions},
  journal =      JRSSB,
  year =     {1974},
  OPTkey =   {},
  volume =   {36},
  number =   {2},
  pages =    {111--147},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}






@Article{StoneM77,
  author =   {M. Stone},
  title =    {Asymptotics for and against cross-validation},
  journal =      {Biometrika},
  year =     {1977},
  OPTkey =   {},
  volume =   {64},
  number =   {1},
  pages =    {29--35},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@TechReport{Storey&TibshiraniTechRep01,
  author =   {J. D. Storey and R. Tibshirani},
  title =    {Estimating false discovery rates under dependence, with applications
to DNA microarrays},
  institution =  {Department of Statistics, Stanford University},
  year =     {2001},
  OPTkey =   {},
  OPTtype =      {},
  number =   {2001-28},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{StoreyJRSSB02,
  author =   {J. D. Storey},
  title =    {A direct approach to false discovery rates},
  journal =      JRSSB,
  year =     {2002},
  OPTkey =   {},
  volume =   {64},
  OPTnumber =    {},
  pages =    {479--498},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{StoreyTechRep01,
  author =   {J. D. Storey},
  title =    {The positive False Discovery Rate: A Bayesian interpretation and the q-value},
  institution =  {Department of Statistics, Stanford University},
  year =     {2001},
  OPTkey =   {},
  OPTtype =      {},
  number =   {2001-12},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{TSH,
  author =   {E. L. Lehmann},
  ALTeditor =    {},
  title =    {Testing Statistical Hypotheses},
  publisher =    {Springer-Verlag, New York},
  year =     {1986},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  edition =      {2nd},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Tibshiranietal02a,
  author =   {R. Tibshirani and T. Hastie and B. Narasimhan and. G. Chu},
  title =    {Diagnosis of multiple cancer types by shrunken centroids of gene expression},
  journal =      PNAS,
  year =     {2002},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTpages =     {},
  OPTmonth =     {},
  note =     {In press},
  OPTannote =    {}
}


@Article{Troendle95,
  author =   {J. F. Troendle},
  title =    {A stepwise resampling method of multiple hypothesis testing},
  journal =      JASA,
  year =     {1995},
  OPTkey =   {},
  volume =   {90},
  OPTnumber =    {},
  pages =    {370--378},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Troendle96,
  author =   {J. F. Troendle},
  title =    {A permutational step-up method of testing multiple outcomes},
  journal =      {Biometrics},
  year =     {1996},
  OPTkey =   {},
  volume =   {52},
  OPTnumber =    {},
  pages =    {846--859},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{VR,
 author = { W. N. Venables and B. D. Ripley },
 title = {Modern Applied Statistics with S--PLUS},
 publisher = {Springer},
 year = {1999}
}


@Book{Vaart96,
  author =       {A. W. van der Vaart  and J. A. Wellner},
  title =        {Weak {C}onvergence and {E}mprical {P}rocesses},
  publisher =    {Springer-Verlag New York},
  pages = {102},
  year =         {1996}
}





@Book{Vaart98,
  author =       {A. W. van der Vaart},
  title =        {Asymptotic Statistics},
  publisher =    {Cambridge University Press},
  pages = {62},
  year =         {1998}
}


@Book{Vapnik,
  author =   {V. N. Vapnik},
  OPTeditor =    {},
  title =    {The nature of statistical learning theory},
  publisher =    {Springer},
  year =     {2000},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  series =   {Statistics for engineering and information science},
  address =      {New York},
  edition =      {2nd},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Vapnik79,
  author =   {V. Vapnik},
  title =    {Estimation of dependences based on empirical data (in Russian)},
  journal =      {Nauka, Moskow},
  year =     {1979},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Book{Vapnik98,
  author =       {V. Vapnik},
  title =        {Statistical Learning Theory},
  publisher =    {Wiley},
  year =         {1998},
  OPTkey =       {},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {New York},
  edition =      {1st},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Book{Venables&Ripley99,
  author =   {W. N. Venables and B. D. Ripley},
  title =    {Modern applied statistics with S-PLUS},
  publisher =    {Springer},
  year =     {1999},
  OPTkey =   {},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  edition =      {3rd},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{Westfall&Young93,
  author =   {P. H. Westfall and S. S. Young},
  OPTeditor =    {},
  title =    {Resampling-based multiple testing: {E}xamples and methods for $p$-value adjustment},
  publisher =    {John Wiley \& Sons},
  year =     {1993},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{,
  author =       {},
  title =        {},
  publisher =    {},
  pages = {},
  year =         {}
}


@InCollection{Westfalletal01,
  author =   {P. H. Westfall and D. V. Zaykin and S. S. Young},
  title =    {Multiple tests for genetic effects in association studies},
  booktitle =    {Biostatistical Methods},
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {143--168},
  publisher = {Humana Press, Toloway, NJ},
  year =     {2001},
  editor =   {S. Looney},
  volume =   {184},
  OPTnumber =    {},
  series =   {Methods in Molecular Biology},
  OPTtype =      {},
  OPTchapter =   {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Westonetal2000,
  author =   {J. Weston and S. Mukherjee and  O. Chappelle and  M. Pontil and  T. Poggio and V. Vapnik},
  title =    {Feature Selection for {SVM}s},
  journal =      {Advances in Neural Processing Systems},
  year =     {2001},
  OPTkey =   {},
  volume =   {13},
  number =   {},
  pages =    {668--674},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Wright92,
  author =   {S. P. Wright},
  title =    {Adjusted P-values for simultaneous inference},
  journal =      {Biometrics},
  year =     {1992},
  OPTkey =   {},
  volume =   {48},
  number =   {4},
  pages =    {1005--1013},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{YangetalJCGS02,
  author =   {Y. H. Yang and M. J. Buckley and S. Dudoit and T. P. Speed},
  title =    {Comparison of methods for image analysis on c{DNA} microarray data},
  journal =      {Journal of Computational and Graphical Statistics},
  year =     {2002},
  OPTkey =   {},
  volume =   {11},
  number =   {1},
  pages =    {108--136},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{YangetalNAR02,
  author =   {Y. H. Yang and S. Dudoit and P. Luu and D. M. Lin and V. Peng and J. Ngai and T. P. Speed},
  title =    {Normalization for c{DNA} microarray data: {A} robust composite method addressing single and multiple slide systematic variation},
  journal =      {Nucleic Acids Research},
  year =     {2002},
  OPTkey =   {},
  volume =   {30},
  number =   {4},
  pages =    {e15},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@InProceedings{YangetalSPIE01,
  author =   {Y. H. Yang and S. Dudoit and P. Luu and T. P. Speed},
  title =    {Normalization for c{DNA} microarray data},
  booktitle =    {Microarrays: Optical Technologies and Informatics},
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {141--152},
  year =     {2001},
  editor =   {Michael L. Bittner and Yidong Chen and Andreas N. Dorsel and Edward R. Dougherty},
  volume =   {4266},
  OPTnumber =    {},
  series =   {Proceedings of SPIE},
  address =      {San Jose, CA},
  month =    {May},
  OPTorganization = {SPIE},
  publisher = {SPIE-International Society for Optical Engineering},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Yekutieli&Benjamini99,
  author =   {D. Yekutieli and Y. Benjamini},
  title =    {Resampling-based false discovery rate controlling multiple test procedures for correlated test statistics},
  journal =      JSPI,
  year =     {1999},
  OPTkey =   {},
  volume =   {82},
  OPTnumber =    {},
  pages =    {171--196},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@InCollection{Youden69,
  author =   {W. J. Youden},
  title =    {Measurement agreement comparisons},
  booktitle =    {Precision measurement and calibration: Statistical concepts and procedures},
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {146--151},
  publisher = {National Bureau of Standards, United States Department of Commerce},
  year =     {1969},
  editor =   {H. H. Ku},
  volume =   {1},
  OPTnumber =    {},
  series =   {Special Publication 300},
  type =     {NBS Miscelaneous Publication 248, Proceedings of the 1962 Standards Laboratory Conference},
  OPTchapter =   {},
  OPTaddress =   {},
  OPTedition =   {},
  month =    {February},
  OPTnote =      {},
  OPTannote =    {}
}




@article{Zhang93,
AUTHOR={Zhang, P.},
TITLE={Model selection via multifold cross-validation},
JOURNAL={Annals of Statistics},
VOLUME={21},
YEAR={1993},
PAGES={299-313}
}

@Article{ZhangetalBioinf02,
  author =   {J. Zhang and V. Carey and R. Gentleman},
  title =    {An extensible application for assembling annotation for
genomic data},
  journal =      {Bioinformatics},
  year =     {2002},
  OPTkey =   {},
  volume =   {},
  number =   {},
  pages =    {},
  OPTmonth =     {},
  note =     {(In press)},
  OPTannote =    {},
  url = {http://www.R-project.org/}
}







@Book{BKRW,
  author =   {P.J. Bickel and C.A.J. Klaassen and Y. Ritov and J. Wellner},
  title =    {Efficient and Adaptive Estimation for Semiparametric Models},
  publisher =    {Springer-Verlag},
  year =     {1997}
}




@Article{bozdoganaic,
  author =   {H. Bozdogan},
  title =    {Akaike's information criterion and recent developments in information complexity},
  journal =      {Journal of Mathematical Psychology},
  year =     {2000},
  volume =   {44},
  pages =    {62-91}
}



@book {cart,
   AUTHOR = {L. Breiman and J. H. Friedman and R. A. Olshen and C. J. Stone},
    TITLE = {Classification and Regression Trees},
PUBLISHER = {Wadsworth \& Brooks/Cole},
  ADDRESS = {Monterey},
     YEAR = {1984},
    PAGES = {},
     ISBN = {}
}

@book {mark,
 author = {M.J. van der Laan and J.M. Robins},
  title = {Unified methods for censored longitudinal  data and causality},
  publisher = {Springer, New York},
  year =     {2003}
}


@Manual{effsize,
  title =    {Teaching Children to Read},
  OPTkey =   {},
  author =   {{National Reading Panel}},
  organization = {National Institute of Child Health and Human Development, National Institutes of Health},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  year =     {1999},
  OPTnote =      {},
  OPTannote =    {}
}


@TechReport{gapstats,
  author =   {R. Tibshirani and  G. Walther and T. Hastie.},
  title =    {Estimating the number of clusters in a dataset via the gap statistic},
  institution =  {Department of Biostatistics, Stanford University},
  year =     {2000},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  month =    {March},
  note =     {\url{http://www-stat.stanford.edu/~tibs/research.html}},
  OPTannote =    {}
}




@InProceedings{gillcar,
  author =   {R.D. Gill and M.J. van der Laan and J.M. Robins},
  title =    {Coarsening at random: characterizations, conjectures and counter-examples},
  booktitle =    {Proceedings of the First Seattle Symposium in Biostatistics},
  pages =    {255-94},
  year =     {1997},
  editor =   {D.Y. Lin and T.R. Fleming},
  address =      {New York},
  publisher = {Springer Verlag}
}
@article{Gill&Robins01,
   AUTHOR = {Gill, R. and Robins, J.M.},
    TITLE = {Causal inference in complex longitudinal studies: continuous case},
  JOURNAL = {Ann. Stat.},
 FJOURNAL = {The Annals of Statistics},
   VOLUME = {29},
     YEAR = {2001},
   NUMBER = {6},
    PAGES = {},
     ISSN = {},
    CODEN = {},
  MRCLASS = {},
 MRNUMBER = {},
}


%uses exponential mode at each node
@Article{jacobsen,
  author =   {M. Jacobsen and N. Keiding},
  title =    {Coarsening at random in general sample spaces and random censoring in continuous time},
  journal =      {Annals of Statistics},
  year =     {1995},
  volume =   {23},
  pages =    {774-86}
}

%very first reference to use trees in survival analysis










@Misc{marray,
  OPTkey =   {},
  author =   {S. Dudoit and Y. H. Yang},
  title =    {Normalization and diagnostic plots for cDNA microarray data, {\tt marrayClasses}, {\tt marrayInput}, {\tt marrayNorm}, {\tt marrayPlots}},
  howpublished = {{\tt R} packages},
  OPTmonth =     {},
  year =     {2002},
  OPTnote =      {},
  OPTannote =    {},
  url =          {www.bioconductor.org},
}

@TechReport{mclust98,
  author =   {C. Fraley and A. E. Raftery},
  title =    {MCLUST: Software for Model-Based Cluster Analysis},
  institution =  {Department of Statistics, University of Washington},
  year =     {1998},
  OPTkey =   {},
  OPTtype =      {},
  number =   {342},
  OPTaddress =   {},
  month =    {November},
  OPTnote =      {},
  OPTannote =    {}
}


@Misc{multtest,
  OPTkey =   {},
  author =   {Y. Ge and S. Dudoit},
  title =    {Multiple Testing Procedures, {\tt multtest}},
  howpublished = {{\tt R} package},
  OPTmonth =     {},
  year =     {2002},
  OPTnote =      {},
  OPTannote =    {},
  url =          {www.bioconductor.org},
}

@InProceedings{robins93,
  author =   {J.M. Robins},
  title =    {Information recovery and bias adjustment in proportional hazards regression analysis of randomized trials using surrogate markers},
  booktitle =    {Proceeding of the Biopharmaceutical section},
  pages =    {24-33},
  year =     {1993},
  organization = {American Statistical Association}
}

@InCollection{robrot,
  author =   {J.M. Robins and A. Rotnitzky},
  title =    {Recovery of information and adjustment for dependent censoring using surrogate markers},
  booktitle =    {AIDS Epidemiology},
  publisher = {Bikh\"{a}user},
  year =     {1992},
  series =   {Methodological issues}
}


@Article{robzhao,
  author =   {J.M. Robins and A. Rotnitzky and L.P. Zhao},
  title =    {Estimation of regression coefficients when some regressors are not always observed},
  journal =      {Journal of the American Statistical Association},
  year =     {1994},
  volume =   {89},
  number =   {427},
  pages =    {846-866},
  month =    {September}
}







@Article{Heitjan&Rubin91,
  author =   {D.F. Heitjan and D.B. Rubin},
  title =    {Ignorability and coarse data},
  journal =      {Annals of statistics},
  year =     {1991},
  volume =   {19},
  number =   {4},
  pages =    {2244-2253},
  month =    {December}
}

@Misc{sma,
  OPTkey =   {},
  author =   {S. Dudoit and Y. H. Yang and B. M. Bolstad},
  title =    {Statistical {M}icroarray {A}nalysis, {\tt sma}},
  howpublished = {{\tt R} package},
  OPTmonth =     {},
  year =     {2001},
  note =     {Contributions from Natalie Thorne, Ingrid L\"{o}nnstedt, and Jessica Mar},
  OPTannote =    {},
  url =          {cran.r-project.org/src/contrib/PACKAGES.html\#sma}
}

@PhdThesis{thesis,
  author =   {S. Dudoit},
  title =    {Linkage analysis of complex human traits using identity by descent data},
  school =   {Department of Statistics, University of California, Berkeley},
  year =     {1999},
  OPTkey =   {},
  OPTaddress =   {},
  type =     {Ph.D. thesis},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Book{vanderVaart&Wellner96,
  author =   {A. van der Vaart and J. Wellner},
  ALTeditor =    {},
  title =    {Weak Convergence and Empirical Processes},
  publisher =    {Springer-Verlag, New York},
  year =     {1996},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@inproceedings{arcones1989boot_mean,
  title={The bootstrap of the mean with arbitrary bootstrap sample size},
  author={Arcones, Miguel A and Gin{\'e}, Evarist},
  booktitle={Annales de l'IHP Probabilit{\'e}s et statistiques},
  volume={25},
  number={4},
  pages={457--481},
  year={1989}
}
@article{gine1989necessary_boot_mean,
  title={Necessary conditions for the bootstrap of the mean},
  author={Gin{\'e}, Evarist and Zinn, Joel},
  journal={The annals of statistics},
  pages={684--691},
  year={1989},
  publisher={JSTOR}
}
@article{arcones1992boot_mestimator,
  title={On the bootstrap of M-estimators and other statistical functionals},
  author={Arcones, Miguel A and Gin{\'e}, Evarist},
  journal={Exploring the limits of bootstrap},
  pages={13--47},
  year={1992},
  publisher={Wiley New York}
}

==> help.tex <==

\subsection{An MLE restricting the variation norm}

%MAKE IT AN ESTIMATOR IN {\CAL Q}_N. of Q_{0n}

Our goal is to construct an estimator $\hat{Q}:{\cal M}_{np}\rightarrow{\cal Q}_n$ of $Q_0=Q(P_0)=\arg\min_{Q\in {\cal Q}}P_0\bar{L}_1(Q)$ so that $d_{01}(Q_n,Q_0)=o_P(n^{-1/4})$. The following Lemma defines such an estimator. 
\begin{lemma}\label{tmlelemma2}
%Let $(0,Q)\rightarrow L(Q)(o)$ be a loss function for a parameter $Q_0$ with $P_0L(Q_0)=\arg\min_{Q\in Q({\cal M})}P_0L(Q)$.

%Suppose that $M_{1Q,n}=\sup_{Q\in {\cal Q}_n} \mid L(Q)-L(Q_{0n})\mid (o)<\infty$.
%Let $M_{Q,v,n}=\sup_{P\in {\cal M}_n}\pl Q(P)\pl_v<\infty$.
%Let $M_{L(Q),v,n}<\infty$. 
%Let $M_{2Q,n}<\infty$.


For a given vector $M\in \openr^{k_1}_{\geq 0}$ of constants, let ${\cal Q}_{n,M}^1\subset \{Q\in {\cal Q}_n:\pl Q\pl_v\leq M,\pl L_1(Q)\pl_v\leq M\}\subset {\cal F}_{v,M}^{k_1}$  be all functions in the parameter space ${\cal Q}_n$ for $Q_{0n}$ 
for which the variation norm of its loss and itself is smaller than $M<\infty$.
If $M>\max(M_{Q,v},M_{L_1(Q),v})$, then ${\cal Q}_{n,M}={\cal Q}_n$.
Let  $Q_{0n}^M\in {\cal Q}_{n,M}^1$ be so that $P_0\bar{L}_1(Q_{0n}^M)=\inf_{Q\in {\cal Q}_{n,M}} P_0\bar{L}_1(Q)$.
%note componentn wise minimum!
%Consider the loss based dissimilarity $d_0(Q,Q_0)=P_0L(Q)-P_0L(Q_0)$, where $P_0L(Q_0)=\min_{Q\in {\cal Q}{(\cal M}}P_0L(Q)$.
%Assume that $\limsup_{n\rightarrow\infty} \sup_{Q\in {\cal Q}_{n,M}}\pl L(Q)\pl_v<\infty$: i.e., the variation norm of $L(Q)$ can be universally bounded in terms of the variation norm of $Q$.
%if we use loglikleihoodl loss then this requires keeping 
%Assume that $d_0(Q_n,Q_0)\rightarrow 0$ implies $\pl L(Q_n)-L(Q_0)\pl_{P_0}\rightarrow 0$.
%the universal bounding and equivalence of norms is only needed for iterative applying the proof and using bound on asymptotic equicontinuity
%Assume that there exists a $M_2<\infty$ so that\begin{equation}\label{MLEa1}\sup_{Q\in {\cal Q}({\cal M})}\frac{P_0\{L(Q)-L(Q_0)\}^2}{P_0 \{L(Q)-L(Q_0)\}}\leq M_2.\end{equation}


Consider an estimator $Q_n^M$ for which \[
P_n \bar{L}_1(Q_n^M)=\inf_{Q\in {\cal Q}_{n,M}} P_n\bar{L}_1(Q)+r_n,\]
where $r_n=o_P(1/\sqrt{n})$.
Then 
\begin{equation}\label{MLEa}
0\leq d_{01}(Q_n^M,Q_{0n}^M)\leq -(P_n-P_0)\{L_1(Q_n^M)-L_1(Q_{0n}^M)\}+r_n,\end{equation}
and
\[d_{01}(Q_n^M,Q_{0n}^M)=o_P(1/\sqrt{n}).\]
%these are vectors!
%Let $M^u_0$ be a value so that for $M>M^u_0$ we have $Q_{0n}^M=Q_{0n}$. 
Then, for any $M>\max(M_{Q,v},M_{L_1(Q),v})$, the estimator $Q_n^{M}$ satisfies:
\[
d_{01}(Q_n^{M},Q_0)=o_P(1/\sqrt{n}).\]
%The analogue applies to $G_n^M$ and loss function $L_2(G)$.
%we need to confirm this constant $\lamba(d)$ since it appears in theorem
In addition, there exists a $\lambda\geq \lambda(d)=0.5+\frac{1}{4(d+1)}$ so that
\[
d_{01}(Q_n^M,Q_{0n}^M)=O_P(n^{-\lambda(d))}).\]
%We should also have a better rate like $r_Q(n)^2$ but not exactly that since this is not epsilon-net.

Consider the rates:
\[
r_{Q,MLE,j}(n)\equiv
J(n^{-1/4},{\cal Q}_{j,n,M}^1,L^2),\]
where
\[
J(\delta,{\cal Q}_{j,nM}^1,L^2)=\sup_{\Lambda}\int_0^{\delta} \left( \log(1+N(\epsilon M,{\cal Q}_{j,n,M}^1,L^2(\Lambda)) \right)^{0.5} d\epsilon ,\mbox{ $j=1,\ldots,k_1$.}\]
Let $r_{Q,MLE}(n)=(r_{Q,MLE,j}(n):j=1,\ldots,k_1)$. In fact, we have
\[
d_{01}(Q_n^M,Q_{0n}^M)=O_P(r_{Q,MLE}^2(n))<O_P(n^{-\lambda(d)}).
\]
\end{lemma}
{\bf Proof:}
We have 
\begin{eqnarray*}
0&\leq & d_{01}(Q_n^M,Q_{0n}^M)=P_0\{L_1(Q_n^M)-L_1(Q_{0n}^M)\}\\
&=&-(P_n-P_0)\{L_1(Q_n^M)-L_1(Q_{0n}^M)\}+P_n \{L_1(Q_n^M)-L_1(Q_{0n}^M)\}\\
&\leq &-(P_n-P_0)\{L_1(Q_n^M)-L_1(Q_{0n}^M)\}+r_n,
\end{eqnarray*}
which proves (\ref{MLEa}).
Since $L_1(Q_n^M)-L_1(Q_{0n}^M)$ falls in a $P_0$-Donsker class ${\cal F}_{v,M}^{k_1}$, it follows that the right-hand side is $O_P(1/\sqrt{n})$, and thus
$d_{01}(Q_n^M,Q_{0n}^M)=O_P(n^{-1/2})$. Since $M_{2,Q}<\infty$, this also implies  that $\pl L_1(Q_n^M)-L_1(Q_{0n}^M)\pl_{P_0}^2=O_P(1/\sqrt{n})$. By empirical process theory we have that $\sqrt{n}(P_n-P_0)f_n\rightarrow_p 0$ if $f_n$ falls in a $P_0$-Donsker class with probability tending to 1, and $P_0f_n^2\rightarrow_p 0$ as $n\rightarrow\infty$. Applying this to $f_n=L_1(Q_n^M)-L_1(Q_{0n}^M)$ shows that $(P_n-P_0)(L_1(Q_n^M)-L(Q_{0n}^M))=o_P(1/\sqrt{n}$, which proves 
$d_{01}(Q_n^M,Q_{0n}^M)=o_P(1/\sqrt{n})$.


The class ${\cal F}_{v,M}$ of $d$-variate cadlag functions on $[0,\tau]$ with variation norm smaller than $M$ can be generated as a convex hull of indicators $\{I_{[0,x]}:x\in [0,\tau]\}$.
Corollary  2.6.12 in van der Vaart, Wellner (1996) shows that the entropy of this class ${\cal F}_{v,M}$ of functions satisfies:
\[
\sup_{\Lambda}\sqrt{\log N(\epsilon\pl F_{v,M}\pl_{P_0},{\cal F}_{v,M},L^2(\Lambda))}\leq K \epsilon^{-(1-1/(d+1)}.\]
Let $\alpha(d)=1/(d+1))$.
A recent theorem in van der Vaart, Wellner establishes the following result for a Donsker class ${\cal F}$ with envelope $F$: If $Pf^2\leq \delta^2 PF^2$, then
\begin{equation}\label{aadz1}
E\pl G_n\pl_{\cal F}\leq J(\delta,{\cal F},L^2)\left(1+\frac{ J(\delta,{\cal F},L_2)}{\delta^2 \sqrt{n} \pl F\pl_{P_0}}\right) \pl F\pl_{P_0},\end{equation}
where
\[
J(\delta,{\cal F},L^2)=\sup_Q \int_0^{\delta} \left( \log(1+N(\epsilon\pl F\pl_{P_0},{\cal F},L^2(Q)) \right)^{0.5} d\epsilon\]
is the entropy integral from $0$ to $\delta$.
We already established that $Pf_n^2=o_P(n^{-1/2})$ for $f_n=L_1(Q_n^M)-L_1(Q_{0n}^M)$. Let ${\cal F}_{v,M,\delta}=\{f\in {\cal F}_{v,M}:\pl f\pl_{P_0}<\delta\}$.
The envelope $F_{v,M,\delta}$ of this class can be selected to be the constant function $M$.
% and its $L^2(P_0)$-norm does not converge to zero if  $\delta=\delta_n$ converges to zero. 
Thus, we can apply this finite sample bound (\ref{aadz1}) with $\delta=\delta_n=n^{-1/4}$. The above bound can be  bounded by $J(\delta_n,{\cal F}_{v,M,\delta_n},L^2)$ which itself is bounded by $O(\delta^{\alpha}_n)$.
This proves that $G_nf_n$ converges to zero at a rate faster than $n^{-\alpha/4}$.
This proves thus that $d_{01}(Q_n^M,Q_{0n}^M)=O_P(n^{-(0.5+\alpha/4)})$, which establishes the second statement of the lemma. 

The final statement involves applying this same inequality (\ref{aad1}) to ${\cal F}={\cal Q}_{j,n,M}^1$ to establish the rate of the MLE of $Q_{j,0,n}^M$ based on the actual entropy of ${\cal Q}_{j,n,M}^1$
instead of the entropy of its dominating set ${\cal F}_{v,M}$, $j=1,\ldots,k_1$.

$\Box$


\subsection{Super-Learning: A cross-validated MLE tuning the variation norm of the fit.}

For an $M\in \openr^{k_1}_{>0}$, let $\hat{Q}_M:{\cal M}_{np}\rightarrow {\cal Q}_{n,M}\subset {\cal F}_{v,M}^{k_1}$ for which $d_{01}(Q_{M,n}=\hat{Q}_M(P_n),Q_{0n}^M)=o_P(n^{-\lambda_1})$ for $\lambda_1\in \openr^{k_1}_{>0}$ with $\lambda_1>0.5$, such as an MLE $Q_{M,n}$ satisfying $P_n L_1(Q_{M,n})=\inf_{Q\in {\cal Q}_{n,M}}P_n L_1(Q)+o_P(n^{-1/2})$ analyzed in the previous subsection. We showed that $\lambda_1$ can be chosen so that $r_{Q,MLE}^2(n)=O(n^{-\lambda_1})$.
Let ${\cal K}_{1,n,v}$ be an ordered collection  $M_1^n<M_2^n<\ldots<M_{K_{1,n,v}}$ of vector constants, and consider the corresponding collection of $K_{1,n,v}$ candidate estimators 
$\hat{Q}_M$, $M\in {\cal K}_{1,n,v}$. We assume that this index set ${\cal K}_{1,n,v}$ is increasing in $n$ and that $\lim\sup_{n\rightarrow\infty} M_{K_{1,n,v}}=\max(M_{Q,v},M_{L_1(Q),v})$, i.e it converges to infinity or it achieves  the maximal  possible value in the case that $M_{Q,v},M_{L_1(Q),v}$ are finite.  
 %where $\lim_{n\rightarrow\infty}M_{J_{1,v,n}}^n>\pl Q_{0}\pl_v$.
  Thus, for all $M\in {\cal K}_{1,n,v}$ with $M>\max(\pl Q_0\pl_v,\pl L_1(Q_0)\pl_v)$, we have that $d_{01}(\hat{Q}_{M}(P_n),Q_0)=o_P(n^{-\lambda_1})$.
In addition, let $\hat{Q}_j:{\cal M}_{np}\rightarrow {\cal Q}_n$, $j\in {\cal K}_{1,n,a}$ be an additional collection of  $K_{1,n,a}$ estimators of $Q_0$, for example, including a variety of parametric model as well as machine learning based estimators.  This defines an index set ${\cal K}_{1,n}={\cal K}_{1,n,v}\cup {\cal K}_{1,n,a}$ representing 
a collection of $K_{1n}=K_{1,n,v}+K_{1,n,a}$ candidate estimators $\{\hat{Q}_{k}:k\in {\cal K}_{1n}\}$.

%Let $B_n\in \{0,1\}^n$ be a random vector with $V$ possible realizations which defines a split in a training sample $\{i:B_n(i)=0\}$ and validation sample$\{i:B_n(i)=1\}$, where $B_n$ is independent of $(O_1,\ldots,O_n)$. Let $q$ be such that $P(\sum_i B_n(i)/n \geq q)=1$.Let $P_{n,B_n}^1,P_{n,B_n}^0$ be the empirical probability distributions of the validation and trainmen sample, respectively.
%Let ${\cal K}_{1n}=\{1,\ldots,J_{1n}\}\cup\{(v,1),\ldots,(v,J_{1,v,n})\}$ be the index set for the $K_{1n}$ candidate estimators.
We define the cross-validation selector as the index
\[
k_{1n}=\hat{K}_1(P_n)=\arg\min_{k\in {\cal K}_{1n}} E_{B_n}P_n L_1(\hat{Q}_k(P_{n,B_n}^0))\]
that minimizes the cross-validated risk $E_{B_n}P_nL_1(\hat{Q}_k(P_{n,B_n}^0))$ over all choices $k$ of candidate estimators. 
Our proposed super-learner is defined by
\begin{equation}\label{SLQ}
Q_n=\hat{Q}(P_n)=E_{B_n}\hat{Q}_{k_n}(P_{n,B_n}^0).\end{equation}

For an $M\in \openr^{k_2}_{>0}$, let  $\hat{G}_M:{\cal M}_{np}\rightarrow {\cal G}_{n,M}\subset {\cal F}_{v,M}^{k_2}$ for which $d_{02}(G_{M,n}=\hat{G}_M(P_n),G_{0n}^M)=O_P(n^{-\lambda_2})$ for a $\lambda_2\in \openr^{k_2}_{>0}$ with $\lambda_2>0.5$. In the previous section we showed that we can select $\lambda_2$ so that
$r_{G,MLE}^2(n)=O(n^{-\lambda_2})$.
Let ${\cal K}_{2,n,v}$ be an ordered collection of $k_2$-dimensional constants, and consider the corresponding collection of candidate estimators 
$\hat{G}_M$, $M\in {\cal K}_{2,n,v}$. We assume the index set ${\cal K}_{2,n,v}$ is increasing in $n$ and that $\lim\sup_{n\rightarrow\infty} M_{K_{2,n,v}}=\max(M_{G,v},M_{L_2(G),v})$, i.e. it converges to infinity or it achieves the maximal possible value in the case that $M_{G,v},M_{L_2(G),v}$ are finite. 
Thus, for all $M\in {\cal K}_{2,n,v}$ with $M>\max(\pl G_0\pl_v,\pl L_2(G_0)\pl_v)$, we have that $d_{02}(\hat{G}_M(P_n),G_0)=O_P(n^{-\lambda_2})$.
In addition, let $\hat{G}_j:{\cal M}_{np}\rightarrow {\cal G}_n$, $j\in {\cal K}_{2,n,a}$, be an additional  collection of $K_{2,n,a}$ estimators of $G_0$.
This defines a collection of $K_{2n}=K_{2,n,v}+K_{2,n,a}$ candidate estimators $\{\hat{G}_k:k\in {\cal K}_{2n}\}$ of $G_0$.

%Let $B_n\in \{0,1\}^n$ be a random vector with $V$ possible realizations which defines a split in a training sample $\{i:B_n(i)=0\}$ and validation sample$\{i:B_n(i)=1\}$, where $B_n$ is independent of $(O_1,\ldots,O_n)$. Let $q$ be such that $P(\sum_i B_n(i)/n \geq q)=1$.Let $P_{n,B_n}^1,P_{n,B_n}^0$ be the empirical probability distributions of the validation and trainmen sample, respectively.
%Let ${\cal K}_{2n}=\{1,\ldots,J_{2n}\}\cup\{(v,1),\ldots,(v,J_{2,v,n})\}$ be the index set for the $K_n$ candidate estimators.
We define the cross-validation selector as the index
\[
k_{2n}=\hat{K}_2(P_n)=\arg\min_{k\in {\cal K}_{2n}} E_{B_n}P_n L_1(\hat{G}_k(P_{n,B_n}^0))\]
that minimizes the cross-validated risk $E_{B_n}P_nL_2(\hat{G}_k(P_{n,B_n}^0))$ over all choices $k$ of candidate estimators. 
Our proposed super-learner of $G_0$ is defined by
\begin{equation}\label{SLQ}
G_n=\hat{G}(P_n)=E_{B_n}\hat{G}_{k_n}(P_{n,B_n}^0).\end{equation}








The following lemma proves that the super-learner $\hat{Q}(P_n)$ converges to $Q_0$ at least at the rate $n^{-\lambda_1}$: $d_{01}(\hat{Q}(P_n),Q_0)=O_P(n^{-\lambda_1})$. In the previous subsection we showed that this worst case rate is given by $r_{Q,MLE}(n)$, so that we have $d_{01}(\hat{Q}(P_n),Q_0)=O_P(r_{Q,MLE}(n))$.
The next lemma also shows that the super-learner is asymptotically equivalent with the oracle selected candidate estimator, or achieves a the parametric rate of a correctly specified parametric model. 
\begin{lemma}\label{thslM1n}
%Assume that $L_1(Q)$ be a convex loss function in the sense that $P_0L_1(\sum_{j=1}^m\alpha_jQ_j)\leq \sum_{j=1}^m\alpha_jP_0L_1(Q_j)$ when $\sum_j\alpha_j=1$ and $\min_j\alpha_j\geq 0$.
Let $\lambda_1$ be chosen so that $r_{Q,MLE}^2(n)=O(n^{-\lambda_1})$.
We have
\begin{equation}\label{conservativebound}
d_{01}(\hat{Q}(P_n),Q_{0n})=O_P(n^{-\lambda_1})+O_P\left(C(M_{1Q,n},M_{2Q,n},\delta)\frac{\log K_{1n}}{n}\right ).\end{equation}

In addition, we have, for any $\delta>0$, 
\[
d_{01}(Q_n,Q_{0n})\leq (1+2\delta) E_{B_n}\min_{k\in {\cal K}_{1n}} d_{01}(\hat{Q}_k(P_{n,B_n}^0),Q_{0n})+O_P\left(C(M_{1Q,n},M_{2Q,n},\delta)\frac{\log K_{1n} }{n} \right),\]
for a constant $C(M_1,M_2,\delta)=2(1+\delta)^2(2M_1/3+M_{2}^2/\delta)$.
If for a fixed $\delta>0$,  $C(M_{1Q,n},M_{2Q,n},\delta)\log K_{1n}/n$ divided by  $E_{B_n}\min_k d_{01}(\hat{Q}_{k}(P_{n,B_n}^0),Q_{0n})$ is $o_P(1)$, then 
\[
\frac{d_{01}(\hat{Q}(P_n),Q_{0n})}{E_{B_n}\min_kd_{01}(\hat{Q}_k(P_{n,B_n}^0),Q_{0n})}-1=o_P(1).\]
If  for a fixed $\delta>0$, $E_{B_n}\min_k d_{01}(\hat{Q}_{k}(P_{n,B_n}^0),Q_{0n})=O_P(C(M_{1Q,n},M_{2Q,n},\delta)\log K_{1n} /n)$, then 
\[
d_{01}(\hat{Q}(P_n),Q_{0n})=O_P(C(M_{1n},M_{2n},\delta)\log K_{1n} /n).\]
\end{lemma}


 The result Lemma \ref{thslM1n} is a simple corollary of the following finite sample oracle inequality for cross-validation (REFS), combined with exploiting the convexity of the loss function allowing us to bring the $E_{B_n}$ inside the loss-based dissimilarity. 

\begin{lemma}
%Suppose that $\sup_{o\in {\cal O},Q\in {\cal Q}_n}\mid L_1(Q)(o)-L_1(Q_{0n})(o)\mid <M_1$ and \[\sup_{Q\in {\cal Q}} \frac{P_0 \{L(Q)-L(Q_0)\}^2}{P_0\{L(Q)-L(Q_0)\}}<M_2.\]
For any $\delta>0$, there exists a constant $C(M_{1Q,n},M_{2Q,n},\delta)=2(1+\delta)^2(2M_{1Q,n}/3+M_{2Q,n}^2/\delta)$ such that
\begin{eqnarray*}
E_0\{E_{B_n}d_{01}(\hat{Q}_{k_{1n} }(P_{n,B_n}^0,Q_0)\}&\leq& (1+2\delta)E_0\{E_{B_n}\min_k d_{01}(\hat{Q}_k(P_{n,B_n}^0),Q_0)\}\\
&& +2C(M_{1Q,n},M_{2Q,n},\delta)\frac{1+\log K_{1n}}{n\bar{B}_n}.
\end{eqnarray*}
Similarly,  for any $\delta>0$, 
\begin{eqnarray*}
E_{B_n}d_{01}(\hat{Q}_{k_{1n}}(P_{n,B_n}^0,Q_0)&\leq& (1+2\delta)E_{B_n}\min_k d_{01}(\hat{Q}_k(P_{n,B_n}^0),Q_0)\}\\
&& +R_n,
\end{eqnarray*}
where $ER_n\leq 2C(M_{1Q,n},M_{2Q,n},\delta)\frac{1+\log K_{1n} }{n\bar{B}_n}$, so that, in particular, $ER_n=O_P(C(M_{1Q,n},M_{2Q,n},\delta)(1+\log K_{1n})/n)$.

If $\log K_{1n}/n $ divided by $E_{B_n}\min_k d_{01}(\hat{Q}_k(P_{n,B_n}^0),Q_0)\}$ converges to zero in probability, 
then we also have
\[
\frac{E_{B_n}d_{01}(\hat{Q}_{k_n}(P_{n,B_n}^0,Q_0)}{E_{B_n}\min_k d_{01}(\hat{Q}_k(P_{n,B_n}^0,Q_0)}\rightarrow_p 1.\]
Similarly, if $\log K_{1n}/n$ divided by $E_0E_{B_n}\min_k d_{01}(\hat{Q}_k(P_{n,B_n}^0),Q_0)\}$ converges to zero,
then we also have
\[
\frac{E_0E_{B_n}d_{01}(\hat{Q}_{k_n}(P_{n,B_n}^0,Q_0)}{E_0E_{B_n}\min_k d_{01}(\hat{Q}_k(P_{n,B_n}^0,Q_0)}\rightarrow 1.\]
\end{lemma}


 
The same lemma applies to the analogue estimator $\hat{G}(P_n)$ of $G_0$.
\begin{lemma}\label{thslM1nG}
%Assume that $L_1(Q)$ be a convex loss function in the sense that $P_0L_1(\sum_{j=1}^m\alpha_jQ_j)\leq \sum_{j=1}^m\alpha_jP_0L_1(Q_j)$ when $\sum_j\alpha_j=1$ and $\min_j\alpha_j\geq 0$.
Let $\lambda_2$ be chosen so that $r_{G,MLE}^2(n)=O(n^{-\lambda_2})$.
We have
\begin{equation}\label{conservativebound}
d_{02}(\hat{G}(P_n),G_{0n})=O_P(n^{-\lambda_2})+O_P\left(C(M_{1G,n},M_{2G,n},\delta)\frac{\log K_{2n}}{n}\right ).\end{equation}

In addition, we have, for any $\delta>0$, 
\[
d_{02}(G_n,G_{0n})\leq (1+2\delta) E_{B_n}\min_{k\in {\cal K}_{2n}} d_{02}(\hat{G}_k(P_{n,B_n}^0),G_{0n})+O_P\left(C(M_{1G,n},M_{2G,n},\delta)\frac{\log K_{2n} }{n} \right),\]
for a constant $C(M_1,M_2,\delta)=2(1+\delta)^2(2M_1/3+M_{2}^2/\delta)$.
If for a fixed $\delta>0$,  $C(M_{1G,n},M_{2G,n},\delta)\log K_{2n}/n$ divided by  $E_{B_n}\min_k d_{02}(\hat{G}_{k}(P_{n,B_n}^0),G_{0n})$ is $o_P(1)$, then 
\[
\frac{d_{02}(\hat{G}(P_n),G_{0n})}{E_{B_n}\min_kd_{02}(\hat{G}_k(P_{n,B_n}^0),G_{0n})}-1=o_P(1).\]
If  for a fixed $\delta>0$, $E_{B_n}\min_k d_{02}(\hat{G}_{k}(P_{n,B_n}^0),G_{0n})=O_P(C(M_{1G,n},M_{2G,n},\delta)\log K_{2n} /n)$, then 
\[
d_{02}(\hat{G}(P_n),G_{0n})=O_P(C(M_{1G,n},M_{2G,n},\delta)\log K_{1n} /n).\]
\end{lemma}



%Appendix material
\subsection{Constraining the variation norm of the data distribution does not affect the canonical gradient of the model}
In the above formulation of the one-step TMLE, we assumed that both $\hat{Q}(P_n)$ and its update $Q_n^*$ are elements of 
${\cal Q}_n$. By construction this holds for our initial estimator $\hat{Q}(P_n)$. The update will naturally be an element of ${\cal Q}_n$ by our assumption that the least favorable submodel $\{Q_{n,\epsilon}:\epsilon\}\subset {\cal Q}_n$ is a submodel of ${\cal Q}_n$. 
However, one might wonder why this would  hold for  a least favorable submodel through $Q_n$ with score equal to the  efficient influence curve at $(Q_n,G_n)$ in the actual model 
${\cal M}$? The universal bound assumptions enforced by ${\cal M}_n$ are not affecting the tangent space at a $P\in {\cal M}_n$: i.e. the tangent space at $P$ in model ${\cal M}$ is identical to the tangent space at $P$ in the model ${\cal M}_n$. This means that the efficient influence at a $P\in {\cal M}_n$ for the model ${\cal M}_n$
is the same as the efficient influence curve at this $P$ for the model ${\cal M}$.  This strongly suggests that a naturally selected least favorable submodel  for model ${\cal M}$ through a $Q\in {\cal M}_n$  will also be a submodel of ${\cal M}_n$ for a small enough range of $\epsilon$ values. Therefore, we expect this to be a non-issue, as also demonstrated in our example.

The fact that supremum norm and $L^2(P_0)$ bounds do not change the tangent space at a $P\in {\cal M}_n$ is easily understood, but one might wonder if a strict bound on the variation norm could restrict the class of possible submodels through $P$ enough so that the closure of the linear span of its scores is a strict subset of the tangent space at $P$ under model ${\cal M}$.
To obtain some insight in this we consider a particular example.

 Let $O$ be a univariate random variable and let ${\cal M}$ be a nonparametric model dominated by the Lebesgue  measure $\mu$ that assumes that all densities are differentiable. 
The tangent space $T(P)$ at $P\in {\cal M}$ for this model is saturated and thus equals $L^2_0(P)$. For a $P\in {\cal M}$, let $p=dP/d\mu$ be its density and let $p^{\prime}$ be its derivative
Let ${\cal M}_n$ be the submodel that enforces that $C=\sup_{P\in {\cal M}_n}\pl p^{\prime}\pl_{\infty}<\infty$.
Let $T_n(P)$ be the tangent space at $P\in {\cal M}_n$ for model ${\cal M}_n$. Suppose that $P$ has compact support ${\cal O}(P)\subset \openr$. 
Consider a submodel $\{p_{\epsilon}=(1+\epsilon S)p:\epsilon\in (-\delta,\delta)\}$ for some $\delta>0$ with score $S\in L^2_0(P)$ at a $P\in {\cal M}_n$ so that 
$\pl p^{\prime}\pl_{\infty}<C<\infty$, where the supremum is over the support ${\cal O}(P)$.
We have $p^{\prime}_{\epsilon}=(1+\epsilon S^{\prime}) p^{\prime}$. This will satisfy $\pl p^{\prime}_{\epsilon}\pl_{\infty}<C$ if 
\[
\pl S^{\prime}\pl_{\infty}< \frac{C-\pl p^{\prime}\pl_{\infty}}{\delta \pl p^{\prime}\pl_{\infty}}.\]
We can select $\delta>0$ equal to an arbitrarily small number larger than 0. This shows that any $S\in L^2_0(P)$ for which 
its derivative $S^{\prime}$ has a bounded supremum norm is an element of the tangent space $T_n(P)$. However, any function in $L^2_0(P)$ can be arbitrarily well approximated  in $L^2_0(P)$  by functions that have a uniformly bounded derivative (where this bound can be arbitrarily large).
This proves that $T_n(P)=L^2_0(P)$ and thus that putting bounds on the derivative do not affect the tangent space of the model. 

Consider now a submodel ${\cal M}_n$ of ${\cal M}$ that enforces $C=\sup_{P\in {\cal M}_n}\pl p\pl_v<\infty$.  As above,  let's consider again the submodel
$\{p_{\epsilon}=(1+\epsilon S)p:\epsilon\in (-\delta,\delta)\}$ for some $\delta>0$ with score $S\in L^2_0(P)$ at a $P\in {\cal M}_n$, so that we know 
$\pl p\pl_v<C$. Let ${\cal O}(P)$ be a compact subset of $\openr$. We have \[
\pl p_{\epsilon}\pl_v\leq \int_{{\cal O}(P)} \mid p(dx)\mid +\epsilon \int_{{\cal O}(P)} p(x)\mid S(dx)\mid +\mid S(x)p(dx) \mid .\]
Since $\pl p\pl_{\infty}\leq C$, we can further conservatively bound the right-hand side by $\pl p\pl_v+\epsilon C(\pl S\pl_v+\pl S\pl_{\infty})$.
Thus, if $\pl S\pl_v< (C-\pl p\pl_v)/(2C\delta)$, then $\{p_{\epsilon}:\epsilon\in (-\delta,\delta)\}\subset {\cal M}_n$.
We can select $\delta>0$ arbitrarily small. This proves that any $S\in L^2_0(P)$ for which $\pl S\pl_v<\infty$ is a score of a parametric submodel of ${\cal M}_n$.
The closure of the linear span of this set in $L^2_0(P)$ equals $L^2_0(P)$ again, so that $T_n(P)=T(P)=L^2_0(P)$.

Based on these two examples, it follows that indeed additional universal variation norm bounds on the model ${\cal M}$ are truly global constraints which do thus not affect the tangent space and accordingly the 
efficient influence curve of a pathwise differentiable target parameter.  As a consequence, at any $P\in {\cal M}_n$, a least favorable submodel of ${\cal M}_n$ through $P$ for model ${\cal M}_n$ will also be a least favorable submodel through $P$ for model ${\cal M}$.





\subsection{Preservation of the desired rate for the targeted estimator}
Above we constructed an initial super-learner $\hat{Q}$ of $Q_0$ satisfying $d_{01}(\hat{Q}(P_n),Q_0)=O_P(n^{-\lambda_1})$ where $\lambda_1\in \openr^{k_1}_{>0}$
can be chosen so that $r_Q^2(n)=O(n^{-\lambda_1})$. In particular, we have $r_Q(n)<r^*(n)<n^{-1/4}$.
Similarly, we have constructed such a super-learner $\hat{G}$ of $G_0$. 
However, our one-step TMLE relies on its targeted version $Q_n^*=Q_{n,\epsilon_n}$, so that we still need to establish a rate for this targeted version, where we can use that we already have a rate for $Q_n$.

\begin{lemma}\label{tmlelemma1}
Suppose $d_{01}(Q_n,Q_{0n})=O_P(n^{-lambda_1})$ for a $\lambda_1\in \openr^{k_1}_{>0}$ with $\lambda_1>0.5$. We can set $\lambda_1$ so that
$n^{-\lambda_1}=O(r_Q^2(n))$.
Suppose also that $\alpha_1\in \openr^{k_1}_{>0}$ is chosen so that for ${\cal F}_{1n}=\{L_1(Q):Q\in {\cal Q}_n\}/M_{L_1(Q)v,n}$ with envelope $F_{1n}<M_{1Q,n}/M_{L_1(Q)v,n}$ we have
\[
\sup_{\Lambda}\sqrt{\log (1+N(\epsilon \pl F_{1n}\pl_{P_0},{\cal F}_{1n},L^2(\Lambda)) )}<K \frac{1}{\epsilon^{1-\alpha_1}}.\]
%note alpha is a vector!!
Let $d_1\in \openn^{k_1}_{>0}$ be the vector of integers indicating the dimension of the domain of $Q=(Q_1,\ldots,Q_{k_1})$. 
In a nonparametric model ${\cal M}_n$ we have that this holds for $\alpha_1 =1/(d_1+1)$, so that we will always have $\alpha_1>1/(d_1+1)$.
Then, 
\begin{eqnarray*}
E_0 d_{01}(Q_n^*,Q_{0n})&\leq& n^{-1/2} n^{-\alpha_1/2} C(M_{L_1(Q)v,n},M_{2Q,n},M_{1Q,n},\alpha_1)+O(n^{-\lambda_1}),
\end{eqnarray*}
where
\[
\begin{array}{l}
C(M_{L_1(Q)v,n},M_{2Q,n},M_{1Q,n},\alpha_1)=\\
M_{L_1(Q)v,n} \left\{M_{2Q,n}M_{L_1(Q)v,n}\}^{\alpha_1}\{ M_{1Q,n}/M_{L_1(Q)v,n}\right\}^{1-\alpha_1^2}\\
+
M_{L_1(Q)v,n}\left\{ M_{1Q,n}/M_{L_1(Q)v,n}\}^{2\alpha_1(1-\alpha_1)}\{M_{2Q,n}M_{L_1(Q)v,n}  \}^{-2(1-\alpha_1)}n^{-\alpha_1/2}\right\}\\
+O(n^{-\lambda_1}).
\end{array}
\]
\end{lemma}
{\bf Proof:}
We have that $P_n L_1(Q_{n,\epsilon_n})=\min_{\epsilon} P_n L_1(Q_{n,\epsilon})$. This yields the following inequality:
\begin{eqnarray*}
0&\leq & d_{01}(Q_n^*,Q_{0n})=P_0L_1(Q_{n,\epsilon_n})-P_0L_1(Q_{0n})\\
&=&P_0L_1(Q_{n,\epsilon_n})-P_0L_1(Q_n)+P_0L_1(Q_n)-P_0L_1(Q_{0n})\\
&=& P_0L_1(Q_{n,\epsilon_n})-P_0L_1(Q_n)+d_{01}(Q_n,Q_{0n})\\
&=& P_0\{L_1(Q_{n,\epsilon_n})-L_1(Q_n)\}  +O_P(n^{-\lambda_1})     \\
&=&-(P_n-P_0)\{L_1(Q_{n,\epsilon_n})-L_1(Q_n)\}+P_n\{L_1(Q_{n,\epsilon_n})-L_1(Q_n)\}
+O_P(n^{-\lambda})\\
&\leq &-(P_n-P_0)\{L_1(Q_{n,\epsilon_n})-L_1(Q_n)\}
+O_P(n^{-\lambda})\\
%&=&-(P_n-P_0)\{L_1(Q_{n,\epsilon_n})-L_1(Q_{0n})\}+(P_n-P_0)\{L_1(Q_n)-L_1(Q_{0n})\}+O_P(n^{-\lambda})\\
\end{eqnarray*}
%We have $\pl L_1(Q_n)-L_1(Q_{0n})\pl_{P_0}^2=O_P(n^{-\lambda})$.
We have that the variation norm and supremum norm of $L_1(Q_n^*)-L_1(Q_n)$ are bounded by $M_{L_1(Q)v,n}$ and $M_{1Q,n}$, respectively.
Let ${\cal F}_n=\{L_1(Q)-L_1(Q_{\epsilon}):Q\in {\cal Q}_n,\epsilon\}$ and note that it is a subset of ${\cal F}_n^+=\{f\in D^{k_1}[0,\tau ]: \pl f\pl_v\leq M_{L_1(Q)v,n},\pl f\pl_{\infty}<M_{1Q,n}\}$.
We also note that the envelope $F_n$ of ${\cal F}_n$ satisfies $\pl F_n\pl_{P_0}\leq M_{1Q,n}$.
Then, the right-hand side of the above inequality can be represented as $(P_n-P_0)f_n+O_P(n^{-\lambda})$ for an $f_n\in {\cal F}_n$.
Let ${\cal F}_{1n}={\cal F}_n/M_{L_1(Q)v,n}$. We have $\pl F_{1n}\pl_{P_0}\leq M_{1Q,n}/M_{L_1(Q)v,n}$.
By assumption we have $\sup_{\Lambda}\sqrt{\log (1+N(\epsilon\pl F_{1n}\pl_{P_0},{\cal F}_{1n},L^2(\Lambda)) } \leq K \epsilon^{-\alpha}$.
We have ${\cal F}_n\subset {\cal F}_n^+$, and the latter has a covering number bounded by the choice $\alpha=1/(d+1)$ so that we know that
$\alpha\leq 1/(d+1)$.
Define $d_{01}^n(Q_n^*,Q_{0n})=d_{01}(Q_n^*,Q_{0n})/M_{L_1(Q)v,n}$. We have
\[
d_{01}^n(Q_n^*,Q_{0n})\leq (P_n-P_0)f_{1n}+O_P(n^{-\lambda_1}/M_{L_1(Q)v,n}),\]
where $f_{1n}\in {\cal F}_{1n}$, $\pl F_{1n}\pl_{P_0} M_{1Q,n}/M_{L_1(Q)v,n}$.
We also want to bound
$\pl f_{1n}\pl_{P_0}$ by $d_{01}^n(Q_n^*,Q_0)$. For this purpose we note 
\begin{eqnarray*}
\pl L_1(Q_n^*)-L_1(Q_n)\pl_{P_0}&\leq& \pl L_1(Q_n^*)-L_1(Q_{0n})\pl_{P_0}+
\pl L_1(Q_n)-L_1(Q_{0n})\pl_{P_0}\\
&\leq& M_{2Q,n} \{d_{01}(Q_n^*,Q_{0n})\}^{0.5}+O_P(n^{-\lambda_1/2})\\
&=& M_{2Q,n} M_{L_1(Q)v,n} \{d_{01}^n(Q_n^*,Q_{0n})\}^{0.5}+O_P(n^{-\lambda_1/2}).
\end{eqnarray*}
So we have the following setting for the analysis of $d_{01}^n(Q_n^*,Q_0)$:
\[
\begin{array}{l}
d_{01}^n(Q_n^*,Q_{0n})\leq (P_n-P_0)f_{1n}+O_P(n^{-\lambda_1}/M_{L_1(Q)v,n})\\
f_{1n}\in {\cal F}_{1n}, \pl F_{1n}\pl< M_{1Q,n}/M_{L_1(Q)v,n}\\
\sup_Q \sqrt{\log (1+N(\epsilon\pl F_{1n}\pl_{P_0},{\cal F}_{1n},L^2(Q)))}< 1/\epsilon^{1-\alpha},\ \alpha=1/(d+1)\\
\pl f_{1n}\pl_{P_0}^\leq  M_{2Q,n}M_{L_1(Q)v,n} \{d_{01}^n(Q_n^*,Q_{0n})\}^{0.5}.
\end{array}
\]
We will now apply the following Lemma \ref{aadlemma1}, which is a corollary of theorem in  recent van der Vaart, Wellner.
Specifically, we apply Lemma \ref{aadlemma1} with $d_0=d_{01}$, $Q_n=Q_n^*$, $Q_0=Q_{0n}$, $f_n=f_{1n}$, ${\cal F}_n={\cal F}_{1n}$ with $M_n=M_{1Q,n}/M_{L_1(Q)v,n}$ and
$M_{2n}=M_{2Q,n}M_{L_1(Q)v,n}$ and $\alpha=1/(d+1)$.
This proves
\[
d_{01}^n(Q_n^*,Q_{0n})\leq n^{-1/2}n^{-\alpha/2} \frac{C(M_{L_1(Q)v,n},M_{2Q,n},M_{1Q,n},\alpha)}{M_{L_1(Q)v,n}}.\]
Thus, 
\[
d_{01}(Q_n^*,Q_{0n})\leq n^{-1/2}n^{-\alpha/2} C(M_{L_1(Q)v,n},M_{2Q,n},M_{1Q,n},\alpha).\]
This completes the proof.  $\Box$

 
 %alpha(d) and alpha should be  vector of length k_1, i..e alpha_1 and alpha_2 of dim k1 and k2
\begin{corollary}
Consider the super-learner $\hat{Q}(P_n)$ defined in (\ref{SLQ}).

Suppose $d_{01}(Q_n,Q_{0n})=O_P(n^{-lambda_1})$ for a $\lambda_1\in \openr^{k_1}_{>0}$ with $\lambda_1>0.5$. We can set $\lambda_1$ so that
$n^{-\lambda_1}=O(r_Q^2(n))$. 
%Suppose $d_{02}(G_n,G_{0n})=O_P(n^{-lambda_2})$ for a $\lambda_2\in \openr^{k_2}_{>0}$ with $\lambda_2>0.5$. We can set $\lambda_2$ so that$n^{-\lambda_2}=O(r_G^2(n))$.

Suppose also that $\alpha_1\in \openr^{k_1}_{>0}$ is chosen so that for ${\cal F}_{1n}=\{L_1(Q):Q\in {\cal Q}_n\}/M_{L_1(Q)v,n}$ with envelope $F_{1n}<M_{1Q,n}/M_{L_1(Q)v,n}$ we have
\[
\sup_{\Lambda}\sqrt{\log (1+N(\epsilon \pl F_{1n}\pl_{P_0},{\cal F}_{1n},L^2(\Lambda)) )}<K \frac{1}{\epsilon^{1-\alpha_1}}.\]
Let $d_1\in \openn^{k_1}_{>0}$ be the vector of integers indicating the dimension of the domain of $Q=(Q_1,\ldots,Q_{k_1})$. 
In a nonparametric model ${\cal M}_n$ we have that this holds for $\alpha_1 =1/(d_1+1)$, so that we will always have $\alpha_1>1/(d_1+1)$.

%Suppose also that $\alpha_2\in \openr^{k_2}_{>0}$ is chosen so that for ${\cal F}_{2n}=\{L_2(G):G\in {\cal G}_n\}/M_{L_2(G)v,n}$ with envelope $F_{2n}<M_{1G,n}/M_{L_2(G)v,n}$ we have\\sup_{\Lambda}\sqrt{\log (1+N(\epsilon \pl F_{2n}\pl_{P_0},{\cal F}_{2n},L^2(\Lambda)) )}<K \frac{1}{\epsilon^{1-\alpha_2}}.\]Let $d_2\in \openn^{k_2}_{>0}$ be the vector of integers indicating the dimension of the domain of $G=(G_1,\ldots,G_{k_2})$. In a nonparametric model ${\cal M}_n$ we have that this holds for $\alpha_2 =1/(d_2+1)$, so that we will always have $\alpha_2>1/(d_2+1)$.


Let $\lambda_1^*=0.5+\alpha_1/4$. 
%where $\alpha(d)=1/(d+1)$.DEFINE  ALPHA FROM PREVIOUS WHICH DEFINES A LAMBDA_1*=0.5+ALPHA/4, CAN SAY VBETTER THAN USING ALPHA(D) INSTEAD OF ALPHA
%they have rate $n^{-\lambda(d)}$, where $\lambda(d)=0.5+\alpha(d)/4$.
Assume that 
\begin{eqnarray*}
\frac{\max(M_{1Q,n},M_{2Q,n}^2)\log K_{1n}}{n}&=&O(n^{-\lambda_1})\\
\frac{\max(M_{1G_n},M_{2G_n}^2)\log K_{2n}}{n}&=&O(n^{-\lambda_1})\\
%for targeted estimator, if we make RHS n^{-\alpha/4}, then rate lambda(d) preserved
n^{-\alpha_1/4} C(M_{L_1(Q)v,n},M_{2Q,n},M_{1Q,n},\alpha_1)&=&O(1).
\end{eqnarray*}
Then, $d_{01}((Q_n^*,Q_0)=o_P(n^{-\lambda_1^*})$.
\end{corollary}














Suppose that the model is bounded. Then we can not only  show that we preserve a rate faster than the desired $n^{-1/2}$, as in the previous lemmas, but we preserve the rate of the initial estimator 
$Q_n$. This is stated in the following lemma.
\begin{lemma}
Assume the model ${\cal M}$ is bounded. 
Assume $d_{01}(Q_n,Q_0)=O_P(n^{-\lambda_1})$ and $d_{02}(G_n,G_0)=O_P(n^{-\lambda_2})$.
For a $\lambda_1\in \openr^{k_1}_{>0}$ and $\lambda_2\in \openr^{k_2}_{>0}$, we define $\lambda=(\lambda_1,\lambda_2)\in \openr^{k_1+k_2}_{>0}$.

Let $S(Q,G,\epsilon)=\frac{d}{d\epsilon}L(Q_{\epsilon})$ (For a universal least favorable submodel we have
$S(Q,G,\epsilon)=D^*(Q_{\epsilon},G)$).
 Let $\epsilon_n=\arg\max_{\epsilon}P_n L(Q_{n,\epsilon})$ and assume it solves $P_n S(Q_n,G_n,\epsilon_n)=0$.
Assume the following analytic properties of the least favorable submodel:
%see proof, all analytic conditions on S(Q,\epsilon) and thus submodel.
\begin{itemize}
\item $d_{01}(Q_{n,\epsilon_n},Q_0)\rightarrow 0$, $d_{01}(Q_n,Q_0)\rightarrow 0$ and  $d_{02}(G_n,G_0)\rightarrow 0$ imply that $\epsilon_n\rightarrow 0$;
\item Along a sequence $(Q_n,G_n)$ with  $d_0((Q_n,G_n),(Q_0,G_0))=O(n^{-\lambda})$, we have
\[
P_0\{S(Q_n,G_n\epsilon_n)-S(Q_n,G_n,\epsilon_{0n})\}=\frac{d}{d\epsilon_{0n}}P_0S(Q_n,G_n,\epsilon_{0n})(\epsilon_n-\epsilon_{0n})+o(\mid \epsilon_n-\epsilon_{0n}\mid);\]
\item For a sequence $\epsilon_{n}\rightarrow 0$ and $(Q_n,G_n)$ with $d_0((Q_n,G_n),(Q_0,G_0))=O(n^{-\lambda})$, we have
 $\frac{d}{d\epsilon_n}P_0S(Q_n,G_n,\epsilon_{n})$ converges to $c_0=-\left . \frac{d}{d\epsilon}P_0S(Q_0,G_0,\epsilon)\right |_{\epsilon =0}>0$ with $c_0>0$.
%\item For a sequence $\epsilon_n\rightarrow 0$ and $(Q_n,G_n)$ with  $d_{0}((Q_n,G)n),(Q_0,G_0))=O(n^{-\lambda})$, we have $\pl S(Q_n,G_n,\epsilon_n)-S(Q_0,G_0,\epsilon_n)\pl_{P_0}=O(n^{-\lambda/2})$;
\item For some $\delta>0$,  $\sup_{\mid \epsilon\mid <\delta, P\in {\cal M}} \pl S(Q,G,\epsilon)\pl_v<\infty$.
\item If $d_0((Q_n,G_n),(Q_0,G_0))=O(n^{-\lambda})$ and $\epsilon_n\rightarrow 0$,  then $P_0\{S(Q_n,G_n,\epsilon_{n})-S(Q_0,G_0,\epsilon_{n}\}=O_P(n^{-\lambda/2})$;
\end{itemize}
Then, 
\[
\epsilon_n=O_P(n^{-\lambda_1/2})\mbox{ and } d_{01}(Q_{n,\epsilon_n},Q_0)=O_P(n^{-\lambda_1}).\]
\end{lemma}
{\bf Proof:}
%clean up notation i.e. add G_n etc
%In this proof $Q_n$ plays the role of $(Q_n,G_n)$.
%Let $S(Q_n,G_n,\epsilon)=\frac{d}{d\epsilon}L(Q_{n,\epsilon})$.
%We have $P_n S(Q_n,\epsilon_n)=0$.
Define $\epsilon_{0n}=\arg\min_{\epsilon}P_0L(Q_{n,\epsilon})$, which solves $P_0 S(Q_n,G_n,\epsilon_{0n})=0$.
We also define $\epsilon_0=0$ which solves $P_0S(Q_0,G_0,\epsilon_0)=0$.
It follows, analogue to the proof of previous Lemma \ref{tmlelemma1}, that $d_{01}(Q_{n,\epsilon_n},Q_{0n})=o_P(1)$. Suppose that
$d_{01}(Q_{n,\epsilon_n},Q_{0n})=o_P(1)$ and $d_{01}(Q_n,Q_{0n})=o_P(1)$ implies $\epsilon_n=o_P(1)$, which also implies $\epsilon_{0n}=o_P(1)$.
Thus, we have $\epsilon_n=o_P(1)$ and $\epsilon_{0n}=o_P(1)$.
Given that we know that $\epsilon_n=o_P(1)$, we want to prove that $\epsilon_n=O_P(n^{-\lambda_1/2})$.
We will prove this by proving $\epsilon_n-\epsilon_{0n}=O_P(n^{-0.5})$ and $\epsilon_{0n}=O_P(n^{-\lambda_1/2})$.
Note
\[
P_0\{S(Q_n,G_n,\epsilon_{n})-S(Q_nG_n,,\epsilon_{0n})\}=-(P_n-P_0)S(Q_n,G_n,\epsilon_n).\]
We assumed differentiability in $\epsilon$ uniformly in the sequence $Q_n$ with $d_{01}(Q_n,Q_0)=O_P(n^{-\lambda_1})$ in the sense that:
\[
P_0\{S(Q_n,G_n,\epsilon_n)-S(Q_n,G_n,\epsilon_{0n})\}=\frac{d}{d\epsilon_{0n}}P_0S(Q_n,G_n,\epsilon_{0n})(\epsilon_n-\epsilon_{0n})+o(\mid \epsilon_n-\epsilon_{0n}\mid).\]
We also assumed that $-\frac{d}{d\epsilon_{0n}}P_0S(Q_n,G_n,\epsilon_{0n})$ converges to $c_0=-\frac{d}{d\epsilon_0}P_0S(Q_0,G_0,\epsilon_0)>0$.
Then, it follows that
\[
\epsilon_n-\epsilon_{0n}=c_0^{-1} (P_n-P_0)S(Q_n,G_n,\epsilon_n)+o(\mid \epsilon_n-\epsilon_{0n}\mid).\]
By assumption, $\sup_{Q\in {\cal Q}, G\in {\cal G},\mid\epsilon\mid<\delta}\pl S(Q,G,\epsilon)\pl_v<C<\infty$, so that it follows that $\epsilon_n-\epsilon_{0n}=O_P(n^{-1/2})$.


Consider now  the equations $P_0S(Q_n,G_n,\epsilon_{0n})=P_0S(Q_0,G_0,\epsilon_0)=0$.
We have
\[
P_0\{S(Q_0,G_0,\epsilon_{0n})-S(Q_0,G_0,\epsilon_0)\}=-P_0\{S(Q_n,G_n,\epsilon_{0n})-S(Q_0,G_0,\epsilon_{0n})\}.\]
Thus, 
\[
\epsilon_{0n}-\epsilon_0=c_0^{-1} P_0\{S(Q_n,G_n,\epsilon_{0n})-S(Q_0,G_0,\epsilon_{0n})\}+o(\mid \epsilon_{0n}-\epsilon_0\mid).\]
We assumed that $P_0\{S(Q_n,G_n,\epsilon_{0n})-S(Q_0,G_0,\epsilon_{0n}\}=O_P(n^{-\lambda_1/2})$ if 
$d_{01}(Q_n,Q_0)=O_P(n^{-\lambda_1})$ and $\epsilon_{0n}=o_P(1)$.
This proves that $\epsilon_{0n}-\epsilon_0=O_P(n^{-\lambda_1/2})+o(\mid \epsilon_{0n}-\epsilon_0\mid)$, and thus
$\epsilon_{0n}=O_P(n^{-\lambda_1/2})$, which proves the first statement of the lemma.

$\Box$





\subsection{Important empirical process results}

A recent theorem in van der Vaart, Wellner establishes the following result for a Donsker class ${\cal F}_{n}$ with envelope $F_{n}$: If $Pf^2\leq \delta^2 PF^2$, then
\[
E\pl G_n\pl_{ {\cal F}_{n} }\leq J(\delta,{\cal F}_{n},L^2)\left(1+\frac{ J(\delta,{\cal F}_{n},L_2)}{\delta^2 \sqrt{n} \pl F_{n}\pl_{P_0}}\right) \pl F_{n}\pl_{P_0},\]
where
\[
J(\delta,{\cal F}_{n},L^2)=\sup_Q \int_0^{\delta} \left( \log(1+N(\epsilon\pl F_{n}\pl_{P_0},{\cal F}_n,L^2(Q)) \right)^{0.5} d\epsilon\]
is the entropy integral from $0$ to $\delta$.
A simple corollary of this theorem is the following lemma.
\begin{lemma}\label{aadlemma0}
Consider ${\cal F}_n$ with $\pl F_n\pl_{P_0}<M_n$, $\sup_Q\sqrt{\log (1+N(\epsilon\pl F_n\pl_{P_0},{\cal F}_n,L^2(Q)) )}<1/\epsilon^{1-\alpha}$.
\[
E\sup_{f\in {\cal F}_n,\pl f\pl_{P_0}<r_0(n)}\mid G_n(f)\mid\leq \{r_0(n)/M_n\}^{\alpha}M_n+\{r_0(n)/M_n\}^{2\alpha-2}n^{-0.5}.\]
If $r_0(n)<n^{-1/4}$, one should select $r_0(n)=n^{-1/4}$ in the above right hand side, giving
\[
E\sup_{f\in {\cal F}_n,\pl f\pl_{P_0}<r_0(n)}\mid G_n(f)\mid\leq \{n^{-0.25}/M_n\}^{\alpha}M_n+\{M_n\}^{2-2\alpha}n^{-\alpha/2}.\]
\end{lemma}



\begin{lemma}\label{aadlemma1}
Consider the following setting
\[
\begin{array}{l}
d_0(Q_n,Q_0)\leq (P_n-P_0)f_n\\
f_n\in {\cal F}_n,\ \pl F_n\pl_{P_0}\leq M_n\\
\sup_Q \sqrt{\log (1+N(\epsilon\pl F_{n}\pl_{P_0},{\cal F}_{n},L^2(Q)))}< 1/\epsilon^{1-\alpha}\\
\pl f_{n}\pl_{P_0}\leq  M_{2n} \{d_{0}(Q_n^*,Q_{0n})\}^{0.5}.
\end{array}
\]
Then
\[
d_0(Q_n,Q_0)\leq n^{-1/2}n^{-\alpha/2} C(M_n,M_{2n},\alpha),\]
where
\[
C(M_n,M_{2n},\alpha)=M_2(n)^{\alpha}M(n)^{1-\alpha^2}+
M(n)^{2\alpha(1-\alpha)}M_2(n)^{-2(1-\alpha)}n^{-\alpha/2}n^{-\alpha/2}.
\]
\end{lemma}

\begin{lemma}\label{aadlemma2}
Consider the following setting.
\begin{eqnarray*}
d_0(Q_n,Q_0)\leq (P_n-P_0)f_n\\
f_n\in {\cal F}_n, \ \pl F_n\pl_{P_0}\leq M_n\\
\pl f_n\pl_{P_0}\leq M_{2n}\sqrt{d_0(Q_n,Q_0)}\\
\sqrt{d_0(Q_n,Q_0)}=O_P(n^{0.25-\delta}), \ 0< \delta< 0.25\\
\sup_Q\sqrt{\log (1+N(\epsilon \pl F_n\pl_{P_0},{\cal F}_n,L^2(Q)) )}< 1/\epsilon^{1-\alpha}, \ 0<\alpha<1.
\end{eqnarray*}
Then,
\[
d_0(Q_n,Q_0)\leq n^{-1/2} C(M_n,M_{2n},\alpha,\delta),\]
where
\begin{eqnarray*}
C(M_n,M_{2n},\alpha,\delta)&=&(M_{2n}/M_n)^{\alpha}M_n n^{-(0.25-\delta)\alpha}\\
&&+ (M_n/M_{2n})^{2(1-\alpha)}n^{-2\delta(1-\alpha)} .
\end{eqnarray*}
If $\sqrt{d_0(Q_n,Q_0)}=O_P(n^{-1/4})$, then
\[
d_0(Q_n,Q_0)\leq n^{-1/2}C(M_n,M_{2n},\alpha),\]
where
\begin{eqnarray*}
C(M_n,M_{2n},\alpha)&=& (M_{2n}/M_n)^{\alpha}M_n n^{-0.25\alpha}\\
&&+ (M_n/M_{2n})^{2(1-\alpha)}n^{-\alpha/2} .
\end{eqnarray*}
\end{lemma}




%Next lemma is not right yet and may be above suffices, we should lose some rate relative to initial since clever covariate blows up with bounds that convergeto infinity.positivity bound will have to slow enough so that $\epsilon_n$ is in interior.



In theorem below we use $\alpha=1/(d+1)$ but just as we did for $L_1(Q)$ etc we should improve this alpha taking into account the actual  model ${\cal M}_n$ which make this class
generated by $D^*(Q_n^*,G_n)$ smaller. 

\begin{lemma}\label{aadlemma3}
Let $f_n=D^*(Q_n^*,G_n)-D^*(Q_0,G_0)$.
Assume $d_0(P_n^*,P_0)=O_P(n^{-\lambda})$ for some $\lambda>0.5$, so that, by our universal bound $M_{2D^*,n}$, 
\[
\pl f_n\pl_{P_0}< M_{2D^*,n} f_{D^*}(d_0(P_n^*,P_0))=O_P(n^{-\lambda/2} M_{2D^*,n}).\]
Assume
$M_{2D^*,n}/M_{D^*v,n}=O( n^{0.5\lambda-0.25})$.
Then, \[
E_0\mid \sqrt{n}(P_n-P_0)f_n\mid \leq  n^{-\alpha/4}C_1(M_{D^*,n},M_{D^*v,n},\alpha)+
n^{-\alpha/2} C_2(M_{D^*,n},M_{D^*v,n},\alpha),\]
where
\begin{eqnarray*}
C_1(M_{D^*,n},M_{D^*v,n})&=& \{M_{D^*,n}^{-1}M_{D^*v,n} \}^{\alpha}M_{D^*,n}\\
C_2(M_{D^*,n},M_{D^*v,n})&=&M_{D^*v,n} \{M_{D^*,n}M_{D^*v,n}^{-1}\}^{2-2\alpha}.
.\end{eqnarray*}
\end{lemma}
{\bf Proof:}
Let ${\cal F}_n=\{f: \pl f\pl_v\leq M_{D^*v,n},\pl f\pl_{\infty}<M_{D^*,n}\}$, and note that its envelope $F_n$ satisfies $\pl F_n\pl_{P_0}\leq M_{D^*,n}$.
Note that $f_n\in {\cal F}_n$. 
Let ${\cal F}_{1n}={\cal F}_n/M_{D^*v,n}$, and note that $(P_n-P_0)f_n=M_{D^*v,n}(P_n-P_0)f_{1n}$ where $f_{1n}=f_n/M_{D^*v,n}\in {\cal F}_{1n}$.
 We have $\pl F_{1n}\pl_{P_0}\leq M_{D^*,n}/M_{D^*v,n}$ and
 $\sup_Q\sqrt{\log (1+N(\epsilon\pl F_{1n}\pl_{P_0},{\cal F}_{1n},L^2(Q)))  } \leq K \epsilon^{-(1-\alpha)}$ with 
$\alpha=1/(d+1)$. 
We can now apply Lemma \ref{aadlemma0} with ${\cal F}_n={\cal F}_{1n}$, $M_n= M_{D^*,n}/M_{D^*v,n}$, $\alpha=1/(d+1)$, $r_0(n)=n^{-\lambda/2}M_{2D^*,n}/M_{D^*v,n}$. 
Since $M_{2D^*,n}/M_{D^*v,n}=O( n^{0.5\lambda-0.25})$
we have $r_0(n)<n^{-1/4}$.
% if >n^{-1/4} then this yields  \[E\pl G_n\pl_{{\cal F}_{1n,\delta=r_0(n)}\leq \left\{\{ n^{-\lambda/2}M_{2D^*,n}M_{D^*v,n}^{-1}M_{D^*,n}^{-1}M_{D^*v,n} \}^{\alpha}M_{D^*,n}M_{D^*v,n}^{-1}+\{n^{-\lambda/2}M_{2D^*,n}M_{D^*v,n}^{-1} M_{D^*,n}^{-1}M_{D^*v,n}\}^{2\alpha-2}n^{-0.5}\right\}.\]
Application of Lemma \ref{aadlemma0} yields
\[
E_0 G_n(f_{1n})\leq n^{-\alpha/4}C_1(M_{D^*,n},M_{D^*v,n},\alpha)/M_{D^*v,n}+
n^{-\alpha/2} C_2(M_{D^*,n},M_{D^*v,n},\alpha)/M_{D^*v,n}.\]
The desired bound for $E_0\mid G_n(f_n)\mid$ is the right-hand side multiplied with $M_{D^*v,n}$. $\Box$





\begin{lemma}\label{aadlemma0}
Consider ${\cal F}_n$ with $\pl F_n\pl_{P_0}<M_n$, $\sup_Q\sqrt{\log (1+N(\epsilon\pl F_n\pl_{P_0},{\cal F}_n,L^2(Q)) )}<1/\epsilon^{1-\alpha}$.
\[
E\sup_{f\in {\cal F}_n,\pl f\pl_{P_0}<r_0(n)}\mid G_n(f)\mid\leq \{r_0(n)/M_n\}^{\alpha}M_n+\{r_0(n)/M_n\}^{2\alpha-2}n^{-0.5}.\]
If $r_0(n)<n^{-1/4}$, one should select $r_0(n)=n^{-1/4}$ in the above right hand side, giving
\[
E\sup_{f\in {\cal F}_n,\pl f\pl_{P_0}<r_0(n)}\mid G_n(f)\mid\leq \{n^{-0.25}/M_n\}^{\alpha}M_n+\{M_n\}^{2-2\alpha}n^{-\alpha/2}.\]
\end{lemma}



The following lemma is needed in the analysis of the CV-TMLE.
\begin{lemma}\label{lemmaaad4}
Let $f_{n,\epsilon_n}\in {\cal F}_n=\{f_{n,\epsilon}:\epsilon\}$ where $\epsilon$ varies over a bounded set in $\openr^p$.
Suppose that $\pl f_{n,\epsilon_n}\pl_{P_0}=O_P(M_{2D^*,n}n^{-\lambda(d)/2}$. The envelope $F_n$ of ${\cal F}_n$ satisfies
$\pl F_n\pl_{P_0}\leq M_{D^*,n}$. We have $\sup_Q N(\epsilon\pl F_n\pl,{\cal F}_n,L^2(Q))< \epsilon^{-p}$.
Then, 
\[
E_0\mid G_n(f_{n,\epsilon_n})\mid \leq O\left( M_{2D^*,n}n^{-\lambda(d)/2}\left\{ \log n+\log\{M_{D^*,n}/M_{2D^*,n}\} \right\}\right) .\]
Define
\[
\tilde{C}(M_{D^*,n},M_{2D^*,n},\log n)\equiv M_{2D^*,n}\left\{ \log n+\log\{M_{D^*,n}/M_{2D^*,n}\right\}.\]
If $\tilde{C}(M_{D^*,n},M_{2D^*,n},\log n)/n^{\lambda/2}=o(1)$, then 
\[
\sqrt{n}(P_n-P_0)f_{n,\epsilon_n}=o_P(1).\]
 \end{lemma}
{\bf Proof:}
For simplicity, let's denote $f_{n,\epsilon_n}$ with $f_n$.
We apply the Theorem in van der Vaart, Wellner stating that 
\begin{equation}\label{b1}
E_0\mid G_n(f_n)\mid \leq J(\delta_n,{\cal F}_n)\left( 1+\frac{J(\delta_n,{\cal F}_n)}{\delta_n^2n^{0.5}\pl F_n\pl_{P_0}}\right) \pl F_n\pl_{P_0},\end{equation}
where $\delta_n=\frac{M_{2D^*,n}} {M_{D^*,n} }n^{-\lambda/2}$ and $J(\delta,{\cal F}_n)=\sup_Q\int_0^{\delta} \sqrt{\log (1+N(\epsilon \pl F_n\pl_{P_0},{\cal F}_n,L^2(Q)) )}d\epsilon$.
It is easy to show that $J(\delta,{\cal F}_n)=-p^{0.5}\int_0^{\delta}(\log \epsilon)^{0.5} d\epsilon$. We can conservatively bound this by replacing $(\log \epsilon)^{0.5}$ by 
$\log \epsilon$, and we have $\int_0^{\delta}\log \epsilon d\epsilon =\delta -\delta\log \delta=\delta(1+\log(\delta^{-1}))$.
The leading term in (\ref{b1}) is given by $J(\delta_n,{\cal F}_n)\pl F_n\pl_{P_0}$. 
This results in the following bound:
\[
M_{2D^*,n}n^{-\lambda/2} \log \{n^{\lambda/2}M_{D^*,n}/M_{2D^*,n}\} ,\]
which results in the stated bound.
$\Box$










































































Let $f_{R_2}:\openr^{k_1+k_2}_{\geq 0}\rightarrow\openr$ be a second order polynomial function so that
\[
\mid R_2(P,P_0)\mid \leq M_{R_2}(P,P_0) f_{R_2}(d_0(P,P_0)),\] 
for some constant $M_{R_2}(P,P_0)<\infty$. By being a second order polynomial function, it has the property that if $r(n)/n^{0.25}\rightarrow 0$, then $f_{R_2}(r(n))=o(n^{-0.5})$.
Similarly, let $f_{D^*}:\openr^{k_1+k_2}_{\geq 0}\rightarrow \openr$ be a second order polynomial function so that 
\[
\pl D^*(Q,G)-D^*(Q_0,G_0)\pl_{P_0}^2\leq M_{2D^*}^2(P,P_0) f_{D^*}(d_0(P,P_0))
\]
for some constant $M_{2D^*}(P,P_0)<\infty$.
We now define a number of universal bounds on the statistical model ${\cal M}$:
\begin{eqnarray*}
\tau&=&\tau({\cal M})=\sup_{P\in {\cal M}}\tau(P)\\
M_{1Q}&=&M_{1Q}({\cal M})=\sup_{Q,Q_0\in {\cal Q}}\pl L_1(Q)-L_1(Q_0)\pl_{\infty}\\
M_{2Q}&=&M_{2Q}({\cal M})=\sup_{P,P_0\in {\cal M}}\frac{ \pl L_1(Q)-L_1(Q_0)\pl_{P_0}}{\{d_{10}(Q,Q_0)\}^{0.5}}\\
M_{1G}&=&M_{1G}({\cal M})=\sup_{G,G_0\in {\cal G}}\pl L_2(G)-L_2(G_0)\pl_{\infty}\\
M_{2G}&=&M_{2G}({\cal M})=\sup_{P,P_0\in {\cal M}}\frac{ \pl L_2(G)-L_2(G_0)\pl_{P_0}}{\{d_{20}(G,G_0)\}^{0.5}}\\
M_{D^*}&=&M_{D^*}({\cal M})=\sup_{Q,G\in {\cal Q},{\cal G}} \pl D^*(Q,G)\pl_{\infty}\\
M_{2D^*}&=&M_{2D^*}({\cal M})=\sup_{P,P_0\in {\cal M}}\frac{\pl D^*(P)-D^*(P_0)\pl_{P_0}}{\{f_{D^*}(d_0(P,P_0))\}^{0.5}} \\
M_{R_2}&=&M_{R_2}({\cal M}=\sup_{P,P_0\in {\cal M}}\frac{\mid R_{2}(P,P_0)\mid}{ f_{R_2}(d_0(P,P_0)) }.
%M_{2D^*}&=&M_{2D^*}({\cal M}=\sup_{P,P_0\in {\cal M}}\frac{\pl D^*(P)-D^*(P_0)\pl_{P_0}^2}{d_0((Q,G),(Q_0,G_0))}
\end{eqnarray*}
Each of these $M_{1Q},M_{2Q},M_{1G},M_{2G}$ are defined as one-dimensional constants by taking the maximum over the components.
The bounds $M_{1Q},M_{2Q}$ guarantee excellent properties of the cross-validation selector based on the loss-function $L_1(Q)$, and  a bound on $M_{2Q}$ shows that the loss-based dissimilarity $d_{01}(Q,Q_0)$   behaves as a square of a norm. Similarly, the bounds $M_{1G},M_{2G}$ imply this for the loss function $L_2(G)$.
We also define the following universal variation norm bounds on the model ${\cal M}$:
\begin{eqnarray*}
M_{Q,v}&=&\sup_{P\in {\cal M}}\pl Q(P)\pl_v\\
M_{G,v}&=&\sup_{P\in {\cal M}}\pl G(P)\pl_v\\
M_{D^*,v}&=&\sup_{P\in {\cal M}}\pl D^*(P)\pl_v\\
M_{L_1(Q),v}&=&\sup_{P\in {cal M}}{\pl L_1(Q)\pl_v}
M_{L_2(G),v}&=&\sup_{P\in {cal M}}{\pl L_2(G)\pl_v}\\
\end{eqnarray*}
% at the end we have to erase these constants if they do not appear in the actual t theorems, then only needed in proofs
%Clarify that these bounds are driven by bounds in sup norm and variation norm on $Q,G$, but also by positivity often a function of $G$ bounded away from zero, so like $(C_Q,C_G,\delta)$.
{\bf Minimax rate bounds:}
We define
\begin{eqnarray*}
{\cal Q}_M&\equiv&{\cal Q}\cap {\cal F}_{v,M}^{k_1}\\
{\cal G}_M&\equiv&{\cal G}\cap {\cal F}_{v,M}^{k_2}
\end{eqnarray*}
the sub-parameter spaces of $Q_0,G_0$ obtained by restricting all its components to have variation norm bounded by $M<\infty$.
Note that $Q_0\in {\cal Q}_M$ for any $M>\pl Q_0\pl_v$, and similarly $G_0\in {\cal G}_M$ for any $M>\pl G_0\pl_v$.
Let
$\sup_{\Lambda}\log N(\epsilon M,{\cal Q}_M,L^2(\Lambda}))$ and $\sup_{\Lambda}\log N(\epsilon M,{\cal G}_M,L^2(\Lambda))$ be the $k_1$ and $k_2$-dimensional universal covering numbers for 
${\cal Q}_M$ and ${\cal G}_M$. Define the corresponding minimax rates
\begin{eqnarray*}
r_Q(n)&\equiv& \arg\min_{\epsilon}\epsilon^2+\frac{\sup_{\Lambda}\log N(\epsilon M,{\cal Q}_M,L^2(\Lambda}))}{n}\\
r_G(n)&\equiv&\arg\min_{\epsilon}\epsilon^2+\frac{\sup_{\Lambda}\log N(\epsilon M,{\cal G}_M,L^2(\Lambda}))}{n},
\end{eqnarray*}
where $r_Q(n)\in \openr^{k_1}$ and $r_G(n)\openr^{k_2}$ are vectors of minimax rates, one for each component of $Q$ and $G$.
Since the universal covering number of ${\cal F}_{v,M}$ is bounded as follows:
\[
\sup_{\Lambda}\log N(\epsilon M,{\cal F}_{v,M},L^2(\Lambda))\leq K \frac{1}{\epsilon^{2(1-\alpha(d))},\]
with $\alpha(d)=1/(d+1)$, it follows that the minimax rate for ${\cal F}_{v,M}$ is given by:
\[
r^*(n)=n^{-1/(4-2\alpha(d))}.\]
Therefore, the minimax rates $r_Q(n)$ and $r_G(n)$ are at least as good as this rate $r^*(n)$ which is faster than $n^{-1/4}$.
%this is great, we have vectors of minimax rates, all better than n^{-0.25}, and we can plug them in $f_{R_2}$ and $f_{D^*}$ to give nice sharp bounds utilizing that
%one might go faster than another an that may be these functions are cross-products so that one can compensate for another. 











C_1(M_{D^*,n},M_{D^*v,n})&=& \{M_{D^*,n}^{-1}M_{D^*v,n} \}^{\alpha}M_{D^*,n}\\
C_2(M_{D^*,n},M_{D^*v,n})&=&M_{D^*v,n} \{M_{D^*,n}M_{D^*v,n}^{-1}\}^{2-2\alpha}.
\begin{eqnarray*}
C(M_{L_1(Q)v,n},M_{2Q,n},M_{1Q,n},\alpha)&=&
M_{L_1(Q)v,n} \left\{M_{2Q,n}M_{L_1(Q)v,n}\}^{\alpha}\{ M_{1Q,n}/M_{L_1(Q)v,n}\right\}^{1-\alpha^2}\\
&&+
M_{L_1(Q)v,n}\left\{ M_{1Q,n}/M_{L_1(Q)v,n}\}^{2\alpha(1-\alpha)}\{M_{2Q,n}M_{L_1(Q)v,n}  \}^{-2(1-\alpha)}n^{-\alpha/2}\right\}\\
&& +O(n^{-\lambda}).
\end{eqnarray*}








We now define a number of universal bounds on the statistical model ${\cal M}$:
\begin{eqnarray*}
\tau&=&\tau({\cal M})=\sup_{P\in {\cal M}}\tau(P)\\
M_{1Q}&=&M_{1Q}({\cal M})=\sup_{Q,Q_0\in {\cal Q}}\pl L_1(Q)-L_1(Q_0)\pl_{\infty}\\
M_{2Q}&=&M_{2Q}({\cal M})=\sup_{P,P_0\in {\cal M}}\frac{ \pl L_1(Q)-L_1(Q_0)\pl_{P_0}^2}{d_{10}(Q,Q_0)}\\
M_{1G}&=&M_{1G}({\cal M})=\sup_{G,G_0\in {\cal G}}\pl L_2(G)-L_2(G_0)\pl_{\infty}\\
M_{2G}&=&M_{2G}({\cal M})=\sup_{P,P_0\in {\cal M}}\frac{ \pl L_2(G)-L_2(G_0)\pl_{P_0}^2}{d_{20}(G,G_0)}\\
M_{D^*}&=&M_{D^*}({\cal M})=\sup_{Q,G\in {\cal Q},{\cal G}} \pl D^*(Q,G)\pl_{\infty}\\
M_{R_2}&=&M_{R_2}({\cal M}=\sup_{P,P_0\in {\cal M}}\frac{\mid R_{2}(P,P_0)\mid}{ d_0((Q,G),(Q_0,G_0)) }.
\end{eqnarray*}
The bounds $M_{1Q},M_{2Q}$ excellent properties of the cross-validation selector based on the loss-function $L_1(Q)$, and  a bound on $M_{2Q}$ shows that the loss-based dissimilarity $d_{01}(Q,Q_0)$   behaves as a square of a norm. Similarly, the bounds $M_{1G},M_{2G}$ imply this for the loss function $L_2(G)$.
We also define the following universal variation norm bounds on the model ${\cal M}$:
\begin{eqnarray*}
M_{Q,v}&=&\sup_{P\in {\cal M}}\pl Q(P)\pl_v\\
M_{G,v}&=&\sup_{P\in {\cal M}}\pl G(P)\pl_v\\
M_{D^*,v}&=&\sup_{P\in {\cal M}}\pl D^*(P)\pl_v\\
M_{L_1(Q),v}&=&\sup_{P\in {cal M}}{\pl L_1(Q)\pl_v}
M_{L_2(G),v}&=&\sup_{P\in {cal M}}{\pl L_2(G)\pl_v}\\
\end{eqnarray*}



\section{Super-learner that achieves a rate faster than $n^{-1/4}$}
Our goal is to construct an estimator $\hat{Q}:{\cal M}_{np}\rightarrow{\cal Q}$ of $Q_0=Q(P_0)=\arg\min_{Q\in {\cal Q}}P_0L(Q)$ so that $d_0(Q_n,Q_0)=o_P(n^{-1/4})$.
In the previous section, we constructed an MLE $\hat{Q}^M:{\cal M}_{np}\rightarrow {\cal Q}_M={\cal Q}\cap {\cal F}_{v,M}$ for which $d_0(Q_n^M=\hat{Q}^M(P_n),Q_{0}^M)=o_P(n^{-1/4})$.
Let $\hat{Q}_{v,j}=\hat{Q}^{M_j}$, $j=1,\ldots,J_{v,n}$, be a collection of such MLEs corresponding with a sequence $M_1<\ldots<M_{J_{v,n}}$, where $\lim_{n\rightarrow\infty}M_{J_{v,n}}>\pl Q_0\pl_v$. Thus, for all $M_j>\pl Q_0\pl_v$, we have that $d_0(Q_{v,j,n},Q_0)=o_P(n^{-1/4})$.
In addition, let $\hat{Q}_j:{\cal M}_{np}\rightarrow {\cal Q}$, $j=1,\ldots,J_n$, be a collection of other estimators of $Q_0$, including a variety of parametric model as well as machine learning based estimators. 
This defines a collection of $K_n=J_{v,n}+J_n$ candidate estimators $\{\hat{Q}_{v,j}:j=1,\ldots,J_{v,n}\}\cup\{\hat{Q}_j: j=1,\ldots,J_n\}$ of $Q_0$.

Let $B_n\in \{0,1\}^n$ be a random vector with $V$ possible realizations which defines a split in a training sample $\{i:B_n(i)=0\}$ and validation sample
$\{i:B_n(i)=1\}$, where $B_n$ is independent of $(O_1,\ldots,O_n)$. 
Let $q$ be such that $P(\sum_i B_n(i)/n \geq q)=1$.
Let $P_{n,B_n}^1,P_{n,B_n}^0$ be the empirical probability distributions of the validation and trainmen sample, respectively.
Let ${\cal K}_n=\{1,\ldots,J_n\}\cup\{(v,1),\ldots,(v,J_{v,n})\}$ be the index set for the $K_n$ candidate estimators.
We define the cross-validation selector as the index
\[
k_n=\hat{K}(P_n)=\arg\min_{k\in {\cal K}_n} E_{B_n}P_n L(\hat{Q}_k(P_{n,B_n}^0))\]
that minimizes the cross-validated risk $E_{B_n}P_nL(\hat{Q}_k(P_{n,B_n}^0))$ over all choices $k$ of candidate estimators. 
We also define an oracle selector
\[
\tilde{k}_{0,n}=\tilde{K}_0(P_n)=\arg\min_{k\in {\cal K}_n} E_{B_n}P_0L(\hat{Q}_k(P_{n,B_n}^0))\]
as the index of the candidate estimator that minimizes the true conditional risk $E_{B_n}P_0L(\hat{Q}_k(P_{n,B_n}^0))$ over the index set for the candidate estimators. 
The cross-validated selected estimator is given by $\hat{Q}_{k_n}:{\cal M}_{np}\rightarrow{\cal Q}$, and the oracle selected estimator is
given by $\hat{Q}_{\tilde{k}_{0,n}}:{\cal M}_{np}\rightarrow{\cal Q}$. Note that
\[
E_{B_n}d_0(\hat{Q}_{\tilde{k}_{0,n}}(P_{n,B_n}^0),Q_0)=\min_{k\in {\cal K}_n} E_{B_n}P_0 L(\hat{Q}_k(P_{n,B_n}^0)).\]


\begin{theorem}\label{thslM1n}
Consider the definitions ${\cal M}_n$, ${\cal Q}_n$, $Q_{0n}$, $M_{1n},M_{2n}$. 
In addition, assume that $L(Q)$ be a convex loss function in the sense that $P_0L(\sum_{j=1}^m\alpha_jQ_j)\leq \sum_{j=1}^m\alpha_jP_0L(Q_j)$ when 
$\sum_j\alpha_j=1$ and $\min_j\alpha_j\geq 0$.

Consider a library of candidate estimators $\hat{Q}_k:{\cal M}_{np}\rightarrow {\cal Q}_n$, $k=1,\ldots,K_n$.
Let
\[
k_n=\hat{K}(P_n)=\arg\min_{k} E_{B_n}P_{n,B_n}^1L(\hat{Q}_k(P_{n,B_n}^0))\]
and let 
\[
Q_n=\hat{Q}(P_n)=E_{B_n}\hat{Q}_{k_n}(P_{n,B_n}^0).\]
Then, for any $\delta>0$, 
\[
d_0(Q_n,Q_{0n})\leq (1+2\delta) E_{B_n}\min_k d_0(\hat{Q}_k(P_{n,B_n}^0),Q_{0n})+O_P(C(M_{1n},M_{2n},\delta)\log K_n/(nq)).\]

If for each $\delta>0$, the fraction of $C(M_{1n},M_{2n},\delta)\log K_n/n$ over  $E_{B_n}\min_k d_0(\hat{Q}_{k}(P_{n,B_n}^0),Q_{0n})$ is $o_P(1)$, then 
\[
\frac{d_0(\hat{Q}(P_n),Q_0)}{E_{B_n}\min_kd_0(\hat{Q}_k(P_{n,B_n}^0),Q_0)}-1=o_P(1).\]
If  for each $\delta>0$, $E_{B_n}\min_k d_0(\hat{Q}_{k}(P_{n,B_n}^0),Q_0)=O_P(C(M_{1n},M_{2n},\delta)(\log K_n /n), then 
\[
d_0(\hat{Q}(P_n),Q_0)=O_P(C(M_{1n},M_{2n},\delta)\log K_n /n).\]

Let $\hat{Q}_1:{\cal M}_{np}\rightarrow {\cal Q}$ be an estimator so that $d_0(\hat{Q}_1(P_n),Q_0)=o_P(n^{-1/2})$.
Then, it follows that (worst case)
\begin{equation}\label{conservativebound}
d_0(\hat{Q}(P_n),Q_0)=o_P(n^{-1/2})+O_P(C(M_{1n},M_{2n},\delta)(\log K_n/n).\end{equation}

%In Lemma \ref{lemmamle1}  we define an estimator $\hat{Q}^{M}$ that minimizes the empirical risk over subset ${\cal Q}_{M}\subset {\cal Q}$ of functions with variation norm smaller than a known upper bound $M$. In Lemma \ref{lemmamlecv} we define an estimator $\hat{Q}_v$ which is defined in terms of  a library of  such candidate estimators $\hat{Q}^{M_j}$ indexed by various bounds $M_j$,  $j=1,\ldots,J_n$, and the cross-validation selector of $M_j$, where $M_{J_n}>\pl  Q_0\pl_v$ for $n$ large enough (allowing for an  unknown bound on the variation norm of $Q_0$, but still relying on $\pl Q_0\pl_v<\infty$). Consider this estimator $\hat{Q}_v$ but instead of enforcing a fixed bound $M_1,M_2$, now only enforce the candidate estimators to be in ${\cal Q}_n\uparrow {\cal Q}$ for a sequence $M_{1n},M_{2n}$ chosen so that $C(M_{1n},M_{2n},\delta)\log K_n/n =o(n^{-1/2})$. In addition to the above assumptions, assume that $\sup_{Q\in {\cal Q}_M}\frac{ \pl L(Q)\pl_v}{\pl Q\pl_v} <\infty$: i.e., the variation norm of $L(Q)$ can be universally bounded in terms of the variation norm of $Q$.
%: this one always holds given our M_2: that $d_0(Q_n,Q_0)\rightarrow 0$ implies $\pl L(Q_n)-L(Q_0)\pl_{P_0}\rightarrow 0$.Then, $d_0(\hat{Q}_v(P_n),Q_0)=o_P(n^{-1/2})$. Thus, by selecting $\hat{Q}_1=\hat{Q}_v$,   the  super-learner $\hat{Q}(P_n)$ above satisfies (\ref{conservative bound}).
\end{theorem}




We have
\begin{equation}\label{conservativebound}
d_{01}(\hat{Q}(P_n),Q_{0n})=O_P(n^{-\lambda})+O_P\left(C(M_{1Q,n},M_{2Q,n},\delta)\frac{\log K_n}{n}\right ).\end{equation}



$M_{1Q,n}M_{2Q,n}n^{-0.5}\rightarrow 0$;


Then, 
\[
d_{01}(Q_n^*,Q_{0n})=O_P(n^{-(0.5+\alpha/4)}M_{1Q,n})+O_P(n^{-\lambda}),
\]










\section{An MLE over model with universal bound on variation norm that converges at desired rate.}

\subsection{MLE minimizing over class of functions with universally bounded variation norm.}

\begin{lemma}
Let $(0,Q)\rightarrow L(Q)(o)$ be a loss function for a parameter $Q_0$ with $P_0L(Q_0)=\arg\min_{Q\in Q({\cal M})}P_0L(Q)$.

%Suppose that $M_{1Q,n}=\sup_{Q\in {\cal Q}_n} \mid L(Q)-L(Q_{0n})\mid (o)<\infty$.
%Let $M_{Q,v,n}=\sup_{P\in {\cal M}_n}\pl Q(P)\pl_v<\infty$.
%Let $M_{L(Q),v,n}<\infty$. 
%Let $M_{2Q,n}<\infty$.


Let ${\cal Q}_{n,M}\subset \{Q\in {\cal Q}_n:\pl Q\pl_v\leq M,\pl L(Q)\pl_V\leq M\}$  be all functions in the parameter space ${\cal Q}_n$ for $Q_{0n}$ 
for which the variation norm of its loss and itself is smaller than $M<\infty$.
Let  $Q_{0n}^M\in {\cal Q}_{n,M}$ be so that $P_0L(Q_{0n}^M)=\inf_{Q\in {\cal Q}_{n,M}} P_0L(Q)$.
%Consider the loss based dissimilarity $d_0(Q,Q_0)=P_0L(Q)-P_0L(Q_0)$, where $P_0L(Q_0)=\min_{Q\in {\cal Q}{(\cal M}}P_0L(Q)$.
%Assume that $\limsup_{n\rightarrow\infty} \sup_{Q\in {\cal Q}_{n,M}}\pl L(Q)\pl_v<\infty$: i.e., the variation norm of $L(Q)$ can be universally bounded in terms of the variation norm of $Q$.
%if we use loglikleihoodl loss then this requires keeping 
%Assume that $d_0(Q_n,Q_0)\rightarrow 0$ implies $\pl L(Q_n)-L(Q_0)\pl_{P_0}\rightarrow 0$.
%the universal bounding and equivalence of norms is only needed for iterative applying the proof and using bound on asymptotic equicontinuity
%Assume that there exists a $M_2<\infty$ so that\begin{equation}\label{MLEa1}\sup_{Q\in {\cal Q}({\cal M})}\frac{P_0\{L(Q)-L(Q_0)\}^2}{P_0 \{L(Q)-L(Q_0)\}}\leq M_2.\end{equation}


Consider an estimator $Q_n^M$ for which \[
P_n L(Q_n^M)=\inf_{Q\in {\cal Q}_{n,M}} P_nL(Q)+r_n,\]
where $r_n=o_P(1/\sqrt{n})$.
Then 
\begin{equation}\label{MLEa}
0\leq d_0(Q_n^M,Q_{0n}^M)\leq -(P_n-P_0)\{L(Q_n^M)-L(Q_{0n}^M)\}+r_n,\end{equation}
and
\[d_0(Q_n^M,Q_{0n}^M)=o_P(1/\sqrt{n}).\]
Let $M^u_0$ be a value so that for $M>M^u_0$ we have $Q_{0n}^M=Q_{0n}$. 
Then, for any $M>M^u_0$, the estimator $Q_n^{M}$ satisfies:
\[
d_0(Q_n^{M},Q_0)=o_P(1/\sqrt{n}).\]


Suppose that $\log (1+N(\epsilon,{\cal Q}_{n,M},d_0))=O(\epsilon^{\lambda-1})$ for a $0<\lambda<1$. 
%Suppose that $\pl G_n(f-g)\pl_{\psi_1}\leq C \pl f-g\pl_{P_0}$. 
Then, for any $M>M^u_0$, 
\begin{equation}\label{MLEclaim1}
d_0(Q_n^{M},Q_0)=O_P\left(n^{-\frac{1}{2-\lambda}\right)+r_n.
\end{equation}
%see lemma below actually proving that we have the bounding of G_n(f-g) in psi_1 norm for empirical process and thereby we can apply the vdc finite sample inequality with delta and eta etc. 
\end{lemma}




\section{The initial estimator using super-learning}

\section{Super-learner that achieves a rate faster than $n^{-1/4}$}

MAKE IT AN ESTIMATOR IN {\CAL Q}_N. of Q_{0n}

Our goal is to construct an estimator $\hat{Q}:{\cal M}_{np}\rightarrow{\cal Q}$ of $Q_0=Q(P_0)=\arg\min_{Q\in {\cal Q}}P_0L(Q)$ so that $d_0(Q_n,Q_0)=o_P(n^{-1/4})$.
In the previous section, we constructed an MLE $\hat{Q}^M:{\cal M}_{np}\rightarrow {\cal Q}_M={\cal Q}\cap {\cal F}_{v,M}$ for which $d_0(Q_n^M=\hat{Q}^M(P_n),Q_{0}^M)=o_P(n^{-1/4})$.
Let $\hat{Q}_{v,j}=\hat{Q}^{M_j}$, $j=1,\ldots,J_{v,n}$, be a collection of such MLEs corresponding with a sequence $M_1<\ldots<M_{J_{v,n}}$, where $\lim_{n\rightarrow\infty}M_{J_{v,n}}>\pl Q_0\pl_v$. Thus, for all $M_j>\pl Q_0\pl_v$, we have that $d_0(Q_{v,j,n},Q_0)=o_P(n^{-1/4})$.
In addition, let $\hat{Q}_j:{\cal M}_{np}\rightarrow {\cal Q}$, $j=1,\ldots,J_n$, be a collection of other estimators of $Q_0$, including a variety of parametric model as well as machine learning based estimators. 
This defines a collection of $K_n=J_{v,n}+J_n$ candidate estimators $\{\hat{Q}_{v,j}:j=1,\ldots,J_{v,n}\}\cup\{\hat{Q}_j: j=1,\ldots,J_n\}$ of $Q_0$.

Let $B_n\in \{0,1\}^n$ be a random vector with $V$ possible realizations which defines a split in a training sample $\{i:B_n(i)=0\}$ and validation sample
$\{i:B_n(i)=1\}$, where $B_n$ is independent of $(O_1,\ldots,O_n)$. 
Let $q$ be such that $P(\sum_i B_n(i)/n \geq q)=1$.
Let $P_{n,B_n}^1,P_{n,B_n}^0$ be the empirical probability distributions of the validation and trainmen sample, respectively.
Let ${\cal K}_n=\{1,\ldots,J_n\}\cup\{(v,1),\ldots,(v,J_{v,n})\}$ be the index set for the $K_n$ candidate estimators.
We define the cross-validation selector as the index
\[
k_n=\hat{K}(P_n)=\arg\min_{k\in {\cal K}_n} E_{B_n}P_n L(\hat{Q}_k(P_{n,B_n}^0))\]
that minimizes the cross-validated risk $E_{B_n}P_nL(\hat{Q}_k(P_{n,B_n}^0))$ over all choices $k$ of candidate estimators. 
We also define an oracle selector
\[
\tilde{k}_{0,n}=\tilde{K}_0(P_n)=\arg\min_{k\in {\cal K}_n} E_{B_n}P_0L(\hat{Q}_k(P_{n,B_n}^0))\]
as the index of the candidate estimator that minimizes the true conditional risk $E_{B_n}P_0L(\hat{Q}_k(P_{n,B_n}^0))$ over the index set for the candidate estimators. 
The cross-validated selected estimator is given by $\hat{Q}_{k_n}:{\cal M}_{np}\rightarrow{\cal Q}$, and the oracle selected estimator is
given by $\hat{Q}_{\tilde{k}_{0,n}}:{\cal M}_{np}\rightarrow{\cal Q}$. Note that
\[
E_{B_n}d_0(\hat{Q}_{\tilde{k}_{0,n}}(P_{n,B_n}^0),Q_0)=\min_{k\in {\cal K}_n} E_{B_n}P_0 L(\hat{Q}_k(P_{n,B_n}^0)).\]


increasing library and at some n>N_0^* it starts containing a hat{Q}^{M_j}$ wit $M_j>M_0$. Take smallest larger than M_0, say M_{j_0}.
Then  min_k d_0(\hatQ_k,Q_{0n})< d-0(hat{Q}^{M_{j_0}},Q_{0n})=o_P(n^{-1/2}).
%we can get rid of $\hat{Q}_1$ below, just for $n>N_0^*$ one of estimators is $\hat{Q}^{M_j}$ for an $M_j>M_0$ for which $d_0=n^{-1/2}$.

\begin{theorem}\label{thslM1n}
Consider the definitions ${\cal M}_n$, ${\cal Q}_n$, $Q_{0n}$, $M_{1n},M_{2n}$. 
In addition, assume that $L(Q)$ be a convex loss function in the sense that $P_0L(\sum_{j=1}^m\alpha_jQ_j)\leq \sum_{j=1}^m\alpha_jP_0L(Q_j)$ when 
$\sum_j\alpha_j=1$ and $\min_j\alpha_j\geq 0$.

Consider a library of candidate estimators $\hat{Q}_k:{\cal M}_{np}\rightarrow {\cal Q}_n$, $k=1,\ldots,K_n$.
Let
\[
k_n=\hat{K}(P_n)=\arg\min_{k} E_{B_n}P_{n,B_n}^1L(\hat{Q}_k(P_{n,B_n}^0))\]
and let 
\[
Q_n=\hat{Q}(P_n)=E_{B_n}\hat{Q}_{k_n}(P_{n,B_n}^0).\]
Then, for any $\delta>0$, 
\[
d_0(Q_n,Q_{0n})\leq (1+2\delta) E_{B_n}\min_k d_0(\hat{Q}_k(P_{n,B_n}^0),Q_{0n})+O_P(C(M_{1n},M_{2n},\delta)\log K_n/(nq)).\]

If for each $\delta>0$, the fraction of $C(M_{1n},M_{2n},\delta)\log K_n/n$ over  $E_{B_n}\min_k d_0(\hat{Q}_{k}(P_{n,B_n}^0),Q_{0n})$ is $o_P(1)$, then 
\[
\frac{d_0(\hat{Q}(P_n),Q_0)}{E_{B_n}\min_kd_0(\hat{Q}_k(P_{n,B_n}^0),Q_0)}-1=o_P(1).\]
If  for each $\delta>0$, $E_{B_n}\min_k d_0(\hat{Q}_{k}(P_{n,B_n}^0),Q_0)=O_P(C(M_{1n},M_{2n},\delta)(\log K_n /n), then 
\[
d_0(\hat{Q}(P_n),Q_0)=O_P(C(M_{1n},M_{2n},\delta)\log K_n /n).\]

Let $\hat{Q}_1:{\cal M}_{np}\rightarrow {\cal Q}$ be an estimator so that $d_0(\hat{Q}_1(P_n),Q_0)=o_P(n^{-1/2})$.
Then, it follows that (worst case)
\begin{equation}\label{conservativebound}
d_0(\hat{Q}(P_n),Q_0)=o_P(n^{-1/2})+O_P(C(M_{1n},M_{2n},\delta)(\log K_n/n).\end{equation}

%In Lemma \ref{lemmamle1}  we define an estimator $\hat{Q}^{M}$ that minimizes the empirical risk over subset ${\cal Q}_{M}\subset {\cal Q}$ of functions with variation norm smaller than a known upper bound $M$. In Lemma \ref{lemmamlecv} we define an estimator $\hat{Q}_v$ which is defined in terms of  a library of  such candidate estimators $\hat{Q}^{M_j}$ indexed by various bounds $M_j$,  $j=1,\ldots,J_n$, and the cross-validation selector of $M_j$, where $M_{J_n}>\pl  Q_0\pl_v$ for $n$ large enough (allowing for an  unknown bound on the variation norm of $Q_0$, but still relying on $\pl Q_0\pl_v<\infty$). Consider this estimator $\hat{Q}_v$ but instead of enforcing a fixed bound $M_1,M_2$, now only enforce the candidate estimators to be in ${\cal Q}_n\uparrow {\cal Q}$ for a sequence $M_{1n},M_{2n}$ chosen so that $C(M_{1n},M_{2n},\delta)\log K_n/n =o(n^{-1/2})$. In addition to the above assumptions, assume that $\sup_{Q\in {\cal Q}_M}\frac{ \pl L(Q)\pl_v}{\pl Q\pl_v} <\infty$: i.e., the variation norm of $L(Q)$ can be universally bounded in terms of the variation norm of $Q$.
%: this one always holds given our M_2: that $d_0(Q_n,Q_0)\rightarrow 0$ implies $\pl L(Q_n)-L(Q_0)\pl_{P_0}\rightarrow 0$.Then, $d_0(\hat{Q}_v(P_n),Q_0)=o_P(n^{-1/2})$. Thus, by selecting $\hat{Q}_1=\hat{Q}_v$,   the  super-learner $\hat{Q}(P_n)$ above satisfies (\ref{conservative bound}).
\end{theorem}



Pay a little attention that Q in in D^k[0,tau], but basically all fine given our general notation bu may be for approximation by linear regression clarify have to do for each component
Now, we have initial estimators.
Now theorems for TMLE and CV TMLE.

given conditions for initial estimator to have the right rate, we can start doing proof for TMLE for bounded model,  and CV-TMLE for unbounded model, and then fill in actual theorem. give conditions on M_2n that are stating slowly enough but also assume a rate for initial faster than root-n and give rate on M_2n in terms of this rate.







\section{Minimum loss-based estimator (MLE) that converges at rate faster than $n^{-1/4}$.}

\subsection{MLE that minimizes over a  Donsker class}

\begin{lemma}
Consider a loss based dissimilarity $d_0(Q,Q_0)=P_0L(Q)-P_0L(Q_0)$, where $P_0L(Q_0)=\min_{Q\in {\cal Q}{(\cal M}}P_0L(Q)$.
Consider an estimator $Q_n$ for which \[
P_n L(Q_n)=\inf_{Q\in Q({\cal M}) } P_nL(Q)+r_n,\]
where $r_n=o_P(1/\sqrt{n})$.
Then 
\begin{equation}\label{MLEa}
0\leq d_0(Q_n,Q_0)\leq -(P_n-P_0)\{L(Q_n)-L(Q_0)\}+r_n.\end{equation}

Assume that there exists a $C<\infty$ so that
\begin{equation}\label{MLEa1}
\sup_{Q\in {\cal Q}({\cal M})}\frac{P_0\{L(Q)-L(Q_0)\}^2}{P_0 \{L(Q)-L(Q_0)\}}\leq C.\end{equation}
In addition, assume  ${\cal F}\equiv \{L(Q)-L(Q_0):Q\in {\cal Q}({\cal M})\}$  is a $P_0$-Donsker class, and assume that $L(Q_n)-L(Q_0)\in {\cal F}$ with probability tending to 1.
Then, $d_0(Q_n,Q_0)=o_P(1/\sqrt{n})$.

Suppose that $\log (1+N(\epsilon,{\cal F},d_0))=O(\epsilon^{\lambda-1})$ for a $0<\lambda<1$. Suppose that $\pl G_n(f-g)\pl_{\psi_1}\leq C \pl f-g\pl_{P_0}$. Then,
\begin{equation}\label{MLEclaim1}
d_0(Q_n,Q_0)=O_P\left(n^{-\frac{1}{2-\lambda}\right)+r_n.
\end{equation}
Similarly, suppose that $\sqrt{\log (1+N(\epsilon,{\cal F},d_0))}=O(\epsilon^{\lambda-1})$ for a $0<\lambda<1$. Suppose that $\pl G_n(f-g)\pl_{\psi_2}\leq C\pl f-g\pl_{P_0}$. Then,
\begin{equation}\label{MLEclaim2}
d_0(Q_n,Q_0)=O_P\left(n^{-\frac{1}{2-\lambda}\right) +r_n.
\end{equation}
\end{lemma}
{\bf Proof:}
We have 
\begin{eqnarray*}
0&\leq & d_0(Q_n,Q_0)=P_0\{L(Q_n)-L(Q_0)\}\\
&=&-(P_n-P_0)\{L(Q_n)-L(Q_0)\}+P_n \{L(Q_n)-L(Q_0)\}\\
&\leq &-(P_n-P_0)\{L(Q_n)-L(Q_0)\}+r_n,
\end{eqnarray*}
which proves (\ref{MLEa}).
Since $L(Q_n)-L(Q_0)$ falls in a $P_0$-Donsker class, it follows that the right-hand side is $O_P(1/\sqrt{n})$. By assumption (\ref{MLEa1}), this also implies  that $\pl L(Q)-L(Q_0)\pl_{P_0}^2=O_P(1/\sqrt{n})$. By empirical process theory we have that $\sqrt{n}(P_n-P_0)f_n\rightarrow_p 0$ if $f_n$ is in a $P_0$-Donsker class and $P_0f_n^2\rightarrow_p 0$ as $n\rightarrow\infty$. Applying this to $f_n=L(Q_n)-L(Q_0)$ shows that $(P_n-P_0)(L(Q_n)-L(Q_0))=o_P(1/\sqrt{n}$, which proves 
$d_0(Q_n,Q_0)=o_P(1/\sqrt{n})$.

By assumption (\ref{MLEa} it follows that $\pl L(Q_n)-L(Q_0)\pl_{P_0}^2=o_P(n^{-1/2})$. Then, with probability tending to 1, $\pl L(Q_n)-L(Q_0)\pl_{P_0}\leq n^{-1/4}$. Let $\delta_n=n^{-1/4}$.
Lemma \ref{lemmahelpa} shows  that if $\log (1+N(\epsilon,{\cal F},d_0)=O(\epsilon^{\lambda -1})$, then  $\sup_{\pl f\pl_{P_0}\leq \delta_n)\mid G_n(f)\mid =O(\delta_n^{\lambda})=O(n^{-1/4 \lambda})$, where $G_n(f)=\sqrt{n}(P_n-P_0)f$. 
Applying this to $-(P_n-P_0)\{L(Q_n)-L(Q_0)\}$ shows that $d_0(Q_n,Q_0)=O_P(n^{-1/2}n^{-1/4 \lambda})+r_n$, which thus also implies 
$\pl L(Q_n)-L(Q_0)\pl_{P_0}^2=O_P(n^{-1/2}n^{-1/4 \lambda})+r_n$.
We can now reapply Lemma \ref{lemmahelpa} but now  with 
$\delta_n^2=\max(r_n,n^{-1/2}n^{-1/4 \lambda})$. The next rate we obtain for $-(P_n-P_0)\{L(Q_n)-L(Q_0)\}$ (and thus $d_0(Q_n,Q_0)$ and $\pl L(Q_n)-L(Q_0)\pl_{P_0}^2$) is given by $\max(r_n,n^{-(1/2+1/4 \lambda +1/8 \lambda^2)})$.
Iteration of this process iteratively applying Lemma \ref{lemmahelpa} each time with the current rate $\delta_n$ for $\pl L(Q_n)-L(Q_0)\pl_{P_0}$ results in a rate $\max(r_n,n^{-a})$, where  $a=\sum_{k=0}^{\infty} 0.5 (0.5\lambda)^k=(2-\lambda)^{-1}$, which proves (\ref{MLEclaim1}). The proof of (\ref{MLEclaim2}) is a similar.
This completes the proof of the lemma. $\Box$

\paragraph{Remark}
Instead of an MLE $Q_n$ satisfying $P_nL(Q_n)\leq \inf_{Q}P_n L(Q)+r_n$, we could have computed a cross-validated $\epsilon$-net estimator of $Q_0$ using that $\log (1+N(\epsilon,{\cal F},L^2(P_0) ) )=O(\epsilon^{\lambda-1})$ for $0<\lambda<1$ of the parameter space of $Q_0$. If the  number of points in the chosen $\epsilon$-nets are of the order as this bound on the covering number $N(\epsilon,{\cal F},L^2(P_0))$, then the cross-validated $\epsilon$-net estimator achieves the rate $\min_{\epsilon}\epsilon^2 +\frac{1}{\epsilon^{\lambda -1} n}$ w.r.t. loss-based dissimilarity $d_0(\cdot,Q_0)$. This rate is thus given by$n^{-\frac{2}{3-\lambda}}$,
which is a better rate than $n^{- This rate is better than the rate $ n^{-1/(2-\lambda)}$. For example, if $\lambda =0.5$ these rates are given by 
$n^{-4/5}$ versus $n^{-2/3}$.

\paragraph{Argument showing that for a $P_0$-Donsker class we have $\int_0^1\sqrt{\log N(\epsilon,{\cal F},L^2(P_0))} d\epsilon<\infty$.}
Consider an empirical process $G_n$ indexed by a class of functions ${\cal F}$ for which $\int_0^1 \sup_{Q}\sqrt{\log N(\epsilon,{\cal F},L^2(Q))} d\epsilon <\infty$.
This entropy integral condition is typically used to conclude that ${\cal F}$ is a uniform Donsker class, but as noted in van der Vaart, Wellner (1996) it is not a necessary condition.
We are not aware of a bound on the covering number $\sup_QN(\epsilon,{\cal F}_{v,M},L^2(Q))$ for the class ${\cal F}_{v,M}$ with variation norm bounded by a universal constant $M<\infty$, even though it is known that it is a universal Donsker class. Here we first make an argument that indicates that $\int_0^1 \sqrt{\log N(\epsilon,{\cal F},L^2(P_0)) d\epsilon <\infty$ is essentially necessary for  ${\cal F}$ being  a $P_0$-Donsker class, providing a strong indication that the covering number of 
${\cal F}_{v,M}$ satisfies the uniform entropy integral condition. 

The argument is as follows. Above we showed  that a minimum empirical risk estimator $Q_n$ of $Q_0$, minimizing $Q\rightarrow P_n L(Q)$ over all functions in ${\cal F}_{v,M}$, satisfies
$d_0(Q_n,Q_0)=P_0L(Q_n)-P_0L(Q_0)=o_P(1/\sqrt{n})$, where we only utilized that $L(Q_n)-L(Q_0)$ falls in a $P_0$-Donsker class and that 
$P_0(L(Q_n)-L(Q_0))^2\leq C P_0(L(Q_n)-L(Q_0))$ for some universal $C$ (which holds for the squared error loss and log-likelihood loss when the loss function is universally bounded). Suppose that the entropy integral $\int_0^1 \sqrt{\log N(\epsilon,{\cal F}_{v,M},L^2(P_0))} d\epsilon $ is not bounded. Then one would have that $\sqrt{\log N(\epsilon,{\cal F},L^2(Q))}\geq $1/\epsilon$.
The cross-validated $\epsilon$-net estimator in van der Laan, Dudoit, van der Vaart (2006), using the smallest possible $\epsilon$-net w.r.t. dissimilarity $d_0$, achieves the rate $\min_{\epsilon}\epsilon^2+\frac{1}{\epsilon^2 n}$ w.r.t. 
$d_0$, which equals $1/\sqrt{n}$. That is, even this perfect $\epsilon$-net estimator converges at a rate {\em not} faster than $1/\sqrt{n}$, while we believe this cross-validated $\epsilon$-net estimator to achieve an optimal possible rate w.r.t. $d_0(\cdot,Q_0)$ since 1) it uses an oracle $\epsilon$-net, 2) it selects $\epsilon$ with an cross-validated selector that is asymptotically equivalent with the oracle selector of $\epsilon$, converges at a rate not faster than $1/\sqrt{n}$. But this then shows that the minimum empirical risk estimator $Q_n$ converges at a faster rate than the cross-validated $\epsilon$-net estimator.  Therefore we conclude that 
$\sqrt{\log N(\epsilon,{\cal F},L^2(P_0)}<< 1/\epsilon$, and thus that the entropy integral $\int_0^1\sqrt{\log N(\epsilon,{\cal F}_{v,M},L^2(P_0))} d\epsilon <\infty$.

%check, this might be a known result in book


\begin{lemma}\label{lemmahelpa}
%Let $p\in \{1,2\}$ and $\psi_p(x)=\exp(x^p)-1$.
Let $\psi_1(x)=\exp(x)-1$. 
For all $f-g$ with $f,g\in {\cal F}$, we have $\pl G_n(f-g)\pl_{\psi_p}\leq C \sigma_0(f-g)$ for some universal $C<\infty$.
In addition, assume that $\log (1+N(\epsilon,{\cal F},\sigma))=O(\epsilon^{\lambda-1})$. 
Then,
\[
\sup_{f,g\in {\cal F},\sigma(f-g)\leq \delta}\pl G_n(f-g)\pl_{\psi_1}=O(\delta^{\lambda}).\]

%Similarly, suppose that for all $f-g$ with $f,g\in {\cal F}$, we have $\pl G_n(f-g)\pl_{\psi_2}\leq C \sigma_0(f-g)$ for some universal $C<\infty$.
%In addition, assume that $\sqrt{\log (1+N(\epsilon,{\cal F},\sigma))}=O(\epsilon^{\lambda-1}$. 
%Then,
%\[\sup_{f,g\in {\cal F},\sigma(f-g)\leq \delta}\pl G_n(f-g)\pl_{\psi_2}=O(\delta^{\lambda}).\]
\end{lemma}
{\bf Proof: }
By Bernstein's inequality we have that
\[
P(\mid G_n(f)/\sigma(f)\mid>x)\leq 2\exp\left(-0.5 \frac{x^2}{1+ Mx/3\sqrt{n}}\right).\]
If $\mid x\mid >1$, then this tail can be bounded by $K\exp( -Cx)$ for some $C,K$. Consider the orlics norm $\pl G_n(f)/\sigma(f)\pl_{\psi_1}$, where $\psi_1(x)=\exp(x)-1$, which is defined by 
\[
\pl X\pl_{\psi_1}=\inf\{c: E \exp(\mid X\mid /c)-1\leq 1\}.\]
By writing $X=XI(\mid X\mid >1)+XI(\mid X\mid <1)$, it follows that 
\begin{eqnarray*}
 \pl X\pl_{\psi_1}&\leq &\leq \inf\left\{c: \exp(1/c)+\sum_{p=1}^{\infty} E\left( \frac{\mid X\mid I(\mid X\mid >1)}{c}\right)^p\frac{1}{p!}\leq 2\\right\}.
 \end{eqnarray*}
 By choosing $c$ larger than some integer such as $10$, i follows that we obtain a bound
 \begin{eqnarray*}
  \pl X\pl_{\psi_1}&\leq&\max\left(10, \inf\left\{c: \sum_{p=1}^{\infty} E\left( \frac{\mid X\mid I(\mid X\mid >1)}{c}\right)^p\frac{1}{p!}\leq 2-\exp(1/10)\\right\}\right)\\
  &=& \max\left( 10,\inf\left\{c: E\exp(\mid XI(\mid X\mid >1)\mid /c)\leq  2-\exp(1/10)\\right\}\right)\\
  &\equiv &\max\left( 10,\pl XI(\mid X\mid >1)\pl_{\psi_1,\exp(0.1)}.
  \end{eqnarray*}
  Theorem 2.2.4 in van der Vaart, Wellner (1996) shows that if $P(\mid X\mid >x)\leq K\exp(-Cx)$, then $\pl X\pl_{\psi_1}\leq (1+K/C)$.
  Thus, in particular, $\pl G_n(f)/\sigma(f) I(\mid G_n(f)/\sigma(f)\mid >1)\pl_{\psi_1}\leq (1+K/C)$.
  We now need a result that says that if $P(\mid X\mid >x)\leq K\exp(-Cx)$, then $\pl X\pl_{\psi_1,\exp(0.1)}\leq M(K,C)$ for some $M(K,C)<\infty$.
  This can be proven explicitly by using the exponential bounds $K\exp(-Cx)$ in the expectation, just like this original result has been proven. 
  %To do
  Therefore, we can conclude that $\pl G_n(f)/\sigma(f)\pl_{\psi_1}<C$ for some $C<\infty$ not depending on $f\in {\cal F}$.

We now apply Theorem 2.2.4 in van der Vaart, Wellner (1996): If $\pl G_n(f-g)\pl_{\psi_1}\leq C \sigma(f-g)$, then for any $\delta,\eta$, we have
\[
\pl \sup_{\sigma(f,g)\leq \delta} \mid G_n(f)-G_n(g)\mid \pl_{\psi_1} \leq K\left\{
\int_0^{\eta} \psi_1^{-1}(N(\epsilon,d)) d\epsilon +\delta \psi_1^{-1} (N^2(\eta,d))\right\}.\]
Then, we have
\[
\pl \sup_{\sigma(f,g)\leq \delta} \mid G_n(f)-G_n(g)\mid \pl_{\psi_1} \leq K\left\{
\int_0^{\eta} \psi_1^{-1}(N(\epsilon,d)) d\epsilon +\delta \psi_1^{-1} (N^2(\eta,d))\right\}\]
By assumption,   $\log (1+N(\epsilon))=\epsilon^{\lambda -1}$ for a $0<\lambda<1$.
Then we can minimize the right-hand side over $\eta$ for a given $\delta$. This yields the choice $\eta(\delta)=\delta$, and plugging this choice in the expression yields the  result:
\[
\pl \sup_{\sigma(f,g)\leq \delta} \mid G_n(f)-G_n(g)\mid \pl_{\psi_1}=O(\frac{1}{\lambda}\delta^{\lambda}=O(\delta^{\lambda})\]
for a fixed $\lambda$. $\Box$








\section{MLE minimizing over functions with bounded variation norm}

\subsection{MLE minimizing over functions with bounded variation norm.}

\begin{lemma}
Let $(0,Q)\rightarrow L(Q)(o)$ be a loss function for a parameter $Q_0$ with $P_0L(Q_0)=\arg\min_{Q\in Q({\cal M})}P_0L(Q)$.
Suppose that $M_1=\sup_{Q\in {\cal Q}} \mid L(Q)-L(Q_0)\mid (o)<\infty$.

Let ${\cal Q}_M={\cal Q}\cap {\cal F}_{v,M}=\{Q(P):P\in {\cal M},Q(P)\in {\cal F}_{v,M}\}$ be all functions in the parameter space for $Q_0$ that have a variation norm smaller than $M<\infty$.
Let  $Q_{0}^M\in {\cal Q}_M$ be so that $P_0L(Q_{0}^M)=\min_{Q\in {\cal Q}_M} P_0L(Q)$.
Consider the loss based dissimilarity $d_0(Q,Q_0)=P_0L(Q)-P_0L(Q_0)$, where $P_0L(Q_0)=\min_{Q\in {\cal Q}{(\cal M}}P_0L(Q)$.
Assume that $\sup_{Q\in {\cal Q}_M}\frac{ \pl L(Q)\pl_v}{\pl Q\pl_v} <\infty$: i.e., the variation norm of $L(Q)$ can be universally bounded in terms of the variation norm of 
$Q$.
Assume that $d_0(Q_n,Q_0)\rightarrow 0$ implies $\pl L(Q_n)-L(Q_0)\pl_{P_0}\rightarrow 0$.
%the universal bounding and equivalence of norms is only needed for iterative applying the proof and using bound on asymptotic equicontinuity
%Assume that there exists a $M_2<\infty$ so that\begin{equation}\label{MLEa1}\sup_{Q\in {\cal Q}({\cal M})}\frac{P_0\{L(Q)-L(Q_0)\}^2}{P_0 \{L(Q)-L(Q_0)\}}\leq M_2.\end{equation}


Consider an estimator $Q_n^M$ for which \[
P_n L(Q_n^M)=\inf_{Q\in {\cal Q}_M} P_nL(Q)+r_n,\]
where $r_n=o_P(1/\sqrt{n})$.
Then 
\begin{equation}\label{MLEa}
0\leq d_0(Q_n^M,Q_0^M)\leq -(P_n-P_0)\{L(Q_n^M)-L(Q_0^M)\}+r_n,\end{equation}
and
\[d_0(Q_n^M,Q_0^M)=o_P(1/\sqrt{n}).\]
If $M^u=\sup_{Q\in {\cal Q}}\pl Q\pl_v<\infty$, then the estimator $Q_n^{M^u}$ satisfies:
\[
d_0(Q_n^{M^u},Q_0)=o_P(1/\sqrt{n}).\]
\end{lemma}

\begin{lemma}
{\bf Upper bound on variation norm is unknown:}

Let $(0,Q)\rightarrow L(Q)(o)$ be a loss function for a parameter $Q_0$ with $P_0L(Q_0)=\arg\min_{Q\in Q({\cal M})}P_0L(Q)$.
Suppose that $M_1=\sup_{Q\in {\cal Q}} \mid L(Q)-L(Q_0)\mid (o)<\infty$.
Let ${\cal Q}_M={\cal Q}\cap {\cal F}_{v,M}=\{Q(P):P\in {\cal M},Q(P)\in {\cal F}_{v,M}\}$ be all functions in the parameter space for $Q_0$ that have a variation norm smaller than $M<\infty$.
Let  $Q_{0}^M\in {\cal Q}_M$ be so that $P_0L(Q_{0}^M)=\min_{Q\in {\cal Q}_M} P_0L(Q)$.
Consider the loss based dissimilarity $d_0(Q,Q_0)=P_0L(Q)-P_0L(Q_0)$, where $P_0L(Q_0)=\min_{Q\in {\cal Q}{(\cal M}}P_0L(Q)$.
Assume that $\sup_{Q\in {\cal Q}_M}\frac{ \pl L(Q)\pl_v}{\pl Q\pl_v} <\infty$: i.e., the variation norm of $L(Q)$ can be universally bounded in terms of the variation norm of 
$Q$.
Assume that $d_0(Q_n,Q_0)\rightarrow 0$ implies $\pl L(Q_n)-L(Q_0)\pl_{P_0}\rightarrow 0$.

Consider now the case that $\sup_{Q\in {\cal Q}}\pl Q\pl_v=\infty$ but $\pl Q_0\pl_v<\infty$ (upper bound is unknown).
Consider a library of estimators $\hat{Q}^{M_j}:{\cal M}_{np}\rightarrow{\cal Q}$, $j=1,\ldots,J_n$, where $M_{J_n}\rightarrow\infty$ as $n\rightarrow\infty$.
Let $\tilde{M}_0=\min\{M_j: M_j\geq \pl Q_0\pl_v\}$, which is only defined when $M_{J_n}>\pl Q_0\pl_v$ (so certainly for $n$ large enough).
Assume that there exists an $M_2<\infty$ so that\begin{equation}\label{MLEa1}\sup_{Q\in {\cal Q}({\cal M})}\frac{P_0\{L(Q)-L(Q_0)\}^2}{P_0 \{L(Q)-L(Q_0)\}}\leq M_2.\end{equation}
Assume that $L(Q)$ is convex in the sense that $P_0L(\sum_j\alpha_jQ_j)\leq \sum_j \alpha_jP_0L(Q_j)$ for vectors $\alpha$ with $\min_j\alpha_j\geq 0$ and
$\sum_j \alpha_j=1$.
Let 
\[
M_n=\arg\min_{M_j} E_{B_n}P_{n,B_n}^1L(\hat{Q}^{M_j}(P_{n,B_n}^0)).\]
Define $Q_n^v=\hat{Q}^v(P_n)=E_{B_n}\hat{Q}^{M_n}(P_{n,B_n}^0)$.
Then, for any $\delta>0$, 
\begin{eqnarray*}
d_0(Q_n^v,Q_0)&\leq& (1+2\delta) E_{B_n}\min_j d_0(\hat{Q}^{M_j}(P_{n,B_n}^0),Q_0)+O_P(C(M_1,M_2,\delta)\log K_n/(nq)).
\end{eqnarray*}
If $n$ is large enough so that $M_{J_n}>\pl Q_0\pl_v$, then 
\begin{eqnarray*}
d_0(Q_n^v,Q_0)&\leq &(1+2\delta) E_{B_n}d_0(\hat{Q}^{\tilde{M}_0}}(P_{n,B_n}^0),Q_0)+O_P(C(M_1,M_2,\delta)\log K_n/(nq))\\
&=&o_P(n^{-1/4})+ O_P(C(M_1,M_2,\delta)\log K_n/(nq)).
\end{eqnarray*}
Thus, $d_0(Q_n^v,Q_0)=o_P(n^{-1/4})$.



\end{lemma}











\subsection{Approximating the functions with finite variation norm by linear combinations of indicator basis functions with bounded $L_1$-norm for coefficient vector}
Recall the representation $f(x)=f(0)+\sum_{s\subset\{1,\ldots,p\}} \int_{0_s}^{\tau_s} f(dx_s,0_{-s})$.
We will now approximate this representation with a finite dimensional linear regression, where the sum of the absolute values of the coefficients in the linear regression will be the actual variation norm. This will allow us to utilize available algorithms such as Lasso to compute an MLE that approximate the desired MLE with arbitrary approximation error.

For a given width $h_m$, let \[
[0,\tau]=\{0,0\}+\cup_{k=0}^{K_m} (kh_m,(k+1)h_m]\times \{0\}+\0\}\times \cup_{l=0}^{L_m} (lh_m,(l+1)h_m]+\cup_{k,l}(kh_m,(k+1)h_m]\times (lh_m,(l+1)h_m] \]
be a partitioning of $[0,\tau]=\{0\}\cup (0,\tau_1]\times \{0\}\cup \{0\}\times (0,\tau_2]\cup (0,\tau]$, where $(0,\tau ]$ is partitioned  in terms of small squares $R_{m}(k,l,(1,2))=(kh_m,(k+1)h_m]\times (lh_m,(l+1)h_m] $ of width $h_m$, 
and the half-lines 
$(0,\tau_1]\times \{0\}$ and $\{0\}\times (0,\tau_2]$ are partitioned in one dimensional intervals $R_{m}(k,1)=(kh_m,(k+1)h_m]\times \{0\}$ and 
$R_{m}(l,2)=\{0\}\times (lh_m,(l+1)h_m]$ of width $h_m$.
Let $df_m(k,l)=f(R_{m}(k,l,(1,2) ) ),df_m(k,0)=f(R_{m}(k,1)),df_m(0,l)=f_m(R_{m}(l,2))$ be the measures that $f$ assigns to the corresponding partition elements. 
Let $df_m$ be the corresponding discrete measure that puts mass $df_m(k,l)$ on the midpoints of the square $R_{m}(k,l,(1,2))$ and $df_m(k,0),df_m(0,l)$ on the midpoints of the intervals $R_{m}(k,1),R_{m}(l,2)$. 
Then,
\begin{eqnarray*}
f(x)&=&f(0,0)+\lim_{h_m\rightarrow 0}\left(  \int_{(0,\tau_1]} I_{(0,x_1]}(u_1)f_m(du_1,0)+\int_{(0,\tau_2]}I_{(0,x_2]}(u_2)f_m(0,du_2)+\int_{(0,\tau]}I_{(0,x]}(u_1,u_2)f_m(du_1,du_2)\right) \\
&=&f(0,0)+\lim_{h_m\rightarrow 0}\left(  \sum_{k}I_{(0,x_1]}(kh_m)df_m(k,0)+\sum_l I_{(0,x_2]}(lh_m)df_m(0,l)+\sum_{k,l}I_{(0,x]}(kh_m,lh_m) df_m(k,l)\right) .
\end{eqnarray*}
In particular, 
\begin{eqnarray*}
\pl f\pl_{v,0}&=&\mid  f(0,0)\mid +\lim_{h_m\rightarrow 0}\left ( 
\sum_k \mid df_m(k,0)\mid+\sum_l \mid df_m(0,l)\mid+\sum_{k,l}\mid df_m(k,l)\mid \right ).
\end{eqnarray*}
Thus, this representation of an $f\in D[0,\tau ]$ with $\pl f\pl_{v,0}=M$ is approximated by a finite linear combination of 
''covariates/basis functions''  $x\rightarrow \phi^m_0(x)=1$ (intercept), $(x_1,x_2)\rightarrow \phi_{k,1}^m(x)=I_{(0,x_1]}(kh_m)$, $(x_1,x_2)\rightarrow \phi^m_{l,2}(x)=I_{(0,x_2]}(lh_m)$,
$(x_1,x_2)\rightarrow \phi^m_{k,l,2}(x)=I_{(0,x]}(kh_m,l h_m)$, $k=0,\ldots,K_m\approx \tau_1/h_m$, $l=0,\ldots,L_m\approx\tau_2/h_m$, plus an intercept,  where the sum of the absolute value of the coefficients of the linear regression  with covariates  $\{\phi^m_0,\phi^m_{k,l,(1,2)},\phi^m_{k,1},\phi^m_{l,2}:k,l\}$  equals $M$. 

Let ${\cal I}_m=\{0,(k,1),(l,2),(k,l,(1,2)): k,l\}$ be the index set for these basis functions so that we can represent the set of basis functions as 
$\{ \phi^m_j: j\in {\cal I}_m\}$, and $f=\sum_{j\in {\cal I}_m}\beta_j^m(f)\phi^m_j$ where $\beta_j^m(f)=f(R_m(j))$ is the measure $f$ assigns to partition element $R_m(j)$, 
$j\in {\cal I}_m$, and $\beta_0^m(f)=f(0)$.

For a given $h_m$ and corresponding partitioning, consider the set
\[
{\cal F}_{v,0,M}^m=\{\sum_{j\in {\cal I}_m}\beta_j\phi_j^m: \sum_{j\in {\cal I}_m}\mid \beta_j\mid< M\}.\]
Let ${\cal F}_{v,0,M}=\{f\in D[0,\tau ]: \pl f\pl_{v,0}<M\}$.
For each $f\in {\cal F}_{v,0,M}$, we have that we can find a  sequence $f_m\in {\cal F}_{v,0,M}^m$, $m=1,\ldots$, so that
$f_m(x)\rightarrow f(x)$ for each $x\in [0,\tau ]$. 
By the dominated convergence theorem this implies that $\int (f_m-f)^2(x)d\lambda(x)\rightarrow 0$ for any bounded measure $\lambda$.
I suspect that we also have
\[
\lim_{m\rightarrow \infty}\sup_{f, \pl f\pl_{v,0}<M} \pl f_m-f\pl_{\lambda}=0.
\]
That is, the step function $f_m=f_m(f)$ approximates $f$ in $L^2(\lambda)$ norm uniformly in all $f$ with $\pl f\pl_{v,0}\leq M$.

We proved the following lemma.
\begin{lemma}
%Consider $f\in D[0,\tau ]$ with $[0,\tau ]\subset\openr^p$.
We define  a variation norm as follows: 
\[
\pl f\pl_{v}=\mid f(0)\mid +\sum_{s\subset \{1,\ldots,d\}}\int_{(0_s,\tau_s]}\mid f(dx_s,o_{-s})\mid,
\]
where for a subset $s\subset \{1,\ldots,d\}$, $x_s=(x_j: j\in s)$ and $x_{-s}=(x_j:j\not \in s)$, and $\sum_s$ is over all subsets of $\{1,\ldots,d\}$.
%If $\pl f\pl_{v,0}<\infty$, then we have the following representation of the function $f$:\[f(x)=f(0)+\sum_{s\in \{1,\ldots,d\}} \int_{(0_s,x_s]}\mid f(du_s,o_{-s}).\]
Let ${\cal F}_{v,M}=\{f\in D[0,\tau ]: \pl f\pl_{v,M}\}$.

We note $[0,\tau ]=\{0\}\cup \cup_{s\subset \{1,\ldots,d\}} (0_s,\tau_s]$.
For every $s\subset \{1,\ldots,d\}$, let $R_m((k_r:r\in s),s)=\prod_{l=1}^{d}(k_l h_m,(k_l+1)h_m]^{I(l\in s)}\{0\}^{I(l\not\in s)}$ be a partitioning in (approximately) $\prod_{r\in s}(\tau_r/h_m)$ squares with width $h_m$
of $(0_s,\tau_s)=\prod_{l=1}^d (0,\tau_l]^{I(l\in s)}\{0\}^{I(l\not\in s)}$, where each $k_r=0,\ldots,K_{r,m}\approx \tau_r/h_m$ runs over approximately $\tau_r/h_m$ integer values.
For each $s\subset\{1,\ldots,d\}$, we define
\[
\phi^m_{(k_r:r\in s),s}(x)=I_{(0_s,x_s]}(k_rh_m: r\in s),\]
as the indicator that a point in $R_m((k_r:r\in s),x)$ is in $(0,x]$.  
Let ${\cal I}_m=\{((k_r:r\in s),s):k_r=1,\ldots,\tau_r/h_m,s\subset \{1,\.ldots,d\}\cup \{0\}$ be the set of indices indicator each of these indicator basis functions, including the basis function 
$\phi^m_0(x)=1$. 

For any function $f\in {\cal F}_{v,M}$, we define
\[
f^m(x)=\sum_{j\in {\cal I}_m} \beta_j^m(f)\phi_j^m(x)
where $\beta_j^m(f)=f(R_m(j))$ is the measure $f$ assigns to the partition element $R_m(j)$.
We have
\[
f(x)=\lim_{h_m\rightarrow 0}f_m(x).\]
We also have that for any finite measure $\Lambda$:
\[
\lim_{h_m\rightarrow 0} \pl f-\lim_{h_m\rightarrow 0}\sum_{j\in {\cal I}_m}\beta_j^m(f)\phi_j^m\pl_{\Lambda} =0.\]
In addition, 
\[
\pl f\pl_{v}=\lim_{h_m\rightarrow 0}\sum_{j\in {\cal I}_m}\mid \beta_j^m(f)\mid .
\]
For a given $h_m$ and corresponding partitioning, consider the set
\[
{\cal F}_{v,M}^m=\{\sum_{j\in {\cal I}_m}\beta_j\phi_j^m: \sum_{j\in {\cal I}_m}\mid \beta_j\mid< M\}.\]
Equivalently, this is defined as
\[
{\cal F}_{v,M}^m=\{f_m(f): f\in {\cal F}_{v,M}\}.\]
This set approximates ${\cal F}_{v,M}$ as $h_m\rightarrow 0$ in the sense that for any function $f\in {\cal F}_{v,M}$ we can construct a sequence
$f_m\in {\cal F}_{v,M}^m$ so that $f(x)=\lim_{m\rightarrow\infty}f_m(x)$ for all $x\in [0,\tau ]$, and $\pl f_m-f\pl_{\Lambda}\rightarrow 0$.

We conjecture that we also have:
\[
\lim_{h_m\rightarrow 0} \sup_{f\in {\cal F}_{v,M}}\pl f_m-f\pl_{\Lambda} =0.\]
\end{lemma}

\subsection{An approximate MLE over functions of bounded variation using $L_1$-penalized regression}
The important implication of the previous approximation result is the following.

Consider $f_0\in {\cal F}_{v,M}$ so that $P_0L(f_0)=\min_{f\in {\cal F}_{v,M}} P_0L(f)$, and let $f_{0,m}\in {\cal F}_{v,M}^m$ be such that $P_0L(f_{0,m})=\min_{f\in {\cal F}_{v,M}^m} P_0L(f)$.
We want to show that $P_0(L(f_{0,m})-L(f_0))\rightarrow 0$. By the above lemma, since $f_0\in {\cal F}_{v,M}$, we can find a sequence $f_{0,m}^*\in {\cal F}_{v,M}^m$ so that
$f_{0,m}^*\rightarrow f_0$ as $m\rightarrow\infty$, pointwise and in $L^2(P_0)$ norm.
Then $P_0L(f_{0,m}^*)-P_0L(f_0)$ also converges to zero as $m\rightarrow\infty$. But, since $f_{0,m}$ minimizes $P_0L(f)$ over all $f\in {\cal F}_{v,M}^m$, we have \[
0\leq P_0L(f_{0,m})-P_0L(f_0)\leq P_0L(f_{0,m}^*)-P_0L(f_0)\rightarrow 0,\]
which proves that $P_0L(f_{0,m})-P_0L(f_0)\rightarrow 0$, as $m\rightarrow\infty$.

Consider now an $f_n\in {\cal F}_{v,M}$ so that $P_nL(f_n)=\min_{f\in {\cal F}_{v,M}}P_nL(f)$, and let $f_{n,m}\in {\cal F}_{v,M}^m$ be such that 
$P_n L(f_{n,m})=\min_{f\in {\cal F}_{v,M}^m} P_nL(f)$. We want to show that $P_n (L(f_{n,m})-L(f_n))\rightarrow 0$ as $m\rightarrow\infty$.
By the above lemma, since $f_n\in {\cal F}_{v,M}$, we can find a sequence $f_{n,m}^*\in {\cal F}_{v,M}^m$ so that 
$f_{n,m}^*\rightarrow f_n$ as $m\rightarrow\infty$, pointwise and thus also in $L^2(P_n)$-norm.

Then $P_nL(f_{n,m}^*)-P_nL(f_n)$ also converges to zero as $m\rightarrow\infty$. But, since $f_{n,m}$ minimizes $P_nL(f)$ over all $f\in {\cal F}_{v,M}^m$, we have \[
0\leq P_nL(f_{n,m})-P_nL(f_n)\leq P_nL(f_{n,m}^*)-P_nL(f_n)\rightarrow 0,\]
which proves that $P_nL(f_{n,m})-P_nL(f_n)\rightarrow 0$, as $m\rightarrow\infty$.

This proves the following lemma.
\begin{lemma}
Let $(0,Q)\rightarrow L(Q)(o)$ be a loss function for a parameter $Q_0=\arg\min_{Q\in Q({\cal M})}P_0L(Q)$.
Let ${\cal Q}_M={\cal Q}\cap {\cal F}_{v,M}=\{Q(P):P\in {\cal M},Q(P)\in {\cal F}_{v,M}\}$ be all functions in the parameter space for $Q_0$ that have a variation norm smaller than $M<\infty$.
Let ${\cal Q}_M^m=\{Q_m: Q\in {\cal Q}_M\}$, where $Q_m=Q_m(Q)$ is defined above as the finite dimensional linear approximation of $Q$ in terms of a partitioning depending on a width $h_m$.  

Consider an $Q_{0}^M\in {\cal Q}_M$ so that $P_0L(Q_{0}^M)=\min_{Q\in {\cal Q}_M} P_0L(Q)$, and let $Q_{0}^{M,m}\in {\cal Q}_M^m$ be such that $P_0L(Q_{0}^{M,m})=\min_{Q\in {\cal Q}_{M}^m} P_0L(Q)$.
Then, $P_0(L(Q_{0}^{M,m})-L(Q_0^M))\rightarrow 0$ as $m\rightarrow\infty$.

Similarly, consider a $Q_n^M\in {\cal Q}_{M}$ so that $P_nL(Q_n^M)=\min_{Q\in {\cal Q}_{M}}P_nL(Q)$, and let $Q_n^{M,m}\in {\cal Q}_{M}^m$ be such that 
$P_n L(Q_{n}^{M,m})=\min_{Q\in {\cal Q}_{M}^m} P_nL(Q)$. Then, $P_n (L(Q_{n}^{M,m}-L(Q_{n}^M) )\rightarrow 0$ as $m\rightarrow\infty$.
\end{lemma}








\section{Super-learner that achieves a rate faster than $n^{-1/4}$}
Our goal is to construct an estimator $\hat{Q}:{\cal M}_{np}\rightarrow{\cal Q}$ of $Q_0=Q(P_0)=\arg\min_{Q\in {\cal Q}}P_0L(Q)$ so that $d_0(Q_n,Q_0)=o_P(n^{-1/4})$.
In the previous section, we constructed an MLE $\hat{Q}^M:{\cal M}_{np}\rightarrow {\cal Q}_M={\cal Q}\cap {\cal F}_{v,M}$ for which $d_0(Q_n^M=\hat{Q}^M(P_n),Q_{0}^M)=o_P(n^{-1/4})$.
Let $\hat{Q}_{v,j}=\hat{Q}^{M_j}$, $j=1,\ldots,J_{v,n}$, be a collection of such MLEs corresponding with a sequence $M_1<\ldots<M_{J_{v,n}}$, where $\lim_{n\rightarrow\infty}M_{J_{v,n}}>\pl Q_0\pl_v$. Thus, for all $M_j>\pl Q_0\pl_v$, we have that $d_0(Q_{v,j,n},Q_0)=o_P(n^{-1/4})$.
In addition, let $\hat{Q}_j:{\cal M}_{np}\rightarrow {\cal Q}$, $j=1,\ldots,J_n$, be a collection of other estimators of $Q_0$, including a variety of parametric model as well as machine learning based estimators. 
This defines a collection of $K_n=J_{v,n}+J_n$ candidate estimators $\{\hat{Q}_{v,j}:j=1,\ldots,J_{v,n}\}\cup\{\hat{Q}_j: j=1,\ldots,J_n\}$ of $Q_0$.

Let $B_n\in \{0,1\}^n$ be a random vector with $V$ possible realizations which defines a split in a training sample $\{i:B_n(i)=0\}$ and validation sample
$\{i:B_n(i)=1\}$, where $B_n$ is independent of $(O_1,\ldots,O_n)$. 
Let $q$ be such that $P(\sum_i B_n(i)/n \geq q)=1$.
Let $P_{n,B_n}^1,P_{n,B_n}^0$ be the empirical probability distributions of the validation and trainmen sample, respectively.
Let ${\cal K}_n=\{1,\ldots,J_n\}\cup\{(v,1),\ldots,(v,J_{v,n})\}$ be the index set for the $K_n$ candidate estimators.
We define the cross-validation selector as the index
\[
k_n=\hat{K}(P_n)=\arg\min_{k\in {\cal K}_n} E_{B_n}P_n L(\hat{Q}_k(P_{n,B_n}^0))\]
that minimizes the cross-validated risk $E_{B_n}P_nL(\hat{Q}_k(P_{n,B_n}^0))$ over all choices $k$ of candidate estimators. 
We also define an oracle selector
\[
\tilde{k}_{0,n}=\tilde{K}_0(P_n)=\arg\min_{k\in {\cal K}_n} E_{B_n}P_0L(\hat{Q}_k(P_{n,B_n}^0))\]
as the index of the candidate estimator that minimizes the true conditional risk $E_{B_n}P_0L(\hat{Q}_k(P_{n,B_n}^0))$ over the index set for the candidate estimators. 
The cross-validated selected estimator is given by $\hat{Q}_{k_n}:{\cal M}_{np}\rightarrow{\cal Q}$, and the oracle selected estimator is
given by $\hat{Q}_{\tilde{k}_{0,n}}:{\cal M}_{np}\rightarrow{\cal Q}$. Note that
\[
E_{B_n}d_0(\hat{Q}_{\tilde{k}_{0,n}}(P_{n,B_n}^0),Q_0)=\min_{k\in {\cal K}_n} E_{B_n}P_0 L(\hat{Q}_k(P_{n,B_n}^0)).\]

\begin{lemma}
Suppose that $\sup_{o\in {\cal O},Q\in {\cal Q}}\mid L(Q)(o)-L(Q_0)(o)\mid <M_1$ and 
\[
\sup_{Q\in {\cal Q}} \frac{P_0 \{L(Q)-L(Q_0)\}^2}{P_0\{L(Q)-L(Q_0)\}}<M_2.\]
Then, for any $\delta>0$, there exists a constant $C(M_1,M_2,\delta)=2(1+\delta)^2(2M_1/3+M_2/\delta)$ such that
\begin{eqnarray*}
E_0\{E_{B_n}d_0(\hat{Q}_{k_n}(P_{n,B_n}^0,Q_0)\}&\leq& (1+2\delta)E_0\{E_{B_n}\min_k d_0(\hat{Q}_k(P_{n,B_n}^0),Q_0)\}\\
&& +2C(M_1,M_2,\delta)\frac{1+\log K_n}{nq}.
\end{eqnarray*}
Similarly,  for any $\delta>0$, there exists a constant $C(M_1,M_2,\delta)=2(1+\delta)^2(2M_1/3+M_2/\delta)$ such that
\begin{eqnarray*}
E_{B_n}d_0(\hat{Q}_{k_n}(P_{n,B_n}^0,Q_0)&\leq& (1+2\delta)E_{B_n}\min_k d_0(\hat{Q}_k(P_{n,B_n}^0),Q_0)\}\\
&& +R_n,
\end{eqnarray*}
where $ER_n\leq 2C(M_1,M_2,\delta)\frac{1+\log K_n}{nq}, so that, in particular, $ER_n=O_P(C(M_1,M_2,\delta)(1+\log K_n)/(nq))$.

If $\log K_n/n $ divided by $E_{B_n}\min_k d_0(\hat{Q}_k(P_{n,B_n}^0),Q_0)\}$ converges to zero in probability, 
then we also have
\[
\frac{E_{B_n}d_0(\hat{Q}_{k_n}(P_{n,B_n}^0,Q_0)}{E_{B_n}\min_k d_0(\hat{Q}_k(P_{n,B_n}^0,Q_0)}\rightarrow_p 1.\]
Similarly, if $\log K_n/n$ divided by $E_0E_{B_n}\min_k d_0(\hat{Q}_k(P_{n,B_n}^0),Q_0)\}$ converges to zero,
then we also have
\[
\frac{E_0E_{B_n}d_0(\hat{Q}_{k_n}(P_{n,B_n}^0,Q_0)}{E_0E_{B_n}\min_k d_0(\hat{Q}_k(P_{n,B_n}^0,Q_0)}\rightarrow 1.\]
\end{lemma}
% in proofs it is all about 0<<-d_0k_n<=(1+2delta)d_0tilde{k}_n+ T_n+R_n, and then we use bernstein etc to study T_n,R_n to get the second order term bound.
%we show ET_n+ER_n converge at this rate. so we could even say that instead of saying O_P(logK_n/n).

Let $k^*_n=(v,j_n)$ indicate the estimator $\hat{Q}_{v,j_n}}$ with $M_{j_n}=\min\{M_j: M_j>\pl Q_0\pl_v\}$.
Note that with probability 1 $M_{j_n}< M^*_0$ for some $\pl Q_0\pl_v<M_0^*<\infty$. Therefore we know that 
$d_0(\hat{Q}_{k^*_n}(P_{n,B_n}^0),Q_0)=o_P(n^{-1/4})$ for each $B_n$. 
This implies that $\min_k d_0(\hat{Q}_k(P_{n,B_n}^0),Q_0)=o_P(n^{-1/4})$.
Since $B_n$ only has finite number of outcomes, this also implies that $E_{B_n}\min_k d_0(\hat{Q}_k(P_{n,B_n}^0),Q_0)=o_P(n^{-1/4})$.
By the finite sample oracle inequality this shows that
\[
E_{B_n}d_0(\hat{Q}_{k_n}(P_{n,B_n}^0),P_0)=o_P(n^{-1/4})+O_P(C(M_1,M_2,\delta)\log K_n/n).\]
We now want to show that under a reasonable condition, this implies
\[
d_0(E_{B_n}\hat{Q}_{k_n}(P_{n,B_n}^0),P_0)=o_P(n^{-1/4})+O_P(C(M_1,M_2,\delta)\log K_n/n).\]
Suppose $Q\rightarrow L(Q)$ is a convex loss function in the sense that $P_0L(\sum_{j=1}^m\alpha_jQ_j)\leq \sum_{j=1}^m\alpha_jP_0L(Q_j)$ when 
$\sum_j\alpha_j=1$ and $\min_j\alpha_j\geq 0$.
Then 
\begin{eqnarray*}
d_0(\hat{Q}(P_n),P_0)&=&  d_0(E_{B_n}\hat{Q}_{k_n}(P_{n,B_n}^0),P_0)\\
&=& P_0L(E_{B_n}\hat{Q}_{k_n}(P_{n,B_n}^0))-P_0L(Q_0)\\
&\leq& E_{B_n}P_0L(\hat{Q}_{k_n}(P_{n,B_n}^0))-P_0L(Q_0)\\
&=&
E_{B_n}d_0(\hat{Q}_{k_n}(P_{n,B_n}^0),P_0)\\
&=& o_P(n^{-1/4})+O_P(C(M_1,M_2,\delta)\log K_n /n).
\end{eqnarray*}
This proves the following theorem.
\begin{theorem}\label{thslM1}
Let $L(Q)$ be a convex loss function in the sense that $P_0L(\sum_{j=1}^m\alpha_jQ_j)\leq \sum_{j=1}^m\alpha_jP_0L(Q_j)$ when 
$\sum_j\alpha_j=1$ and $\min_j\alpha_j\geq 0$.
Let ${\cal Q}=\{Q(P):P\in {\cal M}\}$ be the parameter space of the parameter $Q:{\cal M}\rightarrow Q({\cal M})$.
In addition, assume $\sup_{o\in {\cal O},Q\in {\cal Q}}\mid L(Q)(o)-L(Q_0)(o)\mid <M_1$ and 
\[
\sup_{Q\in {\cal Q}} \frac{P_0 \{L(Q)-L(Q_0)\}^2}{P_0\{L(Q)-L(Q_0)\}}<M_2.\]
Let $d_0(Q,Q_0)=P_0L(Q)-P_0L(Q_0)$.

Consider a library of candidate estimators $\hat{Q}_k:{\cal M}_{np}\rightarrow {\cal Q}$, $k=1,\ldots,K_n$, including this estimator $\hat{Q}_1$.
Let
\[
k_n=\hat{K}(P_n)=\arg\min_{k} E_{B_n}P_{n,B_n}^1L(\hat{Q}_k(P_{n,B_n}^0))\]
and let 
\[
Q_n=\hat{Q}(P_n)=E_{B_n}\hat{Q}_{k_n}(P_{n,B_n}^0).\]
Then, for any $\delta>0$, 
\[
d_0(Q_n,Q_0)\leq (1+2\delta) E_{B_n}\min_k d_0(\hat{Q}_k(P_{n,B_n}^0),Q_0)+O_P(C(M_1,M_2,\delta)\log K_n/(nq)).\]

If the fraction of $\log K_n/n$ over  $E_{B_n}P_0L(\hat{Q}_{\tilde{k}_{0n}}(P_{n,B_n}^0),Q_0)$ is $o_P(1)$, then 
\[
\frac{d_0(\hat{Q}(P_n),Q_0)}{E_{B_n}\min_kd_0(\hat{Q}_k(P_{n,B_n}^0),Q_0)}-1=o_P(1).\]
If  $E_{B_n}P_0L(\hat{Q}_{\tilde{k}_{0n}}(P_{n,B_n}^0),Q_0)=O_P(\log K_n /n), then 
\[
d_0(\hat{Q}(P_n),Q_0)=O_P(\log K_n /n).\]

Let $\hat{Q}_1:{\cal M}_{np}\rightarrow {\cal Q}$ be an estimator so that $d_0(\hat{Q}_1(P_n),Q_0)=o_P(n^{-1/2})$.
Then, it follows that (worst case)
\begin{equation}\label{conservativebound}
d_0(\hat{Q}(P_n),Q_0)=o_P(n^{-1/2})+O_P(C(M_1,M_2,\delta)(\log K_n/n).\end{equation}

In Lemma \ref{lemmamle1}  we define an estimator $\hat{Q}^{M^u}$ that minimizes the empirical risk over subset ${\cal Q}_{M^u}\subset {\cal Q}$ of functions with variation norm smaller than a known upper bond $M^u>\pl Q_0\pl_v$. 
In Lemma \ref{lemmamlecv} we define an estimator $\hat{Q}_v$ which is defined in terms of  a library of  such candidate estimators $\hat{Q}^{M_j}$ indexed by various bounds $M_j$,  $j=1,\ldots,J_n$, 
and the cross-validation selector of $M_j$, where $M_{J_n}>\pl  Q_0\pl_v$ for $n$ large enough (allowing for an  unknown bound on the variation norm of $Q_0$, but still relying on $\pl Q_0\pl_v<\infty$).

In addition to the above assumptions, assume that $\sup_{Q\in {\cal Q}_M}\frac{ \pl L(Q)\pl_v}{\pl Q\pl_v} <\infty$: i.e., the variation norm of $L(Q)$ can be universally bounded in terms of the variation norm of $Q$.
%: this one always holds given our M_2: that $d_0(Q_n,Q_0)\rightarrow 0$ implies $\pl L(Q_n)-L(Q_0)\pl_{P_0}\rightarrow 0$.
Then, $d_0(\hat{Q}^{M^u}(P_n),Q_0)=o_P(n^{-1/2})$ and $d_0(\hat{Q}_v(P_n),Q_0)=o_P(n^{-1/2})$. Thus, by selecting $\hat{Q}_1$ as $\hat{Q}^{M^u}$ or 
$\hat{Q}_v$ in the case that $M^u>\pl Q_0\pl_v$ is known, and selecting $\hat{Q}_1=\hat{Q}_v$ in the case that there is no known upper bound for $\pl Q_0\pl_v<\infty$,   the  super-learner $\hat{Q}(P_n)$ above satisfies (\ref{conservative bound}).


\end{theorem}
If one assumes that $d_0(hat{Q}_{k_n}(P_n),Q_0)/d_0(E_{B_n}\hat{Q}_{k_n}(P_{n,B_n}^0),Q_0) \leq C$ for some $C$  with probabiliy tending to 1, then the above results also provide the desired results for the super-learner $\hat{Q}_{k_n}(P_n)$ instead of $E_{B_n}\hat{Q}_{k_n}(P_{n,B_n}^0)$. 
One would expect that this even holds for $C=1$ or $C=(1+\delta)$ for a small $\delta>0$.

\subsection{A super-learner that also adapts to an unknown supremum norm of $Q_0$.}
The previous theorem for the super-learner using  $\hat{Q}_1=\hat{Q}_v$  applies to any model ${\cal M}$ for which 
$M_1=\sup_{Q\in {\cal Q},o\in {\cal O}}\mid L(Q)-L(Q_0)|(o)<\infty$ and $M_2=\sup_{Q\in {\cal Q}}\pl L(Q)-L(Q_0)\pl_{P_0}^2/d_0(Q,Q_0) <\infty$, achieving the rate
$d_0(Q_n,Q_0)=o_P(n^{-1/2})$ as long as $\pl Q_0\pl_v<\infty$.This will hold when ${\cal O}$ has the described bounded support and $\sup_{Q\in {\cal Q}}\pl Q\pl_{\infty}<\infty$. That is, the model needs to assume a known supremum norm bound on $Q_0$. Such a bound is typically known but it is also possible that the model does not assume a uniform bound on the supremum norm of $Q_0$, even though it is assumed that each $Q$ in the model has a finite supremum norm. 
In this section we construct a super-learner that does not require knowing an upper bound and thus only assumes that $L(Q_0)$ has a finite supremum norm, and this super-learner still achieves the desired rate $o_P(1/\sqrt{n})$ w.r.t. $d_0(Q_n,Q_0)$.

The following lemma shows that if we let the supremum norm of our candidate estimators be bounded by a constant depending on $n$ that converges slowly enough with sample size to infinity, then we still obtain the desired finite sample inequality for the cross-validation selector and its asymptotic equivalence with the oracle selector. 
 In addition, the result provides clear conservative guidance on how to select the supremum norm bound $M_{1n}$ of our candidate estimators.
 We note here that the bound $M_2$ typically directly depends on $M_1$ so that a sequence $M_{1n}$ will imply a sequence $M_{2n}$ that might also converge to infinity at the same rate as $M_{1n}$.

\begin{lemma}
Suppose that $\sup_{o\in {\cal O}}\mid L(Q_0)(o)\mid <\infty$, but $\sup_{o\in {\cal O},P\in {\cal M}}\mid L(Q(P))(o)\mid =\infty$.
Let ${\cal M}_n$ be a sequence of models increasing in $n$, approximating ${\cal M}$, and  for which $M_{1n}=\sup_{o\in {\cal O},P\in {\cal M}_n}\mid L(Q(P))(o)\mid <\infty$, and for $n>N_0$ we have $P_0\in {\cal M}_n$ (where $N_0$ is unknown). Let ${\cal Q}_n=\{Q(P):P\in {\cal M}_n\}$ and let $Q_{0n}=Q^n(P_0)=\arg\min_{Q\in {\cal Q}_n}P_0L(Q)$.
In addition, let
\[
M_{2n}=\sup_{P\in {\cal M}_n} \frac{P_0 \{L(Q(P))-L(Q_{0n})\}^2}{P_0\{L(Q(P))-L(Q_{0n})\}}<infty.\]
Let $\hat{Q}_{k}\in {\cal Q}_n$, $k=1,\ldots,K_n$ be a collection of candidate estimators of $Q_{0n}$, and let $k_n=\arg\min_kE_{B_n}P_{n,B_n}^1L(\hat{Q}_k(P_{n,B_n}^0))$ be the cross-validation selector. 

Then, for any $\delta>0$, there exists a constant $C(M_{1n},M_{2n},\delta)=2(1+\delta)^2(2M_{1n}/3+M_{2n}/\delta)$ such that
\begin{eqnarray*}
E_0\{E_{B_n}d_0(\hat{Q}_{k_n}(P_{n,B_n}^0,Q_{0n})\}&\leq& (1+2\delta)E_0\{E_{B_n}\min_k d_0(\hat{Q}_k(P_{n,B_n}^0),Q_{0n})\}\\
&& +2C(M_{1n},M_{2n},\delta)\frac{1+\log K_n}{nq}.
\end{eqnarray*}
More generally,  for any $\delta>0$, there exists a constant $C(M_{1n},M_{2n},\delta)=2(1+\delta)^2(2M_{1n}/3+M_{2n}/\delta)$ such that
\begin{eqnarray*}
E_{B_n}d_0(\hat{Q}_{k_n}(P_{n,B_n}^0,Q_{0n})&\leq& (1+2\delta)E_{B_n}\min_k d_0(\hat{Q}_k(P_{n,B_n}^0),Q_{0n})\}\\
&& +R_n,
\end{eqnarray*}
where $E_0R_n\leq 2C(M_{1n},M_{2n},\delta)\frac{1+\log K_n}{nq}, so that, in particular, $E_0R_n=O_P(C(M_{1n},M_{2n},\delta)(1+\log K_n)/(nq))$.

If for each $\delta> 0$, $C(M_{1n},M_{2n},\delta)\log K_n/n $ divided by $E_{B_n}\min_k d_0(\hat{Q}_k(P_{n,B_n}^0),Q_{0n})\}$ converges to zero in probability, 
then we also have
\[
\frac{E_{B_n}d_0(\hat{Q}_{k_n}(P_{n,B_n}^0,Q_0)}{E_{B_n}\min_k d_0(\hat{Q}_k(P_{n,B_n}^0,Q_0)}\rightarrow_p 1.\]
Similarly, if  for each $\delta>0$, $C(M_{1n},M_{2n},\delta)\log K_n/n$ divided by $E_0E_{B_n}\min_k d_0(\hat{Q}_k(P_{n,B_n}^0),Q_0)\}$ converges to zero,
then we also have
\[
\frac{E_0E_{B_n}d_0(\hat{Q}_{k_n}(P_{n,B_n}^0,Q_0)}{E_0E_{B_n}\min_k d_0(\hat{Q}_k(P_{n,B_n}^0,Q_0)}\rightarrow 1.\]
\end{lemma}

We can now generalize our Theorem  \ref{thslM1} for the super-learner adapting to the unknown variation norm of $Q_0$ but that assumes a fixed bound $M_1,M_2$  to a Theorem for a more general super-learner that  allows $M_{1n},M_{2n}$ to converge to infinity at a specified slow enough rate, without sacrificing the desired
$d_0(Q_n,Q_0)=o_P(n^{-1/2})$.

\begin{theorem}\label{thslM1n}
Consider the definitions ${\cal M}_n$, ${\cal Q}_n$, $Q_{0n}$, $M_{1n},M_{2n}$. 
In addition, assume that $L(Q)$ be a convex loss function in the sense that $P_0L(\sum_{j=1}^m\alpha_jQ_j)\leq \sum_{j=1}^m\alpha_jP_0L(Q_j)$ when 
$\sum_j\alpha_j=1$ and $\min_j\alpha_j\geq 0$.

Consider a library of candidate estimators $\hat{Q}_k:{\cal M}_{np}\rightarrow {\cal Q}_n$, $k=1,\ldots,K_n$.
Let
\[
k_n=\hat{K}(P_n)=\arg\min_{k} E_{B_n}P_{n,B_n}^1L(\hat{Q}_k(P_{n,B_n}^0))\]
and let 
\[
Q_n=\hat{Q}(P_n)=E_{B_n}\hat{Q}_{k_n}(P_{n,B_n}^0).\]
Then, for any $\delta>0$, 
\[
d_0(Q_n,Q_{0n})\leq (1+2\delta) E_{B_n}\min_k d_0(\hat{Q}_k(P_{n,B_n}^0),Q_{0n})+O_P(C(M_{1n},M_{2n},\delta)\log K_n/(nq)).\]

If for each $\delta>0$, the fraction of $C(M_{1n},M_{2n},\delta)\log K_n/n$ over  $E_{B_n}\min_k d_0(\hat{Q}_{k}(P_{n,B_n}^0),Q_{0n})$ is $o_P(1)$, then 
\[
\frac{d_0(\hat{Q}(P_n),Q_0)}{E_{B_n}\min_kd_0(\hat{Q}_k(P_{n,B_n}^0),Q_0)}-1=o_P(1).\]
If  for each $\delta>0$, $E_{B_n}\min_k d_0(\hat{Q}_{k}(P_{n,B_n}^0),Q_0)=O_P(C(M_{1n},M_{2n},\delta)(\log K_n /n), then 
\[
d_0(\hat{Q}(P_n),Q_0)=O_P(C(M_{1n},M_{2n},\delta)\log K_n /n).\]

Let $\hat{Q}_1:{\cal M}_{np}\rightarrow {\cal Q}$ be an estimator so that $d_0(\hat{Q}_1(P_n),Q_0)=o_P(n^{-1/2})$.
Then, it follows that (worst case)
\begin{equation}\label{conservativebound}
d_0(\hat{Q}(P_n),Q_0)=o_P(n^{-1/2})+O_P(C(M_{1n},M_{2n},\delta)(\log K_n/n).\end{equation}

In Lemma \ref{lemmamle1}  we define an estimator $\hat{Q}^{M}$ that minimizes the empirical risk over subset ${\cal Q}_{M}\subset {\cal Q}$ of functions with variation norm smaller than a known upper bound $M$. 
In Lemma \ref{lemmamlecv} we define an estimator $\hat{Q}_v$ which is defined in terms of  a library of  such candidate estimators $\hat{Q}^{M_j}$ indexed by various bounds $M_j$,  $j=1,\ldots,J_n$, 
and the cross-validation selector of $M_j$, where $M_{J_n}>\pl  Q_0\pl_v$ for $n$ large enough (allowing for an  unknown bound on the variation norm of $Q_0$, but still relying on $\pl Q_0\pl_v<\infty$). Consider this estimator $\hat{Q}_v$ but instead of enforcing a fixed bound $M_1,M_2$, now only enforce the candidate estimators to be in ${\cal Q}_n\uparrow {\cal Q}$ for a sequence $M_{1n},M_{2n}$ chosen so that $C(M_{1n},M_{2n},\delta)\log K_n/n =o(n^{-1/2})$. 

In addition to the above assumptions, assume that $\sup_{Q\in {\cal Q}_M}\frac{ \pl L(Q)\pl_v}{\pl Q\pl_v} <\infty$: i.e., the variation norm of $L(Q)$ can be universally bounded in terms of the variation norm of $Q$.
%: this one always holds given our M_2: that $d_0(Q_n,Q_0)\rightarrow 0$ implies $\pl L(Q_n)-L(Q_0)\pl_{P_0}\rightarrow 0$.
Then, $d_0(\hat{Q}_v(P_n),Q_0)=o_P(n^{-1/2})$. Thus, by selecting $\hat{Q}_1=\hat{Q}_v$,   the  super-learner $\hat{Q}(P_n)$ above satisfies (\ref{conservative bound}).
\end{theorem}

To summarize, we have constructed 1) a super learner for a model ${\cal M}$ that assumes a  fixed upper bound for both the variation norm and supremum norm of $Q_0$ ($\pl Q_0\pl_{\infty}<C$ and \pl Q_0\pl_v<M^u$ for a known $C,C,M^u$), 
2) a super learner for a model ${\cal M}$ that only assumes a fixed upper bound $C$ for the supremum norm of $Q_0$ and only assumes $\pl  Q_0\pl_v<\infty$, 3) 
a super learner for a model ${\cal M}$ that only assumes $\pl Q_0\pl_{\infty}<\infty$ and $\pl Q_0\pl_v<\infty$, and all super-learner achieve the desired rate
$d_0(Q_n,Q_0)=o_P(n^{-1/2})$. 

For super-learner 1) we know that $L(Q_n)$ falls in a $P_0$-Donsker class with probability 1. For  super-learner
2) we know that $\pl Q_n\pl_{\infty}<C$ for a known $C$ but we do not know if $L(Q_n)$ has a variation norm smaller than some possibly unknown $M^v(P_0)<\infty$ with probability tending to 1. If the latter would  hold, then we would know that $L(Q_n)$ falls in a  $P_0$-Donsker class with probability tending to 1. 
For super learner 3) we neither know that $\pl Q_n\pl_{\infty}<C_0=C(P_0)$ for some unknown $C(P_0)<\infty$, nor do we know if  $\pl L(Q_n)\pl_v<M^v_0=M^v(P_0)$ for some unknown $M^v(P_0)<\infty$.  
Assuming that for each $n$, the candidate estimators in the super learner includes estimators with a range of sup-norms and variation norms, ranging from small to infinity when $n$ increases to infinity, the oracle selector for super-learners 2) and 3)   will select a candidate estimator for which both the supremum norm and variation norm are bounded by an upper bound. Since all super-learners are asymptotically equivalent with the oracle selector, there is hope that indeed the super-learner will have a variation norm and supremum norm bounded by some bounded $C_0,M^v_0$ with probability tending to 1, but we have not formally established such a result. 
So without such a formal result in our hands, super-learner 2 and 3 pay a price by not having the Donsker class guarantee, as required for efficiency of the one-step TMLE. Nonetheless, as we will show super-learners 2 and 3 still suffice for asymptotic efficiency of the CV-TMLE that does not rely on a Donsker class condition.
 




\subsection{Preservation of desired rate of convergence of one-step TMLE update of super-learner}
Suppose that $d_0(Q_n,Q_0)=o_P(r_n)$. Let $Q_n^*=Q_{n,\epsilon_n}$ be the one-step TMLE update of $Q_n$. We want to prove that 
$d_0(Q_n^*,Q_0)=o_P(r_n)$. Firstly, we consider the case that we know that $L(Q_n)$ falls in a $P_0$-Donsker class with probability tending to 1, such as class of functions with variation norm smaller than a universal bound $M^u_v$.

The following lemma proves that the result $d_0(Q_n,Q_0)=o_P(n^{-1/2})$ is preserved under no conditions on the behavior of the MLE $\epsilon_n$, except that 
$\{Q_{n,\epsilon}:\epsilon\}\subset {\cal Q}$ is indeed a submodel. Under slightly stronger conditions on the stochastic behavior of the MLE $\epsilon_n$, we can also show that this result will hold for 
any rate $r_n$, but we do not need that for our results so that that is omitted here.

\begin{lemma}
Suppose
\begin{itemize}
\item $d_0(Q_n,Q_0)=o_P(n^{-1/2})$;
\item $\pl L(Q)-L(Q_0)\pl_{P_0}^2\leq M_2 d_0(Q,Q_0)$ for all $Q\in {\cal Q}$.
\item If $Q\in {\cal Q}$, $\{Q_{\epsilon}:\epsilon\}\subset {\cal Q}$.
\item $\{L(Q): Q\in {\cal Q}\}$ is a $P_0$-Donsker class.
\end{itemize}
Then, $d_0(Q_n^*,Q_0)=o_P(n^{-1/2})$.
\end{lemma}
{\bf Proof:}
We have that $P_n L(Q_{n,\epsilon_n})=\min_{\epsilon} P_n L(Q_{n,\epsilon})$. Thus, 
\begin{eqnarray*}
0&\leq & d_0(Q_n^*,Q_0)=P_0L(Q_{n,\epsilon_n})-P_0L(Q_0)\\
&=& -(P_n-P_0)\{L(Q_{n,\epsilon_n})-L(Q_0)\}+P_n\{L(Q_{n,\epsilon_n})-L(Q_0)\}\\
&\leq & -(P_n-P_0)\{L(Q_{n,\epsilon_n})-L(Q_0)\}.
\end{eqnarray*}
We know that $Q_n$ falls in a set ${\cal Q}$ with probability tending to 1, where ${\cal Q}$ is such that $\{L(Q): Q\in {\cal Q}\}$ is a $P_0$-Donsker class. 
By construction,  $Q_{n,\epsilon}\in {\cal Q}$ for all $\epsilon$ since it is a submodel. Thus, $Q_{n,\epsilon_n}\in {\cal Q}$. 
Therefore we can conclude that $L(Q_n^*)-L(Q_0)$ falls in a $P_0$-Donsker class with probability tending to 1. 
This proves that $d_0(Q_n^*,Q_0)=O_P(n^{-1/2})$. By assumption $\pl L(Q_n^*)-L(Q_0)\pl_{P_0}^2\leq M_2 d_0(Q_n^*,Q_0)$.
Thus, $\pl L(Q_n^*)-L(Q_0)\pl_{P_0}^2=O_P(n^{-1/2})$.  By empirical process theory, this shows that $(P_n-P_0)\{L(Q_n^*)-L(Q_0)\}=o_P(n^{-1/2})$.
Thus, this proves $d_0(Q_n^*,Q_0)=o_P(n^{-1/2})$. $\Box$

\subsection{Preservation of the desired rate of convergence of cross-validated one-step TMLE update of super-learner}
Let $\hat{Q}:{\cal M}_{np}\rightarrow {\cal Q}_n$ be the initial estimator of $Q_{0n}=\arg\min_{Q\in {\cal Q}_n}P_0L(Q)$ relying on model ${\cal M}_n$ with 
constants $M_{1n},M_{2n}$ and parameter space ${\cal Q}_n$, where $M_{1n},M_{2n}$ satisfy $C(M_{1n},M_{2n},\delta)/n=o(n^{-1/2})$.
Let $Q_{n,B_n}=\hat{Q}(P_{n,B_n}^0)$ be the estimator applied to the $B_n$-specific training sample, where $B_n$ has  $V<\infty$ possible outcomes, which uses an estimator $G_{n,B_n}=\hat{G}(P_{n,B_n}^0)$.
Let $\{Q_{n,B_n,\epsilon}:\epsilon\}\subset{\cal Q}$ be the least favorable parametric submodel through $Q_{n,B_n}$ whose score at $\epsilon =0$ spans
$D^*(Q_{n,B_n},G_n)$.
Let $\epsilon_n=\arg\min_{\epsilon}E_{B_n}P_{n,B_n}^1 L(Q_{n,B_n,\epsilon}).\]
Note that $\epsilon_n$ is just the cross-validation selector over $\epsilon$.
By the oracle inequality in van der Vaart, Dudoit, van der Laan (2006) extending the previously mentioned oracle inequality for a discrete cross-validation selector to continuous families of candidate estimators, using that the entropy of $\{Q_{\epsilon}:\epsilon}$ for a fixed $Q$ is nicely bounded, we have that for any $\delta>0$,
\[
E_{B_n}d_0(Q_{n,B_n,\epsilon_n},Q_{0n})\leq (1+2\delta) E_{B_n}\min_{\epsilon}d_0(Q_{n,B_n,\epsilon},Q_{0n})+ O_P\left(\frac{C(M_{1n},M_{2n},\delta)}{nq}\right).\]
We chose $M_{1n},M_{2n}$ such that $C(M_{1n},M_{2n},\delta)/n=o(n^{-1/2})$, so that the second order term is $o_P(n^{-1/2})$.
 Since $\epsilon =0$ is a possible choice, we have
 \[
 E_{B_n}\min_{\epsilon}d_0(Q_{n,B_n,\epsilon},Q_{0n})\leq E_{B_n}d_0(Q_{n,B_n},Q_{0n}).\]
Thus,
 \[
E_{B_n}d_0(Q_{n,B_n,\epsilon_n},Q_{0n})\leq (1+2\delta) E_{B_n}d_0(Q_{n,B_n,\epsilon},Q_{0n})+ O_P\left(\frac{C(M_{1n},M_{2n},\delta)}{nq}\right).\]
 In particular, if the initial estimator $\hat{Q}$ satisfies $d_0(\hat{Q}(P_n),Q_{0n})=O_P(r_n)$, then it follows that 
 $d_0(Q_{n,B_n,\epsilon_n},Q_{0n})=O_P(r_n)+O_P\left(\frac{C(M_{1n},M_{2n},\delta)}{nq}\right)$. 
If $r_n=o_P(n^{-1/2})$, then  $d_0(Q_{n,B_n,\epsilon_n},Q_{0n})=o_P(n^{-1/2})$.
If for $n>N_0$ we have $Q_{0n}=Q_0$, then the same results follow for $d_0(Q_{n,B_n,\epsilon_n},Q_0)$.

 So we have the following lemma.
 \begin{lemma}
Let $\hat{Q}:{\cal M}_{np}\rightarrow {\cal Q}_n$ be the initial estimator of $Q_{0n}$ relying on model ${\cal M}_n$ with 
constants $M_{1n},M_{2n}$ and parameter space ${\cal Q}_n$, where $M_{1n},M_{2n}$ satisfy $C(M_{1n},M_{2n},\delta)/n=o(n^{-1/2})$.
Assume that there exists a $N_0$ so that for $n>N_0$ $Q_{0n}=Q_0$. Assume $d_0(\hat{Q}(P_n),Q_0)=O_P(r_n)$.

Let $Q_{n,B_n}=\hat{Q}(P_{n,B_n}^0)$ be the estimator applied to the $B_n$-specific training sample, where $B_n$ has  $V<\infty$ possible outcomes.
Let $\{Q_{n,B_n,\epsilon}:\epsilon\}\subset{\cal Q}$ be the least favorable parametric submodel through $Q_{n,B_n}$ whose score at $\epsilon =0$ spans
$D^*(Q_{n,B_n},G_n)$.
Let $\epsilon_n=\arg\min_{\epsilon}E_{B_n}P_{n,B_n}^1 L(Q_{n,B_n,\epsilon}).\]

Then, \[
d_0(Q_{n,B_n,\epsilon_n},Q_{0})=O_P(r_n)+O_P\left(\frac{C(M_{1n},M_{2n},\delta)}{nq}\right).\] 
If $r_n=o(n^{-1/2})$, then $d_0(Q_{n,B_n,\epsilon_n},Q_{0})=o_P(n^{-1/2})$.
\end{lemma}



\section{Cross-validated TMLE in General Unbounded Models}
Let $\{Q_{\epsilon}:\epsilon\}\subset {\cal Q}_n\subset{\cal Q}$ be a submodel through $Q$ at $\epsilon =0$ satisfying that
$\frac{d}{d\epsilon}L(Q_{\epsilon})$ at $\epsilon=0$ spans $D^*(Q,G)$, where $C_n=\sup_{Q\in {\cal Q}_n}\pl Q\pl_{\infty}<\infty$, while  $\sup_{Q\in {\cal Q}}\pl Q\pl_{\infty}$ could be infinity. Here ${\cal Q}_n\uparrow {\cal Q}$ as $n\rightarrow\infty$.
Let $\hat{Q}:{\cal M}_{np}\rightarrow {\cal Q}_n$ and $\hat{G}:{\cal M_{np}\rightarrow {\cal G}_n\subset {\cal G}= G({\cal M})$ be  initial estimators satisfying $d_{10}(\hat{Q}(P_n),Q_{0n})=o_P(n^{-1/2})$ and $d_{20}(\hat{G}(P_n),G_{0n})=o_P(n^{-1/2})$. Here we are reminded that there exists an $N(P_0)<\infty$ so that for $n>N(P_0)$, $Q_{0n}=Q_0$ and $G_{0n}=G_0$.
Given a cross-validation scheme $B_n\in \{0,1\}^n$, let $P_{n,B_n}^0$ and $P_{n,B_n}^1$ be the empirical distributions of the training and validation sample, and let
$Q_{n,B_n}=\hat{Q}(P_{n,B_n}^0)\in {\cal Q}_n$. Let $\epsilon_n=\arg\min_{\epsilon}E_{B_n}P_{n,B_n}^1L(Q_{n,B_n,\epsilon})$, where the submodel $Q_{n,B_n,\epsilon}$ uses $\hat{G}(P_{n,B_n}^0)$ as an estimator of $G_0$.
Let $Q_{n,B_n}^*=Q_{n,B_n,\epsilon_n}$ be the $B_n$-specific targeted fit of $Q_0$.
The CV-TMLE of $\psi_0$ is defined as $\psi_n^*=E_{B_n}\Psi(Q_{n,B_n,\epsilon_n})$.
If $\frac{d}{\epsilon}L(Q_{\epsilon})=D^*(Q_{\epsilon},G)$, then it follows that $E_{B_n}P_{n,B_n}^1 D^*(Q_{n,B_n}^*,G_{n,B_n})=0$. We only assume that $E_{B_n}P_{n,B_n}^1 D^*(Q_{n,B_n}^*,G_{n,B_n})=o_P(n^{-1/2})$, which by  Lemma ref will hold in great generality if the initial estimators converge at the $o_P(n^{-1/2})$-rate.  By the identity $\Psi(Q_{n,B_n}^*)-\Psi(Q_0)=-P_0 D^*(Q_{n,B_n}^*,G_{n,B_n})+R_2(Q_{n,B_n}^*,Q_0,G_{n,B_n},G_0)$, we also have
\[
E_{B_n}\Psi(Q_{n,B_n}^*)-\Psi(Q_0)=-E_{B_n} P_0 D^*(Q_{n,B_n}^*,G_{n,B_n})+E_{B_n}R_2(Q_{n,B_n}^*,Q_0,G_{n,B_n},G_0).\]
This yields the following identity:
\[
\psi_n^*-\Psi(Q_0)=E_{B_n}(P_{n,B_n}^1-P_0)D^*(Q_{n,B_n}^*,G_{n,B_n})+E_{B_n}R_2(Q_{n,B_n}^*,Q_0,G_{n,B_n},G_0).\]
Since $d_{10}(Q_{n,B_n}^*,Q_0)=o_P(n^{-1/2}$ and $d_{20}(G_{n,B_n},G_0)=o_P(n^{-1/2}$, and the assumed bound on $R_2()$, this  implies that
$R_2(Q_{n,B_n}^*,Q_0,G_{n,B_n},G_0)=o_P(n^{-1/2})$ and thus also $E_{B_n}R_{20}(Q_{n,B_n}^*,Q_0,G_{n,B_n},G_0)=o_P(n^{-1/2})$.

For a given $B_n$, conditional on $P_{n,B_n}^0$, we consider the empirical process
\[
\sqrt{n}(P_{n,B_n}^1-P_0)D^*(Q_{n,B_n,\epsilon_n},G_{n,B_n}).\]
Firstly, we note that this can be viewed as an empirical process $\sqrt{n}(P_n-P_0)f_{n,\epsilon_n}$, where $f_{n,\epsilon}=D^*(Q_{n,\epsilon},G_n)$ is a given function (i.e. not random through $P_n$), but $\epsilon_n=\hat{\epsilon}(P_n)$ is a function of $P_n$.
We have \[
\sqrt{n}(P_n-P_0)f_{n,\epsilon_n}=\sqrt{n}(P_n-P_0)(f_{n,\epsilon_n}-f_0)+\sqrt{n}(P_n-P_0)f_0,\]
where $f_0=D^*(Q_0,G_0)$. If we can prove that $\sqrt{n}(P_n-P_0)(f_{n,\epsilon_n}-f_0)=o_P(1)$, then we have shown that 
$\psi_n^*-\psi_0=E_{B_n}(P_{n,B_n}^1-P_0)D^*(Q_0,G_0)+o_P(n^{-1/2})=\sqrt{n}(P_n-P_0)D^*(Q_0,G_0)+o_P(n^{-1/2})$, establishing the desired asymptotic efficiency. 

So we now analyze $\sqrt{n}(P_n-P_0)(f_{n,\epsilon_n}-f_0)$. 
We know that $d_{10}(Q_{n,\epsilon_n},Q_0)=o_P(n^{-1/2})$ and $d_{20}(G_n,G_0)=o_P(n^{-1/2})$.
We assumed that 
\[
\pl D^*(Q_n,G_n)-D^*(Q_0,G_0)\pl_{P_0}\leq O( r(C_n)\max(d_0(Q_n,Q_0),d_0(G_n,G_0)) ),\]
where $r(C_n)$ is some specified function in $C_n=\sup_{Q\in {\cal Q}_n}\pl Q\pl_{\infty}$. In many cases one expects that this holds for $r(C_n)=1$.
Therefore it follows that $\pl D^*(Q_{n,\epsilon_n},G_n)-D^*(Q_0,G_0)\pl_{P_0}=o_P(r(C_n)n^{-1/4})$.
That is, $\pl f_{n,\epsilon_n}-f_0\pl_{P_0}=o_P(r(C_n)n^{-1/4})$, where $f_0=D^*(Q_0,G_0)$.
Let ${\cal F}_n=\{(f_{n,\epsilon}-f_0)/C_n:\epsilon\}$, and we write $\sqrt{n}(P_n-P_0)(f_{n,\epsilon_n}-f_0)=C_n \sqrt{n}(P_n-P_0)f_{n,\epsilon_n}/C_n$, and now focus on the empirical process $Z_n=(\sqrt{n}(P_n-P_0)f: f\in {\cal F}_n)$. 
The entropy $\sup_{Q}N(\epsilon,{\cal F}_n,L^2(Q))$ is $O(\epsilon^{-d})$. 
For each $\delta_n,\eta$, we have
\[
\pl \sup_{\pl f\pl\leq \delta_n}Z_n(f)\pl_{\psi_1}\leq \int_0^{\delta_n}\sqrt{\log N(\epsilon,{\cal F}_n)}d\epsilon +\eta \sqrt{\log N^2(\eta,{\cal F}_n)}.\]
We select $\delta_n=n^{-1/4}r(C_n)/C_n$ since the probability that $\pl (f_{n,\epsilon_n}-f_0)/C_n\pl_{P_0}<n^{-1/4}r(C_n)/C_n$ converges to 1. 
If we select $\eta=\delta_n$, then the right-hand side is bounded by $O(\delta_n\log \delta_n^{-1})$,
which is $O(n^{-1/4}r(C_n)C_n^{-1}(\log C_n+\log n+\log r(C_n) ))$. 
Thus, we can conclude that $\sqrt{n}(P_n-P_0)\{f_{n,\epsilon_n}-f_0\}=O_P(n^{-1/4}r(C_n)(\log C_n+\log n+\log r(C_n) ) )$.
We assumed that $C_n$ converges slowly enough to infinity so that  $n^{-1/4}r(C_n)(\log C_n+\log n+\log r(C_n) )\rightarrow 0$.
This completes the proof of $(P_{n,B_n}^1-P_0)\{D^*(Q_{n,B_n}^*,G_{n,B_n})-D^*(Q_0,G_0)\}=o_P(n^{-1/2})$, and thereby the asymptotic efficiency of the CV-TMLE.

State theorem, first conditions from above proof  in terms of initial estimator $Q_n,G_n, d_0=o(n^{-1/2})$ (is sum of d_{0j} fine).
That already makes general bound $R_{2n}$, link of $P_0$-norm of $D_n-D_0$ to $d_0$ rate, and assume efficient ic equation is solved with $o_P(n^{-1/2})$.

Then new theorem, focussing a model in which truth has  finite variation norm finite sup norm assumptions and $Q_0,G_0$ are cadlag and bounded variation, defined by assuming this for
each section corresponding with setting the discrete argument of $Q_0$  to a value. both defined by losses $L_1,L_2$ (sum losses themselves fine).
Now, we actually define an SL for both in terms of $L_1$ and specific estimator in library. So state assumptions under which this SL gets the rate.
In other words, we need a theorem which states all the structural conditions, $R_2$-bound, linking norms of $D^*$ to $d_0$, properties of loss function, 
$Q_0,G_0$ bounded var and cadlag, beyond model $M$, pathwise differentiability and what is needed for inheriting rate for one step update, may be also what is needed for lfm to solve efficient en, i.e. lemma above. 

Then we define the SL for $Q_0$ and $G_0$, i.e in terms of MLE over bounded var norm subspace. 
State rate.
Then define CV-TMLE.
Then state asymptotic efficiency of CV-TMLE.
In other word,s make it a single theorem telling the complete story without any proofs or talking, just definitions, assumptions, conclusions.
Later we can decide if description of setting needs to be moved to before theorem, but still it is the whole story, so all in one section.

We do this first for the TMLE assuming  known bunds on supnorm and variation norm. 
then CV-TMLE. 










